Covariance in Non-Commutative Algebra

Consider vector space over non-commutative division algebra. Set of automorphisms of this vector space is group $GL$. Group $GL$ acts on the set of bases of vector space (basis manifold) single transitive and generates active representation. Twin representation on basis manifold is called passive representation. There is no automorphism associated with passive transformation. However passive transformation generates transformation of coordinates of vector with respect to basis. If we consider homomorphism of vector space $V$ into vector space $W$, then we can learn how passive transformation in vector space $V$ generates transformation of coordinates of vector in vector space $W$. Vector in vector space $W$ is called geometric object in vector space $V$. Covariance principle states that geometric object does not depend on the choice of basis. I considered transformation of coordinates of vector and polylinear map.

==> Abstract.MObject.English.tex <==
%auto-ignore

\begin{abstract}
Consider vector space over non-commutative division algebra.
Set of automorphisms of this vector space is group $GL$.
Group $GL$ acts on the set of bases of vector space (basis manifold)
single transitive and generates active representation.
Twin representation on basis manifold is called passive representation.
There is no automorphism associated with passive transformation.
However passive transformation generates
transformation of coordinates of vector with respect to basis.
If we consider homomorphism of vector space $V$ into vector space $W$,
then we can learn how passive transformation in vector space $V$
generates transformation of coordinates of vector in vector space $W$.
Vector in vector space $W$ is called geometric object in vector space $V$.
Covariance principle states that geometric object does not depend
on the choice of basis.
I considered transformation of coordinates of vector and polylinear map.
\end{abstract}


==> Abstract.MObject.Russian.tex <==
%auto-ignore

\begin{abstract}
Рассмотрим векторное пространство над некоммутативной алгеброй с делением.
Множество автоморфизмов этого векторного пространства является группой $GL$.
Группа $GL$ действует на множестве базисов векторного пространства (многообразие базисов)
однотранзитивно и порождает активное представление.
Парное представление на многообразие базисов называется пассивным представлением.
Не существует автоморфизма, ассоциированного с пассивным преобразованием.
Однако пассивное преобразование порождает
преобразование координат вектора относительно базиса.
Если мы рассмотрим гомоморфизм векторного пространства $V$ в векторное пространство $W$,
то мы можем изучить как пассивное преобразование в векторном пространстве $V$
порождает преобразование координат вектора в векторном пространстве $W$.
Вектор в векторном пространстве $W$ называется геометрическим объектом в векторном пространстве $V$.
Принцип ковариантности утверждает, что геометрический объект не зависит
от выбора базиса.
Я рассмотрел преобразование координат вектора и полилинейного отображения.
\end{abstract}


==> Biblio.English.tex <==
%auto-ignore
\OpenBiblio

%22. A.G. Kurosh, Lectures on General Algebra, Chelsea, New York, 1963

\BiblioItem{Doctor Ouch}
{
Kornei Chukovsky. Doctor Ouch.
\\
Translator and illustrator Jan Seabaugh.
\\
Viveca Smith Publishing, 2004, ISBN-10: 0974055107.
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Albert Einstein,
On the Electrodynamics of Moving Bodies, 1905,
\\
The Principle of Relativity: A Collection of Original
Memoirs on the Special and General Theory of Relativity , 37 - 65,
\\
Courier Dover Publications, 1952; ISBN-13: 978-0486600819
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Albert Einstein,
On the Relativity Principle and the Conclusions Drawn from It, 1907,
\\
The Collected Papers of Albert Einstein, Volume 2:
The Swiss Years: Writings, 1900-1909. English translation. 252 - 311.
\\
Anna Beck, translator; Peter Havas, consultant.
Princeton University Press, 1989; ISBN-13: 9780691085494
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Albert Einstein,
Die Grundlage der allgemeinen Relativit\"atstheorie,
Ann. Phys., 1916, {\bf 49}, 769 - 822,\\
Einstein's Annalen Papers: The Complete Collection 1901-1922,
edited by J\"urgen Renn, 517 - 571,\\
Wiley-VCH Verlag GmbH \& Co. KGaA, 2005
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Albert Einstein, Geometry and Experience, (1921)\\
Albert Einstein, Sidelights on Relativity, 25 - 56,\\
Courier Dover Publications, 1983
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Albert Einstein,
Grundgedanken und Probleme der Relativit\"atstheorie, (1923),\\
Nobelstiftelsen, Les Prix Nobel en 1921 - 1922,
Imprimerie Royale, Stockholm, 1923
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Albert Einstein,
Nichtenklidische Geometrie in der Physik Neue Rundschan, (1925)
Berlin, S. 16 - 20
}%

\BiblioItem{Einstein: Isaak Newton}
{
Albert Einstein,
Isaak Newton, 1927,
Out of My Later Years, 
Citadel Press, 1995, 219 - 223
}%

\BiblioItem{Einstein: On Science}
{
Albert Einstein,
On Science, 
Cosmic Religion, with Other Opinions and Aphorisms,142 - 146,
New York, 1931, 97 - 103
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Albert Einstein,
Autobiographical Notes, 1949,\\
Paul A. Schilpp, editor, Albert Einstein: Philosopher-Scientist,
Evanston, 
Illinois, The Library of Living Philosophers, 1949, 1 - 95
}%

\BiblioItem{Feynman 1}
{
Richard Phillips Feynman, Robert B. Leighton, Matthew Linzee Sands.
The Feynman lectures on physics: Volume 1.
Mainly Mechanics, Radiation, and Heat.
Addison\Hyph Wesley, 1965.
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Cite 104, Source unknown
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{https://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{2110.04354}
{
Dimitri Gurevich, Varvara Petrova, Pavel Saponov,
q-Casimir and q-cut-and-join operators related to Reflection Equation Algebras,
eprint \href{https://arxiv.org/abs/2110.04354}{arXiv:gr-qc/2110.04354} (2021)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Steven Weinberg.
The Quantum Theory of Fields. Volume I. Foundations.
Cambridge university press, 1995
}%

\BiblioItem{Weinberg II}
{
Steven Weinberg.
The Quantum Theory of Fields. Volume II. Modern applications.
Cambridge university press, 1996
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.
}%

\BiblioItem{Landau I}
{
L. D. Landau, E. M. Lifshich.
Course of theoretical physics, volume 1.
Mechanics.
\\
Translated from the Russian by J. B. Sykes and J. S. Bell.
Pergamon Press, 1969
}%

\BiblioItem{Landau}
{
L. D. Landau, E. M. Lifshich, The classical theory of fields.
\\
Translated from the Russian by Morton Hamermesh.
Pergamon Press, 1971
}%

\BiblioItem{Landau III}
{
L. D. Landau, E. M. Lifshich,
Course of Theoretical Physics, Volume 3.
Quantum Mechanics Non-Relativistic Theory, Third Edition.
\\
Translated from the Russian by J. B. Sykes and J. S. Bell.
Butterworth-Heinemann, 1981, ISBN 978-0750635394.
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW}
{
Charles W. Misner, Kip S. Thorne, John Archibald Wheeler.
Gravitation.
W. H. Freeman and Company, San Francisco, 1973.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Serge Lang,
Algebra, Springer, 2002
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
G. E. Shilov,
Calculus, Single Variable Functions, Parts 1 - 2,
Moscow, Nauka, 1969
}%

\BiblioItem{Shilov single 3}
{
G. E. Shilov,
Calculus, Single Variable Functions, Part 3,
Moscow, Nauka, 1970
}%

\BiblioItem{Shilov}
{
G. E. Shilov,
Calculus, Multivariable Functions,
Moscow, Nauka, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
A. N. Kolmogorov and S. V. Fomin.
Introductory Real Analysis.
\\
Translated and edited by Richard A. Silverman.
\\
Dover Publication, 1975, ISBN-13: 978-0486612263
}%

\BiblioItem{Lebedev Vorovich}
{
L. P. Lebedev, I. I. Vorovich,
Functional Analysis in Mechanics,
Springer, 2002
}%

\BiblioItem{8176-4374}
{
Mariano Giaquinta, Giuseppe Modica,
Mathematical Analysis: Linear and Metric Structures and Continuity.
\\
Springer, 2007, ISBN-13: 978-0-8176-4374-4
}%

\BiblioItem{319-09203}
{
Ralf Schiffler,
Quiver Representations.
\\
Springer, 2014, ISBN-13: 978-3-319-09203-4
}%

\BiblioItem{511-34545}
{
Ibrahim Assem, Daniel Simson, Andrzej Skowro\'nski,\\
Elements of the Representation Theory
of Associative Algebras.
\\
Volume 1: Techniques of Representation Theory.
\\
Springer, 2014, ISBN-13: 978-3-319-09203-4
}%

\DefBiblioItem{Rashevsky}

\BiblioItem
{Kurosh: High Algebra}
{
A. G. Kurosh, Higher Algebra,
\\
George Yankovsky translator,
\\
Mir Publishers, 1988, ISBN: 978-5030001319
}%

\BiblioItem
{Kurosh: General Algebra}
{
A. G. Kurosh, Lectures on General Algebra,
Chelsea Pub Co, 1965 
}%

\BiblioItem{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{978-0-8176-8384-9}
{
Garret Sobczyk, New Foundations in Mathematics: The Geometric Concept of Number,
\\
Springer, 2013, ISBN: 978-0-8176-8384-9
}%

\BiblioItem{978-0538497817}
{
James Stewart, Calculus,
\\
Cengage Learning, 2012, ISBN: 978-0-538-49781-7
}%

\BiblioItem{470-38334}
{
William E. Boyce, Richard C. DiPrima,
Elementary Differential Equations and Boundary Value Problems,
\\
John Wiley \& Sons, Inc., 2009, ISBN 978-0-470-38334-6
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
B. A. Dubrovin, A. T. Fomenko, S. P. Novikov,
Modern Geometry - Methods and Applications,\\
Part I, The Geometry of Surfaces, Transformation Groups, and Fields,\\
Translated by Robert G. Burns,\\
Springer - New York, 1992
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
B. A. Dubrovin, A. T. Fomenko, S. P. Novikov,
Modern Geometry - Methods and Applications,
Part II: The Geometry and Topology of Manifolds,\\
Translated by Robert G. Burns,\\
Springer - New York, 1985
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Kobayashi S, Nomizu K,
Foundations of Differential Geometry, volume I,\\
Interscience Publishers, 1963
}%

\BiblioItem{Lichnerowicz}
{
Andre Lichnerowicz,
Global Theory of Connections and Holonomy Groups,\\
Kluwer Academic Publishers, 1976, ISBN-13: 978-9028604964
}%

\DefBiblioItem{Korn}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
Peter J. Olver,
Applications of Lie groups to differential equations,\\
Springer, 2000
}%

\BiblioItem{1708.01190}
{
Nathan BeDell,
Doing Algebra over an Associative Algebra,
\\
eprint \href{https://arxiv.org/abs/1708.01190}{arXiv:1708.01190} (2017)
}%

\BiblioItem{Karthika Viji 2021}
{
S. Karthika, M. Viji,
Unit elements in the path algebra of an acyclic quiver,
Indian J Pure Appl Math\\
Published online: 10 June 2021
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.com/science?\_ob=ArticleURL&\_udi=B6TVM-42WP7CR-1&\_user=10&\_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&\_fmt=summary&\_coverDate=04%2F23%2F2001&\_rdoc=1&\_orig=browse&\_srch=%23toc%235538%232001%23997179995%23246657!&\_cdi=5538&view=c&\_acct=C000050221&\_version=1&\_urlVersion=0&\_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%

\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
Izrail Moiseevich Gelfand, Robert Adolfovich Minlos,
Representations of the rotation and Lorentz groups and their applications;\\
Engl. transl. ed. H. K. Farahat; Transl. by G. Cummins and T. Boddongton;\\
Pergamon Press, 1963
}%

\DefBiblioItem{math.QA-0208146}%

\DefBiblioItem{q-alg-9705026}

\BiblioItem{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{0911.4454}
{
Vladimir Retakh,
From factorizations of noncommutative polynomials to combinatorial topology,\\
eprint \href{http://arxiv.org/abs/0911.4454}{arXiv:0911.4454} (2009)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
Mark Aronovich Naimark, Aleksandr Isaakovich Shtern,
Theory of group representations;\\
Heidelberg, 1982
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
Asim Orhan Barut; Ryszard R\c{a}czka;
Theory of group representations and applications;\\
World Scientific Publishing Co. Pre. Ltd., 1986
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{McCrimmon: Jordan Algebras}
{
Kevin McCrimmon;
A Taste of Jordan Algebras;\\
Springer, 2004
}%

\BiblioItem{Zharinov: foundation of mathematical physics}
{
V. V. Zharinov,
Algebraic and geometric foundation of mathematical physics,\\
Lecture courses of the scientific and educational center, 9, Steklov Math. Institute of RAS,\\
Moscow, 2008
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
I. R. Shafarevich,
Basic notions of algebra,\\
Translated from the Russian by M. Reid,\\
Springer, 2005
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Lev Elsgolts,
Differential Equations and the Calculus of Variations,\\
Translated from the Russian by George Yankovsky,\\
MIR Publishers, Moscow, 1977
%University Press of the Pacific, 2003 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
Carl Faith, Algebra: Rings, Modules and Categories I,
Springer - Verlag, Berlin - Heidelberg - New York, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Aleks Kleyn,
Basis Manifold,
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Aleks Kleyn,
Reference Frame in General Relativity,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Aleks Kleyn, Metric\hyph Affine Manifold,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Aleks Kleyn,
Biring of Matrices,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Aleks Kleyn,
Lectures on Linear Algebra over Division Ring,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Aleks Kleyn,
Fibered Universal Algebra,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Aleks Kleyn,
Vector Space Over Division Ring,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Aleks Kleyn,
Fibered Correspondence,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Aleks Kleyn,
Morphism of \Ts{T}Representations,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Aleks Kleyn,
Lorentz Transformation and General Covariance Principle,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\DefBiblioItem{0812.4763}%

\BiblioItem{0906.0135}
{
Aleks Kleyn,
Introduction into Geometry over Division Ring,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Aleks Kleyn,
Quaternion Rhapsody,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Aleks Kleyn,
Representation of Universal Algebra,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2009)
}%

\BiblioItem{0912.4061}
{
Aleks Kleyn,
Linear Equation in Finite Dimensional Algebra,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Aleks Kleyn,
The Matrix of Linear Maps,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Aleks Kleyn,
Linear Maps of Free Algebra,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Aleks Kleyn,
The G\^ateaux Derivative and Integral over Banach Algebra,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Aleks Kleyn,
Polylinear Map of Free Algebra,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1102.1776}
{
Aleks Kleyn, Ivan Kyrchei,
Correspondence between Row\Hyph Column Determinants
and Quasideterminants of Matrices over Quaternion Algebra,\\
eprint \href{http://arxiv.org/abs/1102.1776}{arXiv:1102.1776} (2011)
}%

\BiblioItem{1104.5197}
{
Aleks Kleyn,
$C^*$-Rhapsody,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Aleks Kleyn,
Algebra with Conjugation,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Aleks Kleyn,
Linear Maps of Quaternion Algebra,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Aleks Kleyn,
Orthogonal Basis and Motion in Finsler Geometry,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Aleks Kleyn,
Basis of Representation of Universal Algebra,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Aleks Kleyn, Alexandre Laugier,
Orthonormal Basis in Minkowski Space,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Aleks Kleyn,
Maps of Conjugation of Quaternion Algebra,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Aleks Kleyn,
Algebra of Fractions of Algebra with Conjugation,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}%

\BiblioItem{1211.6965}
{
Aleks Kleyn,
Free Algebra with Countable Basis,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\DefBiblioItem{1302.7204}%

\BiblioItem{1305.4547}
{
Aleks Kleyn,
Normed $\Omega$-Group,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$\Hyph group,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{1412.5425}
{
Aleks Kleyn,
Division in Associative $D$-Algebra,\\
eprint \href{http://arxiv.org/abs/1412.5425}{arXiv:1412.5425} (2014)
}%

\DefBiblioItem{1502.04063}%

\BiblioItem{1505.03625}
{
Aleks Kleyn,
Derivative of Map of Banach algebra,\\
eprint \href{http://arxiv.org/abs/1505.03625}{arXiv:1505.03625} (2015)
}%

\BiblioItem{1506.00061}
{
Aleks Kleyn,
Quadratic Equation over Associative $D$\Hyph Algebra,\\
eprint \href{http://arxiv.org/abs/1506.00061}{arXiv:1506.00061} (2015)
}%

\DefBiblioItem{1601.03259}%

\DefBiblioItem{1801.01628}

\DefBiblioItem{1908.04418}

\BiblioItem{2020.06.01}
{
Aleks Kleyn,
System of Differential Equations over Quaternion Algebra,\\
Geometry of differential equations seminar 2020\\
eprint \href{https://gdeq.org/files/Aleks_Kleyn-2020.06.01.English.pdf}{talk:2020.06.01} (2020)
}%

\BiblioItem{2021.01.06}
{
Aleks Kleyn,
Calculus over Quaternion Algebra,\\
Joint Mathematics Meetings January 2020\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}%

\BiblioItem{2112.00613}
{
Aleks Kleyn,
Polynomial in Non-Commutative Algebra,\\
eprint \href{http://arxiv.org/abs/2112.00613}{arXiv:2112.00613} (2021)
}%

\BiblioItem{322019412}
{
Aleks Kleyn,
Research Diary, 2017\\
eprint \href{https://www.researchgate.net/publication/322019412}{RG:322019412} (2017)
}%

\BiblioItem{323966352}
{
Aleks Kleyn,
Research Diary, 2018\\
eprint \href{https://www.researchgate.net/publication/323966352}{RG:323966352} (2018)
}%

\BiblioItem{348311191}
{
Aleks Kleyn,
Research Diary, 2021\\
eprint \href{https://www.researchgate.net/publication/348311191}{RG:348311191} (2021)
}%

\BiblioItem{323236904}
{
Aleks Kleyn,
Crash Course in Calculus over  Banach Algebra\\
eprint \href{https://www.researchgate.net/publication/323236904}{RG:323236904} (2018)
}%

\DefBiblioItem{2207.06506}

\BiblioItem{MAlgebra2}
{
Aleks Kleyn,
Introduction into Noncommutative Algebra,
Volume 2, Module over Algebra\\
eprint \href{http://arxiv.org/abs/MAlgebra2}{arXiv:MAlgebra2} (2019)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Aleks Kleyn.\\
Linear Algebra over Division Ring: System of Linear Equations.\\
CreateSpace Independent Publishing Platform, 2012;\\
ISBN-13: 978-1-4776-3181-2
}%

\BiblioItem{4975-6381}
{
Aleks Kleyn.\\
Single Variable Calculus: Noncomutative Banach Algebra.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-4975-6381-0
}%

\BiblioItem{4993-2400}
{
Aleks Kleyn.\\
Linear Algebra over Division Ring: Vector Space.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-4993-2400-6
}%

\BiblioItem{5059-9176}
{
Aleks Kleyn.\\
Normed \(\Omega\)-Group.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5059-9176-5
}%

\BiblioItem{5114-6019}
{
Aleks Kleyn.\\
Representation of Universal Algebra: Polymorphism.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5114-6019-4
}%

\BiblioItem{5148-4632}
{
Aleks Kleyn.\\
Noncommutative Algebra: Introduction.\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-5114-6019-4
}%

\BiblioItem{5410-9916}
{
Aleks Kleyn.\\
Lebesgue Integral in Abelian $\Omega$-Group.\\
CreateSpace Independent Publishing Platform, 2016;\\
ISBN-13: 978-1-5410-9916-6
}%

\BiblioItem{9856-6693}
{
Aleks Kleyn,
Crash Course in Calculus over  Banach Algebra\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-9856-6693-1
}%

\BiblioItem{7287-9339}
{
Aleks Kleyn,
Quadratic Equation over Associative $D$\Hyph Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-7287-9339-9
}%

\BiblioItem{9835-2163}
{
Aleks Kleyn,
Differential Equation over Banach Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-9835-2163-8
}%

\BiblioItem{6860-2955}
{
Aleks Kleyn,
Diagram of Representations of Universal Algebras,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: 978-1-6860-2955-4
}%

\BiblioItem{0767-8264}
{
Aleks Kleyn,
System of Differential Equations over Banach Algebra: Exponent,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: 978-1-0767-8264-9
}%

\BiblioItem{8428-0408}
{
Aleks Kleyn,
Introduction into Noncommutative Algebra, Volume 1: Division Algebra,\\
Kindle Direct Publishing, 2022;\\
ISBN-13: 979-8-8428-0408-5
}%

\BiblioItem{CACAA.01.109}
{
Aleks Kleyn,
Mappings of Conjugation of Quaternion Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 1, pages 109 - 121, 2012
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.097}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{CACAA.04.001}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$-group.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 4, Issue 1, pages 1 - 68, 2013
}%

\BiblioItem{CACAA.05.001}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 5, issue 1, pages 1 - 68, 2016 
}%

\BiblioItem{CACAA.06.121}
{
Aleks Kleyn,
Differential Forms in Banach Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 6, issue 2, pages 121 - 214, 2017 
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{1807.05583}
{
V. Sokolov, T. Wolf,
Non\Hyph commutative generalization of integrable quadratic ODE systems,\\
eprint \href{http://arxiv.org/abs/1807.05583}{arXiv:1807.05583} (2019)
}%

\BiblioItem{1506.05848}
{
Rida T. Farouki, Graziano Gentili, Carlotta Giannelli, Alessandra Sestini,
Caterina Stoppato,\\
Solution of a quadratic quaternion equation with mixed coefficients,\\
eprint \href{http://arxiv.org/abs/1506.05848}{arXiv:1506.05848} (2015)
}%

\BiblioItem{2003.05263}
{
Florian-Horia Vasilescu,
Spectrum and Analytic Functional Calculus in Real and Quaternionic Frameworks,\\
eprint \href{http://arxiv.org/abs/2003.05263}{arXiv:2003.05263} (2003)
}%

\BiblioItem{1702.04935}
{
M. Irene Falc\~{a}o, Fernando Miranda, Ricardo Severino, M. Joana Soares,
Weierstrass method for quaternionic polynomial root-finding,\\
eprint \href{http://arxiv.org/abs/1702.04935}{arXiv:1702.04935} (2017)
}%

\DefBiblioItem{1812.03397}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[gr-qc]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
G. S. Asanov.
Finsleroid - space supplemented by angle and scalar product.\\
Hypercomplex Numbers in Geometry and Physics, {\bf 1}, 2004, p. 40 - 62
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[math-ph]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\DefBiblioItem{1510.02224}%

\BiblioItem{1902.09800}
{
Dong Cheng, Kit Ian Kou, Yong Hui Xia.
Floquet Theory for Quaternion-valued Differential Equations.\\
eprint \href{http://arxiv.org/abs/1902.09800}{arXiv:1902.09800} (2019)
}%

\BiblioItem{Zharinov Kursy NOC, 9}
{
В. В. Жаринов,
Алгебро-геометрические основы математической физики.
\\
Лекц. курсы НОЦ, 9, МИАН, М., 2008, 3–209
}%

\BiblioItem{Rund Finsler geometry}
{
Hanno Rund,
The differential geometry of Finsler spaces.
\\
Springer - Verlag, Berlin - G\"ottingen - Heidelberg, 1959
}%

\BiblioItem{Smirnov vol 1}
{
V. I. Smirnov,
A Course of Higher Mathematics, volume I.
\\
Translated by D. E. Brown.
\\
Translation, edited and additions made by I. N. Sneddon.
\\
Pergamon Press, Addison-Wesley Publishing Company, 1964
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Tolstoi about Anna Karenina,
in book A Karenina Companion, by C. J. G. Turner,
published by Wilfrid Laurier University Press (August 1993)
}%

\BiblioItem
{Cohn: Universal Algebra}
{
Paul M. Cohn,
Universal Algebra,
Springer, 1981
}%

\BiblioItem
{Cohn: Algebra 1}
{
Paul M. Cohn,
Algebra, Volume 1,
John Wiley \& Sons, 1982
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\DefBiblioItem{Cohn: Skew Fields}%

\BiblioItem
{Lam: Noncommutative Rings}
{
T. Y. Lam,
A First Course in
Noncommutative Rings,
Springer-Verlag, 1991
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
J.-F. Pommaret,
Partial Differential Equations and Group Theory,
Springer, 1994
}%

\BiblioItem{Bourbaki: Set Theory}
{
N. Bourbaki,
Theory of sets,
Springer, 2004
}%

\BiblioItem{Bourbaki: Algebra 1}
{
N. Bourbaki,
Algebra 1,
Springer, 2004
}%

\BiblioItem{Bourbaki: Algebra 2}
{
N. Bourbaki,
Algebra II, Chapters 4 - 7,//
Translated by P. M. Cohn & J. Howie,//
Springer, 2004
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
N. Bourbaki,
General Topology, Chapters 1 - 4,
Springer, 1989
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
N. Bourbaki,
General Topology, Chapters 5 - 10,
Springer, 1989
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
N. Bourbaki,
Topological Vector Spaces, Chapters 1 - 5,
Transl. by H. G. Eggleston $\&$ S. Madan,
Springer, 2003
}

\BiblioItem{Bourbaki: Group Lie}
{
N. Bourbaki,
Lie Groups and Lie Algebras, Chapters 1 - 3,
%Transl. by H. G. Eggleston $\&$ S. Madan,
Springer, 1989
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
N. Bourbaki,
Lie Groups and Lie Algebras, Chapters 4 - 6,
Translator Andrew Pressley,
Springer, 2002
}

\BiblioItem{Bourbaki: Real Group Lie}
{
N. Bourbaki,
Lie Groups and Lie Algebras, Chapters 7 - 9,
Translator Andrew Pressley,
Springer, 2005
}

\BiblioItem{Shabat: Complex Analysis}
{
Shabat B. V.,
Introduction to Complex Analysis,
%\\ \url{http://www.math.uchicago.edu/~ryzhik/shabat-all.pdf},
%\\Translated from Russian by L.Ryzhik, 2003
%(
Moscow, Nauka, 1969
%)
}

\BiblioItem{Pontryagin: Topological Group}
{
L. S. Pontryagin,
Selected Works, Volume Two, Topological Groups,
Gordon and Breach Science Publishers, 1986
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Eisenhart,
Continuous Groups of Transformations,
Dover Publications, New York, 1961
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Postnikov M. M.,
Geometry IV: Differential geometry,
Moscow, Nauka, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Fikhtengolts G. M.,
Differential and Integral Calculus Course, volume 1,
Moscow, Nauka, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Fikhtengolts G. M.,
Differential and Integral Calculus Course, volume 2,
Moscow, Nauka, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Fikhtengolts G. M.,
Differential and Integral Calculus Course, volume 3,
Moscow, Nauka, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
Krasil'shchik I. S., Lychagin V. V., Vinogradov A. M.,
Geometry of Jet Spaces and Nonlinear Partial Differential Equations,
\\
Translated from the Russian by A. B. Sosinskii,
\\
Gordon and Breach Science Publishers, 1985
}

\BiblioItem{Basic Concepts of Differential Geometry}
{
Alekseyevskii D. V., Vinogradov A. M., Lychagin V. V.,
Basic Concepts of Differential Geometry
\\
VINITI Summary 28
\\
Moscow. VINITI, 1988
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Funct. Anal. Appl. {\bf 2} (1968) 19 - 33;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\DefBiblioItem{Sudbery Quaternionic Analysis}%

\BiblioItem{Sudbery 2657821}
{
A. Sudbery,
Quaternionic Analysis,\\
eprint \href{https://www.researchgate.net/publication/2657821}{ResearchGate:2657821} (1977)
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Elie Cartan, Vladislav V. Goldberg, Serge\u{i} Pavlovich Finikov,\\
Riemannian geometry in an orthogonal frame:
from lectures delivered by Elie Cartan at the Sorbonne in 1926-1927,\\
translated by Vladislav V. Goldberg,\\
World Scientific, 2001
}

\BiblioItem{Cartan differential form}
{
Henri Cartan.
Differential forms.\\
Kershaw Publishing Company Limited, London, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio


==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 94,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{https://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{2110.04354}
{
Dimitri Gurevich, Varvara Petrova, Pavel Saponov,
q-Casimir and q-cut-and-join operators related to Reflection Equation Algebras,
eprint \href{https://arxiv.org/abs/2110.04354}{arXiv:gr-qc/2110.04354} (2021)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem{8176-4374}
{
Mariano Giaquinta, Giuseppe Modica,
Mathematical Analysis: Linear and Metric Structures and Continuity.
\\
Springer, 2007, ISBN-13: 978-0-8176-4374-4
}%

\BiblioItem{319-09203}
{
Ralf Schiffler,
Quiver Representations.
\\
Springer, 2014, ISBN-13: 978-3-319-09203-4
}%

\BiblioItem{511-34545}
{
Ibrahim Assem, Daniel Simson, Andrzej Skowro\'nski,\\
Elements of the Representation Theory
of Associative Algebras.
\\
Volume 1: Techniques of Representation Theory.
\\
Cambridge University Press, 2006, ISBN-13: 978-0-511-34545-6
}%

\DefBiblioItem{Rashevsky}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{978-0-8176-8384-9}
{
Garret Sobczyk, New Foundations in Mathematics: The Geometric Concept of Number,
\\
Springer, 2013, ISBN: 978-0-8176-8384-9
}%

\BiblioItem{978-0538497817}
{
James Stewart, Calculus,
\\
Cengage Learning, 2012, ISBN: 978-0-538-49781-7
}%

\BiblioItem{470-38334}
{
William E. Boyce, Richard C. DiPrima,
Elementary Differential Equations and Boundary Value Problems,
\\
John Wiley \& Sons, Inc., 2009, ISBN 978-0-470-38334-6
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\DefBiblioItem{Korn}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{1708.01190}
{
Nathan BeDell,
Doing Algebra over an Associative Algebra,
\\
eprint \href{https://arxiv.org/abs/1708.01190}{arXiv:1708.01190} (2017)
}%

\BiblioItem{Karthika Viji 2021}
{
S. Karthika, M. Viji,
Unit elements in the path algebra of an acyclic quiver,
Indian J Pure Appl Math\\
Published online: 10 June 2021
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\DefBiblioItem{math.QA-0208146}%

\DefBiblioItem{q-alg-9705026}

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{0911.4454}
{
Vladimir Retakh,
From factorizations of noncommutative polynomials to combinatorial topology,\\
eprint \href{http://arxiv.org/abs/0911.4454}{arXiv:0911.4454} (2009)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{McCrimmon: Jordan Algebras}
{
Kevin McCrimmon;
A Taste of Jordan Algebras;\\
Springer, 2004
}%

\BiblioItem{Zharinov: foundation of mathematical physics}
{
В. В. Жаринов, 
Алгебро-геометрические основы математической физики,\\
Лекционные курсы научно-образовательного центра, 9, МИАН,\\
М., 2008
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники). ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная универсальная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts{T}представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\DefBiblioItem{0812.4763}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1102.1776}
{
Александр Клейн, Иван Кирчей,
Соответствие между строчно\Hyph столбцовыми определителями
и квазидетерминантами матриц над кватернионной алгеброй,\\
eprint \href{http://arxiv.org/abs/1102.1776}{arXiv:1102.1776} (2011)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александер Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\DefBiblioItem{1302.7204}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{1412.5425}
{
Александр Клейн,
Деление в ассоциативной $D$-алгебре,\\
eprint \href{http://arxiv.org/abs/1412.5425}{arXiv:1412.5425} (2014)
}%

\DefBiblioItem{1502.04063}%

\BiblioItem{1505.03625}
{
Александр Клейн,
Производная отображения банаховой алгебры,\\
eprint \href{http://arxiv.org/abs/1505.03625}{arXiv:1505.03625} (2015)
}%

\BiblioItem{1506.00061}
{
Александр Клейн,
Квадратное уравнение над ассоциативной $D$\Hyph алгеброй,\\
eprint \href{http://arxiv.org/abs/1506.00061}{arXiv:1506.00061} (2015)
}%

\DefBiblioItem{1601.03259}%

\DefBiblioItem{1801.01628}

\DefBiblioItem{1908.04418}

\BiblioItem{2020.06.01}
{
Александр Клейн,
Система дифференциальных уравнений над банаховой алгеброй,\\
Geometry of differential equations seminar 2020\\
eprint \href{https://gdeq.org/files/Aleks_Kleyn-2020.06.01.Russian.pdf)}{talk:2020.06.01} (2020)
}%

\BiblioItem{2021.01.06}
{
Александр Клейн,
Математический анализ над алгеброй кватернионов,\\
Joint Mathematics Meetings January 2020\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}%

\BiblioItem{2112.00613}
{
Александр Клейн,
Многочлен в некомутативной алгебре,\\
eprint \href{http://arxiv.org/abs/2112.00613}{arXiv:2112.00613} (2021)
}%

\BiblioItem{322019412}
{
Александр Клейн,
Дневник поиска, 2017\\
eprint \href{https://www.researchgate.net/publication/322019412}{RG:322019412} (2017)
}%

\BiblioItem{323966352}
{
Александр Клейн,
Дневник поиска, 2018\\
eprint \href{https://www.researchgate.net/publication/323966403}{RG:323966403} (2018)
}%

\BiblioItem{348311191}
{
Александр Клейн,
Дневник поиска, 2021\\
eprint \href{https://www.researchgate.net/publication/348311191}{RG:348311191} (2021)
}%

\BiblioItem{323236904}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
eprint \href{https://www.researchgate.net/publication/323238274}{RG:323238274} (2018)
}%

\DefBiblioItem{2207.06506}

\BiblioItem{MAlgebra2}
{
Александр Клейн,
Введение в некоммутативную алгебру,
Том 2, Модуль над алгеброй\\
eprint \href{http://arxiv.org/abs/MAlgebra2}{arXiv:MAlgebra2} (2019)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Александр Клейн.\\
Линейная алгебра над телом: Система линейных уравнений.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-5029-8247-6
}%

\BiblioItem{4975-6381}
{
Александр Клейн.\\
Математический анализ отображений одной переменной: Некоммутативная банахова алгебра.\\
CreateSpace Independent Publishing Platform, 2017;\\
ISBN-13: 978-1-4975-6368-1
}%

\BiblioItem{4993-2400}
{
Александр Клейн.\\
Линейная алгебра над телом: Векторное пространство.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-4993-2394-8
}%

\BiblioItem{5059-9176}
{
Александр Клейн.\\
Нормированная \(\Omega\)-группа.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5059-9235-9
}%

\BiblioItem{5114-6019}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5148-4632}
{
Александр Клейн.\\
Некоммутативная алгебра: Введение.\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5410-9916}
{
Александр Клейн.\\
Интеграл Лебега в абелевой $\Omega$-группе.\\
CreateSpace Independent Publishing Platform, 2016;\\
ISBN-13: 978-1-5410-9984-5
}%

\BiblioItem{9856-6693}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-9856-6808-9
}%

\BiblioItem{7287-9339}
{
Aleks Kleyn,
Quadratic Equation over Associative $D$\Hyph Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-7287-9339-9
}%

\BiblioItem{9835-2163}
{
Aleks Kleyn,
Differential Equation over Banach Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-9835-2163-8
}%

\BiblioItem{6860-2955}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{0767-8264}
{
Александр Клейн,
Система дифференциальных уравнений над банаховой алгеброй: Экспонента,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{8428-0408}
{
Александр Клейн,
Введение в некоммутативную алгебру, Том 1: Алгебра с делением,\\
Kindle Direct Publishing, 2022;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{CACAA.01.109}
{
Aleks Kleyn,
Mappings of Conjugation of Quaternion Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 1, pages 109 - 121, 2012
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.097}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{CACAA.04.001}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$-group.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 4, Issue 1, pages 1 - 68, 2013
}%

\BiblioItem{CACAA.05.001}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 5, issue 1, pages 1 - 68, 2016 
}%

\BiblioItem{CACAA.06.121}
{
Aleks Kleyn,
Differential Forms in Banach Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 6, issue 2, pages 121 - 214, 2017 
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{1807.05583}
{
V. Sokolov, T. Wolf,
Non\Hyph commutative generalization of integrable quadratic ODE systems,\\
eprint \href{http://arxiv.org/abs/1807.05583}{arXiv:1807.05583} (2019)
}%

\BiblioItem{1506.05848}
{
Rida T. Farouki, Graziano Gentili, Carlotta Giannelli, Alessandra Sestini,
Caterina Stoppato,\\
Solution of a quadratic quaternion equation with mixed coefficients,\\
eprint \href{http://arxiv.org/abs/1506.05848}{arXiv:1506.05848} (2015)
}%

\BiblioItem{2003.05263}
{
Florian-Horia Vasilescu,
Spectrum and Analytic Functional Calculus in Real and Quaternionic Frameworks,\\
eprint \href{http://arxiv.org/abs/2003.05263}{arXiv:2003.05263} (2003)
}%

\BiblioItem{1702.04935}
{
M. Irene Falc\~{a}o, Fernando Miranda, Ricardo Severino, M. Joana Soares,
Weierstrass method for quaternionic polynomial root-finding,\\
eprint \href{http://arxiv.org/abs/1702.04935}{arXiv:1702.04935} (2017)
}%

\DefBiblioItem{1812.03397}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\DefBiblioItem{1510.02224}%

\BiblioItem{1902.09800}
{
Dong Cheng, Kit Ian Kou, Yong Hui Xia.
Floquet Theory for Quaternion-valued Differential Equations.\\
eprint \href{http://arxiv.org/abs/1902.09800}{arXiv:1902.09800} (2019)
}%

\BiblioItem{Zharinov Kursy NOC, 9}
{
V. V. Zharinov,
Algebraic and geometric foundation of mathematical physics.
\\
Lekts. Kursy NOC, 9, Steklov Math. Institute of RAS, Moscow, 2008, 3–209 
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 1}
{
Paul M. Cohn,
Algebra, Volume 1,
John Wiley \& Sons, 1982
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\DefBiblioItem{Cohn: Skew Fields}%

\BiblioItem
{Lam: Noncommutative Rings}
{
T. Y. Lam,
A First Course in
Noncommutative Rings,
Springer-Verlag, 1991
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 1 - 3,
перевод с французского Ю. А. Бахтурина И Г. И. Ольшанского
под редакцией А. А. Кириллова И А. И. Кострикина,
М. Мир, 1976
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{Basic Concepts of Differential Geometry}
{
Алексеевский Д. В., Виноградов А. М., Лычагин В. В.,
Основные понятия дифференциальной геометрии
\\
Итоги ВИНИТИ 28
\\
М. ВИНИТИ, 1988
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\DefBiblioItem{Sudbery Quaternionic Analysis}%

\BiblioItem{Sudbery 2657821}
{
A. Sudbery,
Quaternionic Analysis,\\
eprint \href{https://www.researchgate.net/publication/2657821}{ResearchGate:2657821} (1977)
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Commands.tex <==
%auto-ignore
\def\Defined{}
\def\ValueOff{off}%
\def\ValueOn{on}%
\scrollmode
\ifx\FilePrefix\undefined
\newcommand{\FilePrefix}{}
\fi
\ifx\UseRussian\Defined
\usepackage{cmap}
%\usepackage{cmcyralt}
%\usepackage{cmcyr}
%\usepackage{lhcyr}
%\usepackage{cmlgc}
\usepackage[T2A,T2B]{fontenc}
\usepackage[cp1251]{inputenc}
\fi

% if I want to find bug in aux file or some other problem
% I can remove comment from next command and
% put traceon - traceoff before and after code in question
\usepackage{trace}
%\traceon
%\traceoff

\ifx\GJSFRA\Defined
\paperheight 297mm\paperwidth 210mm
\usepackage[top=1.905cm,bottom=1.905cm,inner=1.65cm,outer=1.65cm]{geometry}
\fi
\ifx\Presentation\Defined
\paperheight 215pt
\paperwidth 480pt
\usepackage[margin=1cm]{geometry}
\fi

\ifx\setCACAA\Defined
\usepackage{times,mathptm}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{graphicx,graphics,epsfig}
\usepackage{fancyhdr,fancybox}
\usepackage{verbatim}
\usepackage{setspace}
\fi

\ifx\CreateSpace\Defined
% cover image:
% width =   7.25 inch = 2900 px
% height = 10.50 inch = 4200 px
% resolution >= 300 dpi
% color: tan - rgb(210, 180, 140)
% distance from edge 0.5 inch = 200 px
%page size  = 6    x 9   inches
%\paperheight 228.6mm\paperwidth 152.4mm
%page size  = 7    x 10   inches
\paperheight 254mm\paperwidth 177.8mm
%\paperheight 257mm\paperwidth 182mm
\usepackage[top=1.905cm,bottom=1.905cm,inner=1.905cm,outer=1.27cm]{geometry}
\def\Publisher{CreateSpace Independent Publishing Platform}
\fi

\ifx\KDP\Defined
% cover image:
% width =   7.25 inch = 2900 px
% height = 10.50 inch = 4200 px
% resolution >= 300 dpi
% color: tan - rgb(210, 180, 140)
% distance from edge 0.5 inch = 200 px
%page size  = 7    x 10   inches
\paperheight 10in\paperwidth 7in
%%%\paperheight 254mm\paperwidth 177.8mm
%\paperheight 257mm\paperwidth 182mm
\usepackage[top=\MarginTop,bottom=\MarginBottom,inner=\Gutter,outer=\MarginOut]{geometry}
%%%\ifx\Hardcover\Defined
%%%\usepackage[top=0.25in,bottom=0.31in,inner=0.625in,outer=0.26in]{geometry}
%%%\else
%%%\usepackage[top=1.93cm,bottom=1.93cm,inner=1.93cm,outer=1.52cm]{geometry}
%%%\fi
\def\Publisher{Kindle Direct Publishing}
\fi
\ifx\PublishBook\Defined
%use class \documentclass[12pt]{amsbook}
\def\PrintPaper{}
%page size  = 8.27    x 11.69   inches
%           = 21.0    x 29.7    cm
%           = 600.0   x 848.36  pt
%1 inch/дюйм = 2.54 см
%1 pt = .35 mm = .035 cm
%1 pc = 12 pt
% left/right margin = 2 cm = 57.14 pt
\usepackage{setspace}
\ifx\UseRussian\undefined
\usepackage{pslatex}
\fi
\onehalfspacing
\paperheight 297mm\paperwidth 210mm
% текст начинается на расстоянии 1 дюйм + oddsidemargin от левого края
%%%%\oddsidemargin=-.54cm
%%%%\evensidemargin=-.54cm
%%%\marginparwidth=2cm
%%%%\textwidth=17cm
% top/bottom margin = 2 cm = 57.14pt
\usepackage[margin=2cm]{geometry}
\fi
\raggedbottom
%\usepackage{ifthen}
\usepackage{graphicx}
%\usepackage{footmisc}
%\usepackage[fixpdftex]{xcolor}
\usepackage[all]{xy}
\usepackage{xcolor}
\ifx\PrintPaper\undefined
\definecolor{CoverColor}{rgb}{.82,.7,.55}
\definecolor{Gray}{rgb}{.94,.95,.94}
\definecolor{UrlColor}{rgb}{.9,0,.3}
\definecolor{SymbColor}{rgb}{.4,0,.9}
\definecolor{IndexColor}{rgb}{1,.3,.6}
\definecolor{BlueColor}{rgb}{.1,.6,.8}
\definecolor{Eq}{rgb}{0.8, 0, 1}
\newcommand\BlueText[1]{\textcolor{BlueColor}{#1}}
\newcommand\EqText[1]{\textcolor{Eq}{#1}}%{\textcolor{BlueColor}{#1}}
\newcommand\RedText[1]{\textcolor{red}{#1}}
\else
\definecolor{UrlColor}{rgb}{.1,.1,.1}
\definecolor{SymbColor}{rgb}{.1,.1,.1}
\definecolor{IndexColor}{rgb}{.5,.1,.1}
\newcommand\BlueText[1]{#1}
\newcommand\RedText[1]{#1}
\fi
\usepackage{framed}

\ifx\UseParacol\Defined
\usepackage{paracol}
\setlength{\columnseprule}{0.5pt}
\globalcounter*
\globalcounter{theorem}
\globalcounter{Index}
\globalcounter{Symbols}
\globalcounter{Symbol}
\globalcounter{enumi}
%\globalcounter{equation}
%\globalcounter{footnote}
%\globalcounter{Hfootnote}
\footnotelayout{m}
\usepackage{etoolbox}
\makeatletter
\patchcmd{\pcol@zparacol}{\topskip}{0pt}{}{}
\makeatother
\widowpenalty=150
\clubpenalty=150
\brokenpenalty=100
%\tolerance=10000
\makeatletter
\def\@makefntext{\noindent\@makefnmark}
\makeatother
\fi

%\usepackage{chngcntr}
%%%%\counterwithin*{<counter>}{<within>}
%%\makeatletter
%%I used code
%%\renewcommand{\counterwithin@x}[2]{%
%%\@ifbothcounters {#1}{#2}{\@addtoreset {#1}{#2}\expandafter \def \csname
%% the#1\expandafter \endcsname \expandafter {\csname the#2\expandafter
 %%\endcsname.\expandafter \@arabic \csname c@#1\endcsname }}}
%%old version
%%\renewcommand{\counterwithin}{\@ifstar{\c@t@sinstar}{\c@t@sin}}
%%\renewcommand{\c@t@sinstar}[2]{%
%%  \@ifbothc@t@s{chngcntr}{#1}{#2}{\@addtoreset{#1}{#2}}}
%%\renewcommand{\c@t@sin}[2]{%
%%  \@ifbothc@t@s{chngcntr}{#1}{#2}{\@addtoreset{#1}{#2}%
%%                        \@namedef{the#1}{\@nameuse{the#2}.\arabic{#1}}}}
%%new version
%%\counterwithin*{<counter>}{<within>}
%%\newcommand{\counterwithin}{\@ifstar \counterwithin@s \counterwithin@x}
%%\newcommand{\counterwithin@s}
%%{\@ifbothcounters {#1}{#2}{\@addtoreset {#1}{#2}}}
%%\newcommand{\counterwithin@s}
%%{
%%\@ifbothcounters {#1}{#2}{\@addtoreset {#1}{#2}\expandafter \gdef \csname
%% the#1\expandafter \endcsname \expandafter {\csname the#2\expandafter
%%\endcsname\expandafter \@arabic \csname c@#1\endcsname }}
%%}                         
%%\makeatother

\ifx\UseRussian\Defined
\usepackage[english,russian]{babel}
\selectlanguage{russian}
\else
\ifx\InputEncoding\ValueOn
\UseRawInputEncoding
\fi
\fi
\usepackage{xr-hyper}
%\ifx\Presentation\undefined
\ifx\Link\ValueOff
\usepackage[unicode,draft]{hyperref}
\else
\usepackage[unicode]{hyperref}
\fi
\hypersetup{pdfdisplaydoctitle=true}
%\hypersetup{pdftex}
\hypersetup{colorlinks}
\hypersetup{citecolor=UrlColor}
\hypersetup{urlcolor=UrlColor}
\hypersetup{linkcolor=UrlColor}
\hypersetup{pdffitwindow=true}
\hypersetup{pdfnewwindow=true}
\hypersetup{pdfstartview={FitH}}
\GetTitleStringSetup{expand}
%\fi

% Document structure

\input{Statement}

\newcommand\Prolog
{
%\pagecolor{CoverColor}
\ifx\PrimaryMSC\undefined
\else
%\,\footnotetext[2010]{\textit{{\bf Mathematics Subject Classification}}:
\ifx\SecondaryMSC\undefined
\subjclass[2010]{Primary \PrimaryMSC}
\else
\subjclass[2010]{Primary \PrimaryMSC;
Secondary \SecondaryMSC}
\fi
\fi
\input{Prolog.Parm}%
\ifx\MoveAbstract\undefined
\Input{Abstract.\BookNumber}
\fi
\maketitle
\input{Prolog.Eq}
\ifx\MoveAbstract\undefined
\else
\Input{Abstract.\BookNumber}
\fi
\tableofcontents
\Input{Preface.\BookNumber}
\ePrints{0767-8264,1305.4547}%
\ifx\Semafor\ValueOn%
\Input{Convention}
\fi
}%Prolog
\newcommand\Epilog[1][0]
{
\Input{Biblio}
\Input{Index}
\Input{Symbol}
%Epilog
\def\TempA{PrintCover}%
\def\TempB{#1}%
\ifx\TempA\TempB%
\newpage
\pagestyle{empty}
\includegraphics[scale=.75]{Cover_Front_\BookNumber_\CurrentLanguage}
\newpage
\includegraphics[scale=.75]{Cover_Back_\BookNumber_\CurrentLanguage}
\fi
}%Epilog
\newcounter{Index}
\newcounter{Symbol}
\newcounter{Symbols}

% Macros

\def\hyph{\penalty0\hskip0pt\relax-\penalty0\hskip0pt\relax}
\def\Hyph{-\penalty0\hskip0pt\relax}%
\newcommand{\Basis}[1]{\overline{\overline{#1}}{}}
\newcommand{\Vector}[1]{\overline{#1}{}}
%%\newcommand{\Basis}[1]{\boldsymbol{\overset{\rightarrow}{#1}}}
%%\newcommand{\Vector}[1]{\overset{\rightarrow}{#1}}
\ifx\PrintPaper\undefined
\newcommand{\gi}[1]{\boldsymbol{\textcolor{IndexColor}{\it #1}}}
\else
\newcommand{\gi}[1]{\boldsymbol{\it #1}}
\fi
\newcommand\gii{\gi i}
\newcommand\giI{\gi I}
\newcommand\gij{\gi j}
\newcommand\giJ{\gi J}
\newcommand\gik{\gi k}
\newcommand\gil{\gi l}
\newcommand\gin{\gi n}
\newcommand\gim{\gi m}
\newcommand\giA{\gi 1}

\renewcommand{\arraystretch}{1.5}

\def\Items#1{\ItemList#1,LastItem,}%
\def\LastItem{LastItem}%
\def\ItemList#1,{\def\ViewBook{#1}%
\ifx\ViewBook\LastItem%
\else%
\ifx\ViewBook\BookNumber%
\def\Semafor{on}%
\fi%
\expandafter\ItemList%
\fi%
}%

\newcommand{\ePrints}[1]%
{%
\def\Semafor{off}%
\Items{#1}%
}%

\makeatletter
\newcommand{\NameDef}[1]{%
\expandafter\gdef\csname #1\endcsname%
}%
\newcommand{\xNameDef}[1]{%
\expandafter\xdef\csname #1\endcsname%
}%
\newcommand{\ShowSymbol}[2]{%
\@nameuse{ViewSymbol#1,,,#2}%
}%

\newcommand\DefSymb[3]
{
\AddEq{#2}
{
\symb{#1}{#2}{#3}
}
}
\newcommand\ShowSymb[1]
{
\ShowEq{#1}
\ShowEq{def #1}
}
\newcommand{\symb}[4][]{%
\def\TempA{}%
\def\TempB{#1}%
\ifx\TempA\TempB%
\def\ThisSymbol{#3}%
\else%
\edef\ThisSymbol{#3(#1)}%
\fi%
\@ifundefined{ViewSymbol\ThisSymbol}{%
\addtocounter{Symbols}{1}%
\edef\SymbolId{\arabic{Symbols}}%
\xNameDef{ViewSymbol\ThisSymbol}{\SymbolId}%
\NameDef{ViewSymbol\ThisSymbol:::\SymbolId}{#2}%
\@namedef{RefSymbol}{:}%
}{%
\edef\Symbols{\@nameuse{ViewSymbol\ThisSymbol}}%
\def\aSymbolId{0}%
\@for\Symbol:=\Symbols\do{%
\protected@edef\TempA{#2}%
\protected@edef\TempB{\@nameuse{ViewSymbol\ThisSymbol:::\Symbol}}%
\ifx\TempA\TempB%
\edef\aSymbolId{\Symbol}%
\fi%
}%
\def\Zero{0}%
\ifx\aSymbolId\Zero%
\addtocounter{Symbols}{1}%
\edef\SymbolIds{\@nameuse{ViewSymbol\ThisSymbol},\arabic{Symbols}}%
\xNameDef{ViewSymbol\ThisSymbol}{\SymbolIds}%
\edef\SymbolId{\arabic{Symbols}}%
\NameDef{ViewSymbol\ThisSymbol:::\SymbolId}{#2}%
\else%
\def\SymbolId{\aSymbolId}%
\fi%
\addtocounter{Symbol}{1}%
\@namedef{RefSymbol}{\arabic{Symbol}}%
}%
\@namedef{LabelSymbol}{\label{symbol: \ThisSymbol:\@nameuse{RefSymbol}}}%
\edef\RefIds{RefSymbol\ThisSymbol===\SymbolId}%
\@ifundefined{\RefIds}{%
\xNameDef{\RefIds}{\@nameuse{RefSymbol}}%
}{%
\xNameDef{\RefIds}{\@nameuse{\RefIds},\@nameuse{RefSymbol}}%
}%
\NameDef{ViewSymbol#3,,,#4}{\textcolor{SymbColor}{#2}}%
\def\Temp{#4}%
\def\One{1}%
\def\Two{2}%
\def\Three{3}%
\ifx\Temp\One%
$\@nameuse{ViewSymbol#3,,,#4}$%
\fi%
\ifx\Temp\Two%
\[\@nameuse{ViewSymbol#3,,,#4}\]%
\fi%
\ifx\Temp\Three%
\@nameuse{ViewSymbol#3,,,#4}%
\fi%
\@nameuse{LabelSymbol}%
}%

\newcommand\AddEq[3][0]%
{%
\@ifundefined{ViewEq #2}{%
\expandafter\newcommand\csname ViewEq #2\endcsname[#1]{#3}%
}{%
\errmessage {second entry of AddEq: #2}%
}%
}%

\newcommand\DefEq[2]{%
\@ifundefined{ViewEq #2}{%
\NameDef{ViewEq #2}{#1}%
}{%
\errmessage {second entry of DefEq: #2}%
}%
}%
\newcommand{\DefEquation}[2]{%
\AddEq{#2}%
{%
\begin{equation}%
#1%
\EqLabel{#2}%
\end{equation}%
}%
}%
\newcommand{\AddEquation}[2]{%
\AddEq{#1}{\begin{equation}#2\EqLabel{#1}\end{equation}}%
}%
\def\ViewParm#1{\protect\getParm#1,endParm,}%
\def\endParm{endParm}%
\def\getParm#1,{\def\temp{#1}%
\ifx\temp\endParm%
\else%
\ShowEq{#1}%
\expandafter\getParm%
\fi%
}%

\newcommand{\EqParm}[2]{%
\ViewParm{#2}\ShowEq{#1}%
}%
\newcommand{\EquationParm}[2]{%
%%\DefParm{#2}{#3}%
%%\def\Parm{\@nameuse{ViewParm#3}}%
\@ifundefined{ViewEq #1[#2]}%
{%
\ViewParm{#2}%
\DefEquation{\ShowEq{#1}}{#1[#2]}%
}{}%
\ShowEq{#1[#2]}%
}%
\newcommand\DrawEqParm[3]{%
\ViewParm{#2}%
\@ifundefined{ViewEq #1(#2)}{%
\DefEq%
{%
\ShowEq{#1}%
}{#1(#2)}%
}{%
}%
\DrawEq{#1(#2)}{#3}%
}%
\newcommand\EqRef[2][]%
{%
\def\Semafor{on}%
\def\Temp{}%
\edef\Tempa{#1}%
\ifx\Tempa\Temp%
\def\Semafor{off}%
\fi%
\@ifundefined{xRefDef#1}{%
\def\Semafor{off}%
}{}%
\ifx\Semafor\ValueOff%
\eqref{eq: #2}%
\else%
\citeBib{#1}-\eqref{#1-\TheLanguage-eq: #2}%
\fi%
}%
\newcommand\eqRef[3][]{\EqRef[#1]{#2(#3)}}%
\newcommand\EqRefParm[2]{\EqRef{#1[#2]}}%
\newcommand\eqRefParm[3]{\EqRef{#1(#2)(#3)}}%
\newcommand\EqLabel[1]{\label{eq: #1}}%
\newcommand\ShowEq[1]{%
\@ifundefined{ViewEq #1}{%
\message {error: missed ShowEq #1}%
\newline%
\RedText{missed ShowEq #1}%
\newline%
}{%
%\@nameuse{ViewEq #1}%
\csname ViewEq #1\endcsname
}%
}%

\newcommand\DrawEq[3][]{%
\def\Temp{}%
\def\Tempa{#3}%
\ifx\Tempa\Temp%
\[\ShowEq{#2}#1\]%
\else%
\def\Temp{-}%
\ifx\Tempa\Temp%
$\ShowEq{#2}#1$
\else%
\@ifundefined{ViewEq #2(#3)}{%
\AddEquation{#2(#3)}{\ShowEq{#2}#1}%
  }{%
\errmessage {second entry of DrawEq: #2(#3)}%
}%
\ShowEq{#2(#3)}
\fi%
\fi%
}%
%%\newcommand{\ShowEq}[2]{%
%%\ifcase#1%0
%%$\@nameuse{ViewEq #2}$%
%%\or%1
%%\[%
%%\@nameuse{ViewEq #2}%
%%\]$%
%%\or%2
%%\begin{equation}%
%%\@nameuse{ViewSymbol#3}%
%%\@nameuse{LabelSymbol#3}%
%%\end{equation}
%%\else%
%%\fi%
%%}%
\makeatother
%%\makeatletter
%%\[
%%\begin{array}{r@{\,}l}
%%a&=b\\c&=d
%%\end{array}
%%\refstepcounter{equation}\eqno{\@eqnnum}\EqLabel{a}
%%\]\EqRef{a}
%%\makeatother
\newcommand\Mod[1]{\ensuremath{\mathrm{mod}\,#1}}
\DeclareMathOperator{\Det}{\mathrm{Det}} 
\DeclareMathOperator{\Hom}{\mathrm{Hom}} 
\DeclareMathOperator{\End}{\mathrm{End}} 
\DeclareMathOperator{\rank}{\mathrm{rank}} 
\DeclareMathOperator{\id}{\mathrm{id}} 
\DeclareMathOperator{\const}{\mathrm{const}} 
\newcommand{\subs}{${}_*$\Hyph}
\newcommand{\sups}{${}^*$\Hyph}
\newcommand{\gS}{$*$\Hyph}
\newcommand{\CRstar}{{}^*{}_*}
\newcommand{\RCstar}{{}_*{}^*}
\newcommand{\CRcirc}{{}^{\circ}{}_{\circ}}
\newcommand\RCcirc{{}_{\circ}{}^{\circ}}
\newcommand{\CRbull}{{}^{\bullet}{}_{\bullet}}
\newcommand{\RCbull}{{}_{\bullet}{}^{\bullet}}
\newcommand{\Star}{*}
\newcommand{\RC}{$\RCstar$\Hyph}
\newcommand{\CR}{$\CRstar$\Hyph}
\newcommand{\RCo}{$\RCcirc$\Hyph}
\newcommand{\CRo}{$\CRcirc$\Hyph}
\newcommand{\drc}{$D\RCstar$\Hyph}
\newcommand{\Drc}{$\mathcal D\RCstar$\Hyph}
\newcommand{\dcr}{$D\CRstar$\hyph}
\newcommand{\rcd}{$\RCstar D$\Hyph}
\newcommand{\crd}{$\CRstar D$\Hyph}
\newcommand{\Arc}{$A\RCcirc$\Hyph}
\newcommand{\Acr}{$A\CRcirc$\Hyph}
\newcommand{\rcA}{$\RCcirc A$\Hyph}
\newcommand{\crA}{$\CRcirc A$\Hyph}
\newcommand{\RCPower}[1]{#1\RCstar}
\newcommand{\CRPower}[1]{#1\CRstar}
\newcommand{\RCInverse}{\RCPower{-1}}
\newcommand{\CRInverse}{\CRPower{-1}}
\newcommand{\RCRank}{\rank(\RCstar)}
\newcommand{\CRRank}{\rank(\CRstar)}
%\newcommand{\RCDet}[1]{|#1,\RCstar|}
%\newcommand{\CRDet}[1]{|#1,\CRstar|}
%\newcommand{\RCDet}[1]{\det\left(#1,\RCstar\right)}
%\newcommand{\CRDet}[1]{\det\left(#1,\CRstar\right)}
\newcommand\RCDet{\det(\RCstar)}
\newcommand\RCdet[2]{\aUD{\RCDet}{#1}{#2}\,}
\newcommand\CRDet{\det(\CRstar)}
\newcommand\CRdet[2]{\aUD{\CRDet}{#1}{#2}\,}
\newcommand{\RCGL}[2]{\ensuremath{GL(\gi #1\RCstar #2)}}
\newcommand{\CRGL}[2]{\ensuremath{GL(\gi #1\CRstar #2)}}
\newcommand\sT[1]{$*#1$\Hyph}%
\newcommand\Ts[1]{$#1*$\Hyph}%
\newcommand\sD{$\star D$\Hyph}%
\newcommand\Ds{$D\star$\Hyph}%
\newcommand\VirtFrac{\vphantom{\overset{\rightarrow}{\frac 11}^{\frac 11}}}
\newcommand\VirtVar{\vphantom{\overset{\rightarrow}{1}^1}}
%%\newcommand\pC[2]{{}_{\underline{#1}}^{#2}}%
%%\newcommand\pC[2]{{}^{#1}_{#2}}%
%\newcommand\pC[2]{{}_{#1(#2)}}%
\newcommand\pC[2]{{}_{#1\cdot #2}}%
%\newcommand\pC[2]
%{
%\def\tempa{0}%
%\def\tempb{#2}%
%\ifx\tempa\tempb%
%{}^{#1}%
%\else%
%{}_{#1#2}
%\fi%
%}%
\newcommand\DcrPartial[1]%
{%
\def\tempa{}%
\def\tempb{#1}%
\ifx\tempa\tempc%
(\partial\CRstar)%
\else%
(\partial_{\gi{#1}}\CRstar)%
\fi%
}%
\newcommand\rcDPartial[1]%
{%
\def\tempa{}%
\def\tempb{#1}%
\ifx\tempa\tempc%
(\RCstar\partial)%
\else%
(\RCstar\partial_{\gi{#1}})%
\fi%
}%
%\newcommand\StandPartial[4]%
%{%
%\def\tempa{}%
%\def\tempb{#3}%
%\def\tempc{#4}%
%\ifx\tempa\tempb%
%\else%
%{\vphantom{\frac{#1}{#2}}}^{#3}\!%
%\fi%
%\left(\frac{\partial #1}{\partial #2}%
%\ifx\tempa\tempc%
%\right)%
%\else%
%\right)^{#4}%
%\fi%
%}%
\newcommand\StandPartial[3]%
{%
%\left(\frac{\partial #1}{\partial #2}\right)^{\gi{#3}}%
\frac{d^{\gi{#3}} #1}{d #2}%
}%

\ifx\setCACAA\undefined
\renewcommand{\uppercasenonmath}[1]{}
\renewcommand{\MakeUppercase}[1]{#1}

\setcounter{tocdepth}{2}
\makeatletter
\def\l@chapter{\@tocline{0}{8pt plus1pt}{1pc}{}{}}

\def\part{\newpage\thispagestyle{empty}%
  \null\vfil  \markboth{}{}\secdef\@part\@spart}
\def\@part[#1]#2{%
  \ifnum \c@secnumdepth >-2\relax \refstepcounter{part}%
    \addcontentsline{toc}{part}{\partname\ \thepart.\ #1}%
%        \protect\enspace\protect\noindent#1}%
  \else
    \addcontentsline{toc}{part}{#1}\fi
  \begingroup\centering
  \ifnum \c@secnumdepth >-2\relax
       {\fontsize{\@xviipt}{22}\bfseries
         \partname\ \thepart} \vskip 20\p@ \fi
  \fontsize{\@xxpt}{25}\bfseries
      #1\vfil\vfil\endgroup \newpage\thispagestyle{empty}}

\newcommand\@dotsep{4.5}
\def\dotfill{%
\hbox{$\m@th\mkern \@dotsep mu\hbox{.}\mkern \@dotsep mu$}\hfill}
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \def\@toclevel{#1}%
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup 
        \hyphenpenalty\@M
        \@ifempty{#4}{%
          \@tempdima\csname r@tocindent\number#1\endcsname\relax
        }{%
          \@tempdima#4\relax
        }%
        %\disable@footnotes
        %\parindent\z@
		\parindent .5pc
		%\noindent
		\leftskip#3\relax \advance\leftskip\@tempdima\relax
        \rightskip\@pnumwidth plus4em \parfillskip-\@pnumwidth
        #5\leavevmode\hskip-\@tempdima #6\relax
        \leaders\dotfill
		\hbox to\@pnumwidth{\@tocpagenum{#7}}\par
        \nobreak
    \endgroup
  \fi
}
\makeatother 

\fi

%I use macro PrintBook if I print book
%and chapter is primery counter.
%Otherwise section is primery counter.
\ifx\PrintBook\undefined
\def\Chapter{\section}
\def\Section{\subsection}
\ifx\setCACAA\undefined
\makeatletter
\renewcommand{\@indextitlestyle}{%
\twocolumn[\section{\indexname}]%
\def\IndexSpace{off}%
}
\makeatother 
\ifx\PrintPaper\undefined
\thanks{\href{mailto:Aleks\_Kleyn@MailAPS.org}{Aleks\_Kleyn@MailAPS.org}}
\ePrints{1102.1776,1201.4158}
\ifx\Semafor\ValueOff
\thanks{\ \ \ \url{http://AleksKleyn.dyndns-home.com:4080/}\ \ \ \ \ \url{http://arxiv.org/a/kleyn\_a\_1}}
\thanks{\ \ \ \ \url{http://AleksKleyn.blogspot.com/}}
\fi
\fi
\fi
\else
\def\Chapter{\chapter}
\def\Section{\section}

%\ifx\Presentation\undefined
\pagestyle{headings}
%\fi
\makeatletter
%title page
\def\@maketitle{%
  \cleardoublepage \thispagestyle{empty}%
  \begingroup \topskip\z@skip
  \null\vfil
  \begingroup
  \def\and{\par\medskip}\centering
  \bfseries\authors\par\bigskip
  \par\vspace{24pt}%
  \LARGE\bfseries \centering
  \openup\medskipamount
  \@title
  \par
  \ifx\subtitle\undefined
  \else
  \centerline{\ }
  \centerline{\emph\subtitle}
  \fi
  \ifx\subtitleA\undefined
  \else
  \centerline{\emph\subtitleA}
  \fi
  \ifx\edition\undefined
  \else
  \centerline{\emph\edition}
  \fi
  \endgroup
  %\vfil
  %\ifx\@empty\addresses \else \@setaddresses \fi
  %\vfil
  %\ifx\@empty\@dedicatory
  %\else\begingroup
  %  \centering{\,\footnotesize\itshape\@dedicatory\@@par}%
  %  \endgroup
  %\fi
  \vfill
  %\par\vspace{10pt}\ \par\vspace{10pt}
\noindent
\href{mailto:Aleks\_Kleyn@MailAPS.org}{Aleks\_Kleyn@MailAPS.org}
\newline
\url{http://AleksKleyn.dyndns-home.com:4080/}
\newline
\url{http://arxiv.org/a/kleyn\_a\_1}
\newline
\url{http://AleksKleyn.blogspot.com/}
  \newpage\thispagestyle{empty}
  \begin{center}
    \ifx\@empty\@subjclass\else\@setsubjclass\fi
    \ifx\@empty\@keywords\else\@setkeywords\fi
    \ifx\@empty\@translators\else\vfil\@settranslators\fi
    \ifx\@empty\thankses\else\vfil\@setthanks\fi
  \end{center}
  \vfil
  \@setabstract
  %\@setcopyright
\vfil
  \def\Temp{0000}
  \ifx\copyrightyear\Temp
  \else
  \begin{center}
\begin{tabular}{@{}c}
Copyright\ \copyright\ \copyrightyear\ \copyrightholder
\\
All rights reserved.
\end{tabular}
  \end{center}
  \fi
  \ifx\Publisher\undefined%
  \else
  \begin{center}
\begin{tabular}{@{}c}
\Publisher
\end{tabular}
  \end{center}
  \fi
  \ifx\ISBN\undefined%
  \else%
 \begin{center}
\begin{tabular}{@{}r@{\ }l}
ISBN:&\ISBN
\\
ISBN-13:&\ISBNa
\end{tabular}
  \end{center}
  \fi%
  \ifx\titleNote\undefined
  \else
  \par\vspace{24pt}%
  \centerline{\mdseries\titleNote}
	  \centerline{\Title}
	  \ifx\Subtitle\undefined
	  \else
	  \centerline{\emph\Subtitle}
	  \fi
	  \ifx\Edition\undefined
	  \else
	  \centerline{\Edition}
	  \fi
	  \centerline{\Authors}
  \fi
  \endgroup}
\def\chapter{%
%  \if@openright
%	\cleardoublepage
% \else
	\clearpage
% \fi
  \thispagestyle{plain}\global\@topnum\z@
  \@afterindenttrue \secdef\@chapter\@schapter}
%bibliography and index
\renewcommand{\@indextitlestyle}{%
\twocolumn[\chapter{\indexname}]%
\def\IndexSpace{off}%
\let\@secnumber\@empty
\chaptermark{\indexname}%
%\sectionmark{}%
}
\makeatother 
\email{\href{mailto:Aleks\_Kleyn@MailAPS.org}{Aleks\_Kleyn@MailAPS.org}}
\ePrints{1102.1776,1201.4158}
\ifx\Semafor\ValueOff
%\def\temp{1102.1776}
%\ifx\BookNumber\temp
%\else
\urladdr{\url{http://AleksKleyn.dyndns-home.com:4080/}}
\urladdr{\url{http://arxiv.org/a/kleyn\_a\_1}}
\urladdr{\url{http://AleksKleyn.blogspot.com/}}
\fi
\fi

\newcommand\FrameEqRef[3][]
{
\fbox{%
\eqRef{#2}{#3}%
$\ \ \ $%
\DrawEq[#1]{#2}-
}
}

\newcommand\FrameeqRef[4][]
{
\fbox{
\eqRef[#2]{#3}{#4}
$\ \ \ $
\DrawEq[#1]{#3}-
}
}

\newcommand\FrameEq[2][]
{
\fbox{
\DrawEq[#1]{#2}-
}
}

\newcommand\FrameCiteBib[1]
{
\noindent
\fbox{
\begin{minipage}{350pt}
\setlength{\parindent}{6mm}
\citeBib{#1}
\ShowCiteBib{#1}
\end{minipage}
}
}

\newcommand\arXivOldRef{http://arxiv.org/PS_cache/}
\newcommand\arXivRef{http://arxiv.org/pdf/}
\newcommand\RgRef{https://www.researchgate.net/publication/}
\newcommand\AmazonRef{http://www.amazon.com/s/ref=nb_sb_noss?url=search-alias=aps&field-keywords=aleks+kleyn}
\newcommand\DefRgRef[1]
{
\def\Tempb{#1}
\ifx\Tempa\Tempb
\def\wRef{\RgRef #1}
\fi
}
\newcommand\DefArXivOldRef[2]
{
\def\Tempb{#1}
\ifx\Tempa\Tempb
\def\wRef{\arXivOldRef #2.pdf}
\fi
}
\newcommand\DefArXivRef[2]
{
\def\Tempb{#1}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef #1#2.pdf}
\fi
}
\newcommand\DefAmazonRef[1]
{
\def\Tempb{#1}
\ifx\Tempa\Tempb
\def\wRef{\AmazonRef}
\fi
}
\newcommand\DefCaCaaRef[1]
{
\def\Tempb{CACAA.#1}
\ifx\Tempa\Tempb
\def\wRef{http://www.cliffordanalysis.com/}
\fi
}
\newcommand\wRefDef[2]
{
\def\Tempa{#1}
\DefArXivOldRef{0405.027}{gr-qc/pdf/0405/0405027v3}
\DefArXivOldRef{0405.028}{gr-qc/pdf/0405/0405028v5}
\DefArXivOldRef{0412.391}{math/pdf/0412/0412391v4}
\DefArXivOldRef{0612.111}{math/pdf/0612/0612111v2}
\DefArXivOldRef{0701.238}{math/pdf/0701/0701238v6}
\DefArXivOldRef{0702.561}{math/pdf/0702/0702561v3}
\DefArXivRef{0707.2246}{v2}
\DefArXivRef{0803.3276}{v3}
\DefArXivRef{0812.4763}{v7}
\DefArXivRef{0906.0135}{v3}
\DefArXivRef{0909.0855}{v5}
\DefArXivRef{0912.3315}{v3}
\DefArXivRef{0912.4061}{v2}
\DefArXivRef{1001.4852}{}
\DefArXivRef{1003.3714}{v2}
\DefArXivRef{1003.1544}{v2}
\DefArXivRef{1006.2597}{v2}
\DefArXivRef{1011.3102}{}
\DefArXivRef{1102.1776}{}
\DefArXivRef{1104.5197}{}
\DefArXivRef{1105.4307}{}
\DefArXivRef{1107.1139}{}
\DefArXivRef{1107.5037}{}
\DefArXivRef{1111.6035}{}
\DefArXivRef{1202.6021}{v2}
\DefArXivRef{1211.6965}{}
\DefArXivRef{1302.7204}{v1}
\DefArXivRef{1305.4547}{}
\DefArXivRef{1310.5591}{}
\DefArXivRef{1502.04063}{v2}
\DefArXivRef{1505.03625}{v1}
\DefArXivRef{1506.00061}{}
\DefArXivRef{1601.03259}{v3}
\DefArXivRef{1801.01628}{}
\DefArXivRef{1908.04418}{}
\DefArXivRef{2020.06.01}{}
\DefArXivRef{2021.01.06}{}
\DefArXivRef{2207.06506}{}
\DefRgRef{322019412}
\DefRgRef{323966352}
\DefRgRef{348311191}
\DefAmazonRef{8433-5163}
\DefAmazonRef{8443-0072}
\DefAmazonRef{4776-3181}
\DefAmazonRef{4975-6381}
\DefAmazonRef{4993-2400}
\DefAmazonRef{5059-9176}
\DefAmazonRef{5114-6019}
\DefAmazonRef{5148-4632}
\DefAmazonRef{5410-9916}
\DefAmazonRef{6860-2955}
\DefAmazonRef{0767-8264}
\DefAmazonRef{8428-0408}
\DefCaCaaRef{01.109}
\DefCaCaaRef{01.291}
\DefCaCaaRef{02.097}
\DefCaCaaRef{04.001}
\DefCaCaaRef{05.001}
\DefCaCaaRef{06.121}
 \def\Tempb{GJSFRA.13.1.39}
\ifx\Tempa\Tempb
\def\wRef{http://www.cliffordanalysis.com/}
\fi
\externaldocument[#1-#2-]{\FilePrefix #1.#2}[\wRef]
}

\makeatletter
%to reuse the data of \maketitle:
\newcommand\org@maketitle{}
\let\org@maketitle\maketitle
\def\maketitle{%
\hypersetup{pdftitle={\@title}}%
\hypersetup{pdfauthor={\authors}}%
\hypersetup{pdfsubject=\@keywords}%
\ifx\UseRussian\Defined
\pdfbookmark[1]{\@title}{TitleRussian}
\else
\pdfbookmark[1]{\@title}{TitleEnglish}
\fi
\org@maketitle
}
%Let's patch \make@stripped@name so that the language-prefix
%gets inserted also:
\def\make@stripped@name#1{%
\begingroup
\escapechar\m@ne
\global\let\newname\@empty
%Formerly ---and that's the only modification---the
%next line was: "\protected@edef\Hy@tempa{#1}%"
\protected@edef\Hy@tempa{\CurrentLanguage #1}%
\edef\@tempb{%
\noexpand\@tfor\noexpand\Hy@tempa:=%
\expandafter\strip@prefix\meaning\Hy@tempa
}%
\@tempb\do{%
\if\Hy@tempa\else
\if\Hy@tempa\else
\xdef\newname{\newname\Hy@tempa}%
\fi
\fi
}%
\endgroup
}%
%I change environment for bibliography
%because labels for bibliography also need language prefix
\newenvironment{enumBib}{%
\BibTitle
%\renewcommand\theenumiv{\arabic{enumiv}}\let\p@enumiv\@empty
%\list{\@biblabel{\theenumiv}}{}%{\settowidth\labelwidth{\@biblabel{#1}}%
%\usecounter{enumiv}%
\advance\@enumdepth \@ne
\edef\@enumctr{enum\romannumeral\the\@enumdepth}\list
{\csname biblabel\@enumctr\endcsname}{\usecounter
{\@enumctr}\def\makelabel##1{\hss\llap{\upshape##1}}}
}{%
\endlist
}
\let\endenumBib=\endlist % for efficiency
\def\biblabelenumi{[\LanguagePrefix \theenumi]}
\makeatletter

\newcommand{\BiblioItem}[2]
{
\def\Semafor{off}
\@ifundefined{\LanguagePrefix ViewCite#1}{}{%
\def\Semafor{on}%
}%
\ifx\Semafor\ValueOff
\@ifundefined{xRefDef#1}{}{% 
\def\Semafor{on}%
}%
\fi
\ifx\Semafor\ValueOn
\ifx\IndexState\ValueOff
\begin{enumBib}
%\begin{enumerate}
\def\IndexState{on}
\fi
\item \label{\LanguagePrefix bibitem: #1}#2%
\fi
}
\makeatother
\newcommand{\OpenBiblio}
{
\def\IndexState{off}
}
\newcommand{\CloseBiblio}
{
\ifx\IndexState\ValueOn
\end{enumBib}
%\end{enumerate}
\def\IndexState{off}
\fi
}

\makeatletter
\def\StartCite{[}%
\def\citeBib#1{\protect\showCiteBib#1,endCite,}%
\def\endCite{endCite}%
\def\showCiteBib#1,{\def\temp{#1}%
\ifx\temp\endCite
]%
\def\StartCite{[}%
\else
\StartCite\LanguagePrefix \ref{\LanguagePrefix bibitem: #1}%
\@ifundefined{\LanguagePrefix ViewCite#1}{%
\NameDef{\LanguagePrefix ViewCite#1}{}%
}{%
}%
\def\StartCite{, }%
\expandafter\showCiteBib%
\fi}%
\makeatother

\newcommand\setPdfOutline[5]
{
%1-external link
%2-ref
%3-file
%4-anchor
%5-text in bookmark
\pdfstringdef\tempa{\ref{#1-#2} }
\pdfstringdef\tempb{#5}
\pdfoutline goto file{#3.pdf} name{#4} {\tempa\tempb}
}
\newcommand{\arp}{\ar @{-->}}
%\newcommand{\ars}{\ar @{{}*{*}>}}
%\newcommand{\ars}{\ar @*{[|(2)]}@{.>}}
\newcommand{\ars}{\ar @{.>}}
\newcommand\Bundle[1]{{\mathbb #1}}%{{\bf #1}}
\newcommand{\bundle}[4]%
{%
\def\tempa{}%
\def\tempb{#3}%
\def\tempc{#1}%
\ifx\tempa\tempb%
\ifx\tempa\tempc%
#2%
\else%
\xymatrix{#2:#1\arp[r]&#4}%
\fi%
\else%
\ifx\tempa\tempc%
#2[#3]%
\else%
\xymatrix{#2[#3]:#1\arp[r]&#4}%
\fi%
\fi%
}%
\makeatletter
\newcommand{\AddIndex}[2]%
{%
\@ifundefined{RefIndex#2}{%
\xNameDef{RefIndex#2}{:}%
\@namedef{LabelIndex}{\label{index: #2::}}%
}{%
\addtocounter{Index}{1}%
\xNameDef{RefIndex#2}{\@nameuse{RefIndex#2},\arabic{Index}}%
\@namedef{LabelIndex}{\label{index: #2:\arabic{Index}}}%
}%
\@nameuse{LabelIndex}%
{\bf #1}%
}%

\newcommand{\Index}[2]%
{%
\@ifundefined{RefIndex#2}{%
\def\Semafor{off}%
}{%
\def\Semafor{on}%
}%
\ifx\Semafor\ValueOn%
\def\tempa{}%
\def\tempb{#2}%
\ifx\IndexState\ValueOff%
\ifx\setCACAA\undefined
\begin{theindex}%
\else
\section*{\indexname}%
\begin{itemize}
\fi
\def\IndexState{on}%
\fi%
\ifx\IndexSpace\ValueOn%
\indexspace%
\def\IndexSpace{off}%
\fi%
\item #1%
\ifx\tempa\tempb%
\else%
\edef\PageRefs{\@nameuse{RefIndex#2}}
\def\Sep{\ }%
\@for\PageRef:=\PageRefs\do{%
\Sep
\pageref{index: #2:\PageRef}%
\def\Sep{,\ }%
}%
\fi%
\fi%
}%

%\newcommand{\SubIndex}[3]
%{
%\def\Semafor{off}
%\Items{#1}
%\ifx\Semafor\ValueOn
%\subitem #2 \pageref{index: #3}%\RefPage{#3}
%\fi
%}%
%\newcommand{\AddIndexRef}[2]
%{%
%\def\Semafor{off}
%\Items{#1}
%\ifx\Semafor\ValueOn
%, \pageref{index: #2}%
%\fi%
%}%

\newcommand{\Symb}[4]%
{%
\def\Semafor{off}%
\@ifundefined{ViewSymbol#2}{%
\@ifundefined{ViewSymbol#2(#3-#4)}{%
}{%
\def\Semafor{on}
\edef\ThisSymbol{#2(#3-#4)}%
}%
}{%
\def\Semafor{on}%
\edef\ThisSymbol{#2}%
}%
\ifx\Semafor\ValueOn%
\ifx\IndexState\ValueOff%
\ifx\setCACAA\undefined
\begin{theindex}%
\else
\section*{\indexname}%
\begin{itemize}
\fi
\def\IndexState{on}%
\fi%
\ifx\IndexSpace\ValueOn%
\indexspace%
\def\IndexSpace{off}%
\fi%
\edef\Symbols{\@nameuse{ViewSymbol\ThisSymbol}}%
\@for\Symbol:=\Symbols\do{%
\edef\Temp{ViewSymbol\ThisSymbol:::\Symbol}%
\item $\displaystyle\textcolor{SymbColor}{\@nameuse{\Temp}}$
\ \ #1
\edef\PageRefs{\@nameuse{RefSymbol\ThisSymbol===\Symbol}}
\def\Sep{}%
\@for\PageRef:=\PageRefs\do{%
\Sep
\pageref{symbol: \ThisSymbol:\PageRef}%
\def\Sep{,\ }%
}%
}%
\fi
}

\newcommand{\Symba}[2]
{
\def\Semafor{off}
\@ifundefined{ViewSymbol#2}{%
}{%
\def\Semafor{on}
}%
\ifx\Semafor\ValueOn
\ifx\IndexState\ValueOff
\begin{theindex}
\def\IndexState{on}
\fi
\ifx\IndexSpace\ValueOn
\indexspace
\def\IndexSpace{off}
\fi
\item $\displaystyle\@nameuse{ViewSymbol#2}$\ \ #1
\edef\PageRefs{\@nameuse{RefSymbol#2}}
\def\Sep{}%
\@for\PageRef:=\PageRefs\do{%
\Sep
\pageref{symbol: #2:\PageRef}%
\def\Sep{,\ }%
}%
\fi
}
%\def\CiteBibNote{\xdef\@thefnmark{}\@footnotetext}
\def\CiteBibNote{\,\footnote[0]}
\makeatother
%\newcommand{\SubSymb}[3]
%{
%\def\Semafor{off}
%\Items{#1}
%\ifx\Semafor\ValueOn
%\subitem #2 \pageref{symbol: #3}
%\fi
%}%
%\newcommand{\AddSymbRef}[2]
%{%
%\def\Semafor{off}
%\Items{#1}
%\ifx\Semafor\ValueOn
%, \pageref{symbol: #2}%
%\fi%
%}%

\newcommand{\SetIndexSpace}%
{%
\def\IndexSpace{on}%
}%

\newcommand{\OpenIndex}
{
\def\IndexState{off}
}
\newcommand{\CloseIndex}
{
\ifx\IndexState\ValueOn
\ifx\setCACAA\undefined
\end{theindex}
\else
\end{itemize}
\fi
\def\IndexState{off}
\fi
}
\newcommand\CiteQuotation[2]
{
\leftskip=40pt
\Memos{#1}
\begin{flushright}
\begin{tabular}{r}
\hline
\makebox[100pt][r]{#2}\\
\end{tabular}
\end{flushright}
\leftskip=0pt
}
\newcommand\CiteQuote[2]
{
\leftskip=40pt
\BlueText{#1}%
\begin{flushright}
\begin{tabular}{r}
\hline
\makebox[100pt][r]{#2}\\
\end{tabular}
\end{flushright}
\leftskip=0pt
}
\def\epigraphSkip{150pt}
\newcommand\epigraph[2]
{
\leftskip=\epigraphSkip
\Memos{#1}
\begin{flushright}
\begin{tabular}{r}
\hline
\makebox[100pt][r]{#2}\\
\end{tabular}
\end{flushright}
\leftskip=0pt
}
\def\Memos#1{\MemoList#1//LastMemo//}%
\def\LastMemo{LastMemo}%
\def\MemoList#1//{\def\temp{#1}%
\ifx\temp\LastMemo
\else%
%\begin{flushright}
%\begin{minipage}{\epigraphWidth}
\setlength{\parindent}{5mm}
\par
%\setlength{\parindent}{12pt}
\BlueText{#1}%
%\end{minipage}
%\end{flushright}
\expandafter\MemoList%
\fi%
}     
%\listfiles


==> Index.English.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-form
   {$1$\Hyph form}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- ary fibered relation
   {$2$\Hyph ary fibered relation}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A algebra of polynomials over D algebra
   {$A$\Hyph algebra of polynomials over $D$\Hyph algebra $A$}%
   {algebra of polynomials over algebra}%
\Index%818%A%A number
   {$A$\Hyph number}%
   {A number}%
\Index%603%A%A(A) map
   {$\mathcal A(A)$\Hyph map}%
   {A(A) map}%
\Index%660%A%A* module
   {$A*$\Hyph module}%
   {A*-module}%
\Index%575%A%A*-vector space
   {$A*$\Hyph vector space}%
   {A*-vector space}%
\Index%685%A%A- module
   {$A$\Hyph module}%
   {module over algebra}%
\Index%5%A%A- valued function
   {$A$\Hyph valued function}%
   {A valued function}%
\Index%864%A%A-representation in Omega algebra
   {$A$\Hyph representation in $\Omega$\Hyph algebra}%
   {A representation of algebra}%
\Index%15%A%A-vector space
   {$A$\hyph vector space}%
   {A vector space}%
\Index%830%A%Abelian multiplicative Omega group
   {Abelian multiplicative $\Omega$\Hyph group}%
   {Abelian multiplicative Omega group}%
\Index%645%A%Abelian Omega group
   {Abelian $\Omega$\Hyph group}%
   {Abelian Omega group}%
\Index%869%A%Abelian semigroup
   {Abelian semigroup}%
   {Abelian semigroup}%
\Index%284%A%absolute value
   {absolute value}%
   {absolute value}%
\Index%99%A%active *G representation
   {active \sT{G}representation}%
   {active representation, vector space}%
\Index%100%A%active representation
   {active representation}%
   {active representation}%
\Index%569%A%active representation in basis manifold
   {active representation in basis manifold}%
   {active representation in basis manifold}%
\Index%716%A%active representation of group in basis manifold of tower of representations
   {active representation of group $G(\Vector f)$ in basis manifold of tower of representations}%
   {active representation in basis manifold, tower of representations}%
\Index%326%A%active transformation of basis manifold
   {active transformation of basis manifold}%
   {active transformation of basis}%
\Index%101%A%active transformation on basis manifold
   {active transformation on basis manifold}%
   {active transformation}%
\Index%102%A%active transformation on the set of rcd bases
   {active transformation on the set of \rcd bases}%
   {active transformation, vector space}%
\Index%805%A%additive map
   {additive map}%
   {additive map}%
\Index%110%A%affine basis
   {affine basis}%
   {Affine Basis}%
\Index%579%A%affine functional
   {affine functional}%
   {affine functional}%
\Index%682%A%affine representation of Lie group
   {affine representation of Lie group}%
   {affine representation of Lie group}%
\Index%734%A%affine space
   {affine space}%
   {affine space}%
\Index%733%A%affine structure on set
   {affine structure on set}%
   {affine structure on set}%
\Index%758%A%affine transformation
   {affine transformation}%
   {affine transformation}%
\Index%141%A%affine transformation group
   {affine transformation group}%
   {affine transformation group}%
\Index%142%A%affine transformation group
   {affine transformation group}%
   {affine transformation group}%
\Index%109%A%affine transformation on basis manifold
   {affine transformation on basis manifold}%
   {affine transformation}%
\Index%400%A%algebra of fractions of algebra with conjugation
   {algebra of fractions of algebra with conjugation}%
   {algebra of fractions of algebra with conjugation}%
\Index%487%A%algebra of polynomials over D algebra
   {algebra of polynomials over $D$\Hyph algebra}%
   {algebra of polynomials over D algebra}%
\Index%618%A%algebra of rational mappings of algebra
   {algebra of rational mappings of algebra}%
   {algebra of rational mappings of algebra}%
\Index%797%A%algebra of sets
   {algebra of sets}%
   {algebra of sets}%
\Index%607%A%algebra over ring
   {algebra over ring}%
   {algebra over ring}%
\Index%780%A%algebra with conjugation
   {algebra with conjugation}%
   {algebra with conjugation}%
\Index%907%A%alternation of polylinear map
   {alternation of polylinear map}%
   {alternation of polylinear map}%
\Index%105%A%alternative representation of matrix
   {alternative representation of matrix}%
   {Alternative representation}%
\Index%275%A%anholonomic coordinate
   {anholonomic coordinate}%
   {anholonomic coordinate}%
\Index%278%A%anholonomic coordinates of connection
   {anholonomic coordinates of connection}%
   {anholonomic coordinates of connection}%
\Index%276%A%anholonomic coordinates of vector
   {anholonomic coordinates of vector}%
   {vector anholonomic coordinates}%
\Index%277%A%anholonomic coordinates on manifold
   {anholonomic coordinates on manifold}%
   {anholonomic coordinates on manifold}%
\Index%293%A%anholonomity object
   {anholonomity object}%
   {anholonomity object}%
\Index%929%A%antilinear homomorphism
   {antilinear homomorphism}%
   {antilinear homomorphism}%
\Index%779%A%antilinear map
   {antilinear map}%
   {antilinear map}%
\Index%107%A%antisymmetric 2- ary fibered relation
   {antisymmetric $2$\Hyph ary fibered relation}%
   {antisymmetric 2 ary fibered relation}%
\Index%582%A%Arc basis for vector space
   {$A\RCstar$\Hyph basis for vector space}%
   {Arc basis, vector space}%
\Index%849%A%arity
   {arity}%
   {arity}%
\Index%108%A%arity of operation
   {arity of operation}%
   {arity of operation}%
\Index%617%A%associative D algebra
   {associative $D$\Hyph algebra}%
   {associative D algebra}%
\Index%662%A%associative law
   {associative law}%
   {associative law}%
\Index%943%A%associative multiplicative Omega group
   {associative multiplicative $\Omega$\Hyph group}%
   {associative multiplicative Omega group}%
\Index%89%A%associative Omega group
   {associative $\Omega$\Hyph group}%
   {associative Omega group}%
\Index%866%A%associative operation
   {associative operation}%
   {associative operation}%
\Index%616%A%associator of D algebra
   {associator of $D$\Hyph algebra}%
   {associator of algebra}%
\Index%437%A%augmented matrix
   {augmented matrix}%
   {augmented matrix}%
\Index%95%A%auto parallel line
   {auto parallel line}%
   {auto parallel line}%
\Index%859%A%automorphism
   {automorphism}%
   {automorphism}%
\Index%939%A%automorphism of diagram of representations
   {automorphism of diagram of representations}%
   {automorphism of diagram of representations}%
\Index%94%A%automorphism of representation of Omega algebra
   {automorphism of representation of $\Omega$\Hyph algebra}%
   {automorphism of representation}%
\Index%560%A%automorphism of tower of representations
   {automorphism of tower of representations}%
   {automorphism of tower of representations}%
\Index%22%A%automorphism of vector space
   {automorphism of vector space}%
   {automorphism of vector space}%
\Index%3%A%j i-CR quasideterminant
   {$(^j_i)$\hyph \CR quasideterminant}%
   {j i cr-quasideterminant}%
\Index%282%A%norm of quaternion
   {norm of quaternion}%
   {norm of quaternion}%
\SetIndexSpace%
\Index%799%B%b set
   {$B$\Hyph set}%
   {B set}%
\Index%503%B%Banach D- algebra
   {Banach $D$\Hyph algebra}%
   {Banach algebra}%
\Index%313%B%Banach D- module
   {Banach $D$\Hyph module}%
   {Banach module}%
\Index%114%B%base of fibered correspondence
   {base of fibered correspondence}%
   {base of fibered correspondence}%
\Index%113%B%base of mapping
   {base of mapping}%
   {base of map}%
\Index%115%B%basis
   {basis}%
   {Basis}%
\Index%49%B%basis dual to basis
   {basis dual to basis}%
   {basis dual to basis}%
\Index%223%B%basis dual to basis
   {basis dual to basis}%
   {dual basis}%
\Index%203%B%basis for crd vector space
   {basis for \crd vector space}%
   {basis, crd vector space}%
\Index%106%B%basis for dcr vector space
   {basis for \dcr vector space}%
   {basis, dcr vector space}%
\Index%16%B%basis for drc vector space
   {basis for \drc vector space}%
   {basis, drc vector space}%
\Index%659%B%basis for module
   {basis for module}%
   {basis, module}%
\Index%24%B%basis for rcd vector space
   {basis for \rcd vector space}%
   {basis, rcd vector space}%
\Index%197%B%basis for vector space
   {basis for vector space}%
   {basis, vector space}%
\Index%536%B%basis manifold
   {basis manifold}%
   {basis manifold}%
\Index%256%B%basis manifold of affine space
   {basis manifold of affine space}%
   {Basis Manifold, Affine Space}%
\Index%262%B%basis manifold of central affine space
   {basis manifold of central affine space}%
   {Basis Manifold, Central Affine Space}%
\Index%259%B%basis manifold of Euclid space
   {basis manifold of Euclid space}%
   {Basis Manifold, Euclid Space}%
\Index%260%B%basis manifold of Euclid space
   {basis manifold of Euclid space}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%714%B%basis manifold of tower of representations
   {basis manifold of tower of representations}%
   {basis manifold tower of representations}%
\Index%653%B%basis of algebra L(A,A)
   {basis of algebra $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%699%B%basis of diagram of representations
   {basis of diagram of representations}%
   {basis of diagram of representations}%
\Index%329%B%basis of representation
   {basis of representation}%
   {basis of representation}%
\Index%567%B%basis of tower of representations
   {basis of tower of representations}%
   {basis of tower of representations}%
\Index%116%B%basis vector of representation of Lie group over algebra A
   {basis vector of representation of Lie group over algebra $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%122%B%biring
   {biring}%
   {biring}%
\Index%808%B%Borel algebra
   {Borel algebra}%
   {Borel algebra}%
\Index%798%B%borel set
   {Borel set}%
   {Borel set}%
\Index%803%B%Borel-measurable map
   {Borel\Hyph measurable map}%
   {Borel-measurable map}%
\Index%419%B%bundle of level 2
   {bundle of level $2$}%
   {bundle of level 2}%
\Index%418%B%bundle of level n
   {bundle of level $n$}%
   {bundle of level n}%
\SetIndexSpace%
\Index%6%C%c row of matrix
   {\subs row of matrix}%
   {c row}%
\Index%12%C%c-row of matrix
   {$c$\hyph row of matrix}%
   {c-row}%
\Index%860%C%can be embeded
   {can be embeded}%
   {can be embeded}%
\Index%701%C%cancellation law
   {cancellation law}%
   {cancellation law}%
\Index%913%C%canonical map
   {canonical map}%
   {canonical map}%
\Index%368%C%canonical map
   {canonical map}%
   {canonical map}%
\Index%726%C%canonical remainder of the division
   {canonical remainder of the division}%
   {canonical remainder of the division}%
\Index%599%C%canonical representation of division with remainder
   {canonical representation of division with remainder}%
   {canonical representation of division with remainder}%
\Index%852%C%carrier of Omega-algebra
   {carrier of $\Omega$\Hyph algebra}%
   {carrier of Omega-algebra}%
\Index%443%C%Cartan connection
   {Cartan connection}%
   {Cartan connection}%
\Index%227%C%Cartan curvature
   {Cartan curvature}%
   {Cartan curvature}%
\Index%401%C%Cartan derivative
   {Cartan derivative}%
   {Cartan derivative}%
\Index%925%C%Cartan equation
   {Cartan equation}%
   {Cartan equation}%
\Index%444%C%Cartan symbol
   {Cartan symbol}%
   {Cartan symbol}%
\Index%338%C%Cartan transport
   {Cartan transport}%
   {Cartan transport}%
\Index%865%C%Cartesian power
   {Cartesian power}%
   {Cartesian power}%
\Index%149%C%Cartesian power A of bundle B
   {Cartesian power $\Bundle A$ of bundle $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%148%C%Cartesian power A of set B
   {Cartesian power $A$ of set $B$}%
   {Cartesian power of set}%
\Index%150%C%Cartesian power n of bundle E
   {Cartesian power $n$ of bundle $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%594%C%Cartesian power n of H algebra
   {Cartesian power $n$ of $\mathfrak{H}$\Hyph algebra}%
   {Cartesian power of algebra}%
\Index%655%C%Cartesian power of systems of subsets
   {Cartesian power of systems of subsets}%
   {Cartesian power of systems of subsets}%
\Index%390%C%Cartesian product of groups
   {Cartesian product of groups}%
   {Cartesian product of groups}%
\Index%199%C%Cartesian product of measures
   {Cartesian product of measures}%
   {Cartesian product of measures}%
\Index%825%C%Cartesian product of Omega algebras
   {Cartesian product of \(\Omega\)\Hyph algebras}%
   {Cartesian product of Omega algebras}%
\Index%625%C%Cartesian product of systems of subsets
   {Cartesian product of systems of subsets}%
   {Cartesian product of systems of subsets}%
\Index%175%C%category of drc vector spaces
   {category of \drc vector spaces}%
   {category of drc vector spaces}%
\Index%179%C%category of fibered correspondences over diagonal
   {category of fibered correspondences over diagonal}%
   {category of fibered correspondences over diagonal}%
\Index%177%C%category of left-side representations
   {category of left-side representations}%
   {category of left-side representations}%
\Index%176%C%category of left-side representations of Omega1 algebra
   {category of left-side representations of $\Omega_1$\Hyph algebra $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%178%C%category of reduced fibered correspondences
   {category of reduced fibered correspondences}%
   {category of reduced fibered correspondences}%
\Index%887%C%category of representations
   {category of representations}%
   {category of representations}%
\Index%241%C%Cauchy sequence
   {Cauchy sequence}%
   {Cauchy sequence}%
\Index%722%C%center of A number
   {center of $A$\Hyph number}%
   {center of A number}%
\Index%620%C%center of algebra
   {center of $D$\Hyph algebra $A$}%
   {center of algebra}%
\Index%507%C%center of ring D
   {center of ring $D$}%
   {center of ring}%
\Index%509%C%central affine basis
   {central affine basis}%
   {Central Affine Basis}%
\Index%807%C%closed ball
   {closed ball}%
   {closed ball}%
\Index%80%C%closure of set
   {closure of set}%
   {closure of set}%
\Index%821%C%coefficient of polynomial
   {coefficient of polynomial}%
   {coefficient of polynomial}%
\Index%258%C%colinear vectors
   {colinear vectors}%
   {colinear vectors}%
\Index%92%C%column D* vector
   {column $D*$\Hyph vector}%
   {column D* vector}%
\Index%750%C%column determinant
   {column determinant}%
   {column determinant}%
\Index%124%C%column vector
   {column vector}%
   {column vector}%
\Index%482%C%common factor
   {common factor}%
   {common factor}%
\Index%615%C%commutative D algebra
   {commutative $D$\Hyph algebra}%
   {commutative D algebra}%
\Index%190%C%commutative diagram of correspondences
   {commutative diagram of correspondences}%
   {commutative diagram of correspondences}%
\Index%936%C%commutative diagram of representations of universal algebras
   {commutative diagram of representations of universal algebras}%
   {commutative diagram of representations}%
\Index%964%C%commutative law
   {commutative law}%
   {commutative law}%
\Index%867%C%commutative operation
   {commutative operation}%
   {commutative operation}%
\Index%832%C%commutativity of representations
   {commutativity of representations}%
   {commutativity of representations}%
\Index%614%C%commutator of D algebra
   {commutator of $D$\Hyph algebra}%
   {commutator of algebra}%
\Index%815%C%compact set
   {compact set}%
   {compact set}%
\Index%191%C%compact-open topology
   {compact\hyph open topology}%
   {compact open topology}%
\Index%349%C%complete division ring
   {complete division ring}%
   {complete division ring}%
\Index%764%C%complete measure
   {complete measure}%
   {complete measure}%
\Index%811%C%complete normed Omega group
   {complete normed $\Omega$\Hyph group}%
   {complete Omega group}%
\Index%270%C%complete ring
   {complete ring}%
   {complete ring}%
\Index%348%C%complete system of linear partial differential equations
   {complete system of linear partial differential equations}%
   {Complete System of Linear Partial Differential Equations}%
\Index%128%C%completely integrable system
   {completely integrable system}%
   {completely integrable system}%
\Index%186%C%completion of normed Omega group
   {completion of normed $\Omega$\Hyph group}%
   {completion of normed Omega group}%
\Index%19%C%completion of representation
   {completion of representation}%
   {completion of representation}%
\Index%879%C%component of derivative
   {component of derivative}%
   {component of derivative}%
\Index%883%C%component of derivative of Second Order
   {component of derivative of Second Order}%
   {component of derivative of Second Order}%
\Index%193%C%component of linear map
   {component of linear map}%
   {component of linear map}%
\Index%647%C%component of polylinear map
   {component of polylinear map}%
   {component of polylinear map}%
\Index%629%C%component of the Gateaux derivative
   {component of the G\^ateaux derivative}%
   {component of Gateaux derivative}%
\Index%633%C%component of the Gateaux derivative of second order
   {component of the G\^ateaux derivative of second order}%
   {component of Gateaux derivative of Second Order}%
\Index%394%C%composition of fibered correspondences
   {composition of fibered correspondences}%
   {composition of fibered correspondences}%
\Index%393%C%composition of reduced fibered correspondences
   {composition of reduced fibered correspondences}%
   {composition of reduced fibered correspondences}%
\Index%495%C%condition of reducibility of products
   {condition of reducibility of products}%
   {condition of reducibility of products}%
\Index%873%C%congruence
   {congruence}%
   {congruence}%
\Index%746%C%conjugate of quaternion
   {conjugate of quaternion $x$}%
   {conjugate of quaternion}%
\Index%683%C%conjugated affine space
   {conjugated affine space}%
   {conjugated affine space}%
\Index%580%C%conjugated D module
   {conjugated $D$\Hyph  module}%
   {conjugated D module}%
\Index%789%C%conjugated vector space
   {conjugated vector space}%
   {conjugated vector space}%
\Index%788%C%conjugation in algebra
   {conjugation in algebra}%
   {conjugation in algebra}%
\Index%777%C%conjugation in ring
   {conjugation in ring}%
   {conjugation in ring}%
\Index%23%C%conjugation transformation
   {conjugation transformation}%
   {conjugation transformation}%
\Index%517%C%connected set
   {connected set}%
   {connected set}%
\Index%538%C%connection coefficients in D affine space
   {connection coefficients in affine space}%
   {connection coefficients, affine space}%
\Index%583%C%connection in principal fibre bundle
   {connection in principal fibre bundle}%
   {connection in principal bundle}%
\Index%824%C%contact point of set
   {contact point of set}%
   {contact point of set}%
\Index%668%C%continues basis
   {continues basis}%
   {continues basis}%
\Index%281%C%continuous correspondence
   {continuous correspondence}%
   {continuous correspondence}%
\Index%280%C%continuous map
   {continuous map}%
   {continuous map}%
\Index%610%C%continuous multivariable map
   {continuous multivariable map}%
   {continuous multivariable map}%
\Index%960%C%continuous Schauder basis
   {continuous Schauder basis}%
   {continuous Schauder basis}%
\Index%968%C%contravariant representation
   {contravariant representation}%
   {contravariant representation}%
\Index%781%C%convex set
   {convex set}%
   {convex set}%
\Index%215%C%coordinate isomorphism
   {coordinate isomorphism}%
   {coordinate isomorphism}%
\Index%206%C%coordinate matrix of set of vectors
   {coordinate matrix of set of vectors}%
   {coordinate matrix of set of vectors}%
\Index%691%C%coordinate matrix of vector
   {coordinate matrix of vector}%
   {coordinate matrix of vector}%
\Index%205%C%coordinate matrix of vector field in rcD basis
   {coordinate matrix of vector field in \rcD basis}%
   {coordinate matrix of vector field in drc basis}%
\Index%209%C%coordinate rcd vector space
   {coordinate \rcd vector space}%
   {coordinate rcd vector space}%
\Index%208%C%coordinate reference frame
   {coordinate reference frame}%
   {coordinate reference frame}%
\Index%697%C%coordinate representation
   {coordinate representation}%
   {coordinate representation}%
\Index%720%C%coordinate representation in tuple of Omega- algebras
   {coordinate representation in tuple of $\VX\Omega$\Hyph algebras}%
   {coordinate tower of representations, Omega algebra}%
\Index%213%C%coordinate representation of group in vector space
   {coordinate representation of group in vector space}%
   {coordinate representation, vector space}%
\Index%664%C%coordinate representation of vector
   {coordinate representation of vector}%
   {coordinate representation of vector}%
\Index%210%C%coordinate vector bundle
   {coordinate vector bundle}%
   {coordinate vector bundle}%
\Index%211%C%coordinate vector space
   {coordinate vector space}%
   {coordinate vector space}%
\Index%738%C%coordinates
   {coordinates}%
   {coordinates}%
\Index%558%C%coordinates of A number relative to set
   {coordinates of $A_2$\Hyph number $m$ relative to set $X$}%
   {coordinates relative to set}%
\Index%927%C%coordinates of associator
   {coordinates of associator}%
   {coordinates of associator}%
\Index%25%C%coordinates of basis
   {coordinates of basis}%
   {coordinates of basis}%
\Index%325%C%coordinates of basis of representation
   {coordinates of basis of representation}%
   {coordinates of basis relative to basis, representation}%
\Index%696%C%coordinates of endomorphism of representation
   {coordinates of endomorphism of representation}%
   {coordinates of endomorphism, representation}%
\Index%711%C%coordinates of endomorphism of tower of representations
   {coordinates of endomorphism of tower of representations}%
   {coordinates of endomorphism, tower of representations}%
\Index%221%C%coordinates of geometric object
   {coordinates of geometric object}%
   {coordinates of geometric object}%
\Index%974%C%coordinates of homomorphism
   {coordinates of homomorphism}%
   {coordinates of homomorphism}%
\Index%967%C%coordinates of morphism of diagram of representations
   {coordinates of morphism of diagram of representations}%
   {coordinates of morphism, diagram of representations}%
\Index%730%C%coordinates of point of affine space relative to basis)$
   {coordinates of point $A$ of affine space $\overset{\circ}{A}$ relative to basis $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%945%C%coordinates of reduced morphism of representation
   {coordinates of reduced morphism of representation}%
   {coordinates of reduced morphism of representation}%
\Index%224%C%coordinates of representation
   {coordinates of representation}%
   {coordinates of representation, drc vector space}%
\Index%225%C%coordinates of representation
   {coordinates of representation}%
   {coordinates of representation}%
\Index%222%C%coordinates of set of vectors
   {coordinates of set of vectors}%
   {coordinates of set of vectors}%
\Index%216%C%coordinates of vector
   {coordinates of vector}%
   {coordinates of vector}%
\Index%217%C%coordinates of vector field in Drc basis
   {coordinates of vector field in \Drc basis}%
   {coordinates of vector field in drc basis}%
\Index%286%C%coordinates of vector relative to Hamel basis
   {coordinates of vector relative to Hamel basis}%
   {coordinates of vector, Hamel basis}%
\Index%676%C%coordinates of vector relative to Schauder basis
   {coordinates of vector relative to Schauder basis}%
   {coordinates of vector, Schauder basis}%
\Index%910%C%coproduct in category
   {coproduct of objects in category}%
   {coproduct in category}%
\Index%455%C%correspondence continuous on the set
   {correspondence continuous on the set}%
   {correspondence continuous on the set}%
\Index%454%C%correspondence of homomorphism
   {correspondence of homomorphism}%
   {correspondence of homomorphism}%
\Index%840%C%cosine
   {cosine}%
   {cosine}%
\Index%969%C%covariant representation
   {covariant representation}%
   {covariant representation}%
\Index%949%C%CR exponent
   {\CR exponent}%
   {CR exponent}%
\Index%8%C%CR inverse element of biring
   {\CR inverse element of biring}%
   {cr-inverse element}%
\Index%7%C%CR matrix group
   {\CR matrix group}%
   {cr-matrix group}%
\Index%956%C%cr nonsingular matrix
   {\CR nonsingular matrix}%
   {cr nonsingular matrix}%
\Index%10%C%CR power
   {\CR power}%
   {cr power}%
\Index%9%C%CR product
   {\CR product (product column over row)}%
   {cr-product}%
\Index%589%C%cr product of matrices of maps
   {$\CRcirc$\Hyph product of matrices of maps}%
   {cr product of matrices of maps}%
\Index%705%C%cr singular matrix
   {\CR singular matrix}%
   {cr singular matrix}%
\Index%134%C%cr-inverse matrix
   {\CR inverse matrix}%
   {cr-inverse matrix}%
\Index%954%C%cr-quasideterminant
   {\CR quasideterminant}%
   {cr-quasideterminant}%
\Index%304%C%crd vector
   {\crd vector}%
   {crd vector}%
\Index%11%C%crd vector space
   {\crd vector space}%
   {crd vector space}%
\Index%768%C%Cstar-algebra
   {$C^*$\Hyph algebra}%
   {Cstar-algebra}%
\Index%537%C%curvilinear coordinates of point in affine space
   {curvilinear coordinates of point in affine space}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%581%D%D linear functional
   {$D$\Hyph linear functional}%
   {D linear functional}%
\Index%87%D%D*- matrices vector space
   {$D*$\hyph matrices vector space}%
   {matrices vector space}%
\Index%40%D%D*- vector space
   {$D*$\hyph  vector space}%
   {D* vector space}%
\Index%156%D%D*-module
   {$D*$\Hyph module}%
   {D*-module}%
\Index%549%D%D- affine connection on manifold with affine connections
   {$D$\Hyph affine connection on manifold with affine connections}%
   {D affine connection, affine manifold}%
\Index%251%D%D- algebra
   {$D$\Hyph algebra}%
   {D algebra}%
\Index%71%D%D- module
   {$D$\Hyph module}%
   {D-module}%
\Index%584%D%D- module
   {$D$\Hyph module}%
   {D module}%
\Index%48%D%D- valued variable
   {$D$\Hyph valued variable}%
   {D valued variable}%
\Index%14%D%D- vector function
   {$D$\Hyph vector function}%
   {d vector function}%
\Index%550%D%D-affine connection coefficients on manifold
   {$D$\Hyph affine connection coefficients on manifold}%
   {D affine connection coefficients, manifold}%
\Index%200%D%dcr vector
   {\dcr vector}%
   {dcr vector}%
\Index%18%D%dcr vector space
   {\dcr vector space}%
   {dcr vector space}%
\Index%740%D%definite integral
   {definite integral}%
   {definite integral}%
\Index%878%D%derivative of map
   {derivative of map}%
   {derivative of map}%
\Index%884%D%derivative of order n
   {derivative of order $n$}%
   {derivative of Order n}%
\Index%882%D%derivative of second order
   {derivative of second order}%
   {derivative of Second Order}%
\Index%303%D%determinant of matrix
   {determinant of matrix}%
   {determinant}%
\Index%309%D%deviation of trajectories
   {deviation of trajectories}%
   {deviation of trajectories}%
\Index%153%D%diagonal in bundle
   {diagonal in bundle}%
   {diagonal in bundle}%
\Index%154%D%diagram of correspondences
   {diagram of correspondences}%
   {diagram of correspondences}%
\Index%725%D%diagram of representations
   {diagram of representations}%
   {diagram of representations}%
\Index%935%D%diagram of representations of universal algebras
   {diagram of representations of universal algebras}%
   {diagram of representations of algebras}%
\Index%877%D%differentiable map
   {differentiable map}%
   {differentiable map}%
\Index%919%D%differential equation with separated variables
   {differential equation with separated variables}%
   {differential equation with separated variables}%
\Index%737%D%differential form of degree p
   {differential form of degree $p$}%
   {differential form of degree p}%
\Index%661%D%differential of independent variable
   {differential of independent variable}%
   {differential of independent variable}%
\Index%157%D%differential of map
   {differential of map}%
   {differential of map}%
\Index%902%D%differential p form
   {differential $p$\Hyph form}%
   {differential p form}%
\Index%922%D%differential separable equation
   {differential separable equation}%
   {differential separable equation}%
\Index%417%D%dimension of rcd vector space
   {dimension of \rcd vector space}%
   {dimension of vector space}%
\Index%151%D%direct product of bundles
   {direct product of bundles}%
   {Cartesian product of bundles}%
\Index%410%D%direct product of D- vector spaces
   {direct product of $D$\Hyph vector spaces}%
   {direct product of D vector spaces}%
\Index%415%D%direct product of division rings
   {direct product of division rings}%
   {direct product of division rings}%
\Index%412%D%direct product of G* representations
   {direct product of \Ts{G}representations}%
   {direct product of G* representations}%
\Index%826%D%direct product of Omega algebras
   {direct product of \(\Omega\)\Hyph algebras}%
   {direct product of Omega algebras}%
\Index%411%D%direct product of rcd vector spaces
   {direct product of \rcd vector spaces}%
   {direct product, rcd vector space}%
\Index%414%D%direct product of representations of fibered group
   {direct product of representations of fibered group}%
   {direct product of representations of fibered group}%
\Index%413%D%direct product of representations of group
   {direct product of representations of group}%
   {direct product of representations of group}%
\Index%152%D%direct product of total spaces
   {direct product of total spaces}%
   {Cartesian product of total spaces}%
\Index%911%D%direct sum
   {direct sum}%
   {direct sum}%
\Index%409%D%direct sum of representations
   {direct sum of representations}%
   {direct sum of representations}%
\Index%763%D%direction over commutative ring
   {direction over commutative ring}%
   {direction over commutative ring}%
\Index%672%D%distributive law
   {distributive law}%
   {distributive law}%
\Index%167%D%division algebra
   {division algebra}%
   {division algebra}%
\Index%573%D%division with remainder
   {division with remainder}%
   {division with remainder}%
\Index%598%D%division without remainder
   {division without remainder}%
   {division without remainder}%
\Index%820%D%divisor of polynomial
   {divisor of polynomial}%
   {divisor of polynomial}%
\Index%755%D%double determinant
   {double determinant}%
   {double determinant}%
\Index%36%D%Drc linear map of vector bundles
   {\Drc linear map of vector bundles}%
   {drc linear map of vector bundles}%
\Index%17%D%drc vector
   {\drc vector}%
   {drc vector}%
\Index%28%D%drc vector space
   {\drc vector space}%
   {drc vector space}%
\Index%771%D%Dstar antilinear homomorphism
   {$D\star$\Hyph antilinear homomorphism}%
   {Dstar antilinear homomorphism}%
\Index%41%D%Dstar- vector bundle
   {$\mathcal D\star$\Hyph vector bundle}%
   {Dstar vector bundle}%
\Index%39%D%Dstar- vector field
   {$\mathcal D\star$\Hyph vector field}%
   {Dstar vector field}%
\Index%43%D%Dstar-linear composition of vector fields
   {$\mathcal D\star$\hyph linear composition of vector fields}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-product of vector field over scalar
   {$\mathcal D\star$\hyph product of vector field over scalar}%
   {Dstar product of vector field over scalar, vector space}%
\Index%159%D%dual space of rcd vector space
   {dual space of \rcd vector space}%
   {dual space of rcd vector space}%
\Index%382%D%duality principle for biring
   {duality principle for biring}%
   {duality principle for biring}%
\Index%383%D%duality principle for biring of matrices
   {duality principle for biring of matrices}%
   {duality principle for biring of matrices}%
\SetIndexSpace%
\Index%516%E%effective G* representation
   {effective \Ts{G}representation}%
   {effective G* representation}%
\Index%500%E%effective representation
   {effective representation}%
   {effective representation}%
\Index%521%E%effective representation of division ring
   {effective representation of division ring}%
   {effective representation of division ring}%
\Index%519%E%effective representation of fibered Omega- algebra
   {effective representation of fibered $\Omega$\Hyph algebra}%
   {effective representation of fibered Omega-algebra}%
\Index%518%E%effective representation of group
   {effective representation of group}%
   {effective representation of group}%
\Index%622%E%effective representation of ring
   {effective representation of ring}%
   {effective representation of ring}%
\Index%514%E%effective Tstar- representation of fibered division ring
   {effective \Ts representation of fibered division ring}%
   {effective representation of fibered division ring}%
\Index%520%E%effective Tstar- representation of fibered group
   {effective \Ts representation of fibered group}%
   {effective representation of fibered group}%
\Index%947%E%eigencolumn
   {eigencolumn}%
   {eigencolumn}%
\Index%965%E%eigenrow
   {eigenrow}%
   {eigenrow}%
\Index%946%E%eigenvalue
   {eigenvalue}%
   {eigenvalue}%
\Index%966%E%eigenvector
   {eigenvector}%
   {eigenvector}%
\Index%924%E%Einstein equation
   {Einstein equation}%
   {Einstein equation}%
\Index%858%E%endomorphism
   {endomorphism}%
   {endomorphism}%
\Index%938%E%endomorphism of diagram of representations
   {endomorphism of diagram of representations}%
   {endomorphism of diagram of representations}%
\Index%557%E%endomorphism of representation of Omega algebra
   {endomorphism of representation of $\Omega$\Hyph algebra}%
   {endomorphism of representation}%
\Index%327%E%endomorphism of representation regular on generating set X
   {endomorphism of representation regular on generating set $X$}%
   {endomorphism of representation, regular on set}%
\Index%328%E%endomorphism of representation singular on generating set X
   {endomorphism of representation singular on generating set $X$}%
   {endomorphism of representation, singular on set}%
\Index%559%E%endomorphism of tower of representations
   {endomorphism of tower of representations}%
   {endomorphism of tower of representations}%
\Index%564%E%endomorphism of tower of representations regular on tuple of generating sets
   {endomorphism of tower of representations regular on tuple of generating sets}%
   {endomorphism of representation, regular on tuple}%
\Index%565%E%endomorphism of tower of representations singular on tuple of generating sets
   {endomorphism of tower of representations singular on tuple of generating sets}%
   {endomorphism of representation, singular on tuple}%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\Index%857%E%epimorphism
   {epimorphism}%
   {epimorphism}%
\Index%931%E%equivalence
   {equivalence}%
   {equivalence}%
\Index%706%E%equivalence generated by representation
   {equivalence generated by representation $f$}%
   {equivalence of representation}%
\Index%917%E%equivalent norms
   {equivalent norms}%
   {equivalent norms}%
\Index%51%E%essential parameters in a set of functions
   {essential parameters in a set of functions}%
   {essential parameters}%
\Index%539%E%Euclidean metric on division ring
   {Euclidean metric on division ring}%
   {Euclidean metric on division ring}%
\Index%547%E%Euclidean scalar product in D- vector space
   {Euclidean scalar product in $D$\Hyph vector space}%
   {Euclidean scalar product, vector space}%
\Index%542%E%Euclidean scalar product on division ring
   {Euclidean scalar product on division ring}%
   {Euclidean scalar product on division ring}%
\Index%231%E%everywhere dense subset
   {everywhere dense subset}%
   {everywhere dense subset}%
\Index%920%E%exact differential equation
   {exact differential equation}%
   {exact differential equation}%
\Index%724%E%exact sequence
   {exact sequence}%
   {exact sequence}%
\Index%204%E%expansion of vector relative to basis converges
   {expansion of vector relative to basis converges}%
   {expansion converges}%
\Index%621%E%expansion of vector relative to basis converges normally
   {expansion of vector relative to basis converges normally}%
   {expansion converges normally}%
\Index%836%E%exponent
   {exponent}%
   {exponent}%
\Index%386%E%extension of correspondence
   {extension of correspondence}%
   {extension of correspondence}%
\Index%162%E%extension of measure
   {extension of measure}%
   {extension of measure}%
\Index%508%E%exterior differential
   {exterior differential}%
   {exterior differential}%
\Index%908%E%exterior product
   {exterior product}%
   {exterior product}%
\Index%515%E%extreme line
   {extreme line}%
   {extreme line}%
\SetIndexSpace%
\Index%369%F%factor group
   {factor group}%
   {factor group}%
\Index%434%F%fibered coordinate isomorphism
   {fibered coordinate isomorphism}%
   {fibered coordinate isomorphism}%
\Index%432%F%fibered correspondence from A to B
   {fibered correspondence from $\Bundle A$ to $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%430%F%fibered correspondence in A
   {fibered correspondence in $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%F%fibered correspondence of homomorphism
   {fibered correspondence of homomorphism}%
   {fibered correspondence of homomorphism}%
\Index%427%F%fibered equivalence
   {fibered equivalence}%
   {fibered equivalence}%
\Index%422%F%fibered group
   {fibered group}%
   {fibered group}%
\Index%436%F%fibered identification morphism
   {fibered identification morphism}%
   {fibered identification morphism}%
\Index%424%F%fibered little group
   {fibered little group}%
   {fibered little group}%
\Index%435%F%fibered morphism from bundle A into B
   {fibered morphism from bundle $\Bundle A$ into $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%433%F%fibered natural morphism
   {fibered natural morphism}%
   {fibered natural morphism}%
\Index%420%F%fibered Omega- algebra
   {fibered $\Omega$\Hyph algebra}%
   {fibered Omega-algebra}%
\Index%421%F%fibered Omega- subalgebra
   {fibered $\Omega$\Hyph subalgebra}%
   {fibered Omega-subalgebra}%
\Index%426%F%fibered ordering
   {fibered ordering}%
   {fibered ordering}%
\Index%425%F%fibered preordering
   {fibered preordering}%
   {fibered preordering}%
\Index%428%F%fibered ring
   {fibered ring}%
   {fibered ring}%
\Index%423%F%fibered stability group
   {fibered stability group}%
   {fibered stability group}%
\Index%429%F%fibered subset
   {fibered subset}%
   {fibered subset}%
\Index%923%F%field equation
   {field equation}%
   {field equation}%
\Index%479%F%field-strength tensor
   {field-strength tensor}%
   {field-strength tensor}%
\Index%497%F%filter F converges to A
   {filter $\mathfrak{F}$ converges to $A$}%
   {filter converges}%
\Index%170%F%finite expansion of set
   {finite expansion of set}%
   {finite expansion of set}%
\Index%131%F%Finsler metric
   {Finsler metric}%
   {Finsler metric}%
\Index%77%F%Finsler space
   {Finsler space}%
   {Finsler space}%
\Index%574%F%Finsler structure
   {Finsler structure}%
   {Finsler structure}%
\Index%963%F%first integral
   {first integral}%
   {first integral}%
\Index%337%F%first Newton law
   {first Newton law}%
   {First Newton law}%
\Index%872%F%frame dragging effect
   {frame\Hyph dragging effect}%
   {frame dragging effect}%
\Index%690%F%free A- module
   {free $A$\Hyph module}%
   {free A module}%
\Index%331%F%free Abelian group
   {free Abelian group}%
   {free Abelian group}%
\Index%606%F%free algebra over ring
   {free algebra over ring}%
   {free algebra over ring}%
\Index%612%F%free module
   {free module}%
   {free module}%
\Index%862%F%free representation
   {free representation}%
   {free representation}%
\Index%441%F%free representation of group
   {free representation of group}%
   {free representation of group}%
\Index%442%F%free Tstar- representation of fibered group
   {free \Ts representation of fibered group}%
   {free representation of fibered group}%
\Index%339%F%Frenet transport
   {Frenet transport}%
   {Frenet transport}%
\Index%155%F%function homogeneous of degree
   {function homogeneous of degree $k$}%
   {function homogeneous}%
\Index%504%F%function of division ring Dstar differentiable in the Fr\'echet sense
   {function of division ring \Ds differentiable in the Fr\'echet sense}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%243%F%fundamental sequence
   {fundamental sequence}%
   {fundamental sequence}%
\SetIndexSpace%
\Index%52%G%G- reference frame
   {$G$\Hyph reference frame}%
   {G reference frame}%
\Index%53%G%G-basis of vector space
   {$G$\Hyph basis of vector space}%
   {G-basis}%
\Index%54%G%G-coordinates of basis
   {$G$\Hyph coordinates of basis}%
   {G-coordinates}%
\Index%55%G%G-space
   {$G$\Hyph space}%
   {GSpace}%
\Index%38%G%Gateaux dcr derivative of map of D- vector space V to D- vector space W
   {the G\^ateaux \dcr derivative of map $f$ of $D$\Hyph vector space $V$ to $D$\Hyph vector space $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%627%G%Gateaux derivative of map
   {the G\^ateaux derivative of map}%
   {Gateaux derivative of map}%
\Index%399%G%Gateaux derivative of order n
   {the G\^ateaux derivative of order $n$}%
   {Gateaux derivative of Order n}%
\Index%396%G%Gateaux derivative of second order
   {the G\^ateaux derivative of second order}%
   {Gateaux derivative of Second Order}%
\Index%46%G%Gateaux Dstar derivative of map f of division ring D
   {the G\^ateaux \Ds derivative of map $f$ of division ring $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%453%G%Gateaux mixed partial derivative
   {the G\^ateaux mixed partial derivative}%
   {Gateaux partial derivative of Second Order}%
\Index%511%G%Gateaux partial dcr derivative of map f^b with respect to variable x^a
   {the G\^ateaux partial \dcr derivative of map $f^{\gi b}$ with respect to variable $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%512%G%Gateaux partial derivative
   {the G\^ateaux partial derivative}%
   {Gateaux partial derivative}%
\Index%510%G%Gateaux partial rcd derivative of map fb with respect to variable xa
   {the G\^ateaux partial \rcd derivative of map $f^{\gi b}$ with respect to variable $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\Index%13%G%Gateaux rcd derivative of map f of D-vector space V to D-vector space W
   {the G\^ateaux \rcd derivative of map $f$ of $D$\hyph vector space $V$ to $D$\hyph vector space $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%76%G%Gateaux starD derivative of map f of division ring D
   {the G\^ateaux \sD derivative of map $f$ of division ring $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%332%G%generating set
   {generating set}%
   {generating set}%
\Index%289%G%generator of linear map
   {generator of linear map}%
   {generator of linear map}%
\Index%871%G%geodetic effect
   {geodetic effect}%
   {geodetic effect}%
\Index%700%G%geometric object
   {geometric object}%
   {geometric object}%
\Index%146%G%group algebra
   {group algebra}%
   {group algebra}%
\Index%568%G%group of automorphisms of representation
   {group of automorphisms of representation}%
   {group of automorphisms of representation}%
\SetIndexSpace%
\Index%292%H%Hadamard inverse of matrix
   {Hadamard inverse of matrix}%
   {Hadamard inverse of matrix}%
\Index%783%H%Hamel basis
   {Hamel basis}%
   {Hamel basis}%
\Index%546%H%hermitian conjugated vector
   {hermitian conjugated vector}%
   {hermitian conjugated vector}%
\Index%541%H%hermitian conjugation in division ring
   {hermitian conjugation in division ring}%
   {hermitian conjugation, division ring}%
\Index%747%H%hermitian matrix
   {hermitian matrix}%
   {hermitian matrix}%
\Index%544%H%hermitian metric on division ring
   {hermitian metric on division ring}%
   {hermitian metric on division ring}%
\Index%350%H%hermitian scalar product in D- vector space
   {hermitian scalar product in $D$\Hyph vector space}%
   {hermitian scalar product, vector space}%
\Index%545%H%hermitian scalar product on division ring
   {hermitian scalar product on division ring}%
   {hermitian scalar product on division ring}%
\Index%207%H%highest common factor
   {highest common factor}%
   {highest common factor}%
\Index%885%H%holomorphic map
   {holomorphic map}%
   {holomorphic map}%
\Index%138%H%holonomic coordinates of connection
   {holonomic coordinates of connection}%
   {holonomic coordinates of connection}%
\Index%137%H%holonomic coordinates of vector
   {holonomic coordinates of vector}%
   {vector holonomic coordinates}%
\Index%296%H%homogeneous bundle of fibered group
   {homogeneous bundle of fibered group}%
   {homogeneous bundle of fibered group}%
\Index%631%H%homogeneous linear geometric object
   {homogeneous linear geometric object}%
   {homogeneous linear geometric object}%
\Index%294%H%homogeneous map of degree k over field F
   {homogeneous map of degree $k$ over field $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%689%H%homogeneous polynomial
   {homogeneous polynomial}%
   {homogeneous polynomial}%
\Index%295%H%homogeneous space
   {homogeneous space}%
   {homogeneous space}%
\Index%861%H%homomorphic image
   {homomorphic image}%
   {homomorphic image}%
\Index%854%H%homomorphism
   {homomorphism}%
   {homomorphism}%
\Index%140%H%homomorphism of fibered groups
   {homomorphism of fibered groups}%
   {homomorphism of fibered groups}%
\Index%139%H%homomorphism of fibered universal algebras
   {homomorphism of fibered universal algebras}%
   {homomorphism of fibered universal algebras}%
\Index%959%H%homomorphism of vector space
   {homomorphism of vector space}%
   {homomorphism of vector space}%
\Index%73%H%horizontal component of vector
   {horizontal component of vector}%
   {horizontal component of vector}%
\Index%686%H%horizontal subspace
   {horizontal subspace}%
   {horizontal subspace}%
\Index%765%H%horizontal vector
   {horizontal vector}%
   {horizontal vector}%
\Index%838%H%hyperbolic cosine
   {hyperbolic cosine}%
   {hyperbolic cosine}%
\Index%837%H%hyperbolic sine
   {hyperbolic sine}%
   {hyperbolic sine}%
\SetIndexSpace%
\Index%459%I%ideal of algebra
   {ideal of algebra}%
   {ideal of algebra}%
\Index%970%I%image of map
   {image of map}%
   {image of map}%
\Index%834%I%indefinite integral
   {indefinite integral}%
   {indefinite integral}%
\Index%29%I%independent points
   {independent points}%
   {independent points}%
\Index%385%I%induction over diagram of representations
   {induction over diagram of representations}%
   {induction over diagram of representations}%
\Index%121%I%infinitesimal generator of representation
   {infinitesimal generator of representation}%
   {infinitesimal generator}%
\Index%174%I%infinitesimal generators of group Lie
   {infinitesimal generators of group Lie}%
   {infinitesimal generators of group Lie}%
\Index%918%I%integrable differential equation
   {integrable differential equation}%
   {integrable differential equation}%
\Index%438%I%integrable differential form
   {integrable differential form}%
   {integrable differential form}%
\Index%111%I%integrable form
   {integrable form}%
   {integrable form}%
\Index%693%I%integrable map
   {integrable map}%
   {integrable map}%
\Index%257%I%integral of differential 1 form along path
   {integral of differential $1$\Hyph form along path}%
   {integral of differential 1 form along path}%
\Index%710%I%invariance principle in tower of representations of universal algebras
   {invariance principle in tower of representations of universal algebras}%
   {invariance principle, tower of representations g}%
\Index%291%I%inverse fibered correspondence
   {inverse fibered correspondence}%
   {inverse fibered correspondence}%
\Index%290%I%inverse reduced fibered correspondence
   {inverse reduced fibered correspondence}%
   {inverse reduced fibered correspondence}%
\Index%745%I%involution in quaternion algebra
   {involution in quaternion algebra}%
   {involution, quaternion algebra}%
\Index%855%I%isomorphism
   {isomorphism}%
   {isomorphism}%
\Index%173%I%isomorphism of fibered Omega- algebras
   {isomorphism of fibered $\Omega$\Hyph algebras}%
   {isomorphism of fibered Omega-algebras}%
\Index%266%I%isomorphism of repesentations of Omega- algebra
   {isomorphism of repesentations of $\Omega$\Hyph algebra}%
   {isomorphism of repesentations of Omega algebra}%
\Index%31%I%isomorphism of vector spaces
   {isomorphism of vector spaces}%
   {isomorphism of vector spaces}%
\Index%648%I%isotropic vector
   {isotropic vector}%
   {isotropic vector}%
\Index%680%I%Lebesgue integral
   {Lebesgue integral}%
   {Lebesgue integral}%
\SetIndexSpace%
\Index%596%J%j i $RCcirc quasideterminant
   {$(^j_i)$\hyph $\RCcirc$\Hyph quasideterminant}%
   {j i RCcirc-quasideterminant}%
\Index%890%J%Jacobi matrix of map
   {the Jacobi matrix of map}%
   {Jacobi matrix of map}%
\Index%592%J%Jacobian complete system of differential equations
   {Jacobian complete system of differential equations}%
   {Jacobian complete system of differential equations}%
\Index%593%J%Jacobian complete system of drc differential equations
   {Jacobian complete system of \drv differential equations}%
   {Jacobian complete system of drc differential equations}%
\Index%678%J%ji- quasideterminant
   {$(ji)$\hyph quasideterminant}%
   {j i quasideterminant}%
\Index%527%J%the Jacobi Gateaux matrix of map
   {the Jacobi\Hyph G\^ateaux matrix of map}%
   {Jacobi Gateaux matrix of map}%
\SetIndexSpace%
\Index%971%K%kernel of group-homomorphism
   {kernel of group\Hyph homomorphism}%
   {ker group-homomorphism}%
\Index%874%K%kernel of homomorphism
   {kernel of homomorphism}%
   {kernel of homomorphism}%
\Index%524%K%kernel of inefficiency of G* representation of group G
   {kernel of inefficiency of \Ts{G}representation}%
   {kernel of inefficiency of G* representation}%
\Index%526%K%kernel of inefficiency of representation of fibered group
   {kernel of inefficiency of representation of fibered group}%
   {kernel of inefficiency of representation of fibered group}%
\Index%525%K%kernel of inefficiency of representation of group
   {kernel of inefficiency of representation of group}%
   {kernel of inefficiency of representation of group}%
\Index%522%K%kernel of linear map
   {kernel of linear map}%
   {kernel of linear map}%
\Index%930%K%kernel of map
   {kernel of map}%
   {kernel of map}%
\Index%493%K%Killing equation
   {Killing equation}%
   {Killing equation}%
\Index%494%K%Killing equation of second type
   {Killing equation of second type}%
   {Killing equation second type}%
\Index%123%K%Killing vector of second type
   {Killing vector of second type}%
   {Killing vector second type}%
\Index%445%K%Kronecker symbol
   {Kronecker symbol}%
   {Kronecker symbol}%
\SetIndexSpace%
\Index%501%L%latitude
   {latitude}%
   {latitude}%
\Index%822%L%leading coefficient of polynomial
   {leading coefficient of polynomial}%
   {leading coefficient of polynomial}%
\Index%166%L%Lebesgue extension of measure
   {Lebesgue extension of measure}%
   {Lebesgue extension of measure}%
\Index%164%L%Lebesgue measurable set
   {Lebesgue measurable set}%
   {Lebesgue measurable}%
\Index%165%L%Lebesgue measure
   {Lebesgue measure}%
   {Lebesgue measure}%
\Index%895%L%left A module
   {left $A$\Hyph module}%
   {left A module}%
\Index%896%L%left A vector space
   {left $A$\Hyph vector space}%
   {left A vector space}%
\Index%952%L%left A-column space
   {left $A$\Hyph column space}%
   {left A-column space}%
\Index%955%L%left A-row space
   {left $A$\Hyph row space}%
   {left A-row space}%
\Index%754%L%left cofactor of entry of matrix
   {left cofactor of entry of matrix}%
   {left cofactor, matrix}%
\Index%973%L%left coset
   {left coset}%
   {left coset}%
\Index%585%L%left D vector space of columns
   {left $D$\hyph vector space of columns}%
   {left vector space of columns}%
\Index%576%L%left D vector space of rows
   {left $D$\hyph vector space of rows}%
   {left vector space of rows}%
\Index%301%L%left defined Lie algebra of Lie group
   {left defined Lie algebra of Lie group}%
   {left defined Lie algebra}%
\Index%756%L%left double cofactor of entry of matrix
   {left double cofactor of entry of matrix}%
   {left double cofactor}%
\Index%158%L%left fraction
   {left fraction}%
   {left fraction}%
\Index%681%L%left ideal of algebra
   {left ideal of algebra}%
   {left ideal of algebra}%
\Index%229%L%left invariant vector field
   {left invariant vector field}%
   {left invariant vector}%
\Index%950%L%left linear combination
   {left linear combination}%
   {left linear combination}%
\Index%136%L%left linear dependent
   {left linear dependent}%
   {left linear dependent}%
\Index%237%L%left module
   {left module}%
   {left module}%
\Index%513%L%left principal ideal
   {left principal ideal}%
   {left principal ideal}%
\Index%731%L%left shift of module
   {left shift of module}%
   {left shift of module}%
\Index%240%L%left shift on fibered group
   {left shift on fibered group}%
   {left shift, fibered group}%
\Index%238%L%left shift on group
   {left shift on group}%
   {left shift}%
\Index%239%L%left shift on group
   {left shift on group}%
   {left shift, group}%
\Index%236%L%left structural constant of Lie algebra
   {left structural constant of Lie algebra}%
   {left structural constant of Lie algebra}%
\Index%228%L%left vector space
   {left vector space}%
   {left vector space}%
\Index%812%L%left zero divisor
   {left zero divisor}%
   {left zero divisor}%
\Index%751%L%left-ordered cycle notation of permutation
   {left-ordered cycle notation of permutation}%
   {left-ordered cycle notation of permutation}%
\Index%899%L%left-side A representation
   {left\Hyph side $A_1$\Hyph representation}%
   {left-side A representation}%
\Index%892%L%left-side product
   {left\Hyph side product}%
   {left-side product}%
\Index%271%L%left-side product of map over scalar
   {left-side product of map over scalar}%
   {left-side product of map over scalar}%
\Index%665%L%left-side product of vector over scalar
   {left\Hyph side product of vector over scalar}%
   {left-side product of vector over scalar}%
\Index%184%L%left-side representation
   {left-side representation}%
   {left-side representation}%
\Index%233%L%left-side representation of fibered Omega- algebra
   {left-side representation of fibered $\Omega$\Hyph algebra}%
   {left-side representation of fibered Omega-algebra}%
\Index%232%L%left-side representation of Omega1 algebra A in Omega2 algebra M
   {left-side representation of $\Omega_1$\Hyph algebra $A$ in $\Omega_2$\Hyph algebra $M$}%
   {left-side representation of algebra}%
\Index%234%L%left-side transformation
   {left-side transformation}%
   {left-side transformation}%
\Index%235%L%left-side transformation on bundle
   {left-side transformation on bundle}%
   {left-side transformation of bundle}%
\Index%104%L%Lie algebra of Lie group
   {Lie algebra of Lie group}%
   {algebra Lie group Lie}%
\Index%402%L%Lie derivative
   {Lie derivative}%
   {Lie derivative}%
\Index%404%L%Lie derivative of connection
   {Lie derivative of connection}%
   {Lie derivative of connection}%
\Index%403%L%Lie derivative of metric
   {Lie derivative of metric}%
   {Lie derivative of metric}%
\Index%118%L%Lie group basic operators
   {Lie group basic operators}%
   {Lie group basic operators}%
\Index%246%L%lift of correspondence
   {lift of correspondence}%
   {lift of correspondence}%
\Index%245%L%lift of mapping
   {lift of mapping}%
   {lift of map}%
\Index%365%L%limit of correspondence with respect to the filter
   {limit of correspondence with respect to the filter}%
   {limit of correspondence with respect to the filter}%
\Index%366%L%limit of filter
   {limit of filter}%
   {limit of filter}%
\Index%467%L%limit of sequence
   {limit of sequence}%
   {limit of sequence}%
\Index%367%L%limit set of filter
   {limit set of filter}%
   {limit set of filter}%
\Index%88%L%linear combination
   {linear combination}%
   {linear combination}%
\Index%397%L%linear functional
   {linear functional}%
   {linear functional}%
\Index%37%L%linear G* representation
   {linear \Ts{G}representation}%
   {linear G* representation}%
\Index%630%L%linear geometric object
   {linear geometric object}%
   {linear geometric object}%
\Index%921%L%linear homogeneous equation
   {linear homogeneous equation}%
   {linear homogeneous equation}%
\Index%769%L%linear homomorphism
   {linear homomorphism}%
   {linear homomorphism}%
\Index%35%L%linear map
   {linear map}%
   {linear map}%
\Index%98%L%linear map generated by map
   {linear map generated by map}%
   {linear map generated by map}%
\Index%97%L%linear map of division ring
   {linear map of division ring}%
   {linear map of division ring}%
\Index%244%L%linear representation of group
   {linear representation of group}%
   {linear representation of group}%
\Index%608%L%linear representation of Lie group
   {linear representation of Lie group}%
   {linear representation of Lie group}%
\Index%32%L%linear span
   {linear span}%
   {linear span, vector space}%
\Index%613%L%linear transformation group
   {linear transformation group}%
   {linear transformation group}%
\Index%735%L%linear transformation of affine space
   {linear transformation of affine space}%
   {linear transformation, affine space}%
\Index%833%L%linearly dependent
   {linearly dependent}%
   {linearly dependent}%
\Index%21%L%linearly dependent set
   {linearly dependent set}%
   {linearly dependent set}%
\Index%20%L%linearly dependent vector fields
   {linearly dependent vector fields}%
   {linearly dependent vector fields}%
\Index%34%L%linearly independent set
   {linearly independent set}%
   {linearly independent set}%
\Index%250%L%little group
   {little group}%
   {little group}%
\Index%247%L%local reference frame
   {local reference frame}%
   {local reference frame}%
\Index%248%L%locally compact at point p space
   {locally compact at point $p$ space}%
   {locally compact at point space}%
\Index%249%L%locally compact space
   {locally compact space}%
   {locally compact space}%
\Index%78%L%longitude
   {longitude}%
   {longitude}%
\Index%373%L%Lorentz transformation
   {Lorentz transformation}%
   {Lorentz transformation}%
\SetIndexSpace%
\Index%56%M%m- dimensional parallelepiped
   {$m$\Hyph dimensional parallelepiped}%
   {m dimensional parallelepiped}%
\Index%57%M%m- vector
   {$m$\Hyph vector}%
   {m-vector}%
\Index%61%M%major submatrix
   {major submatrix}%
   {major submatrix}%
\Index%556%M%manifold with D- affine connections
   {manifold with $D$\Hyph affine connections}%
   {manifold with D- affine connections}%
\Index%506%M%map continuous with respect to set of arguments
   {map continuous with respect to set of arguments}%
   {map continuous with respect to set of arguments}%
\Index%505%M%map differentiable in Gateaux sense
   {map differentiable in the G\^ateaux sense}%
   {map differentiable in Gateaux sense}%
\Index%886%M%map is compatible with operation
   {map is compatible with operation}%
   {map is compatible with operation}%
\Index%876%M%map of conjugation
   {map of conjugation}%
   {map of conjugation}%
\Index%502%M%map of n D- valued variables
   {map of $\gi n$ $D$\Hyph valued variables}%
   {map of n D valued variables}%
\Index%316%M%map of type G on manifold
   {map of type $G$ on manifold}%
   {map of type G on manifold}%
\Index%572%M%map polylinear over finite dimensional algebras
   {map polylinear over finite dimensional algebras}%
   {map polylinear over finite dimensional algebras}%
\Index%677%M%map projective over commutative ring
   {map projective over commutative ring}%
   {map projective over commutative ring}%
\Index%312%M%mapping of rings polylinear over commutative ring
   {mapping of rings polylinear over commutative ring}%
   {map polylinear over commutative ring, ring}%
\Index%407%M%mapping space
   {mapping space}%
   {mapping space}%
\Index%894%M%matrix
   {matrix}%
   {matrix}%
\Index%772%M%matrix of antilinear homomorphism
   {matrix of antilinear homomorphism}%
   {matrix of antilinear homomorphism}%
\Index%252%M%matrix of bilinear function
   {matrix of bilinear function}%
   {matrix of bilinear function}%
\Index%595%M%matrix of endomorphisms of Omega algebra
   {matrix of endomorphisms of $\Omega$\Hyph algebra}%
   {matrix of endomorphisms of Omega algebra}%
\Index%253%M%matrix of fibered Drc linear map
   {matrix of fibered \Drc linear map}%
   {matrix of fibered drc linear map}%
\Index%958%M%matrix of homomorphism
   {matrix of homomorphism}%
   {matrix of homomorphism}%
\Index%770%M%matrix of linear homomorphism
   {matrix of linear homomorphism}%
   {matrix of linear homomorphism}%
\Index%194%M%matrix of linear map
   {matrix of linear map}%
   {matrix of linear map}%
\Index%591%M%matrix of linear maps
   {matrix of linear maps}%
   {matrix of linear maps}%
\Index%588%M%matrix of maps
   {matrix of maps}%
   {matrix of maps}%
\Index%552%M%matrix of quadratic map
   {matrix of quadratic map}%
   {matrix of quadratic map, division ring}%
\Index%926%M%Maxwell equation
   {Maxwell equation}%
   {Maxwell equation}%
\Index%800%M%measurable map
   {measurable map}%
   {measurable map}%
\Index%161%M%measure
   {measure}%
   {measure}%
\Index%835%M%method of successive differentiation
   {method of successive differentiation}%
   {method of successive differentiation}%
\Index%96%M%metric tensor in Minkowski space
   {metric tensor in Minkowski space}%
   {metric tensor, Minkowski space}%
\Index%254%M%metric-affine manifold
   {metric-affine manifold}%
   {metric-affine manifold}%
\Index%635%M%Minkowski space
   {Minkowski space}%
   {Minkowski space, Finsler}%
\Index%642%M%minor matrix
   {minor matrix}%
   {minor matrix}%
\Index%611%M%module over ring
   {module over ring}%
   {module over ring}%
\Index%766%M%monomial of power
   {monomial of power $k$}%
   {monomial of power}%
\Index%856%M%monomorphism
   {monomorphism}%
   {monomorphism}%
\Index%698%M%morphism from diagram of representations into diagram of representations
   {morphism from diagram of representations into diagram of representations}%
   {morphism from diagram of representations into diagram of representations}%
\Index%265%M%morphism from tower of representations into tower of representations
   {morphism from tower of representations into tower of representations}%
   {morphism from tower of representations into tower of representations}%
\Index%269%M%morphism of fibered Tstar- representations from F into G
   {morphism of fibered \Ts representations from $\Bundle F$ into $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%732%M%morphism of representation f
   {morphism of representation $f$}%
   {morphism of representation f}%
\Index%268%M%morphism of representations from f into g
   {morphism of representations from $f$ into $g$}%
   {morphism of representations from f into g}%
\Index%267%M%morphism of representations of Omega1 algebra in Omega2 algebra
   {morphism of representations of $\Omega_1$\Hyph algebra in $\Omega_2$\Hyph algebra}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%264%M%morphism of Tstar- representations of fibered Omega- algebra
   {morphism of \Ts representations of fibered $\Omega$\Hyph algebra}%
   {morphism of representations of fibered Omega algebra}%
\Index%586%M%motion of Minkowski space
   {motion of Minkowski space}%
   {motion, Minkowski space}%
\Index%147%M%movement on basis manifold
   {movement on basis manifold}%
   {movement transformation}%
\Index%829%M%multiplicative map
   {multiplicative map}%
   {multiplicative map}%
\Index%828%M%multiplicative Omega group
   {multiplicative $\Omega$\Hyph group}%
   {multiplicative Omega group}%
\SetIndexSpace%
\Index%58%N%n- ary fibered relation
   {$n$\Hyph ary fibered relation}%
   {fibered relation}%
\Index%845%N%n-ary operation on set
   {$n$\Hyph ary operation on set}%
   {n-ary operation on set}%
\Index%875%N%natural homomorphism
   {natural homomorphism}%
   {natural homomorphism}%
\Index%870%N%neutral element of operation
   {neutral element of operation}%
   {neutral element of operation}%
\Index%279%N%nonmetricity
   {nonmetricity}%
   {nonmetricity}%
\Index%272%N%nonsingular bilinear function
   {nonsingular bilinear function}%
   {nonsingular bilinear function}%
\Index%273%N%nonsingular system of linear equations
   {nonsingular system of linear equations}%
   {nonsingular system of linear equations}%
\Index%219%N%nonsingular system of right AU* linear equations
   {nonsingular system of right $A^*$\Hyph linear equations}%
   {nonsingular system of right AU* linear equations}%
\Index%643%N%nonsingular tensor
   {nonsingular tensor}%
   {nonsingular tensor}%
\Index%274%N%nonsingular transformation
   {nonsingular transformation}%
   {nonsingular transformation}%
\Index%742%N%norm in quaternion algebra
   {norm in quaternion algebra}%
   {norm, quaternion algebra}%
\Index%196%N%norm of functional
   {norm of functional}%
   {norm of functional}%
\Index%314%N%norm of map
   {norm of map}%
   {norm of map}%
\Index%928%N%norm of octonion
   {norm of octonion}%
   {norm of octonion}%
\Index%657%N%norm of operation
   {norm of operation}%
   {norm of operation}%
\Index%285%N%norm of polylinear map
   {norm of polylinear map}%
   {norm of polymap}%
\Index%801%N%norm of representation
   {norm of representation}%
   {norm of representation}%
\Index%346%N%norm on D- algebra
   {norm on $D$\Hyph algebra}%
   {norm on D algebra}%
\Index%283%N%norm on D- vector space
   {norm on $D$\Hyph vector space}%
   {norm on D vector space}%
\Index%460%N%norm on D-module
   {norm on $D$\Hyph module}%
   {norm on D module}%
\Index%675%N%norm on Omega group
   {norm on $\Omega$\Hyph group}%
   {norm on Omega group}%
\Index%641%N%norm on ring
   {norm on ring}%
   {norm on ring}%
\Index%692%N%normal basis
   {normal basis}%
   {normal basis}%
\Index%702%N%normal subgroup
   {normal subgroup}%
   {normal subgroup}%
\Index%343%N%normed D-algebra
   {normed $D$\Hyph algebra}%
   {normed D algebra}%
\Index%364%N%normed D-module
   {normed $D$\Hyph module}%
   {normed D module}%
\Index%287%N%normed D-vector space
   {normed $D$\Hyph vector space}%
   {normed D vector space}%
\Index%792%N%normed Omega group
   {normed $\Omega$\Hyph group}%
   {normed Omega group}%
\Index%640%N%normed ring
   {normed ring}%
   {normed ring}%
\Index%632%N%not complete group
   {not complete group}%
   {not complete group}%
\Index%649%N%not complete Omega algebra
   {not complete $\Omega$\Hyph algebra}%
   {not complete Omega algebra}%
\Index%619%N%nucleus of algebra
   {nucleus of $D$\Hyph algebra $A$}%
   {nucleus of algebra}%
\SetIndexSpace%
\Index%639%O%octonion algebra
   {octonion algebra}%
   {octonion algebra}%
\Index%793%O%open ball
   {open ball}%
   {open ball}%
\Index%85%O%open set
   {open set}%
   {open set}%
\Index%300%O%operation on bundle
   {operation on bundle}%
   {operation on bundle}%
\Index%844%O%operation on set
   {operation on set}%
   {operation on set}%
\Index%848%O%operator domain
   {operator domain}%
   {operator domain}%
\Index%623%O%opposite algebra to algebra
   {opposite algebra to algebra $P$}%
   {opposite algebra}%
\Index%408%O%opposite fibered preordering
   {opposite fibered preordering}%
   {opposite fibered preordering}%
\Index%624%O%orbit of linear map
   {orbit of linear map}%
   {orbit of linear map}%
\Index%893%O%orbit of representation
   {orbit of representation}%
   {orbit of representation}%
\Index%306%O%orbit of representation of fibered group
   {orbit of representation of fibered group}%
   {orbit of representation of fibered group}%
\Index%305%O%orbit of representation of group
   {orbit of representation of group}%
   {orbit of representation of group}%
\Index%729%O%origin of coordinate system of affine space
   {origin of coordinate system of affine space}%
   {origin of coordinate system of affine space}%
\Index%637%O%orthogonal basis in Minkowski space
   {orthogonal basis in Minkowski space}%
   {orthogonal basis, Minkowski space}%
\Index%636%O%orthogonality in Minkowski space
   {orthogonality in Minkowski space}%
   {Minkowski orthogonality}%
\Index%308%O%orthonormal basis
   {orthonormal basis}%
   {Orthonormal Basis, division ring}%
\Index%638%O%orthonormal basis in Minkowski space
   {orthonormal basis in Minkowski space}%
   {orthonormal basis, Minkowski space}%
\Index%307%O%orthonornal basis
   {orthonornal basis}%
   {Orthonornal Basis}%
\Index%163%O%outer measure
   {outer measure}%
   {outer measure}%
\SetIndexSpace%
\Index%739%P%parallel shift of affine space
   {parallel shift of affine space}%
   {parallel shift, affine space}%
\Index%317%P%parallelogram
   {parallelogram}%
   {parallelogram}%
\Index%905%P%parity of permutation
   {parity of permutation}%
   {parity of permutation}%
\Index%888%P%partial derivative
   {partial derivative}%
   {partial derivative}%
\Index%889%P%partial derivative of second order
   {partial derivative of second order}%
   {partial derivative of second order}%
\Index%475%P%partial linear map
   {partial linear map}%
   {partial linear map}%
\Index%321%P%passive G-representation
   {passive $G$\Hyph representation}%
   {passive G representation}%
\Index%333%P%passive representation
   {passive representation}%
   {passive representation}%
\Index%695%P%passive representation in basis manifold
   {passive representation in basis manifold}%
   {passive representation in basis manifold}%
\Index%718%P%passive representation of group in basis manifold of tower of representations
   {passive representation of group $G(\Vector f)$ in basis manifold of tower of representations}%
   {passive representation in basis manifold, tower of representations}%
\Index%336%P%passive transformation of basis manifold
   {passive transformation of basis manifold}%
   {passive transformation, vector space}%
\Index%570%P%passive transformation of the basis manifold
   {passive transformation of basis manifold}%
   {passive transformation of basis}%
\Index%717%P%passive transformation of the basis manifold of tower of representations
   {passive transformation of the basis manifold of tower of representations}%
   {passive transformation of basis, tower of representations}%
\Index%335%P%passive transformation on basis manifold
   {passive transformation on basis manifold}%
   {passive transformation}%
\Index%744%P%permutability property of trace
   {permutability property of trace}%
   {permutability property of trace}%
\Index%863%P%permutation
   {permutation}%
   {permutation}%
\Index%416%P%pfaffian derivative
   {pfaffian derivative}%
   {pfaffian derivative}%
\Index%806%P%polyadditive map
   {polyadditive map}%
   {polyadditive map}%
\Index%609%P%polylinear map
   {polylinear map}%
   {polylinear map}%
\Index%345%P%polylinear skew symmetric map
   {polylinear skew symmetric map}%
   {polylinear map skew symmetric}%
\Index%347%P%polylinear symmetric map
   {polylinear symmetric map}%
   {polylinear map symmetric}%
\Index%760%P%polymorphism of representations
   {polymorphism of representations}%
   {polymorphism of representations}%
\Index%804%P%polynomial
   {polynomial}%
   {polynomial}%
\Index%344%P%polyvector
   {polyvector}%
   {polyvector}%
\Index%352%P%potential energy
   {potential energy}%
   {potential energy}%
\Index%171%P%power of measure
   {power of measure}%
   {power of measure}%
\Index%483%P%prime A number
   {prime $A$\Hyph number}%
   {prime A number}%
\Index%767%P%principal ideal
   {principal ideal}%
   {principal ideal}%
\Index%384%P%principle of covariance
   {principle of covariance}%
   {principle of covariance}%
\Index%395%P%product in category
   {product in category}%
   {product in category}%
\Index%388%P%product of geometric object and constant
   {product of geometric object and constant}%
   {product of geometric object and constant}%
\Index%389%P%product of geometric object and constant in vector space
   {product of geometric object and constant in vector space}%
   {product of geometric object and constant, vector space}%
\Index%133%P%product of homomorphisms
   {product of homomorphisms}%
   {product of homomorphisms}%
\Index%172%P%product of measures
   {product of measures}%
   {product of measures}%
\Index%937%P%product of morphisms of diagram of representations
   {product of morphisms of diagram of representations}%
   {product of morphisms of diagram of representations}%
\Index%391%P%product of morphisms of representations of universal algebra
   {product of morphisms of representations of universal algebra}%
   {product of morphisms of representations of universal algebra}%
\Index%561%P%product of morphisms of tower of representations
   {product of morphisms of tower of representations}%
   {product of morphisms of tower of representations}%
\Index%392%P%product of morphisms of Tstar- representations of fibered Omega- algebra
   {product of morphisms of \Ts representations of fibered $\Omega$\Hyph algebra}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%666%P%product of polynomials
   {product of polynomials}%
   {product of polynomials}%
\Index%663%P%product of rings of sets
   {product of rings of sets}%
   {product of rings of sets}%
\Index%387%P%projection of bundle E along fiber E
   {projection of bundle $\Bundle E$ along fiber $E$}%
   {projection of bundle along fiber}%
\Index%195%P%projective map is continuous in direction over field
   {projective map is continuous in direction over field}%
   {projective map is continuous in direction over field}%
\Index%540%P%pseudo-Euclidean metric on division ring
   {pseudo\Hyph Euclidean metric on division ring}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%P%pseudo-Euclidean scalar product in D- vector space
   {pseudo\Hyph Euclidean scalar product in $D$\Hyph vector space}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%P%pseudo-Euclidean scalar product on division ring
   {pseudo-Euclidean scalar product on division ring}%
   {pseudo-Euclidean scalar product on division ring}%
\SetIndexSpace%
\Index%842%Q%quadratic equation
   {quadratic equation}%
   {quadratic equation}%
\Index%555%Q%quadratic form in division ring
   {quadratic form in division ring}%
   {quadratic form, division ring}%
\Index%551%Q%quadratic map of division ring
   {quadratic map of division ring}%
   {Quadratic Map of Division Ring}%
\Index%180%Q%quasi affine transformation on basis manifold
   {quasi affine transformation on basis manifold}%
   {quasi affine transformation}%
\Index%181%Q%quasi affine transformation on basis manifold
   {quasi affine transformation on basis manifold}%
   {quasi affine drc transformation}%
\Index%182%Q%quasi movement on basis manifold
   {quasi movement on basis manifold}%
   {quasi movement, division ring}%
\Index%183%Q%quasi movement on basis manifold
   {quasi movement on basis manifold}%
   {quasi movement}%
\Index%535%Q%quasibasis
   {quasibasis}%
   {quasibasis}%
\Index%604%Q%quasiclosed ring of maps
   {quasiclosed ring of maps}%
   {quasiclosed ring of maps}%
\Index%679%Q%quasideterminant
   {quasideterminant}%
   {quasideterminant definition}%
\Index%962%Q%quasiexponent
   {quasiexponent}%
   {quasiexponent}%
\Index%75%Q%quasimotion of Minkowski space
   {quasimotion of Minkowski space}%
   {Quasimotion, Minkowski space}%
\Index%741%Q%quaternion algebra
   {quaternion algebra}%
   {quaternion algebra}%
\Index%103%Q%quaternion algebra E over the field F
   {quaternion algebra $E$ over the field $F$}%
   {quaternion algebra over the field}%
\Index%827%Q%quotient
   {quotient}%
   {quotient divided by}%
\Index%496%Q%quotient bundle
   {quotient bundle}%
   {quotient bundle}%
\SetIndexSpace%
\Index%4%R%j i-RC quasideterminant
   {$(\aUD{}ji)$\hyph \RC quasideterminant}%
   {j i rc-quasideterminant}%
\Index%59%R%r row of matrix
   {\sups row of matrix}%
   {r row}%
\Index%728%R%R- module
   {$R$\Hyph module}%
   {R- module}%
\Index%72%R%r-row of matrix
   {$r$\hyph row of matrix}%
   {r-row}%
\Index%749%R%rank of Hermitian matrix by principal minors
   {rank of Hermitian matrix by principal minors}%
   {rank of Hermitian matrix by principal minors}%
\Index%67%R%rank of matrix
   {rank of matrix}%
   {rank of matrix}%
\Index%554%R%rank of quadratic map of division ring
   {rank of quadratic map of division ring}%
   {rank of quadratic map, division ring}%
\Index%948%R%RC exponent
   {\RC exponent}%
   {RC exponent}%
\Index%65%R%RC inverse element of biring
   {\RC inverse element of biring}%
   {rc-inverse element}%
\Index%63%R%RC matrix group
   {\RC matrix group}%
   {rc-matrix group}%
\Index%64%R%rc nonsingular matrix
   {\RC nonsingular matrix}%
   {r? nonsingular matrix}%
\Index%68%R%RC power
   {\RC power}%
   {rc power}%
\Index%66%R%RC product
   {\RC product (product of row over column)}%
   {rc-product}%
\Index%590%R%rc product of matrices of maps
   {$\RCcirc$\Hyph product of matrices of maps}%
   {rc product of matrices of maps}%
\Index%62%R%rc quasideterminant
   {\RC quasideterminant}%
   {rc-quasideterminant}%
\Index%60%R%rc singular matrix
   {\RC singular matrix}%
   {rc singular matrix}%
\Index%218%R%rc-inverse matrix
   {\RC inverse matrix}%
   {rc-inverse matrix}%
\Index%601%R%RCcirc nonsingular matrix
   {$\RCcirc$\Hyph nonsingular matrix}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc nonsingular system of additive equations
   {$\RCcirc$\Hyph nonsingular system of additive equations}%
   {RCcirc nonsingular system of additive equations}%
\Index%597%R%RCcirc quasideterminant
   {$\RCcirc$\Hyph quasideterminant}%
   {RCcirc-quasideterminant definition}%
\Index%600%R%RCcirc singular matrix
   {$\RCcirc$\Hyph singular matrix}%
   {RCcirc singular matrix}%
\Index%759%R%rcd affine plane
   {\rcd affine plane}%
   {rcd affine plane}%
\Index%736%R%rcd affine space
   {\rcd affine space}%
   {rcd affine space}%
\Index%27%R%rcd vector
   {\rcd vector}%
   {rcd vector}%
\Index%69%R%rcd vector space
   {\rcd vector space}%
   {rcd vector space}%
\Index%377%R%reduced Cartesian product of bundles
   {reduced Cartesian product of bundles}%
   {reduced Cartesian product of bundles}%
\Index%378%R%reduced Cartesian product of total spaces
   {reduced Cartesian product of total spaces}%
   {reduced Cartesian product of total spaces}%
\Index%379%R%reduced fibered correspondence from A to B
   {reduced fibered correspondence from $\Bundle{A}$ to $\Bundle B$}%
   {reduced fibered correspondence from A to B}%
\Index%380%R%reduced fibered correspondence in A
   {reduced fibered correspondence in $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%831%R%reduced morphism of representations
   {reduced morphism of representations}%
   {reduced morphism of representations}%
\Index%761%R%reduced polymorphism of representations
   {reduced polymorphism of representations}%
   {reduced polymorphism of representations}%
\Index%843%R%reduced quadratic equation
   {reduced quadratic equation}%
   {reduced quadratic equation}%
\Index%381%R%reducible biring
   {reducible biring}%
   {reducible biring}%
\Index%450%R%reference frame in event space
   {reference frame in event space}%
   {reference frame in event space}%
\Index%263%R%reference frame manifold
   {reference frame manifold}%
   {reference frame manifold}%
\Index%439%R%reflexive 2- ary fibered relation
   {reflexive $2$\Hyph ary fibered relation}%
   {reflexive 2 ary fibered relation}%
\Index%932%R%reflexive correspondence
   {reflexive correspondence}%
   {reflexive correspondence}%
\Index%330%R%regular endomorphism
   {regular endomorphism}%
   {regular endomorphism}%
\Index%566%R%regular endomorphism of tower of representations
   {regular endomorphism of tower of representations}%
   {regular endomorphism of tower of representations}%
\Index%553%R%regular quadratic map in division ring
   {regular quadratic map in division ring}%
   {regular quadratic map, division ring}%
\Index%481%R%relatively prime A numbers
   {relatively prime $A$\Hyph numbers}%
   {relatively prime A numbers}%
\Index%484%R%remainder of the division
   {remainder of the division}%
   {remainder of the division}%
\Index%117%R%representation conjugated to representation
   {representation conjugated to representation}%
   {representation conjugated to representation}%
\Index%90%R%representation in Omega2- algebra A*
   {\Ts{A}representation in $\Omega_2$\Hyph algebra}%
   {A* representation of algebra}%
\Index%372%R%representation of group
   {representation of group}%
   {representation of group}%
\Index%528%R%representation of Omega algebra in representation
   {representation of $\Omega$\Hyph algebra in representation}%
   {representation of Omega algebra in representation}%
\Index%529%R%representation of Omega algebra in tower of representations
   {representation of $\Omega$\Hyph algebra in tower of representations}%
   {representation of Omega algebra in tower of representations}%
\Index%370%R%representation of Omega- algebra A in category B
   {representation of $\Omega$\Hyph algebra $A$ in category $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%82%R%representation of Omega1 algebra A in Omega2 algebra *A
   {\sT{A}representation of $\Omega_1$\Hyph algebra $A$ in $\Omega_2$\Hyph algebra}%
   {*A representation of algebra}%
\Index%371%R%representation of Omega1 algebra A in Omega2 algebra M
   {representation of $\Omega_1$\Hyph algebra $A$ in $\Omega_2$\Hyph algebra $M$}%
   {representation of algebra}%
\Index%703%R%representative of geometric object
   {representative of geometric object}%
   {representative of geometric object}%
\Index%474%R%restriction of correspondence \Phi to set C
   {restriction of correspondence $\Phi$ to set $C$}%
   {restriction of correspondence}%
\Index%961%R%right A subs vector space
   {right $A_*$\Hyph vector space}%
   {right A subs vector space}%
\Index%898%R%right A vector space
   {right $A$\Hyph vector space}%
   {right A vector space}%
\Index%951%R%right A-column space
   {right $A$\Hyph column space}%
   {right A-column space}%
\Index%957%R%right A-row space
   {right $A$\Hyph row space}%
   {right A-row space}%
\Index%753%R%right cofactor of entry of matrix
   {right cofactor of entry of matrix}%
   {right cofactor, matrix}%
\Index%704%R%right coset
   {right coset}%
   {right coset}%
\Index%897%R%right D module
   {right $D$\Hyph module}%
   {right D module}%
\Index%671%R%right D vector space of columns
   {right $D$\hyph vector space of columns}%
   {right vector space of columns}%
\Index%654%R%right D vector space of rows
   {right $D$\hyph vector space of rows}%
   {right vector space of rows}%
\Index%302%R%right defined Lie algebra of Lie group
   {right defined Lie algebra of Lie group}%
   {right defined Lie algebra}%
\Index%757%R%right double cofactor of entry of matrix
   {right double cofactor of entry of matrix}%
   {right double cofactor}%
\Index%30%R%right fraction
   {right fraction}%
   {right fraction}%
\Index%42%R%right ideal of algebra
   {right ideal of algebra}%
   {right ideal of algebra}%
\Index%354%R%right invariant vector field
   {right invariant vector field}%
   {right invariant vector}%
\Index%953%R%right linear combination
   {right linear combination}%
   {right linear combination}%
\Index%361%R%right module
   {right module}%
   {right module}%
\Index%670%R%right module over D- algebra A
   {right module over $D$\Hyph algebra $A$}%
   {right module over algebra}%
\Index%242%R%right principal ideal
   {right principal ideal}%
   {right principal ideal}%
\Index%362%R%right shift on group
   {right shift on group}%
   {right shift}%
\Index%363%R%right shift on group
   {right shift on group}%
   {right shift, group}%
\Index%360%R%right structural constant of Lie algebra
   {right structural constant of Lie algebra}%
   {right structural constant of Lie algebra}%
\Index%353%R%right vector space
   {right vector space}%
   {right vector space}%
\Index%813%R%right zero divisor
   {right zero divisor}%
   {right zero divisor}%
\Index%752%R%right-ordered cycle notation of permutation
   {right-ordered cycle notation of permutation}%
   {right-ordered cycle notation of permutation}%
\Index%900%R%right-side A representation
   {right\Hyph side $A_1$\Hyph representation}%
   {right-side A representation}%
\Index%891%R%right-side product
   {right\Hyph side product}%
   {right-side product}%
\Index%674%R%right-side product of vector over scalar
   {right\Hyph side product of vector over scalar}%
   {right-side product of vector over scalar}%
\Index%355%R%right-side representation
   {right-side representation}%
   {right-side representation}%
\Index%358%R%right-side representation of fibered Omega- algebra
   {right-side representation of fibered $\Omega$\Hyph algebra}%
   {right-side representation of fibered Omega-algebra}%
\Index%357%R%right-side representation of Omega1 algebra A in Omega2 algebra M
   {right-side representation of $\Omega_1$\Hyph algebra $A$ in $\Omega_2$\Hyph algebra $M$}%
   {right-side representation of algebra}%
\Index%359%R%right-side transformation
   {right-side transformation}%
   {right-side transformation}%
\Index%188%R%ring has characteristic 0
   {ring has characteristic $0$}%
   {ring has characteristic 0}%
\Index%189%R%ring has characteristic p
   {ring has characteristic $p$}%
   {ring has characteristic p}%
\Index%794%R%ring of sets
   {ring of sets}%
   {ring of sets}%
\Index%577%R%ring of sets generated by semiring of sets
   {ring of sets generated by semiring of sets}%
   {ring of sets generated by semiring}%
\Index%778%R%ring with conjugation
   {ring with conjugation}%
   {ring with conjugation}%
\Index%634%R%root of polynomial
   {root of polynomial}%
   {root of polynomial}%
\Index%202%R%row *D vector
   {row $*D$\Hyph vector}%
   {row *D vector}%
\Index%93%R%row D* vector
   {row $D*$\Hyph vector}%
   {row D* vector}%
\Index%748%R%row determinant
   {row determinant}%
   {row determinant}%
\Index%127%R%row vector
   {row vector}%
   {row vector}%
\SetIndexSpace%
\Index%669%S%$starA- module
   {$\star A$\Hyph module}%
   {starA-module}%
\Index%786%S%scalar algebra of algebra
   {scalar algebra of algebra}%
   {scalar algebra of algebra}%
\Index%775%S%scalar algebra of ring
   {scalar algebra of ring}%
   {scalar algebra of ring}%
\Index%784%S%scalar of element of algebra
   {scalar of element of algebra}%
   {scalar of algebra}%
\Index%773%S%scalar of element of ring
   {scalar of element of ring}%
   {scalar of ring}%
\Index%451%S%scalar potential
   {scalar potential}%
   {scalar potential}%
\Index%791%S%Schauder basis
   {Schauder basis}%
   {Schauder basis}%
\Index%70%S%second axiom of countability
   {second axiom of countability}%
   {second axiom of countability}%
\Index%129%S%second Newton law
   {second Newton law}%
   {Second Newton law}%
\Index%694%S%section of bundle
   {section of bundle}%
   {section of bundle}%
\Index%868%S%semigroup
   {semigroup}%
   {semigroup}%
\Index%169%S%semiring of sets
   {semiring of sets}%
   {semiring of sets}%
\Index%816%S%sequence converges
   {sequence converges}%
   {sequence converges}%
\Index%578%S%sequence converges almost everywhere
   {sequence converges almost everywhere}%
   {converges almost everywhere}%
\Index%817%S%sequence converges uniformly
   {sequence converges uniformly}%
   {sequence converges uniformly}%
\Index%782%S%series converges normally
   {series converges normally}%
   {series converges normally}%
\Index%847%S%set admits operation
   {set admits operation}%
   {set admits operation}%
\Index%846%S%set is closed with respect to operation
   {set is closed with respect to operation}%
   {set is closed with respect to operation}%
\Index%356%S%set is dense in set
   {set is dense in set}%
   {dense in set}%
\Index%562%S%set of coordinates of representation
   {set of coordinates of representation}%
   {coordinate set of representation}%
\Index%628%S%set of invertible elements of algebra
   {set of invertible elements of algebra}%
   {set of invertible elements of algebra}%
\Index%571%S%set of Omega_2- words of representation
   {set of $\Omega_2$\Hyph words of representation}%
   {word set of representation}%
\Index%715%S%set of tuples of coordinates of diagram of representations
   {set of tuples of coordinates of diagram of representations}%
   {coordinate set of diagram of representations}%
\Index%563%S%set of tuples of coordinates of tower of representations
   {set of tuples of coordinates of tower of representations}%
   {coordinate set of tower of representations}%
\Index%942%S%set of tuples of Omega words
   {set of tuples of $\Omega$\Hyph words}%
   {set of tuples of Omega words}%
\Index%709%S%set of tuples of Omega- words of tower of representations
   {set of tuples of $\Vector\Omega$\Hyph words of tower of representations}%
   {word set of tower of representations}%
\Index%626%S%set of zeros of algebra
   {set of zeros of algebra}%
   {set of zeros of algebra}%
\Index%719%S%similarity transformation
   {similarity transformation}%
   {similarity transformation}%
\Index%810%S%simple map
   {simple map}%
   {simple map}%
\Index%405%S%simple polyvector
   {simple polyvector}%
   {simple polyvector}%
\Index%214%S%simplex
   {simplex}%
   {simplex}%
\Index%839%S%sine
   {sine}%
   {sine}%
\Index%299%S%single transitive representation of fibered Omega- algebra
   {single transitive representation of fibered $\Omega$\Hyph algebra}%
   {single transitive representation of fibered Omega-algebra}%
\Index%298%S%single transitive representation of group
   {single transitive representation of group}%
   {single transitive representation of group}%
\Index%297%S%single transitive representation of Omega- algebra A
   {single transitive representation of $\Omega$\Hyph algebra $A$}%
   {single transitive representation of algebra}%
\Index%723%S%singular endomorphism
   {singular endomorphism}%
   {singular endomorphism}%
\Index%130%S%singular linear map
   {singular linear map}%
   {singular linear map}%
\Index%226%S%skew product of vectors
   {skew product of vectors}%
   {skew product of vectors}%
\Index%904%S%skew symmetric polylinear map
   {skew symmetric polylinear map}%
   {skew symmetric polylinear map}%
\Index%406%S%space of orbits of G* representation
   {space of orbits of \Ts{G}representation}%
   {space of orbits of G* representation}%
\Index%684%S%space of orbits of left side representation
   {space of orbits of left\Hyph side representation}%
   {space of orbits of left side representation}%
\Index%342%S%spacelike vector
   {spacelike vector}%
   {spacelike vector}%
\Index%452%S%speed of deviation
   {speed of deviation}%
   {speed of deviation}%
\Index%168%S%spherical coordinates
   {spherical coordinates}%
   {spherical coordinates}%
\Index%841%S%square root
   {square root}%
   {square root}%
\Index%74%S%SRCstar,TRCstar- linear map of vector bundles
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph linear map of vector bundles}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-bimodule
   {($S\star$, $\star T$)\hyph bimodule}%
   {(Sstar,starT)-bimodule}%
\Index%145%S%stability group
   {stability group}%
   {stability group}%
\Index%457%S%stable set of representation
   {stable set of representation}%
   {stable set of representation}%
\Index%881%S%standard component of derivative
   {standard component of derivative}%
   {standard component of derivative}%
\Index%458%S%standard component of Gateaux derivative
   {standard component of the G\^ateaux derivative}%
   {standard component of Gateaux derivative}%
\Index%456%S%standard component of linear map
   {standard component of linear map}%
   {standard component of linear map}%
\Index%462%S%standard component of polylinear map
   {standard component of polylinear map}%
   {standard component of polylinear map}%
\Index%463%S%standard component of tensor
   {standard component of tensor}%
   {standard component of tensor}%
\Index%461%S%standard component over field F of bilitnear map f
   {standard component over field $F$ of bilitnear map $f$}%
   {standard component of bilinear map, division ring}%
\Index%471%S%standard coordinates of basis
   {standard coordinates of basis}%
   {standard coordinates of basis}%
\Index%472%S%standard coordinates of basis
   {standard coordinates of basis}%
   {standard coordinates of basis}%
\Index%880%S%standard representation of derivative
   {standard representation of the derivative}%
   {derivative, standard representation}%
\Index%465%S%standard representation of Gateaux derivative
   {standard representation of the G\^ateaux derivative}%
   {Gateaux derivative, standard representation}%
\Index%464%S%standard representation of linear map
   {standard representation of linear map}%
   {linear map, standard representation}%
\Index%468%S%standard representation of matrix
   {standard representation of matrix}%
   {Standard representation}%
\Index%470%S%standard representation of polylinear map
   {standard representation of polylinear map}%
   {polylinear map, standard representation}%
\Index%466%S%standard representation of quadratic map of division ring over field F
   {standard representation of quadratic map of division ring over field $F$}%
   {quadratic map, standard representation, division ring}%
\Index%469%S%standard representation over field F of bilinear map of division ring
   {standard representation over field $F$ of bilinear map of division ring}%
   {bilinear map, standard representation, division ring}%
\Index%79%S%star R-module
   {$\star R$\hyph module}%
   {starR-module}%
\Index%198%S%starD-product of vector over scalar
   {$\star D$\hyph product of vector over scalar}%
   {starD product of vector over scalar, vector space}%
\Index%261%S%starlike set
   {starlike set}%
   {starlike set}%
\Index%185%S%starT- representation of fibered group
   {\sT representation of fibered group}%
   {starT representation of fibered group}%
\Index%84%S%starT- representation of fibered group
   {\sT representation of fibered group}%
   {starT representation of fibered group}%
\Index%83%S%starT- representation of fibered Omega- algebra
   {\sT representation of fibered $\Omega$\Hyph algebra}%
   {starT representation of fibered Omega-algebra}%
\Index%81%S%starT- shift on fibered group
   {\sT shift on fibered group}%
   {starT shift, fibered group}%
\Index%86%S%starT- transformation on bundle
   {\sT transformation on bundle}%
   {starT transformation of bundle}%
\Index%473%S%structural constants
   {structural constants}%
   {structural constants}%
\Index%853%S%subalgebra of Omega-algebra
   {subalgebra of $\Omega$\Hyph algebra}%
   {subalgebra of Omega-algebra}%
\Index%340%S%subbundle
   {subbundle}%
   {subbundle}%
\Index%341%S%subbundle of Dstar-vector space
   {subbundle of $\mathcal D\star$\hyph vector space}%
   {subbundle of Dstar vector bundle}%
\Index%230%S%subgroup of Omega group
   {subgroup of $\Omega$\Hyph group}%
   {subgroup of Omega group}%
\Index%909%S%submodule
   {submodule}%
   {submodule}%
\Index%912%S%submodule generated by set
   {submodule generated by set}%
   {submodule generated by set}%
\Index%940%S%subrepresentation
   {subrepresentation}%
   {subrepresentation}%
\Index%322%S%subrepresentation generated by set X
   {subrepresentation generated by set $X$}%
   {subrepresentation generated by set}%
\Index%334%S%subrepresentation of representation
   {subrepresentation of representation}%
   {subrepresentation of representation}%
\Index%477%S%sum of geometric objects in vector space
   {sum of geometric objects in vector space}%
   {sum of geometric objects, vector space}%
\Index%476%S%sum of geometrical objects
   {sum of geometric objects}%
   {sum of geometric objects}%
\Index%351%S%sum of maps
   {sum of maps}%
   {sum of maps}%
\Index%667%S%sum of polynomials
   {sum of polynomials}%
   {sum of polynomials}%
\Index%323%S%superposition of coordinates
   {superposition of coordinates}%
   {superposition of coordinates,}%
\Index%712%S%superposition of coordinates of the tower of representations and the element
   {superposition of coordinates of the tower of representations $\Vector f$ and the element $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%446%S%symmetric 2- ary fibered relation
   {symmetric $2$\Hyph ary fibered relation}%
   {symmetric 2 ary fibered relation}%
\Index%447%S%symmetric bilinear map of D- vector space to division ring
   {symmetric bilinear map of $D$\Hyph vector space to division ring}%
   {symmetric bilinear map, vector space to division ring}%
\Index%933%S%symmetric correspondence
   {symmetric correspondence}%
   {symmetric correspondence}%
\Index%903%S%symmetric polylinear map
   {symmetric polylinear map}%
   {symmetric polylinear map}%
\Index%650%S%symmetric polylinear mapping into associative algebra
   {symmetric polylinear mapping into associative algebra}%
   {polylinear map symmetric, associative algebra}%
\Index%906%S%symmetrization of polylinear map
   {symmetrization of polylinear map}%
   {symmetrization of polylinear map}%
\Index%143%S%symmetry group
   {symmetry group}%
   {symmetry group}%
\Index%144%S%symmetry group
   {symmetry group}%
   {SymmetryGroup}%
\Index%448%S%synchronization of reference frame
   {synchronization of reference frame}%
   {synchronization of reference frame}%
\Index%605%S%system of additive equations
   {system of additive equations}%
   {system of additive equations}%
\Index%449%S%system of drc linear equations
   {system of \drc linear equations}%
   {system of drc linear equations}%
\Index%220%S%system of left AD* linear equations
   {system of left $A_*$\Hyph linear equations}%
   {system of left AD* linear equations}%
\Index%201%S%system of linear equations
   {system of linear equations}%
   {system of linear equations}%
\Index%311%S%system of rcd linear equations
   {system of \rcd linear equations}%
   {system of rcd linear equations}%
\Index%721%S%system of right AU* linear equations
   {system of right $A^*$\Hyph linear equations}%
   {system of right AU* linear equations}%
\SetIndexSpace%
\Index%823%T%T1 space
   {$T_1$\Hyph space}%
   {T1 space}%
\Index%499%T%Taylor polynomial
   {Taylor polynomial}%
   {Taylor polynomial, division ring}%
\Index%440%T%Taylor series
   {Taylor series}%
   {Taylor series, division ring}%
\Index%802%T%tensor inverse to tensor
   {tensor inverse to tensor}%
   {inverse tensor}%
\Index%652%T%tensor power
   {tensor power}%
   {tensor power}%
\Index%480%T%tensor product
   {tensor product}%
   {tensor product}%
\Index%47%T%the Fr\'echet Dstar derivative of map f of division ring D at point x
   {the Fr\'echet \Ds derivative of map $f$ of division ring $D$ at point $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%651%T%timelike vector
   {timelike vector}%
   {timelike vector}%
\Index%486%T%topological D- vector space
   {topological $D$\Hyph vector space}%
   {topological D vector space}%
\Index%310%T%topological D-algebra
   {topological $D$\Hyph algebra}%
   {topological D algebra}%
\Index%488%T%topological division ring
   {topological division ring}%
   {topological division ring}%
\Index%790%T%topological ring
   {topological ring}%
   {topological ring}%
\Index%498%T%torsion form
   {torsion form}%
   {torsion form}%
\Index%478%T%torsion tensor
   {torsion tensor}%
   {torsion tensor}%
\Index%120%T%tower of bundles
   {tower of bundles}%
   {tower of bundles}%
\Index%324%T%tower of effective representations
   {tower of effective representations}%
   {tower of effective representations}%
\Index%119%T%tower of representations of Omega algebras
   {tower of representations of $\Omega$\Hyph algebras}%
   {tower of representations of algebras}%
\Index%531%T%tower of subrepresentations
   {tower of subrepresentations}%
   {tower of subrepresentations}%
\Index%532%T%tower of subrepresentations of tower of representations generated by tuple of sets
   {tower of subrepresentations of tower of representations $\Vector f$ generated by tuple of sets $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%743%T%trace of quaternion
   {trace of quaternion}%
   {trace, quaternion algebra}%
\Index%376%T%transformation coordinated with equivalence
   {transformation coordinated with equivalence}%
   {transformation coordinated with equivalence}%
\Index%374%T%transformation of universal algebra
   {transformation of universal algebra}%
   {transformation of universal algebra}%
\Index%375%T%transformation on bundle
   {transformation on bundle}%
   {transformation of bundle}%
\Index%489%T%transitive 2- ary fibered relation
   {transitive $2$\Hyph ary fibered relation}%
   {transitive 2 ary fibered relation}%
\Index%934%T%transitive correspondence
   {transitive correspondence}%
   {transitive correspondence}%
\Index%492%T%transitive representation of fibered Omega- algebra
   {transitive representation of fibered $\Omega$\Hyph algebra}%
   {transitive representation of fibered Omega-algebra}%
\Index%491%T%transitive representation of group
   {transitive representation of group}%
   {transitive representation of group}%
\Index%490%T%transitive representation of Omega- algebra A
   {transitive representation of $\Omega$\Hyph algebra $A$}%
   {transitive representation of algebra}%
\Index%972%T%trivial kernel of homomorphism
   {trivial kernel of homomorphism}%
   {trivial kernel}%
\Index%187%T%Tstar- representation of fibered group
   {\Ts representation of fibered group}%
   {Tstar representation of fibered group}%
\Index%91%T%Tstar- representation of fibered Omega- algebra
   {\Ts representation of fibered $\Omega$\Hyph algebra}%
   {Tstar representation of fibered Omega-algebra}%
\Index%713%T%tuple of equivalence generated by tower of representations
   {tuple of equivalence generated by tower of representations $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%534%T%tuple of generating sets of tower of representations
   {tuple of generating sets of tower of representations}%
   {tuple of generating sets of tower of representations}%
\Index%941%T%tuple of Omega words
   {tuple of $\Omega$\Hyph words}%
   {tuple of Omega words}%
\Index%708%T%tuple of Omega- words of elements of tower of representations relative to tuple of generating sets
   {tuple of $\Vector{\Omega}$\Hyph words of element of tower of representations relative to tuple of generating sets}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%533%T%tuple of stable sets of diagram of representations
   {tuple of stable sets of diagram of representations}%
   {tuple of stable sets of diagram of representations}%
\Index%530%T%tuple of stable sets of tower of representation
   {tuple of stable sets of tower of representation}%
   {tuple of stable sets of tower of representations}%
\Index%587%T%twin representations
   {twin representations}%
   {twin representations}%
\Index%320%T%twin representations of division ring
   {twin representations of division ring}%
   {twin representations of division ring}%
\Index%319%T%twin representations of fibered group
   {twin representations of fibered group}%
   {twin representations of fibered group}%
\Index%318%T%twin representations of group
   {twin representations of group}%
   {twin representations of group}%
\Index%135%T%type of geometric object
   {type of geometric object}%
   {type of geometric object}%
\SetIndexSpace%
\Index%44%U%unit interval
   {unit interval}%
   {unit interval}%
\Index%796%U%unit of ring of sets
   {unit of ring of sets}%
   {unit of ring of sets}%
\Index%315%U%unit sphere in algebra
   {unit sphere in $D$\Hyph algebra}%
   {unit sphere in algebra}%
\Index%160%U%unit sphere in division ring
   {unit sphere in division ring}%
   {unit sphere in division ring}%
\Index%523%U%unit vector
   {unit vector}%
   {unit vector}%
\Index%132%U%unital algebra
   {unital algebra}%
   {unital algebra}%
\Index%916%U%unital extension
   {unital extension}%
   {unital extension}%
\Index%915%U%unital ring
   {unital ring}%
   {unital ring}%
\Index%673%U%unitarity law
   {unitarity law}%
   {unitarity law}%
\Index%851%U%universal algebra
   {universal algebra}%
   {universal algebra}%
\Index%914%U%universally attracting object of category
   {universally attracting object of category}%
   {universally attracting}%
\Index%688%U%universally repelling  object of category
   {universally repelling  object of category}%
   {universally repelling}%
\SetIndexSpace%
\Index%26%V%basis for vector  bundle
   {basis for vector  bundle}%
   {basis, vector bundle}%
\Index%288%V%valued division ring
   {valued division ring}%
   {valued division ring}%
\Index%901%V%vector
   {vector}%
   {vector}%
\Index%192%V%vector *A-space
   {vector $*A$\Hyph space}%
   {*A-vector space}%
\Index%125%V%vector bundle
   {vector bundle}%
   {vector bundle}%
\Index%787%V%vector module of algebra
   {vector module of algebra}%
   {vector module of algebra}%
\Index%776%V%vector module of ring
   {vector module of ring}%
   {vector module of ring}%
\Index%785%V%vector of element of algebra
   {vector of element of algebra}%
   {vector of algebra}%
\Index%774%V%vector of element of ring
   {vector of element of ring}%
   {vector of ring}%
\Index%126%V%vector potential
   {vector potential}%
   {vector potential}%
\Index%727%V%vector space
   {vector space}%
   {vector space}%
\Index%485%V%vector space type
   {vector space type}%
   {vector space type}%
\Index%398%V%vertical component of vector
   {vertical component of vector}%
   {vertical component of vector}%
\Index%687%V%vertical subspace
   {vertical subspace}%
   {vertical subspace}%
\Index%33%V%vertical vector
   {vertical vector}%
   {vertical vector}%
\SetIndexSpace%
\Index%212%W%Wronskian determinant
   {Wronskian determinant}%
   {Wronskian determinant}%
\Index%255%W%Wronskian matrix
   {Wronskian matrix}%
   {Wronskian matrix}%
\SetIndexSpace%
\Index%814%Z%zero divisor
   {zero divisor}%
   {zero divisor}%
\SetIndexSpace%
\Index%809%M%mu measurable map
   {$\mu$\Hyph measurable map}%
   {mu measurable map}%
\SetIndexSpace%
\Index%850%O%Omega algebra
   {$\Omega$\Hyph algebra}%
   {Omega-algebra}%
\Index%644%O%Omega group
   {$\Omega$\Hyph group}%
   {Omega group}%
\Index%944%O%Omega groupoid
   {$\Omega$\Hyph groupoid}%
   {Omega groupoid}%
\Index%646%O%Omega linear mapping
   {$\Omega$\Hyph linear mapping}%
   {Omega linear map}%
\Index%656%O%Omega ring
   {\(\Omega\)\Hyph ring}%
   {Omega ring}%
\Index%707%O%Omega_2- word of element of representation relative to generating set
   {$\Omega_2$\Hyph word of element of representation relative to generating set}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma algebra of sets
   {$\sigma$\Hyph algebra of sets}%
   {sigma algebra of sets}%
\Index%795%S%sigma ring of sets
   {$\sigma$\Hyph ring of sets}%
   {sigma ring of sets}%
\Index%762%S%sigma-additive measure
   {\(\sigma\)\Hyph additive measure}%
   {sigma-additive measure}%

\CloseIndex


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) map}%
\Index%660%A%A*- модуль
   {$A*$\Hyph модуль}%
   {A*-module}%
\Index%575%A%A*-векторное пространство
   {$A*$\Hyph векторное пространство}%
   {A*-vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%15%A%A-векторное пространство
   {$A$\hyph векторное пространство}%
   {A vector space}%
\Index%864%A%A-представление в Omega алгебре
   {$A$\Hyph представление в $\Omega$\Hyph алгебре}%
   {A representation of algebra}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%705%C%cr вырожденная матрица
   {\CR вырожденная матрица}%
   {cr singular matrix}%
\Index%954%C%cr квазидетерминант
   {\CR квазидетерминант}%
   {cr-quasideterminant}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%956%C%cr невырожденная матрица
   {\CR невырожденная матрица}%
   {cr nonsingular matrix}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение
   {\CR произведение (произведение столбца на строку)}%
   {cr-product}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%949%C%CR экспонента
   {\CR экспонента}%
   {CR exponent}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%134%C%cr-обратная матрица
   {\CR обратная матрица}%
   {cr-inverse matrix}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\Index%845%N%n-арная операция на множестве
   {$n$\Hyph арная операция на множестве}%
   {n-ary operation on set}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(\aUD{}ji)$\hyph \RC квазидетерминант}%
   {j i rc-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%rc вырожденная матрица
   {\RC вырожденная матрица}%
   {rc singular matrix}%
\Index%62%R%rc квазидетерминант
   {\RC квазидетерминант}%
   {rc-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%rc невырожденная матрица
   {\RC невырожденная матрица}%
   {r? nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение
   {\RC произведение (произведение строки на столбец)}%
   {rc-product}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%948%R%RC экспонента
   {\RC экспонента}%
   {RC exponent}%
\Index%600%R%RCcirc вырожденная матрица
   {$\RCcirc$\Hyph вырожденная матрица}%
   {RCcirc singular matrix}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица
   {$\RCcirc$\Hyph невырожденная матрица}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%218%R%rc-обратная матрица
   {\RC обратная матрица}%
   {rc-inverse matrix}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%830%А%абелевая мультипликативная Omega группа
   {абелевая мультипликативная $\Omega$\Hyph группа}%
   {Abelian multiplicative Omega group}%
\Index%869%А%абелевая полугруппа
   {абелевая полугруппа}%
   {Abelian semigroup}%
\Index%284%А%абсолютная величина
   {абсолютная величина}%
   {absolute value}%
\Index%859%А%автоморфизм
   {автоморфизм}%
   {automorphism}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%939%А%автоморфизм диаграммы представлений
   {автоморфизм диаграммы представлений}%
   {automorphism of diagram of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%569%А%активное представление в многообразии базисов
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов
   {активное преобразование многообразия базисов}%
   {active transformation of basis}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%741%А%алгебра кватернионов
   {алгебра кватернионов}%
   {quaternion algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%907%А%альтернация полилинейного отображения
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%929%А%антилинейный гомоморфизм
   {антилинейный гомоморфизм}%
   {antilinear homomorphism}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%849%А%арность
   {арность}%
   {arity}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%943%А%ассоциативная мультипликативная Omega группа
   {ассоциативная мультипликативная $\Omega$\Hyph группа}%
   {associative multiplicative Omega group}%
\Index%866%А%ассоциативная операция
   {ассоциативная операция}%
   {associative operation}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%115%Б%базис
   {базис}%
   {Basis}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%26%Б%базис в векторном расслоении
   {базис в векторном расслоении}%
   {basis, vector bundle}%
\Index%197%Б%базис векторного пространства
   {базис векторного пространства}%
   {basis, vector space}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%699%Б%базис диаграммы представлений
   {базис диаграммы представлений}%
   {basis of diagram of representations}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Omega$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%901%В%вектор
   {вектор}%
   {vector}%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%192%В%векторное *A-пространство
   {векторное $*A$\Hyph пространство}%
   {*A-vector space}%
\Index%727%В%векторное пространство
   {векторное пространство}%
   {vector space}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\Hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%481%В%взаимно простые  A числа
   {взаимно простые  $A$\Hyph числа}%
   {relatively prime A numbers}%
\Index%908%В%внешнее произведение
   {внешнее произведение}%
   {exterior product}%
\Index%508%В%внешний дифференциал
   {внешний дифференциал}%
   {exterior differential}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\Index%723%В%вырожденный эндоморфизм
   {вырожденный эндоморфизм}%
   {singular endomorphism}%
\SetIndexSpace%
\Index%871%Г%геодезический эффект
   {геодезический эффект}%
   {geodetic effect}%
\Index%700%Г%геометрический объект
   {геометрический объект}%
   {geometric object}%
\Index%838%Г%гиперболический косинус
   {гиперболический косинус}%
   {hyperbolic cosine}%
\Index%837%Г%гиперболический синус
   {гиперболический синус}%
   {hyperbolic sine}%
\Index%61%Г%главная подматрица
   {главная подматрица}%
   {major submatrix}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%885%Г%голоморфное отображение
   {голоморфное отображение}%
   {holomorphic map}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%854%Г%гомоморфизм
   {гомоморфизм}%
   {homomorphism}%
\Index%959%Г%гомоморфизм векторного пространства
   {гомоморфизм векторного пространства}%
   {homomorphism of vector space}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%861%Г%гомоморфный образ
   {гомоморфный образ}%
   {homomorphic image}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%865%Д%декартова степень
   {декартова степень}%
   {Cartesian power}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%598%Д%деление без остатка
   {деление без остатка}%
   {division without remainder}%
\Index%573%Д%деление с остатком
   {деление с остатком}%
   {division with remainder}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%935%Д%диаграмма представлений универсальных алгебр
   {диаграмма представлений универсальных алгебр}%
   {diagram of representations of algebras}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%661%Д%дифференциал независимой переменной
   {дифференциал независимой переменной}%
   {differential of independent variable}%
\Index%157%Д%дифференциал отображения
   {дифференциал отображения}%
   {differential of map}%
\Index%902%Д%дифференциальная p форма
   {дифференциальная $p$\Hyph форма}%
   {differential p form}%
\Index%737%Д%дифференциальная форма степени p
   {дифференциальная форма степени $p$}%
   {differential form of degree p}%
\Index%919%Д%дифференциальное уравнение с разделёнными переменными
   {дифференциальное уравнение с разделёнными переменными}%
   {differential equation with separated variables}%
\Index%922%Д%дифференциальное уравнение с разделяющимися переменными
   {дифференциальное уравнение с разделяющимися переменными}%
   {differential separable equation}%
\Index%877%Д%дифференцируемое отображение
   {дифференцируемое отображение}%
   {differentiable map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\Index%875%Е%естественный гомоморфизм
   {естественный гомоморфизм}%
   {natural homomorphism}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%964%З%закон коммутативности
   {закон коммутативности}%
   {commutative law}%
\Index%701%З%закон сокращения
   {закон сокращения}%
   {cancellation law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\Index%261%З%звёздное множество
   {звёздное множество}%
   {starlike set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%855%И%изоморфизм
   {изоморфизм}%
   {isomorphism}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%385%И%индукция по диаграмме представлений
   {индукция по диаграмме представлений}%
   {induction over diagram of representations}%
\Index%257%И%интеграл дифференциальной 1 формы вдоль пути
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
\Index%680%И%интеграл Лебега
   {интеграл Лебега}%
   {Lebesgue integral}%
\Index%438%И%интегрируемая дифференциальная форма
   {интегрируемая дифференциальная форма}%
   {integrable differential form}%
\Index%111%И%интегрируемая форма
   {интегрируемая форма}%
   {integrable form}%
\Index%918%И%интегрируемое дифференциальное уравнение
   {интегрируемое дифференциальное уравнение}%
   {integrable differential equation}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%368%К%каноническое отображение
   {каноническое отображение}%
   {canonical map}%
\Index%913%К%каноническое отображение
   {каноническое отображение}%
   {canonical map}%
\Index%599%К%каноническое представление деления с остатком
   {каноническое представление деления с остатком}%
   {canonical representation of division with remainder}%
\Index%726%К%каноническое частное от деления
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%177%К%категория левосторонних представлений
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%887%К%категория представлений
   {категория представлений}%
   {category of representations}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%842%К%квадратное уравнение
   {квадратное уравнение}%
   {quadratic equation}%
\Index%841%К%квадратный корень
   {квадратный корень}%
   {square root}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%535%К%квазибазис
   {квазибазис}%
   {quasibasis}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of maps}%
\Index%962%К%квазиэкспонента
   {квазиэкспонента}%
   {quasiexponent}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%969%К%ковариантное представление
   {ковариантное представление}%
   {covariant representation}%
\Index%258%К%колинеарные векторы
   {колинеарные векторы}%
   {colinear vectors}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%936%К%коммутативная диаграмма представлений универсальных алгебр
   {коммутативная диаграмма представлений универсальных алгебр}%
   {commutative diagram of representations}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%867%К%коммутативная операция
   {коммутативная операция}%
   {commutative operation}%
\Index%832%К%коммутативность представлений
   {коммутативность представлений}%
   {commutativity of representations}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%879%К%компонента производной
   {компонента производной}%
   {component of derivative}%
\Index%883%К%компонента производной второго порядка
   {компонента производной второго порядка}%
   {component of derivative of Second Order}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%873%К%конгруенция
   {конгруенция}%
   {congruence}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%968%К%контравариантное представление
   {контравариантное представление}%
   {contravariant representation}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%210%К%координатное векторное расслоение
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
\Index%697%К%координатное представление
   {координатное представление}%
   {coordinate representation}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%738%К%координаты
   {координаты}%
   {coordinates}%
\Index%558%К%координаты A числа относительно множества
   {координаты $A_2$\Hyph числа $m$ относительно множества $X$}%
   {coordinates relative to set}%
\Index%927%К%координаты ассоциатора
   {координаты ассоциатора}%
   {coordinates of associator}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%221%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
\Index%974%К%координаты гомоморфизма
   {координаты гомоморфизма}%
   {coordinates of homomorphism}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%967%К%координаты морфизма диаграммы представлений
   {координаты морфизма диаграммы представлений}%
   {coordinates of morphism, diagram of representations}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%945%К%координаты приведенного морфизма представления
   {координаты приведенного морфизма представления}%
   {coordinates of reduced morphism of representation}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%910%К%копроизведение в категории
   {копроизведение в категории}%
   {coproduct in category}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%941%К%кортеж Omega слов
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%533%К%кортеж стабильных множеств диаграммы представлений
   {кортеж стабильных множеств диаграммы представлений}%
   {tuple of stable sets of diagram of representations}%
\Index%840%К%косинус
   {косинус}%
   {cosine}%
\Index%904%К%косо симметричное полилинейное отображение
   {косо симметричное полилинейное отображение}%
   {skew symmetric polylinear map}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в аффинном пространстве}%
   {connection coefficients, affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%950%Л%левая линейная комбинация
   {левая линейная комбинация}%
   {left linear combination}%
\Index%896%Л%левое A векторное пространство
   {левое $A$\Hyph векторное пространство}%
   {left A vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%952%Л%левое пространство A-столбцов
   {левое пространство $A$\Hyph столбцов}%
   {left A-column space}%
\Index%955%Л%левое пространство A-строк
   {левое пространство $A$\Hyph строк}%
   {left A-row space}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%899%Л%левостороннее A представление
   {левостороннее $A_1$\Hyph представление}%
   {left-side A representation}%
\Index%184%Л%левостороннее представление
   {левостороннее представление}%
   {left-side representation}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%892%Л%левостороннее произведение
   {левостороннее произведение}%
   {left-side product}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%895%Л%левый A модуль
   {левый $A$\Hyph модуль}%
   {left A module}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%973%Л%левый смежный класс
   {левый смежный класс}%
   {left coset}%
\Index%88%Л%линейная комбинация
   {линейная комбинация}%
   {linear combination}%
\Index%32%Л%линейная оболочка
   {линейная оболочка}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%21%Л%линейно зависимое множество
   {линейно зависимое множество}%
   {linearly dependent set}%
\Index%136%Л%линейно зависимы слева
   {линейно зависимы слева}%
   {left linear dependent}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%833%Л%линейно зависимый
   {линейно зависимый}%
   {linearly dependent}%
\Index%34%Л%линейно независимое множество
   {линейно независимое множество}%
   {linearly independent set}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%921%Л%линейное однородное уравнение
   {линейное однородное уравнение}%
   {linear homogeneous equation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%735%Л%линейное преобразование аффинного пространства
   {линейное преобразование аффинного пространства}%
   {linear transformation, affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%894%М%матрица
   {матрица}%
   {matrix}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%255%М%матрица Вронского
   {матрица Вронского}%
   {Wronskian matrix}%
\Index%958%М%матрица гомоморфизма
   {матрица гомоморфизма}%
   {matrix of homomorphism}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear maps}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of maps}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%890%М%матрица Якоби отображения
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%835%М%метод последовательного дифференцирования
   {метод последовательного дифференцирования}%
   {method of successive differentiation}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%536%М%многообразие базисов
   {многообразие базисов}%
   {basis manifold}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%847%М%множество допускает операцию
   {множество допускает операцию}%
   {set admits operation}%
\Index%846%М%множество замкнуто относительно операции
   {множество замкнуто относительно операции}%
   {set is closed with respect to operation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%942%М%множество кортежей Omega слов
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%715%М%множество кортежей координат диаграммы представлений
   {множество кортежей координат диаграммы представлений}%
   {coordinate set of diagram of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%332%М%множество образующих
   {множество образующих}%
   {generating set}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%860%М%может быть вложена
   {может быть вложена}%
   {can be embeded}%
\Index%856%М%мономорфизм
   {мономорфизм}%
   {monomorphism}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни представлений в башню представлений
   {морфизм из башни представлений в башню представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%698%М%морфизм из диаграммы представлений в диаграмму представлений
   {морфизм из диаграммы представлений в диаграмму представлений}%
   {morphism from diagram of representations into diagram of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%828%М%мультипликативная Omega группа
   {мультипликативная $\Omega$\Hyph группа}%
   {multiplicative Omega group}%
\Index%829%М%мультипликативное отображение
   {мультипликативное отображение}%
   {multiplicative map}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%207%Н%наибольший общий делитель
   {наибольший общий делитель}%
   {highest common factor}%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система линейных уравнений
   {невырожденная система линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%219%Н%невырожденная система правых AU* линейных уравнений
   {невырожденная система правых $A^*$\Hyph линейных уравнений}%
   {nonsingular system of right AU* linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм
   {невырожденный эндоморфизм}%
   {regular endomorphism}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%870%Н%нейтральный элемент операции
   {нейтральный элемент операции}%
   {neutral element of operation}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%834%Н%неопределённый интеграл
   {неопределённый интеграл}%
   {indefinite integral}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%960%Н%непрерывный базис Шаудера
   {непрерывный базис Шаудера}%
   {continuous Schauder basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%928%Н%норма октониона
   {норма октониона}%
   {norm of octonion}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%702%Н%нормальная подгруппа
   {нормальная подгруппа}%
   {normal subgroup}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\Index%852%Н%носитель Omega-алгебры
   {носитель $\Omega$\Hyph алгебры}%
   {carrier of Omega-algebra}%
\SetIndexSpace%
\Index%848%О%область операторов
   {область операторов}%
   {operator domain}%
\Index%970%О%образ отображения
   {образ отображения}%
   {image of map}%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%482%О%общий делитель
   {общий делитель}%
   {common factor}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство
   {однородное пространство}%
   {homogeneous space}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен
   {однородный многочлен}%
   {homogeneous polynomial}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%844%О%операция на множестве
   {операция на множестве}%
   {operation on set}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%740%О%определённый интеграл
   {определённый интеграл}%
   {definite integral}%
\Index%212%О%определитель Вронского
   {определитель Вронского}%
   {Wronskian determinant}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear map}%
\Index%893%О%орбита представления
   {орбита представления}%
   {orbit of representation}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%484%О%остаток от деления
   {остаток от деления}%
   {remainder of the division}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%931%О%отношение эквивалентности
   {отношение эквивалентности}%
   {equivalence}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%886%О%отображение согласовано с операцией
   {отображение согласовано с операцией}%
   {map is compatible with operation}%
\Index%876%О%отображение сопряжения
   {отображение сопряжения}%
   {map of conjugation}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг аффинного пространства
   {параллельный сдвиг аффинного пространства}%
   {parallel shift, affine space}%
\Index%587%П%парные представления
   {парные представления}%
   {twin representations}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное G-представление
   {пассивное $G$\Hyph представление}%
   {passive G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%695%П%пассивное представление в многообразии базисов
   {пассивное представление в многообразии базисов}%
   {passive representation in basis manifold}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%336%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation, vector space}%
\Index%570%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation of basis}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%963%П%первый интеграл
   {первый интеграл}%
   {first integral}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%863%П%перестановка
   {перестановка}%
   {permutation}%
\Index%853%П%подалгебра Omega-алгебры
   {подалгебра $\Omega$\Hyph алгебры}%
   {subalgebra of Omega-algebra}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%909%П%подмодуль
   {подмодуль}%
   {submodule}%
\Index%912%П%подмодуль, порождённым множеством
   {подмодуль, порождённым множеством}%
   {submodule generated by set}%
\Index%940%П%подпредставление
   {подпредставление}%
   {subrepresentation}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%345%П%полилинейное косо симметричное отображение
   {полилинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%868%П%полугруппа
   {полугруппа}%
   {semigroup}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%953%П%правая линейная комбинация
   {правая линейная комбинация}%
   {right linear combination}%
\Index%961%П%правое A subs векторное пространство
   {правое $A_*$\Hyph векторное пространство}%
   {right A subs vector space}%
\Index%898%П%правое A векторное пространство
   {правое $A$\Hyph векторное пространство}%
   {right A vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%951%П%правое пространство A-столбцов
   {правое пространство $A$\Hyph столбцов}%
   {right A-column space}%
\Index%957%П%правое пространство A-строк
   {правое пространство $A$\Hyph строк}%
   {right A-row space}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%900%П%правостороннее A представление
   {правостороннее $A_1$\Hyph представление}%
   {right-side A representation}%
\Index%355%П%правостороннее представление
   {правостороннее представление}%
   {right-side representation}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%891%П%правостороннее произведение
   {правостороннее произведение}%
   {right-side product}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%897%П%правый D модуль
   {правый $D$\Hyph модуль}%
   {right D module}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%704%П%правый смежный класс
   {правый смежный класс}%
   {right coset}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%703%П%представитель геометрического объекта
   {представитель геометрического объекта}%
   {representative of geometric object}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%719%П%преобразование подобия
   {преобразование подобия}%
   {similarity transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%23%П%преобразование сопряжения
   {преобразование сопряжения}%
   {conjugation transformation}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%843%П%приведенное квадратное уравнение
   {приведенное квадратное уравнение}%
   {reduced quadratic equation}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%831%П%приведенный морфизм представлений
   {приведенный морфизм представлений}%
   {reduced morphism of representations}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%384%П%принцип ковариантности
   {принцип ковариантности}%
   {principle of covariance}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%395%П%произведение в категории
   {произведение в категории}%
   {product in category}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%133%П%произведение гомоморфизмов
   {произведение гомоморфизмов}%
   {product of homomorphisms}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%937%П%произведение морфизмов диаграммы представлений
   {произведение морфизмов диаграммы представлений}%
   {product of morphisms of diagram of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%882%П%производная Гато второго порядка
   {производная второго порядка}%
   {derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%878%П%производная отображения
   {производная отображения}%
   {derivative of map}%
\Index%884%П%производная порядка n
   {производная порядка $n$}%
   {derivative of Order n}%
\Index%483%П%простое A число
   {простое $A$\Hyph число}%
   {prime A number}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%684%П%пространство орбит левостороннего представления
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%911%П%прямая сумма
   {прямая сумма}%
   {direct sum}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%67%Р%ранг матрицы
   {ранг матрицы}%
   {rank of matrix}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный изоморфизм}%
   {fibered coordinate isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица
   {расширенная матрица}%
   {augmented matrix}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%932%Р%рефлексивное соответствие
   {рефлексивное соответствие}%
   {reflexive correspondence}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%331%С%свободная абелевая группа
   {свободная абелевая группа}%
   {free Abelian group}%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%862%С%свободное представление
   {свободное представление}%
   {free representation}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль
   {свободный модуль}%
   {free module}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%906%С%симметрирование полилинейного отображения
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%903%С%симметричное полилинейное отображение
   {симметричное полилинейное отображение}%
   {symmetric polylinear map}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%933%С%симметричное соответствие
   {симметричное соответствие}%
   {symmetric correspondence}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%839%С%синус
   {синус}%
   {sine}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%220%С%система левых AD* линейных уравнений
   {система левых $A_*$\Hyph линейных уравнений}%
   {system of left AD* linear equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%721%С%система правых AU* линейных уравнений
   {система правых $A^*$\Hyph линейных уравнений}%
   {system of right AU* linear equations}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%965%С%собственная строка
   {собственная строка}%
   {eigenrow}%
\Index%946%С%собственное значение
   {собственное значение}%
   {eigenvalue}%
\Index%966%С%собственный вектор
   {собственный вектор}%
   {eigenvector}%
\Index%947%С%собственный столбец
   {собственный столбец}%
   {eigencolumn}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%881%С%стандартная компонента производной
   {стандартная компонента производной}%
   {standard component of derivative}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%880%С%стандартное представление производной
   {стандартное представление производной}%
   {derivative, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%323%С%суперпозиция координат
   {суперпозиция координат}%
   {superposition of coordinates,}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение
   {тензорное произведение}%
   {tensor product}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%135%Т%тип геометрического объекта
   {тип геометрического объекта}%
   {type of geometric object}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%724%Т%точная последовательность
   {точная последовательность}%
   {exact sequence}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\Index%934%Т%транзитивное соответствие
   {транзитивное соответствие}%
   {transitive correspondence}%
\Index%972%Т%тривиальное ядро гомоморфизма
   {тривиальное ядро гомоморфизма}%
   {trivial kernel}%
\SetIndexSpace%
\Index%851%У%универсальная алгебра
   {универсальная алгебра}%
   {universal algebra}%
\Index%688%У%универсально отталкивающий  объект категории
   {универсально отталкивающий  объект категории}%
   {universally repelling}%
\Index%914%У%универсально притягивающий объект категории
   {универсально притягивающий объект категории}%
   {universally attracting}%
\Index%132%У%унитальная алгебра
   {унитальная алгебра}%
   {unital algebra}%
\Index%915%У%унитальное кольцо
   {унитальное кольцо}%
   {unital ring}%
\Index%916%У%унитальное расширение
   {унитальное расширение}%
   {unital extension}%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%920%У%уравнение в полных дифференциалах
   {уравнение в полных дифференциалах}%
   {exact differential equation}%
\Index%925%У%уравнение Картана
   {уравнение Картана}%
   {Cartan equation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%926%У%уравнение Максвела
   {уравнение Максвела}%
   {Maxwell equation}%
\Index%923%У%уравнение поля
   {уравнение поля}%
   {field equation}%
\Index%924%У%уравнение Эйнштейна
   {уравнение Эйнштейна}%
   {Einstein equation}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%369%Ф%факторгруппа
   {факторгруппа}%
   {factor group}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%722%Ц%центр A числа
   {центр $A$\Hyph числа}%
   {center of A number}%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%888%Ч%частная производная
   {частная производная}%
   {partial derivative}%
\Index%889%Ч%частная производная второго порядка
   {частная производная второго порядка}%
   {partial derivative of second order}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\Index%827%Ч%частное от деления
   {частное от деления}%
   {quotient divided by}%
\Index%905%Ч%чётность перестановки
   {чётность перестановки}%
   {parity of permutation}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%917%Э%эквивалентные нормы
   {эквивалентные нормы}%
   {equivalent norms}%
\Index%836%Э%экспонента
   {экспонента}%
   {exponent}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%858%Э%эндоморфизм
   {эндоморфизм}%
   {endomorphism}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%938%Э%эндоморфизм диаграммы представлений
   {эндоморфизм диаграммы представлений}%
   {endomorphism of diagram of representations}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%857%Э%эпиморфизм
   {эпиморфизм}%
   {epimorphism}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%872%Э%эффект увлечения системы отсчёта
   {эффект увлечения системы отсчёта}%
   {frame dragging effect}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление
   {эффективное представление}%
   {effective representation}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%874%Я%ядро гомоморфизма
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
\Index%971%Я%ядро гомоморфизма групп
   {ядро гомоморфизма групп}%
   {ker group-homomorphism}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%930%Я%ядро отображения
   {ядро отображения}%
   {kernel of map}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%850%O%Omega алгебра
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%944%O%Omega группоид
   {$\Omega$\Hyph группоид}%
   {Omega groupoid}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> MObject.tex <==
%auto-ignore
%\def\PrintBook{}
%\def\UseRussian{}
\def\UseParacol{}
\def\InputEncoding{on}% for arXiv put off
\input{Commands}
\usepackage{array,arydshln}
\makeatletter
\def\l@subsection{\@tocline{2}{0pt}{3pc}{5pc}{}}
\makeatother

\AddEq{H->L(H->H)}
{
\[\omega:H\rightarrow \mathcal L(R;H\rightarrow H)\]
}

\AddEq{contents}
{
\Prolog
\Input{Text.\BookNumber}
\Epilog
}

\def\texTitle{ Representation Theory of Universal Algebra }
\def\texAuthors{ Aleks Kleyn }
\def\texComments
{
English text - 20 pages; Russian text - 21 pages.
}
\def\texAbstract
{
Theory of representations of universal algebra
is a natural development of the theory of universal algebra.
Morphism of the representation is the map that conserve
the structure of the representation.
Exploring of morphisms of the representation leads to the concepts 
of generating set and basis of representation.
In the book I considered the notion of tower of representations of
F_i-algebras, i=1 ..., n,
as the set of coordinated representations of
F_i-algebras.
}
\def\JRef{this paper was published as chapter 2 of book
Representation Theory: Representation of Universal Algebra,
Lambert Academic Publishing, 2011}


==> Preface.MObject.English.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\section{Preface}

Consider rubber tube directed vertically.
The air that moves inside the pipe
changes the surface of the tube
such way that the horizontal section has the form
\ShowEq{differential equations 1 22-08-05}
where parameters $a$ and $b$ are functions
of coordinate $z$ and time $t$
and are
solution of the system of differential equations
\ShowEq{differential equations 22-08-05}

However, we can measure distance in meters  
or centimeters;
as well we can measure time in minutes or seconds.
We can change direction of axes $x$, $y$
in a plane perpendicular to the axis $z$.
These coordinate transformations will be reflected
in the notation of the equation and its solution.
However, the solution  to a problem does not depend
on the form of this solution in coordinate representation.

Consider more simple example.
Curve of the second order on the plane
has a very complex representation.
However, we can always choose coordinates
with respect to which the curve takes the canonical form
and is an ellipse, hyperbole, parabola or a pair of straight lines.

Symmetry consisting in the independence of the solution from the choice
of coordinates is called covariance.

Tensor algebra is the expression
of covariance in vector space over field.
Our goal is to consider the theory of covariance
in vector space over $D$\Hyph algebra.
Although this theory
is more complex than theory of covariance in vector space over field,
both theories share common features.


==> Preface.MObject.Russian.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\section{Предисловие}

Рассмотрим резиновую трубу, направленную вертикально.
Воздух, который движется внутри трубы,
меняет поверхность трубы
таким образом, что горизонтальное сечение имеет вид
\ShowEq{differential equations 1 22-08-05}
где параметры $a$, $b$ являются функцией
координаты $z$ и времени $t$
и являются
решением системы дифференциальных уравнений
\ShowEq{differential equations 22-08-05}

Однако расстояние может измеряться в метрах
или сантиметрах,
время может измеряться в минутах или секундах.
Мы можем изменить направление осей $x$, $y$
в плоскости, перпендикулярной оси $z$.
Эти преобразования координат отразятся
в записи уравнения и его решения.
Однако решение задачи не зависит от того,
какой вид это решение имеет в координатном представлении.

Рассмотрим более простой пример.
Кривая второго порядка на плоскости
имеет очень сложный вид.
Однако мы всегда можем выбрать координаты,
относительно которых кривая принимает канонический вид
и является элипсом, гиперболой, параболой или парой прямых.

Симметрия, состоящая в независимости решения от выбора
координат, называется ковариантностью.

Тензорная алгебра является выражением
ковариантности в векторном пространстве над полем.
Наша задача рассмотреть теорию ковариантности
в векторном пространстве над $D$\Hyph алгеброй.
Хотя эта теория
сложнее чем теория ковариантности в векторном пространстве над полем,
обе теории имеют общие черты.


==> Preface.MObject.eq.tex <==
%auto-ignore

\AddEquation{differential equations 22-08-05}
{
\begin{array}{r@{\,}l@{\ \ \ \ }r@{\,}l}
\displaystyle\frac{\partial a}{\partial z}&=a_1x+b_1y
&
\displaystyle\frac{\partial b}{\partial z}&=c_1x+d_1y
\\[10pt]
\displaystyle\frac{\partial a}{\partial t}&=a_2x+b_2y
&
\displaystyle\frac{\partial b}{\partial t}&=c_2x+d_2y
\end{array}
}

\AddEquation{differential equations 1 22-08-05}
{
\frac{x^2}{a^2}+\frac{y^2}{b^2}=1
}


==> Prolog.Cite.English.tex <==
%auto-ignore

\DefCiteBib{1302.7204}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}

\DefCiteBib{1801.01628}
{
Aleks Kleyn,
Differential Equation over Banach Algebra,\\
eprint \href{http://arxiv.org/abs/1801.01628}{arXiv:1801.01628} (2018)
}

\DefCiteBib{1908.04418}
{
Aleks Kleyn,
Diagram of Representations of Universal Algebras,\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}

\DefCiteBib{Korn}
{
Granino A. Korn, Theresa M. Korn,
Mathematical Handbook for Scientists and Engineer,
McGraw-Hill Book Company, New York, San Francisco,
Toronto, London, Sydney, 1968
}

\DefCiteBib{Rashevsky}
{
P. K. Rashevsky,
Riemann Geometry and Tensor Calculus,\\
Moscow, Nauka, 1967
}

\DefCiteBib{1502.04063}
{
Aleks Kleyn,
Linear Map of $D$\Hyph Algebra,\\
eprint \href{http://arxiv.org/abs/1502.04063}{arXiv:1502.04063} (2015)
}

\DefCiteBib{0812.4763}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}

\DefCiteBib{1601.03259}
{
Aleks Kleyn,
Introduction into Calculus over Banach Algebra,\\
eprint \href{http://arxiv.org/abs/1601.03259}{arXiv:1601.03259} (2016)
}

\DefCiteBib{2207.06506}
{
Aleks Kleyn,
Introduction into Noncommutative Algebra,
Volume 1, Division Algebra\\
eprint \href{http://arxiv.org/abs/2207.06506}{arXiv:2207.06506} (2022)
}


==> Prolog.Cite.Russian.tex <==
%auto-ignore

\DefCiteBib{1302.7204}
{
Александр Клейн,
Многочлен над ассоциативной $D$-алгеброй,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}

\DefCiteBib{1801.01628}
{
Александр Клейн,
Дифференциальное уравнение над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1801.01628}{arXiv:1801.01628} (2018)
}

\DefCiteBib{1908.04418}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}

\DefCiteBib{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М.,
Наука, 1974
}

\DefCiteBib{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}

\DefCiteBib{1502.04063}
{
Александр Клейн,
Линейное отображение $D$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/1502.04063}{arXiv:1502.04063} (2015)
}

\DefCiteBib{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}

\DefCiteBib{1601.03259}
{
Александр Клейн,
Введение в математический анализ над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1601.03259}{arXiv:1601.03259} (2016)
}

\DefCiteBib{2207.06506}
{
Александр Клейн,
Введение в некоммутативную алгебру,
Том 1, Алгебра с делением\\
eprint \href{http://arxiv.org/abs/2207.06506}{arXiv:2207.06506} (2022)
}


==> Prolog.Cite.tex <==
%auto-ignore

\Input{Prolog.Cite}

\DefCiteBib{1812.03397}
{
Ivan Kyrchei,
Linear differential systems over the quaternion skew field,
eprint \href{http://arxiv.org/abs/1812.03397}{arXiv:1812.03397} (2018)
}

\DefCiteBib{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}

\DefCiteBib{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}

\DefCiteBib{1510.02224}
{
Kit Ian Kou, Yong-Hui Xia.
Linear Quaternion Differential Equations: Basic Theory and Fundamental Results.\\
eprint \href{http://arxiv.org/abs/1510.02224}{arXiv:1510.02224} (2017)
}

\DefCiteBib{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}

\DefCiteBib{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,\\
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}


==> Prolog.Eq.tex <==
%auto-ignore

\def\iI{\ensuremath{i\in I}}%
\def\iIg{\ensuremath{\gii\in\giI}}%
\newcommand\jJg[2]{\ensuremath{\gi{#1}\in\gi{#2}}}%
\def\Times{A_1\times...\times A_n}%
\newcommand\LAA[2]{\ensuremath{\mathcal L(#1;#2\rightarrow #2)}}%
\newcommand\LAB[3]{\ensuremath{\mathcal L(#1;#2\rightarrow #3)}}%
\newcommand\Kn[2][k]{$#1=#2$, ..., $n$}%
\newcommand\Kb[2][k]{$(#1)=(#2)$, ..., $(n)$}%
\newcommand\Ki[2][i]{\ensuremath{\gi{#1}=\gi 1}, ..., \ensuremath{\gi{#2}}}%
\def\ATwo{A_2\otimes A_2}%
\newcommand\AxA[1]{\ensuremath{#1\times #1}}%
\newcommand\AoxA[1]{\ensuremath{#1\otimes #1}}%
\newcommand\BoxB[1]{\AoxA{#1}\Hyph}%
\newcommand\AoxB[2]{\ensuremath{#1\otimes #2}}%

\newcommand\FC[2]{f^{\gi{#1#2}}}%
\newcommand\TensorBasis[1]%
{e_{1\cdot\gi{#1_1}}\otimes...\otimes e_{n\cdot\gi{#1_n}}}%
\newcommand\re{\mathrm{Re}\,}%
\newcommand\im{\mathrm{Im}\,}%

\ePrints{309618526,5284-0163,1801.01628,322019412,323236904,330532713,323966352}
\Items{8428-0408,2207.06506,1908.04418,6860-2955,367250917,1506.00061}%
\Items{2021.01.06,1601.03259,2022.01.05,2021.11.26,2112.00613,348311191,2020.06.01}%
\Items{357606033,MAlgebra2,2204.06320,MObject,2022.11.26,2023.01.07}%
\ifx\Semafor\ValueOn%
\input{Prolog.Cite}%
\fi%

\ePrints{MAlgebra2,1908.04418,6860-2955,1601.03259,4975-6381,5410-9916,1305.4547,1502.04063,1310.5591}%
\Items{309618526,CACAA.06.121,5059-9176,323236904,322019412,5284-0163,1801.01628,9835-2163,9856-6693,0767-8264}%
\Items{8428-0408,2207.06506,CACAA.07,323966352,0921-2370,5148-4632,1506.00061,7287-9339,330532713}%
\Items{2020.06.01,2021.01.06,2204.06320,2022.01.05,348311191,MObject,2022.11.26,2023.01.07}%
\ifx\Semafor\ValueOn%
\Input{Stmt.Representation}%
\fi%

\ePrints{MAlgebra2,309618526,CACAA.06.121,1601.03259,4975-6381,5410-9916,1502.04063,5114-6019}%
\Items{323236904,1908.04418,6860-2955,322019412,5284-0163,1801.01628,9835-2163,9856-6693,0767-8264,MTensor}%
\Items{323966352,0921-2370,CACAA.07,1506.00061,7287-9339,5148-4632}%
\Items{8428-0408,2207.06506,0803.3276,7100-9423,2020.06.01,1211.6965,MAlgebra4,2021.01.06}%
\Items{2021.01.06,2021.11.26,2112.00613,2022.01.05,2204.06320,MObject,2022.11.26}%
\Items{2023.01.07,367250917}%
\ifx\Semafor\ValueOn%
\Input{Stmt.Module}%
\fi%

\ePrints{1801.01628,2020.06.01,339295394,348311191,5284-0163,1506.00061}%
\Items{8428-0408,2207.06506,2204.06320,2022.01.05,1908.04418,6860-2955}%
\Items{MAlgebra2,5148-4632,MObject,2022.11.26,2023.01.07,357606033,367250917}%
\ifx\Semafor\ValueOn%
\Input{Vector.Space.2020.Stmt}%
\fi%

\ePrints{1502.04063,323236904,0803.3276,1801.01628}%
\Items{0767-8264,2020.06.01,0412.391,4827-2437,7100-9423,5284-0163}%
\ifx\Semafor\ValueOn%
\Input{D.Module.Stmt}%
\fi%

\ePrints{1801.01628,5284-0163}%
\Items{2204.06320,2022.01.05,348311191,357606033,2020.06.01}%
\Items{2023.01.07}%
\ifx\Semafor\ValueOn%
\Input{DiffUr.3.Stmt}%
\fi%

\ePrints{8428-0408,2207.06506,367250917}%
\ifx\Semafor\ValueOn%
\input{DiffUr.3.Stmt.Eq}%
\fi%

\ePrints{1908.04418,6860-2955,1801.01628,2020.06.01,5284-0163,0767-8264}%
\Items{8428-0408,2207.06506,2204.06320,2022.01.05}%
\ifx\Semafor\ValueOn%
\Input{Biring.Stmt}%
\fi%

\ePrints{1908.04418,6860-2955,2207.06506,8428-0408,1305.4547,5284-0163,1801.01628}%
\Items{6860-2955,5148-4632,MAlgebra2,5410-9916,1601.03259,309618526,CACAA.06.121,4975-6381,322019412}%
\ifx\Semafor\ValueOn%
\Input{Stmt.Omega}%
\fi%

\ePrints{309618526,CACAA.06.121,4975-6381,1601.03259,323236904}%
\Items{5284-0163,1801.01628,9835-2163,0767-8264,322019412,1211.6965,MAlgebra4}%
\Items{8428-0408,2207.06506,9856-6693,CACAA.07,330532713,2020.06.01,2021.01.06,348311191}%
\ifx\Semafor\ValueOn%
\Input{Stmt.Derivative}%
\fi%

\ePrints{323966352,0921-2370,1908.04418,6860-2955,0803.3276,7100-9423,FAlgebra,0405.027}%
\ifx\Semafor\ValueOn%
\Input{Stmt.Gravity}%
\fi%

\ePrints{324329551}%
\ifx\Semafor\ValueOn%
\input{Stmt.Gravity.Eq}%
\fi%

\ePrints{MAlgebra3,1601.03259,4975-6381,322019412,5284-0163,1801.01628}%
\ifx\Semafor\ValueOn%
\input{Algebra.Complex.2016.Eq}%
\fi%

\ePrints{309618526,323966352,0921-2370,CACAA.06.121,MAlgebra3,CACAA.07,322019412}%
\Items{1506.00061,7287-9339,5284-0163,1801.01628,9835-2163,0767-8264,330532713,2021.01.06}%
\Items{339295394,348311191}%
\ifx\Semafor\ValueOn%
\input{Algebra.Quaternion.2016.Eq}%
\fi%

\ePrints{309618526,323966352,0921-2370,MAlgebra3}%
\ifx\Semafor\ValueOn%
\input{Algebra.Octonion.2016.Eq}%
\fi%

\ePrints{330532713,339295394,348311191,357606033}%
\ifx\Semafor\ValueOn%
\input{Stmt.Module.Eq}%
\fi%

\ePrints{323966352,0921-2370,339295394,2204.06320,2022.01.05,367250917}%
\ifx\Semafor\ValueOn%
\input{Stmt.Derivative.Eq}%
\fi%

\ePrints{339295394,357606033,367250917}%
\ifx\Semafor\ValueOn%
\input{Stmt.Representation.Eq}%
\fi%

\ePrints{2021.11.26,2112.00613,8428-0408,2207.06506,357606033}%
\ifx\Semafor\ValueOn%
\Input{Stmt.2021.11.26}%
\fi%

\ePrints{2022.01.05,MObject,2022.11.26,2204.06320,2023.01.07}%
\ifx\Semafor\ValueOn%
\Input{Stmt.2022.01.05}%
\fi%

\input{Prolog.Ref}%

\AddEq{L D->A=A}
{
$\mathcal L(D;D\rightarrow A)=A$
\qed
}

\AddEq{|x'-x|<delta}
{
\[
\|x'-x\|_1<\delta
\]
}

\AddEquation{fd=da}
{
f\circ d=da
}

\AddEq{fd=df1}
{
\[f\circ d=d(f\circ 1)\]
}

\AddEq{ab=ba}
{
ab=ba
}

\AddEq[1]{a=b}
{
$a_1=b_1$#1
}

\DefEq
{
$\Basis e_i$
}
{tensor product of algebras, basis i}

\AddEq[1]{set a1n}
{
$\{a_1,...,a_n\}$#1
}

\AddEquation{x2+ax+xa=}
{
x^2+(1\otimes a+a\otimes 1)\circ x
=x\left(\frac 12 x+a\right)+\left(\frac 12x+a\right)x
}

\AddEq[1]{Quaternion a}
{
#1=\aU{#1}0+\aU{#1}1i+\aU{#1}2j+\aU{#1}3k
}

\DefEq
{
\symb{a^{\gi{i_1...i_n}}}{standard component of tensor}{}
}
{standard component of tensor}

\AddEquation{module L(A;A) is algebra}
{
\circ:(g,f)\in\mathcal L(D;A\rightarrow A)\times\mathcal L(D;A\rightarrow A)
\rightarrow g\circ f\in\mathcal L(D;A\rightarrow A)
}

\AddEq [3]{f:A->B}
{
\[#1:#2\rightarrow #3\]
}

\DefEq
{
\[
\xymatrix{
&A\ar[rd]^g
\\
A\ar[ru]^f\ar[rr]^{g\circ f}&&A
}
\]
}
{product of linear map, algebra 1}

\DefEquation
{
a=
\ShowSymbol{standard component of tensor}{}
\TensorBasis i
}
{tensor canonical representation, algebra}

\AddEq{k,1n}
{
$k$, $k=1$, ..., $n$,
}

\AddEq{n,1.}
{
$n$, $n=1$, ...,
}

\newcommand{\Tensor}[1]{#1_1\otimes...\otimes #1_n}

\AddEq[1]{set Ai}
{
$#1_i$, \iI,
}

\AddEq{coproduct in category diagram}
{
\[
\xymatrix{
P\ar[d]_h&B_i\ar[l]_{f_i}\ar[dl]^{g_i}&h\circ f_i=g_i
\\
R
}
\]
}

\AddEq[2]{A=Ai iI}
{
\(#1=(#1_i,\iI)\)#2
}

\DefEq
{
\begin{align*}
\re&:A\rightarrow A
\\
\im&:A\rightarrow A
\end{align*}
}
{Re Im A->A}

\DefEq
{
\symb{\re d}{scalar of algebra}{}
\symb{\im d}{vector of algebra}{}
}
{Re Im A->F 0}

\AddEquation{Re Im A->F 1}
{
\begin{matrix}
\ShowSymbol{scalar of algebra}{}=d^{\gi 0}
&\ShowSymbol{vector of algebra}{}=d-d^{\gi 0}
&d\in D
&d=d^{\gii}e_{\gii}
\end{matrix}
}

\DefEq
{
$\ShowSymbol{scalar of algebra}{}$
}
{Re Im A->F 2}

\DefEq
{
$\ShowSymbol{vector of algebra}{}$
}
{Re Im A->F 3}

\DefEq
{
\[
F=\{d\in A:\re d=d\}
\]
}
{Re Im A->F 4}

\DefEq
{
\symb{\re A}{scalar algebra of algebra}1
}
{scalar algebra of algebra}

\DefEq
{
\symb{\im A}{vector module of algebra}{}
\begin{equation}
\EqLabel{vector module of algebra}
\ShowSymbol{vector module of algebra}{}=\{d\in A:\re d=0\}
\end{equation}
}
{vector module of algebra}

\DefEquation
{
C_{\gi{0k}}^{\gil}=C^{\gil}_{\gi{k0}}=\delta^{\gik}_{\gil}
}
{structural constant re algebra, 1}

\DefEquation
{
d=\re d+\im d
}
{d Re Im}

\DefEq
{
\symb{d^*}{conjugation in algebra}{}
}
{conjugation in algebra}

\DefEquation
{
\ShowSymbol{conjugation in algebra}{}=\re d-\im d
}
{conjugation in algebra, 0}

\DefEquation
{
(cd)^*=d^*\,c^*
}
{conjugation in algebra, 1}

\DefEquation
{
\begin{matrix}
C^{\gi 0}_{\gi{kl}}=C^{\gi 0}_{\gi{lk}}
&
C^{\gi p}_{\gi{kl}}=-C^{\gi p}_{\gi{lk}}
\end{matrix}
}
{conjugation in algebra, 5}

\AddEq{p=p circ x}
{
$p(x)=p_1\circ x+p_0$
}

\AddEq{x in C=>fx=gx}
{
$x\in C\Rightarrow f(x)=g(x)$.
}

\AddEq[3]{A in B}
{
$#1\subseteq #2$#3
}

\AddEq{(a+x)2=a2 1}
{
x^2+(1\otimes a+a\otimes 1)\circ x=0
}

\DefEquation
{
p(x)=p_0+p_1\circ x
}
{p=p+p circ x}

\DefEq
{
\[
r(x)=r_0+r_1\circ x+...+r_k\circ x^k
\]
}
{r power k}

\DefEquation
{
\begin{split}
r(x)&=r_0
-((r_{1\cdot 0\cdot s}\otimes r_{1\cdot 1\cdot s})\circ
p^{-1}_1)\circ p_0
\\
&-(((r_{2\cdot 0\cdot s}\circ x)\otimes r_{2\cdot 1\cdot s})\circ
p^{-1}_1)\circ p_0
\\
&-...-(((r_{k\cdot 0\cdot s}\circ x^{k-1})
\otimes r_{k\cdot 1\cdot s})\circ
p^{-1}_1)\circ p_0
\\
&+((r_{1\cdot 0\cdot s}\otimes r_{1\cdot 1\cdot s})\circ
p^{-1}_1)\circ p(x)
\\
&+(((r_{2\cdot 0\cdot s}\circ x)\otimes r_{2\cdot 1\cdot s})\circ
p^{-1}_1)\circ p(x)
\\
&+...+(((r_{k\cdot 0\cdot s}\circ x^{k-1})
\otimes r_{k\cdot 1\cdot s})\circ
p^{-1}_1)\circ p(x)
\\
&=r_0
-((r_{1\cdot 0\cdot s}\otimes r_{1\cdot 1\cdot s}
+(r_{2\cdot 0\cdot s}\circ x)\otimes r_{2\cdot 1\cdot s}
\\
&+...+(r_{k\cdot 0\cdot s}\circ x^{k-1})
\otimes r_{k\cdot 1\cdot s})\circ
p^{-1}_1)\circ p_0
\\
&+((r_{1\cdot 0\cdot s}\otimes r_{1\cdot 1\cdot s}
+(r_{2\cdot 0\cdot s}\circ x)\otimes r_{2\cdot 1\cdot s}
\\
&+...+(r_{k\cdot 0\cdot s}\circ x^{k-1})
\otimes r_{k\cdot 1\cdot s})\circ
p^{-1}_1)\circ p(x)
\end{split}
}
{r=+q circ p 1}

\DefEq
{
\[
ax-xa=1
\]
}
{ax-xa=1}

\DefEquation
{
r(x)=q_{i\cdot 0}(x)p(x)q_{i\cdot 1}(x)
=(q_{i\cdot 0}(x)\otimes q_{i\cdot 1}(x))\circ p(x)
}
{r=qpq(x)}

\DefEq
{
h=f_1...f_n\omega
}
{h=f1...fn omega}

\DefEq
{
\(f_X(g_{1\cdot n})(g_{2\cdot n})\)
}
{f(g1n)(g2n)}

\DefEq
{
\[b_i=f_i(a_i)\]
}
{b=f(a)i}

\AddEq [2]{f->g}
{
\[#1\rightarrow #2\]
}

\AddEq [3]{A->B}
{
$#1\rightarrow #2$#3
}

\DefEq
{
\[h:S_1\rightarrow S_2\]
}
{f->g 1}

\AddEq{polylinear maps category, diagram}
{
\[
\xymatrix{
&S_1\ar[dd]^h
\\
\Times
\ar[ru]^f\ar[rd]_g
\\
&S_2
}
\]
}

\AddEq [3]{map r,R}
{
$(#1,#2)$#3
}

\DefEq
{
\symb{A^{\otimes n}}{tensor power of algebra}{}
\[
\begin{matrix}
\ShowSymbol{tensor power of algebra}{}
=\Tensor A
&
A_1=...=A_n=A
\end{matrix}
\]
}
{tensor power of algebra}

\AddEq{basis of complex field}
{
\[
\begin{array}{rr}
e_{\gi 0}=1&e_{\giA}=i
\end{array}
\]
}

\AddEquation{product of complex field}
{
e_{\giA}^2=-e_{\gi 0}
}

\DefEq
{
\[f:H\rightarrow H\ \ \ y^{\gii}=f^{\gii}_{\gij}x^{\gij}\]
}
{f:H->H ij}

\DefEq
{
\[HE=\{aE:a\in H\}\]
}
{HE set}

\AddEquation{structural constants of complex field}
{
\begin{array}{r@{}rr@{}r}
\aUD C0{00}=&1&\aUD C1{01}=&1
\\
\VirtVar
\aUD C1{10}=&1&\aUD C0{11}=&-1
\end{array}
}

\DefEq
{
\[
x=x^{\gi 0}+x^{\giA}i\rightarrow
f=f^{\gi 0}(x^{\gi 0},x^{\giA})+f^{\giA}(x^{\gi 0},x^{\giA})i
\]
}
{map of complex variable}

\AddEq [1]{Cauchy Riemann equations, complex field, 1}
{
\begin{split}
\frac{\partial #1^{\giA}}{\partial x^{\gi 0}}
&=-\frac{\partial #1^{\gi 0}}{\partial x^{\giA}}
\\[5pt]
\frac{\partial #1^{\gi 0}}{\partial x^{\gi 0}}
&=\hphantom{-\,}\frac{\partial #1^{\giA}}{\partial x^{\giA}}
\end{split}
}

\AddEq [1]{Cauchy Riemann equations, complex field, 2, 1}
{
\frac{\partial #1^{\gi 0}}{\partial x^{\gi 0}}
+i\frac{\partial #1^{\giA}}{\partial x^{\gi 0}}
+i\left(\frac{\partial #1^{\gi 0}}{\partial x^{\giA}}
+i\frac{\partial #1^{\giA}}{\partial x^{\giA}}\right)=
\frac{\partial #1^{\gi 0}}{\partial x^{\gi 0}}
+i\frac{\partial #1^{\giA}}{\partial x^{\gi 0}}
+i\frac{\partial #1^{\gi 0}}{\partial x^{\giA}}
-\frac{\partial #1^{\giA}}{\partial x^{\giA}}=
0
}

\DefEq
{
\[
\begin{matrix}
a\circ E:H\rightarrow H&
a=a^{\gi 0}+a^{\gi 1}i+a^{\gi 2}j+a^{\gi 3}k\in H
\end{matrix}
\]
}
{aE, quaternion}

\AddEq{df=...dx 03}
{
\begin{split}
\frac{d f}{d x}=&-\frac 12
\left(
\frac{\partial f}{\partial x^{\gi 0}}
+\frac{\partial f}{\partial x^{\gi 1}}i
+\frac{\partial f}{\partial x^{\gi 2}}j
+\frac{\partial f}{\partial x^{\gi 3}}k
\right)\bullet E
\\&
+\frac 12\left(
\frac{\partial f}{\partial x^{\gi 0}}
+\frac{\partial f}{\partial x^{\gi 1}}i
\right)\bullet\aU I1
+\frac 12\left(
\frac{\partial f}{\partial x^{\gi 0}}
+\frac{\partial f}{\partial x^{\gi 2}}j
\right)\bullet\aU I2
\\&
+\frac 12\left(
\frac{\partial f}{\partial x^{\gi 0}}
+\frac{\partial f}{\partial x^{\gi 3}}k
\right)\bullet\aU I3
\end{split}
}

\AddEq{tensor product of algebras}
{
\symb{\Tensor A}{tensor product}1
}

\DefEq
{
\[
(f+g)(a)=f(a)+g(a)
\]
}
{(f+g)(a)=}

\AddEquation{sum of transformations of Abelian group, 1}
{
f(a+b)(x)=f(a)(x)+f(b)(x)
}

\ePrints{1502.04063,5114-6019,1211.6965,MAlgebra4}
\ifx\Semafor\ValueOff
\DefEquation
{
f(a)(m)=f(b)(m)
}
{representation of ring, 1}

\AddEquation{representation of ring, 2}
{
f(a-b)(m)=0
}
\fi

\AddEq{polynomials p,r}
{
$p\circ F_{[1]}\circ x^n$, $r\circ F_{[2]}\circ x^m$
}

\DefEq
{
\[
(p\circ F_{[1]}\circ x^n)(r\circ F_{[2]}\circ x^m)
=(p\underline{\otimes}r)\circ
(F_{[1](1)},...,F_{[1](n)},F_{[2](1)},...,F_{[2](m)})
\circ x^{n+m}
\]
}
{pr=p circ r}

\DefEquation
{
p(x)=
(a_{k\cdot 0}\circ x^{k-1})
((1\otimes a_{k\cdot 1})\circ x)
}
{p(x)=a k-1 k 1}

\DefEquation
{
p(x)=
((a_{k\cdot 0}\circ x^{k-1})
\otimes a_{k\cdot 1})\circ x
}
{p(x)=a k-1 k 2}

\DefEq
{
$A_{ij}$, $i=1$, ..., $n$, $j=1$, ..., $m$,
}
{Aij}

\DefEq
{
$\Omega_{ij}$\Hyph%
}
{Omegaij}

\AddEq{polylinear maps category}
{
\[
\xymatrix@C=15pt{
f:\Times\ar[r]&S_1
&
g:\Times\ar[r]&S_2
}
\]
}

\AddEq[1]{R1 X->}
{
\[R_1:#1\rightarrow #1'\]
}

\DefEq
{
\[
R\circ m=R_1(m)
\]
}
{Rm=R1m}

\DefEq
{
$r_1=q_1\circ p_1$, $r_2=q_2\circ p_2$.
}
{r=q*p}

\DefEq
{
\[
r_2:A_2\rightarrow A_2
\]
}
{R:A2->A2}

\DefEq
{
\[
a\pC i0xa\pC i1
\]
}
{Sum over repeated index}

\DefEq
{
\symb{\mathcal L(D;A_1\times...\times A_n\rightarrow S)}{set polylinear maps}1
}
{set polylinear maps}

\DefEquation
{
(A_1\otimes A_2)\otimes A_3=A_1\otimes(A_2\otimes A_3)
=A_1\otimes A_2\otimes A_3
}
{A1xA2xA3}

\DefEq
{
\[
(v_1, ..., v_n)\in V_1\times...\times V_n
\rightarrow v_1\otimes...\otimes v_n\in V_1\otimes...\otimes V_n
\]
}
{V times->V otimes}

\DefEquation
{
\begin{split}
&\,a_1\otimes...\otimes(a_i+b_i)\otimes...\otimes a_n
\\
=&\,a_1\otimes...\otimes a_i\otimes...\otimes a_n+
a_1\otimes...\otimes b_i\otimes...\otimes a_n
\\
&\,a_i, b_i\in A_i
\end{split}
}
{tensors 1, tensor product}

\DefEquation
{
\begin{split}
&a_1\otimes...\otimes(ca_i)\otimes...\otimes a_n=
c(a_1\otimes...\otimes a_i\otimes...\otimes a_n)
\\
&a_i\in A_i\ \ \ c\in D
\end{split}
}
{tensors 2, tensor product}

\AddEq [4]{f: A->B}
{
#1:#2\rightarrow #3#4
}

\AddEq [4]{vf: A->B}
{
$\Vector{#1}:#2\rightarrow #3$#4
}

\AddEq [5]{f:a in A->b in B}
{
\[#1:#2\in #3\rightarrow #4\in #5\]
}

\DefEquation
{
f:A^n\rightarrow A,
a=f\circ(a_1,...,a_n)
}
{polylinear map, algebra}

\DefEquation
{
a=f\pC{s}{0}^n\ \sigma_s(I_{(s\cdot 1)}\circ a_1)
\ f\pC{s}{1}^n\ ...\ \sigma_s(I_{(s\cdot n)}\circ a_n)\ f\pC{s}{n}^n
}
{polylinear map, algebra, canonical morphism}

\DefEq
{
$\{a_1,...,a_n\}$
\[
\sigma_s=
\begin{pmatrix}
a_1&...&a_n
\\
\sigma_s(a_1)&...&\sigma_s(a_n)
\end{pmatrix}
\]
}
{transposition of set of variables, algebra}

\DefEq
{
$I_{(s\cdot 1)}$, ..., $I_{(s\cdot n)}\in\mathcal L(D;A\rightarrow A)$
}
{I1n in L(A;A)}

\DefEq
{
\labelItem{monomial of power 0}
$p_0(x)=a_0$, $a_0\in A$.
}
{p0(x)=a0}

\AddEq{monomial of power k}
{
\labelItem{monomial of power k}
\[
p_k(x)=p_{k-1}(x)(F\circ x)a_k
\]
}

\AddEq{p1(x)=aFxa}
{
$p_1(x)=a_0(F\circ x)a_1$.
}

\AddEq{Basis F=...}
{
$\Basis F=(F_1,...,F_n)$.
}

\AddEq{Fi=Fj}
{
$F_{(i)}=F_{(j)}$
}

\AddEq{F=...}
{
$F=(F_{(1)},...,F_{(k)})$
}

\AddEq[1]{set of homogeneous polynomials}
{
\symb{A_{#1}[x]}{set of homogeneous polynomials}1
}

\DefEq
{
$a\in A^{\otimes (n+1)}$\Pt
}
{a in Aoxn+1}

\DefEq
{
$x_1=...=x_n=x$,
}
{x1=xn=x}

\DefEq
{
\[
a\circ F\circ x^n=a\circ(F_{(1)},...,F_{(n)})\circ(x_1\otimes...\otimes x_n)
\]
}
{a xn=}

\AddEq{F1n in F}
{
$F_{(1)}$, ..., $F_{(n)}\in\Basis F$.
}

\AddEq{F[k]=...}
{
\[
F_{[k]}=(F_{[k](1)},...,F_{[k](n)})
\]
}

\DefEq
{
\[
a=a_{i\cdot 0}\otimes a_{i\cdot 1}\otimes...\otimes a_{i\cdot n}
\ \ \ i\in I
\]
}
{a=oxi}

\DefEq
{
$\sigma=\{\sigma_i\in S(n):i\in I\}$
}
{si in Sn}

\DefEq
{
\[
(a,\sigma):A^{\times n}\rightarrow A
\]
}
{ox:An->A}

\DefEq
{
\begin{align*}
(a,\sigma)\circ (b_1,...,b_n)&=
(a_{i\cdot 0}\otimes a_{i\cdot 1}\otimes...\otimes a_{i\cdot n},\sigma_i)\circ (b_1,...,b_n)
\\&=
a_{i\cdot 0}\sigma_i(b_1)a_{i\cdot 1}...\sigma_i(b_n)a_{i\cdot n}
\end{align*}
}
{ox circ =}

\AddEq{p(x)=a circ xk}
{
\[
\begin{matrix}
p(x)=a_{[s]}\circ F_{[s]}\circ x^k
&a_{[s]}\in A^{\otimes(k+1)}
\end{matrix}
\]
}

\DefEq
{
\symb{A[x]}{algebra of polynomials over algebra}{}
\[
\ShowSymbol{algebra of polynomials over algebra}{}
=\bigoplus_{n=0}^{\infty}A_n[x]
\]
}
{algebra of polynomials over algebra}

\AddEq[3]{a1n}
{
$#1_1$, ..., $#1_{#2}$#3
}

\AddEq[3]{A1n}
{
$#1^1$, ..., $#1^{#2}$#3
}

\AddEq[3]{aU A1n}
{
$\aU{#1}1$, ..., $\aU{#1}{#2}$#3
}

\DefEq
{
$a_0\in U$.
}
{a0 in U}

\DefEq
{
\[
f:U\rightarrow \mathcal L(D;A^p\rightarrow B)
\]
}
{U->L(Ap,B)}

\DefEquation
{
\begin{array}{r@{\ }l}
&((a_0,...,a_n,\sigma)\circ(f_1,...,f_n))\circ(x_1,...,x_n)
\\=&
(a_0\sigma(f_1)a_1...a_{n-1}\sigma(f_n)a_n)\circ(x_1,...,x_n)
\\=&
a_0\sigma(f_1\circ x_1)a_1...a_{n-1}\sigma(f_n\circ x_n)a_n
\end{array}
}
{n linear map A LA}

\AddEq[3]{set polylinear maps An}
{
\symb{\mathcal L(#1;#2^n\rightarrow #3)}{set polylinear maps An}1
}

\DefEquation
{
\begin{array}{r@{\,}l@{\ \ \ }r@{\,}l@{\ \ \ }r@{\,}l}
a_k&=a_{k\cdot 0}\underline{\otimes}(1\otimes a_{k\cdot 1})
&a_{k\cdot 0}&\in A^{\otimes k}&a_{k\cdot 1}&\in A
\end{array}
}
{p(x)=a k-1 k 3}

\AddEq [2]{M M1 Mn}
{
\[#1=\max(#1_1,...,#1_{#2})\]
}

\AddEq [2]{M max M1 Mn}
{
\[#1=\max(\aD{#1}1,...,\aD{#1}{#2})\]
}

\DefEq
{
\[N=\max(N_1,N_2)\]
}
{N N1 N2}

\DefEq
{
f_i(x)=\lim_{m\rightarrow\infty}f_{i\cdot m}(x)
}
{fi(x)=lim}

\DefEq
{
\delta_1\in R,\ \delta_1>0
}
{delta1 in R}

\DefEq
{
\(m>M_i\)
}
{m>Mi}

\DefEq
{
\[h_m=f_{1\cdot m}...f_{n\cdot m}\omega\]
}
{hm=f1m...fnm omega}

\DefEq
{
\[
\epsilon_1(\delta)<\epsilon
\]
}
{e(d)<e}

\DefEq
{
\[\delta_1=0\Rightarrow\epsilon_1=0\]
}
{d1=0=>e1=0}

\DefEq
{
F_i\ge 0
}
{F>0}

\DefEq
{
F_i=\sup\|f_i(x)\|
}
{F=sup|f|}

\AddEq[3]{a in AA}
{
$#1\in #2\otimes #2$#3
}


==> Prolog.Parm.tex <==
%auto-ignore

\newcommand\Multiply[2]{#1#2}

\AddEq{=DA1DA2}
{
\def\DFDT{D1 D2 }%
\def\MF{r1:D1->D2 }%
\def\DF{1}%
\def\DT{2}%
\def\VF{1}%
\def\VT{2}%
\def\MapE{hgf}%
}

\AddEq{=D1D2}
{
\def\DFDT{D1 D2 }%
\def\MF{r1:D1->D2 }%
\def\DF{1}%
\def\DT{2}%
\def\VF{1}%
\def\VT{2}%
\def\MapE{hf}%
}

\AddEq{=DD}
{
\def\DFDT{D }%
\def\MF{}%
\def\DF{}%
\def\DT{}%
\def\VF{1}%
\def\VT{2}%
\def\MapE{f}%
}

\AddEq{def universal}
{
\def\Cols{*}%
\def\Rows{*}%
\renewcommand\ARow[2]{\ensuremath{##1(\gi{##2})}}%
\renewcommand\ACol[2]{\ensuremath{##1(\gi{##2})}}%
\renewcommand\EBase[2]{\ensuremath{##1(\gi{##2})}}%
\def\Product{*}%
\def\ProductA{}%
\def\ProductS{}%
\def\ProductType{}%
\def\ProductTypeA{}%
\def\GL{\RCGL}%
\def\Group{GL}%
\def\ProductVal{}%
}

\AddEq{def opRow}
{%
\def\Product{*Row}%
\def\ProductA{}%
\def\ProductS{}%
\def\ProductType{}%
\def\ProductTypeA{}%
\def\GL{\RCGL}%
\def\Group{GL}%
\def\ProductVal{}%
}

\AddEq{def opCol}
{%
\def\Product{*Col}%
\def\ProductA{}%
\def\ProductS{}%
\def\ProductType{}%
\def\ProductTypeA{}%
\def\GL{\RCGL}%
\def\Group{GL}%
\def\ProductVal{}%
}

\AddEq{def rc}
{%
\def\Product{rc}%
\def\ProductA{cr}%
\def\ProductS{rc }%
\def\ProductType{\RC}%
\def\ProductTypeA{\CR}%
\def\GL{\RCGL}%
\def\Group{\RCGL}%
\def\ProductVal{\RCstar}%
\def\ProductAVal{\CRstar}%
\def\PowerVal{\RCPower}%
\def\PowerAVal{\CRPower}%
\def\InverseVal{\RCInverse}%
\def\InverseAVal{\CRInverse}%
\def\DetVal{\RCDet}%
\def\detVal{\RCdet}%
\def\RankVal{\RCRank}%
}

\AddEq{def cr}
{%
\def\Product{cr}%
\def\ProductA{rc}%
\def\ProductS{cr }%
\def\ProductType{\CR}%
\def\ProductTypeA{\RC}%
\def\GL{\CRGL}%
\def\Group{\CRGL}%
\def\ProductVal{\CRstar}%
\def\ProductAVal{\RCstar}%
\def\PowerVal{\CRPower}%
\def\PowerAVal{\RCPower}%
\def\InverseVal{\CRInverse}%
\def\InverseAVal{\RCInverse}%
\def\DetVal{\CRDet}%
\def\detVal{\CRdet}%
\def\RankVal{\CRRank}%
}

\AddEq{def DModule}
{
\def\AArg{d}%
\def\DTransf{g_1}%
\def\DArg{n}%
\def\Base{D}%
\def\BaseExt{(1)}%
\def\CBase{Z}%
\def\BaseRings{of ring of rational integers $Z$ and commutative ring $D$ }
\def\SidePresentation{}
\def\Algebra{commutative ring}%
\def\ShortAlgebraWS{ring }%
\def\DivAlgebra{field}%
\def\SetRepresentation{Abelian group }%
\def\VectorSet{module }%
\def\VectorSetNS{module}%
\def\VectorsSet{modules }%
\def\VectorsSetNS{modules}%
\def\Division{}%
\def\Module{V}%
\def\ModuleA{W}%
\def\ANumber{d}%
\def\VNumber{a}%
\def\VNumberA{b}%
\def\algebraa{ring }%
\def\Free{free }
%
\ifx\UseRussian\Defined%
\def\To{}%
\def\TO{вых }%
\def\ToV{вое }%
\def\Algebra{ассоциативная $D$\Hyph алгебра}%
\def\algebraa{$D$\Hyph алгебре }%
\def\algebrac{$D$\Hyph алгебра }%
\def\algebrad{$D$\Hyph алгебру }%
\def\algebraD{$D$\Hyph алгебра }%
\def\BaseRings{кольца целых чисел $Z$ и коммутативного кольца $D$ }
\def\From{}%
\def\VectorSetRuA{модуль }%
\def\VectorSetRuANS{модуль}%
\def\VectorSetRuB{модуля }%
\def\VectorSetRuD{модуле }%
\def\VectorSetRuE{модулем }%
\def\VectorsSetRuA{модули }%
\def\VectorSetRuENS{модулем}%
\def\VectorsSetRuB{модулей }%
\def\VectorsSetRuBNS{модулей}%
\def\AlgebraRu{кольцо }%
\def\AlgebraRuNS{коммутативное кольцо}%
\def\ShortAlgebraRuBWS{кольца }%
\def\ShortAlgebraRuCWS{кольцом }%
\def\ShortAlgebraRuDWS{кольце }%
\def\ShortAlgebraRuEWS{кольцо }%
\def\SidePresentationRuWS{}%
\def\SidePresentationRuBWS{}%
\def\SetRepresentationRuA{абелевая группа }%
\def\SetRepresentationRu{абелевой группе }%
\def\DivisionRu{ }%
\def\DivisionRuNS{}%
\def\DivAlgebraRu{поле}%
\def\SideModuleC{}%
\def\FreeRuB{свободного }
\fi
}

\AddEq{def DAlgebra}
{
\def\AArg{d}%
\def\DTransf{g_1}%
\def\DArg{n}%
\def\Base{D}%
\def\BaseExt{(1)}%
\def\CBase{Z}%
\def\BaseRings{of ring of rational integers $Z$ and commutative ring $D$ }
\def\SidePresentation{}
\def\Algebra{commutative ring}%
\def\ShortAlgebraWS{ring }%
\def\DivAlgebra{field}%
\def\SetRepresentation{Abelian group }%
\def\VectorSet{algebra }%
\def\VectorSetNS{algebra}%
\def\VectorsSet{algebras }%
\def\VectorsSetNS{algebras}%
\def\Division{}%
\def\Module{V}%
\def\ModuleA{W}%
\def\ANumber{d}%
\def\VNumber{a}%
\def\VNumberA{b}%
\def\algebraa{ring }%
\def\Free{free }
%
\ifx\UseRussian\Defined%
\def\To{}%
\def\TO{вых }%
\def\ToV{вое }%
\def\Algebra{ассоциативная $D$\Hyph алгебра}%
\def\algebraa{$D$\Hyph алгебре }%
\def\algebrac{$D$\Hyph алгебра }%
\def\algebrad{$D$\Hyph алгебру }%
\def\algebraD{$D$\Hyph алгебра }%
\def\BaseRings{кольца целых чисел $Z$ и коммутативного кольца $D$ }
\def\From{}%
\def\VectorSetRuA{алгебра }%
\def\VectorSetRuANS{алгебра}%
\def\VectorSetRuB{алгебры }%
\def\VectorSetRuD{алгебре }%
\def\VectorSetRuE{алгеброй }%
\def\VectorsSetRuA{модули }%
\def\VectorSetRuENS{модулем}%
\def\VectorsSetRuB{модулей }%
\def\VectorsSetRuBNS{модулей}%
\def\AlgebraRu{кольцо }%
\def\AlgebraRuNS{коммутативное кольцо}%
\def\ShortAlgebraRuBWS{кольца }%
\def\ShortAlgebraRuCWS{кольцом }%
\def\ShortAlgebraRuDWS{кольце }%
\def\ShortAlgebraRuEWS{кольцо }%
\def\SidePresentationRuWS{}%
\def\SidePresentationRuBWS{}%
\def\SetRepresentationRuA{абелевая группа }%
\def\SetRepresentationRu{абелевой группе }%
\def\DivisionRu{ }%
\def\DivisionRuNS{}%
\def\DivAlgebraRu{поле}%
\def\SideModuleC{}%
\def\FreeRuB{свободного }
\fi
}

\AddEq{def DVector}
{
\def\AArg{d}%
\def\DTransf{g_1}%
\def\DArg{n}%
\def\Base{D}%
\def\BaseExt{}%
\def\CBase{}%
\def\BaseRings{of ring of rational integers $Z$ and commutative ring $D$ }
\def\SidePresentation{}
\def\Algebra{field}%
\def\ShortAlgebraWS{field }%
\def\DivAlgebra{field}%
\def\SetRepresentation{Abelian group }%
\def\VectorSet{vector space }%
\def\VectorSetNS{vector space}%
\def\VectorsSet{vector spaces }%
\def\VectorsSetNS{vector spaces}%
\def\Division{}%
\def\Module{V}%
\def\ModuleA{W}%
\def\ANumber{d}%
\def\VNumber{v}%
\def\VNumberA{w}%
\def\algebraa{field }%
\def\Free{}
%
\ifx\UseRussian\Defined%
\def\To{}%
\def\TO{}%
\def\ToV{}%
\def\What{}%
\def\WhatA{ый }%
\def\WhatO{}%
\def\Algebra{кольцо}%
\def\algebraa{кольце }%
\def\algebrac{кольцо }%
\def\algebrad{кольцо }%
\def\algebraD{Кольцо }%
\def\Algebrab{модуль}%
\def\BaseRings{кольца целых чисел $Z$ и коммутативного кольца $D$ }
\def\From{}%
\def\VectorSetRuA{векторное пространство }%
\def\VectorSetRuANS{векторное пространство}%
\def\VectorSetRuB{векторного пространства }%
\def\VectorSetRuD{векторном пространстве }%
\def\VectorSetRuE{векторным пространством }%
\def\VectorSetRuENS{векторным пространством}%
\def\VectorsSetRuA{векторные пространства }%
\def\VectorsSetRuB{векторных пространств }%
\def\VectorsSetRuBNS{векторных пространств}%
\def\AlgebraRu{поле }%
\def\AlgebraRuNS{поле}%
\def\ShortAlgebraRuBWS{поля }%
\def\ShortAlgebraRuCWS{полем }%
\def\ShortAlgebraRuDWS{поле }%
\def\ShortAlgebraRuEWS{поле }%
\def\SidePresentationRuWS{}%
\def\SidePresentationRuBWS{}%
\def\SetRepresentationRuA{абелевая группа }%
\def\SetRepresentationRu{абелевой группе }%
\def\DivisionRu{ }%
\def\DivisionRuNS{}%
\def\DivAlgebraRu{поле}%
\def\SideModuleC{}%
\def\FreeRuB{}
\fi
}

\AddEq{def AModule}
{
\def\AArg{a}%
\def\DTransf{g_{1,4}}%
\def\DArg{d}%
\def\Base{A}%
\def\BaseExt{(1)}%
\def\CBase{D}%
\def\BaseRings{of commutative ring $D$ and $D$\Hyph algebra $A$ }
\def\SidePresentation{\Hyph side }
\def\Algebra{associative $D$\Hyph algebra}%
\def\ShortAlgebraWS{$D$\Hyph algebra }%
\def\DivAlgebra{associative division $D$\Hyph algebra}%
\def\SetRepresentation{$D$\Hyph module }%
\def\VectorSet{module }%
\def\VectorSetNS{module}%
\def\VectorsSet{modules }%
\def\VectorsSetNS{modules}%
\def\Division{}%
\def\Module{A}%
\def\ModuleA{B}%
\def\ANumber{a}%
\def\VNumber{v}%
\def\VNumberA{w}%
\def\algebraa{$D$\Hyph algebra }%
\def\Free{free }
%
\ifx\UseRussian\Defined%
\def\To{вый }%
\def\TO{вых }%
\def\ToV{вое }%
\def\Algebra{ассоциативная $D$\Hyph алгебра}%
\def\algebraa{$D$\Hyph алгебре }%
\def\algebrac{$D$\Hyph алгебра }%
\def\algebrad{$D$\Hyph алгебру }%
\def\algebraD{$D$\Hyph алгебра }%
\def\BaseRings{коммутативного кольца $D$ и $D$\Hyph алгебры $A$ }
\def\From{вого }%
\def\VectorSetRuA{модуль }%
\def\VectorSetRuANS{модуль}%
\def\VectorSetRuB{модуля }%
\def\VectorSetRuD{модуле }%
\def\VectorSetRuE{модулем }%
\def\VectorSetRuENS{модулем}%
\def\VectorsSetRuA{модули }%
\def\VectorsSetRuB{модулей }%
\def\VectorsSetRuBNS{модулей}%
\def\AlgebraRu{ассоциативная $D$\Hyph алгебра }%
\def\AlgebraRuNS{ассоциативная $D$\Hyph алгебра}%
\def\ShortAlgebraRuBWS{$D$\Hyph алгебры }%
\def\ShortAlgebraRuCWS{$D$\Hyph алгеброй }%
\def\ShortAlgebraRuDWS{$D$\Hyph алгебре }%
\def\ShortAlgebraRuEWS{$D$\Hyph алгебру }%
\def\SidePresentationRuWS{востороннее }%
\def\SidePresentationRuBWS{восторонним }%
\def\SetRepresentationRuA{$D$\Hyph модуль }%
\def\SetRepresentationRu{$D$\Hyph модуле }%
\def\DivisionRu{ }%
\def\DivisionRuNS{}%
\def\DivAlgebraRu{ассоциативная $D$\Hyph алгебра с делением}%
\def\SideModuleC{вым }%
\def\FreeRuB{свободного }
\fi
}

\AddEq{def AVector}
{
\def\AArg{a}%
\def\DTransf{g_{1,4}}%
\def\DArg{d}%
\def\Base{A}%
\def\BaseExt{}%
\def\CBase{D}%
\def\BaseRings{of commutative ring $D$ and $D$\Hyph algebra $A$ }
\def\SidePresentation{\Hyph side }
\def\Algebra{associative division $D$\Hyph algebra}%
\def\ShortAlgebraWS{$D$\Hyph algebra }%
\def\DivAlgebra{associative division $D$\Hyph algebra}%
\def\SetRepresentation{$D$\Hyph vector space }%
\def\VectorSet{vector space }%
\def\VectorSetNS{vector space}%
\def\VectorsSet{vector spaces }%
\def\VectorsSetNS{vector spaces}%
\def\Division{division }%
\def\Module{V}%
\def\ModuleA{W}%
\def\ANumber{a}%
\def\VNumber{v}%
\def\VNumberA{w}%
\def\algebraa{$D$\Hyph algebra }%
\def\Free{}
%
\ifx\UseRussian\Defined%
\def\To{вое }%
\def\TO{}%
\def\ToV{}%
\def\What{}%
\def\WhatA{вый }%
\def\WhatO{вое }%
\def\Algebra{кольцо}%
\def\algebraa{кольце }%
\def\algebrac{кольцо }%
\def\algebrad{кольцо }%
\def\algebraD{Кольцо }%
\def\Algebrab{модуль}%
\def\BaseRings{коммутативного кольца $D$ и $D$\Hyph алгебры $A$ }
\def\From{вого }%
\def\VectorSetRuA{векторное пространство }%
\def\VectorSetRuANS{векторное пространство}%
\def\VectorSetRuD{векторном пространстве }%
\def\VectorSetRuB{векторного пространства }%
\def\VectorSetRuE{векторным пространством }%
\def\VectorSetRuENS{векторным пространством}%
\def\VectorsSetRuA{векторные пространства }%
\def\VectorsSetRuB{векторных пространств }%
\def\VectorsSetRuBNS{векторных пространств}%
\def\AlgebraRu{ассоциативная $D$\Hyph алгебра }%
\def\AlgebraRuNS{ассоциативная $D$\Hyph алгебра}%
\def\ShortAlgebraRuBWS{$D$\Hyph алгебры }%
\def\ShortAlgebraRuCWS{$D$\Hyph алгеброй }%
\def\ShortAlgebraRuDWS{$D$\Hyph алгебре }%
\def\ShortAlgebraRuEWS{$D$\Hyph алгебру }%
\def\SidePresentationRuWS{востороннее }%
\def\SidePresentationRuBWS{восторонним }%
\def\SetRepresentationRuA{$D$\Hyph векторное пространство }%
\def\SetRepresentationRu{$D$\Hyph векторном пространстве }%
\def\DivisionRu{ с делением }%
\def\DivisionRuNS{ с делением}%
\def\DivAlgebraRu{ассоциативная $D$\Hyph алгебра с делением}%
\def\SideModuleC{вым }%
\def\FreeRuB{}
\fi
}

\AddEq{def left}
{%
\def\SideNS{left}%
\def\SideWS{left }%
\def\SideWSC{Left }%
\def\DefRow{rc-rows}%
\def\DefCol{cr-cols}%
\def\HSide{\Hyph side }%
\def\ATransf{g_{3,4}}%
\def\OtherSideWS{right }%
\def\OtherSideNS{right}%
\def\RefDistributive##1{(b1+b2).##1.a=}%
\renewcommand\Multiply[2]{##1##2}%
\ifx\UseRussian\Defined%
\def\HSide{востороннее }%
\def\SideRu{ле}%
\def\OtherSideRu{пра}%
\def\SideRuC{Ле}%
\def\What{вым }%
\def\WhatTo{вом }%
\def\Which{вого }%
\fi%
}

\AddEq{def right}
{%
\def\SideNS{right}%
\def\SideWS{right }%
\def\SideWSC{Right }%
\def\DefRow{cr-rows}%
\def\DefCol{rc-cols}%
\def\HSide{\Hyph side }%
\def\ATransf{g_{3,4}}%
\def\OtherSideWS{left }%
\def\OtherSideNS{left}%
\def\RefDistributive##1{a.##1.(b1+b2)=}%
\renewcommand\Multiply[2]{##2##1}
\ifx\UseRussian\Defined%
\def\HSide{востороннее }%
\def\SideRu{пра}%
\def\OtherSideRu{ле}%
\def\SideRuC{Пра}%
\def\What{вым }%
\def\WhatTo{вом }%
\def\Which{вого }%
\fi%
}

\AddEq{def ab=ba}
{
\def\SideNS{}%
\def\SideWS{}%
\def\DefRow{-rows}%
\def\DefCol{-cols}%
\def\HSide{}%
\def\ATransf{g_2}%
\ifx\UseRussian\Defined%
\def\SideRu{}%
\def\SideRuC{}%
\def\What{}%
\def\WhatTo{}%
\def\Which{}%
\fi%
}

\AddEq{=Omega}
{
\def\Base{\Omega}%
\def\Algebrab{group}%
\def\Algebrac{Omega group}%
\def\Module{A}%
\ifx\UseRussian\Defined%
\def\WhatA{ая }%
\def\Algebrab{группа}%
\fi%
}

\DefEq%
{%
\def\Pt{.}%
}%
{=.}%

\DefEq%
{%
\def\Pt{;}%
}%
{=.c}%

\DefEq%
{%
\def\Pt{,}%
}%
{=c}%

\DefEq%
{%
\def\Pt{}%
}%
{=z}%

\AddEq{D= F= A=}
{
\def\PD{}%
\def\PF{}%
\def\PA{}%
}

\DefEq
{
\def\PX{X}
}
{X}

\AddEq{f=f}
{%
\def\Pf{f}%
}%

\AddEq{f=g}
{%
\def\Pf{g}%
}%

\DefEq%
{%
\def\Pf{m}%
}%
{f=m}%

\DefEq
{
\def\Pf{I}%
}
{f=I}

\DefEq
{
\def\pD{D}%
\def\pA{A}%
\def\pB{A}%
}
{A=A}

\DefEq%
{%
\def\pD{D}%
\def\pA{A}%
\def\pB{B}%
}%
{A=AB}

\DefEq
{
\def\pD{D}%
\def\pA{B}%
\def\pB{C}%
}
{A=BC}

\DefEq%
{%
\def\pD{R}%
\def\pA{C}%
\def\pB{C}%
}%
{A=C}%

\DefEq%
{%
\def\pD{C}%
\def\pA{C}%
\def\pB{C}%
}%
{A=CC}%

\DefEq
{
\def\pD{D}%
\def\pA{A_1}%
\def\pB{A_2}%
}
{A=12}

\DefEq
{
\def\pD{D}%
\def\pA{A_2}%
\def\pB{A_2}%
}
{A=2}

\DefEq
{
\def\pD{D}%
\def\pA{A_1\rightarrow A_2}%
\def\pB{A_3}%
}
{A=123}

\DefEq
{
\def\pD{D}%
\def\pA{A_1}%
\def\pB{A_3}%
}
{A=13}

\DefEq
{
\def\pD{D}%
\def\pA{A}%
\def\pB{C}%
}
{A=AC}

\DefEq
{%
\def\Pn{0}%
}%
{n=0}

\DefEq
{%
\def\Pn{n}%
}%
{n=n}

\DefEq
{%
\def\Pn{k}%
}%
{n=k}

\DefEq
{%
\def\Pn{1}%
\def\Pp{p}%
}%
{n=1}

\DefEq
{%
\def\Pn{2}%
\def\Pp{q}%
}%
{n=2}

\DefEq
{%
\def\Pn{3}%
\def\Pp{r}%
}%
{n=3}

\DefEq
{%
\def\tM{1}%
}%
{m=1}

\DefEq
{%
\def\tM{2}%
}%
{m=2}


==> Prolog.Ref.tex <==
%auto-ignore

%определить источник для ссылок
\ifx\UseRussian\Defined
\def\TheoremFollows{Теорема является следствием теоремы }
\else
\def\TheoremFollows{The theorem follows from the theorem }
\fi

\ePrints{4975-6381,9835-2163,0767-8264,7287-9339,9856-6693,5284-0163}%,8428-0408}%
\ifx\Semafor\ValueOn%
\def\RefLinearMapA{4993-2400}%
\xRefDef{4993-2400}
%%\ePrints{8428-0408}%
%%\ifx\Semafor\ValueOff%
\def\RefLinearMap{5114-6019}%	
\xRefDef{5114-6019}
%%\fi
\fi
\ePrints{1601.03259,1506.00061}%
\Items{309618526,CACAA.06.121,1801.01628,CACAA.07,2207.06506,2021.11.26,2112.00613}%
\ifx\Semafor\ValueOn%
\def\RefLinearMap{1502.04063}%
\xRefDef{1502.04063}
\ePrints{2207.06506,1601.03259,2021.11.26,2112.00613,1506.00061}%
\ifx\Semafor\ValueOff%
\def\RefLinearMapA{0701.238}%
\xRefDef{0701.238}
\fi
\fi
\ePrints{348311191}%
\ifx\Semafor\ValueOn%
\def\RefLinearMap{2021.01.06}%
\xRefDef{2021.01.06}
\fi
\ePrints{1211.6965}%
\ifx\Semafor\ValueOn%
\def\RefLinearMap{1003.1544}%
\def\RefLinearMapA{0701.238}%
\xRefDef{1003.1544}
\xRefDef{0701.238}
\fi
\ePrints{MAlgebra4,MAlgebra2,MObject,2022.11.26,2023.01.07,357606033}%
\ifx\Semafor\ValueOn%
\def\RefLinearMap{2207.06506}%
\def\RefLinearMapA{2207.06506}%
\def\SectionTitle{}
\def\ProductType{}
\def\ColN{}
\ShowEq{def right}
\xRefDef{2207.06506}
\fi
\ePrints{5148-4632}%
\ifx\Semafor\ValueOn%
\def\RefLinearMap{8428-0408}%
\def\RefLinearMapA{8428-0408}%
\def\SectionTitle{}
\def\ProductType{}
\def\ColN{}
\ShowEq{def right}
\xRefDef{8428-0408}
\fi
%\ePrints{}%
%\ifx\Semafor\ValueOn%
%\def\RefLinearMap{MAlgebra2}%
%\xRefDef{MAlgebra2}
%\fi

\ePrints{330532713,1801.01628,2021.11.26,2112.00613}
\ifx\Semafor\ValueOn
\def\RefQuadratic{1506.00061}%
\xRefDef{1506.00061}
\fi%
\ePrints{0921-2370,0767-8264,5284-0163}
\ifx\Semafor\ValueOn
\def\RefQuadratic{7287-9339}%
\xRefDef{7287-9339}
\fi

\ePrints{330532713,2207.06506,2204.06320,2022.01.05,348311191}
\Items{2023.01.07}%
\ifx\Semafor\ValueOn
\def\PartA{}
\def\PartB{}
\def\SideRu{}
\ShowEq{def left}
\def\RefDiffEq{1801.01628}%
\xRefDef{1801.01628}
\fi
\ePrints{8428-0408}
\ifx\Semafor\ValueOn
\def\RefDiffEq{0767-8264}%
\xRefDef{0767-8264}
\fi

\ePrints{309618526,1801.01628,322019412,323236904,CACAA.07,330532713,323966352,2207.06506}
\Items{2021.01.06}
\ifx\Semafor\ValueOn
\def\RefCalculus{1601.03259}%
\xRefDef{1601.03259}
\fi%
\ePrints{9835-2163,0767-8264,9856-6693,7287-9339,0921-2370,8428-0408,5284-0163}
\ifx\Semafor\ValueOn
\def\RefCalculus{4975-6381}%
\xRefDef{4975-6381}
\fi

\ePrints{2020.06.01}%1801.01628,
\ifx\Semafor\ValueOn
\def\RefCountable{1211.6965}%
\xRefDef{1211.6965}
\fi
%\ePrints{5284-0163}
%\ifx\Semafor\ValueOn
%\def\RefCountable{4910-5816}%
%\xRefDef{4910-5816}
%\fi

\ePrints{1908.04418,323966352,324329551,0921-2370}
\ifx\Semafor\ValueOn
\def\RefGravity{0803.3276}%
\xRefDef{0803.3276}
\fi%
\ePrints{6860-2955}
\ifx\Semafor\ValueOn
\def\RefGravity{0803.3276}%
\xRefDef{0803.3276}
\fi

\AddEq{SetupRefRepresentation}
{
\def\RefRepresentation{}%
\ePrints{5114-6019,1502.04063,1305.4547}
\ifx\Semafor\ValueOn
\def\RefRepresentation{0912.3315}%
\xRefDef{0912.3315}
\fi
\ePrints{0767-8264}%1801.01628,
\ifx\Semafor\ValueOn
\def\RefRepresentation{6860-2955}%
\xRefDef{6860-2955}
\fi
\ePrints{MAlgebra2,2204.06320,2022.01.05,357606033}%,2021.01.06}
\ifx\Semafor\ValueOn
\def\RefRepresentation{1908.04418}%
\xRefDef{1908.04418}
\fi
}

\AddEq{SetupRefPolymorphism}
{
\def\RefPolymorphism{}%
\ePrints{1801.01628,CACAA.07}%
\ifx\Semafor\ValueOn
\def\RefPolymorphism{1502.04063}%
%xRefDef is defined as RefLinearMap
\fi
\ePrints{MAlgebra2,323236904}%
\ifx\Semafor\ValueOn
\def\RefPolymorphism{1502.04063}%
\xRefDef{1502.04063}
\fi
\ePrints{9856-6693}%
\ifx\Semafor\ValueOn
\def\RefPolymorphism{5114-6019}%
%xRefDef is defined as RefLinearMap
\fi
}

\AddEq{SetupRefOmegaNorm}
{
\def\RefTheoremOmegaNorm{}%
\ePrints{1102.5168,1502.04063}%
\ifx\Semafor\ValueOn%
\def\RefTheoremOmegaNorm{1305.4547}
\xRefDef{1305.4547}
\fi
\ePrints{CACAA.06.121}%
\ifx\Semafor\ValueOn%
\def\RefTheoremOmegaNorm{CACAA.04.001}
\xRefDef{CACAA.04.001}
\fi
}

\AddEq{SetupRefMeasure}
{
\def\RefMeasure{}%
\ePrints{9856-6693}
\ifx\Semafor\ValueOn
\def\RefMeasure{5410-9916}
\xRefDef{5410-9916}
\fi
\ePrints{323236904}%,1801.01628
\ifx\Semafor\ValueOn
\def\RefMeasure{1310.5591}
\xRefDef{1310.5591}
\fi
}

\AddEq{SetupRef}
{
\ShowEq{SetupRefRepresentation}
\ShowEq{SetupRefOmegaNorm}
\ShowEq{SetupRefMeasure}
\ShowEq{SetupRefPolymorphism}
}

\AddEq{PreliminaryRefOn}
{
\ePrints{1506.00061,1601.03259}%
\ifx\Semafor\ValueOn%
\def\RefRepresentation{1502.04063}%
%\xRefDef{1502.04063}
\fi
\ePrints{1801.01628,2207.06506}
\ifx\Semafor\ValueOn
\def\RefRepresentation{1908.04418}%
\xRefDef{1908.04418}
\fi
\ePrints{5148-4632,8428-0408,5284-0163}
\ifx\Semafor\ValueOn
\def\RefRepresentation{6860-2955}%
\xRefDef{6860-2955}
\fi
\ePrints{4975-6381}
\ifx\Semafor\ValueOn
\def\RefRepresentation{5114-6019}%
%xRefDef defined as \RefLinearMap
\fi

\ePrints{9835-2163,9856-6693,0767-8264,5284-0163}%
\ifx\Semafor\ValueOn%
\def\RefPolymorphism{5114-6019}%
%xRefDef is defined as RefLinearMap
\fi

\ShowEq{PreliminaryRefOmegaNormOn}
\ShowEq{PreliminaryRefMeasureOn}
}

\AddEq{PreliminaryRefOmegaNormOn}
{
\ePrints{5410-9916,4975-6381}%
\ifx\Semafor\ValueOn%
\def\RefTheoremOmegaNorm{5059-9176}%
\xRefDef{5059-9176}%
\fi
}

\AddEq{PreliminaryRefOmegaNormOff}
{
\def\RefTheoremOmegaNorm{}%
}

\AddEq{PreliminaryRefMeasureOff}
{
\def\RefMeasure{}%
}

\AddEq{PreliminaryRefMeasureOn}
{
\ePrints{1601.03259,309618526}
\ifx\Semafor\ValueOn
\def\RefMeasure{1310.5591}
\xRefDef{1310.5591}
\fi
\ePrints{4975-6381}
\ifx\Semafor\ValueOn
\def\RefMeasure{5410-9916}
\xRefDef{5410-9916}
\fi
\ePrints{CACAA.06.121}%
\ifx\Semafor\ValueOn%
\def\RefMeasure{CACAA.04.001}
%xRefDef is defined as RefTheoremOmegaNorm
\fi
}

\AddEq{PreliminaryRefOff}
{
\def\RefRepresentation{}%
\def\RefPolymorphism{}%
\ShowEq{PreliminaryRefOmegaNormOff}%
\ShowEq{PreliminaryRefMeasureOff}%
}

\ShowEq{SetupRef}%

\newcommand\ProofTheorem[2]
{
\begin{proof}
\TheoremFollows
\RefTheorem[#1]{#2}.
\end{proof}
}%

\newcommand\proofTheorem[3]
{
\begin{proof}
\TheoremFollows
\refTheorem[#1]{#2}{#3}.
\end{proof}
}%

% конец определения источник для ссылок

\AddEq[1]{ref definition product rc}
{
\RefDefinition{row over column product}#1
}

\AddEq[1]{ref definition product cr}
{
\RefDefinition{column over row product}#1
}

\DefEq
{
\ePrints{1601.03259,4975-6381}%
\ifx\Semafor\ValueOff%
\EqRef[\RefCalculus]{derivative of Order n, algebra},
\else%
\EqRef{derivative of Order n, algebra},
\fi%
}
{ref derivative of Order n, algebra}

\AddEq{ref product in category}
{
\ePrints{8428-0408,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\RefDefinition{product in category, 2020},
\else
\RefDefinition{product in category},
\fi
}

\AddEq[1]{ref definition: left-side representation of algebra}
{
\ePrints{1310.5591,5059-9176,1305.4547}%
\ifx\Semafor\ValueOff%
\ePrints{5410-9916}%
\ifx\Semafor\ValueOn%
\RefDefinition{representation of algebra}#1
\else
\RefDefinition{left-side representation of algebra}#1
\fi
\else
\RefDefinition[\RefRepresentation]{left-side representation of algebra}#1
\fi
}

\DefEq
{
\ePrints{1310.5591}
\ifx\Semafor\ValueOff
\RefDefinition{morphism of representations of universal algebra}.
\else
\RefDefinition[0912.3315]{morphism of representations of universal algebra}.
\fi
}
{ref definition: morphism of representations of universal algebra}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{closed ball}
\else%
\RefDefinition[1305.4547]{closed ball}
\fi%
}
{ref definition: closed ball}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{open ball}\Pt
\else%
\RefDefinition[1305.4547]{open ball}\Pt
\fi%
}
{ref definition: open ball}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{open set},
\else%
\RefDefinition[1305.4547]{open set},
\fi%
}
{ref definition: open set}

\AddEq[1]{ref definition: fundamental sequence}
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\refDefinition{fundamental sequence}{normed Omega group}#1
\else%
\RefDefinition[1305.4547]{fundamental sequence, normed Omega group}#1
\fi%
}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{sequence converges uniformly}\Pt
\else%
\RefDefinition[1305.4547]{sequence converges uniformly}\Pt
\fi%
}
{ref definition: sequence converges uniformly}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{compact set},
\else%
\RefDefinition[1305.4547]{compact set},
\fi%
}
{ref definition: compact set}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefDefinition{Omega group},
\else%
\RefDefinition[1305.4547]{Omega group},
\fi%
}
{ref definition: Omega group}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefItem{|a|>=0}
\else%
\RefItem[1305.4547]{|a|>=0}
\fi%
}
{ref item |a|>=0}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefItem{|a|=0}.
\else%
\RefItem[1305.4547]{|a|=0}.
\fi%
}
{ref item |a|=0}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\RefItem{|a+b|<=|a|+|b|}\Pt
\else%
\RefItem[1305.4547]{|a+b|<=|a|+|b|}\Pt
\fi%
}
{ref item |a+b|<=|a|+|b|}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\EqRef{|a omega|<|omega||a|1n}.
\else%
\EqRef[1305.4547]{|a omega|<|omega||a|1n}.
\fi%
}
{ref EqRef |a omega|<|omega||a|1n}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\EqRef{|a-b|>|a|-|b|},
\else%
\EqRef[1305.4547]{|a-b|>|a|-|b|},
\fi%
}
{ref EqRef |a-b|>|a|-|b|}

\DefEq
{
\ePrints{1310.5591}%
\ifx\Semafor\ValueOff%
\EqRef{|fab|<|f||a||b|}.
\else%
\EqRef[1305.4547]{|fab|<|f||a||b|}.
\fi%
}
{ref |fab|<|f||a||b|}

\AddEq{ref tensor product and polylinear map}
{
\RefTheorem[\RefLinearMap]{there exists tensor product of modules},
\RefTheorem[\RefLinearMap]{tensor product and polylinear map}.
}

\DefEq
{
\ePrints{1502.04063,5114-6019}
\ifx\Semafor\ValueOff
\RefDefinition{reduced morphism of representations},
\else
\xRef[0912.3315]{remark: reduced morphism of representations},
\fi
}
{ref reduced morphism of representations}

\DefEq
{
\RefTheorem[1202.6021]{expand linear mapping, quaternion}.
}
{ref expand linear mapping, quaternion}

\DefEq
{
\RefTheorem[0912.4061]{ax-xa=1 quaternion algebra}.
}
{ref ax-xa=1 quaternion algebra}

\AddEq{ref theorem derivative, representation in algebra}
{
\ePrints{9835-2163,0767-8264}
\ifx\Semafor\ValueOn
\RefTheorem{derivative, representation in algebra},
\else
\RefTheorem[\RefCalculus]{derivative, representation in algebra},
\fi
}

\AddEq{ref partial derivatives equal}
{
\ePrints{9835-2163,0767-8264}
\ifx\Semafor\ValueOn
\EqRef{partial derivatives equal, Direct Sum of Banach Modules},
\else
\ePrints{CACAA.07}
\ifx\Semafor\ValueOff
\EqRef[0812.4763]{Gateaux partial derivatives equal, D vector space},
\else
\EqRef[CACAA.05.001]{partial derivatives equal, D vector space},
\fi
\fi
\EqRef{dM/dy=dN/dx yx},
\EqRef{d int f=f}.
}

\AddEq{ref aE, quaternion, Jacobian matrix}
{
\ePrints{CACAA.07}
\ifx\Semafor\ValueOn
\RefTheorem[CACAA.01.109]{aE, quaternion, Jacobian matrix},
\else
\RefTheorem[1107.1139]{aE, quaternion, Jacobian matrix},
\fi
%\RefTheorem[1202.6021]{aE, quaternion, Jacobian matrix}.
}

\AddEq{ref Ea, quaternion, Jacobian matrix}
{
\ePrints{CACAA.07}
\ifx\Semafor\ValueOn
\RefTheorem[CACAA.01.109]{Ea, quaternion, Jacobian matrix},
\else
\RefTheorem[1107.1139]{Ea, quaternion, Jacobian matrix},
\fi
}

\DefEq
{
\RefTheorem[1003.1544]{quaternion conjugation}.
}
{ref quaternion conjugation}

\DefEq
{
\RefTheorem[1003.1544]{Quaternion over real field, matrix}.
}
{ref Quaternion over real field, matrix}

\DefEq
{
%\ePrints{2207.06506,8428-0408}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1601.03259]{representation of derivative, algebra A->B}.
%\else%
%\refTheorem[1601.03259]{differentiable map}{algebra}.
%\fi%
}
{ref differentiable map A->B}

\DefEq
{
%\ePrints{2207.06506,8428-0408}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1601.03259]{map is continuous, derivative}.
%\else%
%\RefTheorem[1601.03259]{map is continuous, derivative}.
%\fi%
}
{ref map is continuous, derivative}

\DefEq
{
%\ePrints{1601.03259,4975-6381}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1302.7204]{monomial of power k}.
%\else%
%\RefTheorem[1302.7204]{monomial of power k}.
%\fi%
}
{ref monomial of power k}

\DefEq
{
%\ePrints{1601.03259,4975-6381}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1302.7204]{map A(k+1)->pk otimes is polylinear map}.
%\else%
%\RefTheorem[1302.7204]{map A(k+1)->pk otimes is polylinear map}.
%\fi%
}
{ref map A(k+1)->pk otimes is polylinear map}

\DefEq
{
%\ePrints{1105.4307}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1302.7204]{r=+q circ p}.
%\else%
%\RefTheorem[1302.7204]{r=+q circ p}.
%\fi%
}
{ref r=+q circ p}

\DefEq
{
%\ePrints{1105.4307}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1302.7204]{r=+q circ p 1}.
%\else%
%\RefTheorem[1302.7204]{r=+q circ p 1}.
%\fi%
}
{ref r=+q circ p 1}

\DefEq
{
%\ePrints{1506.00061,7287-9339}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1105.4307]{Re Im A->F}.
%\else%
%\RefTheorem[1105.4307]{Re Im A->F}.
%\fi%
}
{ref Re Im A->F}

\DefEq
{
%\ePrints{1506.00061,7287-9339}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1105.4307]{conjugation in algebra}.
%\else%
%\RefTheorem[1105.4307]{conjugation in algebra}.
%\fi%
}
{ref conjugation in algebra}

\DefEq
{
%\ePrints{1506.00061,7287-9339}%
%\ifx\Semafor\ValueOn%
\RefTheorem[1105.4307]{structural constant of algebra with unit}.
%\else%
%\RefTheorem[1105.4307]{structural constant of algebra with unit}.
%\fi%
}
{ref structural constant of algebra with unit}


==> Statement.English.tex <==
%auto-ignore

\newenvironment{ProofRef}[2]{%
\def\TheoremList{theorem}
\def\TheoremRef{}

{\sc Proof of theorem}
\def\Temp{}%
\edef\Tempa{#2}%
\ifx\Tempa\Temp%
\RefTheorem{#1}.
\else
\refTheorem{#1}{#2}.
\fi
}%
{\qed}

\newcommand{\DefLemmaProof}[3][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{proof: #2}
{%
{\sc Proof.}
#3
\hfill\(\odot\)
}
}

\author{Aleks Kleyn}
\ifx\setCACAA\undefined
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{question}[theorem]{Question}
\newtheorem{summary}[theorem]{Summary of Results}
%\theoremstyle{lemma}
\newtheorem{lemma}[theorem]{Lemma}
\else
\theoremstyle{definition}
\theoremstyle{remark}
\fi
\newtheorem{Statement}[theorem]{Statement}
\newtheorem{convention}[theorem]{Convention}
\newtheorem{xca}[theorem]{Exercise}
\ifx\PrintBook\undefined
\newcommand{\BibTitle}{%
\section{References}%
}
\else
\newcommand{\BibTitle}{%
\chapter{References}%
}
\fi


==> Statement.Russian.tex <==
%auto-ignore

\newenvironment{ProofRef}[2]{%
\def\TheoremList{theorem}
\def\TheoremRef{}

{\sc Доказательство теоремы}
\def\Temp{}%
\edef\Tempa{#2}%
\ifx\Tempa\Temp%
\RefTheorem{#1}.
\else
\refTheorem{#1}{#2}.
\fi
}%
{\qed}

\newcommand{\DefLemmaProof}[3][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{proof: #2}
{%
{\sc Доказательство.}
#3
\hfill\(\odot\)
}
}

\author{Александр Клейн}
\ifx\setCACAA\undefined
\newtheorem{theorem}{Теорема}[section]
\newtheorem{corollary}[theorem]{Следствие}
\newtheorem{example}[theorem]{Пример}
\newtheorem{definition}[theorem]{Определение}
\newtheorem{remark}[theorem]{Замечание}
\newtheorem{question}[theorem]{Вопрос}
\newtheorem{summary}[theorem]{Сводка результатов}
%\theoremstyle{lemma}
\newtheorem{lemma}[theorem]{Лемма}
\else
\theoremstyle{definition}
\theoremstyle{remark}
\fi
\newtheorem{Statement}[theorem]{Утверждение}
\newtheorem{convention}[theorem]{Соглашение}
\newtheorem{xca}[theorem]{Exercise}
\ifx\PrintBook\undefined
\newcommand{\BibTitle}{%
\section{Список литературы}%
}
\else
\newcommand{\BibTitle}{%
\chapter{Список литературы}%
}
\fi


==> Statement.tex <==
%auto-ignore

\ifx\SelectlEnglish\undefined
\ifx\UseRussian\undefined
\def\SelectlEnglish{}
\fi
\fi
\ifx\SelectlEnglish\undefined
\newcommand\TheLanguage{Russian}%
\else
\newcommand\TheLanguage{English}%
\fi

\newcommand\LanguagePrefix{}%
\newcommand\Input[1]{\input{\FilePrefix #1.\TheLanguage}}%
\newcommand\CurrentLanguage{\TheLanguage.}%
\newcommand\xRefDef[1]
{
\wRefDef{#1}{\TheLanguage}
\NameDef{xRefDef#1}{}%
}

\Input{Statement}

\newenvironment{Abstract}
{
\leftskip=30pt
\noindent
{\sc\abstractname.}
}
{
\leftskip=0pt
}

\theoremstyle{definition}
\theoremstyle{remark}
\renewenvironment{proof}[1][\proofname]
{\par{\sc #1. }}{\qed}%

\ifx\PrintBook\undefined
%\ifx\Presentation\undefined
\renewcommand\theHsection{\CurrentLanguage\arabic{section}}%
\numberwithin{footnote}{section}
\numberwithin{Hfootnote}{section}
%\fi
\else
\numberwithin{section}{chapter}
\renewcommand\theHchapter{\CurrentLanguage\arabic{chapter}}%
\numberwithin{footnote}{chapter}
\numberwithin{Hfootnote}{chapter}
\fi

\ifx\Presentation\undefined
\numberwithin{equation}{section}
\numberwithin{figure}{section}
\numberwithin{table}{section}
\numberwithin{Item}{section}
\fi

\def\OneTheorem{the theorem }
\def\ManyTheorems{theorems }

\def\LastRef{LastRef}%
\def\PrintTheorem#1{\PrtTheorem#1||LastRef||}%
\def\PrtTheorem#1||#2||{\def\temp{#2}%
\ifx\temp\LastRef%
\gdef\TheoremName{\OneTheorem}
\else%
\gdef\TheoremName{\ManyTheorems}
\expandafter\DoNothing
\fi%
}
\def\DoNothing#1||
{
\def\temp{#1}%
\ifx\temp\LastRef%
\else%
\expandafter\DoNothing
\fi%
}
\def\Refs#1{\RefList#1||LastRef||}%
\def\RefList#1||{\def\temp{#1}%
\ifx\temp\LastRef%
\else%
\TheoremSep\DoTheoremRef{#1}
\gdef\TheoremSep{, }%
\expandafter\RefList
\fi%
}
\def\DoTheoremRef#1{\DoRefs#1|:LastTRef|:}%
\def\LastTRef{LastTRef}%
\def\DoRefs#1|:#2|:{\def\tempA{#2}%
\ifx\tempA\LastTRef%
\RefTheorem{#1}%
\else%
\refTheorem{#1}{#2}%
\fi%
\expandafter\RefNothing%
}
\def\RefNothing#1
{%
}%
\newenvironment{ProofRefA}[1]{%
\gdef\TheoremSep{}%
{\PrintTheorem{#1}}
{\sc Proof of \TheoremName \Refs{#1}.}
}%
{\qed}

\ifx\texFuture\Defined
\begin{ProofRefA}{Polylinear map is geometric object||%
define homomorphism of vector space|:left||define homomorphism of vector space|:right}
\end{ProofRefA}

\begin{ProofRefA}{define homomorphism of vector space|:left}
\end{ProofRefA}
\fi

\definecolor{TheoremColor}{rgb}{.94,.96,.94}%
\definecolor{LemmaColor}{rgb}{.94,.96,.98}%
\definecolor{DefinitionColor}{rgb}{.94,.94,.95}%
\definecolor{QuestionColor}{rgb}{.93,.93,.96}%
\definecolor{SummaryColor}{rgb}{.92,.93,.95}%
\definecolor{ExampleColor}{rgb}{.94,.95,.90}%
\newcommand{\DefineTheoremColor}{%
\colorlet{shadecolor}{TheoremColor}
}%
\newcommand{\DefineLemmaColor}{%
\colorlet{shadecolor}{LemmaColor}
}%
\newcommand{\DefineDefinitionColor}{%
\colorlet{shadecolor}{DefinitionColor}
}%
\newcommand{\DefineQuestionColor}{%
\colorlet{shadecolor}{QuestionColor}
}%
\newcommand{\DefineSummaryColor}{%
\colorlet{shadecolor}{SummaryColor}
}%
\newcommand{\DefineExampleColor}{%
\colorlet{shadecolor}{ExampleColor}
}%

\newenvironment{Shaded}{%
\def\FrameCommand{\fboxsep2pt \colorbox{shadecolor}}%
  \MakeFramed {\FrameRestore}}%
 {\endMakeFramed}

\newenvironment{Convention}
{
\begin{convention}
}
{
\qed
\end{convention}
}

\newenvironment{ShadedConvention}
{
\DefineDefinitionColor
\begin{Shaded}
\begin{Convention}
}{%
\end{Convention}%
\end{Shaded}%
}

\newenvironment{Definition}
{
\begin{definition}
}
{
\qed
\end{definition}
}

\newenvironment{ShadedDefinition}
{
\DefineDefinitionColor
\begin{Shaded}
\begin{Definition}
}{%
\end{Definition}%
\end{Shaded}%
}

\newenvironment{ShadedTheorem}
{
\DefineTheoremColor%
\begin{Shaded}%
\begin{theorem}%
}{%
\end{theorem}%
\end{Shaded}%
}

\newenvironment{Corollary}
{
\begin{corollary}
}
{
\qed
\end{corollary}
}

\newenvironment{ShadedCorollary}
{
\DefineTheoremColor%
\begin{Shaded}%
\begin{Corollary}%
}{%
\end{Corollary}%
\end{Shaded}%
}

\newenvironment{ShadedLemma}
{
\DefineLemmaColor%
\begin{Shaded}%
\begin{lemma}
%\it
}{%
\end{lemma}
\end{Shaded}%
}

\newenvironment{Example}
{
\begin{example}
}
{
\qed
\end{example}
}

\newenvironment{ShadedExample}
{
\DefineExampleColor
\begin{Shaded}
\begin{Example}
}{%
\end{Example}%
\end{Shaded}%
}

\newenvironment{Question}
{
\begin{question}
}
{
\qed
\end{question}
}

\newenvironment{ShadedQuestion}
{
\DefineQuestionColor%
\begin{Shaded}%
\begin{Question}
}{%
\end{Question}
\end{Shaded}%
}

\newenvironment{Summary}
{
\begin{summary}
}
{
\qed
\end{summary}
}

\newenvironment{ShadedSummary}
{
\DefineSummaryColor%
\begin{Shaded}%
\begin{Summary}
}{%
\end{Summary}
\end{Shaded}%
}

\newenvironment{Remark}
{
\begin{remark}
}
{
\qed
\end{remark}
}

%\ifx\texFuture\Defined
\newenvironment{ParacolDefinition}
{
\backgroundcolor{c}{DefinitionColor}
\begin{paracol}{1}%
\begin{definition}
}{%
\qed%
\end{definition}%
\end{paracol}%
\nobackgroundcolor{c}%
}

\newenvironment{ParacolTheorem}
{
\backgroundcolor{c}{TheoremColor}
\begin{paracol}{1}%
\begin{theorem}%
}{%
\end{theorem}%
\end{paracol}%
\nobackgroundcolor{c}
}
%\fi

%\def\DefinitionStyle{Definition}%
\def\DefinitionStyle{ShadedDefinition}%

\newcommand{\DefDefinition}[3][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{definition: #2}
{
\begin{\DefinitionStyle}
\labelDefinition{#2}
#3
\end{\DefinitionStyle}
}
}%

\newcommand{\DefLabeledDefinition}[4][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{definition: #2}
{
\begin{\DefinitionStyle}
\labelDefinition{#2:: #3}
#4
\end{\DefinitionStyle}
}
}%

\newcommand{\DefDefinitionNote}[4][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{definition: #2}
{
\begin{\DefinitionStyle}
\labelDefinition{#2}
#3
\end{\DefinitionStyle}
\footnotetext{\,
#4
}
}
}%

\newcommand{\DefLabeledDefinitionNote}[5][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{definition: #2}
{
\begin{ShadedDefinition}
\labelDefinition{#2:: #3}
#4
\end{ShadedDefinition}
\footnotetext{\,
#5
}
}
}%

\newcommand\ShowDefinition[1]{\ShowEq{definition: #1}}

%\def\TheoremStyle{theorem}%
%\def\TheoremStyle{ParacolTheorem}%
\def\TheoremStyle{ShadedTheorem}%

\newcommand{\DefTheorem}[3][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{theorem: #2}
{
\begin{\TheoremStyle}
\labelTheorem{#2}
#3
\end{\TheoremStyle}
}
}%

\newcommand{\DefLabeledTheorem}[4][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{theorem: #2}
{
\begin{\TheoremStyle}
\labelTheorem{#2:: #3}
#4
\end{\TheoremStyle}
}
}%

\newcommand{\DefTheoremNote}[4][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{theorem: #2}
{
\begin{\TheoremStyle}
\label{theorem: #2}
#3
\end{\TheoremStyle}
\footnotetext{\,
#4
}
}
}%

\newcommand{\DefLabeledTheoremNote}[5][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{theorem: #2}
{
\begin{\TheoremStyle}
\labelTheorem{#2:: #3}
#4
\end{\TheoremStyle}
\footnotetext{\,
#5
}
}
}%

\newcommand{\ShowTheorem}[1]{%
\ShowEq{theorem: #1}%
}%

%\def\LemmaStyle{lemma}%
\def\LemmaStyle{ShadedLemma}%

\newcommand\DefLemma[2]{%
\AddEq{lemma: #1}
{
\begin{\LemmaStyle}
\labelLemma{#1}
#2
\end{\LemmaStyle}
}
}

\newcommand\DefLabeledLemma[4]{%
\AddEq{lemma: #1}
{
\begin{\LemmaStyle}
\labelLemma{#1:: #2}
#3
\end{\LemmaStyle}
}
}

\newcommand{\ShowLemma}[1]{\ShowEq{lemma: #1}}%

%\def\CorollaryStyle{Corollary}%
\def\CorollaryStyle{ShadedCorollary}%

\newcommand{\DefCorollary}[2]{%
\AddEq{corollary: #1}
{
\begin{\CorollaryStyle}
\labelCorollary{#1}
#2
\end{\CorollaryStyle}
}
}

\newcommand{\ShowCorollary}[1]{%
\ShowEq{corollary: #1}%
}%

\newcommand{\DefProof}[3][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{proof: #2}
{%
\begin{proof}
#3
\end{proof}%
}
}

\newcommand{\DefProofSloppy}[3][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{proof: #2}
{%
\begin{sloppypar}
\begin{proof}
#3
\end{proof}%
\end{sloppypar}
}
}

\newcommand{\DefProofRef}[4][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{proof: #2}
{%
\begin{ProofRef}{#2}{#3}
#4
\end{ProofRef}%
}
}

\newcommand{\ShowProof}[1]{\ShowEq{proof: #1}}%

\newcommand{\ProveTheorem}[1]
{
\ShowTheorem{#1}
\ShowProof{#1}
}%

%\def\ExampleStyle{Example}%
\def\ExampleStyle{ShadedExample}%

\newcommand{\DefExample}[2]{%
\AddEq{example: #1}
{
\begin{\ExampleStyle}
\labelExample{#1}
#2
\end{\ExampleStyle}
}
}%

\newcommand{\DefExampleNote}[3]{%
\AddEq{example: #1}
{
\begin{\ExampleStyle}
\labelExample{#1}
#2
\end{\ExampleStyle}
\footnotetext{\,
#3
}
}
}%

\newcommand{\DefLabeledExample}[3]{%
\AddEq{example: #1}
{
\begin{\ExampleStyle}
\labelExample{#1:: #2}
#3
\end{\ExampleStyle}
}
}%

\newcommand{\ShowExample}[1]{%
\ShowEq{example: #1}%
}%

\newcommand\DefRemark[2]{%
\AddEq{remark: #1}
{
\begin{Remark}
\labelRemark{#1}
#2
\end{Remark}
}
}%

\newcommand\DefLabeledRemark[3]{%
\AddEq{remark: #1}
{
\begin{Remark}
\labelRemark{#1:: #2}
#3
\end{Remark}
}
}%

\newcommand\DefLabeledSloppyRemark[3]{%
\AddEq{remark: #1}
{
\begin{sloppypar}
\begin{Remark}
\labelRemark{#1:: #2}
#3
\end{Remark}
\end{sloppypar}
}
}%

\newcommand\DefText[3][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{text: #2}
{
#3
}
}%

\newcommand{\ShowRemark}[1]{%
\ShowEq{remark: #1}%
}%

\newcommand{\ShowText}[1]{%
\ShowEq{text: #1}%
}%

%\def\ConventionStyle{Convention}%
\def\ConventionStyle{ShadedConvention}%

\newcommand\DefConvention[3][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{convention: #2}
{
\begin{\ConventionStyle}
\labelConvention{#2}
#3
\end{\ConventionStyle}
}
}%

\newcommand\DefLabeledConvention[4][]{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{convention: #2}
{
\begin{\ConventionStyle}
\labelConvention{#2:: #3}
#4
\end{\ConventionStyle}
}
}%

\newcommand{\ShowConvention}[1]{%
\ShowEq{convention: #1}%
}%

%\def\QuestionStyle{Question}%
\def\QuestionStyle{ShadedQuestion}%

\newcommand\DefQuestion[2]{%
\AddEq{question: #1}
{
\begin{\QuestionStyle}
\labelQuestion{#1}
#2
\end{\QuestionStyle}
}
}%

\newcommand{\ShowQuestion}[1]{%
\ShowEq{question: #1}%
}%

%\def\SummaryStyle{Summary}%
\def\SummaryStyle{ShadedSummary}%

\newcommand\DefSummary[2]{%
\AddEq{summary: #1}
{
\begin{\SummaryStyle}
\labelSummary{#1}
#2
\end{\SummaryStyle}
}
}%

\newcommand\DefLabeledSummary[3]{%
\AddEq{summary: #1}
{
\begin{\SummaryStyle}
\labelSummary{#1:: #2}
#3
\end{\SummaryStyle}
}
}%

\newcommand{\ShowSummary}[1]{%
\ShowEq{summary: #1}%
}%

\newcommand{\DefCiteBib}[2]{\AddEq{citeBib: #1}{#2}}%
\newcommand{\DefBiblioItem}[1]{\BiblioItem{#1}{\ShowCiteBib{#1}}}%

\newcommand\ShowCiteBib[1]{\ShowEq{citeBib: #1}}

%%%   labels and refs
\makeatletter
\newcommand\StartLabelItem[1][theorem]%
{
%\counterwithin{enumi}{#1}%
\expandafter \def \csname%
 theenumi\expandafter \endcsname \expandafter {\csname the#1\expandafter%
 \endcsname.\expandafter \@arabic \csname c@enumi\endcsname }%
\def\labelenumi{\theenumi:}%
}
\newcommand\StopLabelItem[1][theorem]%
{
\counterwithout{enumi}{#1}%
\def\labelenumi{(\theenumi)}
}
\makeatother
\newcommand\labelConvention[1]{\label{convention: #1}}%
\newcommand\labelTheorem[1]{\label{theorem: #1}}%
\newcommand\labelLemma[1]{\label{lemma: #1}}%
\newcommand\labelCorollary[1]{\label{corollary: #1}}%
\newcommand\labelStatement[1]{\label{statement: #1}}
\newcommand\labelDefinition[1]{\label{definition: #1}}%
\newcommand\labelExample[1]{\label{example: #1}}%
\newcommand\labelRemark[1]{\label{remark: #1}}%
\newcommand\labelSection[1]{\label{section: #1}}%
\newcommand\labelSubsection[1]{\label{subsection: #1}}%
\newcommand\labelChapter[1]{\label{chapter: #1}}%
\newcommand\labelItem[1]{\label{item: #1}}%
\newcommand\labelQuestion[1]{\label{question: #1}}
\newcommand\labelSummary[1]{\label{summary: #1}}
\newcommand\labelFootnote[1]{\label{footnote: #1}}
\makeatletter
\newcommand\xRef[2][]%
{%
\def\Semafor{on}%
\def\Temp{}%
\edef\Tempa{#1}%
\ifx\Tempa\Temp%
\def\Semafor{off}%
\fi%
\@ifundefined{xRefDef#1}{%
\def\Semafor{off}%
}{}%
\ifx\Semafor\ValueOff%
\penalty-1\ref{#2}%
\else%
\penalty-1\citeBib{#1}-\ref{#1-\TheLanguage-#2}%
\fi%
}%
\makeatother
\newcommand\RefConvention[2][]{\xRef[#1]{convention: #2}}
\newcommand\RefTheorem[2][]{\xRef[#1]{theorem: #2}}
\newcommand\refTheorem[3][]{\xRef[#1]{theorem: #2:: #3}}
\newcommand\RefLemma[2][]{\xRef[#1]{lemma: #2}}
\newcommand\refLemma[3][]{\xRef[#1]{lemma: #2:: #3}}
\newcommand\RefStatement[2][]{\xRef[#1]{statement: #2}}
\newcommand\RefCorollary[2][]{\xRef[#1]{corollary: #2}}
\newcommand\RefDefinition[2][]{\xRef[#1]{definition: #2}}
\newcommand\refDefinition[3][]{\xRef[#1]{definition: #2:: #3}}
\newcommand\RefExample[2][]{\xRef[#1]{example: #2}}
\newcommand\refExample[3][]{\xRef[#1]{example: #2:: #3}}
\newcommand\RefRemark[2][]{\xRef[#1]{remark: #2}}
\newcommand\refRemark[3][]{\xRef[#1]{remark: #2:: #3}}
\newcommand\RefSection[2][]{\xRef[#1]{section: #2}}
\newcommand\RefSubsection[2][]{\xRef[#1]{subsection: #2}}
\newcommand\RefChapter[2][]{\xRef[#1]{chapter: #2}}
\newcommand\RefItem[2][]{\xRef[#1]{item: #2}}
\newcommand\RefQuestion[2][]{\xRef[#1]{question: #2}}
\newcommand\RefSummary[2][]{\xRef[#1]{summary: #2}}
\newcommand\refSummary[3][]{\xRef[#1]{summary: #2:: #3}}
\newcommand\RefFootnote[2][]{\,${}^{\xRef[#1]{footnote: #2}}$}
\newcommand\refFootnote[3][]{\,${}^{\xRef[#1]{footnote: #2:: #3}}$}

\makeatletter
\newcommand\AddFootnote[2]
{
\stepcounter{Hfootnote}
\stepcounter{footnote}
\global \let \Hy@saved@currentHref \@currentHref
\hyper@makecurrent {Hfootnote}
\global \let \Hy@footnote@currentHref \@currentHref 
\footnotetext{
\labelFootnote{#1}
\,#2
}
}

\newcommand\ShowPrevFootnote[1]
{
\addtocounter{Hfootnote}{-1}
\addtocounter{footnote}{-1}
\global \let \Hy@saved@currentHref \@currentHref
\hyper@makecurrent {Hfootnote}
\global \let \Hy@footnote@currentHref \@currentHref 
\footnotetext{
\,#1
}
}

\newcommand\ShowNextFootnote[1]
{
\stepcounter{Hfootnote}
\stepcounter{footnote}
\global \let \Hy@saved@currentHref \@currentHref
\hyper@makecurrent {Hfootnote}
\global \let \Hy@footnote@currentHref \@currentHref 
\footnotetext{
\,#1
}
}
\makeatother

\newcommand\DefFootnote[3][]%
{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{footnote: #2}
{
\AddFootnote{#2}{#3}
}
}

\newcommand\DefLabeledFootnote[4][]%
{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{footnote: #2}
{
\AddFootnote{#2:: #3}{#4}
}
}

\newcommand{\ShowFootnote}[1]{%
\ShowEq{footnote: #1}%
}%

\newcommand\DefRef[3][]%
{%
\def\Temp{}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\def\TempB{\AddEq}%
\else%
\def\TempB{\AddEq[#1]}%
\fi%
\TempB{ref: #2}
{
#3
}
}

\newcommand\ShowRef[1]{\ShowEq{ref: #1}}

\ifx\texFuture\Defined
\newcommand\TwoColText[2]
{
\noindent
\begin{minipage}{0.5\textwidth}
\setlength{\parindent}{4mm}
#1
\end{minipage}
\begin{minipage}{0.5\textwidth}
\setlength{\parindent}{4mm}
#2
\end{minipage}
}
\fi

\ifx\UseParacol\Defined
\newcommand\TwoColText[2]
{
\begin{paracol}{2}
#1
\switchcolumn
#2
\end{paracol}
}

\else
\newcommand\TwoColText[2]
{
\noindent
\begin{tabular}{@{}l|r}
\begin{minipage}{0.49\textwidth}
\setlength{\parindent}{4mm}
#1
\end{minipage}
&
\begin{minipage}{0.49\textwidth}
\setlength{\parindent}{4mm}
#2
\end{minipage}
\end{tabular}
}
\fi


==> Stmt.2022.01.05.English.tex <==
%auto-ignore
\input{Stmt.2022.01.05.Eq}

\AddEq{remark: extend linear representation to set of bases 1}
{
%\begin{sloppypar}
Thus we can extend
a \OtherSideNS\Hyph side linear \Group nA\Hyph representation
in \SideWS $A$\Hyph vector space $V$ of \ColN s
to the set of bases
of \SideWS $A$\Hyph vector space $V$.
%\end{sloppypar}
}

\DefText{coordinates of homomorphism}
{
Although the theorem
\refTheorem{define homomorphism A module}{\SideNS(1)}
is true
and can serve as a definition of homomorphism,
this theorem does not give the full picture.

Suppose we are studying a physical phenomenon.
We can give a qualitative picture of this phenomenon.
However, if we want to perform experiment,
we have to choose a set of measuring tools
and to calculate expected measurements.
The set of measuring tools
is a basis in the space of measurements;
and expected measurements are coordinates of experiment
in the space of measurements.

We will extend this remark to the theorem
\refTheorem{define homomorphism A module}{\SideNS(1)}.
To understand the structure of homomorphism
and answer the question how big is the set of homomorphisms,
we have to choose a basis of $A$\Hyph vector space
and consider the change of coordinates of vector with respect to selected basis.

\ShowEq{def AVector}%
There are various conventions for numbering vectors of the basis
and corresponding conventions for the numbering of coordinates of a vector.
\ShowEq{\DefCol}%
For instance, in the theorem
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
we consider coordinates of vector in
\SideWS $\Base$\Hyph \VectorSet of \ColN s.

\ShowTheorem{coordinate matrix of vector}

If the basis \eV is given, then
\ShowEq{V*=coordinate}
is the set of coordinates of vectors $\Vector v\in V$.
The set $V_*$ is left $A$\Hyph vector space
and is isomorphic to left $A$\Hyph vector space $V$.
Therefore, the set $V_*$ does not depend on choice of basis \eV[][.]

If left $A$\Hyph vector space $V$
has dimension $\gi n$, then
left $A$\Hyph vector space $V_*$
is isomorphic to direct sum of $\gi n$ copies of $D$\Hyph algebra $A$.
So in this case we put
\ShowEq{V*=n V cr}

\ShowEq{\DefRow}%
In the theorem
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
we consider coordinates of vector in
\SideWS $\Base$\Hyph \VectorSet of \ColN s.

\ShowTheorem{coordinate matrix of vector}

\ShowRemark{Vector Space Type}

\ShowEq{\DefCol}%
Statements for various forms of representation of coordinates of vector
are similar.
Therefore, we will focus our attention on
\SideWS $\Base$\Hyph \VectorSet of \ColN s.
}

\DefText{22-12-10 Eigenvalue of Matrix of A-Numbers}
{
In following definitions,
we consider different types of eigenvalues
of matrix of $A$\Hyph numbers.
}

\AddEq{remark: Vector Space Type}
{
We considered main formats of presentation of coordinates of vector
of left $A$\Hyph vector space.
It is evident that other formats of presentation of coordinates of vector are also possible.
For instance, we may consider the set of \nmTimes nm matrices
as left $A$\Hyph vector space.
The same way we may consider
main formats of presentation of coordinates of vector
of right $A$\Hyph vector space.
}

\DefSummary{Examples of Geometric Object}
{
\ShowEq{\DefCol}
Let passive transformation $g$ map the basis \eV[1]
into the basis \eV[2][:]
\FrameEqRef[12g{}]{e2i=aij e1j cr-cols}{1->2 l}

Let
\FrameEqRef[k]{aij=.ox.}k
be coordinates of linear map $a$
with respect to the basis \eV[k][,]
$k=1$, $2$.
Then
\newline
\FrameEqRef{a ox 2=g a ox 1 l}1
\newline
Equalities
\newline
\FrameEqRef[fg{\SideNS}{\Cols}]{f2=a f1 a-}{g \SideNS-\Cols}
\newline
and
\newline
\FrameEqRef{a ox 2=g a ox 1 l}1
\newline
are similar.
From the equality
\newline
\FrameEqRef{a ox 2=g a ox 1 g l}1
\newline
it follows that image of linear map
does not depend on choice of basis.

Let the set of tensors
\FrameEqRef{akj1n .ox.}1
be coordinates of polylinear map $a$
with respect to the basis \eV[k], $k=1$, $2$.
Then
\newline
\FrameEqRef{a ox 2=g a ox 1}1
\newline
From the equality
\newline
\FrameEqRef{a ox 2=g a ox 1 g}1
\newline
it follows that image of polylinear map
does not depend on choice of basis.

Consider skew-symmetric polylinear map
\newline
\FrameEqRef{h=aubvc}1
\newline
If we consider determinant like expression
\newline
\FrameEqRef{star uv-vu}1
\newline
then we can represent polylinear map $h$ as
\newline
\FrameEqRef{h=1/2 aubvc 1}1
\newline
Let the set of tensors
\FrameEqRef{akj1n .ox.}1
be coordinates of polylinear map $h$
with respect to the basis \eV[k], $k=1$, $2$.
Then
\newline
\FrameEqRef{huv=12 huv-hvu 5}1
}

\DefText{automorphism basis matrix}
{
Theorems
\refTheorem{coordinate matrix of basis}{\Product-\Cols},
\refTheorem{active transformations, basis, vector space}{\SideNS-\Cols}
show relationship between
\ProductType nonsingular matrices,
bases and automorphisms
of \SideWS $\Base$\Hyph \VectorSet of \ColN s.
}

\DefText{endomorphism=matrix}
{
Therefore, if we choose the basis
\ShowEq{basis e of V}
of left $A$\Hyph vector space $V$ of columns,
then we can identify the set of endomorphisms
of left $A$\Hyph vector space $V$
and the set of $\gin\times\gin$ matrices.
We will see this relation between endomorphisms and matrices
deeper when we consider automorphisms.
}

\DefText{converse theorem is also true}
{
The converse theorem is also true.
}

\DefLabeledSummary{homomorphism of vector space}{\SideNS}
{
\ShowEq{prolog homomorphism of vector space(1)}{}{}1{}{}2
Then homomorphism
\ShowEq{f:A->B}{\Vector f}VW
of \SideWS $A$\Hyph vector space has presentation
\newline
\FrameEqRef[afVW]{f o (ae)=a o f e, vector space \Product-\Cols}1
\FrameEqRef[b{}a{}f{}]{v1=v2*a \SideNS-\Cols}1
\newline
relative to selected bases.
Here
\begin{itemize}
%\setlength{\itemindent}{-1em}
\item
$a$ is coordinate matrix of vector
$\Vector a$ relative the basis $\Basis e_V$.
\item
$b$ is coordinate matrix of vector
\DrawEq[abf]{vb=f(va)}-
relative the basis $\Basis e_W$.
\item
$f$ is coordinate matrix of set of vectors
\ShowEq{(Vector f(e))}
relative the basis $\Basis e_W$.
\end{itemize}
The matrix $f$ is unique and is called
{\bf matrix of homomorphism}
$\Vector f$ relative bases $\Basis e_V$, $\Basis e_W$.

\ShowText{converse theorem is also true}

The map
\ShowEq{f:A->B}{\Vector f}VW
defined by the equality
\newline
\FrameEqRef[afVW]{f o (ae)=a o f e, vector space \Product-\Cols}1
\newline
is homomorphism
of \SideWS $A$\Hyph vector space of \ColN s.
A homomorphism $\Vector f$ which has the given matrix $f$
is unique.
}


==> Stmt.2022.01.05.Eq.tex <==
%auto-ignore

\AddEquation{V*=coordinate}
{
\begin{aligned}
V_*=\{
v:&\Vector v=v\CRstar e,
\Vector v\in V
\}
\end{aligned}
}

\AddEquation{V*=n V cr}
{
V_*=\gi n\CRstar A
}

\AddEq{a ox 2=g a ox 1 g l}
{
\begin{aligned}
a\circ v
&=
\underline{\Entry[t0]a2lk\aU{v_2}k
\Entry[t1]a2lk\aD[2]el}
=
(\Entry[s0]a1ij\aU{v_2}k\aUD gjk
\Entry[s1]a1ij)
\aUD{g^{\CRInverse}}li
\aUD gpl\aD[1]ep
\\ &=
\underline{(\Entry[s0]a1ij\aU{v_1}j
\Entry[s1]a1ij)
\aD[1]ei}
\end{aligned}
}

\AddEq{a ox 2=g a ox 1}
{
\begin{aligned}
&\,\Entry[t0]a2l{k_1...k_n}\otimes
\Entry[t1]a2l{k_1...k_n}...
\otimes \Entry[tn]a2l{k_1...k_n}
\\=&\,
(\Entry[s0]a1i{j_1...j_n}\otimes \aUD g{j_1}{k_1}
\Entry[s1]a1i{j_1...j_n}...
\otimes \aUD g{j_n}{k_n}\Entry[sn]a1i{j_1...j_n})
\aUD{g^{\CRInverse}}li
\end{aligned}
}

\AddEq{star uv-vu}
{
{\det}^*
\begin{pmatrix}
\aU uj&\aU vj\\ \aU uk&\aU vk
\end{pmatrix}
=\aU uj\otimes\aU vk-\aU vj\otimes\aU uk
}

\AddEq{h=1/2 aubvc 1}
{
\aU hi\circ(u\otimes v)
=\frac 12
(\Entry[s0]a{}i{jk}\otimes\Entry[s1]a{}i{jk}\otimes\Entry[s2]a{}i{jk})
\circ{\det}^*
\begin{pmatrix}
\aU uj&\aU vj\\ \aU uk&\aU vk
\end{pmatrix}
}

\AddEq{huv=12 huv-hvu 5}
{
\begin{aligned}
&\,
(\Entry[s0]a2i{jk}\otimes_1\Entry[s1]a2i{jk}\otimes_2\Entry[s2]a2i{jk})
\circ {\det}^*
\begin{pmatrix}
1\otimes_1\aUD{\delta}jq&1\otimes_2\aUD{\delta}jr\\
1\otimes_1\aUD{\delta}kq&1\otimes_2\aUD{\delta}kr
\end{pmatrix}
\\ =&\,
((\Entry[s0]a1i{jk}\otimes_1\Entry[s1]a1i{jk}\otimes_2\Entry[s2]a1i{jk})
\aUD{g^{\RCInverse}_{}}pi)
\circ {\det}^*
\begin{pmatrix}
1\otimes_1\aUD gjq&1\otimes_2\aUD gjr\\
1\otimes_1\aUD gkq&1\otimes_2\aUD gkr
\end{pmatrix}
\end{aligned}
}

\AddEq{h=aubvc}
{
\begin{aligned}
\aU hi\circ(u\otimes v)
&=
\Entry[s0]a{}i{jk}\aU uj\Entry[s1]a{}i{jk}\aU vk\Entry[s2]a{}i{jk}
\\ &=
(\Entry[s0]a{}i{jk}\otimes\Entry[s1]a{}i{jk}\otimes\Entry[s2]a{}i{jk})
\circ(\aU uj\otimes\aU vk)
\end{aligned}
}

\AddEq{a ox 2=g a ox 1 g}
{
\begin{aligned}
a\circ(v_1,...,v_2)
&=
\underline{\Entry[t0]a2l{k_1...k_n}\aU{v_{12}}{k_1}
\Entry[t1]a2l{k_1...k_n}...
\aU{v_{n2}}{k_n}\Entry[tn]a2l{k_1...k_n}\aD[2]el}
\\ &=
(\Entry[s0]a1i{j_1...j_n}\aU{v_{12}}{k_1}\aUD g{j_1}{k_1}
\Entry[s1]a1i{j_1...j_n}...
\aU{v_{n2}}{k_n}\aUD g{j_n}{k_n}\Entry[sn]a1i{j_1...j_n})
\aUD{g^{\CRInverse}}li
\aUD gpl\aD[1]ep
\\ &=
\underline{(\Entry[s0]a1i{j_1...j_n}\aU{v_{11}}{j_1}
\Entry[s1]a1i{j_1...j_n}...
\aU{v_{n1}}{j_n}\Entry[sn]a1i{j_1...j_n})
\aD[1]ei}
\end{aligned}
}

\AddEq{akj1n .ox.}
{
\Entry[s0]aki{j_1...j_n}\otimes...\otimes\Entry[sn]aki{j_1...j_n}
}


==> Stmt.2022.01.05.Russian.tex <==
%auto-ignore
\input{Stmt.2022.01.05.Eq}

\AddEq{remark: extend linear representation to set of bases 1}
{
\begin{sloppypar}
Таким образом, мы можем распространить
\OtherSideRu востороннее линейное \Group nA\Hyph представление
в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsA
на множество базисов
\SideRu вого $A$\Hyph векторного пространства $V$.
\end{sloppypar}
}

\DefText{coordinates of homomorphism}
{
Хотя теорема
\refTheorem{define homomorphism A module}{\SideNS(1)}
верна
и может служить определением гомоморфизма,
эта теорема не даёт полной картины.

Допустим мы изучаем физическое явление.
Мы можем дать качественную картину этого явления.
Но если мы хотим провести эксперимент,
мы должны выбрать набор измерительных инструментов
и рассчитать ожидаемые измерения.
Набор измерительных инструментов
является базисом в пространстве измерений,
а ожидаемые измерения являются координатами эксперимента
в пространстве измерений.

Мы распространим это замечание на теорему
\refTheorem{define homomorphism A module}{\SideNS(1)}.
Для того, чтобы понять структуру гомоморфизма
и ответить на вопрос как велико множество гомоморфизмов,
мы должны выбрать базис $A$\Hyph векторного пространства
и рассмотреть изменение координат вектора относительно выбраного базиса.

\ShowEq{def AVector}%
Существуют различные соглашения о нумерации векторов базиса
и соответствующие соглашения о нумерации координат вектора.
\ShowEq{\DefCol}%
Например, в теореме
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols}
мы рассматриваем координаты вектора в
\SideRu\WhatTo $\Base$\Hyph \VectorSetRuD \ColsNA.

\ShowTheorem{coordinate matrix of vector}

Если базис \eV задан, то
\ShowEq{V*=coordinate}
является множеством координат векторов $\Vector v\in V$.
Множество $V_*$ является левым $A$\Hyph векторным пространством
и изоморфно левому $A$\Hyph векторному пространству $V$.
Следовательно, множество $V_*$ не зависит от выбора базиса \eV[][.]

Если левое $A$\Hyph векторное пространство $V$
имеет размерность $\gi n$, то
левое $A$\Hyph векторное пространство $V_*$
изоморфно прямой сумме $\gi n$ копий $D$\Hyph алгебры $A$.
Поэтому мы в этом случае положим
\ShowEq{V*=n V cr}

\ShowEq{\DefRow}%
В теореме
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols}
мы рассматриваем координаты вектора в
\SideRu\WhatTo $\Base$\Hyph \VectorSetRuD \ColsNA.

\ShowTheorem{coordinate matrix of vector}

\ShowRemark{Vector Space Type}

\ShowEq{\DefCol}%
Утверждения для различных форм представления координат вектора
похожи.
Поэтому мы сосредоточим наше внимание на
\SideRu\WhatTo $\Base$\Hyph \VectorSetRuD \ColsNA.
}

\DefText{22-12-10 Eigenvalue of Matrix of A-Numbers}
{
В последующих определениях
мы рассмотрим различные виды собственных значений
матрицы $A$\Hyph чисел.
}

\AddEq{remark: Vector Space Type}
{
Мы рассмотрели основные форматы представления координат вектора
левого $A$\Hyph векторного пространства.
Очевидно, что возможны и другие форматы представления координат вектора.
Например, мы можем рассматривать множество \nmTimes nm матриц
как левое $A$\Hyph векторное пространство.
Аналогичным образом мы можем рассмотреть
основные форматы представления координат вектора
правого $A$\Hyph векторного пространства.
}

\DefSummary{Examples of Geometric Object}
{
\ShowEq{\DefCol}
Пусть пассивное преобразование $g$ отображает базис \eV[1]
в базис \eV[2][:]
\FrameEqRef[12g{}]{e2i=aij e1j cr-cols}{1->2 l}

Пусть
\FrameEqRef[k]{aij=.ox.}k
- координаты линейного отображения $a$
относительно базиса \eV[k][,]
$k=1$, $2$.
Тогда
\newline
\FrameEqRef{a ox 2=g a ox 1 l}1
\newline
Равенства
\newline
\FrameEqRef[fg{\SideNS}{\Cols}]{f2=a f1 a-}{g \SideNS-\Cols}
\newline
и
\newline
\FrameEqRef{a ox 2=g a ox 1 l}1
\newline
похожи.
Из равенства
\newline
\FrameEqRef{a ox 2=g a ox 1 g l}1
\newline
следует, что образ линейного отображения
не зависит от выбора базиса.

Пусть множество тензоров
\FrameEqRef{akj1n .ox.}1
является координатами полилинейного отображения $a$
относительно базиса \eV[k], $k=1$, $2$.
Тогда
\newline
\FrameEqRef{a ox 2=g a ox 1}1
\newline
Из равенства
\newline
\FrameEqRef{a ox 2=g a ox 1 g}1
\newline
следует, что образ полилинейного отображения
не зависит от выбора базиса.

Рассмотрим кососимметричное полилинейное отображение
\newline
\FrameEqRef{h=aubvc}1
\newline
Если мы рассмотрим выражение, подобное определителю,
\newline
\FrameEqRef{star uv-vu}1
\newline
то мы можем записать полилинейное отображение $h$ в виде
\newline
\FrameEqRef{h=1/2 aubvc 1}1
\newline
Пусть множество тензоров
\FrameEqRef{akj1n .ox.}1
является координатами полилинейного отображения $h$
относительно базиса \eV[k], $k=1$, $2$.
Тогда
\newline
\FrameEqRef{huv=12 huv-hvu 5}1
}

\DefText{automorphism basis matrix}
{
Теоремы
\refTheorem{coordinate matrix of basis}{\Product-\Cols},
\refTheorem{active transformations, basis, vector space}{\SideNS-\Cols}
показывают связь между
\ProductType невырожденными матрицами,
базисами и автоморфизмами
\SideRu\Which $\Base$\Hyph \VectorSetRuB \ColsNA.
}

\DefText{endomorphism=matrix}
{
Следовательно, если выбран базис
\ShowEq{basis e of V}
левого $A$\Hyph векторного пространства $V$ столбцов,
то мы можем отождествить множество эндомоморфизмов
левого $A$\Hyph векторного пространства $V$
и множество $\gin\times\gin$ матриц.
Эта связь между эндоморфизмами и матрицами
будет видна глубже, если мы рассмотрим автоморфизмы.
}

\DefText{converse theorem is also true}
{
Обратная теорема также верна.
}

\DefLabeledSummary{homomorphism of vector space}{\SideNS}
{
\ShowEq{prolog homomorphism of vector space(1)}{}{}1{}{}2
Тогда гомоморфизм
\ShowEq{f:A->B}{\Vector f}VW
\SideRu вого $A$\Hyph векторного пространства имеет представление
\newline
\FrameEqRef[afVW]{f o (ae)=a o f e, vector space \Product-\Cols}1
\FrameEqRef[b{}a{}f{}]{v1=v2*a \SideNS-\Cols}1
\newline
относительно выбранных базисов.
Здесь
\begin{itemize}
%\setlength{\itemindent}{-1em}
\item
$a$ - координатная матрица вектора
$\Vector a$ относительно базиса $\Basis e_V$.
\item
$b$ - координатная матрица вектора
\DrawEq[abf]{vb=f(va)}-
относительно базиса $\Basis e_W$.
\item
$f$ - координатная матрица множества векторов
\ShowEq{(Vector f(e))}
относительно базиса $\Basis e_W$.
\end{itemize}
Матрица $f$ определена однозначно и называется
{\bf матрицей гомоморфизма}
$\Vector f$ относительно базисов $\Basis e_V$, $\Basis e_W$.

\ShowText{converse theorem is also true}

Отображение
\ShowEq{f:A->B}{\Vector f}VW
определённое равенством
\newline
\FrameEqRef[afVW]{f o (ae)=a o f e, vector space \Product-\Cols}1
\newline
является гомоморфизмом
\SideRu вого $A$\Hyph векторного пространства \ColsNA.
Гомоморфизм $\Vector f$, который имеет данную матрицу $f$,
определён однозначно.
}


==> Stmt.Module.English.tex <==
%auto-ignore
\input{Stmt.Module.Eq}

\DefExample{Abelian Group is Z module}
{
From theorems
\RefTheorem{action of ring of rational integers in Abelian group},
\RefTheorem{Abelian group is free}
and the definition
\refDefinition{module over algebra}{\SideWS \VectorSetNS},
it follows that free Abelian group $G$ is module over ring of integers $Z$.
}

\DefText[2]{ix-xi-1 roots}
{
the polynomial
\DrawEq[1]{ix-xi-1}{#1}
have no root
and the polynomial
\DrawEq[k]{ix-xi-1}{#2}
has the set of roots
\DrawEq{x=c12+j}{#2}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{module over ring}
Let commutative ring $D$ has unit $1$.
Effective representation
\DrawEq{D->*V}{def}
of ring $D$
in an Abelian group $V$
is called
\AddIndex{module over ring}{module over ring} $D$
or
\AddIndex{$D$\Hyph module}{D module}.
Effective representation
\eqRef{D->*V}{def}
of commutative ring $D$ in an Abelian group $V$
is called
\AddIndex{vector space over field}{vector space over field} $D$
or
\AddIndex{$D$\Hyph vector space}{D vector space}.
\end{ShadedDefinition}
}
{... definition: module over ring}
%\DefEq

\DefTheorem{tensor product of D-algebras is D-algebra}
{
Let
\ShowEq{A1...n}
be $D$\Hyph algebras.
Tensor product
$\Tensor A$
of $D$\Hyph modules
\ShowEq{A1...n}
is $D$\Hyph algebra,
if we define product by the equality
\ShowEq{xA1n*xA1n->oxA1n=}
}

\DefTheorem{representation of algebra H2 in LH}
{
Let product in algebra
\AoxA H
be defined according to rule
\DrawEq[pq]{product in algebra AA}{RH}
A representation
\DrawEq[RH]{h:AoxA->L(A)}H
of $R$\Hyph algebra
\AoxA H
in Abelian group
\ShowEq{L(A->B)}RHH{}
defined by the equality
\DrawEq[RH]{representation AA in LA}{RH}
is left \BoxB{H}module.
If we put $g=E$
where
\ShowEq{product in algebra AA 3}RHE
is identity map,
then we indentify the linear map
\DrawEq[fHH{}]{f: A->B}-
of quaternion algebra and tensor
\DrawEq{linear map f, basis E}1
using the following equality
\ShowEq{value of linear map f, basis E}
}

\DefProof{representation of algebra H2 in LH}
{
The theorem follows from the statement
that the map
\ShowEq{Eox=x}
generates any linear map of quaternion algebra.
}

\DefDefinition{square root}
{
The root
\ShowEq{square root}
of the equation
\DrawEq{x2=a}{root}
in $D$\Hyph algebra $A$
is called
\AddIndex{square root}{square root}
of $A$\Hyph number $a$.
}

\DefDefinition{polynomial*polynomial}
{
Bilinear map
\ShowEq{polynomial*polynomial}
is defined by the equality
\ShowEq{polynomial*polynomial, 1}
}

\DefTheorem{(a*b)x=(ax)(bx)}
{
For any tensors
\ShowEq{a in Aoxn}a{n+1},
\ShowEq{a in Aoxn}b{m+1}{},
product of homogeneous polynomials
\ShowEq{polynomials a o x,b o x}
is defined by the equality
\ShowEq{(a*b)x=(ax)(bx)}
}

\DefTheorem{x2=a quaternion root}
{
Let $H$ be quaternion algebra and $a$ be $H$\Hyph number.
\StartLabelItem
\begin{enumerate}
\item
Since
\ShowEq{Re sqrt a ne 0}
then the equation
\DrawEq{x2=a}{}
has roots
\ShowEq{x=x12}
such that
\ShowEq{x2=-x1}
\labelItem{Re sqrt a ne 0}
\item
Since $a=0$, then the equation
\DrawEq{x2=a}{}
has root $x=0$ with multiplicity $2$.
\labelItem{a=0}
\item
Since conditions
\RefItem{Re sqrt a ne 0},
\RefItem{a=0}
are not true,
then the equation
\DrawEq{x2=a}{}
has infinitly many roots such that
\ShowEq{|x|=sqrt a}
\labelItem{Re sqrt a=0}
\end{enumerate}
}

\DefDefinition{polylinear map of algebras, property}
{
The polylinear map of $D$\Hyph algebra $A$
\ShowEq{f:A->B}f{A^n}A
satisfies to equalities
\DrawEq[f]{f(ai+bi)=fai+fbi}{1}
\DrawEq[f]{f(pai)=pfai}{1}
\ShowEq{polylinear map of algebras, 1}AD
Let us denote
\ShowEq{set polylinear maps An}DAA
set of $n$\hyph linear maps
of $D$\Hyph algebra $A$.
}

\DefRemark{monomial of power k}
{
In the theorem
\RefTheorem{monomial of power k},
I considered recursive representation of a monomial in associative $D$\Hyph algebra.
Since product is independent of the way
in which brackets are placed,
recursive representation of a monomial is not unique
in associative $D$\Hyph algebra.
For instance, I can use any of the following forms
\ShowEq{ax^2bxcx^3d}
to represent monomial $ax^2bxcx^3d$.
I chose the equality
\EqRef{monomial of power k, F=1}
as the most simple for algorithm of division of polynomials.
}

\DefTheorem{monomial of power k}
{
Let $p_k(x)$ be
\AddIndex{monomial of power}{monomial of power} $k$
over associative $D$\Hyph algebra $A$.
Then
\StartLabelItem
\begin{enumerate}
\item
Monomial of power $0$ has form
\ShowEq{p0(x)=a0}
\item
If $k>0$, then
\labelItem{monomial of power k}
\ShowEq{monomial of power k, F=1}
where $a_k\in A$.
\end{enumerate}
}

\DefProof{monomial of power k}
{
We prove the theorem by induction over power
$n$ of monomial.

Let $n=0$.
We get the statement
\RefItem{monomial of power 0}
since monomial $p_0(x)$ is constant.

Let $n=k$. Last factor of monomial $p_k(x)$ is either $a_k\in A$,
or has form $x^l$, $l\ge 1$.
In the later case we assume $a_k=1$.
Factor preceding $a_k$ has form $x^l$, $l\ge 1$.
We can represent this factor as $x^{l-1}x$.
Therefore, we proved the statement.
}

\DefTheorem{r=+q circ p}
{
Let
\ShowEq{p=p circ x}
be polynomial of power $1$ and $p_1$ be nonsingular tensor.
Let
\ShowEq{r power k}
be polynomial of power $k$.
Then
\ShowEq{r=+q circ p}
where
\ShowEq{qij i j}
is homogeneous polynomial of power $i$.
}

\DefLabeledDefinition{linear map of A vector space}{\SideNS}
{
\ShowText{algebra over ring ()}
Let $V$, $W$ be \SideWS vector spaces over $D$\Hyph algebra $A$.
Linear map
\ShowEq{f:A->B}fVW
of $D$\Hyph vector space $V$
into $D$\Hyph vector space $W$
is called
\AddIndex{linear map}{linear map}
of \SideWS $A$\Hyph vector space $V$
into \SideWS $A$\Hyph vector space $W$.
Let us denote
\ShowEq{set linear maps, VW module}
set of linear maps
of \SideWS $A$\Hyph vector space $V$
into \SideWS $A$\Hyph vector space $W$.
}

\DefDefinition{component of linear map, basis E}
{
Expression
\ShowEq{component of linear map, basis E}
in equality
\eqRef{linear map f, basis E}1
is called
\AddIndex{component of linear map}
{component of linear map} $f$.
}

\DefTheorem{representation of algebra A2 in LA}
{
Let $A$ be $D$\Hyph algebra.
Let product in $D$\Hyph module
\AoxA A
be defined according to rule
\DrawEq[pq]{product in algebra AA}{}
A representation
\DrawEq[DA]{h:AoxA->L(A)}{}
of $D$\Hyph algebra
\AoxA A
in module
\ShowEq{L(A->B)}DAA{}
defined by the equality
\DrawEq[DA]{representation AA in LA}{}
allows us to identify tensor
\ShowEq{d in AxoA}A
and linear map
\ShowEq{product in algebra AA 2}DA{\delta}{}
where
\ShowEq{product in algebra AA 3}DA{\delta}
is identity map.
Linear map
\ShowEq{a ox b}{\delta}
has form
\ShowEq{a ox b c=}
}

\AddEq[1]{theorem: matrices fUD I}
{
\begin{ShadedTheorem}
\labelTheorem{#1, matrices fUD I}
Maps of conjugation
have
standard representation
\ShowEq{#1. standard representation I}
\end{ShadedTheorem}
}

\AddEq[2]{proof: matrices fUD I}
{
According to the equality
\EqRef{#2x= #1},
the map of conjugation
\ShowEq{Map of Conjugation}{#2}
has the matrix
\ShowEq{#1. matrix I#2}
The equality
\DrawEq[{#2}{}]{#1.fUD->fUU I}{#1#2}
follows from equalities
\EqRef{#1.fUD->fUU},
\EqRef{#1. matrix I#2}.
}

\DefTheorem{unit of algebra and ring}
{
Let $D$ be commutative ring.
Let $A$ be associative $D$\Hyph algebra with unit \(1_A\).
\StartLabelItem
\begin{enumerate}
\item
The map
\ShowEq{f:a in A->b in B}fdD{d1_A}A
is isomorphism of the ring $D$ into the center of the algebra $A$
and allows to identify \(D\)\Hyph number \(d\)
and \(A\)\Hyph number \(d\,1_A\).
\labelItem{isomorphism d->d1}
\item
The ring \(D\) is subalgebra of algebra $A$.
\labelItem{D is subalgebra of A}
\item
\ShowEq{D in Z(A)}
\end{enumerate}
}

\DefProof{unit of algebra and ring}
{
Let
\ShowEq{d12 in D}
According to the statement
\RefItem{distributive law, module},
\ShowEq{d1+d2 in A}
According to the definition
\RefDefinition{algebra over ring},
\ShowEq{d1 d2 in A}
The statement
\RefItem{isomorphism d->d1}
follows from equalities
\EqRef{d1+d2 in A},
\EqRef{d1 d2 in A}.
The statement
\RefItem{D is subalgebra of A}
follows from the statement
\RefItem{isomorphism d->d1}.

According to the definition
\RefDefinition{algebra over ring},
\ShowEq{ad=da in A}
The statement
\RefItem{D in Z(A)}
follows from the equation
\EqRef{ad=da in A}.
}

\DefTheorem{multiplication in algebra is distributive over addition}
{
The multiplication in the algebra $A$ is distributive over addition
\ShowEq{(a+b)c=.}
\ShowEq{a(b+c)=.}
}

\DefDefinition{module over commutative ring}
{
Effective representation of commutative ring $D$
in an Abelian group $V$
\DrawEq{D->*V}{module}
is called
\AddIndex{module over ring}{module over ring} $D$
or
\AddIndex{$D$\Hyph module}{D module}.
$V$\Hyph number is called
\AddIndex{vector}{vector}.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
If $D$ is a field, then the Abelian group $V$
is called
\AddIndex{vector space}{vector space} over field $D$
or
\AddIndex{$D$\Hyph vector space}{D vector space}.
\fi
}

\DefDefinition{linear map of algebra}
{
\ShowEq{def DModule}
\ShowEq{=DD}
Linear map
%\ShowEq{f:A->B}fHH
%of quaternion algebra $H$
\ShowEq{f:A->B}fAA
of $D$\Hyph algebra $A$
satisfies to equalities
\DrawEq[fab]{f(a+b)=...}{D }
\DrawEq[{}fa]{f(da)=h... module}{module}
\ShowEq{D ab in A, d in D}DA
Let us denote
%\ShowEq{set linear maps, module}RHH
\ShowEq{set linear maps, module}DAA
set of linear maps
%of quaternion algebra $H$.
of $D$\Hyph algebra $A$.
}

\DefLabeledDefinitionNote{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Coproduct in category of \SideWS $\Base$\Hyph \VectorsSet is called
\AddIndex{direct sum}{direct sum}.\,\footnotemark
We will use notation
\ShowEq{direct sum of modules}{\Module}{\ModuleA}
for direct sum of \SideWS $\Base$\Hyph \VectorsSet $V$ and $W$.
}{
See also the definition
of direct sum of modules in
\citeBib{Serge Lang},
page 128.
On the same page, Lang proves the existence of direct sum of modules.
}

\DefLabeledTheorem{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Let
\ShowEq{set Bi}{\Module}
be set of \SideWS $\Base$\Hyph \VectorsSetNS.
Then the representation
\ShowEq{\SideWS D->*o+A}{\Base}{\Module}{\ANumber}{\VNumber}
of the \algebraa $\Base$
in direct sum of Abelian groups
\ShowEq{o+Ai}{\Module}
is direct sum of \SideWS $\Base$\Hyph modules
\ShowEq{o+Ai}{\Module}
}

\DefProof{direct sum of D modules}
{
Let
\ShowEq{set f:A->B}f{\Module_i}W
be set of linear maps into \SideWS $\Base$\Hyph module $W$.
We define the map
\ShowEq{f:A->B}f{\Module}{\ModuleA}
by the equality
\DrawEq{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
The sum in the right side of the equality
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
is finite, since all summands, except for a finite number, equal $0$.
From the equality
\ShowEq{fi(x+y)=}
and the equality
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS},
it follows that
\ShowEq{f(x+y)i=}
From the equality
\ShowEq{fi(dx)=}
and the equality
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS},
it follows that
\ShowEq{f(dx)i=}
Therefore, the map $f$ is linear map.
The equality
\ShowEq{flj=fj}
follows from equalities
\EqRef{lj(x)=0x0},
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
Since the map $\lambda_i$ is injective,
then the map $f$ is unique.
Therefore, the theorem folows from definitions
\RefDefinition{coproduct in category},
\RefDefinition{direct sum of Abelian groups}.
}

\DefProof{cr-power, 1}
{
The equality
\ShowEq{cr-power, 1 1}
follows from equalities
\eqRef{cr power, 0}1,
\eqRef{cr-power, n}1.
The equality
\EqRef{cr-power, 1}
follows from the equality
\EqRef{cr-power, 1 1}.
}

\DefProof{rc-power, 1}
{
The equality
\ShowEq{rc-power, 1 1}
follows from equalities
\eqRef{rc power, 0}1,
\eqRef{rc-power, n}1.
The equality
\EqRef{rc-power, 1}
follows from the equality
\EqRef{rc-power, 1 1}.
}

\DefTheorem{a in ZAb=>b in ZAa}
{
Since
\ShowEq{c in ZAa}ab,
then
\ShowEq{c in ZAa}ba.
}

\DefProof{a in ZAb=>b in ZAa}
{
Let
\ShowEq{c in ZAa}ab.
The equality
\DrawEq{ab=ba}Z
follows from the statement
\eqRef{c in S=>bc=cb}{Z(A,b)}.
The theorem follows from the equality
\eqRef{ab=ba}Z.
}

\DefTheorem{a in ZAb, c in ZA=>a in ZAbc}
{
Since
\ShowEq{c in ZAa}ab{}
and
\ShowEq{c in ZA}c
then
\ShowEq{c in ZAa}a{bc}.
}

\DefProof{a in ZAb, c in ZA=>a in ZAbc}
{
The equality
\ShowEq{a(bc)=...=(bc)a}
follows from definitions
\RefDefinition{nucleus of algebra},
\RefDefinition{center of algebra}
and from the theorem
\RefTheorem{c in S=>bc=cb submodule of A}.
The theorem follows from the equality
\EqRef{a(bc)=...=(bc)a}
and from the theorem
\RefTheorem{c in S=>bc=cb submodule of A}.
}

\DefTheorem{c in Za=> p(c) in Za}
{
Let $A$ be non\Hyph commutative $D$\Hyph algebra.
For any $a\in A$, if
\ShowEq{c in ZAa}ca,
then
\DrawEq[{p(c)}a{}{}]{c in ZAa}1
for any polynomial
\DrawEq{p(c) p in D}1
}

\DefProof{c in Za=> p(c) in Za}
{
}

\DefTheorem{c in S=>bc=cb submodule of A}
{
Let $A$ be non\Hyph commutative $D$\Hyph algebra.
For any $b\in A$, there exists subalgebra
\ShowEq{center of A number}
of $D$\Hyph algebra $A$ such that
\DrawEq[{Z(A,b)}{}]{c in S=>bc=cb}{Z(A,b)}
$D$\Hyph algebra
\ShowEq{center Ac}{}
is called
\AddIndex{center of $A$\Hyph number}{center of A number}
$b$.
}

\DefProof{c in S=>bc=cb submodule of A}
{
The subset
\ShowEq{center Ac}{}
is not empty because
\ShowEq{c in ZAa}0b,
\ShowEq{c in ZAa}bb.
Let
\ShowEq{d in D c in S 12}
Then
\ShowEq{dcb=bdc}
And this implies
\ShowEq{dc in S}
Therefore, the set
\ShowEq{center Ac}{}
is $D$\Hyph module.

Let
\ShowEq{c in ZAb}
Then
\ShowEq{c1c2 in ZAb}
From the equality
\EqRef{c1c2 in ZAb},
it follows that
\ShowEq{c1 c2 in ZAb}
Therefore, $D$\Hyph module
\ShowEq{center Ac}{}
is $D$\Hyph algebra.
}

\DefTheorem{set of maps B->A is Abelian group}
{
Let $A$ be algebra over commutative ring $D$.
For any set $B$,
the set of maps $A^B$ is Abelian group with respect to operation
\ShowEq{(f+g)x=}x
}

\DefProof{set of maps B->A is Abelian group}
{
The theorem follows from definitions
\refDefinition{module over algebra}{\SideWS \VectorSetNS},
\RefDefinition{algebra over ring}.
}

\DefLabeledDefinition{module over algebra}{\SideWS \VectorSetNS}
{
Let $\Base$ be \Algebra.
Effective \SideNS\SidePresentation representation
\DrawEq{\SideWS \Base->*V}{\SideWS \VectorSetNS}
of \ShortAlgebraWS $\Base$
in \SetRepresentation $V$
is called
\AddIndex{\SideWS \VectorSet}{\SideWS \VectorSetNS}
over \ShortAlgebraWS $\Base$.
We will also say that \SetRepresentation $V$ is
\AddIndex{\SideWS $\Base$\Hyph \VectorSetNS}{\SideWS A \VectorSetNS}.
$V$\Hyph number is called
\AddIndex{vector}{vector}.
Bilinear map
\DrawEq{\SideWS \Base*V->V}{\VectorSet}
generated by \SideNS\SidePresentation representation
\DrawEq{\Base*V->V to \SideWS product}{\VectorSetNS}
is called
%\AddIndex{\SideNS\SidePresentation product}{\SideNS\SidePresentation product}
\SideNS\SidePresentation product
of vector over scalar.
}

\DefLabeledTheorem{module over algebra}{\SideNS}
{
The following diagram of representations describes \SideWS $\Base$\Hyph module $V$
\DrawEq[{}{}{}{}]{diagram of representations, \SideWS module}1
The diagram of representations
\eqRef{diagram of representations, \SideWS module}1
holds
\AddIndex{commutativity of representations}{commutativity of representations}
\BaseRings
in Abelian group $V$
\ShowEq{\SideWS module, a d v}
}

\DefProof{module over algebra}
{
The diagram of representations
\eqRef{diagram of representations, \SideWS module}1
follows from the definition
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
and from the theorem
\def\Temp{}
\ifx\SideNS\Temp
\RefTheorem{action of ring of rational integers in Abelian group}.
\else
\RefTheorem{Free Algebra over Ring}.
\fi
Since \SideNS\HSide transformation $\ATransf(a)$
is endomorphism
of $\CBase$\Hyph module $V$,
we obtain the equality
\EqRef{\SideWS module, a d v}.
}

\DefProof{Free Algebra over Ring}
{
The structure of $D$\Hyph module $A$ is generated by effective representation
\ShowEq{f:A->*B}{g_{12}}DA
of ring $D$ in Abelian group $A$.

\begin{ShadedLemma}
\labelLemma{structure of D algebra is generated by product}
{\it
Let the structure of $D$\Hyph algebra $A$
defined in $D$\Hyph module $A$,
be generated by product
\DrawEq{product in D algebra}{}
\AddIndex{Left shift of $D$\Hyph module $A$}{left shift of module}
defined by equation
\ShowEq{l(v):w->vw}
generates the representation
\ShowEq{endomorphism of module from product, 1}
of $D$\Hyph module $A$
in $D$\Hyph module $A$
}
\end{ShadedLemma}

{\sc Proof.}
According to definitions
\RefDefinition{algebra over ring}
and
\RefDefinition{polylinear map of modules},
left shift of $D$\Hyph module $A$
is linear map.
According to the definition
\refDefinition{linear map of D module}1,
the map \(l(v)\)
is endomorphism of $D$\Hyph module $A$.
The equation
\ShowEq{l(v1+v2)w}
follows from the definition
\RefDefinition{polylinear map of modules}
and from the equation
\EqRef{l(v):w->vw}.
\ShowEq{def sum of linear maps}
\ShowEq{ref sum of linear maps}
the equation
\ShowEq{l(v1+v2)}
follows from equation
\EqRef{l(v1+v2)w}.
The equation
\ShowEq{l(dv)w}
follows from the definition
\RefDefinition{polylinear map of modules}
and from the equation
\EqRef{l(v):w->vw}.
\ShowEq{ref sum of linear maps}
the equation
\ShowEq{l(dv)}
follows from equation
\EqRef{l(dv)w}.
The lemma follows from equalities
\EqRef{l(v1+v2)},
\EqRef{l(dv)}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{representation of D module in D module determines the product}
{\it
The representation
\ShowEq{endomorphism of module from product, 1}
of $D$\Hyph module $A$ in $D$\Hyph module $A$
determines the product in
$D$\Hyph module $A$ according to rule
\ShowEq{endomorphism of module from product, 8}
}
\end{ShadedLemma}

{\sc Proof.}
Since map $g_{23}\circ v$ is endomorphism of $D$\Hyph module $A$, then
\ShowEq{endomorphism of module from product, 3}
Since the map $g_{23}$ is
linear map
\ShowEq{g23:A->L}
then,
\ShowEq{ref sum and product over scalar, linear map}
\ShowEq{endomorphism of module from product, 4}
\ShowEq{endomorphism of module from product, 7}
From equations
\EqRef{endomorphism of module from product, 3},
\EqRef{endomorphism of module from product, 4},
\EqRef{endomorphism of module from product, 7}
and the definition
\RefDefinition{polylinear map of modules},
it follows that the map $g_{23}$ is bilinear map.
Therefore, the map $g_{23}$ determines the product in
$D$\Hyph module $A$ according to rule
\ShowEq{endomorphism of module from product, 8}
\hfill\(\odot\)

The theorem follows from lemmas
\RefLemma{structure of D algebra is generated by product},
\RefLemma{representation of D module in D module determines the product}.
}

\DefLabeledTheorem{A module -> algebra is associative}{\SideNS}
{
Let $g$ be effective left\Hyph side representation of $D$\Hyph algebra $A$
in $D$\Hyph module $V$.
Then $D$\Hyph algebra $A$ is associative.
}

\DefProof{A module -> algebra is associative}
{
Let
\ShowEq{abc in A, v in v}
Since \SideNS\Hyph side representation
$g$ is \SideNS\Hyph side representation
of the multiplicative group
of $D$\Hyph algebra $A$,
we obtain the equality
\DrawEq{\SideWS module, associative law}0
The equality
\ShowEq{a(b(cv))=(a(bc))v \SideNS}
follows from the equality
\eqRef{\SideWS module, associative law}0.
Since
\ShowEq{cv \SideNS}
the equality
\ShowEq{a(b(cv))=((ab)c)v \SideNS}
follows from the equality
\eqRef{\SideWS module, associative law}0.
The equality
\ShowEq{(a(bc))v=((ab)c)v \SideNS}
follows from equalities
\EqRef{a(b(cv))=(a(bc))v \SideNS},
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Since $v$ is any vector of $A$\Hyph module $V$,
the equality
\ShowEq{a(bc)=(ab)c \SideNS}
follows from the equality
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Therefore, $D$\Hyph algebra $A$ is associative.
}

\DefLabeledTheoremNote{definition of A module}{\SideWS \VectorSetNS}
{
Let $V$ be \SideWS $\Base$\Hyph module.
For any vector $v\in V$,
vector generated by the diagram of representations
\eqRef{diagram of representations, \SideWS module}1
has the following form
\ShowEq{\SideWS module, (a+n)v=av+nv}
\StartLabelItem
\begin{enumerate}
\item
The set of maps
\ShowEq{\SideWS module, a+n:V->V}
generates\,\footnotemark
\algebraa $\Base_{(1)}$
where the sum is defined by the equality
\DrawEq{(a+n)+(b+m)=}{\SideWS module}
and the product is defined by the equality
\DrawEq{(a+n)(b+m)=}{\SideWS module}
The \algebraa $\Base_{(1)}$ is called
\AddIndex{unital extension}{unital extension}
of the \algebraa $\Base$.
\begin{table}[h]
%\caption{Active and Passive Representations}
%\label{table:Passive and Active Representations}
\begin{tabular}{|l|l|l|}
\hline
If \algebraa $\Base$ has unit, then
\ShowEq{A1=A unital extension}
If \algebraa $\Base$ is ideal of $\CBase$, then
\ShowEq{A1=D unital extension}
Otherwise
\ShowEq{A1=A+D unital extension}
\end{tabular}
\end{table}
\item
The \algebraa $\Base$ is \SideWS ideal of \algebraa $\Base_{(1)}$.
\labelItem{Algebra is \SideWS ideal of algebra (1)}
\item
The set of transormations
\EqRef{\SideWS module, (a+n)v=av+nv}
is \SideNS\HSide representation of \algebraa $\Base_{(1)}$ in Abelian group $V$.
\labelItem{\SideWS representation of D1 in Abelian group}
\end{enumerate}
We use the notation
\ShowEq{set of vectors generated by vector \Base}
for the set of vectors generated by vector $v$.
}
{See the definition of unital extension also on the pages
\citeBib{McCrimmon: Jordan Algebras}\Hyph 52,
\citeBib{Zharinov: foundation of mathematical physics}\Hyph 64.}

\DefLabeledTheorem{definition of A module, property}{\SideNS}
{
Following conditions hold for \SideWS $\Base$\Hyph module $V$:
\StartLabelItem
\begin{enumerate}
\item 
\AddIndex{associative law}{associative law}
\labelItem{associative law, \SideWS module}
\DrawEq{associative law, \SideWS module}1
\item 
\AddIndex{distributive law}{distributive law}
\labelItem{distributive law, \SideWS module}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{unitarity law}{unitarity law}
\labelItem{unitarity law, \SideWS \Base-module}
\ShowEq{unitarity law, \SideWS \Base-module}
\end{enumerate}
for any
\ShowEq{p,q in D, v,w in V}
}

\AddEq{proof: definition of A module}
{%
{\sc Proof of theorems
\refTheorem{definition of A module}{\SideWS \VectorSetNS},
\refTheorem{definition of A module, property}{\SideNS}.}
Let $v\in V$.

\begin{ShadedLemma}
\labelLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}
{\it
Let
\ShowEq{module, d in D}
\ShowEq{module, a in A}
The map
\EqRef{\SideWS module, a+n:V->V}
is endomorphism of Abelian group $V$.
}
\end{ShadedLemma}

{\sc Proof.}
Statements
\ShowEq{\SideWS module, dv in V}
\ShowEq{\SideWS module, av in V}
follow from the theorems
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{module over algebra}{\SideNS}.
Since $V$ is Abelian group, then
\ShowEq{\SideWS module, dv+av in V}
Therefore,
for any $\CBase$\Hyph number $\DArg$
and for any $\Base$\Hyph number $a$,
we defined the map
\EqRef{\SideWS module, a+n:V->V}.
Since transformation $\DTransf(\DArg)$
and \SideNS\HSide transformation $\ATransf(a)$
are endomorphisms of Abelian group $V$,
then the map
\EqRef{\SideWS module, a+n:V->V}
is endomorphism of Abelian group $V$.
\hphantom{aaaa}\hfill\(\odot\)

Let $\Base_{(1)}$ be the set of maps
\EqRef{\SideWS module, a+n:V->V}.
The equality
\eqRef{distributive law, \SideWS module, 1}1
follows from the lemma
\RefLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}.

Let
\ShowEq{p,q in D1}
According to the statement
\RefItem{representation of D1 in Abelian group},
we define the sum of $\Base_{(1)}$\Hyph numbers $p$ and $q$ by the equality
\eqRef{distributive law, \SideWS module, 2}1.
The equality
\ShowEq{\SideWS module, (a+n)+(b+m)=, 1}
follows from the equality
\eqRef{distributive law, \SideWS module, 2}1.
Since representation
$\DTransf$ is homomorphism of the aditive group of ring $\CBase$,
we obtain the equality
\ShowEq{distributive law, \CBase, \SideWS module, 2}
Since \SideNS\HSide representation
$\ATransf$ is homomorphism of the aditive group of \algebraa $\Base$,
we obtain the equality
\ShowEq{distributive law, \Base, \SideWS module, 2}
Since $V$ is Abelian group, then the equality
\ShowEq{\SideWS module, (a+n)+(b+m)=}
follows from equalities
\EqRef{\SideWS module, (a+n)+(b+m)=, 1},
\EqRef{distributive law, \CBase, \SideWS module, 2},
\EqRef{distributive law, \Base, \SideWS module, 2}.
From the equality
\EqRef{\SideWS module, (a+n)+(b+m)=},
it follows that the definition
\eqRef{(a+n)+(b+m)=}{\SideWS module}
of sum on the set $\Base_{(1)}$ does not depend on vector $v$.

Equalities
\eqRef{associative law, \SideWS module}1,
\EqRef{unitarity law, \SideWS \Base-module}
follow from the statement
\RefItem{\SideWS representation of D1 in Abelian group}.
Let
\ShowEq{p,q in D1}
\def\Temp{}
\ifx\SideNS\Temp
Since representation $\DTransf$ is representation
of the multiplicative group of ring $\CBase$,
we obtain the equality
\DrawEq{associative law, \CBase, \SideWS module}1
Since representation $g_2$ is representation
of the multiplicative group of ring $D$,
we obtain the equality
\DrawEq{\SideWS module, associative law}1
Since the ring $D$
is Abelian group,
we obtain the equality
\DrawEq{associative law, \CBase\Base, \SideWS module}1
The equality
\ShowEq{module, (a+n)(b+m)=}
follows from equalities
\ShowEq{ref module, (a+n)(b+m)=}
The equality
\eqRef{(a+n)(b+m)=}{\SideWS module}
follows from the equality
\EqRef{module, (a+n)(b+m)=}.
\else%
Since the product in $D$\Hyph algebra $A$ can be non associative,
then, based on the theorem
\refTheorem{definition of A module, property}{\SideNS},
we consider product
of $\Base_{(1)}$\Hyph numbers $p$ and $q$
as bilinear map
\ShowEq{f:D1xD1->D1}
such that following equalities are true
\DrawEq{fab=ab}{\SideWS module}
\DrawEq{f1p=p}{\SideWS module}
The equality
\DrawEq{pq=fpq}{\SideWS module}
follows from equalities
\eqRef{fab=ab}{\SideWS module},
\eqRef{f1p=p}{\SideWS module}.
The equality
\eqRef{(a+n)(b+m)=}{\SideWS module}
follows from the equality
\eqRef{pq=fpq}{\SideWS module}.
\fi%

The statement
\RefItem{Algebra is \SideWS ideal of algebra (1)}
follows from the equality
\eqRef{(a+n)(b+m)=}{\SideWS module}.
\qed
}

\DefLabeledDefinition{submodule}{\SideWS module}
{
Subrepresentation of \SideWS $\Base$\Hyph module $V$ is called
\AddIndex{submodule}{submodule}
of \SideWS $\Base$\Hyph module $V$.
}

\AddEq{theorem: submodule}
{
\begin{ShadedTheorem}
\labelTheorem{submodule, \SideWS module}
Let
\ShowEq{vi V}{}
be set of vectors of \SideWS $\Base$\Hyph module $V$.
If vectors
\ShowEq{set vi cols}v
belongs submodule $V'$ of \SideWS $\Base$\Hyph module $V$,
then linear combination of vectors
\ShowEq{set vi cols}v
belongs submodule $V'$.
\end{ShadedTheorem}
}

\DefProof{submodule}
{
The theorem follows from
the theorem
\refTheorem{set of vectors generated by set of vectors}{\SideWS module}
and definitions
\refDefinition{linear combination of vectors}{\SideNS},
\refDefinition{submodule}{\SideWS module}.
}

\AddEq{ref in item cvk module}
{
theorems
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{definition of A \VectorSetNS}{\SideNS}
}

\AddEq{ref in item cvk vector space}
{
the theorem
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
the definition
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
}

\DefLabeledTheorem{set of automorphisms}{\SideNS}
{
The set $GL(V)$
of automorphisms
of \SideWS $A$\Hyph vector space $V$
is group.
}

\DefLabeledTheorem{active transformations in module}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Any automorphism $\Vector f$ of \SideWS $A$\Hyph vector space $V$
has form
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{automorphism}
where $f$ is a \ProductType nonsingular matrix.
Matrices of automorphisms of \SideWS $A$\Hyph vector space $V$ of \ColN s form a group
$GL(V_*)$
isomorphic to group $GL(V)$.
%\Group nA.
Automorphisms of \SideWS $A$\Hyph vector space of \ColsWS form
a \OtherSideNS\Hyph side linear
effective representation
\DrawEq[{GL(V_*)}{V_*}{}]{A->*B}{\SideNS-\Cols}
of the group $GL(V_*)$
in \SideWS $A$\Hyph vector space $V_*$.
}

\DefLabeledTheoremNote{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
{
Let $V$ be \SideWS $\Base$\Hyph \VectorSetNS.
The set of vectors generated by the set of vectors
\ShowEq{v(i) V}{}
has form\,\footnotemark
\DrawEq[{\Base}{\BaseExt}]{w=sum vi, \SideWS module}{\Base}
}
{For a set $A$,
we denote by $|A|$ the cardinal number of the set $A$.
The notation $|A|<\infty$ means that the set $A$ is finite.}

\AddEq{ref module structure of subrepresentations}
{
and theorems
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{definition of A module}{\SideWS \VectorSetNS},
}

\AddEq{ref vector space structure of subrepresentations}
{
and the theorems
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
}

\DefLabeledLemma{w=w12 in Xk-1}{\SideWS \VectorSetNS}
{\leftskip=25pt
Let
\ShowEq{w=w12 in Xk-1}.
Then $w\in J(v)$.
}

\DefLabeledLemma{w=aw in Xk-1}{\SideWS \VectorSetNS}
{\leftskip=25pt
Let
\ShowEq{w=aw in Xk-1,\SideNS}
Then $w\in J(v)$.
}

\DefProof{set of vectors generated by set of vectors}
{
We prove the theorem by induction based on the theorem
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

For any
\ShowEq{vk in Jv},
let
\ShowEq{c(i)=dik}
Then
\DrawEq[{\Base_{\BaseExt}}{}]{v(k)=sum v(i), \SideWS module}{\Base}
From equalities
\eqRef{w=sum vi, \SideWS module}{\Base},
\eqRef{v(k)=sum v(i), \SideWS module}{\Base},
it follows that
the theorem is true on the set
\ShowEq{X0=v in J}

Let
\ShowEq{Xk in Jv}{k-1}
Acording to the definition
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
\ShowEq{ref \VectorSet structure of subrepresentations}
if $w\in X_k$, then or
\ShowEq{w=w12 in Xk-1},
either
\ShowEq{w=aw in Xk-1,\SideNS}

{\leftskip=25pt
\ShowLemma{w=w12 in Xk-1}

{\sc Proof.}
According to the equality
\eqRef{w=sum vi, \SideWS module}{\Base},
there exist $\Base_{\BaseExt}$\Hyph numbers
\ShowEq{g(i)12}w
such that
\DrawEq[w]{w()12= \SideNS}{\VectorSetNS}
where sets
\DrawEq[w]{|c(i)12 ne 0|}{\SideWS \VectorSetNS}
are finite.
Since $V$ is \SideWS $\Base$\Hyph \VectorSetNS,
then from equalities
\eqRef{distributive law, \SideWS module, 2}1,
\eqRef{w()12= \SideNS}{\VectorSetNS},
it follows that
\DrawEq[w]{w()1+w()2= \SideNS}{\VectorSetNS}
From the equality
\eqRef{|c(i)12 ne 0|}{\SideWS \VectorSetNS},
it follows that
the set
\ShowEq{|gi() 1+2 ne 0|}w
is finite.
\hfill\(\odot\)

\ShowLemma{w=aw in Xk-1}

{\sc Proof.}
According to the statement
\RefItem[\RefRepresentation]{ax in Xk+1},
for any $\Base_{\BaseExt}$\Hyph number $a$,
\ShowEq{aw in Xk \SideWS module}
According to the equality
\eqRef{w=sum vi, \SideWS module}{\Base},
there exist $\Base_{\BaseExt}$\Hyph numbers
\ShowEq{set au v(i)}w
such that
\ShowEq{w()= \SideWS module}
where
\DrawEq{|w(i) ne 0|}{\SideWS module}
From the equality
\EqRef{w()= \SideWS module}
it follows that
\ShowEq{aw()= \SideWS module}
From the statement
\eqRef{|w(i) ne 0|}{\SideWS module},
it follows that
the set
\ShowEq{\SideWS module, |aw(i) ne 0|}
is finite.
\hfill\(\odot\)

\,
}

From lemmas
\refLemma{w=w12 in Xk-1}{\SideWS \VectorSetNS},
\refLemma{w=aw in Xk-1}{\SideWS \VectorSetNS},
it follows that
\ShowEq{Xk in Jv}k
}

\DefLabeledTheorem{d in D->d in D1}{\SideWS module}
{
The map
\ShowEq{f:a in A->b in B}{I_{(1)}}d{\Base}{d+0}{\Base_{(1)}}
is homomorphism of \algebraa $\Base$
into \algebraa $\Base_{(1)}$.
}

\DefProof{d in D->d in D1}
{
The equality
\DrawEq[{\AArg}]{(d1+0)+(d2+0)}{\SideWS module}
follows from the equality
\eqRef{(a+n)+(b+m)=}{\SideWS module}.
The equality
\DrawEq[{\AArg}]{(d1+0)(d2+0)}{\SideWS module}
follows from the equality
\eqRef{(a+n)(b+m)=}{\SideWS module}.
The theorem follows from equalities
\eqRef{(d1+0)+(d2+0)}{\SideWS module},
\eqRef{(d1+0)(d2+0)}{\SideWS module}.
}

\DefLabeledTheorem{da in DA->da in D1A}{\SideWS module}
{
The map
\ShowEq{da in DA->da in D1A}
is morphism of \SideWS $\Base$\Hyph module $V$
into \SideWS $\Base_{(1)}$\Hyph module $V$.
}

\DefProof{da in DA->da in D1A}
{
The equality
\ShowEq{da in DA->da in D1A 1, \SideWS module}
follows from the theorem
\refTheorem{d in D->d in D1}{\SideWS module}.
The theorem follows from the equality
\EqRef{da in DA->da in D1A 1, \SideWS module}
and the definition
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra}.
}

\AddEq{convention: da in DA->da in D1A}
{
\begin{convention}
\labelConvention{da in DA->da in D1A, \SideWS module}
According to theorems
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\refTheorem{da in DA->da in D1A}{\SideWS module},
the set of words generating
\SideWS $\Base$\Hyph module $V$,
is the same as the set of words generating
\SideWS $\Base_{(1)}$\Hyph module $V$.
Therefore, without loss of generality,
we will assume that \algebraa $\Base$
has unit.
\qed
\end{convention}
}

\DefLabeledConvention{linear combination of vectors}{\SideNS}
{
If it is necessary to explicitly show
that we multiply vector $v(\gii)$
over $\Base_{\BaseExt}$\Hyph number $c(i)$ on the \SideNS,
then we will call the expression
\ShowEq{the \SideWS linear combination()}
\AddIndex{\SideWS linear combination}{\SideWS linear combination}.
We will use this convention to similar terms.
For instance, we will say that a vector
\ShowEq{w=c(i)v(i).\SideNS}
linearly depends
on vectors
\ShowEq{set vi *}v
on the \SideNS.
}

\DefLabeledDefinition{linear combination of vectors}{\SideNS}
{
Let $\Module$ be \SideNS\HSide \VectorSetNS.
Let
\ShowEq{v(i) V}{}
be set of vectors.
\ShowEq{\SideWS linear combination()}%
The expression
\ShowEq{A linear combination() =}
is called
\AddIndex{linear combination}{linear combination} of vectors
\ShowEq{v(i)}
A vector
\ShowEq{w=c(i)v(i).\SideNS}
is called
\AddIndex{linearly dependent}{linearly dependent}
on vectors
\ShowEq{v(i)}
}

\DefLabeledDefinition{generating set of module}{\SideNS}
{
$J(v)$
is called
\AddIndex{submodule generated by set}
{submodule generated by set} $v$,
and $v$ is a
\AddIndex{generating set}{generating set}
of submodule $J(v)$.
In particular, a
\AddIndex{generating set}{generating set}
of \SideWS $\Base$\Hyph module $V$
is a subset $X\subset V$ such that
\ShowEq{generating set of module}
}

\DefLabeledDefinition{generating set of vector space}{\SideNS}
{
$J(v)$
is called
vector subspace generated by set $v$,
and $v$ is a
\AddIndex{generating set}{generating set}
of vector subspace $J(v)$.
In particular, a
\AddIndex{generating set}{generating set}
of \SideWS $\Base$\Hyph vector space $V$
is a subset $X\subset V$ such that
\ShowEq{generating set of module}
}

\DefText{generating set of module}
{
The following definition follows from the theorems
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
and from the definition
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\DefText{quasibasis of module}
{
The following definition follows from the theorems
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
and from the definition
\RefDefinition[\RefRepresentation]{basis of representation}.
}

\DefLabeledDefinition{basis of module}{\SideNS}
{
If the set $X\subset V$ is generating set of \SideWS $\Base$\Hyph \VectorSet
$V$, then any set $Y$, $X\subset Y\subset V$
also is generating set of \SideWS $\Base$\Hyph \VectorSet $V$.
If there exists minimal set $X$ generating
the \SideWS $\Base$\Hyph \VectorSet $V$, then the set $X$ is called
\AddIndex{quasibasis}{quasibasis} of \SideWS $\Base$\Hyph \VectorSet $V$.
}

\DefLabeledTheorem{linearly depends on rest of vectors}{\SideWS module}
{
Let $\Base$ be \DivAlgebra.
Since the equation
\DrawEq[wv]{\SideWS wi vi=0}{1 \Cols}
implies existence of index
\ShowEq{i=j}
such that
\ShowEq{wj ne 0}w,
then the vector
\ARow vj{}
linearly depends on rest of vectors $v$.
}

\DefProof{linearly depends on rest of vectors}
{
The theorem follows from the equality
\ShowEq{\SideWS vj=sum vi}vw
and from the definition
\refDefinition{linear combination of vectors}{\SideNS}.
}

\DefText{0=0vi}
{
It is evident that for any set of vectors
\ARow vi{}
\ShowEq{\SideWS 0=0vi}
}

\DefLabeledDefinitionNote{linearly independent vectors}{\SideNS}
{
The set of vectors\,\footnotemark
\ShowEq{set vi *}v
of \SideWS $\Base$\Hyph \VectorSet $V$ is
\AddIndex{linearly independent}{linearly independent set}
if
\ShowEq{w(i)=0}
follows from the equation
\DrawEq{\SideWS w(i) v(i)=0}{}
Otherwise the set of vectors
\ShowEq{set vi *}v
is \AddIndex{linearly dependent}{linearly dependent set}.
}
{I follow to the definition in
\citeBib{Serge Lang}, page 130.}

\DefLabeledTheorem{quasibasis of module}{\SideNS}
{
The set of vectors
\ShowEq{basis, module}
is quasibasis of \SideWS $\Base$\Hyph module
$V$, if following statements are true.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{vector is linear combination of set, \SideWS module}
Arbitrary vector $v\in V$
is linear combination of
vectors of the set $\Basis e$.
\item
\labelItem{cannot be represented as a linear combination, \SideWS module}
Vector $e(\gii)$
cannot be represented as a linear combination
of the remaining vectors of the set $\Basis e$.
\end{enumerate}
}

\DefProof{quasibasis of module}
{
According to the statement
\RefItem{vector is linear combination of set, \SideWS module},
the theorem
\refTheorem{set of vectors generated by set of vectors}{\SideWS module}
and the definition
\refDefinition{linear combination of vectors}{\SideNS},
the set $\Basis e$ generates \SideWS $\Base$\Hyph module $V$
(the definition
\refDefinition{generating set of module}{\SideNS}).
According to the statement
\RefItem{cannot be represented as a linear combination, \SideWS module},
the set $\Basis e$ is minimal set
generating \SideWS $\Base$\Hyph module $V$.
According to the definitions
\refDefinition{basis of  module}{\SideNS},
the set $\Basis e$ is a quasibasis of \SideWS $\Base$\Hyph module $V$.
}

\DefLabeledTheorem{basis over division algebra}{\SideNS}
{
Let $\Base$ be \Algebra.
The set of vectors
\ShowEq{basis, module}
is a
\AddIndex{basis of \SideWS $\Base$\Hyph vector space}{basis, vector space} $V$
if vectors
\ARow ei
are linearly independent and any vector $v\in V$
linearly depends on vectors
\ARow ei.
}

\DefLabeledTheorem{vector space is free module}{}
{
The \SideWS $\Base$\Hyph vector space
is free $\Base$\Hyph module.
}

\DefProof{basis over division algebra}
{
Let the set of vectors
\ShowEq{set vi \Cols}e
be linear dependent. Then the equation
\DrawEq[we]{\SideWS wi vi=0}{}
implies existence of index $\gii=\gij$ such that
\ShowEq{wj ne 0}w.
According to the theorem
\refTheorem{linearly depends on rest of vectors}{\SideWS module},
the vector
\ARow ej{}
linearly depends on rest of vectors of the set $\Basis e$.
According to the definition
\refDefinition{basis of module}{\SideNS},
the set of vectors
\ShowEq{set vi \Cols}e
is not a basis for \SideWS $\Base$\Hyph vector space $V$.

Therefore, if the set of vectors
\ShowEq{set vi \Cols}e
is a basis, then these vectors
are linearly independent.
Since an arbitrary vector $v\in V$
is linear combination of vectors
\ShowEq{set vi \Cols}e
then the set of vectors $v$,
\ShowEq{set vi \Cols}e
is not linearly independent.
}

\DefLabeledConvention{unit of algebra in basis}{\Cols}
{
Let \eV be the basis of $D$\Hyph algebra of \ColsWS $A$.
If $D$\Hyph algebra $A$ has unit,
then we assume that \ARow e0 is the unit of $D$\Hyph algebra $A$.
}

\DefTheoremNote{algebra A2 representation in LA}
{
Let $A_1$ and $A_2$ be $D$\Hyph algebras.
Let product in algebra \AoxA A
be defined according to rule
\DrawEq[pq]{product in algebra AA}{A2}
A linear map
\ShowEq{representation A2 in LA}
defined by the equality
\ShowEq{representation A2 in LA, 1}
is representation\,\footnotemark
of algebra $\ATwo$
in module
\ShowEq{L(A->B)}D{A_1}{A_2}.
}
{See the definition of representation
of $\Omega$\Hyph algebra in the definition
\ShowEq{ref definition: representation of algebra}.}

\DefLabeledTheorem[4]{matrix generates D module homomorphism}{\Cols(#1#2)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrix of numbers}D{#3}fiIjJ
The map\refFootnote{homomorphism of D module}{\Cols(#1#2)}
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{module, coordinates \Cols}
%\newline
defined by the equality
\ShowText{define homomorphism D module by matrix(#1)}
is homomorphism
of $D_{#1}$\Hyph module $V_{#2}$
into $D_{#3}$\Hyph module $V_{#4}$.
The homomorphism
\eqRef{homomorphism D algebra #1#2}{module, coordinates \Cols}
which has the given%
\ShowText{define homomorphism by given matrix()}%
is unique.
}

\DefProof[5]{matrix generates D module homomorphism}
{
The equality
\ShowEq{fo(v+w) \Cols(#1)}
\begin{sloppypar}
\noindent
follows from equalities
\ShowRef{homomorphism of D module}{#1}{#2}{#5}
From the equality
\EqRef{fo(v+w) \Cols(#1)},
it follows that the map $\Vector f$ is homomorphism
of Abelian group.
The equality
\end{sloppypar}
\ShowEq{fo(va) \Cols(#1)}
follows from the equality
\eqRef{left homomorphism, f av=}{f D module #1#2}.
From the equality
\EqRef{fo(va) \Cols(#1)},
and definitions
\RefDefinition{Morphism of Diagram of Representations},
\refDefinition{linear map of D module}{#1#2},
it follows that the map
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{module, coordinates \Cols}
\newline
\begin{sloppypar}
\noindent
is homomorphism
of $D_{#1}$\Hyph module of \ColN s $V_{#2}$
into $D_{#3}$\Hyph module of \ColN s $V_{#4}$.
\end{sloppypar}

Let $f$ be
matrix of homomorphisms $\Vector f$, $\Vector g$
relative to bases
\ShowEq{Bases eVW}12{}.%
The equality
\ShowEq{fov=gov \Cols(#1)}
follows from the theorem
\refTheorem{linear map of D module}{#1#2}.
Therefore, $\Vector f=\Vector g$.
}

\DefLabeledTheorem[4]{matrix generates D algebra homomorphism}{\Cols(#1#2)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrix of numbers and C}D{#3}fiIjJ{#1}{#2}
The map\refFootnote{homomorphism of d algebra}{#1#2\Cols}
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{module, coordinates \Cols}
%\newline
defined by the equality
\ShowText{define homomorphism D module by matrix(#1)}
is homomorphism
of $D_{#1}$\Hyph algebra $A_{#2}$
into $D_{#3}$\Hyph algebra $A_{#4}$.
The homomorphism
\eqRef{homomorphism D algebra #1#2}{module, coordinates \Cols}
which has the given%
\ShowText{define homomorphism by given matrix()}%
is unique.
}

\DefProof[5]{matrix generates D algebra homomorphism}
{
According to the theorem
\refTheorem{matrix generates D module homomorphism}{\Cols(#1#2)},
the map
\eqRef{homomorphism D algebra #1#2}{module, coordinates \Cols}
is homomorphism
of $D_{#1}$\Hyph module $A_{#2}$
into $D_{#3}$\Hyph module $A_{#4}$
and the homomorphism
\eqRef{homomorphism D algebra #1#2}{module, coordinates \Cols}
is unique.

Let
\ShowEq{a=ai ei}a1i,
\ShowEq{a=ai ei}b1i.
The equality
\DrawEq{algebra, homomorphism and product abe #1#2}{\Cols}
follows from the equality
\eqRef{algebra, homomorphism and product #1#2}{\Cols}.
\ShowText{matrix generates D algebra homomorphism (#1)}
The equality
\DrawEq{algebra, homomorphism and product abe 3(#1)}{\Cols}
follows from the equality
\eqRef{algebra, homomorphism and product abe 2(#1)}{\Cols}
and the equality
\ShowRef{homomorphism of d algebra, coordinates 1}{#1}{#2}
The equality
\DrawEq{algebra, homomorphism and product abe 4(#1)}{\Cols}
follows from the equality
\ShowEq{algebra, homomorphism and product, 1}
The equality
\DrawEq{algebra, homomorphism and product abe 5(#1)}{\Cols}
follows from the equality
\eqRef{algebra, homomorphism and product abe 4(#1)}{\Cols}
and the equality
\ShowRef{homomorphism of d algebra, coordinates 1}{#1}{#2}
The equality
\ShowRef{homomorphism, f vw=}{#1}{#2}
follows from equalities
\ShowRef{algebra, homomorphism and product 1}{#1}{#2}
According to the theorem
\refTheorem{homomorphism from A1 to A2, D algebra}{#1#2},
the map
\eqRef{homomorphism D algebra #1#2}{module, coordinates \Cols}
is homomorphism
of $D_{#1}$\Hyph algebra $A_{#2}$
into $D_{#3}$\Hyph algebra $A_{#4}$.
}

\DefText{matrix generates D algebra homomorphism (1)}
{
Since the map $h$ is homomorphism
of the ring $D_1$ into the ring $D_2$, then
\DrawEq{algebra, homomorphism and product abe 2}{\Cols}
The equality
\DrawEq{algebra, homomorphism and product abe 2(1)}{\Cols}
follows from the equality
\eqRef{algebra, homomorphism and product abe 2}{\Cols}
and the equality
\ShowRef{product in algebra}
}

\DefText{matrix generates D algebra homomorphism ()}
{
The equality
\DrawEq{algebra, homomorphism and product abe 2()}{\Cols}
follows from the equality
\ShowRef{product in algebra}
}

\DefLabeledFootnote[4]{homomorphism of D module}{\Cols(#1#2)}
{
In theorems
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
\refTheorem{matrix generates D module homomorphism}{\Cols(#1#2)},
we use the following convention.
\ShowEq{Let be basis of module}1{}iI{}D{#1}V{#2}
\ShowEq{Let be basis of module}2{}jJ{}D{#3}V{#4}
}

\DefLabeledFootnote[6]{homomorphism of A module}{\SideNS-\Cols(#1#2#3)}
{
In theorems
\refTheorem{homomorphism A module}{\SideNS-\Cols(#1#2#3)},
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)},
we use the following convention.
\ShowEq{prolog homomorphism of vector space(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
}

\DefLabeledDefinition[4]{homomorphism from A1 to A2, D algebra}{#1#2}
{
\ShowText{algebra over ring (#1#2)}
Let diagram of representations
\DrawEq[{#1}{1.}{#2}h]{diagram of representations of D algebra}{->1(#1#2)}
describe $D_1$\Hyph algebra $A_1$.
Let diagram of representations
\DrawEq[{#3}{2.}{#4}h]{diagram of representations of D algebra}{->2(#1#2)}
describe $D_2$\Hyph algebra $A_2$.
Morphism
\DrawEq[fA]{homomorphism D algebra #1#2}1
of diagram of representations
\eqRef{diagram of representations of D algebra}{->1(#1#2)}
into diagram of representations
\eqRef{diagram of representations of D algebra}{->2(#1#2)}
is called
\AddIndex{homomorphism}{homomorphism}
of $D_{#1}$\Hyph algebra $A_{#2}$
into $D_{#3}$\Hyph algebra $A_{#4}$.
Let us denote
\ShowEq{set homomorphisms, D algebra #1#2}
set of homomorphisms
of $D_{#1}$\Hyph algebra $A_{#2}$
into $D_{#3}$\Hyph algebra $A_{#4}$.
}

\DefLabeledTheorem[5]{homomorphism from A1 to A2, D algebra}{#1#2}
{
Homomorphism
\newline
\FrameEqRef[fA]{homomorphism D algebra #1#2}1
\newline
of $D_{#1}$\Hyph algebra $A_{#2}$
into $D_{#3}$\Hyph algebra $A_{#4}$
is linear map
\eqRef[fA]{homomorphism D algebra #1#2}1
of $D_{#1}$\Hyph module $A_{#2}$
into $D_{#3}$\Hyph module $A_{#4}$
such that
\DrawEq[fab]{homomorphism, f vw=}{(#1#2)g}
and satisfies following equalities
\ShowEq{define homomorphism of D algebra #1#2}{#1}{#2}{#5}
}

\DefProof[4]{homomorphism from A1 to A2, D algebra}
{
According to definitions
\ShowRef{Morphism of Diagram of Representations}
the map
\eqRef{homomorphism D algebra #1#2}1
is morphism of representation $h_{1.12}$
describing $D_{#1}$\Hyph module $A_{#2}$
into representation $h_{2.12}$
describing $D_{#3}$\Hyph module $A_{#4}$.
Therefore, the map $f$ is linear map of $D_{#1}$\Hyph module $A_{#2}$
into $D_{#3}$\Hyph module $A_{#4}$ and equalities
\ShowEq{ref homomorphism of D algebra(#1)}{#1}{#2}
follow from the theorem
\refTheorem{linear map of D module}{#1#2}.

According to definitions
\ShowRef{Morphism of Diagram of Representations}
the map $f$
is morphism of representation $h_{1.23}$
into representation $h_{2.23}$.
The equality
\DrawEq{morphism of representation, algebra, 23}{#1#2}
follows from the equality
\eqRef{morphism of representations of universal algebra, 2m}{representation}.
From equalities
\eqRef{diagram of representations of D algebra}{->1(#1#2)},
\eqRef{diagram of representations of D algebra}{->2(#1#2)},
\eqRef{morphism of representation, algebra, 23}{#1#2},
it follows that
\DrawEq{algebra, morphism of representation 23, 1}{#1#2}
The equality
\eqRef{homomorphism, f vw=}{(#1#2)g}
follows from equalities
\eqRef{product in D algebra}{definition},
\eqRef{algebra, morphism of representation 23, 1}{#1#2}.
}

\AddEq{definition: unital algebra}
{
\begin{ShadedDefinition}
\labelDefinition{unital algebra}
If the product in $D$\Hyph algebra $A$ has unit element,
then $D$\Hyph algebra $A$ is called
\AddIndex{unital algebra}{unital algebra}\,\footnotemark
\end{ShadedDefinition}
\footnotetext{\,
See the definition of unital $D$\Hyph algebra also on the pages
\citeBib{McCrimmon: Jordan Algebras}\Hyph 137.
}
}

\DefDefinition{division algebra}
{
\(D\)\Hyph algebra \(A\) is called
\AddIndex{division algebra}{division algebra},
if for any \(A\)\Hyph number \(a\ne 0\)
there exists \(A\)\Hyph number \(a^{-1}\).
}

\DefTheorem{division algebra}
{
Let $A$ be associative division $D$\Hyph algebra.
The statement
\ShowEq{ab=ac a ne 0}
implies $b=c$.
}

\DefProof{division algebra}
{
The equality
\ShowEq{ab=ac a ne 0 1}
follows from the statement
\EqRef{ab=ac a ne 0 1}.
}

\DefLabeledDefinition[4]{linear map of D module}{#1#2}
{
Morphism of representations
\DrawEq[fV]{homomorphism D algebra #1#2}{module}
of $D_{#1}$\Hyph module $V_{#2}$
into $D_{#3}$\Hyph module $V_{#4}$
is called homomorphism or
\AddIndex{linear map}{linear map}
of $D_{#1}$\Hyph module $V_{#2}$
into $D_{#3}$\Hyph module $V_{#4}$.
Let us denote
\ShowEq{set linear maps, module (#1#2)}DV
set of linear maps
of $D_{#1}$\Hyph module $V_{#2}$
into $D_{#3}$\Hyph module $V_{#4}$.
}

\DefTheorem[3]{module of skew symmetric polylinear maps}
{
The set
\ShowEq{module of skew symmetric polylinear maps}{#1}{#2}{#3}
of skew symmetric polylinear maps
is $D$\Hyph module.
}

\AddEq[3]{remark: module of skew symmetric polylinear maps}
{
Without loss of generality, we assume
\ShowEq{L(A1,A0,B)=}{#1}{#2}{#3}
}

\DefTheorem{norm in D module A->B}
{
Let $A$ be normed $D$\Hyph module with norm $|x|_A$.
Let $B$ be normed $D$\Hyph module with norm $|y|_B$.
The map
\ShowEq{f in BA->|f|}
defined by the equality
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
is the norm in $D$\Hyph module $B^A$
and the value
\ShowEq{show|f|}
is called
\AddIndex{norm of map $f$}{norm of map}.
}

\DefTheorem{set of A->B is D module}
{
Let $A$ be Banach $D$\Hyph module with norm $|x|_A$.
Let $B$ be Banach $D$\Hyph module with norm $|y|_B$.
\StartLabelItem
\begin{enumerate}
\item
The set
$B^A$
of maps
\ShowEq{f:A->B}fAB
is $D$\Hyph module.
\labelItem{set of A->B is D module}
\item
The map
\ShowEq{f in BA->|f|}
defined by the equality
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
is the norm in $D$\Hyph module $B^A$
and the value
\ShowEq{show|f|}
is called
\AddIndex{norm of map $f$}{norm of map}.
\labelItem{norm of map}
\end{enumerate}
}

\DefTheorem{symmetrization of polylinear map}
{
Let
\ShowEq{f in L(A->B)}D{A^n}B{}
be a polylinear map.
Then the map
\ShowEq{symmetrization of polylinear map}
\EqParm{<f>}{=z}
defined by the equality
\ShowEq{symmetrization of polylinear map =}
is symmetric polylinear map
and is called
\AddIndex{symmetrization of polylinear map}{symmetrization of polylinear map}
$f$.
}

\DefTheorem{exterior product = skew symmetric}
{
Exterior product satisfies the following equation
\ShowEq{exterior product = skew symmetric}
}

\DefProof{exterior product = skew symmetric}
{
The equality
\EqRef{exterior product = skew symmetric}
follows from equalities
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =}.
}

\DefDefinition{exterior product polylinear map}
{
The skew symmetric polylinear map
\ShowEq{exterior product}
\ShowEq{exterior product =}
is called
\AddIndex{exterior product}{exterior product}.
}

\AddEq{remark: product of polylinear maps}
{
If $B_1=B_2$, then, in the right side of the equality
\EqRef{hpq(fg)=},
we consider product of $B_1$\Hyph numbers
\ShowEq{f()},
\ShowEq{g()}.
According to the theorem
\RefTheorem{Free Algebra over Ring},
this definition is compatible with the definition
\RefDefinition{product of polylinear maps}.
}

\AddEq{definition: product of polylinear maps}
{
\begin{ShadedDefinition}
\labelDefinition{product of polylinear maps}
Let $A$, $B_2$ be free algebras over commutative ring $D$.\,\footnotemark
Let
\ShowEq{h:B1->*B2}
be left\Hyph side representation of
free associative $D$\Hyph algebra $B_1$ in $D$\Hyph module $B_2$.
The map
\ShowEq{hpq:Lpq->Lp+q}
is defined by the equality
\ShowEq{hpq(fg)=}
where, in the right side of the equality
\EqRef{hpq(fg)=},
we consider left\Hyph side product
of $B_2$\Hyph number
\ShowEq{g()}{}
over $B_1$\Hyph number
\ShowEq{f()}.
\end{ShadedDefinition}
\footnotetext{\,
To define product of skew symmetric polylinear maps,
I follow definition in section
\citeBib{Cartan differential form}-1.4 of chapter 1,
pages 12 - 14.
}
}

\DefDefinition{symmetric polylinear map}
{
Let $A$, $B$ be algebras over commutative ring $D$.
A polylinear map
\ShowEq{f in L(A->B)}D{A^n}B{}
is called
\AddIndex{symmetric}{symmetric polylinear map},
if
\ShowEq{fa=fsa}
for any permutation $\sigma$ of the set
\ShowEq{set a1n}.
}

\DefTheoremNote{fx1n=0, xi=xi1}
{
A polylinear map
\ShowEq{f in L(A->B)}D{A^n}B{}
is skew symmetric iff
\ShowEq{fx1n=0}
as soon as
$a_i=a_{i+1}$
for at list one\,\footnotemark
\ShowEq{1<=i<n}
}{
In the book
\citeBib{Cartan differential form},
page 9,
Henri Cartan considered the theorem
\RefTheorem{fx1n=0, xi=xi1}
as definition of skew symmetric map.
}

\DefTheorem[3]{alternation of polylinear map}
{
Let
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
be a polylinear map.
Then the map
\ShowEq{alternation of polylinear map}
\ShowEq{[f]}{}
defined by the equality
\ShowEq{alternation of polylinear map =}
is skew symmetric polylinear map
and is called
\AddIndex{alternation of polylinear map}{alternation of polylinear map}
$f$.
}

\DefDefinition[3]{skew symmetric polylinear map}
{
A polylinear map
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
is called
\AddIndex{skew symmetric}{skew symmetric polylinear map},
if
\ShowEq{fa=sfsa}
for any permutation $\sigma$ of the set
\ShowEq{set a1n}.
}

\DefLabeledTheorem{linear dependence between vectors of basis}{\SideWS module}
{
Let $\Base$ be \Algebra.
Let $\Basis e$ be quasibasis of \SideWS $\Base$\Hyph \VectorSet $V$.
Let
\DrawEq[ce]{\SideWS wi vi=0}{we \Cols}
be linear dependence of vectors of the quasibasis $\Basis e$.
Then
\StartLabelItem
\begin{enumerate}
\item
$\Base_{\BaseExt}$\Hyph number
\ShowEq{ci i in I}
does not have inverse element
in \ShortAlgebraWS $\Base_{\BaseExt}$.
\item
The set $\Base'$ of matrices
\ShowEq{c=ci i in I}
generates \SideWS $\Base$\Hyph module $\Base'$.
\end{enumerate}
}

\DefProof{linear dependence between vectors of basis}
{
Let there exist matrix
\ShowEq{c=ci i in I}
such that the equality
\eqRef{\SideWS wi vi=0}{we \Cols}
is true and there exist index
\ShowEq{i=j}
such that
\ShowEq{wj ne 0}c.
If we assume that $\Base$\Hyph number
\ACol cj
has inverse one, then the equality
\ShowEq{\SideWS vj=sum vi}ec
follows from the equality
\eqRef{\SideWS wi vi=0}{we \Cols}.
Therefore, the vector
\ARow ej{}
is linear combination of other vectors of the set $\Basis e$
and the set $\Basis e$ is not quasibasis.
Therefore, our assumption is false,
and $\Base_{\BaseExt}$\Hyph number
\ACol cj
does not have inverse.

Let matrices
\ShowEq{b in D'}b,
\ShowEq{b in D'}c.
From equalities
\DrawEq[be]{\SideWS wi vi=0}{}
\DrawEq[ce]{\SideWS wi vi=0}{}
it follows that
\ShowEq{(b+c)*e, \SideWS module}
Therefore, the set $\Base'$ is Abelian group.

Let matrix
\ShowEq{b in D'}c{}
and $a\in\Base$.
From the equality
\DrawEq[ce]{\SideWS wi vi=0}{}
it follows that
\ShowEq{(ac)*e, \SideWS module}
Therefore, Abelian group $\Base'$ is \SideWS $\Base$\Hyph module.
}

\DefLabeledTheorem{coordinates of vector with linear dependence}{\SideWS module}
{
Let \SideWS $\Base$\Hyph module $V$
have the quasibasis $\Basis e$ such that in the equality
\DrawEq[ce]{\SideWS wi vi=0}{2 we \Cols}
there exists index
\ShowEq{i=j}
such that
\ShowEq{wj ne 0}c.
Then
\StartLabelItem
\begin{enumerate}
\item
The matrix
\ShowEq{c=ci i in I}
determines coordinates of vector $0\in V$ with respect to basis $\Basis e$.
\labelItem{coordinates of vector 0 with linear dependence, \SideWS module}
\item
Coordinates of vector $\Vector v$ with respect to basis $\Basis e$
are uniquely determined up to a choice of coordinates of vector $0\in V$.
\labelItem{coordinates of vector with linear dependence, \SideWS module}
\end{enumerate}
}

\DefProof{coordinates of vector with linear dependence}
{
The statement
\RefItem{coordinates of vector 0 with linear dependence, \SideWS module}
follows from the equality
\eqRef{\SideWS wi vi=0}{2 we \Cols}
and from the definition
\refDefinition{coordinates of vector}{\SideWS \VectorSetNS}.

Let vector $\Vector v$ have expansion
\DrawEq{vv=ve \SideWS module}{2}
with respect to quasibasis $\Basis e$.
The equality
\ShowEq{v=v+0, \SideWS module}
follows from equalities
\eqRef{\SideWS wi vi=0}{2 we \Cols},
\eqRef{vv=ve \SideWS module}{2}.
The statement
\RefItem{coordinates of vector with linear dependence, \SideWS module}
follows from equalities
\eqRef{vv=ve \SideWS module}{2},
\EqRef{v=v+0, \SideWS module}
and from the definition
\refDefinition{coordinates of vector}{\SideWS \VectorSetNS}.
}

\DefLabeledTheorem{quasibasis of module is basis}{\SideWS \VectorSetNS}
{
Let \SideWS $\Base$\Hyph module $V$
have the quasibasis $\Basis e$ such that the equality
\DrawEq[ce]{\SideWS wi vi=0}{3 ce \Cols}
implies that
\ShowEq{ci=0 1n}
Then quasibasis $\Basis e$ is
basis of \SideWS $\Base$\Hyph module $V$.
}

\DefProof{quasibasis of module is basis}
{
The theorem follows from the definition
\RefDefinition{basis of representation}
and the theorem
\refTheorem{coordinates of vector with linear dependence}{\SideWS module}.
}

\DefLabeledDefinitionNote{free module over ring}{\SideNS}
{
The \SideWS $\Base$\Hyph module $V$ is
\AddIndex{free \SideWS $\Base$\Hyph module}{free module},\,\footnotemark
if \SideWS $\Base$\Hyph module $V$ has basis.
}
{
I follow to the
definition in \citeBib{Serge Lang}, page 135.
}

\DefProof{coordinates of vector of free module}
{
The theorem follows from the theorem
\refTheorem{coordinates of vector with linear dependence}{\SideWS module}
and from definitions
\refDefinition{linearly independent vectors}{\SideNS},
\refDefinition{free module over ring}{\SideNS}.
}

\DefTheoremNote{standard representation of map A->A, associative algebra}
{
Let $A$ be finite dimensional associative $D$\Hyph algebra.
Let $\Basis e$ be basis of $D$\Hyph module $A$.
Let $\Basis F$
be the basis\,\footnotemark
of left \BoxB{A}module
\ShowEq{L(A->B)}DAA.
\StartLabelItem
\begin{enumerate}
\item
The linear map
\ShowEq{f in L(A->B)}DAA{}
has the following expansion
\labelItem{map f generated by basis F, associative algebra}
\DrawEq{map f generated by basis F}{associative algebra}
where
\ShowEq{fk= in AxA}
\item
The linear map $f$ has the standard representation
\labelItem{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, o, associative algebra}
\end{enumerate}
}{
If $D$\Hyph module $A$
is not free $D$\Hyph nodule,
then we may consider the set
\ShowEq{Ik 1n}
of linear independent linear maps. The theorem is true for any linear map
\ShowEq{f:A->B}fAA
generated by the set of linear maps $\Basis F$.
}

\DefProof{standard representation of map A->A, associative algebra}
{
Since $\Basis F$ is the basis of left \BoxB{A}module
\ShowEq{L(A->B)}DAA,
then according to the definition
\refDefinition{free module over ring}{\SideNS},
there exists expansion
\DrawEq[A]{expansion of linear map with respect to basis}A
of the linear map $f$ with respect to the basis $\Basis F$.
According to the definition
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{associative algebra}
The equality
\eqRef{map f generated by basis F}{associative algebra}
follows from equalities
\eqRef{expansion of linear map with respect to basis}A,
\eqRef{f=fkxfk}{associative algebra}.
According to theorem
\RefTheorem{standard component of tensor, algebra},
the standard representation of the tensor $f^k$ has form
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
The equation
\EqRef{standard representation of map A->A, associative algebra}
follows from equations
\eqRef{map f generated by basis F}{associative algebra},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheoremNote{set FoG generates left module L(A;B), n<m}
{
Let $A$ be $D$\Hyph module,
\ShowEq{n=dim A}nA.
Let $B$ be associative $D$\Hyph algebra,
\ShowEq{n=dim A}mB.
Let $\Basis F$ be basis of left \BoxB{B}module
\ShowEq{L(A->B)}DBB.
Let
\ShowEq{gi n<m}
Let
\ShowEq{f:A->B}GAB
be linear map of maximal rank.
The set
\DrawEq{F o G}1
generates left \BoxB{B}module\,\footnotemark
\ShowEq{L(A->B)}DAB.
}{
I do not claim that this set is a basis,
because maps
\ShowEq{FijG}
can be linearly dependent.
}

\DefProof{set FoG generates left module L(A;B), n<m}
{
Let
\ShowEq{f:A->B}gAB
be a linear map.
Let $\Basis e_A$ be the basis of $D$\Hyph module $A$.
Let $\Basis e_B$ be the basis of $D$\Hyph module $B$.
According to the theorem
\ShowEq{ref linear map of D1 D2 module, coordinates}
the linear map $G$ has coordinates
\ShowEq{matrix amn}Gmn
with respect to bases $\Basis e_A$, $\Basis e_B$
and the linear map $g$ has coordinates
\ShowEq{matrix amn}gmn
with respect to bases $\Basis e_A$, $\Basis e_B$.
A row $G_{\gii}$ of the matrix $G$,
as well a row $g_{\gii}$ of the matrix $g$,
is coordinates of linear form
\ShowEq{A->B}AD.
Since the matrix $G$ has maximal rank,
then rows of the matrix $G$ generate $D$\Hyph module
\ShowEq{L(A->B)}DAD{}
and rows of the matrix $g$ are linear combination of rows of the matrix $G$
\ShowEq{g=CG}
Since we can consider the matrix $C$
as coordinates of linear map
\ShowEq{f:A->B}CBB
then the equality
\ShowEq{g=(cF)G}
follows from the equality
\EqRef{g=CG}
and from the equality
\ShowEq{C=cF}
Since
\ShowEq{Gkj in D}
then the equality
\ShowEq{g=c(FG)}
follows from the equality
\EqRef{g=(cF)G}.
Therefore, the map $g$ belongs to
linear span of the set of maps
\eqRef{F o G}1.
}

\DefTheorem{set FoG generates left module L(A;B), n>m}
{
Let
\ShowEq{n=dim A}nA,
\ShowEq{n=dim A}mB.
Let $\Basis F$ be basis of left \BoxB{B}module
\ShowEq{L(A->B)}DBB.
Let
\ShowEq{gi n>m}
Let
\ShowEq{f:A->B}GAB
be linear map of maximal rank.
The set
\DrawEq{F o G}{}
generates the set of maps
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B), n>m}
{
The proof of the theorem is similar to the proof of the theorem
\RefTheorem{set FoG generates left module L(A;B), n<m}.
However, since number of rows of the matrix $G$ less then dimention
of $D$\Hyph module $A$, then rows of the matrix $G$ do not generate $D$\Hyph module
\ShowEq{L(A->B)}DAD{}
and the map $G$ has non trivial kernel.
In particular, rows of the matrix $g$ linearly depend on rows of the matrix $G$
iff
\ShowEq{ker G in ker g}g.
}

\DefTheorem{set FoG generates left module L(A;B)}
{
Let $\Basis F$ be basis of left \BoxB{B}module
\ShowEq{L(A->B)}DBB.
Let
\ShowEq{f:A->B}GAB
be linear map of maximal rank.
The set
\DrawEq{F o G}{}
generates the set of maps
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B)}
{
It is easy to see that theorem
\RefTheorem{set FoG generates left module L(A;B), n<m}
is particular case of the theorem
\RefTheorem{set FoG generates left module L(A;B), n>m},
because, in the theorem
\RefTheorem{set FoG generates left module L(A;B), n>m},
$\ker G=\emptyset$.
}

\AddEq{remark: set FoG generates left module L(A;B), n>m}
{
From the theorem
\RefTheorem{set FoG generates left module L(A;B), n>m},
it follows that
choice of the map $G$ depends on the map $g$.
}

\DefTheorem{basis D module L(D->A)}
{
%Let identity map
%\ShowEq{f:A->B}IDD
%is the basis of $D$\Hyph module
%\ShowEq{L(A->B)}DDD.
Let $\Basis e$ be the basis of $D$\Hyph module $A$.
Then the set of maps
\ShowEq{d->dei}i
is the basis of $D$\Hyph module
\ShowEq{L(A->B)}DDA.
}

\DefProof{basis D module L(D->A)}
{
The theorem follows from the equality
\ShowEq{f(t)=fit ei}
}

\DefDefinition{component of linear map}
{
Expression
\ShowEq{component of linear map}
in equality
\EqRef{fk= in AxA}
is called
\AddIndex{component of linear map}
{component of linear map} $f$.
Expression
\ShowEq{standard component of linear map}
in the equality
\EqRef{standard representation of map A->A, associative algebra}
is called
\AddIndex{standard component of linear map}
{standard component of linear map} $f$.
}

\DefTheorem{endomorphism of module from product}
{
The representation
\ShowEq{endomorphism of module from product}
of $D$\Hyph module $A$ in $D$\Hyph module $A$
is equivalent to structure of $D$\Hyph algebra $A$.
}

\DefLabeledConvention{sum av() convention}{\SideNS}
{
We will use summation convention
in which repeated index
in linear combination
implies summation with respect to repeated index.
In this case we assume that we know the set
of summation index and do not use summation symbol
\ShowEq{av=sum av()\SideNS}
If needed to clearly show a set of indices, I will do it.
}

\DefConvention{av=sum av convention}
{
We will use Einstein summation convention
in which repeated index (one above and one below)
implies summation with respect to repeated index.
In this case we assume that we know the set
of summation index and do not use summation symbol
\ShowEq{av=sum av convention}
If needed to clearly show a set of indices, I will do it.
}

\DefTheorem{effective representation of the ring}
{
%Let ring $D$ has unit $e$.
Representation
\ShowEq{f:A->*B}fDA
of the ring $D$
in an Abelian group $A$ is
\AddIndex{effective}{effective representation}
iff
$a=0$ follows from equation $f(a)=0$.
}

\DefProof{effective representation of the ring}
{
Suppose $a$, $b\in R$
cause the same transformation. Then
\ShowEq{representation of ring, 1}
for any $m\in A$.
From equalities
\EqRef{sum of transformations of Abelian group, 1},
\EqRef{representation of ring, 1},
it follows that
\ShowEq{representation of ring, 2}
The equality
\ShowEq{f(a-b)=0}
follows from equalities
\EqRef{0ov=0},
\EqRef{representation of ring, 2}.
Therefore, the representation $f$ is effective
iff $a=b$.
}

\DefTheorem{Representation of ring f(0)=v0}
{
Representation
\ShowEq{f:A->*B}fDA
of the ring $D$
in an Abelian group $A$
satisfies the equality
\ShowEq{f(0)=v0}
where
\ShowEq{0:A->A}
such that
\ShowEq{0ov=0}
}

\DefProof{Representation of ring f(0)=v0}
{
The equality
\ShowEq{fa=fa+f0}
follows from the equality
\EqRef{sum of transformations of Abelian group, 1}.
The equality
\ShowEq{f0x=0}
follows from the equality
\EqRef{fa=fa+f0}.
The equality
\EqRef{0ov=0}
follows from the equalities
\EqRef{f(0)=v0},
\EqRef{f0x=0}.
}

\DefText{sum of transformations of Abelian group}
{
We define the sum of transformations $f$ and $g$ of an Abelian group
according to rule
\ShowEq{(f+g)(a)=}
Therefore, considering the representation
\ShowEq{f:A->*B}fDA
of the ring $D$ in the Abelian group $A$, we assume
\ShowEq{f(a)+f(b)=}
According to the definition
\RefDefinition{representation of algebra},
the map $f$ is homomorphism of the ring $D$.
Therefore
\ShowEq{f(a+b)=f(a)+f(b)}
The equalty
\ShowEq{sum of transformations of Abelian group, 1}
follows from equalities
\EqRef{f(a)+f(b)=},
\EqRef{f(a+b)=f(a)+f(b)}.
}

\AddEq{remark: we do not have definition of determinant for division algebra}
{
According to
\citeBib{q-alg-9705026},
\citeBib{math.QA-0208146},
we do not have an appropriate definition
of a determinant for a division algebra.\,\footnote{
Professor Kyrchei
uses double determinant
(see the definition in the section
\citeBib{1812.03397}\Hyph 2.2)
to solve system of linear equations in quaternion algebra
and to solve eigenvalues problem 
(see the section
\citeBib{1812.03397}\Hyph 2.5).
I confine myself by consideration of quasideterminant,
because I am interested in a wider set of algebras.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOn

\FrameCiteBib{1812.03397}
\fi
}
However, we can define a quasideterminant which finally gives a
similar picture.
In definition
\RefDefinition{RC-quasideterminant},
I follow the definition
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=9}{1.2.2}.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOn

\FrameCiteBib{q-alg-9705026}
\FrameCiteBib{math.QA-0208146}
\fi
}

\DefConvention{basis of algebra as basis of module}
{
According to definitions
\refDefinition{free module over ring}{},
\RefDefinition{algebra over ring},
free $D$\Hyph algebra $A$ is
$D$\Hyph module $A$,
which has a basis \eV[][.]
However, generally speaking, \eV is not a
basis of $D$\Hyph algebra $A$,
because there is product in $D$\Hyph algebra $A$.
For instance, in quaternion algebra, any quaternion
\ShowEq{any quaternion}
can be represented as
\ShowEq{any quaternion i j ij}
However, for most problems
using a basis of $D$\Hyph module $A$ is easier than
using a basis of $D$\Hyph algebra $A$.
For instance, it is easier to determine coordinates of $H$\Hyph number with respect to the basis
$(1,i,j,k)$
of $R$\Hyph vector space $H$,
than to determine coordinates of $H$\Hyph number with respect to the basis
$(1,i,j)$
of $R$\Hyph algebra $H$.
Therefore the phrase "we consider basis of $D$\Hyph algebra $A$"
means that we consider $D$\Hyph algebra $A$
and basis of $D$\Hyph module $A$.
}

\DefConvention{we use separate color for index of element}
{
Let $A$ be free algebra
with finite or countable basis.
Considering expansion of element of algebra $A$ relative basis $\Basis e$
we use the same root letter to denote this element and its coordinates.
In expression $a^2$, it is not clear whether this is component
of expansion of element
$a$ relative basis, or this is operation $a^2=aa$.
To make text clearer we use separate color for index of element
of algebra. For instance,
\ShowEq{Expansion relative basis in algebra}
}

\DefTheorem{direct sum of n Abelian groups}
{
Direct sum of Abelian groups
\ShowEq{a1n}An{}
coincides with their Cartesian product
\ShowEq{A1o+An=A1xAn}A
}

\AddEq{remark: direct sum of n Abelian groups}
{
Let
\ShowEq{a1o+.n}An
be direct sum of Abelian groups
\ShowEq{a1n}An.
According to the proof of the theorem
\RefTheorem{direct sum of Abelian groups},
any $A$\Hyph number $a$ has form
$(a_1,...,a_n)$
where $a_i\in A_i$.
We also will use notation
\ShowEq{a=a1 o+ an}
}

\AddEq{theorem: direct sum of n D modules}
{
\begin{ShadedTheorem}
\labelTheorem{direct sum of n \SideWS \Base-\VectorsSetNS}
Direct sum of \SideWS $\Base$\Hyph \VectorsSet
\ShowEq{a1n}{\Module}n{}
coincides with their Cartesian product
\ShowEq{A1o+An=A1xAn}{\Module}
\end{ShadedTheorem}
}

\DefLabeledTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
{
Let
\ShowEq{A 1n}{\Module}n{}
be $\Base$\Hyph \VectorsSet and
\ShowEq{A 1o+.n}{\Module}n
Let us represent $\VNumber$\Hyph number
\ShowEq{A 1o+.n}{\VNumber}n
as column vector
\DrawEq[{\VNumber}n]{a=(a1.n col)}{}
Let us represent a linear map
\ShowEq{f:A->B}f{\Module}{\ModuleA}
as row vector
\DrawEq[fn]{a=(a1.n row)}{}
\ShowEq{f:A->B}{\aD fi}{\aU {\Module}i}{\ModuleA}
Then we can represent value of the map $f$ in $\Module$\Hyph number $\VNumber$
as product of matrices
\DrawEq[{\VNumber}{}]{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
}

\DefProof{foa=fi ai}
{
The theorem follows from the definition
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
}

\DefLabeledTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS}
{
Let
\ShowEq{A 1n}{\ModuleA}m{}
be $\Base$\Hyph \VectorsSet and
\ShowEq{A 1o+.n}{\ModuleA}m
Let us represent $\ModuleA$\Hyph number
\ShowEq{A 1o+.n}{\VNumberA}m
as column vector
\DrawEq[{\VNumberA}m]{a=(a1.n col)}{}
Then the linear map
\ShowEq{f:A->B}f{\Module}{\ModuleA}
has representation as column vector of maps
\DrawEq[fm]{a=(a1.n col)}{}
such way that, if
\ShowEq{b=foa}{\VNumberA}{\VNumber}
then
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{}
}

\DefProof{foa=fi a}
{
The theorem follows from the theorem
\RefTheorem{map from product into product}.
}

\DefTheorem{standard component of tensor, module}
{
Tensor product $\Tensor A$ of free
finite dimensional modules
$A_1$, ..., $A_n$ over the commutative ring $D$ is free
finite dimensional module.

Let
\ShowEq{tensor product of algebras, basis i}
be the basis of module $A_i$ over ring $D$.
We can represent any tensor $a\in\Tensor A$ in the following form
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
The expression
$\ShowSymbol{standard component of tensor}{}$
is defined uniquely and
is called
\AddIndex{standard component of tensor}{standard component of tensora}.
}

\DefLabeledTheorem{map of direct sum of modules}{\SideWS \Base-\VectorsSetNS}
{
Let
\ShowEq{A 1n}{\Module}n,
\ShowEq{A 1n}{\ModuleA}m{}
be $\Base$\Hyph \VectorsSet and
\ShowEq{A 1o+.n}{\Module}n
\ShowEq{A 1o+.n}{\ModuleA}m
Let us represent $\Module$\Hyph number
\ShowEq{A 1o+.n}{\VNumber}n
as column vector
\DrawEq[{\VNumber}n]{a=(a1.n col)}{v,\SideWS \Base-\VectorsSetNS}
Let us represent $\ModuleA$\Hyph number
\ShowEq{A 1o+.n}{\VNumberA}m
as column vector
\DrawEq[{\VNumberA}m]{a=(a1.n col)}{w,\SideWS \Base-\VectorsSetNS}
Then the linear map
\ShowEq{f:A->B}fVW
has representation as a matrix of maps
\DrawEq[fnm]{a=(a11.nm matrix)}{f,\SideWS \Base-\VectorsSetNS}
such way that, if
\ShowEq{b=foa}{\VNumberA}{\VNumber}
then
\DrawEq[f{\VNumberA}{\VNumber}nm]{b=f rco a}{\SideWS \Base-\VectorsSetNS}
The map
\ShowEq{fij:->}{\Module}{\ModuleA}
is a linear map and is called
\AddIndex{partial linear map}{partial linear map}.
}

\DefProof{map of direct sum of modules}
{
According to the theorem
\refTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS},
there exists the set of linear maps
\ShowEq{fi:->}
such that
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{\SideWS \Base-\VectorsSetNS}
According to the theorem
\refTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS},
for every $\gii$,
there exists the set of linear maps
\ShowEq{fij:->}{\Module}{\ModuleA}
such that
\DrawEq{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}
If we identify matrices
\ShowEq{fij=(fi)j}
then the equality
\eqRef{b=f rco a}{\SideWS \Base-\VectorsSetNS}
follows from equalities
\eqRef{foa=fi a}{\SideWS \Base-\VectorsSetNS},
\eqRef{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}.
}

\DefDefinition{Matrix of tensors}
{
Let $a$ be a matrix and
\ShowEq{a in Aoxn}{\aUD aij}n.
The matrix $a$ is called matrix of tensors
\ShowEq{Aoxn}n.
}

\AddEq{remark: map of direct sum of modules}
{
Let
\ShowEq{aU A1n}Bm{}
be $D$\Hyph algebras.
Then we can represent linear map $\aUD fij$
using \BoxB{\aU Bi}number.
}

\DefText{Free Algebra over Ring}
{
Let $D$ be commutative ring and $A$ be Abelian group.
%We initially consider the vertical representation,
%and then we consider the horizontal representation.
The diagram of representations
\DrawEq[{}{}{}g]{diagram of representations of D algebra}{}
generates the structure of $D$\Hyph algebra $A$.
}

\DefText[4]{linear map of A module, coordinates 111}
{
\ShowText{Let be module of}V{#2}{}D_{#1}{algebra}%module
\ShowText{Let be module of}V{#4}{}D_{#3}{algevra}%module
\ShowEq{Let be basis of module}1{}iI{}D{#1}V{#2}
\ShowEq{Let be basis of module}2{}jJ{}D{#3}V{#4}
}

\DefText[1]{linear map of A module, coordinates 11}
{
}

\DefText[1]{linear map of A module, coordinates 1}
{
}

\DefLabeledTheorem[7]{linear map of A module, coordinates}{\SideWS \Base\DF\Base\DT}
{
\ShowText{linear map of A module, coordinates #1#2#3}
\ShowEq{Let be basis of module}A{#2}kK{}D{#1}A{#2}
\ShowEq{Let be basis of module}A{#5}lL{}D{#4}A{#5}
\ShowEq{Let be basis of module}V{#3}iI{\SideWS}A{#2}V{#3}
\ShowEq{Let be basis of module}V{#6}jJ{\SideWS}A{#5}V{#6}
Then linear map
\newline
\FrameEqRef[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{\SideNS-\Cols}
\newline
%\ShowEq{show linear map \MapE}{\Vector g}{\Vector f}
has presentation
\DrawEq[#7]{f:A1->A2, A module}{#1#2#3}
\ShowEq{linear map in \SideWS A module}
\DrawEq{linear map in A module}{\SideNS}
%\DrawEq[g]{r2:A1->A2, \DFDT module}{1 \SideWS g}
%\ShowEq{linear map in \SideWS A module}
%\DrawEq{linear map in A module}{\SideNS}
relative to selected bases. Here
\begin{itemize}
\ShowText{homomorphism of vector space, algebra(#2)}{#1}{#2}{#3}{#4}{#5}{6}
\ShowText{homomorphism of vector space, algebra 1}{#1}{#2}{#3}{#4}{#5}{6}
\[===\]
%\ShowEq{coordinates of the linear map}a{\Base}ghiI{D_2}{}b
%\ShowEq{coordinates of the linear map}v{\Module}fgkK{\Base_\DT}{\SideWS}w
\end{itemize}
The map
\ShowEq{fij:-> \SideWS A}
is a linear map and is called
\AddIndex{partial linear map}{partial linear map}.
}

\AddEq [9]{coordinates of the linear map}
{
\item $#1$ is coordinate matrix of $#2_1$\Hyph number
$\Vector #1$
relative the basis
\ShowEq{basis e}{#2_1}{}
\DrawEq [#1{#2_1}]{va=ae1, #8module}{#1 \DFDT\SideWS module}
\def\Temp{D1 D2 }
\ifx\DFDT\Temp
\item
\ShowEq{h(a)=...}{#1}{#4}{#5}{#6}
is a matrix of $#7$\Hyph numbers.
\fi
\item $#9$ is coordinate matrix of vector
\DrawEq[#1#9#3]{vb=f(va)}{#1 \DFDT\SideWS \VectorSetNS}
relative the basis
\ShowEq{basis e}{#2_2}{}
\DrawEq [#9{#2_2}]{va=ae1, #8module}{#9 \DFDT\SideWS module}
\item $#3$ is coordinate matrix of set of vectors
\ShowEq{Vector f(e1) module}#3#2#5#6
relative the basis
\ShowEq{basis e}{#2_2}.
The matrix $#3$ is
called \AddIndex{matrix of linear map}{matrix of linear map}
$\Vector #3$ relative bases
\ShowEq{basis e}{#2_1}{}
and
\ShowEq{basis e}{#2_2}.
}

\DefProof{linear map of A module, coordinates}
{
The equality
\eqRef{r2:A1->A2, \DFDT module}{1 \SideWS g}
follows from the theorem
\RefTheorem{linear map of D1 D2 module, coordinates}.

\ShowEq{module as direct sum}1kK
\ShowEq{module as direct sum}2lL
The equality
\eqRef{linear map in A module}{\SideNS}
follows from the theorem
\RefTheorem{map of direct sum of modules}.
}

\AddEq[3]{module as direct sum}
{
$A_{#1}$\Hyph module $V_{#1}$ is direct sum
\ShowEq{V=o+Ae}#1#2#3
}

\DefTheorem{representation of algebra An in LAnA}
{
Consider $D$\Hyph algebra $A$.
A representation
\ShowEq{representation An in LAnA}DA
of algebra \AOn
in module \LAnA
defined by the equality
\DrawEq[DA]{representation An in LAnA, 1}{}
allows us to identify tensor
\ShowEq{product in algebra An 1}
and transposition $\sigma\in S^n$
with map
\DrawEq[DA]{product in algebra An 2}{DA}
where
\ShowEq{product in algebra AA 3}DA{\delta}
is identity map.
}

\DefDefinition{linear map from A1 to A2, algebra}
{
Let $A_1$ and
$A_2$ be algebras over commutative ring $D$.
The linear map
of the $D_{\DF}$\Hyph module $A_\VF$
into the $D_{\DT}$\Hyph module $A_\VT$
is called
\AddIndex{linear map}{linear map}
of $D_{\DF}$\Hyph algebra $A_\VF$ into $D_{\DT}$\Hyph algebra $A_\VT$.

Let us denote
\ShowEq{set linear maps, module (1)}DA
set of linear maps
of $D$\Hyph algebra
$A_\VF$
into $D$\Hyph algebra
$A_\VT$.
}

\DefText[4]{notation for linear map}
{
If the map
\eqRef{homomorphism D algebra #1#2}{module}
is linear map of $D_{#1}$\Hyph module $V_{#2}$ into $D_{#3}$\Hyph module $V_{#4}$,
then, according to the definition
\refDefinition[\RefRepresentation]{side representation of group}{left},
I use notation
\DrawEq{f circ a =}{}
for image of the map $f$.
}

\DefTheorem{linear map times constant, algebra}
{
Let map
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
be linear map of $D$\Hyph algebra $A_1$ into $D$\Hyph algebra $A_2$.
Then maps
\ShowEq{linear map times constant, algebra}
defined by equalities
\ShowEq{linear map times constant, 0, algebra}
are linear.
}

\DefTheorem{linear map AA LAA}
{
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
Consider $D$\Hyph algebras $A_1$ and $A_2$.
For given map
\ShowEq{f in L(A->B)}D{A_1}{A_2},
\else
For given map
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
of $D$\Hyph algebra $A_1$ into $D$\Hyph algebra $A_2$,
\fi
there exists linear map
\ShowEq{linear map AA LAA}
defined by the equality
\ShowEq{linear map AA LAA, 1}
\ShowEq{linear map AA LAA, 2}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{conjugation transformation}
Let $A_1$ be free $D$\Hyph module.
Let $A_2$ be free associative $D$\Hyph algebra.
Let $\Basis F$ be the basis of left \BoxB{A_2}module
\ShowEq{L(A->B)}D{A_1}{A_2}.
For any map
\ShowEq{Ik in I}
there exists set of linear maps
\ShowEq{conjugation transformation}
\ShowEq{conjugation transformation:}
of $D$\Hyph module
$A_1\otimes A_1$
into $D$\Hyph module
$A_2\otimes A_2$
such that
\ShowEq{conjugation transformation =}
The map
\ShowEq{show conjugation transformation}
is called
\AddIndex{conjugation transformation}{conjugation transformation}.
\end{ShadedTheorem}
}
{theorem: conjugation transformation}
%\DefEq

\DefProof{conjugation transformation}
{
According to the theorem
\RefTheorem{product of linear map, algebra},
for any tensor
$a\in A_1\otimes A_1$,
the map
\ShowEq{x->Ik a x}
is linear.
According to the statement
\RefItem{map f generated by basis F},%, associative algebra},
there exists expansion
\ShowEq{expansion Ik a x}
Let
\ShowEq{b=Ikl a}
The equality
\EqRef{conjugation transformation =}
follows from equalities
\EqRef{expansion Ik a x},
\EqRef{b=Ikl a}.
From equalities
\ShowEq{Ikl a1+a2}
\ShowEq{Ikl d a}
it follows that the map $I_k^l$ is linear map.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps}
Let $A_1$ be free $D$\Hyph module.
Let $A_2$, $A_2$ be free associative $D$\Hyph algebras.
Let $\Basis F$ be the basis of left \BoxB{A_2}module
\ShowEq{L(A->B)}D{A_1}{A_2}.
Let $\Basis G$ be the basis of left \BoxB{A_3}module
\ShowEq{L(A->B)}D{A_2}{A_3}.
\StartLabelItem
\begin{enumerate}
\item
The set of maps
\labelItem{basis of composition of linear maps}
\DrawEq{JlIk}{linear map}
is the basis of left \BoxB{A_3}module
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
\item
Let
\ShowEq{expansion of f with respect to basis I}
be expansion of linear map
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
with respect to the basis $\Basis I$.
Let
\ShowEq{expansion of g with respect to basis J}
be expansion of linear map
\ShowEq{f:A->B}g{A_2}{A_3}
with respect to the basis $\Basis J$.
Then linear map
\DrawEq{h=g o f}{123}
has expansion
\labelItem{hlk=glfk}
\ShowEq{expansion of h with respect to basis K}
with respect to the basis $\Basis K$ where
\ShowEq{hlk=glfk}
\end{enumerate}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps}
%\DefEq

\DefProof{representation of composition of linear maps}
{
The equality
\ShowEq{h(a)1}
follows from equalities
\EqRef{expansion of f with respect to basis I},
\EqRef{expansion of g with respect to basis J},
\eqRef{h=g o f}{123}.
The equality
\ShowEq{h(a)2}
follows from equalities
\eqRef{JlIk}{linear map},
\EqRef{h(a)1}
and from the theorem
\RefTheorem{conjugation transformation}.
From the equality
\EqRef{h(a)2}
it follows that set of maps $\Basis K$ generates
left \BoxB{A_3}module\newline
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
From the equality
\ShowEq{aK=aJI}
it follows that
\ShowEq{aJ=0}
and, therefore, $a^{lk}=0$.
Therefore, the set $\Basis K$ is the basis of
left \BoxB{A_3}module
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
}

\DefDefinition{similar A numbers}
{
$A$\Hyph numbers $a$ and $b$ are called similar,
if there exists $A$\Hyph number $c$ such that
\ShowEq{similar A numbers}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps A->A}
Let $A$ be free associative $D$\Hyph algebra.
Let left \BoxB{A}module
\ShowEq{L(A->B)}DAA{}
is generated by the identity map $F_0=\delta$.
Let
\ShowEq{expansion of f A->A}
be expansion of linear map
\ShowEq{f:A->B}fAA
Let
\ShowEq{expansion of g A->A}
be expansion of linear map
\ShowEq{f:A->B}gAA
Then linear map
\DrawEq{h=g o f}{A}
has expansion
\ShowEq{expansion of h A->A}
where
\ShowEq{hlk=glfk 01}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{proof}
The equality
\ShowEq{h(a)}
follows from equalities
\EqRef{expansion of f A->A},
\EqRef{expansion of g A->A},
\eqRef{h=g o f}{A}.
The equality
\EqRef{hlk=glfk 01}
follows from the equality
\EqRef{h(a)}.
\end{proof}
}
{proof: representation of composition of linear maps A->A}
%\DefEq

\DefTheorem{h generated by f, associative algebra}
{
Consider $D$\Hyph algebra $A_1$
and associative $D$\Hyph algebra $A_2$.
Consider the representation of algebra $\ATwo$
in the module
\ShowEq{L(A->B)}D{A_1}{A_2}.
The map
\ShowEq{h:A1->A2}
generated by the map
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
has form
\ShowEq{h generated by f, associative algebra}
}

\DefTheorem{coordinates of map A->A, algebra}
{
Let $A$ be free finite dimensional associative $D$\Hyph algebra.
Let $\Basis e$ be basis of $D$\Hyph module $A$.
Let
\ShowEq{structural constants, algebra}
be structural constants of algebra $A$.
Let $\Basis F$ be the basis
of left \BoxB{A}module
\ShowEq{L(A->B)}DAA{}
and
\ShowEq{coordinates of map Ik}
be coordinates of map $F_k$ with respect to basis $\Basis e$.
Coordinates
\ShowEq{Coordinates of map f}
of the map
\ShowEq{f in L(A->B)}DAA{}
and its standard components
\ShowEq{standard components of map f}k
are connected by the equation
\DrawEq{coordinates of map A->A, 2}{associative algebra}
}

\DefProof{coordinates of map A->A, algebra}
{
Relative to basis
$\Basis e$, linear maps $f$ and $I_k$ have form
\ShowEq{coordinates of map f, associative algebra}
\ShowEq{coordinates of map Fk, associative algebra}
The equality
\ShowEq{coordinates of map A->A, 3, associative algebra}
follows from equalities
\EqRef{standard representation of map A->A, associative algebra},
\EqRef{coordinates of map f, associative algebra},
\EqRef{coordinates of map Fk, associative algebra}.
Since vectors $\aD ek$
are linear independent and $x^{\gi i}$ are arbitrary,
then the equation
\eqRef{coordinates of map A->A, 2}{associative algebra}
follows from the equation
\EqRef{coordinates of map A->A, 3, associative algebra}.
}

\DefTheorem{coordinates of map A1 A2 FoG, algebra}
{
Let $\Basis e_1$ be basis of the finite dimensional
$D$\Hyph module $A_1$.
Let $\Basis e_2$ be basis of the finite dimensional associative
$D$\Hyph algebra $A_2$.
Let
\ShowEq{f in L(A->B)}D{A_1}{A_2}.
Let
\ShowEq{structural constants, algebra}
be structural constants of algebra $A_2$.
Let $\Basis F$ be the basis
of left \BoxB{A_2}module
\ShowEq{L(A->B)}D{A_2}{A_2}{}
and
\ShowEq{coordinates of map Ik}
be coordinates of map $F_k$ with respect to basis $\Basis e_2$.
Let
\ShowEq{f:A->B}GAB
be linear map of maximal rank such that
\ShowEq{ker G in ker g}f{}
and
\ShowEq{coordinates of map G}
be coordinates of map $G$ with respect to bases $\Basis e_1$ and $\Basis e_2$.
Coordinates
\ShowEq{Coordinates of map f}
of the map $f$
and its standard components
\ShowEq{standard components of map f}k
are connected by the equation
\DrawEq[f-]{coordinates of map A1 A2, FoG, associative algebra}f
}

\AddEq[1]{theorem: maps of conjugation as basis}
{
\begin{ShadedTheorem}
\labelTheorem{maps of conjugation as basis, algebra #1}
The set of linear maps
\ShowEq{vI=EI}
is the basis
of left $#1$\Hyph vector space
\ShowEq{L(A->B)}R{#1}{#1}
and a linear map
\ShowEq{f in L(A->B)}R{#1}{#1}{}
have expansion
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
where
$#1$\Hyph numbers
\ShowEq{a... #1}
are defined by the equality
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq[1]{theorem: linear map, maps of conjugation, algebra}
{
\begin{ShadedTheorem}
\labelTheorem{linear map, maps of conjugation, algebra #1}
A linear map
\ShowEq{f in L(A->B)}R{#1}{#1}{}
have expansion
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
where
\ShowEq{vI=EI}
and $#1$\Hyph numbers
\ShowEq{a... #1}
are defined by the equality
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq [1]{proof: L is left vector space}
{
\begin{proof}
According to the theorem
\RefTheorem{linear map, maps of conjugation, algebra #1},
the expansion
\EqRef{linear map of algebra #1, structure, 1}
of the linear map $f$
exists and is unique.
Therefore, the set
\ShowEq{I=(E,I)}{#1}{}
is basis of left $#1$\Hyph vector space
\ShowEq{L(A->B)}R{#1}{#1}.
\end{proof}
}

\DefTheorem{f=.E+.I+.J+.K}
{
Let
\ShowEq{f:H->H ij}
be linear map of quaternion algebra.
Let
\DrawEq{fi=fij ej}H
be quaternions represented by rows of the matrix $f$
\ShowEq{fi=fij ej H}
Then
\ShowEq{f=.E+.I+.J+.K}
}

\DefProof{f=.E+.I+.J+.K}
{
Equalities
\ShowEq{a0=f03}
\ShowEq{a1=f03}
\ShowEq{a2=f03}
\ShowEq{a3=f03}
follow from the equality
\EqRef{a...= H}.
The equalitiy
\EqRef{f=.E+.I+.J+.K}
follows from equalities
\ShowEq{f=.E+.I+.J+.K ref}
}

\DefTheorem{f=.I0.7}
{
Let
\ShowEq{f:H->H ij}
be linear map of quaternion algebra.
Let
\DrawEq{fi=fij ej}O
Then
\ShowEq{f=.I0.7}
}

\DefProof{f=.I0.7}
{
Equalities
\ShowEq{a0=f0.7}
follow from the equality
\EqRef{a...= H}.
The equalitiy
\EqRef{f=.I0.7}
follows from equalities
\ShowEq{f=.I0.7 ref}
}

\DefDefinition{maps of conjugation, complex field}
{
\ShowEq{C maps of conjugation}
Complex field has following
\AddIndex{maps of conjugation}{map of conjugation}
\ShowEq{C list maps of conjugation}
}

\DefTheorem{HE is algebra isomorphic to quaternion algebra}
{
The set
\ShowEq{HE set}
is $R$\Hyph algebra isomorphic to quaternion algebra.
}

\DefProof{HE is algebra isomorphic to quaternion algebra}
{
The theorem follows from equalities
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
based on the theorem
\RefTheorem{linear map, maps of conjugation, algebra H}.
}

\DefDefinition{algebra, left and right action on L}
{
Let $A$ be $D$\Hyph module
and $B$ be $D$\Hyph algebra.
For any map
\ShowEq{f in L(A->B)}DAB{}
and $b\in B$,
we define left side transformation of the map $f$ using equality
\ShowEq{b o f =}
and right side transformation of the map $f$ using equality
\ShowEq{b * f =}
}

\DefDefinition{projection maps, complex field}
{
Following projection maps are defined in complex field
\ShowEq{projection maps, complex field}
}

\DefTheorem{Expansion of projection maps relative E,I}
{
Expansion of projection maps relative basis
\ShowEq{e=(E,I)}{}
has form
\ShowEq{projection mappings 1, complex field}
}

\DefProof{Expansion of projection maps relative E,I}
{
The theorem follows from the theorem
\RefTheorem{linear map, maps of conjugation, algebra C}
and from the definition
\RefDefinition{projection maps, complex field}.
}

\DefTheorem{f=.E+.I}
{
Let
\DrawEq[fCC{}]{f: A->B}{}
be linear map of complex field.
Let
\DrawEq{fi=fij ej}C
Then
\ShowEq{f=.E+.I}
}

\DefProof{f=.E+.I}
{
Equalities
\ShowEq{a0=f01}
\ShowEq{a1=f01}
follow from the equality
\EqRef{a...= C}.
The equalitiy
\EqRef{f=.E+.I}
follows from equalities
\ShowEq{f=.E+.I ref}
}

\DefDefinition{polylinear map of algebras}
{
Let $A_1$, ..., $A_n$, $S$ be $D$\Hyph algebras.
Polylinear map
\ShowEq{f:A->B}f{\Times}S
of $D$\Hyph modules
$A_1$, ..., $A_n$
into $D$\Hyph module $S$
is called
\AddIndex{polylinear map}{polylinear map} of $D$\Hyph algebras
$A_1$, ..., $A_n$
into $D$\Hyph algebra $S$.
Let us denote
\ShowEq{set polylinear maps}
set of polylinear maps
of $D$\Hyph modules
$A_1$, ..., $A_n$
into $D$\Hyph module
$S$.
Let us denote
\ShowEq{set polylinear maps An}DAS
set of $n$\hyph linear maps
of $D$\Hyph module $A$ ($A_1=...=A_n=A$)
into $D$\Hyph module
$S$.
}

\DefTheorem{sum of linear maps, D module}
{
Let $A_1$, $A_2$ be $D$\Hyph modules.
The map
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
defined by equation
\ShowEq{sum of maps, D module}
is called
\AddIndex{sum of maps}{sum of maps}
$f$ and $g$
and is linear map.
The set
$\mathcal L(D;A_1;A_2)$
is an Abelian group
relative sum of maps.
}

\DefTheorem{sum of polylinear maps, module}
{
Let $D$ be the commutative ring.
Let $A_1$, ..., $A_n$, $S$ be $D$\Hyph modules.
The map
\ShowEq{sum of maps,,polylinear}
\ShowEq{sum of maps, 1, polylinear}
defined by the equality
\ShowEq{sum of  maps, polylinear}
is called
\AddIndex{sum of polylinear maps}{sum of maps}
$f$ and $g$
and is polylinear map.
The set
\ShowEq{module of polylinear maps}
is an Abelian group
relative sum of maps.
}

\DefCorollary{sum of linear maps, D module}
{
Let $A_1$, $A_2$ be $D$\Hyph modules.
The map
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
defined by equation
\ShowEq{sum of maps, D module}
is called
\AddIndex{sum of maps}{sum of maps}
$f$ and $g$
and is linear map.
The set \LAB D{A_1}{A_2}
is an Abelian group
relative sum of maps.
}

\AddEq{definition: linear map A module}
{
\begin{ShadedDefinition}
\labelDefinition{linear map \SideWS A module}
Let
\ShowEq{Ai, i=}A
be algebra over commutative ring $D_i$.
Let
\ShowEq{Ai, i=}V
be
\ShowEq{\SideWS column module}{A_i}
module.
Morphism of diagram of representations
\ShowEq{A module diagram for linear}1
into diagram of representations
\ShowEq{A module diagram for linear}2
is called
\AddIndex{linear map}{linear map}
of
\ShowEq{\SideWS column module}{A_1}
module $V_1$ into
\ShowEq{\SideWS column module}{A_2}
module $V_2$.
Let us denote
\ShowEq{set linear maps, \SideWS A12 module}
set of linear maps
of
\ShowEq{\SideWS column module}{A_1}
module $V_1$ into
\ShowEq{\SideWS column module}{A_2}
module $V_2$.
\qed
\end{ShadedDefinition}
}

\DefText{homomorphism A module}
{
\section{General Definition}

\ShowText{def homomorphism A module}111222{h(p)}{(g\circ a)}

\section{Homomorphism When Rings
\ShowEq{A1=A2 pdf}D}

\ShowText{def homomorphism A module}{}11{}22p{(g\circ a)}

\section{Homomorphism When \texorpdfstring{$D$}{D}-algebras
\ShowEq{A1=A2 pdf}A}

\ShowText{def homomorphism A module}{}{}1{}{}2pa
}

\DefText{algebra over ring (11)}
{
Let
\ShowEq{Ai, i=}A
be \Division algebra over commutative ring $D_i$.%
}

\DefText{algebra over ring (1)}
{
Let
\ShowEq{Ai, i=}A
be \Division algebra over commutative ring $D$.%
}

\DefText{algebra over ring ()}
{
Let $A$
be \Division algebra over commutative ring $D$.%
}

\DefText{module over algebra (11)}
{
Let
\ShowEq{Ai, i=}V
be \SideWS $A_i$\Hyph \VectorSetNS.
}

\DefText{module over algebra (1)}
{
Let
\ShowEq{Ai, i=}V
be \SideWS $A$\Hyph \VectorSetNS.
}

\DefLabeledDefinition[6]{homomorphism A module}{\SideNS(#1#2#3)}
{
Let diagram of representations
\DrawEq[{#1}{#2}{#3}{1.}]{diagram of representations, \SideWS module}{->1(#1#2#3)}
describe
\SideWS $A_{#2}$\Hyph \VectorSet $V_{#3}$.
Let diagram of representations
\DrawEq[{#4}{#5}{#6}{2.}]{diagram of representations, \SideWS module}{->2(#1#2#3)}
describe
\SideWS $A_{#5}$\Hyph \VectorSet $V_{#6}$.
Morphism
\DrawEq[gf]{homomorphism A module #1#2#3}{\SideNS}
of diagram of representations
\eqRef{diagram of representations, \SideWS module}{->1(#1#2#3)}
into diagram of representations
\eqRef{diagram of representations, \SideWS module}{->2(#1#2#3)}
is called
\AddIndex{homomorphism}{homomorphism}
of \SideWS $A_{#2}$\Hyph \VectorSet $V_{#3}$
into \SideWS $A_{#5}$\Hyph \VectorSet $V_{#6}$.
Let us denote
\ShowEq{set homomorphisms, A module #1#2#3 \SideNS}
set of homomorphisms
of \SideWS $A_{#2}$\Hyph \VectorSet $V_{#3}$
into \SideWS $A_{#5}$\Hyph \VectorSet $V_{#6}$.
%\ShowEq{set homomorphisms, \SideWS A12 module}
%set of homomorphisms of
%\ShowEq{\SideWS column module}{A_1}
%module $V_1$ into
%\ShowEq{\SideWS column module}{A_2}
%module $V_2$.
}

\DefLabeledTheorem[8]{define homomorphism A module}{\SideNS(#1#2#3)}
{
The homomorphism
\newline
\FrameEqRef[gf]{homomorphism A module #1#2#3}{\SideNS}
\newline
of \SideWS $A_{#2}$\Hyph \VectorSet $V_{#3}$
into \SideWS $A_{#5}$\Hyph \VectorSet $V_{#6}$
satisfies following equalities
\ShowEq{define homomorphism of A module #1#2#3}{#1}{#2}{#3}{#7}{#8}
}

\DefProof[6]{define homomorphism A module}
{
\ShowText{define homomorphism of vector space(#2)}{#1}{#2}{#3}{#4}
The equality
\eqRef{homomorphism, f v+w=}{f(#1#2)\SideWS A module}
follows from the definition
\refDefinition{homomorphism A module}{\SideNS(#1#2#3)},
since, accorfing to the definition
\RefDefinition{morphism of representations of universal algebra},
the map $f$ is homomorpism of Abelian group.
The equality
\eqRef{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module}
follows from the equality
\EqRef{morphism of representations of universal algebra}
because the map
\DrawEq[gf]{homomorphism A module #2#3}{}
is morphism of representation $g_{1.34}$
into representation $g_{2.34}$.
}

\DefTheorem{L(An;B) is free D module}
{
Let $A_1$, ..., $A_n$, $B$ be free modules over commutative ring $D$.
$D$\Hyph module
\ShowEq{L(A->B)}D{A_1\times...\times A_n}B{}
is free $D$\Hyph module.
}

\DefLabeledTheoremNote[5]{linear map of D module}{#1#2}
{
Linear map
\newline
\FrameEqRef[fV]{homomorphism D algebra #1#2}{module}
\newline
of $D_{#1}$\Hyph module $V_{#2}$
into $D_{#3}$\Hyph module $V_{#4}$
satisfies to equalities\,\footnotemark
\ShowEq{define homomorphism of D module #1#2}{#1}{#2}{#5}
}
{\,
In some books
(for instance, on page \citeBib{Serge Lang}\Hyph 119) the theorem
\refTheorem{linear map of D module}{#1#2}
is considered as a definition.
}

\DefText{linear map of D module (11)}
{
According to definitions
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
the map $h$
is homomorphism of ring $D_1$
into ring $D_2$.
Equalities
\ShowEq{ref linear map of D module 1}
follow from this statement.
}

\DefText{linear map of D module (1)}
{
}

\DefProof[2]{linear map of D module}
{
\ShowText{linear map of D module (#1#2)}
From the definition
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
it follows that
the map $f$ is a homomorphism of the Abelian group $V_1$
into the Abelian group $V_2$ (the equality
\eqRef{homomorphism, f v+w=}{f D module #1#2}).
The equality
\eqRef{left homomorphism, f av=}{f D module #1#2}
follows from the equality
\EqRef[\RefRepresentation]{morphism of representations of universal algebra}.
}

\DefDefinition{polylinear map of modules}
{
Let $D$ be the commutative ring.
Reduced polymorphism of $D$\Hyph modules
$A_1$, ..., $A_n$ into $D$\Hyph module $S$
\ShowEq{f:A->B}f{\Times}S
is called
\AddIndex{polylinear map}{polylinear map} of $D$\Hyph modules
$A_1$, ..., $A_n$
into $D$\Hyph module $S$.

We denote
\ShowEq{set polylinear maps}
the set of polylinear maps
of $D$\Hyph modules
$A_1$, ..., $A_n$
into $D$\Hyph module
$S$.
Let us denote
\ShowEq{set polylinear maps An}DAS
set of $n$\hyph linear maps
of $D$\Hyph module $A$ ($A_1=...=A_n=A$)
into $D$\Hyph module
$S$.
}

\DefTheorem{polylinear map of modules}
{
Let $D$ be the commutative ring.
The polylinear map of $D$\Hyph modules
$A_1$, ..., $A_n$
into $D$\Hyph module $S$
\ShowEq{f:A->B}f{\Times}S
satisfies to equalities
\DrawEq[f]{f(ai+bi)=fai+fbi}{}
\DrawEq[f]{f(pai)=pfai}{}
\ShowEq{polylinear map of algebras, 1}{A_i}D
}

\DefTheorem{there exists tensor product of modules}
{
Let $A_1$, ..., $A_n$ be
modules over commutative ring $D$.
There exists  and unique \AddIndex{tensor product}{tensor product}
\ShowEq{tensor product of modules}
\ShowEq{f:xA->oxA}
of $D$\Hyph modules $A_1$, ..., $A_n$.
We use notation
\ShowEq{fxa=oxa}
for the image of the map $f$.
}

\DefTheorem{tensor product and polylinear map}
{
Let $A_1$, ..., $A_n$ be
modules over commutative ring $D$.
Let
\ShowEq{map f, 1, tensor product}
be
polylinear map defined by the equality
\ShowEq{map f, tensor product}
Let
\ShowEq{map g, tensor product}
be polylinear map into $D$\Hyph module $V$.
There exists a linear map
\ShowEq{map h, tensor product}
such that the diagram
\ShowEq{map gh, tensor product}
is commutative.
The map \(h\) is defined by the equality
\ShowEq{g=h, tensor product}
}

\DefProof{polylinear map of modules}
{
The theorem follows from definitions
\RefDefinition[\RefRepresentation]{reduced polymorphism of representations},
\refDefinition{linear map of D module}1,
\RefDefinition{polylinear map of modules}
and from the theorem
\refTheorem{linear map of D module}1.
}

\DefProof{sum of polylinear maps, module}
{
According to the theorem
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{sum of maps f}
\DrawEq[f]{f(pai)=pfai}{sum of maps f}
\DrawEq[g]{f(ai+bi)=fai+fbi}{sum of maps g}
\DrawEq[g]{f(pai)=pfai}{sum of maps g}
The equality
\ShowEq{sum of maps, 31, polylinear}
follows from the equalities
\EqRef{sum of maps, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps f},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps g}.
The equality
\ShowEq{sum of maps, 32, polylinear}
follows from the equalities
\EqRef{sum of maps, polylinear},
\eqRef{f(pai)=pfai}{sum of maps f},
\eqRef{f(pai)=pfai}{sum of maps g}.
From equalities
\EqRef{sum of maps, 31, polylinear},
\EqRef{sum of maps, 32, polylinear}
and from the theorem
\RefTheorem{polylinear map of modules},
it follows that the map
\EqRef{sum of maps, 1, polylinear}
is linear map of $D$\Hyph modules.

Let
\ShowEq{module of polylinear maps, 1}
For any
\ShowEq{module of polylinear maps, 2}
Therefore, sum of polylinear maps is commutative and associative.

From the equality
\EqRef{sum of maps, polylinear},
it follows that the map
\ShowEq{0:A1n->S}
is zero of addition
\ShowEq{0+f=f 1n}
From the equality
\EqRef{sum of maps, polylinear},
it follows that the map
\ShowEq{-f:A1n->S}
is map inversed to map \(f\)
\ShowEq{f-f=0}
because
\ShowEq{f-f=0 1n}
From the equality
\ShowEq{sum of maps, 4, polylinear}
it follows that sum of maps is commutative.
Therefore, the set
\ShowEq{module of polylinear maps}
is an Abelian group.
}

\DefTheorem{module of polylinear maps}
{
Let $D$ be the commutative ring.
Let $A_1$, ..., $A_n$, $S$ be $D$\Hyph modules.
The map
\ShowEq{product of map over scalar,,polylinear}
\ShowEq{product of map over scalar, 1, polylinear}
defined by equality
\ShowEq{product of map over scalar, polylinear}
is polylinear map
and is called
\AddIndex{product of map $f$ over scalar}
{product of map over scalar} $d$.
The representation
\ShowEq{a:LA1n->LA1n}
of ring $D$ in Abelian group
\ShowEq{module of polylinear maps}
generates structure of $D$\Hyph module.
}

\DefProof{module of polylinear maps}
{
According to the theorem
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{product of map over scalar}
\DrawEq[f]{f(pai)=pfai}{product of map over scalar}
The equality
\ShowEq{product of map over scalar, 31, polylinear}
follows from equalities
\EqRef{product of map over scalar, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{product of map over scalar}.
The equality
\ShowEq{product of map over scalar, 32, polylinear}
follows from equalities
\EqRef{product of map over scalar, polylinear},
\eqRef{f(pai)=pfai}{product of map over scalar}.
From equalities
\EqRef{product of map over scalar, 31, polylinear},
\EqRef{product of map over scalar, 32, polylinear}
and from the theorem
\RefTheorem{polylinear map of modules},
it follows that the map
\EqRef{product of map over scalar, 1, polylinear}
is polylinear map of $D$\Hyph modules.

The equality
\DrawEq{(p+q)f=pf+qf}{polylinear}
follows from the equality
\ShowEq{(p+q)f=pf+qf 1}
The equality
\DrawEq{p(qf)=(pq)f}{polylinear}
follows from the equality
\ShowEq{p(qf)=(pq)f 1}
From equalities
\eqRef{(p+q)f=pf+qf}{polylinear}
\eqRef{p(qf)=(pq)f}{polylinear}
it follows that the map
\EqRef{a:LA1n->LA1n}
is representation of ring $D$
in Abelian group
\ShowEq{module of polylinear maps}.
Since specified representation is effective,
then, according to the definition
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
and the theorem
\RefTheorem{sum of polylinear maps, module},
Abelian group
\ShowEq{L(A->B)}D{A_1}{A_2}{}
is $D$\Hyph module.
}

\DefCorollary{product of linear map over scalar, D module}
{
Let $A_1$, $A_2$ be $D$\Hyph modules.
The map
\ShowEq{product of map over scalar,,D module}
\ShowEq{product of map over scalar, 1, D module}
defined by the equality
\ShowEq{product of map over scalar, D module}
is linear map
and is called
\AddIndex{product of map $f$ over scalar}
{product of map over scalar} $d$.
The representation
\ShowEq{a:LA12->LA12}
of ring $D$ in Abelian group
\ShowEq{L(A->B)}D{A_1}{A_2}{}
generates structure of $D$\Hyph module.
}

\DefLabeledTheoremNote{linear map of A module}{\Base\DF\Module\VF->\Base\DT\Module\VT, \SideNS}
{
Linear map
\ShowEq{show linear map \MapE}gf
of \SideWS $\Base_\DF$\Hyph module $\Module_\VF$
into \SideWS $\Base_\DT$\Hyph module $\Module_\VT$
satisfies to equalities\,\footnotemark
\ShowEq{property linear map \MapE}
}
{
In some books
(for instance, on page \citeBib{Serge Lang}\Hyph 119) the theorem
\refTheorem{linear map of A module}{\Base\DF\Module\VF->\Base\DT\Module\VT, \SideNS}
is considered as a definition.
}

\DefProof[2]{linear map of module}
{
From definitions
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\refDefinition{linear map of D module}{#1#2},
it follows that
the map $h$ is a homomorphism of the ring $D_1$
into the ring $D_2$ (the equalities
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module})
and the map $f$ is a homomorphism of the Abelian group $A_1$
into the Abelian group $A_2$ (the equality
\eqRef{f(a+b)=...}{D1 D2 \SideWS module}).
The equality
\eqRef{f(da)=h... \SideWS module}{\DFDT \SideWS module}
follows from the equality
%\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{representation}.
}

\DefProof{linear map of A module}
{
From definitions
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map \SideWS A module},
it follows that
\begin{itemize}
\item
the map $h$ is a homomorphism of the ring $D_1$
into the ring $D_2$ (the equalities
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module});
\item
the map $g$ is homomorphism of the Abelian group $A_1$
into the Abelian group $A_2$ (the equality
\eqRef{f(a+b)=...}{g \DFDT \SideWS module});
\item
the map $f$ is homomorphism of the Abelian group $V_1$
into the Abelian group $V_2$ (the equality
\eqRef{f(a+b)=...}{f \DFDT \SideWS module}).
\end{itemize}
Equalities
\eqRef{f(da)=h... \SideWS module}{g \DFDT},
\eqRef{f(da)=h... \SideWS module}{f \DFDT}
follow from the equality
\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
%\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{representation}.
}

\DefTheorem{complex field over real field}
{
Consider complex field $C$ as two-dimensional algebra over real field.
Let
\ShowEq{basis of complex field}
be the basis of algebra $C$.
Then in this basis product has form
\ShowEq{product of complex field}
and structural constants have form
\ShowEq{structural constants of complex field}
}

\DefProof{complex field over real field}
{
Equalities
\EqRef{product of complex field} and
\EqRef{structural constants of complex field}
follow from the equality $i^2=-1$.
}

\DefLabeledTheorem[1]{maps of conjugation antilinear}{#1}
{
Maps of conjugation
\ShowEq{I... #1}
are \DoVerb antilinear homomorphisms.
}

\DefProof[1]{maps of conjugation antilinear}
{
The product of $#1$\Hyph numbers
\ShowEq{#1 number Ea}a
and
\ShowEq{#1 number Ea}b
has form
\DrawEq[ab]{#1 product aEx}{ab}
\ShowText{maps of conjugation antilinear #1}
}

\DefText{maps of conjugation antilinear H}
{
\ShowEq{H items maps of conjugation antilinear}
}

\DefText{maps of conjugation antilinear O}
{
To prove the theorem, it is enough to consider map $\aU I1$,
because the proof is the same for other maps.
\ShowEq{item maps of conjugation antilinear}O1
}

\DefTheorem{coordinates of map A1 A2, algebra}
{
Let $\Basis e_1$ be basis of the free finite dimensional
$D$\Hyph module $A_1$.
Let $\Basis e_2$ be basis of the free finite dimensional associative
$D$\Hyph algebra $A_2$.
Let
\ShowEq{structural constants, algebra}
be structural constants of algebra $A_2$.
Let $\Basis F$ be the basis
of left \BoxB{A_2}module
\ShowEq{L(A->B)}D{A_1}{A_2}{}
and
\ShowEq{coordinates of map Ik}
be coordinates of map $F_k$ with respect to bases $\Basis e_1$ and $\Basis e_2$.
Coordinates
\ShowEq{Coordinates of map f}
of the map
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
and its standard components
\ShowEq{standard components of map f}k
are connected by the equation
\DrawEq[f-]{coordinates of map A1 A2, 2, associative algebra}f
}

\DefProof{coordinates of map A1 A2, algebra}
{
Relative to bases
$\Basis e_1$ and $\Basis e_2$, linear maps $f$ and $I_k$ have form
\ShowEq{coordinates of map f 18, associative algebra}
\ShowEq{coordinates of map Ik, associative algebra}
The equality
\ShowEq{coordinates of map A1 A2, 3, associative algebra}
follows from equalities
\EqRef{standard representation of map A1 A2, associative algebra},
\EqRef{coordinates of map f 18, associative algebra},
\EqRef{coordinates of map Ik, associative algebra}.
Since vectors $e_{2\cdot\gik}$
are linear independent and $x^{\gi i}$ are arbitrary,
then the equality
\eqRef{coordinates of map A1 A2, 2, associative algebra}f
follows from the equation
\EqRef{coordinates of map A1 A2, 3, associative algebra}.
}

\DefTheorem{linear map in L(A,A), associative algebra}
{
Let $A_1$ be $D$\Hyph algebra.
Let $A_2$ be free finite dimensional associative $D$\Hyph algebra.
Let $\Basis e$ be basis of $D$ module $A_2$.
Left \BoxB{A_2}module
\ShowEq{L(A->B)}D{A_1}{A_2}{}
has finite
\AddIndex{basis}{basis of algebra L(A,A)} $\Basis I$.
\StartLabelItem
\begin{enumerate}
\item
The linear map
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
has form
\labelItem{f in L(A,A), 1, associative algebra}
\ShowEq{f in L(A,A), 1, associative algebra}
\item
Its standard representation has form
\labelItem{f in L(A,A), 2, associative algebra}
\ShowEq{f in L(A,A), 2, associative algebra}
\end{enumerate}
}

\DefTheoremNote{standard representation of map A1 A2, associative algebra}
{
Let $A_1$ be free $D$\Hyph module.
Let $A_2$ be free finite dimensional associative $D$\Hyph algebra.
Let $\Basis e$ be basis of $D$\Hyph module $A_2$.
Let $\Basis F$
be the basis of left \BoxB{A_2}module
\ShowEq{L(A->B)}D{A_1}{A_2}.\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
The map
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
has the following expansion
\labelItem{map f generated by basis F}
\DrawEq{map f generated by basis F}{expansion}
where
\ShowEq{fk= in A2xA2}
\item
The map $f$ has the standard representation
\labelItem{standard representation of map A1 A2, associative algebra}
\ShowEq{standard representation of map A1 A2, associative algebra}
\end{enumerate}
}{
If $D$\Hyph module $A_1$ or $D$\Hyph module $A_2$
is not free $D$\Hyph nodule,
then we may consider the set
\ShowEq{Ik 1n}
of linear independent linear maps. The theorem is true for any linear map
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
generated by the set of linear maps $\Basis F$.
}

\DefProof{standard representation of map A1 A2, associative algebra}
{
Since $\Basis F$ is the basis of left \BoxB{A_2}module
\ShowEq{L(A->B)}D{A_1}{A_2},
then according to the definition
\ShowEq{ref definition: basis of representation}
and the theorem
\ShowEq{RefTheorem set of vectors generated by set of vectors, module}
there exists expansion
\DrawEq[{A_2}]{expansion of linear map with respect to basis}{A2}
of the linear map $f$ with respect to the basis $\Basis I$.
According to the definition
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{module}
The equality
\eqRef{map f generated by basis F}{expansion}
follows from equalities
\eqRef{expansion of linear map with respect to basis}{A2},
\eqRef{f=fkxfk}{module}.
According to theorem
\RefTheorem{standard component of tensor, algebra},
the standard representation of the tensor $f^k$ has form
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
The equation
\EqRef{standard representation of map A1 A2, associative algebra}
follows from equations
\eqRef{map f generated by basis F}{expansion},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheorem{map > bullet map}
{
Let $A$ be $D$\Hyph algebra.
For any $A$\Hyph number $a$, the map
\ShowEq{f->ao f}
defined by the equality
\ShowEq{ao f=a f o}
is endomorphism of $D$\Hyph module
\ShowEq{L(A->B)}DAA.
}

\DefProof{map > bullet map}
{
}

\DefTheorem{a > a bullet}
{
$D$\Hyph module
\ShowEq{L(A->B)}DAA
is left $A$\Hyph module generated by the representation
\ShowEq{a > a bullet}
}

\DefProof{a > a bullet}
{
}

\AddEq[3]{theorem: ao Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix}
The map
\DrawEq[{#1}{#2}]{map ao}{#1#2}
has matrix
\ShowEq{maps of conjugation, Jacobian matrix}{#1}{#2}{#3}
\DrawEq[{#1}{#2}]{a o, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix}
{
\begin{proof}
The product of $#2$\Hyph numbers
\ShowEq{#2 number Ea}a
and
\ShowEq{#2 number #1a}x
has form
\DrawEq[ax]{#2 product a#1x}{}
Therefore, function
\eqRef{map ao}{#1#2}
has Jacobian matrix
\eqRef{a o, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq [2]{item maps of conjugation antilinear}
{

The equality
\ShowEq{#1#2 product ab}
follows from the equalities
\EqRef{#2x= #1},
\eqRef{#1 product aEx}{ab}.
From the equality
\eqRef{#1 product aEx}{ab},
it follows that product of $#1$\Hyph numbers
\ShowEq{#1 number #2a}b
and
\ShowEq{#1 number #2a}a
has form
\ShowEq{#1 #2b*#2a}
From equalities
\EqRef{#1#2 product ab},
\EqRef{#1 #2b*#2a},
it follows that the map $\aU I#2$
is \DoVerb linear antihomomorphism.
}

\AddEq[2]{theorem: ao Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix 1}
\DrawEq[#1]{ao, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix 1}
{
\begin{proof}
The equality
\eqRef{ao, #2 matrix 1}{#1}
follows from the chain of equalities
\ShowEq{a#1, #2 matrix 2}
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix}
The map
\DrawEq[{#1}{#2}]{map a*}{#1#2}
has matrix
\ShowEq{maps of conjugation, Jacobian matrix}{#1}{#2}r
\DrawEq[{#1}{#2}]{a *, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix}
{
\begin{proof}
The product of $#2$\Hyph numbers
\ShowEq{#2 number #1a}x
and
\ShowEq{#2 number Ea}a
has form
\ShowEq{#2 product #1xa}
Therefore, function
\eqRef{map a*}{#1#2}
has Jacobian matrix
\eqRef{a *, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix 1}
\DrawEq[#1]{a*, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix 1}
{
\begin{proof}
The equality
\eqRef{a*, #2 matrix 1}{#1}
follows from the chain of equalities
\ShowEq{#1a, #2 matrix 2}
\end{proof}%
}

\DefDefinition{antilinear homomorphism}
{
The map
\ShowEq{f in L(A->B)}DAA{}
is called
\AddIndex{antilinear homomorphism}{antilinear homomorphism}
if the map $f$ satisfies the equality
\ShowEq{fab=fbfa}
}

\DefDefinition{quaternion maps of conjugation}
{
\ShowEq{H maps of conjugation}
Quaternion algebra has following
\AddIndex{maps of conjugation}{map of conjugation}
\ShowEq{H list maps of conjugation}
We also use notation
\ShowEq{I0=E}
}

\DefDefinition{octonion maps of conjugation}
{
\ShowEq{O maps of conjugation}
Octonion algebra has following
\AddIndex{maps of conjugation}{map of conjugation}
\ShowEq{O list maps of conjugation}
We also use notation
\ShowEq{I0=E}
}

\AddEq[1]{theorem: L is left vector space}
{
\begin{ShadedTheorem}
\labelTheorem{L(#1->#1) is left #1-vector space}
$#1\otimes #1$\Hyph module
\ShowEq{L(A->B)}R{#1}{#1}
is left $#1$\Hyph vector space
and has the basis
\ShowEq{I=(E,I)}{#1}.
\end{ShadedTheorem}
}

\AddEq [9]{Let be basis of vector space}
{%
Let the set of vectors
\DrawEq[{#1}{#2}{#3}]{basis e of module #8}{#9}
be a basis of \SideWS $#4_{#5}$\Hyph \VectorSet $#6_{#7}$.%
}%

\AddEq [3]{Let be Basis of vector space}
{%
Let \eV[#1]
be a basis of \SideWS $#2$\Hyph vector space $#3$.%
}%

\AddEq [9]{Let be basis of module}
{%
Let
\DrawEq[{#1_{#2}}{#3}{#4}]{basis e of module \Cols}-
be a basis of #5 $#6_{#7}$\Hyph \VectorSet of \ColsWS $#8_{#9}$.
}

\AddEq [9]{Let be basis of algebra}
{%
Let the set of vectors
\DrawEq[{#1_{#2}}{#3}{#4}]{basis e of module \Cols}{#9}
be a basis of $#5_{#6}$\Hyph algebra of \ColsWS $#7_{#8}$.%
}

\AddEq [9]{Let be basis of algebra and C}
{%
Let the set of vectors
\DrawEq[{#1}{#3}{#4}]{basis e of module \Cols}{#9}
be a basis and
\ShowEq{structural constants of algebra}{#2}kij,
\ShowEq{kij in I}{#4}
be structural constants of $#5_{#6}$\Hyph algebra of \ColsWS $#7_{#8}$.%
}

\AddEq [5]{Let e be basis 1n}
{
Let
\ShowEq{basis e of module 1n}{#1}{#2}
be a basis of #3 $#4$\Hyph module $#5$.
}

\DefText[5]{coordinates of the linear map 1}
{
\item $#1$ is coordinate matrix of $#2_1$\Hyph number
$\Vector #1$
relative the basis \eV[#3]
\DrawEq [{#1}{#3}{}]{va=ae1, module (#5)(\Cols)}{\SideNS-\VectorSet #1 #4}
}

\DefText[5]{coordinates of the linear map 2(1)}
{
\item
\ShowEq{h(a)=...}{#1}{#2}{#3}{#4}
is a matrix of $#5$\Hyph numbers.
}

\DefText[5]{coordinates of the linear map 2()}
{
}

\DefText[7]{coordinates of the linear map 3}
{
\item $#6$ is coordinate matrix of $#2_2$\Hyph number
\DrawEq[#1#6#4]{vb=f(va)}{#1 #7(\Cols)\SideNS-\VectorSetNS}
relative the basis \eV[#3]
\DrawEq [#6{#3}]{va=ae1, module (#5)(\Cols)}{#6 #7\SideNS-\VectorSetNS}
}

\DefText[6]{coordinates of the linear map 4}
{
\item $#1$ is coordinate matrix of set of $#2_2$\Hyph numbers
\ShowEq{Vector f(e1) module}#1{#3}#5#6
relative the basis \eV[#4][.]
}

\DefText[6]{Let be module of}
{
Let $#1_{#2}$ be #3 $#4_{#5}$\Hyph #6 of \ColTNS.
}

\DefText[2]{we identify linear map and matrix}
{
On the basis of theorems
\refTheorem{linear map of D module, coordinates}{#1#2cols},
\refTheorem{matrix generates D module homomorphism}{cols(#1#2)},
as well on the basis of theorems
\refTheorem{linear map of D module, coordinates}{#1#2rows},
\refTheorem{matrix generates D module homomorphism}{rows(#1#2)},
we identify the linear map
\DrawEq[{\Vector f}V]{homomorphism D algebra #1#2}{}
and the matrix $f$ of its presentation.
}

\DefLabeledFootnote[4]{homomorphism of d algebra}{#1#2\Cols}
{
In theorems
\refTheorem{homomorphism of d algebra, coordinates}{#1#2\Cols},
\refTheorem{matrix generates D algebra homomorphism}{\Cols(#1#2)},
we use the following convention.
\ShowEq{Let be basis of algebra and C}11iID{#1}A{#2}-
\ShowEq{Let be basis of algebra and C}22jJD{#3}A{#4}-
}
 
\DefLabeledTheorem[5]{homomorphism of d algebra, coordinates}{#1#2\Cols}
{
The homomorphism\refFootnote{homomorphism of d algebra}{#1#2\Cols}
\DrawEq[{\Vector f}A]{homomorphism D algebra #1#2}{}
of $D_{#1}$\Hyph algebra $A_{#2}$
into $D_{#3}$\Hyph algebra $A_{#4}$ has presentation
\DrawEq[f{#5}{}]{f:V1->V2, D module \Cols}{algebra(#1#2)}
\DrawEq[hf{#2}{#4}a]{f o ea=efa i (#1#2)}{(\Cols)algebra}
\DrawEq[hf12]{f o ea=efa (#1#2)(\Cols)}{algebra}
relative to selected bases. Here
\begin{itemize}
\ShowText{coordinates of the linear map 1}aA1{(#1)(#2)}{}
\ShowText{coordinates of the linear map 2(#1)}ahiI{D_{#3}}
\ShowText{coordinates of the linear map 3}aA2f{}b{(#1)(#2)}
\ShowText{coordinates of the linear map 4}fA{#2}{#4}iI
\ShowText{Morphism of D algebra}{#1}{#2}f
\end{itemize}
}

%\DefProofRef[4]{homomorphism of d algebra, coordinates}{#1#2\Cols}
\DefProof[4]{homomorphism of d algebra, coordinates}
{
Equalities
\ShowRef{homomorphism of d algebra, coordinates}{#1}{#2}{#4}
follow from theorems
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
\refTheorem{homomorphism from A1 to A2, D algebra}{#1#2}.

The equality
\DrawEq{algebra, homomorphism and product eiej(#1#2)}{\Cols}
follows from equalities
\ShowRef{algebra, homomorphism and product eiej}{#1}{#2}{#3}
The equality
\DrawEq{algebra, homomorphism and product eiej 4(#1#2)}{\Cols}
follows from the equality
\ShowRef{algebra, homomorphism and product eiej 1}{#1}{#2}
and the equality
\eqRef{algebra, homomorphism and product eiej(#1#2)}{\Cols}.
The equality
\DrawEq{algebra, homomorphism and product eiej 5}{(#1#2)\Cols}
follows from the equality
\ShowRef{homomorphism, f vw=}{#1}{#2}
The equality
\DrawEq{algebra, homomorphism and product eiej 2(#1#2)}{\Cols}
follows from the equality
\ShowEq{algebra, homomorphism and product, 1}
and the equality
\eqRef{algebra, homomorphism and product eiej 5}{(#1#2)\Cols}.
The equality
\DrawEq{algebra, homomorphism and product eiej 3(#1#2)}{\Cols}
follows from equalities
\eqRef{algebra, homomorphism and product eiej 4(#1#2)}{\Cols},
\eqRef{algebra, homomorphism and product eiej 2(#1#2)}{\Cols}.
The equality
\ShowRef{algebra, homomorphism and product}{#1}{#2}f
follows from the equality
\eqRef{algebra, homomorphism and product eiej 3(#1#2)}{\Cols},
and and the theorem
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
}

\DefLabeledTheorem[5]{linear map of D module, coordinates}{#1#2\Cols}
{
Linear map\refFootnote{homomorphism of D module}{\Cols(#1#2)}
\DrawEq[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
has presentation
\DrawEq[hf{#2}{#4}{}]{f o ea=efa (#1#2)(\Cols)}{module}
\DrawEq[hf{#2}{#4}a]{f o ea=efa i (#1#2)}{(\Cols)module}
\DrawEq[f{#5}{}]{f:V1->V2, D module \Cols}{#1#2}
relative to selected bases. Here
\begin{itemize}
\ShowText{coordinates of the linear map 1}aV1{(#1)(#2)}{}
\ShowText{coordinates of the linear map 2(#1)}ahiI{D_{#3}}
\ShowText{coordinates of the linear map 3}aV2f{}b{(#1)(#2)}
\ShowText{coordinates of the linear map 4}fV{#2}{#4}iI
\end{itemize}
}

\DefProofRef[5]{linear map of D module, coordinates}{#1#2\Cols}
{
Since
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
\newline
is a linear map, then the equality
\ShowEq{vb=h(e1)a (#1)(#2)(\Cols)\SideNS}
follows from equalities
\ShowRef{vb=h(e1)a}{#1}{#2}{#5}
$V_2$\Hyph number
\ShowEq{f(e1)(\Cols)\SideNS}
has expansion
\DrawEq{f(e1)=(\Cols)\SideNS}{(#1)(#2)}
relative to basis $\Basis e_2$.
Combining \EqRef{vb=h(e1)a (#1)(#2)(\Cols)\SideNS}
and \eqRef{f(e1)=(\Cols)\SideNS}{(#1)(#2)}, we get
\ShowEq{vb=a f e (#1)(#2)(\Cols)\SideNS}
\eqRef{f:V1->V2, D module \Cols}{#1#2}
follows from comparison of
\newline
\FrameEqRef[b2]{va=ae1, module ()(\Cols)}{b {(#1)(#2)}\SideNS-\VectorSetNS}
\newline
and \EqRef{vb=a f e (#1)(#2)(\Cols)\SideNS} and
the theorem
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
}

\DefDefinitionNote{algebra over ring}
{
Let $D$ be commutative ring.
$D$\Hyph module $A$ is called
\AddIndex{algebra over ring}{algebra over ring} $D$
or
\AddIndex{$D$\Hyph algebra}{D algebra},
if we defined product\,\footnotemark
in $A$
\DrawEq{product in D algebra}{definition}
where $C$ is bilinear map
\ShowEq{product in algebra, definition 1}
If $A$ is free
$D$\Hyph module, then $A$ is called
\AddIndex{free algebra over ring}{free algebra over ring} $D$.
}
{
I follow the definition
given in
\citeBib{Richard D. Schafer}, page 1,
\citeBib{0105.155}, page 4. The statement which
is true for any $D$\Hyph module,
is true also for $D$\Hyph algebra.
}

\DefText{algebra inherits type of module}
{
$D$\Hyph algebra $A$ inherits type of $D$\Hyph module $A$.
}

\DefLabeledDefinition{type of algebra}{\Cols}
{
$D$\Hyph algebra $A$ is called
$D$\Hyph algebra of \ColTNS,
if $D$\Hyph module $A$
is $D$\Hyph module of \ColTNS.
}

\DefLabeledTheorem{associative product in algebra}{\Cols}
{
Since the algebra $A$ is commutative, then
\DrawEq{commutative product in algebra, 1}{\Cols}
Since the algebra $A$ is associative, then
\DrawEq{associative product in algebra, 1}{\Cols}
}

\DefProof{associative product in algebra}
{
For commutative algebra,
the equation
\eqRef{commutative product in algebra, 1}{\Cols}
follows from equation
\ShowEq{commutative product in algebra}
For associative algebra,
the equation
\eqRef{associative product in algebra, 1}{\Cols}
follows from equation
\ShowEq{associative product in algebra}
}

\DefLabeledTheorem{product in algebra}{\Cols}
{
\ShowEq{Let be basis of algebra}{}{}iID{}A{}-
Let
\ShowEq{a b in basis of algebra}
We can get the product of $a$, $b$ according to rule
\DrawEq{product in algebra}{\Cols}
where
\ShowEq{structural constants of algebra symb}
are \AddIndex{structural constants}{structural constants}
of algebra $A$ over ring $D$.
The product of basis vectors in the algebra $A$ is defined according to rule
\DrawEq{product of basis vectors, algebra}{\Cols}
}

\DefProof{product in algebra}
{
The equality
\eqRef{product of basis vectors, algebra}{\Cols}
is corollary of the statement that \eV
is the basis of $D$\Hyph algebra $A$.
Since the product in the algebra is a bilinear map,
then we can write the product of $a$ and $b$ as
\DrawEq{product in algebra, 1}{\Cols}
From equalities
\eqRef{product of basis vectors, algebra}{\Cols},
\eqRef{product in algebra, 1}{\Cols},
it follows that
\DrawEq{product in algebra, 2}{\Cols}
Since \eV is a basis of the algebra $A$, then the equality
\eqRef{product in algebra}{\Cols}
follows from the equality
\eqRef{product in algebra, 2}{\Cols}.
}

\DefText{D-module type}
{
Organization of coordinates of vector in matrix
is called $D$\Hyph module type.

In this section, we consider column vector
and row vector.
it is evident that there exist other forms of representation of vector.
For instance, we can represent coordinates of vector as
\nmTimes nm matrix or as triangular matrix.
Format of representation depends on considered problem.
}

\DefText{D-module type 1}
{
If a statement depends on the format of representation of vector,
we will specify either type of $D$\Hyph module,
or format of representation of basis.
Both ways of specifying the type of $D$\Hyph module are equivalent.
}

\DefText{Morphism of D algebra, injection 11}
{
(and therefore,
\ShowEq{Morphism of D algebra, injection}
}

\DefText{Morphism of D algebra, injection 1}
{
}

\DefText[3]{Morphism of D algebra}
{
\item There is relation between the matrix of homomorphism
and structural constants
\DrawEq[{#3}]{algebra, homomorphism and product (#1#2)}{\Cols(\SideNS)}
}

\DefText{algebra, homomorphism and product 11}
{
Since the map $h$ is homomorphism of rings,
then the equality
\DrawEq{algebra, homomorphism and product, 4}{\Cols}
follows from the equality
\eqRef{algebra, homomorphism and product eiej(11)}{\Cols}.
The equality
\DrawEq{algebra, homomorphism and product, 5 11}{\Cols}
follows from the theorem
\refTheorem{homomorphism of d algebra, coordinates}{11\Cols}
and the equality
\eqRef{algebra, homomorphism and product, 4}{\Cols}.
}

\DefText{algebra, homomorphism and product 1}
{
The equality
\DrawEq{algebra, homomorphism and product, 5 1}{\Cols}
follows from the theorem
\refTheorem{homomorphism of d algebra, coordinates}{1\Cols}
and the equality
\eqRef{algebra, homomorphism and product eiej(1)}{\Cols}.
}

\DefDefinition{commutator of algebra}
{
The \AddIndex{commutator}{commutator of algebra}
\ShowEq{commutator of algebra}
measures commutativity in $D$\Hyph algebra $A$.
$D$\Hyph algebra $A$ is called
\AddIndex{commutative}{commutative D algebra},
if
\ShowEq{commutative D algebra}
}

\DefDefinitionNote{nucleus of algebra}
{
The set\,\footnotemark
\ShowEq{nucleus of algebra}
is called the
\AddIndex{nucleus of an $D$\Hyph algebra $A$}{nucleus of algebra}.
}
{The definition is based on
the similar definition in
\citeBib{Richard D. Schafer}, p. 13.}

\DefDefinition{associator of algebra}
{
The \AddIndex{associator}{associator of algebra}
\ShowEq{associator of algebra}
\ShowEq{associator of algebra =}
measures associativity in $D$\Hyph algebra $A$.
$D$\Hyph algebra $A$ is called
\AddIndex{associative}{associative D algebra},
if
\ShowEq{associative D algebra}
}

\DefTheorem{associator of algebra}
{
Let $\Basis e$ be basis of $D$\Hyph algebra $A$. Then
\ShowEq{associator of algebra = A}
where
\AddIndex{coordinates of associator}{coordinates of associator}
are defined by the equality
\ShowEq{coordinates of associator}
\ShowEq{coordinates of associator =}
}

\DefProof{associator of algebra}
{
The equality
\ShowEq{associator of algebra = Ae}
follows from the equality
\EqRef{associator of algebra =}.
The equality
\EqRef{coordinates of associator =}
follows from the equality
\EqRef{associator of algebra = Ae}.
}

\DefDefinitionNote{center of algebra}
{
The set\,\footnotemark
\ShowEq{center of algebra}
is called the
\AddIndex{center of an $D$\Hyph algebra $A_1$}{center of algebra}.
}{
The definition is based on
the similar definition in
\citeBib{Richard D. Schafer}, page 14.
}

\DefDefinition{otimes -}
{
Bilinear map
\ShowEq{otimes -}
is defined by the equality
\ShowEq{otimes -, 1}
}


==> Stmt.Module.Eq.tex <==
%auto-ignore
\ePrints{1506.00061,7287-9339,0803.3276,7100-9423,357606033,2023.01.07}
\ifx\Semafor\ValueOff
\input{Stmt.Module.Ref}
\fi

\newcommand\aUD[3]{\ensuremath{{#1}^{\gi{#2}}_{\gi{#3}}}}%
\newcommand\Entry[5][]{#2_{#3}^{}\AUD{{}}{#4}{#5}{}_{#1}}%
\newcommand\aU[3][]{\ensuremath{#2^{#1\gi{#3}}}}%
\newcommand\aD[3][]{\ensuremath{#2_{#1\gi{#3}}}}%
\newcommand\eV[1][]
{
\def\argA{#1}%
\eVA%
}
\newcommand\eVA[1][]{\ensuremath{\Basis e_{\argA}}{#1} }%
\newcommand\EV[2]{e_{#1\cdot\gi{#2}}}
\newcommand\ECol[2]{\ensuremath{e_{#1\gi{#2}}}}
\newcommand\ERow[2]{\ensuremath{\aU{e_{#1}}{#2}}}
\newcommand\AOn[1][A]{\ensuremath{#1^{n+1\otimes}}}
\newcommand\LAnA[1][A]{\ensuremath{\mathcal L(D;#1^n\rightarrow #1)}}
\newcommand\nTimes[1][n]{$\gi{#1}\times\gi{#1}$ }
\newcommand\nmTimes[2]{$\gi{#1}\times\gi{#2}$ }
\def\Eij{\ARow ei\ARow ej}

\newcommand{\LAVW}{\mathcal L(A\CRcirc;V\rightarrow W)}

\newcommand\Ei
{
\begin{pmatrix}
1&0&0&0\\
0&-1&0&0\\
0&0&1&0\\
0&0&0&1
\end{pmatrix}
}

\newcommand\Ej
{
\begin{pmatrix}
1&0&0&0\\
0&1&0&0\\
0&0&-1&0\\
0&0&0&1
\end{pmatrix}
}

\newcommand\Ek
{
\begin{pmatrix}
1&0&0&0\\
0&1&0&0\\
0&0&1&0\\
0&0&0&-1
\end{pmatrix}
}

\newcommand\KR[1]
{
\left(
\begin{array}{rr@{}rr@{}rr@{}r}
\end{array}
\right)
}

\newcommand\PMatrix[4][]
{
\begin{pmatrix}
\aUD {#2}11#1&...&\aUD {#2}1{#3}#1\\
...&...&...\\
\aUD {#2}{#4}1#1&...&\aUD {#2}{#4}{#3}#1
\end{pmatrix}
}

\newcommand\ColMatrix[2]
{
\begin{pmatrix}
\aU {#1}1\\...\\ \aU {#1}{#2}
\end{pmatrix}
}

\newcommand\RowMatrix[2]
{
\begin{pmatrix}
\aD {#1}1&...&\aD {#1}{#2}
\end{pmatrix}
}

\AddEq{basis e of V}
{
$\eV=(\aD e1,...,\aD en)$
}

\AddEq{basis e=1}
{
$\eV=\{1\}$.
}

\AddEq[1]{Let aij rco bij}
{
\ShowEq{a in Aoxn}{\aUD aij}2,
\ShowEq{a in Aoxn}{\aUD bij}2#1
}

\AddEquation{aij rco bij}
{
\PMatrix anm
\RCcirc
\PMatrix bkn
=
\begin{pmatrix}
\aUD a1i\circ\aUD bi1&...&\aUD a1i\circ\aUD bik\\
...&...&...\\
\aUD ami\circ\aUD bi1&...&\aUD ami\circ\aUD bik
\end{pmatrix}
}

\AddEq{a rco b ij}
{
\aUD{(a\RCcirc b)}ij=\aUD aik\circ\aUD bkj
}

\AddEq{matrix vx}
{
\[
a=
\begin{pmatrix}
\aU v1&\aU x1\\
\aU v2&\aU x2
\end{pmatrix}
\]
}

\AddEquation{qdet21 vx}
{
\RCdet 21a=
\aU v2-\aU x2(\aU x1)^{-1}\aU v1
}

\AddEq{any quaternion}
{
\[
a=\aU a0+\aU a1i+\aU a2j+\aU a3k
\]
}

\AddEq{any quaternion i j ij}
{
\[
a=\aU a0+\aU a1i+\aU a2j+\aU a3ij
\]
}

\DefText{D-Algebra Type}
{
\ShowConvention{basis of algebra as basis of module}

\ShowConvention{we use separate color for index of element}

\ShowText{algebra inherits type of module}

\ShowEq{def ab=ba}%
\TwoColText
{
\ShowEq{\DefCol}%
\ShowDefinition{type of algebra}
\ShowConvention{unit of algebra in basis}
}
{
\ShowEq{\DefRow}%
\ShowDefinition{type of algebra}
\ShowConvention{unit of algebra in basis}
}
}

\DefText{Preliminary product in algebra}
{
\TwoColText
{
\ShowEq{\DefCol}%
\ShowTheorem{product in algebra}
\proofTheorem{\RefLinearMap}{product in algebra}{\Cols}
}
{
\ShowEq{\DefRow}%
\ShowTheorem{product in algebra}
\proofTheorem{\RefLinearMap}{product in algebra}{\Cols}
}
}

\AddEq{spectrum of matrix}
{
\ProductType $\mathrm{spec}(a)$
}

\AddEq[2]{left map a En}
{
\ensuremath{\Vector{\eV[#2]#1}}
}

\AddEq[2]{right map a En}
{
\ensuremath{\Vector{#1\eV[#2]}}
}

\AddEq[2]{fov=b e o v}
{
\Vector f\circ{#2}=
\ShowEq{\SideWS map a En}{#1}{}
\circ{#2}
}

\AddEq [3]{L(A->B)}
{
\ensuremath{\mathcal L(#1;#2\rightarrow #3)}%
}

\AddEq{conjugation in algebra, 4}
{
\[
\begin{matrix}
\giA\le\gik\le\gin&\giA\le\gil\le\gin&\giA\le\gi p\le\gin
\end{matrix}
\]
}

\AddEquation{structural constants Cikl}
{
\begin{matrix}
\aUD Ck{k0}=\aUD Ck{0k}=1
&
\aUD Cp{kl}=-\aUD Cp{lk}
\end{matrix}
}

\AddEquation{structural constants C000}
{
\begin{matrix}
\hphantom{\aUD C0{00}=}
\aUD C0{00}=1
&\aUD C0{kl}=\hphantom{-}\aUD C0{lk}
\end{matrix}
}

\AddEq{x=c12+j}
{
x=C_1+C_2i+\frac 12 j
}

\AddEq[1]{ix-xi-1}
{
p_{#1}(x)=ix-xi-#1
}

\AddEq{characteristic polynomial}
{
\det(a-b\aD En)
}

\AddEq{projection maps, quaternion}
{
\begin{matrix}
P^{\gi 0}\circ a=a^{\gi 0}&P^{\gi 0\cdot}_{}{}^{\gi 0}_{\gi 0}=1&
R^{\gi 0}\circ a=a^{\gi 0}&R^{\gi 0\cdot}_{}{}^{\gi 0}_{\gi 0}=1
\\
P^{\giA}\circ a=a^{\giA}i&P^{\giA\cdot}_{}{}^{\giA}_{\giA}=1&
R^{\giA}\circ a=a^{\giA}&R^{\giA\cdot}_{}{}^{\gi 0}_{\giA}=1
\\
P^{\gi 2}\circ a=a^{\gi 2}j&P^{\gi 2\cdot}_{}{}^{\gi 2}_{\gi 2}=1&
R^{\gi 2}\circ a=a^{\gi 2}&R^{\gi 2\cdot}_{}{}^{\gi 0}_{\gi 2}=1
\\
P^{\gi 3}\circ a=a^{\gi 3}k&P^{\gi 3\cdot}_{}{}^{\gi 3}_{\gi 3}=1&
R^{\gi 3}\circ a=a^{\gi 3}&R^{\gi 3\cdot}_{}{}^{\gi 0}_{\gi 3}=1
\end{matrix}
}

\AddEq{P0z=}
{
P^{\gi 0}\circ x=\frac 14(1\otimes 1-i\otimes i-j\otimes j-k\otimes k)\circ x
=\frac 14(x-ix i-jx j-kx k)
}

\AddEq{P1z=}
{
P^{\gi 1}\circ x=\frac 14(1\otimes 1-i\otimes i+j\otimes j+k\otimes k)\circ x
=\frac 14(x-ix i+jx j+kx k)
}

\AddEq{P2z=}
{
P^{\gi 2}\circ x=\frac 14(1\otimes 1+i\otimes i-j\otimes j+k\otimes k)\circ x
=\frac 14(x+ix i-jx j+kx k)
}

\AddEq{P3z=}
{
P^{\gi 3}\circ x=\frac 14(1\otimes 1+i\otimes i+j\otimes j-k\otimes k)\circ x
=\frac 14(x+ix i+jx j-kx k)
}

\AddEquation{polynomial*polynomial}
{
*:A^{n\otimes}\times A^{m\otimes}
\rightarrow A^{n+m-1\otimes}
}

\AddEquation{polynomial*polynomial, 1}
{
(a_1\otimes...\otimes a_n)*(b_1\otimes...\otimes b_n)
=
a_1\otimes...\otimes a_{n-1}\otimes a_nb_1\otimes b_2\otimes...\otimes b_n
}

\AddEq{polynomials a o x,b o x}
{
$a\circ x^n$, $b\circ x^m$
}

\AddEquation{(a*b)x=(ax)(bx)}
{
(a*b)\circ x^{n+m}=(a\circ x^n)(b\circ x^m)
}

\AddEq{x=i,j}
{
$x=i$, $x=j$.
}

\AddEquation{p=a1 o ij+a2 o ji}
{
p(x)=a_1\circ((x-i)(x-j))+a_2\circ((x-j)(x-i))
}

\AddEq{r=xx+1}
{
r(x)=x^2+1
}

\AddEquation{a1 o ij+a2 o ji=xx+1}
{
a_1\circ(x^2-ix-xj+k)+a_2\circ(x^2-jx-xi-k)=x^2+1
}

\AddEq{square root}
{
\symb{\sqrt a}{square root}{}%
$x=\ShowSymbol{square root}{}$
}

\AddEq{x2=a}
{
x^2=a
}

\AddEq{Re sqrt a ne 0}
{
$\re\sqrt a\ne 0$,
}

\AddEq{x=x12}
{
$x=x_1$, $x=x_2$
}

\AddEquation{x2=-x1}
{
x_2=-x_1
}

\AddEquation{|x|=sqrt a}
{
\begin{matrix}
x\in\im H&a\in\re H&|x|=\sqrt{-a}
\end{matrix}
}

\AddEq[1]{aij=.ox.}
{
\Entry a{#1}ij=\AoxB{\Entry[s0]a{#1}ij}{\Entry[s1]a{#1}ij}
}

\AddEquation{vi=aij o wj}
{
\aU vi=(\AoxB{\Entry[s1]a{}ij}{\Entry[s2]a{}ij})\circ\aU wj
=\Entry[s1]a{}ij\aU wj\Entry[s2]a{}ij
}

\AddEq[1]{a1 o+a2 o=xx+1 (ij) x x2=}
{
a_1\circ #1+a_2\circ #1=#1
}

\AddEquation{a1 o+a2 o=xx+1 xx}
{
a_1\circ x^2+a_2\circ x^2=x^2
}

\AddEquation{a1 o+a2 o=xx+1 x}
{
a_1\circ (ix)+a_1\circ (xj)+a_2\circ (jx)+a_2\circ (xi)=0
}

\AddEquation{a1 o+a2 o=xx+1 1}
{
a_1\circ k-a_2\circ k=1
}

\AddEquation{a1 o+a2 o=xx+1 x x=1}
{
a_1\circ i+a_1\circ j+a_2\circ j+a_2\circ i=0
}

\AddEq{D*V->V to product}
{
(a,v)\rightarrow av
}

\AddEq{A*V->V to left product}
{
(a,v)\rightarrow av
}

\AddEq{A*V->V to right product}
{
(v,a)\rightarrow va
}

\AddEq{a rc x=b pdf}
{
\texorpdfstring{$a\RCstar x=b$}{a rc x=b}
}

\AddEquation{coordinates of map f 18, associative algebra}
{
f\circ x=f^{\gii}_{\gij}x^{\gij}e_{2\cdot\gii}
}

\AddEquation{coordinates of map Ik, associative algebra}
{
F_k\circ x=F_{k\cdot}^{}{}^{\gii}_{\gij}x^{\gij}e_{2\cdot\gii}
}

\AddEquation{coordinates of map A1 A2, 3, associative algebra}
{
\begin{split}
f^{\gik}_{\gil}x^{\gil}e_{2\cdot\gik}
&=
f^{k\cdot\gi{ij}} e_{2\cdot\gii}
F_{k\cdot}^{}{}^{\gim}_{\gil}x^{\gil}e_{2\cdot\gim}
e_{2\cdot\gij}
\\
&=
f^{k\cdot\gi{ij}}
F_{k\cdot}^{}{}^{\gim}_{\gil}x^{\gil}
C^{\gi p}_{\gi{im}}
C^{\gik}_{\gi{pj}}
e_{2\cdot\gik}
\end{split}
}

\AddEq [2]{coordinates of map A1 A2, 2, associative algebra}
{
\def\Cdot{}
\def\Temp{-}%
\edef\Tempa{#2}%
\ifx\Tempa\Temp%
\else
\def\Cdot{#2\cdot}
\fi
#1^{\gik}_{\gil}=#1^{k\cdot\gi{ij}}
F_{k\cdot}^{}{}^{\gim}_{\gil}
C_{\Cdot}{}^{\gi p}_{\gi{im}}C_{\Cdot}{}^{\gik}_{\gi{pj}}
}

\AddEq{1 ox i-i ox 1}
{
\[
i\otimes 1-1\otimes i\in H^{2\otimes}
\]
}

\AddEquation{1 ox i-i ox 1 matrix}
{
\begin{pmatrix}
0&-1&0&0\\
1&0&0&0\\
0&0&0&-1\\
0&0&1&0
\end{pmatrix}
-
\begin{pmatrix}
0&-1&0&0\\
1&0&0&0\\
0&0&0&1\\
0&0&-1&0
\end{pmatrix}
=
\begin{pmatrix}
0&0&0&0\\
0&0&0&0\\
0&0&0&-2\\
0&0&2&0
\end{pmatrix}
}

\AddEquation{ax^2bxcx^3d}
{
\begin{split}
ax^2bxcx^3d&=ax(xbxcx^3)=(ax)x(bxcx^3d)=(ax^2b)x(cx^3d)
\\
&=(ax^2bxc)x(x^2d)=(ax^2bxcx)x(xd)=(ax^2bxcx^2)xd
\end{split}
}

\AddEquation{f in L(A,A), 2, associative algebra}
{
f=
a^{k\cdot \gi{ij}}(e_{\gii}\otimes e_{\gij})\circ F_k
=
a^{k\cdot \gi{ij}}e_{\gii}I_ke_{\gij}
}

\AddEquation{standard representation of map A1 A2, associative algebra}
{
f=
f^{k\cdot\gi{ij}}(\aU ei\otimes \aU ej)\circ F_k
=
f^{k\cdot\gi{ij}}\aU eiF_k\aU ej
}

\AddEquation{f(a)+f(b)=}
{
(f(a)+f(b))(x)=f(a)(x)+f(b)(x)
}

\AddEquation{f(a+b)=f(a)+f(b)}
{
f(a+b)=f(a)+f(b)
}

\AddEquation{f(a-b)=0}
{
f(a-b)=\Vector 0
}

\AddEquation{f(0)=v0}
{
f(0)=\Vector 0
}

\AddEq{0:A->A}
{
\ShowEq{f:A->B}{\Vector 0}AA
}

\AddEquation{0ov=0}
{
\Vector 0\circ v=0
}

\AddEquation{fa=fa+f0}
{
f(a)(x)=f(a+0)(x)=f(a)(x)+f(0)(x)
}

\AddEquation{f0x=0}
{
f(0)(x)=0
}

\AddEq[3]{a in Aoxn}
{
$#1\in A^{#2\otimes}$#3
}

\AddEq[2]{Aoxn}
{
$A^{#1\otimes}$#2
}

\DefText{definition of A module}
{
\ShowEq{def AModule}
\ShowEq{def universal}

\ShowTheorem{A module -> algebra is associative}
\ShowProof{A module -> algebra is associative}

\ShowDefinition{module over algebra}

\ShowEq{def AVector}
\ShowDefinition{module over algebra}

\ShowEq{def AModule}
\ShowTheorem{module over algebra}
\ShowProof{module over algebra}

\def\TheoremStyle{ParacolTheorem}%
\ShowTheorem{definition of A module}
\def\TheoremStyle{ShadedTheorem}%
\ShowTheorem{definition of A module, property}
\ShowProof{definition of A module}
}

\AddEq{X0=v in J}
{
$X_0=v\subseteq J(v)$.
}

\DefText{linear combination of vectors}
{
\ProveTheorem{set of vectors generated by set of vectors}

\ProveTheorem{d in D->d in D1}

\ProveTheorem{da in DA->da in D1A}

\ShowConvention{da in DA->da in D1A}

\ShowDefinition{linear combination of vectors}

\ShowConvention{sum av() convention}

\ProveTheorem{linearly depends on rest of vectors}

\ShowText{0=0vi}

\ShowDefinition{linearly independent vectors}
}

\DefText{basis of module}
{
\ShowText{generating set of module}

\ShowDefinition{generating set of module}

\ShowText{quasibasis of module}

\ShowDefinition{basis of module}

\ShowDefinition{coordinates of vector}

\ProveTheorem{quasibasis of module}

\ProveTheorem{linear dependence between vectors of basis}

\ProveTheorem{coordinates of vector with linear dependence}

\ProveTheorem{quasibasis of module is basis}

\ShowDefinition{free module over ring}

%\ShowEq{def \Base{}Vector}
\ShowTheorem{vector space is free module}
\ShowProof{basis over division algebra}

\ShowTheorem{coordinates of vector}
\ShowProof{coordinates of vector of free module}
}

\AddEq{ci=0 1n}
{
$\ACol ci=0$, $\gii=\gi 1$, ..., $\gin$.
}

\AddEq[2]{homomorphism D algebra 11}
{
(
\ShowEq{f: A->B}h{D_1}{D_2}\ \ \,
\ShowEq{f: A->B}{#1}{#2_1}{#2_2}{}
)
}

\AddEq[2]{homomorphism D algebra 1}
{
\ShowEq{f: A->B}{#1}{#2_1}{#2_2}{}
}

\AddEq[2]{homomorphism A module 111}
{
(
\ShowEq{f: A->B}h{D_1}{D_2}{}\ \ \,
\ShowEq{f: A->B}{#1}{A_1}{A_2}{}\ \ \,
\ShowEq{f: A->B}{#2}{V_1}{V_2}{}
)
}

\AddEq[2]{homomorphism A module 11}
{
(
\ShowEq{f: A->B}{#1}{A_1}{A_2}{}\ \ \,
\ShowEq{f: A->B}{#2}{V_1}{V_2}{}
)
}

\AddEq[2]{homomorphism A module 1}
{
\ShowEq{f: A->B}{#2}{V_1}{V_2}{}
}

\AddEq{ref linear map of D module 1}
{
\eqRef{homomorphism, f(p+q)=}{D module},
\eqRef{homomorphism, f(pq)=}{D module}.
}

\AddEq[2]{ref homomorphism of D algebra(1)}
{
\eqRef{homomorphism, f(p+q)=}1,
\eqRef{homomorphism, f(pq)=}1,
\ShowEq{ref homomorphism of D algebra()}{#1}{#2}
}

\AddEq[2]{ref homomorphism of D algebra()}
{
\eqRef{homomorphism, f v+w=}{(#1#2)g},
\eqRef{left homomorphism, f av=}{(#1#2)g}
}

\AddEq[3]{ref homomorphism of A vector space(1)}
{
\eqRef{homomorphism, f(p+q)=}{\SideWS A module},
\eqRef{homomorphism, f(pq)=}{\SideWS A module},
\ShowEq{ref homomorphism of A vector space()}{#1}{#2}{#3}
}

\AddEq[3]{ref homomorphism of A vector space()}
{
\eqRef{homomorphism, f v+w=}{g(#1#2)\SideWS A module},
\eqRef{homomorphism, f vw=}{(#1#2)\SideWS A module},
\eqRef{\SideWS homomorphism, f av=}{(#1#2)}
}

\AddEq[3]{define homomorphism of D algebra 11}
{
\DrawEq[hpq]{homomorphism, f(p+q)=}1
\DrawEq[hpq]{homomorphism, f(pq)=}1
\ShowEq{define homomorphism of D algebra 1}{#1}{#2}{#3}
}

\AddEq[3]{define homomorphism of D algebra 1}
{
\DrawEq[fab]{homomorphism, f v+w=}{(#1#2)g}
\FrameEqRef[fab]{homomorphism, f vw=}{(#1#2)g}
\DrawEq[fp{#3}a]{left homomorphism, f av=}{(#1#2)g}
\ShowEq{ap AD #1#2}
}

\AddEq[5]{define homomorphism of module 111}
{
\DrawEq[fpq]{homomorphism, f(p+q)=}{\SideNS}
\DrawEq[fpq]{homomorphism, f(pq)=}{\SideNS}
\ShowEq{define homomorphism of module 11}{#1}{#2}{#3}{#4}{#5}
}

\AddEq[5]{define homomorphism of module 11}
{
\DrawEq[gab]{homomorphism, f v+w=}{({#1}{#2}{#3})g \SideNS}
\DrawEq[gab]{homomorphism, f vw=}{({#1}{#2}{#3})g \SideNS}
\DrawEq[gp{#4}a]{left homomorphism, f av=}{({#1}{#2}{#3})g \SideNS}
\ShowEq{define homomorphism of module 1}{#1}{#2}{#3}{#4}{#5}
}

\AddEq[5]{define homomorphism of module 1}
{
\DrawEq[hvw]{homomorphism, f v+w=}{({#1}{#2}{#3})h \SideNS}
\DrawEq[ha{#5}v]{\SideWS homomorphism, f av=}{({#1}{#2}{#3})h \SideNS}
\ShowEq{vap VAD #1#2#3}
}

\AddEq[5]{define homomorphism of A module 111}
{
\DrawEq[hpq]{homomorphism, f(p+q)=}{\SideWS A module}
\DrawEq[hpq]{homomorphism, f(pq)=}{\SideWS A module}
\ShowEq{define homomorphism of A module 11}{#1}{#2}{#3}{#4}{#5}
}

\AddEq[5]{define homomorphism of A module 11}
{
\DrawEq[gab]{homomorphism, f v+w=}{g(#1#2)\SideWS A module}
\DrawEq[gab]{homomorphism, f vw=}{(#1#2)\SideWS A module}
\DrawEq[gp{#4}a]{\SideWS homomorphism, f av=}{(#1#2)}
\ShowEq{define homomorphism of A module 1}{#1}{#2}{#3}{#4}{#5}
}

\AddEq[5]{define homomorphism of A module 1}
{
\DrawEq[fuv]{homomorphism, f v+w=}{f(#1#2)\SideWS A module}
\DrawEq[fa{#5}v]{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module}
\ShowEq{vap VAD #1#2#3}
}

\AddEq[3]{define homomorphism of D module 11}
{
\DrawEq[hpq]{homomorphism, f(p+q)=}{D module}
\DrawEq[hpq]{homomorphism, f(pq)=}{D module}
\ShowEq{define homomorphism of D module 1}{#1}{#2}{#3}
}

\AddEq[3]{define homomorphism of D module 1}
{
\DrawEq[fab]{homomorphism, f v+w=}{f D module #1#2}
\DrawEq[fp{#3}a]{left homomorphism, f av=}{f D module #1#2}
\ShowEq{vp VD #1#2}
}

\AddEq{morphism of representation, algebra, 23}
{
\BlueText{f\circ (h_{1.23}(a)(b))}
=h_{2.23}(\RedText{f\circ a})
(\BlueText{f\circ b})
}

\AddEq{algebra, morphism of representation 23, 1}
{
f\circ (C_1\circ (a,b))=C_2\circ (f\circ a,f\circ b)
}

\DefText[7]{homomorphism of A module 1}
{
\ShowFootnote{homomorphism of A module}{#1}{#2}{#3}{#4}{#5}{#6}
\ShowTheorem{homomorphism A module}{#1}{#2}{#3}{#4}{#5}{#6}
\AddIndex{}{matrix of homomorphism}
\AddIndex{}{coordinates of homomorphism}
\ShowProof{homomorphism A module}{#1}{#2}{#3}{#4}{#5}{#6}

\ShowTheorem{matrix generates A module homomorphism}{#1}{#2}{#3}{#4}{#5}{#6}
\ShowProof{matrix generates A module homomorphism}{#1}{#2}{#3}{#4}{#5}{#6}{#7}

\ShowRemark{homomorphism of vector space 2}{#1}{#2}{#3}
}

\DefText[7]{homomorphism of A module (1)}
{
\ShowEq{\DefCol}
\ShowText{homomorphism of A module 1}{#1}{#2}{#3}{#4}{#5}{#6}{#7}

\ShowEq{\DefRow}
\ShowText{homomorphism of A module 1}{#1}{#2}{#3}{#4}{#5}{#6}{#7}
}

\DefText[7]{homomorphism of A module ()}
{
\TwoColText
{
\ShowEq{\DefCol}
\ShowFootnote{homomorphism of A module}{#1}{#2}{#3}{#4}{#5}{#6}
}
{
\ShowEq{\DefRow}
\ShowFootnote{homomorphism of A module}{#1}{#2}{#3}{#4}{#5}{#6}
}

\TwoColText
{
\ShowEq{\DefCol}
\ShowTheorem{homomorphism A module}{#1}{#2}{#3}{#4}{#5}{#6}
}
{
\ShowEq{\DefRow}
\ShowTheorem{homomorphism A module}{#1}{#2}{#3}{#4}{#5}{#6}
}
\AddIndex{}{matrix of homomorphism}
\AddIndex{}{coordinates of homomorphism}
\TwoColText
{
\ShowEq{\DefCol}
\ShowProof{homomorphism A module}{#1}{#2}{#3}{#4}{#5}{#6}
}
{
\ShowEq{\DefRow}
\ShowProof{homomorphism A module}{#1}{#2}{#3}{#4}{#5}{#6}
}

\TwoColText
{
\ShowEq{\DefCol}
\ShowTheorem{matrix generates A module homomorphism}{#1}{#2}{#3}{#4}{#5}{#6}
\ShowProof{matrix generates A module homomorphism}{#1}{#2}{#3}{#4}{#5}{#6}{#7}
}
{
\ShowEq{\DefRow}
\ShowTheorem{matrix generates A module homomorphism}{#1}{#2}{#3}{#4}{#5}{#6}
\ShowProof{matrix generates A module homomorphism}{#1}{#2}{#3}{#4}{#5}{#6}{#7}
}

\TwoColText
{
\ShowEq{\DefCol}
\ShowRemark{homomorphism of vector space 2}{#1}{#2}{#3}
}
{
\ShowEq{\DefRow}
\ShowRemark{homomorphism of vector space 2}{#1}{#2}{#3}
}
}

\DefText[8]{def homomorphism A module}
{
\ShowText{algebra over ring (#1#2)}%
\ShowText{module over algebra (#2#3)}%

\ShowDefinition{homomorphism A module}{#1}{#2}{#3}{#4}{#5}{#6}

\ShowText{notation for homomorphism of module}

\ShowTheorem{define homomorphism A module}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
\ShowProof{define homomorphism A module}{#1}{#2}{#3}{#4}{#5}{#6}

\ShowText{homomorphism of A module (#1)}{#1}{#2}{#3}{#4}{#5}{#6}{#8}

%\ShowDefinition{iso end aut morphism vector space}

%\ShowTheorem{set of automorphisms}
}

\AddEq[1]{A1=A2 pdf}
{
\texorpdfstring{$#1_1=#1_2=#1$}{#1 1=#1 2=#1}
}

\DefText[6]{linear map of D module}
{
\,

\ShowDefinition{linear map of D module}{#1}{#2}{#3}{#4}

\ShowText{notation for linear map}{#1}{#2}{#3}{#4}

\ShowTheorem{linear map of D module}{#1}{#2}{#3}{#4}{#5}
\ShowProof{linear map of D module}{#1}{#2}

\ShowEq{\DefCol}
\ShowFootnote{homomorphism of D module}{#1}{#2}{#3}{#4}
\ShowEq{\DefRow}
\ShowFootnote{homomorphism of D module}{#1}{#2}{#3}{#4}

\TwoColText
{
\ShowEq{\DefCol}
\ShowTheorem{linear map of D module, coordinates}{#1}{#2}{#3}{#4}{#6}
}
{
\ShowEq{\DefRow}
\ShowTheorem{linear map of D module, coordinates}{#1}{#2}{#3}{#4}{#6}
}

\ShowEq{\DefCol}
\ShowProof{linear map of D module, coordinates}{#1}{#2}{#3}{#4}{#5}

\ShowEq{\DefRow}
\ShowProof{linear map of D module, coordinates}{#1}{#2}{#3}{#4}{#5}

\TwoColText
{
\ShowEq{\DefCol}
\ShowTheorem{matrix generates D module homomorphism}{#1}{#2}{#3}{#4}
}
{
\ShowEq{\DefRow}
\ShowTheorem{matrix generates D module homomorphism}{#1}{#2}{#3}{#4}
}

\TwoColText
{
\ShowEq{\DefCol}
\ShowProof{matrix generates D module homomorphism}{#1}{#2}{#3}{#4}{#5}
}
{
\ShowEq{\DefRow}
\ShowProof{matrix generates D module homomorphism}{#1}{#2}{#3}{#4}{#5}
}

\ShowText{we identify linear map and matrix}{#1}{#2}
}

\AddEq{linear map, 0, D algebra}
{
\[f\circ 0=0\]
}

\AddEq[4]{D->*o+A}
{
\[
\xymatrix
{
#1\ar[r]|(.4){*}&\displaystyle\bigoplus_{\iI}#2_i
}
\ \ \ \ \ \,
#3\left(\bigoplus_{\iI}#4_i\right)=\bigoplus_{\iI}#3 #4_i
\]
}

\AddEq[4]{left D->*o+A}
{
\[
\xymatrix
{
#1\ar[r]|(.4){*}&\displaystyle\bigoplus_{\iI}#2_i
}
\ \ \ \ \ \,
#3\left(\bigoplus_{\iI}#4_i\right)=\bigoplus_{\iI}#3 #4_i
\]
}

\AddEq[4]{right D->*o+A}
{
\[
\xymatrix
{
#1\ar[r]|(.4){*}&\displaystyle\bigoplus_{\iI}#2_i
}
\ \ \ \ \ \,
\left(\bigoplus_{\iI}#4_i\right)#3=\bigoplus_{\iI}#4_i #3
\]
}

\AddEq[1]{f(pai)=pfai}
{
#1\circ(
a_1, ...,
pa_i, ...,
a_n)
=
p#1\circ(
a_1, ...,
a_i, ...,
a_n)
}

\AddEq[4]{a=ai ei}
{
\ensuremath{#1=\ACol{#1}{#3}\EBase {#2}{#3}#4}
}

\AddEquation{sum of maps, 31, polylinear}
{
\begin{split}
&(f+g)\circ(x_1,...,x_i+y_i,...,x_n)
\\
=&\,f\circ(x_1,...,x_i+y_i,...,x_n)
+g\circ(x_1,...,x_i+y_i,...,x_n)
\\
=&\,f\circ (x_1,...,x_i,...,x_n)+f\circ (x_1,...,y_i,...,x_n)
\\
+&g\circ (x_1,...,x_i,...,x_n)+g\circ (x_1,...,y_i,...,x_n)
\\
=&(f+g)\circ (x_1,...,x_i,...,x_n)
+(f+g)\circ (x_1,...,y_i,...,x_n)
\end{split}
}

\AddEquation{sum of maps, 32, polylinear}
{
\begin{split}
&(f+g)\circ(x_1,...,px_i,...,x_n)
\\
=&f\circ(x_1,...,px_i,...,x_n)+g\circ(x_1,...,px_i,...,x_n)
\\
=&pf\circ (x_1,...,x_i,...,x_n)+pg\circ (x_1,...,x_i,...,x_n)
\\
=&p(f\circ (x_1,...,x_i,...,x_n)+g\circ (x_1,...,x_i,...,x_n))
\\
=&p(f+g)\circ (x_1,...,x_i,...,x_n)
\end{split}
}

\AddEq{module of polylinear maps, 1}
{
$f$, $g$, $h\in\mathcal L(D;A_1\times...\times A_2\rightarrow S)$.
}

\AddEq{module of polylinear maps, 2}
{
$a=(a_1,...,a_n)$, $a_1\in A_1$, ..., $a_n\in A_n$,
\begin{align*}
(f+g)\circ a=&f\circ a+g\circ a=g\circ a+f\circ a
\\
=&(g+f)\circ a
\\
((f+g)+h)\circ a=&
(f+g)\circ a+h\circ a=(f\circ a+g\circ a)+h\circ a
\\
=&f\circ a+(g\circ a+h\circ a)=f\circ a+(g+h)\circ a
\\
=&(f+(g+h))\circ a
\end{align*}
}

\AddEq{0:A1n->S}
{
\[
0:v\in A_1\times...\times A_n\rightarrow 0\in S
\]
}

\AddEq{0+f=f 1n}
{
\[
(0+f)\circ (a_1,...,a_n)=0\circ (a_1,...,a_n)+f\circ (a_1,...,a_n)=f\circ (a_1,...,a_n)
\]
}

\AddEq{f-f=0 1n}
{
\begin{align*}
(f+(-f))\circ (a_1,...,a_n)&=f\circ (a_1,...,a_n)+(-f)\circ (a_1,...,a_n)
\\&=f\circ (a_1,...,a_n)-f\circ (a_1,...,a_n)
\\&=0
=0\circ (a_1,...,a_n)
\end{align*}
}

\AddEq{sum of maps, 4, polylinear}
{
\begin{align*}
(f+g)\circ (a_1,...,a_n)
&=f\circ (a_1,...,a_n)+g\circ (a_1,...,a_n)\\
&=g\circ (a_1,...,a_n)+f\circ (a_1,...,a_n)\\
&=(g+f)\circ (a_1,...,a_n)
\end{align*}
}

\AddEq{f-f=0}
{
\[
f+(-f)=0
\]
}

\AddEq{-f:A1n->S}
{
\[
-f:(a_1,...,a_n)\in A_1\times...\times A_n\rightarrow -(f\circ(a_1,...,a_n))\in S
\]
}

\AddEq{(p+q)f=pf+qf 1}
{
\begin{align*}
((p+q)f)\circ (x_1,...,x_n)=&(p+q)(f\circ (x_1,...,x_n))
\\
=&p(f\circ (x_1,...,x_n))+q(f\circ (x_1,...,x_n))
\\
=&(pf)\circ (x_1,...,x_n)+(qf)\circ (x_1,...,x_n)
\end{align*}
}

\AddEq{(p+q)f=pf+qf}
{
(p+q)f=pf+qf
}

\AddEq{p(qf)=(pq)f}
{
p(qf)=(pq)f
}

\AddEq{p(qf)=(pq)f 1}
{
\begin{align*}
(p(qf))\circ (x_1,...,x_n)=&p\ (qf)\circ (x_1,...,x_n)
=p\ (q\ f\circ (x_1,...,x_n))
\\
=&(pq)\ f\circ (x_1,...,x_n)=((pq)f)\circ (x_1,...,x_n)
\end{align*}
}

\AddEquation{product of map over scalar, 1, D module}
{
\begin{matrix}
\ShowSymbol{product of map over scalar}{D module}:A_1\rightarrow A_2
&d\in D&f\in\mathcal L(D;A_1\rightarrow A_2)
\end{matrix}
}

\AddEq{endomorphism of module from product, 1}
{
\[
\begin{matrix}
\vcenter
{
\xymatrix
{
A\ar[r]|{*}^{g_{23}}&A
}
}
&
\begin{matrix}
g_{23}:v\rightarrow l\circ v
\\
g_{23}\circ v:w\rightarrow (l\circ v)\circ w
\end{matrix}
\end{matrix}
\]
}

\AddEquation{a:LA12->LA12}
{
a:f\in\mathcal L(D;A_1\rightarrow A_2)\rightarrow af\in\mathcal L(D;A_1\rightarrow A_2)
}

\AddEquation{product of map over scalar, D module}
{
(\ShowSymbol{product of map over scalar}{D module})\circ x=d(f\circ x)
}

\AddEq[2]{b=foa}
{
$#1=f\circ #2$,
}

\AddEq[1]{f(ai+bi)=fai+fbi}
{
#1\circ(
a_1, ...,
a_i+ b_i, ...,
a_n)
=
#1\circ(
a_1, ...,
a_i, ...,
a_n)
+
#1\circ(
a_1, ...,
b_i, ...,
a_n)
}

\AddEq[1]{w=sum vi 2015}
{
J(v)=\left\{w:w=\sum_{\iIg}\aU ci\aD vi,\aU ci\in #1,
|\{\gii:\aU ci\ne 0\}|<\infty\right\}
}

\AddEq{p,q in D, v,w in V}
{
$p$, $q \in \Base_{\BaseExt}$, $v$, $w \in V$.
}

\AddEq[1]{o+Ai}
{
\[#1=\bigoplus_{\iI}#1_i\]
}

\AddEq{a=a1 o+ an}
{
\[a=a_1\oplus...\oplus a_n\]
}

\AddEq[2]{A1o+.n}
{
\[
#1=#1^1\oplus...\oplus #1^#2
\]
}

\AddEq[2]{A 1o+.n}
{
\[
#1=\aU{#1}1\oplus...\oplus \aU{#1}#2
\]
}

\AddEq[2]{a1o+.n}
{
\[
#1=#1_1\oplus...\oplus #1_#2
\]
}

\AddEq[1]{A1o+An=A1xAn}
{
\[
#1_1\oplus...\oplus #1_n=#1_1\times...\times #1_n
\]
}

\AddEq{rcd linear span, 0}
{
\[
\Vector a=\RowMatrix{\Vector a}n
=(\aD{\Vector a}i,\iIg)
\]
}

\AddEq{rcd linear span, 2}
{
\Vector b=\Vector a\RCstar x
}

\AddEq{rcd linear span, 6}
{
$\Vector b$, $\aD{\Vector a}i$
}

\AddEq{rcd linear span, 7}
{
\begin{align}
\EqLabel{rcd linear span, b}
\Vector b&=e\RCstar b\\
\EqLabel{rcd linear span, ai}
\aD{\Vector a}i&=e\RCstar\aD ai
\end{align}
}

\AddEq{rcd linear span, 8}
{
e\RCstar b=e\RCstar a\RCstar x
}

\AddEq{system of rcd linear equations}
{
a\RCstar x=b
}

\AddEq{inverce quaternion}
{
\[
x^{-1}=|x|^{-2}x^*
\]
}

\AddEq[2]{a=(a1.n set)}
{
#1=\AcMatrix{#1}{#2}
}

\AddEq[2]{a=(a1.n col)}
{
#1=\ColMatrix{#1}{#2}
}

\AddEq[2]{a=(a1.n row)}
{
#1=\RowMatrix{#1}{#2}
}

\AddEq{Expansion relative basis in algebra}
{
\[
a=a^{\gi i}e_{\gi i}
\]
}

\AddEq{av=sum av convention}
{
\[\aU ci\aD vi=\sum_{\gii\in\giI}\aU ci\aD vi\]
}

\AddEq{av=sum av()}
{
\[c(\gii)v(\gii)=\sum_{\gii\in\giI}c(\gii)v(\gii)\]
}

\AddEq{av=sum av()left}
{
\[c(\gii)v(\gii)=\sum_{\gii\in\giI}c(\gii)v(\gii)\]
}

\AddEq{av=sum av()right}
{
\[v(\gii)c(\gii)=\sum_{\gii\in\giI}v(\gii)c(\gii)\]
}

\AddEq[1]{foa=fi ai}
{
f\circ #1=
\RowMatrix fn
\RCcirc
\ColMatrix {#1}n
=\aD fi\circ\aU {#1}i
}

\AddEq{fioa=fij aj}
{
\aU fi\circ\VNumber=
\RowMatrix{\aU fi}n
\RCcirc
\ColMatrix{\VNumber}n
=\aUD fij\circ \aU{\VNumber}j
}

\AddEq{fij=(fi)j}
{
\[
\begin{pmatrix}
\RowMatrix{\aU f1}n
\\...\\
\RowMatrix{\aU fm}n
\end{pmatrix}
=
\PMatrix fnm
\]
}

\AddEq{vI=EI}
{
$\Vector I=(E,\aU I1,\aU I2,\aU I3)$
}

\AddEq[2]{foa=fi a}
{
\ColMatrix {#1}m
=
\ColMatrix fm
\circ #2=
\begin{pmatrix}
\aU f1\circ #2\\...\\ \aU fm\circ #2
\end{pmatrix}
}

\AddEq[3]{a=(a11.nm matrix)}
{
#1=\PMatrix {#1}{#2}{#3}
}

\AddEq[5]{b=f rco a}
{
\ColMatrix{#2}{#5}
=
\PMatrix {#1}{#4}{#5}
\RCcirc
\ColMatrix {#3}{#4}
=
\begin{pmatrix}
\aUD {#1}1i\circ\aU {#3}i\\
...\\
\aUD {#1}{#5}i\circ\aU {#3}i
\end{pmatrix}
}

\AddEq{fi:->}
{
\ShowEq{f:A->B}{\aU fi}{\Module}{\aU{\ModuleA}i}
}

\AddEquation{ft=tf1}
{
f(t)=tf(1)
}

\AddEq[2]{fij:->}
{
\ShowEq{f:A->B}{\aUD fij}{\aU {#1}j}{\aU {#2}i}
}

\AddEq{fij:-> left A}
{
\ShowEq{f:A->B}{f^{\gii}_{\gij}}{A_2(g\circ e_{V_1\cdot\gij})}{A_2e_{\gii}}
}

\AddEq{fij:-> right A}
{
\ShowEq{f:A->B}{f^{\gii}_{\gij}}{(g\circ e_{V_1\cdot\gij})A_2}{e_{\gii}A_2}
}

\DefProof{direct sum of n Abelian groups}
{
\TheoremFollows
\RefTheorem{direct sum of Abelian groups}.
}

\AddEq[2]{direct sum of modules}
{
\symb{#1\oplus #2}{direct sum}1
}

\AddEq[1]{c in ZA}
{
$#1\in Z(A)$,
}

\AddEq[1]{ca=ac}
{
c_{#1}a=ac_{#1}
}

\AddEquation{a(bc)=...=(bc)a}
{
a(bc)=(ab)c=(ba)c=b(ac)=b(ca)=(bc)a
}

\AddEq{c in ZAb}
{
$c_1$, $c_2\in Z(A,b)$.
}

\AddEq{c1 c2 in ZAb}
{
$c_1c_2\in Z(A,b)$.
}

\AddEquation{c1c2 in ZAb}
{
b(c_1c_2)=(bc_1)c_2=(c_1b)c_2=c_1(bc_2)=c_1(c_2b)=(c_1c_2)b
}

\AddEq[1]{(f+g)x=}
{
\[(f+g)(#1)=f(#1)+g(#1)\]
}

\AddEq[1]{(fp)x=}
{
\[(fp)(#1)=f(#1)p\]
}

\DefTheorem{cr-power, 1}
{
\ShowEq{cr-power, 1}
}

\AddEquation{cr-power, 1}
{
a^{\CRPower 1}=a
}

\AddEquation{cr-power, 1 1}
{
a^{\CRPower 1}=a^{\CRPower 0}\CRstar a=\UnitNMatrix\CRstar a=a
}

\DefTheorem{rc-power, 1}
{
\ShowEq{rc-power, 1}
}

\AddEquation{rc-power, 1}
{
a^{\RCPower 1}=a
}

\AddEquation{rc-power, 1 1}
{
a^{\RCPower 1}=a^{\RCPower 0}\RCstar a=\UnitNMatrix\RCstar a=a
}

\AddEq{center of A number}
{
\symb{Z(A,b)}{center of A number}1
}

\AddEq[1]{center Ac}
{
$Z(A,b)$#1
}

\AddEq[1]{c in S=>bc=cb}
{
c\in #1\Leftrightarrow cb=bc
}

\AddEq[3]{c in ZAa}
{
\ensuremath{#1\in Z(A,#2)}#3
}

\AddEq{p(c) p in D}
{
\begin{aligned}
p(x)&=p_0+p_1x+...+p_nx^n\\ &p_0,\ ...,\ p_n\in D 
\end{aligned}
}

\AddEq{c=p(b)}
{
\[
c=p(b)
\]
}

\AddEq{d in D c in S 12}
{
$d_1$, $d_2\in D$, $c_1$, $c_2\in Z(A,b)$.
}

\AddEq{dcb=bdc}
{
\begin{align*}
(d_1c_1+d_2c_2)b&=d_1c_1b+d_2c_2b=bd_1c_1+bd_2c_2\\&=b(d_1c_1+d_2c_2)
\end{align*}
}

\AddEq{dc in S}
{
$d_1c_1+d_2c_2\in Z(A,b)$.
}

\DefProof{direct sum of n D modules}
{
\TheoremFollows
\refTheorem{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}.
}

\AddEq{v=veV}
{
$v=v^{\gi i}\EV V i$.
}

\AddEquation{linear map in left A module}
{
f\circ(v\CRstar e_V )=(f_{\gi i}^{\gi j}\circ g\circ v^{\gi i})\ \EV W j
}

\AddEquation{linear map in right A module}
{
f\circ(e_V\RCstar v)=\EV W j(f_{\gi i}^{\gi j}\circ g\circ v^{\gi i})\ 
}

\AddEq{linear map in A module}
{
w=f\RCcirc (g\circ v)
}

\AddEq [1]{Ai, i=}
{
$#1_i$, $i=1$, $2$,
}

\AddEquation{module, (a+n)v=av+nv}
{
(a+n)v=av+nv\ \ \ a\in D\ \ \ n\in Z
}

\AddEquation{left module, (a+n)v=av+nv}
{
(a+n)v=av+nv\ \ \ a\in A\ \ \ n\in D
}

\AddEquation{right module, (a+n)v=av+nv}
{
v(a+n)=va+vn\ \ \ a\in A\ \ \ n\in D
}

\AddEq{(a+n)+(b+m)=}
{
(a+n)+(b+m)=(a+b)+(n+m)
}

\AddEq[1]{(d1+0)+(d2+0)}
{
(#1_1+0)+(#1_2+0)=(#1_1+#1_2)+(0+0)=(#1_1+#1_2)+0
}

\AddEquation{module, (a+n)+(b+m)=}
{
\begin{split}
((a+n)+(b+m))v&=av+nv+bv+mv=av+bv+nv+mv\\
&=(a+b)v+(n+m)v=((a+b)+(n+m))v
\end{split}
}

\AddEquation{g=CG}
{
g^{\gii}_{\gik}=C^{\gii}_{\gij}G^{\gij}_{\gik}
}

\AddEq [3]{matrix amn}
{
\[
#1=
\begin{pmatrix}
\aUD{#1}11&...&\aUD{#1}1{#3}\\
...&...&...\\
\aUD{#1}{#2}1&...&\aUD{#1}{#2}{#3}
\end{pmatrix}
\]
}

\AddEquation{g=(cF)G}
{
g^{\gii}_{\gik}=(c_{1.k.l}F_{k\cdot}^{}{}^{\gii}_{\gij}c_{2.k.l})G^{\gij}_{\gik}
}

\AddEq{C=cF}
{
\[
C=c_{1.k.l}F_kc_{2.k.l}
\]
}

\AddEq{Gkj in D}
{
$G^{\gij}_{\gik}\in D$,
}

\AddEquation{g=c(FG)}
{
g^{\gii}_{\gik}=c_{1.k.l}(F_{k\cdot}^{}{}^{\gii}_{\gij}G^{\gij}_{\gik})c_{2.k.l}
}

\AddEquation{left module, (a+n)+(b+m)=}
{
\begin{split}
((a+n)+(b+m))v&=av+nv+bv+mv=av+bv+nv+mv\\
&=(a+b)v+(n+m)v=((a+b)+(n+m))v
\end{split}
}

\AddEquation{right module, (a+n)+(b+m)=}
{
\begin{split}
v((a+n)+(b+m))&=va+vn+vb+vm=va+vb+vn+vm\\
&=v(a+b)+v(n+m)=v((a+b)+(n+m))
\end{split}
}

\AddEquation{module, (a+n)+(b+m)=, 1}
{
((a+n)+(b+m))v=(a+n)v+(b+m)v
}

\AddEquation{left module, (a+n)+(b+m)=, 1}
{
((a+n)+(b+m))v=(a+n)v+(b+m)v
}

\AddEquation{right module, (a+n)+(b+m)=, 1}
{
v((a+n)+(b+m))=v(a+n)+v(b+m)
}

\AddEq{(a+n)(b+m)=}
{
(a+n)(b+m)=(ab+ma+nb)+(nm)
}

\AddEq[1]{(d1+0)(d2+0)}
{
(#1_1+0)(#1_2+0)=(#1_1#1_2+0#1_1+0#1_2)+(0\,0)=(#1_1#1_2)+0
}

\AddEq{da in DA->da in D1A}
{
\[
(
I_{(1)}:d\in \Base\rightarrow d+0\in \Base_{(1)},
\id:v\in V\rightarrow v\in V
)
\]
}

\AddEquation{da in DA->da in D1A 1, module}
{
(d+0)v=dv+0v=dv+0=dv
}

\AddEquation{da in DA->da in D1A 1, left module}
{
(d+0)v=dv+0v=dv+0=dv
}

\AddEquation{da in DA->da in D1A 1, right module}
{
v(d+0)=vd+v0=vd+0=vd
}

\AddEq [1]{A module diagram for linear}
{
\[
\xymatrix
{
A_{#1}&&V_{#1}\\
&D_{#1}\ar[lu]|{*}\ar[ru]|{*}
}
\]
}

\DefEquation
{
f^k=f^{k\cdot\gi{ij}}e_{\gii}\otimes e_{\gij}
}
{standard representation of map A1 A2, 3, associative algebra}

\AddEquation{A=re+im}
{
A=\re A\oplus\im A
}

\AddEquation{standard representation of map A->A, associative algebra}
{
f=
f^{k\cdot\gi{ij}}(\aD ei\otimes \aD ej)\circ F_k
}

\AddEq{standard representation of map A->A, o, associative algebra}
{
\[
f\circ x=
f^{k\cdot\gi{ij}}\aU ei(F_k\circ x)\aU ej
\]
}

\AddEq{product of map over scalar,,D module}
{
\symb{d\,f}{product of map over scalar}{D module}
}

\AddEq{product of map over scalar,,polylinear}
{
\symb{d\,f}{product of map over scalar}{polylinear}
}

\AddEquation{product of map over scalar, 1, polylinear}
{
\begin{matrix}
\ShowSymbol{product of map over scalar}{polylinear}{}:
A_1\times...\times A_n\rightarrow S
&d\in D&f\in\mathcal L(D;A_1\times...\times A_n\rightarrow S)
\end{matrix}
}

\AddEquation{product of map over scalar, 31, polylinear}
{
\begin{split}
&\,(pf)\circ(x_1,...,x_i+y_i,...,x_n)
\\
=&\,p\ f\circ(x_1,...,x_i+y_i,...,x_n)
\\
=&\,p\ (f\circ (x_1,...,x_i,...,x_n)+f\circ (x_1,...,y_i,...,x_n))
\\
=&\,p(f\circ (x_1,...,x_i,...,x_n))+p(f\circ (x_1,...,y_i,...,x_n))
\\
=&\,(pf)\circ (x_1,...,x_i,...,x_n)+(pf)\circ (x_1,...,y_i,...,x_n)
\end{split}
}

\AddEquation{product of map over scalar, 32, polylinear}
{
\begin{split}
& \,(pf)\circ(x_1,...,qx_i,...,x_n)
\\=& \,p(f\circ(x_1,...,qx_i,...,x_n))
=pq(f\circ (x_1,...,x_i,...,x_n))
\\=& \,qp(f\circ (x_1,...,x_n))
=q(pf)\circ (x_1,...,x_n)
\end{split}
}

\AddEquation{product of map over scalar, polylinear}
{
(\ShowSymbol{product of map over scalar}{polylinear}{})\circ (a_1,...,a_n)
=d(f\circ (a_1,...,a_n))
}

\DefCorollary{Free Algebra over Ring}
{
\ShowText{Free Algebra over Ring}
}

\AddEquation{a:LA1n->LA1n}
{
a:f\in\mathcal L(D;A_1\times...\times A_n\rightarrow S)\rightarrow
af\in\mathcal L(D;A_1\times...\times A_n\rightarrow S)
}

\DefTheorem{Free Algebra over Ring}
{
\ShowText{Free Algebra over Ring}
}

\AddEq{D*V->V}
{
(a,v)\in D\times V\rightarrow av\in V
}

\AddEq{left A*V->V}
{
(a,v)\in A\times V\rightarrow av\in V
}

\AddEq{right A*V->V}
{
(v,a)\in V\times A\rightarrow va\in V
}

\AddEquation{l(v1+v2)w}
{
(l\circ (v_1+v_2))\circ w=(v_1+v_2)w=v_1w+v_2w
=(l\circ v_1)\circ w+(l\circ v_2)\circ w
}

\AddEquation{l(v1+v2)}
{
l\circ (v_1+v_2)=l\circ v_1+l\circ v_2
}

\AddEquation{l(dv)w}
{
(l\circ (dv))\circ w=(dv)w=d(vw)
=d((l\circ v)\circ w)
}

\AddEquation{l(dv)}
{
l\circ (dv)=d(l\circ v)
}

\AddEq{g23:A->L}
{
\[g_{23}:A\rightarrow\mathcal L(D;A\rightarrow A)\]
}

\AddEquation{coordinates of map A->A, 3, associative algebra}
{
\begin{split}
\aUD fkl\aU xl\aD ek
&=
f^{k\cdot\gi{ij}} \aD ei
\aUD {F_{k\cdot}^{}{}}ml\aU xl\aD em
\aD ej
\\
&=
f^{k\cdot\gi{ij}}
\aUD {F_{k\cdot}^{}{}}ml\aU xl
\aUD Cp{im}\aUD Ck{pj}
\aD ek
\end{split}
}

\DefEq
{
f=f^k\circ F_k
}
{map f generated by basis F}

\AddEquation{fk= in A2xA2}
{
f^k=f^k_{s_k\cdot 0}\otimes f^k_{s_k\cdot 1}\ \ \ \ f^k\in A_2\otimes A_2
}

\AddEq [3]{n=dim A}
{
$\gi #1=\dim #2$#3
}

\AddEq{gi n<m}
{
$\gi n\le\gi m$.
}

\AddEq{gi n>m}
{
$\gi n>\gi m$.
}

\AddEquation{set ker G in ker g}
{
\{g\in\mathcal L(D;A\rightarrow B):\ker G\subseteq\ker g\}
}

\AddEquation{fk= in AxA}
{
f^k=f^k_{s_k\cdot 0}\otimes f^k_{s_k\cdot 1}\ \ \ \ f^k\in A\otimes A
}

\AddEquation{fk= in (Ax)A}
{
f^k=(f^k_{s_k\cdot 0}\otimes) f^k_{s_k\cdot 1}\ \ \ \ f^k\in A\otimes A
}

\DefEquation
{
f=f_{s\cdot 0}\otimes f_{s\cdot 1}
}
{expansion of f A->A}

\DefEquation
{
f=f^k\circ F_k
}
{expansion of f with respect to basis I}

\DefEquation
{
g=g_{t\cdot 0}\otimes g_{t\cdot 1}
}
{expansion of g A->A}

\DefEquation
{
g=g^l\circ G_l
}
{expansion of g with respect to basis J}

\DefEquation
{
h=h_{ts\cdot 0}\otimes h_{ts\cdot 1}
}
{expansion of h A->A}

\DefEquation
{
h=h^{lk}\circ K_{lk}
}
{expansion of h with respect to basis K}

\DefEquation
{
h\circ a=g\circ f\circ a
=g^l\circ J_l\circ f^k\circ I_k\circ a 
}
{h(a)1}

\DefEquation
{
\begin{split}
h\circ a=g\circ f\circ a
&=g^l\circ(J^m_l\circ f^k)\circ
J_m\circ I_k\circ a
\\&=g^l\circ(J^m_l\circ f^k)\circ K_{mk}\circ a
\end{split}
}
{h(a)2}

\DefEquation
{
\begin{split}
h_{ts\cdot 0}&=g_{t\cdot 0}f_{s\cdot 0}
\\
h_{ts\cdot 1}&=f_{s\cdot 1}g_{t\cdot 1}
\end{split}
}
{hlk=glfk 01}

\DefEq
{
\[a^{lk}K_{lk}=(a^{lk}\circ J_l)\circ I_k=0\]
}
{aK=aJI}

\DefEquation
{
\begin{split}
h\circ a&=g\circ f\circ a
\\&=(g_{t\cdot 0}\otimes g_{t\cdot 1})\circ(f_{s\cdot 0}\otimes f_{s\cdot 1})\circ a
\\&=(g_{t\cdot 0}\otimes g_{t\cdot 1})\circ(f_{s\cdot 0}a f_{s\cdot 1})
\\&=g_{t\cdot 0}f_{s\cdot 0}a f_{s\cdot 1} g_{t\cdot 1}
\end{split}
}
{h(a)}

\DefEq
{
\[a^{lk}\circ J_l=0\]
}
{aJ=0}

\DefEquation
{
h^{lk}=g^l\circ (G^k_m\circ f^m)
}
{hlk=glfk}

\DefEq
{
\Basis H=\{H_{lk}:H_{lk}=G_l\circ F_k, G_l\in\Basis G, F_k\in\Basis F\}
}
{JlIk}

\DefEq
{
h=g\circ f
}
{h=g o f}

\AddEq[2]{h:AoxA->L(A)}
{
\xymatrix
{
h:#2\otimes #2\ar[r]|{*}&\mathcal L(#1;#2\rightarrow #2)
}
\ \ \ h(p):g\rightarrow p\circ g
}

\AddEq[2]{representation AA in LA}
{
\begin{matrix}
(a\otimes b)\circ g=agb
&a,b\in #2&g\in\mathcal L(#1;#2\rightarrow #2)
\end{matrix}
}

\ePrints{5114-6019}
\ifx\Semafor\ValueOff
\AddEq{component of linear map}
{
\symb{f^k_{s_k\cdot p}}{component of linear map, division ring}1,
$p=0$, $1$,
}

\AddEq{standard component of linear map}
{
\symb{f^{k\cdot\gi{ij}}}{standard component of linear map}1
}
\fi

\AddEq[2]{product in algebra AA}
{
(#1_0\otimes #1_1)\circ(#2_0\otimes #2_1)=(#1_0 #2_0)\otimes(#2_1 #1_1)
}

\AddEquation{representation A2 in LA}
{
\xymatrix
{
h:\ATwo\ar[r]|(.4){*}&\mathcal L(D;A_1\rightarrow A_2)
}
}

\AddEquation{representation A2 in LA, 1}
{
\begin{matrix}
(a\otimes b)\circ f=afb
&a,b\in A_2&f\in\mathcal L(D;A_1\rightarrow A_2)
\end{matrix}
}

\AddEq{xA1n*xA1n->oxA1n=}
{
\[
(a_1,...,a_n)*(b_1,...,b_n)=(a_1b_1)\otimes...\otimes(a_nb_n)
\]
}

\DefEquation
{
(a\otimes b)\circ c=acb
}
{a ox b c=}

\AddEq[1]{a ox b}
{
$(a\otimes b)\circ #1$
}

\AddEq[1]{d in AxoA}
{
$d\in\AxA{#1}$
}

\AddEq[4]{product in algebra AA 2}
{
$d\circ #3\in\mathcal L(#1;#2\rightarrow #2)$#4
}

\DefEq
{
$A_1$, ..., $A_n$
}
{A1...n}

\AddEq{diagram of representations, module}
{
\xymatrix
{
D\ar[r]|{*}^{g_2}&V\\
&Z\ar[u]|{*}_{g_1}
}
}

\AddEq[8]{diagram of representations, left right module}
{
\begin{matrix}
\vcenter
{
\xymatrix
{
A_{#6}\ar[r]|{*}^{g_{#8 23}}&
A_{#6}\ar[r]|{*}^{g_{#8 34}}&V_{#7}
\\
&D_{#5}\ar[u]|{*}_{g_{#8 12}}\ar@/_1pc/[ur]|{*}_{g_{#8 14}}\ar[ul]|(.4){*}^{g_{#8 12}}
}
}
&
\begin{array}{r@{\,}l}
g_{12}(d):a&\rightarrow d\,a
\\
g_{23}(v):w&\rightarrow
C(w, v)
\\
C&\in\mathcal L(A^2\rightarrow A)
\\
g_{3,4}(a):v&\rightarrow #3\,#4
\\
g_{1,4}(d):v&\rightarrow #1\,#2
\end{array}
\end{matrix}
}

\AddEq{diagram of representations, left module nonassociative}
{
\[
\begin{matrix}
\vcenter
{
\xymatrix
{
A\ar[rd]|{*}^{g_{23}}\ar[rr]|{*}^{g_{34}}&&V
\\
&A
\\
&D\ar[u]|{*}_{g_{12}}\ar@/_1pc/[uur]|{*}_{g_{14}}\ar[uul]|(.4){*}^{g_{12}}
}
}
&
\begin{array}{r@{\,}l}
g_{12}(d):a&\rightarrow d\,a
\\
g_{23}(v):w&\rightarrow
C(w, v)
\\
C&\in\mathcal L(A^2\rightarrow A)
\\
g_{34}(a):v&\rightarrow v\,a
\\
g_{14}(d):v&\rightarrow d\,v
\end{array}
\end{matrix}
\]
}

\AddEq[4]{diagram of representations, left module}
{
\ShowEq{diagram of representations, left right module}dvav{#1}{#2}{#3}{#4}
}

\AddEq[4]{diagram of representations, right module}
{
\ShowEq{diagram of representations, left right module}vdva{#1}{#2}{#3}{#4}
}

\AddEq{A1=A unital extension}
{
%\labelItem{A1=A \SideWS unital extension}
&$\CBase\subseteq\Base$&$\Base_{(1)}=\Base$\\
\hline
}

\AddEq{A1=D unital extension}
{
%\labelItem{A1=D \SideWS unital extension}
&$\Base\subseteq\CBase$&$\Base_{(1)}=\CBase$\\
\hline
}

\AddEq{A1=A+D unital extension}
{
&\multicolumn{2}{c|}{$\Base_{(1)}=\Base\oplus\CBase$}\\
%&&$\Base_{(1)}=\Base\oplus\CBase$\\
\hline
}

\AddEq{set of vectors generated by vector A}
{
\symb[A-0]{A_{(1)}v}{set of vectors generated by vector}1
}

\AddEq{set of vectors generated by vector D}
{
\symb[D-0]{D_{(1)}v}{set of vectors generated by vector}1
}

\AddEq{D->*V}
{
\begin{matrix}
\xymatrix
{
f:D\ar[r]|{*}&V
}
&
f(d):v\rightarrow d\,v
\end{matrix}
}

\AddEq{right A->*V}
{
\begin{matrix}
\xymatrix
{
f:A\ar[r]|{*}&V
}
&
f(a):v\in V\rightarrow va\in V
&a\in A
\end{matrix}
}

\AddEq{left A->*V}
{
\begin{matrix}
\xymatrix
{
f:A\ar[r]|{*}&V
}
&
f(a):v\in V\rightarrow av\in V
&a\in A
\end{matrix}
}

\AddEq{module, associative law}
{
(ab)v=a(bv)
}

\AddEquation{module, (a+n)(b+m)=}
{
\begin{split}
((a+n)(b+m))v&=(a+n)((b+m)v)=(a+n)(bv+mv)\\
&=a(bv+mv)+n(bv+mv)\\
&=a(bv)+a(mv)+n(bv)+n(mv)\\
&=(ab)v+m(av)++n(bv)+(nm)v\\
&=(ab)v+(ma)v++(nb)v+(nm)v\\
&=((ab+ma+nb)+nm)v
\end{split}
}

\AddEq{fab=ab}
{
f(a,b)=ab\ \ \ a,b\in\Base
}

\AddEq{f1p=p}
{
f(1,p)=f(p,1)=p\ \ \ p\in\Base_{(1)}\ \ \ 1\in\CBase_{(1)}
}

\AddEq{pq=fpq}
{
\begin{split}
(a+n)(b+m)&=f(a+n,b+m)\\
&=f(a,b)+f(a,m)+f(n,b)+f(n,m)\\
&=f(a,b)+mf(a,1)+nf(1,b)+nf(1,m)\\
&=ab+ma+nb+nm
\end{split}
}

\AddEq{f:D1xD1->D1}
{
\[
f:\Base_{(1)}\times\Base_{(1)}\rightarrow\Base_{(1)}
\]
}

\AddEq{distributive law, module, 1}
{
p(v+w)=pv+pw
}

\AddEq{distributive law, module, 2}
{
(p+q)v=pv+qv
}

\AddEq{p,q in D1}
{
$p=a+n\in\Base_{(1)}$, $q=b+m\in\Base_{(1)}$.
}

\AddEq [4]{h:D1->D2 f:A1->A2}
{
\[
\begin{pmatrix}
#1:#2_1\rightarrow #2_2&
#3:#4_1\rightarrow #4_2
\end{pmatrix}
\]
}

\AddEq{set linear maps, D12 module}
{
\symb{\mathcal L(\Base_1\rightarrow \Base_2;\Module_1\rightarrow \Module_2)}{set linear maps}1
}

\AddEq{set linear maps, VW module}
{
\symb{\mathcal L(A;V\rightarrow W)}{set linear maps}1
}

\AddEq{set linear maps, left A12 module}
{
\symb{\mathcal L(D_1\rightarrow D_2;A_1\CRstar\rightarrow A_2\CRstar;V_1\rightarrow V_2)}{set linear maps}1
}

\AddEq{set homomorphisms, D algebra 11}
{
\symb{\Hom(D_1\rightarrow D_2;A_1\rightarrow A_2)}{set homomorphisms}1
}

\AddEq{set homomorphisms, D algebra 1}
{
\symb{\Hom(D;A_1\rightarrow A_2)}{set homomorphisms}1
}

\AddEq{set homomorphisms, A module 111 left}
{
\symb{\Hom(D_1\rightarrow D_2;A_1\rightarrow A_2;*V_1\rightarrow *V_2)}{set homomorphisms}1
}

\AddEq{set homomorphisms, A module 11 left}
{
\symb{\Hom(D;A_1\rightarrow A_2;*V_1\rightarrow *V_2)}{set homomorphisms}1
}

\AddEq{set homomorphisms, A module 1 left}
{
\symb{\Hom(D;A;*V_1\rightarrow *V_2)}{set homomorphisms}1
}

\AddEq{set homomorphisms, A module 111 right}
{
\symb{\Hom(D_1\rightarrow D_2;A_1\rightarrow A_2;V_1*\rightarrow V_2*)}{set homomorphisms}1
}

\AddEq{set homomorphisms, A module 11 right}
{
\symb{\Hom(D;A_1\rightarrow A_2;V_1*\rightarrow V_2*)}{set homomorphisms}1
}

\AddEq{set homomorphisms, A module 1 right}
{
\symb{\Hom(D;A;V_1*\rightarrow V_2*)}{set homomorphisms}1
}

\AddEq{set homomorphisms, left A12 module}
{
\symb{\Hom(D_1\rightarrow D_2;A_1\CRstar\rightarrow A_2\CRstar;V_1\rightarrow V_2)}{set homomorphisms}1
}

\AddEq{set linear maps, right A12 module}
{
\symb{\mathcal L(D_1\rightarrow D_2;\RCstar A_1\rightarrow\RCstar A_2;V_1\rightarrow V_2)}{set linear maps}1
}

\AddEq{set homomorphisms, right A12 module}
{
\symb{\Hom(D_1\rightarrow D_2;\RCstar A_1\rightarrow\RCstar A_2;V_1\rightarrow V_2)}{set homomorphisms}1
}

\AddEq [1]{left column module}
{
$#1\CRstar$\Hyph
}

\AddEq [1]{right column module}
{
$\RCstar #1$\Hyph
}

\AddEquation{unitarity law, D-module}
{
1v=v
}

\AddEq{associative law, module}
{
(pq)v=p(qv)
}

\AddEq{associative law, left module}
{
(pq)v=p(qv)
}

\AddEq{associative law, right module}
{
v(pq)=(vp)q
}

\AddEq{left module, associative law}
{
(ab)v=a(bv)
}

\AddEq{associative law, Z, module}
{
(mn)v=m(nv)
}

\AddEq{associative law, ZD, module}
{
(md)v=m(dv)
}

\AddEq{associative law, D, left module}
{
(cd)v=c(dv)
}

\AddEq{associative law, DA, left module}
{
(da)v=d(av)
}

\AddEq{distributive law, left module, 1}
{
p(v+w)=pv+pw
}

\AddEq{distributive law, left module, 2}
{
(p+q)v=pv+qv
}

\AddEquation{distributive law, Z, module, 2}
{
(n+m)v=nv+mv
}

\AddEquation{distributive law, D, module, 2}
{
(a+b)v=av+bv
}

\AddEquation{distributive law, D, left module, 2}
{
(n+m)v=cn+dm
}

\AddEquation{distributive law, A, left module, 2}
{
(a+b)v=av+bv
}

\AddEquation{distributive law, D, right module, 2}
{
v(n+m)=vn+vm
}

\AddEquation{distributive law, A, right module, 2}
{
v(a+b)=va+vb
}

\AddEq{distributive law, right module, 1}
{
(v+w)p=vp+wp
}

\AddEq{distributive law, right module, 2}
{
v(p+q)=vp+vq
}

\AddEquation{aw in Xk module}
{
aw\in X_{k+1}
}

\AddEquation{aw in Xk left module}
{
aw\in X_{k+1}
}

\AddEquation{aw in Xk right module}
{
wa\in X_{k+1}
}

\AddEq[2]{w1+w2 in Jv}
{
$#1_1+#1_2\in J(#2)$.
}

\AddEquation{v=v+0, module}
{
\Vector v=\Vector v+0=
\ACol vi
\ARow ei+
\ACol ci
\ARow ei=
(\ACol vi+
\ACol ci)
\ARow ei
}

\AddEquation{v=v+0, left module}
{
\Vector v=\Vector v+0=
\ACol vi
\ARow ei+
\ACol ci
\ARow ei=
(\ACol vi+
\ACol ci)
\ARow ei
}

\AddEquation{v=v+0, right module}
{
\Vector v=\Vector v+0=
\ARow ei
\ACol vi+
\ARow ei
\ACol ci=
\ARow ei
(\ACol vi+
\ACol ci)
}

\AddEq{px x-i x-j}
{
\[
p(x)=2(x-i)(x-j)+(x-j)(x-i)
%=2x^2-2ix-2xj+2ij+x^2-jx-xi+ji
=3x^2-2ix-2xj-jx-xi+k
\]
}

\AddEq{px x-i x-j 1}
{
\[
p(x)=((3-a)(x\otimes 1)+a\otimes x)\circ x-2ix-2xj
-jx-xi+k
\]
}

\AddEq{rx x-i}
{
r(x)=x-i
}

\AddEq{p(x)=sr 2}
{
\begin{align*}
p(x)&=(3-a)(r(x)+i)x+ax(r(x)+i)-2ix-2xj-jx-xi+k
\\
&=(3-a)r(x)x+(3-a)ix+axr(x)+axi-2ix-2xj-jx-xi+k
\\
&=(3-a)r(x)x+axr(x)+(3-a)i(r(x)+i)
\\
&+a(r(x)+i)i-2i(r(x)+i)-2(r(x)+i)j-j(r(x)+i)-(r(x)+i)i+k\\
&=(3-a)r(x)x+axr(x)+3ir(x)-3-air(x)+a
\\
&+ar(x)i-a-2ir(x)+2-2r(x)j-2k-jr(x)+k-r(x)i+1+k
\\
&=(3-a)r(x)x+axr(x)+3ir(x)-air(x)
\\
&+ar(x)i-2ir(x)-2r(x)j-jr(x)-r(x)i
\end{align*}
}

\AddEq{p=s2r}
{
\[p(x)=s_2(a,x)\circ r(x)\]
}

\AddEq{s2(x)=}
{
\begin{align*}
s_2(a,x)&=(3-a)\otimes x+ax\otimes 1+(3-a)i\otimes 1
\\
&+a\otimes i-2i\otimes 1-2\otimes j-j\otimes 1-1\otimes i
\\
&=(3-a)\otimes x+(ax-j-2i+(3-a)i)\otimes 1
+(a-1)\otimes i-2\otimes j
\\
&=(3-a)\otimes x+(ax-j+i-ai)\otimes 1
+(a-1)\otimes i-2\otimes j
\end{align*}
}

\AddEq{s2(1,x)=}
{
\begin{align*}
s_2(1,x)&=2\otimes x+(x-j-2i+2i)\otimes 1
+(1-1)\otimes i-2\otimes j
\\
&=2\otimes (x-j)+(x-j)\otimes 1
\end{align*}
}

\AddEq{s12 in AA}
{
$s_1(x)$, $s_2(x)\in A\otimes A$
}

\AddEq[1]{px=sx o rx}
{
\[
p(x)=s_{#1}(x)\circ r(x)
\]
}

\AddEq{(sx-sx)rx=0}
{
\[
(s_1(x)-s_2(x))\circ r(x)=0
\]
}

\AddEquation{x p0 x*+xQ+Rx*-S=0 3}
{
\begin{split}
p(x)&=(-4\otimes 1\otimes 1-4\otimes i\otimes i-4\otimes j\otimes j
-4\otimes k\otimes k)\circ x^2
\\&+(4\otimes i+2j\otimes 1-2k\otimes i-2\otimes j+2i\otimes k)\circ x+1+2k
\\&=-4x^2-4xixi-4xjxj
-4xkxk 
\\&+4xi+2jx-2kxi-2xj+2ixk+1+2k
\end{split}
}

\AddEquation{q(x)=}
{
q(x)=x-\frac{1}{4}(i+j)
}

\AddEquation{4x=4q+}
{
4x=4q(x)+i+j
}

\AddEquation{rj j-i}
{
r(j)=j-i
}

\AddEq{p(x)=sr}
{
\begin{align*}
p(x)&=3(r(x)+i)x-2ix-2xj-jx-xi+k
\\
%&=3r(x)x+3ix-2ix-2xj-jx-xi+k
&=3r(x)x+ix-2xj-jx-xi+k
\\
&=3r(x)x+i(r(x)+i)-2(r(x)+i)j-j(r(x)+i)-(r(x)+i)i+k
%&=3r(x)x+ir(x)-1-2r(x)j-2ij-jr(x)-ji-r(x)i-ii+k
%&=3r(x)x+ir(x)-1-2r(x)j-2k-jr(x)+k-r(x)i+1+k
\\
&=3r(x)x+ir(x)-2r(x)j-jr(x)-r(x)i
\\
&=(3\otimes x+i\otimes 1-2\otimes j-j\otimes 1-1\otimes i)\circ r(x)
%3\otimes j+i\otimes 1-2\otimes j-j\otimes 1-1\otimes i
%1\otimes (j-i)-(j-i)\otimes 1
\end{align*}
}

\AddEq{s(x)=}
{
\[
s(x)=3\otimes x+i\otimes 1-2\otimes j-j\otimes 1-1\otimes i
\]
}

\AddEq{s(j)=}
{
\[
s(j)=1\otimes (j-i)-(j-i)\otimes 1\ne 0\otimes 0
\]
}

\AddEq[1]{Xk in Jv}
{
$X_{#1}\subseteq J(v)$.
}

\AddEq{w1+w2 in V}
{
w_1+w_2\in X_{k+1}
}

\AddEquation{unitarity law, left A-module}
{
1v=v
}

\AddEquation{left module, a d v}
{
a(dv)=d(av)
}

\AddEquation{module, a d v}
{
a(nv)=n(av)
}

\AddEq{abc in A, v in v}
{
$a$, $b$, $c\in A$, $v\in V$.
}

\AddEquation{a(b(cv))=(a(bc))v left}
{
a(b(cv))=a((bc)v)=(a(bc))v
}

\AddEquation{a(b(cv))=(a(bc))v right}
{
((vc)b)a=(v(cb))a=v((cb)a)
}

\AddEquation{a(b(cv))=((ab)c)v left}
{
a(b(cv))=(ab)(cv)=((ab)c)v
}

\AddEquation{a(b(cv))=((ab)c)v right}
{
((vc)b)a=(vc)(ba)=v(c(ba))
}

\AddEquation{(a(bc))v=((ab)c)v left}
{
(a(bc))v=((ab)c)v
}

\AddEquation{(a(bc))v=((ab)c)v right}
{
v((cb)a)=v(c(ba))
}

\AddEquation{a(bc)=(ab)c left}
{
a(bc)=(ab)c
}

\AddEquation{a(bc)=(ab)c right}
{
(cb)a=c(ba)
}

\AddEq{cv left}
{
$cv\in A$,
}

\AddEq{cv right}
{
$vc\in A$,
}

\AddEq{right module, associative law}
{
v(ab)=(va)b
}

\AddEq{associative law, D, right module}
{
v(dc)=(vd)c
}

\AddEq{associative law, DA, right module}
{
v(ad)=(va)d
}

\AddEquation{unitarity law, right A-module}
{
v1=v
}

\AddEquation{right module, a d v}
{
(vd)a=(va)d
}

\AddEq{c,d in Z, a,b in D, v,w in V}
{
$m$, $n\in Z$, $a$, $b \in D$, $v$, $w \in V$.
}

\AddEq [1]{vi V}
{
$v=(\aD vi\in V,\iIg)$#1
}

\AddEq [1]{v(i) V}
{
$v=(v(\gii)\in V,\iIg)$#1
}

\AddEq[2]{vv in V}
{
$\Vector{#1}\in #2$
}

\AddEq[3]{polynomial p(x)}
{
\[
#1(x)=\sum_{#2=0}^{#3}#1_{#2}x^{#2}
\]
}

\AddEquation{polynomial p*r(x)}
{
p(x)*r(x)=
(p*r)(x)=\sum_{j=0}^{m+n}(\sum_{i=0}^jp_ir_{j-i})x^j
}

\AddEq{x-=}
{
\[
\tilde{x}=hxh^{-1}=
(i-j)x(i-j)^{-1}=\frac 12(i-j)x(j-i)
\]
}

\AddEquation{L(x-)=}
{
L(\tilde{x})=\frac 12(i-j)x(j-i)-i
}

\AddEquation{p(x)=L(x-)R(x)}
{
x^2-(i+j)x+k=(\frac 12(i-j)x(j-i)-i)(x-j)
}

\AddEquation{p(i+j)=L(i+j-)R(i+j)}
{
(i+j)^2-(i+j)(i+j)+k=(\frac 12(i-j)(i+j)(j-i)-i)(i+j-j)
}

\AddEquation{p(i+j)=L(i+j-)R(i+j) 1}
{
\begin{split}
k&=(\frac 12(i^2+ij-ji-j^2)(j-i)-i)i\\
&=(k(j-i)-i)i=(-i-j-i)i
\end{split}
}

\AddEq{linear map f, basis E}
{
f=f\pC s0\otimes f\pC s1\in\AoxA H
}

\AddEquation{value of linear map f, basis E}
{
f\circ a=(f\pC s0\otimes f\pC s1)\circ a=f\pC s0\,a\,f\pC s1
}

\AddEq{Eox=x}
{
\[E\circ x=x\]
}

\AddEq{component of linear map, basis E}
{
\symb{f\pC sp}{component of linear map, division ring}1,
$p=0$, $1$,
}

\AddEq{vv=ve left module}
{
\Vector v=\ACol vi\ARow ei
}

\AddEq{vv=ve right module}
{
\Vector v=\ARow ei\ACol vi
}

\AddEq{vv=ve module}
{
\Vector v=
\ACol vi
\ARow ei
}

\AddEq{coordinate matrix of vector}
{
$v=(\ACol vi,\iIg)$
}

\AddEquation{w= module}
{
w=\sum_{\iIg}\aU wi\aD vi
}

\AddEquation{w= left module}
{
w=\sum_{\iIg}\aU wi\aD vi
}

\AddEquation{w= right module}
{
w=\sum_{\iIg}\aD vi\aU wi
}

\AddEquation{w()= module}
{
w=\sum_{\iIg}w(\gii)v(\gii)
}

\AddEquation{w()= left module}
{
w=\sum_{\iIg}w(\gii)v(\gii)
}

\AddEquation{w()= right module}
{
w=\sum_{\iIg}v(\gii)w(\gii)
}

\AddEquation{aw= module}
{
aw=a\sum_{\iIg}\aU wi\aD vi
=\sum_{\iIg}a(\aU wi\aD vi)
=\sum_{\iIg}(a\aU wi)\aD vi
}

\AddEquation{aw= left module}
{
aw=a\sum_{\iIg}\aU wi\aD vi
=\sum_{\iIg}a(\aU wi\aD vi)
=\sum_{\iIg}(a\aU wi)\aD vi
}

\AddEquation{aw= right module}
{
wa=\left(\sum_{\iIg}\aD vi\aU wi\right)a
=\sum_{\iIg}(\aD vi\aU wi)a
=\sum_{\iIg}(\aD vi\aU wia)
}

\AddEquation{aw()= module}
{
aw=a\sum_{\iIg}w(\gii)v(\gii)
=\sum_{\iIg}a(w(\gii)v(\gii))
=\sum_{\iIg}(aw(\gii))v(\gii)
}

\AddEquation{aw()= left module}
{
aw=a\sum_{\iIg}w(\gii)v(\gii)
=\sum_{\iIg}a(w(\gii)v(\gii))
=\sum_{\iIg}(aw(\gii))v(\gii)
}

\AddEquation{aw()= right module}
{
wa=\left(\sum_{\iIg}v(\gii)w(\gii)\right)a
=\sum_{\iIg}(v(\gii)w(\gii))a
=\sum_{\iIg}(\aD viw(\gii)a)
}

\AddEq[1]{set au vi}
{
$\aU {#1}i$, \iIg,
}

\AddEq[1]{set au v(i)}
{
$#1(\gii)$, \iIg,
}

\AddEq[1]{set au v1n}
{
$\aU {#1}1$, ..., $\aU {#1}n$
}

\AddEq{basis, module}
{
\symb{\Basis{e}=(
\ARow ei,
\iIg)}{basis for module}1
}

\AddEq[3]{set vi Acols}
{%
$\ACol {#1}{#2}$, \jJg{#2}{#3},
}

\AddEq[1]{set vi cols}
{%
$\aD {#1}i$, \iIg,
}

\AddEq[1]{set vi *}
{%
$#1(\gii)$, \iIg,
}

\AddEquation{coordinate transformation, ba}
{
v''^k=b^{-1}{}^k_ia^{-1}{}^i_jv^j=(ab)^{-1}{}^k_jv^j
}

\AddEq[3]{passive coordinate transformation}
{
v#1^i=#3^{-1}{}^i_jv#2^j
}

\AddEq[3]{w.e, left-cols}
{
#1\CRstar #2=
\ColMatrix{#1}{#3}
\CRstar
\RowMatrix{#2}{#3}
=\ShowEq{w.e 1, cr}{#1}{#2}
}

\AddEq[3]{w.e, right-rows}
{
#2\CRstar #1=
\ColMatrix{#2}{#3}
\CRstar
\RowMatrix{#1}{#3}
=\ShowEq{w.e 1, cr}{#2}{#1}
}

\AddEq[3]{w.e, left-rows}
{
#1\RCstar #2=
\RowMatrix{#1}{#3}
\RCstar
\ColMatrix{#2}{#3}
=\ShowEq{w.e 1, rc}{#1}{#2}
}

\AddEq[3]{w.e, right-cols}
{
#2\RCstar #1=
\RowMatrix{#2}{#3}
\RCstar
\ColMatrix{#1}{#3}
=\ShowEq{w.e 1, rc}{#2}{#1}
}

\AddEq[3]{w.e, -cols}
{
#1 #2=
\ColMatrix{#1}{#3}
\RowMatrix{#2}{#3}
=\ShowEq{w.e 1, -cols}{#1}{#2}
}

\AddEq[3]{w.e, -rows}
{
#2 #1=
\ColMatrix{#2}{#3}
\RowMatrix{#1}{#3}
=\ShowEq{w.e 1, -rows}{#1}{#2}
}

\AddEq[2]{w.e 1, cr}
{
\aU {#1}i\aD {#2}i
}

\AddEq[2]{w.e 1, rc}
{
\aD {#1}i\aU {#2}i
}

\AddEq[2]{w.e 1, -cols}
{
\aU {#1}i\aD {#2}i
}

\AddEq[2]{w.e 1, -rows}
{
\aD {#1}i\aU {#2}i
}

\AddEq[1]{vector w=w*e left-cols}
{
\Vector {#1}=
\ShowEq{w.e, left-cols}{#1}en
}

\AddEq[1]{vector w=w*e left-rows}
{
\Vector {#1}=
\ShowEq{w.e, left-rows}{#1}en
}

\AddEq[1]{vector w=w*e right-cols}
{
\Vector {#1}=
\ShowEq{w.e, right-cols}{#1}en
}

\AddEq[1]{vector w=w*e right-rows}
{
\Vector {#1}=
\ShowEq{w.e, right-rows}{#1}en
}

\AddEq[1]{vector w=w*e -cols}
{
\Vector {#1}=
\ShowEq{w.e, -cols}{#1}en
}

\AddEq[1]{vector w=w*e -rows}
{
\Vector {#1}=
\ShowEq{w.e, -rows}{#1}en
}

\AddEq[3]{w=w*eC left-cols}
{
\ensuremath{\Vector {#1}=
\aU {#1}i\aD [#2]ei}#3
}

\AddEq[2]{w=w*e left-cols}
{
\ensuremath{\Vector {#1}=
\ShowEq{w.e 1, cr}{#1}e}#2
}

\AddEq[2]{w=w*e left-rows}
{
\ensuremath{\Vector {#1}=
\ShowEq{w.e 1, rc}{#1}e}#2
}

\AddEq[2]{w=w*e right-cols}
{
\ensuremath{\Vector {#1}=
\ShowEq{w.e 1, rc}e{#1}}#2
}

\AddEq[2]{w=w*e right-rows}
{
\ensuremath{\Vector {#1}=
\ShowEq{w.e 1, cr}e{#1}}#2
}

\AddEq[2]{w=w*e -cols}
{
\ensuremath{\Vector {#1}=
\ShowEq{w.e 1, cr}{#1}e}#2
}

\AddEq[2]{w=w*e -rows}
{
\ensuremath{\Vector {#1}=
\ShowEq{w.e 1, rc}{#1}e}#2
}

\AddEquation{similar A numbers}
{
a=c^{-1}bc
}

\AddEquation{endomorphism of module from product}
{
\xymatrix
{
g_{23}:A\ar[r]|{*}&A
}
}

\DefEquation
{
l\circ v:w\in A\rightarrow v\,w\in A
}
{l(v):w->vw}

\AddEq[2]{representation An in LAnA}
{
\[
\xymatrix
{
h:\AOn[#2]\times S_n\ar[r]|{*}&\LAnAB {#1}{#2}{#2}
}
\]
}

\AddEq[2]{representation An in LAnA, 1}
{
\begin{matrix}
(a_0\otimes...\otimes a_n,\sigma)\circ(f_1\otimes...\otimes f_n)
=a_0\sigma(f_1)a_1...a_{n-1}\sigma(f_n)a_n
\\
\begin{matrix}
a_0,...,a_n\in #2&\sigma\in S_n&f_1,...,f_n\in\mathcal L(#1;#2\rightarrow #2)
\end{matrix}
\end{matrix}
}

\DefEq
{
$d\in\AOn$
}
{product in algebra An 1}

\AddEq[2]{product in algebra An 2}
{
\begin{matrix}
(d,\sigma)\circ(f_1,...,f_n)&f_i=\delta\in\mathcal L(#1;#2\rightarrow #2)
\end{matrix}
}

\AddEq[3]{product in algebra AA 3}
{
$#3\in\mathcal L(#1;#2\rightarrow #2)$
}

\AddEq[2]{wi vi=0}
{
\ACol {#1}i\ARow {#2}i=0
}

\AddEq[2]{left wi vi=0}
{
\ACol {#1}i\ARow {#2}i=0
}

\AddEq[2]{right wi vi=0}
{
\ARow {#2}i\ACol {#1}i=0
}

\AddEq{w(i)=0}
{
$w(\gii)=0$, \iIg,
}

\AddEq{w(i) v(i)=0}
{
w(\gii)v(\gii)=0
}

\AddEq{left w(i) v(i)=0}
{
w(\gii)v(\gii)=0
}

\AddEq{right w(i) v(i)=0}
{
v(\gii)w(\gii)=0
}

\AddEq{0=0vi}
{
\[
\ACol wi=0
\Rightarrow
\ACol wi
\ARow vi
=0
\]
}

\AddEq{left 0=0vi}
{
\[
\ACol wi=0
\Rightarrow
\ACol wi
\ARow vi
=0
\]
}

\AddEq{right 0=0vi}
{
\[
\ACol wi=0
\Rightarrow
\ARow vi
\ACol wi
=0
\]
}

\AddEq[2]{vj=sum vi}
{
\[
\ARow {#1}j{}
=\sum_{\gii\in \giI\setminus\{\gij\}}
\frac
{\ACol {#2}i{}}
{\ACol {#2}j{}}
\ARow {#1}i{}
\]
}

\AddEq[2]{left vj=sum vi}
{
\[
\ARow {#1}j{}
=\sum_{\gii\in \giI\setminus\{\gij\}}
(\ACol {#2}j{})^{-1}
\ACol {#2}i{}
\ARow {#1}i{}
\]
}

\AddEq[2]{right vj=sum vi}
{
\[
\ARow {#1}j{}
=\sum_{\gii\in \giI\setminus\{\gij\}}
\ARow {#1}i{}
\ACol {#2}i{}
(\ACol {#2}j{})^{-1}
\]
}

\AddEq[2]{b in D'}
{
$#1=(
\ACol {#1}i,
\iIg)\in\Base'$#2
}

\AddEq[2]{wj ne 0}
{
$\ACol {#1}j{}\ne 0$#2
}

\AddEq[2]{w12 in Jv}
{
$#1_1$, $#1_2\in X_k\subseteq J(#2)$.
}

\AddEq[1]{w=w12 in Xk-1}
{
$w=w_1+w_2$, $w_1$, $w_2\in X_{k-1}$#1
}

\AddEq{w=aw in Xk-1,}
{
$w=aw_1$, $a\in\Base_{\BaseExt}$, $w_1\in X_{k-1}$.
}

\AddEq{w=aw in Xk-1,left}
{
$w=aw_1$, $a\in\Base_{\BaseExt}$, $w_1\in X_{k-1}$.
}

\AddEq{w=aw in Xk-1,right}
{
$w=w_1a$, $a\in\Base_{\BaseExt}$, $w_1\in X_{k-1}$.
}

\AddEq{generating set of module}
{
$J(X)=V$.
}

\AddEq[2]{w=sum vi, module}
{
J(v)=\left\{w:w=\sum_{\iIg}c(\gii)v(\gii),c(\gii)\in #1_{#2},
|\{\gii:c(\gii)\ne 0\}|<\infty\right\}
}

\AddEq[2]{w=sum vi, left module}
{
J(v)=\left\{w:w=\sum_{\iIg}c(\gii)v(\gii),c(\gii)\in #1_{#2},
|\{\gii:c(\gii)\ne 0\}|<\infty\right\}
}

\AddEq[2]{w=sum vi, right module}
{
J(v)=\left\{w:w=\sum_{\iIg}v(\gii)c(\gii),c(\gii)\in #1_{#2},
|\{\gii:c(\gii)\ne 0\}|<\infty\right\}
}

\AddEq{vectors generated by set of vectors}
{
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{\SideWS module, sum cvk in Jv}
\item
\ShowEq{v,w in Jv=>v+w in Jv}
\item
\ShowEq{vector space, v in Jv=>av in Jv}
\end{enumerate}
%\StopLabelItem
}

\AddEq{vectors generated by set of vectors 2018}
{
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{vk in v}
\labelItem{vector space, vk in Jv}
\item
\ShowEq{vector space, cvk in Jv}
\item
\ShowEq{vector space, sum cvk in Jv}
\item
\ShowEq{v,w in Jv=>v+w in Jv}
\item
\ShowEq{vector space, v in Jv=>av in Jv}
\end{enumerate}
%\StopLabelItem
}

\AddEq[1]{vk in Jv}
{%
$v(\gik)\in J(v)$#1
}

\AddEq{module, d in D}
{
$\DArg\in \CBase$,
}

\AddEq{module, dv in V}
{%
$\DArg v\in V$,
}

\AddEq{left module, dv in V}
{%
$\DArg v\in V$,
}

\AddEq{right module, dv in V}
{%
$v\DArg \in V$,
}

\AddEq{module, a in A}
{
$a\in \Base$.
}

\AddEq{module, av in V}
{%
$av\in V$
}

\AddEq{left module, av in V}
{%
$av\in V$
}

\AddEq{right module, av in V}
{%
$va\in V$
}

\AddEq{module, dv+av in V}
{%
\[\DArg v+av\in V\ \ \ \DArg\in \CBase\ \ \ a\in \Base\]
}

\AddEq{left module, dv+av in V}
{%
\[\DArg v+av\in V\ \ \ \DArg\in \CBase\ \ \ a\in \Base\]
}

\AddEq{right module, dv+av in V}
{%
\[v\DArg +va\in V\ \ \ \DArg\in \CBase\ \ \ a\in \Base\]
}

\AddEq{module, cvk in Jv}
{%
$c(\gik)v(\gik)\in J(v)$, $c(\gik)\in \Base_{\BaseExt}$,
\jJg kI
\labelItem{\VectorSetNS, cvk in Jv}
}

\AddEq{vector space, cvk in Jv}
{%
$c^{\gik}v_{\gik}\in J(v)$, $c^{\gik}\in \Base$,
\jJg kI
\labelItem{vector space, cvk in Jv}
}

\AddEquation{module, a+n:V->V}
{
a+n:v\in V\rightarrow (a+n)v\in V
}

\AddEquation{left module, a+n:V->V}
{
a+n:v\in V\rightarrow (a+n)v\in V
}

\AddEquation{right module, a+n:V->V}
{
a+n:v\in V\rightarrow v(a+n)\in V
}

\AddEq{module, sum cvk in Jv}
{%
$\displaystyle\sum_{\jJg kI}c(\gik)v(\gik)\in J(v)$,
$c(\gik)\in\Base_{\BaseExt}$, $|\{\gii:c(\gii)\ne 0\}|<\infty$
\labelItem{\VectorSetNS, sum cvk in Jv}
}

\AddEq{vector space, sum cvk in Jv}
{%
$\displaystyle\sum_{\jJg kI}c^{\gik}v_{\gik}\in J(v)$,
$c^{\gik}\in\Base$, $|\{\gii:c^{\gii}\ne 0\}|<\infty$
\labelItem{vector space, sum cvk in Jv}
}

\AddEq{left module, sum cvk in Jv}
{%
$\displaystyle\sum_{\jJg kI}(\gik)v(\gik)\in J(v)$,
$c(\gik)\in\Base_{\BaseExt}$, $|\{\gii:c(\gii)\ne 0\}|<\infty$
\labelItem{left \VectorSetNS, sum cvk in Jv}
}

\AddEq{right module, sum cvk in Jv}
{%
$\displaystyle\sum_{\jJg kI}v(\gik)c(\gik)\in J(v)$,
$c(\gik)\in\Base_{\BaseExt}$, $|\{\gii:c(\gii)\ne 0\}|<\infty$
\labelItem{right \VectorSetNS, sum cvk in Jv}
}

\AddEq[1]{|ci12 ne 0|}
{
H_1=\{\iIg:\aU{#1_1}i\ne 0\}
\ \ \ \,
H_2=\{\iIg:\aU{#1_2}i\ne 0\}
}

\AddEq[1]{|c(i)12 ne 0|}
{
H_1=\{\iIg:#1_1(\gii)\ne 0\}
\ \ \ \,
H_2=\{\iIg:#1_2(\gii)\ne 0\}
}

\AddEq{|wi ne 0|}
{
|\{\iIg:\aU wi\ne 0\}|<\infty
}

\AddEq{|w(i) ne 0|}
{
|\{\iIg:w(\gii)\ne 0\}|<\infty
}

\AddEq{module, |aw(i) ne 0|}
{
$\{\iIg:aw(\gii)\ne 0\}$
}

\AddEq{left module, |aw(i) ne 0|}
{
$\{\iIg:aw(\gii)\ne 0\}$
}

\AddEq{right module, |aw(i) ne 0|}
{
$\{\iIg:w(\gii)a\ne 0\}$
}

\AddEq{module, |awi ne 0|}
{
$\{\iIg:a\aU wi\ne 0\}$
}

\AddEq{left module, |awi ne 0|}
{
$\{\iIg:a\aU wi\ne 0\}$
}

\AddEq{right module, |awi ne 0|}
{
$\{\iIg:\aU wia\ne 0\}$
}

\AddEq{v,w in Jv=>v+w in Jv}
{
$w_1$, $w_2\in J(v)\Rightarrow w_1+w_2\in J(v)$
\labelItem{\SideWS module, v,w in Jv=>v+w in Jv}
}

\AddEq{v in Jv=>av in Jv}
{
$a\in\Base_{(1)}$,
$w\in J(v)\Rightarrow aw\in J(v)$
\labelItem{\SideWS module, v in Jv=>av in Jv}
}

\AddEq{vector space, v in Jv=>av in Jv}
{
$a\in\Base_{\BaseExt}$,
$w\in J(v)\Rightarrow aw\in J(v)$
\labelItem{\SideWS vector space, v in Jv=>av in Jv}
}

\AddEq[1]{gi12}
{
$\aU{#1_1}i$, $\aU{#1_2}i$, \iIg,
}

\AddEq[1]{g(i)12}
{
$#1_1(\gii)$, $#1_2(\gii)$, \iIg,
}

\AddEq[1]{w1+w2= 1 }
{
#1_1+#1_2=\sum_{\iIg}(\aU{#1_1}i+\aU{#1_2}i)v_{\gii}
}

\AddEq[1]{w1+w2= 1 left}
{
#1_1+#1_2=\sum_{\iIg}(\aU{#1_1}i+\aU{#1_2}i)v_{\gii}
}

\AddEq[1]{w1+w2= 1 right}
{
#1_1+#1_2=\sum_{\iIg}v_{\gii}\aU{#1_1}i+\aU{#1_2}i)
}

\AddEq[1]{|gi 1+2 ne 0|}
{
\[
\{\iIg:\aU{#1_1}i+\aU{#1_2}i\ne 0\}\subseteq H_1\cup H_2
\]
}

\AddEq[1]{|gi() 1+2 ne 0|}
{
\[
\{\iIg:#1_1(\gii)+#1_2(\gii)\ne 0\}\subseteq H_1\cup H_2
\]
}

\AddEq[1]{w1+w2= }
{
#1_1+#1_2=\sum_{\iIg}\aU{#1_1}iv_{\gii}+\sum_{\iIg}\aU{#1_2}iv_{\gii}
=\sum_{\iIg}(\aU{#1_1}iv_{\gii}+\aU{#1_2}iv_{\gii})
}

\AddEq[1]{w1+w2= left}
{
#1_1+#1_2=\sum_{\iIg}\aU{#1_1}iv_{\gii}+\sum_{\iIg}\aU{#1_2}iv_{\gii}
=\sum_{\iIg}(\aU{#1_1}iv_{\gii}+\aU{#1_2}iv_{\gii})
}

\AddEq[1]{w1+w2= right}
{
#1_1+#1_2=\sum_{\iIg}v_{\gii}\aU{#1_1}i+\sum_{\iIg}v_{\gii}\aU{#1_2}i
=\sum_{\iIg}(v_{\gii}\aU{#1_1}i+v_{\gii}\aU{#1_2}i)
}

\AddEq[1]{w()1+w()2= }
{
\begin{split}
#1_1+#1_2&=\sum_{\iIg}#1_1(\gii)v(\gii)+\sum_{\iIg}#1_2(\gii)v(\gii)
=\sum_{\iIg}(#1_1(\gii)v(\gii)+#1_2(\gii)v(\gii))
\\ &=\sum_{\iIg}(#1_1(\gii)+#1_2(\gii))v(\gii)
\end{split}
}

\AddEq[1]{w()1+w()2= left}
{
\begin{split}
#1_1+#1_2&=\sum_{\iIg}#1_1(\gii)v(\gii)+\sum_{\iIg}#1_2(\gii)v(\gii)
=\sum_{\iIg}(#1_1(\gii)v(\gii)+#1_2(\gii)v(\gii))
\\ &=\sum_{\iIg}(#1_1(\gii)+#1_2(\gii))v(\gii)
\end{split}
}

\AddEq[1]{w()1+w()2= right}
{
\begin{split}
#1_1+#1_2&=\sum_{\iIg}v(\gii)#1_1(\gii)+\sum_{\iIg}v(\gii)#1_2(\gii)
=\sum_{\iIg}(v(\gii)#1_1(\gii)+v(\gii)#1_2(\gii))
\\ &=\sum_{\iIg}v(\gii)(#1_1(\gii)+#1_2(\gii))
\end{split}
}

\AddEq[1]{w12= }
{
#1_1=\sum_{\iIg}\aU{#1_1}i\aD vi
\ \ \ \,
#1_2=\sum_{\iIg}\aU{#1_2}i\aD vi
}

\AddEq[1]{w12= left}
{
#1_1=\sum_{\iIg}\aU{#1_1}i\aD vi
\ \ \ \,
#1_2=\sum_{\iIg}\aU{#1_2}i\aD vi
}

\AddEq[1]{w12= right}
{
#1_1=\sum_{\iIg}\aD vi\aU{#1_1}i
\ \ \ \,
#1_2=\sum_{\iIg}\aD vi\aU{#1_2}i
}

\AddEq[1]{w()12= }
{
#1_1=\sum_{\iIg}#1_1(\gii)v(\gii)
\ \ \ \,
#1_2=\sum_{\iIg}#1_2(\gii)v(\gii)
}

\AddEq[1]{w()12= left}
{
#1_1=\sum_{\iIg}#1_1(\gii)v(\gii)
\ \ \ \,
#1_2=\sum_{\iIg}#1_2(\gii)v(\gii)
}

\AddEq[1]{w()12= right}
{
#1_1=\sum_{\iIg}v(\gii)#1_1(\gii)
\ \ \ \,
#1_2=\sum_{\iIg}v(\gii)#1_2(\gii)
}

\AddEquation{vk=sum vi, module}
{
v_{\gik}=\sum_{\iIg}\aU ci\aD vi
}

\AddEquation{vk=sum vi, left module}
{
v_{\gik}=\sum_{\iIg}\aU ci\aD vi
}

\AddEquation{vk=sum vi, right module}
{
\aD vk=\sum_{\iIg}\aD vi\aU ci
}

\AddEq[1]{v(k)=sum v(i), module}
{
v(\gik)=\sum_{\iIg}c(\gii)v(\gii)
\ \ \ c(\gii)\in #1
}

\AddEq[1]{v(k)=sum v(i), left module}
{
v(\gik)=\sum_{\iIg}c(\gii)v(\gii)
\ \ \ c(\gii)\in #1
}

\AddEq[1]{v(k)=sum v(i), right module}
{
v(\gik)=\sum_{\iIg}v(\gii)c(\gii)
\ \ \ c(\gii)\in #1
}

\AddEq[1]{ci=dik}
{
$c^{\gii}=\delta^{\gii}_{\gik}\in #1$.
}

\AddEq{c(i)=dik}
{
\[
c(\gii)=
\left\{
\begin{array}{l}
1,\ \gii=\gik\\
0
\end{array}
\right.
\]
}

\AddEq{vk in v}
{
$v_{\gik}\in v$,
}

\AddEq{v(i)}
{
$v(\gii)$.
}

\AddEq{w=c(i)v(i).}
{
$w=\sum c(\gii)v(\gii)$
}

\AddEq{w=c(i)v(i).left}
{
$w=\sum c(\gii)v(\gii)$
}

\AddEq{w=c(i)v(i).right}
{
$w=\sum v(\gii)c(\gii)$
}

\AddEq{w=w cr v}
{
\[\Vector w=\ShowSymbol{linear combination}{\SideWS cr}\]
}

\AddEq{g number linear combination}
{%
\symb{g^is_i}{linear combination}{}%
}

\AddEq{linear combination()}
{%
\symb{\sum c(\gii)v(\gii)}{linear combination}{i}%
}

\AddEq{left linear combination()}
{%
\symb{\sum c(\gii)v(\gii)}{linear combination}{left i}%
}

\AddEq{right linear combination()}
{%
\symb{\sum v(\gii)c(\gii)}{linear combination}{right i}%
}

\AddEq{the left linear combination()}
{%
$c(\gii)v(\gii)$
}

\AddEq{the right linear combination()}
{%
$v(\gii)c(\gii)$
}

\AddEq{A linear combination() =}
{
$\ShowSymbol{linear combination}{\SideWS i}$, $c(\gii)\in\Base_{\BaseExt}$,
}

\AddEq{(b+c)*e, module}
{
\[
(\ACol bi+
\ACol ci)
\ARow ei=0
\]
}

\AddEq{(b+c)*e, left module}
{
\[
(\ACol bi+
\ACol ci)
\ARow ei=0
\]
}

\AddEq{(b+c)*e, right module}
{
\[
\ARow ei
(\ACol bi+
\ACol ci)
=0
\]
}

\AddEq{(ac)*e, module}
{
\[
(a
\ACol ci)
\ARow ei=0
\]
}

\AddEq{(ac)*e, left module}
{
\[
(a
\ACol ci)
\ARow ei=0
\]
}

\AddEq{(ac)*e, right module}
{
\[
\ARow ei(a
\ACol ci)=0
\]
}

\AddEq{sum of maps,,D module}
{
\symb{f+g}{sum of maps}{D module}
}

\AddEquation{sum of maps, 1, D module}
{
\begin{matrix}
\ShowSymbol{sum of maps}{D module}:A_1\rightarrow A_2
&f,g\in\LAB D{A_1}{A_2}
\end{matrix}
}

\DefEquation
{
(\ShowSymbol{sum of maps}{D module})\circ x=f\circ x+g\circ x
}
{sum of maps, D module}

\AddEq [4]{f in L(A->B)}
{
$f\in\LAB{#1}{#2}{#3}$#4
}

\AddEquation{fa=sfsa}
{
f\circ(a_1, ..., a_n)=|\sigma|(f\circ\sigma\circ(a_1,...,a_n))
}

\DefEq
{
}
{}

\AddEq[1]{[f]}
{
$\ShowSymbol{alternation of polylinear map}{}$#1
}

\AddEq{alternation of polylinear map}
{
\symb{[f]}{alternation of polylinear map}{}
}

\AddEq{fx1n=0}
{
\[
f\circ(a_1,...,a_n)=0
\]
}

\AddEq{1<=i<n}
{
$i$, $1\le i<n$.
}

\AddEq{fa=fsa}
{
\[
f\circ(a_1, ..., a_n)=f\circ\sigma\circ(a_1,...,a_n)
\]
}

\AddEq{symmetrization of polylinear map}
{
\symb{<f>}{symmetrization of polylinear map}{}
}

\AddEq{<f>}
{
$\ShowSymbol{symmetrization of polylinear map}{}\circ(a_1,...,a_n)$\Pt
}

\AddEq[1]{f()}
{
$f\circ(a_1,...,a_p)$#1
}

\AddEq{h:B1->*B2}
{
\[
\xymatrix
{
h:B_1\ar[r]|{*}&B_2
}
\]
}

\AddEq[3]{L(A1,A0,B)=}
{
\begin{align}
\mathcal{LA}(#1;#2\rightarrow #3)&=\mathcal L(#1;#2\rightarrow #3)\\
\mathcal{LA}(#1;#2^0\rightarrow #3)&=#3
\end{align}
}

\newcommand\LAnAB[3]{\ensuremath{\mathcal{LA}(#1;#2^n\rightarrow #3)}}

\AddEq[3]{module of skew symmetric polylinear maps}
{
\symb{\LAnAB{#1}{#2}{#3}}{module of skew symmetric polylinear maps}{1}
}

\AddEquation{exterior product = skew symmetric}
{
(f\wedge g)\circ(a_1,...,a_{p+q})=
\frac 1{p!q!}\sum_{\sigma\in S(p+q)}|\sigma|((f\wedge g)\circ\sigma\circ(a_1,...,a_{p+q}))
}

\AddEquation{exterior product =}
{
(\ShowSymbol{exterior product}{1})\circ(a_1,...,a_{p+q})=\frac {(p+q)!}{p!q!}
[fg]\circ(a_1,...,a_{p+q})
}

\AddEq{exterior product}
{
\symb{f\wedge g}{exterior product}{1}
}

\AddEquation{hpq(fg)=}
{
(fg)\circ(a_1,...,a_{p+q})=(f\circ(a_1,...,a_p))(g\circ(a_{p+1},...,a_{p+q}))
}

\AddEq{hpq:Lpq->Lp+q}
{
\[
fg:\mathcal L(D;A^p\rightarrow B)\times\mathcal L(D;A^q\rightarrow C)\rightarrow \mathcal L(D;A^{p+q}\rightarrow C)
\]
}

\AddEq[1]{g()}
{
$g\circ(a_{p+1},...,a_{p+q})$#1
}

\AddEq{symmetrization of polylinear map =}
{
\[
\ShowSymbol{symmetrization of polylinear map}{}\circ(a_1,...,a_n)
=\frac 1{n!}
\sum_{\sigma\in S(n)}f\circ\sigma\circ(a_1,...,a_n)
\]
}

\AddEquation{alternation of polylinear map =}
{
\ShowSymbol{alternation of polylinear map}{}\circ(a_1,...,a_n)
=\frac 1{n!}\sum_{\sigma\in S(n)}|\sigma|(f\circ\sigma\circ(a_1,...,a_n))
}

\AddEq[3]{A 1n}
{
$\aU{#1}1$, ..., $\aU{#1}{#2}$#3
}

\AddEq{fab=fbfa}
{
\[
f(ab)=f(b)f(a)
\]
}

\AddEq{b o f =}
{
\[
(b\circ f)\circ x=b(f\circ x)
\]
}

\AddEq{b * f =}
{
\[
(b*f)\circ x=(f\circ x)b
\]
}

\DefEq
{
$F_k\in\Basis F$,
}
{Ik in I}

\DefEquation
{
x\rightarrow I_k\circ a\circ x
}
{x->Ik a x}

\DefEquation
{
b^l=I^l_k\circ a
}
{b=Ikl a}

\DefEq
{
\begin{align*}
(I_k^l\circ(a_1+\aD a2))\circ I_l\circ x
&=I_k\circ(a_1+\aD a2)\circ x
\\&=I_k\circ a_1\circ x+I_k\circ \aD a2\circ x
\\&=(I_k^l\circ a_1)\circ I_l\circ x+(I_k^l\circ a_1)\circ I_l\circ x
\end{align*}
}
{Ikl a1+a2}

\DefEq
{
\begin{align*}
(I_k^l\circ(da))\circ I_l\circ x
&=I_k\circ(da)\circ x
=I_k\circ(d(a\circ x))
\\&=d(I_k\circ a\circ x)
=d((I_k^l\circ a)\circ I_l\circ x)
\\&=(d(I_k^l\circ a))\circ I_l\circ x
\end{align*}
}
{Ikl d a}

\DefEquation
{
I_k\circ a\circ x=b^l\circ I_l\circ x\ \ \ \ b^l\in A_2\times A_2
}
{expansion Ik a x}

\DefEq
{
\symb{F_k^l}{conjugation transformation}{}
}
{conjugation transformation}

\DefEq
{
\[
\ShowSymbol{conjugation transformation}{}
:A_1\otimes A_1\rightarrow A_2\otimes A_2
\]
}
{conjugation transformation:}

\DefEquation
{
F_k\circ a\circ x=(\ShowSymbol{conjugation transformation}{}\circ a)\circ F_l\circ x
}
{conjugation transformation =}

\DefEq
{
$\ShowSymbol{conjugation transformation}{}$
}
{show conjugation transformation}

\DefEq
{
$\aUD Cp{kl}$
}
{structural constants, algebra}

\AddEq{ci i in I}
{
\ACol ci, \iIg,
}

\AddEq{c=ci i in I}
{
$c=(\ACol ci,\iIg)$
}

\AddEq{i=j}
{
$\gii=\gij$
}

\AddEq{Coordinates of map f}
{
$\aUD fkl$
}

\AddEq[1]{standard components of map f}
{
\def\Cdot{}
\def\Temp{-}%
\edef\Tempa{#1}%
\ifx\Tempa\Temp%
\else
\def\Cdot{#1\cdot}
\fi
$\aU {f^{\Cdot}_{}{}}{ij}$
}

\AddEq{linear map over ring, left side}
{
$\aUD flk$
}

\AddEq{left shift algebra, 2}
{
\[
(a,b)_1\circ x=(a,b,x)
\]
}

\AddEquation{left shift algebra}
{
l(a)\circ x=ax
}

\AddEquation{left shift algebra, 3}
{
\begin{split}
(l(a)\circ l(b))\circ x
&=l(a)\circ(l(b)\circ x)
\\
&=a(bx)=(ab)x-(a,b,x)
\\
&=l(ab)\circ x-(a,b)_1\circ x
\end{split}
}

\AddEquation{left shift algebra, 1}
{
l(a)\circ l(b)=l(ab)-(a,b)_1
}

\AddEquation{right shift algebra}
{
r(a)\circ x=xa
}

\AddEquation{right shift algebra, 3}
{
\begin{split}
(r(a)\circ r(b))\circ x
&=r(a)\circ(r(b)\circ x)
\\
&=(xb)a=x(ba)+(x,b,a)
\\
&=r(ba)\circ x+(x,b,a)
\end{split}
}

\AddEquation{right shift algebra, 1}
{
r(a)\circ r(b)=r(ba)+(b,a)_2
}

\AddEq{right shift algebra, 2}
{
\[
(b,a)_2\circ x=(x,b,a)
\]
}

\AddEq{f over A}
{
\[
f:x\in A\rightarrow (ax)b\in A
\]
}

\AddEq{g over A}
{
\[
\begin{matrix}
g:A\rightarrow A
&&
g=(cf)d
\end{matrix}
\]
}

\AddEquation{linear map, standard representation, nonassociative algebra}
{
f\circ x=\aU f{ij}\ (\aD eix)\aD ej
}

\AddEq{linear map, standard representation, nonassociative algebra, 1}
{
\[
f\circ x=\aU f{ij}\aD ei(x\aD ej)
\]
}

\AddEquation{coordinates of map A1 A2, 2, nonassociative algebra}
{
\aUD gkl
=\aUD fml\aU g{ij}
\aUD Cp{im}\aUD Ck{pj}
}

\AddEquation{coordinates of map A1 A2, 21, nonassociative algebra}
{
\aUD gkl
=\aUD fml \aU g{ij}
\aUD Ck{ip}\aUD Cp{mj}
}

\DefEq
{
$F_{k\cdot}^{}{}_{\gii}^{\gij}$
}
{coordinates of map Ik}

\DefEq
{
$G_{\gii}^{\gij}$
}
{coordinates of map G}

\AddEq{projection maps, complex field}
{
\begin{align*}
P^{\gi 0}\circ a&=\aU a0&P^{\gi 0\cdot}_{}{}^{\gi 0}_{\gi 0}&=1&
R^{\gi 0}\circ a&=\aU a0&R^{\gi 0\cdot}_{}{}^{\gi 0}_{\gi 0}&=1
\\
P^{\giA}\circ a&=\aU a1i&P^{\giA\cdot}_{}{}^{\giA}_{\giA}&=1&
R^{\giA}\circ a&=\aU a1&R^{\giA\cdot}_{}{}^{\gi 0}_{\giA}&=1
\end{align*}
}

\AddEq [1]{e=(E,I)}
{
$\eV=(E,I)$#1
}

\AddEq{projection mappings 1, complex field}
{
\begin{align*}
P^{\gi 0}&=\frac 12\circ E+\frac 12\circ I&
R^{\gi 0}&=\frac 12\circ E+\frac 12\circ I
\\
P^{\giA}&=\frac 12\circ E-\frac 12\circ I&
R^{\giA}&=-\frac i2\circ E+\frac i2\circ I
\end{align*}
}

\AddEquation{df/dx= complex field}
{
\frac{df}{dx}=
\frac 12\left(\frac{\partial f}{\partial \aU x0}
-i\frac{\partial f}{\partial x^{\gi 1}}\right)\circ E
+\frac 12\left(\frac{\partial f}{\partial \aU x0}
+i\frac{\partial f}{\partial x^{\gi 1}}\right)\circ I
}

\DefEquation
{
f=\aD a0\circ E+a_1\circ I+\aD a2\circ J+\aD a3\circ K
}
{expand linear mapping, quaternion}

\AddEquation{fi=fij ej H}
{
\begin{pmatrix}
\aD f0\\ \aD f1\\ \aD f2\\ \aD f3
\end{pmatrix}
=
\begin{pmatrix}
\aUD f00&\aUD f10&\aUD f20&\aUD f30\\
\aUD f01&\aUD f11&\aUD f21&\aUD f31\\
\aUD f02&\aUD f12&\aUD f22&\aUD f32\\
\aUD f03&\aUD f13&\aUD f23&\aUD f33
\end{pmatrix}
\begin{pmatrix}
1\\i\\j\\k
\end{pmatrix}
=
\begin{pmatrix}
\aUD f00+\aUD f10i+\aUD f20j+\aUD f30k\\
\aUD f01+\aUD f11i+\aUD f21j+\aUD f31k\\
\aUD f02+\aUD f12i+\aUD f22j+\aUD f32k\\
\aUD f03+\aUD f13i+\aUD f23j+\aUD f33k
\end{pmatrix}
}

\AddEq{fi=fij ej}
{
\aD fi=\aUD fji \aD ej
}

\AddEquation{f=.E+.I}
{
f=\frac 12(\aD f0-i\aD f1)\circ E+\frac 12(\aD f0+i\aD f1)\circ I
}

\AddEquation{a0=f01}
{
\begin{split}
\aD a0&=\aUD a00+\aUD a10i
=\frac 12(\aUD f00+\aUD f11+(\aUD f10-\aUD f01)i)
\\&=\frac 12(\aUD f00+\aUD f10i+\aUD f11-\aUD f01i)
\\&=\frac 12((\aUD f00+\aUD f10i)-(\aUD f01+\aUD f11i)i)
\end{split}
}

\AddEquation{a1=f01}
{
\begin{split}
a_1&=\aUD a01+\aUD a11i
=\frac 12(\aUD f00-\aUD f11+(\aUD f10+\aUD f01)i)
\\&=\frac 12(\aUD f00+\aUD f10i-\aUD f11+\aUD f01i)
\\&=\frac 12((\aUD f00+\aUD f10i)+(\aUD f01+\aUD f11i)i)
\end{split}
}

\AddEquation{a...= C}
{
\ShowEq{matrix a algebra C}
=
\ShowEq{matrix af algebra C}
\ShowEq{matrix f algebra C}
}

\AddEq [2]{map ao}
{
\def\Map{\aU I#1}
\edef\Tempa{#1}%
\def\Temp{E}
\ifx\Tempa\Temp%
\def\Map{E}
\fi
\def\Temp{I}
\ifx\Tempa\Temp%
\def\Map{I}
\fi
\begin{matrix}
a\bullet \Map:b\in #2\rightarrow a(\Map\circ b)\in #2&a\in #2
\end{matrix}
}

\AddEquation{f->ao f}
{
a\bullet:f\in
\ShowEq{L(A->B)}DAA
\rightarrow a\bullet f\in
\ShowEq{L(A->B)}DAA
}

\AddEquation{ao f=a f o}
{
(a\bullet f)\circ b=a(f\circ b)
}

\AddEquation{f->a* f}
{
a\star:f\in
\ShowEq{L(A->B)}DAA
\rightarrow a\star f\in
\ShowEq{L(A->B)}DAA
}

\AddEquation{a* f=(f o)a}
{
(a\star f)\circ b=(f\circ b)a
}

\AddEq [2]{map a*}
{
\def\Map{E}
\def\Temp{E}
\edef\Tempa{#1}%
\ifx\Tempa\Temp%
\else
\def\Map{\aU I#1}
\fi
\begin{matrix}
\Map\bullet a:b\in #2\rightarrow (\Map\circ b)a\in #2&a\in #2
\end{matrix}
}

\AddEq [1]{ao, H matrix 1}
{
#1_l(a)=E_l(a)\RCcirc #1
}

\AddEq [1]{a*, H matrix 1}
{
#1_r(a)=E_r(a)\RCcirc #1
}

\AddEq {aI, H matrix 2}
{
\begin{align*}
E_l(a)\RCcirc I
&=
\ShowEq{H aE Jacobian matrix}a
\RCcirc\Ei
\\
&=
\ShowEq{H a1 Jacobian matrix}a
=
I_l(a)
\end{align*}
}

\AddEq {aJ, H matrix 2}
{
\begin{align*}
E_l(a)\RCcirc J
&=
\ShowEq{H aE Jacobian matrix}a
\RCcirc\Ej
\\
&=
\ShowEq{H a2 Jacobian matrix}a
=
J_l(a)
\end{align*}
}

\AddEq{aK, H matrix 2}
{
\begin{align*}
E_l(a)\RCcirc K
&=
\ShowEq{H aE Jacobian matrix}a
\RCcirc\Ek
\\
&=
\ShowEq{H a3 Jacobian matrix}a
=
K_l(a)
\end{align*}
}

\AddEq{Ia, H matrix 2}
{
\begin{align*}
E_r(a)\RCcirc I
&=
\ShowEq{H Ea Jacobian matrix}a
\RCcirc\Ei
\\
&=
\ShowEq{H 1a Jacobian matrix}a
=
I_r(a)
\end{align*}
}

\AddEq{Ja, H matrix 2}
{
\begin{align*}
E_r(a)\RCcirc J
&=
\ShowEq{H Ea Jacobian matrix}a
\RCcirc\Ej
\\
&=
\ShowEq{H 2a Jacobian matrix}a
=
J_r(a)
\end{align*}
}

\AddEq{Ka, H matrix 2}
{
\begin{align*}
E_r(a)\RCcirc K
&=
\ShowEq{H Ea Jacobian matrix}a
\RCcirc\Ek
\\
&=
\ShowEq{H 3a Jacobian matrix}a
=
K_r(a)
\end{align*}
}

\AddEq[3]{maps of conjugation, Jacobian matrix}
{
\gdef\Map{\aU I#1}
\gdef\Letter{I}
\def\Temp{E}
\edef\Tempa{#1}%
\ifx\Tempa\Temp%
\gdef\Map{E}
\gdef\Letter{E}
\fi
\def\Temp{I}
\ifx\Tempa\Temp%
\gdef\Map{I}
\fi
\symb[\Letter-0]{\Map_{#3}(a)}{maps of conjugation, Jacobian matrix}{#1#2}
}

\AddEq[2]{a o, Jacobian matrix}
{
\ShowSymbol{maps of conjugation, Jacobian matrix}{#1#2}=
\ShowEq{#2 a#1 Jacobian matrix}a
}

\AddEq[2]{a *, Jacobian matrix}
{
\ShowSymbol{maps of conjugation, Jacobian matrix}{#1#2}=
\ShowEq{#2 #1a Jacobian matrix}a
}

\AddEq[1]{ao, C, Jacobian matrix}
{
\symb[#1-0]{#1(a)}{maps of conjugation, Jacobian matrix}{}
}

\AddEquation{aE, C, matrix}
{
\ShowSymbol{maps of conjugation, Jacobian matrix}{}=
\begin{pmatrix}
\aU a0&-a^{\gi 1}\\
a^{\gi 1}&\hphantom{-}\aU a0
\end{pmatrix}
}

\AddEquation{aI, C, matrix}
{
\ShowSymbol{maps of conjugation, Jacobian matrix}{}=
\begin{pmatrix}
\aU a0&\hphantom{-}a^{\gi 1}\\
a^{\gi 1}&-\aU a0
\end{pmatrix}
}

\AddEquation{f in L(A,A), 2, nonassociative algebra}
{
f
=a^{k\cdot \gi{ij}}(\aU ei\otimes\aU ej)\circ F_k
=
a^{k\cdot \gi{ij}}(\aU eiI_k)\aU ej
}

\AddEquation{system 1 of linear equations, quaternion}
{
\begin{split}
i\aU x1j+j\aU x2k&=i+j
\\
k\aU x1i+i\aU x2j&=i-j
\end{split}
}

\AddEquation{system 1 of linear equations, quaternion, 1}
{
\begin{split}
(i\otimes j)\circ\aU x1+(j\otimes k)\circ\aU x2&=i+j
\\
(k\otimes i)\circ\aU x1+(i\otimes j)\circ\aU x2&=i-j
\end{split}
}

\AddEquation{system 1 of linear equations, quaternion, 2}
{
\begin{pmatrix}
i\otimes j&j\otimes k\\
k\otimes i&i\otimes j
\end{pmatrix}
\RCcirc
\begin{pmatrix}
c\aU x1\\\aU x2
\end{pmatrix}
=
\begin{pmatrix}
i+j\\i-j
\end{pmatrix}
}

\AddEq{system 1 of linear equations, quaternion, 3}
{
\[
a=
\begin{pmatrix}
i\otimes j&j\otimes k\\
k\otimes i&i\otimes j
\end{pmatrix}
\]
}

\AddEq{system 1 of linear equations, quaternion, 4}
{
\ShowEq{system 1 of linear equations, quaternion, 4 1 1}
\ShowEq{system 1 of linear equations, quaternion, 4 1 2}
\ShowEq{system 1 of linear equations, quaternion, 4 2 1}
\ShowEq{system 1 of linear equations, quaternion, 4 2 2}
}

\AddEquation{system 1 of linear equations, quaternion, 4 1 1}
{
\begin{split}
\aUD{\det\left(a,\RCcirc\right)}11&=\aUD a11
-\aUD a1{[1]}\RCcirc
(\aUD a{[1]}{[1]})^{-1\RCcirc}\RCcirc
\aUD a{[1]}1
=\aUD a11
-\aUD a12\circ
(\aUD a22)^{-1}\circ
\aUD a21
\\
&=i\otimes j
-(j\otimes k)\circ
(i\otimes j)^{-1}\circ
(k\otimes i)
\\
&=i\otimes j
-(j\otimes k)\circ
(i\otimes j)\circ
(k\otimes i)
=i\otimes j
-(-1)\otimes (-1)
\\
&=i\otimes j
-1\otimes 1
\end{split}
}

\AddEquation{system 1 of linear equations, quaternion, 4 1 2}
{
\begin{split}
\aUD{\det\left(a,\RCcirc\right)}12&=\aUD a12
-\aUD a1{[2]}\RCcirc
(\aUD a{[1]}{[2]})^{-1\RCcirc}\RCcirc
\aUD a{[1]}2
=\aUD a12
-\aUD a11\circ
(\aUD a21)^{-1}\circ
\aUD a22
\\
&=j\otimes k
-(i\otimes j)\circ
(k\otimes i)^{-1}\circ
(i\otimes j)
\\
&=j\otimes k
-(i\otimes j)\circ
(k\otimes i)\circ
(i\otimes j)
=j\otimes k
-(-k)\otimes i
\\
&=j\otimes k
+k\otimes i
\end{split}
}

\AddEquation{system 1 of linear equations, quaternion, 4 2 1}
{
\begin{split}
\aUD{\det\left(a,\RCcirc\right)}21&=\aUD a21
-\aUD a2{[1]}\RCcirc
(\aUD a{[2]}{[1]})^{-1\RCcirc}\RCcirc
\aUD a{[2]}1
=\aUD a21
-\aUD a22\circ
(\aUD a12)^{-1}\circ
\aUD a11
\\
&=k\otimes i
-(i\otimes j)\circ
(j\otimes k)^{-1}\circ
(i\otimes j)
\\
&=k\otimes i
-(i\otimes j)\circ
(j\otimes k)\circ
(i\otimes j)
=k\otimes i
-(-j)\otimes k
\\
&=k\otimes i
+j\otimes k
\end{split}
}

\AddEquation{system 1 of linear equations, quaternion, 4 2 2}
{
\begin{split}
\aUD{\det\left(a,\RCcirc\right)}22&=\aUD a22
-\aUD a2{[2]}\RCcirc
(\aUD a{[2]}{[2]})^{-1\RCcirc}\RCcirc
\aUD a{[2]}2
=\aUD a22
-\aUD a21\circ
(\aUD a11)^{-1}\circ
\aUD a12
\\
&=i\otimes j
-(k\otimes i)\circ
(i\otimes j)^{-1}\circ
(j\otimes k)
\\
&=i\otimes j
-(k\otimes i)\circ
(i\otimes j)\circ
(j\otimes k)
=i\otimes j
-(-1)\otimes (-1)
\\
&=i\otimes j
-1\otimes 1
\end{split}
}

\AddEquation{fg=1 e o e}
{
\begin{split}
\aU f{ij}\aUD C0{ik}\aUD C0{lj}\aU g{kl}&=1\\
\aU f{ij}\aUD Cp{ik}\aUD Cq{lj}\aU g{kl}&=0\ \ \ p+q>0
\end{split}
}

\AddEq{g o h=1}
{
\[g\circ h=\aD e0\otimes\aD e0\]
}

\AddEq{f1=...}
{
\[f_1=-1\otimes 1+i\otimes j\]
}

\AddEq{f2=...}
{
\[f_2=k\otimes i+j\otimes k\]
}

\AddEq[2]{g=f-1}
{
$g_{#1}=f_{#1}^{-1}$#2
}

\AddEq[3]{row set 1n}
{
$\aD {#1}1$, ..., $\aD {#1}{#2}$#3
}

\AddEq[3]{column set 1n}
{
$\aU {#1}1$, ..., $\aU {#1}{#2}$#3
}

\AddEq[3]{row() 1n}
{
$#1(\gi 1)=\aD {#1}1$, ..., $#1(\gi{#2})=\aD {#1}{#2}$#3
}

\AddEq[3]{col() 1n}
{
$#1(\gi 1)=\aU {#1}1$, ..., $#1(\gi{#2})=\aU {#1}{#2}$#3
}

\AddEq[5]{system of linear equations left column row}
{
\begin{split}
\aU {#1}1\aUD {#2}11+...+\aU {#1}{#4}\aUD {#2}1{#4}&=\aU {#3}1
\\...&=...\\
\aU {#1}1\aUD {#2}{#5}1+...+\aU {#1}{#4}\aUD {#2}{#5}{#4}&=\aU {#3}{#5}
\end{split}
}

\AddEq[5]{system of linear equations linear map}
{
\begin{split}
\aUD {#2}1{11}\aU {#1}1\aUD {#2}1{12}+...+\aUD {#2}1{{#4}1}\aU {#1}{#4}\aUD {#2}1{{#4}2}
&=\aU {#3}1
\\...&=...\\
\aUD {#2}{#5}{11}\aU {#1}1\aUD {#2}{#5}{12}+...+\aUD {#2}{#5}{{#4}1}\aU {#1}{#4}\aUD {#2}{#5}{{#4}2}
&=\aU {#3}{#5}
\end{split}
}

\AddEquation{fg=1 e o e g1}
{
\left\{
\begin{matrix}
-\aUD C0{0k}\aUD C0{l0}\aU g{kl}+
\aUD C0{1k}\aUD C0{l2}\aU g{kl}=1\\
-\aUD C0{0k}\aUD C1{l0}\aU g{kl}+
\aUD C0{1k}\aUD C1{l2}\aU g{kl}=0\\
-\aUD C0{0k}\aUD C2{l0}\aU g{kl}+
\aUD C0{1k}\aUD C2{l2}\aU g{kl}=0\\
-\aUD C0{0k}\aUD C3{l0}\aU g{kl}+
\aUD C0{1k}\aUD C3{l2}\aU g{kl}=0\\
-\aUD C1{0k}\aUD C0{l0}\aU g{kl}+
\aUD C1{1k}\aUD C0{l2}\aU g{kl}=0\\
-\aUD C1{0k}\aUD C1{l0}\aU g{kl}+
\aUD C1{1k}\aUD C1{l2}\aU g{kl}=0\\
-\aUD C1{0k}\aUD C2{l0}\aU g{kl}+
\aUD C1{1k}\aUD C2{l2}\aU g{kl}=0\\
-\aUD C1{0k}\aUD C3{l0}\aU g{kl}+
\aUD C1{1k}\aUD C3{l2}\aU g{kl}=0
\end{matrix}
\ \ \ \ \,
\begin{matrix}
-\aUD C2{0k}\aUD C0{l0}\aU g{kl}+
\aUD C2{1k}\aUD C0{l2}\aU g{kl}=0\\
-\aUD C2{0k}\aUD C1{l0}\aU g{kl}+
\aUD C2{1k}\aUD C1{l2}\aU g{kl}=0\\
-\aUD C2{0k}\aUD C2{l0}\aU g{kl}+
\aUD C2{1k}\aUD C2{l2}\aU g{kl}=0\\
-\aUD C2{0k}\aUD C3{l0}\aU g{kl}+
\aUD C2{1k}\aUD C3{l2}\aU g{kl}=0\\
-\aUD C3{0k}\aUD C0{l0}\aU g{kl}+
\aUD C3{1k}\aUD C0{l2}\aU g{kl}=0\\
-\aUD C3{0k}\aUD C1{l0}\aU g{kl}+
\aUD C3{1k}\aUD C1{l2}\aU g{kl}=0\\
-\aUD C3{0k}\aUD C2{l0}\aU g{kl}+
\aUD C3{1k}\aUD C2{l2}\aU g{kl}=0\\
-\aUD C3{0k}\aUD C3{l0}\aU g{kl}+
\aUD C3{1k}\aUD C3{l2}\aU g{kl}=0
\end{matrix}
\right.
}

\AddEquation{fg=1 e o e g1 1}
{
\left\{
\begin{matrix}
\BlueText{-\aU g{00}+\aU g{12}=1}\\
-\aU g{01}+\aU g{13}=0\\
-\aU g{02}-\aU g{10}=0\\
-\aU g{03}+\aU g{11}=0\\
-\aU g{10}-\aU g{02}=0\\
-\aU g{11}-\aU g{03}=0\\
\BlueText{-\aU g{12}+\aU g{00}=0}\\
-\aU g{13}+\aU g{01}=0
\end{matrix}
\ \ \ \ \,
\begin{matrix}
-\aUD C2{0k}\aUD C0{l0}\aU g{kl}+
\aUD C2{1k}\aUD C0{l2}\aU g{kl}=0\\
-\aUD C2{0k}\aUD C1{l0}\aU g{kl}+
\aUD C2{1k}\aUD C1{l2}\aU g{kl}=0\\
-\aUD C2{0k}\aUD C2{l0}\aU g{kl}+
\aUD C2{1k}\aUD C2{l2}\aU g{kl}=0\\
-\aUD C2{0k}\aUD C3{l0}\aU g{kl}+
\aUD C2{1k}\aUD C3{l2}\aU g{kl}=0\\
-\aUD C3{0k}\aUD C0{l0}\aU g{kl}+
\aUD C3{1k}\aUD C0{l2}\aU g{kl}=0\\
-\aUD C3{0k}\aUD C1{l0}\aU g{kl}+
\aUD C3{1k}\aUD C1{l2}\aU g{kl}=0\\
-\aUD C3{0k}\aUD C2{l0}\aU g{kl}+
\aUD C3{1k}\aUD C2{l2}\aU g{kl}=0\\
-\aUD C3{0k}\aUD C3{l0}\aU g{kl}+
\aUD C3{1k}\aUD C3{l2}\aU g{kl}=0
\end{matrix}
\right.
}

\AddEquation{fg=1 e o e g2}
{
\left\{
\begin{matrix}
\aUD C0{3k}\aUD C0{l1}\aU g{kl}+
\aUD C0{2k}\aUD C0{l3}\aU g{kl}=1\\
\aUD C0{3k}\aUD C1{l1}\aU g{kl}+
\aUD C0{2k}\aUD C1{l3}\aU g{kl}=0\\
\aUD C0{3k}\aUD C2{l1}\aU g{kl}+
\aUD C0{2k}\aUD C2{l3}\aU g{kl}=0\\
\aUD C0{3k}\aUD C3{l1}\aU g{kl}+
\aUD C0{2k}\aUD C3{l3}\aU g{kl}=0\\
\aUD C1{3k}\aUD C0{l1}\aU g{kl}+
\aUD C1{2k}\aUD C0{l3}\aU g{kl}=0\\
\aUD C1{3k}\aUD C1{l1}\aU g{kl}+
\aUD C1{2k}\aUD C1{l3}\aU g{kl}=0\\
\aUD C1{3k}\aUD C2{l1}\aU g{kl}+
\aUD C1{2k}\aUD C2{l3}\aU g{kl}=0\\
\aUD C1{3k}\aUD C3{l1}\aU g{kl}+
\aUD C1{2k}\aUD C3{l3}\aU g{kl}=0
\end{matrix}
\ \ \ \ \,
\begin{matrix}
\aUD C2{3k}\aUD C0{l1}\aU g{kl}+
\aUD C2{2k}\aUD C0{l3}\aU g{kl}=0\\
\aUD C2{3k}\aUD C1{l1}\aU g{kl}+
\aUD C2{2k}\aUD C1{l3}\aU g{kl}=0\\
\aUD C2{3k}\aUD C2{l1}\aU g{kl}+
\aUD C2{2k}\aUD C2{l3}\aU g{kl}=0\\
\aUD C2{3k}\aUD C3{l1}\aU g{kl}+
\aUD C2{2k}\aUD C3{l3}\aU g{kl}=0\\
\aUD C3{3k}\aUD C0{l1}\aU g{kl}+
\aUD C3{2k}\aUD C0{l3}\aU g{kl}=0\\
\aUD C3{3k}\aUD C1{l1}\aU g{kl}+
\aUD C3{2k}\aUD C1{l3}\aU g{kl}=0\\
\aUD C3{3k}\aUD C2{l1}\aU g{kl}+
\aUD C3{2k}\aUD C2{l3}\aU g{kl}=0\\
\aUD C3{3k}\aUD C3{l1}\aU g{kl}+
\aUD C3{2k}\aUD C3{l3}\aU g{kl}=0
\end{matrix}
\right.
}

\AddEquation{fg=1 e o e g2 1}
{
\left\{
\begin{matrix}
\BlueText{\aU g{31}+\aU g{23}=1}\\
-\aU g{30}-\aU g{22}=0\\
-\aU g{33}+\aU g{21}=0\\
\aU g{32}-\aU g{20}=0\\
\aU g{21}-\aU g{33}=0\\
-\aU g{20}+\aU g{32}=0\\
\BlueText{-\aU g{23}-\aU g{31}=0}\\
\aU g{22}+\aU g{30}=0
\end{matrix}
\ \ \ \ \,
\begin{matrix}
\aUD C2{3k}\aUD C0{l1}\aU g{kl}+
\aUD C2{2k}\aUD C0{l3}\aU g{kl}=0\\
\aUD C2{3k}\aUD C1{l1}\aU g{kl}+
\aUD C2{2k}\aUD C1{l3}\aU g{kl}=0\\
\aUD C2{3k}\aUD C2{l1}\aU g{kl}+
\aUD C2{2k}\aUD C2{l3}\aU g{kl}=0\\
\aUD C2{3k}\aUD C3{l1}\aU g{kl}+
\aUD C2{2k}\aUD C3{l3}\aU g{kl}=0\\
\aUD C3{3k}\aUD C0{l1}\aU g{kl}+
\aUD C3{2k}\aUD C0{l3}\aU g{kl}=0\\
\aUD C3{3k}\aUD C1{l1}\aU g{kl}+
\aUD C3{2k}\aUD C1{l3}\aU g{kl}=0\\
\aUD C3{3k}\aUD C2{l1}\aU g{kl}+
\aUD C3{2k}\aUD C2{l3}\aU g{kl}=0\\
\aUD C3{3k}\aUD C3{l1}\aU g{kl}+
\aUD C3{2k}\aUD C3{l3}\aU g{kl}=0
\end{matrix}
\right.
}

\AddEq[1]{Map of Conjugation}
{
\def\Temp{0}%
\def\Tempa{#1}%
\ifx\Tempa\Temp%
\ensuremath{E}
\else
\ensuremath{\aU I{#1}}
\fi
}

\AddEquation{H.fUD<-fUU}
{
\begin{split}
&
\ShowEq{quaternion matrix fUD}
\\=&
\ShowEq{quaternion matrix fUD<-fUU}
\ShowEq{quaternion matrix fUU}f
\end{split}
}

\AddEq[1]{H.fUD->fUU I}
{
\begin{split}
&
\ShowEq{quaternion matrix fUU}f
\\=&
\ShowEq{quaternion matrix fUD->fUU}
\ShowEq{H. matrix fUD I#1}
\end{split}
}

\AddEquation{H.fUD->fUU}
{
\begin{split}
&
\ShowEq{quaternion matrix fUU}f
\\=&
\ShowEq{quaternion matrix fUD->fUU}
\ShowEq{quaternion matrix fUD}
\end{split}
}

\AddEq{quaternion, 3, 1}
{
\[
\ShowEq{quaternion matrix fUD<-fUU}^{-1}
=
\ShowEq{quaternion matrix fUD->fUU}
\]
}

\AddEq{D in Z(A)}
{
\(D\subset Z(A)\).
\labelItem{D in Z(A)}
}

\AddEquation{H.fUD<-fUU f1 1}
{
\begin{split}
&
\ShowEq{quaternion matrix fUD}
\\=&
\ShowEq{quaternion matrix fUD<-fUU}
\left(
\begin{array}{rrrr}
-1&0&0&0\\
0&0&0&-1\\
0&0&0&0\\
0&0&0&0
\end{array}
\right)
\\=&
\left(
\begin{array}{rrrr}
-1&0&0&1\\
-1&0&0&1\\
-1&0&0&-1\\
-1&0&0&-1
\end{array}
\right)
\end{split}
}

\AddEquation{H.fUD<-fUU f2 1}
{
\begin{split}
&
\ShowEq{quaternion matrix fUD}
\\=&
\ShowEq{quaternion matrix fUD<-fUU}
\left(
\begin{array}{rrrr}
0&0&0&0\\
0&0&0&0\\
0&-1&0&0\\
0&0&-1&0
\end{array}
\right)
\\=&
\left(
\begin{array}{rrrr}
0&1&1&0\\
0&-1&-1&0\\
0&1&-1&0\\
0&-1&1&0
\end{array}
\right)
\end{split}
}

\AddEquation{matrix f1}
{
f_1=
\left(
\begin{array}{rrrr}
-1&0&0&1\\
0&-1&-1&0\\
0&-1&-1&0\\
1&0&0&-1
\end{array}
\right)
}

\AddEquation{matrix f2}
{
f_2=
\left(
\begin{array}{rrrr}
0&1&1&0\\
1&0&0&-1\\
1&0&0&-1\\
0&-1&-1&0
\end{array}
\right)
}

\AddEq[1]{f=...ei o ek}
{
#1=\aU {#1}{ij}\aD ei\otimes\aD ej
}

\AddEquation{fg=...ei o ek}
{
f\circ g=\aU {(f\circ g)}{pq}\aD ep\otimes\aD eq
}

\AddEquation{fg=CCfg}
{
\aU {(f\circ g)}{pq}=\aU f{ij}\aU g{kl}\aUD Cp{ik}\aUD Cq{lj}
}

\AddEquation{fg=...e o e}
{
f\circ g=\aU f{ij}\aU g{kl}(\aD ei\aD ek)\otimes(\aD el\aD ej)
}

\AddEquation{fg=...C e o e}
{
f\circ g=\aU f{ij}\aU g{kl}\aUD Cp{ik}\aUD Cq{lj}\aD ep\otimes\aD eq
}

\AddEq[2]{f in AoA}
{
$#1\in A\otimes A$#2
}

\AddEq[2]{texorpdf L(D;A->A)}
{%
\texorpdfstring{%
\ShowEq{L(A->B)}#1#2#2{}%
}{L(#1;#2->#2)}%
}

\AddEq{I0=E}
{
$\aU I0=E$.
}

\AddEquation{a > a bullet}
{
\xymatrix
{
\bullet:A\ar[r]|(.4){*}&
\ShowEq{L(A->B)}DAA
}
\ \ \ \ \ \,
a\bullet:f\rightarrow a\bullet f
}

\AddEq{coordinates of map A->A, 2}
{
\aUD fkl=\aU {f^{k\cdot}_{}{}}{ij}
\aUD {F_{k\cdot}^{}{}}ml
\aUD Cp{im}\aUD Ck{pj}
}

\AddEq [2]{coordinates of map A1 A2, FoG, associative algebra}
{
\def\Cdot{}
\def\Temp{-}%
\edef\Tempa{#2}%
\ifx\Tempa\Temp%
\else
\def\Cdot{#2\cdot}
\fi
#1^{\gik}_{\gil}=#1^{k\cdot\gi{ij}}
F_{k\cdot}^{}{}^{\gim}_{\gi r}G^{\gi r}_{\gil}
C_{\Cdot}{}^{\gi p}_{\gi{im}}C_{\Cdot}{}^{\gik}_{\gi{pj}}
}

\AddEq [2]{coordinates of map A->B}
{
\def\Cdot{}
\def\Temp{-}%
\edef\Tempa{#2}%
\ifx\Tempa\Temp%
\else
\def\Cdot{#2\cdot}
\fi
#1^{\gik}_{\gil}=#1^{k\cdot\gi{ij}}
F_{k\cdot}^{}{}^{\gim}_{\gi r}G^{\gi r}_{\gil}
C_{\Cdot}{}^{\gi p}_{\gi{im}}C_{\Cdot}{}^{\gik}_{\gi{pj}}
}

\AddEquation{a...= H}
{
\begin{split}
&\,
\ShowEq{matrix a algebra H}
\\ = &\,
\ShowEq{matrix af algebra H}
\ShowEq{matrix f algebra H}
\end{split}
}

\AddEquation{a0=f03}
{
\begin{split}
\aD a0&=\aUD a00+\aUD a10i+\aUD a20j+\aUD a30k
\\&=\frac 12
(-\aUD f00+\aUD f11+\aUD f22+\aUD f33
+(-\aUD f10-\aUD f01+\aUD f32-\aUD f23)i
\\&+(-\aUD f20-\aUD f31-\aUD f02+\aUD f13)j
+(-\aUD f30+\aUD f21-\aUD f12-\aUD f03)k)
\\&=\frac 12
((-\aUD f00-\aUD f10i-\aUD f20j-\aUD f30k)
+(-\aUD f01i+\aUD f11+\aUD f21k-\aUD f31j)
\\&+(-\aUD f02j-\aUD f12k+\aUD f22+\aUD f32i)
+(-\aUD f03k+\aUD f13j-\aUD f23i+\aUD f33))
\\&=\frac 12
(-(\aUD f00+\aUD f10i+\aUD f20j+\aUD f30k)
-(\aUD f01+\aUD f11i+\aUD f21j+\aUD f31k)i
\\&-(\aUD f02+\aUD f12i+\aUD f22j+\aUD f32k)j
-(\aUD f03+\aUD f13i+\aUD f23j+\aUD f33k)k)
\end{split}
}

\AddEquation{a1=f03}
{
\begin{split}
\aD a1&=\aUD a01+\aUD a11i+\aUD a21j+\aUD a31k
\\&=\frac 12
(\aUD f00-\aUD f11+(\aUD f10+\aUD f01)i+(\aUD f20+\aUD f31)j+(\aUD f30-\aUD f21)k)
\\&=\frac 12
((\aUD f00+\aUD f10i+\aUD f20j+\aUD f30k)+(\aUD f01i-\aUD f11-\aUD f21k+\aUD f31j))
\\&=\frac 12
((\aUD f00+\aUD f10i+\aUD f20j+\aUD f30k)+(\aUD f01+\aUD f11i+\aUD f21j+\aUD f31k)i)
\end{split}
}

\AddEquation{a2=f03}
{
\begin{split}
\aD a2&=\aUD a02+\aUD a12i+\aUD a22j+\aUD a32k
\\&=\frac 12
(\aUD f00-\aUD f22+(\aUD f10-\aUD f32)i+(\aUD f20+\aUD f02)j+(\aUD f30+\aUD f12)k)
\\&=\frac 12
(\aUD f00-\aUD f22+\aUD f10i-\aUD f32i+\aUD f20j+\aUD f02j+\aUD f30k+\aUD f12k)
\\&=\frac 12
((\aUD f00+\aUD f10i+\aUD f20j+\aUD f30k)+(\aUD f02j+\aUD f12k-\aUD f22-\aUD f32i))
\\&=\frac 12
((\aUD f00+\aUD f10i+\aUD f20j+\aUD f30k)+(\aUD f02+\aUD f12i+\aUD f22j+\aUD f32k)j)
\end{split}
}

\AddEquation{a3=f03}
{
\begin{split}
\aD a3&=\aUD a03+\aUD a13i+\aUD a23j+\aUD a33k
\\&=\frac 12
(\aUD f00-\aUD f33+(\aUD f10+\aUD f23)i+(\aUD f20-\aUD f13)j+(\aUD f30+\aUD f03)k)
\\&=\frac 12
((\aUD f00+\aUD f10i+\aUD f30k+\aUD f20j)+(\aUD f03k-\aUD f13j+\aUD f23i-\aUD f33))
\\&=\frac 12
((\aUD f00+\aUD f10i+\aUD f30k+\aUD f20j)+(\aUD f03+\aUD f13i+\aUD f23j+\aUD f33k)k)
\end{split}
}

\AddEq{a0=f07 1}
{
\begin{align*}
\aD a0&=\aUD a00\aD e0+\aUD a10\aD e1+\aUD a20\aD e2+\aUD a30\aD e3
+\aUD a40\aD e4+\aUD a50\aD e5+\aUD a60\aD e6+\aUD a70\aD e7
\\&=\frac 12
((-5\aUD f00+\aUD f11+\aUD f22+\aUD f33+\aUD f44+\aUD f55+\aUD f66+\aUD f77)\aD e0
\\&+(-5\aUD f10-\aUD f01+\aUD f32-\aUD f23+\aUD f54-\aUD f45-\aUD f76+\aUD f67)\aD e1
\\&+(-5\aUD f20-\aUD f31-\aUD f02+\aUD f13+\aUD f64+\aUD f75-\aUD f46-\aUD f57)\aD e2
\\&+(-5\aUD f30+\aUD f21-\aUD f12-\aUD f03+\aUD f74-\aUD f65+\aUD f56-\aUD f47)\aD e3
\\&+(-5\aUD f40-\aUD f51-\aUD f62-\aUD f73-\aUD f04+\aUD f15+\aUD f26+\aUD f37)\aD e4
\\&+(-5\aUD f50+\aUD f41-\aUD f72+\aUD f63-\aUD f14-\aUD f05-\aUD f36+\aUD f27)\aD e5
\\&+(-5\aUD f60+\aUD f71+\aUD f42-\aUD f53-\aUD f24+\aUD f35-\aUD f06-\aUD f17)\aD e6
\\&+(-5\aUD f70-\aUD f61+\aUD f52+\aUD f43-\aUD f34-\aUD f25+\aUD f16-\aUD f07)\aD e7)
\end{align*}
}

\AddEq{a0=f07 2}
{
\begin{align*}
\aD a0&=\frac 12
(-5\aUD f00\aD e0+\aUD f11\aD e0+\aUD f22\aD e0+\aUD f33\aD e0
+\aUD f44\aD e0+\aUD f55\aD e0+\aUD f66\aD e0+\aUD f77\aD e0
\\&-5\aUD f10\aD e1-\aUD f01\aD e1+\aUD f32\aD e1-\aUD f23\aD e1
+\aUD f54\aD e1-\aUD f45\aD e1-\aUD f76\aD e1+\aUD f67\aD e1
\\&-5\aUD f20\aD e2-\aUD f31\aD e2-\aUD f02\aD e2+\aUD f13\aD e2
+\aUD f64\aD e2+\aUD f75\aD e2-\aUD f46\aD e2-\aUD f57\aD e2
\\&-5\aUD f30\aD e3+\aUD f21\aD e3-\aUD f12\aD e3-\aUD f03\aD e3
+\aUD f74\aD e3-\aUD f65\aD e3+\aUD f56\aD e3-\aUD f47\aD e3
\\&-5\aUD f40\aD e4-\aUD f51\aD e4-\aUD f62\aD e4-\aUD f73\aD e4
-\aUD f04\aD e4+\aUD f15\aD e4+\aUD f26\aD e4+\aUD f37\aD e4
\\&-5\aUD f50\aD e5+\aUD f41\aD e5-\aUD f72\aD e5+\aUD f63\aD e5
-\aUD f14\aD e5-\aUD f05\aD e5-\aUD f36\aD e5+\aUD f27\aD e5
\\&-5\aUD f60\aD e6+\aUD f71\aD e6+\aUD f42\aD e6-\aUD f53\aD e6
-\aUD f24\aD e6+\aUD f35\aD e6-\aUD f06\aD e6-\aUD f17\aD e6
\\&-5\aUD f70\aD e7-\aUD f61\aD e7+\aUD f52\aD e7+\aUD f43\aD e7
-\aUD f34\aD e7-\aUD f25\aD e7+\aUD f16\aD e7-\aUD f07\aD e7)
\end{align*}
}

\AddEq{a0=f07 3}
{
\begin{align*}
\aD a0&=\frac 12
(-5(\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3
+\aUD f40\aD e4+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\&+(-\aUD f01\aD e1+\aUD f11\aD e0+\aUD f21\aD e3-\aUD f31\aD e2
+\aUD f41\aD e5-\aUD f51\aD e4-\aUD f61\aD e7+\aUD f71\aD e6)
\\&+(-\aUD f02\aD e2-\aUD f12\aD e3+\aUD f22\aD e0+\aUD f32\aD e1
+\aUD f42\aD e6+\aUD f52\aD e7-\aUD f62\aD e4-\aUD f72\aD e5)
\\&+(-\aUD f03\aD e3+\aUD f13\aD e2-\aUD f23\aD e1+\aUD f33\aD e0
+\aUD f43\aD e7-\aUD f53\aD e6+\aUD f63\aD e5-\aUD f73\aD e4)
\\&+(-\aUD f04\aD e4-\aUD f14\aD e5-\aUD f24\aD e6-\aUD f34\aD e7
+\aUD f44\aD e0+\aUD f54\aD e1+\aUD f64\aD e2+\aUD f74\aD e3)
\\&+(-\aUD f05\aD e5+\aUD f15\aD e4-\aUD f25\aD e7+\aUD f35\aD e6
-\aUD f45\aD e1+\aUD f55\aD e0-\aUD f65\aD e3+\aUD f75\aD e2)
\\&+(-\aUD f06\aD e6+\aUD f16\aD e7+\aUD f26\aD e4-\aUD f36\aD e5
-\aUD f46\aD e2+\aUD f56\aD e3+\aUD f66\aD e0-\aUD f76\aD e1)
\\&+(-\aUD f07\aD e7-\aUD f17\aD e6+\aUD f27\aD e5+\aUD f37\aD e4
-\aUD f47\aD e3-\aUD f57\aD e2+\aUD f67\aD e1+\aUD f77\aD e0)
\end{align*}
}

\AddEquation{a0=f07}
{
\begin{split}
\aD a0&=-\frac 12
(5(\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3
+\aUD f40\aD e4+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)\aD e0
\\&+(\aUD f01\aD e0+\aUD f11\aD e0+\aUD f21\aD e2+\aUD f31\aD e3
+\aUD f41\aD e4+\aUD f51\aD e5+\aUD f61\aD e6+\aUD f71\aD e7)\aD e1
\\&+(\aUD f02\aD e0+\aUD f12\aD e1+\aUD f22\aD e2+\aUD f32\aD e3
+\aUD f42\aD e4+\aUD f52\aD e5+\aUD f62\aD e6+\aUD f72\aD e7)\aD e2
\\&+(\aUD f03\aD e0+\aUD f13\aD e2+\aUD f23\aD e2+\aUD f33\aD e0
+\aUD f43\aD e4+\aUD f53\aD e5+\aUD f63\aD e6+\aUD f73\aD e7)\aD e3
\\&+(\aUD f04\aD e0+\aUD f14\aD e1+\aUD f24\aD e2+\aUD f34\aD e3
+\aUD f44\aD e4+\aUD f54\aD e5+\aUD f64\aD e6+\aUD f74\aD e7)\aD e4
\\&+(\aUD f05\aD e0+\aUD f15\aD e1+\aUD f25\aD e2+\aUD f35\aD e3
+\aUD f45\aD e4+\aUD f55\aD e5+\aUD f65\aD e3+\aUD f75\aD e7)\aD e5
\\&+(\aUD f06\aD e6+\aUD f16\aD e1+\aUD f26\aD e2+\aUD f36\aD e3
+\aUD f46\aD e4+\aUD f56\aD e5+\aUD f66\aD e6+\aUD f76\aD e7)\aD e6
\\&+(\aUD f07\aD e0+\aUD f17\aD e1+\aUD f27\aD e2+\aUD f37\aD e3
+\aUD f47\aD e4+\aUD f57\aD e5+\aUD f67\aD e6+\aUD f77\aD e7)\aD e7
\end{split}
}

\AddEquation{a1=f07}
{
\begin{split}
\aD a1&=\aUD a01\aD e0+\aUD a11\aD e1+\aUD a21\aD e2+\aUD a31\aD e3
+\aUD a41\aD e4+\aUD a51\aD e5+\aUD a61\aD e6+\aUD a71\aD e7
\\&=\frac 12
((\aUD f00-\aUD f11)\aD e0+(\aUD f10+\aUD f01)\aD e1
+(\aUD f20+\aUD f31)\aD e2+(\aUD f30-\aUD f21)\aD e3
\\ &
+(\aUD f40+\aUD f51)\aD e4+(\aUD f50-\aUD f41)\aD e5
+(\aUD f60-\aUD f71)\aD e6+(\aUD f70+\aUD f61)\aD e7)
\\&=\frac 12
(\aUD f00\aD e0-\aUD f11\aD e0+\aUD f10\aD e1+\aUD f01\aD e1
+\aUD f20\aD e2+\aUD f31\aD e2+\aUD f30\aD e3-\aUD f21\aD e3
\\ &
+\aUD f40\aD e4+\aUD f51\aD e4+\aUD f50\aD e5-\aUD f41\aD e5
+\aUD f60\aD e6-\aUD f71\aD e6+\aUD f70\aD e7+\aUD f61\aD e7)
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f01\aD e1-\aUD f11\aD e0-\aUD f21\aD e3+\aUD f31\aD e2
-\aUD f41\aD e5+\aUD f51\aD e4+\aUD f61\aD e7-\aUD f71\aD e6))
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f01\aD e0+\aUD f11\aD e1+\aUD f21\aD e2+\aUD f31\aD e3
+\aUD f41\aD e4+\aUD f51\aD e5+\aUD f61\aD e6+\aUD f71\aD e7)\aD e1)
\end{split}
}

\AddEquation{a2=f07}
{
\begin{split}
\aD a2&=\aUD a02\aD e0+\aUD a12\aD e1+\aUD a22\aD e2+\aUD a32\aD e3
+\aUD a42\aD e4+\aUD a52\aD e5+\aUD a62\aD e6+\aUD a72\aD e7
\\&=\frac 12
((\aUD f00-\aUD f22)\aD e0+(\aUD f10-\aUD f32)\aD e1
+(\aUD f20+\aUD f02)\aD e2+(\aUD f30+\aUD f12)\aD e3
\\ &
+(\aUD f40+\aUD f62)\aD e4+(\aUD f50+\aUD f72)\aD e5
+(\aUD f60-\aUD f42)\aD e6+(\aUD f70-\aUD f52)\aD e7)
\\&=\frac 12
(\aUD f00\aD e0-\aUD f22\aD e0+\aUD f10\aD e1-\aUD f32\aD e1
+\aUD f20\aD e2+\aUD f02\aD e2+\aUD f30\aD e3+\aUD f12\aD e3
\\ &
+\aUD f40\aD e4+\aUD f62\aD e4+\aUD f50\aD e5+\aUD f72\aD e5
+\aUD f60\aD e6-\aUD f42\aD e6+\aUD f70\aD e7-\aUD f52\aD e7)
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f02\aD e2+\aUD f12\aD e3-\aUD f32\aD e1-\aUD f22\aD e0
-\aUD f42\aD e6-\aUD f52\aD e7+\aUD f62\aD e4+\aUD f72\aD e5))
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f02\aD e0+\aUD f12\aD e1+\aUD f22\aD e2+\aUD f32\aD e3
+\aUD f42\aD e4+\aUD f52\aD e5+\aUD f62\aD e6+\aUD f72\aD e7)\aD e2)
\end{split}
}

\AddEquation{a3=f07}
{
\begin{split}
\aD a3&=\aUD a03\aD e0+\aUD a13\aD e1+\aUD a23\aD e2+\aUD a33\aD e3
+\aUD a43\aD e4+\aUD a53\aD e5+\aUD a63\aD e6+\aUD a73\aD e7
\\&=\frac 12
((\aUD f00-\aUD f33)\aD e0+(\aUD f10+\aUD f23)\aD e1
+(\aUD f20-\aUD f13)\aD e2+(\aUD f30+\aUD f03)\aD e3
\\ &
+(\aUD f40+\aUD f73)\aD e4+(\aUD f50-\aUD f63)\aD e5
+(\aUD f60+\aUD f53)\aD e6+(\aUD f70-\aUD f43)\aD e7)
\\&=\frac 12
(\aUD f00\aD e0-\aUD f33\aD e0+\aUD f10\aD e1+\aUD f23\aD e1
+\aUD f20\aD e2-\aUD f13\aD e2+\aUD f30\aD e3+\aUD f03\aD e3
\\ &
+\aUD f40\aD e4+\aUD f73\aD e4+\aUD f50\aD e5-\aUD f63\aD e5
+\aUD f60\aD e6+\aUD f53\aD e6+\aUD f70\aD e7-\aUD f43\aD e7)
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f03\aD e3-\aUD f13\aD e2+\aUD f23\aD e1-\aUD f33\aD e0
-\aUD f43\aD e7+\aUD f53\aD e6-\aUD f63\aD e5+\aUD f73\aD e4))
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f03\aD e0+\aUD f13\aD e1+\aUD f23\aD e2+\aUD f33\aD e3
+\aUD f43\aD e4+\aUD f53\aD e5+\aUD f63\aD e6+\aUD f73\aD e7)\aD e3)
\end{split}
}

\AddEquation{a4=f07}
{
\begin{split}
\aD a4&=\aUD a04\aD e0+\aUD a14\aD e1+\aUD a24\aD e2+\aUD a34\aD e3
+\aUD a44\aD e4+\aUD a54\aD e5+\aUD a64\aD e6+\aUD a74\aD e7
\\&=\frac 12
((\aUD f00-\aUD f44)\aD e0+(\aUD f10-\aUD f54)\aD e1
+(\aUD f20-\aUD f64)\aD e2+(\aUD f30-\aUD f74\aD e3
\\ &
+(\aUD f40+\aUD f04)\aD e4+(\aUD f50+\aUD f14)\aD e5
+(\aUD f60+\aUD f24)\aD e6+(\aUD f70+\aUD f34)\aD e7)
\\&=\frac 12
(\aUD f00\aD e0-\aUD f44\aD e0+\aUD f10\aD e1-\aUD f54\aD e1
+\aUD f20\aD e2-\aUD f64\aD e2+\aUD f30\aD e3-\aUD f74\aD e3
\\ &
+\aUD f40\aD e4+\aUD f04\aD e4+\aUD f50\aD e5+\aUD f14\aD e5
+\aUD f60\aD e6+\aUD f24\aD e6+\aUD f70\aD e7+\aUD f34\aD e7)
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f04\aD e4+\aUD f14\aD e5+\aUD f24\aD e6+\aUD f34\aD e7
-\aUD f44\aD e0-\aUD f54\aD e1-\aUD f64\aD e2-\aUD f74\aD e3))
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f04\aD e0+\aUD f14\aD e1+\aUD f24\aD e2+\aUD f34\aD e3
+\aUD f44\aD e4+\aUD f54\aD e5+\aUD f64\aD e6+\aUD f74\aD e7)\aD e4)
\end{split}
}

\AddEquation{a5=f07}
{
\begin{split}
\aD a5&=\aUD a05\aD e0+\aUD a15\aD e1+\aUD a25\aD e2+\aUD a35\aD e3
+\aUD a45\aD e4+\aUD a55\aD e5+\aUD a65\aD e6+\aUD a75\aD e7
\\&=\frac 12
((\aUD f00-\aUD f55)\aD e0+(\aUD f10+\aUD f45)\aD e1
+(\aUD f20-\aUD f75)\aD e2+(\aUD f30+\aUD f65)\aD e3
\\ &
+(\aUD f40-\aUD f15)\aD e4+(\aUD f50+\aUD f05)\aD e5
+(\aUD f60-\aUD f35)\aD e6+(\aUD f70+\aUD f25)\aD e7)
\\&=\frac 12
(\aUD f00\aD e0-\aUD f55\aD e0+\aUD f10\aD e1+\aUD f45\aD e1
+\aUD f20\aD e2-\aUD f75\aD e2+\aUD f30\aD e3+\aUD f65\aD e3
\\ &
+\aUD f40\aD e4-\aUD f15\aD e4+\aUD f50\aD e5+\aUD f05\aD e5
+\aUD f60\aD e6-\aUD f35\aD e6+\aUD f70\aD e7+\aUD f25\aD e7)
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f05\aD e5-\aUD f15\aD e4+\aUD f25\aD e7-\aUD f35\aD e6
+\aUD f45\aD e1-\aUD f55\aD e0+\aUD f65\aD e3-\aUD f75\aD e2))
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f05\aD e0+\aUD f15\aD e1+\aUD f25\aD e2+\aUD f35\aD e3
+\aUD f45\aD e4+\aUD f55\aD e5+\aUD f65\aD e6+\aUD f75\aD e7)\aD e5)
\end{split}
}

\AddEquation{a6=f07}
{
\begin{split}
\aD a6&=\aUD a06\aD e0+\aUD a16\aD e1+\aUD a26\aD e2+\aUD a36\aD e3
+\aUD a46\aD e4+\aUD a56\aD e5+\aUD a66\aD e6+\aUD a76\aD e7
\\&=\frac 12
((\aUD f00-\aUD f66)\aD e0+(\aUD f10+\aUD f76)\aD e1
+(\aUD f20+\aUD f46)\aD e2+(\aUD f30-\aUD f56\aD e3
\\ &
+(\aUD f40-\aUD f26)\aD e4+(\aUD f50+\aUD f36)\aD e5
+(\aUD f60+\aUD f06)\aD e6+(\aUD f70-\aUD f16)\aD e7)
\\&=\frac 12
(\aUD f00\aD e0-\aUD f66\aD e0+\aUD f10\aD e1+\aUD f76\aD e1
+\aUD f20\aD e2+\aUD f46\aD e2+\aUD f30\aD e3-\aUD f56\aD e3
\\ &
+\aUD f40\aD e4-\aUD f26\aD e4+\aUD f50\aD e5+\aUD f36\aD e5
+\aUD f60\aD e6+\aUD f06\aD e6+\aUD f70\aD e7-\aUD f16\aD e7)
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f06\aD e6-\aUD f16\aD e7-\aUD f26\aD e4+\aUD f36\aD e5
+\aUD f46\aD e2-\aUD f56\aD e3-\aUD f66\aD e0+\aUD f76\aD e1))
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f06\aD e0+\aUD f16\aD e1+\aUD f26\aD e2+\aUD f36\aD e3
+\aUD f46\aD e4+\aUD f56\aD e5+\aUD f66\aD e6+\aUD f76\aD e7)\aD e6)
\end{split}
}

\AddEquation{a7=f07}
{
\begin{split}
\aD a7&=\aUD a07\aD e0+\aUD a17\aD e1+\aUD a27\aD e2+\aUD a37\aD e3
+\aUD a47\aD e4+\aUD a57\aD e5+\aUD a67\aD e6+\aUD a77\aD e7
\\&=\frac 12
((\aUD f00-\aUD f77)\aD e0+(\aUD f10-\aUD f67)\aD e1
+(\aUD f20+\aUD f57)\aD e2+(\aUD f30+\aUD f47)\aD e3
\\ &
+(\aUD f40-\aUD f37)\aD e4+(\aUD f50-\aUD f27)\aD e5
+(\aUD f60+\aUD f17)\aD e6+(\aUD f70+\aUD f07)\aD e7)
\\&=\frac 12
(\aUD f00\aD e0-\aUD f77\aD e0+\aUD f10\aD e1-\aUD f67\aD e1
+\aUD f20\aD e2+\aUD f57\aD e2+\aUD f30\aD e3+\aUD f47\aD e3
\\ &
+\aUD f40\aD e4-\aUD f37\aD e4+\aUD f50\aD e5-\aUD f27\aD e5
+\aUD f60\aD e6+\aUD f17\aD e6+\aUD f70\aD e7+\aUD f07\aD e7)
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f07\aD e7+\aUD f17\aD e6-\aUD f27\aD e5-\aUD f37\aD e4
+\aUD f47\aD e3+\aUD f57\aD e2-\aUD f67\aD e1-\aUD f77\aD e0))
\\&=\frac 12
((\aUD f00\aD e0+\aUD f10\aD e1+\aUD f20\aD e2+\aUD f30\aD e3+\aUD f40\aD e4
+\aUD f50\aD e5+\aUD f60\aD e6+\aUD f70\aD e7)
\\ &
+(\aUD f07\aD e7+\aUD f17\aD e1+\aUD f27\aD e2+\aUD f37\aD e4
+\aUD f61\aD e6+\aUD f47\aD e4+\aUD f57\aD e5+\aUD f77\aD e7)\aD e7)
\end{split}
}

\AddEq{a0=f0.7}
{
\ShowEq{a0=f07 1}
\ShowEq{a0=f07 2}
\ShowEq{a0=f07 3}
\ShowEq{a0=f07}
\ShowEq{a1=f07}
\ShowEq{a2=f07}
\ShowEq{a3=f07}
\ShowEq{a4=f07}
\ShowEq{a5=f07}
\ShowEq{a6=f07}
\ShowEq{a7=f07}
}

\AddEquation{f=.E+.I+.J+.K}
{
\begin{split}
f=&-\frac 12
\left(
\aD f0
+\aD f1i
+\aD f2j
+\aD f3k
\right)\bullet E
\\&
+\frac 12\left(
\aD f0
+\aD f1i
\right)\bullet\aU I1
+\frac 12\left(
\aD f0
+\aD f2j
\right)\bullet\aU I2
%\\&
+\frac 12\left(
\aD f0
+\aD f3k
\right)\bullet\aU I3
\end{split}
}

\AddEq[2]{ab=a*(.E+.I+.J+.K)b}
{
#1 #2=
(#2^*\bullet E+(i#2^*)\bullet\aU I1+(j#2^*)\bullet\aU I2+(k#2^*)\bullet\aU I3)\circ #1
}

\AddEquation{f=.I0.7}
{
\begin{split}
f=&-\frac 12
\left(
5\aD f0+\aD f1i+\aD f2j+\aD f3k
\aD f4l+\aD f5il+\aD f6jl+\aD f7kl
\right)\circ E
\\&
+\frac 12\left(
\aD f0+\aD f1i
\right)\circ\aU I1
+\frac 12\left(
\aD f0+\aD f2j
\right)\circ\aU I2
+\frac 12\left(
\aD f0+\aD f3k
\right)\circ\aU I3
\\&
+\frac 12\left(
\aD f0+\aD f4l
\right)\circ\aU I4
+\frac 12\left(
\aD f0+\aD f5il
\right)\circ\aU I5
+\frac 12\left(
\aD f0+\aD f6jl
\right)\circ\aU I6
\\&
+\frac 12\left(
\aD f0+\aD f7kl
\right)\circ\aU I7
\end{split}
}

\AddEquation{a...= O}
{
\begin{split}
&\,
\ShowEq{matrix a algebra O}
\\ = &\,
\ShowEq{matrix af algebra O}
\\ * &\,
\ShowEq{matrix f algebra O}
\end{split}
}

\AddEq [2]{I=(E,I)}
{
\def\Set{\aU I1,\aU I2,\aU I3}
\def\Temp{O}%
\edef\Tempa{#1}%
\ifx\Tempa\Temp%
\def\Set{\aU Ii,\gi i=\gi 1,...,\gi 7}
\fi
$\Basis I=(E,\Set)$#2
}

\AddEq{F o G}
{
\Basis F\circ G=\{F_k\circ G:F_k\in \Basis F\}
}

\AddEq{FijG}
{
$F_i\circ G$, \iI,
}

\AddEquation{coordinates of map Fk, associative algebra}
{
F_k\circ x=\aUD {F_{k\cdot}^{}{}}ij\aU xj\aD ei
}

\AddEq [1]{linear map over ring, determinant=0, 1}
{
\[
\rank
\begin{pmatrix}
\mathcal C^{\cdot}{}_{\gim}^{\gik}{}_{\cdot\gi{ij}}
&#1_{\gim}^{\gik}
\end{pmatrix}
=\rank\mathcal C
\]
}

\AddEq[1]{linear map over ring, matrix}
{
\def\Cdot{}
\def\Temp{-}%
\edef\Tempa{#1}%
\ifx\Tempa\Temp%
\else
\def\Cdot{#1\cdot}
\fi
\mathcal C=
\left(
\mathcal C^{\cdot}{}_{\gim}^{\gik}{}_{\cdot\gi{ij}}
\right)
=
\left(
C_{\Cdot}{}^{\gi p}_{\gi{im}}C_{\Cdot}{}^{\gik}_{\gi{pj}}
\right)
}

\AddEq{linear map over ring, row of matrix}
{
${}^{\cdot}{}_{\gim}^{\gik}$
}

\AddEq{linear map over ring, column of matrix}
{
${}_{\cdot\gi{ij}}$
}

\AddEquation{coordinates of map f, associative algebra}
{
f\circ x=\aUD fij\aU xj\aD ei
}

\DefEq
{
\[
\Basis F=\{F_k\in\mathcal L(D;A_1\rightarrow A_2): k=1, ..., n\}
\]
}
{Ik 1n}

\AddEquation{h generated by f, associative algebra}
{
h=
(
a\pC{s}{0}
\otimes
a\pC{s}{1}
)
\circ f
=a\pC{s}{0}
f
a\pC{s}{1}
}

\DefEq
{
\[
h:A_1\rightarrow A_2
\]
}
{h:A1->A2}

\AddEquation{f in L(A,A), 1, associative algebra}
{
f=
(
a_{k\cdot s_k\cdot 0}
\otimes
a_{k\cdot s_k\cdot 1}
)
\circ I_k
=
\sum_{\gik}
a_{k\cdot s_k\cdot 0}
I_k
a_{k\cdot s_k\cdot 1}
}

\DefEq
{
\[
f\in B^A\rightarrow \|f\|\in R
\]
}
{f in BA->|f|}

\AddEq{norm of map}
{
\symb{\|f\|}{norm of map}{}
}

\DefEquation
{
\ShowSymbol{norm of map}{}=
\text{sup}\frac{\|f(x)\|_B}{\|x\|_A}
}
{norm of map, algebra}

\DefEq
{
$\ShowSymbol{norm of map}{}$
}
{show|f|}

\DefEq
{
\symb{f+g}{sum of maps}{polylinear}
}
{sum of maps,,polylinear}

\DefEquation
{
\begin{matrix}
\ShowSymbol{sum of maps}{polylinear}:A_1\times...\times A_n\rightarrow S
&f,g\in\mathcal L(D;A_1\times...\times A_n\rightarrow S)
\end{matrix}
}
{sum of maps, 1, polylinear}

\AddEq{f=fkxfk}
{
f^k=f^k_{s_k\cdot 0}\otimes f^k_{s_k\cdot 1}
}

\AddEq [1]{expansion of linear map with respect to basis}
{
f=f^k\circ I_k\ \ \ f^k\in #1\otimes #1
}

\DefEquation
{
(\ShowSymbol{sum of maps}{polylinear})\circ (a_1,...,a_n)
=f\circ (a_1,...,a_n)+g\circ (a_1,...,a_n)
}
{sum of  maps, polylinear}

\AddEq{module of polylinear maps}
{
$\mathcal L(D;A_1\times...\times A_n\rightarrow S)$
}

\AddEquation{dg h12 xox}
{
dg=(h_2h_1-h_1h_2)x+x(h_1h_2-h_2h_1)
}

\AddEquation{a0=}
{
\aD a0=-\frac 12(\aD f0+\aD f1i+\aD f2j+\aD f3k)
}

\AddEquation{a1=}
{
a_1=\frac 12(\aD f0+\aD f1i)
}

\AddEquation{a2=}
{
\aD a2=\frac 12(\aD f0+\aD f2j)
}

\AddEquation{a3=}
{
\aD a3=\frac 12(\aD f0+\aD f3k)
}

\AddEq[3]{set linear maps, module}
{
\symb{\mathcal L(#1;#2\rightarrow #3)}{set linear maps}1
}

\AddEq[2]{set linear maps, module (1)}
{
\symb{\mathcal L(#1;#2_1\rightarrow #2_2)}{set linear maps}1
}

\AddEq[2]{set linear maps, module (11)}
{
\symb{\mathcal L(#1_1\rightarrow #1_2;#2_1\rightarrow #2_2)}{set linear maps}1
}

\AddEq{set homomorphisms, D algebra}
{
\symb{\Hom(D;A_1\rightarrow A_2)}{set of homomorphisms}1
}

\AddEquation{Am->A(n+m) 1}
{
(p\circ x^n)\circ (q\circ x^m)=(p\underline{\otimes}q)\circ x^{n+m}
}

\AddEq[1]{d->dei}
{
\[
\aD P#1:d\in D\rightarrow d\aD e#1\in A
\]
}

\AddEq{f(t)=fit ei}
{
\[
f\circ t=(\aU fit)\aD ei=\aD Pi\circ(\aU fit)
\]
}

\AddEq{map f, 1, tensor product}
{
\[
f:A_1\times...\times A_n\rightarrow\Tensor A
\]
}

\AddEq{tensor product of modules}
{
\symb{\Tensor A}{tensor product}{}
}

\AddEq{f:xA->oxA}
{
\[f:A_1\times...\times A_n\rightarrow\ShowSymbol{tensor product}{}\]
}

\AddEquation{map f, tensor product}
{
f\circ(d_1,...,d_n)=\Tensor d
}

\AddEq{map g, tensor product}
{
\[
g:A_1\times...\times A_n\rightarrow V
\]
}

\AddEq{map h, tensor product}
{
\[
h:\Tensor A\rightarrow V
\]
}

\AddEquation{map gh, tensor product}
{
\xymatrix{
&\Tensor A\ar[dd]^h
\\
\Times
\ar[ru]^f\ar[rd]_g
\\
&V
}
}

\AddEquation{g=h, tensor product}
{
h\circ(\Tensor a)=g\circ(a_1,...,a_n)
}

\AddEq{fxa=oxa}
{
\[f\circ(a_1,...,a_n)=\Tensor a\]
}

\AddEq[2]{polylinear map of algebras, 1}
{
\[
\begin{matrix}
1\le i\le n
&
a_i, b_i \in #1
&
p\in #2
\end{matrix}
\]
}

\AddEq{aE+bE=(a+b)E}
{
\[(aE)\circ x+(bE)\circ x=ax+bx=(a+b)x=((a+b)E)\circ x\]
}

\AddEq{aE o bE=(ab)E}
{
\[(aE)\circ (bE)\circ x=(aE)\circ (bx)=a(bx)=(ab)x=((ab)E)\circ x\]
}

\AddEq{g=gE}
{
\[g(x)=g^k(x)\circ E_k\ \ \ \ g^k:A\rightarrow B\]
}

\AddEq{linear map times constant, algebra}
{
$a\circ f$, $b\star f$, $a$, $b\in A_2$,
}

\AddEq{linear map times constant, 0, algebra}
{
\begin{align*}
(a\circ f)\circ x&=a(f\circ x)
\\
(b\star f)\circ x&=(f\circ x)b
\end{align*}
}

\AddEq{linear map AA LAA}
{
\[
h:\ATwo\rightarrow \mathcal L(D;A_1\rightarrow A_2)
\]
}

\AddEquation{linear map AA LAA, 1}
{
(a\otimes b)\circ f=b\star (a\circ f)
}

\AddEq{linear map AA LAA, 2}
{
\[
((a\otimes b)\circ f)\circ x=a(f\circ x)b
\]
}

\AddEq{f circ a =}
{
f\circ a=f(a)
}

\AddEq [5]{matrix AIJ}
{
\[
#1=(#1^{\gi #2}_{\gi #4},\gi #2\in\gi #3,\gi #4\in\gi #5)
\]
}

\AddEq{d12 in D}
{
\(d_1\), \(d_2\in D\).
}

\AddEquation{d1 d2 in A}
{
(d_11_A)(d_21_A)=d_1(1_A(d_21_A))=d_1(d_2(1_A1_A))
=d_1(d_21_A)=(d_1d_2)1_A
}

\AddEquation{ad=da in A}
{
a(d1_A)=d(a1_A)=d(1_Aa)=(d1_A)a
}

\AddEquation{d1+d2 in A}
{
d_11_A+d_21_A=(d_1+d_2)1_A
}

\AddEq{fi(dx)=}
{
\[
f_i(dx_i)=df_i(x_i)
\]
}

\AddEq{f(dx)i=}
{
\begin{align*}
f((dx_i,i\in I))&=
\sum_{i\in I}f_i(dx_i)=
\sum_{i\in I}df_i(x_i)
=d\sum_{i\in I}f_i(x_i)
\\&=df((x_i,i\in I))
\end{align*}
}

\AddEquation{linear map, f a+b=}
{
f\circ(a+b)=f\circ a+f\circ b
}

\AddEquation{linear map, f pa=}
{
f\circ(pa)=p(f\circ a)
}

\AddEq [1]{ab V p D}
{
\[
\begin{matrix}
a,b\in #1
&
p\in D
\end{matrix}
\]
}

\AddEq[3]{homomorphism, f v+w=}
{
#1\circ(#2+#3)=#1\circ #2+#1\circ #3
}

\AddEq[3]{homomorphism, f vw=}
{
#1\circ(#2#3)=(#1\circ #2)(#1\circ #3)
}

\AddEq[3]{homomorphism, f(p+q)=}
{
#1(#2+#3)=#1(#2)+#1(#3)
}

\AddEq[3]{homomorphism, f(pq)=}
{
#1(#2#3)=#1(#2)#1(#3)
}

\AddEquation{left linear map, f dv=}
{
f\circ(dv)=d(f\circ v)
}

\AddEquation{right linear map, f dv=}
{
f\circ(vd)=(f\circ v)d
}

\AddEq[4]{left homomorphism, f av=}
{
#1\circ(#2#4)=#3(#1\circ #4)
}

\AddEq[4]{right homomorphism, f av=}
{
#1\circ(#4#2)=(#1\circ #4)#3
}

\AddEq{D1 D2 ab in A, d in D}
{
\[
\begin{matrix}
a,b\in \Module_{\VF}
&d,d_1,d_2\in \Base_{\DF}
\end{matrix}
\]
}

\AddEq{D1 D2 uv in V, ab in A, d in D}
{
\[
\begin{matrix}
u,v\in V_1
&a,b\in A_1
&d,d_1,d_2\in D_1
\end{matrix}
\]
}

\AddEq[2]{D ab in A, d in D}
{
\[
\begin{matrix}
a,b\in #2
&
d\in #1
\end{matrix}
\]
}

\AddEq{ap AD 11}
{
\[
p,q\in D_1
\ \ \ \,
a,b\in A_1
\]
}

\AddEq{ap AD 1}
{
\[
p\in D
\ \ \ \,
a,b\in A_1
\]
}

\AddEq{vp VD 11}
{
\[
p,q\in D_1
\ \ \ \,
v,w\in V_1
\]
}

\AddEq{vp VD 1}
{
\[
p\in D
\ \ \ \,
v,w\in V_1
\]
}

\AddEq{vap VAD 111}
{
\[
p,q\in D_1
\ \ \ \,
a,b\in A_1
\ \ \ \,
u,v\in V_1
\]
}

\AddEq{vap VAD 11}
{
\[
p\in D
\ \ \ \,
a,b\in A_1
\ \ \ \,
u,v\in V_1
\]
}

\AddEq{vap VAD 1}
{
\[
a\in A
\ \ \ \,
u,v\in V_1
\]
}

\AddEq{commutator of algebra}
{
\symb{[a,b]}{commutator of algebra}{}
\[
\ShowSymbol{commutator of algebra}{}=ab-ba
\]
}

\AddEq{commutative D algebra}
{
\[
[a,b]=0
\]
}

\AddEquation{associator of algebra =}
{
\ShowSymbol{associator of algebra}{}=(ab)c-a(bc)
}

\AddEquation{associator of algebra = Ae}
{
\begin{split}
(a,b,c)&=(\aUD Ck{pl}(ab)^{\gi p}c^{\gil}-\aUD Ck{ip}a^{\gii}(bc)^{\gi p})e_{\gik}
\\
&=(\aUD Ck{pl}\aUD Cp{ij}-\aUD Ck{ip}\aUD Cp{jl})a^{\gii}b^{\gij}c^{\gil}e_{\gik}
\end{split}
}

\AddEq{associator of algebra}
{
\symb{(a,b,c)}{associator of algebra}{}
}

\AddEquation{associator of algebra = A}
{
(a,b,c)=A^{\gi k}_{\gi{ijl}}a^{\gii}b^{\gij}c^{\gil}e_{\gik}
}

\AddEq{coordinates of associator}
{
\symb{A^{\gi k}_{\gi{ijl}}}{coordinates of associator}{}
}

\AddEquation{coordinates of associator =}
{
\ShowSymbol{coordinates of associator}{}=
\aUD Ck{pl}\aUD Cp{ij}-\aUD Ck{ip}\aUD Cp{jl}
}

\AddEq{associative D algebra}
{
\[
(a,b,c)=0
\]
}

\AddEq{nucleus of algebra}
{
\symb{N(A)}{nucleus of algebra}{}
\[
\ShowSymbol{nucleus of algebra}{}=
\{
a\in A:
\forall b, c\in A,
(a,b,c)=(b,a,c)=(b,c,a)=0
\}
\]
}

\AddEq{center of algebra}
{
\symb{Z(A)}{center of algebra}{}
\[
\ShowSymbol{center of algebra}{}=
\{
a\in A:
a\in N(A),
\forall b\in A,
ab=ba
\}
\]
}

\AddEq[3]{f(a+b)=...}
{
#1\circ(#2+#3)=#1\circ #2+#1\circ #3
}

\DefEq
{
\[\Vector r_2:A_1\rightarrow A_2\]
}
{r2:A1->A2}

\AddEq{property linear map hf}
{
\DrawEq{h(d1+d2)=...}{\SideWS module}
\DrawEq{h(d1d2)=...}{\SideWS module}
\DrawEq[fab]{f(a+b)=...}{\DFDT \SideWS module}
\DrawEq[hfa]{f(da)=h... \SideWS module}{\DFDT \SideWS module}
\ShowEq{D1 D2 ab in A, d in D}
}

\AddEq{property linear map hgf}
{
\DrawEq{h(d1+d2)=...}{\SideWS module}
\DrawEq{h(d1d2)=...}{\SideWS module}
\DrawEq[gab]{f(a+b)=...}{g \DFDT \SideWS module}
\DrawEq[hga]{f(da)=h... \SideWS module}{g \DFDT}
\DrawEq[fuv]{f(a+b)=...}{f \DFDT \SideWS module}
\DrawEq[hfu]{f(da)=h... \SideWS module}{f \DFDT}
\ShowEq{D1 D2 uv in V, ab in A, d in D}
}

\AddEq[2]{show linear map hgf}
{
\[
\begin{pmatrix}
h:D_1\rightarrow D_2&
#1:A_1\rightarrow A_2&
#2:V_1\rightarrow V_2
\end{pmatrix}
\]
}

\AddEq[2]{show linear map hf}
{
\ShowEq{h:D1->D2 f:A1->A2}{#1} \Base {#2} \Module
}

\AddEq[2]{show linear map f}
{
\ShowEq{f:A->B}{#2}{\Module_1}{\Module_2}
}

\AddEq [3]{V=o+Ae}
{
\[
V_{#1}=\bigoplus_{\gi #2\in\gi #3}A_{#1}\EV{V_{#1}}#2
\]
}

\AddEq{w in Jv}
{
$w\in X_k\subseteq J(v)$.
}

\AddEq[3]{f(da)=h... module}
{
\def\Temp{}%
\edef\Tempa{#1}%
\ifx\Tempa\Temp%
\def\Koef{d}%
\else
\def\Koef{#1(d)}
\fi
#2\circ(d#3)=\Koef(#2\circ #3)
}

\AddEq[3]{f(da)=h... left module}
{
#2\circ(d#3)=#1(d)(#2\circ #3)
}

\AddEq[3]{f(da)=h... right module}
{
#2\circ(d#3)=(#2\circ #3)#1(d)
}

\AddEquation{D , f(da)=... module}
{
f\circ(da)=(h\circ d)(f\circ a)
}

\AddEquation{D , f(da)=... left module}
{
f\circ(da)=(h\circ d)(f\circ a)
}

\AddEquation{D , f(da)=... right module}
{
f\circ(ad)=(f\circ a)(h\circ d)
}

\AddEq{h(d1+d2)=...}
{
h(d_1+d_2)=h(d_1)+h(d_2)
}

\AddEq{h(d1d2)=...}
{
h(d_1d_2)=h(d_1)h(d_2)
}

\AddEq{property linear map f}
{
\DrawEq[fab]{f(a+b)=...}{D }
\DrawEq[{}fa]{f(da)=h... module}{\DFDT \SideWS module}
\ShowEq{D ab in A, d in D}D{A_1}
}

\AddEq{commutative product in algebra, 1}
{
\AUD Cp{ij}=\AUD Cp{ji}
}

\AddEq{associative product in algebra, 1}
{
\AUD Cp{ij}\AUD Cq{pk}
=
\AUD Cq{ip}\AUD Cp{jk}
}

\AddEq{commutative product in algebra}
{
\[
\ARow ei\ARow ej
=
\ARow ej\ARow ei
\]
}

\AddEq{associative product in algebra}
{
\[
(\ARow ei\ARow ej)\ARow ek
=
\ARow ei(\ARow ej\ARow ek)
\]
}

\AddEq [3]{basis ei}
{
\[\eV[#1]=(\ECol{#1}{#2},\jJg {#2}{#3})\]
}

\AddEq [3]{basis e of module cols}
{
\eV[#1]=(\ECol{#1}{#2},\jJg {#2}{#3})
}

\AddEq[3]{basis e of module rows}
{
\eV[#1]=(\ERow{#1}{#2},\jJg {#2}{#3})
}

\AddEq {basis e of module}
{
\eV=(\ARow ej,\jJg jJ)
}

\AddEq [2]{basis e of module 1n}
{
\[\eV[#1]=(\EV{#1}1,...,\EV{#1}{#2})\]
}

\AddEquation{(a+b)c=.}
{
(a+b)c=ac+bc
}

\AddEquation{a(b+c)=.}
{
a(b+c)=ab+ac
}

\AddEq[1]{f:A1->A2, A module}
{
b=#1\CRstar f
}

\AddEq[2]{f:V1->V2, D module cols}
{
b=#1#2
}

\AddEq[2]{f:V1->V2, D module rows}
{
b=#2#1
}

\AddEquation{ab=ac a ne 0}
{
ab=ac\ \ \ \ a\ne 0
}

\AddEquation{ab=ac a ne 0 1}
{
b=(a^{-1}a)b=a^{-1}(\BlueText{ab})=a^{-1}(\BlueText{ac})=(a^{-1}a)c=c
}

\AddEq[2]{ker G in ker g}
{
$\ker G\subseteq\ker #1$#2
}

\AddEq [2]{va=ae1, module (left)(cols)}
{
\Vector #1=#1\CRstar e_{#2}
}

\AddEq [2]{va=ae1, module ()(cols)}
{
\Vector #1= e_{#2}#1
}

\AddEq [2]{va=ae1, module (right)(cols)}
{
\Vector #1=e_{#2}\RCstar #1
}

\AddEq [2]{va=ae1, module (left)(rows)}
{
\Vector #1=#1\RCstar e_{#2}
}

\AddEq [2]{va=ae1, module ()(rows)}
{
\Vector #1=#1 e_{#2}
}

\AddEq [2]{va=ae1, module (right)(rows)}
{
\Vector #1=e_{#2}\CRstar #1
}

\AddEq{Morphism of D algebra, injection}
{
$h(\ACol ai)$, $h(\ACol bi)$)
}

\AddEq[1]{algebra, homomorphism and product (11)}
{
h(\AUD{C_1^{}{}}k{ij})\AUD {#1}lk
=\AUD {#1}pi\AUD {#1}qj\AUD{C_2^{}{}}l{pq}
}

\AddEq[1]{algebra, homomorphism and product (1)}
{
\AUD{C_{1}^{}{}}k{ij}\AUD {#1}lk
=\AUD {#1}pi\AUD {#1}qj\AUD{C_2^{}{}}l{pq}
}

\AddEq[1]{kij in I}
{
$\gik$, $\gii$, \jJg j{#1},
}

\AddEq{algebra, homomorphism and product abe 2}
{
\begin{aligned}
&\,h(\AUD{C_1^{}{}}k{ij})\AUD flkh(\ACol ai)h(\ACol bj)\EBase 2l
\\ =&\,h(\AUD{C_1^{}{}}k{ij}\ACol ai\ACol bj)\AUD flk\EBase 2l
\end{aligned}
}

\AddEq{algebra, homomorphism and product abe 2(1)}
{
\begin{aligned}
&\,h(\AUD{C_1^{}{}}k{ij})\AUD flkh(\ACol ai)h(\ACol bj)\EBase 2l
\\ =&\,h(\ACol {(ab)}k)\AUD flk\EBase 2l
\end{aligned}
}

\AddEq{algebra, homomorphism and product abe 2()}
{
\begin{aligned}
&\,\AUD{C_1^{}{}}k{ij}\AUD flk\ACol ai\ACol bj\EBase 2l
\\ =&\,\ACol {(ab)}k\AUD flk\EBase 2l
\end{aligned}
}

\AddEq{algebra, homomorphism and product abe 3(1)}
{
\begin{aligned}
&\,h(\AUD{C_1^{}{}}k{ij})\AUD flkh(\ACol ai)h(\ACol bj)\EBase 2l
\\ =&\,f\circ(ab)
\end{aligned}
}

\AddEq{algebra, homomorphism and product abe 3()}
{
\begin{aligned}
&\,\AUD{C_1^{}{}}k{ij}\AUD flk\ACol ai\ACol bj\EBase 2l
\\ =&\,f\circ(ab)
\end{aligned}
}

\AddEq{algebra, homomorphism and product abe 11}
{
\begin{aligned}
&\, h(\AUD{C_1^{}{}}k{ij})\AUD flkh(\ACol ai)h(\ACol bj)\EBase 2l
\\ =&\,\AUD fpi\AUD fqj\AUD{C_2^{}{}}l{pq}h(\ACol ai)h(\ACol bj)\EBase 2l
\end{aligned}
}

\AddEq{algebra, homomorphism and product abe 1}
{
\begin{aligned}
&\, \AUD{C_{1}^{}{}}k{ij}\AUD flk\ACol ai\ACol bj\EBase 2l
\\ =&\,\AUD fpi\AUD fqj\AUD{C_2^{}{}}l{pq}\ACol ai\ACol bj\EBase 2l
\end{aligned}
}

\AddEq{algebra, homomorphism and product abe 5(1)}
{
\begin{aligned}
&\, \AUD fpi\AUD fqj\AUD{C_2^{}{}}l{pq}h(\ACol ai)h(\ACol bj)\EBase 2l
\\ =&\,(f\circ a)(f\circ b)
\end{aligned}
}

\AddEq{algebra, homomorphism and product abe 5()}
{
\begin{aligned}
&\, \AUD fpi\AUD fqj\AUD{C_2^{}{}}l{pq}\ACol ai\ACol bj\EBase 2l
\\ =&\,(f\circ a)(f\circ b)
\end{aligned}
}

\AddEq{algebra, homomorphism and product abe 4(1)}
{
\begin{aligned}
&\, \AUD fpi\AUD fqj\AUD{C_2^{}{}}l{pq}h(\ACol ai)h(\ACol bj)\EBase 2l
\\ =&\,(h(\ACol ai)\AUD fpi\EBase 2p)(h(\ACol bj)\AUD fqj\EBase 2q)
\end{aligned}
}

\AddEq{algebra, homomorphism and product abe 4()}
{
\begin{aligned}
&\, \AUD fpi\AUD fqj\AUD{C_2^{}{}}l{pq}\ACol ai\ACol bj\EBase 2l
\\ =&\,(\ACol ai\AUD fpi\EBase 2p)(\ACol bj\AUD fqj\EBase 2q)
\end{aligned}
}

\AddEq{a, b in A1}
{
\[
\begin{matrix}
a,b\in A_1&
a=\ACol ai\EBase 1i&
b=\ACol bi\EBase 1i
\end{matrix}
\]
}

\AddEq{algebra, homomorphism and product, 1}
{
\newline
\FrameEqRef{product of basis vectors, algebra}{\Cols}
\newline
}

\AddEq{algebra, homomorphism and product eiej(11)}
{
\Vector f\circ (\EBase 1i\EBase 1j)
=h(C_1^{}\AUD{{}}k{ij})\Vector f\circ \EBase 1k
}

\AddEq{algebra, homomorphism and product eiej(1)}
{
\Vector f\circ (\EBase 1i\EBase 1j)
=C_1^{}\AUD{{}}k{ij}\Vector f\circ \EBase 1k
}

\AddEq{algebra, homomorphism and product eiej 4(11)}
{
\Vector f\circ (\EBase 1i\EBase 1j)
=h(C_1^{}\AUD{{}}k{ij})\aUD flk\EBase 2l
}

\AddEq{algebra, homomorphism and product eiej 4(1)}
{
\Vector f\circ (\EBase 1i\EBase 1j)
=C_1^{}\AUD{{}}k{ij}\aUD flk\EBase 2l
}

\AddEq{algebra, homomorphism and product, 4}
{
\Vector f\circ (ab)
=h(C_1^{}\AUD{{}}k{ij})
h(\ACol ai)h(\ACol bj)\Vector f\circ \EBase 1k
}

\AddEq{algebra, homomorphism and product, 5 11}
{
\Vector f\circ (ab)
=h(C_1^{}\AUD{{}}k{ij})h(\ACol ai)h(\ACol bj)
\AUD flk\EBase 2l
}

\AddEq{algebra, homomorphism and product, 5 1}
{
\Vector f\circ (ab)
=C_1^{}\AUD{{}}k{ij}\ACol ai\ACol bj
\AUD flk\EBase 2l
}

\AddEq{algebra, homomorphism and product eiej 5}
{
\begin{aligned}
&\,\Vector f\circ (\EBase 1i\EBase 1j)\\ =&\,
(\Vector f\circ \EBase 1i)(\Vector f\circ \EBase 1j)\\ =&\,
\AUD fpi\EBase 2p
\AUD fqj\EBase 2q
\end{aligned}
}

\AddEq{algebra, homomorphism and product eiej 2(11)}
{
\Vector f\circ (\EBase 1i\EBase 2j)=
\AUD fpi
\AUD fqj
C_2^{}\AUD{{}}l{pq}
\EBase 2l
}

\AddEq{algebra, homomorphism and product eiej 2(1)}
{
\Vector f\circ (\EBase 1i\EBase 2j)=
\AUD fpi
\AUD fqj
C_2^{}\AUD{{}}l{pq}
\EBase 2l
}

\AddEq{algebra, homomorphism and product eiej 3(11)}
{
h(C_1^{}\AUD{{}}k{ij})
\AUD flk\EBase 2l
=
\AUD fpi
\AUD fqj
C_2^{}\AUD{{}}l{pq}
\EBase 2l
}

\AddEq{algebra, homomorphism and product eiej 3(1)}
{
C_1^{}\AUD{{}}k{ij}
\AUD flk\EBase 2l
=
\AUD fpi
\AUD fqj
C_2^{}\AUD{{}}l{pq}
\EBase 2l
}

\AddEq{product in D algebra}
{
v\,w=C\circ(v,w)
}

\AddEq{product in algebra, definition 1}
{
\[
C:A\times A\rightarrow A
\]
}

\DefEq
{
\[
\underline{\otimes}:A^{n\otimes }\times A^{m\otimes }
\rightarrow A^{n+m-1\otimes}
\]
}
{otimes -}

\AddEq{a b in basis of algebra}
{
\[
\begin{matrix}
a=\ACol ai\ARow ei&b=\ACol bi\ARow ei&a, b\in A
\end{matrix}
\]
}

\AddEq{product in algebra}
{
\ACol{(ab)}k=\AUD Ck{ij}\ACol ai\ACol bj
}

\AddEq{product of basis vectors, algebra}
{
\ARow ei\ARow ej=
\AUD Ck{ij}\ARow ek
}

\AddEq{product in algebra, 1}
{
ab=\ACol ai\ACol bj\Eij
}

\AddEq{product in algebra, 2}
{
ab=\ACol ai\ACol bj
\AUD Ck{ij}\ARow ek
}

\AddEq[4]{diagram of representations of D algebra}%D F A g
{
\begin{matrix}
\vcenter
{
\xymatrix
{
A_{#3}\ar[rr]|{*}^{#4_{#2 23}}&&
A_{#3}
\\
&D_{#1}\ar[ur]|{*}_{#4_{#2 12}}\ar[ul]|{*}_{#4_{#2 12}}
}
}
&
\begin{array}{r@{\,}l}
#4_{#2 12}(d):v&\rightarrow d\,v
\\
#4_{#2 23}(v):w&\rightarrow
C_{#3}\circ(v, w)
\\
C_{#3}&\in\mathcal L(D_{#1};A_{#3}^2\rightarrow A_{#3})
\end{array}
\end{matrix}
}

\AddEq{endomorphism of module from product, 8}
{
\[
ab=(g_{23}\circ a)\circ b
\]
}

\AddEquation{endomorphism of module from product, 3}
{
\begin{array}{r@{\,}l}
(g_{23}\circ v)(w_1+w_2)&=(g_{23}\circ v)\circ w_1+(g_{23}\circ v)\circ w_2
\\
(g_{23}\circ v)\circ (dw)&=d((g_{23}\circ v)\circ w)
\end{array}
}

\AddEquation{endomorphism of module from product, 4}
{
(g_{23}\circ (v_1+v_2))\circ w
=(g_{23}\circ v_1+g_{23}\circ v_2)(w)
=(g_{23}\circ v_1)\circ w+(g_{23}\circ v_2)\circ w
}

\AddEquation{endomorphism of module from product, 7}
{
(g_{23}\circ(d\,v))\circ w
=(d\,(g_{23}\circ v))\circ w
=d\,((g_{23}\circ v)\circ w)
}

\AddEquation{r=+q circ p}
{
\begin{split}
r(x)&=s_0+(q_0+q_1(x)+...+q_{k-1}(x))\circ p(x)
\end{split}
}

\AddEq{qij i j}
{
$q_i\in A_i[x]\otimes A$, $i=0$, ..., $k-1$,
}

\AddEquation{monomial of power k, F=1}
{
p_k(x)=p_{k-1}(x)xa_k
}

\AddEq{a circ x=b}
{
a\circ x=b
}

\AddEq[5]{structural constants of algebra}
{
\ensuremath{C_{#1}^{}{}\AUD {}{#2}{#3#4}{#5}}
}

\AddEq{structural constants of algebra symb}
{
\symb{
\ShowEq{structural constants of algebra}{}kij{}
}{structural constants}1
}

\AddEquation{otimes -, 1}
{
(a_1\otimes...\otimes a_n)\underline{\otimes}(b_1\otimes...\otimes b_n)
=
a_1\otimes...\otimes a_{n-1}\otimes a_nb_1\otimes b_2\otimes...\otimes b_n
}

\AddEq[3]{a=oxai}
{
$#1=#1_0\otimes...\otimes #1_{#2}$#3
}

\AddEq[3]{vb=f(va)}
{
\Vector #2=\Vector #3\circ\Vector #1
}

\AddEquation{vb=h(e1)a (1)(1)(cols)}
{
\Vector b=\Vector f\circ\Vector a=\Vector f\circ(e_1a)
= (\Vector f\circ e_1)h(a)
}

\AddEquation{vb=h(e1)a (1)(1)(rows)}
{
\Vector b=\Vector f\circ\Vector a=\Vector f\circ(a e_1)
= h(a)(\Vector f\circ e_1)
}

\AddEquation{vb=h(e1)a ()(1)(cols)}
{
\Vector b=\Vector f\circ\Vector a=\Vector f\circ(e_1a)
= (\Vector f\circ e_1)a
}

\AddEquation{vb=h(e1)a ()(1)(rows)}
{
\Vector b=\Vector f\circ\Vector a=\Vector f\circ(ae_1)
= a(\Vector f\circ e_1)
}

\AddEq[5]{f o ea=efa i (11)}
{
\Vector{#2}\circ(\ACol {#5}i\EBase {#3}i)
= #1(\ACol {#5}i)\AUD {#2}ki\EBase {#4}k
}

\AddEq[5]{f o ea=efa i (1)}
{
\Vector{#2}\circ(\ACol {#5}i\EBase {#3}i)
= \ACol {#5}i\AUD {#2}ki\EBase {#4}k
}

\AddEq[4]{f o ev=efv i (11)}
{
\Vector{#2}\circ(\Multiply{\ACol vi}{\EBase {#3}i})
= \Multiply{(\Vector{#1}\circ \ACol vi)}{\Multiply{\AUD {#2}ki}{\EBase {#4}k}}
}

\AddEq[4]{f o ev=efv i (1)}
{
\Vector{#2}\circ(\Multiply{\ACol vi}\Multiply{\EBase {#3}i})
= \Multiply{\ACol vi}{\Multiply{\AUD {#2}ki}{\EBase {#4}k}}
}

\AddEq[4]{f o ea=efa (11)(cols)}
{
\Vector{#2}\circ(e_{#3}a)
= e_{#4}#2#1(a)
}

\AddEq[4]{f o ea=efa (11)(rows)}
{
\Vector{#2}\circ(a e_{#3})
= #1(a)#2e_{#4}
}

\AddEq[4]{f o ea=efa (1)(cols)}
{
\Vector{#2}\circ(e_{#3}a)
= e_{#4}#2a
}

\AddEq[4]{f o ea=efa (1)(rows)}
{
\Vector{#2}\circ(ae_{#3})
= a#2e_{#4}
}

\DefRef{Morphism of Diagram of Representations}
{
\RefDefinition{morphism of representations of universal algebra},
\RefDefinition{Morphism of Diagram of Representations},
}

\AddEquation{vb=h(e1)a (1)(1)(1)(cols)left}
{
\Vector b=\Vector f\circ\Vector a=\Vector f\circ(a\CRstar e_1)
= h(a)\CRstar(\Vector f\circ e_1)
}

\AddEquation{vb=h(e1)a (1)(1)(1)(cols)right}
{
\Vector b=\Vector a\diamond\Vector f=(e_1\RCstar a)\diamond\Vector f
= (e_1\diamond\Vector f)\RCstar h(a)
}

\AddEquation{vb=h(e1)a (1)(1)(1)(rows)left}
{
\Vector b=\Vector f\circ\Vector a=\Vector f\circ(a\CRstar e_1)
= h(a)\CRstar(\Vector f\circ e_1)
}

\AddEquation{vb=h(e1)a (1)(1)(1)(rows)right}
{
\Vector b=\Vector a\diamond\Vector f=(e_1\RCstar a)\diamond\Vector f
= (e_1\diamond\Vector f)\RCstar h(a)
}

\AddEq{f(e1)(cols)}
{
$\Vector f\circ\aD[1]ei$
}

\AddEq{f(e1)(rows)}
{
$\Vector f\circ\aU{e_1}i$
}

\AddEq{f(e1)(cols)left}
{
$\Vector f\circ\aD[1]ei$
}

\AddEq{f(e1)(cols)right}
{
$\aD[1]ei\diamond\Vector f$
}

\AddEq{f(e1)(rows)left}
{
$\Vector f\circ\aU{e_1}i$
}

\AddEq{f(e1)(rows)right}
{
$\aU{e_1}i\diamond\Vector f$
}

\AddEq{f(e1)=(cols)}
{
\Vector f\circ\aD[1]ei
=e_2\aD fi
=\aD[2]ej\aUD fji
}

\AddEq{f(e1)=(cols)left}
{
\Vector f\circ\aD[1]ei
=\aD fi\CRstar e_2
=\aUD fji\aD[2]ej
}

\AddEq{f(e1)=(cols)right}
{
\aD[1]ei\diamond\Vector f
=e_2\RCstar\aD fi
=\aD[2]ej\aUD fji
}

\AddEq{f(e1)=(rows)}
{
\Vector f\circ\aU{e_1}i
=\aD fie_2
=\aUD fij \aU{e_2}j
}

\AddEq{f(e1)=(rows)left}
{
\Vector f\circ\aU{e_1}i
=\aD fi\RCstar e_2
=\aUD fij\aU{e_2}j
}

\AddEq{f(e1)=(rows)right}
{
\aU{e_1}i\diamond\Vector f
=e_2\CRstar\aD fi
=\aU{e_2}j\aUD fij
}

\AddEquation{vb=a f e (1)(1)(cols)left}
{
\Vector b=h(a)\CRstar f\CRstar e_2
}

\AddEquation{vb=a f e ()(1)(cols)left}
{
\Vector b=a\CRstar f\CRstar e_2
}

\AddEquation{vb=a f e ()(1)(cols)}
{
\Vector b=e_2fa
}

\AddEquation{vb=a f e (1)(1)(cols)}
{
\Vector b=e_2fh(a)
}

\AddEquation{vb=a f e ()(1)(cols)right}
{
\Vector b=e_2\RCstar f\RCstar a
}

\AddEquation{vb=a f e (1)(1)(cols)right}
{
\Vector b=e_2\RCstar f\RCstar h(a)
}

\AddEquation{vb=a f e (1)(1)(rows)left}
{
\Vector b=h(a)\RCstar f\RCstar e_2
}

\AddEquation{vb=a f e ()(1)(rows)left}
{
\Vector b=a\RCstar f\RCstar e_2
}

\AddEquation{vb=a f e ()(1)(rows)}
{
\Vector b=afe_2
}

\AddEquation{vb=a f e (1)(1)(rows)}
{
\Vector b=h(a)fe_2
}

\AddEquation{vb=a f e ()(1)(rows)right}
{
\Vector b=e_2\CRstar f\CRstar a
}

\AddEquation{vb=a f e (1)(1)(rows)right}
{
\Vector b=e_2\CRstar f\CRstar h(a)
}

\AddEq [4]{h(a)=...}
{
$#2(#1)=(#2(\ARow {#1}{#3}),\gi #3\in\gi #4)$
}

\AddEq[4]{Vector f(e1) module}
{
$(\Vector #1\circ\EBase {#2}{#3},\jJg{#3}{#4})$
}


==> Stmt.Module.Ref.tex <==
%auto-ignore

\AddEq{ref theorem coordinates of map A1 A2, algebra}
{
\ePrints{9835-2163,0767-8264}
\ifx\Semafor\ValueOn
\RefTheorem{coordinates of map A1 A2 FoG, algebra}.
\else
\ePrints{5284-0163,1801.01628,CACAA.07}%
\ifx\Semafor\ValueOn
%\def\RefPolymorphism{1502.04063}%
\RefTheorem{coordinates of map A1 A2, algebra}.
\else
\RefTheorem[\RefPolymorphism]{coordinates of map A1 A2, algebra}.
\fi
\fi
}

\AddEq{RefTheorem set of vectors generated by set of vectors, module}
{
\ePrints{1502.04063,5114-6019}%
\ifx\Semafor\ValueOn%
\RefTheorem{set of vectors generated by the set of vectors},
\else%
\refTheorem{set of vectors generated by set of vectors}{module},
\fi%
}

\AddEq{ref definition: basis of representation}
{
\ePrints{1502.04063,5114-6019,MAlgebra2}%
\ifx\Semafor\ValueOn%
\RefDefinition[0912.3315]{basis of representation}
\else%
\RefDefinition{basis of representation}
\fi
}

\AddEq{f=.I0.7 ref}
{
\EqRef{linear map of algebra O, structure, 1},
\eqRef{fi=fij ej}O,
\EqRef{a0=f07},
\EqRef{a1=f07},
\EqRef{a2=f07},
\EqRef{a3=f07},
\EqRef{a4=f07},
\EqRef{a5=f07},
\EqRef{a5=f07},
\EqRef{a7=f07}.
}

\AddEq{f=.E+.I+.J+.K ref}
{
\EqRef{linear map of algebra H, structure, 1},
\eqRef{fi=fij ej}H,
\EqRef{a0=f03},
\EqRef{a1=f03},
\EqRef{a2=f03},
\EqRef{a3=f03}.
}

\AddEq{f=.E+.I ref}
{
\EqRef{linear map of algebra C, structure, 1},
\eqRef{fi=fij ej}C,
\EqRef{a0=f01},
\EqRef{a1=f01}.
}

\DefRef[3]{homomorphism of d algebra, coordinates}
{
\newline
\FrameEqRef[f{#3}{}]{f:V1->V2, D module \Cols}{algebra(#1#2)}
\newline
\FrameEqRef[hf12a]{f o ea=efa i (#1#2)}{(\Cols)algebra}
\newline
\FrameEqRef[hf12]{f o ea=efa (#1#2)(\Cols)}{algebra}
\newline
%\eqRef{f:V1->V2, D module \Cols}{algebra(#1#2)},
%\eqRef{f o ea=efa (#1#2)(\Cols)}{algebra}
}

\DefRef[3]{algebra, homomorphism and product}
{
\newline
\FrameEqRef[{#3}{}]{algebra, homomorphism and product (#1#2)}{\Cols(\SideNS)}
\newline
}

\DefRef[3]{matrix generates A module homomorphism()}
{
\newline
\FrameEqRef{\RefDistributive{\Product}}1
\FrameEqRef[fa{#3}v]{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module}
\FrameEqRef[vf{V_1}{V_2}]{f o (ae)=ga o f e, vector space \Product-\Cols}{\SideNS(#1#21)}
\newline
}

\DefRef[3]{matrix generates A module homomorphism(1)}
{
\newline
\FrameEqRef{\RefDistributive{\Product}}1
\FrameEqRef[gab]{homomorphism, f v+w=}{g(#1#2)\SideWS A module}
\FrameEqRef[fa{#3}v]{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module}
\FrameEqRef[vf{V_1}{V_2}]{f o (ae)=ga o f e, vector space \Product-\Cols}{\SideNS(#1#21)}
\newline
}

\DefRef[3]{fo(va)()}
{
\newline
\FrameEqRef[fa{#3}v]{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module}
\FrameEqRef[vf{V_1}{V_2}]{f o (ae)=ga o f e, vector space \Product-\Cols}{\SideNS(111)}
\newline
}

\DefRef[3]{fo(va)(1)}
{
\newline
\FrameEqRef[fa{#3}v]{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module}
\FrameEqRef[gab]{homomorphism, f vw=}{(#1#2)g}
\newline
\FrameEqRef[vf{V_1}{V_2}]{f o (ae)=ga o f e, vector space \Product-\Cols}{\SideNS(111)}
\newline
}

\DefRef[2]{homomorphism, f vw=}
{
\newline
\FrameEqRef[fab]{homomorphism, f vw=}{(#1#2)g}
\newline
}

\DefRef[2]{homomorphism of d algebra, coordinates 1}
{
\newline
\FrameEqRef[hf12a]{f o ea=efa i (#1#2)}{(\Cols)algebra}
\newline
}

\DefRef[3]{homomorphism of D module}
{
\newline
\FrameEqRef[fab]{homomorphism, f v+w=}{f D module #1#2}
\newline
\FrameEqRef[fp{#3}a]{left homomorphism, f av=}{f D module #1#2}
\newline
}

\DefRef[3]{vb=h(e1)a}
{
\newline
\FrameEqRef[fp{#3}a]{left homomorphism, f av=}{f D module #1#2}
\FrameEqRef[a1{}]{va=ae1, module ()(\Cols)}{\SideNS-\VectorSet a (#1)(#2)}
\newline
}

\DefRef[2]{algebra, homomorphism and product 1}
{
\eqRef{algebra, homomorphism and product abe #1#2}{\Cols},
\eqRef{algebra, homomorphism and product abe 3(#1)}{\Cols},
\eqRef{algebra, homomorphism and product abe 5(#1)}{\Cols}.
}

\DefRef{product in algebra}
{
\newline
\FrameEqRef{product in algebra}{\Cols}
\newline
}

\DefRef[3]{algebra, homomorphism and product eiej}
{
\newline
\FrameEqRef{product of basis vectors, algebra}{\Cols}
\newline
\FrameEqRef[fp{#3}a]{left homomorphism, f av=}{(#1#2)g}
\newline
}

\DefRef[2]{algebra, homomorphism and product eiej 1}
{
\newline
\FrameEqRef{f(e1)=(\Cols)\SideNS}{(#1)(#2)}
\newline
}

\AddEq{ref linear map of D1 D2 module, coordinates}
{
\ePrints{9835-2163,0767-8264}
\ifx\Semafor\ValueOn
\refTheorem{linear map of D module, coordinates}1,
\else
\refTheorem[\RefLinearMap]{linear map of D module}1,
%\RefTheorem[\RefLinearMap]{linear map of D1 D2 module, coordinates},
\fi
}

\AddEq{ref module, (a+n)(b+m)=}
{
\EqRef{\SideWS module, a d v},
\EqRef{\SideWS module, (a+n)v=av+nv},
\eqRef{associative law, \SideWS module}1,
\eqRef{associative law, \CBase, \SideWS module}1,
\eqRef{\SideWS module, associative law}1,
\eqRef{associative law, \CBase\Base, \SideWS module}1.
}

\AddEq{def sum of linear maps}
{
\ifx\SelectlEnglish\undefined
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
\def\defTheorem{Согласно теореме}
\else
\def\defTheorem{Согласно следствию}
\fi
\else
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
\def\defTheorem{According to the theorem}
\else
\def\defTheorem{According to the corollary}
\fi
\fi
}

\DefEq
{
\defTheorem
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
\RefTheorem{sum of linear maps, D module},
\else
\RefCorollary{sum of linear maps, D module},
\fi
}
{ref sum of linear maps}

\AddEq [1]{ref definition: representation of algebra}
{
%\ePrints{5114-6019}%
%\ifx\Semafor\ValueOn%
%\RefDefinition[0912.3315]{left-side representation of algebra}#1
%\else%
\refDefinition[\RefRepresentation]{side representation of group}{left}#1
%%\RefDefinition[\RefRepresentation]{representation of algebra}#1
%\fi
}

\AddEq{ref sum and product over scalar, linear map}
{
\ifx\SelectlEnglish\undefined
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
согласно теоремам
\else
согласно следствиям
\fi
\else
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
according to theorems
\else
according to corollarys
\fi
\fi
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
\RefTheorem{sum of linear maps, D module},
\RefTheorem{product of linear map over scalar, D module},
\else
\RefCorollary{sum of linear maps, D module},
\RefCorollary{product of linear map over scalar, D module},
\fi
}

\AddEq{ref map j, representation, tensor product}
{
\ePrints{MAlgebra2}%
\ifx\Semafor\ValueOn%
\EqRef[\RefPolymorphism]{map j, representation, tensor product},
\else%
\ePrints{2207.06506,8428-0408}%
\ifx\Semafor\ValueOn%
\EqRef[\RefLinearMap]{map j, representation, tensor product},
\else
\EqRef{map j, representation, tensor product},
\fi
\fi
}


==> Stmt.Module.Russian.tex <==
%auto-ignore
\input{Stmt.Module.Eq}

\DefExample{Abelian Group is Z module}
{
Из теорем
\RefTheorem{action of ring of rational integers in Abelian group},
\RefTheorem{Abelian group is free}
и определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
следует, что свободная абелевая группа $G$ является модулем над кольцом целых чисел $Z$.
}

\DefText[2]{ix-xi-1 roots}
{
многочлен
\DrawEq[1]{ix-xi-1}{#1}
не имеет корней
и многочлен
\DrawEq[k]{ix-xi-1}{#2}
имеет множество корней
\DrawEq{x=c12+j}{#2}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{module over ring}
Пусть коммутативное кольцо $D$ имеет единицу $1$.
Эффективное представление
\DrawEq{D->*V}{def}
кольца $D$
в абелевой группе $V$
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
Эффективное представление
\eqRef{D->*V}{def}
поля $D$ в абелевой группе $V$
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\end{ShadedDefinition}
}
{... definition: module over ring}
%\DefEq

\DefTheorem{tensor product of D-algebras is D-algebra}
{
Пусть
\ShowEq{A1...n}
- $D$\Hyph алгебры.
Тензорное произведение
$\Tensor A$
$D$\Hyph модулей
\ShowEq{A1...n}
является $D$\Hyph алгеброй,
если мы определим произведение согласно правилу
\ShowEq{xA1n*xA1n->oxA1n=}
}

\DefTheorem{representation of algebra H2 in LH}
{
Пусть произведение в алгебре
\AoxA H
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{RH}
Представление
\DrawEq[RH]{h:AoxA->L(A)}H
$R$\Hyph алгебры
\AoxA H
в абелевой группе
\ShowEq{L(A->B)}RHH,
определённое равенством
\DrawEq[RH]{representation AA in LA}{RH}
является левым \BoxB{H}модулем.
Если мы положим $g=E$,
где
\ShowEq{product in algebra AA 3}RHE
- тождественное отображение,
то мы можем отождествить линейное отображение
\DrawEq[fHH{}]{f: A->B}-
алгебры кватернионов и тензор
\DrawEq{linear map f, basis E}1
опираясь на равенство
\ShowEq{value of linear map f, basis E}
}

\DefProof{representation of algebra H2 in LH}
{
Теорема является следствием утверждения
что отображение
\ShowEq{Eox=x}
порождает любое линейное отображение алгебры кватернионов
}

\DefDefinition{square root}
{
Решение
\ShowEq{square root}
уравнения
\DrawEq{x2=a}{root}
в $D$\Hyph алгебре $A$
называется
\AddIndex{квадратным корнем}{square root}
$A$\Hyph числа $a$.
}

\DefDefinition{polynomial*polynomial}
{
Билинейное отображение
\ShowEq{polynomial*polynomial}
определено равенством
\ShowEq{polynomial*polynomial, 1}
}

\DefTheorem{(a*b)x=(ax)(bx)}
{
Для любых тензоров
\ShowEq{a in Aoxn}a{n+1},
\ShowEq{a in Aoxn}b{m+1}{},
произведение однородных многочленов
\ShowEq{polynomials a o x,b o x}
определено равенством
\ShowEq{(a*b)x=(ax)(bx)}
}

\DefTheorem{x2=a quaternion root}
{
Пусть $H$ - алгебра кватернионов и $a$ - $H$\Hyph число.
\StartLabelItem
\begin{enumerate}
\item
Если
\ShowEq{Re sqrt a ne 0}
то уравнение
\DrawEq{x2=a}{}
имеет корни
\ShowEq{x=x12}
такие, что
\ShowEq{x2=-x1}
\labelItem{Re sqrt a ne 0}
\item
Если $a=0$, то уравнение
\DrawEq{x2=a}{}
имеет корень $x=0$ кратности $2$.
\labelItem{a=0}
\item
Если условия
\RefItem{Re sqrt a ne 0},
\RefItem{a=0}
не верны,
то уравнение
\DrawEq{x2=a}{}
имеет бесконечно много корней таких, что
\ShowEq{|x|=sqrt a}
\labelItem{Re sqrt a=0}
\end{enumerate}
}

\DefDefinition{polylinear map of algebras, property}
{
Полилинейное отображение $D$\Hyph алгебры $A$
\ShowEq{f:A->B}f{A^n}A
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{1}
\DrawEq[f]{f(pai)=pfai}{1}
\ShowEq{polylinear map of algebras, 1}AD
Обозначим
\ShowEq{set polylinear maps An}DAA
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A$.
}

\DefRemark{monomial of power k}
{
В теореме
\RefTheorem{monomial of power k}
я рассмотрел рекурсивное представление одночлена в ассоциативной $D$\Hyph алгебре.
Так как скобки в произведении
я могу расставить произвольно,
то в ассоциативной $D$\Hyph алгебре
рекурсивное представление одночлена неоднозначно.
Например, одночлен $ax^2bxcx^3d$
может быть записан в любой из следующих форм
\ShowEq{ax^2bxcx^3d}
Я выбрал равенство
\EqRef{monomial of power k, F=1}
как самое простое для алгоритма деления многочленов.
}

\DefTheorem{monomial of power k}
{
Пусть $p_k(x)$ -
\AddIndex{одночлен степени}{monomial of power} $k$
над ассоциативной $D$\Hyph алгеброй $A$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Одночлен степени $0$ имеет вид
\ShowEq{p0(x)=a0}
\item
Если $k>0$, то
\labelItem{monomial of power k}
\ShowEq{monomial of power k, F=1}
где $a_k\in A$.
\end{enumerate}
}

\DefProof{monomial of power k}
{
Мы докажем утверждение теоремы индукцией по степени
$n$ одночлена.

Пусть $n=0$.
Так как одночлен $p_0(x)$ является константой,
то мы получаем утверждение
\RefItem{monomial of power 0}.

Пусть $n=k$. Последний множитель одночлена $p_k(x)$ является либо $a_k\in A$,
либо имеет вид $x^l$, $l\ge 1$.
В последнем случае мы положим $a_k=1$.
Множитель, предшествующий $a_k$, имеет вид $x^l$, $l\ge 1$.
Мы можем представить этот множитель в виде $x^{l-1}x$.
Следовательно, утверждение доказано.
}

\DefTheorem{r=+q circ p}
{
Пусть
\ShowEq{p=p circ x}
- многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p}
где
\ShowEq{qij i j}
- однородный многочлен степени $i$.
}

\DefLabeledDefinition{linear map of A vector space}{\SideNS}
{
\ShowText{algebra over ring ()}
Пусть $V$, $W$ - \SideRu вые векторные пространства над $D$\Hyph алгеброй $A$.
Линейное отображение
\ShowEq{f:A->B}fVW
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu вого $A$\Hyph векторного пространства $V$
в \SideRu вое $A$\Hyph векторное пространство $W$.
Обозначим
\ShowEq{set linear maps, VW module}
множество линейных отображений
\SideRu вого $A$\Hyph векторного пространства $V$
в \SideRu вое $A$\Hyph векторное пространство $W$.
}

\DefDefinition{component of linear map, basis E}
{
Выражение
\ShowEq{component of linear map, basis E}
в равенстве
\eqRef{linear map f, basis E}1
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
}

\DefTheorem{representation of algebra A2 in LA}
{
Пусть $A$ является $D$\Hyph алгеброй.
Пусть произведение в $D$\Hyph модуле
\AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{}
Представление
\DrawEq[DA]{h:AoxA->L(A)}{}
$D$\Hyph алгебры
\AoxA A
в модуле
\ShowEq{L(A->B)}DAA,
определённое равенством
\DrawEq[DA]{representation AA in LA}{}
позволяет отождествить тензор
\ShowEq{d in AxoA}A
с линейным отображением
\ShowEq{product in algebra AA 2}DA{\delta},
где
\ShowEq{product in algebra AA 3}DA{\delta}
- тождественное отображение.
Линейное отображение
\ShowEq{a ox b}{\delta}
имеет вид
\ShowEq{a ox b c=}
}

\AddEq[1]{theorem: matrices fUD I}
{
\begin{ShadedTheorem}
\labelTheorem{#1, matrices fUD I}
Отображения сопряжения
имеют
стандартное представление
\ShowEq{#1. standard representation I}
\end{ShadedTheorem}
}

\AddEq[2]{proof: matrices fUD I}
{
Согласно равенству
\EqRef{#2x= #1},
отображение сопряжения
\ShowEq{Map of Conjugation}{#2}
имеет матрицу
\ShowEq{#1. matrix I#2}
Равенство
\DrawEq[{#2}{}]{#1.fUD->fUU I}{#1#2}
является следствием равенств
\EqRef{#1.fUD->fUU},
\EqRef{#1. matrix I#2}.
}

\DefTheorem{unit of algebra and ring}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с единицей \(1_A\).
\StartLabelItem
\begin{enumerate}
\item
Отображение
\ShowEq{f:a in A->b in B}fdD{d1_A}A
является изоморфизмом кольца $D$ в центр алгебры $A$
и позволяет отождествить \(D\)\Hyph число \(d\)
и \(A\)\Hyph число \(d\,1_A\).
\labelItem{isomorphism d->d1}
\item
Кольцо \(D\) является подалгеброй алгебры $A$.
\labelItem{D is subalgebra of A}
\item
\ShowEq{D in Z(A)}
\end{enumerate}
}

\DefProof{unit of algebra and ring}
{
Пусть
\ShowEq{d12 in D}
Согласно утверждению
\RefItem{distributive law, module},
\ShowEq{d1+d2 in A}
Согласно определению
\RefDefinition{algebra over ring},
\ShowEq{d1 d2 in A}
Утверждение
\RefItem{isomorphism d->d1}
является следствием равенств
\EqRef{d1+d2 in A},
\EqRef{d1 d2 in A}.
Утверждение
\RefItem{D is subalgebra of A}
является следствием утверждения
\RefItem{isomorphism d->d1}.

Согласно определению
\RefDefinition{algebra over ring},
\ShowEq{ad=da in A}
Утверждение
\RefItem{D in Z(A)}
следует из равенства
\EqRef{ad=da in A}.
}

\DefTheorem{multiplication in algebra is distributive over addition}
{
Произведение в алгебре $A$ дистрибутивно по отношению к сложению
\ShowEq{(a+b)c=.}
\ShowEq{a(b+c)=.}
}

\DefDefinition{module over commutative ring}
{
Эффективное представление коммутативного кольца $D$
в абелевой группе $V$
\DrawEq{D->*V}{module}
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
Если $D$ - поле, то абелевая группа $V$
называется
\AddIndex{векторным пространством}{vector space} над полем $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\fi
}

\DefDefinition{linear map of algebra}
{
\ShowEq{def DModule}
\ShowEq{=DD}
Линейное отображение
%\ShowEq{f:A->B}fHH
%алгебры кватернионов $H$
\ShowEq{f:A->B}fAA
$D$\Hyph алгебры $A$
удовлетворяет равенствам
\DrawEq[fab]{f(a+b)=...}{D }
\DrawEq[{}fa]{f(da)=h... module}{module}
\ShowEq{D ab in A, d in D}DA
Обозначим
%\ShowEq{set linear maps, module}RHH
\ShowEq{set linear maps, module}DAA
множество линейных отображений
%алгебры кватернионов $H$.
$D$\Hyph алгебры $A$.
}

\DefLabeledDefinitionNote{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Копроизведение в категории \SideRu\TO $\Base$\Hyph \VectorsSetRuB называется
\AddIndex{прямой суммой}{direct sum}.\,\footnotemark
Мы будем пользоваться записью
\ShowEq{direct sum of modules}{\Module}{\ModuleA}
для прямой суммы \SideRu\TO $\Base$\Hyph \VectorsSetRuB $\Module$ и $\ModuleA$.
}{
Смотри так же определение
прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}

\DefLabeledTheorem{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{set Bi}{\Module}
- семейство \SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.
Тогда представление
\ShowEq{\SideWS D->*o+A}{\Base}{\Module}{\ANumber}{\VNumber}
\ShortAlgebraRuBWS $\Base$
в прямой сумме абелевых групп
\ShowEq{o+Ai}{\Module}
является прямой суммой \SideRu\TO $\Base$\Hyph модулей
\ShowEq{o+Ai}{\Module}
}

\DefProof{direct sum of D modules}
{
Пусть
\ShowEq{set f:A->B}f{\Module_i}{\ModuleA}
семейство линейных отображений в \SideRu\To $\Base$\Hyph модуль $V$.
Мы определим отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
пользуясь равенством
\DrawEq{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
Сумма в правой части равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
конечна, так как все слагаемые, кроме конечного числа, равна $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(x+y)i=}
Из равенства
\ShowEq{fi(dx)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(dx)i=}
Следовательно, отображение $f$ является линейным отображением.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\EqRef{lj(x)=0x0},
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\RefDefinition{direct sum of Abelian groups}.
}

\DefProof{cr-power, 1}
{
Равенство
\ShowEq{cr-power, 1 1}
является следствием равенств
\eqRef{cr power, 0}1,
\eqRef{cr-power, n}1.
Равенство
\EqRef{cr-power, 1}
является следствием равенства
\EqRef{cr-power, 1 1}.
}

\DefProof{rc-power, 1}
{
Равенство
\ShowEq{rc-power, 1 1}
является следствием равенств
\eqRef{rc power, 0}1,
\eqRef{rc-power, n}1.
Равенство
\EqRef{rc-power, 1}
является следствием равенства
\EqRef{rc-power, 1 1}.
}

\DefTheorem{a in ZAb=>b in ZAa}
{
Если
\ShowEq{c in ZAa}ab,
то
\ShowEq{c in ZAa}ba.
}

\DefProof{a in ZAb=>b in ZAa}
{
Пусть
\ShowEq{c in ZAa}ab.
Равенство
\DrawEq{ab=ba}Z
является следствием утверждения
\eqRef{c in S=>bc=cb}{Z(A,b)}.
Теорема является следстием равенства
\eqRef{ab=ba}Z.
}

\DefTheorem{a in ZAb, c in ZA=>a in ZAbc}
{
Если
\ShowEq{c in ZAa}ab{}
и
\ShowEq{c in ZA}c
то
\ShowEq{c in ZAa}a{bc}.
}

\DefProof{a in ZAb, c in ZA=>a in ZAbc}
{
Равенство
\ShowEq{a(bc)=...=(bc)a}
является следствием определений
\RefDefinition{nucleus of algebra},
\RefDefinition{center of algebra}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
Теоремя является следствием равенства
\EqRef{a(bc)=...=(bc)a}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
}

\DefTheorem{c in Za=> p(c) in Za}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $a\in A$, если
\ShowEq{c in ZAa}ca,
то
\DrawEq[{p(c)}a{}{}]{c in ZAa}1
для любого многочлена
\DrawEq{p(c) p in D}1
}

\DefProof{c in Za=> p(c) in Za}
{
}

\DefTheorem{c in S=>bc=cb submodule of A}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $b\in A$ существует подалгебра
\ShowEq{center of A number}
$D$\Hyph алгебры $A$ такая, что
\DrawEq[{Z(A,b)}{}]{c in S=>bc=cb}{Z(A,b)}
$D$\Hyph алгебра
\ShowEq{center Ac}{}
называется
\AddIndex{центром $A$\Hyph числа}{center of A number}
$b$.
}

\DefProof{c in S=>bc=cb submodule of A}
{
Подмножество
\ShowEq{center Ac}{}
не пусто так как
\ShowEq{c in ZAa}0b,
\ShowEq{c in ZAa}bb.
Пусть
\ShowEq{d in D c in S 12}
Тогда
\ShowEq{dcb=bdc}
Откуда следует
\ShowEq{dc in S}
Следовательно, множество
\ShowEq{center Ac}{}
является $D$\Hyph модулем.

Пусть
\ShowEq{c in ZAb}
Тогда
\ShowEq{c1c2 in ZAb}
Из равенства
\EqRef{c1c2 in ZAb}
следует, что
\ShowEq{c1 c2 in ZAb}
Следовательно, $D$\Hyph модуль
\ShowEq{center Ac}{}
является $D$\Hyph алгеброй.
}

\DefTheorem{set of maps B->A is Abelian group}
{
Пусть $A$ - алгебра над коммутативным кольцом $D$.
Для любого множества $B$
множество отображений $A^B$ является абелевой группой относительно операции
\ShowEq{(f+g)x=}x
}

\DefProof{set of maps B->A is Abelian group}
{
Теорема является следствием определений
\refDefinition{module over algebra}{\SideWS \VectorSetNS},
\RefDefinition{algebra over ring}.
}

\DefLabeledDefinition{module over algebra}{\SideWS \VectorSetNS}
{
Пусть $\Base$ - \AlgebraRuNS \DivisionRuNS.
Эффективное \SideRu \SidePresentationRuWS представление
\DrawEq{\SideWS \Base->*V}{\SideWS \VectorSetNS}
\ShortAlgebraRuBWS $\Base$
в \SetRepresentationRu $V$
называется
\AddIndex{\SideRu \SideModuleC \VectorSetRuE}{\SideWS \VectorSetNS}
над \ShortAlgebraRuCWS $\Base$.
Мы также будем говорить, что \SetRepresentationRuA $V$ является
\AddIndex{\SideRu \SideModuleC $\Base$\Hyph \VectorSetRuENS}{\SideWS A \VectorSetNS}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Билинейное отображение
\DrawEq{\SideWS \Base*V->V}{\VectorSet}
порождённое \SideRu \SidePresentationRuBWS представлением
\DrawEq{\Base*V->V to \SideWS product}{\VectorSetNS}
называется
%\AddIndex{\SideRu \SidePresentationRuBWS произведением}{\SideNS\SidePresentation product}
\SideRu \SidePresentationRuBWS произведением
вектора на скаляр.
}

\DefLabeledTheorem{module over algebra}{\SideNS}
{
Следующая диаграмма представлений описывает \SideRu\To $\Base$\Hyph модуль $V$
\DrawEq[{}{}{}{}]{diagram of representations, \SideWS module}1
В диаграмме представлений
\eqRef{diagram of representations, \SideWS module}1
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
\BaseRings
в абелевой группе $V$
\ShowEq{\SideWS module, a d v}
}

\DefProof{module over algebra}
{
Диаграмма представлений
\eqRef{diagram of representations, \SideWS module}1
является следствием определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теоремы
\def\Temp{}
\ifx\SideNS\Temp
\RefTheorem{action of ring of rational integers in Abelian group}.
\else
\RefTheorem{Free Algebra over Ring}.
\fi
Равенство
\EqRef{\SideWS module, a d v}
является следствием утверждения, что
\SideRu\HSide преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph модуля $V$.
}

\DefProof{Free Algebra over Ring}
{
Структура $D$\Hyph модуля $A$ порождена эффективным представлением
\ShowEq{f:A->*B}{g_{12}}DA
кольца $D$ в абелевой группе $A$.

\begin{ShadedLemma}
\labelLemma{structure of D algebra is generated by product}
{\it
Пусть в $D$\Hyph модуле $A$
определена структура $D$\Hyph алгебры $A$,
порождённая произведением
\DrawEq{product in D algebra}{}
\AddIndex{Левый сдвиг $D$\Hyph модуля $A$}{left shift of module},
определённый равенством
\ShowEq{l(v):w->vw}
порождает представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$
в $D$\Hyph модуле $A$
}
\end{ShadedLemma}

{\sc Доказательство.}
Согласно определениям
\RefDefinition{algebra over ring}
и
\RefDefinition{polylinear map of modules},
левый сдвиг $D$\Hyph модуля $A$
является линейным отображением.
Согласно определению
\refDefinition{linear map of D module}1,
отображение \(l\circ v\)
является эндоморфизмом $D$\Hyph модуля $A$.
Равенство
\ShowEq{l(v1+v2)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{def sum of linear maps}
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(v1+v2)}
является следствием равенства
\EqRef{l(v1+v2)w}.
Равенство
\ShowEq{l(dv)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(dv)}
является следствием равенства
\EqRef{l(dv)w}.
Лемма является следствием равенств
\EqRef{l(v1+v2)},
\EqRef{l(dv)}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{representation of D module in D module determines the product}
{\it
Представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
}
\end{ShadedLemma}

{\sc Доказательство.}
Поскольку отображение $g_{23}\circ v$ является эндоморфизмом $D$\Hyph модуля $A$, то
\ShowEq{endomorphism of module from product, 3}
Поскольку отображение $g_{23}$
является линейным отображением
\ShowEq{g23:A->L}
то,
\ShowEq{ref sum and product over scalar, linear map}
\ShowEq{endomorphism of module from product, 4}
\ShowEq{endomorphism of module from product, 7}
Из равенств
\EqRef{endomorphism of module from product, 3},
\EqRef{endomorphism of module from product, 4},
\EqRef{endomorphism of module from product, 7}
и определения
\RefDefinition{polylinear map of modules},
следует, что отображение $g_{23}$ является билинейным отображением.
Следовательно, отображение $g_{23}$ определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\hfill\(\odot\)

Теорема является следствием лем
\RefLemma{structure of D algebra is generated by product},
\RefLemma{representation of D module in D module determines the product}.
}

\DefLabeledTheorem{A module -> algebra is associative}{\SideNS}
{
Пусть $g$ - эффективное левостороннее представление $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$.
Тогда $D$\Hyph алгебра $A$ ассоциативна.
}

\DefProof{A module -> algebra is associative}
{
Пусть
\ShowEq{abc in A, v in v}
Равенство
\DrawEq{\SideWS module, associative law}0
является следствием утверждения, что \SideRu востороннее представление
$g$ является
\SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$.
Равенство
\ShowEq{a(b(cv))=(a(bc))v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Так как
\ShowEq{cv \SideNS}
равенство
\ShowEq{a(b(cv))=((ab)c)v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Равенство
\ShowEq{(a(bc))v=((ab)c)v \SideNS}
является следствием равенств
\EqRef{a(b(cv))=(a(bc))v \SideNS},
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Поскольку $v$ - произвольный вектор $A$\Hyph модуля $V$,
равенство
\ShowEq{a(bc)=(ab)c \SideNS}
является следствием равенства
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Следовательно, $D$\Hyph алгебра $A$ ассоциативна.
}

\DefLabeledTheoremNote{definition of A module}{\SideWS \VectorSetNS}
{
Пусть $V$ является \SideRu\What $\Base$\Hyph модулем.
Для любого вектора $v\in V$,
вектор, порождённый диаграммой представлений
\eqRef{diagram of representations, \SideWS module}1,
имеет следующий вид
\ShowEq{\SideWS module, (a+n)v=av+nv}
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\ShowEq{\SideWS module, a+n:V->V}
порождает\,\footnotemark
\algebrad $\Base_{(1)}$
где сложение определено равенством
\DrawEq{(a+n)+(b+m)=}{\SideWS module}
и произведение определено равенством
\DrawEq{(a+n)(b+m)=}{\SideWS module}
\algebraD $\Base_{(1)}$ называется
\AddIndex{унитальным расширением}{unital extension}
\ShortAlgebraRuBWS $\Base$.
\begin{table}[h]
%\caption{Active and Passive Representations}
%\label{table:Passive and Active Representations}
\begin{tabular}{|l|l|l|}
\hline
Если \algebrac $\Base$ имеет единицу, то
\ShowEq{A1=A unital extension}
Если \algebrac $\Base$ является идеалом $\CBase$, то
\ShowEq{A1=D unital extension}
В противном случае
\ShowEq{A1=A+D unital extension}
\end{tabular}
\end{table}
\item
\algebraD $\Base$ является \SideRu\What идеалом \ShortAlgebraRuBWS $\Base_{(1)}$.
\labelItem{Algebra is \SideWS ideal of algebra (1)}
\item
Множество преобразований
\EqRef{\SideWS module, (a+n)v=av+nv}
порождает \SideRu\HSide представление \ShortAlgebraRuBWS $\Base_{(1)}$ в абелевой группе $V$.
\labelItem{\SideWS representation of D1 in Abelian group}
\end{enumerate}
Мы будем пользоваться обозначением
\ShowEq{set of vectors generated by vector \Base}
для множества векторов, порождённых вектором $v$.
}
{Смотри определение унитального расширения также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 52,
\citeBib{Zharinov: foundation of mathematical physics}\Hyph 64.}

\DefLabeledTheorem{definition of A module, property}{\SideNS}
{
Элементы \SideRu\From $\Base$\Hyph модуля $V$ удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закон ассоциативности}{associative law}
\labelItem{associative law, \SideWS module}
\DrawEq{associative law, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\labelItem{distributive law, \SideWS module}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{закон унитарности}{unitarity law}
\labelItem{unitarity law, \SideWS \Base-module}
\ShowEq{unitarity law, \SideWS \Base-module}
\end{enumerate}
для любых
\ShowEq{p,q in D, v,w in V}
}

\AddEq{proof: definition of A module}
{%
{\sc Доказательство теорем
\refTheorem{definition of A module}{\SideWS \VectorSetNS},
\refTheorem{definition of A module, property}{\SideNS}.}
Пусть $v\in V$.

\begin{ShadedLemma}
\labelLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}
{\it
Пусть 
\ShowEq{module, d in D}
\ShowEq{module, a in A}
Отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
}
\end{ShadedLemma}

{\sc Доказательство.}
Утверждения
\ShowEq{\SideWS module, dv in V}
\ShowEq{\SideWS module, av in V}
являются следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{module over algebra}{\SideNS}.
Так как $V$ является абелевой группой, то
\ShowEq{\SideWS module, dv+av in V}
Следовательно,
для любого $\CBase$\Hyph числа $\DArg$
и любого $\Base$\Hyph числа $a$,
мы определили отображение
\EqRef{\SideWS module, a+n:V->V}.
Поскольку преобразование $\DTransf(\DArg)$
и \SideRu\HSide преобразование $\ATransf(a)$
являются эндоморфизмами абелевой группы $V$,
то отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
\hfill\(\odot\)

Пусть $\Base_{(1)}$ - множество отображений
\EqRef{\SideWS module, a+n:V->V}.
Равенство
\eqRef{distributive law, \SideWS module, 1}1
является следствием леммы
\RefLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}.

Пусть
\ShowEq{p,q in D1}
Согласно утверждению
\RefItem{representation of D1 in Abelian group},
мы определим сумму $\Base_{(1)}$\Hyph чисел $p$ и $q$ равенством
\eqRef{distributive law, \SideWS module, 2}1.
Равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=, 1}
является следствием равенства
\eqRef{distributive law, \SideWS module, 2}1.
Равенство
\ShowEq{distributive law, \CBase, \SideWS module, 2}
является следствием утверждения, что представление
$\DTransf$ является гомоморфизмом аддитивной группы кольца $\CBase$.
Равенство
\ShowEq{distributive law, \Base, \SideWS module, 2}
является следствием утверждения, что \SideRu\HSide представление
$\ATransf$ является гомоморфизмом аддитивной группы \ShortAlgebraRuBWS $\Base$.
Так как $V$ является абелевой группой, то равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=}
является следствием равенств
\EqRef{\SideWS module, (a+n)+(b+m)=, 1},
\EqRef{distributive law, \CBase, \SideWS module, 2},
\EqRef{distributive law, \Base, \SideWS module, 2}.
Из равенства
\EqRef{\SideWS module, (a+n)+(b+m)=}
следует, что определение
\eqRef{(a+n)+(b+m)=}{\SideWS module}
суммы на множестве $\Base_{(1)}$ не зависит от вектора $v$.

Равенства
\eqRef{associative law, \SideWS module}1,
\EqRef{unitarity law, \SideWS \Base-module}
являются следствием утверждения
\RefItem{\SideWS representation of D1 in Abelian group}.
Пусть
\ShowEq{p,q in D1}
\def\Temp{}
\ifx\SideNS\Temp
Равенство
\DrawEq{associative law, \CBase, \SideWS module}1
является следствием утверждения, что представление $\DTransf$
является представлением мультипликативной группы кольца $\CBase$.
Равенство
\DrawEq{\SideWS module, associative law}1
является следствием утверждения, что представление $g_2$
является представлением мультипликативной группы кольца $D$.
Равенство
\DrawEq{associative law, \CBase\Base, \SideWS module}1
является следствием утверждения, что кольцо $D$
является абелевой группой.
Равенство
\ShowEq{module, (a+n)(b+m)=}
является следствием равенств
\ShowEq{ref module, (a+n)(b+m)=}%
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\EqRef{module, (a+n)(b+m)=}.
\else%
Так как произведение в $D$\Hyph алгебре $A$ может быть неассоциативным,
то опираясь на теорему
\refTheorem{definition of A module, property}{\SideNS},
мы рассмотрим произведение
$\Base_{(1)}$\Hyph чисел $p$ и $q$
как билинейное отображение
\ShowEq{f:D1xD1->D1}
такое, что верны равенства
\DrawEq{fab=ab}{\SideWS module}
\DrawEq{f1p=p}{\SideWS module}
Равенство
\DrawEq{pq=fpq}{\SideWS module}
является следствием равенств
\eqRef{fab=ab}{\SideWS module},
\eqRef{f1p=p}{\SideWS module}.
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\eqRef{pq=fpq}{\SideWS module}.
\fi%

Утверждение
\RefItem{Algebra is \SideWS ideal of algebra (1)}
является следствием равенства
\eqRef{(a+n)(b+m)=}{\SideWS module}.
\qed
}

\DefLabeledDefinition{submodule}{\SideWS module}
{
Подпредставление $\Base$\Hyph \SideRu\From модуля $V$ называется
\AddIndex{подмодулем}{submodule}
\SideRu\From $\Base$\Hyph модуля $V$.
}

\AddEq{theorem: submodule}
{
\begin{ShadedTheorem}
\labelTheorem{submodule, \SideWS module}
Пусть
\ShowEq{vi V}{}
- множество векторов \SideRu\From $\Base$\Hyph модуля $V$.
Если векторы
\ShowEq{set vi cols}v
принадлежат подмодулю $V'$ \SideRu\From $\Base$\Hyph модуля $V$,
то линейная комбинация векторов
\ShowEq{set vi cols}v
принадлежит подмодулю $V'$.
\end{ShadedTheorem}
}

\DefProof{submodule}
{
Теорема является следствием
теоремы
\refTheorem{set of vectors generated by set of vectors}{\SideWS module}
и определений
\refDefinition{linear combination of vectors}{\SideNS},
\refDefinition{submodule}{\SideWS module}.
}

\AddEq{ref in item cvk module}
{
теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{definition of A \VectorSetNS}{\SideNS}
}

\AddEq{ref in item cvk vector space}
{
теоремы
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
}

\DefLabeledTheorem{set of automorphisms}{\SideNS}
{
Множество $GL(V)$
автоморфизмов
\SideRu вого $A$\Hyph векторного пространства $V$
является группой.
}

\DefLabeledTheorem{active transformations in module}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Любой автоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства
$V$ имеет вид
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{automorphism}
где $f$ - \ProductType невырожденная матрица.
Матрицы автоморфизмов \SideRu вого $A$\Hyph векторного пространства \ColsA порождают группу
%\Group nA.
$GL(V_*)$,
изоморфную группе $GL(V)$.
Автоморфизмы \SideRu вого $A$\Hyph векторного пространства \ColsA порождают
\OtherSideRu востороннее линейное
эффективное представление
\DrawEq[{GL(V_*)}{V_*}{}]{A->*B}{\SideNS-\Cols}
группы $GL(V_*)$
в \SideRu вом $A$\Hyph векторном пространстве $V_*$.
}

\DefLabeledTheoremNote{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
{
Пусть $V$ - \SideRu\To $\Base$\Hyph \VectorSetRuANS.
Множество векторов, порождённое множеством векторов
\ShowEq{v(i) V},
имеет вид\,\footnotemark
\DrawEq[{\Base}{\BaseExt}]{w=sum vi, \SideWS module}{\Base}
}
{Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.}

\AddEq{ref module structure of subrepresentations}
{
и теоремам
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{definition of A module}{\SideWS \VectorSetNS},
}

\AddEq{ref vector space structure of subrepresentations}
{
и теореме
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
}

\DefLabeledLemma{w=w12 in Xk-1}{\SideWS \VectorSetNS}
{\leftskip=25pt
Пусть
\ShowEq{w=w12 in Xk-1}.
Тогда $w\in J(v)$.
}

\DefLabeledLemma{w=aw in Xk-1}{\SideWS \VectorSetNS}
{\leftskip=25pt
Пусть
\ShowEq{w=aw in Xk-1,\SideNS}
Тогда $w\in J(v)$.
}

\DefProof{set of vectors generated by set of vectors}
{
Мы докажем теорему по индукции, опираясь на теорему
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

Для произвольного
\ShowEq{vk in Jv}{}
положим
\ShowEq{c(i)=dik}
Тогда
\DrawEq[{\Base_{\BaseExt}}{}]{v(k)=sum v(i), \SideWS module}{\Base}
Из равенств
\eqRef{w=sum vi, \SideWS module}{\Base},
\eqRef{v(k)=sum v(i), \SideWS module}{\Base}.
следует, что
теорема верна на множестве
\ShowEq{X0=v in J}

Пусть
\ShowEq{Xk in Jv}{k-1}
Согласно определению
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
\ShowEq{ref \VectorSet structure of subrepresentations}
если $w\in X_k$, то либо
\ShowEq{w=w12 in Xk-1},
либо
\ShowEq{w=aw in Xk-1,\SideNS}

{\leftskip=25pt
\ShowLemma{w=w12 in Xk-1}

{\sc Доказательство.}
Согласно равенству
\eqRef{w=sum vi, \SideWS module}{\Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{g(i)12}w
такие, что
\DrawEq[w]{w()12= \SideNS}{\VectorSetNS}
где множества
\DrawEq[w]{|c(i)12 ne 0|}{\SideWS \VectorSetNS}
конечны.
Так как $V$ - \SideRu\To $\Base$\Hyph \VectorSetRuANS,
то из равенств
\eqRef{distributive law, \SideWS module, 2}1,
\eqRef{w()12= \SideNS}{\VectorSetNS}
следует, что
\DrawEq[w]{w()1+w()2= \SideNS}{\VectorSetNS}
Из равенства
\eqRef{|c(i)12 ne 0|}{\SideWS \VectorSetNS}
следует, что
множество
\ShowEq{|gi() 1+2 ne 0|}w
конечно.
\hfill\(\odot\)

\ShowLemma{w=aw in Xk-1}

{\sc Доказательство.}
Согласно утверждению
\RefItem[\RefRepresentation]{ax in Xk+1},
для любого $\Base_{\BaseExt}$\Hyph числа $a$,
\ShowEq{aw in Xk \SideWS module}
Согласно равенству
\eqRef{w=sum vi, \SideWS module}{\Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{set au v(i)}w
такие, что
\ShowEq{w()= \SideWS module}
где
\DrawEq{|w(i) ne 0|}{\SideWS module}
Из равенства
\EqRef{w()= \SideWS module}
следует, что
\ShowEq{aw()= \SideWS module}
Из утверждения
\eqRef{|w(i) ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{\SideWS module, |aw(i) ne 0|}
конечно.
\hfill\(\odot\)

\,
}

Из лемм
\refLemma{w=w12 in Xk-1}{\SideWS \VectorSetNS},
\refLemma{w=aw in Xk-1}{\SideWS \VectorSetNS}
следует, что
\ShowEq{Xk in Jv}k
}

\DefLabeledTheorem{d in D->d in D1}{\SideWS module}
{
Отображение
\ShowEq{f:a in A->b in B}{I_{(1)}}d{\Base}{d+0}{\Base_{(1)}}
является гомоморфизмом \ShortAlgebraRuBWS $\Base$
в \ShortAlgebraRuEWS $\Base_{(1)}$.
}

\DefProof{d in D->d in D1}
{
Равенство
\DrawEq[{\AArg}]{(d1+0)+(d2+0)}{\SideWS module}
является следствием равенства
\eqRef{(a+n)+(b+m)=}{\SideWS module}.
Равенство
\DrawEq[{\AArg}]{(d1+0)(d2+0)}{\SideWS module}
является следствием равенства
\eqRef{(a+n)(b+m)=}{\SideWS module}.
Теорема является следствием равенств
\eqRef{(d1+0)+(d2+0)}{\SideWS module},
\eqRef{(d1+0)(d2+0)}{\SideWS module}.
}

\DefLabeledTheorem{da in DA->da in D1A}{\SideWS module}
{
Отображение
\ShowEq{da in DA->da in D1A}
является морфизмом \SideRu\From $\Base$\Hyph модуля $V$
в \SideRu\To $\Base_{(1)}$\Hyph модуль $V$.
}

\DefProof{da in DA->da in D1A}
{
Равенство
\ShowEq{da in DA->da in D1A 1, \SideWS module}
является следствием теоремы
\refTheorem{d in D->d in D1}{\SideWS module}.
Теорема является следствием равенства
\EqRef{da in DA->da in D1A 1, \SideWS module}
и определения
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra}.
}

\AddEq{convention: da in DA->da in D1A}
{
\begin{convention}
\labelConvention{da in DA->da in D1A, \SideWS module}
Согласно теоремам
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\refTheorem{da in DA->da in D1A}{\SideWS module},
множество слов, порождающих
\SideRu\To $\Base$\Hyph модуль $V$,
совпадает с множество слов, порождающих
\SideRu\To $\Base_{(1)}$\Hyph модуль $V$.
Поэтому, не нарушая общности,
мы будем предполагать, что \algebrac $\Base$
имеет единицу.
\qed
\end{convention}
}

\DefLabeledConvention{linear combination of vectors}{\SideNS}
{
Если необходимо явно указать,
что мы умножаем вектор $v(\gii)$
на $\Base_{\BaseExt}$\Hyph число $c(i)$ с\SideRu ва,
то мы будем называть выражение
\ShowEq{the \SideWS linear combination()}
\AddIndex{\SideRu вой линейной комбинацией}{\SideWS linear combination}.
Мы будем применять это соглашение к аналогичным терминам.
Например, мы будем говорить, что вектор
\ShowEq{w=c(i)v(i).\SideNS}
линейно зависит
от векторов
\ShowEq{set vi *}v
с\SideRu ва.
}

\DefLabeledDefinition{linear combination of vectors}{\SideNS}
{
Пусть $\Module$ - \SideRu\HSide \VectorSetRuA.
Пусть
\ShowEq{v(i) V}{}
- множество векторов.
\ShowEq{\SideWS linear combination()}%
Выражение
\ShowEq{A linear combination() =}
называется
\AddIndex{линейной комбинацией}{linear combination} векторов
\ShowEq{v(i)}
Вектор
\ShowEq{w=c(i)v(i).\SideNS}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от векторов
\ShowEq{v(i)}
}

\DefLabeledDefinition{generating set of module}{\SideNS}
{
$J(v)$
называется
\AddIndex{подмодулем, порождённым множеством}
{submodule generated by set} $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
подмодуля $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu\From $\Base$\Hyph модуля $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
}

\DefLabeledDefinition{generating set of vector space}{\SideNS}
{
$J(v)$
называется
векторным подпространством, порождённым множеством $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
векторного подпространства $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu вого $\Base$\Hyph векторного пространства $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
}

\DefText{generating set of module}
{
Следующее определение является следствием теорем
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\DefText{quasibasis of module}
{
Следующее определение является следствием теорем
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{basis of representation}.
}

\DefLabeledDefinition{basis of module}{\SideNS}
{
Если множество $X\subset V$ является множеством образующих
\SideRu\From $\Base$\Hyph \VectorSetRuB $V$, то любое множество $Y$, $X\subset Y\subset V$
также является множеством образующих \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
Если существует минимальное множество $X$, порождающее
\SideRu\To $\Base$\Hyph \VectorSetRuA $V$, то такое множество $X$ называется
\AddIndex{квазибазисом}{quasibasis} \SideRu\From $D$\Hyph \VectorSetRuB $V$.
}

\DefLabeledTheorem{linearly depends on rest of vectors}{\SideWS module}
{
Пусть $\Base$ - \DivAlgebraRu.
Если уравнение
\DrawEq[wv]{\SideWS wi vi=0}{1 \Cols}
предполагает существования индекса
\ShowEq{i=j}
такого, что
\ShowEq{wj ne 0}w,
то вектор
\ARow vj{}
линейно зависит от остальных векторов $v$.
}

\DefProof{linearly depends on rest of vectors}
{
Теорема является следствием равенства
\ShowEq{\SideWS vj=sum vi}vw
и определения
\refDefinition{linear combination of vectors}{\SideNS}.
}

\DefText{0=0vi}
{
Очевидно, что для любого множества векторов
\ARow vi{}
\ShowEq{\SideWS 0=0vi}
}

\DefLabeledDefinitionNote{linearly independent vectors}{\SideNS}
{
Множество векторов\,\footnotemark
\ShowEq{set vi *}v
\SideRu\From $\Base$\Hyph \VectorSetRuB $V$
\AddIndex{линейно независимо}{linearly independent set},
если
\ShowEq{w(i)=0}
следует из уравнения
\DrawEq{\SideWS w(i) v(i)=0}{}
В противном случае, множество векторов
\ShowEq{set vi *}v
\AddIndex{линейно зависимо}{linearly dependent set}.
}
{Я следую определению в
\citeBib{Serge Lang}, страница 100.}

\DefLabeledTheorem{quasibasis of module}{\SideNS}
{
Множество векторов
\ShowEq{basis, module}
является квазибазисом \SideRu\From $\Base$\Hyph модуля
$V$, если верны следующие утверждения.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{vector is linear combination of set, \SideWS module}
Произвольный вектор $v\in V$
является линейной комбинацией
векторов множества $\Basis e$.
\item
\labelItem{cannot be represented as a linear combination, \SideWS module}
Вектор $e(\gii)$
нельзя представить в виде линейной комбинации
остальных векторов множества $\Basis e$.
\end{enumerate}
}

\DefProof{quasibasis of module}
{
Согласно утверждению
\RefItem{vector is linear combination of set, \SideWS module},
теореме
\refTheorem{set of vectors generated by set of vectors}{\SideWS module}
и определению
\refDefinition{linear combination of vectors}{\SideNS},
множество $\Basis e$ порождает \SideRu\To $\Base$\Hyph модуль $V$
(определение
\refDefinition{generating set of module}{\SideNS}).
Согласно утверждению
\RefItem{cannot be represented as a linear combination, \SideWS module},
множество $\Basis e$ является минимальным множеством,
порождающим \SideRu\To $\Base$\Hyph модуль $V$.
Согласно определению
\refDefinition{generating set of module}{\SideNS},
множество $\Basis e$ является квазибазисом  \SideRu\From $\Base$\Hyph модуля $V$.
}

\DefLabeledTheorem{basis over division algebra}{\SideNS}
{
Пусть $\Base$ - \AlgebraRuNS\DivisionRuNS.
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом \SideRu\From $\Base$\Hyph векторного пространства}{basis, vector space}
$V$, если векторы
\ARow ei
линейно независимы и любой вектор $v\in V$
линейно зависит от векторов
\ARow ei.
}

\DefLabeledTheorem{vector space is free module}{}
{
\SideRuC\WhatO $\Base$\Hyph векторное пространство
является свободным $\Base$\Hyph модулем.
}

\DefProof{basis over division algebra}
{
Пусть множество векторов
\ShowEq{set vi \Cols}e
линейно зависимо. Тогда в равенстве
\DrawEq[we]{\SideWS wi vi=0}{}
существует индекс $\gii=\gij$ такой, что
\ShowEq{wj ne 0}w.
Согласно теореме
\refTheorem{linearly depends on rest of vectors}{\SideWS module},
вектор
\ARow ej{}
линейно зависит от остальных векторов множества $\Basis e$.
Согласно определению
\refDefinition{basis of module}{\SideNS},
множество векторов
\ShowEq{set vi \Cols}e
не является базисом \SideRu\From $\Base$\Hyph векторного пространства $V$.

Следовательно, если множество векторов
\ShowEq{set vi \Cols}e
является базисом, то эти векторы
линейно независимы.
Так как произвольный вектор $v\in V$
является линейной комбинацией векторов
\ShowEq{set vi \Cols}e
то множество векторов $v$,
\ShowEq{set vi \Cols}e
не является линейно независимым.
}

\DefLabeledConvention{unit of algebra in basis}{\Cols}
{
Пусть \eV - базис $D$\Hyph алгебры \ColsA $A$.
Если $D$\Hyph алгебра $A$ имеет единицу,
положим \ARow e0 - единица $D$\Hyph алгебры $A$.
}

\DefTheoremNote{algebra A2 representation in LA}
{
Пусть $A_1$ и $A_2$ являются $D$\Hyph алгебрами.
Пусть произведение в алгебре \AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{A2}
Линейное отображение
\ShowEq{representation A2 in LA}
определённое равенством
\ShowEq{representation A2 in LA, 1}
является представлением\,\footnotemark
алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
}
{Определение представления
$\Omega$\Hyph алгебры дано в определении
\ShowEq{ref definition: representation of algebra}.}

\DefLabeledTheorem[4]{matrix generates D module homomorphism}{\Cols(#1#2)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrix of numbers}D{#3}fiIjJ
Отображение\refFootnote{homomorphism of D module}{\Cols(#1#2)}
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{module, coordinates \Cols}
%\newline
определённое равенством
\ShowText{define homomorphism D module by matrix(#1)}
является гомоморфизмом
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$.
Гомоморфизм
\eqRef{homomorphism D algebra #1#2}{module, coordinates \Cols},
который имеет%
\ShowText{define homomorphism by given matrix()}%
определён однозначно.
}

\DefProof[5]{matrix generates D module homomorphism}
{
Равенство
\ShowEq{fo(v+w) \Cols(#1)}
\begin{sloppypar}
\noindent
является следствием равенств
\ShowRef{homomorphism of D module}{#1}{#2}{#5}
Из равенства
\EqRef{fo(v+w) \Cols(#1)}
следует, что отображение $\Vector f$ является гомоморфизмом
абелевой группы.
Равенство
\end{sloppypar}
\ShowEq{fo(va) \Cols(#1)}
является следствием равенства
\eqRef{left homomorphism, f av=}{f D module #1#2}.
Из равенства
\EqRef{fo(va) \Cols(#1)}
и определений
\RefDefinition{Morphism of Diagram of Representations},
\refDefinition{linear map of D module}{#1#2}
следует, что отображение
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{module, coordinates \Cols}
\newline
\begin{sloppypar}
\noindent
является гомоморфизмом
$D_{#1}$\Hyph модуля \ColsA $V_{#2}$
в $D_{#3}$\Hyph модуль \ColsA $V_{#4}$.
\end{sloppypar}

Пусть $f$ -
матрица гомоморфизмов $\Vector f$, $\Vector g$
относительно базисов
\ShowEq{Bases eVW}12{}.%
Равенство
\ShowEq{fov=gov \Cols(#1)}
является следствием теоремы
\refTheorem{linear map of D module}{#1#2}.
Следовательно, $\Vector f=\Vector g$.
}

\DefLabeledTheorem[4]{matrix generates D algebra homomorphism}{\Cols(#1#2)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrix of numbers and C}D{#3}fiIjJ{#1}{#2}
Отображение\refFootnote{homomorphism of d algebra}{#1#2\Cols}
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{module, coordinates \Cols}
%\newline
определённое равенством
\ShowText{define homomorphism D module by matrix(#1)}
является гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
Гомоморфизм
\eqRef{homomorphism D algebra #1#2}{module, coordinates \Cols},
который имеет%
\ShowText{define homomorphism by given matrix()}%
определён однозначно.
}

\DefProof[5]{matrix generates D algebra homomorphism}
{
Согласно теореме
\refTheorem{matrix generates D module homomorphism}{\Cols(#1#2)},
отображение
\eqRef{homomorphism D algebra #1#2}{module, coordinates \Cols}
является гомоморфизмом
$D_{#1}$\Hyph модуля $A_{#2}$
в $D_{#3}$\Hyph модуль $A_{#4}$
и гомоморфизм
\eqRef{homomorphism D algebra #1#2}{module, coordinates \Cols}
определён однозначно.

Пусть
\ShowEq{a=ai ei}a1i,
\ShowEq{a=ai ei}b1i.
Равенство
\DrawEq{algebra, homomorphism and product abe #1#2}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product #1#2}{\Cols}.
\ShowText{matrix generates D algebra homomorphism (#1)}
Равенство
\DrawEq{algebra, homomorphism and product abe 3(#1)}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product abe 2(#1)}{\Cols}
и равенства
\ShowRef{homomorphism of d algebra, coordinates 1}{#1}{#2}
Равенство
\DrawEq{algebra, homomorphism and product abe 4(#1)}{\Cols}
является следствием равенства
\ShowEq{algebra, homomorphism and product, 1}
Равенство
\DrawEq{algebra, homomorphism and product abe 5(#1)}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product abe 4(#1)}{\Cols}
и равенства
\ShowRef{homomorphism of d algebra, coordinates 1}{#1}{#2}
Равенство
\ShowRef{homomorphism, f vw=}{#1}{#2}
является следствием равенств
\ShowRef{algebra, homomorphism and product 1}{#1}{#2}
Согласно теореме
\refTheorem{homomorphism from A1 to A2, D algebra}{#1#2},
отображение
\eqRef{homomorphism D algebra #1#2}{module, coordinates \Cols}
является гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
}

\DefText{matrix generates D algebra homomorphism (1)}
{
Так как отображение $h$ является гомоморфизмом
кольца $D_1$ в кольцо $D_2$, то
\DrawEq{algebra, homomorphism and product abe 2}{\Cols}
Равенство
\DrawEq{algebra, homomorphism and product abe 2(1)}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product abe 2}{\Cols}
и равенства
\ShowRef{product in algebra}
}

\DefText{matrix generates D algebra homomorphism ()}
{
Равенство
\DrawEq{algebra, homomorphism and product abe 2()}{\Cols}
является следствием равенства
\ShowRef{product in algebra}
}

\DefLabeledFootnote[4]{homomorphism of D module}{\Cols(#1#2)}
{
В теоремах
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
\refTheorem{matrix generates D module homomorphism}{\Cols(#1#2)},
мы опираемся на следующее соглашение.
\ShowEq{Let be basis of module}1{}iI{}D{#1}V{#2}
\ShowEq{Let be basis of module}2{}jJ{}D{#3}V{#4}
}

\DefLabeledFootnote[6]{homomorphism of A module}{\SideNS-\Cols(#1#2#3)}
{
В теоремах
\refTheorem{homomorphism A module}{\SideNS-\Cols(#1#2#3)},
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)},
мы опираемся на следующее соглашение.
\ShowEq{prolog homomorphism of vector space(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
}

\DefLabeledDefinition[4]{homomorphism from A1 to A2, D algebra}{#1#2}
{
\ShowText{algebra over ring (#1#2)}
Пусть
\DrawEq[{#1}{1.}{#2}h]{diagram of representations of D algebra}{->1(#1#2)}
диаграмма представлений, описывающая $D_1$\Hyph алгебру $A_1$.
Пусть
\DrawEq[{#3}{2.}{#4}h]{diagram of representations of D algebra}{->2(#1#2)}
диаграмма представлений, описывающая $D_2$\Hyph алгебру $A_2$.
Морфизм
\DrawEq[fA]{homomorphism D algebra #1#2}1
диаграммы представлений
\eqRef{diagram of representations of D algebra}{->1(#1#2)}
в диаграмму представлений
\eqRef{diagram of representations of D algebra}{->2(#1#2)}
называется
\AddIndex{гомоморфизмом}{homomorphism}
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
Обозначим
\ShowEq{set homomorphisms, D algebra #1#2}
множество гомоморфизмов
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
}

\DefLabeledTheorem[5]{homomorphism from A1 to A2, D algebra}{#1#2}
{
Гомоморфизм
\newline
\FrameEqRef[fA]{homomorphism D algebra #1#2}1
\newline
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$
- это линейное отображение
\eqRef[fA]{homomorphism D algebra #1#2}1
$D_{#1}$\Hyph модуля $A_{#2}$
в $D_{#3}$\Hyph модуль $A_{#4}$
такое, что
\DrawEq[fab]{homomorphism, f vw=}{(#1#2)g}
и удовлетворяет следующим равенствам
\ShowEq{define homomorphism of D algebra #1#2}{#1}{#2}{#5}
}

\DefProof[4]{homomorphism from A1 to A2, D algebra}
{
Согласно определениям
\ShowRef{Morphism of Diagram of Representations}
отображение
\eqRef{homomorphism D algebra #1#2}1
явлется морфизмом представления $h_{1.12}$,
описывающего $D_{#1}$\Hyph модуль $A_{#2}$,
в представления $h_{2.12}$,
описывающего $D_{#3}$\Hyph модуль $A_{#4}$.
Следовательно, отображение $f$ является линейным отображением $D_{#1}$\Hyph модуля $A_{#2}$
в $D_{#3}$\Hyph модуль $A_{#4}$ и равенства
\ShowEq{ref homomorphism of D algebra(#1)}{#1}{#2}
являются следствием теоремы
\refTheorem{linear map of D module}{#1#2}.

Согласно определениям
\ShowRef{Morphism of Diagram of Representations}
отображение $f$
явлется морфизмом представления $h_{1.23}$
в представления $h_{2.23}$.
Равенство
\DrawEq{morphism of representation, algebra, 23}{#1#2}
следует из равенства
\eqRef{morphism of representations of universal algebra, 2m}{representation}.
Из равенств
\eqRef{diagram of representations of D algebra}{->1(#1#2)},
\eqRef{diagram of representations of D algebra}{->2(#1#2)},
\eqRef{morphism of representation, algebra, 23}{#1#2},
следует
\DrawEq{algebra, morphism of representation 23, 1}{#1#2}
Равенство
\eqRef{homomorphism, f vw=}{(#1#2)g}
следует из равенств
\eqRef{product in D algebra}{definition},
\eqRef{algebra, morphism of representation 23, 1}{#1#2}.
}

\AddEq{definition: unital algebra}
{
\begin{ShadedDefinition}
\labelDefinition{unital algebra}
Если произведение в $D$\Hyph алгебре $A$ имеет единичный элемент,
то $D$\Hyph алгебра $A$ называется
\AddIndex{унитальной алгеброй}{unital algebra}.\,\footnotemark
\end{ShadedDefinition}
\footnotetext{\,
Смотри определение унитальной алгебры также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 137.
}
}

\DefDefinition{division algebra}
{
\(D\)\Hyph алгебра \(A\) называется
\AddIndex{алгеброй с делением}{division algebra},
если для любого \(A\)\Hyph числа \(a\ne 0\)
существует \(A\)\Hyph число \(a^{-1}\).
}

\DefTheorem{division algebra}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Из утверждения
\ShowEq{ab=ac a ne 0}
следует, что $b=c$.
}

\DefProof{division algebra}
{
Равенство
\ShowEq{ab=ac a ne 0 1}
является следствием утверждения
\EqRef{ab=ac a ne 0 1}.
}

\DefLabeledDefinition[4]{linear map of D module}{#1#2}
{
Морфизм представлений
\DrawEq[fV]{homomorphism D algebra #1#2}{module}
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$
называется гомоморфизмом или
\AddIndex{линейным отображением}{linear map}
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$.
Обозначим
\ShowEq{set linear maps, module (#1#2)}DV
множество линейных отображений
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$.
}

\DefTheorem[3]{module of skew symmetric polylinear maps}
{
Множество
\ShowEq{module of skew symmetric polylinear maps}{#1}{#2}{#3}
косо симметричных полилинейных отображений
является $D$\Hyph модулем.
}

\AddEq[3]{remark: module of skew symmetric polylinear maps}
{
Не нарушая общности, мы положим
\ShowEq{L(A1,A0,B)=}{#1}{#2}{#3}
}

\DefTheorem{norm in D module A->B}
{
Пусть $A$ - нормированный $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - нормированный $D$\Hyph модуль с нормой $|y|_B$.
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
}

\DefTheorem{set of A->B is D module}
{
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $|y|_B$.
\StartLabelItem
\begin{enumerate}
\item
Множество
$B^A$
отображений
\ShowEq{f:A->B}fAB
является $D$\Hyph модулем.
\labelItem{set of A->B is D module}
\item
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\labelItem{norm of map}
\end{enumerate}
}

\DefTheorem{symmetrization of polylinear map}
{
Пусть
\ShowEq{f in L(A->B)}D{A^n}B{}
- полилинейное отображение.
Тогда отображение
\ShowEq{symmetrization of polylinear map}
\EqParm{<f>}{=c}
определённое равенством
\ShowEq{symmetrization of polylinear map =}
является симметричным полилинейным отображением
и называется
\AddIndex{симметрированием полилинейного отображения}{symmetrization of polylinear map}
$f$.
}

\DefTheorem{exterior product = skew symmetric}
{
Внешнее произведение удовлетворяет следующему равенству
\ShowEq{exterior product = skew symmetric}
}

\DefProof{exterior product = skew symmetric}
{
Равенство
\EqRef{exterior product = skew symmetric}
является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =}.
}

\DefDefinition{exterior product polylinear map}
{
Косо симметричное полилинейное отображение
\ShowEq{exterior product}
\ShowEq{exterior product =}
называется
\AddIndex{внешним произведением}{exterior product}.
}

\AddEq{remark: product of polylinear maps}
{
Если $B_1=B_2$, то в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем произведение $B_1$\Hyph чисел
\ShowEq{f()},
\ShowEq{g()}.
Согласно теореме
\RefTheorem{Free Algebra over Ring},
это определение совместимо с определением
\RefDefinition{product of polylinear maps}.
}

\AddEq{definition: product of polylinear maps}
{
\begin{ShadedDefinition}
\labelDefinition{product of polylinear maps}
Пусть $A$, $B_2$ - свободные алгебры над коммутативным кольцом $D$.\,\footnotemark
Пусть
\ShowEq{h:B1->*B2}
левостороннее представление
свободной ассоциативной $D$\Hyph алгебры $B_1$ в $D$\Hyph модуле $B_2$.
Отображение
\ShowEq{hpq:Lpq->Lp+q}
определено равенством
\ShowEq{hpq(fg)=}
где в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем левостороннее произведение
$B_2$\Hyph числа
\ShowEq{g()}{}
на $B_1$\Hyph число
\ShowEq{f()}.
\end{ShadedDefinition}
\footnotetext{\,
Я дал определение произведения косо симметричных полилинейных отображениий
согласно определению в разделе
\citeBib{Cartan differential form}-1.4 главы 3,
страницы 195 - 198.
}
}

\DefDefinition{symmetric polylinear map}
{
Пусть $A$, $B$ - алгебры над коммутативным кольцом $D$.
Полилинейное отображение
\ShowEq{f in L(A->B)}D{A^n}B{}
называется
\AddIndex{симметричным}{symmetric polylinear map},
если
\ShowEq{fa=fsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}.
}

\DefTheoremNote{fx1n=0, xi=xi1}
{
Полилинейное отображение
\ShowEq{f in L(A->B)}D{A^n}B{}
косо симметрично тогда и только тогда, когда
\ShowEq{fx1n=0}
при условии
$a_i=a_{i+1}$
хотя бы для одного\,\footnotemark
\ShowEq{1<=i<n}
}{
В книге
\citeBib{Cartan differential form},
страница 192,
Анри Картан рассматривает теорему
\RefTheorem{fx1n=0, xi=xi1}
как определение косо симметричного отображения.
}

\DefTheorem[3]{alternation of polylinear map}
{
Пусть
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
- полилинейное отображение.
Тогда отображение
\ShowEq{alternation of polylinear map}
\ShowEq{[f]},
определённое равенством
\ShowEq{alternation of polylinear map =}
является косо симметричным полилинейным отображением
и называется
\AddIndex{альтернацией полилинейного отображения}{alternation of polylinear map}
$f$.
}

\DefDefinition[3]{skew symmetric polylinear map}
{
Полилинейное отображение
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
называется
\AddIndex{косо симметричным}{skew symmetric polylinear map},
если
\ShowEq{fa=sfsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}.
}

\DefLabeledTheorem{linear dependence between vectors of basis}{\SideWS module}
{
Пусть $\Base$ - \Algebra.
Пусть $\Basis e$ - квазибазис \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
Пусть
\DrawEq[ce]{\SideWS wi vi=0}{we \Cols}
линейная зависимость векторов квазибазиса $\Basis e$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
$\Base_{\BaseExt}$\Hyph число
\ShowEq{ci i in I}
не имеет обратного элемента
в \ShortAlgebraRuDWS $\Base_{\BaseExt}$.
\item
Множество $\Base'$ матриц
\ShowEq{c=ci i in I}
порождает \SideRu\To $\Base$\Hyph модуль $\Base'$.
\end{enumerate}
}

\DefProof{linear dependence between vectors of basis}
{
Допустим существует матрица
\ShowEq{c=ci i in I}
такая, что равенство
\eqRef{\SideWS wi vi=0}{we \Cols}
верно и существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}c.
Если мы положим, что $\Base$\Hyph число
\ACol cj
имеет обратный, то равенство
\ShowEq{\SideWS vj=sum vi}ec
является следствием равенства
\eqRef{\SideWS wi vi=0}{we \Cols}.
Следовательно вектор
\ARow ej{}
является линейной комбинацией остальных векторов множества $\Basis e$
и множество $\Basis e$ не является квазибазисом.
Следовательно, наше предположение неверно,
и $\Base_{\BaseExt}$\Hyph число
\ACol cj
не имеет обратного.

Пусть матрицы
\ShowEq{b in D'}b,
\ShowEq{b in D'}c.
Из равенств
\DrawEq[be]{\SideWS wi vi=0}{}
\DrawEq[ce]{\SideWS wi vi=0}{}
следует
\ShowEq{(b+c)*e, \SideWS module}
Следовательно, множество $\Base'$ является абелевой группой.

Пусть матрица
\ShowEq{b in D'}c{}
и $a\in\Base$.
Из равенства
\DrawEq[ce]{\SideWS wi vi=0}{}
следует
\ShowEq{(ac)*e, \SideWS module}
Следовательно, абелевая группа $\Base'$ является \SideRu\What $\Base$\Hyph модулем.
}

\DefLabeledTheorem{coordinates of vector with linear dependence}{\SideWS module}
{
Пусть \SideRu\To $\Base$\Hyph модуль $V$
имеет квазибазис $\Basis e$ такой, что в равенстве
\DrawEq[ce]{\SideWS wi vi=0}{2 we \Cols}
существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}c.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Матрица
\ShowEq{c=ci i in I}
определяет координаты вектора $0\in V$ относительно базиса $\Basis e$.
\labelItem{coordinates of vector 0 with linear dependence, \SideWS module}
\item
Координаты вектора $\Vector v$ относительно базиса $\Basis e$
определены однозначно с точностью до выбора координат вектора $0\in V$.
\labelItem{coordinates of vector with linear dependence, \SideWS module}
\end{enumerate}
}

\DefProof{coordinates of vector with linear dependence}
{
Утверждение
\RefItem{coordinates of vector 0 with linear dependence, \SideWS module}
является следствием равенства
\eqRef{\SideWS wi vi=0}{2 we \Cols}
и определения
\refDefinition{coordinates of vector}{\SideWS \VectorSetNS}.

Пусть вектор $\Vector v$ имеет разложение
\DrawEq{vv=ve \SideWS module}{2}
относительно квазибазиса $\Basis e$.
Равенство
\ShowEq{v=v+0, \SideWS module}
является следствием равенств
\eqRef{\SideWS wi vi=0}{2 we \Cols},
\eqRef{vv=ve \SideWS module}{2}.
Утверждение
\RefItem{coordinates of vector with linear dependence, \SideWS module}
является следствием равенств
\eqRef{vv=ve \SideWS module}{2},
\EqRef{v=v+0, \SideWS module}
и определения
\refDefinition{coordinates of vector}{\SideWS \VectorSetNS}.
}

\DefLabeledTheorem{quasibasis of module is basis}{\SideWS \VectorSetNS}
{
Пусть \SideRu\To $\Base$\Hyph модуль $V$
имеет квазибазис $\Basis e$ такой, что из равенства
\DrawEq[ce]{\SideWS wi vi=0}{3 ce \Cols}
следует, что
\ShowEq{ci=0 1n}
Тогда квазибазис $\Basis e$ является
базисом \SideRu\From $\Base$\Hyph модуля $V$.
}

\DefProof{quasibasis of module is basis}
{
Теорема является следствием определения
\RefDefinition{basis of representation}
и теоремы
\refTheorem{coordinates of vector with linear dependence}{\SideWS module}.
}

\DefLabeledDefinitionNote{free module over ring}{\SideNS}
{
\SideRuC\To $\Base$\Hyph модуль $V$ -
\AddIndex{свободный \SideRu\To $\Base$\Hyph модуль}{free module},\,\footnotemark
если \SideRu\To $\Base$\Hyph модуль $V$ имеет базис.
}
{
Я следую
определению в \citeBib{Serge Lang}, страница 103.
}

\DefProof{coordinates of vector of free module}
{
Теорема является следствием теоремы
\refTheorem{coordinates of vector with linear dependence}{\SideWS module}
и определений
\refDefinition{linearly independent vectors}{\SideNS},
\refDefinition{free module over ring}{\SideNS}.
}

\DefTheoremNote{standard representation of map A->A, associative algebra}
{
Пусть $A$ - конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis F$
- базис\,\footnotemark
левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}DAA{}
имеет следующее разложение
\labelItem{map f generated by basis F, associative algebra}
\DrawEq{map f generated by basis F}{associative algebra}
где
\ShowEq{fk= in AxA}
\item
Линейное отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, o, associative algebra}
\end{enumerate}
}{
Если $D$\Hyph модуль $A$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\ShowEq{f:A->B}fAA
порождённого множеством линейных отображений $\Basis F$.
}

\DefProof{standard representation of map A->A, associative algebra}
{
Поскольку $\Basis F$ является базисом левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA,
то согласно определению
\refDefinition{free module over ring}{\SideNS},
существует разложение
\DrawEq[A]{expansion of linear map with respect to basis}A
линейного отображения $f$ относительно базиса $\Basis F$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{associative algebra}
Равенство
\eqRef{map f generated by basis F}{associative algebra}
является следствием равенств
\eqRef{expansion of linear map with respect to basis}A,
\eqRef{f=fkxfk}{associative algebra}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A->A, associative algebra}
следует из равенств
\eqRef{map f generated by basis F}{associative algebra},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheoremNote{set FoG generates left module L(A;B), n<m}
{
Пусть $A$ - $D$\Hyph модуль,
\ShowEq{n=dim A}nA.
Пусть $B$ - ассоциативная $D$\Hyph алгебра,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{gi n<m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}1
порождает левый \BoxB{B}модуль\,\footnotemark
\ShowEq{L(A->B)}DAB.
}{
Я не утверждаю, что это множество является базисом,
так как отображения
\ShowEq{FijG}
могут быть линейно зависимыми.
}

\DefProof{set FoG generates left module L(A;B), n<m}
{
Пусть
\ShowEq{f:A->B}gAB
линейное отображение.
Пусть $\Basis e_A$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis e_B$ - базис $D$\Hyph модуля $B$.
Согласно теореме
\ShowEq{ref linear map of D1 D2 module, coordinates}
линейное отображение $G$ имеет координаты
\ShowEq{matrix amn}Gmn
относительно базисов $\Basis e_A$, $\Basis e_B$
и линейное отображение $g$ имеет координаты
\ShowEq{matrix amn}gmn
относительно базисов $\Basis e_A$, $\Basis e_B$.
Строка $G_{\gii}$ матрицы $G$,
также как строка $g_{\gii}$ матрицы $g$,
является координатами линейной формы
\ShowEq{A->B}AD.
Поскольку матрица $G$ имеет максимальный ранг,
то строки матрицы $G$ порождают $D$\Hyph модуль
\ShowEq{L(A->B)}DAD{}
и строки матрицы $g$ являются линейной комбинацией строк матрицы $G$
\ShowEq{g=CG}
Поскольку мы можем рассматривать матрицу $C$
как координаты линейного отображения
\ShowEq{f:A->B}CBB
то равенство
\ShowEq{g=(cF)G}
является следствием равенства
\EqRef{g=CG}
и равенства
\ShowEq{C=cF}
Поскольку
\ShowEq{Gkj in D}
то равенство
\ShowEq{g=c(FG)}
является следствием равенства
\EqRef{g=(cF)G}.
Следовательно, отображение $g$ принадллежит
линейной оболочке множества отображений
\eqRef{F o G}1.
}

\DefTheorem{set FoG generates left module L(A;B), n>m}
{
Пусть
\ShowEq{n=dim A}nA,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{gi n>m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B), n>m}
{
Доказательство теоремы похоже на доказательство теоремы
\RefTheorem{set FoG generates left module L(A;B), n<m}.
Однако, так как число строк матрицы $G$ меньше размерности
$D$\Hyph модуля $A$, то строки матрицы $G$ не порождают $D$\Hyph модуль
\ShowEq{L(A->B)}DAD{}
и отображение $G$ имеет нетривиальное ядро.
В частности, строки матрицы $g$ линейно зависят от строк матрицы $G$
тогда и только тогда, когда
\ShowEq{ker G in ker g}g.
}

\DefTheorem{set FoG generates left module L(A;B)}
{
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B)}
{
Нетрудно убедиться, что теорема
\RefTheorem{set FoG generates left module L(A;B), n<m}
является частным случаем теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
так как в теореме
\RefTheorem{set FoG generates left module L(A;B), n>m}
$\ker G=\emptyset$.
}

\AddEq{remark: set FoG generates left module L(A;B), n>m}
{
Из теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
следует, что
выбор отображения $G$ зависит от отображения $g$.
}

\DefTheorem{basis D module L(D->A)}
{
%Пусть тождественное отображение
%\ShowEq{f:A->B}IDD
%является базисом $D$\Hyph модуля
%\ShowEq{L(A->B)}DDD.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Тогда множество отображений
\ShowEq{d->dei}i
является базисом $D$\Hyph модуля
\ShowEq{L(A->B)}DDA.
}

\DefProof{basis D module L(D->A)}
{
Теорема является следствием равенства
\ShowEq{f(t)=fit ei}
}

\DefDefinition{component of linear map}
{
Выражение
\ShowEq{component of linear map}
в равенстве
\EqRef{fk= in AxA}
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
Выражение
\ShowEq{standard component of linear map}
в равенстве
\EqRef{standard representation of map A->A, associative algebra}
называется
\AddIndex{стандартной компонентой линейного отображения}
{standard component of linear map} $f$.
}

\DefTheorem{endomorphism of module from product}
{
Представление
\ShowEq{endomorphism of module from product}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
эквивалентно структуре $D$\Hyph алгебры $A$.
}

\DefLabeledConvention{sum av() convention}{\SideNS}
{
Мы будем пользоваться соглашением о сумме,
в котором повторяющийся индекс
в линейной комбинации
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av()\SideNS}
Я буду явно указывать множество индексов, если это необходимо.
}

\DefConvention{av=sum av convention}
{
Мы будем пользоваться соглашением Эйнштейна о сумме,
в котором повторяющийся индекс (один вверху и один внизу)
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av convention}
Я буду явно указывать множество индексов, если это необходимо.
}

\DefTheorem{effective representation of the ring}
{
%Пусть кольцо $D$ имеет единицу $e$.
Представление
\ShowEq{f:A->*B}fDA
кольца $D$
в абелевой группе $A$
\AddIndex{эффективно}{effective representation}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
}

\DefProof{effective representation of the ring}
{
Если $a$, $b\in R$
порождают одно и то же преобразование, то
\ShowEq{representation of ring, 1}
для любого $m\in A$.
Из равенств
\EqRef{sum of transformations of Abelian group, 1},
\EqRef{representation of ring, 1}
следует, что
\ShowEq{representation of ring, 2}
Равенство
\ShowEq{f(a-b)=0}
является следствием равенств
\EqRef{0ov=0},
\EqRef{representation of ring, 2}.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
}

\DefTheorem{Representation of ring f(0)=v0}
{
Представление
\ShowEq{f:A->*B}fDA
кольца $D$
в абелевой группе $A$
удовлетворяет равенству
\ShowEq{f(0)=v0}
где
\ShowEq{0:A->A}
отображение такое, что
\ShowEq{0ov=0}
}

\DefProof{Representation of ring f(0)=v0}
{
Равенство
\ShowEq{fa=fa+f0}
является следствием равенства
\EqRef{sum of transformations of Abelian group, 1}.
Равенство
\ShowEq{f0x=0}
является следствием равенства
\EqRef{fa=fa+f0}.
Равенство
\EqRef{0ov=0}
является следствием равенств
\EqRef{f(0)=v0},
\EqRef{f0x=0}.
}

\DefText{sum of transformations of Abelian group}
{
Сумма преобразований $f$ и $g$ абелевой группы определяется согласно
правилу
\ShowEq{(f+g)(a)=}
Поэтому, рассматривая представление
\ShowEq{f:A->*B}fDA
кольца $D$ в абелевой группе $A$, мы полагаем
\ShowEq{f(a)+f(b)=}
Согласно определению
\RefDefinition{representation of algebra},
отображение $f$ является гомоморфизмом кольца $D$.
Следовательно
\ShowEq{f(a+b)=f(a)+f(b)}
Равенство
\ShowEq{sum of transformations of Abelian group, 1}
является следствием равенств
\EqRef{f(a)+f(b)=},
\EqRef{f(a+b)=f(a)+f(b)}.
}

\AddEq{remark: we do not have definition of determinant for division algebra}
{
Согласно
\citeBib{q-alg-9705026},
\citeBib{math.QA-0208146},
у нас нет определения
детерминанта в случае алгебры с делением.\,\footnote{
В алгебре кватернионов профессор Кирчей
пользуется двойным определителем
(смотри определение в разделе
\citeBib{1812.03397}\Hyph 2.2)
для решения системы линейных уравнений
и для решения задачи о собственных значениях
(смотри раздел
\citeBib{1812.03397}\Hyph 2.5).
Я ограничился рассмотрением квазидетерминантов,
так как меня интересует более широкий класс алгебр.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOn

\FrameCiteBib{1812.03397}
\fi
}
Тем не менее, мы можем определить квазидетерминант,
который в конечном итоге даёт похожую картину.
В определении
\RefDefinition{RC-quasideterminant},
я следую определению
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=9}{1.2.2}.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOn

\FrameCiteBib{q-alg-9705026}
\FrameCiteBib{math.QA-0208146}
\fi
}

\DefConvention{basis of algebra as basis of module}
{
Согласно определениям
\refDefinition{free module over ring}{},
\RefDefinition{algebra over ring}
свободная $D$\Hyph алгебра $A$ - это
$D$\Hyph модуль $A$,
который имеет базис \eV[][.]
Однако, вообще говоря, \eV не является
базисом $D$\Hyph алгебры $A$,
так как в $D$\Hyph алгебре $A$ определено произведение.
Например, в алгебре кватернионов произвольный кватернион
\ShowEq{any quaternion}
может быть представлен в виде
\ShowEq{any quaternion i j ij}
Однако при решении большинства задач
использование базиса $D$\Hyph модуля $A$ проще, чем
использование базиса $D$\Hyph алгебры $A$.
Например, легче определить координаты $H$\Hyph числа относительно базиса
$(1,i,j,k)$
$R$\Hyph векторного пространства $H$,
чем определить координаты $H$\Hyph числа относительно базиса
$(1,i,j)$
$R$\Hyph алгебры $H$.
Поэтому фраза "мы рассматриваем базис $D$\Hyph алгебры $A$"
означает, что мы рассматриваем $D$\Hyph алгебру $A$
и базис $D$\Hyph модуля $A$.
}

\DefConvention{we use separate color for index of element}
{
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
}

\DefTheorem{direct sum of n Abelian groups}
{
Прямая сумма абелевых групп
\ShowEq{a1n}An{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}A
}

\AddEq{remark: direct sum of n Abelian groups}
{
Пусть
\ShowEq{a1o+.n}An
прямая сумма абелевых групп
\ShowEq{a1n}An.
Согласно доказательству теоремы
\RefTheorem{direct sum of Abelian groups},
произвольное $A$\Hyph число $a$ имеет вид
$(a_1,...,a_n)$
где $a_i\in A_i$.
Мы также будем пользоваться записью
\ShowEq{a=a1 o+ an}
}

\AddEq{theorem: direct sum of n D modules}
{
\begin{ShadedTheorem}
\labelTheorem{direct sum of n \SideWS \Base-\VectorsSetNS}
Прямая сумма \SideRu вых $\Base$\Hyph \VectorsSetRuB
\ShowEq{a1n}{\Module}n{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}{\Module}
\end{ShadedTheorem}
}

\DefLabeledTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\Module}n{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\Module}n
Представим $\VNumber$\Hyph число
\ShowEq{A 1o+.n}{\VNumber}n
как вектор столбец
\DrawEq[{\VNumber}n]{a=(a1.n col)}{}
Представим линейное отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
как вектор строку
\DrawEq[fn]{a=(a1.n row)}{}
\ShowEq{f:A->B}{\aD fi}{\aU {\Module}i}{\ModuleA}
Тогда значение отображения $f$ в $\Module$\Hyph числе $\VNumber$
можно представить как произведение матриц
\DrawEq[{\VNumber}{}]{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
}

\DefProof{foa=fi ai}
{
Теорема является следствием определения
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
}

\DefLabeledTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\ModuleA}m{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\ModuleA}m
Представим $\ModuleA$\Hyph число
\ShowEq{A 1o+.n}{\VNumberA}m
как вектор столбец
\DrawEq[{\VNumberA}m]{a=(a1.n col)}{}
Тогда линейное отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
имеет представление как вектор столбец отображений
\DrawEq[fm]{a=(a1.n col)}{}
таким образом, что если
\ShowEq{b=foa}{\VNumberA}{\VNumber}
то
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{}
}

\DefProof{foa=fi a}
{
Теорема является следствием теоремы
\RefTheorem{map from product into product}.
}

\DefTheorem{standard component of tensor, module}
{
Тензорное произведение $\Tensor A$ свободных
конечномерных модулей
$A_1$, ..., $A_n$
над коммутативным кольцом $D$ является свободным
конечномерным модулем.

Пусть
\ShowEq{tensor product of algebras, basis i}
- базис модуля $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
Выражение
$\ShowSymbol{standard component of tensor}{}$
определено однозначно и называется
\AddIndex{стандартной компонентой тензора}{standard component of tensor}.
}

\DefLabeledTheorem{map of direct sum of modules}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\Module}n,
\ShowEq{A 1n}{\ModuleA}m{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\Module}n
\ShowEq{A 1o+.n}{\ModuleA}m
Представим $\Module$\Hyph число
\ShowEq{A 1o+.n}{\VNumber}n
как вектор столбец
\DrawEq[{\VNumber}n]{a=(a1.n col)}{v,\SideWS \Base-\VectorsSetNS}
Представим $\ModuleA$\Hyph число
\ShowEq{A 1o+.n}{\VNumberA}m
как вектор столбец
\DrawEq[{\VNumberA}m]{a=(a1.n col)}{w,\SideWS \Base-\VectorsSetNS}
Тогда линейное отображение
\ShowEq{f:A->B}fVW
имеет представление как матрица отображений
\DrawEq[fnm]{a=(a11.nm matrix)}{f,\SideWS \Base-\VectorsSetNS}
таким образом, что если
\ShowEq{b=foa}{\VNumberA}{\VNumber}
то
\DrawEq[f{\VNumberA}{\VNumber}nm]{b=f rco a}{\SideWS \Base-\VectorsSetNS}
Отображение
\ShowEq{fij:->}{\Module}{\ModuleA}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}
}

\DefProof{map of direct sum of modules}
{
Согласно теореме
\refTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS},
существует множество линейных отображений
\ShowEq{fi:->}
таких, что
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{\SideWS \Base-\VectorsSetNS}
Согласно теореме
\refTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS},
для каждого $\gii$,
существует множество линейных отображений
\ShowEq{fij:->}{\Module}{\ModuleA}
таких, что
\DrawEq{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}
Если мы отождествим матрицы
\ShowEq{fij=(fi)j}
то равенство
\eqRef{b=f rco a}{\SideWS \Base-\VectorsSetNS}
является следствием равенств
\eqRef{foa=fi a}{\SideWS \Base-\VectorsSetNS},
\eqRef{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}.
}

\DefDefinition{Matrix of tensors}
{
Пусть $a$ - матрица и
\ShowEq{a in Aoxn}{\aUD aij}n.
Матрица $a$ называется матрицей тензоров
\ShowEq{Aoxn}n.
}

\AddEq{remark: map of direct sum of modules}
{
Пусть
\ShowEq{aU A1n}Bm{}
- $D$\Hyph алгебры.
Тогда мы можем записать линейное отображение $\aUD fij$
с помощью \BoxB{\aU Bi}чисел.
}

\DefText{Free Algebra over Ring}
{
Пусть $D$ - коммутативное кольцо и $A$ - абелевая группа.
%Мы сперва рассматриваем вертикальное представление,
%а затем горизонтальные.
Диаграмма представлений
\DrawEq[{}{}{}g]{diagram of representations of D algebra}{}
порождает структуру $D$\Hyph алгебры $A$.
}

\DefText[4]{linear map of A module, coordinates 111}
{
\ShowText{Let be module of}V{#2}{}D{#1}{алгеброй}%{модулем}
\ShowText{Let be module of}V{#4}{}D{#3}{алгеброй}%{модулем}
\ShowEq{Let be basis of module}1{}iI{}D{#1}V{#2}
\ShowEq{Let be basis of module}2{}jJ{}D{#3}V{#4}
}

\DefText[1]{linear map of A module, coordinates 11}
{
}

\DefText[1]{linear map of A module, coordinates 1}
{
}

\DefLabeledTheorem[7]{linear map of A module, coordinates}{\SideWS \Base\DF\Base\DT}
{
\ShowText{linear map of A module, coordinates #1#2#3}
\ShowEq{Let be basis of module}A{#2}kK{}D{#1}A{#2}
\ShowEq{Let be basis of module}A{#5}lL{}D{#4}A{#5}
\ShowEq{Let be basis of module}V{#3}iI{\SideRu\Which}A{#2}V{#3}
\ShowEq{Let be basis of module}V{#6}jJ{\SideRu\Which}A{#5}V{#6}
Тогда линейное отображение
\newline
\FrameEqRef[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{\SideNS-\Cols}
\newline
%\ShowEq{show linear map \MapE}{\Vector g}{\Vector f}
имеет представление
\DrawEq[#7]{f:A1->A2, A module}{#1#2#3}
\ShowEq{linear map in \SideWS A module}
\DrawEq{linear map in A module}{\SideNS}
%\DrawEq[g]{r2:A1->A2, \DFDT module}{1 \SideWS g}
%\ShowEq{linear map in \SideWS A module}
%\DrawEq{linear map in A module}{\SideNS}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowText{homomorphism of vector space, algebra(#2)}{#1}{#2}{#3}{#4}{#5}{6}
\ShowText{homomorphism of vector space, algebra 1}{#1}{#2}{#3}{#4}{#5}{6}
\[====\]
%\ShowEq{coordinates of the linear map}a{\Base}ghiI{D_2}{}b
%\ShowEq{coordinates of the linear map}v{\Module}fgkK{\Base_\DT}{\SideWS}w
\end{itemize}
Отображение
\ShowEq{fij:-> \SideWS A}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}.
}

\AddEq [9]{coordinates of the linear map}
{
\item $#1$ - координатная матрица $#2_1$\Hyph числа
$\Vector #1$
относительно базиса
\ShowEq{basis e}{#2_1}{}
\DrawEq [#1{#2_1}]{va=ae1, #8module}{#1 \DFDT\SideWS module}
\def\Temp{D1 D2 }
\ifx\DFDT\Temp
\item
\ShowEq{h(a)=...}{#1}{#4}{#5}{#6}
- матрица $#7$\Hyph чисел.
\fi
\item $#9$ - координатная матрица вектора
\DrawEq[#1#9#3]{vb=f(va)}{#1 \DFDT\SideWS \VectorSetNS}
относительно базиса
\ShowEq{basis e}{#2_2}{}
\DrawEq [#9{#2_2}]{va=ae1, #8module}{#9 \DFDT\SideWS module}
\item $#3$ - координатная матрица множества векторов
\ShowEq{Vector f(e1) module}#3#2#5#6
относительно базиса
\ShowEq{basis e}{#2_2}.
Мы будем называть матрицу $#3$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
$\Vector #3$ относительно базисов
\ShowEq{basis e}{#2_1}{}
и
\ShowEq{basis e}{#2_2}.
}

\DefProof{linear map of A module, coordinates}
{
Равенство
\eqRef{r2:A1->A2, \DFDT module}{1 \SideWS g}
является следствием теоремы
\RefTheorem{linear map of D1 D2 module, coordinates}.

\ShowEq{module as direct sum}1kK
\ShowEq{module as direct sum}2lL
Равенство
\eqRef{linear map in A module}{\SideNS}
является следствием теоремы
\RefTheorem{map of direct sum of modules}.
}

\AddEq [3]{module as direct sum}
{
$A_{#1}$\Hyph модуль $V_{#1}$ является прямой суммой
\ShowEq{V=o+Ae}#1#2#3
}

\DefTheorem{representation of algebra An in LAnA}
{
Рассмотрим $D$\Hyph алгебру $A$.
Представление
\ShowEq{representation An in LAnA}DA
алгебры \AOn
в модуле \LAnA,
определённое равенством
\DrawEq[DA]{representation An in LAnA, 1}{}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\DrawEq[DA]{product in algebra An 2}{DA}
где
\ShowEq{product in algebra AA 3}DA{\delta}
- тождественное отображение.
}

\DefDefinition{linear map from A1 to A2, algebra}
{
Пусть $A_1$ и
$A_2$ - алгебры над коммутативным кольцом $D$.
Линейное отображение
$D_{\DF}$\Hyph модуля $A_\VF$
в $D_{\DT}$\Hyph модуль $A_\VT$
называется
\AddIndex{линейным отображением}{linear map}
$D_{\DF}$\Hyph алгебры $A_\VF$ в $D_{\DT}$\Hyph алгебру $A_\VT$.

Обозначим
\ShowEq{set linear maps, module}D{A_1}{A_2}
множество линейных отображений
$D$\Hyph алгебры
$A_\VF$
в $D$\Hyph алгебру
$A_\VT$.
}

\DefText[4]{notation for linear map}
{
Если отображение
\eqRef{homomorphism D algebra #1#2}{module}
является линейным отображением $D_{#1}$\Hyph модуля $V_{#2}$ в $D_{#3}$\Hyph модуль $V_{#4}$,
то, согласно определению
\refDefinition[\RefRepresentation]{side representation of group}{left},
я пользуюсь обозначением
\DrawEq{f circ a =}{}
для образа отображения $f$.
}

\DefTheorem{linear map times constant, algebra}
{
Пусть отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
является линейным отображением $D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
}

\DefTheorem{linear map AA LAA}
{
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
\else
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$
\fi
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
\ShowEq{linear map AA LAA, 2}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{conjugation transformation}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Для любого отображения
\ShowEq{Ik in I}
существует множество линейных отображений
\ShowEq{conjugation transformation}
\ShowEq{conjugation transformation:}
$D$\Hyph модуля
$A_1\otimes A_1$
в $D$\Hyph модуль
$A_2\otimes A_2$
таких, что
\ShowEq{conjugation transformation =}
Отображение
\ShowEq{show conjugation transformation}
называется
\AddIndex{преобразованием сопряжения}{conjugation transformation}.
\end{ShadedTheorem}
}
{theorem: conjugation transformation}
%\DefEq

\DefProof{conjugation transformation}
{
Согласно теореме
\RefTheorem{product of linear map, algebra},
для произвольного тензора
$a\in A_1\otimes A_1$,
отображение
\ShowEq{x->Ik a x}
является линейным.
Согласно утверждению
\RefItem{map f generated by basis F},%, associative algebra},
существует разложение
\ShowEq{expansion Ik a x}
Положим
\ShowEq{b=Ikl a}
Равенство
\EqRef{conjugation transformation =}
является следствием равенств
\EqRef{expansion Ik a x},
\EqRef{b=Ikl a}.
Из равенств
\ShowEq{Ikl a1+a2}
\ShowEq{Ikl d a}
следует, что отображение $I_k^l$ является линейным.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$, $A_3$ - свободные ассоциативные $D$\Hyph алгебры.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Пусть $\Basis G$ - базис левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_2}{A_3}.
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\labelItem{basis of composition of linear maps}
\DrawEq{JlIk}{linear map}
является базисом левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
\item
Пусть линейное отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
имеет разложение
\ShowEq{expansion of f with respect to basis I}
относительно базиса $\Basis I$.
Пусть линейное отображение
\ShowEq{f:A->B}g{A_2}{A_3}
имеет разложение
\ShowEq{expansion of g with respect to basis J}
относительно базиса $\Basis J$.
Тогда линейное отображение
\DrawEq{h=g o f}{123}
имеет разложение
\labelItem{hlk=glfk}
\ShowEq{expansion of h with respect to basis K}
относительно базиса $\Basis K$, где
\ShowEq{hlk=glfk}
\end{enumerate}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps}
%\DefEq

\DefProof{representation of composition of linear maps}
{
Равенство
\ShowEq{h(a)1}
является следствием равенств
\EqRef{expansion of f with respect to basis I},
\EqRef{expansion of g with respect to basis J},
\eqRef{h=g o f}{123}.
Равенство
\ShowEq{h(a)2}
является следствием равенств
\eqRef{JlIk}{linear map},
\EqRef{h(a)1}
и теоремы
\RefTheorem{conjugation transformation}.
Из равенства
\EqRef{h(a)2}
следует, что множество отображений $\Basis K$ порождает
левый \BoxB{A_3}модуля\newline
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
Из равенства
\ShowEq{aK=aJI}
следует, что
\ShowEq{aJ=0}
и, следовательно, $a^{lk}=0$.
Следовательно, множество $\Basis K$ является базисом
левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
}

\DefDefinition{similar A numbers}
{
$A$\Hyph числа $a$ и $b$ называются подобными,
если существует $A$\Hyph число $c$ такое, что
\ShowEq{similar A numbers}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps A->A}
Пусть $A$ - свободная ассоциативная $D$\Hyph алгеба.
Пусть левый \BoxB{A}модуль
\ShowEq{L(A->B)}DAA{}
порождён тождественным отображением $F_0=\delta$.
Пусть линейное отображение
\ShowEq{f:A->B}fAA
имеет разложение
\ShowEq{expansion of f A->A}
Пусть линейное отображение
\ShowEq{f:A->B}gAA
имеет разложение
\ShowEq{expansion of g A->A}
Тогда линейное отображение
\DrawEq{h=g o f}{A}
имеет разложение
\ShowEq{expansion of h A->A}
где
\ShowEq{hlk=glfk 01}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)}
является следствием равенств
\EqRef{expansion of f A->A},
\EqRef{expansion of g A->A},
\eqRef{h=g o f}{A}.
Равенство
\EqRef{hlk=glfk 01}
является следствием равенства
\EqRef{h(a)}.
\end{proof}
}
{proof: representation of composition of linear maps A->A}
%\DefEq

\DefTheorem{h generated by f, associative algebra}
{
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
Отображение
\ShowEq{h:A1->A2}
порождённое отображением
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
имеет вид
\ShowEq{h generated by f, associative algebra}
}

\DefTheorem{coordinates of map A->A, algebra}
{
Пусть $A$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A$.
Пусть $\Basis F$ - базис
левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}DAA{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq{coordinates of map A->A, 2}{associative algebra}
}

\DefProof{coordinates of map A->A, algebra}
{
Относительно базисов
$\Basis e$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f, associative algebra}
\ShowEq{coordinates of map Fk, associative algebra}
Равенство
\ShowEq{coordinates of map A->A, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A->A, associative algebra},
\EqRef{coordinates of map f, associative algebra},
\EqRef{coordinates of map Fk, associative algebra}.
Так как векторы $\aD ek$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A->A, 2}{associative algebra}
следует из равенства
\EqRef{coordinates of map A->A, 3, associative algebra}.
}

\DefTheorem{coordinates of map A1 A2 FoG, algebra}
{
Пусть $\Basis e_1$ - базис конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{f in L(A->B)}D{A_1}{A_2}.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_2}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e_2$.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга такое, что
\ShowEq{ker G in ker g}f{}
и
\ShowEq{coordinates of map G}
- координаты отображения $G$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения $f$
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, FoG, associative algebra}f
}

\AddEq[1]{theorem: maps of conjugation as basis}
{
\begin{ShadedTheorem}
\labelTheorem{maps of conjugation as basis, algebra #1}
Множество линейных отображений
\ShowEq{vI=EI}
является базисом
левого $#1$\Hyph векторного пространства
\ShowEq{L(A->B)}R{#1}{#1}
и линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где
$#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq[1]{theorem: linear map, maps of conjugation, algebra}
{
\begin{ShadedTheorem}
\labelTheorem{linear map, maps of conjugation, algebra #1}
Линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где
\ShowEq{vI=... #1}
и $#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq [1]{proof: L is left vector space}
{
\begin{proof}
Согласно теореме
\RefTheorem{linear map, maps of conjugation, algebra #1},
разложение
\EqRef{linear map of algebra #1, structure, 1}
линейного отображения $f$
существует и единственно.
Следовательно, множество
\ShowEq{I=(E,I)}{#1}{}
является базисом левого $#1$\Hyph векторного пространства
\ShowEq{L(A->B)}R{#1}{#1}.
\end{proof}
}

\DefTheorem{f=.E+.I+.J+.K}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}H
кватернионы, представленные строками матрицы $f$.
\ShowEq{fi=fij ej H}
Тогда
\ShowEq{f=.E+.I+.J+.K}
}

\DefProof{f=.E+.I+.J+.K}
{
Равенства
\ShowEq{a0=f03}
\ShowEq{a1=f03}
\ShowEq{a2=f03}
\ShowEq{a3=f03}
являются следствием равенства
\EqRef{a...= H}.
Равенство
\EqRef{f=.E+.I+.J+.K}
является следствием равенств
\ShowEq{f=.E+.I+.J+.K ref}
}

\DefTheorem{f=.I0.7}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}O
Тогда
\ShowEq{f=.I0.7}
}

\DefProof{f=.I0.7}
{
Равенства
\ShowEq{a0=f0.7}
являются следствием равенства
\EqRef{a...= O}.
Равенство
\EqRef{f=.I0.7}
является следствием равенств
\ShowEq{f=.I0.7 ref}
}

\DefDefinition{maps of conjugation, complex field}
{
\ShowEq{C maps of conjugation}
Поле комплексных чисел имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{C list maps of conjugation}
}

\DefTheorem{HE is algebra isomorphic to quaternion algebra}
{
Множество
\ShowEq{HE set}
является $R$\Hyph алгеброй, изоморфной алгебре кватернионов.
}

\DefProof{HE is algebra isomorphic to quaternion algebra}
{
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map, maps of conjugation, algebra H}.
}

\DefDefinition{algebra, left and right action on L}
{
Пусть $A$ - $D$\Hyph модуль
и $B$ - $D$\Hyph алгебра.
Для произвольного отображения
\ShowEq{f in L(A->B)}DAB{}
и $b\in B$,
мы определим левосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b o f =}
и правосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b * f =}
}

\DefDefinition{projection maps, complex field}
{
Следующие отображения проекции определены в поле комплексных чисел
\ShowEq{projection maps, complex field}
}

\DefTheorem{Expansion of projection maps relative E,I}
{
Разложение отображений проекции относительно базиса
\ShowEq{e=(E,I)}{}
имеет вид
\ShowEq{projection mappings 1, complex field}
}

\DefProof{Expansion of projection maps relative E,I}
{
Теорема является следствием теоремы
\RefTheorem{linear map, maps of conjugation, algebra C}
и определения
\RefDefinition{projection maps, complex field}.
}

\DefTheorem{f=.E+.I}
{
Пусть
\DrawEq[fCC{}]{f: A->B}{}
линейное отображение поля комплексных чисел.
Пусть
\DrawEq{fi=fij ej}C
Тогда
\ShowEq{f=.E+.I}
}

\DefProof{f=.E+.I}
{
Равенства
\ShowEq{a0=f01}
\ShowEq{a1=f01}
являются следствием равенства
\EqRef{a...= C}.
Равенство
\EqRef{f=.E+.I}
является следствием равенств
\ShowEq{f=.E+.I ref}
}

\DefDefinition{polylinear map of algebras}
{
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Полилинейное отображение
\ShowEq{f:A->B}f{\Times}S
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$,
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefTheorem{sum of linear maps, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
}

\DefTheorem{sum of polylinear maps, module}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,polylinear}
\ShowEq{sum of maps, 1, polylinear}
определённое равенством
\ShowEq{sum of  maps, polylinear}
называется
\AddIndex{суммой полилинейных отображений}{sum of maps}
$f$ и $g$
и является полилинейным отображением.
Множество
\ShowEq{module of polylinear maps}
является абелевой группой
относительно суммы отображений.
}

\DefCorollary{sum of linear maps, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество \LAB D{A_1}{A_2}
является абелевой группой
относительно суммы отображений.
}

\AddEq{definition: linear map A module}
{
\begin{ShadedDefinition}
\labelDefinition{linear map \SideWS A module}
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
-
\ShowEq{\SideWS column module}{A_i}
модуль.
Морфизм диаграммы представлений
\ShowEq{A module diagram for linear}1
в диаграмму представлений
\ShowEq{A module diagram for linear}2
называется
\AddIndex{линейным отображением}{linear map}
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
Обозначим
\ShowEq{set linear maps, \SideWS A12 module}
множество линейных отображений
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
\qed
\end{ShadedDefinition}
}

\DefText{homomorphism A module}
{
\section{Общее определение}

\ShowText{def homomorphism A module}111222{h(p)}{(g\circ a)}

\section{Гомоморфизм, когда кольца
\ShowEq{A1=A2 pdf}D}

\ShowText{def homomorphism A module}{}11{}22p{(g\circ a)}

\section{Гомоморфизм, когда \texorpdfstring{$D$}{D}-алгебры
\ShowEq{A1=A2 pdf}A}

\ShowText{def homomorphism A module}{}{}1{}{}2pa
}

\DefText{algebra over ring (11)}
{
Пусть
\ShowEq{Ai, i=}A
- алгебра\DivisionRu над коммутативным кольцом $D_i$.%
}

\DefText{algebra over ring (1)}
{
Пусть
\ShowEq{Ai, i=}A
- алгебра\DivisionRu над коммутативным кольцом $D$.%
}

\DefText{algebra over ring ()}
{
Пусть $A$
- алгебра\DivisionRu над коммутативным кольцом $D$.%
}

\DefText{module over algebra (11)}
{
Пусть
\ShowEq{Ai, i=}V
- \SideRu\To $A_i$\Hyph модуль.
}

\DefText{module over algebra (1)}
{
Пусть
\ShowEq{Ai, i=}V
- \SideRu\To $A$\Hyph \VectorSetRuANS.
}

\DefLabeledDefinition[6]{homomorphism A module}{\SideNS(#1#2#3)}
{
Пусть
\DrawEq[{#1}{#2}{#3}{1.}]{diagram of representations, \SideWS module}{->1(#1#2#3)}
диаграмма представлений, описывающая
\SideRu\To $A_{#2}$\Hyph \VectorSetRuA $V_{#3}$.
Пусть
\DrawEq[{#4}{#5}{#6}{2.}]{diagram of representations, \SideWS module}{->2(#1#2#3)}
диаграмма представлений, описывающая
\SideRu\To $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
Морфизм
\DrawEq[gf]{homomorphism A module #1#2#3}{\SideNS}
диаграммы представлений
\eqRef{diagram of representations, \SideWS module}{->1(#1#2#3)}
в диаграмму представлений
\eqRef{diagram of representations, \SideWS module}{->2(#1#2#3)}
называется
\AddIndex{гомоморфизмом}{homomorphism}
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRu\To $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
Обозначим
\ShowEq{set homomorphisms, A module #1#2#3 \SideNS}
множество гомоморфизмов
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRu\To $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
%\ShowEq{set homomorphisms, \SideWS A12 module}
%множество гомоморфизмов
%\ShowEq{\SideWS column module}{A_1}
%модуля $V_1$ в
%\ShowEq{\SideWS column module}{A_2}
%модуль $V_2$.
}

\DefLabeledTheorem[8]{define homomorphism A module}{\SideNS(#1#2#3)}
{
Гомоморфизм
\newline
\FrameEqRef[gf]{homomorphism A module #1#2#3}{\SideNS}
\newline
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRu\To $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$
удовлетворяет следующим равенствам
\ShowEq{define homomorphism of A module #1#2#3}{#1}{#2}{#3}{#7}{#8}
}

\DefProof[6]{define homomorphism A module}
{
\ShowText{define homomorphism of vector space(#2)}{#1}{#2}{#3}{#4}
Равенство
\eqRef{homomorphism, f v+w=}{f(#1#2)\SideWS A module}
является следствием определения
\refDefinition{homomorphism A module}{\SideNS(#1#2#3)},
так как, согласно определению
\RefDefinition{morphism of representations of universal algebra},
отображение $f$ является гомоморфизмом абелевой группы.
Равенство
\eqRef{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module}
является следствием равенства
\EqRef{morphism of representations of universal algebra},
так как отображение
\DrawEq[gf]{homomorphism A module #2#3}{}
является морфизмом представления $g_{1.34}$
в представление $g_{2.34}$.
}

\DefTheorem{L(An;B) is free D module}
{
Пусть $A_1$, ..., $A_n$, $B$ - свободные модули над коммутативным кольцом $D$.
$D$\Hyph модуль
\ShowEq{L(A->B)}D{A_1\times...\times A_n}B{}
является свободным $D$\Hyph модулем.
}

\DefLabeledTheoremNote[5]{linear map of D module}{#1#2}
{
Линейное отображение
\newline
\FrameEqRef[fV]{homomorphism D algebra #1#2}{module}
\newline
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$
удовлетворяет равенствам\,\footnotemark
\ShowEq{define homomorphism of D module #1#2}{#1}{#2}{#5}
}
{\,
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\refTheorem{linear map of D module}{#1#2}
рассматривается как определение.
}

\DefText{linear map of D module (11)}
{
Согласно определению
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
отображение $h$
явлется гомоморфизмом кольца $D_1$
в кольцо $D_2$.
Равенства
\ShowEq{ref linear map of D module 1}
являются следствием этого утверждения.
}

\DefText{linear map of D module (1)}
{
}

\DefProof[2]{linear map of D module}
{
\ShowText{linear map of D module (#1#2)}
Из определения
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
следует, что
отображение $f$ является гомоморфизмом абелевой группы $V_1$
в абелеву группу $V_2$ (равенство
\eqRef{homomorphism, f v+w=}{f D module #1#2}).
Равенство
\eqRef{left homomorphism, f av=}{f D module #1#2}
является следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of universal algebra}.
}

\DefDefinition{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Приведенный полиморфизм $D$\Hyph модулей
$A_1$, ..., $A_n$ в $D$\Hyph модуль $S$
\ShowEq{f:A->B}f{\Times}S
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.

Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefTheorem{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Полилинейное отображение $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\ShowEq{f:A->B}f{\Times}S
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{}
\DrawEq[f]{f(pai)=pfai}{}
\ShowEq{polylinear map of algebras, 1}{A_i}D
}

\DefTheorem{there exists tensor product of modules}
{
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
\AddIndex{Тензорное произведение}{tensor product}
\ShowEq{tensor product of modules}
\ShowEq{f:xA->oxA}
$D$\Hyph модулей $A_1$, ..., $A_n$ существует и единственно.
Мы пользуемся обозначением
\ShowEq{fxa=oxa}
для образа отображения $f$.
}

\DefTheorem{tensor product and polylinear map}
{
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
Пусть
\ShowEq{map f, 1, tensor product}
полилинейное отображение,
определённое равенством
\ShowEq{map f, tensor product}
Пусть
\ShowEq{map g, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует линейное отображение
\ShowEq{map h, tensor product}
такое, что диаграмма
\ShowEq{map gh, tensor product}
коммутативна.
Отображение \(h\) определено равенством
\ShowEq{g=h, tensor product}
}

\DefProof{polylinear map of modules}
{
Теорема является следствием определений
\RefDefinition[\RefRepresentation]{reduced polymorphism of representations},
\refDefinition{linear map of D module}1,
\RefDefinition{polylinear map of modules}
и теоремы
\refTheorem{linear map of D module}1.
}

\DefProof{sum of polylinear maps, module}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{sum of maps f}
\DrawEq[f]{f(pai)=pfai}{sum of maps f}
\DrawEq[g]{f(ai+bi)=fai+fbi}{sum of maps g}
\DrawEq[g]{f(pai)=pfai}{sum of maps g}
Равенство
\ShowEq{sum of maps, 31, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps f},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps g}.
Равенство
\ShowEq{sum of maps, 32, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(pai)=pfai}{sum of maps f},
\eqRef{f(pai)=pfai}{sum of maps g}.
Из равенств
\EqRef{sum of maps, 31, polylinear},
\EqRef{sum of maps, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{sum of maps, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Пусть
\ShowEq{module of polylinear maps, 1}
Для любого
\ShowEq{module of polylinear maps, 2}
Следовательно, сумма полилинейных отображений коммутативна и ассоциативна.

Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{0:A1n->S}
является нулём операции сложения
\ShowEq{0+f=f 1n}
Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{-f:A1n->S}
является отображением, обратным отображению \(f\)
\ShowEq{f-f=0}
так как
\ShowEq{f-f=0 1n}
Из равенства
\ShowEq{sum of maps, 4, polylinear}
следует, что сумма отображений коммутативно.
Следовательно, множество $\\$
\ShowEq{module of polylinear maps}
является абелевой группой.
}

\DefTheorem{module of polylinear maps}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,polylinear}
\ShowEq{product of map over scalar, 1, polylinear}
определённое равенством
\ShowEq{product of map over scalar, polylinear}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является полилинейным отображением.
Представление
\ShowEq{a:LA1n->LA1n}
кольца $D$ в абелевой группе
\ShowEq{module of polylinear maps}
порождает структуру $D$\Hyph модуля.
}

\DefProof{module of polylinear maps}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{product of map over scalar}
\DrawEq[f]{f(pai)=pfai}{product of map over scalar}
Равенство
\ShowEq{product of map over scalar, 31, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{product of map over scalar}.
Равенство
\ShowEq{product of map over scalar, 32, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(pai)=pfai}{product of map over scalar}.
Из равенств
\EqRef{product of map over scalar, 31, polylinear},
\EqRef{product of map over scalar, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{product of map over scalar, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Равенство
\DrawEq{(p+q)f=pf+qf}{polylinear}
является следствием равенства
\ShowEq{(p+q)f=pf+qf 1}
Равенство
\DrawEq{p(qf)=(pq)f}{polylinear}
является следствием равенства
\ShowEq{p(qf)=(pq)f 1}
Из равенств
\eqRef{(p+q)f=pf+qf}{polylinear},
\eqRef{p(qf)=(pq)f}{polylinear},
следует, что отображение
\EqRef{a:LA1n->LA1n}
является представлением кольца $D$
в абелевой группе
\ShowEq{module of polylinear maps}.
Так как указанное представление эффективно,
то, согласно определению
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теореме
\RefTheorem{sum of polylinear maps, module},
абелевая группа
\ShowEq{L(A->B)}D{A_1}{A_2}{}
является $D$\Hyph модулем.
}

\DefCorollary{product of linear map over scalar, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,D module}
\ShowEq{product of map over scalar, 1, D module}
определённое равенством
\ShowEq{product of map over scalar, D module}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является линейным отображением.
Представление
\ShowEq{a:LA12->LA12}
кольца $D$ в абелевой группе
\ShowEq{L(A->B)}D{A_1}{A_2}{}
порождает структуру $D$\Hyph модуля.
}

\DefLabeledTheoremNote{linear map of A module}{\Base\DF\Module\VF->\Base\DT\Module\VT, \SideNS}
{
Линейное отображение
\ShowEq{show linear map \MapE}gf
\SideRu\From $\Base_\DF$\Hyph модуля $\Module_\VF$
в \SideRu\To $\Base_\DT$\Hyph модуль $\Module_\VT$
удовлетворяет равенствам\,\footnotemark
\ShowEq{property linear map \MapE}
}
{
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\refTheorem{linear map of A module}{\Base\DF\Module\VF->\Base\DT\Module\VT, \SideNS}
рассматривается как определение.
}

\DefProof[2]{linear map of module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\refDefinition{linear map of D module}{#1#2}
следует, что
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module})
и отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{D1 D2 \SideWS module}).
Равенство
\eqRef{f(da)=h... \SideWS module}{\DFDT \SideWS module}
является следствием равенства
%\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{representation}.
}

\DefProof{linear map of A module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map \SideWS A module}
следует, что
\begin{itemize}
\item
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module});
\item
отображение $g$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{g \DFDT \SideWS module}).
\item
отображение $f$ является гомоморфизмом абелевой группы $V_1$
в абелеву группу $V_2$ (равенство
\eqRef{f(a+b)=...}{f \DFDT \SideWS module}).
\end{itemize}
Равенства
\eqRef{f(da)=h... \SideWS module}{g \DFDT},
\eqRef{f(da)=h... \SideWS module}{f \DFDT}
являются следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
%\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{representation}.
}

\DefTheorem{complex field over real field}
{
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
}

\DefProof{complex field over real field}
{
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
}

\DefLabeledTheorem[1]{maps of conjugation antilinear}{#1}
{
Отображения сопряжения
\ShowEq{I... #1}
\DoVerb являются антилинейными гомоморфизмами.
}

\DefProof[1]{maps of conjugation antilinear}
{
Произведение $#1$\Hyph чисел
\ShowEq{#1 number Ea}a
и
\ShowEq{#1 number Ea}b
имеет вид
\DrawEq[ab]{#1 product aEx}{ab}
\ShowText{maps of conjugation antilinear #1}
}

\DefText{maps of conjugation antilinear H}
{
\ShowEq{H items maps of conjugation antilinear}
}

\DefText{maps of conjugation antilinear O}
{
Для доказательства теоремы достаточно рассмотреть отображение $\aU I1$,
так как доказательство аналогично для остальных отображений.
\ShowEq{item maps of conjugation antilinear}O1
}

\DefTheorem{coordinates of map A1 A2, algebra}
{
Пусть $\Basis e_1$ - базис свободного конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, 2, associative algebra}f
}

\DefProof{coordinates of map A1 A2, algebra}
{
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f 18, associative algebra}
\ShowEq{coordinates of map Ik, associative algebra}
Равенство
\ShowEq{coordinates of map A1 A2, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A1 A2, associative algebra},
\EqRef{coordinates of map f 18, associative algebra},
\EqRef{coordinates of map Ik, associative algebra}.
Так как векторы $e_{2\cdot\gik}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A1 A2, 2, associative algebra}f
следует из равенства
\EqRef{coordinates of map A1 A2, 3, associative algebra}.
}

\DefTheorem{linear map in L(A,A), associative algebra}
{
Пусть $A_1$ - $D$\Hyph алгебра.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Левый \BoxB{A_2}модуль
\ShowEq{L(A->B)}D{A_1}{A_2}{}
имеет конечный
\AddIndex{базис}{basis of algebra L(A,A)} $\Basis I$.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
имеет вид
\labelItem{f in L(A,A), 1, associative algebra}
\ShowEq{f in L(A,A), 1, associative algebra}
\item
Его стандартное представление имеет вид
\labelItem{f in L(A,A), 2, associative algebra}
\ShowEq{f in L(A,A), 2, associative algebra}
\end{enumerate}
}

\DefTheoremNote{standard representation of map A1 A2, associative algebra}
{
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Пусть $\Basis F$
- базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
Отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
имеет следующее разложение
\labelItem{map f generated by basis F}
\DrawEq{map f generated by basis F}{expansion}
где
\ShowEq{fk= in A2xA2}
\item
Отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A1 A2, associative algebra}
\ShowEq{standard representation of map A1 A2, associative algebra}
\end{enumerate}
}{
Если $D$\Hyph модуль $A_1$ или $D$\Hyph модуль $A_2$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
порождённого множеством линейных отображений $\Basis F$.
}

\DefProof{standard representation of map A1 A2, associative algebra}
{
Поскольку $\Basis F$ является базисом левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2},
то согласно определению
\ShowEq{ref definition: basis of representation}
и теореме
\ShowEq{RefTheorem set of vectors generated by set of vectors, module}
%существует разложение
\DrawEq[{A_2}]{expansion of linear map with respect to basis}{A2}
линейного отображения $f$ относительно базиса $\Basis I$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{module}
Равенство
\eqRef{map f generated by basis F}{expansion}
является следствием равенств
\eqRef{expansion of linear map with respect to basis}{A2},
\eqRef{f=fkxfk}{module}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A1 A2, associative algebra}
следует из равенств
\eqRef{map f generated by basis F}{expansion},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheorem{map > bullet map}
{
Пусть $A$ - $D$\Hyph алгебра.
Для любого $A$\Hyph числа $a$, отображение
\ShowEq{f->ao f}
определённое равенством
\ShowEq{ao f=a f o}
является эндоморфизмом $D$\Hyph модуля
\ShowEq{L(A->B)}DAA.
}

\DefProof{map > bullet map}
{
}

\DefTheorem{a > a bullet}
{
$D$\Hyph модуль
\ShowEq{L(A->B)}DAA
является левым $A$\Hyph модулем, порождённым представлением
\ShowEq{a > a bullet}
}

\DefProof{a > a bullet}
{
}

\AddEq[3]{theorem: ao Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map ao}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2{#3}
\DrawEq[{#1}{#2}]{a o, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number Ea}a
и
\ShowEq{#2 number #1a}x
имеет вид
\DrawEq[ax]{#2 product a#1x}{}
Следовательно, отображение
\eqRef{map ao}{#1#2}
имеет матрицу Якоби
\eqRef{a o, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq [2]{item maps of conjugation antilinear}
{

Равенство
\ShowEq{#1#2 product ab}
является следствием равенств
\EqRef{#2x= #1},
\eqRef{#1 product aEx}{ab}.
Из равенства
\eqRef{#1 product aEx}{ab}
следует, что произведение $#1$\Hyph чисел
\ShowEq{#1 number #2a}b
и
\ShowEq{#1 number #2a}a
имеет вид
\ShowEq{#1 #2b*#2a}
Из равенств
\EqRef{#1#2 product ab},
\EqRef{#1 #2b*#2a}
следует, что отображение $\aU I#2$
\DoVerb является линейным антигомоморфизмом.
}

\AddEq[2]{theorem: ao Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix 1}
\DrawEq[#1]{ao, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{ao, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{a#1, #2 matrix 2}
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map a*}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2r
\DrawEq[{#1}{#2}]{a *, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number #1a}x
и
\ShowEq{#2 number Ea}a
имеет вид
\ShowEq{#2 product #1xa}
Следовательно, отображение
\eqRef{map a*}{#1#2}
имеет матрицу Якоби
\eqRef{a *, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix 1}
\DrawEq[#1]{a*, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{a*, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{#1a, #2 matrix 2}
\end{proof}%
}

\DefDefinition{antilinear homomorphism}
{
Отображение
\ShowEq{f in L(A->B)}DAA{}
называется
\AddIndex{антилинейным гомоморфизмом}{antilinear homomorphism}
если отображение $f$ удовлетворяет равенству
\ShowEq{fab=fbfa}
}

\DefDefinition{quaternion maps of conjugation}
{
\ShowEq{H maps of conjugation}
Алгебра кватернионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{H list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\DefDefinition{octonion maps of conjugation}
{
\ShowEq{O maps of conjugation}
Алгебра октонионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{O list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\AddEq[1]{theorem: L is left vector space}
{
\begin{ShadedTheorem}
\labelTheorem{L(#1->#1) is left #1-vector space}
$#1\otimes #1$\Hyph модуль
\ShowEq{L(A->B)}R{#1}{#1}
является левым $#1$\Hyph векторным пространством
и имеет базис
\ShowEq{I=(E,I)}{#1}.
\end{ShadedTheorem}
}

\AddEq [9]{Let be basis of vector space}
{%
Пусть множество векторов
\DrawEq[{#1}{#2}{#3}]{basis e of module #8}{#9}
является базисом \SideRu вого $#4_{#5}$\Hyph \VectorSetRuB $#6_{#7}$.%
}%

\AddEq [3]{Let be Basis of vector space}
{%
Пусть \eV[#1]
базис \SideRu вого $#2$\Hyph векторного пространства $#3$.%
}%

\AddEq [9]{Let be basis of module}
{%
Пусть
\DrawEq[{#1_{#2}}{#3}{#4}]{basis e of module \Cols}-
базис #5 $#6_{#7}$\Hyph \VectorSetRuB \ColsA $#8_{#9}$.
}

\AddEq [9]{Let be basis of algebra}
{%
Пусть множество векторов
\DrawEq[{#1_{#2}}{#3}{#4}]{basis e of module \Cols}{#9}
является базисом $#5_{#6}$\Hyph алгебры \ColsA $#7_{#8}$.%
}

\AddEq [9]{Let be basis of algebra and C}
{%
Пусть множество векторов
\DrawEq[{#1}{#3}{#4}]{basis e of module \Cols}{#9}
является базисом и
\ShowEq{structural constants of algebra}{#2}kij,
\ShowEq{kij in I}{#4}
- структурные константы $#5_{#6}$\Hyph алгебры \ColsA $#7_{#8}$.%
}

\AddEq [5]{Let e be basis 1n}
{
Пусть
\ShowEq{basis e of module 1n}{#1}{#2}
базис в #3 $#4$\Hyph модуле $#5$.
}

\DefText[5]{coordinates of the linear map 1}
{
\item $#1$ - координатная матрица $#2_1$\Hyph числа
$\Vector #1$
относительно базиса \eV[#3]
\DrawEq [{#1}{#3}{}]{va=ae1, module (#5)(\Cols)}{\SideNS-\VectorSet #1 #4}
}

\DefText[5]{coordinates of the linear map 2(1)}
{
\item
\ShowEq{h(a)=...}{#1}{#2}{#3}{#4}
- матрица $#5$\Hyph чисел.
}

\DefText[5]{coordinates of the linear map 2()}
{
}

\DefText[7]{coordinates of the linear map 3}
{
\item $#6$ - координатная матрица $#2_2$\Hyph числа
\DrawEq[#1#6#4]{vb=f(va)}{#1 #7(\Cols)\SideNS}
относительно базиса \eV[#3]
\DrawEq [#6{#3}]{va=ae1, module (#5)(\Cols)}{#6 #7\SideNS-\VectorSetNS}
}

\DefText[6]{coordinates of the linear map 4}
{
\item $#1$ - координатная матрица множества $#2_2$\Hyph чисел
\ShowEq{Vector f(e1) module}#1{#3}#5#6
относительно базиса \eV[#4][.]
}

\DefText[6]{Let be module of}
{
Пусть  $#1_{#2}$ является #3 $#4_{#5}$\Hyph #6 \ColsNA.
}

\DefText[2]{we identify linear map and matrix}
{
На основании теорем
\refTheorem{linear map of D module, coordinates}{#1#2cols},
\refTheorem{matrix generates D module homomorphism}{cols(#1#2)},
а также на основании теорем
\refTheorem{linear map of D module, coordinates}{#1#2rows},
\refTheorem{matrix generates D module homomorphism}{rows(#1#2)},
мы идентифицируем линейное отображение
\DrawEq[{\Vector f}V]{homomorphism D algebra #1#2}{}
и матрицу $f$ его представления.
}

\DefLabeledFootnote[4]{homomorphism of d algebra}{#1#2\Cols}
{
В теоремах
\refTheorem{homomorphism of d algebra, coordinates}{#1#2\Cols},
\refTheorem{matrix generates D algebra homomorphism}{\Cols(#1#2)},
мы опираемся на следующее соглашение.
\ShowEq{Let be basis of algebra and C}11iID{#1}A{#2}-
\ShowEq{Let be basis of algebra and C}22jJD{#3}A{#4}-
}

\DefLabeledTheorem[5]{homomorphism of d algebra, coordinates}{#1#2\Cols}
{
Гомоморфизм\refFootnote{homomorphism of d algebra}{#1#2\Cols}
\DrawEq[{\Vector f}A]{homomorphism D algebra #1#2}{}
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$ имеет представление
\DrawEq[f{#5}{}]{f:V1->V2, D module \Cols}{algebra(#1#2)}
\DrawEq[hf{#2}{#4}a]{f o ea=efa i (#1#2)}{(\Cols)algebra}
\DrawEq[hf12]{f o ea=efa (#1#2)(\Cols)}{algebra}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowText{coordinates of the linear map 1}aA1{(#1)(#2)}{}
\ShowText{coordinates of the linear map 2(#1)}ahiI{D_{#3}}
\ShowText{coordinates of the linear map 3}aA2f{}b{(#1)(#2)}
\ShowText{coordinates of the linear map 4}fA{#2}{#4}iI
\ShowText{Morphism of D algebra}{#1}{#2}f
\end{itemize}
}

%\DefProofRef[4]{homomorphism of d algebra, coordinates}{#1#2\Cols}
\DefProof[4]{homomorphism of d algebra, coordinates}
{
Равенства
\ShowRef{homomorphism of d algebra, coordinates}{#1}{#2}{#4}
являются следствием теорем
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
\refTheorem{homomorphism from A1 to A2, D algebra}{#1#2}.

Равенство
\DrawEq{algebra, homomorphism and product eiej(#1#2)}{\Cols}
является следствием равенств
\ShowRef{algebra, homomorphism and product eiej}{#1}{#2}{#3}
Равенство
\DrawEq{algebra, homomorphism and product eiej 4(#1#2)}{\Cols}
является следствием равенства
\ShowRef{algebra, homomorphism and product eiej 1}{#1}{#2}
и равенства
\eqRef{algebra, homomorphism and product eiej(#1#2)}{\Cols}.
Равенство
\DrawEq{algebra, homomorphism and product eiej 5}{(#1#2)\Cols}
является следствием равенства
\ShowRef{homomorphism, f vw=}{#1}{#2}
Равенство
\DrawEq{algebra, homomorphism and product eiej 2(#1#2)}{\Cols}
является следствием равенства
\ShowEq{algebra, homomorphism and product, 1}
и равенства
\eqRef{algebra, homomorphism and product eiej 5}{(#1#2)\Cols}.
Равенство
\DrawEq{algebra, homomorphism and product eiej 3(#1#2)}{\Cols}
является следствием равенств
\eqRef{algebra, homomorphism and product eiej 4(#1#2)}{\Cols},
\eqRef{algebra, homomorphism and product eiej 2(#1#2)}{\Cols}.
Равенство
\ShowRef{algebra, homomorphism and product}{#1}{#2}f
следует из равенства
\eqRef{algebra, homomorphism and product eiej 3(#1#2)}{\Cols}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
}

\DefLabeledTheorem[5]{linear map of D module, coordinates}{#1#2\Cols}
{
Линейное отображение\refFootnote{homomorphism of D module}{\Cols(#1#2)}
\DrawEq[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
имеет представление
\DrawEq[hf{#2}{#4}{}]{f o ea=efa (#1#2)(\Cols)}{module}
\DrawEq[hf{#2}{#4}a]{f o ea=efa i (#1#2)}{(\Cols)module}
\DrawEq[f{#5}{}]{f:V1->V2, D module \Cols}{#1#2}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowText{coordinates of the linear map 1}aV1{(#1)(#2)}{}
\ShowText{coordinates of the linear map 2(#1)}ahiI{D_{#3}}
\ShowText{coordinates of the linear map 3}aV2f{}b{(#1)(#2)}
\ShowText{coordinates of the linear map 4}fV{#2}{#4}iI
\end{itemize}
}

\DefProofRef[5]{linear map of D module, coordinates}{#1#2\Cols}
{
Так кaк
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
\newline
линейное отображение, то равенство
\ShowEq{vb=h(e1)a (#1)(#2)(\Cols)\SideNS}
является следствием равенств
\ShowRef{vb=h(e1)a}{#1}{#2}{#5}
$V_2$\Hyph число
\ShowEq{f(e1)(\Cols)\SideNS}
имеет разложение
\DrawEq{f(e1)=(\Cols)\SideNS}{(#1)(#2)}
относительно базиса $\Basis e_2$.
Комбинируя \EqRef{vb=h(e1)a (#1)(#2)(\Cols)\SideNS}
и \eqRef{f(e1)=(\Cols)\SideNS}{(#1)(#2)}, мы получаем
\ShowEq{vb=a f e (#1)(#2)(\Cols)\SideNS}
\eqRef{f:V1->V2, D module \Cols}{#1#2}
следует из сравнения
\newline
\FrameEqRef[b2]{va=ae1, module ()(\Cols)}{b {(#1)(#2)}\SideNS-\VectorSetNS}
\newline
и \EqRef{vb=a f e (#1)(#2)(\Cols)\SideNS} и
теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
}

\DefDefinitionNote{algebra over ring}
{
Пусть $D$ - коммутативное кольцо.
$D$\Hyph модуль $A$ называется
\AddIndex{алгеброй над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгеброй}{D algebra},
если определена операция произведения\,\footnotemark
в $A$
\DrawEq{product in D algebra}{definition}
где $C$ - билинейное отображение
\ShowEq{product in algebra, definition 1}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
}
{
Я следую определению,
приведенному в
\citeBib{Richard D. Schafer}, страница 1,
\citeBib{0105.155}, страница 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.
}

\DefText{algebra inherits type of module}
{
$D$\Hyph алгебра $A$ наследует тип $D$\Hyph модуля $A$.
}

\DefLabeledDefinition{type of algebra}{\Cols}
{
$D$\Hyph алгебра $A$ называется
$D$\Hyph алгеброй \ColsNA,
если $D$\Hyph модуль $A$
является $D$\Hyph модулем \ColsNA.
}

\DefLabeledTheorem{associative product in algebra}{\Cols}
{
Если алгебра $A$ коммутативна, то
\DrawEq{commutative product in algebra, 1}{\Cols}
Если алгебра $A$ ассоциативна, то
\DrawEq{associative product in algebra, 1}{\Cols}
}

\DefProof{associative product in algebra}
{
Для коммутативной алгебры,
равенство
\eqRef{commutative product in algebra, 1}{\Cols}
следует из равенства
\ShowEq{commutative product in algebra}
Для ассоциативной алгебры,
равенство
\eqRef{associative product in algebra, 1}{\Cols}
следует из равенства
\ShowEq{associative product in algebra}
}

\DefLabeledTheorem{product in algebra}{\Cols}
{
\ShowEq{Let be basis of algebra}{}{}iID{}A{}-
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\DrawEq{product in algebra}{\Cols}
где
\ShowEq{structural constants of algebra symb}
- \AddIndex{структурные константы}{structural constants}
алгебры $A$ над кольцом $D$.
Произведение базисных векторов в алгебре $A$ определено согласно правилу
\DrawEq{product of basis vectors, algebra}{\Cols}
}

\DefProofSloppy{product in algebra}
{
Равенство
\eqRef{product of basis vectors, algebra}{\Cols}
является следствием утверждения, что \eV
является базисом $D$\Hyph алгебры $A$.
Так как произведение в алгебре является билинейным отображением,
то произведение $a$ и $b$ можно записать в виде
\DrawEq{product in algebra, 1}{\Cols}
Из равенств
\eqRef{product of basis vectors, algebra}{\Cols},
\eqRef{product in algebra, 1}{\Cols},
следует
\DrawEq{product in algebra, 2}{\Cols}
Так как \eV является базисом алгебры $A$, то равенство
\eqRef{product in algebra}{\Cols}
следует из равенства
\eqRef{product in algebra, 2}{\Cols}.
}

\DefText{D-module type}
{
Организацию координат вектора в матрице
мы будем называть типом $D$\Hyph модуля.

В этом разделе мы рассмотрим вектор\Hyph столбец
и вектор\Hyph строку.
Очевидно, что существуют и другие формы представления вектора.
Например, мы можем записать координаты вектора в виде
\nmTimes nm матрицы или в виде треугольной матриц.
Формат представления зависит от рассматриваемой задачи.
}

\DefText{D-module type 1}
{
Если утверждение зависит от формата представления вектора,
мы будем указывать либо тип $D$\Hyph модуля,
либо формат представления базиса.
Оба способа указания типа $D$\Hyph модуля эквивалентны.
}

\DefText{Morphism of D algebra, injection 11}
{
(а следовательно,
\ShowEq{Morphism of D algebra, injection}
}

\DefText{Morphism of D algebra, injection 1}
{
}

\DefText[3]{Morphism of D algebra}
{
\item Матрица гомоморфизма
и структурные константы связаны соотношением
\DrawEq[{#3}{}]{algebra, homomorphism and product (#1#2)}{\Cols(\SideNS)}
}

\DefText{algebra, homomorphism and product 11}
{
Поскольку отображение $h$ является гомоморфизмом колец,
то равенство
\DrawEq{algebra, homomorphism and product, 4}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product eiej(11)}{\Cols}.
Равенство
\DrawEq{algebra, homomorphism and product, 5 11}{\Cols}
является следствием теоремы
\refTheorem{homomorphism of d algebra, coordinates}{11\Cols}
и равенства
\eqRef{algebra, homomorphism and product, 4}{\Cols}.
}

\DefText{algebra, homomorphism and product 1}
{
Равенство
\DrawEq{algebra, homomorphism and product, 5 1}{\Cols}
является следствием теоремы
\refTheorem{homomorphism of d algebra, coordinates}{1\Cols}
и равенства
\eqRef{algebra, homomorphism and product eiej(1)}{\Cols}.
}

\DefDefinition{commutator of algebra}
{
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
}

\DefDefinitionNote{nucleus of algebra}
{
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это
множество\,\footnotemark
\ShowEq{nucleus of algebra}
}
{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13.}

\DefDefinition{associator of algebra}
{
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
\ShowEq{associator of algebra =}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
}

\DefTheorem{associator of algebra}
{
Пусть $\Basis e$ - базис $D$\Hyph алгебры $A$. Тогда
\ShowEq{associator of algebra = A}
где
\AddIndex{координаты ассоциатора}{coordinates of associator}
определены равенством
\ShowEq{coordinates of associator}
\ShowEq{coordinates of associator =}
}

\DefProof{associator of algebra}
{
Равенство
\ShowEq{associator of algebra = Ae}
является следствием равенства
\EqRef{associator of algebra =}.
Равенство
\EqRef{coordinates of associator =}
является следствием равенства
\EqRef{associator of algebra = Ae}.
}

\DefDefinitionNote{center of algebra}
{
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это
множество\,\footnotemark
\ShowEq{center of algebra}
}{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, страница 14.
}

\DefDefinition{otimes -}
{
Билинейное отображение
\ShowEq{otimes -}
определено равенством
\ShowEq{otimes -, 1}
}


==> Stmt.Representation.English.tex <==
%auto-ignore
\input{Stmt.Representation.Eq}

\DefDefinition{morphism of representations of universal algebra}
{
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$ and
\ShowEq{f:A->*B}g{B_1}{B_2}
be representation of $\Omega_1$\Hyph algebra $B_1$
in $\Omega_2$\Hyph algebra $B_2$.
For
\ShowEq{i=1,2},
let the map
\ShowEq{ri:A->B}
be homomorphism of $\Omega_i$\Hyph algebra.
The tuple of maps
\ShowEq{map r12}r{}
such, that
\ShowEq{morphism of representations of universal algebra, definition, 2}
is called
\AddIndex{morphism of representations from $f$ into $g$}
{morphism of representations from f into g}.
We also say that
\AddIndex{morphism of representations of $\Omega_1$\Hyph algebra
in $\Omega_2$\Hyph algebra}
{morphism of representations of Omega1 algebra in Omega2 algebra} is defined.
}

\DefRemark{morphism of representations of universal algebra}
{
There are two ways
to interpret
\eqRef{morphism of representations of universal algebra, 2m}{representation}
\begin{itemize}
\item Let transformation $\BlueText{f(a)}$ map $m\in A_2$
into $\BlueText{f(a)}(m)$.
Then transformation
\ShowEq{g(r1(a))}
maps
\ShowEq{r2(m)in B2}
into
\ShowEq{r2(f(a,m))}
\item We represent morphism of representations from $f$ into $g$
using diagram
\DrawEq{morphism of representations of universal algebra, 2m 1}{ShadedDefinition}
From \EqRef{morphism of representations of universal algebra, definition, 2},
it follows that diagram $(1)$ is commutative.
\end{itemize}
We also use diagram
\ShowEq{morphism of representations of universal algebra, definition, 2m 2}
instead of diagram
\eqRef{morphism of representations of universal algebra, 2m 1}{ShadedDefinition}.
}

\DefRemark{morphism of representations of universal algebra as map}
{
We may consider a pair of maps $r_1$, $r_2$ as map
\ShowEq{F:A1+A2->B1+B2}
such that
\ShowEq{F:A1+A2->B1+B2 1}
Therefore, hereinafter the tuple of maps
\ShowEq{map r12}r{}
also is called map
and we will use map
\ShowEq{f:A->B}rfg
Let
\ShowEq{a=a12}
be tuple of $A$\Hyph numbers.
We will use notation
\ShowEq{r(a)12}
for image of tuple of $A$\Hyph numbers
with respect to morphism of representations $r$.
}

\DefTheorem{unique morphism of representations of universal algebra}
{
Let the representation
\ShowEq{f:A->*B}f{A_1}{A_2}
of $\Omega_1$\Hyph algebra $A_1$ be single transitive representation
and the representation
\ShowEq{f:A->*B}g{B_1}{B_2}
of $\Omega_1$\Hyph algebra $B_1$ be single transitive representation.
Given homomorphism of $\Omega_1$\Hyph algebra
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
consider a homomorphism of $\Omega_2$\Hyph algebra
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
such that
\ShowEq{map r12}r{}
is morphism
of representations from $f$ into $g$.
The map $H$ is unique up to
choice of image
\ShowEq{n=r2(m)}
of given element $m\in A_2$.
}

\DefConvention[2]{A number}
{
Element of $#1$\Hyph #2 $A$ is called
\AddIndex{$A$\Hyph number}{A number}.
For instance, complex number is also called
$C$\Hyph number, and quaternion is called $H$\Hyph number.
}

\DefTheorem{map is reduced morphism of representations iff}
{
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$ and
\ShowEq{f:A->*B}g{A_1}{B_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $B_2$.
The map
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
is reduced morphism of representations iff
\DrawEq{reduced morphism representation =}{definition}
}

\DefDefinition{morphism of representation f}
{
If representation $f$ and $g$ coincide, then morphism of representations
\ShowEq{map r12}r{}
is called
\AddIndex{morphism of representation $f$}{morphism of representation f}.
}

\DefRemark{notation for morphism of representations}
{
Consider morphism of representations
\ShowEq{r12:A->B}rAB
We denote elements of the set $B_1$ by letter using pattern $b\in B_1$.
However if we want to show that $b$ is image of element
\ShowEq{a in A1},
we use notation $\RedText{r_1(a)}$.
Thus equation
\ShowEq{r1(a)=r1(a)}
means that $\RedText{r_1(a)}$ (in left part of equation)
is image
\ShowEq{a in A1}{}
(in right part of equation).
Using such considerations, we denote
element of set $B_2$ as $\BlueText{r_2(m)}$.
We will follow this convention when we consider correspondences
between homomorphisms of $\Omega_1$\Hyph algebra
and maps between sets
where we defined corresponding representations.
}

\DefTheorem{Tuple of maps is morphism of representations iff}
{
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$ and
\ShowEq{f:A->*B}g{B_1}{B_2}
be representation of $\Omega_1$\Hyph algebra $B_1$
in $\Omega_2$\Hyph algebra $B_2$.
The map
\ShowEq{r12:A->B}rAB
is morphism of representations iff
\DrawEq{morphism of representations of universal algebra, 2m}{representation}
}

\DefDefinition{tower of representations}
{
Consider set of $\Omega_k$\Hyph algebras $A_k$, \Kn1.
Let $A=(A_1,...,A_n)$.
Let $f=(f_{1\,2},...,f_{n-1\,n})$.
Set of representations $f_{k\,k+1}$, \Kn1,
of $\Omega_k$\Hyph algebra $A_k$ in
$\Omega_{k+1}$\Hyph algebra $A_{k+1}$
is called
\AddIndex{tower $(f,A)$ of representations of $\Omega$\Hyph algebras}
{tower of representations of algebras}.
}

\DefDefinition{diagram of representations}
{
\AddIndex{Diagram $(f,A)$ of representations of universal algebras}
{diagram of representations of algebras}
is oriented graph such that
\StartLabelItem
\begin{enumerate}
\item
the vertex of $A_k$, \Kn1, is $\Omega_k$\Hyph algebra;
\item
the edge $f_{kl}$ is representation
of $\Omega_k$\Hyph algebra $A_k$ in
$\Omega_l$\Hyph algebra $A_l$;
\end{enumerate}
We require that this graph
is connected graph and does not have loops.
Let $A_{[0]}$ be set of initial vertices of the graph.
Let $A_{[k]}$ be set of vertices of the graph
for which the maximum path from the initial vertices is $k$.
}

\DefRemark{diagram of representations}
{
Since different vertices of the graph
can be the same algebra,
then we denote
\ShowEq{A=A1n}A{}
the set of universal algebras which are distinct.
From the equality
\ShowEq{A=A(1n)1n}A
it follows that, for any index $(i)$,
there exists at least one index $i$ such that
\ShowEq{A(i)=Ai}i.
If there are two sets of sets
\ShowEq{A=A1n}A,
\ShowEq{A=A1n}B
and there is a map
\ShowEq{hi:Ai->Bi}
for an index $(i)$,
then also there is a map
\ShowEq{f:A->B}{h_i}{A_i}{B_i}
for any index $i$ such that
\ShowEq{A(i)=Ai}i{}
and in this case $h_i=h_{(i)}$.
}

\DefTheorem{diagram of representations}
{
{\bf(}\AddIndex{Induction over diagram of representations}{induction over diagram of representations}{\bf)}.
Let the theorem $\mathcal T$ be true for the set
of universal algebras $A_{[0]}$
of diagram $(f,A)$ of representations of universal algebras.
Let the statement that the theorem $\mathcal T$ is true for the set
of universal algebras $A_{[k]}$
of diagram $(f,A)$ of representations imply the statement
that the theorem $\mathcal T$ is true for the set
of universal algebras $A_{[k+1]}$
of diagram $(f,A)$ of representations.
Then the theorem $\mathcal T$ is true for the set
of universal algebras
of diagram $(f,A)$ of representations.
}

\DefDefinitionNote{commutative diagram of representations}
{
Diagram $(f,A)$ of representations of universal algebras
is called
\AddIndex{commutative}{commutative diagram of representations}
when diagram meets the following requirement.
for each pair of representations
\ShowEq{f:A->*B}{f_{ik}}{A_i}{A_k}
\ShowEq{f:A->*B}{f_{jk}}{A_j}{A_k}
the following equality is true\,\footnotemark
\ShowEq{fik fjk = fjk fik}
}
{
Metaphorically speaking,
representations $f_{ik}$ and $f_{jk}$
are transparent to each other.
}

\DefTheoremNote{diagram of representations, define map fik}
{
Let
\ShowEq{f:i->*j}ij
be representation of $\Omega_i$\Hyph algebra $A_i$
in $\Omega_j$\Hyph algebra $A_j$.
Let
\ShowEq{f:i->*j}jk
be representation of $\Omega_j$\Hyph algebra $A_j$
in $\Omega_k$\Hyph algebra $A_k$.
We represent the fragment\,\footnotemark
\DrawEq[ijk]{Ai->*Aj->*Ak}{}
of the diagram of representations using the diagram
\ShowEq{tower of representations, 1 2 3}
The map
\ShowEq{f:A->End 2 3}
is defined by the equality
\ShowEq{define map f13}
where
\ShowEq{a in A}i,
\ShowEq{a in A}j.
If the representation $f_{jk}$ is effective
and the representation $f_{ij}$ is free,
then the map $f_{ijk}$ is free representation
\ShowEq{f:1->*3}
of $\Omega_i$\Hyph algebra $A_i$
in $\Omega_j$\Hyph algebra
\ShowEq{End Ak}Ak.
}
{
The theorem
\RefTheorem{diagram of representations, define map fik}
states that transformations in diagram of representations are coordinated.
}

\DefDefinition{Morphism of Diagram of Representations}
{
Let
$(f,A)$
be the diagram of representations where
\ShowEq{A=A1n}A{}
is the set of universal algebras.
Let
$(B,g)$
be the diagram of representations where
\ShowEq{A=A1n}B{}
is the set of universal algebras.
The set of maps
\ShowEq{A=A1n}h{}
\ShowEq{hi:Ai->Bi}
is called \AddIndex{morphism from diagram of representations
$(f,A)$ into diagram of representations $(B,g)$}
{morphism from diagram of representations into diagram of representations},
if for any indexes $(i)$, $(j)$, $i$, $j$ such that
\ShowEq{A(i)=Ai}i,
\ShowEq{A(i)=Ai}j{}
and for any representation
\ShowEq{f:A->*B}{f_{ji}}{A_j}{A_i}
the tuple of maps $(h_j\ \ h_i)$ is
morphism of representations from $f_{ji}$ into $g_{ji}$.
}

\AddEq{remark: Morphism of Diagram of Representations}
{
For any representation $f_{ij}$,
\Kn[i]1, \Kn[j]1,
we have diagram
\ShowEq{morphism of diagram of representations of F algebra, level k, diagram}
Equalities
\ShowEq{morphism of diagram of representations, level k}
\ShowEq{morphism of diagram of representations, levels k k+1}
express commutativity of diagram (1).
}

\DefTheorem{reduced polymorphism of representations}
{
Let the map $r_2$ be reduced polymorphism of
effective representations $f_1$, ..., $f_n$ into effective representation $f$.
\begin{itemize}
\item
For any
\ShowEq{k,1n}
the map $r_2$ satisfies to the equality
\ShowEq{reduced polymorphism of representation, ak}
\item
For any
\ShowEq{kl,1n}
the map $r_2$ satisfies to the equality
\ShowEq{reduced polymorphism of representation, akl}
\item
Let $\omega_2\in\Omega_2(p)$.
For any
\ShowEq{k,1n}
the map $r_2$ satisfies to the equality
\ShowEq{reduced polymorphism of representation, omega2}
\end{itemize}
}

\AddEq{remark: morphism of representation of Omega group}
{
\begin{remark}
\labelRemark{morphism of \SideWS representation of Omega group}
Let the map
\ShowEq{f:A->*B}f{A_1}{A_2}
be the \SideNS\Hyph side representation
of multiplicative $\Omega$\Hyph group $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
Let the map
\ShowEq{f:A->*B}g{B_1}{B_2}
be the \SideNS\Hyph side representation
of multiplicative $\Omega$\Hyph group $B_1$
in $\Omega_2$\Hyph algebra $B_2$.
Let the map
\ShowEq{r12:A->B}rAB
be morphism of representations.
We use notation
\ShowEq{r2a=r2 o a}
for image of $A_2$\Hyph number $a_2$
with respect to the map $r_2$.
Then we can write the equality
\eqRef{morphism of representations of universal algebra, 2m}{representation}
in the following form
\ShowEq{morphism of \SideWS representation of Omega group}
\qed
\end{remark}
}

\DefTheorem{proper definition of orbit}
{
Let the map
\ShowEq{f:A->*B}f{A_1}{A_2}
be the left\Hyph side representation
of multiplicative $\Omega$\Hyph group $A_1$.
Let
\ShowEq{orbit, proposition}
Then
\ShowEq{A1a2=A1b2}
}

\AddEq{definition: orbit of representation}
{
\begin{ShadedDefinition}
\labelDefinition{orbit of \SideNS-side representation}
Let $A_1$ be $\Omega$\Hyph groupoid with product
\ShowEq{(ab)->ab}
Let the map
\ShowEq{f:A->*B}f{A_1}{A_2}
be the \SideNS\Hyph side representation
of $\Omega$\Hyph groupoid $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
For any
\ShowEq{a in A}2,
we define
\AddIndex{orbit of representation}{orbit of representation}
of the $\Omega$\Hyph groupoid $A_1$ as set
\ShowEq{orbit of \SideNS-side representation}
\end{ShadedDefinition}
}

\AddEq{Let A->*AB2 be representations}
{
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
Let
\ShowEq{f:A->*B}g{A_1}{B_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $B_2$.
}

\AddEq{Let XY be generating sets}
{
Let $X$ be the generating set of the representation
\ShowEq{f:A->*B}f{A_1}{A_2}
of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
Let $Y$ be the generating set of the representation
\ShowEq{f:A->*B}g{A_1}{B_2}
of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $B_2$.
}

\DefDefinitionNote{product in category}
{
Let $\mathcal A$ be a category.
Let
\ShowEq{set Bi}B
be the set of objects of $\mathcal A$.
Object
\ShowEq{product in category}
and set of morphisms
\ShowEq{set f:A->B}fP{B_i}
is called a
\AddIndex{product of set of objects
\ShowEq{set Bi}B
in category $\mathcal A$}
{product in category}\,\footnotemark
if for any object $R$
and set of morphisms
\ShowEq{set f:A->B}gR{B_i}
there exists a unique morphism
\ShowEq{f:A->B}hRP
such that diagram
\ShowEq{product in category diagram}
is commutative for all $i\in I$.

If $|I|=n$, then we also will use notation
\ShowEq{product in category, 1 n}
for product of set of objects
$\{B_i,\iI\}$ in $\mathcal A$.
}
{
I made definition according to \citeBib{Serge Lang}, page 58.
}

\DefExample{Cartesian product of sets}
{
Let \(\mathcal S\) be the category of sets.\,\footnote{See
also the example in
\citeBib{Serge Lang},
page 59.
}
According to the definition
\ShowEq{ref product in category}
Cartesian product
\ShowEq{Cartesian product of sets}
of family of sets
\ShowEq{Ai iI}A{}
and family of projections on the \(i\)\Hyph th factor
\ShowEq{projection on i factor}
are product in the category \(\mathcal S\).
}

\DefTheorem{product of effective representations}
{
In category
\ShowEq{A1(mA2)}
there exists product
of effective representations of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra
and the product is
effective representation of $\Omega_1$\Hyph algebra $A_1$.
}

\DefTheoremNote{structure of subrepresentations}
{
Let\,\footnotemark
\ShowEq{f:A->*B}g{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
Let $X\subset A_2$.
Define a subset $X_k\subset A_2$ by induction on $k$.
\ShowEq{structure of subrepresentations}
Then
\ShowEq{structure of subrepresentations, 1}
}{
The statement of theorem is similar to the
statement of theorem 5.1, \citeBib{Cohn: Universal Algebra}, page 79.
}

\DefDefinitionNote{direct sum of Abelian groups}
{
Coproduct in category of Abelian groups $Ab$ is called
\AddIndex{direct sum}{direct sum}.\,\footnotemark
We will use notation
\ShowEq{direct sum of Abelian groups}
for direct sum of Abelian groups $A$ and $B$.
}{See also definition in \citeBib{Serge Lang}, pages 36, 37.}

\DefDefinitionNote{coproduct in category}
{
Let $\mathcal A$ be a category.
Let
\ShowEq{set Bi}B
be the set of objects of $\mathcal A$.
Let
\ShowEq{category A[Bi]}
be a category
whose objects are tuples $(P,f)$
where $P$ is object of category $\mathcal A$
and $f$ is set of morphisms
\ShowEq{set f:A->B}f{B_i}P
Universally repelling object of category
\ShowEq{category A[Bi]}
\ShowEq{coproduct in category}
is called a
\AddIndex{coproduct of set of objects
\ShowEq{set Bi}B
in category $\mathcal A$}
{coproduct in category}.\,\footnotemark

If $|I|=n$, then we also will use notation
\ShowEq{coproduct in category, 1 n}
for coproduct of set of objects
\ShowEq{set Bi}B
in $\mathcal A$.
}
{
I made definition according to the definition on page
\citeBib{Serge Lang}\Hyph 59.
}

\AddEq{definition: free Abelian group}
{
\begin{ShadedDefinition}
\labelDefinition{free Abelian group}
Let $S$ be a set and\,\footnotemark
\ShowEq{category AbS}
be category objects of which are maps
\ShowEq{f:A->B}fSG
of the set $S$ into Abelian groups.
If
\ShowEq{f:A->B}fSG
\ShowEq{f:A->B}{f'}S{G'}
are objects of the category
\ShowEq{category AbS},
then morphism from $f$ to $f'$
is the homomorphism of groups
\ShowEq{f:A->B}gG{G'}
such that the diagram
\DrawEq{AbS ff'g}{}
is commutative.
\end{ShadedDefinition}
\footnotetext{\,
See also the definition in \citeBib{Serge Lang}, pages 37.
}
}

\AddEq{theorem: free Abelian group}
{
\begin{ShadedTheorem}
\labelTheorem{free Abelian group}
There exists\,\footnotemark
universally repelling object $G$ of the category
\ShowEq{category AbS}
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{S in G}
\item
The set $S$ generates Abelian group $G$.
\labelItem{set generates Abelian group}
\end{enumerate}
Abelian group $G$ is called
\AddIndex{free Abelian group}{free Abelian group}
generated by the set $S$.
\end{ShadedTheorem}
\footnotetext{\,
See also similar statement in \citeBib{Serge Lang}, pages 38.
}
}

\DefProof{free Abelian group}
{
Let $G$
be set of maps
\ShowEq{f:A->B}hSZ
such that the set
\ShowEq{x in -> h(x)}
is finite.

\begin{ShadedLemma}
{\it
The set $G$ is Abelian group.
}
\end{ShadedLemma}
{\sc Proof.}
Let
\ShowEq{h12 in G}
According to the definition, sets
\ShowEq{H12=}
are finite. Then the set
\ShowEq{H1vH2}
is finite.
Therefore,
\ShowEq{h1+h2 in G}
Properties of Abelian group are evident.
\hfill\(\odot\)

Let $k\in Z$, $x\in S$.
We denote by $k*x$ the map $h$ defined by the equality
\ShowEq{k*x=k}
The map
\ShowEq{f:S->G}
is injective and allows us to identify $S$ and image $f(S)\subseteq G$
(the statement
\RefItem{S in G})
and to use notation
\ShowEq{kx=k*x}
According to the definition of the group $G$,
we can write any map $h\in G$ as
\ShowEq{h=k*x}
where
\ShowEq{k in Z x in S}
and the set
\ShowEq{|kx ne 0|}
is finite.
The statement
\RefItem{set generates Abelian group}
follows from the theorem
\RefTheorem{structure of Abelian group}.

\begin{ShadedLemma}
{\it
The representation
\EqRef{h=k*x}
of the map $h$ is unique.
}
\end{ShadedLemma}
{\sc Proof.}
If the map $h$ admits representations
\ShowEq{h=k12*x i}
then the equality
\ShowEq{k1-k2 *x}
follows from the equality
\EqRef{h=k12*x i}.
\ShowEq{k1=k2 i}
follows from the equality
\EqRef{k1-k2 *x}.
\hfill\(\odot\)

Let
\ShowEq{f:A->B}{f'}S{G'}
be the map of the set $S$ into Abelian group $G'$.
We define the homomorphism
\ShowEq{f:A->B}gG{G'}
with request that
following diagram is commutative
\DrawEq{AbS ff'g}{1}
From the diagram
\eqRef{AbS ff'g}{1},
it follows that
\ShowEq{g(1x)=f'(x)}
According to the theorem
\RefTheorem{homomorphism f(na)=nf(a)},
since the map $g$ is homomorphism of Abelian group, then the equality
\ShowEq{g(x)=}
for any map $h\in G$
follows from equalities
\EqRef{g(1x)=f'(x)},
\EqRef{h=k*x}.
Therefore, homomorphism $g$ is defined uniquely.
According to definitions
\RefDefinition{universally repelling object of category},
\RefDefinition{free Abelian group},
Abelian group $G$ is free group.
}

\DefTheorem{homomorphism f(na)=nf(a)}
{
The homomorphism
\ShowEq{f:A->B}fG{G'}
holds the equality
\ShowEq{f(na)=nf(a)}
}

\DefTheoremNote{coproduct in category}
{
Let $\mathcal A$ be a category.
Let
\ShowEq{set Bi}B
be the set of objects of $\mathcal A$.
Object
\ShowEq{coproduct in category}
and set of morphisms
\ShowEq{set f:A->B}f{B_i}P
is called a
\AddIndex{coproduct of set of objects
\ShowEq{set Bi}B
in category $\mathcal A$}
{coproduct in category}\,\footnotemark
if for any object $R$ and set of morphisms
\ShowEq{set f:A->B}g{B_i}R
there exists a unique morphism
\ShowEq{f:A->B}hPR
such that diagram
\ShowEq{coproduct in category diagram}
is commutative for all $i\in I$.
}{I made definition according to \citeBib{Serge Lang}, page 59.}

\DefProof{coproduct in category}
{
The theorem follows from definitions
\RefDefinition{universally repelling object of category},
\RefDefinition{coproduct in category}.
}

\DefTheoremNote{direct sum of Abelian groups}
{
Let
\ShowEq{set Bi}A
be set of Abelian groups.
Let
\ShowEq{A in xAi}
be such set that
\ShowEq{(xi)in A},
if
$x_i\ne 0$
for finite number of indices $i$.
Then\,\footnotemark
\ShowEq{A=o+Ai}A
}{See also proposition \citeBib{Serge Lang}-7.1, page 37.}

\DefProof{direct sum of Abelian groups}
{
According to the theorem
\RefTheorem[\RefRepresentation]{product exists in category of Omega algebras},
there exists Abelian group $B=\prod A_i$.
According to the statement
\RefItem[\RefRepresentation]{tuple represent A number},
$B$\Hyph number $a$ can be represented as tuple
\ShowEq{set Bi}a
$A_i$\Hyph numbers.
According to the statement
\RefItem[\RefRepresentation]{operation is defined componentwise},
the sum in group $B$ is defined by the equality
\ShowEq{(ai)+(bi)=(ai+bi)}

According to construction,
$A$ is subgroup of Abelian group $B$.
The map
\ShowEq{f:A->B}{\lambda_j}{A_j}A
defined by the equality
\ShowEq{lj(x)=0x0}
is an injective homomorphism.

Let
\ShowEq{set f:A->B}f{A_i}B
be set of homomorphisms into Abelian group $B$.
We define the map
\ShowEq{f:A->B}fAB
by the equality
\DrawEq{fxi,i=sum fxi}{group}
The sum in the right side of the equality
\eqRef{fxi,i=sum fxi}{group}
is finite, since all summands, except for a finite number, equal $0$.
From the equality
\ShowEq{fi(x+y)=}
and the equality
\eqRef{fxi,i=sum fxi}{group},
it follows that
\ShowEq{f(x+y)i=}
Therefore, the map $f$ is homomorphism of Abelian group.
The equality
\ShowEq{flj=fj}
follows from equalities
\EqRef{lj(x)=0x0},
\eqRef{fxi,i=sum fxi}{group}.
Since the map $\lambda_i$ is injective,
then the map $f$ is unique.
Therefore, the theorem folows from definitions
\RefDefinition{coproduct in category},
\RefDefinition{direct sum of Abelian groups}.
}

\AddEq{remark: Non-commutative Sum}
{
Since our childhood, we know that sum does not depend on order of summands.
So, when I learned about non-commutative addition
(\citeBib{Alain Connes 1994}),
I was little bit confused.
However I was lucky to see geometry where sum of vectors is non-commutative.

At school I liked many subjects: physics, chemistry, drafting.
I did not think about mathematics seriously.
I did not like arithmetic, but I liked algebra and geometry.
I did not yet know that all roads lead to mathematics.

Drafting was my favorite subject. My teacher,
Gabis Sergey Aleksandrovich, gave me problem book in drafting;
I solved every problem from this problem book.
After this I introduced my problem and solved it.
To my surprise, the first theorem which we proved on
geometry class next year was exactly the solution to this problem.

I knew that it will be hard to enter college after school.
So I decided to enter technical school after eight class.
Bela Markovna offered me few lessons during summer;
she wanted to see how far I was prepared for the exam on math.
I remember one lesson.
When we considered line and parabola graphs,
Bela Markovna said: it is easy to draw straight line or parabola;
however, what can we do with cardiogram?
I decided to find an analytical expression 
for cardiogram.

My friend offered me to study calculus
together during summer.
Boys who studied at a technical school lived in our building;
they gave me calculus textbook for summer time.
At this moment my friend lost interest to his idea;
and I began to study calculus independently.

The first chapter of the textbook was dedicated to analytic geometry.
So I realized that this is the tool that I need to analyze curves of cardiogram.
analytic geometry determined my future.
I realized that I will prepare myself for math department of university.

I have read a lot of books dedicated to calculus.
However, at some point of time, I got the impression
that one author copied off from another.
I started to look for different books.
I do not remember where did I get the first volume of Fihtengolts.
But this book impressed me very much.
Closer to spring, I felt that the book becomes difficult;
however I continued to read this book.
In March, I had the flu with an unusually high temperature.
But I doubt that it was a flu,
because it became easier to read the first volume of Fihtengolts.

The study of calculus reflected
in my attempts to restore functional
dependence on graph. I did not yet understand
that not every map could be represented analytically.
I drew graphs, made tables of dependence of function increment
on increment of argument.
However soon this idea bothered me;
and I changed direction of my learning.

When I started to read the book dedicated to tensor calculus,
I discovered that simple theorems of linear algebra
substituted complex calculations of analytic geometry
related to classification of second-order curves.
I lost my interest to analytic geometry
after this.

Almost half a century has passed.
And suddenly, analytic geometry brought me
two pleasant surprises.
I discovered that analytic geometry
has interesting structure from the point of view
of the theory of representation of universal algebra.
I identify analytic and affine geometries;
however, I think that this is not big mistake.

The second surprise is related to the fact that I realized
that I have model of affine geometry
in Riemann space.
Since I studied metric\hyph affine manifold for a very long time,
then there was one step left to see model of affine geometry
where sum is non\Hyph commutative.
Henceforth non\Hyph commutative addition
ceased to be abstract concept for me.
}

\DefText{side representation of group}
{
From the equality
\eqRef{* \SideNS-side representation of group}{def},
it follows that
\DrawEq{o \SideNS-side representation of group}{def}
We consider the equality
\eqRef{o \SideNS-side representation of group}{def}
as
\AddIndex{associative law}{associative law}.

\begin{sloppypar}
\begin{example}
Let
\ShowEq{f:A->B}f{A_2}{A_2}
\ShowEq{f:A->B}g{A_2}{A_2}
be endomorphisms of $\Omega_2$\Hyph algebra $A_2$.
Let product
in multiplicative $\Omega$\Hyph group
\ShowEq{End O2}{A_2}{}
is composition of endomorphisms.
Since the product of maps $f$ and $g$ is defined in the same order
as these maps act on $A_2$\Hyph number,
then we consider the equality
\ShowEq{fga= o \SideNS}
as
associative law.
This allows writing of equality
\EqRef{fga= o \SideNS}
without using of brackets
\ShowEq{fga= 1 \SideNS}
as well it allows writing of equality
\eqRef{\SideNS-side representation of group}{def}
in the following form
\DrawEq{\SideNS-side 1 representation of group}{def}
\qed
\end{example}
\end{sloppypar}
}

\AddEq[4]{theorem: select second basis of representation}
{
\begin{ShadedTheorem}
\labelTheorem{select second basis of representation, #4}
Let $#2$ be passive transformation of the
basis manifold of the #3 $#4$.
Let $\Basis e_1$ be the basis of the #3 $#4$,
\ShowEq{e2=e1 o S}{#2}21
For basis $\Basis e_3$, let there exists an active transformation $#1$ such that
\ShowEq{e3=R o e1}{#1}31
Let
\ShowEq{e3=R o e1}{#1}42
Then
\ShowEq{e2=e1 o S}{#2}43
\end{ShadedTheorem}
}

\AddEq[3]{proof: select second basis of representation}
{
\begin{proof}
According to the equality
\eqRef{active transformation}{#3},
active transformation of coordinates of basis $\Basis e_3$ has form
\DrawEq{active transformation, 1}{#3}
Let
\ShowEq{e2=e1 o S}{#2}53
From the equality
\eqRef{passive transformation}{#3},
it follows that
\DrawEq{passive transformation, 1}{#3}
From match of expressions in equalities
\eqRef{active transformation, 1}{#3},
\eqRef{passive transformation, 1}{#3},
it follows that
\ShowEq{Basis e4=Basis e5}
Therefore, the diagram
\ShowEq{passive and active maps}{#1}{#2}
is commutative.
\end{proof}
}

\AddEq[3]{definition: basis manifold}
{
The set
\ShowEq{basis manifold}
of bases of #1 $#2$ is called
\AddIndex{basis manifold}{basis manifold}
of #1 $#2$.
}

\AddEq{ref active representation, representation}
{
According to theorems
\RefTheorem{superposition of coordinates, representation},
\RefTheorem{Automorphism of representation maps a basis into basis},
}

\AddEq{ref active representation, diagram of representations}
{
According to the theorem
\RefTheorem{Automorphism of diagram of representations maps a basis into basis}
and to the definition
\RefDefinition{superposition of coordinates and words, diagram of representations},
}

\AddEq[4]{definition: active representation in basis manifold}
{
\begin{ShadedDefinition}
\labelDefinition{active representation in basis manifold, #1}
\ShowEq{ref active representation, #1}
automorphism $#4$ of the #2 $#3$
generates transformation
\DrawEq[{#4}]{active transformation}{#1}
of the basis manifold of #2.
This transformation is called
\AddIndex{active}{active transformation of basis}.
According to the theorem
\RefTheorem{group of automorphisms of #1},
we defined left\Hyph side representation
\ShowEq{active representation in basis manifold}
\ShowEq{active representation in basis manifold def}
of group $GA(f)$
in basis manifold $\mathcal B[f]$.
Representation $A(f)$ is called
\AddIndex{active representation}{active representation in basis manifold}.
According to the corollary
\RefCorollary{automorphism uniquely defined by image of basis, #1},
this representation is single transitive.
\qed
\end{ShadedDefinition}
}

\AddEq[3]{remark: active representation}
{
\begin{remark}
\labelRemark{active representation, #1}
According to remark
\RefRemark{X is quasibasis of #1},
it is possible that there exist bases of #2 $#3$
such that there is no active transformation between them.
Then we consider the orbit of selected basis
as basis manifold.
Therefore, it is possible that the #2 $#3$ has different basis manifolds.
We will assume that we have chosen a basis manifold.
\end{remark}
}

\AddEq[5]{theorem: Coordinate transformation does not depend}
{
\begin{ShadedTheorem}
\labelTheorem{Coordinate transformation does not depend, #1}
Let passive transformation $#2\in GA(f)$ maps
basis $\Basis e_1\in\mathcal{B}[f]$
into basis $\Basis e_2\in\mathcal{B}[f]$
\DrawEq[{#2}]{passive transformation S}{#1}
Let #4 $#3$ has #5
\DrawEq[1{#3}]{Omega_2 word, basis e}{1 #1}
relative to basis $\Basis e_1$ and has #5
\DrawEq[2{#3}]{Omega_2 word, basis e}{2 #1}
relative to basis $\Basis e_2$.
Coordinate transformation
\DrawEq[{#3}{#2}]{coordinate transformation}{#1}
does not depend on #4 $#3$ or basis $\Basis e_1$, but is
defined only by coordinates of #4 $#3$
relative to basis $\Basis e_1$.
\end{ShadedTheorem}
}

\AddEq[3]{proof: Coordinate transformation does not depend}
{
\begin{proof}
From \eqRef{passive transformation S}{#1}
and
\eqRef{Omega_2 word, basis e}{2 #1},
it follows that
\DrawEq[{#2}{#3}]{Omega word in representation, basis Y, 1}{#1}
Comparing \eqRef{Omega_2 word, basis e}{1 #1}
and
\eqRef{Omega word in representation, basis Y, 1}{#1}
we get
\DrawEq[{#2}{#3}]{coordinate transformation in representation, 1}{#1}
Since $#2$ is automorphism, then the equality
\eqRef{coordinate transformation}{#1}
follows from
\eqRef{coordinate transformation in representation, 1}{#1}
and the theorem
\RefTheorem{coordinates of inverse transformation, #1}.
\end{proof}
}

\AddEq[2]{remark: active and passive transformation}
{
An active transformation changes a basis of the #1
and #2 uniformly
and coordinates of $\Omega_2$\Hyph number relative basis do not change.
A passive transformation changes only the basis and it leads to change
of coordinates of #2 relative to the basis.
}

\AddEq[2]{theorem: Coordinate transformations form right-side representation}
{
\begin{ShadedTheorem}
\labelTheorem{Coordinate transformations form right-side representation, #1}
Coordinate transformations
\eqRef{coordinate transformation}{#1}
form effective contravariant
right\Hyph side representation of group $GA(f)$ which is called
\AddIndex{coordinate representation}{coordinate representation}
in #2.
\end{ShadedTheorem}
}

\AddEq[8]{proof: Coordinate transformations form right-side representation}
{
\begin{proof}
According to corollary
\RefCorollary{map of coordinates of #1},
the transformation
\eqRef{coordinate transformation}{#1}
is the endomorphism of #4\,\footnote{This transformation
does not generate an endomorphism of the #4 $#6$. Coordinates change because
basis relative which we determinate coordinates changes. However,
#7, coordinates of which we are considering, does not change.}
#5

Suppose we have two consecutive passive transformations
$#2$ and $#8$. Coordinate transformation
\DrawEq[{#3}{#2}]{coordinate transformation}{#2 #1}
corresponds to passive transformation $#2$.
Coordinate transformation
\DrawEq[{#3}{#8}]{coordinate transformation}{#8 #1}
corresponds to passive transformation $#8$.
According to the theorem
\RefTheorem{passive representation in basis manifold, diagram of representations},
product of coordinate transformations
\eqRef{coordinate transformation}{#2 #1}
and
\eqRef{coordinate transformation}{#8 #1}
has form
\ShowEq{coordinate transformation in representation, TS}{#3}{#2}{#8}
and is coordinate transformation
corresponding to passive transformation
\ShowEq{coordinate transformation in representation, TS 1}{#8}{#2}
According to theorems
\RefTheorem{coordinates of inverse transformation, #1},
\RefTheorem{coordinates of product of inverse transformation, #1}
and to the definition
\RefDefinition{Left side contravariant representation},
coordinate transformations
form
right\Hyph side contravariant representation of group $GA(f)$.

Suppose coordinate transformation does not change coordinates of selected basis.
Then unit of group $GA(f)$ corresponds to it because representation
is single transitive. Therefore,
coordinate representation is effective.
\end{proof}
}

\AddEq[5]{remark: geometric object}
{
Passive representation $P(g)$ is coordinated
with passive representation $P(f)$,
if there exists homomorphism $h$ of group $GA(f)$ into group $GA(g)$.
Consider diagram
\ShowEq{passive representation coordinated with passive representation}
Since maps $P(f)$, $P(g)$ are isomorphisms of group,
then map $H$ is homomorphism of groups.
Therefore, map $f'$ is representation of group $GA(f)$
in basis manifold $\mathcal B(g)$.
According to design, passive transformation $H(#2)$ of basis manifold $\mathcal B(g)$
corresponds to passive transformation $#2$ of basis manifold $\mathcal B(f)$
\DrawEq[{#2}]{passive transformation of representation g}{#1}
Then coordinate transformation in #3 $#4$ gets form
\DrawEq[{#5}{#2}]{coordinate transformation g}{#1}
}

\AddEq[5]{definition: coordinate of geometric object}
{
\begin{ShadedDefinition}
\labelDefinition{coordinate of geometric object, #1}
Orbit
\ShowEq{coordinates of geometric object}{#3}%
\ShowEq{show coordinates of geometric object}{#2}{#3}
is called
\AddIndex{coordinates of geometric object}{coordinates of geometric object}
defined in the #4 $#5$.
For any basis
\ShowEq{geometric object 1}{#2}
corresponding point 
\eqRef{coordinate transformation g}{#1}
of orbit defines
\AddIndex{coordinates of geometric object}{coordinates of geometric object}
relative basis
\ShowEq{geometric object 2}
\qed
\end{ShadedDefinition}
}

\AddEq[1]{remark: 2 views on geometric object}
{
Since a geometric object is an orbit of representation, we see that
according to the theorem
\RefTheorem{proper definition of orbit}
the definition of the geometric object is a proper definition.

Definition
\RefDefinition{coordinate of geometric object, #1}
introduces a geometric object in coordinate space.
We assume in definition \RefDefinition{geometric object, #1}
that we selected a basis of representation $g$.
This allows using a representative of the geometric object
instead of its coordinates.
}

\AddEq[6]{definition: geometric object}
{
\begin{ShadedDefinition}
\labelDefinition{geometric object, #1}
Orbit
\ShowEq{geometric object}{#3}%
\ShowEq{show geometric object}{#2}{#3}%
is called
\AddIndex{geometric object}{geometric object} 
defined in the #4 $#5$.
We also say that $#3$ is
a \AddIndex{geometric object of type $H$}{type of geometric object}.
For any basis
\ShowEq{geometric object 1}{#2}
corresponding point
\eqRef{coordinate transformation g}{#1}
of orbit defines #6
\ShowEq{geometric object 2, g}{#3}%
called
\AddIndex{representative of geometric object}{representative of geometric object}
in the #4 $#5$.
\qed
\end{ShadedDefinition}
}

\AddEq[1]{theorem: invariance principle}
{
\begin{ShadedTheorem}[invariance principle]
\AddIndex{}{invariance principle}
\labelTheorem{invariance principle, #1}
Representative of geometric object does not depend on selection
of basis $\Basis e_f$.
\end{ShadedTheorem}
}

\AddEq[6]{proof: invariance principle}
{
\begin{proof}
To define representative of geometric object,
we need to select basis $\Basis e_f$ of #2 $#3$,
basis $\Basis e_g$ of #2 $#4$
and coordinates of geometric object
\ShowEq{invariance principle 4}{#5}
Corresponding representative of geometric object
has form
\ShowEq{invariance principle 1}{#5}
Suppose we map basis $\Basis e_f$ to basis $\Basis e_{f1}$
by passive transformation
\ShowEq{invariance principle 2 passive}{#6}
According building this forms passive transformation
\eqRef{passive transformation of representation g}{#1}
and coordinate transformation
\eqRef{coordinate transformation g}{#1}.
Corresponding
representative of geometric object has form
\ShowEq{invariance principle 3 algebra}{#5}{#6}
Therefore representative of geometric object
is invariant relative selection of basis.
\end{proof}
}

\AddEq[1]{theorem: passive representation in basis manifold}
{
\begin{ShadedTheorem}
\labelTheorem{passive representation in basis manifold, #1}
There exists single transitive right\Hyph side representation
\ShowEq{passive representation in basis manifold}
\ShowEq{passive representation in basis manifold def}
of group $GA(f)$
in basis manifold $\mathcal B[f]$.
Representation $P(f)$ is called
\AddIndex{passive representation}{passive representation in basis manifold}.
\end{ShadedTheorem}
}

\DefProof{passive representation in basis manifold}
{
Since $A(f)$ is single transitive left\Hyph side representation of group $GA(f)$,
then single transitive right\Hyph side representation $P(f)$
is uniquely defined
according to the theorem
\RefTheorem{two representations of group}.
}

\AddEq[1]{theorem: passive transformation is automorphism of A(f)}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation is automorphism of A(f), #1}
Passive transformation of the basis manifold
is automorphism of representation $A(f)$.
\end{ShadedTheorem}
}

\DefProof{passive transformation is automorphism of A(f)}
{
The theorem follows from the theorem
\RefTheorem{twin representations of group, automorphism}.
}

\AddEq[3]{theorem: passive transformation}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation, #1}
Transformation of representation $P(f)$
is called
\AddIndex{passive transformation of the basis manifold}
{passive transformation of basis}
of #2.
We also use notation
\ShowEq{passive transformation of basis}{#3}
\ShowEq{passive transformation of basis def}{#3}
to denote the image of basis $\Basis e$ under passive transformation $#3$.
Passive transformation of basis has form
\DrawEq[#3]{passive transformation}{#1}
\end{ShadedTheorem}
}

\AddEq[1]{proof: passive transformation}
{
\begin{proof}
According to the equality
\eqRef{active transformation}{#1},
active transformation acts from left on coordinates
of basis.
The equality
\eqRef{passive transformation}{#1}
follows from theorems
\RefTheorem{shift is automorphism of representation},
\RefTheorem{two representations of group},
\RefTheorem{twin representations of group, automorphism};
according to these theorems,
passive transformation acts from right on coordinates
of basis.
\end{proof}
}

\DefLabeledDefinitionNote{side representation of group}{\SideNS}
{
Let
\ShowEq{End O2}{A_2}{}
be a multiplicative $\Omega$\Hyph group with product\,\footnotemark
\ShowEq{(fg)->fg}
Let an endomorphism $f$ act on $A_2$\Hyph number $a$ on the \SideNS.
We will use notation
\ShowEq{f(a)=o \SideNS}
Let $A_1$ be multiplicative $\Omega$\Hyph group with product
\ShowEq{(ab)->ab}
We call a homomorphism of multiplicative $\Omega$\Hyph group
\DrawEq{representation of group, map}{\SideNS-side}
\AddIndex{\SideNS\Hyph side representation}{\SideNS-side representation}
of multiplicative $\Omega$\Hyph group $A_1$
or
\AddIndex{\SideNS\Hyph side $A_1$\Hyph representation}{\SideNS-side A representation}
in $\Omega_2$\Hyph algebra $A_2$ if the map $f$ holds
\DrawEq{\SideNS-side representation of group}{def}
We identify
an $A_1$\Hyph number $a_1$ and its image $f(a_1)$
and write \SideNS\Hyph side transformation
caused by $A_1$\Hyph number $a_1$
as
\ShowEq{\SideNS-side representation}
In this case, the equality
\eqRef{\SideNS-side representation of group}{def}
gets following form
\DrawEq{* \SideNS-side representation of group}{def}
The map
\ShowEq{A12->A2 1 \SideNS}
generated by \SideNS\Hyph side representation $f$ is called
\AddIndex{\SideNS\Hyph side product}{\SideNS-side product}
of $A_2$\Hyph number $a_2$ over $A_1$\Hyph number $a_1$.
}
{
Very often a product
in multiplicative $\Omega$\Hyph group
\ShowEq{End O2}{A_2}{}
is superposition of endomorphisms
\ShowEq{Act=circ}
However, a product
in multiplicative $\Omega$\Hyph group
\ShowEq{End O2}{A_2}{}
may be different from superposition of endomorphisms.
}

\DefDefinition{reduced morphism of representations}
{
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$ and
\ShowEq{f:A->*B}g{A_1}{B_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $B_2$.
Let
\ShowEq{id:A1->A1 A2->B2}
be morphism of representations.
In this case we identify morphism
\ShowEq{map r,R}{\id}{r_2}{}
of representations of $\Omega_1$\Hyph algebra and corresponding homomorphism $r_2$ of $\Omega_2$\Hyph algebra
and the homomorphism $r_2$ is called
\AddIndex{reduced morphism of representations}
{reduced morphism of representations}.
We will use diagram
\ShowEq{morphism id,R of representations}
to represent reduced morphism $r_2$ of representations of
$\Omega_1$\Hyph algebra.
From diagram it follows
\ShowEq{morphism of representations of universal algebra}
We also use diagram
\ShowEq{morphism id,R of representations 2}
instead of diagram
\EqRef{morphism id,R of representations}.
}

\DefDefinition{action of rational integers in Abelian group}
{
The action of ring of rational integers $Z$
in Abelian group $G$
is defined using following rules
\ShowEq{action of rational integers in Abelian group}
}

\DefTheorem{action of ring of rational integers in Abelian group}
{
The action of ring of rational integers $Z$
in Abelian group $G$
defined in the definition
\RefDefinition{action of rational integers in Abelian group}
is representation.
The following equalities are true
\ShowEq{representation of Z in G}
}

\DefProof{action of ring of rational integers in Abelian group}
{
The equality
\EqRef{1a=a}
follows from the equality
\EqRef{0g=0}
and from the equality
\EqRef{(n+1)g=}
when $n=0$.

\ShowEq{step of proof: action in Abelian group}{(m+n)a=ma+na}

The equality
\ShowEq{(k+n)a-na=ka}
follows from the equality
\EqRef{(m+n)a=ma+na}.
The equality
\EqRef{(m-n)a=ma-na}
follows from the equality
\EqRef{(k+n)a-na=ka},
if we assume
$m=k+n$, $k=m-n$.

\ShowEq{step of proof: action in Abelian group}{(nm)a=n(ma)}

\ShowEq{step of proof: action in Abelian group}{n(a+b)=na+nb}

From the equality
\EqRef{n(a+b)=na+nb},
it follows that the map
\ShowEq{phi(n):G->G}
is an endomorphism of Abelian group $G$.
From equalities
\EqRef{(m+n)a=ma+na},
\EqRef{(nm)a=n(ma)},
it follows that the map
\ShowEq{phi:Z->End(G)}
is a homomorphism of the ring $Z$.
According to the definition
\RefDefinition[\RefRepresentation]{representation of algebra},
the map $\varphi$ is representation
of ring of rational integers $Z$
in Abelian group $G$.
}

\DefDefinitionNote{tensor product of representations}
{
Let $A$ be Abelian multiplicative $\Omega_1$\Hyph group.
Let
\ShowEq{a1n}An{}
be $\Omega_2$\Hyph algebras.\,\footnotemark
Let, for any
\ShowEq{k,1n}
\ShowEq{representation A Ak 1}
be effective representation of multiplicative $\Omega_1$\Hyph group $A$
in $\Omega_2$\Hyph algebra $A_k$.
Consider category $\mathcal A$ whose objects are
reduced polymorphisms of representations $f_1$, ..., $f_n$
\ShowEq{polymorphisms category}
where $S_1$, $S_2$ are $\Omega_2$\Hyph algebras and
\ShowEq{representation of algebra in S1 S2}
are effective representations of multiplicative $\Omega_1$\Hyph group $A$.
We define morphism
\ShowEq{r1->r2}
to be reduced morphism of representations $h:S_1\rightarrow S_2$
making following diagram commutative
\ShowEq{polymorphisms category, diagram}
Universal object
\ShowEq{tensor product of representations}
of category $\mathcal A$ is called
\AddIndex{tensor product}{tensor product}
of representations
\ShowEq{a1n}An.
}
{
I give definition
of tensor product of representations of universal algebra
following to definition in \citeBib{Serge Lang}, p. 601 - 603.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{tensor product of representations}
Since there exists polymorphism of representations,
then there exists tensor product of representations.
\end{ShadedTheorem}
}
{theorem: tensor product of representations}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation, tensor product}
Let
\ShowEq{equivalence, 1, representation, tensor product}
Tensor product is distributive over operation $\omega$
\ShowEq{tensors 1, representation, tensor product}
The representation of multiplicative $\Omega_1$\Hyph group $A$
in tensor product is defined by equality
\ShowEq{tensors 2, representation, tensor product}
\end{ShadedTheorem}
}
{theorem: representation, tensor product}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{tensor product and polymorphism}
Let $B_1$, ..., $B_n$ be
$\Omega_2$\Hyph algebras.
Let
\ShowEq{map f, 1, representation, tensor product}
be reduced polymorphism defined by equality
\ShowEq{map f, representation, tensor product}
Let
\ShowEq{map g, representation, tensor product}
be reduced polymorphism into $\Omega$\Hyph algebra $V$.
There exists morphism of representations
\ShowEq{map h, representation, tensor product}
such that the diagram
\ShowEq{map gh, representation, tensor product}
is commutative.
\end{ShadedTheorem}
}
{theorem: tensor product and polymorphism}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{B times->B otimes}
The map
\ShowEq{B times->B otimes}
is polymorphism.
\end{ShadedTheorem}
}
{theorem: B times->B otimes}
%DefEq

\DefTheorem{|a-b|>|a|-|b|}
{
Let $A$ be normed $\Omega$\Hyph group.
Then
\ShowEq{|a-b|>|a|-|b|}
}

\DefDefinitionNote{free representation of algebra}
{
The representation
\ShowEq{f:A->*B}f{A_1}{A_2}
of the $\Omega_1$\Hyph algebra $A_1$ is called
\AddIndex{free}{free representation},\,\footnotemark
if the statement
\ShowEq{faa=fba}
for any
\ShowEq{a in A}2{}
implies that
\ShowEq{a=b}.
}
{
See similar definition of free representation of group in
\citeBib{Postnikov: Differential Geometry}, page 16.
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
See also the theorem
\RefTheorem{free representation of group}.
\fi
}

\DefDefinition{continuous map, Omega group}
{
A map
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
of normed $\Omega_1$\Hyph group $A_1$ with norm $\|x\|_1$
into normed $\Omega_2$\Hyph group $A_2$ with norm $\|y\|_2$
is called \AddIndex{continuous}{continuous map}, if
for every as small as we please $\epsilon>0$
there exist such $\delta>0$, that
\ShowEq{|x'-x|<delta}
implies
\ShowEq{|f(x)-f(x')|<epsilon}
}

\DefTheorem{continuous map, open set}
{
A map
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
of normed $\Omega_1$\Hyph group $A_1$ with norm $\|x\|_1$
into normed $\Omega_2$\Hyph group $A_2$ with norm $\|y\|_2$
is continuous, iff
preimage of an open set
is the open set.
}

\DefTheorem{image of interval is interval, real field}
{
Let
\ShowEq{f:A->B}fRR
be continuous map of real field.
Then image of interval is interval.
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{norm of operation}
Let $A$
be normed $\Omega$\Hyph group.
For $n$\Hyph ary operation $\omega$, the value
\ShowEq{norm of operation}
\ShowEq{norm of operation, definition}
is called
\AddIndex{norm of operation}{norm of operation} $\omega$.
\qed
\end{ShadedDefinition}
}
{definition: norm of operation}
%\DefEq

\DefTheorem{|fx|<|f||x|1n}
{
Let $A$ be normed $\Omega$\Hyph group.
For $n$\Hyph ary operation $\omega$,
\ShowEq{|a omega|<|omega||a|1n}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{norm of representation}
Let
\ShowEq{f:A->*B}g{A_1}{A_2}
be representation
\ePrints{1305.4547}
\ifx\Semafor\ValueOn
\footnote{
See the definition
\ShowEq{ref definition: left-side representation of algebra}{}
of the representation of universal algebra.
According to the definition
\xRef[1211.6965]{definition: module over ring},
module is representation of ring in Abelian group.
Since ring and Abelian group are $\Omega$\Hyph groups,
then module is representation of $\Omega$\Hyph group.
}
\fi
of $\Omega_1$\Hyph group $A_1$ with norm $\|x\|_1$
in $\Omega_2$\Hyph group $A_2$ with norm $\|x\|_2$.
The value
\ShowEq{norm of representation}
\ShowEq{norm of representation, definition}
is called
\AddIndex{norm of representation}{norm of representation} $f$.
\qed
\end{ShadedDefinition}
}
{definition: norm of representation}
%\DefEq

\DefTheorem{|fab|<|f||a||b|}
{
Let
\ShowEq{f:A->*B}g{A_1}{A_2}
be representation
of $\Omega_1$\Hyph group $A_1$ with norm $\|x\|_1$
in $\Omega_2$\Hyph group $A_2$ with norm $\|x\|_2$.
Then
\ShowEq{|fab|<|f||a||b|}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{open set}
Let $A$ be normed $\Omega$\Hyph group.
A set
$U\subset A$
is called
\AddIndex{open}{open set},\,\footnote{
In topology,
we usually define an open set before we
define base of topology.
In the case of a metric or normed space,
it is more convenient to define an open set,
based on the definition of base of topology.
In such case, the definition is based on one of the properties of
base of topology. An immediate proof
allows us to see that defined such
an open set satisfies the basic properties.
}
if, for any $A$\Hyph number
\ShowEq{a in U},
there exists
\ShowEq{epsilon in R}
such that
\ShowEq{B(a) subset U}
\qed
\end{ShadedDefinition}
}
{definition: open set}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{compact set}
A set $T$ of topological space is called
\AddIndex{compact}{compact set},
if every open cover of $T$ has
finite subcover.\,\footnote{
See also the definition
\citeBib{Kolmogorov Fomin}-1, page 92.
}
\qed
\end{ShadedDefinition}
}
{definition: compact set}
%\DefEq

\DefTheorem{c1+c2 in B}
{
Let $A$ be normed $\Omega$\Hyph group.
For
\ShowEq{c1 c2 in A}
let
\ShowEq{c1 c2 in B}
Then
\ShowEq{c1+c2 in B}
}

\DefLabeledDefinition{limit of sequence}{normed \Algebrac}
{
Let $\Module$
be normed $\Base$\Hyph \Algebrab.
$\Module$\Hyph number $a$ is called 
\AddIndex{limit of a sequence}{limit of sequence}
\ShowEq{[an] in A}
\ShowEq{limit of sequence}
if for any
\ShowEq{epsilon in R}
there exists positive integer $n_0$ depending on $\epsilon$ and such, that
\DrawEq{|an-a|<epsilon}{-}
for every $n>n_0$.
We also say that
\AddIndex{sequence $a_n$ converges}{sequence converges}
to $a$.
}

\AddEq{theorem: limit of sequence}
{
\begin{ShadedTheorem}
\labelTheorem{limit of sequence, normed \Algebrac}
Let $\Module$
be normed $\Base$\Hyph \Algebrab.
$\Module$\Hyph number $a$ is
limit of a sequence
\ShowEq{[an] in A}
\DrawEq{a=lim an}{}
if for any
\ShowEq{epsilon in R}
there exists positive integer $n_0$ depending on $\epsilon$ and such, that
\DrawEq{an in B(a)}{}
for every $n>n_0$.
\end{ShadedTheorem}
}

\DefProof{limit of sequence}
{
The theorem follows from definitions
\RefDefinition{open ball},
\refDefinition{limit of sequence}{normed \Algebrac}.
}

\DefLabeledDefinition{fundamental sequence}{normed \Algebrac}
{
Let $\Module$
be normed $\Base$\Hyph \Algebrab.
The sequence
\ShowEq{[an] in A}
is called 
\AddIndex{fundamental}{fundamental sequence}
or \AddIndex{Cauchy sequence}{Cauchy sequence},
if for every
\ShowEq{epsilon in R}
there exists positive integer $n_0$ depending on $\epsilon$ and such, that
\DrawEq{|ap-aq|<epsilon}{-}
for every $p$, $q>n_0$.
}

\AddEq{theorem: fundamental sequence}
{
\begin{ShadedTheorem}
\labelTheorem{fundamental sequence, normed \Algebrac}
Let $\Module$
be normed $\Base$\Hyph \Algebrab.
The sequence
\ShowEq{[an] in A}
is fundamental sequence,
iff for every
\ShowEq{epsilon in R}
there exists positive integer $n_0$ depending on $\epsilon$ and such, that
\ShowEq{aq in B(ap)}
for every $p$, $q>n_0$.
\end{ShadedTheorem}
}

\DefProof{fundamental sequence}
{
The theorem follows from definitions
\RefDefinition{open ball},
\refDefinition{fundamental sequence}{normed \Algebrac}.
}

\DefTheorem{norm of compact set is bounded}
{
Let $C$ be compact set of
normed $\Omega$\Hyph group $A$.
Then the norm
\ShowEq{|x in C|}
is bounded from both sides.
}

\DefTheorem{lim a=lim b}
{
Let $A$ be normed $\Omega$\Hyph group.
Let $a_n$, $b_n$, $n=1$, ..., be fundamental sequences.
Let
\DrawEq{lim a-b=0}{limit}
If the sequence $a_n$ converges, then
the sequence $b_n$ converges and
\ShowEq{lim a=lim b}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{complete Omega group}
Normed $\Omega$\Hyph group $A$ is called
\AddIndex{complete}{complete Omega group}
if any fundamental sequence of elements
of $\Omega$\Hyph group $A$ converges, i.e.
has limit in $\Omega$\Hyph group $A$.
\qed
\end{ShadedDefinition}
}
{definition: complete Omega group}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{limit of sequence, map to Omega group}
Let
\ShowEq{fn M(X,A)}
be sequence of maps into normed
$\Omega$\Hyph group $A$.
The map
\ShowEq{f M(X,A)}
is called
\AddIndex{limit of sequence}{limit of sequence}
$f_n$, if for any $x\in X$
\DrawEq{f(x)=lim}{}
We also say that
\AddIndex{sequence $f_n$ converges}{sequence converges}
to the map $f$.
\qed
\end{ShadedDefinition}
}
{definition: limit of sequence, map to Omega group}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{sequence converges uniformly}
Let
\ShowEq{fn M(X,A)}
be sequence of maps into normed
$\Omega$\Hyph group $A$.
\AddIndex{Sequence $f_n$ converges uniformly}
{sequence converges uniformly}
to the map $f$,
if for any
\ShowEq{epsilon in R}
there exists $N$ such that
\ShowEq{fn(x) - f(x)}
for any $n>N$.
\qed
\end{ShadedDefinition}
}
{definition: sequence converges uniformly}
%\DefEq

\DefTheorem{sequence converges uniformly, fn-fm}
{
Sequence of maps
\ShowEq{fn M(X,A)}
into normed
$\Omega$\Hyph group $A$ converges uniformly
to the map $f$,
if for any
\ShowEq{epsilon in R}
there exists $N$ such that
\ShowEq{|fn(x)-fm(x)|<e}
for any \(n\), \(m>N\).
}

\DefDefinition{quasibasis of representation}
{
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be representation
of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$
and
\ShowEq{Gen f =}
If, for the set $X\subset A_2$, it is true that
\ShowEq{in Gen}Xf,
then for any set $Y$, $X\subset Y\subset A_2$,
also it is true that
\ShowEq{in Gen}Yf.
If there exists minimal set
\ShowEq{in Gen}Xf,
then the set $X$ is called
\AddIndex{quasibasis}{quasibasis}
of representation $f$.
}

\DefTheorem{X is quasibasis of representation}
{
If the set $X$ is the quasibasis of the representation $f$,
then, for any $m\in X$,
the set $X\setminus\{m\}$ is not
generating set of the representation $f$.
}

\DefRemark{X is quasibasis of representation}
{
The proof of the theorem
\RefTheorem{X is quasibasis of representation}
gives us effective method for constructing the quasibasis of the representation $f$.
Choosing an arbitrary generating set, step by step, we
remove from set those elements which have coordinates
relative to other elements of the set.
If the generating set of the representation is infinite,
then this construction may not have the last step.
If the representation has finite generating set,
then we need a finite number of steps to construct a quasibasis of this representation.
}

\AddEq{remark: representation in form of Omega2-word is ambiguous}
{
We introduced $\Omega_2$\Hyph word of $x\in A_2$ relative generating set $X$
in the definition
\RefDefinition{word of element relative to set, representation}.
From the theorem
\RefTheorem{X is quasibasis of representation},
it follows that if the generating set $X$ is not an quasibasis,
then a choice of $\Omega_2$\Hyph word relative generating set $X$ is ambiguous.
However, even if the generating set $X$ is an quasibasis,
then a representation of $m\in A_2$ in form of $\Omega_2$\Hyph word is ambiguous.
}

\DefDefinitionNote{word of element relative to set, representation}
{
Let $X\subset A_2$.
For each
\ShowEq{x in JX}m{}
there exists
\AddIndex{$\Omega_2$\Hyph word}
{word of element relative to generating set, representation}
defined according to following rules.
\ShowEq{word of element relative to generating set, representation}
\StartLabelItem
\begin{enumerate}
\item If $m\in X$, then $m$ is $\Omega_2$\Hyph word.
\labelItem{word of element relative to set, representation, m in X}
\item If $m_1$, ..., $m_n$ are $\Omega_2$\Hyph words and
$\omega\in\Omega_2(n)$, then $m_1...m_n\omega$
is $\Omega_2$\Hyph word.
\labelItem{word of element relative to set, representation, omega}
\item If $m$ is $\Omega_2$\Hyph word and
\ShowEq{a in A1},
then $f(a)(m)$
is $\Omega_2$\Hyph word.
\labelItem{word of element relative to set, representation, am}
\end{enumerate}
We will identify an element
\ShowEq{x in JX}m{}
and corresponding it $\Omega_2$\Hyph word using equation
\ShowEq{identify element jf(X) and word}
Similarly, for an arbitrary set
\ShowEq{subset of representation}{}
we consider the set of $\Omega_2$\Hyph words\,\footnotemark
\ShowEq{subset of words of representation}
We also use notation
\ShowEq{subset of words of representation, 1}
Denote
\ShowEq{word set of representation}
\AddIndex{the set of $\Omega_2$\Hyph words of representation $J[f,X]$}
{word set of representation}.
}{
The expression $\wXm$
is a special case
of the expression $\wXm[B]$, namely
\ShowEq{subset of words of representation, 2}
}

\DefRemark{three reasons of ambiguity in Omega2-word}
{
There are three reasons of ambiguity in notation of
$\Omega_2$\Hyph word.
\StartLabelItem
\begin{enumerate}
\item
In $\Omega_i$\Hyph algebra $A_i$, $i=1$, $2$,
equalities may be defined.
For instance, if $e$ is unit of multiplicative group $A_i$,
then the equality
\[ae=a\]
is true for any $a\in A_i$.
\item
\begin{sloppypar}
Ambiguity of choice of $\Omega_2$\Hyph word
may be associated with properties of representation.
For instance, if $m_1$, ..., $m_n$ are $\Omega_2$\Hyph words,
$\omega\in\Omega_2(n)$ and
\ShowEq{a in A1},
then\,\footnote{
For instance, let
$\{e_1,e_2\}$
be the basis of vector space over field $k$.
The equation \EqRef{ambiguity of coordinates 1}
has the form of distributive law
\ShowEq{ambiguity of coordinates 1, vector}
}
\ShowEq{ambiguity of coordinates 1}
At the same time, if $\omega$ is operation of
$\Omega_1$\Hyph algebra $A_1$ and operation of
$\Omega_2$\Hyph algebra $A_2$, then we require
that $\Omega_2$\Hyph words
\ShowEq{a1n omega x}
and
\ShowEq{a1n x omega}
describe the same
element of $\Omega_2$\Hyph algebra $A_2$.\,\footnote{For vector space,
this requirement has the form of distributive law
\ShowEq{(a+b)e=ae+be}
}
\DrawEq{ambiguity of coordinates 2}{representation}
\end{sloppypar}
\item
Equalities like
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
persist under morphism of representation.
Therefore we can ignore this
form of ambiguity of $\Omega_2$\Hyph word.
However, a fundamentally different form of ambiguity is possible.
We can see an example of such ambiguity
in theorems
\refTheorem[\RefRepresentation]{linear dependence between vectors of basis}{\SideWS module},
\refTheorem[\RefRepresentation]{coordinates of vector with linear dependence}{\SideWS module}.
\end{enumerate}
So we see that we can define different equivalence relations
on the set of $\Omega_2$\Hyph words.\,\footnote{
Evidently each of the equalities
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
generates some equivalence relation.
}
Our goal is to find a maximum equivalence
on the set of $\Omega_2$\Hyph words which
persist under morphism of representation.
}

\DefTheoremNote{equivalence generated by basis}
{
Let $X$ be quasibasis of the representation
\ShowEq{f:A->*B}f{A_1}{A_2}
For an generating set $X$ of representation $f$,
there exists equivalence
\ShowEq{l fX in w fX}
which is generated exclusively by the following statements.
\StartLabelItem
\begin{enumerate}
\item
%\labelItem{w1 w2 in l fX}
If in $\Omega_2$\Hyph algebra $A_2$ there is an equality
\ShowEq{w1[]=w2[]}
defining structure of $\Omega_2$\Hyph algebra, then
\ShowEq{w1 w2 in l fX}
\item
%\labelItem{fw1m fw2m in l fX}
If in $\Omega_1$\Hyph algebra $A_1$ there is an equality
\ShowEq{w1[]=w2[]}
defining structure of $\Omega_1$\Hyph algebra, then
\ShowEq{fw1m fw2m in l fX}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l}
For any operation
\ShowEq{omega n ari}{}1n,
\ShowEq{(f(a1n)a2,f(a)a2) in l}
\item
%\labelItem{(fa1(a21n),fa1(a2)) in l}
For any operation
\ShowEq{omega n ari}{}2n,
\ShowEq{(fa1(a21n),fa1(a2)) in l}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l 1}
Let
\ShowEq{omega in O1AO2}12.
If the representation $f$ satisfies equality\,\footnotemark
\ShowEq{f(a1n)a2=f(a)a2}
then we can assume that the following equality is true
\ShowEq{(f(a1n)a2,f(a)a2) in l 1}
\end{enumerate}
}
{
Consider a representation of commutative ring $D$
in $D$\Hyph algebra $A$. We will use notation
\ShowEq{f(a)(v)=av}
The operations of addition and multiplication are defined in both algebras.
However the equality
\ShowEq{f(a+b)v=}
is true, and the equality
\ShowEq{f(ab)v=}
is wrong.
}

\DefDefinition{basis of representation}
{
Quasibasis $\Basis e$ of the representation $f$ such that
\ShowEq{rho=lambda}
is called
\AddIndex{basis of representation}{basis of representation} $f$.
}

\DefDefinition{equivalence on the set of Omega2-words}
{
Generating set $X$ of representation $f$
generates equivalence
\ShowEq{rho fX=}
on the set of $\Omega_2$\Hyph words.
}

\DefTheorem{h=f+g, converges uniformly}
{
Let sequence of maps
\ShowEq{fn M(X,A)}
into complete $\Omega$\Hyph group $A$
converge uniformly
to the map $f$.
Let sequence of maps
\ShowEq{gn M(X,A)}
into complete $\Omega$\Hyph group $A$
converge uniformly
to the map $g$.
Then sequence of maps
\ShowEq{hn=fn+gn}
into complete $\Omega$\Hyph group $A$
converges uniformly
to the map
\DrawEq{h=f+g}{converges uniformly}
}

\DefTheorem{representation f generates representation fX}
{
The representation
\ShowEq{f:A->*B}g{A_1}{A_2}
of $\Omega_1$\Hyph group $A_1$ with norm $\|x\|_1$
in $\Omega_2$\Hyph group $A_2$ with norm $\|x\|_2$
generates representation
\ShowEq{f:A->*B}{f_X}{M(X,A_1)}{M(X,A_2)}
of $\Omega_1$\Hyph group
\ShowEq{M(X,A1)}
in $\Omega_2$\Hyph group
\ShowEq{M(X,A2)}
where (
\ShowEq{g1 in M(X,A1)},
\ShowEq{g2 in M(X,A2)}
)
\ShowEq{f(x)g(x):X->A2}
}

\DefTheorem{fX(g1)(g2), converges uniformly}
{
Let
\ShowEq{f:A->*B}g{A_1}{A_2}
be representation
of complete $\Omega_1$\Hyph group $A_1$ with norm $\|x\|_1$
in complete $\Omega_2$\Hyph group $A_2$ with norm $\|x\|_2$.
Let sequence of maps
\ShowEq{g1n M(X,A1)}
converge uniformly
to the map $g_1$.
Let sequence of maps
\ShowEq{g2n M(X,A2)}
converge uniformly
to the map $g_2$.
Let range of the map $g_i$, $i=1$, $2$,
be compact set.
Then the sequence of maps
\ShowEq{f(g1n)(g2n)}
converge uniformly
to the map
\ShowEq{fX(g1)(g2)}.
}

\DefTheorem{set of maps to Omega group}
{
Let
\ShowEq{set of maps to Omega group}
be set of maps of a set $X$ to $\Omega$\Hyph group $A$.
We can define the structure of $\Omega$\Hyph group on the set
\EqParm{M(X,A)}{=.}
}

\DefEq
{
Since $X$ is an arbitrary set, we cannot define
norm in $\Omega$\Hyph group
\EqParm{M(X,A)}{=.}
However we can define the convergence of the sequence in
\EqParm{M(X,A)}{=.c}
therefore, we can define a topology in
\EqParm{M(X,A)}{=.}
}
{remark: set of maps to Omega group}
%\DefEq

\DefDefinition{closed ball}
{
Let $\Module$
be normed $\Base$\Hyph \Algebrab.
Let $a\in \Module$.
The set
\ShowEq{closed ball}
is called
\AddIndex{closed ball}{closed ball}
with center at $a$.
}

\DefDefinition{open ball}
{
Let $\Module$
be normed $\Base$\Hyph \Algebrab.
Let $a\in \Module$.
The set
\ShowEq{open ball}
is called
\AddIndex{open ball}{open ball}
with center at $a$.
}

\DefDefinition{reduced polymorphism of representations}
{
Let
\ShowEq{set of universal algebras 1}
be universal algebras.
Let, for any
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}A{B_k}
be effective representation of $\Omega_1$\Hyph algebra $A$
in $\Omega_2$\Hyph algebra $B_k$.
Let
\ShowEq{f:A->*B}fAB
be effective representation of $\Omega_1$\Hyph algebra $A$
in $\Omega_2$\Hyph algebra $B$.
The map
\ShowEq{reduced polymorphism of representation}
is called
\AddIndex{reduced polymorphism of representations}
{reduced polymorphism of representations}
$f_1$, ..., $f_n$ into representation $f$,
if, for any
\ShowEq{k,1n}
provided that all variables except the variable $x_k\in B_k$
have given value, the map $r_2$
is a reduced morphism of representation $f_k$ into representation $f$.

If $f_1=...=f_n$, then we say that the map $r_2$
is reduced polymorphism of representation $f_1$ into representation $f$.

If $f_1=...=f_n=f$, then we say that the map $r_2$
is reduced polymorphism of representation $f$.
}

\DefConvention{Einstein summation}
{
We will use Einstein summation convention.
When an index is present in
an expression twice (one above and one below) and a set of index is known,
we have the sum with respect to repeated index.
In this case we assume that we know the set
of summation index and do not use summation symbol
\ShowEq{av=sum av}av
If needed to clearly
show set of index, I will do it.
}

\DefTheorem{structure of Abelian group}
{
Let $G$ be Abelian group.
The set of $G$\Hyph numbers generated by the set
\ShowEq{S=si}
has form
\ShowEq{J(S)=gi si}
where the set
\ShowEq{|gi ne 0|}g
is finite.
}

\DefProof{structure of Abelian group}
{
We prove the theorem by induction based on the theorems
\citeBib{Cohn: Universal Algebra}\Hyph 5.1, page 79 and
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

For any $s_k\in S$,
let
\ShowEq{gi=dik}
Then
\ShowEq{sk=sum si}
\ShowEq{sk in JS}
follows from
\EqRef{J(S)=gi si},
\EqRef{sk=sum si}.

Let
\ShowEq{w12 in Jv}gS
Since $G$ is Abelian group,
then, according to the statement
\RefItem[\RefRepresentation]{x1n omega in Xk+1},
\ShowEq{w1+w2 in Jv}gS
According to the equality
\EqRef{J(S)=gi si},
there exist $Z$\Hyph numbers
\ShowEq{gi12}g
such that
\DrawEq[g]{w12= }{group}
where sets
\DrawEq[g]{|ci12 ne 0|}{group}
are finite.
From the equality
\eqRef{w12= }{group},
it follows that
\DrawEq[g]{w1+w2= }{group}
The equality
\DrawEq[g]{w1+w2= 1 }{group}
follows from equalities
\EqRef{(m+n)a=ma+na},
\eqRef{w1+w2= }{group}.
From the equality
\eqRef{|ci12 ne 0|}{group},
it follows that
the set
\ShowEq{|gi 1+2 ne 0|}g
is finite.
From the equality
\eqRef{w1+w2= 1 }{group},
it follows that
\ShowEq{w1+w2 in Jv}gS
}

\AddEq [1]{step of proof: action in Abelian group}
{
From the equality
\EqRef{0g=0},
it follows that the equality
\EqRef{#1}
is true when $n=0$.
\def\TempA{(nm)a=n(ma)}
\def\TempB{#1}
\begin{itemize}
\item
Let the equality
\EqRef{#1}
is true when $n=k\ge 0$.
Then
\ShowEq{#1,n=k}
The equality
\ShowEq{#1,n=k+1}
follows from
\ifx\TempA\TempB
equalities
\EqRef{(n+1)g=},
\EqRef{(m+n)a=ma+na}.
\else
the equality
\EqRef{(n+1)g=}.
\fi
Therefore, the equality
\EqRef{#1}
is true when $n=k+1$.
According to mathematical induction,
the equality
\EqRef{#1}
is true for any $n\ge 0$.
\item
Let the equality
\EqRef{(m+n)a=ma+na}
is true when $n=k\le 0$.
Then
\ShowEq{#1,n=k}
The equality
\ShowEq{#1,n=k-1}
follows from
\ifx\TempA\TempB
equalities
\EqRef{(n-1)g=},
\EqRef{(m-n)a=ma-na}.
\else
the equality
\EqRef{(n-1)g=}.
\fi
Therefore, the equality
\EqRef{#1}
is true when $n=k-1$.
According to mathematical induction,
the equality
\EqRef{#1}
is true for any $n\le 0$.
\item
Therefore, the equality
\EqRef{#1}
is true for any $n\in Z$.
\end{itemize}
}

\DefDefinition{category of representations A1(mA2)}
{
Let $A_1$ be $\Omega_1$\Hyph algebra.
Let $\mathcal A_2$ be category of $\Omega_2$\Hyph algebras.
We define \AddIndex{category
\ShowEq{A1(mA2) symb}
of representations}
{category of representations}
of $\Omega_1$\Hyph algebra $A_1$ in $\Omega_2$\Hyph algebra.
Representations of $\Omega_1$\Hyph algebra $A_1$ in $\Omega_2$\Hyph algebra
are objects of this category.
Reduced morphisms of corresponding representations are morphisms of this category.
}

\DefProofRef{cr transpose}{}
{
We can prove \eqRef{cr transpose}{Theorem}
in case of matrices the same way as we
proved \eqRef{rc transpose}{Theorem}. However it is
more important for us to show that \eqRef{cr transpose}{Theorem}
follows directly from \eqRef{rc transpose}{Theorem}.

Applying \EqRef{double transpose} to each term in left side of
\eqRef{cr transpose}{Theorem} we get
\ShowEq{cr transpose, 1}
From \EqRef{cr transpose, 1} and \eqRef{rc transpose}{Theorem}
it follows that
\ShowEq{cr transpose, 2}
\eqRef{cr transpose}{Theorem} follows from \EqRef{cr transpose, 2}
and \EqRef{double transpose}.
}

\DefProofRef{rc transpose}{}
{
The chain of equalities
\ShowEq{rc transpose, 1}
follows from \EqRef{transpose of matrix, 1},
\EqRef{rc-product of matrices} and
\EqRef{cr-product of matrices}.
The equality \eqRef{rc transpose}{Theorem} follows from
\EqRef{rc transpose, 1}.
}

\DefText{matrix operations 1}
{
According to the custom the product of
matrices $a$ and $b$ is defined as product of
rows of the matrix $a$ and columns of the matrix $b$.
\ePrints{1908.04418,6860-2955,2020.06.01,2204.06320,2022.01.05}
\Items{8428-0408,2207.06506}%
\ifx\Semafor\ValueOn
In non\Hyph commutative algebra, this product
is not enough to solve some problems.
\ePrints{8428-0408,2207.06506}
\ifx\Semafor\ValueOff
\ShowExample{matrix in right vector space}

\ShowExample{matrix in left vector space}

From examples
\RefExample{matrix in right vector space},
\RefExample{matrix in left vector space},
\else
\TwoColText
{
\ShowEq{def left}
\ShowEq{def AVector}%
\ShowEq{\DefCol}
\ShowExample{matrix in vector space}
}
{
\ShowEq{def right}
\ShowEq{def AVector}%
\ShowEq{\DefCol}
\ShowExample{matrix in vector space}
}

From examples
\refExample{matrix in vector space}{left},
\refExample{matrix in vector space}{right}
\fi
it follows that
\else
If the product in
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
$D$\Hyph algebra
\else
$\Omega$\Hyph ring
\fi
is non\Hyph commutative,
\fi
we cannot confine ourselves to traditional product of matrices
and we need to define two products of matrices.
To distinguish between these products we introduced
a new notation.
}

\DefText{matrix operations 2}
{
We also consider following operations on the set of matrices.
}

\DefExample{matrix in left vector space}
{
We represent the basis $\Basis e$
of left vector space $V$
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
over $D$\Hyph algebra $A$
(see the definition
\ShowEq{def left}%
\ShowEq{def AVector}%
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
and the theorem
\refTheorem{basis over division algebra}{left})
\fi
as row of matrix
\DrawEq[en]{a=(a1.n row)}{left basis}
We represent coordinates of vector
\ShowEq{w=w*e left-cols}v{}
as vector column
\DrawEq[vn]{a=(a1.n col)}{left basis}
However, we cannot represent the vector $\Vector v$
as product of matrices
\ShowEq{v=(v)(e)}
because this product is not defined.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
We represent homomorphism
of left vector space $V$
using matrix
\ShowEq{v'=vf}
We cannot express the equality
\EqRef{v'=vf}
as traditional product of matrices $v$ and $f$.
\fi
}

\AddEq{define basis for example}
{
We represent the set of vectors
\ShowEq{\RowN() 1n}en{}
of basis $\Basis e$
of \SideWS vector space $V$
over $D$\Hyph algebra $A$
(see the definition
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
and the theorem
\refTheorem{basis over division algebra}{left})
as
\RowNWS of matrix
\DrawEq[en]{a=(a1.n \RowN)}{\SideWS basis}
We represent coordinates
\ShowEq{\ColNS() 1n}vn{}
of vector
\ShowEq{w=w*e left-cols}v{}
as \ColWS of matrix
\DrawEq[vn]{a=(a1.n \ColNS)}{vn \SideNS-\Cols}
}

\AddEq{vector as matrix product left}
{
Therefore, we can represent the vector $\Vector v$
as product of matrices
\ShowEq{v=(e)(v)}
}

\AddEq{vector as matrix product right}
{
However, we cannot represent the vector $\Vector v$
as product of matrices
\ShowEq{v=(v)(e)}
because this product is not defined.
}

\DefLabeledExample{matrix in vector space}{\SideNS}
{
\ShowEq{define basis for example}
\ShowEq{vector as matrix product \SideNS}
}

\DefExample{matrix in right vector space}
{
We represent the basis $\Basis e$
of right vector space $V$
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
over $D$\Hyph algebra $A$
(see the definition
\ShowEq{def right}%
\ShowEq{def AVector}%
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
and the theorem
\refTheorem{basis over division algebra}{right})
\fi
as row of matrix
\DrawEq[en]{a=(a1.n row)}{right basis}
We represent coordinates of vector
\ShowEq{w=w*e right-cols}v{}
as vector column
\DrawEq[vn]{a=(a1.n col)}{right basis}
Therefore, we can represent the vector $\Vector v$
as product of matrices
\ShowEq{v=(e)(v)}
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
We represent homomorphism
of right vector space $V$
using matrix
\ShowEq{v'=fv}
The equality
\EqRef{v'=fv}
expresses a traditional product of matrices $f$ and $v$.
\fi
}

\DefDefinition{row over column product}
{
Let the nubmer of columns of the matrix $a$ equal the number of rows of the matrix $b$.
\AddIndex{\RC product}{rc-product}
of matrices $a$ and $b$ has form
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
\ShowEq{entry rc-product of matrices}
\ShowEq{rc-product, matrices}
\RC product can be expressed as product of a row of the matrix $a$
over a column of the matrix $b$.
}

\DefDefinition{column over row product}
{
Let the nubmer of rows of the matrix $a$ equal the number of columns of the matrix $b$.
\AddIndex{\CR product}{cr-product}
of matrices $a$ and $b$ has form
\ShowEq{cr-product}
\ShowEq{cr-product of matrices}
\ShowEq{entry cr-product of matrices}
\ShowEq{cr-product, matrices}
\CR product can be expressed as product of a column of the matrix $a$
over a row of the matrix $b$.
}

\DefDefinition{transpose of matrix}
{
The transpose $a^T$ of the matrix $a$
exchanges rows and columns
\ShowEq{transpose of matrix, 1}
}

\DefDefinition{sum of matrices}
{
The sum of matrices $a$ and $b$ is defined by the equality
\ShowEq{(a+b)=}
}

\DefDefinition{rc power}
{
We introduce \AddIndex{\RC power}{rc power} of
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph number
\else
the matrix
\fi
$a$
using recursive definition
\ShowEq{rc power}
\DrawEq{rc power, 0}1
\DrawEq{rc-power, n}1
}

\DefDefinition{cr power}
{
We introduce \AddIndex{\CR power}{cr power} of
$\mathcal{A}$\Hyph number $a$
using recursive definition
\ShowEq{cr power}
\DrawEq{cr power, 0}1
\DrawEq{cr-power, n}1
}

\DefDefinitionNote{Hadamard inverse of matrix}
{
Let
\DrawEq[ann]{a=(a11.nm matrix)}{}
be a matrix of $A$\Hyph numbers.
We call matrix\,\footnotemark
\ShowEq{Hadamard inverse of matrix}
\ShowEq{Hadamard inverse of matrix 2}
\ShowEq{Hadamard inverse of matrix 2 entry}
\AddIndex{Hadamard inverse of matrix}{Hadamard inverse of matrix} $a$
(\citeBib{q-alg-9705026}-\href{https://arxiv.org/pdf/math/9705026.pdf\#Page=4}{page 4}).
}{
The notation in the equality
\EqRef{Hadamard inverse of matrix 2 entry}
means that we exchange rows and columns
in Hadamard inverse.
\label{footnote: index of inverse element}
We can
formally write right site of the equality
\EqRef{Hadamard inverse of matrix 2 entry}
in the following form
\ShowEq{Hadamard inverse of matrix 3}
}

\DefDefinition{transformation coordinated with equivalence}
{
Let $S$ be equivalence on the set $A_2$.
Transformation $f$ is called
\AddIndex{coordinated with equivalence}{transformation coordinated with equivalence} $S$,
when
\ShowEq{fm1 fm2 modS}{}
follows from condition
\ShowEq{m1 m2 modS}.
}

\DefTheorem{transformation correlated with equivalence}
{
Consider equivalence $S$ on set $A_2$.
Consider $\Omega_1$\Hyph algebra
on the set
\ShowEq{End O2}{A_2}.
If any transformation
\ShowEq{f in End A2}{}
is coordinated with equivalence $S$,
then we can define the structure of $\Omega_1$\Hyph algebra
on the set
\ShowEq{End A2/S}S.
}

\DefTheorem{decompositions of morphism of representations}
{
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
be representation of $\Omega_1$\Hyph algebra $B_1$.
Let
\ShowEq{r12:A->B}tAB
be morphism of representations from $f$ into $g$.
Then there exist decompositions of $t_1$ and $t_2$,
which we describe using diagram
\ShowEq{decompositions of morphism of representations, diagram}
\StartLabelItem
\begin{enumerate}
\item
The kernel of homomorphism
\ShowEq{kernel of homomorphism i}
is a congruence on $\Omega_i$\Hyph algebra $A_i$,
\ShowEq{i=1,2}.
\labelItem{kernel of homomorphism i}
\item
There exists decomposition of homomorphism $t_i$,
\ShowEq{i=1,2},
\ShowEq{morphism of representations of algebra, homomorphism, 1}
\labelItem{exists decomposition of homomorphism}
\item
Maps
\ShowEq{morphism of representations of algebra, p1=}
\ShowEq{morphism of representations of algebra, p2=}
are natural homomorphisms.
\labelItem{p12 are natural homomorphisms}
\item
Maps
\ShowEq{morphism of representations of algebra, q1=}
\ShowEq{morphism of representations of algebra, q2=}
are isomorphisms.
\labelItem{q12 are isomorphisms}
\item
Maps
\ShowEq{morphism of representations of algebra, r1=}
\ShowEq{morphism of representations of algebra, r2=}
are monomorphisms.
\labelItem{r12 are monomorphisms}
\item $F$ is representation of $\Omega_1$\Hyph algebra $A_1/s$ in $A_2/s_2$
\item $G$ is representation of $\Omega_1$\Hyph algebra $t_1A_1$ in $t_2A_2$
\item The map
\ShowEq{map r12}p{}
is the morphism of representations $f$ and $F$
\labelItem{(p12) is morphism of representations}
\item The map
\ShowEq{map r12}q{}
is the isomorphism of representations $F$ and $G$
\labelItem{(q12) is isomorphism of representations}
\item The map
\ShowEq{map r12}r{}
is the morphism of representations $G$ and $g$
\labelItem{(r12) is morphism of representations}
\item There exists decompositions of morphism of representations
\labelItem{exists decompositions of morphism of representations}
\ShowEq{decompositions of morphism of representations}
\end{enumerate}
}

\DefDefinition{stable set of representation}
{
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
The set
\ShowEq{B2 subset A2}
is called
\AddIndex{stable set of representation}
{stable set of representation} $f$,
if
\ShowEq{fam in B2}
for each
\ShowEq{a in A1},
$m\in B_2$.
}

\DefTheorem{subrepresentation of representation}
{
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be representation of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
Let set
\ShowEq{B2 subset A2}
be subalgebra of $\Omega_2$\Hyph algebra $A_2$
and stable set of representation $f$.
Then there exists representation
\ShowEq{representation of algebra A in algebra B}
such that
\ShowEq{fB2(a)=}
Representation $f_{B_2}$ is called
\AddIndex{subrepresentation}{subrepresentation}
of representation $f$.
}

\DefTheoremNote{lattice of subrepresentations}
{
The set\,\footnotemark
\ShowEq{lattice of subrepresentations}
of all subrepresentations of representation $f$ generates
a closure system on $\Omega_2$\Hyph algebra $A_2$
and therefore is a complete lattice.
}{
This definition is
similar to definition of the lattice of subalgebras
(\citeBib{Cohn: Universal Algebra}, p. 79, 80).
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn%
In general, in this and subsequent theorems of this chapter,
it is necessary to consider the structure of universal algebras
$A_1$ and $A_2$.
Because the main task of this chapter is
is the study of the structure of the representation,
I deliberately simplified the theorems so
that the details do not obscure the basic statements.
This topic will be discussed in more details in the chapter
\RefChapter{Basis of Diagram of Representations of Universal Algebra},
where theorems will be formulated in general form.
\fi
}

\AddEq{remark: closure operator, representation}
{
We denote the corresponding closure operator by
\ShowEq{closure operator, representation}
Thus
\ShowEq{subrepresentation generated by set}
is the intersection of all subalgebras
of $\Omega_2$\Hyph algebra $A_2$
containing $X$ and stable with respect to representation $f$.
}

\DefDefinition{generating set of representation}
{
\ShowEq{show closure operator, representation}
is called
\AddIndex{subrepresentation}{subrepresentation}
generated by set $X$,
and $X$ is a
generating set
of subrepresentation $J[f,X]$.
In particular, a
\AddIndex{generating set}{generating set}
of representation $f$
is a subset $X\subset A_2$ such that
\ShowEq{generating set of representation}
}

\DefTheoremNote{map of words of representation}
{
\ShowEq{Let A->*AB2 be representations}
Let $X$ be the generating set of representation $f$.
Let
\ShowEq{f:A->B}R{A_2}{B_2}
be reduced morphism of representation\,\footnotemark
and $X'=R(X)$.
Reduced morphism $R$ of representation
generates the map of $\Omega_2$\Hyph words
\ShowEq{map of words of representation}
such that
\StartLabelItem
\begin{enumerate}
\item If
\ShowEq{map of words of representation, m in X, 1}
then
\ShowEq{map of words of representation, m in X}
\item If
\ShowEq{map of words of representation, omega, 1}
then for operation
$\omega\in\Omega_2(n)$ holds
\ShowEq{map of words of representation, omega}
\item If
\ShowEq{map of words of representation, am, 1}
then
\ShowEq{map of words of representation, am}
\end{enumerate}
}{
I considered morphism of representation in the theorem
\RefTheorem[\RefRepresentation]{map of words of diagram of representations}.
}

\DefTheorem{Representation is single transitive iff}
{
Representation is single transitive iff for any $a, b \in A_2$
exists one and only one $g\in A_1$ such that $a=f(g)(b)$.
}

\DefProof{Representation is single transitive iff}
{
The theorem follows from definitions \RefDefinition{free representation of algebra}
and \RefDefinition{transitive representation of algebra}.
}

\DefTheorem{single transitive representation generates algebra}
{
Let
\ShowEq{f:A->*B}f{A_1}{A_2}
be a single transitive representation
of $\Omega_1$\Hyph algebra $A_1$
in $\Omega_2$\Hyph algebra $A_2$.
There is the structure of $\Omega_1$\Hyph algebra on the set $A_2$.
}

\AddEq{theorem: automorphism uniquely defined by image of basis}
{
\begin{ShadedTheorem}
\labelTheorem{automorphism uniquely defined by image of basis}
Let $\Basis e$ be the basis of the representation $f$.
Let
\ShowEq{R1 X->}{\Basis e}
be arbitrary map of the set $\Basis e$.
Consider the map of $\Omega_2$\Hyph words
\ShowEq{map of words of representation, W}{\Basis e}
that satisfies conditions
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega},
\RefItem{map of words of representation, am}
and such that
\ShowEq{map of words of representation, W in X}e{\Basis e}
There exists unique endomorphism of representation $f$\,\footnotemark
\ShowEq{R:A2->A2}
defined by rule
\ShowEq{endomorphism based on map of words of representation}{\Basis e}
\end{ShadedTheorem}
\footnotetext{\,
This statement is
similar to the theorem \citeBib{Serge Lang}-4.1, p. 135.
}
}

\DefDefinition{parity of permutation}
{
The map
\ShowEq{sigma->+-}
defined by the equality
\def\permutation{permutation }
\def\even{even}
\def\odd{odd}
\ShowEq{parity of permutation}
is called
\AddIndex{parity of permutation}{parity of permutation}.
}

\DefText{passive representation of vector space 1}
{
\ShowText{coordinates of vector with respect to basis (1,2) \Cols}v3
Then
\ShowEq{v=vi ei 123, \SideNS-\Cols}
Let passive transformation $g_1$ map the basis
\ShowEq{Basis e in BVG}1
into the basis
\ShowEq{Basis e in BVG}2
\DrawEq[12g1]{e2i=aij e1j \Product-\Cols}{12}
Let passive transformation $g_2$ map the basis
\ShowEq{Basis e in BVG}2
into the basis
\ShowEq{Basis e in BVG}3
\DrawEq[23g2]{e2i=aij e1j \Product-\Cols}{23}
}

\DefText{passive representation of vector space 2}
{
The transformation
\ShowEq{e3=g12 cr e1 \SideNS-\Cols}
is the product of transformations
\eqRef{e2i=aij e1j \Product-\Cols}{12},
\eqRef{e2i=aij e1j \Product-\Cols}{23}.
The coordinate transformation
\DrawEq[v2v1g1{\SideNS}{\Cols}]{v2=v1g-}{1 \SideNS-\Cols}
corresponds to passive transformation $g_1$
and follows from equalities
\EqRef{v=vi ei 123, \SideNS-\Cols},
\eqRef{e2i=aij e1j \Product-\Cols}{12}
and the theorem
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\DefText{passive representation of vector space 3}
{
Similarly,
\ePrints{1908.04418,6860-2955}%
\ifx\Semafor\ValueOff%
according to the theorem
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
\fi
the coordinate transformation
\DrawEq[v3v2g2{\SideNS}{\Cols}]{v2=v1g-}{23 \SideNS-\Cols}
corresponds to passive transformation $g_2$
and follows from equalities
\EqRef{v=vi ei 123, \SideNS-\Cols},
\eqRef{e2i=aij e1j \Product-\Cols}{23}.
The product of coordinate transformations
\eqRef{v2=v1g-}{1 left-cols},
\eqRef{v2=v1g-}{23 left-cols}
has form
\ShowEq{v3=v1 cr g1- cr g2- \SideNS-\Cols}
and is coordinate transformation
corresponding to passive transformation
\EqRef{e3=g12 cr e1 \SideNS-\Cols}.
The equality
\ShowEq{v3=v1 cr g21- \SideNS-\Cols}
follows from equalities
\EqRef{cr-inverse matrix of product},
\EqRef{v3=v1 cr g1- cr g2- \SideNS-\Cols}.
}

\DefText{passive representation of left vector space}
{
\ShowText{passive representation of vector space 1}
\ShowText{passive representation of vector space 2}
\ShowText{passive representation of vector space 3}
}

\DefDefinition{Left side contravariant representation}
{
Left\Hyph side representation
\ShowEq{f:A->*B}f{A_1}{A_2}
is called
\AddIndex{contravariant}{contravariant representation}
if the equality
\ShowEq{Left side contravariant representation}
is true.
}

\DefDefinition{Left side covariant representation}
{
Left\Hyph side representation
\ShowEq{f:A->*B}f{A_1}{A_2}
is called
\AddIndex{covariant}{covariant representation}
if the equality
\ShowEq{Left side covariant representation}
is true.
}

\DefDefinition{cr-inverse matrix}
{
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph number
\else
The matrix
\fi
\ShowEq{cr-inverse element}
is \AddIndex{\CR inverse element}{cr-inverse element}
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
of $\mathcal{A}$\Hyph number
\else
of the matrix
\fi
$a$ if
\DrawEq{cr-inverse matrix}1
\ePrints{2020.06.01}
\ifx\Semafor\ValueOn
Matrix $a$ is called
\CR regular,
if there exists \CR inverse matrix.
\fi
}

\DefDefinition{delta=Matrix}
{
Matrix
\ShowEq{delta=Matrix}
is identity for both products.
}

\DefRemark{pronunciation of product}
{
We will use symbol \RC\,\, or \CR\,\, in name of properties of each product
and in the notation.
We can read the symbol
$\RCstar$ as
$rc$\hyph product (product of row over column)
and the symbol $\CRstar$ as
$cr$\hyph product (product of column over row).
In order to keep this
notation consistent with the existing one we assume that
we have in mind \RC product when
no clear notation is present.
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
This rule we extend to following terminology.
To draw symbol of product,
we put two symbols of product in the place
of index which participate in sum.
For instance, if product of $A$\Hyph numbers has form
$a\circ b$,
then \RC product
of matrices $a$ and $b$ has form
$a\RCcirc b$
and \CR product
of matrices $a$ and $b$ has form
$a\CRcirc b$.
\fi
}

\DefTheorem{quasideterminant rc cr, matrix 2x2}
{
\ShowEq{quasideterminant matrix 2x2 def}
Consider matrix
\ShowEq{inverse matrix 2x2, 0}
Then
\ShowEq{quasideterminant rc, matrix 2x2}
\ShowEq{quasideterminant cr, matrix 2x2}
\ShowEq{rc inverse matrix 2x2}
}

\DefDefinition{RC-quasideterminant}
{
\AddIndex{$(\aUD{}ji)$\hyph \RC quasideterminant}{j i RC-quasideterminant}
of \nTimes matrix $a$
is formal expression
\ShowEq{j i RC-quasideterminant definition}
\ShowEq{j i RC-quasideterminant =}
We consider $\aUD (ji)$\hyph \RC quasideterminant
as an entry of the matrix
\ShowEq{RC-quasideterminant definition}
\ShowEq{RC-quasideterminant definition=}
which is called
\AddIndex{\RC quasideterminant}{RC-quasideterminant}.
}

\DefDefinition{biring}
{
The set $\mathcal A$ is a \AddIndex{biring}{biring}
if we defined on $\mathcal A$ an unary operation, say transpose,
and three binary operations,
say \RC product, \CR product and sum, such that
\begin{itemize}
\item \RC product and sum define structure of ring on $\mathcal A$
\item \CR product and sum define structure of ring on $\mathcal A$
\item both products have common identity $\delta$
\item products satisfy equation
\DrawEq{rc transpose}{}
\item transpose of identity is identity
\DrawEq{transpose of identity}E
\item double transpose is original element
\ShowEq{double transpose}
\end{itemize}
}

\DefTheorem{double transpose is original matrix}
{
Double transpose is original matrix
\ShowEq{double transpose}
}

\DefProof{double transpose is original matrix}
{
The theorem follows from the definition
\RefDefinition{transpose of matrix}.
}

\DefEq
{
\begin{ShadedTheorem}[duality principle for biring]
\AddIndex{}{duality principle for biring}
\labelTheorem{duality principle for biring}
Let $\mathcal{A}$ be true statement about
biring $A$.
If we exchange the same time
\begin{itemize}
\item $a\in A$ and $a^T$
\item \RC product and \CR product
\end{itemize}
then we soon get true statement.
\end{ShadedTheorem}
}
{theorem: duality principle for biring}
%\DefEq

\DefEq
{
\begin{ShadedTheorem}[duality principle for biring of matrices]
\AddIndex{}{duality principle for biring of matrices}
\labelTheorem{duality principle for biring of matrices}
Let $A$ be biring of matrices.
Let $\mathcal{A}$ be true statement about matrices.
If we exchange the same time
\begin{itemize}
\item rows and columns of all matrices
\item \RC product and \CR product
\end{itemize}
then we soon get true statement.
\end{ShadedTheorem}
\begin{proof}
This is the immediate consequence
of the theorem \RefTheorem{duality principle for biring}.
\end{proof}
}
{theorem: duality principle for biring of matrices}
%\DefEq

\DefEq
{
\begin{remark}
\labelRemark{reducible biring}
If product in $\Omega$\Hyph $A$ ring is commutative, then
\ShowEq{reducibility of products}
\AddIndex{Reducible biring}{reducible biring} is
the biring which holds
\AddIndex{condition of reducibility of products}
{condition of reducibility of products}
\EqRef{reducibility of products}.
So, in reducible biring, it is enough to consider only
\RC product. However in case when
the order of factors is essential
we will use \CR product also.
\qed
\end{remark}
}
{remark: reducible biring}
%\DefEq

\DefEq
{
Since left\Hyph side representation and right\Hyph side representation
are based on homomorphism of $\Omega$\Hyph group,
then the following statement is true.

\begin{ShadedTheorem}[duality principle for representation of multiplicative $\Omega$\Hyph group]
\labelTheorem{duality principle, algebra representation}
Any statement which holds for
left\Hyph side representation of multiplicative $\Omega$\Hyph group $A_1$
holds also for right\Hyph side representation of multiplicative $\Omega$\Hyph group $A_1$, if
we will use right\Hyph side product over $A_1$\Hyph number $a_1$ instead of
left\Hyph side product over $A_1$\Hyph number $a_1$.
\qed
\end{ShadedTheorem}
}
{theorem: duality principle, algebra representation}
%\DefEq

\DefTheorem{left right shift}
{
The product
\ShowEq{(ab)->ab}
in multiplicative $\Omega$\Hyph group $A$
determines two different representations.
\begin{itemize}
\EqParm{associative shift}{def left}
\EqParm{associative shift}{def right}
\end{itemize}
}

\AddEq{non associative shift}
{
\item
The \SideWS shift
\ShowEq{\SideWS shift}
is representation
of $\Omega$\Hyph algebra $A$
in $\Omega$\Hyph algebra $A$.
}

\AddEq{associative shift}
{
\item
the \AddIndex{\SideWS shift}{\SideWS shift}
\ShowEq{\SideWS shift =}
\ShowEq{\SideWS shift}
is \SideNS\Hyph side representation
of multiplicative $\Omega$\Hyph group $A$
in $\Omega$\Hyph algebra $A$
\ShowEq{\SideWS shift, product}
}

\DefDefinition{representation of algebra}
{
Let the set $A_2$ be $\Omega_2$\Hyph algebra.
Let
the set of transformations
\ShowEq{End O2}{A_2}{}
be  $\Omega_1$\Hyph algebra.
The homomorphism
\ShowEq{representation of algebra}
of $\Omega_1$\Hyph algebra $A_1$ into
$\Omega_1$\Hyph algebra
\ShowEq{End O2}{A_2}{}
is called
\AddIndex{representation of $\Omega_1$\Hyph algebra}
{representation of algebra}
$A_1$ or
\AddIndex{$A_1$\Hyph representation}{A representation of algebra}
in $\Omega_2$\Hyph algebra $A_2$.
}

\DefEq
{
If multiplicative $\Omega$\Hyph group $A_1$ is Abelian,
then there is no difference between left\Hyph side and right\Hyph side representations.

\begin{ShadedDefinition}
\labelDefinition{representation of Abelian group}
Let $A_1$ be Abelian multiplicative $\Omega$\Hyph group.
We call a homomorphism of multiplicative $\Omega$\Hyph group
\DrawEq{representation of group, map}{Abelian group}
\AddIndex{representation}{representation of algebra}
of multiplicative $\Omega$\Hyph group $A_1$
or
\AddIndex{$A_1$\Hyph representation}{A representation of algebra}
in $\Omega_2$\Hyph algebra $A_2$ if the map $f$ holds
\DrawEq{left-side representation of group}{Abelian}
\end{ShadedDefinition}

Usually we identify a representation of the Abelian multiplicative $\Omega$\Hyph group $A_1$
and a left\Hyph side representation of the multiplicative $\Omega$\Hyph group $A_1$.
However, if it is necessary for us,
we identify a representation of the Abelian multiplicative $\Omega$\Hyph group $A_1$
and a right\Hyph side representation of the multiplicative $\Omega$\Hyph group $A_1$.
}
{definition: representation of Abelian group}
%\DefEq

\DefTheorem{two representations of group}
{
Let $A_1$ be multiplicative $\Omega$\Hyph group.
Let left\Hyph side $A_1$\Hyph representation $f$
on $\Omega_2$\Hyph algebra $A_2$ be single transitive.
Then we can uniquely define a single transitive right\Hyph side $A_1$\Hyph representation $h$
on $\Omega_2$\Hyph algebra $A_2$
such that diagram
\ShowEq{two representations of group}
is commutative for any $a_1$, $b_1\in A_1$.
}

\AddEq{definition: twin representations}
{
Representations $f$ and $h$ are called
\AddIndex{twin representations}{twin representations}
of the multiplicative $\Omega$\Hyph group $A_1$.
}

\DefRemark{one representation of group}
{
It is clear that transformations $L(a)$ and $R(a)$
are different until the multiplicative $\Omega$\Hyph group $A_1$ is nonabelian.
However they both are maps onto.
Theorem \RefTheorem{two representations of group} states that if both
right and left shift presentations exist on the set $A_2$,
then we can define two commuting representations on the set $A_2$.
The right shift or the left shift only cannot represent both types of representation.
To understand why it is so let us change diagram
\EqRef{Diagram: two representations of group}
and assume
\ShowEq{haa=Laa}
instead of
\ShowEq{haa=aRa}
and let us see what expression $h(a_1)$ has at
the point $c_2$. The diagram
\ShowEq{Diagram: two representations of group 1}
is equivalent to the diagram
\ShowEq{Diagram: two representations of group 2}
and we have
\ShowEq{d2=...c2 1}
Therefore
\ShowEq{d2=...c2}
We see that the representation of $h$
depends on its argument.
}

\DefTheorem{single transitive representation of group}
{
If there exists single transitive representation
\ShowEq{f:A->*B}f{A_1}{A_2}
of multiplicative $\Omega$\Hyph group $A_1$
in $\Omega_2$\Hyph algebra $A_2$,
then we can uniquely define coordinates on $A_2$ using $A_1$\Hyph numbers.

If $f$ is left\Hyph side single transitive representation
then $f(a)$ is equivalent to the left shift $L(a)$ on the group $A_1$.
If $f$ is right\Hyph side single transitive representation
then $f(a)$ is equivalent to the right shift $R(a)$ on the group $A_1$.
}

\DefDefinition{algebra of sets}
{
A nonempty system of sets $\mathcal R$ is called
\AddIndex{ring of sets}{ring of sets},\,\footnote{
See also the definition
\citeBib{Kolmogorov Fomin}\Hyph 1,  page 31.}
if condition
\ShowEq{A, B in R}
imply
\ShowEq{A, B in R 1}
A set
\ShowEq{E in R}
is called
\AddIndex{unit of ring of sets}{unit of ring of sets}
if
\ShowEq{A cap E=A}
A ring of sets with unit is called
\AddIndex{algebra of sets}{algebra of sets}.
}

\DefEq
{
\begin{remark}
\labelRemark{A cup/minus B}
For any
\ShowEq{A cup/minus B}
Therefore, if
\ShowEq{A, B in R},
then
\ShowEq{A cup/minus B R}
\qed
\end{remark}
}
{remark: A cup/minus B}
%\DefEq

\DefDefinition{sigma algebra of sets}
{
The ring of sets $\mathcal R$ is called
\AddIndex{\(\sigma\)\Hyph ring of sets}{sigma ring of sets},\,\footnote{
See similar definition in
\citeBib{Kolmogorov Fomin}, page 35, definition 3.}
if condition
\ShowEq{Ai in R}
imply
\ShowEq{Ai in R 1}
\(\sigma\)\Hyph Ring of sets with unit is called
\AddIndex{\(\sigma\)\Hyph algebra of sets}{sigma algebra of sets}.
}

\DefDefinition{Borel algebra}
{
Minimal \(\sigma\)\Hyph algebra
\ShowEq{Borel algebra}
generated by the set of all open balls of normed $\Omega$\Hyph group $A$
is called
\AddIndex{Borel algebra}{Borel algebra}.\,\footnote{
See remark in
\citeBib{Kolmogorov Fomin}, p. 36.
According to the remark
\ref{remark: A cup/minus B},
the set of closed balls also generates
Borel algebra.
}
A set
belonging to Borel algebra
is called
\AddIndex{Borel set}{Borel set}
or
\AddIndex{$B$\Hyph set}{B set}.
}

\DefDefinition{C_X C_Y measurable}
{
Let $\mathcal C_X$ be
\(\sigma\)\Hyph algebra of sets of set $X$.
Let $\mathcal C_Y$ be
\(\sigma\)\Hyph algebra of sets of set $Y$.
The map
\ShowEq{f:A->B}fXY
is called
$(\mathcal C_X,\mathcal C_Y)$\Hyph measurable\,\footnote{
See similar definition in
\citeBib{Kolmogorov Fomin}, page 284.}
if for any set
\ShowEq{CX CY measurable map}
}

\DefEq
{
\begin{example}
\labelExample{measurable map}
Let $\mu$ be a \(\sigma\)\Hyph additive measure defined on the set $X$.
Let
\ShowEq{algebra of sets measurable with respect to measure}
be \(\sigma\)\Hyph algebra of sets measurable with respect to measure $\mu$.
Let
$\mathcal B(A)$
be Borel algebra of
normed $\Omega$\Hyph group $A$.
The map
\ShowEq{f:A->B}fXA
is called
\AddIndex{$\mu$\Hyph measurable}{mu measurable map}\,\footnote{
See similar definition in
\citeBib{Kolmogorov Fomin},  pp. 284, 285, definition 1.
If the measure $\mu$ is defined on the set $X$ by context,
then we also call the map
\ShowEq{f:A->B}fXA
\AddIndex{measurable}{measurable map}.
}
if for any set
\ShowEq{measurable map}
\qed
\end{example}
}
{example: measurable map}
%\DefEq

\DefDefinition{simple map}
{
Let $\mu$ be a \(\sigma\)\Hyph additive measure defined on the set $X$.
The map
\ShowEq{f:A->B}fXA
into normed $\Omega$\Hyph group $A$ is called
\AddIndex{simple map}{simple map},
if this map is $\mu$\Hyph measurable and
its range is finite or countable set.
}

\DefTheorem{measurable simple map}
{
Let range
\ShowEq{range f}
of the map
\ShowEq{f:A->B}fXA
be finite or countable set.
The map $f$ is $\mu$\Hyph measurable iff
all sets
\DrawEq{Fn=}{}
are $\mu$\Hyph measurable.\,\footnote{
See similar theorem in
\citeBib{Kolmogorov Fomin},  page 286, theorem 4.}
}

\DefDefinition{measure}
{
Let \(\mathcal C_m\) be semiring of sets.\,\footnote{
See also the definition
\citeBib{Kolmogorov Fomin}\Hyph 1 on page 270.}
The map
\ShowEq{f:A->B}f{\mathcal C_m}R
is called
\AddIndex{measure}{measure},
if
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{m(A)>0}
\item
The map \(m\) is additive map.
If a set
\ShowEq{A in Cm}
has finite expansion
\DrawEq{A=+Ai Cm}{}
where
\ShowEq{Ai*Aj=0},
then
\ShowEq{m A=+m Ai}
\end{enumerate}
}

\DefDefinition{complete measure}
{
A measure \(\mu\) is called
\AddIndex{complete measure}{complete measure},
if conditions
\ShowEq{B in A, mu(A)=0}
imply
that \(B\) is measurable set.
}

\DefDefinition{sigma-additive measure}
{
Let $\mathcal C_{\mu}$ be
\(\sigma\)\Hyph algebra of sets of set $F$.\,\footnote{
See similar definitions in
\citeBib{Kolmogorov Fomin}, definition 1 on page 270
and definition 2 on page 272.}
The map
%\ShowEq{mu:CF->A}
%into normed $\Omega$\Hyph group $A$ is called
\ShowEq{f:A->B}{\mu}{\mathcal C_{\mu}}R
into real field $R$ is called
\AddIndex{\(\sigma\)\Hyph additive measure}{sigma-additive measure},
if, for any set
\ShowEq{X in Cmu},
following conditions are true.
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{muX>0}
\item
Let
\DrawEq{X=+Xi}{}
be finite or countable union of sets
\ShowEq{Xn in Cmu}
Then
\DrawEqParm{mu(X=+Xi)}X{}
where series on the right converges absolutely.
\labelItem{mu(X=+Xi)}
\end{enumerate}
}

\DefEq
{
Let $\mu$ be a \(\sigma\)\Hyph additive measure defined on the set $X$.
Let effective representation of real field \(R\)
in complete Abelian \(\Omega\)\Hyph group \(A\) be defined.\,\footnote{In
other words,
\(\Omega\)\Hyph group \(A\) is
\(R\)\Hyph vector space.}
}
{remark - measure - effective representation of real field}
%\DefEq

\DefDefinition{series converges normally}
{
Let \(a_i\) be a sequence of \(A\)\Hyph numbers.
If
\ShowEq{sum |ai|<infty}
then we say that the {\bf series}
\ShowEq{sum ai}
\AddIndex{converges normally}
{series converges normally}.\,\footnote{See also
the definition of normal convergence of the series
on page \citeBib{Cartan differential form}-12.}
}

\DefDefinition{Integral of Map over Set of Finite Measure}
{
\(\mu\)\Hyph measurable map
\ShowEq{f:A->B}fXA
is called
\AddIndex{integrable map}{integrable map}
over the set \(X\),\,\footnote{
See also the definition in
\citeBib{Kolmogorov Fomin}, page 296.
}
if there exists a sequence
of simple integrable over the set \(X\) maps
\ShowEq{f:A->B}{f_n}XA
converging uniformly to \(f\).
Since the map \(f\) is integrable map,
then the limit
\ShowEq{integral of map}
\ShowEq{integral of measurable map}
is called
\AddIndex{Lebesgue integral}{Lebesgue integral}
of map \(f\) over the set \(X\).
}

\DefDefinition{integrable map}
{
For simple map
\ShowEq{f:A->B}fXA
consider series
\DrawEq{sum mu(F) f}{integral}
where
\begin{itemize}
\item
The set
\ShowEq{f1...}
is domain of the map \(f\)
\item
Since \(n\ne m\), then
\ShowEq{fn ne fm}
\item
\DrawEq{Fn=}{-}
\end{itemize}
Simple map
\ShowEq{f:A->B}fXA
is called
\AddIndex{integrable map}{integrable map}
over the set \(X\)
if series
\eqRef{sum mu(F) f}{integral}
converges normally.\,\footnote{
See similar definition in
\citeBib{Kolmogorov Fomin}, p. 294.}
Since the map \(f\) is integrable map,
then sum of series
\eqRef{sum mu(F) f}{integral}
is called
\AddIndex{Lebesgue integral}{Lebesgue integral}
of map \(f\) over the set \(X\)
\ShowEq{integral of map}
\ShowEq{integral of simple map}
}

\DefTheorem{|int f|<int|f|}
{
Let
\ShowEq{f:A->B}fXA
be measurable map.
Integral
\ShowEq{int f X}
exists
iff
integral
\ShowEq{int |f| X}
exists.
Then
\DrawEq{|int f|<int|f|}{measurable}
}

\DefTheorem{int |f|<M mu}
{
Let
\ShowEq{f:A->B}fXA
be $\mu$\Hyph measurable map such that
\DrawEq{|f(x)|<M}{}
Since the measure of the set \(X\) is finite, then
\DrawEq{int |f|<M mu}{measurable}
}

\DefTheorem{int f+g X}
{
Let
\ShowEq{f:A->B}fXA
\ShowEq{f:A->B}gXA
be $\mu$\Hyph measurable maps
with compact range.
Since there exist integrals
\ShowEq{int f X}
\ShowEq{int g X}
then there exists integral
\ShowEq{int f+g X}
and
\DrawEq{int f+g X =}{measurable}
}


==> Stmt.Representation.Eq.tex <==
%auto-ignore

\def\Act{\bullet}
\newcommand\wXm[1][m]{w[f,X,#1]}
\newcommand\wXR{w[f\rightarrow g,X,R]}%w[f\rightarrow g,X,Y,R]
\def\UnitNMatrix{\aD En}

\AddEq[1]{i=1,2}
{
$i=1$, $2$#1
}

\AddEquation{morphism of representations of algebra, homomorphism, 1}
{
t_i=r_i\circ q_i\circ p_i
}

\AddEq{morphism of representations of algebra, p1=}
{
\[
\RedText{p_1(a)}=a^{\mathrm{ker}\,t_1}
\]
}

\AddEq{morphism of representations of algebra, p2=}
{
\[
\BlueText{p_2(a)}=a^{\mathrm{ker}\,t_2}
\]
}

\AddEquation{morphism of representations of algebra, q1=}
{
q_1(\RedText{p_1(a)})=\RedText{t_1(a)}
}

\AddEquation{morphism of representations of algebra, q2=}
{
q_2(\BlueText{p_2(a)})=\BlueText{t_2(a)}
}

\AddEq{morphism of representations of algebra, r1=}
{
\[
r_1:\RedText{t_1(a)}\in f(A_1)\rightarrow \RedText{t_1(a)}\in B_1
\]
}

\AddEq{morphism of representations of algebra, r2=}
{
\[
r_2:\BlueText{t_2(a)}\in f(A_2)\rightarrow \BlueText{t_2(a)}\in B_2
\]
}

\AddEq [2]{map r12}
{
$#1=(#1_1,#1_2)$#2
}

\AddEquation{decompositions of morphism of representations}
{
(t_1,t_2)
=
(r_1,r_2)
\circ
(q_1,q_2)
\circ
(p_1,p_2)
}

\AddEq{r1(a)=r1(a)}
{
\[
\RedText{r_1(a)}=r_1(a)
\]
}

\AddEq{g(r1(a))}
{
$g(\RedText{r_1(a)})$
}

\AddEq{r2(m)in B2}
{
$\BlueText{r_2(m)}\in B_2$
}

\AddEq{r2(f(a,m))}
{
$\BlueText{r_2(f(a)(m))}$.
}

\AddEquation{morphism of representations of universal algebra, definition, 2m 2}
{
\xymatrix{
A_2\ar[rr]^{r_2}&&B_2\\
A_1\ar[rr]^{r_1}\ar[u]^f|{*}&&B_1\ar[u]^g|{*}
}
}

\AddEq{n=r2(m)}
{
$n=r_2(m)\in B_2$
}

\AddEq{morphism of representations of universal algebra, 2m}
{
\BlueText{r_2(f(a)(m))}=g(\RedText{r_1(a)})(\BlueText{r_2(m)})
}

\AddEq{morphism of representations of universal algebra, 2m 1}
{
\xymatrix{
&A_2\ar[dd]_(.3){f(a)}\ar[rr]^{r_2}&&B_2\ar[dd]^(.3){g(\RedText{r_1(a)})}\\
&\ar @{}[rr]|{(1)}&&\\
&A_2\ar[rr]^{r_2}&&B_2\\
A_1\ar[rr]^{r_1}\ar@{=>}[uur]^(.3)f&&B_1\ar@{=>}[uur]^(.3)g
}
}

\AddEq[1]{a in A1}
{
$a\in A_1$#1
}

\AddEq{fam in B2}
{
$f(a)(m)\in B_2$
}

\AddEq{B2 subset A2}
{
$B_2\subset A_2$
}

\AddEq{fB2(a)=}
{
$f_{B_2}(a)=f(a)|_{B_2}$.
}

\AddEq{lattice of subrepresentations}
{
\symb{\mathcal B_f}{lattice of subrepresentations}1
}

\AddEq{representation of algebra A in algebra B}
{
\[
\xymatrix
{
f_{B_2}:A_1\ar[r]|{*}&B_2
}
\]
}

\AddEq{rc transpose}
{
(a\RCstar b)^T=a^T\CRstar b^T
}

\AddEq{cr transpose}
{
(a\CRstar b)^T=(a^T)\RCstar (b^T)
}

\DefTheorem{rc transpose}
{
\DrawEq{rc transpose}{Theorem}
}

\DefTheorem{cr transpose}
{
\DrawEq{cr transpose}{Theorem}
}

\AddEquation{rc transpose, 1}
{
\aUD{((a\RCstar b)^T)}ji
=\aUD{(a\RCstar b)}ij
=\aUD aik\aUD bkj
=\aUD{(a^T)}ki\aUD{(b^T)}jk
=\aUD{((a^T)\CRstar (b^T))}ji
}

\AddEquation{L(b)a=}
{
L(b)\circ a=[b,a]
}

\AddEquation{L(c)L(b)a=}
{
L(c)\circ L(b)\circ a=L(c)\circ(L(b)\circ a)=[c,[b,a]]
}

\AddEq{Lie product on set of left shifts}
{
\[
[L(c),L(b)]\circ a=L(c)\circ L(b)\circ a-L(b)\circ L(c)\circ a
\]
}

\AddEquation{[L(c)L(b)]a= 2}
{
[L(c),L(b)]\circ a=L([c,b])\circ a
}

\AddEquation{[L(c)L(b)]a= 1}
{
L(c)\circ L(b)\circ a-L(b)\circ L(c)\circ a=L([c,b])\circ a
}

\AddEquation{Lee identity 1}
{
[c,[b,a]]+[b,[a,c]]=-[a,[c,b]]=[[c,b],a]
}

\AddEquation{Lee identity}
{
[c,[b,a]]+[b,[a,c]]+[a,[c,b]]=0
}

\AddEquation{[L(c)L(b)]a=}
{
\begin{split}
L(c)\circ L(b)\circ a-L(b)\circ L(c)\circ a&=[c,[b,a]]-[b,[c,a]]
\\
&=[c,[b,a]]+[b,[a,c]]
\end{split}
}

\AddEq{direct sum of Abelian groups}
{
\symb{A\oplus B}{direct sum}1
}

\AddEquation{fik fjk = fjk fik}
{
f_{ik}(a_i)(f_{jk}(a_j)(a_k))
=
f_{jk}(a_j)(f_{ik}(a_i)(a_k))
}

\AddEquation{reduced polymorphism of representation, akl}
{
\begin{array}{r@{\,}l}
&r_2(m_1,...,\BlueText{f_k(a)(m_k)},...,m_l,...,m_n)
\\
=&r_2(m_1,...,m_k,...,\BlueText{f_l(a)(m_l)},...,m_n)
\end{array}
}

\ePrints{1502.04063,5114-6019}
\ifx\Semafor\ValueOff
\AddEquation{reduced polymorphism of representation, omega2}
{
\begin{array}{r@{\,}l}
&\,r_2(m_1,...,m_{k\cdot 1}...m_{k\cdot p}\omega_2,...,m_n)
\\
=&\,
r_2(m_1,...,m_{k\cdot 1},...,m_n)
...
r_2(m_1,...,m_{k\cdot p},...,m_n)
\omega_2
\end{array}
}
\fi

\AddEq{kl,1n}
{
$k$, $l$, $k=1$, ..., $n$, $l=1$, ..., $n$,
}

\AddEq{reduced morphism representation =}
{
r_2(f(a)(m))=g(a)(r_2(m))
}

\AddEquation{morphism of representations of universal algebra, definition, 2m-1}
{
\BlueText{r_2(f(a')(r_2^{-1}(m')))}
=f(\RedText{a'})(\BlueText{m'})
}

\AddEq{A in xAi}
{
\[A\subseteq\prod_{\iI}A_i\]
}

\AddEq[1]{A=o+Ai}
{
\[
#1=\bigoplus_{\iI}#1_i
\]
}

\AddEq[1]{m1 m2 modS}
{
$m_1\equiv m_2(\mathrm{mod} S)$#1
}

\AddEq[1]{fm1 fm2 modS}
{
$f(m_1)\equiv f(m_2)(\mathrm{mod}\ S)$#1
}

\AddEq[2]{End A2/S}
{
$\End(\Omega_2;A_2/#1)$#2
}

\AddEq[1]{f in End A2}
{
$f\in\End(\Omega_2;A_2)$#1
}

\AddEq[2]{End O2}
{
$\End(\Omega_2,#1)$#2
}

\AddEq [3]{r12:A->B}
{
\[
(#1_1:#2_1\rightarrow #3_1,\ #1_2:#2_2\rightarrow #3_2)
\]
}

\AddEq{decompositions of morphism of representations, diagram}
{
\[
\xymatrix{
&&A_2/s_2\ar[rrrrr]^{q_2}\ar@{}[drrrrr]|{(5)}&&\ar@{}[dddddll]|{(4)}&
\ar@{}[dddddrr]|{(6)}&&t_2A_2\ar[ddddd]^{r_2}\\
&&&&&&&\\
A_1/s_1\ar[r]^{q_1}\ar@/^2pc/@{=>}[urrr]^F&
t_1A_1\ar[d]^{r_1}\ar@{=>}[urrrrr]^(.4)G&&&
A_2/s_2\ar[r]^{q_2}\ar[lluu]_{F(\RedText{p_1(a)})}&
t_2A_2\ar[d]^{r_2}\ar[rruu]_{G(\RedText{t_1(a)})}\\
A_1\ar[r]_{t_1}\ar[u]^{p_1}\ar@{}[ur]|{(1)}\ar@/_2pc/@{=>}[drrr]^f&
B_1\ar@{=>}[drrrrr]^(.4)g&&&
A_2\ar[r]_{t_2}\ar[u]^{p_2}\ar@{}[ur]|{(2)}\ar[ddll]^{f(a)}&
B_2\ar[ddrr]^{g(\RedText{t_1(a)})}\\
&&&&&&&\\
&&A_2\ar[uuuuu]^{p_2}\ar[rrrrr]_{t_2}\ar@{}[urrrrr]|{(3)}&&&&&B_2
}
\]
}

\AddEq{kernel of homomorphism i}
{
$\mathrm{ker}\,t_i
=t_i\circ t_i^{-1}$
}

\AddEq{fxi,i=sum fxi}
{
f\left(\bigoplus_{\iI}x_i\right)=\sum_{\iI}f_i(x_i)
}

\AddEq{fi(x+y)=}
{
\[
f_i(x_i+y_i)=f_i(x_i)+f_i(y_i)
\]
}

\AddEq{f(x+y)i=}
{
\begin{align*}
f(\bigoplus_{\iI}(x_i+y_i))&=
\sum_{\iI}f_i(x_i+y_i)=
\sum_{\iI}(f_i(x_i)+f_i(y_i))
\\&=\sum_{\iI}f_i(x_i)+\sum_{\iI}f_i(y_i)
\\&=f(\bigoplus_{\iI}x_i)+f(\bigoplus_{\iI}y_i)
\end{align*}
}

\AddEq{structure of subrepresentations}
{
\StartLabelItem
\begin{enumerate}
\item
$X_0=X$
\labelItem{X0=X}
\item
$x\in X_k=>x\in X_{k+1}$
\labelItem{Xk in Xk+1}
\item
$x_1\in X_k$, ..., $x_n\in X_k$, $\omega\in\Omega_2(n)
=>x_1...x_n\omega\in X_{k+1}$
\labelItem{x1n omega in Xk+1}
\item
$x\in X_k$, $a\in A=>f(a)(x)\in X_{k+1}$
\labelItem{ax in Xk+1}
\end{enumerate}
}

\AddEquation{structure of subrepresentations, 1}
{
\bigcup_{k=0}^{\infty}X_k=J[f,X]
}

\AddEquation{lj(x)=0x0}
{
\lambda_j(x)=(\delta^i_jx,\iI)
}

\AddEq{flj=fj}
{
\[
f\circ\lambda_j(x)=\sum_{\iI}f_i(\delta_j^ix)=f_j(x)
\]
}

\AddEq[1]{(xi)in A}
{
$(x_i,\iI)\in A$#1
}

\DefEq
{
$\|x\|$, $x\in C$,
}
{|x in C|}

\DefEquation
{
\|a-b\|\ge|\,\|a\|-\|b\|\,|
}
{|a-b|>|a|-|b|}

\DefEq
{
\[
\|f(x')-f(x)\|_2<\epsilon
\]
}
{|f(x)-f(x')|<epsilon}

\AddEq[1]{End A(O2) B}
{
$\End(A(\Omega_2);B)$#1
}

\AddEq{open ball}
{
\symb{B_o(a,\rho)}{open ball}{}
\[
\ShowSymbol{open ball}{}=
\{
b\in A:\|b-a\|<\rho
\}
\]
}

\AddEq{closed ball}
{
\symb{B_c(a,\rho)}{closed ball}{}
\[
\ShowSymbol{closed ball}{}=
\{
b\in A:\|b-a\|\le\rho
\}
\]
}

\DefEq
{
$f_n\in M(X,A)$, $n=1$, ...,
}
{fn M(X,A)}

\DefEquation
{
\|f_n(x)-f_m(x)\|<\epsilon
}
{|fn(x)-fm(x)|<e}

\DefEq
{
\|a_p-a_q\|<\epsilon
}
{|ap-aq|<epsilon}

\AddEq{[an] in A}
{
$\{a_n\}$, $a_n\in \Module$,
}

\AddEq{aq in B(ap)}
{
\[a_q\in B_o(a_p,\epsilon)\]
}

\AddEq{an in B(a)}
{
a_n\in B_o(a,\epsilon)
}

\AddEq{limit of sequence}
{
\symb{\lim_{n\rightarrow\infty}a_n}{limit of sequence}{}
\[
a=\ShowSymbol{limit of sequence}{}
\]
}

\AddEq{a=lim an}
{
a=\lim_{n\rightarrow\infty}a_n
}

\DefEq
{
\|a_n-a\|<\epsilon
}
{|an-a|<epsilon}

\DefEquation
{
\lim_{n\rightarrow\infty}a_n=\lim_{n\rightarrow\infty}b_n
}
{lim a=lim b}

\DefEq
{
\lim_{n\rightarrow\infty}(a_n-b_n)=0
}
{lim a-b=0}

\DefEq
{
$g_n\in M(X,A)$, $n=1$, ...,
}
{gn M(X,A)}

\DefEq
{
\[h_n=f_n+g_n\]
}
{hn=fn+gn}

\DefEq
{
h=f+g
}
{h=f+g}

\DefEq
{
$c_1$, $c_2\in A$,
}
{c1 c2 in A}

\DefEq
{
$c_1\in B_c(a_1,R_1)$, $c_2\in B_c(a_2,R_2)$.
}
{c1 c2 in B}

\DefEq
{
$g_{1\cdot n}\in M(X,A_1)$, $n=1$, ...,
}
{g1n M(X,A1)}

\DefEq
{
$g_{2\cdot n}\in M(X,A_2)$, $n=1$, ...,
}
{g2n M(X,A2)}

\DefEq
{
$f_X(g_1)(g_2)$
}
{fX(g1)(g2)}

\DefEq
{
$M(X,A_1)$
}
{M(X,A1)}

\DefEq
{
$M(X,A_2)$
}
{M(X,A2)}

\DefEq
{
$g_1\in M(X,A_1)$
}
{g1 in M(X,A1)}

\DefEq
{
$g_2\in M(X,A_2)$
}
{g2 in M(X,A2)}

\DefEquation
{
\begin{split}
f_X(g_1)(g_2)&:X->A_2
\\
(f_X(g_1)(g_2))(x)&=f(g_1(x))(g_2(x))
\end{split}
}
{f(x)g(x):X->A2}

\DefEq
{
\symb{\|\omega\|}{norm of operation}{}
}
{norm of operation}

\DefEquation
{
\ShowSymbol{norm of operation}{}=
\text{sup}\frac{\| a_1...a_n\omega\|}{\|a_1\|...\|a_n\|}
}
{norm of operation, definition}

\DefEquation
{
\|a_1...a_n\omega\|\le\|\omega\|\|a_1\|...\|a_n\|
}
{|a omega|<|omega||a|1n}

\DefEq
{
\symb{\|f\|}{norm of representation}{}
}
{norm of representation}

\DefEquation
{
\ShowSymbol{norm of representation}{}=
\text{sup}\frac{\|f(a_1)(a_2)\|_2}{\|a_1\|_1\|a_2\|_2}
}
{norm of representation, definition}

\DefEquation
{
\|f(a_1)(a_2)\|_2\le\|f\|\|a_1\|_1\|a_2\|_2
}
{|fab|<|f||a||b|}

\DefEquation
{
c_1+c_2\in B_c(a_1+a_2,R_1+R_2)
}
{c1+c2 in B}

\DefEq
{
$f\in M(X,A)$
}
{f M(X,A)}

\DefEq
{
f(x)=\lim_{n\rightarrow\infty}f_n(x)
}
{f(x)=lim}

\DefEq
{
\[\|f_n(x)-f(x)\|<\epsilon\]
}
{fn(x) - f(x)}

\AddEq[1]{a in U}
{
$a \in U$#1
}

\AddEq{sum mu(F) f}
{
\displaystyle\sum_n\mu(F_n)f_n
}

\AddEq{f1...}
{
\(\{f_1,f_2,...\}\)
}

\AddEq{fn ne fm}
{
\(f_n\ne f_m\)
}

\AddEq{Fn=}
{
F_n=\{x\in X:f(x)=f_n\}
}

\AddEq{mu(X=+Xi)}
{
\mu(\PX)=\sum_i\mu(\PX_i)
}

\AddEq{m A=+m Ai}
{
\[
m(A)=\sum_{i=1}^nm(A_i)
\]
\labelItem{m A=+m Ai}
}

\DefEq
{
\(A\), \(B\in\mathcal R\)
}
{A, B in R}

\DefEq
{
$A\cup B\in\mathcal R$, $A\setminus B\in\mathcal R$.
}
{A cup/minus B R}

\DefEq
{
\symb{\mathcal B(A)}{Borel algebra}1
}
{Borel algebra}

\DefEq
{
$C\in\mathcal C_Y$
\[f^{-1}(C)\in\mathcal C_X\]
}
{CX CY measurable map}

\DefEq
{
$C\in\mathcal B(A)$
\[f^{-1}(C)\in\mathcal C_{\mu}\]
}
{measurable map}

\AddEq{range f}
{
\(y_1\), \(y_2\), ...
}

\DefEq
{
\(m(A)\ge 0\)
\labelItem{m(A)>0}
}
{m(A)>0}

\DefEq
{
\(A\in\mathcal C_m\)
}
{A in Cm}

\DefEq
{
A=\bigcup_{i=1}^nA_i\ \ \ A_i\in\mathcal C_m
}
{A=+Ai Cm}

\DefEq
{
\symb{\mathcal C_{\mu}}
{algebra of sets measurable with respect to measure}1
}
{algebra of sets measurable with respect to measure}

\DefEq
{
\(A\triangle B\), \(A\cap B\in\mathcal R\).
}
{A, B in R 1}

\DefEq
{
$E\in\mathcal R$
}
{E in R}

\DefEq
{
\[A\cap E=A\]
}
{A cap E=A}

\DefEq
{
$A_i\in\mathcal R$, $i=1$, ..., $n$, ...,
}
{Ai in R}

\DefEq
{
$A$, $B$
\begin{align*}
A\cup B&=(A\Delta B)\Delta (A\cap B)
\\
A\setminus B&=A\Delta (A\cap B)
\end{align*}
}
{A cup/minus B}

\DefEq
{
\[\bigcup_nA_n\in\mathcal R\]
}
{Ai in R 1}

\DefEq
{
$B_o(a,\epsilon)\subset U$.
}
{B(a) subset U}

\DefEq
{
$M(X,A)$\Pt
}
{M(X,A)}

\DefEq
{
\symb{M(X,A)}{set of maps to Omega group}1
}
{set of maps to Omega group}

\AddEq{transpose of identity}
{
\UnitNMatrix^T=\UnitNMatrix
}

\AddEquation{double transpose}
{
(a^T)^T=a
}

\DefEq
{
\[
\xymatrix
{
f_k:A\ar[r]|{*}&A_k
}
\]
}
{representation A Ak 1}

\DefEq
{
\[
\xymatrix{
r_1:\Times\ar[r]&S_1
&
r_2:\Times\ar[r]&S_2
}
\]
}
{polymorphisms category}

\DefEq
{
\[
\begin{matrix}
\xymatrix
{
g_1:A\ar[r]|{*}&S_1
}
&
\xymatrix
{
g_2:A\ar[r]|{*}&S_2
}
\end{matrix}
\]
}
{representation of algebra in S1 S2}

\DefEq
{
$r_1\rightarrow r_2$
}
{r1->r2}

\DefEq
{
\[
\xymatrix{
&S_1\ar[dd]^h
\\
\Times
\ar[ru]^{r_1}\ar[rd]_{r_2}
\\
&S_2
}
\]
}
{polymorphisms category, diagram}

\DefEq
{
\symb{\Tensor B}{tensor product}1
}
{tensor product of representations}

\DefEq
{
\[
\begin{matrix}
b_k\in B_k&k=1,...,n&
b_{i\cdot 1},...,b_{i\cdot p}\in B_i&\omega\in\Omega_2(p)&a\in A
\end{matrix}
\]
}
{equivalence, 1, representation, tensor product}

\DefEquation
{
\begin{split}
&b_1\otimes...\otimes(b_{i\cdot 1}...b_{i\cdot p}\omega)\otimes...\otimes b_n
\\
=&(b_1\otimes...\otimes b_{i\cdot 1}\otimes...\otimes b_n)...
(b_1\otimes...\otimes b_{i\cdot p}\otimes...\otimes b_n)
\omega
\end{split}
}
{tensors 1, representation, tensor product}

\DefEquation
{
b_1\otimes...\otimes(f_i(a)\circ b_i)\otimes...\otimes b_n=
f(a)\circ(b_1\otimes...\otimes b_i\otimes...\otimes b_n)
}
{tensors 2, representation, tensor product}

\DefEq
{
\[
f:\Times\rightarrow\Tensor B
\]
}
{map f, 1, representation, tensor product}

\DefEquation
{
f\circ(b_1,...,b_n)=\Tensor b
}
{map f, representation, tensor product}

\DefEq
{
\[
g:\Times\rightarrow V
\]
}
{map g, representation, tensor product}

\DefEq
{
\[
h:\Tensor B\rightarrow V
\]
}
{map h, representation, tensor product}

\AddEq{tower of representations}
{
\[
\xymatrix
{
A_1\ar[r]|{*}^{f_{1\,2}}&A_2\ar[r]|{*}^{f_{2\,3}}
&...\ar[r]|{*}^{f_{n-1\,n}}&A_n
}
\]
}

\AddEquation{morphism of diagram of representations, level k}
{
h_j\circ\BlueText{f_{ij}(a_i)}
=g_{ij}(\RedText{h_i(a_i)})\circ h_j
}

\AddEq{hi:Ai->Bi}
{
\ShowEq{f:A->B}{h_{(i)}}{A_{(i)}}{B_{(i)}}
}

\AddEq[2]{A=A1n}
{
$#1=(#1_{(1)}\ \ ...\ \ #1_{(n)})$#2
}

\AddEq[1]{A=A(1n)1n}
{
\[
#1=(#1_{(1)}\ \ ...\ \ #1_{(n)})=(#1_1\ \ ...\ \ #1_n)
\]
}

\AddEq[2]{A(i)=Ai}
{
$A_{(#1)}=A_{#1}$#2
}

\AddEq{closure operator, representation}
{
\symb{J[f]}{closure operator, representation}1.
}

\AddEq{show closure operator, representation}
{
$\ShowSymbol{subrepresentation generated by set}1$
}

\AddEq[1]{map of words of representation, W}
{
\[
w[f\rightarrow g,#1,#1',R_1]:w[f,#1]\rightarrow w[g,#1']
\]
}

\AddEq[2]{map of words of representation, W in X}
{
\[
#1\in #2=>w[f\rightarrow g,#2,#2',R_1](#1)=R_1(#1)
\]
}

\AddEq[1]{endomorphism based on map of words of representation}
{
\[
R(m)=w[f\rightarrow g,#1,#1',R_1](w[f,#1,m])
\]
}

\AddEq{map of words of representation 2}
{
$m'\in J[g,X']$.
}

\AddEq{map of words of representation, m in X, 1}
{
$m\in X$, $m'=R(m)$,
}

\AddEq{map of words of representation}
{
\[
\wXR:w[f,X]\rightarrow w[g,X']
\]
}

\AddEq{a=a12}
{
$a=(a_1,a_2)$
}

\AddEq{r(a)12}
{
\[
r(a)=(r_1(a_1),r_2(a_2))
\]
}

\AddEq{map of words of representation, m in X}
{
\labelItem{map of words of representation, m in X}
\[
\wXR(m)=m'
\]
}

\AddEq{map of words of representation, omega, 1}
{
\[
m_1, ..., m_n\in w[f,X]
\]
\[
\begin{matrix}
m'_1=\wXR(m_1)&...&m'_n=\wXR(m_n)
\end{matrix}
\]
}

\AddEq{map of words of representation, omega}
{
\labelItem{map of words of representation, omega}
\[
\wXR(m_1...m_n\omega)=m_1'...m_n'\omega
\]
}

\AddEq{map of words of representation, am, 1}
{
\[
\begin{matrix}
m\in w[f,X]& m'=\wXR(m)
&a\in A_1
\end{matrix}
\]
}

\AddEq{map of words of representation, am}
{
\labelItem{map of words of representation, am}
\[
\wXR(f(a)(m))=g(a)(m')
\]
}

\AddEq{generating set of representation}
{
$J[f,X]=A_2$.
}

\AddEq{subrepresentation generated by set}
{
\symb{J[f,X]}{subrepresentation generated by set}1
}

\AddEquation{morphism of diagram of representations, levels k k+1}
{
\BlueText{h_j(f_{ij}(a_i)(a_j))}
=g_{ij}(\RedText{h_i(a_i)})(\BlueText{h_j(a_j)})
}

\AddEq[2]{f:i->*j}
{
\ShowEq{f:A->*B}{f_{#1#2}}{A_{#1}}{A_{#2}}
}

\AddEq{f:ij->*k}
{
\ShowEq{f:A->*B}{f_{ij,k}}{A_i\times A_j}{A_k}
}

\AddEq[3]{Ai->*Aj->*Ak}
{
\xymatrix
{
A_{#1}\ar[r]|{*}^{f_{#1#2}}&A_{#2}\ar[r]|{*}^{f_{#2#3}}&A_{#3}
}
}

\AddEquation{tower of representations, 1 2 3}
{
\xymatrix{
\\
A_k\ar@/_3pc/[rrrr]^{f_{jk}(a_j)}="fkaj"
\ar@/^3pc/[rrrr]^{f_{jk}(\RedText{f_{ij}(a_i)(a_j)})}="fkbj"&&&&A_k
\\
\\
&A_j\ar[rr]^{f_{ij}(a_i)}\ar @{}[rl]="aj"&&A_j\ar @{}[rl]="bj"
\\
\\
&&A_i\ar @{}[rl]="ai"\ar@{=>}[uu]^{f_{ij}}&&
\ar @{=>}^{f_{jk}} "aj";"fkaj"
\ar @{=>}@/_3pc/^{f_{jk}} "bj";"fkbj"
\ar @{=>} "fkaj";"fkbj"_{f_{ijk}(a_i)}="ajbj"
\ar @{=>}@/^6pc/ "ai";"ajbj"^{f_{ijk}}
}
}

\AddEquation{tower of representations, ij,k}
{
\xymatrix{
&&A_i\times A_j\ar@{=>}[d]_{f_{ij,k}}
\\
A_k\ar[rrrr]_{f_{jk}(\RedText{f_{ij}(a_i)(a_j)})}="fkbj"&&&&A_k
\\
\\
&A_j\ar[rr]^{f_{ij}(a_i)}\ar @{}[rl]="aj"&&A_j\ar @{}[rl]="bj"
\\
\\
&&A_i\ar @{}[rl]="ai"\ar@{=>}[uu]^{f_{ij}}&&
\ar @{=>}@/_3pc/^{f_{jk}} "bj";"fkbj"
}
}

\AddEq{f:A->End 2 3}
{
\ShowEq{f:A->B}{f_{ijk}}{A_i}{
\ShowEq{End 2 3}
}
}

\AddEq{End 2 3}
{
\ensuremath{\End(\Omega_j,\End(\Omega_k,A_k))}
}

\AddEquation{define map f13}
{
f_{ijk}(a_i)(\BlueText{f_{jk}(a_j)})
=\BlueText{f_{jk}(\RedText{f_{ij}(a_i)(a_j)})}
}

\AddEq{f:1->*3}
{
\ShowEq{f:A->*B}{f_{ijk}}{A_i}{\End(\Omega_k,A_k)}
}

\AddEq[3]{End Ak}
{
$\End(\Omega_{#2},#1_{#2})$#3
}

\AddEquation{morphism of diagram of representations of F algebra, level k, diagram}
{
\xymatrix{
&A_j\ar[dd]_(.3){f_{ij}(a_i)}
\ar[rr]^{h_j}
&&
B_j\ar[dd]^(.3){g_{ij}(\RedText{h_i(a_i)})}\\
&\ar @{}[rr]|{(1)}&&\\
&A_j\ar[rr]^{h_j}&&B_j\\
A_i\ar[rr]^{h_i}\ar@{=>}[uur]^(.3){f_{ij}}
&&
B_i\ar@{=>}[uur]^(.3){g_{ij}}
}
}

\DefEq
{
\[
\xymatrix{
&\Tensor B\ar[dd]^h
\\
\Times
\ar[ru]^f\ar[rd]_g
\\
&V
}
\]
}
{map gh, representation, tensor product}

\DefEq
{
$A$, $B_1$, ..., $B_n$, $B$
}
{set of universal algebras 1}

\DefEq
{
\[
r_2:B_1\times...\times B_n\rightarrow B
\]
}
{reduced polymorphism of representation}

\AddEq{rc-product}
{
\symb{a\RCstar b}{rc-product}{}
}

\AddEquation{rc-product of matrices}
{
\ShowSymbol{rc-product}{}=
\begin{pmatrix}
\aUD aik\aUD bkj
\end{pmatrix}
}

\AddEquation{entry rc-product of matrices}
{
\aUD {(\ShowSymbol{rc-product}{})}ij=
\aUD aik\aUD bkj
}

\AddEquation{rc-product, matrices}
{
\begin{split}
\PMatrix apn\RCstar\PMatrix bmp
&=
\begin{pmatrix}
\aUD a1k\aUD bk1&...&\aUD a1k\aUD bkm\\
...&...&...\\
\aUD ank\aUD bk1&...&\aUD ank\aUD bkm
\end{pmatrix}
\\ &=
\PMatrix{(\ShowSymbol{rc-product}{})}mn
\end{split}
}

\AddEq{cr-product}
{
\symb{a\CRstar b}{cr-product}{}
}

\AddEquation{cr-product of matrices}
{
\ShowSymbol{cr-product}{}=
\begin{pmatrix}
\aUD aki\aUD bjk
\end{pmatrix}
}

\AddEquation{entry cr-product of matrices}
{
\aUD{(\ShowSymbol{cr-product}{})}ij=
\aUD aki\aUD bjk
}

\AddEquation{cr-product, matrices}
{
\begin{split}
\PMatrix amp\CRstar\PMatrix bpn
&=
\begin{pmatrix}
\aUD ak1\aUD b1k&...&\aUD akm\aUD b1k\\
...&...&...\\
\aUD ak1\aUD bnk&...&\aUD akm\aUD bnk
\end{pmatrix}
\\ &=
\PMatrix{(\ShowSymbol{cr-product}{})}mn
\end{split}
}

\AddEquation{(a+b)=}
{
\aUD{(a+b)}ij=\aUD aij+\aUD bij
}

\AddEquation{transpose of matrix, 1}
{
\aUD {(a^T)}ij=\aUD aji
}

\AddEquation{v=(e)(v)}
{
v=
\RowMatrix en
\ColMatrix vn
=\aD ei\aU vi
}

\AddEquation{v'=fv}
{
\aU {v'}i=\aUD fij\aU vj
}

\AddEquation{v'=vf}
{
\aU {v'}i=\aU vj\aUD fij
}

\AddEquation{v=(v)(e)}
{
v=\ColMatrix vn
\ \ \ \ e=\RowMatrix en
}

\AddEquation{reducibility of products}
{
a\RCstar b
=(\aUD aki\aUD bjk)
=(\aUD bjk\aUD aki)
=b\CRstar a
}

\AddEq{(m+n)a=ma+na,n=k}
{
\[(m+k)a=ma+ka\]
}

\AddEq{(m+n)a=ma+na,n=k+1}
{
\begin{align*}
(m+(k+1))a&=((m+k)+1)a=(m+k)a+a=ma+ka+a\\&=ma+(k+1)a
\end{align*}
}

\AddEq{(m+n)a=ma+na,n=k-1}
{
\begin{align*}
(m+(k-1))a&=((m+k)-1)a=(m+k)a-a=ma+ka-a\\&=ma+(k-1)a
\end{align*}
}

\AddEq{n(a+b)=na+nb,n=k}
{
\[k(a+b)=ka+kb\]
}

\AddEq{n(a+b)=na+nb,n=k+1}
{
\begin{align*}
(k+1)(a+b)&=k(a+b)+a+b=ka+kb+a+b\\&=ka+a+kb+b\\&=(k+1)a+(k+1)b
\end{align*}
}

\AddEq{n(a+b)=na+nb,n=k-1}
{
\begin{align*}
(k-1)(a+b)&=k(a+b)-(a+b)=ka+kb-a-b\\&=ka-a+kb-b\\&=(k-1)a+(k-1)b
\end{align*}
}

\AddEq{(nm)a=n(ma),n=k}
{
\[(km)a=k(ma)\]
}

\AddEq{(nm)a=n(ma),n=k+1}
{
\begin{align*}
((k+1)m)a&=(km+m)a=(km)a+ma=k(ma)+ma\\&=(k+1)(ma)
\end{align*}
}

\AddEq{(nm)a=n(ma),n=k-1}
{
\begin{align*}
((k-1)m)a&=(km-m)a=(km)a-ma=k(ma)-ma\\&=(k-1)(ma)
\end{align*}
}

\AddEq{f(na)=nf(a),n=k}
{
\[f(ka)=kf(a)\]
}

\AddEq{f(na)=nf(a),n=k+1}
{
\begin{align*}
f((k+1)a)&=f(ka+a)=f(ka)+f(a)=kf(a)+f(a)\\&=(k+1)f(a)
\end{align*}
}

\AddEq{f(na)=nf(a),n=k-1}
{
\begin{align*}
f((k-1)a)&=f(ka-a)=f(ka)-f(a)=kf(a)-f(a)\\&=(k-1)f(a)
\end{align*}
}

\AddEq{A1(mA2) symb}
{%
\symb{A_1(\mathcal A_2)}{category of representations}1
}

\AddEq[2]{x in JX}
{
$#1\in J[f,X]$#2
}

\AddEq{word of element relative to generating set, representation}
{
\symb{\wXm}
{word of element relative to generating set, representation}1
}

\AddEq{identify element jf(X) and word}
{
\[
m=\wXm
\]
}

\AddEq[1]{subset of representation}
{
$B\subset J_{#1}[f,X]$
}

\AddEq{subset of words of representation, 2}
{
\[
\wXm[\{m\}]=\{\wXm\}
\]
}

\AddEq{subset of words of representation}
{
\symb{\wXm[B]}{subset of words of representation}{}
\[
\ShowSymbol{subset of words of representation}{}
=\{\wXm:m\in B\}
\]
}

\AddEq{subset of words of representation, 1}
{
\[
\wXm[B]=(\wXm,m\in B)
\]
}

\AddEq{word set of representation}
{
\symb{w[f,X]}{word set of representation}1
}

\AddEquation{ambiguity of coordinates 1}
{
f(a)(m_1...m_n\omega)=(f(a)(m_1))...(f(a)(m_n))\omega
}

\AddEq{ambiguity of coordinates 1, vector}
{
\[
a(b^1e_1+b^2e_2)=(ab^1) e_1+(ab^2) e_2
\]
}

\AddEq{a1n omega x}
{
$f(a_1...a_n\omega)(x)$
}

\AddEq{a1n x omega}
{
$(f(a_1)(x))...(f(a_n)(x))\omega$
}

\AddEq{(a+b)e=ae+be}
{
\[(a+b) e_1=ae_1+b e_1\]
}

\AddEq{l fX in w fX}
{
\[
\lambda[f,X]\subseteq w[f,X]\times w[f,X]
\]
}

\AddEq{w1 w2 in l fX}
{
\[
(w_1[f,X,m],w_2[f,X,m])\in\lambda[f,X]
\]
}

\AddEq{fw1m fw2m in l fX}
{
\[
(f(w_1)(w[f,X,m]),f(w_2)(w[f,X,m]))\in\lambda[f,X]
\]
}

\AddEq{(f(a1n)a2,f(a)a2) in l}
{
\[
(f(a_{11}...a_{1n}\omega)(a_2),(f(a_{11})...f(a_{1n})\omega)(a_2))\in\lambda[f,X]
\]
}

\AddEq{(fa1(a21n),fa1(a2)) in l}
{
\[
(f(a_1)(a_{21}...a_{2n}\omega),f(a_1)(a_{21})...f_(a_1)(a_{2n})\omega)
\in\lambda[f,X]
\]
}

\AddEq[3]{omega in O1AO2}
{
$\omega\in\Omega_{#1}(n)\cap\Omega_{#2}(n)$#3
}

\AddEq{f(a)(v)=av}
{
\[f(a)(v)=av\]
}

\AddEq{f(a+b)v=}
{
\[f(a+b)(v)=f(a)(v)+f(b)(v)\]
}

\AddEq{f(ab)v=}
{
\[f(ab)(v)=f(a)(v)f(b)(v)\]
}

\AddEq{f(a1n)a2=f(a)a2}
{
\[
f(a_{11}...a_{1n}\omega)(a_2)=(f(a_{11})(a_2))...(f(a_{1n})(a_2))\omega
\]
}

\AddEq{(f(a1n)a2,f(a)a2) in l 1}
{
\[
(f(a_{11}...a_{1n}\omega)(a_2),(f(a_{11})(a_2))...(f(a_{1n})(a_2))\omega)\in\lambda[f,X]
\]
}

\AddEq{rho=lambda}
{
\[
\rho[f,\Basis e]=\lambda[f,\Basis e]
\]
}

\AddEq{w1[]=w2[]}
{
\[
w_1[f,X,m]=w_2[f,X,m]
\]
}

\AddEq{rho fX=}
{
\[
\rho[f,X]=
\{
(w[f,X,m],w_1[f,X,m]):m\in A_2
\}
\]
}

\AddEq{ambiguity of coordinates 2}
{
f(a_1...a_n\omega)(x)=(f(a_1)(x))...(f(a_n)(x))\omega
}

\AddEq{A1(mA2)}
{
$A_1(\mathcal A_2)$
}

\AddEq[1]{A1(mA2,x)}
{
$\mathcal A(
\xymatrix
{
A_1\ar[r]|{*}&\mathcal A(\Omega_2,X)
}
)$#1
}

\AddEq{X in A2}
{
$X\subset A_2$,
}

\AddEq{product in category}
{
\symb[Pi-1]{\prod_{\iI}B_i}{product in category}{}
\[P=\ShowSymbol{product in category}{}\]
}

\AddEq{coproduct in category}
{
\symb[Pi-1]{\coprod_{\iI}B_i}{coproduct in category}{}
\[P=\ShowSymbol{coproduct in category}{}\]
}

\AddEq{coproduct in category, 1 n}
{
\symb[Pi-1]{\coprod_{i=1}^nB_i}{coproduct in category}{i 1 n}
\symb[B-0]{B_1\coprod...\coprod B_n}{coproduct in category}{1 n}
\[
P=\ShowSymbol{coproduct in category}{i 1 n}
=\ShowSymbol{coproduct in category}{1 n}
\]
}

\AddEq [2]{av=sum av}
{
\[#1^i#2_i=\sum_{\iI}#1^i#2_i\]
}

\AddEquation{f(a)=o left}
{
f(a_2)=f\Act a_2
}

\AddEquation{f(a)=o right}
{
f(a_2)=a_2\Act f
}

\AddEquation{f(a)=* right}
{
f(a)=a\Act f
}

\AddEq{A12->A2 left}
{
\[
(a_1,a_2)\in A_1\times A_2\rightarrow a_1*a_2\in A_2
\]
}

\AddEq{A12->A2 right}
{
\[
(a_1,a_2)\in A_1\times A_2\rightarrow a_2*a_1\in A_2
\]
}

\AddEq{A12->A2 1 left}
{
\[
(a_1,a_2)\in A_1\times A_2\rightarrow a_1*a_2\in A_2
\]
}

\AddEq{A12->A2 1 right}
{
\[
(a_1,a_2)\in A_1\times A_2\rightarrow a_2*a_1\in A_2
\]
}

\AddEquation{fga= o left}
{
(f\circ g)\circ a=f\circ (g\circ a)
}

\AddEquation{fga= o right}
{
a\circ (g\circ f)=(a\circ g)\circ f
}

\DefEq
{
\[f\circ g\circ a=f\circ (g\circ a)=(f\circ g)\circ a\]
}
{fga= 1 left}

\DefEq
{
\[a\circ g\circ f=(a\circ g)\circ f=a\circ (g\circ f)\]
}
{fga= 1 right}

\AddEquation{right shift, product}
{
R(b*c)=R(b)\circ R(c)
}

\AddEquation{left shift, product}
{
L(c*b)=L(c)\circ L(b)
}

\AddEq{right shift =}
{
\symb{R(b)}{right shift}{}
}

\AddEq{right shift}
{
\[a'=a\circ\ShowSymbol{right shift}{}=a*b\]
}

\AddEq{left shift =}
{
\symb{L(b)}{left shift}{}
}

\AddEq{left shift}
{
\[a'=\ShowSymbol{left shift}{}\circ a=b*a\]
}

\DefEq
{
\[
(x_1, ..., x_n)\in B_1\times...\times B_n
\rightarrow x_1\otimes...\otimes x_n\in B_1\otimes...\otimes B_n
\]
}
{B times->B otimes}

\DefEq
{
f:A_1\rightarrow\End(\Omega_2,A_2)
}
{representation of group, map}

\DefEq
{
\[
(\id:A_1\rightarrow A_1,\ r_2:A_2\rightarrow B_2)
\]
}
{id:A1->A1 A2->B2}

\DefEquation
{
\xymatrix{
&A_2\ar[dd]_(.3){f(a)}\ar[rrr]^{r_2}&&&B_2\ar[dd]^(.3){g(a)}\\
&&&&\\
&A_2\ar[rrr]_(.65){r_2}&&&B_2\\
A_1\ar@{=>}[uur]^(.3)f\ar@{=>}[uurrrr]^(.7)g
}
}
{morphism id,R of representations}

\AddEquation{morphism of representations of universal algebra}
{
r_2\circ f(a)=g(a)\circ r_2
}

\DefEq
{
\[
\xymatrix{
A_2\ar[rr]^{r_2}&&B_2\\
&A_1\ar[lu]|{*}^f\ar[ru]|{*}_g
}
\]
}
{morphism id,R of representations 2}

\AddEq{Gen f =}
{
\[
Gen[f]=\{X\subseteq A_2:J[f,X]=A_2\}
\]
}

\AddEq[3]{in Gen}
{
$#1\in Gen[#2]$#3
}

\AddEq[3]{f:A->*B}
{
\[
\xymatrix@C=30pt
{
#1:#2\ar[r]|-{*}&#3
}
\]
}

\AddEq[3]{A->*B}
{
\xymatrix
{
#1\ar[r]|-{*}&#2
}
#3
}

\AddEq{action of rational integers in Abelian group}
{
\begin{align}
\EqLabel{0g=0}
0g&=0
\\
\EqLabel{(n+1)g=}
(n+1)g&=ng+g
\\
\EqLabel{(n-1)g=}
(n-1)g&=ng-g
\end{align}
}

\AddEq{representation of Z in G}
{
\begin{align}
1a&=a
\EqLabel{1a=a}
\\
\EqLabel{(nm)a=n(ma)}
(nm)a&=n(ma)
\\
\EqLabel{(m+n)a=ma+na}
(m+n)a&=ma+na
\\
\EqLabel{(m-n)a=ma-na}
(m-n)a&=ma-na
\\
\EqLabel{n(a+b)=na+nb}
n(a+b)&=na+nb
\end{align}
}

\AddEquation{(k+n)a-na=ka}
{
(k+n)a-na=ka
}

\AddEq{phi(n):G->G}
{
\[
\varphi(n):a\in G\rightarrow na\in G
\]
}

\AddEq{S=si}
{
$S=\{s_i:\iI\}$
}

\AddEquation{J(S)=gi si}
{
J(S)=\left\{g:g=\sum_{\iI}g^is_i, g^i\in Z\right\}
}

\AddEq[1]{|gi ne 0|}
{
$\{\iI:#1^i\ne 0\}$
}

\AddEq{category A(Bi)}
{
$\mathcal A(B_i,\iI)$
}

\AddEq{category A[Bi]}
{
$\mathcal A[B_i,\iI]$
}

\AddEq{gi=dik}
{
$g^i=\delta^i_k$.
}

\AddEquation{sk=sum si}
{
s_k=\sum_{\iI}g^is_i
}

\AddEq{sk in JS}
{%
$s_k\in J(S)$
}

\AddEquation{(ai)+(bi)=(ai+bi)}
{
(a_i,\iI)+(b_i,\iI)=(a_i+b_i,\iI)
}

\AddEq{phi:Z->End(G)}
{
\[
\varphi:Z\rightarrow \End(Ab,G)
\]
}

\AddEq{right-side representation}
{
\[a_2'=a_2\Act f(a_1)=a_2*a_1\]
}

\AddEq{left-side representation}
{
\[a_2'=f(a_1)\Act a_2=a_1*a_2\]
}

\AddEq{right-side representation of group}
{
a_2\Act f(a_1*b_1)=a_2\Act(f(a_1)\Act f(b_1))
}

\AddEq{left-side representation of group}
{
f(a_1*b_1)\Act a_2=(f(a_1)\Act f(b_1))\Act a_2
}

\AddEq{* right-side representation of group}
{
a_2\Act f(a_1*b_1)=a_2*(a_1*b_1)
}

\AddEq{* left-side representation of group}
{
f(a_1*b_1)\Act a_2=(a_1*b_1)*a_2
}

\AddEq{o right-side representation of group}
{
a_2*(a_1*b_1)=(a_2* a_1)* b_1
}

\AddEq{o left-side representation of group}
{
(a_1*b_1)* a_2=a_1*( b_1* a_2)
}

\AddEq{left-side 1 representation of group}
{
f(a_1*b_1)\circ a_2=f(a_1)\circ f(b_1)\circ a_2
}

\AddEq{right-side 1 representation of group}
{
a_2\circ f(a_1*b_1)=a_2\circ f(a_1)\circ f(b_1)
}

\AddEq{morphism of left representation of Omega group}
{
\[
\BlueText{r_2\circ(a_1*a_2)}=\RedText{r_1(a_1)}*(\BlueText{r_2\circ a_2})
\]
}

\AddEq{morphism of right representation of Omega group}
{
\[
\BlueText{r_2\circ(a_2*a_1)}=(\BlueText{r_2\circ a_2})*\RedText{r_1(a_1)}
\]
}

\AddEq{orbit of left-side representation}
{
\symb{A_1*a_2}{orbit of representation}{}
\[
\ShowSymbol{orbit of representation}{}=\{b_2=a_1*a_2:a_1\in A_1\}
\]
}

\AddEq{orbit of right-side representation}
{
\symb{a_2*A_1}{orbit of representation}{}
\[
\ShowSymbol{orbit of representation}{}=\{b_2=a_2*a_1:a_1\in A_1\}
\]
}

\AddEq{space of orbits of representation}
{
\symb{A_2/A_1}{space of orbits of representation}1
}

%\AddEq{space of orbits of effective left-side representation}
%{
%\symb{A_2/A_1}{space of orbits of effective left-side representation}1
%}

%\AddEq{space of orbits of right-side representation}
%{
%\symb{A_2/R(A_1)}{space of orbits of effective right-side representation}1
%}

\AddEq{r2a=r2 o a}
{
\[r_2(a_2)=r_2\circ a_2\]
}

\AddEq[2]{passive and active maps}
{
\[
\xymatrix{
\Basis e_1\in\mathcal B[f]\ar[d]_{#2}\ar[rr]^{#1}&&\Basis e_3\in\mathcal B[f]\ar[d]_{#2}
\\
\Basis e_2\in\mathcal B[f]\ar[rr]^{#1}&&\Basis e_4\in\mathcal B[f]
}
\]
}

\AddEq{sigma->+-}
{
\symb{|\sigma|}{parity of permutation}{}
\[
\ShowSymbol{parity of permutation}{}
:\sigma\in S(n)\rightarrow \{-1,1\}
\]
}

\AddEquation{parity of permutation}
{
\ShowSymbol{parity of permutation}{}=
\left\{
\begin{matrix}
1&\textrm{\permutation}\sigma\textrm{ \even}
\\
-1&\textrm{\permutation}\sigma\textrm{ \odd}
\end{matrix}
\right.
}

\AddEq{Basis e4=Basis e5}
{
$\Basis e_4=\Basis e_5$.
}

\AddEq{passive transformation, 1}
{
\Basis e_5
=\Basis e_3 \circ W[f,\Basis e_1,\Basis e_2]
=W[f,\Basis e_1,\Basis e_3]\circ \Basis e_1\circ W[f,\Basis e_1,\Basis e_2]
}

\AddEq[2]{Omega_2 word, basis e}
{
#2=\Basis e_{#1}\circ W[f,\Basis e_{#1},#2]
}

\AddEq[2]{coordinate transformation in representation, 1}
{
W[f,\Basis e_1,#2]=W[f,\Basis e_1,\Basis e_1\circ #1]\circ W[f,\Basis e_2,#2]
}

\AddEq[2]{Omega word in representation, basis Y, 1}
{
\begin{split}
\Basis e_1\circ W[f,\Basis e_1,#2]&=\Basis e_2\circ W[f,\Basis e_2,#2]
=\Basis e_1\circ W[f,\Basis e_1,\Basis e_2]\circ W[f,\Basis e_2,#2]
\\
&=\Basis e_1\circ W[f,\Basis e_1,\Basis e_1\circ #1]\circ W[f,\Basis e_2,#2]
\end{split}
}

\AddEq[1]{passive transformation S}
{
\Basis e_2=\Basis e_1\circ #1=\Basis e_1\circ W[f,\Basis e_1,\Basis e_1\circ #1]
}

\AddEq[2]{coordinate transformation}
{
W[f,\Basis e_2,#1]=W[f,\Basis e_1\circ #2,\Basis e_1]\circ W[f,\Basis e_1,#1]
}

\AddEq[2]{coordinate transformation in representation, TS 1}
{
$#2\circ #1$.
}

\AddEq[3]{coordinate transformation in representation, TS}
{
\begin{align*}
W[f,\Basis e_3,#1]
&=W[f,\Basis e_1\circ #3,\Basis e_1]\circ W[f,\Basis e_1\circ #2,\Basis e_1]\circ W[f,\Basis e_1,#1]
\\
&=W[f,\Basis e_1\circ #3\circ #2,\Basis e_1]\circ W[f,\Basis e_1,#1]
\end{align*}
}

\AddEq[1]{coordinates of geometric object}
{
\symb[O-0]{\mathcal O(f,g,\Basis e_g,#1)}{coordinates of geometric object}{}
}

\AddEq[2]{show coordinates of geometric object}
{
\begin{align*}
\ShowSymbol{coordinates of geometric object}{}
&=H(GA(f))\circ W[g,\Basis e_g,#2]
\\
&=(W[g,\Basis e_g\circ H(#1),\Basis e_g]\circ W[g,\Basis e_g,#2],\Basis e_f\circ #1,#1\in GA(f))
\end{align*}
}

\AddEq[1]{geometric object 2, g}
{
\[
#1=\Basis e_g\circ W[g,\Basis e_g,#1]
\]
}

\AddEq[2]{invariance principle 3 algebra}
{
\begin{align*}
#1'&=\Basis e_{g1}\circ W[g,\Basis e_{g1},#1']
\\
&=\Basis e_g\circ W[g,\Basis e_g,\Basis e_g\circ H(#2)]
\circ W[g,\Basis e_g\circ H(#2),\Basis e_g]\circ W[g,\Basis e_g,#1]
\\
&=\Basis e_g\circ W[g,\Basis e_g,#1]=#1
\end{align*}
}

\AddEq[1]{invariance principle 2 passive}
{
\[\Basis e_{f1}=\Basis e_f\circ #1\]
}

\AddEq[1]{geometric object}
{
\symb[O-0]{\mathcal O(f,g,#1)}{geometric object}{}%
}

\AddEq[2]{show geometric object}
{
\[
\ShowSymbol{geometric object}{}=
(W[g,\Basis e_g\circ H(#1),\Basis e_g]\circ W[g,\Basis e_g,#2],
\Basis e_g\circ H(#1),\Basis e_f\circ #1,#1\in GA(f))
\]
}

\AddEq[1]{geometric object 1}
{
$\Basis e_{f1}=\Basis e_f\circ #1$
}

\AddEq{geometric object 2}
{
$\Basis e_{f1}$.
}

\AddEq[1]{passive transformation of representation g}
{
\Basis e_{g1}=\Basis e_g\circ H(#1)
}

\AddEq[2]{coordinate transformation g}
{
W[g,\Basis e_{g1},#1]=W[g,\Basis e_g\circ H(#2),\Basis e_g]\circ W[g,\Basis e_g,#1]
}

\AddEq[1]{invariance principle 4}
{
$W[g,\Basis e_g,#1]$.
}

\AddEq{passive representation coordinated with passive representation}
{
\[
\xymatrix{
\mathcal \End(B[f])\ar[rr]^H
&&
\mathcal \End(B[g])
\\
GA(f)\ar[u]^{P(f)}\ar[rr]_h\ar[urr]_{f'}
&&
GA(g)\ar[u]_{P(g)}
}
\]
}

\AddEq{active transformation, 1}
{
\Basis e_4
=W[f,\Basis e_1,\Basis e_3]\circ \Basis e_2
=W[f,\Basis e_1,\Basis e_3]\circ \Basis e_1\circ W[f,\Basis e_1,\Basis e_2]
}

\AddEq{basis manifold}
{
\symb{\mathcal B[f]}{basis manifold}1
}

\AddEq{passive representation in basis manifold def}
{
\ShowEq{f:A->*B}{\ShowSymbol{passive representation in basis manifold}{}}
{GA(f)}{\mathcal B[f]}
}

\AddEq{passive representation in basis manifold}
{
\symb{P(f)}{passive representation in basis manifold}{}
}

\AddEq[1]{passive transformation of basis def}
{
\[
#1(\Basis e)=
\ShowSymbol{passive transformation of basis}{}
\]
}

\AddEq[1]{passive transformation of basis}
{
\symb{\ecS[#1]}{passive transformation of basis}{}
}

\AddEq[1]{passive transformation}
{
\begin{split}
#1:\Basis h&\rightarrow\Basis h\circ #1
%\\
%W[f,\Basis e, \Basis h\circ #1]&=W[f,\Basis e,\Basis h]\circ W[f,\Basis e,\ecS[#1]]
\\
\Basis h\circ #1&=\Basis h\circ W[f,\Basis e,\ecS[#1]]
%=\Basis e\circ W[f,\Basis e,\Basis h]\circ W[f,\Basis e,\ecS[#1]]
\end{split}
}

\AddEq[1]{active transformation}
{
\begin{split}
#1:\Basis h&\rightarrow #1\circ\Basis h
\\
#1\circ\Basis h&
=W[f,\Basis e,\Rce[#1]]\circ\Basis h
%=W[f,\Basis e,\Rce[#1]]\circ\Basis e\circ W[f,\Basis e,\Basis h]
%\\
%W[f,\Basis e,#1\circ\Basis h]&=W[f,\Basis e,\Rce[#1]]\circ W[f,\Basis e,\Basis h]
\end{split}
}

\AddEq[3]{e2=e1 o S}
{
$\Basis e_{#2}=\Basis e_{#3}\circ #1$.
}

\AddEq[3]{e3=R o e1}
{
$\Basis e_{#2}=\Rce[#1]_{#3}$.
}

\DefText{two matrix products}
{
\ShowDefinition{row over column product}

\ShowDefinition{column over row product}
}

\DefText{matrix operations}
{
\ShowText{matrix operations 1}

\ShowText{two matrix products}

\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
\ShowText{matrix operations 2}

\ShowDefinition{transpose of matrix}

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOff
\ShowTheorem{double transpose is original matrix}
\ShowProof{double transpose is original matrix}
\fi

\ShowDefinition{sum of matrices}
\fi

\ShowEq{remark: pronunciation of product}

\ePrints{5284-0163,1801.01628,2207.06506,8428-0408}
\ifx\Semafor\ValueOn
\ShowEq{product of matrices is distributive over addition}
\fi

\ePrints{2020.06.01,2022.01.05}
\ifx\Semafor\ValueOff
\TwoColText
{
\ShowTheorem{rc transpose}
}
{
\ShowTheorem{cr transpose}
}
\ShowProof{rc transpose}
\ShowProof{cr transpose}
\fi
}

\AddEquation{cr transpose, 1}
{
(a\CRstar b)^T=((a^T)^T\CRstar (b^T)^T)^T
}

\AddEquation{cr transpose, 2}
{
(a\CRstar b)^T=((a^T\RCstar b^T)^T)^T
}

\DefText{matrix over Omega ring}
{
\ShowDefinition{matrix over Omega ring}

\ShowConvention{Einstein summation}

\ShowText{matrix operations}

\ShowDefinition{biring}

\ShowTheorem{duality principle for biring}

\ShowTheorem{duality principle for biring of matrices}

\ShowEq{power matrix}

\ShowText{matrix product}

\ShowRemark{reducible biring}
}

\DefText{matrix product}
{
\TwoColText
{
\ShowEq{def rc}
\ShowTheorem{two products equal}
\begin{sloppypar}
\ShowProof{two products equal}
\end{sloppypar}
}
{
\ShowEq{def cr}
\ShowTheorem{two products equal}
\begin{sloppypar}
\ShowProof{two products equal}
\end{sloppypar}
}

\TwoColText
{
\ShowEq{def rc}
\ProveTheorem{inverse matrix of product}
}
{
\ShowEq{def cr}
\ProveTheorem{inverse matrix of product}
}
}

\AddEq{delta=Matrix}
{
\gdef\UnitNMatrix{\delta}
$\UnitNMatrix=(\aUD {\delta}ij)$
}

\AddEq{rc-inverse matrix}
{
a\RCstar a^{\RCInverse}=\UnitNMatrix
}

\AddEq{cr-inverse matrix}
{
a\CRstar a^{\CRInverse}=\UnitNMatrix
}

\ePrints{1908.04418,6860-2955}%
\ifx\Semafor\ValueOff%
\AddEquation{v=vi ei 123, left-cols}
{
\begin{aligned}
\Vector v&=v_1\CRstar\Basis e_1=v_2\CRstar\Basis e_2\\&=v_3\CRstar\Basis e_3
\end{aligned}
}
\else
\AddEquation{v=vi ei 123, left-cols}
{
\Vector v=v_1\CRstar\Basis e_1=v_2\CRstar\Basis e_2=v_3\CRstar\Basis e_3
}
\fi

\AddEquation{v=vi ei 123, right-cols}
{
\begin{aligned}
\Vector v&=\Basis e_1\RCstar v_1=\Basis e_2\RCstar v_2\\&=\Basis e_3\RCstar v_3
\end{aligned}
}

\AddEquation{v=vi ei 123, left-rows}
{
\begin{aligned}
\Vector v&=v_1\RCstar\Basis e_1=v_2\RCstar\Basis e_2\\&=v_3\RCstar\Basis e_3
\end{aligned}
}

\AddEquation{v=vi ei 123, right-rows}
{
\begin{aligned}
\Vector v&=\Basis e_1\CRstar v_1=\Basis e_2\CRstar v_2\\&=\Basis e_3\CRstar v_3
\end{aligned}
}

\AddEquation{v=vi ei 12, left-cols}
{
\Vector v=v_1\CRstar\Basis e_1=v_2\CRstar\Basis e_2
}

\AddEquation{v=vi ei 12, right-cols}
{
\Vector v=\Basis e_1\RCstar v_1=\Basis e_2\RCstar v_2
}

\AddEquation{v=vi ei 12, left-rows}
{
\Vector v=v_1\RCstar\Basis e_1=v_2\RCstar\Basis e_2
}

\AddEquation{v=vi ei 12, right-rows}
{
\Vector v=\Basis e_1\CRstar v_1=\Basis e_2\CRstar v_2
}

\AddEq{Basis e i=12}
{
$\Basis e_i$, $i=1$, $2$.
}

\AddEq{Basis e i=13}
{
$\Basis e_i$, $i=1$, $2$, $3$.
}

\AddEq[4]{e2i=aij e1j cr-cols}
{
\Basis e_{#2}=#3_{#4}\CRstar\Basis e_{#1}
}

\AddEq[4]{e2i=aij e1j rc-cols}
{
\Basis e_{#2}=\Basis e_{#1}\RCstar #3_{#4}
}

\AddEq[4]{e2i=aij e1j cr-rows}
{
\Basis e_{#2}=\Basis e_{#1}\CRstar #3_{#4}
}

\AddEq[4]{e2i=aij e1j rc-rows}
{
\Basis e_{#2}=#3_{#4}\RCstar\Basis e_{#1}
}

\AddEq[1]{Basis e in BVG}
{
$\Basis e_{#1}\in
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}$
}

\AddEquation{e3=g12 cr e1 left-cols}
{
\Basis e_3=(g_2\CRstar g_1)\CRstar\Basis e_1
}

\AddEquation{e3=g12 cr e1 right-cols}
{
\Basis e_3=\Basis e_1\RCstar(g_1\RCstar g_2)
}

\AddEquation{e3=g12 cr e1 left-rows}
{
\Basis e_3=(g_2\RCstar g_1)\RCstar\Basis e_1
}

\AddEquation{e3=g12 cr e1 right-rows}
{
\Basis e_3=\Basis e_1\CRstar(g_1\CRstar g_2)
}

\AddEquation{v1 cr e1=v2 cr g cr e1, left-cols}
{
v_1\CRstar\Basis e_1=v_2\CRstar g\CRstar\Basis e_1
}

\AddEquation{v1 cr e1=v2 cr g cr e1, right-cols}
{
\Basis e_1\RCstar v_1=\Basis e_1\RCstar g\RCstar v_2
}

\AddEquation{v1 cr e1=v2 cr g cr e1, left-rows}
{
v_1\RCstar\Basis e_1=v_2\RCstar g\RCstar\Basis e_1
}

\AddEquation{v1 cr e1=v2 cr g cr e1, right-rows}
{
\Basis e_1\CRstar v_1=\Basis e_1\CRstar g\CRstar v_2
}

\AddEq[6]{v1=v2*a left-cols}
{
#1_{#2}=#3_{#4}\CRstar #5_{#6}
}

\AddEq[6]{v1=v2*a right-cols}
{
#1_{#2}=#5_{#6}\RCstar #3_{#4}
}

\AddEq[6]{v1=v2*a left-rows}
{
#1_{#2}=#3_{#4}\RCstar #5_{#6}
}

\AddEq[6]{v1=v2*a right-rows}
{
#1_{#2}=#5_{#6}\CRstar #3_{#4}
}

\AddEq[4]{v1g- left-cols}
{
#1_{#2}\CRstar #3_{#4}^{\CRInverse}
}

\AddEq[4]{v1g- right-cols}
{
#3_{#4}^{\RCInverse}\RCstar #1_{#2}
}

\AddEq[4]{v1g- left-rows}
{
#1_{#2}\RCstar #3_{#4}^{\RCInverse}
}

\AddEq[4]{v1g- right-rows}
{
#3_{#4}^{\CRInverse}\CRstar #1_{#2}
}

\AddEq[8]{v2=v1g-}
{
#1_{#2}=
\ShowEq{v1g- #7-#8}{#3}{#4}{#5}{#6}
}

\AddEquation{v3=v1 cr g21- left-cols}
{
v_3=v_1\CRstar (g_2\CRstar g_1)^{\CRInverse}
}

\AddEquation{v3=v1 cr g21- right-cols}
{
v_3=(g_2\RCstar g_1)^{\RCInverse}\RCstar v_1
}

\AddEquation{v3=v1 cr g21- left-rows}
{
v_3=v_1\RCstar (g_2\RCstar g_1)^{\RCInverse}
}

\AddEquation{v3=v1 cr g21- right-rows}
{
v_3=(g_2\CRstar g_1)^{\CRInverse}\CRstar v_1
}

\AddEquation{v3=v1 cr g1- cr g2- left-cols}
{
v_3=v_1\CRstar g_1^{\CRInverse}\CRstar g_2^{\CRInverse}
}

\AddEquation{v3=v1 cr g1- cr g2- right-cols}
{
v_3=g_2^{\RCInverse}\RCstar g_1^{\RCInverse}\RCstar v_1
}

\AddEquation{v3=v1 cr g1- cr g2- left-rows}
{
v_3=v_1\RCstar g_1^{\RCInverse}\RCstar g_2^{\RCInverse}
}

\AddEquation{v3=v1 cr g1- cr g2- right-rows}
{
v_3=g_2^{\CRInverse}\CRstar g_1^{\CRInverse}\CRstar v_1
}

\AddEq{rc power, 0}
{
a^{\RCPower 0}=\UnitNMatrix
}

\AddEq{rc power}
{
\symb{a^{\RCPower k}}{rc power}{}
}

\AddEq{rc-power, n}
{
\ShowSymbol{rc power}{}=a^{\RCPower{k-1}}\RCstar a
}

\AddEq{cr power, 0}
{
a^{\CRPower 0}=\UnitNMatrix
}

\AddEq{cr power}
{
\symb{a^{\CRPower k}}{cr power}{}
}

\AddEq{cr-power, n}
{
\ShowSymbol{cr power}{}=a^{\CRPower{k-1}}\CRstar a
}

\AddEq{Hadamard inverse of matrix 3}
{
\[
(\aUD aji)^{-1}=\frac 1{\aUD aij}
\]
}

\AddEquation{Hadamard inverse of matrix 2}
{
\ShowSymbol{Hadamard inverse of matrix}{}
=
\begin{pmatrix}
(\aUD a11)^{-1}&...&(\aUD an1)^{-1}\\
...&...&...\\
(\aUD a1n)^{-1}&...&(\aUD ann)^{-1}
\end{pmatrix}
}

\AddEquation{Hadamard inverse of matrix 2 entry}
{
\aUD{(\ShowSymbol{Hadamard inverse of matrix}{})}ij
=(\aUD {(a^T)}ij)^{-1}=(\aUD aji)^{-1}
}

\AddEq{Hadamard inverse of matrix}
{
\symb{\mathcal{H}a}{Hadamard inverse of matrix}{}
}

\AddEq{RC-quasideterminant definition}
{
\symb{\RCDet\,a}{RC-quasideterminant definition}{}
}

\AddEquation{RC-quasideterminant definition=}
{
\begin{split}
\ShowSymbol{RC-quasideterminant definition}{}&=
\begin{pmatrix}
\RCdet 11a&...&\RCdet 1na\\
...&...&...\\
\RCdet n1a&...&\RCdet nna
\end{pmatrix}
\\ &=
\begin{pmatrix}
(\aUD{(a^{\RCInverse})}11)^{-1}&...&(\aUD{(a^{\RCInverse})}n1)^{-1}\\
...&...&...\\
(\aUD{(a^{\RCInverse})}1n)^{-1}&...&(\aUD{(a^{\RCInverse})}nn)^{-1}
\end{pmatrix}
\end{split}
}

\AddEq{j i RC-quasideterminant definition}
{
\symb{\RCdet jia}{j i RC-quasideterminant definition}{}
}

\AddEquation{j i RC-quasideterminant =}
{
\ShowSymbol{j i RC-quasideterminant definition}{}
=\minorD
-\minorC\RCstar
\left(\minorA\right)^{\RCInverse}\RCstar
\minorB
=(\aUD{(a^{\RCInverse})}ij)^{-1}
}

\AddEq{inverse matrix 2x2, 0}
{
\[
a=
\begin{pmatrix}
\aUD a11&\aUD a12
\\
\aUD a21&\aUD a22
\end{pmatrix}
\]
}

\AddEq{quasideterminant matrix 2x2 def}
{
\def\aAA{(\aUD a11)^{-1}}
\def\aBA{(\aUD a21)^{-1}}
\def\aAB{(\aUD a12)^{-1}}
\def\aBB{(\aUD a22)^{-1}}
\def\BAA{\aUD a11-\aUD a12\aBB\aUD a21}
\def\BAB{\aUD a12-\aUD a11\aBA\aUD a22}
\def\BBA{\aUD a21-\aUD a22\aAB\aUD a11}
\def\BBB{\aUD a22-\aUD a21\aAA\aUD a12}
\def\CAA{\aUD a11-\aUD a21\aBB\aUD a12}
\def\CAB{\aUD a12-\aUD a22\aBA\aUD a11}
\def\CBA{\aUD a21-\aUD a11\aAB\aUD a22}
\def\CBB{\aUD a22-\aUD a12\aAA\aUD a21}
%\def\AAA{(\BAA)^{-1}}
%\def\AAB{(\BBA)^{-1}}
\def\ABA{(\BAB)^{-1}}
%\def\ABB{(\BBB)^{-1}}
\def\DAA{(\CAA)^{-1}}
\def\DBA{(\CAB)^{-1}}
\def\DAB{(\CBA)^{-1}}
\def\DBB{(\CBB)^{-1}}
\def\UMBA{\aUD{(a^{\RCInverse})}21}
\def\UMAB{\aUD{(a^{\RCInverse})}12}
}

\AddEquation{quasideterminant rc, matrix 2x2}
{
\RCDet a=
\begin{pmatrix}
\BAA&\BAB
\\
\BBA&\BBB
\end{pmatrix}
\ifx\texFuture\Defined
\aUD a11-\aUD a12(\aUD a22)^{-1}\aUD a21&\aUD a12-\aUD a11(\aUD a21)^{-1}\aUD a22
\\
\aUD a21-\aUD a22(\aUD a12)^{-1}\aUD a11&\aUD a22-\aUD a21(\aUD a11)^{-1}\aUD a12
\fi
}

\AddEquation{diagram of representations, left module nonassociative 1}
{
\begin{matrix}
\vcenter
{
\xymatrix
{
A\ar[rr]|{*}^{g_{34}}&&V
\\
&D\ar[ur]|{*}_{g_{14}}\ar[ul]|(.4){*}^{g_{12}}
}
}
&
\begin{array}{r@{\,}l}
g_{12}(d):a&\rightarrow d\,a
\\
g_{34}(a):v&\rightarrow a\,v
\\
g_{14}(d):v&\rightarrow d\,v
\end{array}
\end{matrix}
}

\AddEquation{quasideterminant cr, matrix 2x2}
{
\CRDet a=
\begin{pmatrix}
\CAA&\CAB
\\
\CBA&\CBB
\end{pmatrix}
}

\AddEquation{rc inverse matrix 2x2}
{
a^{\RCInverse}=
\begin{pmatrix}
\DAA&\DAB
\\
\DBA&\DBB
\end{pmatrix}
}

\AddEquation{orbit, proposition}
{
b_2\in A_1*a_2
}

\AddEquation{A1a2=A1b2}
{
A_1*a_2=A_1*b_2
}

\AddEq{AbS ff'g}
{
\xymatrix
{
G\ar[rr]^g&&G'\\
&S\ar[ul]^f\ar[ur]_{f'}
}
}

\AddEq{S in G}
{
$S\subseteq G$.
\labelItem{S in G}
}

\AddEq{h12 in G}
{
$h_1$, $h_2\in G$.
}

\AddEq{H12=}
{
\begin{align*}
H_1&=\{x\in S:h_1(x)\ne 0\}
\\
H_2&=\{x\in S:h_2(x)\ne 0\}
\end{align*}
}

\AddEq{H1vH2}
{
\[
\{x\in S:h_1(x)+h_2(x)\ne 0\}\subseteq H_1\cup H_2
\]
}

\AddEq{h1+h2 in G}
{
$h_1+h_2\in G$.
}

\AddEq{k*x=k}
{
\[
h(y)=\left\{
\begin{matrix}
k&y=x\\
0&y\ne x
\end{matrix}
\right.
\]
}

\AddEq{f:S->G}
{
\[f:x\in S\rightarrow 1*x\in G\]
}

\AddEquation{h=k*x}
{
h=\sum_{x\in S}k_xx
}

\AddEq{kx=k*x}
{
\[kx=k(1*x)=k*x\]
}

\AddEq{|kx ne 0|}
{
$\{x:k_x\ne 0\}$
}

\AddEq{k in Z x in S}
{
$k_x\in Z$, $x \in S$,
}

\AddEquation{h=k12*x i}
{
\sum_{i=1}^nk_1^i*x_i=\sum_{i=1}^nk_2^i*x_i
}

\AddEquation{k1-k2 *x}
{
\sum_{i=1}^n(k_1^i-k_2^i)*x_i=0
}

\AddEq{k1=k2 i}
{
$k_1^i=k_2^i$, $i=1$, ..., $n$,
}

\AddEquation{g(1x)=f'(x)}
{
g(1x)=f'(x)
}

\AddEquation{f(na)=nf(a)}
{
f(na)=nf(a)
}

\AddEquation{g(x)=}
{
g(h)=
g\left(\sum_{x\in S}k_xx\right)=\sum_{x\in S}g(k_xx)=\sum_{x\in S}k_xg(1x)=\sum_{x\in S}k_xf'(x)
}

\AddEq{x in -> h(x)}
{
$\{x\in S:h(x)\ne 0\}$
}

\AddEq{category AbS}
{
$Ab(S)$
}

\DefText{representation of group}
{
\ShowEq{def left}
\ShowDefinition{side representation of group}
\ShowText{side representation of group}
\ShowRemark{morphism of representation of Omega group}
\ShowEq{def right}
\ShowDefinition{side representation of group}
\ShowText{side representation of group}
\ShowRemark{morphism of representation of Omega group}
\ShowDefinition{representation of Abelian group}
}

\AddEquation{Left side contravariant representation}
{
a_1^{-1}*(b_1^{-1}*a_2)=(b_1*a_1)^{-1}*a_2
}

\AddEq{Left side covariant representation}
{
\[
a_1*(b_1*a_2)=(a_1*b_1)*a_2
\]
}

\AddEq{two representations of group}
{
\[
\xymatrix{
A_2\ar[rr]^{h(a_1)}\ar[d]^{f(b_1)} & & A_2\ar[d]^{f(b_1)}\\
A_2\ar[rr]_{h(a_1)}& &A_2
}
\]
}

\AddEq{d2=...c2 1}
{
$d_2=b_1b_2=b_1a_1a_2=b_1a_1b_1^{-1}c_2$.
}

\AddEq{d2=...c2}
{
\[h(a_1)\Act c_2=(b_1a_1b_1^{-1})c_2\]
}

\AddEq{Diagram: two representations of group 1}
{
\[\xymatrix{
a_2\ar[rrr]^{h(a_1)=L(a_1) }\ar[d]^{f(b_1)=L(b_1)}
&&& b_2\ar[d]^{f(b_1)=L(b_1)}\\
c_2\ar[rrr]_{h(a_1)}&&&d_2
}\]
}

\AddEq{Diagram: two representations of group 2}
{
\[\xymatrix{
a_2\ar[rrr]^{h(a_1)=L(a_1)} &&& b_2\ar[d]^{f(b_1)=L(b_1)}\\
c_2\ar[rrr]_{h(a_1)}\ar[u]_{(f(b_1))^{-1}=L(b^{-1}_1)}&&&d_2
}\]
}

\AddEq{haa=aRa}
{
\[a_2\Act h(a_1)=a_2\circ R(a_1)=b_2\]
}

\AddEq{haa=Laa}
{
\[h(a_1)\Act a_2=L(a_1)\circ a_2=b_2\]
}

\AddEq{(fg)->fg}
{
\[
(f,g)\rightarrow f\Act g
\]
}

\AddEq{Act=circ}
{
\[f\Act g=f\circ g\]
}

\AddEq{(ab)->ab}
{
\[
(a,b)\rightarrow a*b
\]
}

\DefEq
{
\[\sum_{i=1}^{\infty}\|a^i\|<\infty\]
}
{sum |ai|<infty}

\DefEq
{
\[\sum_{i=1}^{\infty}a^i\]
}
{sum ai}

\AddEq{integral of map}
{
\symb{\int_X d\mu(x)f(x)}{Lebesgue integral}{}
}

\AddEquation{integral of simple map}
{
\ShowSymbol{Lebesgue integral}{}=
\sum_n \mu(F_n)f_n
}

\AddEquation{integral of measurable map}
{
\ShowSymbol{Lebesgue integral}{}=
\lim_{n\rightarrow\infty}\int_X d\mu(x)f_n(x)
}

\DefEq
{
\[\int_Xd\mu(x)f(x)\]
}
{int f X}

\DefEq
{
\[\int_Xd\mu(x)g(x)\]
}
{int g X}

\DefEq
{
\[\int_Xd\mu(x)(f(x)+g(x))\]
}
{int f+g X}

\DefEq
{
\int_Xd\mu(x)(f(x)+g(x))=
\int_Xd\mu(x)f(x)+
\int_Xd\mu(x)g(x)
}
{int f+g X =}

\DefEq
{
\[\int_Xd\mu(x)\|f(x)\|\]
}
{int |f| X}

\DefEq
{
\left\|\int_Xd\mu(x)f(x)\right\|\le\int_Xd\mu(x)\|f(x)\|
}
{|int f|<int|f|}

\DefEq
{
\|f(x)\|\le M
}
{|f(x)|<M}

\DefEq
{
\int_Xd\mu(x) \|f(x)\|\le M \mu(X)
}
{int |f|<M mu}



==> Stmt.Representation.Russian.tex <==
%auto-ignore
\input{Stmt.Representation.Eq}

\DefDefinition{morphism of representations of universal algebra}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Для
\ShowEq{i=1,2},
пусть отображение
\ShowEq{ri:A->B}
является гомоморфизмом $\Omega_i$\Hyph алгебры.
Кортеж отображений
\ShowEq{map r12}r{}
таких, что
\ShowEq{morphism of representations of universal algebra, definition, 2}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
}

\DefRemark{morphism of representations of universal algebra}
{
Мы можем интерпретировать
\eqRef{morphism of representations of universal algebra, 2m}{representation}
двумя способами
\begin{itemize}
\item Пусть преобразование $\BlueText{f(a)}$ отображает $m\in A_2$
в $\BlueText{f(a)}(m)$.
Тогда преобразование
\ShowEq{g(r1(a))}
отображает
\ShowEq{r2(m)in B2}
в
\ShowEq{r2(f(a,m))}
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\DrawEq{morphism of representations of universal algebra, 2m 1}{ShadedDefinition}
Из \EqRef{morphism of representations of universal algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
Мы будем также пользоваться диаграммой
\ShowEq{morphism of representations of universal algebra, definition, 2m 2}
вместо диаграммы
\eqRef{morphism of representations of universal algebra, 2m 1}{ShadedDefinition}.
}

\DefRemark{morphism of representations of universal algebra as map}
{
Мы можем рассматривать пару отображений $r_1$, $r_2$ как отображение
\ShowEq{F:A1+A2->B1+B2}
такое, что
\ShowEq{F:A1+A2->B1+B2 1}
Поэтому в дальнейшем кортеж отображений
\ShowEq{map r12}r{}
мы будем также называть отображением
и пользоваться записью
\ShowEq{f:A->B}rfg
Пусть
\ShowEq{a=a12}
- кортеж $A$\Hyph чисел.
Мы будем пользоваться записью
\ShowEq{r(a)12}
для образа кортежа $A$\Hyph чисел
при морфизме представлений $r$.
}

\DefTheorem{unique morphism of representations of universal algebra}
{
Если представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивно
и представление
\ShowEq{f:A->*B}g{B_1}{B_2}
$\Omega_1$\Hyph алгебры $B_1$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
гомоморфизм $\Omega_2$\Hyph алгебры
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
такой, что
\ShowEq{map r12}r{}
является морфизмом
представлений из $f$ в $g$,
определён однозначно
с точностью до выбора образа
\ShowEq{n=r2(m)}
заданного элемента $m\in A_2$.
}

\DefConvention[2]{A number}
{
Элемент $#1$\Hyph #2 $A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
}

\DefTheorem{map is reduced morphism of representations iff}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
является приведенным морфизмом представлений тогда и только тогда, когда
\DrawEq{reduced morphism representation =}{definition}
}

\DefDefinition{morphism of representation f}
{
Если представления $f$ и $g$ совпадают, то морфизм представлений
\ShowEq{map r12}r{}
называется
\AddIndex{морфизмом представления $f$}{morphism of representation f}.
}

\DefRemark{notation for morphism of representations}
{
Рассмотрим морфизм представлений
\ShowEq{r12:A->B}rAB
Мы можем обозначать элементы множества $B_1$, пользуясь буквой по образцу $b\in B_1$.
Но если мы хотим показать, что $b$ является образом элемента
\ShowEq{a in A1},
мы будем пользоваться обозначением $\RedText{r_1(a)}$.
Таким образом, равенство
\ShowEq{r1(a)=r1(a)}
означает, что $\RedText{r_1(a)}$ (в левой части равенства)
является образом
\ShowEq{a in A1}{}
(в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $B_2$ в виде $\BlueText{r_2(m)}$.
Мы будем следовать этому соглащению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами,
где определены соответствующие представления.
}

\DefTheorem{Tuple of maps is morphism of representations iff}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений тогда и только тогда, когда
\DrawEq{morphism of representations of universal algebra, 2m}{representation}
}

\DefDefinition{tower of representations}
{
Рассмотрим множество $\Omega_k$\Hyph алгебр $A_k$, \Kn1.
Положим $A=(A_1,...,A_n)$.
Положим $f=(f_{1\,2},...,f_{n-1\,n})$.
Множество представлений $f_{k\,k+1}$, \Kn1, 
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_{k+1}$\Hyph алгебре $A_{k+1}$
называется
\AddIndex{башней $(f,A)$ представлений $\Omega$\Hyph алгебр}
{tower of representations of algebras}.
}

\DefDefinition{diagram of representations}
{
\AddIndex{Диаграмма $(f,A)$ представлений универсальных алгебр}
{diagram of representations of algebras}
- это такой ориентированный граф, что
\StartLabelItem
\begin{enumerate}
\item
вершина $A_k$, \Kn1, является $\Omega_k$\Hyph алгеброй;
\item
ребро $f_{kl}$ является представлением
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_l$\Hyph алгебре $A_l$;
\end{enumerate}
Мы будем требовать, чтобы этот граф
был связным и не содержал циклов.
Мы будем полагать, что $A_{[0]}$ - это множество начальных вершин графа.
Мы будем полагать, что $A_{[k]}$ - это множество вершин графа,
для которых максимальный путь от начальных вершин равен $k$.
}

\DefRemark{diagram of representations}
{
Так как в разных вершинах графа
может быть одна и таже алгебра,
то мы обозначим
\ShowEq{A=A1n}A{}
множество универсальных алгебр, которые попарно различны.
Из равенства
\ShowEq{A=A(1n)1n}A
следует, что для любого индекса $(i)$
существует по крайней мере один индекс $i$ такой, что
\ShowEq{A(i)=Ai}i.
Если даны два набора множеств
\ShowEq{A=A1n}A,
\ShowEq{A=A1n}B
и определено отображение
\ShowEq{hi:Ai->Bi}
для некоторого индекса $(i)$,
то также определено отображение
\ShowEq{f:A->B}{h_i}{A_i}{B_i}
для любого индекса $i$ такого, что
\ShowEq{A(i)=Ai}i{}
и в этом случае $h_i=h_{(i)}$.
}

\DefTheorem{diagram of representations}
{
{\bf(}\AddIndex{Индукция по диаграмме представлений}{induction over diagram of representations}{\bf)}.
Пусть теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[0]}$
диаграммы $(f,A)$ представлений универсальных алгебр.
Пусть из утверждения, что теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[k]}$
диаграммы $(f,A)$ представлений, следует утверждение,
что теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[k+1]}$
диаграммы $(f,A)$ представлений.
Тогда теорема $\mathcal T$ верна для множества
универсальных алгебр
диаграммы $(f,A)$ представлений.
}

\DefDefinitionNote{commutative diagram of representations}
{
Диаграмма $(f,A)$ представлений универсальных алгебр
называется
\AddIndex{коммутативной}{commutative diagram of representations},
если выполнено следующее условие.
для каждой пары представлений
\ShowEq{f:A->*B}{f_{ik}}{A_i}{A_k}
\ShowEq{f:A->*B}{f_{jk}}{A_j}{A_k}
следующее равенство верно\,\footnotemark
\ShowEq{fik fjk = fjk fik}
}
{
Образно говоря,
представления $f_{ik}$ и $f_{jk}$
прозрачны друг для друга.
}

\DefTheoremNote{diagram of representations, define map fik}
{
Пусть
\ShowEq{f:i->*j}ij
представление $\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре $A_j$.
Пусть
\ShowEq{f:i->*j}jk
представление $\Omega_j$\Hyph алгебры $A_j$
в $\Omega_k$\Hyph алгебре $A_k$.
Мы можем описать фрагмент\,\footnotemark
\DrawEq[ijk]{Ai->*Aj->*Ak}{}
диаграмы представлений с помощью диаграммы
\ShowEq{tower of representations, 1 2 3}
Отображение
\ShowEq{f:A->End 2 3}
определено равенством
\ShowEq{define map f13}
где
\ShowEq{a in A}i,
\ShowEq{a in A}j.
Если представление $f_{jk}$ эффективно
и представление $f_{ij}$ свободно,
то отображение $f_{ijk}$ является свободным представлением
\ShowEq{f:1->*3}
$\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре
\ShowEq{End Ak}Ak.
}
{
Теорема
\RefTheorem{diagram of representations, define map fik}
утверждает, что преобразования в башне представлений согласованы.
}

\DefDefinition{Morphism of Diagram of Representations}
{
Пусть
$(f,A)$
- диаграмма представлений, где
\ShowEq{A=A1n}A{}
- множество универсальных алгебр.
Пусть
$(B,g)$
- диаграмма представлений, где
\ShowEq{A=A1n}B{}
- множество универсальных алгебр.
Множество отображений
\ShowEq{A=A1n}h{}
\ShowEq{hi:Ai->Bi}
называется \AddIndex{морфизмом из диаграммы представлений
$(f,A)$ в диаграмму представлений $(B,g)$}
{morphism from diagram of representations into diagram of representations},
если для любых индексов $(i)$, $(j)$, $i$, $j$ таких, что
\ShowEq{A(i)=Ai}i,
\ShowEq{A(i)=Ai}j,
и для каждого представления
\ShowEq{f:A->*B}{f_{ji}}{A_j}{A_i}
пара отображений $(h_j\ \ h_i)$ является
морфизмом представлений из $f_{ji}$ в $g_{ji}$.
}

\AddEq{remark: Morphism of Diagram of Representations}
{
Для любого представления $f_{ij}$,
\Kn[i]1, \Kn[j]1,
мы имеем диаграмму
\ShowEq{morphism of diagram of representations of F algebra, level k, diagram}
Равенства
\ShowEq{morphism of diagram of representations, level k}
\ShowEq{morphism of diagram of representations, levels k k+1}
выражают коммутативность диаграммы (1).
}

\DefTheorem{reduced polymorphism of representations}
{
Пусть отображение $r_2$ - приведенный полиморфизм
эффективных представлений $f_1$, ..., $f_n$ в эффективное представление $f$.
\begin{itemize}
\item
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, ak}
\item
Для любого
\ShowEq{kl,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, akl}
\item
Пусть $\omega_2\in\Omega_2(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, omega2}
\end{itemize}
}

\AddEq{remark: morphism of representation of Omega group}
{
\begin{remark}
\labelRemark{morphism of \SideWS representation of Omega group}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть отображение
\ShowEq{f:A->*B}g{B_1}{B_2}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений.
Мы будем пользоваться записью
\ShowEq{r2a=r2 o a}
для образа $A_2$\Hyph числа $a_2$
при отображении $r_2$.
Тогда мы можем записать равенство
\eqRef{morphism of representations of universal algebra, 2m}{representation}
следующим образом
\ShowEq{morphism of \SideWS representation of Omega group}
\qed
\end{remark}
}

\DefTheorem{proper definition of orbit}
{
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$.
Если
\ShowEq{orbit, proposition}
то
\ShowEq{A1a2=A1b2}
}

\AddEq{definition: orbit of representation}
{
\begin{ShadedDefinition}
\labelDefinition{orbit of \SideNS-side representation}
Пусть $A_1$ является $\Omega$\Hyph группоидом с произведением
\ShowEq{(ab)->ab}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является \SideRu восторонним представлением
$\Omega$\Hyph группоида $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Для любого
\ShowEq{a in A}2,
мы определим
\AddIndex{орбиту представления}{orbit of representation}
$\Omega$\Hyph группоида $A_1$ как множество
\ShowEq{orbit of \SideNS-side representation}
\end{ShadedDefinition}
}

\AddEq{Let A->*AB2 be representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
}

\AddEq{Let XY be generating sets}
{
Пусть $X$ - множество образующих представления
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $Y$ - множество образующих представления
\ShowEq{f:A->*B}g{A_1}{B_2}
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
}

\DefDefinitionNote{product in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{product in category}
и множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
называется
\AddIndex{произведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{product in category}\,\footnotemark,
если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}gR{B_i}
существует единственный морфизм
\ShowEq{f:A->B}hRP
такой, что диаграмма
\ShowEq{product in category diagram}
коммутативна для всех $i\in I$.

Если $|I|=n$, то для произведения множества объектов
$\{B_i,\iI\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product in category, 1 n}
}
{
Определение дано согласно \citeBib{Serge Lang},
страница 45.
}

\DefExample{Cartesian product of sets}
{
Пусть \(\mathcal S\) - категория множеств.\,\footnote{Смотри
также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\ShowEq{ref product in category}
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}A{}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
}

\DefTheorem{product of effective representations}
{
В категории
\ShowEq{A1(mA2)}
существует произведение
эффективных представлений $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре
и это произведение является
эффективным представлением $\Omega_1$\Hyph алгебры $A_1$.
}

\DefTheoremNote{structure of subrepresentations}
{
Пусть\,\footnotemark
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $X\subset A_2$.
Определим подмножество $X_k\subset A_2$ индукцией по $k$.
\ShowEq{structure of subrepresentations}
Тогда
\ShowEq{structure of subrepresentations, 1}
}{
Утверждение теоремы аналогично
утверждению теоремы 5.1, \citeBib{Cohn: Universal Algebra}, страница 94.
}

\DefDefinitionNote{direct sum of Abelian groups}
{
Копроизведение в категории абелевых групп $Ab$ называется
\AddIndex{прямой суммой}{direct sum}.\,\footnotemark
Мы будем пользоваться записью
\ShowEq{direct sum of Abelian groups}
для прямой суммы абелевых групп $A$ и $B$.
}{Определение дано согласно \citeBib{Serge Lang}, страница 55.}

\DefDefinitionNote{coproduct in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Пусть
\ShowEq{category A[Bi]}
- категория,
объектами которой являются кортежи $(P,f)$,
где $P$ - объект категории $\mathcal A$
и $f$ - множество морфизмов
\ShowEq{set f:A->B}f{B_i}P
Универсально отталкивающий объект категории
\ShowEq{category A[Bi]}
\ShowEq{coproduct in category}
называется
\AddIndex{копроизведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{coproduct in category}.\,\footnotemark

Если $|I|=n$, то для копроизведения множества объектов
\ShowEq{set Bi}B
в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{coproduct in category, 1 n}
}
{
Определение дано согласно определению на странице
\citeBib{Serge Lang}\Hyph 46.
}

\AddEq{definition: free Abelian group}
{
\begin{ShadedDefinition}
\labelDefinition{free Abelian group}
Пусть $S$ - множество и\,\footnotemark
\ShowEq{category AbS}
- категория, объектами которой являются отображения
\ShowEq{f:A->B}fSG
множества $S$ в абелевые группы.
Если
\ShowEq{f:A->B}fSG
\ShowEq{f:A->B}{f'}S{G'}
объекты категории
\ShowEq{category AbS},
то морфизм из $f$ в $f'$
- это гомоморфизм групп
\ShowEq{f:A->B}gG{G'}
такой, что диаграмма
\DrawEq{AbS ff'g}{}
коммутативна.
\end{ShadedDefinition}
\footnotetext{\,
Смотри также определение в \citeBib{Serge Lang}, страницы 56, 57.
}
}

\AddEq{theorem: free Abelian group}
{
\begin{ShadedTheorem}
\labelTheorem{free Abelian group}
Универсально отталкивающий объект $G$ категории
\ShowEq{category AbS}
существует.\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{S in G}
\item
Множество $S$ порождает абелевую группу $G$.
\labelItem{set generates Abelian group}
\end{enumerate}
Абелевая группа $G$ называется
\AddIndex{свободной абелевой группой}{free Abelian group},
порождённой множеством $S$.
\end{ShadedTheorem}
\footnotetext{\,
Смотри аналогичное утверждение в \citeBib{Serge Lang}, страница 57.
}
}

\DefProof{free Abelian group}
{
Пусть $G$
- множество отображений
\ShowEq{f:A->B}hSZ
таких, что множество
\ShowEq{x in -> h(x)}
конечно.

\begin{ShadedLemma}
{\it
Множество $G$ является абелевой группой.
}
\end{ShadedLemma}
{\sc Доказательство.}
Пусть
\ShowEq{h12 in G}
Согласно определению, множества
\ShowEq{H12=}
конечны.
Тогда конечно множество
\ShowEq{H1vH2}
Следовательно,
\ShowEq{h1+h2 in G}
Свойства абелевой группы очевидны.
\hfill\(\odot\)

Пусть $k\in Z$, $x\in S$.
Обозначим через $k*x$ отображение $h$, определённое равенством
\ShowEq{k*x=k}
Отображение
\ShowEq{f:S->G}
инъективно и позволяет отождествить $S$ и образ $f(S)\subseteq G$
(утверждение
\RefItem{S in G})
и пользоваться записью
\ShowEq{kx=k*x}
Согласно определению множества $G$,
любое отображение $h\in G$ может быть записано в виде
\ShowEq{h=k*x}
где
\ShowEq{k in Z x in S}
и множество
\ShowEq{|kx ne 0|}
конечно.
Утверждение
\RefItem{set generates Abelian group}
является следствием теоремы
\RefTheorem{structure of Abelian group}.

\begin{ShadedLemma}
{\it
Представление
\EqRef{h=k*x}
отображения $h$ единственно.
}
\end{ShadedLemma}
{\sc Доказательство.}
Если отображение $h$ допускает представления
\ShowEq{h=k12*x i}
то равенство
\ShowEq{k1-k2 *x}
является следствием равенства
\EqRef{h=k12*x i}.
\ShowEq{k1=k2 i}
следует из равенства
\EqRef{k1-k2 *x}.
\hfill\(\odot\)

Пусть
\ShowEq{f:A->B}{f'}S{G'}
отображение множества $S$ в абелевую группу $G'$.
Мы определим гомоморфизм
\ShowEq{f:A->B}gG{G'}
таким образом, чтобы диаграмма
\DrawEq{AbS ff'g}{1}
была коммутативной.
Из диаграммы
\eqRef{AbS ff'g}{1}
следует, что
\ShowEq{g(1x)=f'(x)}
Согласно теореме
\RefTheorem{homomorphism f(na)=nf(a)},
так как отображение $g$ - гомоморфизм абелевой группы, то равенство
\ShowEq{g(x)=}
для любого отображения $h\in G$
является следствием равенств
\EqRef{g(1x)=f'(x)},
\EqRef{h=k*x}.
Следовательно, гомоморфизм $g$ определён однозначно.
Согласно определениям
\RefDefinition{universally repelling object of category},
\RefDefinition{free Abelian group},
абелевая группа $G$ является свободной группой.
}

\DefTheorem{homomorphism f(na)=nf(a)}
{
Гомоморфизм
\ShowEq{f:A->B}fG{G'}
удовлетворяет равенству
\ShowEq{f(na)=nf(a)}
}

\DefTheoremNote{coproduct in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{coproduct in category}
и множество морфизмов
\ShowEq{set f:A->B}f{B_i}P
называется
\AddIndex{копроизведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{coproduct in category},\,\footnotemark
если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}g{B_i}R
существует единственный морфизм
\ShowEq{f:A->B}hPR
такой, что диаграмма
\ShowEq{coproduct in category diagram}
коммутативна для всех $i\in I$.
}{Определение дано согласно \citeBib{Serge Lang}, страница 46.}

\DefProof{coproduct in category}
{
Теорема является следствием определений
\RefDefinition{universally repelling object of category},
\RefDefinition{coproduct in category}.
}

\DefTheoremNote{direct sum of Abelian groups}
{
Пусть
\ShowEq{set Bi}A
- семейство абелевых групп.
Пусть
\ShowEq{A in xAi}
такое множество, что
\ShowEq{(xi)in A},
если
$x_i\ne 0$
для конечного числа индексов $i$.
Тогда\,\footnotemark
\ShowEq{A=o+Ai}A
}{Смотри также предложение \citeBib{Serge Lang}-10, страница 55.}

\DefProof{direct sum of Abelian groups}
{
Согласно теореме
\RefTheorem[\RefRepresentation]{product exists in category of Omega algebras},
существует абелевая группа $B=\prod A_i$.
Согласно утверждению
\RefItem[\RefRepresentation]{tuple represent A number},
мы можем представить $B$\Hyph число $a$ в виде кортежа
\ShowEq{set Bi}a
$A_i$\Hyph чисел.
Согласно утверждению
\RefItem[\RefRepresentation]{operation is defined componentwise},
сумма в группе $B$ определена равенством
\ShowEq{(ai)+(bi)=(ai+bi)}

Согласно построению
$A$ является подгруппой абелевой группы $B$.
Отображение
\ShowEq{f:A->B}{\lambda_j}{A_j}A
определённое равенством
\ShowEq{lj(x)=0x0}
является инъективным гомоморфизмом.

Пусть
\ShowEq{set f:A->B}f{A_i}B
семейство гомоморфизмов в абелевую группу $B$.
Мы определим отображение
\ShowEq{f:A->B}fAB
пользуясь равенством
\DrawEq{fxi,i=sum fxi}{group}
Сумма в правой части равенства
\eqRef{fxi,i=sum fxi}{group}
конечна, так как все слагаемые, кроме конечного числа, равна $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\eqRef{fxi,i=sum fxi}{group}
следует, что
\ShowEq{f(x+y)i=}
Следовательно, отображение $f$ является гомоморфизмом абелевой группы.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\EqRef{lj(x)=0x0},
\eqRef{fxi,i=sum fxi}{group}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\RefDefinition{direct sum of Abelian groups}.
}

\AddEq{remark: Non-commutative Sum}
{
С детства мы знаем, что от перестановки мест слагаемых сумма не меняется.
Поэтому, когда услышал о некоммутативном сложении
(\citeBib{Alain Connes 1994}),
я слегка растерялся.
Однако мне недавно повезло встретить геометрию, где сумма векторов некоммутативна.

В школе я увлекался многими вещами: физикой, химией, черчением.
Математика была немного в стороне.
Я не любил арифметику, но мне нравились алгебра и геометрия.
Я тогда ещё не знал, что все пути ведут в математику.

Черчение было моим любим предметом. Мой учитель,
Габис Сергей Александрович, подарил мне сборник задач по черчению,
и я добросовестно все их перерешал.
А потом придумал свою собственную задачу и решил её.
К моему удивлению, первая теорема, которую мы доказывали на
уроке геометрии на следующий год, была именно решением этой задачи.

Я понимал, что после школы мне будет сложно поступить в институт.
Поэтому после восьмого класса я решил что я буду поступать в техникум.
Бела Марковна предложила позаниматься со мной летом,
посмотреть насколько я готов к экзамену по математике.
Один из уроков остался в моей памяти.
Когда мы рассматривали графики прямой и параболы,
Бела Марковна сказала: нарисовать прямую или параболу легко,
а как быть с кардиограммой?
И я загорелся идеей найти аналитическое выражение 
для кардиограммы.

Мой товарищ предложил мне на протяжении лета
вместе изучать математический анализ.
В нашем доме жили мальчики, которые учились в техникуме,
и они одолжили мне свой учебник по математическому анализу.
К этому времени мой товарищ потерял интерес к своей идее,
и я стал изучать математический анализ самостоятельно.

Первая глава учебника была посвящена аналитической геометрии.
И я понял, что это то что мне нужно для анализа кривых кардиограммы.
Аналитическая геометрия решила моё будущее.
Я понял, что буду готовиться в университет на механико-математический факультет.

Я перечитал много книг по математическому анализу.
Но в какой-то момент у меня сложилось впечатление
что один автор списывает у другого.
Я стал искать другие книги.
Не помню откуда у меня появился первый том Фихтенгольца.
Но эта книга произвела на меня неизгладимое впечатление.
Ближе к весне я почувствовал, что книга становится трудной,
но продолжал читать.
В марте у меня был грипп с необычайно высокой температурой.
Но я сомневаюсь, что это был грипп,
так как после этого первый том Фихтенгольца стал для меня понятен.

Изучение математического анализа отразилось
на моих попытках восстановить функциональную
зависимость с графика. Я тогда ещё не понимал,
что не всякое отображение может быть представлено аналитически.
Я рисовал графики, составлял таблицы приращения функции
в зависимости от приращения аргумента.
Но вскоре эта затея мне надоела,
и я сменил занятие.

Когда мне в руки попала книга по тензорному исчислению,
я обнаружил, что сложные построения аналитической геометрии
по классификации кривых второго порядка
можно заменить простыми теоремами линейной алгебры.
После этого, мой интерес к аналитической геометрии
заметно стал меньше.

Прошло почти полвека.
И неожиданно аналитическая геометрия преподнесла мне
два приятных сюрприза.
Сперва я обнаружил, что аналитическая геометрия
является интересной структурой с точки зрения
теории представлений универсальных алгебр.
Точнее, я отождествляю аналитическую и аффинную геометрии,
но я думаю, что это небольшая ошибка.

Второй сюрприз связан с тем, что я понял,
что я могу построить модель аффинной геометрии
в римановом пространстве.
Так как я очень долго занимался метрико\Hyph аффинными многообразиями,
то оставался один шаг, чтобы увидеть модель аффинной геометрии,
где сумма некоммутативна.
С этого момента некоммутативное сложение перестало быть для меня
абстрактной концепцией.
}

\DefText{side representation of group}
{
Из равенства
\eqRef{* \SideNS-side representation of group}{def}
следует, что
\DrawEq{o \SideNS-side representation of group}{def}
Мы можем рассматривать равенство
\eqRef{o \SideNS-side representation of group}{def}
как
\AddIndex{закон ассоциативности}{associative law},

\begin{sloppypar}
\begin{example}
Пусть
\ShowEq{f:A->B}f{A_2}{A_2}
\ShowEq{f:A->B}g{A_2}{A_2}
эндоморфизмы $\Omega_2$\Hyph алгебры $A_2$.
Пусть произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
является композицией эндоморфизмов.
Так как произведение отображений $f$ и $g$ определено в том же порядке,
как эти отображения действуют на $A_2$\Hyph число,
то мы можем рассматривать равенство
\ShowEq{fga= o \SideNS}
как
закон ассоциативности,
который позволяет записывать равенство
\EqRef{fga= o \SideNS}
без использования скобок
\ShowEq{fga= 1 \SideNS}
а также записать равенство
\eqRef{\SideNS-side representation of group}{def}
в виде
\DrawEq{\SideNS-side 1 representation of group}{def}
\qed
\end{example}
\end{sloppypar}
}

\AddEq[4]{theorem: select second basis of representation}
{
\begin{ShadedTheorem}
\labelTheorem{select second basis of representation, #4}
Пусть $#2$ - пассивное преобразование
многообразия базисов #3 $#4$.
Пусть $\Basis e_1$ - базис #3 $#4$,
\ShowEq{e2=e1 o S}{#2}21
Пусть для базиса $\Basis e_3$ существует активное преобразование $#1$ такое, что
\ShowEq{e3=R o e1}{#1}31
Положим
\ShowEq{e3=R o e1}{#1}42
Тогда
\ShowEq{e2=e1 o S}{#2}43
\end{ShadedTheorem}
}

\AddEq[3]{proof: select second basis of representation}
{
\begin{proof}
Согласно равенству
\eqRef{active transformation}{#3},
активное преобразование координат базиса $\Basis e_3$ имеет вид
\DrawEq{active transformation, 1}{#3}
Пусть
\ShowEq{e2=e1 o S}{#2}53
Из равенства
\eqRef{passive transformation}{#3}
следует, что
\DrawEq{passive transformation, 1}{#3}
Из совпадения выражений в равенствах
\eqRef{active transformation, 1}{#3},
\eqRef{passive transformation, 1}{#3}
следует, что
\ShowEq{Basis e4=Basis e5}
Следовательно,
коммутативна диаграмма
\ShowEq{passive and active maps}{#1}{#2}
\end{proof}
}

\AddEq[2]{definition: basis manifold}
{
Множество
\ShowEq{basis manifold}
базисов #1 $#2$ называется
\AddIndex{многообразием базисов}{basis manifold}
#1 $#2$.
}

\AddEq{ref active representation, representation}
{
Согласно теоремам
\RefTheorem{superposition of coordinates, representation},
\RefTheorem{Automorphism of representation maps a basis into basis},
}

\AddEq{ref active representation, diagram of representations}
{
Согласно теореме
\RefTheorem{Automorphism of diagram of representations maps a basis into basis}
и определению
\RefDefinition{superposition of coordinates and words, diagram of representations},
}

\AddEq[4]{definition: active representation in basis manifold}
{
\begin{ShadedDefinition}
\labelDefinition{active representation in basis manifold, #1}
\ShowEq{ref active representation, #1}
автоморфизм $#4$ #2 $#3$
порождает преобразование
\DrawEq[{#4}]{active transformation}{#1}
многообразия базисов #2.
Это преобразование называется
\AddIndex{активным}{active transformation of basis}.
Согласно теореме
\RefTheorem{group of automorphisms of #1},
определено левостороннее представление
\ShowEq{active representation in basis manifold}
\ShowEq{active representation in basis manifold def}
группы $GA(f)$
в многообразии базисов $\mathcal B[f]$.
Представление $A(f)$ называется
\AddIndex{активным представлением}{active representation in basis manifold}.
Согласно следствию
\RefCorollary{automorphism uniquely defined by image of basis, #1},
это представление однотранзитивно.
\qed
\end{ShadedDefinition}
}

\AddEq[4]{remark: active representation}
{
\begin{remark}
\labelRemark{active representation, #1}
Согласно замечанию
\RefRemark{X is quasibasis of #1},
могут существовать базисы #2 $#3$,
не связанные активным преобразованием.
В этом случае мы в качестве многообразия базисов будем рассматривать
орбиту выбранного базиса.
Следовательно, #4 $#3$ может иметь различные многообразия базисов.
Мы будем предполагать, что мы выбрали многообразие базисов.
\end{remark}
}

\AddEq[6]{theorem: Coordinate transformation does not depend}
{
\begin{ShadedTheorem}
\labelTheorem{Coordinate transformation does not depend, #1}
Допустим пассивное преобразование $#2\in GA(f)$ отображает
базис $\Basis e_1\in\mathcal{B}[f]$
в базис $\Basis e_2\in\mathcal{B}[f]$
\DrawEq[{#2}]{passive transformation S}{#1}
Допустим #6 $#3$ имеет #5
\DrawEq[1{#3}]{Omega_2 word, basis e}{1 #1}
относительно базиса $\Basis e_1$ и имеет #5
\DrawEq[2{#3}]{Omega_2 word, basis e}{2 #1}
относительно базиса $\Basis e_2$.
Преобразование координат
\DrawEq[{#3}{#2}]{coordinate transformation}{#1}
не зависит от #4 $#3$ или базиса $\Basis e_1$, а
определенно исключительно координатами #4 $#3$
относительно базиса $\Basis e_1$.
\end{ShadedTheorem}
}

\AddEq[3]{proof: Coordinate transformation does not depend}
{
\begin{proof}
Из \eqRef{passive transformation S}{#1}
и
\eqRef{Omega_2 word, basis e}{2 #1}
следует, что
\DrawEq[{#2}{#3}]{Omega word in representation, basis Y, 1}{#1}
Сравнивая \eqRef{Omega_2 word, basis e}{1 #1}
и
\eqRef{Omega word in representation, basis Y, 1}{#1}
получаем, что
\DrawEq[{#2}{#3}]{coordinate transformation in representation, 1}{#1}
Так как $#2$ - автоморфизм представления, то равенство
\eqRef{coordinate transformation}{#1}
следует из
\eqRef{coordinate transformation in representation, 1}{#1}
и теоремы
\RefTheorem{coordinates of inverse transformation, #1}.
\end{proof}
}

\AddEq[3]{remark: active and passive transformation}
{
Активное преобразование изменяет базис #1 и
#2 согласовано
и координаты #3 относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к изменению
координат #3 относительно базиса.
}

\AddEq[2]{theorem: Coordinate transformations form right-side representation}
{
\begin{ShadedTheorem}
\labelTheorem{Coordinate transformations form right-side representation, #1}
Преобразования координат
\eqRef{coordinate transformation}{#1}
порождают эффективное контравариантное
правостороннее представление группы $GA(f)$, называемое
\AddIndex{координатным представлением}{coordinate representation}
в #2.
\end{ShadedTheorem}
}

\AddEq[8]{proof: Coordinate transformations form right-side representation}
{
\begin{proof}
Согласно следствию
\RefCorollary{map of coordinates of #1},
преобразование
\eqRef{coordinate transformation}{#1}
является эндоморфизмом #4\,\footnote{Это преобразование
не порождает эндоморфизма #4 $#6$. Координаты меняются, поскольку меняется
базис, относительно которого мы определяем координаты. Однако
#7, координаты которого мы рассматриваем, не меняется.}
#5

Допустим мы имеем два последовательных пассивных преобразования
$#2$ и $#8$. Преобразование координат
\DrawEq[{#3}{#2}]{coordinate transformation}{#2 #1}
соответствует пассивному преобразованию $#2$.
Преобразование координат
\DrawEq[{#3}{#8}]{coordinate transformation}{#8 #1}
соответствует пассивному преобразованию $#8$.
Согласно теореме
\RefTheorem{passive representation in basis manifold, #1},
произведение преобразований координат
\eqRef{coordinate transformation}{#2 #1}
и
\eqRef{coordinate transformation}{#8 #1}
имеет вид
\ShowEq{coordinate transformation in representation, TS}{#3}{#2}{#8}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\ShowEq{coordinate transformation in representation, TS 1}{#8}{#2}
Согласно теоремам
\RefTheorem{coordinates of inverse transformation, #1},
\RefTheorem{coordinates of product of inverse transformation, #1}
и определению
\RefDefinition{Left side contravariant representation}
преобразования координат
порождают
правостороннее контравариантное представление группы $GA(f)$.

Если координатное преобразование не изменяет координаты выбранного базиса,
то ему соответствует единица группы $GA(f)$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
\end{proof}
}

\AddEq[5]{remark: geometric object}
{
Пассивное представление $P(g)$ согласовано
с пассивным представлением $P(f)$,
если существует гомоморфизм $h$ группы $GA(f)$ в группу $GA(g)$.
Рассмотрим диаграмму
\ShowEq{passive representation coordinated with passive representation}
Так как отображения $P(f)$, $P(g)$ являются изоморфизмами группы,
то отображение $H$ является гомоморфизмом групп.
Следовательно, отображение $f'$ является представлением группы $GA(f)$
в многообразии базисов $\mathcal B(g)$.
Согласно построению, пассивному преобразованию $#2$ многообразии базисов $\mathcal B(f)$
соответствует пассивное преобразование $H(#2)$ многообразия базисов $\mathcal B(g)$
\DrawEq[{#2}]{passive transformation of representation g}{#1}
Тогда координатное преобразование в #3 $#4$ принимает вид
\DrawEq[{#5}{#2}]{coordinate transformation g}{#1}
}

\AddEq[5]{definition: coordinate of geometric object}
{
\begin{ShadedDefinition}
\labelDefinition{coordinate of geometric object, #1}
Мы будем называть
орбиту
\ShowEq{coordinates of geometric object}{#3}%
\ShowEq{show coordinates of geometric object}{#2}{#3}
\AddIndex{координатами геометрического объекта}{coordinates of geometric object},
определёнными в #4 $#5$.
Для любого базиса
\ShowEq{geometric object 1}{#2}
соответствующая точка
\eqRef{coordinate transformation g}{#1}
орбиты  определяет
\AddIndex{координаты геометрического объекта}{coordinates of geometric object}
относительно базиса
\ShowEq{geometric object 2}
\qed
\end{ShadedDefinition}
}

\AddEq[1]{remark: 2 views on geometric object}
{
Так как геометрический объект - это орбита представления,
то согласно теореме
\RefTheorem{proper definition of orbit}
определение геометрического объекта корректно.

Определение
\RefDefinition{coordinate of geometric object, #1}
строит геометрический объект в координатном пространстве.
Определение \RefDefinition{geometric object, #1} предполагает,
что мы выбрали базис представления $g$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.
}

\AddEq[7]{definition: geometric object}
{
\begin{ShadedDefinition}
\labelDefinition{geometric object, #1}
Мы будем называть
орбиту
\ShowEq{geometric object}{#3}%
\ShowEq{show geometric object}{#2}{#3}%
\AddIndex{геометрическим объектом}{geometric object},
определённым в #4 $#5$.
Мы будем также говорить, что $#3$ - это
\AddIndex{геометрический объект типа $H$}{type of geometric object}.
Для любого базиса
\ShowEq{geometric object 1}{#2}
соответствующая точка 
\eqRef{coordinate transformation g}{#1}
орбиты  определяет #6
\ShowEq{geometric object 2, g}{#3}%
#7 мы называем
\AddIndex{представителем геометрического объекта}{representative of geometric object}
в #4 $#5$.
\qed
\end{ShadedDefinition}
}

\AddEq[1]{theorem: invariance principle}
{
\begin{ShadedTheorem}[принцип инвариантности]
\AddIndex{}{invariance principle}
\labelTheorem{invariance principle, #1}
Представитель геометрического объекта не зависит от выбора
базиса $\Basis e_f$.
\end{ShadedTheorem}
}

\AddEq[6]{proof: invariance principle}
{
\begin{proof}
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Basis e_f$ #2 $#3$,
базис $\Basis e_g$ #2 $#4$
и координаты геометрического объекта
\ShowEq{invariance principle 4}{#5}
Соответствующий представитель геометрического
объекта имеет вид
\ShowEq{invariance principle 1}{#5}
Базис $\Basis e_{f1}$ связан с базисом
$\Basis e_f$ пассивным преобразованием
\ShowEq{invariance principle 2 passive}{#6}
Согласно построению это порождает пассивное преобразование
\eqRef{passive transformation of representation g}{#1}
и координатное преобразование
\eqRef{coordinate transformation g}{#1}.
Соответствующий
представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3 algebra}{#5}{#6}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
\end{proof}
}

\AddEq[1]{theorem: passive representation in basis manifold}
{
\begin{ShadedTheorem}
\labelTheorem{passive representation in basis manifold, #1}
Существует однотранзитивное правостороннее представление
\ShowEq{passive representation in basis manifold}
\ShowEq{passive representation in basis manifold def}
группы $GA(f)$
в многообразии базисов $\mathcal B[f]$.
Представление $P(f)$ называется
\AddIndex{пассивным представлением}{passive representation in basis manifold}.
\end{ShadedTheorem}
}

\DefProof{passive representation in basis manifold}
{
Поскольку $A(f)$ - однотранзитивное левостороннее представление группы $GA(f)$,
то однотранзитивное правостороннее представление $P(f)$
определено однозначно
согласно теореме
\RefTheorem{two representations of group}.
}

\AddEq[1]{theorem: passive transformation is automorphism of A(f)}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation is automorphism of A(f), #1}
Пассивное преобразование многообразия базисов
является автоморфизмом представления $A(f)$.
\end{ShadedTheorem}
}

\DefProof{passive transformation is automorphism of A(f)}
{
Теорема является следствием теоремы
\RefTheorem{twin representations of group, automorphism}.
}

\AddEq[3]{theorem: passive transformation}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation, #1}
Преобразование представления $P(f)$
называется
\AddIndex{пассивным преобразованием многообразия базисов}
{passive transformation of basis}
#2.
Мы будем пользоваться записью
\ShowEq{passive transformation of basis}{#3}
\ShowEq{passive transformation of basis def}{#3}
для обозначения образа базиса $\Basis e$ при пассивном преобразовании $#3$.
Пассивное преобразование базиса имеет вид
\DrawEq[#3]{passive transformation}{#1}
\end{ShadedTheorem}
}

\AddEq[1]{proof: passive transformation}
{
\begin{proof}
Согласно равенству
\eqRef{active transformation}{#1},
активное преобразование действует на координаты
базиса слева.
Равенство
\eqRef{passive transformation}{diagram of representations}
следует из теорем
\RefTheorem{shift is automorphism of representation},
\RefTheorem{two representations of group},
\RefTheorem{twin representations of group, automorphism},
согласно которым
пассивное преобразование действует на координаты
базиса справа.
\end{proof}
}

\DefLabeledDefinitionNote{side representation of group}{\SideNS}
{
Пусть
\ShowEq{End O2}{A_2}{}
- мультипликативная $\Omega$\Hyph группа с произведением\,\footnotemark
\ShowEq{(fg)->fg}
Пусть эндоморфизм $f$ действует на $A_2$\Hyph число $a$ с\SideRu ва.
Мы будем пользоваться записью
\ShowEq{f(a)=o \SideNS}
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа с произведением
\ShowEq{(ab)->ab}
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{\SideNS-side}
\AddIndex{\SideRu восторонним представлением}{\SideNS-side representation}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{\SideRu восторонним $A_1$\Hyph представлением}{\SideNS-side A representation}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{\SideNS-side representation of group}{def}
Мы будем отождествлять
$A_1$\Hyph число $a_1$ с его образом $f(a_1)$
и записывать \SideRu востороннее преобразование,
порождённое $A_1$\Hyph числом $a_1$,
в форме
\ShowEq{\SideNS-side representation}
В этом случае равенство
\eqRef{\SideNS-side representation of group}{def}
принимает вид
\DrawEq{* \SideNS-side representation of group}{def}
Отображение
\ShowEq{A12->A2 1 \SideNS}
порождённое \SideRu восторонним представлением $f$, называется
\AddIndex{\SideRu восторонним произведением}{\SideNS-side product}
$A_2$\Hyph числа $a_2$ на $A_1$\Hyph число $a_1$.
}
{
Очень часто произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
совпадает с суперпозицией эндоморфизмов
\ShowEq{Act=circ}
Однако произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
может отличаться от суперпозиции эндоморфизмов.
}

\DefDefinition{reduced morphism of representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть
\ShowEq{id:A1->A1 A2->B2}
морфизм представлений.
В этом случае мы можем отождествить морфизм
\ShowEq{map r,R}{\id}{r_2}{}
представлений $\Omega_1$\Hyph алгебры и соответствующий гомоморфизм $r_2$ $\Omega_2$\Hyph алгебры
и будем называть гомоморфизм $r_2$
\AddIndex{приведенным морфизмом представлений}
{reduced morphism of representations}.
Мы будем пользоваться диаграммой
\ShowEq{morphism id,R of representations}
для представления приведенного морфизма $r_2$ представлений
$\Omega_1$\Hyph алгебры.
Из диаграммы следует
\ShowEq{morphism of representations of universal algebra}
Мы будем также пользоваться диаграммой
\ShowEq{morphism id,R of representations 2}
вместо диаграммы
\EqRef{morphism id,R of representations}.
}

\DefDefinition{action of rational integers in Abelian group}
{
Мы определим действие кольца целых чисел $Z$
в абелевой группе $G$
согласно правилу
\ShowEq{action of rational integers in Abelian group}
}

\DefTheorem{action of ring of rational integers in Abelian group}
{
Действие кольца целых чисел $Z$
в абелевой группе $G$,
рассмотренное в определении
\RefDefinition{action of rational integers in Abelian group},
является представлением.
Верны следующие равенства
\ShowEq{representation of Z in G}
}

\DefProof{action of ring of rational integers in Abelian group}
{
Равенство
\EqRef{1a=a}
является следствием равенства
\EqRef{0g=0}
и равенства
\EqRef{(n+1)g=},
когда $n=0$.

\ShowEq{step of proof: action in Abelian group}{(m+n)a=ma+na}

Равенство
\ShowEq{(k+n)a-na=ka}
является следствием равенства
\EqRef{(m+n)a=ma+na}.
Равенство
\EqRef{(m-n)a=ma-na}
является следствием равенства
\EqRef{(k+n)a-na=ka},
если мы положим
$m=k+n$, $k=m-n$.

\ShowEq{step of proof: action in Abelian group}{(nm)a=n(ma)}

\ShowEq{step of proof: action in Abelian group}{n(a+b)=na+nb}

Из равенства
\EqRef{n(a+b)=na+nb}
следует, что отображение
\ShowEq{phi(n):G->G}
является эндоморфизмом абелевой группы $G$.
Из равенств
\EqRef{(m+n)a=ma+na},
\EqRef{(nm)a=n(ma)}
следует, что отображение
\ShowEq{phi:Z->End(G)}
является гомоморфизмом кольца $Z$.
Согласно определению
\RefDefinition[\RefRepresentation]{representation of algebra},
отображение $\varphi$ является представлением
кольца целых чисел $Z$
в абелевой группе $G$.
}

\DefDefinitionNote{tensor product of representations}
{
Пусть $A$ является абелевой мультипликативной $\Omega_1$\Hyph группой.
Пусть
\ShowEq{a1n}An{}
- $\Omega_2$\Hyph алгебры.\,\footnotemark
Пусть для любого
\ShowEq{k,1n}
\ShowEq{representation A Ak 1}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $A_k$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
приведенные полиморфизмы представлений $f_1$, ..., $f_n$
\ShowEq{polymorphisms category}
где $S_1$, $S_2$ - $\Omega_2$\Hyph алгебры и
\ShowEq{representation of algebra in S1 S2}
эффективные представления мультипликативной $\Omega_1$\Hyph группы $A$.
Мы определим морфизм
\ShowEq{r1->r2}
как приведенный морфизм представлений $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{polymorphisms category, diagram}
Универсальный объект
\ShowEq{tensor product of representations}
категории $\mathcal A$ называется
\AddIndex{тензорным произведением}{tensor product}
представлений
\ShowEq{a1n}An.
}
{
Я определяю
тензорное произведение представлений универсальной алгебры
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{tensor product of representations}
Если существует полиморфизм представлений,
то тензорное произведение представлений существует.
\end{ShadedTheorem}
}
{theorem: tensor product of representations}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation, tensor product}
Пусть
\ShowEq{equivalence, 1, representation, tensor product}
Тензорное произведение дистрибутивно относительно операции $\omega$
\ShowEq{tensors 1, representation, tensor product}
Представление мультипликативной $\Omega_1$\Hyph группы $A$
в тензорном произведении определено равенством
\ShowEq{tensors 2, representation, tensor product}
\end{ShadedTheorem}
}
{theorem: representation, tensor product}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{tensor product and polymorphism}
Пусть $B_1$, ..., $B_n$ -
$\Omega_2$\Hyph алгебры.
Пусть
\ShowEq{map f, 1, representation, tensor product}
приведенный полиморфизм, определённый равенством
\ShowEq{map f, representation, tensor product}
Пусть
\ShowEq{map g, representation, tensor product}
приведенный полиморфизм в $\Omega_2$\Hyph алгебру $V$.
Существует морфизм представлений
\ShowEq{map h, representation, tensor product}
такой, что диаграмма
\ShowEq{map gh, representation, tensor product}
коммутативна.
\end{ShadedTheorem}
}
{theorem: tensor product and polymorphism}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{B times->B otimes}
Отображение
\ShowEq{B times->B otimes}
является полиморфизмом.
\end{ShadedTheorem}
}
{theorem: B times->B otimes}
%DefEq

\DefTheorem{|a-b|>|a|-|b|}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Тогда
\ShowEq{|a-b|>|a|-|b|}
}

\DefDefinitionNote{free representation of algebra}
{
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnotemark
если из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что
\ShowEq{a=b}.
}
{
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
Смотри также теорему
\RefTheorem{free representation of group}.
\fi
}

\DefDefinition{continuous map, Omega group}
{
Отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{|x'-x|<delta}
влечёт
\ShowEq{|f(x)-f(x')|<epsilon}
}

\DefTheorem{continuous map, open set}
{
Отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
непрерывно тогда и только тогда, когда
прообраз открытого множества
является открытым множеством.
}

\DefTheorem{image of interval is interval, real field}
{
Пусть
\ShowEq{f:A->B}fRR
непрерывное отображение поля действительных чисел.
Тогда образ интервала является интервалом.
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{norm of operation}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$, величина
\ShowEq{norm of operation}
\ShowEq{norm of operation, definition}
называется
\AddIndex{нормой операции}{norm of operation} $\omega$.
\qed
\end{ShadedDefinition}
}
{definition: norm of operation}
%\DefEq

\DefTheorem{|fx|<|f||x|1n}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$,
\ShowEq{|a omega|<|omega||a|1n}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{norm of representation}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление\
\ePrints{1305.4547}
\ifx\Semafor\ValueOn
\footnote{
Смотри определение
\ShowEq{ref definition: left-side representation of algebra}{}
представления универсальной алгебры.
Согласно определению
\xRef[1211.6965]{definition: module over ring},
модуль - это представление кольца в абелевой группе.
Так как кольцо и абелева группа являются $\Omega$\Hyph группами,
то модуль - это представление $\Omega$\Hyph группы.
}
\fi
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Величина
\ShowEq{norm of representation}
\ShowEq{norm of representation, definition}
называется
\AddIndex{нормой представления}{norm of representation} $f$.
\qed
\end{ShadedDefinition}
}
{definition: norm of representation}
%\DefEq

\DefTheorem{|fab|<|f||a||b|}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Тогда
\ShowEq{|fab|<|f||a||b|}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{open set}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Множество
$U\subset A$
называется
\AddIndex{открытым}{open set},\,\footnote{
В топологии
обычно сперва определяют открытое множество,
а затем базу топологии.
В случае метрического или нормированного пространства,
удобнее дать определение открытого множества,
опираясь на определение базы топологии.
В этом случае определение основано на одном из свойств
базы топологии. Непосредственная проверка
позволяет убедиться, что определённое таким образом
открытое множество удовлетворяет основным свойствам.
}
если для любого $A$\Hyph числа
\ShowEq{a in U}{}
существует
\ShowEq{epsilon in R}
такое, что
\ShowEq{B(a) subset U}
\qed
\end{ShadedDefinition}
}
{definition: open set}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{compact set}
Множество $T$ топологического пространства называется
\AddIndex{компактным}{compact set},
если любое его открытое покрытие содержит
конечное подпокрытие.\,\footnote{
Смотри также определение в
\citeBib{Kolmogorov Fomin}, страница 98.
}
\qed
\end{ShadedDefinition}
}
{definition: compact set}
%\DefEq

\DefTheorem{c1+c2 in B}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для
\ShowEq{c1 c2 in A}
пусть
\ShowEq{c1 c2 in B}
Тогда
\ShowEq{c1+c2 in B}
}

\DefLabeledDefinition{limit of sequence}{normed \Algebrac}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
$\Module$\Hyph число $a$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
\ShowEq{[an] in A}
\ShowEq{limit of sequence}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|an-a|<epsilon}{-}
для любого $n>n_0$.
Мы будем также говорить, что
\AddIndex{последовательность $a_n$ сходится}{sequence converges}
к $a$.
}

\AddEq{theorem: limit of sequence}
{
\begin{ShadedTheorem}
\labelTheorem{limit of sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
$\Module$\Hyph число $a$ является 
пределом последовательности
\ShowEq{[an] in A}
\DrawEq{a=lim an}{}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{an in B(a)}{}
для любого $n>n_0$.
\end{ShadedTheorem}
}

\DefProof{limit of sequence}
{
Следствие определений
\RefDefinition{open ball},
\refDefinition{limit of sequence}{normed \Algebrac}.
}

\DefLabeledDefinition{fundamental sequence}{normed \Algebrac}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|ap-aq|<epsilon}{-}
для любых $p$, $q>n_0$.
}

\AddEq{theorem: fundamental sequence}
{
\begin{ShadedTheorem}
\labelTheorem{fundamental sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
является фундаментальной последовательностью,
тогда и только тогда, когда для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\ShowEq{aq in B(ap)}
для любых $p$, $q>n_0$.
\end{ShadedTheorem}
}

\DefProof{fundamental sequence}
{
Следствие определений
\RefDefinition{open ball},
\refDefinition{fundamental sequence}{normed \Algebrac}.
}

\DefTheorem{norm of compact set is bounded}
{
Пусть $C$ - компактное множество
нормированной $\Omega$\Hyph группы $A$.
Тогда норма
\ShowEq{|x in C|}
ограничена сверху и снизу.
}

\DefTheorem{lim a=lim b}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть $a_n$, $b_n$, $n=1$, ..., - фундаментальные последовательности.
Пусть
\DrawEq{lim a-b=0}{limit}
Если последовательность $a_n$ сходится, то
последовательность $b_n$ сходится и
\ShowEq{lim a=lim b}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{complete Omega group}
Нормированная $\Omega$\Hyph группа $A$ называется 
\AddIndex{полной}{complete Omega group}
если любая фундаментальная последовательность элементов
$\Omega$\Hyph группы $A$ сходится, т. е.
имеет предел в этой $\Omega$\Hyph группе.
\qed
\end{ShadedDefinition}
}
{definition: complete Omega group}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{limit of sequence, map to Omega group}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
Отображение
\ShowEq{f M(X,A)}
называется
\AddIndex{пределом последовательности}{limit of sequence}
$f_n$, если для любого $x\in X$
\DrawEq{f(x)=lim}{}
Мы будем также говорить, что
\AddIndex{последовательность $f_n$ сходится}{sequence converges}
к отображению $f$.
\qed
\end{ShadedDefinition}
}
{definition: limit of sequence, map to Omega group}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{sequence converges uniformly}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
\AddIndex{Последовательность $f_n$ сходится равномерно}
{sequence converges uniformly}
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{fn(x) - f(x)}
для любого $n>N$.
\qed
\end{ShadedDefinition}
}
{definition: sequence converges uniformly}
%\DefEq

\DefTheorem{sequence converges uniformly, fn-fm}
{
Последовательность отображений
\ShowEq{fn M(X,A)}
в нормированную
$\Omega$\Hyph группу $A$ сходится равномерно
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{|fn(x)-fm(x)|<e}
для любых \(n\), \(m>N\).
}

\DefDefinition{quasibasis of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
и
\ShowEq{Gen f =}
Если для множества $X\subset A_2$ верно
\ShowEq{in Gen}Xf,
то для любого множества $Y$, $X\subset Y\subset A_2$,
также верно
\ShowEq{in Gen}Yf.
Если существует минимальное множество
\ShowEq{in Gen}Xf,
то множество $X$ называется
\AddIndex{квазибазисом}{quasibasis}
представления $f$.
}

\DefTheorem{X is quasibasis of representation}
{
Если множество $X$ является квазибазисом представления $f$,
то для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
}

\DefRemark{X is quasibasis of representation}
{
Доказательство теоремы
\RefTheorem{X is quasibasis of representation}
даёт нам эффективный метод построения квазибазиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить квазибазис этого представления.
}

\AddEq{remark: representation in form of Omega2-word is ambiguous}
{
Мы ввели $\Omega_2$\Hyph слово элемента $x\in A_2$ относительно множества образующих $X$
в определении
\RefDefinition{word of element relative to set, representation}.
Из теоремы
\RefTheorem{X is quasibasis of representation}
следует, что если множество образующих $X$ не является квазибазисом,
то выбор $\Omega_2$\Hyph слова относительно множества образующих $X$ неоднозначен.
Но даже если множество образующих $X$ является квазибазисом,
то представление $m\in A_2$ в виде $\Omega_2$\Hyph слова неоднозначно.
}

\DefDefinitionNote{word of element relative to set, representation}
{
Пусть $X\subset A_2$.
Для любого
\ShowEq{x in JX}m{}
существует
\AddIndex{$\Omega_2$\Hyph слово}
{word of element relative to generating set, representation}
\ShowEq{word of element relative to generating set, representation},
определённое согласно следующему правилам.
\StartLabelItem
\begin{enumerate}
\item Если $m\in X$, то $m$ - $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, m in X}
\item Если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова и
$\omega\in\Omega_2(n)$, то $m_1...m_n\omega$
- $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, omega}
\item Если $m$ - $\Omega_2$\Hyph слово и
\ShowEq{a in A1},
то $f(a)(m)$
- $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, am}
\end{enumerate}
Мы будем отождествлять элемент
\ShowEq{x in JX}m{}
и соответствующее ему $\Omega_2$\Hyph слово, выражая это равенством
\ShowEq{identify element jf(X) and word}
Аналогично, для произвольного множества
\ShowEq{subset of representation}{}
рассмотрим множество $\Omega_2$\Hyph слов\,\footnotemark
\ShowEq{subset of words of representation}
Мы будем также пользоваться записью
\ShowEq{subset of words of representation, 1}
Обозначим
\ShowEq{word set of representation}
\AddIndex{множество $\Omega_2$\Hyph слов представления $J[f,X]$}
{word set of representation}.
}{
Выражение $\wXm$
является частным случаем
выражения $\wXm[B]$, а именно
\ShowEq{subset of words of representation, 2}
}

\DefRemark{three reasons of ambiguity in Omega2-word}
{
Существует три источника неоднозначности в записи
$\Omega_2$\Hyph слова.
\StartLabelItem
\begin{enumerate}
\item
В $\Omega_i$\Hyph алгебре $A_i$, $i=1$, $2$,
могут быть определены равенства.
Например, если $e$ - единица мультипликативной группы $A_i$,
то верно равенство
\[ae=a\]
для любого $a\in A_i$.
\item
\begin{sloppypar}
Неоднозначность выбора $\Omega_2$\Hyph слова
может быть связана со свойствами представления.
Например, если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова,
$\omega\in\Omega_2(n)$ и
\ShowEq{a in A1},
то\,\footnote{
Например, пусть
$\{e_1,e_2\}$
- базис векторного пространства над полем $k$.
Равенство \EqRef{ambiguity of coordinates 1}
принимает форму закона дистрибутивности
\ShowEq{ambiguity of coordinates 1, vector}
}
\ShowEq{ambiguity of coordinates 1}
В тоже время, если $\omega$ является операцией
$\Omega_1$\Hyph алгебры $A_1$ и операцией
$\Omega_2$\Hyph алгебры $A_2$, то мы можем потребовать,
что $\Omega_2$\Hyph слова
\ShowEq{a1n omega x}
и
\ShowEq{a1n x omega}
описывают один и тот же
элемент $\Omega_2$\Hyph алгебры $A_2$.\,\footnote{Для векторного пространства
это требование принимает форму закона дистрибутивности
\ShowEq{(a+b)e=ae+be}
}
\DrawEq{ambiguity of coordinates 2}{representation}
\end{sloppypar}
\item
Равенства вида
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
сохраняются при морфизме представления.
Поэтому мы можем игнорировать эту
форму неоднозначности записи $\Omega_2$\Hyph слова.
Однако возможна принципиально другая форма неоднозначности,
пример которой можно найти
в теоремах
\refTheorem[\RefRepresentation]{linear dependence between vectors of basis}{\SideWS module},
\refTheorem[\RefRepresentation]{coordinates of vector with linear dependence}{\SideWS module}.
\end{enumerate}
Таким образом, мы видим, что на множестве $\Omega_2$\Hyph слов
можно определить различные отношения эквивалентности.\,\footnote{
Очевидно, что каждое из равенств
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
порождает некоторое отношение эквивалентности.
}
Наша задача - найти максимальное отношение эквивалентности
на множестве $\Omega_2$\Hyph слов, которое
сохраняется при морфизме представления.
}

\DefTheoremNote{equivalence generated by basis}
{
Пусть $X$ - квазибазис представления
\ShowEq{f:A->*B}f{A_1}{A_2}
Для любого множества образующих $X$ представления $f$
существует отношение эквивалентности
\ShowEq{l fX in w fX}
которое порождено исключительно следующими утверждениями.
\StartLabelItem
\begin{enumerate}
\item
%\labelItem{w1 w2 in l fX}
Если в $\Omega_2$\Hyph алгебре $A_2$ существует равенство
\ShowEq{w1[]=w2[]}
определяющее структуру $\Omega_2$\Hyph алгебры, то
\ShowEq{w1 w2 in l fX}
\item
%\labelItem{fw1m fw2m in l fX}
Если в $\Omega_1$\Hyph алгебре $A_1$ существует равенство
\ShowEq{w1[]=w2[]}
определяющее структуру $\Omega_1$\Hyph алгебры, то
\ShowEq{fw1m fw2m in l fX}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l}
Для любой операции
\ShowEq{omega n ari}{}1n,
\ShowEq{(f(a1n)a2,f(a)a2) in l}
\item
%\labelItem{(fa1(a21n),fa1(a2)) in l}
Для любой операции
\ShowEq{omega n ari}{}2n,
\ShowEq{(fa1(a21n),fa1(a2)) in l}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l 1}
Пусть
\ShowEq{omega in O1AO2}12.
Если представление $f$ удовлетворяет равенству\,\footnotemark
\ShowEq{f(a1n)a2=f(a)a2}
то мы можем предположить, что верно равенство
\ShowEq{(f(a1n)a2,f(a)a2) in l 1}
\end{enumerate}
}
{
Рассмотрим представление коммутативного кольца $D$
в $D$\Hyph алгебре $A$. Мы будем пользоваться записью
\ShowEq{f(a)(v)=av}
В обеих алгебрах определены операции сложения и умножения.
Однако равенство
\ShowEq{f(a+b)v=}
верно, а равенство
\ShowEq{f(ab)v=}
является ошибочным.
}

\DefDefinition{basis of representation}
{
Квазибазис $\Basis e$ представления $f$ такой, что
\ShowEq{rho=lambda}
называется
\AddIndex{базисом представления}{basis of representation} $f$.
}

\DefDefinition{equivalence on the set of Omega2-words}
{
Множество образующих $X$ представления $f$
порождает отношение эквивалентности
\ShowEq{rho fX=}
на множестве $\Omega_2$\Hyph слов.
}

\DefTheorem{h=f+g, converges uniformly}
{
Пусть последовательность отображений
\ShowEq{fn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f$.
Пусть последовательность отображений
\ShowEq{gn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $g$.
Тогда последовательность отображений
\ShowEq{hn=fn+gn}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f+g}{converges uniformly}
}

\DefTheorem{representation f generates representation fX}
{
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$
порождает представление
\ShowEq{f:A->*B}{f_X}{M(X,A_1)}{M(X,A_2)}
$\Omega_1$\Hyph группы
\ShowEq{M(X,A1)}
в $\Omega_2$\Hyph группе
\ShowEq{M(X,A2)}
где (
\ShowEq{g1 in M(X,A1)},
\ShowEq{g2 in M(X,A2)}
)
\ShowEq{f(x)g(x):X->A2}
}

\DefTheorem{fX(g1)(g2), converges uniformly}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
полной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в полной $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть последовательность отображений
\ShowEq{g1n M(X,A1)}
сходится равномерно
к отображению $g_1$.
Пусть последовательность отображений
\ShowEq{g2n M(X,A2)}
сходится равномерно
к отображению $g_2$.
Пусть множество значений отображения $g_i$, $i=1$, $2$,
компактно.
Тогда последовательность отображений
\ShowEq{f(g1n)(g2n)}
сходится равномерно
к отображению
\ShowEq{fX(g1)(g2)}.
}

\DefTheorem{set of maps to Omega group}
{
Пусть
\ShowEq{set of maps to Omega group}
- множество отображений множества $X$ в $\Omega$\Hyph группу $A$.
Мы можем определить структуру $\Omega$\Hyph группы на множестве
\EqParm{M(X,A)}{=.}
}

\DefEq
{
Так как $X$ - произвольное множество, мы не можем определить
норму в $\Omega$\Hyph группе
\EqParm{M(X,A)}{=.}
Однако мы можем определить сходимость последовательности в
\EqParm{M(X,A)}{=.c}
следовательно, мы можем определить топологию в
\EqParm{M(X,A)}{=.}
}
{remark: set of maps to Omega group}
%\DefEq

\DefDefinition{closed ball}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{closed ball}
называется
\AddIndex{замкнутым шаром}{closed ball}
с центром в $a$.
}

\DefDefinition{open ball}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{open ball}
называется
\AddIndex{открытым шаром}{open ball}
с центром в $a$.
}

\DefDefinition{reduced polymorphism of representations}
{
Пусть
\ShowEq{set of universal algebras 1}
- универсальные алгебры.
Пусть, для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}A{B_k}
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{f:A->*B}fAB
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{reduced polymorphism of representation}
называется
\AddIndex{приведенным полиморфизмом представлений}
{reduced polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменной $x_k\in B_k$
имеют заданное значение, отображение $r_2$
является приведенным морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f$.
}

\DefConvention{Einstein summation}
{
Мы будем пользоваться соглашением Эйнштейна о сумме.
Это означает, что, когда индекс присутствует в
выражении дважды (один вверху и один внизу) и множество индексов известно,
это выражение подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}av
Я буду явно указывать множество
индексов, если это необходимо.
}

\DefTheorem{structure of Abelian group}
{
Пусть $G$ - абелевая группа.
Множество $G$\Hyph чисел, порождённое множеством
\ShowEq{S=si},
имеет вид
\ShowEq{J(S)=gi si}
где множество
\ShowEq{|gi ne 0|}g
конечно.
}

\DefProof{structure of Abelian group}
{
Мы докажем теорему по индукции, опираясь на теоремы
\citeBib{Cohn: Universal Algebra}\Hyph 5.1, страница 94, и
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

Для произвольного $s_k\in S$,
положим
\ShowEq{gi=dik}
Тогда
\ShowEq{sk=sum si}
\ShowEq{sk in JS}
следует из
\EqRef{J(S)=gi si},
\EqRef{sk=sum si}.

Пусть
\ShowEq{w12 in Jv}gS
Так как $G$ является абелевой группой,
то, согласно утверждению
\RefItem[\RefRepresentation]{x1n omega in Xk+1},
\ShowEq{w1+w2 in Jv}gS
Согласно равенству
\EqRef{J(S)=gi si},
существуют $Z$\Hyph числа
\ShowEq{gi12}g
такие, что
\DrawEq[g]{w12= }{group}
где множества
\DrawEq[g]{|ci12 ne 0|}{group}
конечны.
Из равенства
\eqRef{w12= }{group}
следует, что
\DrawEq[g]{w1+w2= }{group}
Равенство
\DrawEq[g]{w1+w2= 1 }{group}
является следствием равенств
\EqRef{(m+n)a=ma+na},
\eqRef{w1+w2= }{group}.
Из равенства
\eqRef{|ci12 ne 0|}{group}
следует, что
множество
\ShowEq{|gi 1+2 ne 0|}g
конечно.
Из равенства
\eqRef{w1+w2= 1 }{group}
следует, что
\ShowEq{w1+w2 in Jv}gS
}

\AddEq [1]{step of proof: action in Abelian group}
{
Из равенства
\EqRef{0g=0}
следует, что равенство
\EqRef{#1}
верно, когда $n=0$.
\def\TempA{(nm)a=n(ma)}
\def\TempB{#1}
\begin{itemize}
\item
Пусть равенство
\EqRef{#1}
верно, когда $n=k\ge 0$.
Тогда
\ShowEq{#1,n=k}
Равенство
\ShowEq{#1,n=k+1}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n+1)g=},
\EqRef{(m+n)a=ma+na}.
\else
равенства
\EqRef{(n+1)g=}.
\fi
Следовательно, равенство
\EqRef{#1}
верно, когда $n=k+1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1}
верно для любого $n\ge 0$.
\item
Пусть равенство
\EqRef{(m+n)a=ma+na}
верно, когда $n=k\le 0$.
Тогда
\ShowEq{#1,n=k}
Равенство
\ShowEq{#1,n=k-1}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n-1)g=},
\EqRef{(m-n)a=ma-na}.
\else
равенства
\EqRef{(n-1)g=}.
\fi
Следовательно, равенство
\EqRef{#1}
верно, когда $n=k-1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1}
верно для любого $n\le 0$.
\item
Следовательно, равенство
\EqRef{#1}
верно для любого $n\in Z$.
\end{itemize}
}

\DefDefinition{category of representations A1(mA2)}
{
Пусть $A_1$ - $\Omega_1$\Hyph алгебра.
Пусть $\mathcal A_2$ - категория $\Omega_2$\Hyph алгебр.
Мы определим \AddIndex{категорию
\ShowEq{A1(mA2) symb}
представлений}
{category of representations}
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Объектами этой категории являются представления
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Морфизмами этой категории являются приведенные морфизмы соответствующих представлений.
}

\DefProofRef{cr transpose}{}
{
Мы можем доказать \eqRef{cr transpose}{Theorem} в случае матриц тем же
образом, что мы
доказали \eqRef{rc transpose}{Theorem}. Тем не менее для нас более
важно показать, что \eqRef{cr transpose}{Theorem}
следует непосредственно из \eqRef{rc transpose}{Theorem}.

Применяя \EqRef{double transpose} к каждому слагаемому в левой части
\eqRef{cr transpose}{Theorem}, мы получим
\ShowEq{cr transpose, 1}
Из \EqRef{cr transpose, 1} и \eqRef{rc transpose}{Theorem}
следует, что
\ShowEq{cr transpose, 2}
\eqRef{cr transpose}{Theorem} следует из \EqRef{cr transpose, 2}
и \EqRef{double transpose}.
}

\DefProofRef{rc transpose}{}
{
Цепочка равенств
\ShowEq{rc transpose, 1}
следует из \EqRef{transpose of matrix, 1},
\EqRef{rc-product of matrices} и
\EqRef{cr-product of matrices}.
Равенство \eqRef{rc transpose}{Theorem} следует из
\EqRef{rc transpose, 1}.
}

\DefText{matrix operations 1}
{
Согласно традиции произведение
матриц $a$ и $b$ определено как произведение
строк матрицы $a$ и столбцов матрицы $b$.
\ePrints{1908.04418,6860-2955,2020.06.01,2204.06320,2022.01.05}
\Items{8428-0408,2207.06506}%
\ifx\Semafor\ValueOn
В некоммутативной алгебре этой операции умножения
недостаточно для решения некоторых задач.
\ePrints{8428-0408,2207.06506}
\ifx\Semafor\ValueOff
\ShowExample{matrix in right vector space}

\ShowExample{matrix in left vector space}

Из примеров
\RefExample{matrix in right vector space},
\RefExample{matrix in left vector space}
\else
\TwoColText
{
\ShowEq{def left}
\ShowEq{def AVector}%
\ShowEq{\DefCol}
\ShowExample{matrix in vector space}
}
{
\ShowEq{def right}
\ShowEq{def AVector}%
\ShowEq{\DefCol}
\ShowExample{matrix in vector space}
}

Из примеров
\refExample{matrix in vector space}{left},
\refExample{matrix in vector space}{right}
\fi
следует, что
\else
Если произведение в
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
$D$\Hyph алгебре
\else
$\Omega$\Hyph кольце
\fi
некоммутативно,
\fi
мы не можем ограничиться традиционным произведением матриц
и нам нужно определить два вида произведения матриц.
Чтобы различать эти произведения, мы вводим
новые обозначения.
}

\DefText{matrix operations 2}
{
Мы так же определим следующие операции на множестве матриц.
}

\DefExample{matrix in left vector space}
{
Мы представим базис $\Basis e$
левого векторного пространства $V$
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
над $D$\Hyph алгеброй $A$
(смотри определение
\ShowEq{def left}%
\ShowEq{def AVector}%
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теорему
\refTheorem{basis over division algebra}{left})
\fi
как строку матрицы
\DrawEq[en]{a=(a1.n row)}{left basis}
Мы можем представить координаты вектора
\ShowEq{w=w*e left-cols}v{}
как вектор столбец
\DrawEq[vn]{a=(a1.n col)}{left basis}
Однако мы не можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(v)(e)}
так как это произведение не определено.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
Линейный гомоморфизм
левого векторного пространства $V$
может быть представлен с помощью матрицы
\ShowEq{v'=vf}
Равенство
\EqRef{v'=vf}
не может быть выражено как традиционное произведение матриц $v$ и $f$.
\fi
}

\AddEq{define basis for example}
{
Мы представим множество векторов
\ShowEq{\RowN() 1n}en{}
базиса $\Basis e$
\SideRu вого векторного пространства $V$
над $D$\Hyph алгеброй $A$
(смотри определение
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теорему
\refTheorem{basis over division algebra}{left})
в виде
\RowA матрицы
\DrawEq[en]{a=(a1.n \RowN)}{\SideWS basis}
Мы представим координаты
\ShowEq{\ColNS() 1n}vn{}
вектора
\ShowEq{w=w*e left-cols}v{}
в виде \ColA матрицы
\DrawEq[vn]{a=(a1.n \ColNS)}{vn \SideNS-\Cols}
}

\AddEq{vector as matrix product left}
{
Поэтому мы можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(e)(v)}
}

\AddEq{vector as matrix product right}
{
Однако мы не можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(v)(e)}
так как это произведение не определено.
}

\DefLabeledExample{matrix in vector space}{\SideNS}
{
\ShowEq{define basis for example}
\ShowEq{vector as matrix product \SideNS}
}

\DefExample{matrix in right vector space}
{
Мы представим базис $\Basis e$
правого векторного пространства $V$
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
над $D$\Hyph алгеброй $A$
(смотри определение
\ShowEq{def right}%
\ShowEq{def AVector}%
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теорему
\refTheorem{basis over division algebra}{right})
\fi
как строку матрицы
\DrawEq[en]{a=(a1.n row)}{right basis}
Мы можем представить координаты вектора
\ShowEq{w=w*e right-cols}v{}
как вектор столбец
\DrawEq[vn]{a=(a1.n col)}{right basis}
Поэтому мы можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(e)(v)}
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
Линейный гомоморфизм
правого векторного пространства $V$
может быть представлен с помощью матрицы
\ShowEq{v'=fv}
Равенство
\EqRef{v'=fv}
выражает традиционное произведение матриц $f$ и $v$.
\fi
}

\DefDefinition{row over column product}
{
Пусть число столбцов матрицы $a$ равно числу строк матрицы $b$.
\AddIndex{\RC произведение}{rc-product}
матриц $a$ и $b$ имеет вид
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
\ShowEq{entry rc-product of matrices}
\ShowEq{rc-product, matrices}
\RC произведение может быть выражено как произведение строк матрицы $a$
и столбцов матрицы $b$.
}

\DefDefinition{column over row product}
{
Пусть число строк матрицы $a$ равно числу столбцов матрицы $b$.
\AddIndex{\CR произведение}{cr-product}
матриц $a$ и $b$ имеет вид
\ShowEq{cr-product}
\ShowEq{cr-product of matrices}
\ShowEq{entry cr-product of matrices}
\ShowEq{cr-product, matrices}
\CR произведение может быть выражено как произведение столбцов матрицы $a$
и строк матрицы $b$.
}

\DefDefinition{transpose of matrix}
{
Транспонирование $a^T$ матрицы $a$
меняет местами строки и столбцы
\ShowEq{transpose of matrix, 1}
}

\DefDefinition{sum of matrices}
{
Сумма матриц $a$ и $b$ определена равенством
\ShowEq{(a+b)=}
}

\DefDefinition{rc power}
{
Мы определим \AddIndex{\RC степень}{rc power}
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph числа
\else
матрицы
\fi
$a$,
пользуясь рекурсивным правилом
\ShowEq{rc power}
\DrawEq{rc power, 0}1
\DrawEq{rc-power, n}1
}

\DefDefinition{cr power}
{
Мы определим \AddIndex{\CR степень}{cr power}
$\mathcal{A}$\Hyph числа $a$,
пользуясь рекурсивным правилом
\ShowEq{cr power}
\DrawEq{cr power, 0}1
\DrawEq{cr-power, n}1
}

\DefDefinitionNote{Hadamard inverse of matrix}
{
Пусть
\DrawEq[ann]{a=(a11.nm matrix)}{}
матрица $A$\Hyph чисел.
Мы называем матрицу\,\footnotemark
\ShowEq{Hadamard inverse of matrix}
\ShowEq{Hadamard inverse of matrix 2}
\ShowEq{Hadamard inverse of matrix 2 entry}
\AddIndex{обращением Адамара матрицы}{Hadamard inverse of matrix} $a$
(\citeBib{q-alg-9705026}-\href{https://arxiv.org/pdf/math/9705026.pdf\#Page=4}{page 4}).
}{
Запись в равенстве
\EqRef{Hadamard inverse of matrix 2 entry}
означает, что
при обращении Адамара столбцы и строки меняются местами.
\label{footnote: index of inverse element}
Мы можем
формально записать правую часть равенства
\EqRef{Hadamard inverse of matrix 2 entry}
следующим образом
\ShowEq{Hadamard inverse of matrix 3}
}

\DefDefinition{transformation coordinated with equivalence}
{
Пусть на множестве $A_2$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия
\ShowEq{m1 m2 modS}{}
следует
\ShowEq{fm1 fm2 modS}.
}

\DefTheorem{transformation correlated with equivalence}
{
Пусть на множестве $A_2$ определена эквивалентность $S$.
Пусть на множестве
\ShowEq{End O2}{A_2}{}
определена $\Omega_1$\Hyph алгебра.
Если любое преобразование
\ShowEq{f in End A2},
согласованно с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве
\ShowEq{End A2/S}S.
}

\DefTheorem{decompositions of morphism of representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$.
Пусть
\ShowEq{r12:A->B}tAB
морфизм представлений из $f$ в $g$.
Тогда для отображений $t_1$, $t_2$ существуют разложения,
которые можно описать диаграммой
\ShowEq{decompositions of morphism of representations, diagram}
\StartLabelItem
\begin{enumerate}
\item
Ядро гомоморфизма
\ShowEq{kernel of homomorphism i}
является конгруэнцией на $\Omega_i$\Hyph алгебре $A_i$,
\ShowEq{i=1,2}.
\labelItem{kernel of homomorphism i}
\item
Существует разложение гомоморфизма $t_i$,
\ShowEq{i=1,2},
\ShowEq{morphism of representations of algebra, homomorphism, 1}
\labelItem{exists decomposition of homomorphism}
\item
Отображения
\ShowEq{morphism of representations of algebra, p1=}
\ShowEq{morphism of representations of algebra, p2=}
являются естественными гомоморфизмами.
\labelItem{p12 are natural homomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, q1=}
\ShowEq{morphism of representations of algebra, q2=}
являются изоморфизмами.
\labelItem{q12 are isomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, r1=}
\ShowEq{morphism of representations of algebra, r2=}
являются мономорфизмами.
\labelItem{r12 are monomorphisms}
\item $F$ - представление $\Omega_1$\Hyph алгебры $A_1/s$ в $A_2/s_2$
\item $G$ - представление $\Omega_1$\Hyph алгебры $t_1A_1$ в $t_2A_2$
\item Отображение
\ShowEq{map r12}p{}
является морфизмом представлений $f$ и $F$
\labelItem{(p12) is morphism of representations}
\item Отображение
\ShowEq{map r12}q{}
является изоморфизмом представлений $F$ и $G$
\labelItem{(q12) is isomorphism of representations}
\item Отображение
\ShowEq{map r12}r{}
является морфизмом представлений $G$ и $g$
\labelItem{(r12) is morphism of representations}
\item Существует разложение морфизма представлений
\labelItem{exists decompositions of morphism of representations}
\ShowEq{decompositions of morphism of representations}
\end{enumerate} 
}

\DefDefinition{stable set of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Множество
\ShowEq{B2 subset A2}
называется
\AddIndex{стабильным множеством представления}
{stable set of representation} $f$,
если
\ShowEq{fam in B2}
для любых
\ShowEq{a in A1},
$m\in B_2$.
}

\DefTheorem{subrepresentation of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть множество
\ShowEq{B2 subset A2}
является подалгеброй $\Omega_2$\Hyph алгебры $A_2$
и стабильным множеством представления $f$.
Тогда существует представление
\ShowEq{representation of algebra A in algebra B}
такое, что
\ShowEq{fB2(a)=}
Представление $f_{B_2}$ называется
\AddIndex{подпредставлением}{subrepresentation}
представления $f$.
}

\DefTheoremNote{lattice of subrepresentations}
{
Множество\,\footnotemark
\ShowEq{lattice of subrepresentations}
всех подпредставлений представления $f$ порождает
систему замыканий на $\Omega_2$\Hyph алгебре $A_2$
и, следовательно, является полной структурой.
}{
Это определение
аналогично определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94).
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn%
Вообще говоря, в этой и последующих теоремах 
этой главы необходимо рассмотреть структуру универсальных алгебр
$A_1$ и $A_2$.
Так как основная задача этой главы -
это изучение структуры представления,
я сознательно упростил теоремы, чтобы детали не заслоняли
основные утверждения.
Более подробно эта тема будет раскрыта в главе
\RefChapter{Basis of Diagram of Representations of Universal Algebra},
где теоремы будут сформулированы в общем виде.
\fi
}

\AddEq{remark: closure operator, representation}
{
Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, representation}
Таким образом,
\ShowEq{subrepresentation generated by set}
является пересечением всех подалгебр
$\Omega_2$\Hyph алгебры $A_2$,
содержащих $X$ и стабильных относительно представления $f$.
}

\DefDefinition{generating set of representation}
{
\ShowEq{show closure operator, representation}
называется
\AddIndex{подпредставлением}{subrepresentation},
порождённым множеством $X$,
а $X$ -
множеством образующих
подпредставления $J[f,X]$.
В частности,
\AddIndex{множеством образующих}{generating set}
представления $f$
будет такое подмножество $X\subset A_2$, что
\ShowEq{generating set of representation}
}

\DefTheoremNote{map of words of representation}
{
\ShowEq{Let A->*AB2 be representations}
Пусть $X$ - множество образующих представления $f$.
Пусть
\ShowEq{f:A->B}R{A_2}{B_2}
приведенный морфизм представления\,\footnotemark
и $X'=R(X)$.
Приведенный морфизм $R$ представления
порождает отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation}
такое, что
\StartLabelItem
\begin{enumerate}
\item Если
\ShowEq{map of words of representation, m in X, 1}
то
\ShowEq{map of words of representation, m in X}
\item Если
\ShowEq{map of words of representation, omega, 1}
то для операции
$\omega\in\Omega_2(n)$ справедливо
\ShowEq{map of words of representation, omega}
\item Если
\ShowEq{map of words of representation, am, 1}
то
\ShowEq{map of words of representation, am}
\end{enumerate}
}{
Я рассмотрел морфизм представления в теореме
\RefTheorem[\RefRepresentation]{map of words of diagram of representations}.
}

\DefTheorem{Representation is single transitive iff}
{
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in A_2$
существует одно и только одно $g\in A_1$ такое, что $a=f(g)(b)$.
}

\DefProof{Representation is single transitive iff}
{
Следствие определений \RefDefinition{free representation of algebra}
и \RefDefinition{transitive representation of algebra}.
}

\DefTheorem{single transitive representation generates algebra}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
однотранзитивное представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Существует структура $\Omega_1$\Hyph алгебры на множестве $A_2$.
}

\AddEq{theorem: automorphism uniquely defined by image of basis}
{
\begin{ShadedTheorem}
\labelTheorem{automorphism uniquely defined by image of basis}
Пусть $\Basis e$ - базис представления $f$.
Пусть
\ShowEq{R1 X->}{\Basis e}
произвольное отображение множества $\Basis e$.
Рассмотрим отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation, W}{\Basis e}
удовлетворяющее условиям
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega},
\RefItem{map of words of representation, am},
и такое, что
\ShowEq{map of words of representation, W in X}e{\Basis e}
Существует единственный эндоморфизм представлнения $f$\,\footnotemark
\ShowEq{R:A2->A2}
определённый правилом
\ShowEq{endomorphism based on map of words of representation}{\Basis e}
\end{ShadedTheorem}
\footnotetext{\,
Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.
}
}

\DefDefinition{parity of permutation}
{
Отображение
\ShowEq{sigma->+-}
определённое равенством
\def\permutation{перестановка }
\def\even{чётная}
\def\odd{не\even}
\ShowEq{parity of permutation}
называется
\AddIndex{чётностью перестановки}{parity of permutation}.
}

\DefText{passive representation of vector space 1}
{
\ShowText{coordinates of vector with respect to basis (1,2) \Cols}v3
Тогда
\ShowEq{v=vi ei 123, \SideNS-\Cols}
Пусть пассивное преобразование $g_1$ отображает базис
\ShowEq{Basis e in BVG}1
в базис
\ShowEq{Basis e in BVG}2
\DrawEq[12g1]{e2i=aij e1j \Product-\Cols}{12}
Пусть пассивное преобразование $g_2$ отображает базис
\ShowEq{Basis e in BVG}2
в базис
\ShowEq{Basis e in BVG}3
\DrawEq[23g2]{e2i=aij e1j \Product-\Cols}{23}
}

\DefText{passive representation of vector space 2}
{
Преобразование
\ShowEq{e3=g12 cr e1 \SideNS-\Cols}
является произведением преобразований
\eqRef{e2i=aij e1j \Product-\Cols}{12},
\eqRef{e2i=aij e1j \Product-\Cols}{23}.
Преобразование координат
\DrawEq[v2v1g1{\SideNS}{\Cols}]{v2=v1g-}{1 \SideNS-\Cols}
соответствует пассивному преобразованию $g_1$
и является следствием равенств
\EqRef{v=vi ei 123, \SideNS-\Cols},
\eqRef{e2i=aij e1j \Product-\Cols}{12}
и теоремы
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\DefText{passive representation of vector space 3}
{
Аналогично,
\ePrints{1908.04418,6860-2955}%
\ifx\Semafor\ValueOff%
согласно теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
\fi
преобразование координат
\DrawEq[v3v2g2{\SideNS}{\Cols}]{v2=v1g-}{23 \SideNS-\Cols}
соответствует пассивному преобразованию $g_2$
и является следствием равенств
\EqRef{v=vi ei 123, \SideNS-\Cols},
\eqRef{e2i=aij e1j \Product-\Cols}{23}.
Произведение преобразований координат
\eqRef{v2=v1g-}{1 left-cols},
\eqRef{v2=v1g-}{23 left-cols}
имеет вид
\ShowEq{v3=v1 cr g1- cr g2- \SideNS-\Cols}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\EqRef{e3=g12 cr e1 \SideNS-\Cols}.
Равенство
\ShowEq{v3=v1 cr g21- \SideNS-\Cols}
является следствием равенств
\EqRef{cr-inverse matrix of product},
\EqRef{v3=v1 cr g1- cr g2- \SideNS-\Cols}.
}

\DefText{passive representation of left vector space}
{
\ShowText{passive representation of vector space 1}
\ShowText{passive representation of vector space 2}
\ShowText{passive representation of vector space 3}
}

\DefDefinition{Left side contravariant representation}
{
Левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется
\AddIndex{контравариантным}{contravariant representation},
если равенство
\ShowEq{Left side contravariant representation}
верно.
}

\DefDefinition{Left side covariant representation}
{
Левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется
\AddIndex{ковариантным}{covariant representation},
если равенство
\ShowEq{Left side covariant representation}
верно.
}

\DefDefinition{cr-inverse matrix}
{
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph число
\else
Матрица
\fi
\ShowEq{cr-inverse element}
- это \AddIndex{\CR обратный элемент}{cr-inverse element}
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph числа
\else
матрицы
\fi
$a$, если
\DrawEq{cr-inverse matrix}1
\ePrints{2020.06.01}
\ifx\Semafor\ValueOn
Матрица $a$ называется
\CR невырожденной,
если существует \CR обратная матрица.
\fi
}

\DefDefinition{delta=Matrix}
{
Матрица
\ShowEq{delta=Matrix}
является единицей для обоих произведений.
}

\DefRemark{pronunciation of product}
{
Мы будем пользоваться символом \RC\,\, или \CR\,\,  в имени свойств
каждого произведения и в обозначениях.
Мы можем читать символ
$\RCstar$ как
$rc$\hyph произведение (произведение строки на столбец)
и символ $\CRstar$ как
$cr$\hyph произведение (произведение столбца на строку).
Для совместимости
обозначений с существующими мы будем иметь
в виду \RC произведение, когда
нет явных обозначений.
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
Это правило мы распространим на последующую терминологию.
Символ произведения
сформирован из двух символов операции произведения, которые записываются на
месте индекса суммирования.
Например, если произведение $A$\Hyph чисел имеет вид
$a\circ b$,
то \RC произведение
матриц $a$ и $b$ имеет вид
$a\RCcirc b$
и \CR произведение
матриц $a$ и $b$ имеет вид
$a\CRcirc b$.
\fi
}

\DefTheorem{quasideterminant rc cr, matrix 2x2}
{
\ShowEq{quasideterminant matrix 2x2 def}
Рассмотрим матрицу
\ShowEq{inverse matrix 2x2, 0}
Тогда
\ShowEq{quasideterminant rc, matrix 2x2}
\ShowEq{quasideterminant cr, matrix 2x2}
\ShowEq{rc inverse matrix 2x2}
}

\DefDefinition{RC-quasideterminant}
{
\AddIndex{$(\aUD{}ji)$\hyph \RC квазидетерминант}{j i RC-quasideterminant}
\nTimes матрицы $a$
- это формальное выражение
\ShowEq{j i RC-quasideterminant definition}
\ShowEq{j i RC-quasideterminant =}
Мы можем рассматривать $\aUD (ji)$\hyph \RC квазидетерминант
как элемент матрицы
\ShowEq{RC-quasideterminant definition}
\ShowEq{RC-quasideterminant definition=}
которую мы будем называть
\AddIndex{\RC квазидетерминантом}{RC-quasideterminant}.
}

\DefDefinition{biring}
{
\AddIndex{Бикольцо}{biring} $\mathcal A$ - это множество,
на котором мы определили унарную операцию, называемую транспозицией,
и три бинарных операции,
называемые \RC произведение, \CR произведение и сумма, такие что
\begin{itemize}
\item \RC произведение и сумма определяют структуру кольца на $\mathcal A$
\item \CR произведение и сумма определяют структуру кольца на $\mathcal A$
\item оба произведения имеют общую единицу $\delta$
\item произведения удовлетворяют равенству
\DrawEq{rc transpose}{}
\item транспозиция единицы есть единица
\DrawEq{transpose of identity}E
\item двойная транспозиция есть исходный элемент
\ShowEq{double transpose}
\end{itemize}
}

\DefTheorem{double transpose is original matrix}
{
Двойная транспозиция есть исходная матрица
\ShowEq{double transpose}
}

\DefProof{double transpose is original matrix}
{
Теорема является следствием определения
\RefDefinition{transpose of matrix}.
}

\DefEq
{
\begin{ShadedTheorem}[принцип двойственности для бикольца]
\AddIndex{}{duality principle for biring}
\labelTheorem{duality principle for biring}
Пусть $\mathcal{A}$ - истинное утверждение о
бикольце $A$.
Если мы заменим одновременно
\begin{itemize}
\item $a\in A$ и $a^T$
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}
}
{theorem: duality principle for biring}
%\DefEq

\DefEq
{
\begin{ShadedTheorem}[принцип двойственности для бикольца матриц]
\AddIndex{}{duality principle for biring of matrices}
\labelTheorem{duality principle for biring of matrices}
Пусть $A$ является бикольцом матриц.
Пусть $\mathcal{A}$ - истинное утверждение о матрицах.
Если мы заменим одновременно
\begin{itemize}
\item строки и столбцы всех матриц
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}
\begin{proof}
Непосредственное следствие
теоремы \RefTheorem{duality principle for biring}.
\end{proof}
}
{theorem: duality principle for biring of matrices}
%\DefEq

\DefEq
{
\begin{remark}
\labelRemark{reducible biring}
Если произведение в $\Omega$\Hyph кольце коммутативно, то
\ShowEq{reducibility of products}
\AddIndex{Приводимое бикольцо}{reducible biring}
- это бикольцо, в котором выполняется
\AddIndex{условие приводимости произведений}
{condition of reducibility of products}
\EqRef{reducibility of products}.
Поэтому в приводимом бикольце достаточно рассматривать только
\RC произведение. Однако в тех случаях, когда
порядок сомножителей существенен,
мы будем пользоваться также \CR произведением.
\qed
\end{remark}
}
{remark: reducible biring}
%\DefEq

\DefEq
{
Так как левостороннее представление и правостороннее представление
опирается на гомоморфизм $\Omega$\Hyph группы,
то верно следующее утверждение.

\begin{ShadedTheorem}[принцип двойственности для представления мультипликативной $\Omega$\Hyph группы]
\labelTheorem{duality principle, algebra representation}
Любое утверждение, справедливое для
левостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$,
будет справедливо для правостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$, если
мы будем пользоваться правосторонним произведением на $A_1$\Hyph число $a_1$ вместо
левостороннего произведения на $A_1$\Hyph число $a_1$.
\qed
\end{ShadedTheorem}
}
{theorem: duality principle, algebra representation}
%\DefEq

\DefTheorem{left right shift}
{
Произведение
\ShowEq{(ab)->ab}
в мультипликативной $\Omega$\Hyph группе $A$
определяет два различных представления.
\begin{itemize}
\EqParm{associative shift}{def left}
\EqParm{associative shift}{def right}
\end{itemize}
}

\AddEq{non associative shift}
{
\item
\SideRuC вый сдвиг
\ShowEq{\SideWS shift}
является представлением
$\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебре $A$.
}

\AddEq{associative shift}
{
\item
\AddIndex{\SideRuC вый сдвиг}{\SideWS shift}
\ShowEq{\SideWS shift =}
\ShowEq{\SideWS shift}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $A$
в $\Omega$\Hyph алгебре $A$
\ShowEq{\SideWS shift, product}
}

\DefDefinition{representation of algebra}
{
Пусть множество $A_2$ является $\Omega_2$\Hyph алгеброй.
Пусть
на множестве преобразований
\ShowEq{End O2}{A_2}{}
определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{representation of algebra}
$\Omega_1$\Hyph алгебры $A_1$ в
$\Omega_1$\Hyph алгебру
\ShowEq{End O2}{A_2}{}
называется
\AddIndex{представлением $\Omega_1$\Hyph алгебры}
{representation of algebra}
$A_1$ или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$.
}

\DefEq
{
Если мультипликативная $\Omega$\Hyph группа $A_1$ - абелевая,
то нет разницы между левосторонним и правосторонним представлениями.

\begin{ShadedDefinition}
\labelDefinition{representation of Abelian group} 
Пусть $A_1$ - абелевая мультипликативная $\Omega$\Hyph группа.
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{Abelian group}
\AddIndex{представлением}{representation of algebra}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{left-side representation of group}{Abelian}
\end{ShadedDefinition}

Обычно мы отождествляем представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и левостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
Однако, если это необходимо нам,
мы можем отождествить представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и правостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
}
{definition: representation of Abelian group}
%\DefEq

\DefTheorem{two representations of group}
{
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа.
Пусть левостороннее $A_1$\Hyph представление $f$
на $\Omega_2$\Hyph алгебре $A_2$ однотранзитивно.
Тогда мы можем однозначно определить однотранзитивное правостороннее $A_1$\Hyph представление $h$
на $\Omega_2$\Hyph алгебре $A_2$
такое, что диаграмма
\ShowEq{two representations of group}
коммутативна для любых $a_1$, $b_1\in A_1$.
}

\AddEq{definition: twin representations}
{
Мы будем называть представления $f$ и $h$
\AddIndex{парными представлениями}{twin representations}
мультипликативной $\Omega$\Hyph группы $A_1$.
}

\DefRemark{one representation of group}
{
Очевидно, что преобразования $L(a)$ и $R(a)$
отличаются, если мультипликативная $\Omega$\Hyph группа $A_1$ неабелева.
Тем не менее, они являются отображениями на.
Теорема \RefTheorem{two representations of group} утверждает, что, если оба
представления правого и левого сдвига существуют на множестве $A_2$,
то мы можем определить два перестановочных представления на множестве $A_2$.
Только правый или левый сдвиг не может представлять оба типа представления.
Чтобы понять почему это так, мы можем изменить диаграмму
\EqRef{Diagram: two representations of group}
и предположить
\ShowEq{haa=Laa}
вместо
\ShowEq{haa=aRa}
и проанализировать, какое выражение $h(a_1)$ имеет в
точке $c_2$. Диаграмма
\ShowEq{Diagram: two representations of group 1}
эквивалентна диаграмме
\ShowEq{Diagram: two representations of group 2}
и мы имеем
\ShowEq{d2=...c2 1}
Следовательно
\ShowEq{d2=...c2}
Мы видим, что представление $h$
зависит от его аргумента.
}

\DefTheorem{single transitive representation of group}
{
Если существует однотранзитивное представление
\ShowEq{f:A->*B}f{A_1}{A_2}
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$,
то мы можем однозначно определить координаты на $A_2$, пользуясь $A_1$\Hyph числами.

Если $f$ - левостороннее однотранзитивное однотранзитивное представление,
то $f(a)$ эквивалентно левому сдвигу $L(a)$ на группе $A_1$.
Если $f$ - правостороннее однотранзитивное представление, то $f(a)$ эквивалентно
правому сдвигу $R(a)$ на группе $A_1$.
}

\DefDefinition{algebra of sets}
{
Непустая система множеств $\mathcal R$ называется
\AddIndex{кольцом множеств}{ring of sets},\,\footnote{
Смотри так же определение
\citeBib{Kolmogorov Fomin}\Hyph 1, страница 41.}
если условие
\ShowEq{A, B in R}
влечёт
\ShowEq{A, B in R 1}
Множество
\ShowEq{E in R}
называется
\AddIndex{единицей кольца множеств}{unit of ring of sets},
если
\ShowEq{A cap E=A}
Кольцо множеств с единицей называется
\AddIndex{алгеброй множеств}{algebra of sets}.
}

\DefEq
{
\begin{remark}
\labelRemark{A cup/minus B}
Для любых
\ShowEq{A cup/minus B}
Следовательно, если
\ShowEq{A, B in R},
то
\ShowEq{A cup/minus B R}
\qed
\end{remark}
}
{remark: A cup/minus B}
%\DefEq

\DefDefinition{sigma algebra of sets}
{
Кольцо множеств $\mathcal R$ называется
\AddIndex{\(\sigma\)\Hyph кольцом множеств}{sigma ring of sets},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, страница 45, определение 3.}
если условие
\ShowEq{Ai in R}
влечёт
\ShowEq{Ai in R 1}
\(\sigma\)\Hyph Кольцо множеств с единицей называется
\AddIndex{\(\sigma\)\Hyph алгеброй множеств}{sigma algebra of sets}.
}

\DefDefinition{Borel algebra}
{
Минимальная \(\sigma\)\Hyph алгебра
\ShowEq{Borel algebra}
над совокупностью всех открытых шаров нормированной $\Omega$\Hyph группы $A$,
называется
\AddIndex{алгеброй Бореля}{Borel algebra}.\,\footnote{
Смотри определение в
\citeBib{Kolmogorov Fomin}, с. 46.
Согласно замечанию
\ref{remark: A cup/minus B},
алгебра Бореля может быть также порождена множеством
замкнутых шаров.
}
Множество,
принадлежащее алгебре Бореля,
называется
\AddIndex{борелевским множеством}{Borel set}
или
\AddIndex{$B$\Hyph множеством}{B set}.
}

\DefDefinition{C_X C_Y measurable}
{
Пусть $\mathcal C_X$ -
\(\sigma\)\Hyph алгебра множеств множества $X$.
Пусть $\mathcal C_Y$ -
\(\sigma\)\Hyph алгебра множеств множества $Y$.
Отображение
\ShowEq{f:A->B}fXY
называется
$(\mathcal C_X,\mathcal C_Y)$\Hyph измеримым,\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282.}
если для всякого множества
\ShowEq{CX CY measurable map}
}

\DefEq
{
\begin{example}
\labelExample{measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{algebra of sets measurable with respect to measure}
- \(\sigma\)\Hyph алгебра измеримых относительно меры $\mu$ множеств.
Пусть
$\mathcal B(A)$
- алгебра Бореля
нормированной $\Omega$\Hyph группы $A$.
Отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{$\mu$\Hyph измеримым}{mu measurable map},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282, определение 1.
Если мера $\mu$ на множестве $X$ определена в контексте,
мы также будем называть отображение
\ShowEq{f:A->B}fXA
\AddIndex{измеримым}{measurable map}.
}
если для всякого множества
\ShowEq{measurable map}
\qed
\end{example}
}
{example: measurable map}
%\DefEq

\DefDefinition{simple map}
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Отображение
\ShowEq{f:A->B}fXA
в нормированную $\Omega$\Hyph группу $A$ называется
\AddIndex{простым отображением}{simple map},
если это отображение $\mu$\Hyph измеримо и
принимает не более, чем счётное множество значений.
}

\DefTheorem{measurable simple map}
{
Пусть отображение
\ShowEq{f:A->B}fXA
принимает не более, чем счётное множество значений
\ShowEq{range f}
.
Отображение $f$ $\mu$\Hyph измеримо тогда и только тогда, когда
все множества
\DrawEq{Fn=}{}
$\mu$\Hyph измеримы.\,\footnote{
Смотри аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страница 292, теорема 1.}
}

\DefDefinition{measure}
{
Пусть \(\mathcal C_m\) - полукольцо множеств.\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 265.}
Отображение
\ShowEq{f:A->B}f{\mathcal C_m}R
называется
\AddIndex{мерой}{measure},
если
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{m(A)>0}
\item
Отображение \(m\) аддитивно.
Если множество
\ShowEq{A in Cm}
имеет конечное разлоение
\DrawEq{A=+Ai Cm}{}
где
\ShowEq{Ai*Aj=0},
то
\ShowEq{m A=+m Ai}
\end{enumerate}
}

\DefDefinition{complete measure}
{
Мера \(\mu\) называется
\AddIndex{полной}{complete measure},
если из условий
\ShowEq{B in A, mu(A)=0}
следует,
что множество \(B\) измеримо.
}

\DefDefinition{sigma-additive measure}
{
Пусть $\mathcal C_{\mu}$ -
\(\sigma\)\Hyph алгебра множеств множества $F$.\,\footnote{
Смотри аналогичные определения в
\citeBib{Kolmogorov Fomin}, определение 1 на странице 265
и определение 3 на странице 268.}
Отображение
%\ShowEq{mu:CF->A}
%в нормированную $\Omega$\Hyph группу $A$ называется
\ShowEq{f:A->B}{\mu}{\mathcal C_{\mu}}R
в поле действительных чисел $R$ называется
\AddIndex{\(\sigma\)\Hyph аддитивной мерой}{sigma-additive measure},
если для любого множества
\ShowEq{X in Cmu}
выполнены следующие условия.
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{muX>0}
\item
Пусть
\DrawEq{X=+Xi}{}
конечное или счётное объединение множеств
\ShowEq{Xn in Cmu}
Тогда
\DrawEqParm{mu(X=+Xi)}X{}
где ряд в правой части сходится абсолютно.
\labelItem{mu(X=+Xi)}
\end{enumerate}
}

\DefEq
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть определено эффективное представление поля действительных чисел \(R\)
в полной абелевой \(\Omega\)\Hyph группе \(A\).\,\footnote{
Другими словами,
\(\Omega\)\Hyph группа \(A\) является
\(R\)\Hyph векторным пространством.}
}
{remark - measure - effective representation of real field}
%\DefEq

\DefDefinition{series converges normally}
{
Пусть \(a_i\) - последовательность \(A\)\Hyph чисел.
Если
\ShowEq{sum |ai|<infty}
то мы будем говорить, что {\bf ряд}
\ShowEq{sum ai}
\AddIndex{сходится нормально}
{series converges normally}.\,\footnote{Смотри также
определение нормальной сходимости ряда
на странице \citeBib{Cartan differential form}-12.}
}

\DefDefinition{Integral of Map over Set of Finite Measure}
{
\(\mu\)\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 3, страницы 294, 295.
}
если существует последовательность
простых  отображений
\ShowEq{f:A->B}{f_n}XA
сходящаяся равномерно к \(f\).
Если отображение \(f\) интегрируемо,
то предел
\ShowEq{integral of map}
\ShowEq{integral of measurable map}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\).
}

\DefDefinition{integrable map}
{
Для простого отображения
\ShowEq{f:A->B}fXA
рассмотрим ряд
\DrawEq{sum mu(F) f}{integral}
где
\begin{itemize}
\item
Множество
\ShowEq{f1...}
является областью определения отображения \(f\)
\item
Если \(n\ne m\), то
\ShowEq{fn ne fm}
\item
\DrawEq{Fn=}{-}
\end{itemize}
Простое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),
если ряд
\eqRef{sum mu(F) f}{integral}
сходится нормально.\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, определение 2, с. 293.}
Если отображение \(f\) интегрируемо,
то сумма ряда
\eqRef{sum mu(F) f}{integral}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\)
\ShowEq{integral of map}
\ShowEq{integral of simple map}
}

\DefTheorem{|int f|<int|f|}
{
Пусть
\ShowEq{f:A->B}fXA
измеримое отображение.
Интеграл
\ShowEq{int f X}
существует
тогда и только тогда, когда
интеграл
\ShowEq{int |f| X}
существует.
Тогда
\DrawEq{|int f|<int|f|}{measurable}
}

\DefTheorem{int |f|<M mu}
{
Пусть $\mu$\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
удовлетворяет условию
\DrawEq{|f(x)|<M}{}
Если мера множества \(X\) конечна, то
\DrawEq{int |f|<M mu}{measurable}
}

\DefTheorem{int f+g X}
{
Пусть
\ShowEq{f:A->B}fXA
\ShowEq{f:A->B}gXA
$\mu$\Hyph измеримые отображения
с компактным множеством значений.
Если существуют интегралы
\ShowEq{int f X}
\ShowEq{int g X}
то существует интеграл
\ShowEq{int f+g X}
и
\DrawEq{int f+g X =}{measurable}
}


==> Symbol.English.tex <==
%auto-ignore
\def\indexname{Special Symbols and Notations}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {direct sum}%
   {direct sum}%
   {0}{0}%
\Symb%
   {unit interval}%
   {unit interval}%
   {0}{0}%

\SetIndexSpace%A%0
\Symb%
   {set of vectors whose expansion relative to the basis $\Basis e$ converges normally}%
   {A plus Schauder}%
   {A}{0}%
\Symb%
   {active representation in basis manifold}%
   {active representation in basis manifold}%
   {A}{0}%
\Symb%
   {$A$\Hyph algebra of polynomials over $D$\Hyph algebra $A$}%
   {algebra of polynomials over algebra}%
   {A}{0}%
\Symb%
   {algebra of polynomials over $D$\Hyph algebra $A$}%
   {algebra of polynomials over D algebra}%
   {A}{0}%
\Symb%
   {algebra of rational mappings of algebra $A$}%
   {algebra of rational mappings of algebra}%
   {A}{0}%
\Symb%
   {affine space}%
   {An}%
   {A}{0}%
\Symb%
   {associator of $D$\Hyph algebra}%
   {associator of algebra}%
   {A}{0}%
\Symb%
   {category of left-side representations of $\Omega_1$\Hyph algebra $A$}%
   {category of left-side representations of Omega1 algebra}%
   {A}{0}%
\Symb%
   {category of representations}%
   {category of representations}%
   {A}{0}%
\Symb%
   {commutator of $D$\Hyph algebra}%
   {commutator of algebra}%
   {A}{0}%
\Symb%
   {component of linear map}%
   {component of linear map, vector}%
   {A}{0}%
\Symb%
   {component $p$ of polylinear mapping $\Vector A$}%
   {component of polyadditive map, D vector space}%
   {A}{0}%
\Symb%
   {component of polylinear map}%
   {component of polylinear map, vector}%
   {A}{0}%
\Symb%
   {conjugated $D$\Hyph  module}%
   {conjugated D module}%
   {A}{0}%
\Symb%
   {coordinates of associator}%
   {coordinates of associator}%
   {A}{0}%
\Symb%
   {\CR power of element $A$ of biring}%
   {cr power}%
   {A}{0}%
\Symb%
   {\crd vector}%
   {crd vector}%
   {A}{0}%
\Symb%
   {\CR inverse matrix}%
   {cr-inverse matrix}%
   {A}{0}%
\Symb%
   {\CR product}%
   {cr-product}%
   {A}{0}%
\Symb%
   {\dcr vector}%
   {dcr vector}%
   {A}{0}%
\Symb%
   {derivative of left shift}%
   {derivative of left shift}%
   {A}{0}%
\Symb%
   {derivative of left shift in $1$\Hyph parameter Lie group}%
   {derivative of left shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {derivative of left shift in $1$\Hyph parameter Lie D group}%
   {derivative of left shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {derivative of right shift}%
   {derivative of right shift}%
   {A}{0}%
\Symb%
   {derivative of right shift in $1$\Hyph parameter Lie group}%
   {derivative of right shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {derivative of right shift in $1$\Hyph parameter Lie D group}%
   {derivative of right shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {derivative of left shift}%
   {derivative of Tstar shift}%
   {A}{0}%
\Symb%
   {\drc vector}%
   {drc vector}%
   {A}{0}%
\Symb%
   {coordinates of vector $a$ relative to Hamel basis}%
   {Hamel basis, coordinates}%
   {A}{0}%
\Symb%
   {hermitian conjugation in division ring}%
   {hermitian conjugation, division ring}%
   {A}{0}%
\Symb%
   {tensor inverse to tensor $a$}%
   {inverse tensor}%
   {A}{0}%
\Symb%
   {isomorphic}%
   {isomorphic}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph\CR quasideterminant}%
   {j i CR quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(ji)$\hyph quasideterminant of matrix $\bfA$}%
   {j i quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph quasideterminant}%
   {j i RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph \RC quasideterminant}%
   {j i RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {left fraction}%
   {left fraction}%
   {A}{0}%
\Symb%
   {left principal ideal}%
   {left principal ideal}%
   {A}{0}%
\Symb%
   {left shift in $D$\Hyph algebra}%
   {left shift, D algebra}%
   {A}{0}%
\Symb%
   {linear combination}%
   {linear combination}%
   {A}{0}%
\Symb%
   {little group}%
   {little group}%
   {A}{0}%
\Symb%
   {transformation of matrix}%
   {matrix, replacing its column}%
   {A}{0}%
\Symb%
   {transformation of matrix}%
   {matrix, replacing its row}%
   {A}{0}%
\Symb%
   {minor matrix}%
   {minor matrix}%
   {A}{0}%
\Symb%
   {norm on $D$\Hyph module}%
   {norm on D module}%
   {A}{0}%
\Symb%
   {$\Omega$\Hyph algebra}%
   {Omega-algebra}%
   {A}{0}%
\Symb%
   {opposite algebra to algebra $A$}%
   {opposite algebra}%
   {A}{0}%
\Symb%
   {orbit of linear map}%
   {orbit of linear map}%
   {A}{0}%
\Symb%
   {derivative}%
   {overline nabla_l, definition 2}%
   {A}{0}%
\Symb%
   {partial linear map}%
   {partial linear map}%
   {A}{0}%
\Symb%
   {principal ideal}%
   {principal ideal}%
   {A}{0}%
\Symb%
   {quasideterminant of matrix $\bfA$}%
   {quasideterminant definition}%
   {A}{0}%
\Symb%
   {\RC power of element $A$ of biring}%
   {rc power}%
   {A}{0}%
\Symb%
   {$\RCcirc$\Hyph quasideterminant}%
   {RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {\rcd vector}%
   {rcd vector}%
   {A}{0}%
\Symb%
   {\RC inverse matrix}%
   {rc-inverse matrix}%
   {A}{0}%
\Symb%
   {\RC product}%
   {rc-product}%
   {A}{0}%
\Symb%
   {\RC quasideterminant}%
   {RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {right principal ideal}%
   {right principal ideal}%
   {A}{0}%
\Symb%
   {right shift in $D$\Hyph algebra}%
   {right shift, D algebra}%
   {A}{0}%
\Symb%
   {coordinates of vector $a$ relative to Schauder basis}%
   {Schauder basis, coordinates}%
   {A}{0}%
\Symb%
   {set of additive maps}%
   {set additive maps}%
   {A}{0}%
\Symb%
   {set of homogeneous polynomials}%
   {set of homogeneous polynomials}%
   {A}{0}%
\Symb%
   {set of invertible elements of algebra $A$}%
   {set of invertible elements of algebra}%
   {A}{0}%
\Symb%
   {set of vectors generated by vector $v$}%
   {set of vectors generated by vector}%
   {A}{0}%
\Symb%
   {set of zeros of algebra $A$}%
   {set of zeros of algebra}%
   {A}{0}%
\Symb%
   {set of polylinear maps of rings $R_1$, ..., $R_n$ into module $S$}%
   {set polylinear maps, ring}%
   {A}{0}%
\Symb%
   {simplex}%
   {simplex}%
   {A}{0}%
\Symb%
   {skew product of vectors $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
   {A}{0}%
\Symb%
   {space of orbits of left\Hyph side representation}%
   {space of orbits of left side representation}%
   {A}{0}%
\Symb%
   {space of orbits of representation}%
   {space of orbits of representation}%
   {A}{0}%
\Symb%
   {space of orbits of effective right\Hyph side representation}%
   {space of orbits of right-side representation}%
   {A}{0}%
\Symb%
   {square root}%
   {square root}%
   {A}{0}%
\Symb%
   {stability group}%
   {stability group}%
   {A}{0}%
\Symb%
   {\sT shift}%
   {starT shift, fibered group}%
   {A}{0}%
\Symb%
   {tensor power of algebra $A$}%
   {tensor power of algebra}%
   {A}{0}%
\Symb%
   {anholonomic coordinates of vector}%
   {vector anholonomic coordinates}%
   {A}{0}%
\Symb%
   {holonomic coordinates of vector}%
   {vector holonomic coordinates}%
   {A}{0}%

\SetIndexSpace%B%0
\Symb%
   {basis manifold of tower of representations $\Vector f$}%
   {basis manifold tower of representations}%
   {B}{0}%
\Symb%
   {basis manifold of affine space}%
   {Basis Manifold, Affine Space}%
   {B}{0}%
\Symb%
   {basis manifold of central affine space}%
   {BCAn}%
   {B}{0}%
\Symb%
   {basis manifold of Euclid space}%
   {BEn}%
   {B}{0}%
\Symb%
   {Borel algebra}%
   {Borel algebra}%
   {B}{0}%
\Symb%
   {canonical remainder of the division}%
   {canonical remainder of the division}%
   {B}{0}%
\Symb%
   {Cartesian power}%
   {Cartesian power}%
   {B}{0}%
\Symb%
   {Cartesian power $\Bundle A$ of bundle $\Bundle B$}%
   {Cartesian power A of bundle B}%
   {B}{0}%
\Symb%
   {Cartesian power $A$ of set $B$}%
   {Cartesian power of set}%
   {B}{0}%
\Symb%
   {closed ball}%
   {closed ball}%
   {B}{0}%
\Symb%
   {closure of set}%
   {closure of set}%
   {B}{0}%
\Symb%
   {coproduct in category}%
   {coproduct in category}%
   {B}{0}%
\Symb%
   {basis manifold of central affine space}%
   {FCAn}%
   {B}{0}%
\Symb%
   {basis manifold of Euclid space}%
   {FEn}%
   {B}{0}%
\Symb%
   {lattice of subrepresentations}%
   {lattice of subrepresentations}%
   {B}{0}%
\Symb%
   {lattice of towers of subrepresentations of tower of representations $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
   {B}{0}%
\Symb%
   {open ball}%
   {open ball}%
   {B}{0}%
\Symb%
   {product in category}%
   {product in category}%
   {B}{0}%
\Symb%
   {right fraction}%
   {right fraction}%
   {B}{0}%
\Symb%
   {tensor power of representation}%
   {tensor power of representation}%
   {B}{0}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph algebra of sets measurable with respect to measure $\mu$}%
   {algebra of sets measurable with respect to measure}%
   {C}{0}%
\Symb%
   {central affine space}%
   {CAn}%
   {C}{0}%
\Symb%
   {central affine space}%
   {central affine space}%
   {C}{0}%
\Symb%
   {continuity class}%
   {class Cn}%
   {C}{0}%
\Symb%
   {$j$th column determinant of matrix $\bfA$}%
   {column determinant}%
   {C}{0}%
\Symb%
   {cosine}%
   {cosine}%
   {C}{0}%
\Symb%
   {$\CRcirc$\Hyph product of matrices of maps}%
   {cr product of matrices of maps}%
   {C}{0}%
\Symb%
   {hyperbolic cosine}%
   {hyperbolic cosine}%
   {C}{0}%
\Symb%
   {left structural constant of Lie algebra}%
   {left structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {right structural constant of Lie algebra}%
   {right structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {set of continuous multivariable maps}%
   {set continuous multivariable maps}%
   {C}{0}%
\Symb%
   {structural constants}%
   {structural constants}%
   {C}{0}%

\SetIndexSpace%D%0
\Symb%
   {basis vector of representation of Lie group over algebra $A$}%
   {basis vector of representation of Lie group over algebra A}%
   {D}{0}%
\Symb%
   {coordinates of basis vector of representation of Lie group over algebra $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
   {D}{0}%
\Symb%
   {component of derivative of map $f(x)$}%
   {component of derivative}%
   {D}{0}%
\Symb%
   {component of derivative of second order of map $f(x)$}%
   {component of derivative of Second Order}%
   {D}{0}%
\Symb%
   {component of the G\^ateaux derivative of map $f(x)$}%
   {component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {component of the G\^ateaux derivative of map $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
   {D}{0}%
\Symb%
   {component of the G\^ateaux derivative of second order of map $f(x)$}%
   {component of Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {component of the G\^ateaux derivative of second order of map $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
   {D}{0}%
\Symb%
   {component of the G\^ateaux derivative of map $f(x)$}%
   {component of Gateaux derivative, vector space}%
   {D}{0}%
\Symb%
   {conjugation in algebra}%
   {conjugation in algebra}%
   {D}{0}%
\Symb%
   {conjugation in ring}%
   {conjugation in ring}%
   {D}{0}%
\Symb%
   {coordinate \rcd vector space}%
   {coordinate rcd vector space}%
   {D}{0}%
\Symb%
   {coordinate reference frame}%
   {coordinate reference frame, extensive definition}%
   {D}{0}%
\Symb%
   {coordinate vector bundle}%
   {coordinate vector bundle}%
   {D}{0}%
\Symb%
   {derivative of map $f$}%
   {derivative of map}%
   {D}{0}%
\Symb%
   {derivative of map $f$}%
   {derivative of map inline}%
   {D}{0}%
\Symb%
   {derivative of order $n$}%
   {derivative of Order n}%
   {D}{0}%
\Symb%
   {derivative of order $n$}%
   {derivative of Order n inline}%
   {D}{0}%
\Symb%
   {derivative of second order}%
   {derivative of Second Order}%
   {D}{0}%
\Symb%
   {derivative of second order}%
   {derivative of Second Order inline}%
   {D}{0}%
\Symb%
   {diagonal in bundle $\Bundle A$}%
   {diagonal in bundle, 1}%
   {D}{0}%
\Symb%
   {differential of independent variable}%
   {differential of independent variable}%
   {D}{0}%
\Symb%
   {differential of map $f$}%
   {differential of map}%
   {D}{0}%
\Symb%
   {direct product of division rings $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
   {D}{0}%
\Symb%
   {double determinant of matrix $\bfA$}%
   {double determinant}%
   {D}{0}%
\Symb%
   {exterior differential}%
   {exterior differential}%
   {D}{0}%
\Symb%
   {the Fr\'echet \Ds derivative of map $f$ of division ring}%
   {Frechet Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {the G\^ateaux \dcr derivative of map $f$ of $D$\Hyph vector space $V$ to $D$\Hyph vector space $W$}%
   {Gateaux dcr derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {the G\^ateaux derivative of map $f$}%
   {Gateaux derivative of map}%
   {D}{0}%
\Symb%
   {the G\^ateaux derivative of map $f$}%
   {Gateaux derivative of map, fraction}%
   {D}{0}%
\Symb%
   {the G\^ateaux derivative of order $n$}%
   {Gateaux derivative of Order n}%
   {D}{0}%
\Symb%
   {the G\^ateaux derivative of order $n$ of map $f$ of division ring}%
   {Gateaux derivative of Order n, division ring}%
   {D}{0}%
\Symb%
   {the G\^ateaux derivative of order $n$ of map $f$ of algebra}%
   {Gateaux derivative of Order n, fraction, algebra}%
   {D}{0}%
\Symb%
   {the G\^ateaux derivative of order $n$ of map $f$ of division ring}%
   {Gateaux derivative of Order n, fraction, division ring}%
   {D}{0}%
\Symb%
   {the G\^ateaux derivative of second order}%
   {Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {the G\^ateaux derivative of second order of mapping $f$ of algebra}%
   {Gateaux derivative of Second Order, fraction, algebra}%
   {D}{0}%
\Symb%
   {the G\^ateaux derivative of second order of map $f$ of division ring}%
   {Gateaux derivative of Second Order, fraction, division ring}%
   {D}{0}%
\Symb%
   {the G\^ateaux differential of map $f$}%
   {Gateaux differential of map, vector}%
   {D}{0}%
\Symb%
   {the G\^ateaux \Ds derivative of map $f$ of division ring $D$}%
   {Gateaux Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {the G\^ateaux Jacobian of map of $D$\Hyph vector space}%
   {Gateaux Jacobian of map, D vector space}%
   {D}{0}%
\Symb%
   {the G\^ateaux partial \dcr derivative of map $f^{\gi b}$ with respect to variable $v^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {the G\^ateaux partial \dcr derivative of map $f^{\gi b}$ with respect to variable $v^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {the G\^ateaux partial \dcr derivative of map $f^{\gi b}$ with respect to variable $v^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {the G\^ateaux partial derivative}%
   {Gateaux partial derivative}%
   {D}{0}%
\Symb%
   {the G\^ateaux mixed partial derivative}%
   {Gateaux partial derivative of Second Order}%
   {D}{0}%
\Symb%
   {the G\^ateaux partial \rcd derivative of map $f^{\gi b}$ with respect to variable $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {the G\^ateaux partial \rcd derivative of map $f^{\gi b}$ with respect to variable $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {the G\^ateaux partial \rcd derivative of map $f^{\gi b}$ with respect to variable $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {the G\^ateaux \rcd derivative of map $f$ of $D$\hyph vector space $V$ to $D$\hyph vector space $W$}%
   {Gateaux rcd derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {the G\^ateaux \sD derivative of map $f$ of division ring $D$}%
   {Gateaux starD derivative of map, division ring}%
   {D}{0}%
\Symb%
   {Jacobi matrix of map}%
   {Jacobi matrix of map}%
   {D}{0}%
\Symb%
   {matrices vector space}%
   {matrices vector space}%
   {D}{0}%
\Symb%
   {Cartan derivative}%
   {overbrace D}%
   {D}{0}%
\Symb%
   {derivative}%
   {overline D}%
   {D}{0}%
\Symb%
   {partial derivative}%
   {partial derivative}%
   {D}{0}%
\Symb%
   {partial derivative of second order}%
   {partial derivative of second order}%
   {D}{0}%
\Symb%
   {derivative $e_{(k)}$}%
   {partial(k)}%
   {D}{0}%
\Symb%
   {product of map over scalar}%
   {product of map over scalar}%
   {D}{0}%
\Symb%
   {set of vectors generated by vector $v$}%
   {set of vectors generated by vector}%
   {D}{0}%
\Symb%
   {speed of deviation}%
   {speed of deviation}%
   {D}{0}%
\Symb%
   {standard component of derivative}%
   {standard component of derivative}%
   {D}{0}%
\Symb%
   {standard component of the G\^ateaux derivative}%
   {standard component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {vector space type}%
   {vector space type}%
   {D}{0}%

\SetIndexSpace%E%0
\Symb%
   {affine basis}%
   {Affine Basis}%
   {E}{0}%
\Symb%
   {basis}%
   {Basis}%
   {E}{0}%
\Symb%
   {basis for module}%
   {basis for module}%
   {E}{0}%
\Symb%
   {basis in vector space $\Vector V$}%
   {basis in V}%
   {E}{0}%
\Symb%
   {basis of $D$\Hyph module $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
   {E}{0}%
\Symb%
   {basis manifold}%
   {basis manifold}%
   {E}{0}%
\Symb%
   {basis for vector space}%
   {basis of vector space}%
   {E}{0}%
\Symb%
   {basis for \crd vector space}%
   {basis, crd vector space}%
   {E}{0}%
\Symb%
   {basis for \dcr vector space}%
   {basis, dcr vector space}%
   {E}{0}%
\Symb%
   {basis for \drc vector space}%
   {basis, drc vector space}%
   {E}{0}%
\Symb%
   {basis for \rcd vector space}%
   {basis, rcd vector space}%
   {E}{0}%
\Symb%
   {basis for vector bundle}%
   {basis, vector bundle}%
   {E}{0}%
\Symb%
   {basis of $(n)$\hyph vector space}%
   {basis,n vector space}%
   {E}{0}%
\Symb%
   {Cartesian power of total spaces}%
   {Cartesian power of total spaces}%
   {E}{0}%
\Symb%
   {Cartesian product of total spaces}%
   {Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {central affine basis}%
   {Central Affine Basis}%
   {E}{0}%
\Symb%
   {\CR exponent}%
   {CR exponent}%
   {E}{0}%
\Symb%
   {form of reference frame}%
   {dual forms, reference frame}%
   {E}{0}%
\Symb%
   {Euclid space}%
   {Euclid space}%
   {E}{0}%
\Symb%
   {Euclid space}%
   {Euclid space, division ring}%
   {E}{0}%
\Symb%
   {exponent}%
   {exponent}%
   {E}{0}%
\Symb%
   {Hamel basis}%
   {Hamel basis}%
   {E}{0}%
\Symb%
   {identical transformation of bundle}%
   {identical transformation of bundle}%
   {E}{0}%
\Symb%
   {map of conjugation}%
   {map of conjugation}%
   {E}{0}%
\Symb%
   {linear automorphism of quaternioin algebra}%
   {mapping E, quaternion}%
   {E}{0}%
\Symb%
   {linear automorphism of quaternioin algebra}%
   {mapping E_1, quaternion}%
   {E}{0}%
\Symb%
   {linear automorphism of quaternioin algebra}%
   {mapping E_2, quaternion}%
   {E}{0}%
\Symb%
   {Jacobian matrix of maps of conjugation}%
   {maps of conjugation, Jacobian matrix}%
   {E}{0}%
\Symb%
   {orthonornal basis}%
   {Orthonornal Basis}%
   {E}{0}%
\Symb%
   {image of basis $\Basis e$ under passive transformation $S$}%
   {passive transformation of basis}%
   {E}{0}%
\Symb%
   {pseudo Euclid space}%
   {pseudo Euclid space}%
   {E}{0}%
\Symb%
   {pseudo Euclid space}%
   {pseudo Euclid space, division ring}%
   {E}{0}%
\Symb%
   {quasiexponent}%
   {quasiexponent}%
   {E}{0}%
\Symb%
   {quaternion algebra over the field $F$}%
   {quaternion algebra over the field}%
   {E}{0}%
\Symb%
   {quaternion division algebra over the field}%
   {quaternion division algebra over the fieldL}%
   {E}{0}%
\Symb%
   {\RC exponent}%
   {RC exponent}%
   {E}{0}%
\Symb%
   {reduced Cartesian product of total spaces}%
   {reduced Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {Schauder basis}%
   {Schauder basis}%
   {E}{0}%
\Symb%
   {set of \CR eigenvalues}%
   {set of cr-eigenvalues}%
   {E}{0}%
\Symb%
   {set of endomorphisms}%
   {set of endomorphisms}%
   {E}{0}%
\Symb%
   {set of \RC eigenvalues}%
   {set of rc-eigenvalues}%
   {E}{0}%
\Symb%
   {set of nonsingular \sT transformations of bundle $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {set of transformations of universal algebra}%
   {set of transformations}%
   {E}{0}%
\Symb%
   {set of nonsingular \Ts transformations of bundle $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {standard coordinates of basis}%
   {standard coordinates of basis}%
   {E}{0}%
\Symb%
   {standard coordinates of reference frame}%
   {standard coordinates of reference frame}%
   {E}{0}%
\Symb%
   {vector field of reference frame}%
   {vector field of reference frame}%
   {E}{0}%
\Symb%
   {vector of basis}%
   {vector of basis}%
   {E}{0}%

\SetIndexSpace%F%0
\Symb%
   {alternation of polylinear map}%
   {alternation of polylinear map}%
   {F}{0}%
\Symb%
   {component of linear map $f$ of division ring}%
   {component of linear map, division ring}%
   {F}{0}%
\Symb%
   {component of polylinear map}%
   {component of polylinear map}%
   {F}{0}%
\Symb%
   {conjugation transformation}%
   {conjugation transformation}%
   {F}{0}%
\Symb%
   {exterior product}%
   {exterior product}%
   {F}{0}%
\Symb%
   {fibered morphism from bundle $\Bundle A$ into $\Bundle B$}%
   {fibered morphism from A into B}%
   {F}{0}%
\Symb%
   {filter $\mathfrak{F}$ converges to set $A$}%
   {filter converges}%
   {F}{0}%
\Symb%
   {homomorphism of fibered universal algebras}%
   {homomorphism of fibered universal algebras}%
   {F}{0}%
\Symb%
   {inverse fibered correspondence}%
   {inverse fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {inverse reduced fibered correspondence}%
   {inverse reduced fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {map to Cartesian product}%
   {map to Cartesian product}%
   {F}{0}%
\Symb%
   {norm of functional}%
   {norm of functional}%
   {F}{0}%
\Symb%
   {norm of map}%
   {norm of map}%
   {F}{0}%
\Symb%
   {norm of polylinear map}%
   {norm of polymap}%
   {F}{0}%
\Symb%
   {norm of representation}%
   {norm of representation}%
   {F}{0}%
\Symb%
   {orbit of representation of the group}%
   {orbit of representation}%
   {F}{0}%
\Symb%
   {orthonormal basis}%
   {Orthonormal Basis, division ring}%
   {F}{0}%
\Symb%
   {quaternion algebra  over field ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
   {F}{0}%
\Symb%
   {reference frame}%
   {reference frame}%
   {F}{0}%
\Symb%
   {reference frame, extensive definition}%
   {reference frame, extensive definition}%
   {F}{0}%
\Symb%
   {standard component of biadditive map $f$ over field $F$}%
   {standard component of biadditive map, division ring}%
   {F}{0}%
\Symb%
   {standard component of linear map}%
   {standard component of linear map, G}%
   {F}{0}%
\Symb%
   {standard component of polylinear map}%
   {standard component of polylinear map}%
   {F}{0}%
\Symb%
   {standard component of quadratic map $f$ over field $F$}%
   {standard component of quadratic map, division ring}%
   {F}{0}%
\Symb%
   {standard component of tensor}%
   {standard component of tensor}%
   {F}{0}%
\Symb%
   {sum of maps}%
   {sum of maps}%
   {F}{0}%
\Symb%
   {symmetrization of polylinear map}%
   {symmetrization of polylinear map}%
   {F}{0}%

\SetIndexSpace%G%0
\Symb%
   {affine transformation group}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {affine transformation group}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {Cartesian product of groups $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
   {G}{0}%
\Symb%
   {\CR matrix group}%
   {cr-matrix group}%
   {G}{0}%
\Symb%
   {fibered little group of section $h$}%
   {fibered little group}%
   {G}{0}%
\Symb%
   {fibered stability group of section $h$}%
   {fibered stability group}%
   {G}{0}%
\Symb%
   {group of automorphisms of representation $f$}%
   {group of automorphisms of representation}%
   {G}{0}%
\Symb%
   {group of homomorphisms of vector space $\Vector V$}%
   {GV}%
   {G}{0}%
\Symb%
   {indefinite integral}%
   {indefinite integral}%
   {G}{0}%
\Symb%
   {left defined Lie algebra of Lie group}%
   {left defined Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {Lie algebra of Lie group}%
   {Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {linear transformation group}%
   {linear transformation group}%
   {G}{0}%
\Symb%
   {little group}%
   {little group}%
   {G}{0}%
\Symb%
   {orbit of effective Ts representation of group}%
   {orbit of effective starT representation of fibered group}%
   {G}{0}%
\Symb%
   {orbit of effective \Ts representation of fibered group}%
   {orbit of effective Tstar representation of fibered group}%
   {G}{0}%
\Symb%
   {\RC matrix group}%
   {rc-matrix group}%
   {G}{0}%
\Symb%
   {right defined Lie algebra of Lie group}%
   {right defined Lie algebra}%
   {G}{0}%
\Symb%
   {stability group}%
   {stability group}%
   {G}{0}%

\SetIndexSpace%H%0
\Symb%
   {Hadamard inverse of matrix}%
   {Hadamard inverse of matrix}%
   {H}{0}%
\Symb%
   {horizontal component of vector}%
   {horizontal component of vector}%
   {H}{0}%
\Symb%
   {horizontal subspace}%
   {horizontal subspace}%
   {H}{0}%
\Symb%
   {quaternion algebra}%
   {quaternion algebra}%
   {H}{0}%
\Symb%
   {quaternion algebra}%
   {quaternion algebra H a b}%
   {H}{0}%
\Symb%
   {set of homomorphisms}%
   {set of homomorphisms}%
   {H}{0}%

\SetIndexSpace%I%0
\Symb%
   {image of map}%
   {image of map}%
   {I}{0}%
\Symb%
   {infinitesimal generator of representation}%
   {infinitesimal generator i of representation}%
   {I}{0}%
\Symb%
   {infinitesimal generator of representation}%
   {infinitesimal generator of representation}%
   {I}{0}%
\Symb%
   {Lie group infinitesimal generators}%
   {Lie group infinitesimal generators}%
   {I}{0}%
\Symb%
   {map of conjugation}%
   {map of conjugation}%
   {I}{0}%
\Symb%
   {Jacobian matrix of maps of conjugation}%
   {maps of conjugation, Jacobian matrix}%
   {I}{0}%
\Symb%
   {vector module of algebra $A$}%
   {vector module of algebra}%
   {I}{0}%
\Symb%
   {vector module of ring $D$}%
   {vector module of ring}%
   {I}{0}%
\Symb%
   {vector of element $d$ of algebra}%
   {vector of algebra}%
   {I}{0}%
\Symb%
   {vector of element $d$ of ring}%
   {vector of ring}%
   {I}{0}%

\SetIndexSpace%J%0
\Symb%
   {closure operator of representation $f$}%
   {closure operator, representation}%
   {J}{0}%
\Symb%
   {closure operator of tower of representations $\Vector f$}%
   {closure operator, tower of representations}%
   {J}{0}%
\Symb%
   {Jacobian matrix of right shift}%
   {Ea, quaternion, Jacobian matrix}%
   {J}{0}%
\Symb%
   {map of conjugation}%
   {map of conjugation}%
   {J}{0}%
\Symb%
   {Jacobian matrix of maps of conjugation}%
   {maps of conjugation, Jacobian matrix}%
   {J}{0}%
\Symb%
   {subrepresentation generated by generating set $X$}%
   {subrepresentation generated by set}%
   {J}{0}%
\Symb%
   {tower of subrepresentations of tower of representations $\Vector f$ generated by tuple of sets $\VX X$}%
   {subrepresentation generated by tuple of sets}%
   {J}{0}%

\SetIndexSpace%K%0
\Symb%
   {kernel of group\Hyph homomorphism}%
   {ker group-homomorphism}%
   {K}{0}%
\Symb%
   {kernel of homomorphism}%
   {kernel of homomorphism}%
   {K}{0}%
\Symb%
   {kernel of linear map}%
   {kernel of linear map}%
   {K}{0}%
\Symb%
   {kernel of map}%
   {kernel of map}%
   {K}{0}%
\Symb%
   {map of conjugation}%
   {map of conjugation}%
   {K}{0}%
\Symb%
   {Jacobian matrix of maps of conjugation}%
   {maps of conjugation, Jacobian matrix}%
   {K}{0}%

\SetIndexSpace%L%0
\Symb%
   {Cartesian power of systems of subsets}%
   {Cartesian power of systems of subsets}%
   {L}{0}%
\Symb%
   {Cartesian product of systems of subsets}%
   {Cartesian product of systems of subsets}%
   {L}{0}%
\Symb%
   {left $ij$th cofactor of entry of matrix}%
   {left cofactor, matrix}%
   {L}{0}%
\Symb%
   {left double $ij$th cofactor of entry of matrix}%
   {left double cofactor}%
   {L}{0}%
\Symb%
   {left shift}%
   {left shift}%
   {L}{0}%
\Symb%
   {left vector space of algebra $A$}%
   {left vector space of algebra A}%
   {L}{0}%
\Symb%
   {left vector space of maps}%
   {left vector space of maps B->A}%
   {L}{0}%
\Symb%
   {Lie derivative of connection}%
   {Lie derivative of connection}%
   {L}{0}%
\Symb%
   {Lie derivative of metric}%
   {Lie derivative of metric}%
   {L}{0}%
\Symb%
   {limit of correspondence $\Phi$ with respect to the filter $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
   {L}{0}%
\Symb%
   {limit of sequence}%
   {limit of sequence}%
   {L}{0}%
\Symb%
   {linear combination}%
   {linear combination}%
   {L}{0}%
\Symb%
   {module of skew symmetric polylinear maps}%
   {module of skew symmetric polylinear maps}%
   {L}{0}%
\Symb%
   {passive transformation}%
   {passive transformation}%
   {L}{0}%
\Symb%
   {$D$\Hyph module of continuous linear mappings of normed $D$\Hyph module $A_1$ into normed $D$\Hyph module $A_2$}%
   {set continuous linear mappings, module}%
   {L}{0}%
\Symb%
   {set of continuous linear maps}%
   {set continuous linear maps, vector}%
   {L}{0}%
\Symb%
   {set of continuous polylinear maps}%
   {set continuous polylinear maps}%
   {L}{0}%
\Symb%
   {set of linear maps}%
   {set linear maps}%
   {L}{0}%
\Symb%
   { inverse matrices}%
   {set of inverse matrices}%
   {L}{0}%
\Symb%
   {set of left-side nonsingular transformations of universal algebra $M$}%
   {set of left-side nonsingular transformations}%
   {L}{0}%
\Symb%
   {set of polylinear maps}%
   {set polylinear maps}%
   {L}{0}%
\Symb%
   {set of $n$\hyph linear maps}%
   {set polylinear maps An}%
   {L}{0}%
\Symb%
   {set of polylinear maps}%
   {set polylinear maps, D vector space}%
   {L}{0}%
\Symb%
   {set of polylinear maps of algebras $A_1$, ..., $A_n$ into algebra $A$}%
   {set polylinear maps, finite dimensional algebra}%
   {L}{0}%

\SetIndexSpace%M%0
\Symb%
   {set of left-side transformations of the universal algebra $M$}%
   {set of left-side transformations}%
   {M}{0}%
\Symb%
   {set of maps to $\Omega$\Hyph group $A$}%
   {set of maps to Omega group}%
   {M}{0}%
\Symb%
   {set of right-side transformations of universal algebra $M$}%
   {set of right-side transformations}%
   {M}{0}%
\Symb%
   {space of orbits of \Ts{G}representation}%
   {space of orbits of G* representation}%
   {M}{0}%

\SetIndexSpace%N%0
\Symb%
   {norm of quaternion $x$}%
   {norm, quaternion algebra}%
   {N}{0}%
\Symb%
   {nucleus of $D$\Hyph algebra $A$}%
   {nucleus of algebra}%
   {N}{0}%

\SetIndexSpace%O%0
\Symb%
   {coordinates of geometric object}%
   {coordinates of geometric object}%
   {O}{0}%
\Symb%
   {geometric object}%
   {geometric object}%
   {O}{0}%
\Symb%
   {octonion algebra}%
   {octonion algebra}%
   {O}{0}%
\Symb%
   {orbit of representation of fibered group $\Bundle G$}%
   {orbit of representation of fibered group}%
   {O}{0}%
\Symb%
   {tensor product}%
   {tensor product}%
   {O}{0}%

\SetIndexSpace%P%0
\Symb%
   {bundle}%
   {bundle}%
   {P}{0}%
\Symb%
   {bundle of level $2$}%
   {bundle of level 2}%
   {P}{0}%
\Symb%
   {bundle of level $n$}%
   {bundle of level n}%
   {P}{0}%
\Symb%
   {Cartesian power $n$ of bundle $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
   {P}{0}%
\Symb%
   {Cartesian product of bundles}%
   {Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {passive representation in basis manifold}%
   {passive representation in basis manifold}%
   {P}{0}%
\Symb%
   {reduced Cartesian product of bundles}%
   {reduced Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {set of nonsingular \sT transformations of bundle $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
   {P}{0}%
\Symb%
   {set of nonsingular \Ts transformations of bundle $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%
   {P}{0}%

\SetIndexSpace%R%0
\Symb%
   {active transformation}%
   {active transformation}%
   {R}{0}%
\Symb%
   {Cartan curvature}%
   {Cartan curvature}%
   {R}{0}%
\Symb%
   {\CR rank of matrix}%
   {cr-rank of matrix}%
   {R}{0}%
\Symb%
   {diagonal in bundle  $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
   {R}{0}%
\Symb%
   {diagonal in bundle $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
   {R}{0}%
\Symb%
   {image of $m$ under endomorphism $R$ of effective representation}%
   {endomorphism image, effective representation}%
   {R}{0}%
\Symb%
   {image of tuple $\VX a$ under endomorphism $\VX r$ of tower of effective representations}%
   {endomorphism image, tower of effective representations}%
   {R}{0}%
\Symb%
   {curvature}%
   {GLn curvature_overline}%
   {R}{0}%
\Symb%
   {product of rings of sets}%
   {product of rings of sets}%
   {R}{0}%
\Symb%
   {$\RCcirc$\Hyph product of matrices of maps}%
   {rc product of matrices of maps}%
   {R}{0}%
\Symb%
   {\RC rank of matrix}%
   {rc-rank of matrix}%
   {R}{0}%
\Symb%
   {right $ij$th cofactor of entry of matrix}%
   {right cofactor, matrix}%
   {R}{0}%
\Symb%
   {right double $ij$th cofactor of entry of matrix}%
   {right double cofactor}%
   {R}{0}%
\Symb%
   {right shift}%
   {right shift}%
   {R}{0}%
\Symb%
   {right vector space of algebra $A$}%
   {right vector space of algebra A}%
   {R}{0}%
\Symb%
   {right vector space of maps}%
   {right vector space of maps B->A}%
   {R}{0}%
\Symb%
   {$i$th row determinant of matrix $\bfA$}%
   {row determinant}%
   {R}{0}%
\Symb%
   {scalar algebra of algebra $A$}%
   {scalar algebra of algebra}%
   {R}{0}%
\Symb%
   {scalar algebra of ring $D$}%
   {scalar algebra of ring}%
   {R}{0}%
\Symb%
   {scalar of element $d$ of algebra}%
   {scalar of algebra}%
   {R}{0}%
\Symb%
   {scalar of element $d$ of ring}%
   {scalar of ring}%
   {R}{0}%
\Symb%
   { inverse matrices}%
   {set of inverse matrices}%
   {R}{0}%
\Symb%
   {set of right-side nonsingular transformations of universal algebra $M$}%
   {set of right-side nonsingular transformations}%
   {R}{0}%
\Symb%
   {spherical coordinates}%
   {spherical coordinates}%
   {R}{0}%

\SetIndexSpace%S%0
\Symb%
   {composition of fibered correspondences}%
   {composition of fibered correspondences}%
   {S}{0}%
\Symb%
   {hyperbolic sine}%
   {hyperbolic sine}%
   {S}{0}%
\Symb%
   {inverse fibered correspondence}%
   {inverse fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {inverse reduced fibered correspondence}%
   {inverse reduced fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {Lebesgue integral}%
   {Lebesgue integral}%
   {S}{0}%
\Symb%
   {linear span in vector space}%
   {linear span, vector space}%
   {S}{0}%
\Symb%
   {image of basis $\VX  X$ under passive transformation $\VX s$}%
   {passive transformation of basis, tower of representations}%
   {S}{0}%
\Symb%
   {set of permutations}%
   {set of permutations}%
   {S}{0}%
\Symb%
   {set of transpositions}%
   {set of transpositions}%
   {S}{0}%
\Symb%
   {sine}%
   {sine}%
   {S}{0}%
\Symb%
   {symmetric group}%
   {symmetric group}%
   {S}{0}%

\SetIndexSpace%T%0
\Symb%
   {category of left-side representations}%
   {category of left-side representations}%
   {T}{0}%
\Symb%
   {tangent plane to Lie group $G$}%
   {tangent plane to Lie group}%
   {T}{0}%
\Symb%
   {trace of quaternion $x$}%
   {trace, quaternion algebra}%
   {T}{0}%

\SetIndexSpace%V%0
\Symb%
   {affine space}%
   {affine space}%
   {V}{0}%
\Symb%
   {conjugated affine space}%
   {conjugated affine space}%
   {V}{0}%
\Symb%
   {conjugated vector space}%
   {conjugated vector space}%
   {V}{0}%
\Symb%
   {coordinate vector space}%
   {coordinate vector space}%
   {V}{0}%
\Symb%
   {coordinates in vector space}%
   {coordinates in vector space}%
   {V}{0}%
\Symb%
   {direct product of $\RCstar D_i$\hyph vector spaces $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
   {V}{0}%
\Symb%
   {dual space of \rcd vector space $\Vector V$}%
   {dual space of rcd vector space}%
   {V}{0}%
\Symb%
   {hermitian conjugated vector}%
   {hermitian conjugated vector}%
   {V}{0}%
\Symb%
   {linear composition of vectors}%
   {linear composition of vectors}%
   {V}{0}%
\Symb%
   {set of vectors generated by vector $v$}%
   {set of vectors generated by vector}%
   {V}{0}%
\Symb%
   {vector space}%
   {V}%
   {V}{0}%
\Symb%
   {vector space of initial values of system of differential equations}%
   {vector space of initial values}%
   {V}{0}%
\Symb%
   {vector space of solutions of system of differential equations}%
   {vector space of solutions}%
   {V}{0}%
\Symb%
   {vertical component of vector}%
   {vertical component of vector}%
   {V}{0}%
\Symb%
   {vertical subspace}%
   {vertical subspace}%
   {V}{0}%

\SetIndexSpace%W%0
\Symb%
   {set of coordinates of representation $J(f,X)$}%
   {coordinate set of representation}%
   {W}{0}%
\Symb%
   {set of tuples of coordinates of tower of representations $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
   {W}{0}%
\Symb%
   {coordinates of basis $X'$ relative to basis $X$ of representation}%
   {coordinates of basis relative to basis, representation}%
   {W}{0}%
\Symb%
   {coordinates of element $m$ relative to set $X$}%
   {coordinates of element relative to set, representation}%
   {W}{0}%
\Symb%
   {tuple of coordinates of element $\Vector a*$ relative to tuple of sets $\VX X$}%
   {coordinates of element, tower of representations}%
   {W}{0}%
\Symb%
   {coordinates of element $m$ of representation $f$ relative to set $X$}%
   {coordinates relative to set}%
   {W}{0}%
\Symb%
   {geometric object}%
   {geometric object}%
   {W}{0}%
\Symb%
   {set of tuples of $\Omega$\Hyph words}%
   {set of tuples of Omega words}%
   {W}{0}%
\Symb%
   {set of coordinates of set $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
   {W}{0}%
\Symb%
   {coordinates of tuple of sets $\VX B$ relative to tuple of sets $\VX X$}%
   {subset of coordinates of tower of representations}%
   {W}{0}%
\Symb%
   {coordinates of set $B_k$ relative to tuple of sets $\VX X$}%
   {subset of coordinates of tower of representations, k}%
   {W}{0}%
\Symb%
   {set of $\Omega_2$\Hyph words representing set $B\subset J(f,X)$}%
   {subset of words of representation}%
   {W}{0}%
\Symb%
   {superposition of coordinates}%
   {superposition of coordinates}%
   {W}{0}%
\Symb%
   {superposition of coordinates of the tower of representations $\Vector f$ and the element $\VX a$}%
   {superposition of coordinates, tower of representations}%
   {W}{0}%
\Symb%
   {tuple of $\Omega$\Hyph words}%
   {tuple of Omega words}%
   {W}{0}%
\Symb%
   {$\Omega_2$\Hyph word representing element $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {set of $\Omega_2$\Hyph words of representation $J(f,X)$}%
   {word set of representation}%
   {W}{0}%
\Symb%
   {set of tuples of $\VX{\Omega}$\Hyph words of tower of representations $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
   {W}{0}%
\Symb%
   {tuple of words of element $\Vector a*$ relative to tuple of sets $\VX X$}%
   {words of element, tower of representations}%
   {W}{0}%

\SetIndexSpace%X%0
\Symb%
   {conjugate of quaternion $x$}%
   {conjugate of quaternion}%
   {X}{0}%
\Symb%
   {local basis of affine space}%
   {local basis of affine space}%
   {X}{0}%
\Symb%
   {Wronskian matrix}%
   {Wronskian matrix}%
   {X}{0}%
\Symb%
   {anholonomic coordinate}%
   {x(k)}%
   {X}{0}%

\SetIndexSpace%Z%0
\Symb%
   {center of $A$\Hyph number}%
   {center of A number}%
   {Z}{0}%
\Symb%
   {center of $D$\Hyph algebra $A$}%
   {center of algebra}%
   {Z}{0}%
\Symb%
   {center of ring $D$}%
   {center of ring}%
   {Z}{0}%

\SetIndexSpace%Delta%1
\Symb%
   {deviation of trajectories}%
   {deviation of trajectories}%
   {Delta}{1}%
\Symb%
   {identical transformation}%
   {identical transformation}%
   {Delta}{1}%
\Symb%
   {image of vector $\Vector e_k\in\Basis e$ under isomorphism to coordinate vector space}%
   {image of vector e_k, coordinate vector space}%
   {Delta}{1}%
\Symb%
   {Kronecker symbol}%
   {Kronecker symbol}%
   {Delta}{1}%

\SetIndexSpace%Gamma%1
\Symb%
   {anholonomic coordinates of connection}%
   {anholonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {Cartan symbol}%
   {Cartan symbol}%
   {Gamma}{1}%
\Symb%
   {connection}%
   {conection overline}%
   {Gamma}{1}%
\Symb%
   {connection coefficients in $D$\Hyph affine space}%
   {connection coefficients, D affine space}%
   {Gamma}{1}%
\Symb%
   {connection in $D$\Hyph affine manifold}%
   {connection, affine manifold}%
   {Gamma}{1}%
\Symb%
   {$D$\Hyph affine connection coefficients on manifold}%
   {D affine connection coefficients, manifold}%
   {Gamma}{1}%
\Symb%
   {holonomic coordinates of connection}%
   {holonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {Cartan connection}%
   {overbrace Gamma i kl}%
   {Gamma}{1}%
\Symb%
   {set of sections of bundle}%
   {set of sections of bundle}%
   {Gamma}{1}%

\SetIndexSpace%Lambda%1
\Symb%
   {inverse operator to operator $\psi_l$}%
   {inverse operator to operator psi l}%
   {Lambda}{1}%
\Symb%
   {inverse operator to operator $\psi_r$}%
   {inverse operator to operator psi r}%
   {Lambda}{1}%

\SetIndexSpace%Mu%1
\Symb%
   {Cartesian product of measures}%
   {Cartesian product of measures}%
   {Mu}{1}%
\Symb%
   {power of measure}%
   {power of measure}%
   {Mu}{1}%
\Symb%
   {product of measures}%
   {product of measures}%
   {Mu}{1}%
\Symb%
   {product of measures}%
   {product of measures, otimes}%
   {Mu}{1}%

\SetIndexSpace%Omega%1
\Symb%
   {anholonomity object}%
   {anholonomity object}%
   {Omega}{1}%
\Symb%
   {definite integral}%
   {definite integral}%
   {Omega}{1}%
\Symb%
   {integral of differential $1$\Hyph form along path}%
   {integral of differential 1 form along path}%
   {Omega}{1}%
\Symb%
   {norm of operation}%
   {norm of operation}%
   {Omega}{1}%
\Symb%
   {operator domain}%
   {operator domain}%
   {Omega}{1}%
\Symb%
   {set of differential $p$\Hyph forms}%
   {set of differential p forms}%
   {Omega}{1}%
\Symb%
   {set of $n$\Hyph ary operations of $\Omega$\Hyph algebra}%
   {set of n-ary operations}%
   {Omega}{1}%
\Symb%
   {set of $n$\Hyph ary operators}%
   {set of n-ary operators}%
   {Omega}{1}%

\SetIndexSpace%Psi%1
\Symb%
   {left basic operator of Lie group over algebra $A$}%
   {L basic operator of Lie group over algebra A}%
   {Psi}{1}%
\Symb%
   {left basic operator of group Lie}%
   {Lie Basic Operator L}%
   {Psi}{1}%
\Symb%
   {left basic operator of Lie 1-parameter group}%
   {Lie Basic Operator L, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {left basic operator of Lie 1-parameter group over algebra $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {right basic operator of group Lie}%
   {Lie Basic Operator R}%
   {Psi}{1}%
\Symb%
   {right basic operator of Lie 1-parameter group}%
   {Lie Basic Operator R, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {right basic operator of Lie 1-parameter group over algebra $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {right basic operator of Lie group over algebra $A$}%
   {R basic operator of Lie group over algebra A}%
   {Psi}{1}%

\SetIndexSpace%Sigma%1
\Symb%
   {fibered subset}%
   {fibered subset}%
   {Sigma}{1}%
\Symb%
   {parity of permutation}%
   {parity of permutation}%
   {Sigma}{1}%
\Symb%
   {subbundle}%
   {subbundle}%
   {Sigma}{1}%

\SetIndexSpace%Nabla%2
\Symb%
   {Cartan derivative}%
   {overbrace nabla_l}%
   {Nabla}{2}%
\Symb%
   {derivative}%
   {overline nabla_l, definition 1}%
   {Nabla}{2}%

\SetIndexSpace%Phi%1
\Symb%
   {Lie group composition law}%
   {Lie group composition law}%
   {Phi}{1}%
\Symb%
   {restriction of correspondence $\Phi$ to set $C$}%
   {restriction of correspondence}%
   {Phi}{1}%

\SetIndexSpace%Pi%1
\Symb%
   {Cartesian product of bundles}%
   {Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {Cartesian product of groups $G_i$, $i\in I$}%
   {Cartesian product of groups}%
   {Pi}{1}%
\Symb%
   {Cartesian product of groups $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
   {Pi}{1}%
\Symb%
   {Cartesian product of total spaces}%
   {Cartesian product of total spaces, definition 2}%
   {Pi}{1}%
\Symb%
   {coproduct in category}%
   {coproduct in category}%
   {Pi}{1}%
\Symb%
   {direct product of division rings $D_i$, $i\in I$}%
   {direct product of division rings}%
   {Pi}{1}%
\Symb%
   {direct product of division rings $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
   {Pi}{1}%
\Symb%
   {direct product of $\RCstar D_i$\hyph vector spaces $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
   {Pi}{1}%
\Symb%
   {direct product of $\RCstar D_i$\hyph vector spaces}%
   {direct product, rcd vector space, i 1 n}%
   {Pi}{1}%
\Symb%
   {product in category}%
   {product in category}%
   {Pi}{1}%
\Symb%
   {reduced Cartesian product of bundles}%
   {reduced Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {reduced Cartesian product of total spaces}%
   {reduced Cartesian product of total spaces, definition 2}%
   {Pi}{1}%

\CloseIndex


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {прямая сумма}%
   {direct sum}%
   {0}{0}%
\Symb%
   {единичный интервал}%
   {unit interval}%
   {0}{0}%

\SetIndexSpace%A%0
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
   {A}{0}%
\Symb%
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
   {A}{0}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
   {A}{0}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
   {A}{0}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
   {A}{0}%
\Symb%
   {аффинное пространство}%
   {An}%
   {A}{0}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
   {A}{0}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
   {A}{0}%
\Symb%
   {категория представлений}%
   {category of representations}%
   {A}{0}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
   {A}{0}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
   {A}{0}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
   {A}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
   {A}{0}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
   {A}{0}%
\Symb%
   {координаты ассоциатора}%
   {coordinates of associator}%
   {A}{0}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
   {A}{0}%
\Symb%
   {\crd вектор}%
   {crd vector}%
   {A}{0}%
\Symb%
   {\CR обратная матрица}%
   {cr-inverse matrix}%
   {A}{0}%
\Symb%
   {\CR произведение}%
   {cr-product}%
   {A}{0}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
   {A}{0}%
\Symb%
   {\drc вектор}%
   {drc vector}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
   {A}{0}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
   {A}{0}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
   {A}{0}%
\Symb%
   {изоморфны}%
   {isomorphic}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {левая дробь}%
   {left fraction}%
   {A}{0}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
   {A}{0}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
   {A}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {A}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {minor matrix}%
   {A}{0}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
   {A}{0}%
\Symb%
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
   {A}{0}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
   {A}{0}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear map}%
   {A}{0}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
   {A}{0}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
   {A}{0}%
\Symb%
   {главный идеал}%
   {principal ideal}%
   {A}{0}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
   {A}{0}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
   {A}{0}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
   {A}{0}%
\Symb%
   {\RC обратная матрица}%
   {rc-inverse matrix}%
   {A}{0}%
\Symb%
   {\RC произведение}%
   {rc-product}%
   {A}{0}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
   {A}{0}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
   {A}{0}%
\Symb%
   {множество аддитивных отображений}%
   {set additive maps}%
   {A}{0}%
\Symb%
   {множество однородных многочленов}%
   {set of homogeneous polynomials}%
   {A}{0}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
   {A}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {A}{0}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
   {A}{0}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
   {A}{0}%
\Symb%
   {симплекс}%
   {simplex}%
   {A}{0}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
   {A}{0}%
\Symb%
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
   {A}{0}%
\Symb%
   {пространство орбит представления}%
   {space of orbits of representation}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного правостороннего представления}%
   {space of orbits of right-side representation}%
   {A}{0}%
\Symb%
   {квадратный корень}%
   {square root}%
   {A}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {A}{0}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
   {A}{0}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
   {A}{0}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
   {A}{0}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
   {A}{0}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
   {B}{0}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
   {B}{0}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
   {B}{0}%
\Symb%
   {каноническое частное от деления}%
   {canonical remainder of the division}%
   {B}{0}%
\Symb%
   {декартова степень}%
   {Cartesian power}%
   {B}{0}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
   {B}{0}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
   {B}{0}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
   {B}{0}%
\Symb%
   {замыкание множества}%
   {closure of set}%
   {B}{0}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
   {B}{0}%
\Symb%
   {структура подпредставлений}%
   {lattice of subrepresentations}%
   {B}{0}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
   {B}{0}%
\Symb%
   {открытый шар}%
   {open ball}%
   {B}{0}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {B}{0}%
\Symb%
   {правая дробь}%
   {right fraction}%
   {B}{0}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
   {B}{0}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
   {C}{0}%
\Symb%
   {класс непрерывности}%
   {class Cn}%
   {C}{0}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
   {C}{0}%
\Symb%
   {косинус}%
   {cosine}%
   {C}{0}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
   {C}{0}%
\Symb%
   {гиперболический косинус}%
   {hyperbolic cosine}%
   {C}{0}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
   {C}{0}%
\Symb%
   {структурные константы}%
   {structural constants}%
   {C}{0}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
   {D}{0}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
   {D}{0}%
\Symb%
   {компонента производной отображения $f(x)$}%
   {component of derivative}%
   {D}{0}%
\Symb%
   {компонента производной второго порядка отображения $f(x)$}%
   {component of derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
   {D}{0}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
   {D}{0}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
   {D}{0}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
   {D}{0}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
   {D}{0}%
\Symb%
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map inline}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n inline}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order inline}%
   {D}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
   {D}{0}%
\Symb%
   {дифференциал независимой переменной}%
   {differential of independent variable}%
   {D}{0}%
\Symb%
   {дифференциал отображения $f$}%
   {differential of map}%
   {D}{0}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
   {D}{0}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
   {D}{0}%
\Symb%
   {внешний дифференциал}%
   {exterior differential}%
   {D}{0}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
   {D}{0}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
   {D}{0}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
   {D}{0}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
   {D}{0}%
\Symb%
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
   {D}{0}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
   {D}{0}%
\Symb%
   {производная Картана}%
   {overbrace D}%
   {D}{0}%
\Symb%
   {производная}%
   {overline D}%
   {D}{0}%
\Symb%
   {частная производная}%
   {partial derivative}%
   {D}{0}%
\Symb%
   {частная производная второго порядка}%
   {partial derivative of second order}%
   {D}{0}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
   {D}{0}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
   {D}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {D}{0}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
   {D}{0}%
\Symb%
   {стандартная компонента производной}%
   {standard component of derivative}%
   {D}{0}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%
   {D}{0}%

\SetIndexSpace%E%0
\Symb%
   {аффинный базис}%
   {Affine Basis}%
   {E}{0}%
\Symb%
   {базис}%
   {Basis}%
   {E}{0}%
\Symb%
   {базис модуля}%
   {basis for module}%
   {E}{0}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
   {E}{0}%
\Symb%
   {многообразие базисов}%
   {basis manifold}%
   {E}{0}%
\Symb%
   {базис векторного пространства}%
   {basis of vector space}%
   {E}{0}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
   {E}{0}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
   {E}{0}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
   {E}{0}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
   {E}{0}%
\Symb%
   {базис в векторного расслоения}%
   {basis, vector bundle}%
   {E}{0}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
   {E}{0}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
   {E}{0}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
   {E}{0}%
\Symb%
   {\CR экспонента}%
   {CR exponent}%
   {E}{0}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
   {E}{0}%
\Symb%
   {экспонента}%
   {exponent}%
   {E}{0}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
   {E}{0}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
   {E}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
   {E}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {E}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
   {E}{0}%
\Symb%
   {образ базиса $\Basis e$ при пассивном преобразовании $S$}%
   {passive transformation of basis}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
   {E}{0}%
\Symb%
   {квазиэкспонента}%
   {quasiexponent}%
   {E}{0}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
   {E}{0}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
   {E}{0}%
\Symb%
   {\RC экспонента}%
   {RC exponent}%
   {E}{0}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
   {E}{0}%
\Symb%
   {множество \CR собственных значений}%
   {set of cr-eigenvalues}%
   {E}{0}%
\Symb%
   {множество эндоморфизмов}%
   {set of endomorphisms}%
   {E}{0}%
\Symb%
   {множество \RC собственных значений}%
   {set of rc-eigenvalues}%
   {E}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {множество преобразований универсальной алгебры}%
   {set of transformations}%
   {E}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
   {E}{0}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
   {E}{0}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
   {E}{0}%
\Symb%
   {вектор базиса}%
   {vector of basis}%
   {E}{0}%

\SetIndexSpace%F%0
\Symb%
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
   {F}{0}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
   {F}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
   {F}{0}%
\Symb%
   {преобразование сопряжения}%
   {conjugation transformation}%
   {F}{0}%
\Symb%
   {внешнее произведение}%
   {exterior product}%
   {F}{0}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
   {F}{0}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
   {F}{0}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
   {F}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
   {F}{0}%
\Symb%
   {норма функционала}%
   {norm of functional}%
   {F}{0}%
\Symb%
   {норма отображения}%
   {norm of map}%
   {F}{0}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
   {F}{0}%
\Symb%
   {норма представления}%
   {norm of representation}%
   {F}{0}%
\Symb%
   {орбита представления группы}%
   {orbit of representation}%
   {F}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
   {F}{0}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
   {F}{0}%
\Symb%
   {система отсчёта}%
   {reference frame}%
   {F}{0}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
   {F}{0}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
   {F}{0}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
   {F}{0}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
   {F}{0}%
\Symb%
   {сумма отображений}%
   {sum of maps}%
   {F}{0}%
\Symb%
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
   {F}{0}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
   {G}{0}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
   {G}{0}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
   {G}{0}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
   {G}{0}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
   {G}{0}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
   {G}{0}%
\Symb%
   {неопределённый интеграл}%
   {indefinite integral}%
   {G}{0}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
   {G}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {G}{0}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
   {G}{0}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
   {G}{0}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
   {G}{0}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
   {G}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {G}{0}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
   {H}{0}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
   {H}{0}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
   {H}{0}%
\Symb%
   {алгебра кватернионов}%
   {quaternion algebra}%
   {H}{0}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
   {H}{0}%
\Symb%
   {множество гомоморфизмов}%
   {set of homomorphisms}%
   {H}{0}%

\SetIndexSpace%I%0
\Symb%
   {образ отображения}%
   {image of map}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
   {I}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {I}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {I}{0}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
   {I}{0}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%
   {I}{0}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
   {J}{0}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
   {J}{0}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
   {J}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {J}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {J}{0}%
\Symb%
   {подпредставление, порождённое множеством образующих $X$}%
   {subrepresentation generated by set}%
   {J}{0}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
   {J}{0}%

\SetIndexSpace%K%0
\Symb%
   {ядро гомоморфизма групп}%
   {ker group-homomorphism}%
   {K}{0}%
\Symb%
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
   {K}{0}%
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%
   {K}{0}%
\Symb%
   {ядро отображения}%
   {kernel of map}%
   {K}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {K}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {K}{0}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
   {L}{0}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
   {L}{0}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
   {L}{0}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
   {L}{0}%
\Symb%
   {левый сдвиг}%
   {left shift}%
   {L}{0}%
\Symb%
   {левое векторное пространство алгебры $A$}%
   {left vector space of algebra A}%
   {L}{0}%
\Symb%
   {левое векторное пространство отображений}%
   {left vector space of maps B->A}%
   {L}{0}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
   {L}{0}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
   {L}{0}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
   {L}{0}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
   {L}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {L}{0}%
\Symb%
   {модуль косо симметричных полилинейных отображений}%
   {module of skew symmetric polylinear maps}%
   {L}{0}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
   {L}{0}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
   {L}{0}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
   {L}{0}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
   {L}{0}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
   {L}{0}%
\Symb%
   {множество обратных матриц}%
   {set of inverse matrices}%
   {L}{0}%
\Symb%
   {множество левосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of left-side nonsingular transformations}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
   {L}{0}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
   {L}{0}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
   {M}{0}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
   {M}{0}%
\Symb%
   {множество правосторонних преобразований универсальной алгебры $M$}%
   {set of right-side transformations}%
   {M}{0}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
   {M}{0}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
   {N}{0}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
   {N}{0}%

\SetIndexSpace%O%0
\Symb%
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
   {O}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {O}{0}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
   {O}{0}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
   {O}{0}%
\Symb%
   {тензорное произведение}%
   {tensor product}%
   {O}{0}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
   {P}{0}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
   {P}{0}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
   {P}{0}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
   {P}{0}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {пассивное представление группы $GA(f)$ в многообразии базисов $\mathcal B[f]$}%
   {passive representation in basis manifold}%
   {P}{0}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
   {P}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%
   {P}{0}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
   {R}{0}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
   {R}{0}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
   {R}{0}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
   {R}{0}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
   {R}{0}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
   {R}{0}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
   {R}{0}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
   {R}{0}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
   {R}{0}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
   {R}{0}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
   {R}{0}%
\Symb%
   {правый сдвиг}%
   {right shift}%
   {R}{0}%
\Symb%
   {правое векторное пространство алгебры $A$}%
   {right vector space of algebra A}%
   {R}{0}%
\Symb%
   {правое векторное пространстао отображений}%
   {right vector space of maps B->A}%
   {R}{0}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
   {R}{0}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
   {R}{0}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
   {R}{0}%
\Symb%
   {множество обратных матриц}%
   {set of inverse matrices}%
   {R}{0}%
\Symb%
   {множество правосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of right-side nonsingular transformations}%
   {R}{0}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%
   {R}{0}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
   {S}{0}%
\Symb%
   {гиперболический синус}%
   {hyperbolic sine}%
   {S}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {интеграл Лебега}%
   {Lebesgue integral}%
   {S}{0}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
   {S}{0}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of permutations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of transpositions}%
   {S}{0}%
\Symb%
   {синус}%
   {sine}%
   {S}{0}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%
   {S}{0}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений}%
   {category of left-side representations}%
   {T}{0}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
   {T}{0}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%
   {T}{0}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
   {V}{0}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
   {V}{0}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
   {V}{0}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
   {V}{0}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
   {V}{0}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
   {V}{0}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
   {V}{0}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
   {V}{0}%
\Symb%
   {линейная комбинация векторов}%
   {linear composition of vectors}%
   {V}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {V}{0}%
\Symb%
   {векторное пространство}%
   {V}%
   {V}{0}%
\Symb%
   {векторное пространство начальных значений системы дифференциальных уравнений}%
   {vector space of initial values}%
   {V}{0}%
\Symb%
   {векторное пространство решений системы дифференциальных уравнений}%
   {vector space of solutions}%
   {V}{0}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
   {V}{0}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%
   {V}{0}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
   {W}{0}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
   {W}{0}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates relative to set}%
   {W}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {W}{0}%
\Symb%
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
   {W}{0}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
   {W}{0}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
   {W}{0}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат}%
   {superposition of coordinates}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
   {W}{0}%
\Symb%
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
   {W}{0}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
   {W}{0}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%
   {W}{0}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
   {X}{0}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
   {X}{0}%
\Symb%
   {матрица Вронского}%
   {Wronskian matrix}%
   {X}{0}%
\Symb%
   {неголономная координата}%
   {x(k)}%
   {X}{0}%

\SetIndexSpace%Z%0
\Symb%
   {центр $A$\Hyph числа}%
   {center of A number}%
   {Z}{0}%
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
   {Z}{0}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%
   {Z}{0}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
   {Delta}{1}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
   {Delta}{1}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
   {Delta}{1}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%
   {Delta}{1}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
   {Gamma}{1}%
\Symb%
   {связность}%
   {conection overline}%
   {Gamma}{1}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
   {Gamma}{1}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
   {Gamma}{1}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
   {Gamma}{1}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
   {Gamma}{1}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%
   {Gamma}{1}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
   {Lambda}{1}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%
   {Lambda}{1}%

\SetIndexSpace%Mu%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
   {Mu}{1}%
\Symb%
   {степень меры}%
   {power of measure}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%
   {Mu}{1}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%
   {Omega}{1}%
\Symb%
   {определённый интеграл}%
   {definite integral}%
   {Omega}{1}%
\Symb%
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
   {Omega}{1}%
\Symb%
   {норма операции}%
   {norm of operation}%
   {Omega}{1}%
\Symb%
   {область операторов}%
   {operator domain}%
   {Omega}{1}%
\Symb%
   {множество дифференциальных $p$\Hyph форм}%
   {set of differential p forms}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операций $\Omega$\Hyph алгебры}%
   {set of n-ary operations}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операторов}%
   {set of n-ary operators}%
   {Omega}{1}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%
   {Psi}{1}%

\SetIndexSpace%Sigma%1
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
   {Sigma}{1}%
\Symb%
   {чётность перестановки}%
   {parity of permutation}%
   {Sigma}{1}%
\Symb%
   {подрасслоение}%
   {subbundle}%
   {Sigma}{1}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
   {Nabla}{2}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%
   {Nabla}{2}%

\SetIndexSpace%Phi%1
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%
   {Phi}{1}%
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
   {Phi}{1}%

\SetIndexSpace%Pi%1
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
   {Pi}{1}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
   {Pi}{1}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
   {Pi}{1}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%
   {Pi}{1}%

\CloseIndex


==> Text.2022.11.26.English.tex <==
%auto-ignore
\input{Text.\BookNumber.Eq}

\section{Product of matrices in non-commutative algebra}

Before we begin to consider vector space
over non\Hyph commutative division algebra $A$,
I recall that there are two operations of product of matrices
with entries from algebra $A$.

\ShowText{two matrix products}

\section{Homomorphism of Left \texorpdfstring{$A$}{A}-Vector Space}

Let $A$ be non\Hyph commutative division $D$\Hyph algebra.
Then we can consider left or right
$A$\Hyph vector space.
We may confine ourselves to considering of left $A$\Hyph vector space,
because statements for right $A$\Hyph vector space are similar.
\ShowEq{def left}

We will start by considering of the set of homomorphisms
of left $A$\Hyph vector space.
Homomorphism is a map that preserves the structure of algebra.
In particular, the theorem
\refTheorem{define homomorphism A module}{\SideNS(1)}
is true.

\ShowText{22 11 26 homomorphism}

%\section{Basis Manifold for Left \texorpdfstring{$A$}{A}-Vector Space}

\ShowText{22 11 26 Basis Manifold}

\section{Passive Transformation}

\ShowText{22 11 26 passive transformation}

\section{Geometric Object}

\ShowText{22 11 26 Geometric Object}

\section{Examples of Geometric Object}

\ShowEq{\DefCol}
According to the theorem
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
a vector is geometric object.
The set of endomorphisms of left $A$\Hyph  vector space
as well as the set of linear or polylinear
maps are $A$\Hyph vector space.
So we can ask if endomorphism or
polylinear map is geometric object.

\ShowText{22 11 26 Examples of Geometric Object}

\ShowEq{\DefCol}
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
an endomorphism of vector space is geometric object.
Indeed, when we change basis,
we see transformation of coordinates of vector and coordinates of endomorphism.
However, change of coordinates agreed and image of vector for
given endomorphism does not depend on choice of basis.

Let \eV be the basis of left vector space $V$ of columns.
Linear map
\ShowEq{f:A->B}aVV
has form
\DrawEq[avwnn]{b=f rco a}1
\DrawEq[ann]{a=(a11.nm matrix)}{}
with respect to the basis \eV[][.]
Since partial map $\aUD aij$
is linear map of $D$\Hyph algebra $A$,
then we can write linear map $\aUD aij$ as
\DrawEq[{}{}]{aij=.ox.}a
The equality
\ShowEq{vi=aij o wj}
follows from equalities
\newline
\FrameEqRef[avwnn]{b=f rco a}1
\newline
\FrameEqRef[{}{}]{aij=.ox.}a

\ShowSummary{Examples of Geometric Object}

\ShowEq{\DefCol}
Let passive transformation $g$ map the basis \eV[1]
into the basis \eV[2]
\DrawEq[12g{}]{e2i=aij e1j cr-cols}{1->2 l}

Let
\DrawEq[k]{aij=.ox.}k
be coordinates of linear map $a$
with respect to the basis \eV[k][,]
$k=1$, $2$.

Let
\ShowEq{vj wj}
be coordinates of vectors
$v$, $w$
with respect to the basis
\ShowEq{eV 12}
Then
\DrawEq[k]{wki=a ox vkj}k
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[v1v2g{}]{v1=v2*a left-cols}{v12g l}
\DrawEq[w1w2g{}]{v1=v2*a left-cols}{w12g l}
Equalities
\ShowEq{w2ig=a ox v2jg}
\DrawEq{w2i=a ox v2jg g-}1
follow from equalities
\newline
\FrameEqRef[v1v2g{}]{v1=v2*a left-cols}{v12g l}
\FrameEqRef[w1w2g{}]{v1=v2*a left-cols}{w12g l}
\newline
\FrameEqRef[1]{wki=a ox vkj}k
(k=1).
\newline
The equality
\DrawEq{a ox 2=g a ox 1 l}1
follows from equalities
\newline
\FrameEqRef[2]{wki=a ox vkj}k
(k=2),
\newline
\FrameEqRef{w2i=a ox v2jg g-}1

The equality
\DrawEq{a ox 2=g a ox 1 g l}1
follows from equalities
\newline
\FrameEqRef[v1v2g{}]{v1=v2*a left-cols}{v12g l}
\newline
\FrameEqRef{a ox 2=g a ox 1 l}1
\newline
From the equality
\eqRef{a ox 2=g a ox 1 g l}1
it follows that image of linear map
does not depend on choice of basis.

It is easy to see the similarity of equalities
\newline
\FrameEqRef[fg{\SideNS}{\Cols}]{f2=a f1 a-}{g \SideNS-\Cols}
\newline
and
\newline
\FrameEqRef{a ox 2=g a ox 1 l}1
\newline
If $D$\Hyph algebra $A$ is commutative,
then these equalities are the same.

\begin{\TheoremStyle}
\labelTheorem{Polylinear map is geometric object}
Polylinear map
\DrawEq[a{V^n}V{}]{f: A->B}{AnA}
is geometric object.
\end{\TheoremStyle}

\begin{proof}
Without loss of generality,
we consider proof of the theorem
for left $A$\Hyph vector space of columns.

\ShowEq{\DefCol}
Let passive transformation $g$ map the basis \eV[1]
into the basis \eV[2]
\DrawEq[12g{}]{e2i=aij e1j cr-cols}{1->2}

Let
\ShowEq{vij wj}
be coordinates of vectors
\ShowEq{set vi w}
with respect to the basis
\ShowEq{eV 12}
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[v{i1}v{i2}g{}]{v1=v2*a left-cols}{v12ig}
\DrawEq[w1w2g{}]{v1=v2*a left-cols}{w12g}

Let the set of tensors
\DrawEq{akj1n .ox.}1
be coordinates of polylinear map $a$
with respect to the basis \eV[k].
Then\,\footnote{\,
In this proof, there is no need to consider
posibility to change an order of variables in every term
since we are interested in single term.
If the order of variables in this term changes,
then we can change this order
before we start calculations in the proof.
}
\DrawEq[k]{wki=a ox vkj1n}k
Equalities
\ShowEq{w2ig=a ox v2j1ng}
\DrawEq{w2i=a ox v2j1ng g-}1
follow from equalities
\newline
\FrameEqRef[v{i1}v{i2}g{}]{v1=v2*a left-cols}{v12ig}
\FrameEqRef[w1w2g{}]{v1=v2*a left-cols}{w12g}
\newline
\FrameEqRef[1]{wki=a ox vkj1n}k
(k=1).
\newline
The equality
\DrawEq{a ox 2=g a ox 1}1
follows from equalities
\newline
\FrameEqRef[2]{wki=a ox vkj1n}k
(k=2),
\newline
\FrameEqRef{w2i=a ox v2j1ng g-}1

The equality
\DrawEq{a ox 2=g a ox 1 g}1
follows from equalities
\newline
\FrameEqRef[v{i1}v{i2}g{}]{v1=v2*a left-cols}{v12ig}
\newline
\FrameEqRef{a ox 2=g a ox 1}1
\newline
From the equality
\eqRef{a ox 2=g a ox 1 g}1
it follows that image of polylinear map
does not depend on choice of basis.
\end{proof}

We consider transformation skew-symmetric
polylinear map using the bilinear map as an example.
Let
\DrawEq{huv=12 huv-hvu}1
where the map $h$ has the form
\DrawEq{h=aubvc}1
The equality
\DrawEq{h=1/2 aubvc}1
follows from equalities
\eqRef{huv=12 huv-hvu}1,
\eqRef{h=aubvc}1.
If we consider determinant like expression
\DrawEq{star uv-vu}1
then the equality
\eqRef{h=1/2 aubvc}1
gets the form
\DrawEq{h=1/2 aubvc 1}1
Let passive transformation $g$ map the basis \eV[1]
into the basis \eV[2]
\DrawEq[12g{}]{e2i=aij e1j cr-cols}{1->2 skew}
The equality
\ShowEq{huv=12 huv-hvu 1}
follows from equalities
\newline
\FrameEqRef{h=1/2 aubvc}1
\DrawEq[w1w2g{}]{v1=v2*a left-cols}{w12g}
\DrawEq[u1u2g{}]{v1=v2*a left-cols}{u12g}
\DrawEq[u1u2g{}]{v1=v2*a left-cols}{v12g}
The equality
\ShowEq{huv=12 huv-hvu 2}
follows from the equality
\EqRef{huv=12 huv-hvu 1}.
The equality
\ShowEq{huv=12 huv-hvu 3}
follows from the equality
\newline
\FrameEqRef{h=1/2 aubvc}1
The equality
\ShowEq{huv=12 huv-hvu 4}
follows from the equality
\EqRef{huv=12 huv-hvu 2},
\EqRef{huv=12 huv-hvu 3}.
The equality
\DrawEq{huv=12 huv-hvu 5}1
follows from the equality
\eqRef{star uv-vu}1,
\EqRef{huv=12 huv-hvu 4}.


==> Text.2022.11.26.Eq.tex <==
%auto-ignore

\DefText{22 11 26 homomorphism}
{
\ShowEq{def left}
\ShowEq{\DefCol}

\ShowTheorem{define homomorphism A module}
\proofTheorem{\RefLinearMap}{define homomorphism A module}{\SideNS(1)}
\newline
\FrameCiteBib{\RefLinearMap}

\ShowDefinition{iso end aut morphism vector space}

\ShowTheorem{set of automorphisms}

\ShowText{coordinates of homomorphism}

%\ShowSummary{homomorphism of vector space}

\ColRowTheorem{homomorphism A module}
\AddIndex{}{matrix of homomorphism}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{homomorphism A module}{\SideNS-\Cols(1)}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{homomorphism A module}{\SideNS-\Cols(1)}
}

\ShowText{converse theorem is also true}

\TwoColText
{
\ShowEq{\DefCol}
\ShowTheorem{matrix generates A module homomorphism}{}{}1{}{}2
\proofTheorem{\RefLinearMap}{matrix generates homomorphism}{\SideNS-\Cols}
}
{
\ShowEq{\DefRow}
\ShowTheorem{matrix generates A module homomorphism}{}{}1{}{}2
\proofTheorem{\RefLinearMap}{matrix generates homomorphism}{\SideNS-\Cols}
}

\ShowText{endomorphism=matrix}
}

\DefText{22 11 26 Basis Manifold}
{

\ColRowTheorem{active transformations in module}
\TwoColText
{
\ShowEq{\DefCol}
\begin{proof}
\TheoremFollows
\refTheorem[\RefLinearMap]{automorphism of vector space}{\Product-\Cols},
\refTheorem[\RefLinearMap]{Automorphisms of vector space form a group}{\Product-\Cols},
\refTheorem[\RefLinearMap]{active transformations, vector space}{\SideNS-\Cols}.
\end{proof}
}
{
\ShowEq{\DefRow}
\begin{proof}
\TheoremFollows
\refTheorem[\RefLinearMap]{automorphism of vector space}{\Product-\Cols},
\refTheorem[\RefLinearMap]{Automorphisms of vector space form a group}{\Product-\Cols},
\refTheorem[\RefLinearMap]{active transformations, vector space}{\SideNS-\Cols}.
\end{proof}
}

\ShowText{automorphism basis matrix}

\ColRowTheorem{coordinate matrix of basis}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{coordinate matrix of basis}{\Product-\Cols}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{coordinate matrix of basis}{\Product-\Cols}
}

\ColRowTheorem{active transformations, basis, vector space}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{active transformations, basis, vector space}{\SideNS-\Cols}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{active transformations, basis, vector space}{\SideNS-\Cols}
}

\ShowText{extend linear representation to set of bases 1}
\ShowText{extend linear representation to set of bases 2}

\ColRowText{extend linear representation to set of bases 3}

%\ColRowTheorem{active representation is single transitive}
%\TwoColText
%{
%\ShowEq{\DefCol}
%\proofTheorem{\RefLinearMap}{active representation is single transitive}{\SideNS-\Cols}
%}
%{
%\ShowEq{\DefRow}
%\proofTheorem{\RefLinearMap}{active representation is single transitive}{\SideNS-\Cols}
%}
}

\DefText{22 11 26 Examples of Geometric Object}
{
\ColRowText{passive transformation and endomorphism}
\ColRowTheorem{passive transformation and endomorphism}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{passive transformation and endomorphism}{\SideNS-\Cols}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{passive transformation and endomorphism}{\SideNS-\Cols}
}
}

\DefText{22 11 26 passive transformation}
{
\ShowText{linear G* representation}

\AddIndex{}{SymmetryGroup}
\ColRowDefinition{Symmetry Group}

\ShowDefinition{active G-representation}

\ShowText{active G-representation}

\AddIndex{}{basis manifold}
\ColRowDefinition{basis manifold of vector space}

\ShowTheorem{representation on basis manifold, vector space}
\proofTheorem{\RefLinearMap}{representation on basis manifold, vector space}{\SideNS}

\ColRowTheorem{exists representation, commuting with active}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{exists representation, commuting with active}{\SideNS-\Cols}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{exists representation, commuting with active}{\SideNS-\Cols}
}

\ShowRemark{passive transformation, vector space}

\AddIndex{}{passive transformation, vector space}
\AddIndex{}{passive G representation}
\ColRowDefinition{passive transformation, vector space}
}

\DefText{22 11 26 Geometric Object}
{
\ShowText{Passive Transformation}

\ColRowText{transformation of coordinates of vector}
\ColRowTheorem{passive transformation of vector space}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{passive transformation of vector space}{\SideNS-\Cols}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{passive transformation of vector space}{\SideNS-\Cols}
}

\ColRowText{Geometric Object of Vector Space}

\ShowEq{symb coordinates of geometric object}%
\AddIndex{}{coordinates of geometric object}%
\ColRowDefinition{coordinates of geometric object, vector space}

\AddIndex{}{geometric object}%
\AddIndex{}{representative of geometric object}%
\ColRowDefinition{geometric object, vector space}

\AddIndex{}{principle of covariance}

\ShowTheorem{principle of covariance}
%\ColRowTheorem{principle of covariance}
}

\AddEq[1]{wki=a ox vkj1n}
{
\aU{w_{#1}}i=
\Entry[s0]a{#1}i{j_1...j_n}\aU{v_{1{#1}}}{j_1}
\Entry[s1]a{#1}i{j_1...j_n}...\aU{v_{n#1}}{j_n}\Entry[sn]a{#}i{j_1...j_n}
}

\AddEquation{huv=12 huv-hvu 1}
{
\begin{split}
\aU{w_2}p\aUD gip
&=\frac 12
(\Entry[s0]a1i{jk}\otimes_1\Entry[s1]a1i{jk}\otimes_2\Entry[s2]a1i{jk})
\\ &\circ ((\aU{u_2}q\aUD gjq)\otimes(\aU{v_2}r\aUD gkr)
-(\aU{v_2}r\aUD gjr)\otimes(\aU{u_2}q\aUD gkq))
\\ &=\frac 12
(\Entry[s0]a1i{jk}\otimes_1\Entry[s1]a1i{jk}\otimes_2\Entry[s2]a1i{jk})
\\ &\circ
((1\otimes_1\aUD gjq)\otimes(1\otimes_2\aUD gkr)
-(1\otimes_2\aUD gjr)\otimes(1\otimes_1\aUD gkq))
\circ(\aU{u_2}q\otimes\aU{v_2}r)
\end{split}
}

\AddEquation{huv=12 huv-hvu 2}
{
\begin{split}
\aU{w_2}p
&=\frac 12
((\Entry[s0]a1i{jk}\otimes_1\Entry[s1]a1i{jk}\otimes_2\Entry[s2]a1i{jk})
\aUD{g^{\RCInverse}_{}}pi)
\\ &\circ
((1\otimes_1\aUD gjq)\otimes(1\otimes_2\aUD gkr)
-(1\otimes_2\aUD gjr)\otimes(1\otimes_1\aUD gkq))
\circ(\aU{u_2}q\otimes\aU{v_2}r)
\end{split}
}

\AddEquation{huv=12 huv-hvu 3}
{
\begin{split}
\aU{w_2}p
&=\frac 12
(\Entry[s0]a2i{jk}\otimes_1\Entry[s1]a2i{jk}\otimes_2\Entry[s2]a2i{jk})
\\ &\circ
((1\otimes_1\aUD{\delta}jq)\otimes(1\otimes_2\aUD{\delta}kr)
-(1\otimes_2\aUD{\delta}jr)\otimes(1\otimes_1\aUD{\delta}kq))
\circ(\aU{u_2}q\otimes\aU{v_2}r)
\end{split}
}

\AddEquation{huv=12 huv-hvu 4}
{
\begin{split}
&\,
(\Entry[s0]a2i{jk}\otimes_1\Entry[s1]a2i{jk}\otimes_2\Entry[s2]a2i{jk})
\\ \circ &\,
((1\otimes_1\aUD{\delta}jq)\otimes(1\otimes_2\aUD{\delta}kr)
-(1\otimes_2\aUD{\delta}jr)\otimes(1\otimes_1\aUD{\delta}kq))
\\ =&\,
((\Entry[s0]a1i{jk}\otimes_1\Entry[s1]a1i{jk}\otimes_2\Entry[s2]a1i{jk})
\aUD{g^{\RCInverse}_{}}pi)
\\ \circ &\,
((1\otimes_1\aUD gjq)\otimes(1\otimes_2\aUD gkr)
-(1\otimes_2\aUD gjr)\otimes(1\otimes_1\aUD gkq))
\end{split}
}

\AddEq{h=1/2 aubvc}
{
\aU wi=\aU hi\circ(u\otimes v)
=\frac 12
(\Entry[s0]a{}i{jk}\otimes_1\Entry[s1]a{}i{jk}\otimes_2\Entry[s2]a{}i{jk})
\circ (\aU uj\otimes\aU vk-\aU vj\otimes\aU uk)
}

\AddEq{huv=12 huv-hvu}
{
w=h\circ(u\otimes v)=\frac 12h\circ(u\otimes v-v\otimes u)
}

\AddEq[1]{wki=a ox vkj}
{
\aU{w_{#1}}i=
\Entry[s0]a{#1}ij\aU{v_{#1}}j
\Entry[s1]a{#1}ij
}

\AddEquation{w2ig=a ox v2j1ng}
{
\aU{w_2}l\aUD gil=
\Entry[s0]a1i{j_1...j_n}\aU{v_{12}}{k_1}\aUD g{j_1}{k_1}
\Entry[s1]a1i{j_1...j_n}...
\aU{v_{n2}}{k_n}\aUD g{j_n}{k_n}\Entry[sn]aki{j_1...j_n}
}

\AddEquation{w2ig=a ox v2jg}
{
\aU{w_2}l\aUD gil=
\Entry[s0]a1ij\aU{v_2}k\aUD gjk
\Entry[s1]a1ij
}

\AddEq{w2i=a ox v2j1ng g-}
{
\aU{w_2}l=
(\Entry[s0]a1i{j_1...j_n}\aU{v_{12}}{k_1}\aUD g{j_1}{k_1}
\Entry[s1]a1i{j_1...j_n}...
\aU{v_{n2}}{k_n}\aUD g{j_n}{k_n}\Entry[sn]aki{j_1...j_n})
\aUD{g^{\CRInverse}}li
}

\AddEq{w2i=a ox v2jg g-}
{
\aU{w_2}l=
(\Entry[s0]a1ij\aU{v_2}k\aUD gjk
\Entry[s1]a1ij)
\aUD{g^{\CRInverse}}li
}

\AddEq{a ox 2=g a ox 1 l}
{
\Entry[t0]a2lk\otimes
\Entry[t1]a2lk
=
(\Entry[s0]a1ij\otimes \aUD gjk
\Entry[s1]a1ij)
\aUD{g^{\CRInverse}}li
}

\AddEq{vij wj}
{
$\aU{v_{ik}}j$, $\aU{w_k}j$
}

\AddEq{vj wj}
{
$\aU{v_k}j$, $\aU{w_k}j$
}

\AddEq{eV 12}
{
\eV[k], $k=1$, $2$.
}

\AddEq{set vi w}
{
$v_i$, $i=1$, ..., $n$, $w$
}


==> Text.MObject.English.tex <==
%auto-ignore
\input{Text.\BookNumber.Eq}

\section{Product of matrices in non-commutative algebra}

Before we begin to consider vector space
over non\Hyph commutative division algebra $A$,
I recall that there are two operations of product of matrices
with entries from algebra $A$.

\ShowText{two matrix products}

\section{Homomorphism of Left \texorpdfstring{$A$}{A}-Vector Space}

Let $A$ be non\Hyph commutative division $D$\Hyph algebra.
Then we can consider left or right
$A$\Hyph vector space.
We may confine ourselves to considering of left $A$\Hyph vector space,
because statements for right $A$\Hyph vector space are similar.
\ShowEq{def left}

We will start by considering of the set of homomorphisms
of left $A$\Hyph vector space.
Homomorphism is a map that preserves the structure of algebra.
In particular, the theorem
\refTheorem{define homomorphism A module}{\SideNS(1)}
is true.

\ShowText{22 11 26 homomorphism}

%\section{Basis Manifold for Left \texorpdfstring{$A$}{A}-Vector Space}

\ShowText{22 11 26 Basis Manifold}

\section{Passive Transformation}

\ShowText{22 11 26 passive transformation}

\section{Geometric Object}

\ShowText{22 11 26 Geometric Object}

\section{Examples of Geometric Object}

\ShowEq{\DefCol}
According to the theorem
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
a vector is geometric object.
The set of endomorphisms of left $A$\Hyph  vector space
as well as the set of linear or polylinear
maps are $A$\Hyph vector space.
So we can ask if endomorphism or
polylinear map is geometric object.

\ShowText{22 11 26 Examples of Geometric Object}

\ShowEq{\DefCol}
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
an endomorphism of vector space is geometric object.
Indeed, when we change basis,
we see transformation of coordinates of vector and coordinates of endomorphism.
However, change of coordinates agreed and image of vector for
given endomorphism does not depend on choice of basis.

Let \eV be the basis of left vector space $V$ of columns.
Linear map
\ShowEq{f:A->B}aVV
has form
\DrawEq[avwnn]{b=f rco a}1
\DrawEq[ann]{a=(a11.nm matrix)}{}
with respect to the basis \eV[][.]
Since partial map $\aUD aij$
is linear map of $D$\Hyph algebra $A$,
then we can write linear map $\aUD aij$ as
\DrawEq[{}{}]{aij=.ox.}a
The equality
\ShowEq{vi=aij o wj}
follows from equalities
\newline
\FrameEqRef[avwnn]{b=f rco a}1
\newline
\FrameEqRef[{}{}]{aij=.ox.}a

\ShowSummary{Examples of Geometric Object}

\ShowEq{\DefCol}
Let passive transformation $g$ map the basis \eV[1]
into the basis \eV[2]
\DrawEq[12g{}]{e2i=aij e1j cr-cols}{1->2 l}

Let
\DrawEq[k]{aij=.ox.}k
be coordinates of linear map $a$
with respect to the basis \eV[k][,]
$k=1$, $2$.

Let
\ShowEq{vj wj}
be coordinates of vectors
$v$, $w$
with respect to the basis
\ShowEq{eV 12}
Then
\DrawEq[k]{wki=a ox vkj}k
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[v1v2g{}]{v1=v2*a left-cols}{v12g l}
\DrawEq[w1w2g{}]{v1=v2*a left-cols}{w12g l}
Equalities
\ShowEq{w2ig=a ox v2jg}
\DrawEq{w2i=a ox v2jg g-}1
follow from equalities
\newline
\FrameEqRef[v1v2g{}]{v1=v2*a left-cols}{v12g l}
\FrameEqRef[w1w2g{}]{v1=v2*a left-cols}{w12g l}
\newline
\FrameEqRef[1]{wki=a ox vkj}k
(k=1).
\newline
The equality
\DrawEq{a ox 2=g a ox 1 l}1
follows from equalities
\newline
\FrameEqRef[2]{wki=a ox vkj}k
(k=2),
\newline
\FrameEqRef{w2i=a ox v2jg g-}1

The equality
\DrawEq{a ox 2=g a ox 1 g l}1
follows from equalities
\newline
\FrameEqRef[v1v2g{}]{v1=v2*a left-cols}{v12g l}
\newline
\FrameEqRef{a ox 2=g a ox 1 l}1
\newline
From the equality
\eqRef{a ox 2=g a ox 1 g l}1
it follows that image of linear map
does not depend on choice of basis.

It is easy to see the similarity of equalities
\newline
\FrameEqRef[fg{\SideNS}{\Cols}]{f2=a f1 a-}{g \SideNS-\Cols}
\newline
and
\newline
\FrameEqRef{a ox 2=g a ox 1 l}1
\newline
If $D$\Hyph algebra $A$ is commutative,
then these equalities are the same.

\begin{\TheoremStyle}
\labelTheorem{Polylinear map is geometric object}
Polylinear map
\DrawEq[a{V^n}V{}]{f: A->B}{AnA}
is geometric object.
\end{\TheoremStyle}

\begin{proof}
Without loss of generality,
we consider proof of the theorem
for left $A$\Hyph vector space of columns.

\ShowEq{\DefCol}
Let passive transformation $g$ map the basis \eV[1]
into the basis \eV[2]
\DrawEq[12g{}]{e2i=aij e1j cr-cols}{1->2}

Let
\ShowEq{vij wj}
be coordinates of vectors
\ShowEq{set vi w}
with respect to the basis
\ShowEq{eV 12}
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[v{i1}v{i2}g{}]{v1=v2*a left-cols}{v12ig}
\DrawEq[w1w2g{}]{v1=v2*a left-cols}{w12g}

Let the set of tensors
\DrawEq{akj1n .ox.}1
be coordinates of polylinear map $a$
with respect to the basis \eV[k].
Then\,\footnote{\,
In this proof, there is no need to consider
posibility to change an order of variables in every term
since we are interested in single term.
If the order of variables in this term changes,
then we can change this order
before we start calculations in the proof.
}
\DrawEq[k]{wki=a ox vkj1n}k
Equalities
\ShowEq{w2ig=a ox v2j1ng}
\DrawEq{w2i=a ox v2j1ng g-}1
follow from equalities
\newline
\FrameEqRef[v{i1}v{i2}g{}]{v1=v2*a left-cols}{v12ig}
\FrameEqRef[w1w2g{}]{v1=v2*a left-cols}{w12g}
\newline
\FrameEqRef[1]{wki=a ox vkj1n}k
(k=1).
\newline
The equality
\DrawEq{a ox 2=g a ox 1}1
follows from equalities
\newline
\FrameEqRef[2]{wki=a ox vkj1n}k
(k=2),
\newline
\FrameEqRef{w2i=a ox v2j1ng g-}1

The equality
\DrawEq{a ox 2=g a ox 1 g}1
follows from equalities
\newline
\FrameEqRef[v{i1}v{i2}g{}]{v1=v2*a left-cols}{v12ig}
\newline
\FrameEqRef{a ox 2=g a ox 1}1
\newline
From the equality
\eqRef{a ox 2=g a ox 1 g}1
it follows that image of polylinear map
does not depend on choice of basis.
\end{proof}

We consider transformation skew-symmetric
polylinear map using the bilinear map as an example.
Let
\DrawEq{huv=12 huv-hvu}1
where the map $h$ has the form
\DrawEq{h=aubvc}1
The equality
\DrawEq{h=1/2 aubvc}1
follows from equalities
\eqRef{huv=12 huv-hvu}1,
\eqRef{h=aubvc}1.
If we consider determinant like expression
\DrawEq{star uv-vu}1
then the equality
\eqRef{h=1/2 aubvc}1
gets the form
\DrawEq{h=1/2 aubvc 1}1
Let passive transformation $g$ map the basis \eV[1]
into the basis \eV[2]
\DrawEq[12g{}]{e2i=aij e1j cr-cols}{1->2 skew}
The equality
\ShowEq{huv=12 huv-hvu 1}
follows from equalities
\newline
\FrameEqRef{h=1/2 aubvc}1
\FrameEqRef[w1w2g{}]{v1=v2*a left-cols}{w12g}
\DrawEq[u1u2g{}]{v1=v2*a left-cols}{u12g}
\DrawEq[u1u2g{}]{v1=v2*a left-cols}{v12g}
The equality
\ShowEq{huv=12 huv-hvu 2}
follows from the equality
\EqRef{huv=12 huv-hvu 1}.
The equality
\ShowEq{huv=12 huv-hvu 3}
follows from the equality
\newline
\FrameEqRef{h=1/2 aubvc}1
The equality
\ShowEq{huv=12 huv-hvu 4}
follows from the equality
\EqRef{huv=12 huv-hvu 2},
\EqRef{huv=12 huv-hvu 3}.
The equality
\DrawEq{huv=12 huv-hvu 5}1
follows from the equality
\eqRef{star uv-vu}1,
\EqRef{huv=12 huv-hvu 4}.


==> Text.MObject.Eq.tex <==
%auto-ignore

\DefText{22 11 26 homomorphism}
{
\ShowEq{def left}
\ShowEq{\DefCol}
\ShowEq{def AModule}

\ShowDefinition{homomorphism A module}{}{}1{}{}2

\ShowText{notation for homomorphism of module}

\ShowTheorem{define homomorphism A module}{}{}1{}{}2pa
\proofTheorem{\RefLinearMap}{define homomorphism A module}{\SideNS(1)}
\ePrints{2022.11.26}%
\ifx\Semafor\ValueOn%
\newline
\FrameCiteBib{\RefLinearMap}
\fi

\ShowDefinition{iso end aut morphism vector space}

\ShowTheorem{set of automorphisms}

\ShowText{coordinates of homomorphism}

%\ShowSummary{homomorphism of vector space}

\ShowEq{\DefCol}
\ShowFootnote{homomorphism of A module}{}{}1{}{}2
\ShowEq{\DefRow}
\ShowFootnote{homomorphism of A module}{}{}1{}{}2
\TwoColText
{
\ShowEq{\DefCol}
\ShowTheorem{homomorphism A module}{}{}1{}{}2
}
{
\ShowEq{\DefRow}
\ShowTheorem{homomorphism A module}{}{}1{}{}2
}
\AddIndex{}{matrix of homomorphism}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{homomorphism A module}{\SideNS-\Cols(1)}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{homomorphism A module}{\SideNS-\Cols(1)}
}

\ShowText{converse theorem is also true}

\TwoColText
{
\ShowEq{\DefCol}
\ShowTheorem{matrix generates A module homomorphism}{}{}1{}{}2
\proofTheorem{\RefLinearMap}{matrix generates A module homomorphism}{\SideNS-\Cols(1)}
}
{
\ShowEq{\DefRow}
\ShowTheorem{matrix generates A module homomorphism}{}{}1{}{}2
\proofTheorem{\RefLinearMap}{matrix generates A module homomorphism}{\SideNS-\Cols(1)}
}

\ShowText{endomorphism=matrix}
}

\DefText{22 11 26 Basis Manifold}
{

\ColRowTheorem{active transformations in module}
\TwoColText
{
\ShowEq{\DefCol}
\begin{proof}
\TheoremFollows
\refTheorem[\RefLinearMap]{automorphism of vector space}{\Product-\Cols},
\refTheorem[\RefLinearMap]{Automorphisms of vector space form a group}{\Product-\Cols},
\refTheorem[\RefLinearMap]{active transformations, vector space}{\SideNS-\Cols}.
\end{proof}
}
{
\ShowEq{\DefRow}
\begin{proof}
\TheoremFollows
\refTheorem[\RefLinearMap]{automorphism of vector space}{\Product-\Cols},
\refTheorem[\RefLinearMap]{Automorphisms of vector space form a group}{\Product-\Cols},
\refTheorem[\RefLinearMap]{active transformations, vector space}{\SideNS-\Cols}.
\end{proof}
}

\ShowText{automorphism basis matrix}

\ColRowTheorem{coordinate matrix of basis}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{coordinate matrix of basis}{\Product-\Cols}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{coordinate matrix of basis}{\Product-\Cols}
}

\ColRowTheorem{active transformations, basis, vector space}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{active transformations, basis, vector space}{\SideNS-\Cols}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{active transformations, basis, vector space}{\SideNS-\Cols}
}

\ShowText{extend linear representation to set of bases 1}
\ShowText{extend linear representation to set of bases 2}

\ColRowText{extend linear representation to set of bases 3}

%\ColRowTheorem{active representation is single transitive}
%\TwoColText
%{
%\ShowEq{\DefCol}
%\proofTheorem{\RefLinearMap}{active representation is single transitive}{\SideNS-\Cols}
%}
%{
%\ShowEq{\DefRow}
%\proofTheorem{\RefLinearMap}{active representation is single transitive}{\SideNS-\Cols}
%}
}

\DefText{22 11 26 Examples of Geometric Object}
{
\ColRowText{passive transformation and endomorphism}
\ColRowTheorem{passive transformation and endomorphism}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{passive transformation and endomorphism}{\SideNS-\Cols}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{passive transformation and endomorphism}{\SideNS-\Cols}
}
}

\DefText{22 11 26 passive transformation}
{
\ShowText{linear G* representation}

\AddIndex{}{SymmetryGroup}
\ColRowDefinition{Symmetry Group}

\ShowDefinition{active G-representation}

\ShowText{active G-representation}

\AddIndex{}{basis manifold}
\ColRowDefinition{basis manifold of vector space}

\ShowTheorem{representation on basis manifold, vector space}
\proofTheorem{\RefLinearMap}{representation on basis manifold, vector space}{\SideNS}

\ColRowTheorem{exists representation, commuting with active}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{exists representation, commuting with active}{\SideNS-\Cols}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{exists representation, commuting with active}{\SideNS-\Cols}
}

\ShowRemark{passive transformation, vector space}

\AddIndex{}{passive transformation, vector space}
\AddIndex{}{passive G representation}
\ColRowDefinition{passive transformation, vector space}
}

\DefText{22 11 26 Geometric Object}
{
\ShowText{Passive Transformation}

\ColRowText{transformation of coordinates of vector}
\ColRowTheorem{passive transformation of vector space}
\TwoColText
{
\ShowEq{\DefCol}
\proofTheorem{\RefLinearMap}{passive transformation of vector space}{\SideNS-\Cols}
}
{
\ShowEq{\DefRow}
\proofTheorem{\RefLinearMap}{passive transformation of vector space}{\SideNS-\Cols}
}

\ColRowText{Geometric Object of Vector Space}

\ShowEq{symb coordinates of geometric object}%
\AddIndex{}{coordinates of geometric object}%
\ColRowDefinition{coordinates of geometric object, vector space}

\AddIndex{}{geometric object}%
\AddIndex{}{representative of geometric object}%
\ColRowDefinition{geometric object, vector space}

\AddIndex{}{principle of covariance}

\ShowTheorem{principle of covariance}
%\ColRowTheorem{principle of covariance}
}

\AddEq[1]{wki=a ox vkj1n}
{
\aU{w_{#1}}i=
\Entry[s0]a{#1}i{j_1...j_n}\aU{v_{1{#1}}}{j_1}
\Entry[s1]a{#1}i{j_1...j_n}...\aU{v_{n#1}}{j_n}\Entry[sn]a{#1}i{j_1...j_n}
}

\AddEquation{huv=12 huv-hvu 1}
{
\begin{split}
\aU{w_2}p\aUD gip
&=\frac 12
(\Entry[s0]a1i{jk}\otimes_1\Entry[s1]a1i{jk}\otimes_2\Entry[s2]a1i{jk})
\\ &\circ ((\aU{u_2}q\aUD gjq)\otimes(\aU{v_2}r\aUD gkr)
-(\aU{v_2}r\aUD gjr)\otimes(\aU{u_2}q\aUD gkq))
\\ &=\frac 12
(\Entry[s0]a1i{jk}\otimes_1\Entry[s1]a1i{jk}\otimes_2\Entry[s2]a1i{jk})
\\ &\circ
((1\otimes_1\aUD gjq)\otimes(1\otimes_2\aUD gkr)
-(1\otimes_2\aUD gjr)\otimes(1\otimes_1\aUD gkq))
\circ(\aU{u_2}q\otimes\aU{v_2}r)
\end{split}
}

\AddEquation{huv=12 huv-hvu 2}
{
\begin{split}
\aU{w_2}p
&=\frac 12
((\Entry[s0]a1i{jk}\otimes_1\Entry[s1]a1i{jk}\otimes_2\Entry[s2]a1i{jk})
\aUD{g^{\RCInverse}_{}}pi)
\\ &\circ
((1\otimes_1\aUD gjq)\otimes(1\otimes_2\aUD gkr)
-(1\otimes_2\aUD gjr)\otimes(1\otimes_1\aUD gkq))
\circ(\aU{u_2}q\otimes\aU{v_2}r)
\end{split}
}

\AddEquation{huv=12 huv-hvu 3}
{
\begin{split}
\aU{w_2}p
&=\frac 12
(\Entry[s0]a2i{jk}\otimes_1\Entry[s1]a2i{jk}\otimes_2\Entry[s2]a2i{jk})
\\ &\circ
((1\otimes_1\aUD{\delta}jq)\otimes(1\otimes_2\aUD{\delta}kr)
-(1\otimes_2\aUD{\delta}jr)\otimes(1\otimes_1\aUD{\delta}kq))
\circ(\aU{u_2}q\otimes\aU{v_2}r)
\end{split}
}

\AddEquation{huv=12 huv-hvu 4}
{
\begin{split}
&\,
(\Entry[s0]a2i{jk}\otimes_1\Entry[s1]a2i{jk}\otimes_2\Entry[s2]a2i{jk})
\\ \circ &\,
((1\otimes_1\aUD{\delta}jq)\otimes(1\otimes_2\aUD{\delta}kr)
-(1\otimes_2\aUD{\delta}jr)\otimes(1\otimes_1\aUD{\delta}kq))
\\ =&\,
((\Entry[s0]a1i{jk}\otimes_1\Entry[s1]a1i{jk}\otimes_2\Entry[s2]a1i{jk})
\aUD{g^{\RCInverse}_{}}pi)
\\ \circ &\,
((1\otimes_1\aUD gjq)\otimes(1\otimes_2\aUD gkr)
-(1\otimes_2\aUD gjr)\otimes(1\otimes_1\aUD gkq))
\end{split}
}

\AddEq{h=1/2 aubvc}
{
\aU wi=\aU hi\circ(u\otimes v)
=\frac 12
(\Entry[s0]a{}i{jk}\otimes_1\Entry[s1]a{}i{jk}\otimes_2\Entry[s2]a{}i{jk})
\circ (\aU uj\otimes\aU vk-\aU vj\otimes\aU uk)
}

\AddEq{huv=12 huv-hvu}
{
w=h\circ(u\otimes v)=\frac 12h\circ(u\otimes v-v\otimes u)
}

\AddEq[1]{wki=a ox vkj}
{
\aU{w_{#1}}i=
\Entry[s0]a{#1}ij\aU{v_{#1}}j
\Entry[s1]a{#1}ij
}

\AddEquation{w2ig=a ox v2j1ng}
{
\aU{w_2}l\aUD gil=
\Entry[s0]a1i{j_1...j_n}\aU{v_{12}}{k_1}\aUD g{j_1}{k_1}
\Entry[s1]a1i{j_1...j_n}...
\aU{v_{n2}}{k_n}\aUD g{j_n}{k_n}\Entry[sn]aki{j_1...j_n}
}

\AddEquation{w2ig=a ox v2jg}
{
\aU{w_2}l\aUD gil=
\Entry[s0]a1ij\aU{v_2}k\aUD gjk
\Entry[s1]a1ij
}

\AddEq{w2i=a ox v2j1ng g-}
{
\aU{w_2}l=
(\Entry[s0]a1i{j_1...j_n}\aU{v_{12}}{k_1}\aUD g{j_1}{k_1}
\Entry[s1]a1i{j_1...j_n}...
\aU{v_{n2}}{k_n}\aUD g{j_n}{k_n}\Entry[sn]aki{j_1...j_n})
\aUD{g^{\CRInverse}}li
}

\AddEq{w2i=a ox v2jg g-}
{
\aU{w_2}l=
(\Entry[s0]a1ij\aU{v_2}k\aUD gjk
\Entry[s1]a1ij)
\aUD{g^{\CRInverse}}li
}

\AddEq{a ox 2=g a ox 1 l}
{
\Entry[t0]a2lk\otimes
\Entry[t1]a2lk
=
(\Entry[s0]a1ij\otimes \aUD gjk
\Entry[s1]a1ij)
\aUD{g^{\CRInverse}}li
}

\AddEq{vij wj}
{
$\aU{v_{ik}}j$, $\aU{w_k}j$
}

\AddEq{vj wj}
{
$\aU{v_k}j$, $\aU{w_k}j$
}

\AddEq{eV 12}
{
\eV[k], $k=1$, $2$.
}

\AddEq{set vi w}
{
$v_i$, $i=1$, ..., $n$, $w$
}


==> Text.MObject.Russian.tex <==
%auto-ignore
\input{Text.\BookNumber.Eq}

\section{Произведение матриц в некоммутативной алгебре}

Прежде чем мы начнём рассматривать векторные пространства
над некоммутативной алгеброй $A$ с делением,
я напомню, что существует две операции произведения матриц
с элементами из алгебры $A$.

\ShowText{two matrix products}

\section{Гомоморфизм левого \texorpdfstring{$A$}{A}-векторного пространства}

Пусть $A$ - некоммутативная $D$\Hyph алгебра с делением.
Тогда мы можем рассматривать левое или правое
$A$\Hyph векторное пространство.
Мы можем ограничиться рассмотрением левого $A$\Hyph векторного пространства,
так как утверждения для правого $A$\Hyph векторного пространства аналогичны.
\ShowEq{def left}

Мы начнём с рассмотрения множества гомомрфизмов
левого $A$\Hyph векторного пространства.
Гомоморфизм - это отображение, которое сохраняет структуру алгебры.
В частности,
верна теорема
\refTheorem{define homomorphism A module}{\SideNS(1)}.

\ShowText{22 11 26 homomorphism}

%\section{Многообразие базисов левого \texorpdfstring{$A$}{A}-векторного пространства}

\ShowText{22 11 26 Basis Manifold}

\section{Пассивное преобразование}

\ShowText{22 11 26 passive transformation}

\section{Геометрический объект}

\ShowText{22 11 26 Geometric Object}

\section{Примеры геометрического объекта}

\ShowEq{\DefCol}
Согласно теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
вектор является геометрическим объектом.
Множество эндоморфизмов левого $A$\Hyph векторного пространства,
также как и множество линейных или полилинейных
отображений являются $A$\Hyph векторными пространствами.
Поэтому мы можем спросить является ли эндоморфизм или
полилинейное отображение геометрическим объектом.

\ShowText{22 11 26 Examples of Geometric Object}

\ShowEq{\DefCol}
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
эндоморфизм векторного пространства является геометрическим объектом.
Действительно, при замене базиса
мы видим преобразование координат вектора и координат эндоморфизма.
Но изменение координат согласовано, и образ вектора при
заданом эндоморфизме не зависит от выбора базиса.

Пусть \eV - базис левого векторного пространства $V$ столбцов.
Линейное отображение
\ShowEq{f:A->B}aVV
имеет вид
\DrawEq[avwnn]{b=f rco a}1
\DrawEq[ann]{a=(a11.nm matrix)}{}
относительно базиса \eV[][.]
Так как частное отображение $\aUD aij$
является линейным отображением $D$\Hyph алгебры $A$,
то мы можем записать линейное отображение $\aUD aij$ в виде
\DrawEq[{}{}]{aij=.ox.}a
Равенство
\ShowEq{vi=aij o wj}
является следствием равенств
\newline
\FrameEqRef[avwnn]{b=f rco a}1
\newline
\FrameEqRef[{}{}]{aij=.ox.}a

\ShowSummary{Examples of Geometric Object}

\ShowEq{\DefCol}
Пусть пассивное преобразование $g$ отображает базис \eV[1]
в базис \eV[2]
\DrawEq[12g{}]{e2i=aij e1j cr-cols}{1->2 l}

Пусть
\DrawEq[k]{aij=.ox.}k
координаты линейного отображения $a$
относительно базиса \eV[k][,]
$k=1$, $2$.

Пусть
\ShowEq{vj wj}
координаты векторов
$v$, $w$
относительно базиса
\ShowEq{eV 12}
Тогда
\DrawEq[k]{wki=a ox vkj}k
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[v1v2g{}]{v1=v2*a left-cols}{v12g l}
\DrawEq[w1w2g{}]{v1=v2*a left-cols}{w12g l}
Равенства
\ShowEq{w2ig=a ox v2jg}
\DrawEq{w2i=a ox v2jg g-}1
являются следствием равенств
\newline
\FrameEqRef[v1v2g{}]{v1=v2*a left-cols}{v12g l}
\FrameEqRef[w1w2g{}]{v1=v2*a left-cols}{w12g l}
\newline
\FrameEqRef[1]{wki=a ox vkj}k
(k=1).
\newline
Равенство
\DrawEq{a ox 2=g a ox 1 l}1
является следствием равенств
\newline
\FrameEqRef[2]{wki=a ox vkj}k
(k=2),
\newline
\FrameEqRef{w2i=a ox v2jg g-}1

Равенство
\DrawEq{a ox 2=g a ox 1 g l}1
является следствием равенств
\newline
\FrameEqRef[v1v2g{}]{v1=v2*a left-cols}{v12g l}
\newline
\FrameEqRef{a ox 2=g a ox 1 l}1
\newline
Из равенства
\eqRef{a ox 2=g a ox 1 g l}1
следует, что образ линейного отображения
не зависит от выбора базиса.

Нетрудно видеть сходство равенств
\newline
\FrameEqRef[fg{\SideNS}{\Cols}]{f2=a f1 a-}{g \SideNS-\Cols}
\newline
и
\newline
\FrameEqRef{a ox 2=g a ox 1 l}1
\newline
Если $D$\Hyph алгебра $A$ коммутативна,
эти равенства совпадают.

\begin{\TheoremStyle}
\labelTheorem{Polylinear map is geometric object}
Полилинейное отображение
\DrawEq[a{V^n}V{}]{f: A->B}{AnA}
является геометрическим объектом.
\end{\TheoremStyle}

\begin{proof}
Не нарушая общности,
мы рассмотрим доказательство теоремы
для левого $A$\Hyph векторного пространства столбцов.

\ShowEq{\DefCol}
Пусть пассивное преобразование $g$ отображает базис \eV[1]
в базис \eV[2]
\DrawEq[12g{}]{e2i=aij e1j cr-cols}{1->2}

Пусть
\ShowEq{vij wj}
координаты векторов
\ShowEq{set vi w}
относительно базиса
\ShowEq{eV 12}
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[v{i1}v{i2}g{}]{v1=v2*a left-cols}{v12ig}
\DrawEq[w1w2g{}]{v1=v2*a left-cols}{w12g}

Пусть множество тензоров
\DrawEq{akj1n .ox.}1
является координатами полилинейного отображения $a$
относительно базиса \eV[k].
Тогда\,\footnote{\,
В этом доказательстве нет необходимости рассматривать
возможность изменений порядка переменных в каждом слагаемом,
так как нас интересует одно слагаемое.
Если в этом слагаемом меняется порядок переменных,
то мы можем изменить этот порядок до того,
как мы начнём вычисления в доказательстве.
}
\DrawEq[k]{wki=a ox vkj1n}k
Равенства
\ShowEq{w2ig=a ox v2j1ng}
\DrawEq{w2i=a ox v2j1ng g-}1
являются следствием равенств
\newline
\FrameEqRef[v{i1}v{i2}g{}]{v1=v2*a left-cols}{v12ig}
\FrameEqRef[w1w2g{}]{v1=v2*a left-cols}{w12g}
\newline
\FrameEqRef[1]{wki=a ox vkj1n}k
(k=1).
\newline
Равенство
\DrawEq{a ox 2=g a ox 1}1
является следствием равенств
\newline
\FrameEqRef[2]{wki=a ox vkj1n}k
(k=2),
\newline
\FrameEqRef{w2i=a ox v2j1ng g-}1

Равенство
\DrawEq{a ox 2=g a ox 1 g}1
является следствием равенств
\newline
\FrameEqRef[v{i1}v{i2}g{}]{v1=v2*a left-cols}{v12ig}
\newline
\FrameEqRef{a ox 2=g a ox 1}1
\newline
Из равенства
\eqRef{a ox 2=g a ox 1 g}1
следует, что образ полилинейного отображения
не зависит от выбора базиса.
\end{proof}

Мы рассмотрим преобразование кососимметричного
полилинейного отображения на примере билинейного отображения.
Положим
\DrawEq{huv=12 huv-hvu}1
где отображение $h$ имеет вид
\DrawEq{h=aubvc}1
Равенство
\DrawEq{h=1/2 aubvc}1
является следствием равенств
\eqRef{huv=12 huv-hvu}1,
\eqRef{h=aubvc}1.
Если мы рассмотрим выражение, подобное определителю,
\DrawEq{star uv-vu}1
то равенство
\eqRef{h=1/2 aubvc}1
примет вид
\DrawEq{h=1/2 aubvc 1}1
Пусть пассивное преобразование $g$ отображает базис \eV[1]
в базис \eV[2]
\DrawEq[12g{}]{e2i=aij e1j cr-cols}{1->2 skew}
Равенство
\ShowEq{huv=12 huv-hvu 1}
является следствием равенств
\newline
\FrameEqRef{h=1/2 aubvc}1
\FrameEqRef[w1w2g{}]{v1=v2*a left-cols}{w12g}
\DrawEq[u1u2g{}]{v1=v2*a left-cols}{u12g}
\DrawEq[u1u2g{}]{v1=v2*a left-cols}{v12g}
Равенство
\ShowEq{huv=12 huv-hvu 2}
является следствием равенства
\EqRef{huv=12 huv-hvu 1}.
Равенство
\ShowEq{huv=12 huv-hvu 3}
является следствием равенства
\newline
\FrameEqRef{h=1/2 aubvc}1
Равенство
\ShowEq{huv=12 huv-hvu 4}
является следствием равенства
\EqRef{huv=12 huv-hvu 2},
\EqRef{huv=12 huv-hvu 3}.
Равенство
\DrawEq{huv=12 huv-hvu 5}1
является следствием равенства
\eqRef{star uv-vu}1,
\EqRef{huv=12 huv-hvu 4}.


==> Vector.Space.2020.Stmt.English.tex <==
%auto-ignore
\input{Vector.Space.2020.Stmt.Eq}

\DefLabeledDefinition{eigenvalue of matrix}{\Product}
{
$A$\Hyph number $b$ is called
{\bf\ProductType eigenvalue}
of the matrix $f$
if the matrix
$f-b\aD En$
is \ProductType singular matrix.
}

\DefLabeledDefinition{eigenvector of matrix}{\Product-\Cols}
{
Let $A$\Hyph number $b$ be
\ProductType eigenvalue
of the matrix $f$.
A \ColWS $v$ is called
{\bf eigen\ColWS}
of matrix $f$ corresponding to \ProductType eigenvalue $b$,
if the following equality is true
\DrawEq{\Product-eigen\Cols}1
}

\DefLabeledTheorem{0 is eigenvalue of multiplicity}{\Product}
{
Let $f$ be $\gin\times\gin$ matrix of $A$\Hyph numbers and
\ShowEq{\Product-rank a=k<n}
Then $0$ is \ProductType eigenvalue of multiplicity
$\gin-\gik$.
}

\DefProof{0 is eigenvalue of multiplicity}
{
The theorem follows from the equality
\[a=a-0E\]
from the definition
\refDefinition{eigenvalue of matrix}{\Product}
and the theorem
\RefTheorem{star rows system of linear equations, solution}.
}

\DefLabeledTheorem{eigenvalues of pair of matrices}{\Product}
{
Let $f$ be $\gin\times\gin$ matrix of $A$\Hyph numbers.
Let $g$ be non\Hyph \ProductType singular $\gin\times\gin$ matrix of $A$\Hyph numbers.
Then non\Hyph zero \ProductType eigenvalues of the pair of matrices $(f,g)$
are roots of any equation
\DrawEq{\Product-det ij f-bg =0}{}
}

\DefProofSloppy{eigenvalues of pair of matrices}
{
The theorem follows from the theorem
\refTheorem{singular matrix and quasideterminant}{\Product}
and from the definition
\refDefinition{eigenvalues of pair of matrices}{\Product}.
}

\DefLabeledTheorem{eigenvalues of matrix}{\Product}
{
Let $f$ be $\gin\times\gin$ matrix of $A$\Hyph numbers.
Then non\Hyph zero \RC eigenvalues of the matrix $f$
are roots of any equation
\DrawEq{\Product-det ij a=0}{}
}

\DefProofSloppy{eigenvalues of matrix}
{
The theorem follows from the theorem
\refTheorem{singular matrix and quasideterminant}{\Product}
and from the definition
\refDefinition{Eigenvalue of Endomorphism}{\SideNS}.
}

\AddEq[6]{theorem: product of homomorphisms, A vector space}
{
\begin{ShadedTheorem}
\labelTheorem{product of homomorphisms, \SideWS A vector space, \ColN}
Let $U$, $V$, $W$ be
\SideWS $A$\Hyph vector spaces of \ColN s.
\ShowEq{Let be Basis of vector space}UAU
\ShowEq{Let be Basis of vector space}VAV
\ShowEq{Let be Basis of vector space}WAW
The homomorphism
\ShowEq{vf: A->B}fUW{}%
is product of homomorphisms
\ShowEq{vf: A->B}hVW,%
\ShowEq{vf: A->B}gUV{}%
iff
matrix $f$ of homomorphism $\Vector f$
relative to bases
\ShowEq{Bases eVW}UW{}{}
is equal to the \ProductType product of matrix $#1$ of the homomorphism $\Vector{#1}$
relative to bases
\ShowEq{Bases eVW}{#2}{#3}{}{}
over matrix $#4$ of the homomorphism $\Vector{#4}$
relative to bases
\ShowEq{Bases eVW}{#5}{#6}{}
\DrawEq[f{#1}{\ProductVal}{#4}]{f=g*h}{\Product-\Cols}
\end{ShadedTheorem}
}

\AddEq[2]{proof: product of homomorphisms, A vector space}
{
\begin{proof}
According to the theorem
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}
\DrawEq[ufUW]{f o (ae)=a o f e, vector space \Product-\Cols}{f product \Product-\Cols}
\DrawEq[ugUV]{f o (ae)=a o f e, vector space \Product-\Cols}{g product \Product-\Cols}
\DrawEq[vhVW]{f o (ae)=a o f e, vector space \Product-\Cols}{h product \Product-\Cols}
According to the theorem
\refTheorem{product of homomorphisms is homomorphism, A vector space}{\SideNS},
the equality
\ShowEq{f o v=g o h o v \SideNS-\Cols}
follows from equalities
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{g product \Product-\Cols},
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{h product \Product-\Cols}.
The equality
\eqRef{f=g*h}{\Product-\Cols}
follows from equalities
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{f product \Product-\Cols},
\EqRef{f o v=g o h o v \SideNS-\Cols}
and the theorem
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}.

Let
\DrawEq[f{#1}{\ProductVal}{#2.}]{f=g*h}-
According to the theorem
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)},
there exist homomorphisms
\ShowEq{vf: A->B}fUV,%
\ShowEq{vf: A->B}gUV,%
\ShowEq{vf: A->B}hUV{}%
such that
\ShowEq{fov=(gh)ov \SideNS-\Cols}
From the equality
\EqRef{fov=(gh)ov \SideNS-\Cols}
and the theorem
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS},
it follows that
the homomorphism $\Vector f$
is product of homomorphisms $\Vector h$, $\Vector g$.
\end{proof}
}

\DefLabeledTheorem{product of homomorphisms is homomorphism, A vector space}{\SideNS}
{
Let $U$, $V$, $W$ be \SideWS $A$\Hyph vector spaces.
Let diagram of maps
\DrawEq{diagram product of homomorphisms, A vector space}{\SideNS}
%%%%%\newline
\DrawEq{f o u=h o g o u}{\SideNS}
be commutative diagram
where maps $g$, $h$ are
homomorphisms of \SideWS $A$\Hyph vector space.
The map
\ShowEq{f=h o g}
is homomorphism
of \SideWS $A$\Hyph vector space
and is called
\AddIndex{product of homomorphisms}{product of homomorphisms}
$h$, $g$.
}

\DefProof{product of homomorphisms is homomorphism, A vector space}
{
The equality
\eqRef{f o u=h o g o u}{\SideNS}
follows from the commutativity of the diagram
\eqRef{diagram product of homomorphisms, A vector space}{\SideNS}.
The equality
\DrawEq{(h o g)o(u+v)=}{\SideWS vector space}
follows from equalities
\eqRef{\SideWS homomorphism, f av=}1,
\eqRef{f o u=h o g o u}{\SideNS}.
The equality
\ShowEq{(h o g)o(av)= \SideNS}
follows from equalities
\eqRef{\SideWS homomorphism, f av=}1,
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.
The theorem follows from the theorem
\refTheorem{define homomorphism A module}{\SideNS(1)}
and equalities
\eqRef{(h o g)o(u+v)=}{\SideWS vector space},
\EqRef{(h o g)o(av)= \SideNS}.
}

\DefLabeledTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS}
{
Let $V$, $W$ be \SideWS $A$\Hyph vector spaces
and maps
\DrawEq[gVW,]{f: A->B}-
\DrawEq[hVW{}]{f: A->B}-
be homomorphisms
of \SideWS $A$\Hyph vector space.
Let the map
\DrawEq[fVW{}]{f: A->B}-
be defined by the equality
\DrawEq{sum of homomorphisms f o v=}{\SideWS vector space}
The map $f$ is homomorphism
of \SideWS $A$\Hyph vector space
and is called
\AddIndex{sum
\ShowEq{f=g+h}
of homomorphisms}{sum of maps}
$g$ and $h$.
}

\DefProof{sum of homomorphisms is homomorphism, A vector space}
{
According to the theorem
\refTheorem{definition of vector space}{\SideNS}
(the equality
\eqRef{commutative law}{\SideWS vector space}),
the equality
\newline
\DrawEq{(g+h)o(u+v)=}{\SideWS vector space}
\begin{sloppypar}
\noindent
follows from equalities
\eqRef{homomorphism, f v+w=}{\SideNS},
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.
According to the theorem
\refTheorem{definition of vector space}{\SideNS}
(the equality
\eqRef{distributive law, \SideWS module, 1}1),
the equality
\ShowEq{(g+h)o(av)= \SideNS}
\end{sloppypar}
\noindent
follows from equalities
\eqRef{\SideWS homomorphism, f av=}1,
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.

The theorem follows from the theorem
\refTheorem{define homomorphism A module}{\SideNS(1)}
and equalities
\eqRef{(g+h)o(u+v)=}{\SideWS vector space},
\EqRef{(g+h)o(av)= \SideNS}.
}

\DefLabeledTheorem{sum of homomorphisms, A vector space}{\SideNS-\Cols}
{
Let $V$, $W$ be
\SideWS $A$\Hyph vector spaces of \ColN s.
\ShowEq{Let be Basis of vector space}VAV
\ShowEq{Let be Basis of vector space}WAW
The homomorphism
\ShowEq{vf: A->B}fVW{}%
is sum of homomorphisms
\ShowEq{vf: A->B}gVW,%
\ShowEq{vf: A->B}hVW{}%
iff
matrix $f$ of homomorphism $\Vector f$
relative to bases
\ShowEq{Bases eVW}VW{}{}
is equal to the sum of the matrix $g$ of the homomorphism $\Vector g$
relative to bases
\ShowEq{Bases eVW}VW{}{}
and the matrix $h$ of the homomorphism $\Vector h$
relative to bases
\ShowEq{Bases eVW}VW{}.
}

\DefProof{sum of homomorphisms, A vector space}
{
According to theorem
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}
\DrawEq[afUV]{f o (ae)=a o f e, vector space \Product-\Cols}{f sum \Product-\Cols}
\DrawEq[agUV]{f o (ae)=a o f e, vector space \Product-\Cols}{g sum \Product-\Cols}
\DrawEq[ahUV]{f o (ae)=a o f e, vector space \Product-\Cols}{h sum \Product-\Cols}
According to the theorem
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS},
the equality
\ShowEq{fov=gov+hov \SideNS-\Cols}
follows from equalities
\eqRef{a.\Product.(b1+b2)=}1,
\eqRef{(b1+b2).\Product.a=}1,
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{g sum \Product-\Cols},
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{h sum \Product-\Cols}.
The equality
\ShowEq{f=g+h}
follows from equalities
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{f sum \Product-\Cols},
\EqRef{fov=gov+hov \SideNS-\Cols}
and the theorem
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}.

Let
\ShowEq{f=g+h}
According to the theorem
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)},
there exist homomorphisms
\ShowEq{vf: A->B}fUV,%
\ShowEq{vf: A->B}gUV,%
\ShowEq{vf: A->B}hUV{}%
such that
\ShowEq{fov=(g+h)ov \SideNS-\Cols}
From the equality
\EqRef{fov=(g+h)ov \SideNS-\Cols}
and the theorem
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS},
it follows that
the homomorphism $\Vector f$
is sum of homomorphisms $\Vector g$, $\Vector h$.
}

\AddEq{definition: vector space of maps B->A n}
{
\begin{ShadedDefinition}
\labelDefinition{\SideWS vector space of maps B->A n}
Let $D$ be commutative ring with unit.
Let $A$ be associative division $D$\Hyph algebra.
For any set $B$
and any integer $n>0$,
we introduce \SideWS vector space
\ShowEq{\SideWS vector space of maps B->A n}
using definition by induction
\ShowEq{\SideWS vector space of maps B->A k}
\end{ShadedDefinition}
}

\DefLabeledDefinition{vector space of algebra A n}{\SideNS}
{
Let $D$ be commutative ring with unit.
Let $A$ be associative division $D$\Hyph algebra.
For any integer $n>0$,
we introduce \SideWS vector space
\ShowEq{\SideWS vector space of algebra A n}
using definition by induction
\ShowEq{\SideWS vector space of algebra A k}
}

\DefTheorem{coordinates of vector of vector space}
{
Coordinates of vector $v\in V$ relative to basis $\Basis e$
of left $\Base$\Hyph vector space $V$
are uniquely defined.
}

\DefLabeledTheorem{coordinates of vector}{\SideNS-\Cols}
{
Coordinates of vector $v\in V$ relative to basis $\Basis e$
of \SideWS \Free $\Base$\Hyph \VectorSet $V$
are uniquely defined.
The equality
\DrawEq{e*v=e*w,\SideNS}{\Cols}
implies the equality
\ShowEq{=> v=w}
}

\DefProof{coordinates of vector}
{
According to the theorem
\refTheorem{basis over division algebra}{\SideNS},
the system of vectors
\ShowEq{expansion relative basis, vector space, 0}
is linearly dependent and in equality
\DrawEq{expansion relative basis, vector space, 1}{\SideNS-\Cols}
at least $b$ is different from $0$. Then equality
\DrawEq{expansion relative basis, vector space, 2}{\SideNS-\Cols}
follows from
\eqRef{expansion relative basis, vector space, 1}{\SideNS-\Cols}.
The equality
\DrawEq{expansion relative basis, vector space}{\SideNS-\Cols}
follows from the equality
\eqRef{expansion relative basis, vector space, 2}{\SideNS-\Cols}.

Assume we get another expansion
\DrawEq{expansion relative basis, vector space, 3}{\SideNS-\Cols}
We subtract
\eqRef{expansion relative basis, vector space}{\SideNS-\Cols}
from
\eqRef{expansion relative basis, vector space, 3}{\SideNS-\Cols}
and get
\DrawEq{expansion relative basis, vector space, 4}{\SideNS-\Cols}
Since vectors \ARow ei are linearly independent,
then the equality
\DrawEq{expansion relative basis, vector space, 5}{\SideNS-\Cols}
follows from the equality
\eqRef{expansion relative basis, vector space, 4}{\SideNS-\Cols}.
Therefore, the theorem follows from the equality
\eqRef{expansion relative basis, vector space, 5}{\SideNS-\Cols}.
}

\DefProof{coordinates of vector 2022}
{
According to the theorem
\refTheorem{basis over division algebra}{\SideNS},
the system of vectors
\ShowEq{expansion relative basis, vector space, (0)}
is linearly dependent and in equality
\ShowEq{expansion relative basis, vector space, 1 \SideNS}
at least $b$ is different from $0$. Then equality
\ShowEq{expansion relative basis, vector space, 2 \SideNS}
follows from
\EqRef{expansion relative basis, vector space, 1 \SideNS}.
The equality
\ShowEq{expansion relative basis, vector space \SideNS}
follows from the equality
\EqRef{expansion relative basis, vector space, 2 \SideNS}.

Assume we get another expansion
\ShowEq{expansion relative basis, vector space, 3 \SideNS}
We subtract
\EqRef{expansion relative basis, vector space \SideNS}
from
\EqRef{expansion relative basis, vector space, 3 \SideNS}
and get
\ShowEq{expansion relative basis, vector space, 4 \SideNS}
Since vectors \ARow ei are linearly independent,
then the equality
\DrawEq{expansion relative basis, vector space, 5()}{\SideNS}
follows from the equality
\EqRef{expansion relative basis, vector space, 4 \SideNS}.
Therefore, the theorem follows from the equality
\eqRef{expansion relative basis, vector space, 5()}{\SideNS}.
}

\DefProof{coordinates of vector *}
{
The theorem follows from the theorem
\refTheorem{coordinates of vector}{\SideNS-*}.
}

\DefExample{system of linear equations, right vector space of columns}
{
Let $V$ be a right $A$\Hyph vector space of columns and
row
\ShowEq{rcd linear span, 0}
be set of vectors.
The vector $\Vector b$
linearly dependends on vectors $\aD{\Vector a}i$,
if linear equation
\DrawEq{rcd linear span, 2}f
where
\DrawEq[xn]{a=(a1.n col)}{}
is column of unknown coefficients of expansion
has a solution.
Suppose
\DrawEq[{}jJ]{basis e of module cols}-
is a basis.
Then vectors
\ShowEq{rcd linear span, 6}
have expansion
\ShowEq{rcd linear span, 7}
If we substitute \EqRef{rcd linear span, b}
and \EqRef{rcd linear span, ai}
into
\eqRef{rcd linear span, 2}f
we get
\DrawEq{rcd linear span, 8}f
Applying theorem \RefTheorem{coordinates of vector of vector space}
to
\eqRef{rcd linear span, 8}f
we get
\AddIndex{system of linear equations}
{system of linear equations}
\DrawEq{system of rcd linear equations}f

Let
\ShowEq{a1n= b= column}
Then we can write system of linear equations
\eqRef{system of rcd linear equations}f
in the following form
\ShowEq{star rows system of linear equations 1}
The equality
\ShowEq{star rows system of linear equations}
follows from equalities
\ePrints{339295394}%
\ifx\Semafor\ValueOn%
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
and
\else%
\EqRef{rc-product of matrices},
\fi%
\EqRef{star rows system of linear equations 1}.
If we write the sum
\EqRef{star rows system of linear equations}
as row, we will get
\DrawEq{star rows system of linear equations 2}2
We see in the system of linear equations
\eqRef{star rows system of linear equations 2}2,
that $A$\Hyph column $b$ is right linear composition of $A$\Hyph columns
\ShowEq{aD1n}
}

\DefLabeledDefinition{rank of matrix}{\Product}
{
If submatrix $\aUD aST$ is \ProductType nonsingular matrix
then we say that
\ProductType rank of matrix $a$ is not less then $\gik$.
{\bf\ProductType rank of matrix} $a$,
\ShowEq{\Product-rank of matrix}
is the maximal value of $\gik$.
We call an appropriate submatrix the
{\bf \ProductType major submatrix}.
}

\DefLabeledTheorem{vector space of maps B->A}{\SideNS}
{
Let $D$ be commutative ring with unit.
Let $A$ be associative division $D$\Hyph algebra.
For any set $B$,
the representation
\ShowEq{representation \SideWS vector space of maps B->A}
is \SideWS vector space
\ShowEq{\SideWS vector space of maps B->A}
over $D$\Hyph algebra $A$.
}

\DefProof{vector space of maps B->A}
{
According to the theorem
\RefTheorem{set of maps B->A is Abelian group},
the set of maps $A^B$ is Abelian group.
From the equality
\ShowEq{\SideWS a(h+g)=}
and definitions
\RefDefinition{homomorphism},
\RefDefinition{endomorphism},
it follows that the map $f(a)$ is endomorphism of Abelian group $A^B$.
From equalities
\ShowEq{\SideWS (a1+a2)h=}
\ShowEq{\SideWS a1a2h=}
and definitions
\RefDefinition{homomorphism},
\RefDefinition{representation of algebra},
it follows that the map $f$ is
representation of $D$\Hyph algebra $A$ in Abelian group $A^B$.
The theorem follows from the definition
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
}

\DefText{linear span, vector space}
{
\subsection{\SideWSC
\texorpdfstring{$A$}{A}-vector space of \ColN s}
\ShowText{linear span in vector space}
}

\DefLabeledDefinition{coordinates of vector}{\SideWS \VectorSetNS}
{
Let $\Basis e$ be the quasibasis of \SideWS $\Base$\Hyph \VectorSet $V$
and vector
\ShowEq{vv in V}vV
has expansion
\DrawEq{vv=ve \SideWS module}{Definition}
with respect to the quasibasis $\Basis e$.
$\Base_{\BaseExt}$\Hyph numbers $\ACol vi$ are called
\AddIndex{coordinates}{coordinates}
of vector $\Vector v$ with respect to the quasibasis $\Basis e$.
Matrix of $\Base_{\BaseExt}$\Hyph numbers
\ShowEq{coordinate matrix of vector}
is called
\AddIndex{coordinate matrix of vector}{coordinate matrix of vector}
$\Vector v$ in quasibasis $\Basis e$.
}

\DefLabeledTheorem{matrix and system of linear equations}{\SideNS-\Cols}
{
Consider the matrix
\DrawEq{matrix a = set ai \Cols}{\SideNS}
Then the system of linear equations
\eqRef{a*x=b \SideNS}{\Cols}
can be represented as
\ShowEq{a*x=b \SideNS-\Cols}
\DrawEq{a*x=b 1 \SideNS-\Cols}1
}

\DefProof{matrix and system of linear equations}
{
The equality
\EqRef{a*x=b \SideNS-\Cols}
follows from equalities
\eqRef{linear span, b \SideNS}{b \Cols},
\eqRef{a=(a1.n set)}{xm \SideNS-\Cols},
\eqRef{a*x=b \SideNS}{\Cols},
\eqRef{matrix a = set ai \Cols}{\SideNS}
and from the definition
\RefDefinition{\RowNWS over \ColNWS product}.
}

\DefLabeledTheoremNote{nonsingular system of linear equations}{\SideNS-\Cols}
{
Solution of nonsingular system of linear equations
\newline
\FrameEqRef{a*x=b 1 \SideNS-\Cols}1
\newline
is determined uniquely and can be presented
in either form\,\footnotemark
\DrawEq{x=a-*b, matrix \SideNS}{\Cols}
\DrawEq{x=a-*b, quasideterminant \SideNS}{\Cols}
}
{
We can see a solution of system
\eqRef{a*x=b 1 \SideNS-\Cols}1
in theorem
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=19}{1.6.1}.
I repeat this statement because I slightly changed the notation.
}

\DefProof{nonsingular system of linear equations}
{
Multiplying both sides of the equation
\eqRef{a*x=b 1 \SideNS-\Cols}1
from left by $a^{\InverseVal}$, we get
\eqRef{x=a-*b, matrix \SideNS}{\Cols}.
Using definition
\newline
\FrameEqRef{quasideterminant and inverse}{\Product}
\newline
we get
\eqRef{x=a-*b, quasideterminant \SideNS}{\Cols}.
Based on the theorem
\RefTheorem{two rc-products equal},
the solution is unique.
}

\DefLabeledDefinition{nonsingular system of linear equations}{\SideNS-\Cols}
{
Let $a$
be \ProductType nonsingular matrix. We call appropriate
system of linear equations
\newline
\FrameEqRef{a*x=b 1 \SideNS-\Cols}1
\newline
\AddIndex{nonsingular system of linear equations}
{nonsingular system of linear equations}.
}

\DefLabeledTheorem{linear span and system of equations}{\SideNS-\Cols}
{
Let
\DrawEq{basis e of module}-
be a basis.
Let vectors
\ShowEq{linear span, 6}
have expansion
\DrawEq[b]{linear span, b \SideNS}{b \Cols}
\DrawEq[{\ARow ai}{}]{linear span, b \SideNS}{a \Cols}
The vector $\Vector b$
linearly dependends on vectors $\ARow{\Vector a}i$
\ShowEq{linear span, 1}
if there exist \ColWS of $A$\Hyph numbers
\DrawEq[xm]{a=(a1.n set)}{xm \SideNS-\Cols}
which satisfy the
\AddIndex{system of linear equations}
{system of linear equations}
\DrawEq{a*x=b \SideNS}{\Cols}
}

\DefProof{linear span and system of equations}
{
The equality
\DrawEq{e*b=e*a*x \SideNS}{\Cols}
follows from equalities
\eqRef{linear span, 2 \SideNS}{\SideNS-\Cols},
\eqRef{linear span, b \SideNS}{b \Cols},
\eqRef{linear span, b \SideNS}{a \Cols}.
The equality
\DrawEq{b=a*x \SideNS}{\Cols}
follows from the equality
\eqRef{e*b=e*a*x \SideNS}{\Cols}
and the theorem
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
The equality
\eqRef{a*x=b \SideNS}{\Cols}
follows from the equality
\eqRef{b=a*x \SideNS}{\Cols}.
}

\DefLabeledTheorem{linear span is vector space}{\SideNS-\Cols}
{
$\spanb$ is subspace of \SideWS $A$\Hyph vector space of \ColN s.
}

\DefProof{linear span is vector space}
{
Suppose
\ShowEq{linear span, vector space, 1}
According to the theorem
\refTheorem{vector in linear span}{\SideNS-\Cols}
\DrawEq[bb]{linear span, 2 \SideNS}{b \SideNS-\Cols}
\DrawEq[cc]{linear span, 2 \SideNS}{c \SideNS-\Cols}
Then
\ShowEq{linear span, 3 \SideNS}
This proves the statement.
}

\DefLabeledDefinition{module type}{\SideNS-\Cols}
{
We represented the set of vectors
\ShowEq{\RowN() 1n}vm{}
as
\RowNWS of matrix
\DrawEq[vm]{a=(a1.n \RowN)}{}
and the set of $\Base_{\BaseExt}$\Hyph nummbers
\ShowEq{\ColNS() 1n}cm{}
as
\ColWS of matrix
\DrawEq[cm]{a=(a1.n \ColNS)}{cm \SideNS-\Cols}
Corresponding representation of \SideWS $\Base$\Hyph \VectorSet $V$ is called
\AddIndex{\SideWS $\Base$\Hyph \VectorSet of \ColN s}{\SideWS A-\ColNWS space},
and $V$\Hyph number is called
\AddIndex{\ColWS vector}{\ColNWS vector}.
}

\DefLabeledTheorem{linear combination in module type}{\SideNS-\Cols}
{
We can represent linear combination
\ShowEq{linear combination, \SideNS-\Cols}cvm
of vectors
\ShowEq{\RowNWS set 1n}vm{}
as \ProductType product of matrices
\DrawEq[cvm]{w.e, \SideNS-\Cols}{cv}
}

\DefProof{linear combination in module type}
{
The theorem follows from definitions
\refDefinition{linear combination of vectors}{\SideNS},
\refDefinition{module type}{\SideNS-\Cols}.
}

\DefLabeledTheorem{vector in linear span}{\SideNS-\Cols}
{
Let $V$ be a \SideWS $A$\Hyph vector space of \ColsWS and
\RowNWS
\ShowEq{linear span, 0}
be set of vectors.
The vector $\Vector b$
linearly dependends on vectors $\ARow{\Vector a}i$
\ShowEq{linear span, 1}
if there exist \ColWS of $A$\Hyph numbers
\DrawEq[xm]{a=(a1.n set)}{}
such that the following equality is true
\DrawEq[bx]{linear span, 2 \SideNS}{\SideNS-\Cols}
}

\DefProof{vector in linear span}
{
The equality
\eqRef{linear span, 2 \SideNS}{\SideNS-\Cols}
follows from the definition
\refDefinition{linear span, vector space}{\SideNS-\Cols}
and the theorem
\refTheorem{linear combination in module type}{\SideNS-\Cols}.
}

\DefLabeledDefinition{linear span, vector space}{\SideNS-\Cols}
{
Let $V$ be a \SideWS $A$\Hyph vector space of \ColsWS and
\ShowEq{linear span, set}
be set of vectors.
\AddIndex{Linear span}{linear span, vector space}
in \SideWS $A$\Hyph vector space of \ColsWS is set
\ShowEq{linear span, vector space}
of vectors linearly dependent on vectors
\ARow {\Vector a}i.
}

\DefLabeledTheorem{vector space of algebra A}{\SideNS}
{
Let $D$ be commutative ring with unit.
Let $A$ be associative division $D$\Hyph algebra.
The representation generated by \SideWS shift
\ShowEq{representation \SideWS vector space of algebra A}
is \SideWS vector space
\ShowEq{\SideWS vector space of algebra A}
over $D$\Hyph algebra $A$.
}

\DefProof{vector space of algebra A}
{
According to definitions
\refDefinition{module over algebra}{\SideWS \VectorSetNS},
\RefDefinition{algebra over ring},
$D$\Hyph algebra $A$ is Abelian group.
From the equality
\ShowEq{\SideWS a(b+c)=}
and definitions
\RefDefinition{homomorphism},
\RefDefinition{endomorphism},
it follows that the map
\ShowEq{\SideWS a->ab}
is endomorphism of Abelian group $A$.
From equalities
\ShowEq{\SideWS (a1+a2)b=}
\ShowEq{\SideWS a1a2b=}
and definitions
\RefDefinition{homomorphism},
\RefDefinition{representation of algebra},
it follows that the map $f$ is
representation of $D$\Hyph algebra $A$ in Abelian group $A$.
The theorem follows from the definition
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
}

\AddEq{def row text}
{%
\def\ColWS{row }%
\def\ColsWS{rows }%
\def\ColTNS{rows}%
\def\RowsNS{columns}%
\def\RowsRWSA{columns }%
}
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\AddEq{def col text}
{%
\def\ColWS{column }%
\def\ColsWS{columns }%
\def\ColTNS{columns}%
\def\RowsNS{rows}%
\def\RowsRWSA{rows }%
}
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\DefLabeledDefinition{spectrum of matrix}{\Product}
{
The set
\ShowEq{spectrum of matrix}
of all left and right
\ProductType eigenvalues is called
\ProductType spectrum of the matrix a.
}

\DefLabeledTheorem{vector space over algebra}{\SideNS}
{
The following diagram of representations describes \SideWS $A$\Hyph vector space $V$
\DrawEq[{}{}{}{}]{diagram of representations, \SideWS module}1
The diagram of representations
\EqRef{diagram of representations, \SideWS module}
holds
\AddIndex{commutativity of representations}{commutativity of representations}
of commutative ring $D$ and $D$\Hyph algebra $A$
in Abelian group $V$
\ShowEq{\SideWS module, a d v}
}

\DefProof{vector space over algebra}
{
The diagram of representations
\EqRef{diagram of representations, \SideWS module}
follows from the definition
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
and from the theorem
\RefTheorem{Free Algebra over Ring}.
Since \SideNS\HSide transformation $\ATransf(a)$
is endomorphism
of $\CBase$\Hyph vector space $V$,
we obtain the equality
\EqRef{\SideWS module, a d v}.
}

\DefLabeledTheorem{definition of vector space}{\SideNS}
{
Let $V$ be \SideWS $A$\Hyph vector space.
Following conditions hold for $V$\Hyph numbers:
\begin{itemize}
\item 
\AddIndex{commutative law}{commutative law}
\DrawEq{commutative law}{\SideWS vector space}
\item 
if $D$\Hyph algebra $A$ is associative, then
\AddIndex{associative law}{associative law}
holds
\DrawEq{associative law, \SideWS module}1
\item 
\AddIndex{distributive law}{distributive law}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{unitarity law}{unitarity law}
\ShowEq{unitarity law, \SideWS A-module}
\end{itemize}
for any
\ShowEq{p,q in A, v,w in V}
}

\DefProof{definition of vector space}
{
The equality
\eqRef{commutative law}{\SideWS vector space}
follows from definitions
\refDefinition{module over algebra}{vector space},
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
Since \SideNS-side transformation $p$
is endomorphism of the Abelian group $V$,
we obtain the equation
\eqRef{distributive law, \SideWS module, 1}1.
Since representation
$g_{3,4}$
is homomorphism of the additive group
of $D$\Hyph algebra $A$,
we obtain the equation
\eqRef{distributive law, \SideWS module, 2}1.
Since representation
$g_{3,4}$
is \SideNS\Hyph side representation
of the multiplicative group of $D$\Hyph algebra $A$,
we obtain the equality
\EqRef{unitarity law, \SideWS A-module}.
Since representation
$g_{3,4}$
is \SideNS\Hyph side representation
of the multiplicative group of $D$\Hyph algebra $A$,
we obtain the equality
\eqRef{associative law, \SideWS module}1
when $D$\Hyph algebra $A$ is associative.
}

\DefLabeledTheorem{coordinate matrix of vector}{\SideNS-\Cols}
{
If we write vectors of basis $\Basis e$
as \RowNWS of matrix
\DrawEq[en]{a=(a1.n \RowN)}{type \SideNS-\Cols}
and coordinates of vector
\ShowEq{w=w*e \SideNS-\Cols}w{}
with respect to basis $\Basis e$ as
\ColWS of matrix
\DrawEq[wn]{a=(a1.n \ColNS)}{type \SideNS-\Cols}
then we can represent the vector
$\Vector w$
as \ProductType product of matrices
\DrawEq[w]{vector w=w*e \SideNS-\Cols}w
}

\DefProof{coordinate matrix of vector}
{
The theorem follows from the theorem
\refTheorem{linear combination in module type}{\SideNS-\Cols}.
}

\DefLabeledExample{Vector Space Type}{\SideNS-\Cols}
{
\ePrints{2022.01.05}
\ifx\Semafor\ValueOff
We represented the set of vectors
\ShowEq{\RowNWS set 1n}vm{}
as
\RowNWS of matrix
\DrawEq[vm]{a=(a1.n \RowN)}{}
and the set of $A$\Hyph nummbers
\ShowEq{\ColNWS set 1n}cm{}
as
\ColWS of matrix
\DrawEq[cm]{a=(a1.n \ColNS)}{cm \SideNS-\Cols}
Thus we can represent linear combination of vectors
\ShowEq{\RowNWS set 1n}vm{}
as \ProductType product of matrices
\DrawEq[{\ParmA}{\ParmB}m]{w.e, \SideNS-\Cols}{\ParmA\ParmB}
In particular,
if
\else
If
\fi
we write vectors of basis $\Basis e$ as
\RowNWS of matrix
\DrawEq[en]{a=(a1.n \RowN)}{\SideNS-\Cols}
and coordinates of vector
\ShowEq{w=w*e \SideNS-\Cols}w{}
with respect to basis $\Basis e$ as
\ColWS of matrix
\DrawEq[wn]{a=(a1.n \ColNS)}{\SideNS-\Cols}
then we can represent the vector
$\Vector w$
as \ProductType product of matrices
\DrawEq[w]{vector w=w*e \SideNS-\Cols}w
Corresponding representation of vector space $V$ is called
\AddIndex{\SideWS $A$\Hyph vector space of \ColN s}{\SideWS A-\ColNWS space},
and $V$\Hyph number is called
\AddIndex{\ColWS vector}{\ColNWS vector}.
}

\DefRemark{Left and Right Eigenvalues not equal 0}
{
According to the definition given above,
sets of left and right \ProductType eigenvalues coincide.
However, we considered the most simple case.
Cohn considers definitions

\ShowEq{def right}
\ShowEq{\DefCol}
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
\ShowEq{def left}
\ShowEq{\DefRow}
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1

\noindent
where $a_2$ is non\Hyph \ProductType singular matrix
as starting point for research.
}

\AddEq{remark: Left and Right Eigenvalues not equal}
{
Let multiplicity of all \SideWS \ProductType eigenvalues
of \nTimes matrix $a_2$ equal $1$.
Let \nTimes matrix $a_2$ do not have $\gin$
\SideWS \ProductType eigenvalues,
but have
\ShowEq{gik<gin}
\SideWS \ProductType eigenvalues.
In such case, the matrix $u_2$ in the equality

\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1

\noindent
is
\ShowEq{gin x gik \SideNS}
matrix and the matrix $a_1$
is \nTimes[k] matrix.
However, the equality
\eqRef{A \ProductS U=U \ProductS D \SideNS}1
does not imply that
\ShowEq{rank rc u2 =k}

Let
\ShowEq{rank rc u2 =k}
Then there exists
\ShowEq{gin x gik \OtherSideNS}
matrix
\ShowEq{a in left}w{u_2}{\OtherSideNS}{}
such that
\ShowEq{w rc u2=Ek \SideNS}
The equality
\ShowEq{w rc a2 rc u2=a1 \SideNS}
follows from equalities
\eqRef{A \ProductS U=U \ProductS D \SideNS}1,
\EqRef{w rc u2=Ek \SideNS}.

Let
\ShowEq{rank rc u2 <k}
Then 
there exists linear dependence between
\SideWS eigenvectors.
In such case,
sets of left and right \ProductType eigenvalues do not coincide.
}

\DefText[4]{define homomorphism of vector space(1)}
{
According to definitions
\ShowRef{define homomorphism A module}
the map
\DrawEq[gA]{homomorphism D algebra #1#2}{\SideWS vector}
is homomorphism
of $D_{#1}$\Hyph algebra $A_{#2}$
into $D_{#3}$\Hyph algebra $A_{#4}$.
Therefore, equalities
\ShowEq{ref homomorphism of A vector space(#1)}{#1}{#2}{#3}
follow from the theorem
\refTheorem{linear map of D module}{#1#2}.
}

\DefText[4]{define homomorphism of vector space()}
{
}

\AddEq{remark: colinear vectors}
{
Vectors $v$ and
\ShowEq{av \SideNS}
are called
\OtherSideWS
\AddIndex{colinear}{colinear vectors}.
The statement that vectors $v$ and $w$ are
\OtherSideWS colinear vectors
does not imply that
vectors $v$ and $w$ are \SideWS linearly dependent.
}

\DefText[7]{be extended basis}
{
Let the basis
\DrawEq[{#1}{#2}{#3}{#4}{#5}{#6}]{extended basis}{#7}
be extension of the basis \eV[1][.]
}

\DefLabeledTheorem{Two bases of module}{\SideNS-\Cols}
{
\ShowEq{Let be basis of algebra}{}{}kKD{}A{}-
\ShowEq{Let be basis of module}1{}iI{\SideWS}A{}V{}
Then the set of $V$\Hyph numbers
\DrawEq[2{}{}{}ik]{extended basis}{\SideNS-\Cols}
is the basis of $D$\Hyph \VectorSet $V$.
The basis \eV[2] is called extension of the basis \eV[1][.]
}

\DefProofRef{Two bases of module}{\SideNS-\Cols}
{
The theorem follows from the theorem
\refTheorem{basis over division algebra}{\SideNS}
and from lemmas
\refLemma{Two bases of module 1}{\SideNS-\Cols},
\refLemma{Two bases of module 2}{\SideNS-\Cols}.
}

\DefLabeledLemma{Two bases of module 1}{\SideNS-\Cols}
{
The set of $V$\Hyph numbers \EBase 2{ik}
generates $D$\Hyph \VectorSet $V$.
}

\DefLemmaProof{Two bases of module 1}
{
Let
\DrawEq{Two bases of module 1 a}{\SideNS-\Cols}
be any $V$\Hyph number.
For any $A$\Hyph number \ACol ai,
according to the definition
\RefDefinition{algebra over ring}
and the convention
\RefConvention{basis of algebra as basis of module},
there exist $D$\Hyph numbers \ACol a{ik} such that
\DrawEq{Two bases of module 1 ai}{\SideNS-\Cols}
The equality
\DrawEq{Two bases of module 1 a=ai}{\SideNS-\Cols}
follows from equalities
\eqRef{extended basis}{\SideNS-\Cols},
\eqRef{Two bases of module 1 a}{\SideNS-\Cols},
\eqRef{Two bases of module 1 ai}{\SideNS-\Cols}.
The lemma
follows from the equality
\eqRef{Two bases of module 1 a=ai}{\SideNS-\Cols}.
}

\DefLabeledLemma{Two bases of module 2}{\SideNS-\Cols}
{
The set of $V$\Hyph numbers \EBase 2{ik}
is linearly independent over the ring $D$.
}

\DefLemmaProof{Two bases of module 2}
{
Let
\DrawEq{extended basis 1}{\SideNS-\Cols}
The equality
\DrawEq{extended basis 2}{\SideNS-\Cols}
follows from equalities
\eqRef{extended basis}{\SideNS-\Cols},
\eqRef{extended basis 1}{\SideNS-\Cols}.
According to the theorem
\refTheorem{basis over division algebra}{\SideNS},
the equality
\DrawEq{extended basis 3}{\SideNS-\Cols}
follows from the equality
\eqRef{extended basis 2}{\SideNS-\Cols}.
The equality
\DrawEq{extended basis 4}{\SideNS-\Cols}
follows from the equality
\eqRef{extended basis 3}{\SideNS-\Cols}.
Therefore,
the set of $V$\Hyph numbers \EBase 2{ik}
is linearly independent over the ring $D$.
}

\DefLabeledTheorem{product vector over scalar}{\SideNS}
{
\ShowEq{ab in A,v in V}
\DrawEq{(av)b=a(vb)}{\SideNS}
}

\DefProof{product vector over scalar}
{
According to the theorem
\refTheorem{similarity transformation}{\SideNS-\Cols}
and to the definition
\refDefinition{product vector over scalar}{\SideNS},
the equality
\ShowEq{(av)b= \SideNS}
follows from the equality
\eqRef{\SideWS homomorphism, f av=}1.

The equality
\eqRef{(av)b=a(vb)}{\SideNS}
follows from the equality
\EqRef{(av)b= \SideNS}.
}

\DefLabeledDefinition{product vector over scalar}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
Bilinear map
\DrawEq{\OtherSideWS A*V->V}2
generated by \OtherSideNS\Hyph side representation
\ShowEq{twin to \SideWS product}
is called
\AddIndex{\OtherSideNS\Hyph side product}{\OtherSideNS-side product}
of vector over scalar.
}

\DefLabeledLemma{rcd dcr basis}{\SideNS}
{
We can identify basis manifold
\ShowEq{basis manifold of V, \SideNS-cols}{\aD En}{\GL nA}{}
and the set of \ProductType regular matrices \GL nA.
}

\AddEq{proof: rcd dcr basis 1}
{
\begin{sloppypar}
{\sc Proof.}
According to the remark
\refRemark{identify basis and matrix of coordinates}{\SideNS-\Cols},
we can identify a basis $\Basis e$
of \SideWS $A$\Hyph vector space $V$
and the matrix $e$ of coordinates of basis $\Basis e$
withb respect to the basis $\Basis{\aD En}$
\ShowEq{be=e cr En \SideNS}
\hfill\(\odot\)
\end{sloppypar}
}

\DefLabeledDefinition{dimension of vector space}{\SideNS}
{
We call
\AddIndex{dimension of \SideWS $A$\Hyph vector space}{dimension of vector space}
the number of vectors in a basis.
}

\DefLabeledTheorem{coordinate matrix of basis}{\Product-\Cols}
{
\ShowEq{Let V be vector space of}.
The coordinate matrix of basis $\Basis{g}$ relative basis $\Basis e$ of
\SideWS $A$\Hyph vector space $V$ is \ProductType nonsingular matrix.
}

\DefProof{coordinate matrix of basis}
{
According to the theorem
\refTheorem{rank of matrix}{\Product-\Cols},
\CR rank of the coordinate matrix of basis $\Basis{g}$ relative basis $\Basis e$
equal to the dimension of left $A$\Hyph space of columns.
This proves the statement of the theorem.
}

\DefLabeledTheorem{automorphism of vector space}{\Product-\Cols}
{
\ShowEq{Let V be vector space of}.
Let $\Basis e$ be a basis of \SideWS $A$\Hyph vector space $V$.
Then any automorphism $\Vector f$ of \SideWS $A$\Hyph vector space $V$
has form
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{automorphism}
where $f$ is a \ProductType nonsingular matrix.
}

\DefProof{automorphism of vector space}
{
The equality
\eqRef{v1=v2*a \SideNS-\Cols}{automorphism}
follows from theorem
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}.
Because $\Vector f$ is an isomorphism,
for each vector $\Vector v'$ there exist one and only one vector $\Vector v$ such that
\ShowEq{v'=fov}
Therefore, system of linear equations
\eqRef{v1=v2*a \SideNS-\Cols}{automorphism}
has a unique solution. According to corollary
\RefCorollary{nonsingular rows system of linear equations}
matrix $f$ is a \ProductType nonsingular matrix.
}

\DefLabeledTheorem{Automorphisms of vector space form a group}{\Product-\Cols}
{
Matrices of automorphisms of \SideWS $A$\Hyph space $V$ of \ColN s form a group \Group nA.
}

\DefProof{Automorphisms of vector space form a group}
{
If we have two automorphisms $\Vector f$ and $\Vector g$ then we can write
\ShowEq{Automorphisms of vector space, \Product-\Cols}
Therefore, the resulting automorphism has matrix $f\ProductVal g$.
}

\DefLabeledTheorem{av=bv=>a=b}{\SideNS-\Cols}
{
If \SideWS $A$\Hyph vector space $V$
has finite dimension,
then the statement
\DrawEq{av=bv, v \SideNS}{\Cols}
implies $a=b$.
}

\DefProof{av=bv=>a=b}
{
Let the set of vectors
\DrawEq[{}jJ]{basis e of module cols}-
be the basis of left $A$\Hyph vector space $V$.
According to theorems
\refTheorem{definition of vector space}{\SideNS},
\refTheorem{coordinates of vector}{\SideNS-\Cols},
the equality
\ShowEq{avi=bvi \SideNS-\Cols}
follows from the equality
\eqRef{av=bv, v \SideNS}{\Cols}.
The theorem follows from the equality
\EqRef{avi=bvi \SideNS-\Cols},
if we assume $v=\aD e1$.
}

\DefText[7]{matrix of numbers}
{
Let
\ShowEq{matrix fIJ}{#3}{#4}{#5}{#6}{#7}
be matrix of $#1_{#2}$\Hyph numbers.
}

\DefText[9]{matrix of numbers and C}
{
Let
\ShowEq{matrix fIJ}{#3}{#4}{#5}{#6}{#7}
be matrix of $#1_{#2}$\Hyph numbers
which satisfy the equality
\ShowRef{algebra, homomorphism and product}{#8}{#9}{#3}
}

\DefText{map be homomorphism of ring (1)}
{
Let the map
\DrawEq[h{D_1}{D_2}{}]{f: A->B}{}
be homomorphism of the ring $D_1$ into the ring $D_2$.
}

\DefText{map be homomorphism of ring ()}
{
}

\DefLabeledTheorem[6]{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrices of numbers(#2#3)}{#4}{#5}{#1}{#2}
The map\refFootnote{homomorphism of A module}{\SideNS-\Cols(#1#2#3)}
\newline
\FrameEqRef[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{Vector \SideNS-\Cols}
\newline
defined by the equality
\ShowText{define homomorphism A module by matrix(#1#2#3)}
is homomorphism
of \SideWS $A$\Hyph vector space of \ColN s.
The homomorphism
\eqRef{homomorphism A module #1#2#3}{Vector \SideNS-\Cols}
which has the given%
\ShowText{define homomorphism by given matrix(#2)}%
is unique.
}

\DefText{define homomorphism by given matrix(1)}
{
set of matrices $(g,f)$
}

\DefText{define homomorphism by given matrix()}
{
matrix $f$
}

\DefText[4]{matrix generates homomorphism (1)}
{
According to the theorem
\refTheorem{matrix generates D algebra homomorphism}{\Cols(#1#2)},
the map
\DrawEq[{\Vector g}A]{homomorphism D algebra #1#2}{(\SideNS-\Cols)algebra}
is homomorphism
of $D_{#1}$\Hyph algebra $A_{#2}$
into $D_{#3}$\Hyph algebra $A_{#4}$
and the homomorphism
\eqRef{homomorphism D algebra #1#2}{(\SideNS-\Cols)algebra}
is unique.

}

\DefText[4]{matrix generates homomorphism ()}
{
}

\DefProof[7]{matrix generates A module homomorphism}
{
\ShowText{matrix generates homomorphism (#2)}{#1}{#2}{#4}{#5}
The equality
\DrawEq{fo(v+w) (#2)\SideNS-\Cols}{(#1#2)}
\begin{sloppypar}
\noindent
follows from equalities
\ShowRef{matrix generates A module homomorphism(#2)}{#2}{#3}{#7}
From the equality
\eqRef{fo(v+w) (#2)\SideNS-\Cols}{(#1#2)},
it follows that the map $\Vector f$ is homomorphism
of Abelian group.
The equality
\end{sloppypar}
\DrawEq{fo(va) (#2)\SideNS-\Cols}{(#1#2)}
follows from equalities
\ShowRef{fo(va)(#2)}{#2}{#3}{#7}
From the equality
\eqRef{fo(va) (#2)\SideNS-\Cols}{(#1#2)},
and definitions
\RefDefinition{Morphism of Diagram of Representations},
\refDefinition{homomorphism A module}{\SideNS(#1#2#3)},
it follows that the map
\newline
\FrameEqRef[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{Vector \SideNS-\Cols}
\newline
\begin{sloppypar}
\noindent
is homomorphism
of $A_{#2}$\Hyph \VectorSet of \ColN s $V_{#3}$
into $A_{#5}$\Hyph \VectorSet of \ColN s $V_{#6}$.
\end{sloppypar}

Let $f$ be
matrix of homomorphisms $\Vector f$, $\Vector g$
relative to bases
\ShowEq{Bases eVW}VW{}.%
The equality
\ShowEq{fov=gov \SideNS-\Cols}
follows from the theorem
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}.
Therefore, $\Vector f=\Vector g$.
}

\DefLabeledTheorem[6]{homomorphism A module}{\SideNS-\Cols(#1#2#3)}
{
The homomorphism\refFootnote{homomorphism of A module}{\SideNS-\Cols(#1#2#3)}
\DrawEq[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{Vector \SideNS-\Cols}
of \SideWS $A_{#2}$\Hyph \VectorSet $V_{#3}$
into \SideWS $A_{#5}$\Hyph \VectorSet $V_{#6}$
has presentation
\ShowText{g:A1->A2, D module(#1#2#3)}
\ShowText{f o (ae)=a o f e (#2#3)}{#1}{#2}{#3}
relative to selected bases.
Here
\begin{itemize}
\ShowText{homomorphism of vector space, algebra(#2)}{#1}{#2}{#3}{#4}{#5}{#6}
\ShowText{homomorphism of vector space, algebra 1}{#1}{#2}{#3}{#4}{#5}{#6}
\end{itemize}
\ShowText{matrix of homomorphism relative bases #2#3}{#1}{#2}{#3}
}

\DefText[3]{matrix of homomorphism relative bases 11}
{
The set of matrices $(g,f)$ is unique and is called
{\bf coordinates of homomorphism}
\eqRef{homomorphism A module #1#2#3}{Vector \SideNS}
relative bases \eV[V_1][,] \eV[V_2][.]
}

\DefText[3]{matrix of homomorphism relative bases 1}
{
The matrix $f$ is unique and is called
{\bf matrix of homomorphism}
$\Vector f$ relative bases \eV[1][,] \eV[2][.]
}

\DefText[6]{Proof, homomorphism of vector space(1)}
{
According to definitions
\ShowRef{Proof, homomorphism of vector space}{#1}{#2}{#3}%
the map
\DrawEq[{\Vector g}A]{homomorphism D algebra #1#2}{\SideNS-\Cols}
is homomorphism
of $D_{#1}$\Hyph algebra $A_{#2}$
into $D_{#4}$\Hyph algebra $A_{#5}$.
Therefore, equalities
\ShowRef{Proof, homomorphism of vector space 1}{#1}{#2}{#3}%
follow from equalities
\ShowRef{Proof, homomorphism of vector space 2}{#1}{#2}{#3}%
From the theorem
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
it follows that the matrix $g$ is unique.

}

\DefText[6]{Proof, homomorphism of vector space()}
{%
}

\DefProof[6]{homomorphism A module}
{
\ShowText{Proof, homomorphism of vector space(#2)}{#1}{#2}{#3}{#4}{#5}{#6}%
Vector
\ShowEq{vv in V}v{V_1}
has expansion
\DrawEq[v{V_1}]{\SideWS homomorphism \Product, 1}{v#1#2#3}
relative to the basis \eV[V_1][.]
Vector
\ShowEq{vv in V}w{V_2}
has expansion
\DrawEq[w{V_2}]{\SideWS homomorphism \Product, 1}{w#1#2#3}
relative to the basis \eV[V_2][.]
Since $\Vector f$ is a homomorphism,
then the equality
\DrawEq{vv=v*eV \SideWS \Product(#2)}{(#1)}
follows from equalities
\eqRef{homomorphism, f v+w=}{f(#1#2)\SideWS A module},
\eqRef{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module}.
$V_2$\Hyph number
\ShowEq{Vector f(e) \Cols}
has expansion
\DrawEq{f o ei=fij ej \SideWS \Product}{#1#2#3}
relative to basis \eV[V_2][.]
The equality
\DrawEq{vb=a cr f cr e \SideWS \Product(#2)}{(#1)}
follows from equalities
\eqRef{vv=v*eV \SideWS \Product(#2)}{(#1)},
\eqRef{f o ei=fij ej \SideWS \Product}{#1#2#3}.
The equality
\eqRef{v1=v2*a \SideNS-\Cols}{\SideNS(#1#2#3)}
follows from comparison of
\eqRef{\SideWS homomorphism \Product, 1}{w#1#2#3}
and \eqRef{vb=a cr f cr e \SideWS \Product(#2)}{(#1)} and
the theorem
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
From the equality
\eqRef{f o ei=fij ej \SideWS \Product}{#1#2#3}
and from the theorem
\refTheorem{coordinates of vector}{\SideNS-\Cols},
it follows that the matrix $f$ is unique.
}

\DefText{notation for homomorphism of module}
{
We will use notation
\DrawEq{f circ a =}{}
for image of homomorphism $f$.
}

\DefText{be division algebra}
{
Let $D$\Hyph algebra $A$ be division algebra.
}

\DefTheorem{division algebra has unit}
{
\ShowText{be division algebra}
$D$\Hyph algebra $A$ has unit.
}

\DefTheorem{division D algebra, ring D is the field}
{
\ShowText{be division algebra}
The ring $D$ is the field
and subset of the center of $D$\Hyph algebra $A$.
}

\AddEq[3]{remark: homomorphism of vector space 2}
{
On the basis of theorems
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)(#1#2#3)},
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols}
we identify the homomorphism
$\Vector f$
of \SideWS $A$\Hyph vector space $V$ of \ColN s
and the matrix of its presentation
\newline
\FrameEqRef[afVW]{f o (ae)=a o f e, vector space \Product-\Cols}1
}

\DefLabeledDefinition{similarity transformation}{\SideNS}
{
The endomorphism
\ShowEq{\SideWS map a En}a{}
of \SideWS $A$\Hyph vector space $V$
is called
\AddIndex{similarity transformation}{similarity transformation}
with respect to the basis $\Basis e$.
}

\AddEq{passive transformation for two bases}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
be bases of \SideWS $A$\Hyph vector space $V$.
Let $g$
be passive transformation
of basis $\Basis e_1$ into basis $\Basis e_2$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
}

\DefLabeledTheorem{covariance of eigenvalue}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
be bases of \SideWS $A$\Hyph vector space $V$.

\begin{Statement}
\labelStatement{covariance of eigenvalue \SideNS-\Cols}
Eigenvalue $b$
of the endomorphism $\Vector f$
with respect to the basis $\Basis e_1$
does not depend on the choice of the basis $\Basis e_2$.
\hfill\(\odot\)
\end{Statement}

\begin{Statement}
\labelStatement{covariance of eigenvector \SideNS-\Cols}
Eigenvector $\Vector v$
of the endomorphism $\Vector f$
corresponding to eigenvalue $b$
does not depend on the choice of the basis $\Basis e_2$.
\hfill\(\odot\)
\end{Statement}
}

\DefProof{covariance of eigenvalue}
{
Let
\ShowEq{Ai, i=}f
be the matrix of endomorphism $f$ with respect to the basis $\Basis e_i$.
Let $b$ be eigenvalue
of the endomorphism $\Vector f$
with respect to the basis $\Basis e_1$
and
$\Vector v$ be eigenvector
of the endomorphism $\Vector f$
corresponding to eigenvalue $b$.
Let
\ShowEq{Ai, i=}v
be the matrix of vector $\Vector v$ with respect to the basis $\Basis e_i$.

Suppose first that
\ShowEq{basis e1=e2}
Then $\aD En$
is passive transformation
of basis $\Basis e_1$ into basis $\Basis e_2$
\DrawEq[12{\aD En^{}{}}{}]{e2i=aij e1j \Product-\Cols}{}
According to the theorem
\refTheorem{similarity transformation, change of basis}{\SideNS-\Cols},
the similarity transformation
\ShowEq{\SideWS map a En}b1
has the matrix
\ShowEq{ga*g- \SideNS-En}
with respect to the basis $\Basis e_2$.
Therefore, according to the theorem
\refTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols},
we proved following statements.

\begin{ShadedLemma}
\labelLemma{matrix f-bEn singular \SideNS-\Cols}
The matrix
\ShowEq{f-bEn \SideNS}1{}
is \ProductType singular matrix.
\hfill\(\odot\)
\end{ShadedLemma}

\begin{ShadedLemma}
\labelLemma{vector v1 f-bEn \SideNS-\Cols}
The \ColWS vector $v_1$ satisfies to the system of linear equations
\ShowEq{(f-bEn)v \Product-\Cols}
\hfill\(\odot\)
\end{ShadedLemma}

Suppose that
\ShowEq{basis e1 ne e2}
According to the theorem
\refTheorem{exists representation, commuting with active}{\SideNS-\Cols},
there exists unique passive transformation
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
and $g$ is \ProductType non\Hyph singular matrix.
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[fg{\SideNS}{\Cols}]{f2=a f1 a-}{covariance \SideNS-\Cols}
\begin{sloppypar}
\noindent
According to the theorem
\refTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols},
if $b$ is eigenvalue of endomorphism $\Vector f$,
then we have to prove the lemma
\RefLemma{matrix f-ae singular \SideNS-\Cols}.
\end{sloppypar}

\begin{ShadedLemma}
\labelLemma{matrix f-ae singular \SideNS-\Cols}
The matrix
\[\ShowEq{(f-ae)v matrix}f2bg\]
is \ProductType singular matrix.
\hfill\(\odot\)
\end{ShadedLemma}

\begin{sloppypar}
Since the equality
\ShowEq{f-ae->f-be}
follows from the equality
\eqRef{f2=a f1 a-}{covariance \SideNS-\Cols},
then the lemma
\RefLemma{matrix f-ae singular \SideNS-\Cols}
follows from the lemma
\RefLemma{matrix f-bEn singular \SideNS-\Cols}.
Therefore, we proved the statement
\RefStatement{covariance of eigenvalue \SideNS-\Cols}.
\end{sloppypar}

According to the theorem
\refTheorem{eigenvector coordinates}{\SideNS-\Cols},
if $\Vector v$ is eigenvector of endomorphism $\Vector f$,
then we have to prove the lemma
\RefLemma{vector v2 f-bEn \SideNS-\Cols}.

\begin{ShadedLemma}
\labelLemma{vector v2 f-bEn \SideNS-\Cols}
The \ColWS vector $v_2$ satisfies to the system of linear equations
\ShowEq{(f-bEn)v2 \Product-\Cols}
\end{ShadedLemma}

\begin{sloppypar}
{\sc Proof.}
According to the theorem
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
\DrawEq[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{covariance \SideNS-\Cols}
Since the equality
\ShowEq{f-ae->f-be \SideNS-\Cols}
follows from equalities
\eqRef{f2=a f1 a-}{covariance \SideNS-\Cols},
\eqRef{v2=v1g-}{covariance \SideNS-\Cols},
then the lemma
\RefLemma{vector v2 f-bEn \SideNS-\Cols}
follows from the lemma
\RefLemma{vector v1 f-bEn \SideNS-\Cols}.
\hfill\(\odot\)
\end{sloppypar}

Therefore, we proved the statement
\RefStatement{covariance of eigenvector \SideNS-\Cols}.
}

\DefLabeledTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols}
{
\ShowEq{passive transformation for two bases}
Let $f$ be the matrix of endomorphism $\Vector f$
with respect to the basis $\Basis e_2$.
$A$\Hyph number $b$ is eigenvalue
of endomorphism $\Vector f$ iff the matrix
\DrawEq[f{}bg]{(f-ae)v matrix}{\SideNS-\Cols}
is \ProductType singular.
}

\DefProof{eigenvalue of endomorphism, matrix is singular}
{
The theorem folows from theorems
\RefTheorem{star rows system of linear equations},
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\DefLabeledTheorem{eigenvector coordinates}{\SideNS-\Cols}
{
\ShowEq{passive transformation for two bases}
Let $f$ be the matrix of endomorphism $\Vector f$
and $v$ be the matrix of vector $\Vector v$
with respect to the basis $\Basis e_2$.
The vector $\Vector v$ is
eigenvector
of the endomorphism $\Vector f$
with respect to the basis $\Basis e_1$
iff
there exists $A$\Hyph number $b$ such that
the system of linear equations
\DrawEq[fgbv]{(f-ae)v \Product-\Cols}{fgbv}
has non\Hyph trivial solution.
}

\DefProof{eigenvector coordinates}
{
According to theorems
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)},
\refTheorem{similarity transformation, change of basis}{\SideNS-\Cols},
the equality
\ShowEq{e*f*v=e*ae*v \SideNS-\Cols}
follows from the equality
\eqRef{fov=b e o v}{\SideNS}.
The equality
\eqRef{(f-ae)v \Product-\Cols}{fgbv}
follows from the equality
\EqRef{e*f*v=e*ae*v \SideNS-\Cols}
and from the theorem
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
Since the case $\Vector v=0$ is not interesting for us,
the system of linear equations
\eqRef{(f-ae)v \Product-\Cols}{fgbv}
should have non\Hyph trivial solution.
}

\AddEq{remark: eigenvector coordinates}
{
The definition
\refDefinition{Eigenvalue of Endomorphism}{\SideNS}
does not depend on structure of coordinates
of \SideWS $A$\Hyph vector space $V$.
As soon as we choose the basis $\Basis e$
of \SideWS $A$\Hyph vector space $V$,
we see additional structure
which is reflected in theorems
\refTheorem{eigenvector coordinates}{\SideNS-cols},
\refTheorem{eigenvector coordinates}{\SideNS-rows}.
}

\AddEq{remark: eigenvector of matrix}
{
The same matrix may correspond to different endomorphisms
depending on whether we consider left or right
$A$\Hyph vector space.
Therefore, we must consider all definitions
of eigenvectors which may correspond to given matrix.
From theorems
\refTheorem{eigenvector coordinates}{left-cols},
\refTheorem{eigenvector coordinates}{right-cols},
\refTheorem{eigenvector coordinates}{left-rows},
\refTheorem{eigenvector coordinates}{right-rows},
it follows that for given matrix there exist
four types of eigenvectors and
four types of eigenvalues.
Couple eigenvector and eigenvalue of a certain type
is used in solving the problem
where corresponding type of $A$\Hyph vector space arises.
This statement is reflected in the names
of eigenvector and eigenvalue.

Eigenvector of endomorphism depends on
choice of two bases. However when we
consider eigenvector of matrix,
it is not the choice of bases that is important for us,
but the matrix of passive transformation between these bases.
}

\DefLabeledDefinition{eigenvalues of pair of matrices}{\Product}
{
$A$\Hyph number $b$ is called
{\bf \ProductType eigenvalue}
of the pair of matrices $(f,g)$
where $g$ is the \ProductType non\Hyph singular matrix
if the matrix
\DrawEq[f{}bg]{(f-ae)v matrix}{}
is \ProductType singular matrix.
}

\DefLabeledDefinition{eigenvector of pair of matrices}{\Product-\ColN}
{
Let $A$\Hyph number $b$ be
\ProductType eigenvalue of the pair of matrices
\ShowEq{pair of matrices \Product-\ColN}{}
where $g$ is the \ProductType non\Hyph singular matrix.
A \ColWS $v$ is called
{\bf eigen\ColWS}
of the pair of matrices $(f,g)$ corresponding to \ProductType eigenvalue $b$,
if the following equality is true
\DrawEq{\Product-eigen\Cols(f,g)}{}
}

\AddEq{proof: eigencolumn of matrix}
{
The definition
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN}
follows from the definition
\refDefinition{eigenvalues of pair of matrices}{\Product}
and from the theorem
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\AddEq{proof: eigenrow of matrix}
{
Since
\ShowEq{bg.\Product.g-}
then the definition
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN}
follows from the definition
\refDefinition{eigenvalues of pair of matrices}{\Product}
and from the theorem
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\AddEq{theorem: representation Ao2->V}
{
\begin{ShadedTheorem}
\labelTheorem{representation Ao2->V \SideNS}
Let $f$, $g(\Basis e)$
be twin representations of $D$\Hyph algebra $A$
in $D$\Hyph module $V$
and $\Basis e$ be the basis of \SideWS $A$\Hyph vector space $V$.
Let product in $D$\Hyph module
\AoxA A
be defined according to rule
\DrawEq[pq]{product in algebra AA}{}
Then representation
\ShowEq{representation Ao2->V}
of $D$\Hyph algebra \AoxA A in $D$\Hyph module $V$
defined by the equality
\ShowEq{representation Ao2->V =}
is left \AoxA A\Hyph module.
\end{ShadedTheorem}
}

\AddEq{theorem: twin representation in vector space}
{
\begin{ShadedTheorem}
\labelTheorem{twin representation in \SideWS vector space}
\ShowEq{Let V be vector space}{}
\ShowEq{f:A->*B}fAV
An effective \OtherSideNS\Hyph side representation
\ShowEq{f:A->*B}{g(\Basis e)}AV
of $D$\Hyph algebra $A$
in \SideWS $A$\Hyph vector space $V$
depends on the basis $\Basis e$ of \SideWS $A$\Hyph vector space $V$.
The folowing diagram
\newline
\DrawEq{twin representations of algebra}{\SideNS}
is commutative for any $a$, $b\in A$.
\eqRef{(av)b=a(vb)}{\SideNS}.
\end{ShadedTheorem}
}

\DefProof{twin representation in vector space}
{
Commutativity of the diagram
\eqRef{twin representations of algebra}{\SideNS}
follows from the equality
}

\DefLabeledDefinition{twin representation in vector space}{\SideNS}
{
We call representations $f$ and $g(\Basis e)$
considered in the theorem
\RefTheorem{twin representation in \SideWS vector space}
{\bf twin representations}
of the $D$\Hyph algebra $A$.
The equality
\eqRef{(av)b=a(vb)}{\SideNS}
represents
{\bf associative law}
for twin representations.
This allows us writing of such expression without using of brackets.
}

\DefLabeledTheorem{set of similarity transformations}{\SideNS}
{
Let $V$ be \SideWS $A$\Hyph vector space of columns
and $\Basis e$ be basis of \SideWS $A$\Hyph vector space $V$.
The set of similarity transformations
\ShowEq{\SideWS map a En}a{}
of \SideWS $A$\Hyph vector space $V$
is \OtherSideNS\Hyph side effective representation
of $D$\Hyph algebra $A$
in \SideWS $A$\Hyph vector space $V$.
}

\DefProof{set of similarity transformations}
{
Consider the set of matrices
\ShowEq{\SideWS a En}
of similarity transformations
\ShowEq{\SideWS map a En}a{}
whith respecpect to the basis $\Basis e$.
Let $V^*$ be the set of coordinates of $V$\Hyph numbers
whith respecpect to the basis $\Basis e$.
According to theorems
\RefTheorem{Geometric objects form A vector space, \SideNS-cols},
\RefTheorem{Geometric objects form A vector space, \SideNS-rows},
the set $V^*$ is \SideWS $A$\Hyph vector space.
According to the theorem
\refTheorem{similarity transformation}{\SideNS-\Cols},
the map
\ShowEq{\SideWS map a En}a{}
is the endomorphism
of \SideWS $A$\Hyph vector space of columns.

\ColRowLemma{map a in A->aE in hom is homomorphism}

\ColRowProof{map a in A->aE in hom is homomorphism}

\ColRowProof{set of similarity transformations 1}
}

\AddEq{proof: set of similarity transformations 1}
{
According to the definition
\refDefinition{side representation of group}{\SideNS}
and the lemma
\refLemma{map a in A->aE in hom is homomorphism}{\SideNS-\Cols},
the map
\eqRef{a in A->aE hom \SideNS}{\Cols}
is \OtherSideNS\Hyph side representation
of $D$\Hyph algebra $A$
in \SideWS $A$\Hyph vector space $V^*$.
According to the theorem
\RefTheorem{division algebra},
the equality
\ShowEq{aEn=bEn \SideNS}
implies $a=b$.
According to the definition
\RefDefinition{effective representation of algebra},
the representation
\eqRef{a in A->aE hom \SideNS}{\Cols}
is effective.

According to theorems
\refTheorem{passive transformation and sum of endomorphisms}{\SideNS-\Cols},
\RefTheorem{passive transformation and product of endomorphisms, vector space, \SideNS-\Cols},
the representation
\eqRef{a in A->aE hom \SideNS}{\Cols}
is covariant with respect to choice of basis 
of \SideWS $A$\Hyph vector space $V$.
According to the theorem
\refTheorem{similarity transformation}{\SideNS-\Cols},
the set of maps
\ShowEq{\SideWS map a En}a{}
is \OtherSideNS\Hyph side representation
of $D$\Hyph algebra $A$
in \SideWS $A$\Hyph vector space $V$.
}

\DefLabeledLemma{map a in A->aE in hom is homomorphism}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
The map
\DrawEq{a in A->aE hom \SideNS}{\Cols}
is homomorphism of $D$\Hyph algebra $A$.
}

\AddEq{proof: map a in A->aE in hom is homomorphism}
{
{\sc Proof.}
According to the theorem
\refTheorem{homomorphism from A1 to A2, D algebra}1,
the lemma follows from equalities
\ShowEq{(a+b)aE \SideNS}
\ShowEq{(daE)v \SideNS}
\ShowEq{(ab)E \SideNS-\Cols}
\hfill\(\odot\)
}

\DefText{passive transformation and endomorphism}
{
We consider transformation of coordinates of endomorphism
of \SideWS $A$\Hyph vector space of \ColsWS
in the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols}.
}

\DefLabeledTheorem{passive transformation and endomorphism}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
$\Basis e_1$, $\Basis e_2$ be bases in \SideWS $A$\Hyph vector space $V$.
Let $g$ be passive transformation of basis $\Basis e_1$ into basis $\Basis e_2$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}%g
Let $f$ be endomorphism of \SideWS $A$\Hyph vector space $V$.
Let
\ShowEq{Ai, i=}f
be the matrix of endomorphism $f$ with respect to the basis $\Basis e_i$.
Then
\DrawEq[fg{\SideNS}{\Cols}]{f2=a f1 a-}{g \SideNS-\Cols}
}

\AddEq[1]{remark: passive transformation and endomorphism}
{
Let
\ShowEq{Ai, i=}{#1}
be the matrix of vector $#1$ with respect to the basis $\Basis e_i$.
Then
\DrawEq[{#1}1{#1}2g{}]{v1=v2*a \SideNS-\Cols}{#1}
follows from the theorem
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\AddEq{proof: passive transformation and endomorphism}
{
{\sc Proof of the Theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols}.}
Let endomorphism $f$ maps a vector $v$ into a vector $w$
\DrawEq{w=f o v}{\SideNS-\Cols}
\ShowEq{passive transformation and endomorphism}

According to the theorem
\refTheorem{homomorphism A module}{\SideNS-cols(1)},
equalities
\DrawEq[w1v1f1]{v1=v2*a \SideNS-\Cols}{v1}
\DrawEq[w2v2f2]{v1=v2*a \SideNS-\Cols}{v2}
follow from the equality
\eqRef{w=f o v}{\SideNS-\Cols}.
The equality
\DrawEq[g]{w2=...v2 a f1 \SideNS-\Cols}g
follows from equalities
\eqRef{v1=v2*a \SideNS-\Cols}v,
\eqRef{v1=v2*a \SideNS-\Cols}{v1},
\eqRef{v1=v2*a \SideNS-\Cols}w.
Since $g$ is regular matrix,
then the equality
\DrawEq[g]{w2=...v2 a f1 a- \SideNS-\Cols}g
follows from the equality
\eqRef{w2=...v2 a f1 \SideNS-\Cols}g.
The equality
\DrawEq[g]{v2 f2=v2 a f1 a- \SideNS-\Cols}g
follows from equalities
\eqRef{v1=v2*a \SideNS-\Cols}{v2},
\eqRef{w2=...v2 a f1 a- \SideNS-\Cols}g.
The equality
\eqRef{f2=a f1 a-}{g \SideNS-\Cols}
follows from the equality
\eqRef{v2 f2=v2 a f1 a- \SideNS-\Cols}g.
\qed
}

\DefText[2]{coordinates of vector with respect to basis (1,2) cols}
{
Let
\DrawEq[{#1_i}n]{a=(a1.n col)}{#2,\SideNS-\Cols}
be matrix of coordinates of the vector $\Vector{#1}$
with respect to the basis
\ShowEq{Basis e i=1#2}
}

\DefText[2]{coordinates of vector with respect to basis (1,2) rows}
{
Let
\ShowEq{phantom a**b}
\DrawEq[{#1_i^{}{}}n]{a=(a1.n row)}{}
\ShowEq{phantom a**b}
be matrix of coordinates of the vector $\Vector{#1}$
with respect to the basis
\ShowEq{Basis e i=1#2}
}

\AddEq[2]{convention: passive transformation maps the basis 1->2}
{%
Let passive transformation $g\in #1$ map the basis \eV[1]
into the basis \eV[2]
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{12 #2}
}

\DefLabeledTheorem{passive transformation of vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
\ShowConvention{passive transformation maps the basis 1->2}{G(V_*)}1
\ShowText{coordinates of vector with respect to basis (1,2) \Cols}v2
Coordinate transformations
\DrawEq[v1v2g{}]{v1=v2*a \SideNS-\Cols}{v21g}
\DrawEq[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{12 \SideNS-\Cols}
do not depend on vector $\Vector v$ or basis $\Basis e$, but is
defined only by coordinates of vector $\Vector v$
relative to basis $\Basis e$.
}

\DefProof{passive transformation of vector space}
{
According to the theorem
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
\ShowEq{v=vi ei 12, \SideNS-\Cols                                                                }
The equality
\ShowEq{v1 cr e1=v2 cr g cr e1, \SideNS-\Cols}
follows from equalities
\eqRef{e2i=aij e1j \Product-\Cols}{12 1},
\EqRef{v=vi ei 12, \SideNS-\Cols}.
According to the theorem
\refTheorem{coordinates of vector}{\SideNS-\Cols},
the coordinate transformation
\eqRef{v1=v2*a \SideNS-\Cols}{v21g}
follows from the equality
\EqRef{v1 cr e1=v2 cr g cr e1, \SideNS-\Cols}.
Because $g$ is \ProductType nonsingular matrix,
coordinate transformation
\eqRef{v2=v1g-}{12 \SideNS-\Cols}
follows from the equality
\eqRef{v1=v2*a \SideNS-\Cols}{v21g}.
}

\DefLabeledTheorem{passive transformation and sum of endomorphisms}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
Let endomorphism $\Vector f$ of \SideWS $A$\Hyph vector space $V$ is sum of endomorphisms
$\Vector f_1$, $\Vector f_2$.
The matrix $f$ of endomorphism $\Vector f$ equal to the sum of matrices $f_1$, $f_2$ of endomorphisms
$\Vector f_1$, $\Vector f_2$
and this equality does not depend on the choice of a basis.
}

\AddEq{two endomorphisms and two bases}
{
Let $\Basis e$, $\Basis e'$ be bases of \SideWS $A$\Hyph vector space $V$
and $g$ be passive transformation of basis $\Basis e$ into basis $\Basis e'$
\ShowEq{\SideWS e'=e*a}{}
Let $f$
be the matrix of endomorphism $\Vector f$ with respect to the basis $\Basis e$.
Let $f'$
be the matrix of endomorphism $\Vector f$ with respect to the basis $\Basis e'$.
Let
\ShowEq{Ai, i=}f
be the matrix of endomorphism $\Vector f_i$ with respect to the basis $\Basis e$.
Let
\ShowEq{Ai, i=}{f'}
be the matrix of endomorphism $\Vector f_i$ with respect to the basis $\Basis e'$.
}

\DefProof{passive transformation and sum of endomorphisms}
{
\ShowEq{two endomorphisms and two bases}
According to the theorem
\refTheorem{sum of homomorphisms, A vector space}{\SideNS-\Cols},
\DrawEq[{}{}]{f=f1+f2 endo}{\SideNS-\Cols}
\DrawEq[{'}{}]{f=f1+f2 endo}{\SideNS-\Cols'}
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[{}{}]{f'=g f g- \SideNS-\Cols}f
\DrawEq[1]{f'=g f g- \SideNS-\Cols}1
\DrawEq[2]{f'=g f g- \SideNS-\Cols}2
The equality
\ShowEq{f1+f2=g.g- \SideNS-\Cols}
follows from equalities
\ShowEq{f1+f2=g.g-}
From equalities
\eqRef{f=f1+f2 endo}{\SideNS-\Cols'},
\EqRef{f1+f2=g.g- \SideNS-\Cols}
it follows that the equality
\eqRef{f=f1+f2 endo}{\SideNS-\Cols}
is covariant with respect to choice of basis 
of \SideWS $A$\Hyph vector space $V$.
}

\AddEq{theorem: passive transformation and product of endomorphisms}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation and product of endomorphisms, vector space, \SideNS-\Cols}
\ShowEq{Let V be vector space of}.
Let endomorphism $\Vector f$ of \SideWS $A$\Hyph vector space $V$
is product of endomorphisms
$\Vector f_1$, $\Vector f_2$.
The matrix $f$ of endomorphism $\Vector f$ equal
to the \ProductType product of matrices
\ShowEq{f1 f2 \SideNS}
of endomorphisms
\ShowEq{vf1 vf2 \SideNS}
and this equality does not depend on the choice of a basis.
\end{ShadedTheorem}
}

\DefLabeledDefinition{coordinates of geometric object, vector space}{\SideNS-\Cols}
{
Orbit
\ShowEq{def coordinates of geometric object, \SideNS-\Cols}
of representation $F_1$
is called
{\bf coordinate manifold of geometric object}
in \SideWS $A$\Hyph vector space $V$ of \ColN s.
For any basis
\newline
\FrameEqRef[{V1}{V2}g{}]{e2i=aij e1j \Product-\Cols}{GOeV}
\newline
corresponding point
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
of orbit defines
{\bf coordinates of geometric object}
in coordinate \SideWS $A$\Hyph vector space
relative basis \eV[V2].
}

\DefLabeledDefinition{Left and Right Eigenvalues}{\SideNS-\Cols}
{
Let $a_2$ be \nTimes matrix
which is \ProductType similar to diagonal matrix $a_1$
\ShowEq{D diagonal matrix}{a_1}n
Thus, there exist non\Hyph \ProductType singular matrix $u_2$ such that
\DrawEq{U-*A*U=D \Product-\SideNS}1
\DrawEq[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
The \ColWS
\ShowEq{ARow u2i \Cols}u2i
of the matrix $u_2$ satisfies to the equality
\DrawEq[2u]{A*Ui=Ui di \Product-\SideNS}u
The $A$\Hyph number $b(\gi i)$ is called \SideWS \ProductType {\bf eigenvalue}
and \ColWS vector
\ShowEq{ARow u2i \Cols}u2i
is called
\AddIndex{eigen\ColWS}{eigen\ColN}
for \SideWS \ProductType eigenvalue $b(\gi i)$.
}

\DefLabeledTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
{
Eigenvector
\ShowEq{ARow u2i \Cols}u2i
of the matrix $a_2$
for \SideWS \ProductType eigenvalue $b(\gi i)$
does not depend on the choice of the basis $\Basis e_2$
\ShowEq{e1i=u2i*e2 \SideNS-\Cols}
}

\AddEq{remark: Eigenvector does not depend on basis}
{
The equality
\EqRef{e1i=u2i*e2 \SideNS-\Cols}
follows from the equality
\eqRef{e2i=aij e1j \Product-\Cols}{21u2}.
However, these equalities have different meaning.
The equality
\eqRef{e2i=aij e1j \Product-\Cols}{21u2}
is representation of passive transformation.
In the equality
\EqRef{e1i=u2i*e2 \SideNS-\Cols},
we see
the expansion of the eigenvector
for given \SideWS \ProductType eigenvalue with respect to selected basis.
The goal of the proof of the theorem
\refTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
is to explain the meaning of the equality
\EqRef{e1i=u2i*e2 \SideNS-\Cols}.
}

\DefProof{Eigenvector does not depend on basis}
{
According to the theorem
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)},
we can consider the matrix $a_2$ as matrix of automorphism $a$
of \SideWS $A$\Hyph vector space with respect to the basis $\Basis e_2$.
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
the matrix $u_2$ is the matrix is the matrix of passive transformation
\DrawEq[21u2]{e2i=aij e1j \Product-\Cols}{21u2}
and the matrix $a_1$ is the matrix of automorphism $a$
of \SideWS $A$\Hyph vector space with respect to the basis $\Basis e_1$.

The coordinate matrix of the basis $\Basis e_1$ with respect to the basis $\Basis e_1$
is identity matrix $\aD En$.
Therefore, the vector
\ShowEq{ARow u2i \Cols}e1i
is
eigen\ColWS for \SideWS \ProductType eigenvalue $b(\gi i)$
\DrawEq[1e]{A*Ui=Ui di \Product-\SideNS}e
The equality
\ShowEq{U-*A*U*E=E*D \Product-\SideNS}
follows from equalities
\eqRef{U-*A*U=D \Product-\SideNS}1,
\eqRef{A*Ui=Ui di \Product-\SideNS}e.
The equality
\ShowEq{A*U*E=U*E*D \Product-\SideNS}
follows from the equality
\EqRef{U-*A*U*E=E*D \Product-\SideNS}.
The equality
\ShowEq{U*Ei=Ui \Product-\SideNS}
follows from equalities
\eqRef{A*Ui=Ui di \Product-\SideNS}u,
\EqRef{A*U*E=U*E*D \Product-\SideNS}.
The theorem follows from equalities
\eqRef{e2i=aij e1j \Product-\Cols}{21u2},
\EqRef{U*Ei=Ui \Product-\SideNS}.
}

\DefLabeledTheorem{right eigenvalue is eigenvalue}{\SideNS-\Cols}
{
Any \SideWS \ProductType eigenvalue $b(\gi i)$
is \ProductType eigenvalue.
Eigen\ColWS $\ARow ui$
for \SideWS \ProductType eigenvalue $b(\gi i)$
is eigen\ColWS
for \ProductType eigenvalue $b(\gi i)$.
}

\DefProof{right eigenvalue is eigenvalue}
{
All entries of the row of the matrix
\DrawEq{a1-di En}{\Product-\SideNS}
are equal to zero.
Therefore, the matrix
\eqRef{a1-di En}{\Product-\SideNS}
is \ProductType singular
and \SideWS \ProductType eigenvalue $b(\gii)$
is \ProductType eigenvalue.
Since
\DrawEq{e1ij=01 \Cols}{\SideNS}
then eigenvector
\ShowEq{ARow u2i \Cols}e1i
for \SideWS \ProductType eigenvalue $b(\gii)$
is eigenvector for \ProductType eigenvalue $b(\gii)$.
The equality
\ShowEq{a1*e1=di e1 \Product-\SideNS}
follows from the definition
\refDefinition{eigenvector of matrix}{\Product-\Cols}.

From the equality
\eqRef{U-*A*U=D \Product-\SideNS}1,
it follows that we can present the matrix
\eqRef{a1-di En}{\Product-\SideNS}
as
\ShowEq{U-*A*U-di En \Product-\SideNS}
Since the matrix
\eqRef{a1-di En}{\Product-\SideNS}
is \ProductType singular,
then the matrix
\ShowEq{A-U-*di*U \Product-\SideNS}
is \ProductType singular also.
Therefore,
and \SideWS \ProductType eigenvalue $b(\gii)$
is \ProductType eigenvalue
of the pair of matrices $(a_2,u_2)$.

Equalities
\ShowEq{U-*A*U*e1=di e1 \Product-\SideNS}
\ShowEq{A*U*e1=... \Product-\SideNS}
follow from equalities
\eqRef{U-*A*U=D \Product-\SideNS}1,
\EqRef{a1*e1=di e1 \Product-\SideNS}.
From equalities
\EqRef{e1i=u2i*e2 \SideNS-\Cols},
\EqRef{A*U*e1=... \Product-\SideNS}
and from the theorem
\refTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols},
it follows that
eigen\ColWS
\ShowEq{ARow u2i \Cols}u2i
of the matrix $a_2$
for \SideWS \ProductType eigenvalue $b(\gi i)$
is
eigen\ColWS
\ShowEq{ARow u2i \Cols}u2i
of the pair of matrices $(a_2,u_2)$ corresponding to \ProductType eigenvalue $b(\gii)$.
}

\DefLabeledRemark{right eigenvalue is eigenvalue}{\SideNS-\Cols}
{
The equality
\ShowEq{di*ui=ui*di \Product-\SideNS}
follows from the theorem
\refTheorem{right eigenvalue is eigenvalue}{\SideNS-\Cols}.
The equality
\EqRef{di*ui=ui*di \Product-\SideNS}
seems unusual.
However, if we slightly change it
\ShowEq{di*ui=ui*di 1 \Product-\SideNS}
then the equality
\EqRef{di*ui=ui*di 1 \Product-\SideNS}
follows from the equality
\EqRef{e1i=u2i*e2 \SideNS-\Cols}.
}

\DefLabeledTheorem[1]{Eigenvalue a ox a, c in AAA[b]}{\SideNS-\Cols}
{
Let the \ColWS vector $v$ be
eigen\ColWS for \SideWS \ProductTypeO eigenvalue $b$
of the matrix $a$.
Let $A$\Hyph number $b$ satisfy the condition
\DrawEq[b{}{s#1}]{b in AAA[a]}{bs#1-\Cols}
Then
for any polynomial
\DrawEq{p(c) p in D}{\SideNS-\Cols}
the \ColWS vector
\ShowEq{eigenvector cv \SideNS-\Cols}
\ShowEq{c=p(b)}
is also
eigen\ColWS for \SideWS \ProductTypeO eigenvalue $b$.
}

\DefProof[2]{Eigenvalue a ox a, c in AAA[b]}
{
According to the theorem
\RefTheorem{c in Za=> p(c) in Za},
the equality
\ShowEq{as ox as o cv = ..., \SideNS-\Cols}
follows from the condition
\eqRef{b in AAA[a]}{bs#1-\Cols}.
According to the definition
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols},
the equality
\EqRef{as ox as o cv = ..., \SideNS-\Cols}
implies that
the \ColWS vector $#2$ is
eigen\ColWS for \SideWS \ProductTypeO eigenvalue $b$
of the matrix $a$.
}

\DefLabeledDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
{
$A$\Hyph number $b$ is called
\SideWS \ProductTypeO {\bf eigenvalue}
of the matrix $a$
if there exists \ColWS vector $v$ such that
\DrawEq[v]{Eigenvalue of Linear Map \SideNS-\Cols}d
The \ColWS vector $v$ is called
{\bf eigen\ColWS} for \SideWS \ProductTypeO eigenvalue $b$.
}

\DefLabeledTheorem[1]{Eigenvalue of Linear Map a ox a, 1}{\SideNS-\Cols}
{
Let entries of the matrix $a$ satisfy the equality
\DrawEq{as ox as=a1 ox a2, #1}{\SideNS-\Cols}
Then \SideWS \ProductTypeO eigenvalue $b$
is \SideWS \ProductType eigenvalue of the matrix $a_{#1}$.
}

\DefProofRef[1]{Eigenvalue of Linear Map a ox a, 1}{\SideNS-\Cols}
{
The equality
\DrawEq{as ox as o v = v a12, #1, \Cols}{1-\SideNS}
follows from the equality
\FrameEqRef{as ox as=a1 ox a2, #1}{\SideNS-\Cols}.
\newline
The equality
\ShowEq{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols}
follows from the equality
\eqRef{as ox as o v = v a12, #1, \Cols}{1-\SideNS}.
The equality
\ShowEq{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}
follows from the definition
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
of \SideWS \ProductTypeO eigenvalue
of the matrix $a$.
The equality
\ShowEq{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
follows from equalities
\EqRef{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols},
\EqRef{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}.
The theorem follows from the equality
\EqRef{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
and from the definition
\refDefinition{Left and Right Eigenvalues}{\SideNS-\Cols}
of \SideWS \ProductType eigenvalue
of the matrix $a_{#1}$.
}

\DefLabeledTheorem[1]{Eigenvalue of Linear Map a ox a, 2}{\SideNS-\Cols}
{
Let entries of the matrix $a$ satisfy the equality
\DrawEq{as ox as=a1 ox a2, #1}{\SideNS-\Cols}
Then \SideWS \ProductTypeO eigenvalue $b$
is \ProductTypeA eigenvalue of the matrix $a_{#1}$.
}

\DefProofRef[1]{Eigenvalue of Linear Map a ox a, 2}{\SideNS-\Cols}
{
The equality
\DrawEq{as ox as o v = v a12, #1, \Cols}{2-\SideNS}
follows from the equality
\FrameEqRef{as ox as=a1 ox a2, #1}{\SideNS-\Cols}.
\newline
The equality
\ShowEq{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols}
follows from the equality
\eqRef{as ox as o v = v a12, #1, \Cols}{2-\SideNS}.
The equality
\ShowEq{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}
follows from the definition
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
of \SideWS \ProductTypeO eigenvalue
of the matrix $a$.
The equality
\ShowEq{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
follows from equalities
\EqRef{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols},
\EqRef{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}.
The theorem follows from the equality
\EqRef{as ox as o v = v a12, matrix, #1 \SideNS-\Cols},
from the definition
\refDefinition{eigenvalue of matrix}{\ProductA}
of \ProductType eigenvalue
of the matrix $a_{#1}$
and from the definition
\refDefinition{eigenvector of matrix}{\ProductA-\Cols}
of corresponding eigenvector $v$.
}

\DefLabeledTheoremNote[1]{n eigenvectors}{#1}
{
Let $\Base$ be \Algebra.
Let $V$ be $\Base$\Hyph vector space.
If endomorphism has $\gik$ different
eigenvalues\,\footnotemark
\ShowEq{di 1n}bk,
then eigenvectors
\ShowEq{di 1n}vk{}
which correspond to different eigenvalues
are linearly independent.
}
{
See also the theorem on the page
\citeBib{Kurosh: High Algebra}\Hyph 203.
}

\AddEq{remark: n eigenvectors}
{
However, the theorem
\refTheorem{n eigenvectors}{algebra}
is not correct.
We will consider the proof separately
for left and right $A$\Hyph vector spaces.
}

\DefProof{n eigenvectors}
{
We will prove the theorem by induction with respect to $\gik$.

Since eigenvector is non\Hyph zero, the theorem is true for $\gik=\gi 1$.

\begin{Statement}
\labelStatement{theorem is true for k=m-1 \SideNS}
Let the theorem be true for $\gik=\gim-\gi 1$.
\hfill\(\odot\)
\end{Statement}

\begin{sloppypar}
According to theorems
\ShowEq{ref 1 for n eigenvectors}
we can assume that
\ShowEq{e2=e1}
Let
\ShowEq{di 1n+1}bm{}
be different eigenvalues and
\ShowEq{di 1n+1}vm{}
corresponding eigenvectors
\ShowEq{fovi=di vi \SideNS}
\ShowEq{di ne dj}
Let the statement
\RefStatement{ai vi=0 \SideNS}
be true.
\end{sloppypar}

\begin{Statement}
\labelStatement{ai vi=0 \SideNS}
There exists linear dependence
\ShowEq{ai vi=0 \SideNS}
where
\ShowEq{a1 ne 0}
\hfill\(\odot\)
\end{Statement}

The equality
\ShowEq{ai f vi=0 \SideNS}
follows from the equality
\EqRef{ai vi=0 \SideNS}
and the theorem
\ShowEq{ref 2 for n eigenvectors}
The equality
\ShowEq{ai di vi=0 \SideNS}
follows from equalities
\EqRef{fovi=di vi \SideNS},
\EqRef{ai f vi=0 \SideNS}.
Since the product is non\Hyph commutative,
we cannot reduce expression
\EqRef{ai di vi=0 \SideNS}
to linear dependence.
}

\AddEq{remark: Eigenvalue and conjugate class}
{
According to theorems
\refTheorem{Eigenvalue and conjugate class}{\SideNS-\Cols},
\refTheorem{Coefficient comutes with matrix}{\SideNS-\Cols},
the set of eigen\ColsWS
for given \SideWS \ProductType eigenvalue
is not $A$\Hyph vector space.
}

\DefLabeledTheorem{Eigenvalue and conjugate class}{\SideNS-\Cols}
{
Let $A$\Hyph number $b$ be \SideWS \ProductType eigenvalue of the matrix
$a_2$.\refFootnote{Eigenvalue and conjugate class}{\Product}
Then any $A$\Hyph number which $A$\Hyph conjugated with $A$\Hyph number $b$,
is \SideWS \ProductType eigenvalue of the matrix $a_2$.
}

\DefLabeledFootnote{Eigenvalue and conjugate class}{\Product}
{
See the similar statement and proof on the page
\citeBib{Cohn: Skew Fields}\Hyph 375.
}

\DefProof{Eigenvalue and conjugate class}
{
Let $v$ be
eigen\ColWS for \SideWS \ProductType eigenvalue $b$.
Let $c\ne 0$ be $A$\Hyph number.
The theorem follows from the equality
\ShowEq{conjugate eigenvalue \SideNS-\Cols}
}

\DefLabeledTheorem[2]{Coefficient comutes with matrix}{\SideNS-\Cols}
{
Let $v$ be eigen\ColWS for \SideWS \ProductType eigenvalue $b$.
The vector $#1#2$
is eigen\ColWS for \SideWS \ProductType eigenvalue $b$
iff
$A$\Hyph number $c$ commutes with all entries of the matrix $a_2$.
}

\DefProof[2]{Coefficient comutes with matrix}
{
The vector $#1#2$
is eigen\ColWS for \SideWS \ProductType eigenvalue $b$
iff
the following equality is true
\ShowEq{Coefficient comutes with matrix \SideNS-\Cols}
The equality
\EqRef{Coefficient comutes with matrix \SideNS-\Cols}
holds iff
$A$\Hyph number $c$ commutes with all entries of the matrix $a_2$.
}

\DefLabeledDefinition{geometric object, vector space}{\SideNS-\Cols}
{
Let us say the coordinates $w_1$ of vector $\Vector w$
with respect to the basis \eV[W1] are given.
The set of vectors
\DrawEq[w2{w_2}{W2}]{geometric object representative, \SideNS-\Cols}{w=we}
is called
{\bf geometric object}
defined in \SideWS $A$\Hyph vector space $V$ of \ColN s.
For any basis \eV[W2][,]
corresponding point
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
of coordinate manifold defines the vector
\DrawEq[w2{w_2}{W2}]{geometric object representative, \SideNS-\Cols}{w=we 1}
which is called
{\bf representative of geometric object}
in \SideWS $A$\Hyph vector space $V$ in basis \eV[V2][.]
}

\AddEq{remark: geometric object, vector space}
{
Since a geometric object is an orbit of representation, we see that
according to theorem
\RefTheorem{proper definition of orbit}
the definition of the geometric object is a proper definition.

We also say that $\Vector w$ is
a \AddIndex{geometric object of type $F$}{type of geometric object}.

Definitions
\refDefinition{coordinates of geometric object, vector space}{\SideNS-cols},
\refDefinition{coordinates of geometric object, vector space}{\SideNS-rows}
introduce a geometric object in coordinate space.
We assume in definitions
\refDefinition{geometric object, vector space}{\SideNS-cols},
\refDefinition{geometric object, vector space}{\SideNS-rows}
that we selected
a basis of vector space $W$.
This allows using a representative of the geometric object
instead of its coordinates.
}

\DefText{Geometric Object of Vector Space}
{
\begin{sloppypar}
Let $V$, $W$ be \SideWS $A$\Hyph vector spaces of \ColN s 
and $G(V_*)$ be symmetry group
of \SideWS $A$\Hyph vector space $V$.
Homomorphism
\DrawEq[F{G(V_*)}{GL(W_*)}{}]{f: A->B}{FG \SideNS-\Cols}
maps passive transformation $g\in G(V_*)$
\DrawEq[{V1}{V2}g{}]{e2i=aij e1j \Product-\Cols}{GOeV}
of \SideWS $A$\Hyph vector spaces $V$
into passive transformation
\ShowEq{Fg in GL}
\DrawEq[{W1}{W2}{F(g)}{}]{e2i=aij e1j \Product-\Cols}{GOeW}
of \SideWS $A$\Hyph vector spaces $W$.
\end{sloppypar}

Then coordinate transformation in
\SideWS $A$\Hyph vector space $W$ gets form
\DrawEq{coordinate transformation, vector space W, \SideNS-\Cols}1
Therefore, the map
\DrawEq{F1(g)=F(g)**-\Product}{\SideNS}
is \OtherSideNS\Hyph side representation
\ShowEq{f:A->*B}{F_1}{G(V_*)}{W_*}
of group $G(V_*)$ in the set $W_*$.
}

\DefProof{passive transformation and product of endomorphisms}
{
\ShowEq{two endomorphisms and two bases}
According to the theorem
\RefTheorem{product of homomorphisms, \SideWS A vector space, \ColN},
\DrawEq[{}{}]{f=f1*f2 endo \SideNS-\Cols}{\Product}
\DrawEq[{'}{}]{f=f1*f2 endo \SideNS-\Cols}{\Product'}
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[{}{}]{f'=g f g- \SideNS-\Cols}{f*}
\DrawEq[1]{f'=g f g- \SideNS-\Cols}{1*}
\DrawEq[2]{f'=g f g- \SideNS-\Cols}{2*}
The equality
\ShowEq{f1*f2=g.g- \SideNS-\Cols}
follows from equalities
\ShowEq{f1*f2=g.g-}
From equalities
\eqRef{f=f1*f2 endo \SideNS-\Cols}{\Product'},
\EqRef{f1*f2=g.g- \SideNS-\Cols}
it follows that the equality
\eqRef{f=f1*f2 endo \SideNS-\Cols}{\Product}
is covariant with respect to choice of basis 
of \SideWS $A$\Hyph vector space $V$.
}

\AddEq{theorem: finite dimension->representation is free}
{
\begin{ShadedTheorem}
\labelTheorem{finite dimension->representation is free, \SideNS}
If \SideWS $A$\Hyph vector space $V$
has finite dimension,
then corresponding representation is free.
\end{ShadedTheorem}
}

\DefProof{finite dimension->representation is free}
{
The theorem follows from the definition
\RefDefinition{free representation of algebra}
and from theorems
\refTheorem{av=bv=>a=b}{\SideNS-cols},
\refTheorem{av=bv=>a=b}{\SideNS-rows}.
}

\AddEq[1]{Let V be vector space}
{
Let $V$ be a \SideWS $A$\Hyph vector space#1
}

\AddEq[1]{Let V be vector space of}
{
Let $V$ be a \SideWS $A$\Hyph vector space of \ColN s#1
}

\AddEq{Let V be vector space of and}
{
Let $V$ be a \SideWS $A$\Hyph vector space of \ColsWS and
}

\AddEq{Let V be vector space of and basis}
{
\ShowEq{Let V be vector space of and}
$\Basis e$ be basis of \SideWS $A$\Hyph vector space $V$.
}

\AddEq{Let V be vector space and basis}
{
\ShowEq{Let V be vector space}{}
and $\Basis e$ be basis of \SideWS $A$\Hyph vector space $V$.
}

\AddEq{remark: automorphism of vector space, group}
{
\ShowEq{Let V be vector space of}.
We proved in the theorem
\refTheorem{automorphism of vector space}{\Product-\Cols}
that, if we select a basis
of \SideWS $A$\Hyph vector space $V$,
then we can identify any automorphism $\Vector f$
of \SideWS $A$\Hyph vector space $V$
with \ProductType nonsingular matrix $f$.
Corresponding transformation of coordinates of vector
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{}
is called
\AddIndex{linear transformation}{linear transformation}.
}

\DefLabeledDefinition{Symmetry Group}{\SideNS-\Cols}
{
Normal subgroup $G(V)$ of the group $GL(V)$ such that subgroup $G(V)$ generates
automorphisms which hold properties of the selected structure
is called
{\bf symmetry group}.

Without loss of generality we identify element $g$ of group $G(V)$
with corresponding transformation of representation
and write its action on vector $v\in V$ as
$v\ProductVal g$.
}

\DefText{definition: linear G* representation}
{
The \OtherSideNS\Hyph side representation
of group $G$ in \SideWS $A$\Hyph vector space is called
\AddIndex{linear $G$\Hyph representation}{linear G* representation}.
}

\DefText{linear G* representation}
{
Let us define an additional structure on \SideWS $A$\Hyph vector space $V$.
Then not every automorphism keeps properties of the selected structure.
For imstance, if we introduce norm in
\SideWS $A$\Hyph vector space $V$,
then we are interested in automorphisms which preserve the norm of the vector.
}

\DefLabeledDefinition{active G-representation}{\SideNS}
{
The \OtherSideNS\Hyph side representation
of group $G(V)$ in the set of bases of \SideWS $A$\Hyph vector space $V$ is called
\AddIndex{active \SideNS\Hyph side $G$\Hyph representation}
{active representation, vector space}.
}

\DefText{active G-representation}
{
If the basis \eV is given, then
we can identify the automorphism
of \SideWS $A$\Hyph vector space $V$
and its coordinates with respect to the basis \eV[][.]
The set $G(V_*)$ of coordinates of automorphisms
with respect to the basis \eV is group
isomorphic to the group $G(V)$.

Not every two bases can be mapped by a transformation
from the symmetry group
because not every nonsingular linear transformation belongs to
the representation of group $G(V)$.
Therefore, we can represent
the set of bases as a union of orbits of group $G(V)$.
In particular, if the basis $\eV\in G(V)$,
then the group $G(V)$ is orbit of the basis \eV[][.]
}

\DefLabeledTheorem{representation on basis manifold, vector space}{\SideNS}
{
Active \OtherSideNS\Hyph side $G(V)$\Hyph representation on basis manifold
is single transitive representation.
}

\DefProof{representation on basis manifold, vector space}
{
The theorem follows from the theorem
\refTheorem{active representation is single transitive}{\SideNS-cols}
and the definition
\refDefinition{basis manifold of vector space}{\SideNS-cols},
as well the theorem follows from the theorem
\refTheorem{active representation is single transitive}{\SideNS-rows}
and the definition
\refDefinition{basis manifold of vector space}{\SideNS-rows}.
}

\DefLabeledDefinition{basis manifold of vector space}{\SideNS-\Cols}
{
We call orbit
\ShowEq{basis manifold of vector space, \SideNS-\Cols}
of the selected basis $\Basis e$
the {\bf basis manifold}
of \SideWS $A$\Hyph vector space $V$ of \ColN s.
}

\DefLabeledTheorem{active transformations, vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Automorphisms of \SideWS $A$\Hyph vector space of \ColsWS form
a \OtherSideNS\Hyph side linear
effective \Group nA\Hyph representation.
}

\DefProof{active transformations, vector space}
{
Let $a$, $b$ be matrices of automorphisms $\Vector a$ and $\Vector b$
with respect to basis $\Basis e$.
According to the theorem
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)},
coordinate transformation has following form
\DrawEq[{v'}{}v{}a{}]{v1=v2*a \SideNS-\Cols}{v'}
\DrawEq[{v''}{}{v'}{}b{}]{v1=v2*a \SideNS-\Cols}{v''}
The equality
\ShowEq{a*b, \SideNS-\Cols}
\DrawEq[{v''}{}v{}{\TheProduct}{}]{v1=v2*a \SideNS-\Cols}{}
\begin{sloppypar}
\noindent
follows from equalities
\eqRef{v1=v2*a \SideNS-\Cols}{v'},
\eqRef{v1=v2*a \SideNS-\Cols}{v''}.
According to the theorem
\RefTheorem{product of homomorphisms, \SideWS A vector space, \ColN},
the product of automorphisms $\Vector a$ and $\Vector b$
has matrix \TheProduct.
Therefore, automorphisms of \SideWS $A$\Hyph vector space of \ColsWS form
a \OtherSideNS\Hyph side linear
\Group nA\Hyph representation.
\end{sloppypar}

It remains to  prove that
the kernel of inefficiency consists only of identity.
Identity transformation
satisfies to equation
\ShowEq{active transformations, vector space, 2, \SideNS-\Cols}
Choosing values of coordinates as
\ShowEq{ai=delta ik, \Cols}
where we selected $\gik$ we get
\ShowEq{identity transformation, vector space, \SideNS-\Cols}
From \EqRef{identity transformation, vector space, \SideNS-\Cols} it follows
\ShowEq{identity transformation, vector space, 1, \Cols}
Since $\gik$ is arbitrary, we get the conclusion $a=\delta$.
}

\DefLabeledTheorem{active transformations, basis, vector space}{\SideNS-\Cols}
{
Automorphism $a$ acting on each vector of basis of
\SideWS $A$\Hyph vector space of \ColN s
maps a basis into another basis.
}

\DefProof{active transformations, basis, vector space}
{
Let $\Basis e$ be basis of \SideWS $A$\Hyph vector space $V$ of \ColN s.
According to theorem
\refTheorem{automorphism of vector space}{\Product-\Cols},
vector
\ShowEq{vector of basis \Cols}e
maps into a vector
\ShowEq{vector of basis \Cols}{e'}
\DrawEq{automorphism, vector space, 1, \SideNS-\Cols}1
\begin{sloppypar}
\noindent
Let vectors
\ShowEq{vector of basis \Cols}{e'}
be linearly dependent.
Then $\lambda\ne 0$
in the equality
\ShowEq{automorphism, vector space, 2, \SideNS-\Cols}
\end{sloppypar}
\noindent
From equations \eqRef{automorphism, vector space, 1, \SideNS-\Cols}1
and \EqRef{automorphism, vector space, 2, \SideNS-\Cols} it follows that
\ShowEq{automorphism, vector space, 3, \SideNS-\Cols}
and $\lambda\ne 0$. This
contradicts to the statement that vectors
\ShowEq{vector of basis \Cols}e
are linearly independent.
Therefore vectors
\ShowEq{vector of basis \Cols}{e'}
are linearly independent
and form basis.
}

\DefText{extend linear representation to set of bases 1}
{
Thus we can extend
a \OtherSideNS\Hyph side linear $GL(V_*)$\Hyph representation
in \SideWS $A$\Hyph vector space $V_*$
to the set of bases
of \SideWS $A$\Hyph vector space $V$.
}

\DefText{extend linear representation to set of bases 2}
{
Transformation of this \OtherSideNS-side representation
on the set of bases
of \SideWS $A$\Hyph vector space $V$ is called
\AddIndex{active transformation}{active transformation, vector space}
because the homomorphism of the \SideWS $A$\Hyph vector space induced this transformation
(\BlueText{See also definition in the section
\citeBib{Korn}\Hyph 14.1\Hyph 3
as well the definition on the page
\citeBib{Rashevsky}\Hyph 214}).

\ePrints{2022.01.05,2022.11.26}%
\ifx\Semafor\ValueOn%
\FrameCiteBib{Korn}

\FrameCiteBib{Rashevsky}
\fi
}

\DefText{extend linear representation to set of bases 3}
{
\begin{sloppypar}
According to definition we write the action
of the transformation $a\in GL(V_*)$ on the basis $\Basis e$ as
\ShowEq{active transformation, vector space, \SideNS-\Cols}.
Consider the equality
\DrawEq{active transformation ae x=a ex, \SideNS-\Cols}1
The expression
\ShowEq{active transformation, vector space, \SideNS-\Cols}{}
on the left side of the equality
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
is image of basis \eV with respect to active transformation $a$.
The expression
\ShowEq{active transformation ae x=a ex 1, \SideNS-\Cols}
on the right side of the equality
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
is expansion of vector $\Vector v$ with respect to basis \eV[][.]
Therefore,
the expression on the right side of the equality
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
is image of vector $\Vector v$ with respect to endomorphism $a$
and the expression on the left side of the equality
\newline
\FrameEqRef{active transformation ae x=a ex, \SideNS-\Cols}1
\newline
is expansion of image of vector $\Vector v$
with respect to image of basis \eV[][.]
Therefore, from the equality
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
it follows that endomorphism $a$ of \SideWS $A$\Hyph vector space and
corresponding active transformation $a$ act synchronously
and coordinates $a\circ \Vector v$ of image of the vector $\Vector v$ with respect to
the image
\ShowEq{active transformation, vector space, \SideNS-\Cols}{}
of the basis \eV
are the same as coordinates of the vector $\Vector v$ with respect to the basis $\Basis e$.
\end{sloppypar}
}

\DefLabeledTheorem{active representation is single transitive}{\SideNS-\Cols}
{
Active \OtherSideNS\Hyph side \Group nA\Hyph representation on the set of bases
is single transitive representation.
The set of bases identified with tragectory
\ShowEq{basis manifold of V, \SideNS-\Cols}e{\Group nA}{}
of active \OtherSideNS\Hyph side \Group nA\Hyph representation
is called
the {\bf basis manifold}
of \SideWS $A$\Hyph vector space $V$.
}

\DefLabeledTheorem{exists representation, commuting with active}{\SideNS-\Cols}
{
On the basis manifold
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
of \SideWS $A$\Hyph vector space of \ColN s,
there exists single transitive
\SideNS\Hyph side $G(V)$\Hyph representation, commuting with active.
}

\AddEq{proof: exists representation, commuting with active}
{
%\begin{sloppypar}
\begin{proof}
Theorem
\refTheorem{representation on basis manifold, vector space}{\SideNS}
means that the basis manifold
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
is a homogenous space of group $G$.
The theorem follows from the theorem
\RefTheorem{two representations of group}.
\end{proof}
%\end{sloppypar}
}

\AddEq{remark: passive transformation, vector space}
{
\ePrints{2022.11.26,MObject}%
\ifx\Semafor\ValueOn%
Transformation of
\else
As we see from remark
\RefRemark{one representation of group}
transformation of
\fi
\SideNS\Hyph side $G(V)$\Hyph representation is different from an active transformation
and cannot be reduced to
transformation of space $V$.
}

\DefLabeledDefinition{passive transformation, vector space}{\SideNS-\Cols}
{
A transformation of
\SideNS\Hyph side $G(V)$\Hyph representation is called
{\bf passive transformation}
of basis manifold
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
of \SideWS $A$\Hyph vector space of \ColN s,
and the \SideNS\Hyph side $G(V)$\Hyph representation is called
{\bf passive \SideNS\Hyph side $G(V)$\Hyph representation}.
According to the definition
we write the passive transformation of basis $\Basis e$
defined by element $a\in G(V)$ as
\ShowEq{passive transformation symbol, \SideNS-\Cols}
}

\AddEq[1]{table: Passive and Active Representations}
{
\ShowEq{def #1}\SideWS $A$\Hyph vector space&\ShowEq{def #1}\ShowEq{\DefRow}\Group nA&
\ShowEq{def #1}\OtherSideNS-side&\ShowEq{def #1}\SideNS-side\\
of rows&&&\\[10pt]
\hline
\ShowEq{def #1}\SideWS $A$\Hyph vector space&\ShowEq{def #1}\ShowEq{\DefCol}\Group nA&
\ShowEq{def #1}\OtherSideNS-side&\ShowEq{def #1}\SideNS-side\\
of columns&&&\\
\hline
}

\DefLabeledTheorem{principle of covariance}{\SideNS}%-\Cols}
{
{\bf(Principle of covariance).}
Representative of geometric object does not depend on selection
of basis \eV[V2][.]
}

\DefProof{principle of covariance}
{
To define representative of geometric object,
we need to select basis $\Basis e_V$,
basis $\Basis e_W$
and coordinates of geometric object $w^\alpha$.
Corresponding representative of geometric object
has form
\DrawEq[w{}wW]{geometric object representative, \SideNS-\Cols}{}
Suppose we map basis $\Basis e_V$
to basis $\Basis e'_V$
by passive transformation
\DrawEq[V]{passive transformation e->e', \SideNS-\Cols}{}
According construction this generates passive transformation
\newline
\FrameEqRef[{W1}{W2}{F(g)}{}]{e2i=aij e1j \Product-\Cols}{GOeW}
\newline
and coordinate transformation
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
Corresponding representative of geometric object has form
\ShowEq{invariance principle 3, \SideNS-\Cols}
Therefore representative of geometric object
is invariant relative selection of basis.
}

\AddEq{definition: sum of geometric objects}
{
\begin{ShadedDefinition}
\labelDefinition{sum of geometric objects, \SideNS-\Cols}
\ShowEq{Let V be vector space of and}
\ShowEq{sum of geometric objects, 1}
be geometric objects of the same type
defined in \SideWS $A$\Hyph vector space $V$.
Geometric object
\ShowEq{sum of geometric objects, 2}
is called \AddIndex{sum
\ShowEq{sum of geometric objects, 3}
of geometric objects}{sum of geometric objects}
$\Vector w_1$ and $\Vector w_2$.
\end{ShadedDefinition}
}

\AddEq{definition: product of geometric object and constant}
{
\begin{ShadedDefinition}
\labelDefinition{product of geometric object and constant, \SideNS-\Cols}
\ShowEq{Let V be vector space of and}
\DrawEq[w1{w_1}W]{geometric object representative, \SideNS-\Cols}{}
be geometric object
defined in \SideWS $A$\Hyph vector space $V$.
Geometric object
\ShowEq{product of geometric object and constant, 2, \SideNS}
is called \AddIndex{product
\ShowEq{product of geometric object and constant, 3, \SideNS}
of geometric object $\Vector w_1$ and constant $k\in A$}
{product of geometric object and constant}.
\end{ShadedDefinition}
}

\AddEq{theorem: Geometric objects form A vector space}
{
\begin{ShadedTheorem}
\labelTheorem{Geometric objects form A vector space, \SideNS-\Cols}
Geometric objects of type $F$
defined in \SideWS $A$\Hyph vector space $V$ of \ColN s
form \SideWS $A$\Hyph vector space of \ColN s.
\end{ShadedTheorem}
}

\DefProof{Geometric objects form A vector space}
{
The statement of theorems
\RefTheorem{Geometric objects form A vector space, \SideNS-cols},
\RefTheorem{Geometric objects form A vector space, \SideNS-rows}
follows from immediate verification
of the properties of vector space.
}

\DefLabeledTheorem{coordinate matrix of basis and passive transformation}{\SideNS-\Cols}
{
The coordinate matrix of basis $\Basis e'$ relative basis $\Basis e$
of \SideWS $A$\Hyph vector space $V$ of \ColsWS
is identical with the matrix of passive transformation mapping
basis $\Basis e$ to basis $\Basis e'$.
}

\DefProof{coordinate matrix of basis and passive transformation}
{
According to the theorem
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
the coordinate matrix of basis $\Basis e'$ relative basis $\Basis e$
consist from \Rows which are coordinate matrices of vectors
$\aD{\Vector e'}i$ relative the basis $\Basis e$. Therefore,
\ShowEq{coordinate matrix of basis and passive transformation, \SideNS-\Cols}{e'}
At the same time the passive transformation $a$ mapping one basis to another has a form
\ShowEq{coordinate matrix of basis and passive transformation, \SideNS-\Cols}a
According to the theorem
\refTheorem{coordinates of vector}{\SideNS-\Cols},
\ShowEq{coordinate matrix of basis and passive transformation, \Cols}
for any $\gii$. This proves the theorem.
}

\DefLabeledSloppyRemark{identify basis and matrix of coordinates}{\SideNS-\Cols}
{
According to theorems
\RefTheorem{single transitive representation of group},
\refTheorem{coordinate matrix of basis and passive transformation}{\SideNS-\Cols},
we can identify a basis $\Basis e'$ 
of the basis manifold
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
of \SideWS $A$\Hyph vector space of columns
and the matrix $g$ of coordinates of the basis $\Basis e'$
with respect to the basis $\Basis e$
\DrawEq[{}{}]{passive transformation e->e', \SideNS-\Cols}1
Since $\Basis e'=\Basis e$, then the equality
\eqRef{passive transformation e->e', \SideNS-\Cols}1
gets form
\ShowEq{passive transformation e->e, \SideNS-\Cols}
Based on the equality
\EqRef{passive transformation e->e, \SideNS-\Cols},
we will use notation
\ShowEq{basis manifold of V, \SideNS-\Cols}{\aD En}G{}
for basis manifold
\ShowEq{basis manifold of V, \SideNS-\Cols}eG.
}

\DefText{Passive Transformation}
{
An active transformation changes bases and vectors uniformly
and coordinates of vector relative basis do not change.
A passive transformation changes only the basis and it leads to transformation
of coordinates of vector relative to basis.
}

\DefText{transformation of coordinates of vector}
{
We consider transformation of coordinates of vector in the theorem
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\AddEq{remark: active representation is single transitive}
{
To prove theorems
\refTheorem{active representation is single transitive}{\SideNS-cols},
\refTheorem{active representation is single transitive}{\SideNS-rows},
it is sufficient to show that
at least one transformation of \OtherSideNS\Hyph side representation is defined for any two bases
and this transformation is unique.
}

\AddEq{left active representation is single transitive}
{
coordinate matrix of original basis over matrix of automorphism
\ShowEq{left e'=e*a}{}
}

\AddEq{right active representation is single transitive}
{
matrix of automorphism over coordinate matrix of original basis
\ShowEq{right e'=e*a}{}
}

\DefProofSloppy{active representation is single transitive}
{
Homomorphism $a$ operating on basis $\Basis e$ has form
\DrawEq{automorphism, vector space, 1, \SideNS-\Cols}{}
where
\ShowEq{vector of basis \Cols}{e'}
is coordinate matrix of vector
\ShowEq{vector of basis \Cols}{\Vector e'}
relative basis $\Basis h$ and
\ShowEq{vector of basis \Cols}e
is coordinate matrix of vector
\ShowEq{vector of basis \Cols}{\Vector e}
relative basis $\Basis h$.
Therefore, coordinate matrix of image of basis equal to
\ProductType product of
\ShowEq{\SideWS active representation is single transitive}
According to the theorem
\refTheorem{coordinate matrix of basis}{\Product-\Cols},
matrices $g$ and $e$ are nonsingular. Therefore, matrix
\ShowEq{homomorphism on A basis, \SideNS-\Cols}
is the matrix of automorphism mapping basis $\Basis e$
to basis $\Basis e'$.

Suppose elements $g_1$, $g_2$ of group $G$ and basis $\Basis e$ satisfy equation
\ShowEq{two transformations on basis manifold, \SideNS-\Cols}
According to the theorems
\refTheorem{coordinate matrix of basis}{\Product-\Cols}
and
\RefTheorem{two cr-products equal},
we get $g_1=g_2$.
This proves statement of theorem.
}

\DefLabeledTheorem{representation of homomorphism relative different bases}{\SideNS-\Cols}
{
Let
\ShowEq{Bases e12}V{}
be bases of \SideWS $A$\Hyph vector space $V$ of columns.
Let
\ShowEq{Bases e12}W{}
be bases of \SideWS $A$\Hyph vector space $W$ of columns.
Let $a_1$ be matrix of homomorphism
\DrawEq{A:V->W}{different bases \SideNS-\Cols}
relative to bases
\ShowEq{Bases eVW}VW1{}
and $a_2$ be matrix of homomorphism
\eqRef{A:V->W}{different bases \SideNS-\Cols}
relative to bases
\ShowEq{Bases eVW}VW2.
Suppose the basis $\Basis e_{V1}$ has coordinate matrix $b$ relative
the basis $\Basis e_{V2}$
\DrawEq[Vb]{coordinate matrix, f, g, \SideNS-\Cols}{}
and $\Basis e_{W1}$ has coordinate matrix $c$ relative
the basis $\Basis e_{W2}$
\DrawEq[Wc]{coordinate matrix, f, g, \SideNS-\Cols}C
Then there is relationship between matrices $a_1$ and $a_2$
\DrawEq[c]{representation of homomorphism relative different bases, \SideNS-\Cols}{}
}

\DefProof{representation of homomorphism relative different bases}
{
Vector $\Vector v\in V$ has expansion
\ShowEq{expansion of vector v, \SideNS-\Cols}
relative to bases
\ShowEq{Bases e12}V.
Since $a$ is homomorphism, we can write it as
\ShowEq{representation of homomorphism relative different bases, 1, \SideNS-\Cols}
relative to bases
\ShowEq{Bases eVW}VW1{}
and as
\ShowEq{representation of homomorphism relative different bases, 2, \SideNS-\Cols}
relative to bases
\ShowEq{Bases eVW}VW2.
According to the theorem
\refTheorem{coordinate matrix of basis}{\Product-\Cols},
matrix $c$ has \ProductType inverse and from equation
\eqRef{coordinate matrix, f, g, \SideNS-\Cols}C it follows that
\ShowEq{coordinate matrix, W2, W1, \SideNS-\Cols}
The equality
\ShowEq{representation of homomorphism relative different bases, 3, \SideNS-\Cols}
\begin{sloppypar}
\noindent
follows from equalities
\EqRef{representation of homomorphism relative different bases, 2, \SideNS-\Cols},
\EqRef{coordinate matrix, W2, W1, \SideNS-\Cols}.
From the theorem
\refTheorem{coordinates of vector}{\SideNS-\Cols}
and comparison of equations
\EqRef{representation of homomorphism relative different bases, 1, \SideNS-\Cols}
and \EqRef{representation of homomorphism relative different bases, 3, \SideNS-\Cols} it follows that
\ShowEq{representation of homomorphism relative different bases, 4, \SideNS-\Cols}
Since vector $a$ is arbitrary vector,
the statement of theorem follows
from the theorem
\refTheorem{active transformations, vector space}{\SideNS-\Cols}
and equation
\EqRef{representation of homomorphism relative different bases, 4, \SideNS-\Cols}.
\end{sloppypar}
}

\DefLabeledTheorem{coordinate transformations form representation, vector space}{\SideNS-\Cols}
{
Coordinate transformations
\newline
\FrameEqRef[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{12 \SideNS-\Cols}
\newline
form effective linear
\OtherSideNS\Hyph side contravariant $G$\Hyph representation which is called
{\bf coordinate representation in \SideWS $A$\Hyph vector space}
of \ColN s.
}

\DefProof{coordinate transformations form representation, vector space}
{
\ShowText{passive representation of left vector space}
According to the definition
\RefDefinition{Left side contravariant representation},
coordinate transformations
form linear right\Hyph side contravariant $G$\Hyph representation.
Suppose coordinate transformation does not change vectors $\delta_k$.
Then unit of group $G$ corresponds to it because representation
is single transitive. Therefore,
coordinate representation is effective.
}

\AddEq{theorem: representation of automorphism relative different bases}
{
\begin{ShadedTheorem}
\labelTheorem{representation of automorphism relative different bases, \SideNS-\Cols}
Let $\Vector a$ be automorphism
of left $A$\Hyph vector space $V$ of columns.
Let $a_1$ be matrix of this automorphism defined
relative to basis $\Basis e_1$ and
$a_2$ be matrix of the same automorphism defined
relative to basis $\Basis e_2$.%g
Suppose the basis $\Basis e_1$ has coordinate matrix $b$ relative
the basis $\Basis e_2$
\DrawEq[{}b]{coordinate matrix, f, g, \SideNS-\Cols}{}
Then there is relationship between matrices $a_1$ and $a_2$
\DrawEq[c]{representation of homomorphism relative different bases, \SideNS-\Cols}{}
\end{ShadedTheorem}
}

\DefProof{representation of automorphism relative different bases}
{
Statement follows from theorem
\refTheorem{representation of homomorphism relative different bases}{\SideNS-\Cols},
because in this case $c=b$.
}

\DefLabeledTheorem[4]{basis of vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
\ShowEq{Let be basis of vector space}{#2}iIA{#1}V{#2}{\Cols}-
\ShowEq{Let be basis of vector space}{#4}jJA{#3}V{#4}{\Cols}-
If $|I|$ and $|J|$ are finite numbers then
\ShowEq{|I|=|J|}
}

\DefProof{basis of vector space}
{
Let
\ShowEq{|I|=m}Im{}
and
\ShowEq{|I|=m}Jn.
Let
\DrawEq{m<n gi}{1 \SideNS-\Cols}
Because $\Basis e_1$ is a basis, any vector
\ShowEq{basis e2 of V \Cols}
has expansion
\ShowEq{basis e2 relative e1 \SideNS-\Cols}
Because $\Basis e_2$ is a basis,
\DrawEq{basis e2 of V lambda}{\SideNS-\Cols}
should follow from
\ShowEq{basis e2 relative e1, lambda, \SideNS-\Cols}
Because $\Basis e_1$ is a basis we get
\ShowEq{basis e2 relative e1, lambda=0, \SideNS-\Cols}
According to
\eqRef{m<n gi}{1 \SideNS-\Cols},
\ShowEq{Rank a<m \Product}
and system of linear equations
\EqRef{basis e2 relative e1, lambda=0, \SideNS-\Cols}
has more variables then equations. According to the theorem
\RefTheorem{star rows system of linear equations, solution},
we get the statement $\lambda\ne 0$ which contradicts
statement \eqRef{basis e2 of V lambda}{\SideNS-\Cols}. 
Therefore, statement
\DrawEq{m<n gi}-
is not valid.
In the same manner we can prove that the statement
\ShowEq{n<m gi}
is not valid.
This completes the proof of the theorem.
}

\AddEq{definition: linearly independent, AoxA module}
{
\begin{ShadedDefinition}
\labelDefinition{linearly independent, AoxA module \Cols}
Let $V$ be left \AoxA A\Hyph module of \ColN s.
The set of vectors
\ShowEq{Vector A \Cols}
of left \AoxA A\Hyph module $V$ is
{\bf linearly independent}
if
\ShowEq{AoxA linearly independent 1 \Cols},
follows from the equaility
\ShowEq{AoxA linearly independent \Cols}
Otherwise the set of vectors $\aD ai$
is {\bf linearly dependent}.
\end{ShadedDefinition}
}

\AddEq{definition: basis, AoxA module}
{
\begin{ShadedDefinition}
\labelDefinition{basis, AoxA module \Cols}
We call set of vectors
\ShowEq{basis, AoxA module \Cols}
\AddIndex{basis}{basis}
for \AoxA A\Hyph module $V$
if the set of vectors
\ShowEq{basis vector \Cols}
is linearly independent and adding to this set any other vector
we get a new set which is linearly dependent.
\end{ShadedDefinition}
}

\DefLabeledDefinition{Eigenvalue of Endomorphism}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
The vector $v\in V$ is called
{\bf eigenvector}
of the endomorphism
\ShowEq{f:A->B}{\Vector f}VV
with respect to the basis $\Basis e$,
if there exists $b\in A$ such that
\DrawEq[bv]{fov=b e o v}{\SideNS}
$A$\Hyph number $b$ is called
{\bf eigenvalue}
of the endomorphism $f$
with respect to the basis $\Basis e$.
}

\DefLabeledTheorem{no endomorphism fov=bv}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
If
\ShowEq{b not in ZA},
then there is no endomorphism $\Vector f$ such that
\ShowEq{fov=bv \SideNS}
%where $f$ is the matrix of endomorphism $\Vector f$.
}

\DefProofSloppy{no endomorphism fov=bv}
{
Let there exist endomorphism $\Vector f$
such that the equality
\EqRef{fov=bv \SideNS}
is true.
The equality
\ShowEq{b(av)=a(bv) \SideNS}
follows from equalities
\eqRef{associative law, \SideWS module}1,
\eqRef{\SideWS homomorphism, f av=}1,
\EqRef{fov=bv \SideNS}.
According to the theorem
\refTheorem{av=bv=>a=b}{\SideNS-\Cols},
the equality
\DrawEq{ab=ba}{\SideNS}
for any $a\in A$
follows from the equality
\EqRef{b(av)=a(bv) \SideNS}.
The equality
\eqRef{ab=ba}{\SideNS}
for any $a\in A$
contradicts to the statement
\ShowEq{b not in ZA}.
Therefore, considered endomorphism $\Vector f$
does not exist.
}

\AddEq{remark: Eigenvalue of Endomorphism}
{
\begin{sloppypar}
According to the theorem
\refTheorem{no endomorphism fov=bv}{\SideNS},
as opposed to the \OtherSideNS\Hyph side product
of vector over scalar,
\SideNS\Hyph side product
of vector over scalar
is not endomorphism
of \SideWS $A$\Hyph vector space.
Comparing the definition
\refDefinition{similarity transformation}{\SideNS}
and the theorem
\refTheorem{no endomorphism fov=bv}{\SideNS},
we see that similarity transformation
in non\Hyph commutative algebra
and similarity transformation
in commutative algebra
play the same role.
\end{sloppypar}
}

\DefLabeledTheorem{similarity transformation, change of basis}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
be bases of \SideWS $A$\Hyph vector space $V$.
Let $g$
be passive transformation
of basis $\Basis e_1$ into basis $\Basis e_2$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
The similarity transformation
\ShowEq{\SideWS map a En}a1
has the matrix
\DrawEq[ag]{ga*g- \SideNS-\Cols}a
with respect to the basis $\Basis e_2$.
}

\DefProof{similarity transformation, change of basis}
{
According to the theorem
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
the similarity transformation
\ShowEq{\SideWS map a En}a1
has the matrix
\ShowEq{ga*g- 1 \SideNS-\Cols}
with respect to the basis $\Basis e_2$.
The theorem follows from the expression
\EqRef{ga*g- 1 \SideNS-\Cols}.
}

\DefLabeledTheorem{similarity transformation}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Let
\ShowEq{dim V=n}
and $\aD En$ be \nTimes identity matrix.
For any $A$\Hyph number $a$, there exist endomorphism
\ShowEq{\SideWS map a En}a{}
of \SideWS $A$\Hyph vector space $V$
which has the matrix
\ShowEq{\SideWS a En}
whith respecpect to the basis $\Basis e$.
}

\DefProof{similarity transformation}
{
Let $\Basis e$ be the basis
of \SideWS $A$\Hyph vector space of columns.
According to the theorem
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)}
and the definition
\refDefinition{iso end aut morphism vector space}{\SideNS},
the map
\ShowEq{v in V -> av in V \SideNS-\Cols}
is endomorphism
of \SideWS $A$\Hyph vector space $V$.
}

\DefLabeledDefinitionNote{iso end aut morphism vector space}{\SideNS}
{
Homomorphism
\ShowEq{f:A->B}fVW
is called\,\footnotemark
\AddIndex{isomorphism}{isomorphism}
between \SideWS $A$\Hyph vector spaces $V$ and $W$,
if correspondence $f^{-1}$ is homomorphism.
A homomorphism
\ShowEq{f:A->B}fVV
in which source and target are the same
\SideWS $A$\Hyph vector space
is called
\AddIndex{endomorphism}{endomorphism}.
Endomorphism
\ShowEq{f:A->B}fVV
of \SideWS $A$\Hyph vector space $V$
is called
\AddIndex{automorphism}{automorphism},
if correspondence $f^{-1}$ is endomorphism.
}
{
I follow the definition on
page \citeBib{Cohn: Universal Algebra}\Hyph 49.
}

\DefText{Basis Manifold}
{
\section{Dimension of \SideWSC \texorpdfstring{$A$}{A}\Hyph Vector Space}

\ShowText{Dimension of Vector Space}

\section{Basis Manifold for \SideWSC \texorpdfstring{$A$}{A}-Vector Space}
%\labelSection{Basis Manifold for Vector Space}

\ShowEq{Basis Manifold for Vector Space}

\section{Passive Transformation in \SideWSC \texorpdfstring{$A$}{A}-Vector Space}

\ShowEq{Passive Transformation}
}

\DefLabeledTheorem[3]{rank of matrix}{\Product-\Cols}
{
Let $a$ be a matrix,
\ShowEq{\Product-rank a=k<m}{#1}
and $\SA T$ is \ProductType major submatrix.
Then \ColWS \ARow a{#2} is
a \SideWS linear composition of \ColsWS \ARow a{#3}
\ShowEq{rank of matrix, \Product-\Cols}
\ShowEq{rank of matrix, 1, \Product-\Cols}
\ShowEq{rank of matrix, 2, \Product-\Cols}
}

\DefProof[5]{rank of matrix}
{
If the matrix $a$ has $\gik$ \RowsNS, then assuming that \ColWS \ARow a{#2}
is a \SideWS linear combination
\EqRef{rank of matrix, 1, \Product-\Cols}
of \ColsWS \ARow a{#3} with coefficients $\Coef$,
we get system of \SideWS linear equations
\EqRef{rank of matrix, 2, \Product-\Cols}.
We assume that $\ACol x{#4}=\Coef$ are unknown variables
in the system of \SideWS linear equations
\EqRef{rank of matrix, 2, \Product-\Cols}.
According to the theorem
\refTheorem{nonsingular system of linear equations}{\SideNS-\Cols},
the system of \SideWS linear equations
\EqRef{rank of matrix, 2, \Product-\Cols}
has a unique solution
and this solution is nontrivial because all \ \, \ProductType quasideterminants are
different from $0$.

It remains to prove this statement in case when a number of \RowsRWSA of the matrix $a$
is more than $\gik$.
I get \ColWS \ARow a{#2} and \RowNWS $\ACol a{#5}$.
According to assumption, submatrix
$\SATpr$ is a \RC singular matrix
and its \ProductType quasideterminant
\DrawEq{singular matrix and quasideterminant}{\SideNS-\Cols}
According to the equality
\eqRef{j i quasideterminant =}{\Product}
the equality
\eqRef{singular matrix and quasideterminant}{\SideNS-\Cols}
has form
\ShowEq{rank of matrix, 4, \Product}
Matrix
\ShowEq{rank of matrix, 5, \Product-\Cols}
does not depend on $\gi{#5}$, Therefore, for any
\ShowEq{\rIn}
\ShowEq{rank of matrix, 6, \Product-\Cols}
To prove the equality
\EqRef{rank of matrix, 2, \Product-\Cols},
it is necessary to prove the equality
\ShowEq{rank of matrix, 9, \Product-\Cols}
From the equality
\ShowEq{rank of matrix, 7, \Product-\Cols}
it follows that
\ShowEq{rank of matrix, 8, \Product-\Cols}
The equality
\EqRef{rank of matrix, 9, \Product-\Cols}
follows from equalities
\EqRef{rank of matrix, 5, \Product-\Cols},
\EqRef{rank of matrix, 8, \Product-\Cols}.
The equality
\EqRef{rank of matrix, 2, \Product-\Cols}
follows from equalities
\EqRef{rank of matrix, 6, \Product-\Cols},
\EqRef{rank of matrix, 9, \Product-\Cols}.
}

\DefLabeledTheorem{set of eigenvectors is vector space}{\Product-\Cols}
{
Let $A$\Hyph number $b$ be
\ProductType eigenvalue
of the matrix $a$.
The set of eigen\ColsWS
of matrix $a$ corresponding to \ProductType eigenvalue $b$
is \SideWS $A$\Hyph vector space of \ColN s.
}

\DefProof{set of eigenvectors is vector space}
{
According to the definitions
\refDefinition{eigenvalue of matrix}{\Product},
\refDefinition{eigenvector of matrix}{\Product-\Cols},
coordinates of eigen\ColWS
are solution of the system of linear equations
\ShowEq{\Product-eigen\Cols=0}
with \ProductType singular matrix \ShowEq{f-bEn \SideNS}{}.
According to the theorem
\RefTheorem{Solutions homogenous system of linear equations},
the set of solutions of the system of linear equations
\EqRef{\Product-eigen\Cols=0}
is \SideWS $A$\Hyph vector space of \ColN s.
}

\DefLabeledTheorem{set of eigenvectors fg is vector space}{\Product-\Cols}
{
Let $A$\Hyph number $b$ be
\ProductType eigenvalue of the pair of matrices
\ShowEq{pair of matrices \Product-\ColN}{}
where $g$ is the \ProductType non\Hyph singular matrix.
The set of eigen\ColsWS
of the pair of matrices $(f,g)$ corresponding to \ProductType eigenvalue $b$
is \SideWS $A$\Hyph vector space of \ColN s.
}

\DefProof{set of eigenvectors fg is vector space}
{
According to the definitions
\refDefinition{eigenvalues of pair of matrices}{\Product},
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN},
coordinates of eigen\ColWS
are solution of the system of linear equations
\ShowEq{\Product-eigen\Cols=0 fg}
with \ProductType singular matrix
\[f-\ShowEq{ga*g- \SideNS-\Cols}bg\]
According to the theorem
\RefTheorem{Solutions homogenous system of linear equations},
the set of solutions of the system of linear equations
\EqRef{\Product-eigen\Cols=0 fg}
is \SideWS space of \ColN s.
}

\DefRemark{simplify definitions of eigenvalue}
{
Let
\ShowEq{gij in ZA}
Then
\ShowEq{gb rc g-=b}
\ShowEq{gb cr g-=b}
From equalities
\EqRef{gb rc g-=b},
\EqRef{gb cr g-=b},
it follows that,
if the condition
\EqRef{gij in ZA},
is satisfied,
then we can simplify definitions
of eigenvalue and eigenvector of matrix
and get definitions
which correspond to definitions
in commutative algebra.
}

\DefLabeledTheorem{columns of matrix are linearly dependent}{\Product-\Cols}
{
Let matrix $a$ have $\gi{\Lbls}$ \ColN s.
If
\ShowEq{\Product-rank a=k<m}{\Lbls}
then \ColsWS of the matrix are \SideWS linearly dependent
\DrawEq[{\lambda}a]{columns of matrix are linearly dependent}{}
}

\DefProof[1]{columns of matrix are linearly dependent}
{
Let \ColWS \ARow a{#1} be a \SideWS linear composition of \Rows
\EqRef{rank of matrix, 1, \Product-\Cols}. We assume
\ShowEq{\Cols-of-matrix linearly dependent, 1}
and the rest
\ShowEq{\Cols-of-matrix linearly dependent, 2}
}


==> Vector.Space.2020.Stmt.Eq.tex <==
%auto-ignore

\def\spanb{\text{span}(\ARow{\Vector a}i,\iIg)}

\newcommand\ARow[2]{\aU {#1}{#2}}
\newcommand\ACol[2]{\aD {#1}{#2}}
\newcommand\EBase[2]{\ECol {##1}{##2}}%

\newcommand\ColRowTheorem[1]
{
\TwoColText
{
\ShowEq{\DefCol}
\ShowTheorem{#1}
}
{
\ShowEq{\DefRow}
\ShowTheorem{#1}
}
}

\newcommand\ColRowLemma[1]
{
\TwoColText
{
\ShowEq{\DefCol}
\ShowLemma{#1}
}
{
\ShowEq{\DefRow}
\ShowLemma{#1}
}
}

\newcommand\ColRowProof[1]
{
\TwoColText
{
\ShowEq{\DefCol}
\ShowProof{#1}
}
{
\ShowEq{\DefRow}
\ShowProof{#1}
}
}

\newcommand\ProveColRowTheorem[1]
{
\ColRowTheorem{#1}
\ColRowProof{#1}
}

\newcommand\ColRowRemark[1]
{
\TwoColText
{
\ShowEq{\DefCol}
\ShowRemark{#1}
}
{
\ShowEq{\DefRow}
\ShowRemark{#1}
}
}

\newcommand\ColRowText[1]
{
\TwoColText
{
\ShowEq{\DefCol}
\ShowText{#1}
}
{
\ShowEq{\DefRow}
\ShowText{#1}
}
}

\newcommand\ColRowDefinition[1]
{
\TwoColText
{
\ShowEq{\DefCol}
\ShowDefinition{#1}
}
{
\ShowEq{\DefRow}
\ShowDefinition{#1}
}
}

\newcommand\AUD[3]{\ACol{\ARow{#1}{#3}}{#2}}%

\AddEq{def row}
{%
\def\ProductTypeO{\CRo}%
\def\Lbls{m}%
\def\Cols{rows}%
\def\Coef{\pRs}%
\def\rIn{r in N-T}%
\renewcommand\ARow[2]{\aU {##1}{##2}}%
\renewcommand\ACol[2]{\aD {##1}{##2}}%
\renewcommand\EBase[2]{\ERow {##1}{##2}}%
\def\ArMatrix{\ColMatrix}
\def\AcMatrix{\RowMatrix}
\def\ColN{row}%
\def\ColNS{row}%
\def\ColNWS{row }%
\def\RowLbWS{row }%
\def\RowN{col}%
\def\Rows{cols}%
\def\RowNWS{column }%
\ShowEq{def row text}%
}

\AddEq{def col}
{%
\def\ProductTypeO{\RCo}%
\def\Lbls{n}%
\def\Cols{cols}%
\def\Coef{\tRr}%
\def\rIn{p in M-S}%
\renewcommand\ARow[2]{\aD {##1}{##2}}%
\renewcommand\ACol[2]{\aU {##1}{##2}}%
\renewcommand\EBase[2]{\ECol {##1}{##2}}%
\def\ArMatrix{\RowMatrix}
\def\AcMatrix{\ColMatrix}
\def\ColN{column}%
\def\ColNWS{column }%
\def\ColNS{col}%
\def\RowN{row}%
\def\Rows{rows}%
\def\RowNWS{row }%
\ShowEq{def col text}%
}

\AddEq{rc-rows}
{%
\ShowEq{def rc}%
\ShowEq{def row}%
}

\AddEq{rc-cols}
{%
\ShowEq{def rc}%
\ShowEq{def col}%
}

\AddEq{cr-rows}
{%
\ShowEq{def cr}%
\ShowEq{def row}%
}

\AddEq{cr-cols}
{%
\ShowEq{def cr}%
\ShowEq{def col}%
}

\AddEq{-rows}
{%
\ShowEq{def opRow}%
\ShowEq{def row}%
}

\AddEq{-cols}
{%
\ShowEq{def opCol}%
\ShowEq{def col}%
}

\AddEq[6]{prolog homomorphism of vector space(1)}
{
\ShowEq{Let be basis of vector space}{#3}iIA{#2}V{#3}{\Cols}-
\ShowEq{Let be basis of vector space}{#6}jJA{#5}V{#6}{\Cols}-
}

\AddEq[6]{prolog homomorphism of vector space(11)}
{
\ShowEq{Let be basis of algebra and C}{A_{#2}}{#2}kKD{#1}A{#2}-
\ShowEq{Let be basis of algebra and C}{A_{#5}}{#5}lLD{#4}A{#5}-
\ShowEq{Let be basis of vector space}{{V_{#3}}}iIA{#2}V{#3}{\Cols}-
\ShowEq{Let be basis of vector space}{{V_{#6}}}jJA{#5}V{#6}{\Cols}-
}

\AddEq[6]{prolog homomorphism of vector space(111)}
{
\ShowEq{Let be basis of algebra and C}{A_{#2}}{#2}kKD{#1}A{#2}-
\ShowEq{Let be basis of algebra and C}{A_{#5}}{#5}lLD{#4}A{#5}-
\ShowEq{Let be basis of vector space}{{V_{#3}}}iIA{#2}V{#3}{\Cols}-
\ShowEq{Let be basis of vector space}{{V_{#6}}}jJA{#5}V{#6}{\Cols}-
}

\DefRef{define homomorphism A module}
{
\ShowRef{Morphism of Diagram of Representations}%
\refDefinition{module over algebra}{\SideWS \VectorSetNS},
}

\DefRef[3]{Proof, homomorphism of vector space}
{%
\ShowRef{Morphism of Diagram of Representations}%
\refDefinition{homomorphism from A1 to A2, D algebra}{#1#2},
\refDefinition{homomorphism A module}{\SideNS(#1#2#3)},
}

\DefRef[3]{Proof, homomorphism of vector space 1}
{
\eqRef{f:V1->V2, D module \Cols}{#1#2#3\SideNS},
\eqRef{f o ea=efa i (#1#2)}{(\Cols-\SideNS)algebra},
\eqRef{f o ea=efa (#1#2)(\Cols)}{#1#2#3\SideNS}
}

\DefRef[3]{Proof, homomorphism of vector space 2}
{
\eqRef{f:V1->V2, D module \Cols}{algebra(#1#2)},
\eqRef{f o ea=efa i (#2#3)}{(#1)(\Cols)algebra, \SideNS-module},
\eqRef{f o ea=efa (#1#2)(\Cols)}{algebra}.
}

\DefText{g:A1->A2, D module(111)}
{
\DrawEq[g{h(a)}{}]{f:V1->V2, D module \Cols}{111\SideNS}
\DrawEq[hg12a]{f o ea=efa i (11)}{(\Cols-\SideNS)algebra}
\DrawEq[hg{A_1}{A_2}]{f o ea=efa (11)(\Cols)}{111\SideNS}
}

\DefText{g:A1->A2, D module(11)}
{
\DrawEq[ga]{f:V1->V2, D module \Cols}{11\SideNS}
\DrawEq[hg{A_1}{A_2}{}]{f o ea=efa i \SideNS(1)}{(\Cols)algebra}
\DrawEq[hf{A_1}{A_2}]{f o ea=efa (1)(\Cols)}{11\SideNS}
}

\DefText{g:A1->A2, D module(1)}
{
}

\DefText{Vector Space Type}
{
\,

\ShowDefinition{module type}

\ProveTheorem{linear combination in module type}

\ProveTheorem{coordinate matrix of vector}

\ShowTheorem{coordinates of vector}
\ShowProof{coordinates of vector *}

\ShowTheorem{Two bases of module}
\ShowLemma{Two bases of module 1}
\ShowProof{Two bases of module 1}
\ShowLemma{Two bases of module 2}
\ShowProof{Two bases of module 2}
\ShowProof{Two bases of module}
}

\AddEq[6]{extended basis}
{
\eV[#1_{#2}#3_{#4}]=(\EBase {#1_{#2}#3_{#4}}{#5#6}
=\Multiply{\EBase{#3_{#4}}#6}{\EBase {#1_{#2}}#5})
}

\AddEq{Two bases of module 1 a}
{
a=\Multiply{\ACol ai}{\EBase 1i}
}

\AddEq{Two bases of module 1 ai}
{
\ACol ai=\Multiply{\ACol a{ik}}{\EBase{}k}
}

\AddEq{Two bases of module 1 a=ai}
{
a=\Multiply{\Multiply{\ACol a{ik}}{\EBase{}k}}{\EBase 1i}
=\Multiply{\ACol a{ik}}{\EBase 2{ik}}
}

\AddEq{extended basis 1}
{
\Multiply{\ACol a{ik}}{\EBase 2{ik}}=0
}

\AddEq{extended basis 2}
{
\Multiply{\ACol a{ik}}{\Multiply{\EBase{}k}{\EBase 1i}}=0
}

\AddEq{extended basis 3}
{
\Multiply{\ACol a{ik}}{\EBase{}k}=0\ \ \ \jJg kK
}

\AddEq{extended basis 4}
{
\ACol a{ik}=0\ \ \ \jJg kK\ \ \ \jJg iI
}

\AddEq{linear span, 0}
{
\[
\Vector a=\ArMatrix{\Vector a}m
=(\ARow{\Vector a}i,\iIg)
\]
}

\AddEq{linear span, 6}
{
$\Vector b$, $\ARow{\Vector a}i$
}

\AddEq{e*v=e*w,}
{
v\ProductVal e=w\ProductVal e\ \ \ \ \ACol vi\ARow ei=\ACol wi\ARow ei
}

\AddEq{e*v=e*w,left}
{
v\ProductVal e=w\ProductVal e\ \ \ \ \ACol vi\ARow ei=\ACol wi\ARow ei
}

\AddEq{e*v=e*w,right}
{
e\ProductVal v=e\ProductVal w\ \ \ \ \ARow ei\ACol vi=\ARow ei\ACol wi
}

\AddEq{matrix a = set ai cols}
{
a=
\begin{pmatrix}
\AcMatrix{\ARow a1}n&...&\AcMatrix{\ARow am}n
\end{pmatrix}
=\PMatrix amn
}

\AddEq{matrix a = set ai rows}
{
a=
\begin{pmatrix}
\AcMatrix{\ARow a1}n\\...\\ \AcMatrix{\ARow am}n
\end{pmatrix}
=\PMatrix anm
}

\AddEq{=> v=w}
{
\[
v=w\ \ \ \ \ACol vi=\ACol wi
\]
}

\AddEq[1]{linear span, b left}
{
\Vector{#1}=#1\ProductVal e=\ACol{#1}j\ARow ej
\ \ \ \ \ #1=\AcMatrix {#1}n
}

\AddEq[1]{linear span, b right}
{
\Vector{#1}=e\ProductVal #1=\ARow ej\ACol{#1}j
\ \ \ \ \ #1=\AcMatrix {#1}n
}

\AddEq{e*b=e*a*x left}
{
\ACol bj\ARow ej=\ACol xi(\ACol{\ARow ai}j\ARow ej)
=(\ACol xi\ACol{\ARow ai}j)\ARow ej
}

\AddEq{e*b=e*a*x right}
{
\ARow ej\ACol bj=(\ARow ej\ACol{\ARow ai}j)\ACol xi
=\ARow ej(\ACol{\ARow ai}j\ACol xi)
}

\AddEq{b=a*x left}
{
\ACol bj=\ACol xi\ACol{\ARow ai}j
}

\AddEq{b=a*x right}
{
\ACol bj=\ACol{\ARow ai}j\ACol xi
}

\AddEq{a*x=b left}
{
\begin{split}
\ACol x1\ACol{\ARow a1}1+...+\ACol xm\ACol{\ARow am}1&=\ACol b1
\\...&...\\
\ACol x1\ACol{\ARow a1}n+...+\ACol xm\ACol{\ARow am}n&=\ACol bn
\end{split}
}

\AddEq{a*x=b right}
{
\begin{split}
\ACol{\ARow a1}1\ACol x1+...+\ACol{\ARow am}1\ACol xm&=\ACol b1
\\...&...\\
\ACol{\ARow a1}n\ACol x1+...+\ACol{\ARow am}n\ACol xm&=\ACol bn
\end{split}
}

\DefText{linear span in vector space}
{
\,

\ShowDefinition{linear span, vector space}

\ProveTheorem{vector in linear span}

\ProveTheorem{linear span is vector space}

\ProveTheorem{linear span and system of equations}

\ProveTheorem{matrix and system of linear equations}

\ShowDefinition{nonsingular system of linear equations}

\ProveTheorem{nonsingular system of linear equations}
}

\AddEq{x=a-*b, matrix right}
{
x=a^{\InverseVal}\ProductVal b
}

\AddEq{x=a-*b, matrix left}
{
x=b\ProductVal a^{\InverseVal}
}

\AddEq{x=a-*b, quasideterminant right}
{
x=\mathcal H\DetVal a\ProductVal b
}

\AddEq{x=a-*b, quasideterminant left}
{
x=b\ProductVal \mathcal H\DetVal a
}

\AddEquation{a*x=b left-cols}
{
\ColMatrix xm\CRstar\PMatrix amn=\ColMatrix bn
}

\AddEquation{a*x=b right-cols}
{
\PMatrix amn\RCstar\ColMatrix xm=\ColMatrix bn
}

\AddEquation{a*x=b left-rows}
{
\RowMatrix xm\RCstar\PMatrix anm=\ColMatrix bn
}

\AddEquation{a*x=b right-rows}
{
\PMatrix anm\CRstar\RowMatrix xm=\RowMatrix bn
}

\AddEq{a*x=b 1 left-cols}
{
x\CRstar a=b
}

\AddEq{a*x=b 1 right-cols}
{
a\RCstar x=b
}

\AddEq{a*x=b 1 left-rows}
{
x\RCstar a=b
}

\AddEq{a*x=b 1 right-rows}
{
a\CRstar x=b
}

\AddEq{linear span, 1}
{
\[
\Vector b\in\spanb
\]
}

\AddEq{linear span, 3 right}
{
\begin{align*}
\Vector b+\Vector c
=\Vector a\ProductVal b+\Vector a\ProductVal c
=\Vector a\ProductVal(b+c)
&\in\spanb\\
\Vector bk=(\Vector a\ProductVal b)k=\Vector a\ProductVal(bk)
&\in\spanb
\end{align*}
}

\AddEq{linear span, 3 left}
{
\begin{align*}
\Vector b+\Vector c
=a\ProductVal b+a\ProductVal c
=a\ProductVal(b+c)
&\in\spanb\\
\Vector bk=(a\ProductVal b)k=a\ProductVal(bk)
&\in\spanb
\end{align*}
}

\AddEq[2]{linear span, 2 right}
{
\Vector{#1}=\Vector a\ProductVal #2=\ARow{\Vector a}i\ACol{#2}i
}

\AddEq[2]{linear span, 2 left}
{
\Vector{#1}=#2\ProductVal\Vector a=\ACol{#2}i\ARow{\Vector a}i
}

\AddEq{linear span, vector space, 2}
{
\begin{align*}
\Vector b&=a\RCstar b\\
\Vector c&=a\RCstar c
\end{align*}
}

\AddEq[1]{b not in ZA}
{
$b\not\in Z(A)$#1
}

\AddEq[2]{D diagonal matrix}
{
\[
#1=\mathrm{diag}(b(\gi 1),...,b(\gi {#2}))
\]
}

\AddEq[3]{A rc U=U rc D right}
{
a_{#1}\RCstar u_{#2}=u_{#2}\RCstar #3
}

\AddEq[3]{A rc U=U rc D left}
{
u_{#2}\RCstar a_{#1}=#3\RCstar u_{#2}
}

\AddEq[3]{A cr U=U cr D left}
{
u_{#2}\CRstar a_{#1}=#3\CRstar u_{#2}
}

\AddEq[3]{A cr U=U cr D right}
{
a_{#1}\CRstar u_{#2}=u_{#2}\CRstar #3
}

\AddEq{U-*A*U=D rc-right}
{
u_2^{\RCInverse}\RCstar a_2\RCstar u_2=a_1
}

\AddEq{U-*A*U=D rc-left}
{
u_2\RCstar a_2\RCstar u_2^{\RCInverse}=a_1
}

\AddEq{U-*A*U=D cr-left}
{
u_2\CRstar a_2\CRstar u_2^{\CRInverse}=a_1
}

\AddEq{U-*A*U=D cr-right}
{
u_2^{\CRInverse}\CRstar a_2\CRstar u_2=a_1
}

\AddEq{U-*A*U-di En rc-right}
{
\begin{align*}
&\,u_2^{\RCInverse}\RCstar a_2\RCstar u_2-b(\gii)\aD En
\\ = &\, 
u_2^{\RCInverse}\RCstar( a_2-u_2b(\gii)\RCstar u_2^{\RCInverse})\RCstar u_2
\end{align*}
}

\AddEq{U-*A*U-di En rc-left}
{
\begin{align*}
&\,u_2\RCstar a_2\RCstar u_2^{\RCInverse}-b(\gii)\aD En
\\ = &\, 
u_2\RCstar( a_2-u_2^{\RCInverse}\RCstar b(\gii)u_2)\RCstar u_2^{\RCInverse}
\end{align*}
}

\AddEq{U-*A*U-di En cr-left}
{
\begin{align*}
&\,u_2\CRstar a_2\CRstar u_2^{\CRInverse}-b(\gii)\aD En
\\ = &\, 
u_2\CRstar( a_2-u_2^{\CRInverse}\CRstar b(\gii)u_2)\CRstar u_2^{\CRInverse}
\end{align*}
}

\AddEq{U-*A*U-di En cr-right}
{
\begin{align*}
&\,u_2^{\CRInverse}\CRstar a_2\CRstar u_2-b(\gii)\aD En
\\ = &\, 
u_2^{\CRInverse}\CRstar( a_2-u_2b(\gii)\CRstar u_2^{\CRInverse})\CRstar u_2
\end{align*}
}

\AddEquation{A-U-*di*U rc-right}
{
a_2-u_2b(\gii)\RCstar u_2^{\RCInverse}
}

\AddEquation{A-U-*di*U rc-left}
{
a_2-u_2^{\RCInverse}\RCstar b(\gii)u_2
}

\AddEquation{A-U-*di*U cr-left}
{
a_2-u_2^{\CRInverse}\CRstar b(\gii)u_2
}

\AddEquation{A-U-*di*U cr-right}
{
a_2-u_2b(\gii)\CRstar u_2^{\CRInverse}
}

\AddEquation{a1*e1=di e1 rc-left}
{
\ShowEq{ARow u2i \Cols}e1i
\RCstar a_1
=\ShowEq{ARow u2i \Cols}e1i
b(\gii)
}

\AddEq[3]{linear combination, -rows}
{
\[
\sum_{\gii=\gi 1}^{\gi{#3}}#1(\gii)#2(\gii)=\aD{#1}i\aU{#2}i
\]
}

\AddEq[3]{linear combination, left-rows}
{
\[
\sum_{\gii=\gi 1}^{\gi{#3}}#1(\gii)#2(\gii)=\aD{#1}i\aU{#2}i
\]
}

\AddEq[3]{linear combination, right-cols}
{
\[
\sum_{\gii=\gi 1}^{\gi{#3}}#2(\gii)#1(\gii)=\aD{#2}i\aU{#1}i
\]
}

\AddEq[3]{linear combination, left-cols}
{
\[
\sum_{\gii=\gi 1}^{\gi{#3}}#1(\gii)#2(\gii)=\aU{#1}i\aD{#2}i
\]
}

\AddEq[3]{linear combination, right-rows}
{
\[
\sum_{\gii=\gi 1}^{\gi{#3}}#2(\gii)#1(\gii)=\aU{#2}i\aD{#1}i
\]
}

\AddEq[3]{linear combination, -cols}
{
\[
\sum_{\gii=\gi 1}^{\gi{#3}}#1(\gii)#2(\gii)=\aU{#1}i\aD{#2}i
\]
}

\AddEquation{a1*e1=di e1 rc-right}
{
a_1\RCstar
\ShowEq{ARow u2i \Cols}e1i
=b(\gii)
\ShowEq{ARow u2i \Cols}e1i
}

\AddEquation{a1*e1=di e1 cr-left}
{
\ShowEq{ARow u2i \Cols}e1i
\CRstar a_1
=\ShowEq{ARow u2i \Cols}e1i
b(\gii)
}

\AddEquation{a1*e1=di e1 cr-right}
{
a_1\CRstar
\ShowEq{ARow u2i \Cols}e1i
=b(\gii)
\ShowEq{ARow u2i \Cols}e1i
}

\AddEquation{U-*A*U*e1=di e1 rc-left}
{
\ShowEq{ARow u2i \Cols}e1i
\RCstar u_2\RCstar a_2\RCstar u_2^{\RCInverse}
=\ShowEq{ARow u2i \Cols}e1i
b(\gii)
}

\AddEquation{U-*A*U*e1=di e1 rc-right}
{
u_2^{\RCInverse}\RCstar a_2\RCstar u_2\RCstar
\ShowEq{ARow u2i \Cols}e1i
=b(\gii)
\ShowEq{ARow u2i \Cols}e1i
}

\AddEquation{U-*A*U*e1=di e1 cr-left}
{
\ShowEq{ARow u2i \Cols}e1i
\CRstar u_2\CRstar a_2\CRstar u_2^{\CRInverse}
=\ShowEq{ARow u2i \Cols}e1i
b(\gii)
}

\AddEquation{U-*A*U*e1=di e1 cr-right}
{
u_2^{\CRInverse}\CRstar a_2\CRstar u_2\CRstar
\ShowEq{ARow u2i \Cols}e1i
=b(\gii)
\ShowEq{ARow u2i \Cols}e1i
}

\AddEquation{A*U*e1=... rc-left}
{
\begin{aligned}
&\,\ShowEq{ARow u2i \Cols}e1i
\RCstar u_2\RCstar a_2
\\ =&\,\ShowEq{ARow u2i \Cols}e1i
b(\gii)\RCstar u_2
\\ =&\,\ShowEq{ARow u2i \Cols}e1i
\RCstar u_2\RCstar u_2^{\RCInverse}\RCstar
b(\gii)u_2
\end{aligned}
}

\AddEquation{A*U*e1=... rc-right}
{
\begin{aligned}
&\,a_2\RCstar u_2\RCstar
\ShowEq{ARow u2i \Cols}e1i
\\ =&\,u_2\RCstar b(\gii)
\ShowEq{ARow u2i \Cols}e1i
\\ =&\,u_2b(\gii)\RCstar 
u_2^{\RCInverse}\RCstar u_2\RCstar
\ShowEq{ARow u2i \Cols}e1i
\end{aligned}
}

\AddEquation{A*U*e1=... cr-left}
{
\begin{aligned}
&\,\ShowEq{ARow u2i \Cols}e1i
\CRstar u_2\CRstar a_2
\\ =&\,\ShowEq{ARow u2i \Cols}e1i
b(\gii)\CRstar u_2
\\ =&\,\ShowEq{ARow u2i \Cols}e1i
\CRstar u_2\CRstar u_2^{\CRInverse}\CRstar
b(\gii)u_2
\end{aligned}
}

\AddEquation{A*U*e1=... cr-right}
{
\begin{aligned}
&\,a_2\CRstar u_2\CRstar
\ShowEq{ARow u2i \Cols}e1i
\\ =&\,u_2\CRstar b(\gii)
\ShowEq{ARow u2i \Cols}e1i
\\ =&\,u_2b(\gii)\CRstar 
u_2^{\CRInverse}\CRstar u_2\CRstar
\ShowEq{ARow u2i \Cols}e1i
\end{aligned}
}

\AddEq{expansion relative basis, vector space, 0}
{
$\Vector v$, $\aD ei$, \iIg,
}

\AddEq{expansion relative basis, vector space, (0)}
{
$\Vector v$, $e(\gii)$, \iIg,
}

\AddEq{expansion relative basis, vector space, 1}
{
b\Vector v+c\CRstar e=0
}

\AddEquation{expansion relative basis, vector space, 1 left}
{
b\Vector v+c(\gii) e(\gii)=0
}

\AddEquation{expansion relative basis, vector space, 1 right}
{
\Vector vb+e(\gii)c(\gii) =0
}

\AddEq{expansion relative basis, vector space, 2}
{
\Vector v=(-cb^{-1})\CRstar e
}

\AddEquation{expansion relative basis, vector space, 2 left}
{
\Vector v=(-b^{-1}c(\gii)) e(\gii)
}

\AddEquation{expansion relative basis, vector space, 2 right}
{
\Vector v= e(\gii)(-c(\gii)b^{-1})
}

\AddEq{expansion relative basis, vector space, 3}
{
\Vector v=v'\RCstar e
}

\AddEquation{expansion relative basis, vector space, 3 left}
{
\Vector v=v'(\gii) e(\gii)
}

\AddEquation{expansion relative basis, vector space, 3 right}
{
\Vector v=e(\gii)v'(\gii)
}

\AddEq{expansion relative basis, vector space, 4}
{
0=(v'-v)\CRstar e
}

\AddEquation{expansion relative basis, vector space, 4 left}
{
0=(v'(\gii)-v(\gii)) e(\gii)
}

\AddEquation{expansion relative basis, vector space, 4 right}
{
0= e(\gii)(v'(\gii)-v(\gii))
}

\AddEq{expansion relative basis, vector space, 5}
{
v'-v=0
}

\AddEq{expansion relative basis, vector space, 5()}
{
v'(\gii)-v(\gii)=0\ \ \ \,\iIg
}

\AddEq{expansion relative basis, vector space}
{
\Vector v=v\CRstar e
}

\AddEquation{expansion relative basis, vector space left}
{
\Vector v=v(\gii) e(\gii)\ \ \ \,v(\gii)=-b^{-1}c(\gii)
}

\AddEquation{expansion relative basis, vector space right}
{
\Vector v=e(\gii)v(\gii)\ \ \ \,v(\gii)=-c(\gii)b^{-1}
}

\AddEq{linear span, set}
{
$\{\ARow {\Vector a}i\in V, \iIg\}$
}

\AddEq{linear span, vector space}
{
\symb{\spanb}{linear span, vector space}1
}

\AddEq{e2=e1}
{
$\Basis e_2=\Basis e_1$.
}

\AddEquation{di*ui=ui*di rc-left}
{
\ShowEq{ARow u2i \Cols}u1i
\RCstar u_2^{\RCInverse}\RCstar
b(\gii)u_2=b(\gii)
\ShowEq{ARow u2i \Cols}u1i
}

\AddEquation{di*ui=ui*di rc-right}
{
u_2b(\gii)\RCstar 
u_2^{\RCInverse}\RCstar
\ShowEq{ARow u2i \Cols}u1i
=
\ShowEq{ARow u2i \Cols}u1i
b(\gii)
}

\AddEquation{di*ui=ui*di cr-left}
{
\ShowEq{ARow u2i \Cols}u1i
\CRstar u_2^{\CRInverse}\CRstar
b(\gii)u_2=b(\gii)
\ShowEq{ARow u2i \Cols}u1i
}

\AddEquation{di*ui=ui*di cr-right}
{
u_2b(\gii)\CRstar 
u_2^{\CRInverse}\CRstar
\ShowEq{ARow u2i \Cols}u1i
=
\ShowEq{ARow u2i \Cols}u1i
b(\gii)
}

\AddEquation{di*ui=ui*di 1 rc-left}
{
\begin{aligned}
&\,\ShowEq{ARow u2i \Cols}u1i
\RCstar u_2^{\RCInverse}
b(\gii)\\ =&\,b(\gii)
\ShowEq{ARow u2i \Cols}u1i
\RCstar u_2^{\RCInverse}
\end{aligned}
}

\AddEquation{di*ui=ui*di 1 rc-right}
{
\begin{aligned}
&\,b(\gii) 
u_2^{\RCInverse}\RCstar
\ShowEq{ARow u2i \Cols}u1i
\\ =&\,
u_2^{\RCInverse}\RCstar
\ShowEq{ARow u2i \Cols}u1i
b(\gii)
\end{aligned}
}

\AddEquation{di*ui=ui*di 1 cr-left}
{
\begin{aligned}
&\,\ShowEq{ARow u2i \Cols}u1i
\CRstar u_2^{\CRInverse}
b(\gii)\\ =&\,b(\gii)
\ShowEq{ARow u2i \Cols}u1i
\CRstar u_2^{\CRInverse}
\end{aligned}
}

\AddEquation{di*ui=ui*di 1 cr-right}
{
\begin{aligned}
&\,b(\gii) 
u_2^{\CRInverse}\CRstar
\ShowEq{ARow u2i \Cols}u1i
\\ =&\,
u_2^{\CRInverse}\CRstar
\ShowEq{ARow u2i \Cols}u1i
b(\gii)
\end{aligned}
}

\AddEq[3]{di 1n}
{
$#1(\gi 1)$, ..., $#1(\gi{#2})$#3
}

\AddEq[3]{di 1n+1}
{
$#1(\gi 1)$, ..., $#1(\gi{#2}-\gi 1)$, $#1(\gi{#2})$#3
}

\AddEq{di ne dj}
{
\[\gii\ne\gij\Rightarrow b(\gii)\ne b(\gij)\]
}

\AddEq{ref 1 for n eigenvectors}
{
\ePrints{348311191}%
\ifx\Semafor\ValueOn%
\refTheorem[\RefDiffEq]{covariance of eigenvalue}{\SideNS-cols},
\refTheorem[\RefDiffEq]{covariance of eigenvalue}{\SideNS-rows},
\else%
\refTheorem{covariance of eigenvalue}{\SideNS-cols},
\refTheorem{covariance of eigenvalue}{\SideNS-rows},
\fi%
}

\AddEq{ref 2 for n eigenvectors}
{
\ePrints{348311191}%
\ifx\Semafor\ValueOn%
\refTheorem[\RefDiffEq]{define homomorphism of vector space}{\SideNS}.
\else%
\refTheorem{define homomorphism A module}{\SideNS(1)}.
\fi%
}

\DefText{Left and Right Eigenvalues}
{
\AddIndex{}{eigenvalue}
\TwoColText
{
\ShowEq{def left}
\ShowEq{\LeftText}
\ShowDefinition{Left and Right Eigenvalues}
}
{
\ShowEq{def right}
\ShowEq{\RightText}
\ShowDefinition{Left and Right Eigenvalues}
}
}

\DefText[6]{homomorphism of vector space, algebra(1)}
{
\ShowText{coordinates of the linear map 1}aA{A_1}{(#1)(#2)}{}
\ShowText{coordinates of the linear map 2(#1)}ahkK{D_{#4}}
\ShowText{coordinates of the linear map 3}aA{A_2}g{}b{(#1)(#2)}
\ShowText{coordinates of the linear map 4}gA{A_{#2}}{A_{#5}}kK
\ShowText{Morphism of D algebra}{#1}{#2}g
}

\DefText[6]{homomorphism of vector space, algebra()}
{
}

\DefText[6]{homomorphism of vector space, algebra 1}
{
\ShowText{coordinates of the linear map 1}vV{V_1}{(#1)(#2)(#3)}{\SideNS}
\ShowText{coordinates of the linear map 2(#2)}vgiI{A_{#5}}
\ShowText{coordinates of the linear map 3}vV{V_2}f{\SideNS}w{(#1)(#2)}
\ShowText{coordinates of the linear map 4}fV{V_{#3}}{V_{#6}}iI
}

\AddEq[1]{Left and Right Eigenvalues 1}
{
\ShowText{Left and Right Eigenvalues}

\ShowEq{def #1}
\ShowDefinition{spectrum of matrix}

\TwoColText
{
\ShowEq{def left}
\ShowEq{\LeftText}
\ShowTheorem{Eigenvalue and conjugate class}
}
{
\ShowEq{def right}
\ShowEq{\RightText}
\ShowTheorem{Eigenvalue and conjugate class}
}

\ShowFootnote{Eigenvalue and conjugate class}

\TwoColText
{
\ShowEq{def left}
\ShowEq{\LeftText}
\ShowProof{Eigenvalue and conjugate class}
}
{
\ShowEq{def right}
\ShowEq{\RightText}
\ShowProof{Eigenvalue and conjugate class}
}

\TwoColText
{
\ShowEq{def left}
\ShowEq{\LeftText}
\ShowTheorem{Coefficient comutes with matrix}vc
\ShowProof{Coefficient comutes with matrix}vc
}
{
\ShowEq{def right}
\ShowEq{\RightText}
\ShowTheorem{Coefficient comutes with matrix}cv
\ShowProof{Coefficient comutes with matrix}cv
}

\TwoColText
{
\ShowEq{def left}
\ShowEq{\LeftText}
\ShowRemark{Eigenvalue and conjugate class}
}
{
\ShowEq{def right}
\ShowEq{\RightText}
\ShowRemark{Eigenvalue and conjugate class}
}

\TwoColText
{
\ShowEq{def left}
\ShowEq{\LeftText}
\ShowTheorem{Eigenvector does not depend on basis}
\begin{sloppypar}
\ShowProof{Eigenvector does not depend on basis}
\end{sloppypar}
}
{
\ShowEq{def right}
\ShowEq{\RightText}
\ShowTheorem{Eigenvector does not depend on basis}
\begin{sloppypar}
\ShowProof{Eigenvector does not depend on basis}
\end{sloppypar}
}

\TwoColText
{
\ShowEq{def left}
\ShowEq{\LeftText}
\ShowRemark{Eigenvector does not depend on basis}
}
{
\ShowEq{def right}
\ShowEq{\RightText}
\ShowRemark{Eigenvector does not depend on basis}
}

\TwoColText
{
\ShowEq{def left}
\ShowEq{\LeftText}
\begin{sloppypar}
\ProveTheorem{right eigenvalue is eigenvalue}
\end{sloppypar}
}
{
\ShowEq{def right}
\ShowEq{\RightText}
\begin{sloppypar}
\ProveTheorem{right eigenvalue is eigenvalue}
\end{sloppypar}
}

\TwoColText
{
\ShowEq{def left}
\ShowEq{\LeftText}
\begin{sloppypar}
\ShowRemark{right eigenvalue is eigenvalue}
\end{sloppypar}
}
{
\ShowEq{def right}
\ShowEq{\RightText}
\begin{sloppypar}
\ShowRemark{right eigenvalue is eigenvalue}
\end{sloppypar}
}

%\ProveTheorem{n eigenvalues}
}

\AddEq{prove n eigenvectors}
{
\ShowEq{def AVector}
\ShowTheorem{n eigenvectors}{algebra}

\ShowRemark{n eigenvectors}

\TwoColText
{
\ShowEq{def left}
\ShowProof{n eigenvectors}
}
{
\ShowEq{def right}
\ShowProof{n eigenvectors}
}
}

\AddEq{gik<gin}
{
$\gik$, $\gik<\gin$,
}

\AddEq{rank rc u2 =k}
{
\[
\RCRank u_2=\gik
\]
}

\AddEq{rank rc u2 <k}
{
\[
\RCRank u_2<\gik
\]
}

\AddEquation{w rc u2=Ek left}
{
u_2\RCstar w=\aD Ek
}

\AddEquation{w rc u2=Ek right}
{
w\RCstar u_2=\aD Ek
}

\AddEquation{w rc a2 rc u2=a1 left}
{
u_2\RCstar a_2\RCstar w=a_1
}

\AddEquation{w rc a2 rc u2=a1 right}
{
w\RCstar a_2\RCstar u_2=a_1
}

\AddEq{gin x gik left}
{
$\gin\times\gik$
}

\AddEq{gin x gik right}
{
$\gik\times\gin$
}

\AddEq{as ox as=a1 ox a2, 1}
{
\Entry[s0]a{}ij\otimes\Entry[s1]a{}ij
=1\otimes\Entry a1ij
}

\AddEq{as ox as=a1 ox a2, 0}
{
\Entry[s0]a{}ij\otimes\Entry[s1]a{}ij
=\Entry a0ij\otimes 1
}

\AddEquation{as ox as o cv = ..., left-cols}
{
\begin{split}
&\,(\Entry[s0]a{}ij\otimes\Entry[s1]a{}ij)\circ (c\aU vj)
\\=&\,\Entry[s0]a{}ijc\aU vj\Entry[s1]a{}ij
\\=&\,c(\Entry[s0]a{}ij\aU vj\Entry[s1]a{}ij)
\\=&\,cb\aU vi=b(c\aU vi)
\end{split}
}

\AddEquation{as ox as o cv = ..., right-cols}
{
\begin{split}
&\,(\Entry[s0]a{}ij\otimes\Entry[s1]a{}ij)\circ (\aU vjc)
\\=&\,\Entry[s0]a{}ij\aU vjc\Entry[s1]a{}ij
\\=&\,(\Entry[s0]a{}ij\aU vj\Entry[s1]a{}ij)c
\\=&\,\aU vibc=(\aU vic)b
\end{split}
}

\AddEquation{as ox as o cv = ..., left-rows}
{
\begin{split}
&\,(\Entry[s0]a{}ij\otimes\Entry[s1]a{}ij)\circ (c\aD vi)
\\=&\,\Entry[s0]a{}ijc\aD vi\Entry[s1]a{}ij
\\=&\,c(\Entry[s0]a{}ij\aD vi\Entry[s1]a{}ij)
\\=&\,cb\aD vj=b(c\aD vj)
\end{split}
}

\AddEquation{as ox as o cv = ..., right-rows}
{
\begin{split}
&\,(\Entry[s0]a{}ij\otimes\Entry[s1]a{}ij)\circ (\aD vic)
\\=&\,\Entry[s0]a{}ij\aD vic\Entry[s1]a{}ij
\\=&\,(\Entry[s0]a{}ij\aD vi\Entry[s1]a{}ij)c
\\=&\,\aD vjbc=(\aD vfc)b
\end{split}
}

\AddEq{as ox as o v = v a12, 1, cols}
{
(\Entry[s0]a{}ij\otimes\Entry[s1]a{}ij)\circ \aU vj
=(1\otimes\Entry a1ij)\circ \aU vj
=\aU vj\Entry a1ij
}

\AddEquation{as ox as o v = v a12, matrix, 0 left-cols}
{
\PMatrix{a_0^{}{}}nn\RCstar\ColMatrix vn=
b\ColMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 1 left-cols}
{
\ColMatrix vn\CRstar\PMatrix{a_1^{}{}}nn=
b\ColMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 0 right-cols}
{
\PMatrix{a_0^{}{}}nn\RCstar\ColMatrix vn=
\ColMatrix vnb
}

\AddEquation{as ox as o v = v a12, matrix, 1 right-cols}
{
\ColMatrix vn\CRstar\PMatrix{a_1^{}{}}nn=
\ColMatrix vnb
}

\AddEquation{as ox as o v = v a12, matrix, 0 right-rows}
{
\PMatrix{a_0^{}{}}nn\CRstar\RowMatrix vn=
\RowMatrix vnb
}

\AddEquation{as ox as o v = v a12, matrix, 1 right-rows}
{
\RowMatrix vn\RCstar\PMatrix{a_1^{}{}}nn=
\RowMatrix vnb
}

\AddEquation{as ox as o v = v a12, matrix, 0 left-rows}
{
\PMatrix{a_0^{}{}}nn\CRstar\RowMatrix vn=
b\RowMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 1 left-rows}
{
\RowMatrix vn\RCstar\PMatrix{a_1^{}{}}nn=
b\RowMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 0 1 left-cols}
{
\PMatrix{a_0^{}{}}nn\RCstar\ColMatrix vn=
\ShowEq{matrix of maps n x n}
\RCcirc\ColMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 1 1 left-cols}
{
\ColMatrix vn\CRstar\PMatrix{a_1^{}{}}nn=
\ShowEq{matrix of maps n x n}
\RCcirc\ColMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 0 1 right-cols}
{
\PMatrix{a_0^{}{}}nn\RCstar\ColMatrix vn=
\ShowEq{matrix of maps n x n}
\RCcirc\ColMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 1 1 right-cols}
{
\ColMatrix vn\CRstar\PMatrix{a_1^{}{}}nn=
\ShowEq{matrix of maps n x n}
\RCcirc\ColMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 0 1 right-rows}
{
\PMatrix{a_0^{}{}}nn\CRstar\RowMatrix vn=
\ShowEq{matrix of maps n x n}
\CRcirc\RowMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 1 1 right-rows}
{
\RowMatrix vn\RCstar\PMatrix{a_1^{}{}}nn=
\ShowEq{matrix of maps n x n}
\CRcirc\RowMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 0 1 left-rows}
{
\PMatrix{a_0^{}{}}nn\CRstar\RowMatrix vn=
\ShowEq{matrix of maps n x n}
\CRcirc\RowMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 1 1 left-rows}
{
\RowMatrix vn\RCstar\PMatrix{a_1^{}{}}nn=
\ShowEq{matrix of maps n x n}
\CRcirc\RowMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 0 2 left-cols}
{
\ShowEq{matrix of maps n x n}
\RCcirc\ColMatrix vn
= b\ColMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 1 2 left-cols}
{
\ShowEq{matrix of maps n x n}
\RCcirc\ColMatrix vn
= b\ColMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 0 2 right-cols}
{
\ShowEq{matrix of maps n x n}
\RCcirc\ColMatrix vn
= \ColMatrix vnb
}

\AddEquation{as ox as o v = v a12, matrix, 1 2 right-cols}
{
\ShowEq{matrix of maps n x n}
\RCcirc\ColMatrix vn
= \ColMatrix vnb
}

\AddEquation{as ox as o v = v a12, matrix, 0 2 right-rows}
{
\ShowEq{matrix of maps n x n}
\CRcirc\RowMatrix vn
= \RowMatrix vnb
}

\AddEquation{as ox as o v = v a12, matrix, 1 2 right-rows}
{
\ShowEq{matrix of maps n x n}
\CRcirc\RowMatrix vn
= \RowMatrix vnb
}

\AddEquation{as ox as o v = v a12, matrix, 0 2 left-rows}
{
\ShowEq{matrix of maps n x n}
\CRcirc\RowMatrix vn
= b\RowMatrix vn
}

\AddEquation{as ox as o v = v a12, matrix, 1 2 left-rows}
{
\ShowEq{matrix of maps n x n}
\CRcirc\RowMatrix vn
= b\RowMatrix vn
}

\AddEq{as ox as o v = v a12, 0, cols}
{
(\Entry[s0]a{}ij\otimes\Entry[s1]a{}ij)\circ \aU vj
=(\Entry a0ij\otimes 1)\circ \aU vj
=\Entry a0ij\aU vj
}

\AddEq{as ox as o v = v a12, 1, rows}
{
(\Entry[s0]a{}ij\otimes\Entry[s1]a{}ij)\circ \aD vi
=(1\otimes\Entry a1ij)\circ \aD vi
=\aD vi\Entry a1ij
}

\AddEq{as ox as o v = v a12, 0, rows}
{
(\Entry[s0]a{}ij\otimes\Entry[s1]a{}ij)\circ \aD vi
=(\Entry a0ij\otimes 1)\circ \aD vi
=\Entry a0ij\aD vi
}

\AddEq{Eigenvalue of Matrix of Linear Map}
{
\AddIndex{}{eigenvalue}
\TwoColText
{
\ShowEq{def left}
\ShowEq{\DefMatrix}
\ShowDefinition{Eigenvalue of Matrix of Linear Map}
}
{
\ShowEq{def right}
\ShowEq{\DefMatrix}
\ShowDefinition{Eigenvalue of Matrix of Linear Map}
}

\TwoColText
{
\ShowEq{def left}
\ShowEq{\DefMatrix}
\ShowTheorem{Eigenvalue of Linear Map a ox a, 1}1
}
{
\ShowEq{def right}
\ShowEq{\DefMatrix}
\ShowTheorem{Eigenvalue of Linear Map a ox a, 1}0
}

\ShowEq{def left}
\ShowEq{\DefMatrix}
\ShowProof{Eigenvalue of Linear Map a ox a, 1}1

\ShowEq{def right}
\ShowEq{\DefMatrix}
\ShowProof{Eigenvalue of Linear Map a ox a, 1}0

\TwoColText
{
\ShowEq{def left}
\ShowEq{\DefMatrix}
\ShowTheorem{Eigenvalue of Linear Map a ox a, 2}0
}
{
\ShowEq{def right}
\ShowEq{\DefMatrix}
\ShowTheorem{Eigenvalue of Linear Map a ox a, 2}1
}

\ShowEq{def left}
\ShowEq{\DefMatrix}
\ShowProof{Eigenvalue of Linear Map a ox a, 2}0

\ShowEq{def right}
\ShowEq{\DefMatrix}
\ShowProof{Eigenvalue of Linear Map a ox a, 2}1

\TwoColText
{
\ShowEq{def left}
\ShowEq{\DefMatrix}
\ShowTheorem{Eigenvalue a ox a, c in AAA[b]}0
\ShowProof{Eigenvalue a ox a, c in AAA[b]}0{cv}
}
{
\ShowEq{def right}
\ShowEq{\DefMatrix}
\ShowTheorem{Eigenvalue a ox a, c in AAA[b]}1
\ShowProof{Eigenvalue a ox a, c in AAA[b]}1{vc}
}
}

\AddEq{eigenvector cv left-cols}
{
\[
cv=\ColMatrix{cv}n
\]
}

\AddEq{eigenvector cv right-cols}
{
\[
vc=
\begin{pmatrix}
\aU v1c\\...\\ \aU vnc
\end{pmatrix}
\]
}

\AddEq{eigenvector cv left-rows}
{
\[
cv=\RowMatrix{cv}n
\]
}

\AddEq{eigenvector cv right-rows}
{
\[
vc=
\begin{pmatrix}
\aD v1c&...& \aD vnc
\end{pmatrix}
\]
}

\AddEq[1]{Eigenvalue of Linear Map left-cols}
{
a\RCcirc #1=b#1
}

\AddEq[1]{Eigenvalue of Linear Map right-cols}
{
a\RCcirc #1=#1b
}

\AddEq[1]{Eigenvalue of Linear Map left-rows}
{
a\CRcirc #1=b#1
}

\AddEq[1]{Eigenvalue of Linear Map right-rows}
{
a\CRcirc #1=#1b
}

\AddEq{a=matrix of maps n x n}
{
a=
\ShowEq{matrix of maps n x n}
}

\AddEq{matrix of maps n x n}
{
\begin{pmatrix}
\Entry[s0]a{}11\otimes\Entry[s1]a{}11&...&\Entry[s0]a{}1n\otimes\Entry[s1]a{}1n\\
...&...&...\\
\Entry[s0]a{}n1\otimes\Entry[s1]a{}n1&...&\Entry[s0]a{}nn\otimes\Entry[s1]a{}nn
\end{pmatrix}
}

\AddEq{Left and Right Eigenvalues not equal}
{
\ShowRemark{Left and Right Eigenvalues not equal 0}

\TwoColText
{
\ShowEq{def left}
\ShowEq{\DefRow}
\ShowRemark{Left and Right Eigenvalues not equal}
}
{
\ShowEq{def right}
\ShowEq{\DefCol}
\ShowRemark{Left and Right Eigenvalues not equal}
}
}

\AddEquation{ai vi=0 left}
{
\begin{aligned}
&\,a(\gi 1)v(\gi 1)+ ...\\ +&\,a(\gi m-\gi 1)v(\gi m-\gi 1)\\ +&\,a(\gim)v(\gim)=0
\end{aligned}
}

\AddEquation{ai vi=0}
{
a(\gi 1)v(\gi 1)+ ...+a(\gi m-\gi 1)v(\gi m-\gi 1)+a(\gim)v(\gim)=0
}

\AddEquation{ai vi=0 right}
{
\begin{aligned}
&\,v(\gi 1)a(\gi 1)+ ...\\ +&\,v(\gi m-\gi 1)a(\gi m-\gi 1)\\ +&\,v(\gim)a(\gim)=0
\end{aligned}
}

\AddEquation{ai f vi=0}
{
a(\gi 1)(f\circ v(\gi 1)) + ... +a(\gi m-\gi 1)(f\circ v(\gi m-\gi 1))
+a(\gim)(f\circ v(\gim))=0
}

\AddEquation{ai f vi=0 left}
{
\begin{aligned}
&\,a(\gi 1)(f\circ v(\gi 1)) + ...\\ +&\,a(\gi m-\gi 1)(f\circ v(\gi m-\gi 1))
\\ +&\,a(\gim)(f\circ v(\gim))=0
\end{aligned}
}

\AddEquation{ai f vi=0 right}
{
\begin{aligned}
&\,(f\circ v(\gi 1))a(\gi 1)+ ...\\ +&\,(f\circ v(\gi m-\gi 1))a(\gi m-\gi 1)
\\ +&\,(f\circ v(\gim))a(\gim)=0
\end{aligned}
}

\AddEquation{ai di vi=0 left}
{
\begin{aligned}
&\,a(\gi 1)v(\gi 1)b(\gi 1) + ...
\\ +&\,a(\gi m-\gi 1)\\ *&\,v(\gi m-\gi 1)b(\gi m-\gi 1)
\\ +&\,a(\gim)v(\gi m)b(\gi m) =0
\end{aligned}
}

\AddEquation{ai di vi=0}
{
\begin{aligned}
&\,a(\gi 1)b(\gi 1)v(\gi 1) + ...
\\ +&\,a(\gi m-\gi 1)b(\gi m-\gi 1)v(\gi m-\gi 1)
+a(\gim)b(\gi m)v(\gi m) =0
\end{aligned}
}

\AddEquation{ai di vi=0 right}
{
\begin{aligned}
&\,b(\gi 1)v(\gi 1)a(\gi 1)+ ...
\\ +&\,b(\gi m-\gi 1)v(\gi m-\gi 1)\\ *&\,a(\gi m-\gi 1)
\\ +&\,b(\gi m)v(\gi m)a(\gim) =0
\end{aligned}
}

\AddEq{a1 ne 0}
{
$a(\gi 1)\ne 0$.
}

\AddEq{Corollary e c-ac=}
{
\begin{\CorollaryStyle}
\labelCorollary{e c-ac=c- eat c}
\ShowEq{ce c-ac c-=eat}
\ShowEq{e c-ac=c- eat c}
\end{\CorollaryStyle}
}

\AddEquation{U-*A*U*E=E*D rc-right}
{
\begin{aligned}
&\,u_2^{\RCInverse}\RCstar a_2\RCstar u_2\RCstar\aD[1]ei
\\ =&\,\aD[1]eib(\gii)
\end{aligned}
}

\AddEquation{U-*A*U*E=E*D rc-left}
{
\aU{e_1}i\RCstar u_2\RCstar a_2\RCstar u_2^{\RCInverse}=b(\gii)\aU{e_1}i
}

\AddEquation{U-*A*U*E=E*D cr-left}
{
\aD[1]ei\CRstar u_2\CRstar a_2\CRstar u_2^{\CRInverse}=b(\gii)\aD[1]ei
}

\AddEquation{U-*A*U*E=E*D cr-right}
{
u_2^{\CRInverse}\CRstar a_2\CRstar u_2\CRstar\aU{e_1}i=\aU{e_1}ib(\gii)
}

\AddEquation{A*U*E=U*E*D rc-right}
{
a_2\RCstar u_2\RCstar\aD[1]ei=u_2\RCstar\aD[1]eib(\gii)
}

\AddEquation{A*U*E=U*E*D rc-left}
{
\aU{e_1}i\RCstar u_2\RCstar a_2=b(\gii)\aU{e_1}i\RCstar u_2
}

\AddEquation{A*U*E=U*E*D cr-left}
{
\aD[1]ei\CRstar u_2\CRstar a_2=b(\gii)\aD[1]ei\CRstar u_2
}

\AddEquation{A*U*E=U*E*D cr-right}
{
a_2\CRstar u_2\CRstar\aU{e_1}i=u_2\CRstar\aU{e_1}ib(\gii)
}

\AddEquation{U*Ei=Ui rc-right}
{
u_2\RCstar\aD[1]ei=\aD[2]ui
}

\AddEquation{U*Ei=Ui rc-left}
{
\aU{e_1}i\RCstar u_2=\aU{u_2}i
}

\AddEquation{U*Ei=Ui cr-left}
{
\aD[1]ei\CRstar u_2=\aD[2]ui
}

\AddEquation{U*Ei=Ui cr-right}
{
u_2\CRstar\aU{e_1}i=\aU{u_2}i
}

\AddEquation{e1i=u2i*e2 left-cols}
{
\ShowEq{ARow u2i \Cols}e1i
=
\ShowEq{ARow u2i \Cols}u2i
\CRstar\Basis e_2
}

\AddEquation{e1i=u2i*e2 right-cols}
{
\ShowEq{ARow u2i \Cols}e1i
=
\Basis e_2\RCstar
\ShowEq{ARow u2i \Cols}u2i
}

\AddEquation{e1i=u2i*e2 left-rows}
{
\ShowEq{ARow u2i \Cols}e1i
=
\ShowEq{ARow u2i \Cols}u2i
\RCstar\Basis e_2
}

\AddEquation{e1i=u2i*e2 right-rows}
{
\ShowEq{ARow u2i \Cols}e1i
=
\Basis e_2\CRstar
\ShowEq{ARow u2i \Cols}u2i
}

\AddEq{a1-di En}
{
a_1-b(\gii)\aD En
}

\AddEq{e1ij=01 cols}
{
\Entry e1ji=\aUD{\delta}ji
}

\AddEq{e1ij=01 rows}
{
\Entry e1ij=\aUD{\delta}ij
}

\AddEq[2]{A*Ui=Ui di rc-right}
{
a_{#1}\RCstar\aD[{#1}{}]{#2}i=\aD[{#1}{}]{#2}ib(\gii)
}

\AddEq[2]{A*Ui=Ui di rc-left}
{
\aU{#2_{#1}}i\RCstar a_{#1}=b(\gii)\aU{#2_{#1}}i
}

\AddEq[2]{A*Ui=Ui di cr-right}
{
a_{#1}\CRstar\aU{#2_{#1}}i=\aU{#2_{#1}}ib(\gii)
}

\AddEq[2]{A*Ui=Ui di cr-left}
{
\aD[{#1}{}]{#2}i\CRstar a_{#1}=b(\gii)\aD[{#1}{}]{#2}i
}

\AddEq{symb coordinates of geometric object}
{
\symb{\mathcal O(V,W,\Basis e_V,w)}{coordinates of geometric object}{}
}

\AddEq{conjugate eigenvalue left-cols}
{
\[
cv\CRstar a_2=cb v=cb c^{-1}\,cv
\]
}

\AddEq{conjugate eigenvalue right-cols}
{
\[
a_2\RCstar vc=vb c=vc\,c^{-1}b c
\]
}

\AddEq{conjugate eigenvalue left-rows}
{
\[
cv\RCstar a_2=cb v=cb c^{-1}\,cv
\]
}

\AddEq{conjugate eigenvalue right-rows}
{
\[
a_2\CRstar vc=vb c=vc\,c^{-1}b c
\]
}

\AddEquation{Coefficient comutes with matrix left-cols}
{
b\aU vic=\aU vja_2^{}\aUD{}ijc=\aU vjca_2^{}\aUD{}ij
}

\AddEquation{Coefficient comutes with matrix right-cols}
{
c\aU vib=ca_2^{}\aUD{}ij\aU vj=\aUD aijc\aU vj
}

\AddEquation{Coefficient comutes with matrix left-rows}
{
b\aD vic=\aD vja_2^{}\aUD{}jic=\aD vjca_2^{}\aUD{}ji
}

\AddEquation{Coefficient comutes with matrix right-rows}
{
c\aD vib=ca_2^{}\aUD{}ji\aD vj=a_2^{}\aUD{}jic\aD vj
}

\AddEq{Vector A cols}
{
$\aD ai$, \iIg,
}

\AddEq{Vector A rows}
{
$\aU ai$, \iIg,
}

\AddEq[1]{AoxA linearly independent 1 cols}
{
$\aU bi\aU ci=0$, $\gii=\gi 1$, ..., $\gin$#1
}

\AddEq{AoxA linearly independent cols}
{
\[\aU bi\aD ai\aU ci=0\]
}

\AddEq[1]{AoxA linearly independent 1 rows}
{
$\aD bi\aD ci=0$, $\gii=\gi 1$, ..., $\gin$#1
}

\AddEq{AoxA linearly independent rows}
{
\[\aD bi\aU ai\aD ci=0\]
}

\AddEq{basis of AoxA module}
{
\symb{\Basis{e}}{Basis}{}
}

\AddEq{basis, AoxA module cols}
{
\[
\ShowSymbol{Basis}{}
=(\aD ei,\iIg)
\]
}

\AddEq{basis, AoxA module rows}
{
\[
\ShowSymbol{Basis}{}
=(\aU ei,\iIg)
\]
}

\AddEquation{def coordinates of geometric object, left-cols}
{
\begin{aligned}
&\,\ShowSymbol{coordinates of geometric object}{}
\\=&\,(w\CRstar F(G)^{\CRInverse},G\CRstar \eV[V])
\end{aligned}
}

\AddEquation{def coordinates of geometric object, right-cols}
{
\begin{aligned}
&\,\ShowSymbol{coordinates of geometric object}{}
\\=&\,(F(G)^{\RCInverse}\RCstar w,\eV[V]\RCstar G)
\end{aligned}
}

\AddEquation{def coordinates of geometric object, left-rows}
{
\begin{aligned}
&\,\ShowSymbol{coordinates of geometric object}{}
\\=&\,(w\RCstar F(G)^{\RCInverse},G\RCstar \eV[V])
\end{aligned}
}

\AddEquation{def coordinates of geometric object, right-rows}
{
\begin{aligned}
&\,\ShowSymbol{coordinates of geometric object}{}
\\=&\,(F(G)^{\CRInverse}\CRstar w,\eV[V]\CRstar G)
\end{aligned}
}

\AddEq[4]{geometric object representative, left-cols}
{
\Vector #1_{#2}=#3\CRstar e_{#4}
}

\AddEq[4]{geometric object representative, right-cols}
{
\Vector #1_{#2}=e_{#4}\RCstar #3
}

\AddEq[4]{geometric object representative, left-rows}
{
\Vector #1_{#2}=#3\RCstar e_{#4}
}

\AddEq[4]{geometric object representative, right-rows}
{
\Vector #1_{#2}=e_{#4}\CRstar #3
}

\AddEq{invariance principle 3, left-cols}
{
\[
\begin{aligned}
\Vector w'&=w'\CRstar e'_W\\
&=w\CRstar F(a)^{\CRInverse}\CRstar F(a)\CRstar e_W\\
&=w\CRstar e_W=\Vector w
\end{aligned}
\]
}

\AddEq{invariance principle 3, right-cols}
{
\[
\begin{aligned}
\Vector w'&=e'_W\RCstar w'\\
&=e_W\RCstar F(a)\RCstar F(a)^{\RCInverse}\RCstar w\\
&=e_W\RCstar w=\Vector w
\end{aligned}
\]
}

\AddEq{invariance principle 3, left-rows}
{
\[
\begin{aligned}
\Vector w'&=w'\RCstar e'_W\\
&=w\RCstar F(a)^{\RCInverse}\RCstar F(a)\RCstar e_W\\
&=w\RCstar e_W=\Vector w
\end{aligned}
\]
}

\AddEq{invariance principle 3, right-rows}
{
\[
\begin{aligned}
\Vector w'&=e'_W\CRstar w'\\
&=e_W\CRstar F(a)\CRstar F(a)^{\CRInverse}\CRstar w\\
&=e_W\CRstar w=\Vector w
\end{aligned}
\]
}

\AddEquation{coordinate matrix, W2, W1, left-cols}
{
\Basis e_{W2}=c^{\CRInverse}\CRstar \Basis e_{W1}
}

\AddEquation{coordinate matrix, W2, W1, right-cols}
{
\Basis e_{W2}=e_{W1}\RCstar \Basis c^{\RCInverse}
}

\AddEquation{coordinate matrix, W2, W1, left-rows}
{
\Basis e_{W2}=c^{\RCInverse}\RCstar \Basis e_{W1}
}

\AddEquation{coordinate matrix, W2, W1, right-rows}
{
\Basis e_{W2}=e_{W1}\CRstar \Basis c^{\CRInverse}
}

\AddEq{sum of geometric objects, 1}
{
\DrawEq[w1{w_1}W]{geometric object representative, \SideNS-\Cols}{}
\DrawEq[w2{w_2}W]{geometric object representative, \SideNS-\Cols}{}
}

\AddEq{sum of geometric objects, 2}
{
\DrawEq[w{}{(w_1+w_2)}W]{geometric object representative, \SideNS-\Cols}{}
}

\AddEq{product of geometric object and constant, 2, left}
{
\DrawEq[w2{(kw_1)}W]{geometric object representative, \SideNS-\Cols}{}
}

\AddEq{product of geometric object and constant, 2, right}
{
\DrawEq[w2{(w_1k)}W]{geometric object representative, \SideNS-\Cols}{}
}

\AddEq{product of geometric object and constant, 3, left}
{
\[\Vector w_2=k\Vector w_1\]
}

\AddEq{product of geometric object and constant, 3, right}
{
\[\Vector w_2=\Vector w_1k\]
}

\AddEq{sum of geometric objects, 3}
{
\[\Vector w=\Vector w_1+\Vector w_2\]
}

\AddEquation{representation of homomorphism relative different bases, 3, left-cols}
{
\Vector w=v\CRstar b\CRstar a_2\CRstar c^{\CRInverse}\CRstar e_{W1}
}

\AddEquation{representation of homomorphism relative different bases, 4, left-cols}
{
v\CRstar a_1=v\CRstar b\CRstar a_2\CRstar c^{\CRInverse}
}

\AddEquation{representation of homomorphism relative different bases, 3, right-cols}
{
\Vector w=e_{W1}\RCstar c^{\RCInverse}\RCstar a_2\RCstar b\RCstar v
}

\AddEquation{representation of homomorphism relative different bases, 4, right-cols}
{
v\CRstar a_1=c^{\RCInverse}\RCstar a_2\RCstar b\RCstar v
}

\AddEquation{representation of homomorphism relative different bases, 3, left-rows}
{
\Vector w=v\RCstar b\RCstar a_2\RCstar c^{\RCInverse}\RCstar e_{W1}
}

\AddEquation{representation of homomorphism relative different bases, 4, left-rows}
{
v\CRstar a_1=v\RCstar b\RCstar a_2\RCstar c^{\RCInverse}
}

\AddEquation{representation of homomorphism relative different bases, 3, right-rows}
{
\Vector w=e_{W1}\CRstar c^{\CRInverse}\CRstar a_2\CRstar b\CRstar v
}

\AddEquation{representation of homomorphism relative different bases, 4, right-rows}
{
v\CRstar a_1=c^{\CRInverse}\CRstar a_2\CRstar b\CRstar v
}

\AddEquation{representation of homomorphism relative different bases, 1, left-cols}
{
\Vector w=v\CRstar a_1\CRstar e_{W1}
}

\AddEquation{representation of homomorphism relative different bases, 2, left-cols}
{
\Vector w=v\RCstar b\CRstar a_2\CRstar e_{W2}
}

\AddEquation{representation of homomorphism relative different bases, 1, right-cols}
{
\Vector w=e_{W1}\RCstar a_1\RCstar v
}

\AddEquation{representation of homomorphism relative different bases, 2, right-cols}
{
\Vector w=e_{W2}\RCstar a_2\RCstar b\RCstar v
}

\AddEquation{representation of homomorphism relative different bases, 1, left-rows}
{
\Vector w=v\RCstar a_1\RCstar e_{W1}
}

\AddEquation{representation of homomorphism relative different bases, 2, left-rows}
{
\Vector w=v\CRstar b\RCstar a_2\RCstar e_{W2}
}

\AddEquation{representation of homomorphism relative different bases, 1, right-rows}
{
\Vector w=e_{W1}\CRstar a_1\CRstar v
}

\AddEquation{representation of homomorphism relative different bases, 2, right-rows}
{
\Vector w=e_{W2}\RCstar a_2\CRstar b\CRstar v
}

\AddEq{expansion of vector v, left-cols}
{
\[
\Vector v=v\CRstar e_{V1}=v\CRstar b\CRstar e_{V2}
\]
}

\AddEq{expansion of vector v, right-cols}
{
\[
\Vector v=e_{V1}\CRstar v=e_{V2}\CRstar b\CRstar v
\]
}

\AddEq{expansion of vector v, left-rows}
{
\[
\Vector v=v\RCstar e_{V1}=v\RCstar b\RCstar e_{V2}
\]
}

\AddEq{expansion of vector v, right-rows}
{
\[
\Vector v=e_{V1}\RCstar v=e_{V2}\RCstar b\RCstar v
\]
}

\AddEq[1]{representation of homomorphism relative different bases, left-cols}
{
a_1=b\CRstar a_2\CRstar #1^{\CRInverse}
}

\AddEq[1]{representation of homomorphism relative different bases, right-cols}
{
a_1=#1^{\RCInverse}\RCstar a_2\RCstar b
}

\AddEq[1]{representation of homomorphism relative different bases, left-rows}
{
a_1=b\RCstar a_2\RCstar #1^{\RCInverse}
}

\AddEq[1]{representation of homomorphism relative different bases, right-rows}
{
a_1=#1^{\CRInverse}\CRstar a_2\CRstar b
}

\AddEq[2]{coordinate matrix, f, g, left-cols}
{
\Basis e_{#1 1}=#2\CRstar\Basis e_{#1 2}
}

\AddEq[2]{coordinate matrix, f, g, right-cols}
{
\Basis e_{#1 1}=\Basis e_{#1 2}\RCstar #2
}

\AddEq[2]{coordinate matrix, f, g, left-rows}
{
\Basis e_{#1 1}=#2\RCstar\Basis e_{#1 2}
}

\AddEq[2]{coordinate matrix, f, g, right-rows}
{
\Basis e_{#1 1}=\Basis e_{#1 2}\CRstar #2
}

\AddEq{a*b, left-cols}
{
\gdef\TheProduct{\ensuremath{a\CRstar b}}%
}

\AddEq{a*b, right-cols}
{
\gdef\TheProduct{\ensuremath{b\RCstar a}}%
}

\AddEq{a*b, left-rows}
{
\gdef\TheProduct{\ensuremath{a\RCstar b}}%
}

\AddEq{a*b, right-rows}
{
\gdef\TheProduct{\ensuremath{b\CRstar a}}%
}

\AddEq{two transformations on basis manifold, left-cols}
{
\[
e\CRstar g_1=e\CRstar g_2
\]
}

\AddEq{two transformations on basis manifold, right-cols}
{
\[
g_1\RCstar e=g_2\RCstar e
\]
}

\AddEq{two transformations on basis manifold, left-rows}
{
\[
e\RCstar g_1=e\RCstar g_2
\]
}

\AddEq{two transformations on basis manifold, right-rows}
{
\[
g_1\CRstar e=g_2\CRstar e
\]
}

\AddEq[3]{basis manifold of V, left-cols}
{
\ensuremath{\Basis {#1}\CRstar #2(V)}#3
}

\AddEq[3]{basis manifold of V, right-cols}
{
\ensuremath{#2(V)\RCstar \Basis {#1}}#3
}

\AddEq[3]{basis manifold of V, left-rows}
{
\ensuremath{\Basis {#1}\RCstar #2(V)}#3
}

\AddEq[3]{basis manifold of V, right-rows}
{
\ensuremath{#2(V)\CRstar \Basis {#1}}#3
}

\AddEq{basis manifold of vector space, left-cols}
{
\symb{\Basis e\CRstar G(V)}{basis manifold}1
}

\AddEq{basis manifold of vector space, right-cols}
{
\symb{G(V)\RCstar \Basis e}{basis manifold}1
}

\AddEq{basis manifold of vector space, left-rows}
{
\symb{\Basis e\RCstar G(V)}{basis manifold}1
}

\AddEq{basis manifold of vector space, right-rows}
{
\symb{G(V)\CRstar \Basis e}{basis manifold}1
}

\AddEq{Fg in GL}
{
$F(g)\in GL(W_*)$
}

\AddEq[1]{coordinate matrix of basis and passive transformation, left-cols}
{
\[
\aD{\Vector e'}i=\aD {#1}i\CRstar\Vector e
\]
}

\AddEq[1]{coordinate matrix of basis and passive transformation, right-cols}
{
\[
\aD{\Vector e'}i=\Vector e\RCstar\aD {#1}i
\]
}

\AddEq[1]{coordinate matrix of basis and passive transformation, left-rows}
{
\[
\aU{\Vector e'}i=\aU {#1}i\RCstar\Vector e
\]
}

\AddEq[1]{coordinate matrix of basis and passive transformation, right-rows}
{
\[
\aU{\Vector e'}i=\Vector e\CRstar\aU {#1}i
\]
}

\AddEq{coordinate matrix of basis and passive transformation, cols}
{
\[
\aD {e'}i=\aD ai
\]
}

\AddEq{coordinate matrix of basis and passive transformation, rows}
{
\[
\aU {e'}i=\aU ai
\]
}

\AddEq[1]{passive transformation e->e', left-cols}
{
\Basis e'_{#1}=g\CRstar \Basis e_{#1}
}

\AddEq[1]{passive transformation e->e', left-rows}
{
\Basis e'_{#1}=g\RCstar \Basis e_{#1}
}

\AddEq[1]{passive transformation e->e', right-cols}
{
\Basis e'_{#1}=\Basis e_{#1}\RCstar g
}

\AddEq[1]{passive transformation e->e', right-rows}
{
\Basis e'_{#1}=\Basis e_{#1}\CRstar g
}

\AddEquation{passive transformation e->e, left-cols}
{
\Basis e=\aD En\CRstar \Basis e
}

\AddEquation{passive transformation e->e, left-rows}
{
\Basis e=\aD En\RCstar \Basis e
}

\AddEquation{passive transformation e->e, right-cols}
{
\Basis e=\Basis e\RCstar \aD En
}

\AddEquation{passive transformation e->e, right-rows}
{
\Basis e=\Basis e\CRstar \aD En
}

\AddEq{homomorphism on A basis, left-cols}
{
\[
a=e^{\CRInverse}\CRstar e'
\]
}

\AddEq{homomorphism on A basis, right-cols}
{
\[
a=e'\RCstar e^{\RCInverse}
\]
}

\AddEq{homomorphism on A basis, left-rows}
{
\[
a=e^{\RCInverse}\RCstar e'
\]
}

\AddEq{homomorphism on A basis, right-rows}
{
\[
a=e'\CRstar e^{\CRInverse}
\]
}

\AddEq{passive transformation symbol, left-cols}
{
$a\CRstar \Basis e$.
}

\AddEq{passive transformation symbol, right-cols}
{
$\Basis e\RCstar a$.
}

\AddEq{passive transformation symbol, left-rows}
{
$a\RCstar \Basis e$.
}

\AddEq{passive transformation symbol, right-rows}
{
$\Basis e\CRstar a$.
}

\AddEq[1]{active transformation, vector space, left-cols}
{
$\Basis e\CRstar a$#1
}

\AddEq[1]{active transformation, vector space, right-cols}
{
$a\RCstar\Basis e$#1
}

\AddEq[1]{active transformation, vector space, left-rows}
{
$\Basis e\RCstar a$#1
}

\AddEq[1]{active transformation, vector space, right-rows}
{
$a\CRstar\Basis e$#1
}

\AddEq{active transformation ae x=a ex, left-cols}
{
v\CRstar\EqText{\Basis e\CRstar a}=\EqText{v\CRstar\Basis e}\CRstar a
}

\AddEq{active transformation ae x=a ex, right-cols}
{
\EqText{a\RCstar\Basis e}\RCstar v=a\RCstar\EqText{\Basis e\RCstar v}
}

\AddEq{active transformation ae x=a ex, left-rows}
{
v\RCstar\EqText{\Basis e\RCstar a}=\EqText{v\RCstar\Basis e}\RCstar a
}

\AddEq{active transformation ae x=a ex, right-rows}
{
\EqText{a\CRstar\Basis e }\CRstar v=a\CRstar\EqText{\Basis e \CRstar v}
}

\AddEq{active transformation ae x=a ex 1, left-cols}
{
$v\CRstar\Basis e$
}

\AddEq{active transformation ae x=a ex 1, right-cols}
{
$\Basis e\RCstar v$
}

\AddEq{active transformation ae x=a ex 1, left-rows}
{
$v\RCstar\Basis e$
}

\AddEq{active transformation ae x=a ex 1, right-rows}
{
$\Basis e \CRstar v$
}

\AddEq{v*g, left-cols}
{
$v\CRstar g$.
}

\AddEq{v*g, right-cols}
{
$g\RCstar v$.
}

\AddEq{v*g, left-rows}
{
$v\RCstar g$.
}

\AddEq{v*g, right-rows}
{
$g\CRstar v$.
}

\AddEq{active transformations, vector space, 2, left-cols}
{
\[
\aU vi=\aU vj\aUD aij
\]
}

\AddEq{active transformations, vector space, 2, right-cols}
{
\[
\aU vi=\aUD aij\aU vj
\]
}

\AddEq{active transformations, vector space, 2, left-rows}
{
\[
\aD vi=\aD vj\aUD aji
\]
}

\AddEq{active transformations, vector space, 2, right-rows}
{
\[
\aD vi=\aUD aji\aD vj
\]
}

\AddEq{ai=delta ik, cols}
{
$\aU vi=\aUD{\delta}ik$
}

\AddEq{ai=delta ik, rows}
{
$\aD vi=\aUD{\delta}ki$
}

\AddEq{identity transformation, vector space, 1, cols}
{
\[
\aUD{\delta}ik=\aUD aik
\]
}

\AddEq{identity transformation, vector space, 1, rows}
{
\[
\aUD{\delta}ki=\aUD aki
\]
}

\AddEquation{identity transformation, vector space, left-cols}
{
\aUD{\delta}ik=\aUD{\delta}jk\aUD aij
}

\AddEquation{identity transformation, vector space, right-cols}
{
\aUD{\delta}ik=\aUD aij\aUD{\delta}jk
}

\AddEquation{identity transformation, vector space, left-rows}
{
\aUD{\delta}ki=\aUD{\delta}kj\aUD aji
}

\AddEquation{identity transformation, vector space, right-rows}
{
\aUD{\delta}ik=\aUD aji\aUD{\delta}kj
}

\AddEq{automorphism, vector space, 1, left-cols}
{
\aD{e'}i=\aD ei\CRstar a
}

\AddEq{automorphism, vector space, 1, right-cols}
{
\aD{e'}i=a\RCstar \aD ei
}

\AddEq{automorphism, vector space, 1, left-rows}
{
\aU{e'}i=\aU ei\RCstar a
}

\AddEq{automorphism, vector space, 1, right-rows}
{
\aU{e'}i=a\CRstar \aU ei
}

\AddEquation{b(av)=a(bv) left}
{
\begin{aligned}
\RedText{(ba)v}&=\BlueText{b(av)=\Vector f\circ(av)}
\\ &=\BlueText{a(\Vector f\circ v)=a(bv)}
\\ &=\RedText{(ab)v}
\end{aligned}
}

\AddEquation{b(av)=a(bv) right}
{
\begin{aligned}
\RedText{v(ab)}&=\BlueText{(va)b=\Vector f\circ(va)}
\\ &=\BlueText{(\Vector f\circ v)a=(vb)a}
\\ &=\RedText{v(ba)}
\end{aligned}
}

\AddEq{p,q in A, v,w in V}
{
$p$, $q \in A$, $v$, $w \in V$.
}

\AddEquation{fov=bv left}
{
\Vector f\circ v=bv
}

\AddEquation{fov=bv right}
{
\Vector f\circ v=vb
}

\AddEquation{fovi=di vi left}
{
f\circ v(\gi i)=v(\gii)b(\gii)
}

\AddEquation{fovi=di vi right}
{
f\circ v(\gi i)=b(\gii)v(\gii)
}

\AddEquation{fovi=di vi}
{
f\circ v(\gi i)=b(\gii)v(\gii)
}

\AddEq{basis vector cols}
{
$\aD ei$
}

\AddEq{basis vector rows}
{
$\aU ei$
}

\AddEquation{automorphism, vector space, 2, left-cols}
{
\lambda\CRstar e'=0
}

\AddEquation{automorphism, vector space, 2, right-cols}
{
e'\RCstar\lambda =0
}

\AddEquation{automorphism, vector space, 2, left-rows}
{
\lambda\RCstar e'=0
}

\AddEquation{automorphism, vector space, 2, right-rows}
{
e'\CRstar\lambda =0
}

\AddEq{automorphism, vector space, 3, left-cols}
{
\[
\lambda\CRstar e'\CRstar a^{\CRInverse}
=\lambda\CRstar e=0
\]
}

\AddEq{automorphism, vector space, 3, right-cols}
{
\[
a^{\CRInverse}\RCstar e' \RCstar\lambda
=e\RCstar\lambda =0
\]
}

\AddEq{automorphism, vector space, 3, left-rows}
{
\[
\lambda\RCstar e'\RCstar a^{\CRInverse}
=\lambda\RCstar e=0
\]
}

\AddEq{automorphism, vector space, 3, right-rows}
{
\[
a^{\CRInverse}\CRstar e' \CRstar\lambda
=e\CRstar\lambda =0
\]
}

\AddEq[1]{vector of basis cols}
{
\ensuremath{\aD {#1}i}
}

\AddEq[1]{vector of basis rows}
{
\ensuremath{\aU {#1}i}
}

\AddEq[3]{ARow u2i cols}
{
\ensuremath{\aD[#2]{#1}{#3}}
}

\AddEq[3]{ARow u2i rows}
{
\ensuremath{\aU {#1_{#2}}{#3}}
}

\AddEq{Automorphisms of vector space, cr-rows}
{
\[
\begin{aligned}
v'&=f\CRstar v\\
v''=g\CRstar v'&=g\CRstar f\CRstar v
\end{aligned}
\]
}

\AddEq{Automorphisms of vector space, rc-rows}
{
\[
\begin{aligned}
v'&=v\RCstar f\\
v''=v'\RCstar g&=v\RCstar f\RCstar g
\end{aligned}
\]
}

\AddEq{Automorphisms of vector space, cr-cols}
{
\[
\begin{aligned}
v'&=v\CRstar f\\
v''=v'\CRstar g&=v\CRstar f\CRstar g
\end{aligned}
\]
}

\AddEq{Automorphisms of vector space, rc-cols}
{
\[
\begin{aligned}
v'&=f\RCstar v\\
v''=g\RCstar v'&=g\RCstar f\RCstar v
\end{aligned}
\]
}

\AddEq{basis e2 of V cols}
{
\ECol 2j, $\gi j\in\gi J$,
}

\AddEq{basis e2 of V rows}
{
\ERow 2j, $\gi j\in\gi J$,
}

\AddEq{basis e2 of V lambda}
{
\lambda=0
}

\AddEq{basis e2 relative e1 left-cols}
{
\[
\ECol 2j=\aD aj\CRstar e_1
\]
}

\AddEq{basis e2 relative e1 right-cols}
{
\[
\ECol 2j=e_1\RCstar \aD aj
\]
}

\AddEq{basis e2 relative e1 right-rows}
{
\[
\ERow 2j=e_1\CRstar \aU aj
\]
}

\AddEq{basis e2 relative e1 left-rows}
{
\[
\ERow 2j=\aU aj\RCstar e_1
\]
}

\AddEquation{basis e2 relative e1, lambda, right-cols}
{
e_2\RCstar \lambda
= e_1\RCstar a\RCstar\lambda=0
}

\AddEquation{basis e2 relative e1, lambda, left-cols}
{
\lambda\CRstar e_2
=\lambda\CRstar a\CRstar e_1=0
}

\AddEquation{basis e2 relative e1, lambda, right-rows}
{
e_2\CRstar \lambda
= e_1\CRstar a\CRstar\lambda=0
}

\AddEquation{basis e2 relative e1, lambda, left-rows}
{
\lambda\RCstar e_2
=\lambda\RCstar a\RCstar e_1=0
}

\AddEquation{basis e2 relative e1, lambda=0, right-cols}
{
a\RCstar\lambda=0
}

\AddEquation{basis e2 relative e1, lambda=0, left-cols}
{
\lambda\CRstar a=0
}

\AddEquation{basis e2 relative e1, lambda=0, right-rows}
{
a\CRstar\lambda=0
}

\AddEquation{basis e2 relative e1, lambda=0, left-rows}
{
\lambda\RCstar a=0
}

\AddEquation{avi=bvi left-cols}
{
a\aU vi=b\aU vi
}

\AddEquation{avi=bvi right-cols}
{
\aU via=\aU vib
}

\AddEquation{avi=bvi left-rows}
{
a\aD vi=b\aD vi
}

\AddEquation{avi=bvi right-rows}
{
\aD via=\aD vib
}

\AddEq{Rank a<m cr}
{
$\CRRank a\le\gi m$
}

\AddEq{Rank a<m rc}
{
$\RCRank a\le\gi m$
}

\AddEq{av=bv, v left}
{
\forall v\in V,av=bv\ \ \ \ a,b\in A
}

\AddEq{av=bv, v right}
{
\forall v\in V,va=vb\ \ \ \ a,b\in A
}

\AddEq[1]{w=v.rc.f}
{
w_{#1}=f_{#1}\RCstar v_{#1}
}

\AddEq[1]{w=v.cr.f}
{
w_{#1}=v_{#1}\CRstar f_{#1}
}

\AddEq[1]{v2 f2=v2 a f1 a- left-cols}
{
v_2\CRstar f_2=v_2\CRstar #1\CRstar f_1\CRstar #1^{\CRInverse}
}

\AddEq[1]{v2 f2=v2 a f1 a- right-cols}
{
f_2\RCstar v_2=#1^{\RCInverse}\RCstar f_1\RCstar #1\RCstar v_2
}

\AddEq[1]{v2 f2=v2 a f1 a- left-rows}
{
v_2\RCstar f_2=v_2\RCstar #1\RCstar f_1\RCstar #1^{\RCInverse}
}

\AddEq[1]{v2 f2=v2 a f1 a- right-rows}
{
f_2\CRstar v_2=#1^{\CRInverse}\CRstar f_1\CRstar #1\CRstar v_2
}

\AddEq[1]{w2=...v2 a f1 a- left-cols}
{
w_2=v_1\CRstar f_1=v_2\CRstar #1\CRstar f_1\CRstar #1^{\CRInverse}
}

\AddEq[1]{w2=...v2 a f1 a- right-cols}
{
w_2=f_1\RCstar v_1=#1^{\RCInverse}\RCstar f_1\RCstar #1\RCstar v_2
}

\AddEq[1]{w2=...v2 a f1 a- left-rows}
{
w_2=v_1\RCstar f_1=v_2\RCstar #1\RCstar f_1\RCstar #1^{\RCInverse}
}

\AddEq[1]{w2=...v2 a f1 a- right-rows}
{
w_2=f_1\CRstar v_1=#1^{\CRInverse}\CRstar f_1\CRstar #1\CRstar v_2
}

\AddEq[1]{w2=...v2 a f1 left-cols}
{
w_2\CRstar #1=v_1\CRstar f_1=v_2\CRstar #1\CRstar f_1
}

\AddEq[1]{w2=...v2 a f1 right-cols}
{
#1\RCstar w_2=f_1\RCstar v_1=f_1\RCstar #1\RCstar v_2
}

\AddEq[1]{w2=...v2 a f1 left-rows}
{
w_2\RCstar #1=v_1\RCstar f_1=v_2\RCstar #1\RCstar f_1
}

\AddEq[1]{w2=...v2 a f1 right-rows}
{
#1\CRstar w_2=f_1\CRstar v_1=f_1\CRstar #1\CRstar v_2
}

\AddEq[4]{f2=a f1 a-}
{
#1_2=
\ShowEq{a f1 a- #3-#4}{#1}{#2}
}

\AddEq[2]{a f1 a- left-cols}
{
#2\CRstar #1_1\CRstar #2^{\CRInverse}
}

\AddEq[2]{a f1 a- right-cols}
{
#2^{\RCInverse}\RCstar #1_1\RCstar #2
}

\AddEq[2]{a f1 a- left-rows}
{
#2\RCstar #1_1\RCstar #2^{\RCInverse}
}

\AddEq[2]{a f1 a- right-rows}
{
#2^{\CRInverse}\CRstar #1_1\CRstar #2
}

\AddEq[1]{f'=g f g- left-cols}
{
f'_{#1}=g\CRstar f_{#1}\CRstar g^{\CRInverse}
}

\AddEq[1]{f'=g f g- right-cols}
{
f'_{#1}=g^{\RCInverse}\RCstar f_{#1}\RCstar g
}

\AddEq[1]{f'=g f g- left-rows}
{
f'_{#1}=g\RCstar f_{#1}\RCstar g^{\RCInverse}
}

\AddEq[1]{f'=g f g- right-rows}
{
f'_{#1}=g^{\CRInverse}\CRstar f_{#1}\CRstar g
}

\AddEquation{f1+f2=g.g- left-cols}
{
\begin{aligned}
f'&=g\CRstar f\CRstar g^{\CRInverse}
\\ &=g\CRstar (f_1+f_2)\CRstar g^{\CRInverse}
\\ &=g\CRstar f_1\CRstar g^{\CRInverse}\\ &+g\CRstar f_2\CRstar g^{\CRInverse}
\\ &=f'_1+f'_2
\end{aligned}
}

\AddEquation{f1+f2=g.g- right-cols}
{
\begin{aligned}
f'&=g^{\RCInverse}\RCstar f\RCstar g
\\ &=g^{\RCInverse}\RCstar (f_1+f_2)\RCstar g
\\ &=g^{\RCInverse}\RCstar f_1\RCstar g\\ &+g^{\RCInverse}\RCstar f_2\RCstar g
\\ &=f'_1+f'_2
\end{aligned}
}

\AddEquation{f1+f2=g.g- left-rows}
{
\begin{aligned}
f'&=g\RCstar f\RCstar g^{\RCInverse}
\\ &=g\RCstar (f_1+f_2)\RCstar g^{\RCInverse}
\\ &=g\RCstar f_1\RCstar g^{\RCInverse}\\ &+g\RCstar f_2\RCstar g^{\RCInverse}
\\ &=f'_1+f'_2
\end{aligned}
}

\AddEquation{f1+f2=g.g- right-rows}
{
\begin{aligned}
f'&=g^{\CRInverse}\CRstar f\CRstar g
\\ &=g^{\CRInverse}\CRstar (f_1+f_2)\CRstar g
\\ &=g^{\CRInverse}\CRstar f_1\CRstar g\\ &+g^{\CRInverse}\CRstar f_2\CRstar g
\\ &=f'_1+f'_2
\end{aligned}
}

\AddEquation{f1*f2=g.g- left-cols}
{
\begin{aligned}
f'&=g\CRstar f\CRstar g^{\CRInverse}
\\ &=g\CRstar f_1\CRstar f_2\CRstar g^{\CRInverse}
\\ &=g\CRstar f_1\CRstar g^{\CRInverse}\\ &\CRstar g\CRstar f_2\CRstar g^{\CRInverse}
\\ &=f'_1\CRstar f'_2
\end{aligned}
}

\AddEquation{f1*f2=g.g- right-cols}
{
\begin{aligned}
f'&=g^{\RCInverse}\RCstar f\RCstar g
\\ &=g^{\RCInverse}\RCstar f_1\RCstar f_2\RCstar g
\\ &=g^{\RCInverse}\RCstar f_1\RCstar g\\ &\RCstar g^{\RCInverse}\RCstar f_2\RCstar g
\\ &=f'_1\RCstar f'_2
\end{aligned}
}

\AddEquation{f1*f2=g.g- left-rows}
{
\begin{aligned}
f'&=g\RCstar f\RCstar g^{\RCInverse}
\\ &=g\RCstar f_1\RCstar f_2\RCstar g^{\RCInverse}
\\ &=g\RCstar f_1\RCstar g^{\RCInverse}\\ &\RCstar g\RCstar f_2\RCstar g^{\RCInverse}
\\ &=f'_1\RCstar f'_2
\end{aligned}
}

\AddEquation{f1*f2=g.g- right-rows}
{
\begin{aligned}
f'&=g^{\CRInverse}\CRstar f\CRstar g
\\ &=g^{\CRInverse}\CRstar f_1\CRstar f_2\CRstar g
\\ &=g^{\CRInverse}\CRstar f_1\CRstar g\\ &\CRstar g^{\CRInverse}\CRstar f_2\CRstar g
\\ &=f'_1\CRstar f'_2
\end{aligned}
}

\AddEq{f1*f2=g.g-}
{
\eqRef{f=f1*f2 endo \SideNS-\Cols}{\Product},
\eqRef{f'=g f g- \SideNS-\Cols}{f*},
\eqRef{f'=g f g- \SideNS-\Cols}{1*},
\eqRef{f'=g f g- \SideNS-\Cols}{2*}.
}

\AddEq{f1+f2=g.g-}
{
\eqRef{f=f1+f2 endo}{\SideNS-\Cols},
\eqRef{f'=g f g- \SideNS-\Cols}f,
\eqRef{f'=g f g- \SideNS-\Cols}1,
\eqRef{f'=g f g- \SideNS-\Cols}2.
}

\AddEq[2]{Bases e12}
{
\eV[#1 1], \eV[#1 2]#2
}

\AddEq{A:V->W}
{
a:V\rightarrow W
}

\AddEq[4]{(f-ae)v cr-cols}
{
{#4}\CRstar(\ShowEq{(f-ae)v matrix}{#1}{}{#3}{#2})=0
}

\AddEq[4]{(f-ae)v rc-cols}
{
(\ShowEq{(f-ae)v matrix}{#1}{}{#3}{#2})\RCstar {#4}=0
}

\AddEq[4]{(f-ae)v cr-rows}
{
(\ShowEq{(f-ae)v matrix}{#1}{}{#3}{#2})\CRstar {#4}=0
}

\AddEq[4]{(f-ae)v rc-rows}
{
{#4}\RCstar(\ShowEq{(f-ae)v matrix}{#1}{}{#3}{#2})=0
}

\AddEquation{(f-bEn)v cr-cols}
{
v_1\CRstar(\ShowEq{f-bEn left}1)=0
}

\AddEquation{(f-bEn)v rc-cols}
{
(\ShowEq{f-bEn right}1)\RCstar v_1=0
}

\AddEquation{(f-bEn)v cr-rows}
{
(\ShowEq{f-bEn right}1)\CRstar v_1=0
}

\AddEquation{(f-bEn)v rc-rows}
{
v_1\RCstar(\ShowEq{f-bEn left}1)=0
}

\AddEquation{(f-bEn)v2 cr-cols}
{
v_2\CRstar(f_2-\ShowEq{ga*g- \SideNS-\Cols}bg)=0
}

\AddEquation{(f-bEn)v2 rc-cols}
{
(f_2-\ShowEq{ga*g- \SideNS-\Cols}bg)\RCstar v_2=0
}

\AddEquation{(f-bEn)v2 cr-rows}
{
(f_2-\ShowEq{ga*g- \SideNS-\Cols}bg)\CRstar v_2=0
}

\AddEquation{(f-bEn)v2 rc-rows}
{
v_2\RCstar(f_2-\ShowEq{ga*g- \SideNS-\Cols}bg)=0
}

\AddEq[4]{(f-ae)v matrix}
{
\ensuremath{#1_{#2}-\ShowEq{ga*g- \SideNS-\Cols}{#3}{#4}}
}

\AddEq{bg.rc.g-}
{
\[
\begin{aligned}
\ShowEq{ga*g- left-rows}bg
&=g\RCstar (bg^{\RCInverse})
\\ &=(g^{\RCInverse})^{\RCInverse}\RCstar (bg^{\RCInverse})
\end{aligned}
\]
}

\AddEquation{gb rc g-=b}
{
\ShowEq{ga*g- right-cols}bg
=(g^{\RCInverse}\RCstar  g)b=\aD Enb
}

\AddEquation{gb cr g-=b}
{
\ShowEq{ga*g- left-cols}bg
=b(g\CRstar g^{\CRInverse})=b\aD En
}

\AddEquation{gij in ZA}
{
\aUD gij\in Z(A)\ \ \ \,\gii=\gi 1, ..., \gin\ \ \ \,\gij=\gi 1, ..., \gin
}

\AddEq{bg.cr.g-}
{
\[
\begin{aligned}
\ShowEq{ga*g- right-rows}bg
&=(g^{\CRInverse} b)\CRstar g
\\ &=(g^{\CRInverse} b)\CRstar (g^{\CRInverse})^{\CRInverse}
\end{aligned}
\]
}

\AddEq{rc-eigencols(f,g)}
{
f\RCstar v=\ShowEq{ga*g- \SideNS-\Cols}bg\RCstar v
}

\AddEq{cr-eigencols(f,g)}
{
v\CRstar f=v\CRstar \ShowEq{ga*g- \SideNS-\Cols}bg
}

\AddEq{rc-eigenrows(f,g)}
{
v\RCstar f=v\RCstar \ShowEq{ga*g- \SideNS-\Cols}bg
}

\AddEq{cr-eigenrows(f,g)}
{
f\CRstar v=\ShowEq{ga*g- \SideNS-\Cols}bg\CRstar v
}

\AddEq[1]{pair of matrices rc-column}
{
$(f,g)$#1
}

\AddEq[1]{pair of matrices cr-column}
{
$(f,g)$#1
}

\AddEq[1]{pair of matrices rc-row}
{
$(f,g^{\RCInverse})$#1
}

\AddEq[1]{pair of matrices cr-row}
{
$(f,g^{\CRInverse})$#1
}

\AddEq{rc-eigencols}
{
f\RCstar v=bv
}

\AddEq{rc-eigenrows}
{
v\RCstar f=vb
}

\AddEq{cr-eigencols}
{
v\CRstar f=vb
}

\AddEq{cr-eigenrows}
{
f\CRstar v=bv
}

\AddEq{gi in I, gj in J}
{
\[
\gii\in\giI,\ \gij\in\giJ
\]
}

\AddEquation{rc-det ij aIJ=0}
{
\RCdet ij\,\aUD{(a-bE)}IJ=0
}

\AddEquation{cr-det ij aIJ=0}
{
\CRdet ij\,\aUD{(a-bE)}IJ=0
}

\AddEq{rc-det ij a=0}
{
\RCdet ij\,(a-bE)=0
}

\AddEq{cr-det ij a=0}
{
\CRdet ij\,(a-bE)=0
}

\AddEq{f-ae->f-be}
{
\[
\begin{aligned}
&\, \ShowEq{(f-ae)v matrix}f2bg
\\ =&\,\ShowEq{a f1 a- \SideNS-\Cols}fg
-\ShowEq{ga*g- \SideNS-\Cols}bg
\\ =&\,
\ShowEq{g(f-bEn)g \SideNS-\Cols}
\end{aligned}
\]
}

\AddEq{f-ae->f-be left-cols}
{
\[
\begin{aligned}
&\, v_2\CRstar(\ShowEq{(f-ae)v matrix}f2bg)
\\ =&\,
v_2\CRstar(\ShowEq{a f1 a- \SideNS-\Cols}fg
-\ShowEq{ga*g- \SideNS-\Cols}bg)
\\ =&\,
\ShowEq{v1g- \SideNS-\Cols}v1g{}\CRstar
\ShowEq{g(f-bEn)g \SideNS-\Cols}
\end{aligned}
\]
}

\AddEq{f-ae->f-be right-cols}
{
\[
\begin{aligned}
&\,(\ShowEq{(f-ae)v matrix}f2bg)\RCstar v_2
\\ =&\,
(\ShowEq{a f1 a- \SideNS-\Cols}fg
-\ShowEq{ga*g- \SideNS-\Cols}bg)\RCstar v_2
\\ =&\,
\ShowEq{g(f-bEn)g \SideNS-\Cols}\RCstar
\ShowEq{v1g- \SideNS-\Cols}v1g{}
\end{aligned}
\]
}

\AddEq{f-ae->f-be left-rows}
{
\[
\begin{aligned}
&\, v_2\RCstar(\ShowEq{(f-ae)v matrix}f2bg)
\\ =&\,
v_2\RCstar(\ShowEq{a f1 a- \SideNS-\Cols}fg
-\ShowEq{ga*g- \SideNS-\Cols}bg)
\\ =&\,
\ShowEq{v1g- \SideNS-\Cols}v1g{}\RCstar
\ShowEq{g(f-bEn)g \SideNS-\Cols}
\end{aligned}
\]
}

\AddEq{f-ae->f-be right-rows}
{
\[
\begin{aligned}
&\,(\ShowEq{(f-ae)v matrix}f2bg)\CRstar v_2
\\ =&\,
(\ShowEq{a f1 a- \SideNS-\Cols}fg
-\ShowEq{ga*g- \SideNS-\Cols}bg)\CRstar v_2
\\ =&\,
\ShowEq{g(f-bEn)g \SideNS-\Cols}\CRstar
\ShowEq{v1g- \SideNS-\Cols}v1g{}
\end{aligned}
\]
}

\AddEq{rc-det ij f-bg IJ=0}
{
\[
\RCdet ij\,\aUD{(\ShowEq{(f-ae)v matrix}f{}bg)}IJ=0
\]
\[
\gii\in\giI,\ \gij\in\giJ
\]
}

\AddEq{cr-det ij f-bg IJ=0}
{
\[
\CRdet ij\,\aUD{(\ShowEq{(f-ae)v matrix}f{}bg)}IJ=0
\]
\[
\gii\in\giI,\ \gij\in\giJ
\]
}

\AddEq{rc-det ij f-bg =0}
{
\RCdet ij\,(\ShowEq{(f-ae)v matrix}f{}bg)=0
}

\AddEq{cr-det ij f-bg =0}
{
\CRdet ij\,(\ShowEq{(f-ae)v matrix}f{}bg)=0
}

\AddEq{rc-rank a=k<n}
{
\[\RCstar\rank a=\gik<\gin\]
}

\AddEq{cr-rank a=k<n}
{
\[\CRstar\rank a=\gik<\gin\]
}

\AddEquation{rc-eigencols=0 fg}
{
(f-\ShowEq{ga*g- \SideNS-\Cols}bg)\RCstar v=0
}

\AddEquation{rc-eigenrows=0 fg}
{
v\RCstar(f-\ShowEq{ga*g- \SideNS-\Cols}bg)=0
}

\AddEquation{cr-eigencols=0 fg}
{
v\CRstar(f-\ShowEq{ga*g- \SideNS-\Cols}bg)=0
}

\AddEquation{cr-eigenrows=0 fg}
{
(f-\ShowEq{ga*g- \SideNS-\Cols}bg)\CRstar v=0
}

\AddEquation{rc-eigencols=0}
{
(\ShowEq{f-bEn right}{})\RCstar v=0
}

\AddEquation{rc-eigenrows=0}
{
v\RCstar(\ShowEq{f-bEn left}{})=0
}

\AddEquation{cr-eigencols=0}
{
v\CRstar(\ShowEq{f-bEn left}{})=0
}

\AddEquation{cr-eigenrows=0}
{
(\ShowEq{f-bEn right}{})\CRstar v=0
}

\AddEq{basis e1=e2}
{
$\Basis e_1=\Basis e_2$.
}

\AddEq{basis e1 ne e2}
{
$\Basis e_1\ne\Basis e_2$.
}

\AddEq[2]{f-bEn left}
{
\ensuremath{f_{#1}-\aD Enb}#2
}

\AddEq[2]{f-bEn right}
{
\ensuremath{f_{#1}-b\aD En}#2
}

\AddEq[4]{Bases eVW}
{
\eV[#1 #3][,] \eV[#2 #3][#4]
}

\AddEq{f=g+h}
{
\[f=g+h\]
}

\AddEquation{fov=(g+h)ov left-cols}
{
\begin{aligned}
&\,\Vector f\circ (v\CRstar e_U)
\\=&\,v\CRstar f\CRstar e_V
\\=&\,v\CRstar(g+h)\CRstar e_V
\\=&\,v\CRstar g\CRstar e_V+v\CRstar h\CRstar e_V
\\=&\,\Vector g\circ (v\CRstar e_U)+\Vector h\circ (v\CRstar e_U)
\end{aligned}
}

\AddEquation{fov=(g+h)ov right-cols}
{
\begin{aligned}
&\,\Vector f\circ (e_U\RCstar v)
\\=&\,e_V\RCstar f\RCstar v
\\=&\,e_V\RCstar(g+h)\RCstar v
\\=&\,e_V\RCstar g\RCstar v+e_V\RCstar h\RCstar v
\\=&\,\Vector g\circ (e_U\RCstar v)+\Vector h\circ (e_U\RCstar v)
\end{aligned}
}

\AddEquation{fov=(g+h)ov left-rows}
{
\begin{aligned}
&\,\Vector f\circ (v\RCstar e_U)
\\=&\,v\RCstar f\RCstar e_V
\\=&\,v\RCstar(g+h)\RCstar e_V
\\=&\,v\RCstar g\RCstar e_V+v\RCstar h\RCstar e_V
\\=&\,\Vector g\circ (v\RCstar e_U)+\Vector h\circ (v\CRstar e_U)
\end{aligned}
}

\AddEquation{fov=(g+h)ov right-rows}
{
\begin{aligned}
&\,\Vector f\circ (e_U\CRstar v)
\\=&\,e_V\CRstar f\CRstar v
\\=&\,e_V\CRstar(g+h)\CRstar v
\\=&\,e_V\CRstar g\CRstar v+e_V\CRstar h\CRstar v
\\=&\,\Vector g\circ (e_U\CRstar v)+\Vector h\circ (e_U\RCstar v)
\end{aligned}
}

\AddEquation{fov=(gh)ov left-cols}
{
\begin{aligned}
&\,\Vector f\circ (u\CRstar e_U)
=u\CRstar f\CRstar e_W
\\=&\,u\CRstar g\CRstar h\CRstar e_W
\\=&\,\Vector h\circ(u\CRstar g\CRstar e_V)
\\=&\,\Vector h\circ(\Vector g\circ(u\CRstar e_U))
\\=&\,(\Vector h\circ\Vector g)\circ(u\CRstar e_U)
\end{aligned}
}

\AddEquation{fov=(gh)ov right-cols}
{
\begin{aligned}
&\,\Vector f\circ (e_U\RCstar u)
=e_W\RCstar f\RCstar u
\\=&\,e_W\RCstar h\RCstar g\RCstar u
\\=&\,\Vector h\circ(e_V\RCstar g\RCstar u)
\\=&\,\Vector h\circ(\Vector g\circ(e_U\RCstar u))
\\=&\,(\Vector h\circ\Vector g)\circ(e_U\RCstar u)
\end{aligned}
}

\AddEquation{fov=(gh)ov left-rows}
{
\begin{aligned}
&\,\Vector f\circ (u\RCstar e_U)
=u\RCstar f\RCstar e_W
\\=&\,u\RCstar g\RCstar h\RCstar e_W
\\=&\,\Vector h\circ(u\RCstar g\RCstar e_V)
\\=&\,\Vector h\circ(\Vector g\circ(u\RCstar e_U))
\\=&\,(\Vector h\circ\Vector g)\circ(u\RCstar e_U)
\end{aligned}
}

\AddEquation{fov=(gh)ov right-rows}
{
\begin{aligned}
&\,\Vector f\circ (e_U\CRstar u)
=e_W\CRstar f\CRstar u
\\=&\,e_W\CRstar h\CRstar g\CRstar u
\\=&\,\Vector h\circ(e_V\CRstar g\CRstar u)
\\=&\,\Vector h\circ(\Vector g\circ(e_U\CRstar u))
\\=&\,(\Vector h\circ\Vector g)\circ(e_U\CRstar u)
\end{aligned}
}

\AddEq{w=f o v}
{
w=f\circ v
}

\AddEquation{fov=gov+hov left-cols}
{
\begin{aligned}
&\,\Vector f\circ(v\CRstar e_U)
\\=&\,\Vector g\circ(v\CRstar e_U)+\Vector h\circ(v\CRstar e_U)
\\=&\,v\CRstar g\CRstar e_V+v\CRstar h\CRstar e_V
\\=&\,v\CRstar(g+h)\CRstar e_V
\end{aligned}
}

\AddEquation{fov=gov+hov right-cols}
{
\begin{aligned}
&\,\Vector f\circ(e_U\RCstar v)
\\=&\,\Vector g\circ(e_U\RCstar v)+\Vector h\circ(e_U\RCstar v)
\\=&\,e_V\RCstar g\RCstar v+e_V\RCstar h\RCstar v
\\=&\,e_V\RCstar (g+h)\RCstar v
\end{aligned}
}

\AddEquation{fov=gov+hov left-rows}
{
\begin{aligned}
&\,\Vector f\circ(v\RCstar e_U)
\\=&\,\Vector g\circ(v\RCstar e_U)+\Vector h\circ(v\RCstar e_U)
\\=&\,v\RCstar g\RCstar e_V+v\RCstar h\RCstar e_V
\\=&\,v\RCstar(g+h)\CRstar e_V
\end{aligned}
}

\AddEquation{fov=gov+hov right-rows}
{
\begin{aligned}
&\,\Vector f\circ(e_U\CRstar v)
\\=&\,\Vector g\circ(e_U\CRstar v)+\Vector h\circ(e_U\CRstar v)
\\=&\,e_V\CRstar g\CRstar v+e_V\CRstar h\CRstar v
\\=&\,e_V\CRstar (g+h)\CRstar v
\end{aligned}
}

\AddEquation{f o v=g o h o v left-cols}
{
\begin{aligned}
&\,\Vector f\circ(u\CRstar e_U)
\\=&\,\Vector h\circ(\Vector g\circ(u\CRstar e_U))
\\=&\,\Vector h\circ(u\CRstar g\CRstar e_V)
\\=&\,u\CRstar g\CRstar h\CRstar e_W
\end{aligned}
}

\AddEquation{f o v=g o h o v right-cols}
{
\begin{aligned}
&\,\Vector f\circ(e_U\RCstar u)
\\=&\,\Vector h\circ(\Vector g\circ(e_U\RCstar u))
\\=&\,\Vector h\circ(u\RCstar g\RCstar e_V)
\\=&\,e_W\RCstar h\RCstar g\RCstar u
\end{aligned}
}

\AddEquation{f o v=g o h o v left-rows}
{
\begin{aligned}
&\,\Vector f\circ(u\RCstar e_U)
\\=&\,\Vector h\circ(\Vector g\circ(u\RCstar e_U))
\\=&\,\Vector h\circ(u\RCstar g\RCstar e_V)
\\=&\,u\RCstar g\RCstar h\RCstar e_W
\end{aligned}
}

\AddEquation{f o v=g o h o v right-rows}
{
\begin{aligned}
&\,\Vector f\circ(e_U\CRstar u)
\\=&\,\Vector h\circ(\Vector g\circ(e_U\CRstar u))
\\=&\,\Vector h\circ(u\CRstar g\CRstar e_V)
\\=&\,u\CRstar g\CRstar h\CRstar e_W
\end{aligned}
}

\AddEq{sum of homomorphisms f o v=}
{
\forall v\in V: f\circ v=g\circ v+h\circ v
}

\AddEq{commutative law}
{
v+w=w+v
}

\AddEq{(g+h)o(u+v)=}
{
\begin{aligned}
&\,f\circ (u+v)
\\=&\,g\circ(u+v)+h\circ(u+v)
\\=&\,g\circ u+g\circ v
\\+&\,h\circ u+h\circ u
\\=&\,f\circ u+f\circ v
\end{aligned}
}

\AddEq{(h o g)o(u+v)=}
{
\begin{aligned}
&\,f\circ (u+v)
\\=&\,h\circ (g\circ(u+v))
\\=&\,h\circ (g\circ u+g\circ v))
\\=&\,h\circ (g\circ u)+h\circ (g\circ v)
\\=&\,f\circ u+f\circ v
\end{aligned}
}

\AddEquation{(g+h)o(av)= left}
{
\begin{aligned}
&\,f\circ (av)
\\=&\,g\circ(av)+h\circ(av)
\\=&\,a(g\circ v)+a(h\circ v)
\\=&\,a(g\circ v+h\circ v)
\\=&\,a(f\circ v)
\end{aligned}
}

\AddEquation{(h o g)o(av)= right}
{
\begin{aligned}
f\circ (va)
&=h \circ (g\circ(va))
\\ &=h\circ ((g\circ v)a)
\\ &=(h\circ (g\circ v))a
\\ &=(f\circ v)a
\end{aligned}
}

\AddEquation{(h o g)o(av)= left}
{
\begin{aligned}
f\circ (av)
&=h \circ (g\circ(av))
\\ &=h\circ (a(g\circ v))
\\ &=a(h\circ (g\circ v))
\\ &=a(f\circ v)
\end{aligned}
}

\AddEquation{(g+h)o(av)= right}
{
\begin{aligned}
&\,f\circ (va)
\\=&\,g\circ(va)+h\circ(va)
\\=&\,(g\circ v)a+(h\circ v)a
\\=&\,(g\circ v+h\circ v)a
\\=&\,(f\circ v)a
\end{aligned}
}

\AddEq{f=h o g}
{
$f=h\circ g$
}

\AddEq{f1 f2 left}
{
$f_1$, $f_2$
}

\AddEq{f1 f2 right}
{
$f_2$, $f_1$
}

\AddEq{vf1 vf2 left}
{
$\Vector f_1$, $\Vector f_2$
}

\AddEq{vf1 vf2 right}
{
$\Vector f_2$, $\Vector f_1$
}

\AddEq{diagram product of homomorphisms, A vector space}
{
\xymatrix{
U\ar[rr]^f\ar[dr]^g & & W\\
&V\ar[ur]^h &
}
}

\AddEq{f o u=h o g o u}
{
\begin{aligned}
\forall u\in U:
f\circ u&=(h\circ g)\circ u
\\ &=h\circ(g\circ u)
\end{aligned}
}

\AddEq{Vector f(e) cols}
{
\ensuremath{\Vector f\circ \aD[V_1]ei}
}

\AddEq{Vector f(e) rows}
{
\ensuremath{\Vector f\circ \aU{e_{V_1}}i}
}

\AddEq[4]{f=g*h}
{
#1=#2 #3 #4
}

\DefText{define homomorphism A module by matrix(111)}
{
\newline
\FrameEqRef[hg{A_1}{A_2}]{f o ea=efa (11)(\Cols)}{111\SideNS}
\newline
\FrameEqRef[vf{V_1}{V_2}]{f o (ae)=ga o f e, vector space \Product-\Cols}{\SideNS(111)}
\newline
}

\DefText{define homomorphism A module by matrix(11)}
{
\newline
\FrameEqRef[hf{A_1}{A_2}]{f o ea=efa (1)(\Cols)}{11\SideNS}
\newline
\FrameEqRef[vf{V_1}{V_2}]{f o (ae)=ga o f e, vector space \Product-\Cols}{\SideNS(11)}
\newline
}

\DefText{define homomorphism A module by matrix(1)}
{
\newline
\FrameEqRef[vf12]{f o (ae)=a o f e, vector space \Product-\Cols}{\SideNS(1)}
\newline
}

\DefText{define homomorphism D module by matrix(1)}
{
\newline
\FrameEqRef[hf12{}]{f o ea=efa (11)(\Cols)}{module}
\newline
}

\DefText{define homomorphism D module by matrix()}
{
\newline
\FrameEqRef[hf12{}]{f o ea=efa (1)(\Cols)}{module}
\newline
}

\DefText[3]{f o (ae)=a o f e (11)}
{
\DrawEq[w{}{(\Vector g\circ v)}{}f{}]{v1=v2*a \SideNS-\Cols}{\SideNS(#1#2#3)}
\DrawEq[gf{V_1}{V_2}{}]{f o ev=efv i (11)}{(#1)(\Cols)algebra, \SideNS-module}
\DrawEq[vf{V_1}{V_2}]{f o (ae)=ga o f e, vector space \Product-\Cols}{\SideNS(#1#2#3)}
}

\DefText[3]{f o (ae)=a o f e (1)}
{
\DrawEq[w{}v{}f{}]{v1=v2*a \SideNS-\Cols}{\SideNS(#1#2#3)}
\DrawEq[vf{V_1}{V_2}{}]{f o ev=efv i (1)}{()(\Cols)algebra, \SideNS-module}
\DrawEq[vf12]{f o (ae)=a o f e, vector space \Product-\Cols}{\SideNS(#1#2#3)}
}

\AddEq[4]{f o (ae)=a o f e, vector space cr-cols}
{
\Vector{#2}\circ(#1\CRstar e_{#3})=#1\CRstar #2\CRstar e_{#4}
}

\AddEq[4]{f o (ae)=a o f e, vector space rc-cols}
{
\Vector{#2}\circ(e_{#3}\RCstar #1)=e_{#4}\RCstar #2\RCstar #1
}

\AddEq[4]{f o (ae)=a o f e, vector space cr-rows}
{
\Vector{#2}\circ(e_{#3}\CRstar #1)=e_{#4}\CRstar #2\CRstar #1
}

\AddEq[4]{f o (ae)=a o f e, vector space rc-rows}
{
\Vector{#2}\circ(#1\RCstar e_{#3})=#1\RCstar #2\RCstar e_{#4}
}

\AddEq[4]{f o (ae)=ga o f e, vector space cr-cols}
{
\Vector{#2}\circ(#1\CRstar e_{#3})=(\Vector g\circ #1)\CRstar #2\CRstar e_{#4}
}

\AddEq[4]{f o (ae)=ga o f e, vector space rc-cols}
{
\Vector{#2}\circ(e_{#3}\RCstar #1)=e_{#4}\RCstar #2\RCstar (\Vector g\circ #1)
}

\AddEq[4]{f o (ae)=ga o f e, vector space cr-rows}
{
\Vector{#2}\circ(e_{#3}\CRstar #1)=e_{#4}\CRstar #2\CRstar (\Vector g\circ #1)
}

\AddEq[4]{f o (ae)=ga o f e, vector space rc-rows}
{
\Vector{#2}\circ(#1\RCstar e_{#3})=(\Vector g\circ #1)\RCstar #2\RCstar e_{#4}
}

\AddEq[2]{left homomorphism cr, 1}
{
\Vector {#1}=#1\CRstar e_{#2}
}

\AddEq[2]{left homomorphism rc, 1}
{
\Vector {#1}=#1\RCstar e_{#2}
}

\AddEq[2]{right homomorphism cr, 1}
{
\Vector {#1}=e_{#2}\CRstar #1
}

\AddEq[2]{right homomorphism rc, 1}
{
\Vector {#1}=e_{#2}\RCstar #1
}

\AddEq{vb=a cr f cr e left cr()}
{
\Vector w=v\CRstar f\CRstar e_{V_2}
}

\AddEq{vb=a cr f cr e left rc()}
{
\Vector w=v\RCstar f\RCstar e_{V_2}
}

\AddEq{vb=a cr f cr e right rc()}
{
\Vector w=e_{V_2}\RCstar f\RCstar v
}

\AddEq{vb=a cr f cr e right cr()}
{
\Vector w=e_{V_2}\CRstar f\CRstar v
}

\AddEq{vb=a cr f cr e left cr(1)}
{
\Vector w=(\Vector g\circ v)\CRstar f\CRstar e_{V_2}
}

\AddEq{vb=a cr f cr e left rc(1)}
{
\Vector w=(\Vector g\circ v)\RCstar f\RCstar e_{V_2}
}

\AddEq{vb=a cr f cr e right rc(1)}
{
\Vector w=e_{V_2}\RCstar f\RCstar (\Vector g\circ v)
}

\AddEq{vb=a cr f cr e right cr(1)}
{
\Vector w=e_{V_2}\CRstar f\CRstar (\Vector g\circ v)
}

\AddEq{vv=v*eV left cr()}
{
\begin{aligned}
\Vector w&=\Vector f\circ \Vector v=\Vector f\circ (v\CRstar e_{V_1})
\\ &=v\CRstar (\Vector f\circ e_{V_1})
\end{aligned}
}

\AddEq{vv=v*eV left rc()}
{
\begin{aligned}
\Vector w&=\Vector f\circ \Vector v=\Vector f\circ (v\RCstar e_{V_1})
\\ &=v\RCstar (\Vector f\circ e_{V_1})
\end{aligned}
}

\AddEq{vv=v*eV right rc()}
{
\begin{aligned}
\Vector w&=\Vector f\circ \Vector v=\Vector f\circ (e_{V_1}\RCstar v)
\\ &=(\Vector f\circ e_{V_1})\RCstar v
\end{aligned}
}

\AddEq{vv=v*eV right cr()}
{
\begin{aligned}
\Vector w&=\Vector f\circ \Vector v=\Vector f\circ (e_{V_1}\CRstar v)
\\ &=(\Vector f\circ e_{V_1})\CRstar v
\end{aligned}
}

\AddEq{vv=v*eV left cr(1)}
{
\begin{aligned}
\Vector w&=\Vector f\circ \Vector v=\Vector f\circ (v\CRstar e_{V_1})
\\ &=(\Vector g\circ v)\CRstar (\Vector f\circ e_{V_1})
\end{aligned}
}

\AddEq{vv=v*eV left rc(1)}
{
\begin{aligned}
\Vector w&=\Vector f\circ \Vector v=\Vector f\circ (v\RCstar e_{V_1})
\\ &=(\Vector g\circ v)\RCstar (\Vector f\circ e_{V_1})
\end{aligned}
}

\AddEq{vv=v*eV right rc(1)}
{
\begin{aligned}
\Vector w&=\Vector f\circ \Vector v=\Vector f\circ (e_{V_1}\RCstar v)
\\ &=(\Vector f\circ e_{V_1})\RCstar (\Vector g\circ v)
\end{aligned}
}

\AddEq{vv=v*eV right cr(1)}
{
\begin{aligned}
\Vector w&=\Vector f\circ \Vector v=\Vector f\circ (e_{V_1}\CRstar v)
\\ &=(\Vector f\circ e_{V_1})\CRstar (\Vector g\circ v)
\end{aligned}
}

\AddEq{f o ei=fij ej left cr}
{
\ShowEq{Vector f(e) cols}
=\aD fi\CRstar e_{V_2}
=\aUD fji \aD[V_2]ej
}

\AddEq{f o ei=fij ej left rc}
{
\ShowEq{Vector f(e) rows}
=\aU fi\RCstar e_{V_2}
=\aUD fij \aU{e_{V_2}}j
}

\AddEq{f o ei=fij ej right cr}
{
\ShowEq{Vector f(e) rows}
=e_{V_2}\CRstar \aU fi
=\aD[V_2]ej\aUD fij
}

\AddEq{f o ei=fij ej right rc}
{
\ShowEq{Vector f(e) cols}
=e_{V_2}\RCstar \aD fi
=\aU{e_{V_2}}j\aUD fji
}

\AddEq{ga*g- left-En}
{
\[
\ShowEq{ga*g- \SideNS-\Cols}b{\aD En}
=\aD Enb
\]
}

\AddEq{ga*g- right-En}
{
\[
\ShowEq{ga*g- \SideNS-\Cols}b{\aD En}
=b\aD En
\]
}

\AddEq{g(f-bEn)g left-cols}
{
g\CRstar(
\ShowEq{f-bEn left}1{}
)\CRstar g^{\CRInverse}
}

\AddEq{g(f-bEn)g right-cols}
{
g^{\RCInverse}\RCstar(
\ShowEq{f-bEn right}1{}
)\RCstar g
}

\AddEq{g(f-bEn)g left-rows}
{
g\RCstar(
\ShowEq{f-bEn left}1{}
)\RCstar g^{\RCInverse}
}

\AddEq{g(f-bEn)g right-rows}
{
g^{\CRInverse}\CRstar(
\ShowEq{f-bEn right}1{}
)\CRstar g
}

\AddEq[2]{ga*g- left-cols}
{
\ensuremath{#2#1\CRstar #2^{\CRInverse}}
}

\AddEq[2]{ga*g- right-cols}
{
\ensuremath{#2^{\RCInverse}\RCstar #1 #2}
}

\AddEq[2]{ga*g- left-rows}
{
\ensuremath{#2#1\RCstar #2^{\RCInverse}}
}

\AddEq[2]{ga*g- right-rows}
{
\ensuremath{#2^{\CRInverse}\CRstar #1 #2}
}

\AddEquation{ga*g- 1 left-cols}
{
g\CRstar \aD Ena\CRstar g^{\CRInverse}
}

\AddEquation{ga*g- 1 right-cols}
{
g^{\RCInverse}\RCstar a\aD En\RCstar g
}

\AddEquation{ga*g- 1 left-rows}
{
g\RCstar \aD Ena\RCstar g^{\RCInverse}
}

\AddEquation{ga*g- 1 right-rows}
{
g^{\CRInverse}\CRstar a\aD En\CRstar g
}

\AddEq{(a+b)aE left}
{
\[
\aD En(a+b)=\aD Ena+\aD Enb 
\]
}

\AddEq{(a+b)aE right}
{
\[
(a+b)\aD En=a\aD En+b\aD En
\]
}

\AddEq{(daE)v left}
{
\[
\aD En(ba)=b(\aD Ena)
\]
}

\AddEq{(daE)v right}
{
\[
(ba)\aD En=b(a\aD En)
\]
}

\AddEq{aEn=bEn left}
{
\[
\aD Ena=\aD Enb
\]
}

\AddEq{aEn=bEn right}
{
\[
a\aD En=b\aD En
\]
}

\AddEq[2]{e in basis manifold}
{
$\Basis e_{#1}\in
\ShowEq{basis manifold of V, \SideNS-\Cols}{\aD En}{#2}{}$
}

\AddEq{F1(g)=F(g)**-rc}
{
F_1(g)=F(g)^{\RCInverse}
}

\AddEq{F1(g)=F(g)**-cr}
{
F_1(g)=F(g)^{\CRInverse}
}

\AddEq{coordinate transformation, vector space W, left-cols}
{
w_2=w_1\CRstar F(g)^{\CRInverse}
}

\AddEq{coordinate transformation, vector space W, right-cols}
{
w_2=F(g)^{\RCInverse}\RCstar w_1
}

\AddEq{coordinate transformation, vector space W, left-rows}
{
w_2=w_1\RCstar F(g)^{\RCInverse}
}

\AddEq{coordinate transformation, vector space W, right-rows}
{
w_2=F(g)^{\CRInverse}\CRstar w_1
}

\AddEq[1]{f=f1+f2 endo}
{
f#1=f#1_1+f#1_2
}

\AddEq[1]{left e'=e*a}
{
\DrawEq[{e'_{#1}}{e_{#1}}{\ProductVal}g]{f=g*h}{}
}

\AddEq[1]{right e'=e*a}
{
\DrawEq[{e'_{#1}}g{\ProductVal}{e_{#1}}]{f=g*h}{}
}

\AddEq[1]{f=f1*f2 endo left-cols}
{
f#1=f#1_1\RCstar f#1_2
}

\AddEq[1]{f=f1*f2 endo right-cols}
{
f#1=f#1_1\CRstar f#1_2
}

\AddEq[1]{f=f1*f2 endo left-rows}
{
f#1=f#1_1\CRstar f#1_2
}

\AddEq[1]{f=f1*f2 endo right-rows}
{
f#1=f#1_1\RCstar f#1_2
}

\AddEq[5]{matrix fIJ}
{
\[
#1=(\AUD{#1}{#2}{#4},\jJg{#2}{#3},\jJg{#4}{#5})
\]
}

\DefText[4]{matrices of numbers(11)}
{
\ShowText{matrix of numbers and C}D{#1}gkKlL{#3}{#4}
\ShowText{matrices of numbers(1)}{#1}{#2}{}{}
}

\DefText[4]{matrices of numbers(1)}
{
\ShowText{matrix of numbers}A{#2}fiIjJ
}

\AddEq{passive transformation and endomorphism}
{
\,\newline
\TwoColText
{
\ShowRemark{passive transformation and endomorphism}v
}
{
\ShowRemark{passive transformation and endomorphism}w
}
}

\AddEq{fov=gov cols()}
{
\[
\Vector f\circ(e_1v)=e_2fv =\Vector g\circ(e_1v)
\]
}

\AddEq{fov=gov rows()}
{
\[
\Vector f\circ(ve_1)=vfe_2=\Vector g\circ(ve_1)
\]
}

\AddEq{fov=gov cols(1)}
{
\[
\Vector f\circ(e_1v)=e_2fh(v) =\Vector g\circ(e_1v)
\]
}

\AddEq{fov=gov rows(1)}
{
\[
\Vector f\circ(ve_1)=h(v)fe_2=\Vector g\circ(ve_1)
\]
}

\AddEq{fov=gov left-cols}
{
\[
\Vector f\circ(v\CRstar e_V)=v\CRstar f\CRstar e_W=\Vector g\circ(v\CRstar e_V)
\]
}

\AddEq{fov=gov left-rows}
{
\[
\Vector f\circ(v\RCstar e_V)=v\RCstar f\RCstar e_W=\Vector g\circ(v\RCstar e_V)
\]
}

\AddEq{fov=gov right-cols}
{
\[
\Vector f\circ(e_V\RCstar v)=e_W\RCstar f\RCstar v=\Vector g\circ(e_V\RCstar v)
\]
}

\AddEq{fov=gov right-rows}
{
\[
\Vector f\circ(e_V\CRstar v)=e_W\CRstar f\CRstar v=\Vector g\circ(e_V\CRstar v)
\]
}

\AddEquation{fo(v+w) cols(1)}
{
\begin{aligned}
&\,\Vector f\circ(e_1(v+w))
\\=&\,e_2fh(v+w) 
\\=&\,e_2f(h(v)+h(w)) 
\\=&\,e_2fh(v)+e_2fh(w) 
\\=&\,\Vector f\circ(e_1v)+\Vector f\circ(e_1w)
\end{aligned}
}

\AddEquation{fo(v+w) rows(1)}
{
\begin{aligned}
&\,\Vector f\circ((v+w)e_1)
\\=&\,h(v+w)f e_2 
\\=&\,(h(v)+h(w)) fe_2
\\=&\,h(v)fe_2+h(w)f e_2
\\=&\,\Vector f\circ(ve_1)+\Vector f\circ(we_1)
\end{aligned}
}

\AddEquation{fo(v+w) cols()}
{
\begin{aligned}
&\,\Vector f\circ(e_1(v+w))
\\=&\,e_2f(v+w) 
\\=&\,e_2fv+e_2fw 
\\=&\,\Vector f\circ(e_1v)+\Vector f\circ(e_1w)
\end{aligned}
}

\AddEquation{fo(v+w) rows()}
{
\begin{aligned}
&\,\Vector f\circ((v+w)e_1)
\\=&\,(v+w)f e_2 
\\=&\,vfe_2+wf e_2
\\=&\,\Vector f\circ(ve_1)+\Vector f\circ(we_1)
\end{aligned}
}

\AddEq{fo(v+w) ()left-cols}
{
\begin{aligned}
&\,\Vector f\circ((v+w)\CRstar e_{V_1})
\\=&\,(v+w)\CRstar f\CRstar e_{V_2} 
\\=&\,v\CRstar f\CRstar e_{V_2}+w\CRstar f\CRstar e_{V_2}
\\=&\,\Vector f\circ(v\CRstar e_{V_1})+\Vector f\circ(w\CRstar e_{V_1})
\end{aligned}
}

\AddEq{fo(v+w) ()left-rows}
{
\begin{aligned}
&\,\Vector f\circ((v+w)\RCstar e_{V_1})
\\=&\,(v+w)\RCstar f\RCstar e_{V_2} 
\\=&\,v\RCstar f\RCstar e_{V_2}+w\RCstar f\RCstar e_{V_2}
\\=&\,\Vector f\circ(v\RCstar e_{V_1})+\Vector f\circ(w\RCstar e_{V_1})
\end{aligned}
}

\AddEq{fo(v+w) ()right-cols}
{
\begin{aligned}
&\,\Vector f\circ(e_{V_1}\RCstar(v+w))\\=&\,e_{V_2}\RCstar f\RCstar(v+w)
\\=&\,e_{V_2}\RCstar f\RCstar v+e_{V_2}\RCstar f\RCstar w
\\=&\,\Vector f\circ(e_{V_1}\RCstar v)+\Vector f\circ(e_{V_1}\RCstar w)
\end{aligned}
}

\AddEq{fo(v+w) ()right-rows}
{
\begin{aligned}
&\,\Vector f\circ(e_{V_1}\CRstar(v+w))\\=&\,e_{V_2}\CRstar f\CRstar(v+w)
\\=&\,e_{V_2}\CRstar f\CRstar v+e_{V_2}\CRstar f\CRstar w
\\=&\,\Vector f\circ(e_{V_1}\CRstar v)+\Vector f\circ(e_{V_1}\CRstar w)
\end{aligned}
}

\AddEq{fo(v+w) (1)left-cols}
{
\begin{aligned}
&\,\Vector f\circ((v+w)\CRstar e_{V_1})
\\=&\,(g\circ(v+w))\CRstar f\CRstar e_{V_2} 
\\=&\,(g\circ v)\CRstar f\CRstar e_{V_2}+(g\circ w)\CRstar f\CRstar e_{V_2}
\\=&\,\Vector f\circ(v\CRstar e_{V_1})+\Vector f\circ(w\CRstar e_{V_1})
\end{aligned}
}

\AddEq{fo(v+w) (1)left-rows}
{
\begin{aligned}
&\,\Vector f\circ((v+w)\RCstar e_{V_1})
\\=&\,(g\circ(v+w))\RCstar f\RCstar e_{V_2} 
\\=&\,(g\circ v)\RCstar f\RCstar e_{V_2}+(g\circ w)\RCstar f\RCstar e_{V_2}
\\=&\,\Vector f\circ(v\RCstar e_{V_1})+\Vector f\circ(w\RCstar e_{V_1})
\end{aligned}
}

\AddEq{fo(v+w) (1)right-cols}
{
\begin{aligned}
&\,\Vector f\circ(e_{V_1}\RCstar(v+w))\\=&\,e_{V_2}\RCstar f\RCstar(g\circ(v+w))
\\=&\,e_{V_2}\RCstar f\RCstar(g\circ v)+e_{V_2}\RCstar f\RCstar(g\circ w)
\\=&\,\Vector f\circ(e_{V_1}\RCstar v)+\Vector f\circ(e_{V_1}\RCstar w)
\end{aligned}
}

\AddEq{fo(v+w) (1)right-rows}
{
\begin{aligned}
&\,\Vector f\circ(e_{V_1}\CRstar(v+w))\\=&\,e_{V_2}\CRstar f\CRstar(g\circ(v+w))
\\=&\,e_{V_2}\CRstar f\CRstar(g\circ v)+e_{V_2}\CRstar f\CRstar(g\circ w)
\\=&\,\Vector f\circ(e_{V_1}\CRstar v)+\Vector f\circ(e_{V_1}\CRstar w)
\end{aligned}
}

\AddEquation{fo(va) cols(1)}
{
\begin{aligned}
&\,\Vector f\circ(e_1(av) )\\=&\, e_2f h(av) 
\\=&\,h(a)(e_2f h(v))
\\=&\,h(a)(\Vector f\circ(e_1 v))
\end{aligned}
}

\AddEquation{fo(va) rows(1)}
{
\begin{aligned}
&\,\Vector f\circ((av) e_1)\\=&\,h(av) f e_2
\\=&\,h(a)( h(v)fe_2)
\\=&\,h(a)(\Vector f\circ( ve_1))
\end{aligned}
}

\AddEquation{fo(va) cols()}
{
\begin{aligned}
&\,\Vector f\circ(e_1(av) )\\=&\,e_2f (av)
\\=&\,a(e_2f v)
\\=&\,a(\Vector f\circ(e_1 v))
\end{aligned}
}

\AddEquation{fo(va) rows()}
{
\begin{aligned}
&\,\Vector f\circ((av)e_1)\\=&\,(av) f e_2
\\=&\,a( vfe_2)
\\=&\,a(\Vector f\circ( ve_1))
\end{aligned}
}

\AddEq{fo(va) ()left-cols}
{
\begin{aligned}
&\,\Vector f\circ((av)\CRstar e_{V_1})\\=&\,(av)\CRstar f\CRstar e_{V_2} 
\\=&\,a(v\CRstar f\CRstar e_{V_2})
\\=&\,a(\Vector f\circ(v\CRstar e_{V_1}))
\end{aligned}
}

\AddEq{fo(va) ()left-rows}
{
\begin{aligned}
&\,\Vector f\circ((av)\RCstar e_{V_1})\\=&\,(av)\RCstar f\CRstar e_{V_2} 
\\=&\,a(v\RCstar f\RCstar e_{V_2})
\\=&\,a(\Vector f\circ(v\RCstar e_{V_1}))
\end{aligned}
}

\AddEq{fo(va) ()right-cols}
{
\begin{aligned}
&\,\Vector f\circ(e_{V_1}\RCstar(va))\\=&\,e_{V_2}\RCstar f\RCstar(va)
\\=&\,(e_{V_2}\RCstar f\RCstar v)a
\\=&\,(\Vector f\circ(e_{V_1}\RCstar v))a
\end{aligned}
}

\AddEq{fo(va) ()right-rows}
{
\begin{aligned}
&\,\Vector f\circ(e_{V_1}\CRstar(va))\\=&\,e_{V_2}\CRstar f\CRstar(va)
\\=&\,(e_{V_2}\CRstar f\CRstar v)a
\\=&\,(\Vector f\circ(e_{V_1}\CRstar v))a
\end{aligned}
}

\AddEq{fo(va) (1)left-cols}
{
\begin{aligned}
&\,\Vector f\circ((av)\CRstar e_{V_1})\\=&\,(\Vector g\circ(av))\CRstar f\CRstar e_{V_2} 
\\=&\,(\Vector g\circ a)((\Vector g\circ v)\CRstar f\CRstar e_{V_2})
\\=&\,(\Vector g\circ a)(\Vector f\circ(v\CRstar e_{V_1}))
\end{aligned}
}

\AddEq{fo(va) (1)left-rows}
{
\begin{aligned}
&\,\Vector f\circ((av)\RCstar e_{V_1})\\=&\,(\Vector g\circ(av))\RCstar f\CRstar e_{V_2} 
\\=&\,(\Vector g\circ a)((\Vector g\circ v)\RCstar f\RCstar e_{V_2})
\\=&\,(\Vector g\circ a)(\Vector f\circ(e_{V_1}\CRstar v))
\end{aligned}
}

\AddEq{fo(va) (1)right-cols}
{
\begin{aligned}
&\,\Vector f\circ(e_{V_1}\RCstar(va))\\=&\,e_{V_2}\RCstar f\RCstar(\Vector g\circ(va))
\\=&\,(e_{V_2}\RCstar f\RCstar(\Vector g\circ v))(\Vector g\circ a)
\\=&\,(\Vector f\circ(e_{V_1}\RCstar v))(\Vector g\circ a)
\end{aligned}
}

\AddEq{fo(va) (1)right-rows}
{
\begin{aligned}
&\,\Vector f\circ(e_{V_1}\CRstar(va))\\=&\,e_{V_2}\CRstar f\CRstar(\Vector g\circ(va))
\\=&\,(e_{V_2}\CRstar f\CRstar(\Vector g\circ v))(\Vector g\circ a)
\\=&\,(\Vector f\circ(e_{V_1}\CRstar v))(\Vector g\circ a)
\end{aligned}
}

\AddEquation{e*f*v=e*ae*v left-cols}
{
\begin{aligned}
&\,\RedText{v\CRstar f\CRstar e}
=\Vector f\circ\Vector v
=\Vector{b\Basis e}\circ\Vector v
\\ =&\,\RedText{v\CRstar
\ShowEq{ga*g- \SideNS-\Cols}bg
\CRstar e}
\end{aligned}
}

\AddEquation{e*f*v=e*ae*v right-cols}
{
\begin{aligned}
&\,\RedText{e\RCstar f\RCstar v}
=\Vector f\circ\Vector v
=\Vector{b\Basis e}\circ\Vector v
\\ =&\,\RedText{e\RCstar
\ShowEq{ga*g- \SideNS-\Cols}bg
\RCstar v}
\end{aligned}
}

\AddEquation{e*f*v=e*ae*v left-rows}
{
\begin{aligned}
&\,\RedText{v\RCstar f\RCstar e}
=\Vector f\circ\Vector v
=\Vector{b\Basis e}\circ\Vector v
\\ =&\,\RedText{v\RCstar
\ShowEq{ga*g- \SideNS-\Cols}bg
\RCstar e}
\end{aligned}
}

\AddEquation{e*f*v=e*ae*v right-rows}
{
\begin{aligned}
&\,\RedText{e\CRstar f\CRstar v}
=\Vector f\circ\Vector v
=\Vector{\Basis eb}\circ\Vector v
\\ =&\,\RedText{e\CRstar
\ShowEq{ga*g- \SideNS-\Cols}bg
\CRstar v}
\end{aligned}
}

\AddEq{phantom a**b}
{
\[\vphantom{a^b}\]
}

\AddEquation{twin to left product}
{
(v,a)\rightarrow
\ShowEq{left map a En}a{}
\circ v
}

\AddEquation{twin to right product}
{
(a,v)\rightarrow
\ShowEq{right map a En}a{}
\circ v
}

\AddEq{av left}
{
$va$
}

\AddEq{av right}
{
$av$
}

\AddEquation{(av)b= left}
{
\begin{aligned}
(av)b
&=
\ShowEq{left map a En}b{}
\circ(av)\\ &=a(
\ShowEq{left map a En}b{}
\circ v)=a(vb)
\end{aligned}
}

\AddEquation{(av)b= right}
{
\begin{aligned}
a(vb)&=
\ShowEq{right map a En}a{}
\circ(vb)\\ &=(
\ShowEq{right map a En}a{}
\circ v)b=(av)b
\end{aligned}
}

\AddEq{twin representations of algebra}
{
\xymatrix{
V\ar[rr]^{f(a)}\ar[d]^{g(\Basis e)(b)} & & V\ar[d]^{g(\Basis e)(b)}\\
V\ar[rr]_{f(a)}& &V
}
}

\AddEq{representation Ao2->V}
{
\ShowEq{f:A->*B}h{\AoxA A}V
}

\AddEq{representation Ao2->V =}
{
\[
h(a\otimes b)\circ v=avb
\]
}

\AddEq{(av)b=a(vb)}
{
(av)b=a(vb)
}

\AddEq{ab in A,v in V}
{
$\forall a$, $b\in A$, $v\in V$
}

\AddEq{be=e cr En right}
{
\[
\Basis e=e\CRstar\Basis{\aD En}
\]
}

\AddEq{be=e cr En left}
{
\[
\Basis e=\Basis{\aD En}\RCstar e
\]
}

\AddEq{a in A->aE hom left}
{
a\in A\rightarrow \aD Ena\in\End(A,V^*)
}

\AddEq{a in A->aE hom right}
{
a\in A\rightarrow a\aD En\in\End(A,V^*)
}

\AddEq{(ab)E left-cols}
{
\[
\aD En(ab)=(\aD Ena)\CRstar(\aD Enb)
\]
}

\AddEq{(ab)E right-cols}
{
\[
((ab)\aD En)=(a\aD En)\RCstar(b\aD En)
\]
}

\AddEq{(ab)E left-rows}
{
\[
\aD En(ab)=(\aD Ena)\RCstar(\aD Enb)
\]
}

\AddEq{(ab)E right-rows}
{
\[
((ab)\aD En)=(a\aD En)\CRstar(b\aD En)
\]
}

\AddEq{dim V=n}
{
$\dim V=\gin$
}

\AddEq{left a En}
{
$\aD Ena$
}

\AddEq{right a En}
{
$a\aD En$
}

\AddEq{v in V -> av in V right-cols}
{
\[
\Vector{a\Basis e}:e\RCstar v\in V\rightarrow
e\RCstar (a\aD En)\RCstar v\in V
\]
}

\AddEq{v in V -> av in V left-cols}
{
\[
\Vector{\Basis ea}:v\CRstar e\in V\rightarrow
v\CRstar (\aD Ena)\CRstar e\in V
\]
}

\AddEq{v in V -> av in V right-rows}
{
\[
\Vector{a\Basis e}:e\CRstar v\in V\rightarrow
e\CRstar (a\aD En)\CRstar v\in V
\]
}

\AddEq{v in V -> av in V left-rows}
{
\[
\Vector{\Basis ea}:v\RCstar e\in V\rightarrow
v\RCstar (\aD Ena)\RCstar e\in V
\]
}

\AddEq{basis e1 e2}
{
$\Basis e_1$, $\Basis e_2$
}

\AddEq{a1n= b= column}
{
\[
\aD a1=
\ColMatrix{\aD a1}m
\ \ \ ...\ \ \ \,
\aD an=
\ColMatrix{\aD an}m
\ \ \ \,
b=
\ColMatrix bm
\]
}

\AddEquation{star rows system of linear equations 1}
{
\begin{pmatrix}
\aUD a11 &...&\aUD a1n\\
... & ... & ... \\
\aUD am1 &...&\aUD amn
\end{pmatrix}
\RCstar
\begin{pmatrix}
\aU x1\\...\\ \aU xn
\end{pmatrix}
=
\begin{pmatrix}
\aU b1\\...\\ \aU bm
\end{pmatrix}
}

\AddEq{star rows system of linear equations 2}
{
\begin{array}{cccc}
\aUD a11\aU x1 &+...&+\aUD a1n\aU xn&=\aU b1\\
... & ... & ...& ... \\
\aUD am1\aU x1 &+...&+\aUD amn\aU xn&=\aU bm
\end{array}
}

\AddEquation{star rows system of linear equations, rank}
{
\RCRank(\aUD aji)=\RCRank
\begin{pmatrix}
\aUD aji&\aU bj
\end{pmatrix}
}

\AddEquation{star rows system of linear equations}
{
\aUD aji\aU xi=\aU bj
}

\AddEq{aD1n}
{
$\aD a1$, ..., $\aD an$.
}

\AddEq[1]{rc-rank a=k<m}
{
\[\RCRank a=\gik<\gi{#1}\]
}

\AddEq[1]{cr-rank a=k<m}
{
\symb{\CRRank  a}{cr-rank of matrix}{}
$$\ShowSymbol{cr-rank of matrix}{}=\gik<\gi{#1}$$
}

\AddEq{rc-rank of matrix}
{
\symb{\RCRank a}{rc-rank of matrix}1,
}

\AddEq{cr-rank of matrix}
{
\symb{\CRRank a}{cr-rank of matrix}1,
}

\AddEq[2]{left a rc b}
{
#1\ProductVal #2
}

\AddEq[2]{right a rc b}
{
#2\ProductVal #1
}

\AddEq{rows-of-matrix linearly dependent, 1}
{
$\aD {\lambda}p=-1$, $\aD {\lambda}s=\pRs$
}

\AddEq{rows-of-matrix linearly dependent, 2}
{
$\aD {\lambda}c=0$.
}

\AddEq[2]{columns of matrix are linearly dependent}
{
\ShowEq{\SideWS a rc b}{#1}{#2}=0
}

\AddEq{cols-of-matrix linearly dependent, 1}
{
$\aU {\lambda}r=-1$, $\aU {\lambda}t=\aUD Rtr$
}

\AddEq{cols-of-matrix linearly dependent, 2}
{
$\aU {\lambda}c=0$.
}

\AddEq{representation left vector space of maps B->A}
{
\[
\xymatrix@C=30pt
{
f:A\ar[r]|-{*}&A^B
}
\ \ \ f(a):g\in A^B\rightarrow ag\in A^B
\ \ \ (ag)(b)=ag(b)
\]
}

\AddEq{representation right vector space of maps B->A}
{
\[
\xymatrix@C=30pt
{
f:A\ar[r]|-{*}&A^B
}
\ \ \ f(a):g\in A^B\rightarrow ga\in A^B
\ \ \ (ga)(b)=g(b)a
\]
}

\AddEq{representation left vector space of algebra A}
{
\[
\xymatrix@C=30pt
{
f:A\ar[r]|-{*}&A
}
\ \ \ f(a):b\in A\rightarrow ab\in A
\]
}

\AddEq{representation right vector space of algebra A}
{
\[
\xymatrix@C=30pt
{
f:A\ar[r]|-{*}&A
}
\ \ \ f(a):b\in A\rightarrow ba\in A
\]
}

\AddEquation{left a->ab}
{
f(a):b\in A\rightarrow ab\in A
}

\AddEquation{right a->ab}
{
f(a):b\in A\rightarrow ba\in A
}

\AddEq{left vector space of maps B->A n}
{
\symb{\mathcal L^nA^B}{left vector space of maps B->A}1
}

\AddEq{right vector space of maps B->A n}
{
\symb{\mathcal R^nA^B}{right vector space of maps B->A}1
}

\AddEq{left vector space of algebra A n}
{
\symb{\mathcal L^nA}{left vector space of algebra A}1
}

\AddEq{right vector space of algebra A n}
{
\symb{\mathcal R^nA}{right vector space of algebra A}1
}

\AddEq{left vector space of maps B->A k}
{
\begin{align*}
\mathcal L^1A^B&=\mathcal LA^B\\
\mathcal L^kA^B&=\mathcal L^{k-1}A^B\oplus\mathcal LA^B
\end{align*}
}

\AddEq{right vector space of maps B->A k}
{
\begin{align*}
\mathcal R^1A^B&=\mathcal RA^B\\
\mathcal R^kA^B&=\mathcal R^{k-1}A^B\oplus\mathcal RA^B
\end{align*}
}

\AddEq{left vector space of algebra A k}
{
\begin{align*}
\mathcal L^1A&=\mathcal LA\\
\mathcal L^kA&=\mathcal L^{k-1}A\oplus\mathcal LA
\end{align*}
}

\AddEq{right vector space of algebra A k}
{
\begin{align*}
\mathcal R^1A&=\mathcal RA\\
\mathcal R^kA&=\mathcal R^{k-1}A\oplus\mathcal RA
\end{align*}
}

\AddEq{left vector space of maps B->A}
{
\symb{\mathcal LA^B}{left vector space of maps B->A}1
}

\AddEq{right vector space of maps B->A}
{
\symb{\mathcal RA^B}{right vector space of maps B->A}1
}

\AddEq{left vector space of algebra A}
{
\symb{\mathcal LA}{left vector space of algebra A}1
}

\AddEq{right vector space of algebra A}
{
\symb{\mathcal RA}{right vector space of algebra A}1
}

\AddEq{left a(h+g)=}
{
\[
a(h(b)+g(b))=ah(b)+ag(b)
\]
}

\AddEq{right a(h+g)=}
{
\[
(h(b)+g(b))a=h(b)a+g(b)a
\]
}

\AddEq{left a(b+c)=}
{
\[
a(b+c)=ab+ac
\]
}

\AddEq{right a(b+c)=}
{
\[
(b+c)a=ba+ca
\]
}

\AddEq{left (a1+a2)h=}
{
\[
(a_1+a_2)h(b)=a_1h(b)+a_2h(b)
\]
}

\AddEq{right (a1+a2)h=}
{
\[
h(b)(a_1+a_2)=h(b)a_1+h(b)a_2
\]
}

\AddEq{left a1a2h=}
{
\[
(a_2a_1)h(b)=a_2(a_1h(b))
\]
}

\AddEq{right a1a2h=}
{
\[
h(b)(a_1a_2)=(h(b)a_1)a_2
\]
}

\AddEq{left (a1+a2)b=}
{
\[
(a_1+a_2)b=a_1b+a_2b
\]
}

\AddEq{right (a1+a2)b=}
{
\[
b(a_1+a_2)=ba_1+ba_2
\]
}

\AddEq{left a1a2b=}
{
\[
(a_2a_1)b=a_2(a_1b)
\]
}

\AddEq{right a1a2b=}
{
\[
b(a_1a_2)=(ba_1)a_2
\]
}

\AddEquation{rank of matrix, rc-cols}
{
a_{\gi N\setminus\gi T}=\aD aT\RCstar R
}

\AddEquation{rank of matrix, 1, rc-cols}
{
\aD ar=\aD aT\RCstar \aD Rr
}

\AddEquation{rank of matrix, 2, rc-cols}
{
\aUD aar=\aUD aat\ \tRr
}

\AddEquation{rank of matrix, rc-rows}
{
a^{\gi M\setminus\gi S}=R\RCstar \aU aS
}

\AddEquation{rank of matrix, 1, rc-rows}
{
\aU ap=\aU Rp\RCstar\aU aS
}

\AddEquation{rank of matrix, 2, rc-rows}
{
\aUD apb=\aUD Rps\aUD asb
}

\AddEquation{rank of matrix, cr-rows}
{
a^{\gi M\setminus\gi S}=\aU aS\CRstar R
}

\AddEquation{rank of matrix, 1, cr-rows}
{
\aU ap=\aU aS\CRstar\aU Rp
}

\AddEquation{rank of matrix, 2, cr-rows}
{
\aUD abp=\aUD abs\aUD Rsp
}

\AddEquation{rank of matrix, cr-cols}
{
a_{\gi N\setminus\gi T}=R\CRstar\aD aT
}

\AddEquation{rank of matrix, 1, cr-cols}
{
\aD ar=\aD Rr\CRstar\aD aT
}

\AddEquation{rank of matrix, 2, cr-cols}
{
\aUD air=\aUD Rtr\aUD ait
}

\AddEq{rank of matrix, 4, rc}
{
\[
\pA r
-\pA T\RCstar
\SATm\RCstar \SA r=0
\]
}

\AddEq{rank of matrix, 4, cr}
{
\[
\pA r
-\SA r\CRstar
\SATm\CRstar\pA T =0
\]
}

\AddEquation{rank of matrix, 5, rc-cols}
{
\aD Rr
=\SATm\RCstar \SA r
}

\AddEquation{rank of matrix, 5, rc-rows}
{
\aU Rp
=\pA T\RCstar\SATm
}

\AddEquation{rank of matrix, 5, cr-cols}
{
\aD Rr
=\SA r\CRstar\SATm
}

\AddEquation{rank of matrix, 5, cr-rows}
{
\aU Rp
=\SATm\CRstar\pA T
}

\AddEquation{rank of matrix, 6, rc-cols}
{
\pA r=\pA T\RCstar\aD Rr
}

\AddEquation{rank of matrix, 6, rc-rows}
{
\pA r=\aU Rp\RCstar \SA r
}

\AddEquation{rank of matrix, 6, cr-cols}
{
\pA r=\aD Rr\CRstar\pA T
}

\AddEquation{rank of matrix, 6, cr-rows}
{
\pA r=\SA r\CRstar \aU Rp
}

\AddEq{rank of matrix, 7, rc-cols}
{
\[
\aUD akT\RCstar\SATm
=\aUD {\delta}kS
\]
}

\AddEq{rank of matrix, 7, rc-rows}
{
\[
\SATm\RCstar \SA l
=\Tdl
\]
}

\AddEq{rank of matrix, 7, cr-cols}
{
\[
\SATm\CRstar\aUD akT
=\aUD {\delta}kS
\]
}

\AddEq{rank of matrix, 7, cr-rows}
{
\[
\SA l\CRstar\SATm
=\Tdl
\]
}

\AddEquation{rank of matrix, 8, rc-cols}
{
\begin{split}
\aUD akr&=
\aUD {\delta}kS\RCstar\SA r
\\ &=
\aUD akT\RCstar\SATm
\RCstar
\SA r
\end{split}
}

\AddEquation{rank of matrix, 8, rc-rows}
{
\begin{split}
\pA l&=
\pA T\RCstar \Tdl
\\ &=
\pA T\RCstar
\SATm\RCstar \SA l
\end{split}
}

\AddEquation{rank of matrix, 8, cr-cols}
{
\begin{split}
\aUD akr&=
\SA r\CRstar\aUD {\delta}kS
\\ &=
\SA r
\CRstar
\SATm\CRstar\aUD akT
\end{split}
}

\AddEquation{rank of matrix, 8, cr-rows}
{
\begin{split}
\pA l&=
\Tdl\CRstar\pA T
\\ &=
\SA l\CRstar\SATm
\CRstar
\pA T
\end{split}
}

\AddEquation{rank of matrix, 9, rc-cols}
{
\aUD akr=
\aUD akT\RCstar \aD Rr
}

\AddEquation{rank of matrix, 9, rc-rows}
{
\pA l=
\aU Rp\RCstar \SA l
}

\AddEquation{rank of matrix, 9, cr-cols}
{
\aUD akr=
\aD Rr\CRstar \aUD akT
}

\AddEquation{rank of matrix, 9, cr-rows}
{
\pA l=
\SA l\CRstar \aU Rp
}


==> Vector.Space.2020.Stmt.Russian.tex <==
%auto-ignore
\input{Vector.Space.2020.Stmt.Eq}

\DefLabeledDefinition{eigenvalue of matrix}{\Product}
{
$A$\Hyph число $b$ называется
{\bf\ProductType собственным значением}
матрицы $f$,
если матрица
$f-b\aD En$
- \ProductType вырожденная матрица.
}

\DefLabeledDefinition{eigenvector of matrix}{\Product-\Cols}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением
матрицы $f$.
\ColC $v$ называется
{\bf собственн\ColB}
матрицы $f$, соответствующ\FinB \ProductType собственному значению $b$,
если верно равенство
\DrawEq{\Product-eigen\Cols}1
}

\DefLabeledTheorem{0 is eigenvalue of multiplicity}{\Product}
{
Пусть $f$ - $\gin\times\gin$ матрица $A$\Hyph чисел и
\ShowEq{\Product-rank a=k<n}
Тогда $0$ является \ProductType собственным значением кратности
$\gin-\gik$.
}

\DefProof{0 is eigenvalue of multiplicity}
{
Теорема является следствием равенства
\[a=a-0E\]
определения
\refDefinition{eigenvalue of matrix}{\Product}
и теоремы
\RefTheorem{star rows system of linear equations, solution}.
}

\DefLabeledTheorem{eigenvalues of pair of matrices}{\Product}
{
Пусть $f$ - $\gin\times\gin$ матрица $A$\Hyph чисел.
Пусть $g$ - \ProductType невырожденная $\gin\times\gin$ матрица $A$\Hyph чисел.
Тогда ненулевые \ProductType собственные значения пары матриц $(f,g)$
являются корнями любого уравнения
\DrawEq{\Product-det ij f-bg =0}{}
}

\DefProofSloppy{eigenvalues of pair of matrices}
{
Теорема является следствием теоремы
\refTheorem{singular matrix and quasideterminant}{\Product}
и определения
\refDefinition{eigenvalues of pair of matrices}{\Product}.
}

\DefLabeledTheorem{eigenvalues of matrix}{\Product}
{
Пусть $f$ - $\gin\times\gin$ матрица $A$\Hyph чисел.
Тогда ненулевые \RC собственные значения матрицы $f$
являются корнями любого уравнения
\DrawEq{\Product-det ij a=0}{}
}

\DefProofSloppy{eigenvalues of matrix}
{
Теорема является следствием теоремы
\refTheorem{singular matrix and quasideterminant}{\Product}
и определения
\refDefinition{Eigenvalue of Endomorphism}{\SideNS}.
}

\AddEq[6]{theorem: product of homomorphisms, A vector space}
{
\begin{ShadedTheorem}
\labelTheorem{product of homomorphisms, \SideWS A vector space, \ColN}
Пусть $U$, $V$, $W$ -
\SideRu вые $A$\Hyph векторные пространства \ColsNA.
\ShowEq{Let be Basis of vector space}UAU
\ShowEq{Let be Basis of vector space}VAV
\ShowEq{Let be Basis of vector space}WAW
Гомоморфизм
\ShowEq{vf: A->B}fUW{}%
является произведением гомоморфизмов
\ShowEq{vf: A->B}hVW,%
\ShowEq{vf: A->B}gUV{}%
тогда и только тогда, когда
матрица $f$ гомоморфизма $\Vector f$
относительно базисов
\ShowEq{Bases eVW}UW{}{}
равна \ProductType произведению матрицы $#1$ гомоморфизма $\Vector{#1}$
относительно базисов
\ShowEq{Bases eVW}{#2}{#3}{}{}
на матрицу $#4$ гомоморфизма $\Vector{#4}$
относительно базисов
\ShowEq{Bases eVW}{#5}{#6}{}
\DrawEq[f{#1}{\ProductVal}{#4}]{f=g*h}{\Product-\Cols}
\end{ShadedTheorem}
}

\AddEq[2]{proof: product of homomorphisms, A vector space}
{
\begin{proof}
Согласно теореме
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}
\DrawEq[ufUW]{f o (ae)=a o f e, vector space \Product-\Cols}{f product \Product-\Cols}
\DrawEq[ugUV]{f o (ae)=a o f e, vector space \Product-\Cols}{g product \Product-\Cols}
\DrawEq[vhVW]{f o (ae)=a o f e, vector space \Product-\Cols}{h product \Product-\Cols}
Согласно теореме
\refTheorem{product of homomorphisms is homomorphism, A vector space}{\SideNS},
равенство
\ShowEq{f o v=g o h o v \SideNS-\Cols}
является следствием равенств
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{g product \Product-\Cols},
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{h product \Product-\Cols}.
Равенство
\eqRef{f=g*h}{\Product-\Cols}
является следствием равенств
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{f product \Product-\Cols},
\EqRef{f o v=g o h o v \SideNS-\Cols}
и теоремы
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}.

Пусть
\DrawEq[f{#1}{\ProductVal}{#2.}]{f=g*h}-
Согласно теореме
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)},
существуют гомоморфизмы
\ShowEq{vf: A->B}fUV,%
\ShowEq{vf: A->B}gUV,%
\ShowEq{vf: A->B}hUV{}%
такие, что
\ShowEq{fov=(gh)ov \SideNS-\Cols}
Из равенства
\EqRef{fov=(gh)ov \SideNS-\Cols}
и теоремы
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS}
следует, что
гомоморфизм $\Vector f$
является произведением гомоморфизмов $\Vector h$, $\Vector g$.
\end{proof}
}

\DefLabeledTheorem{product of homomorphisms is homomorphism, A vector space}{\SideNS}
{
Пусть $U$, $V$, $W$ - \SideRu вые $A$\Hyph векторные пространства.
Предположим, что мы имеем
коммутативную диаграмму отображений
\DrawEq{diagram product of homomorphisms, A vector space}{\SideNS}
\newline
\DrawEq{f o u=h o g o u}{\SideNS}
где отображения $g$, $h$ являются
гомоморфизмами \SideRu вого $A$\Hyph векторного пространства.
Отображение
\ShowEq{f=h o g}
является гомоморфизмом
\SideRu вого $A$\Hyph векторного пространства
и называется
\AddIndex{произведением гомоморфизмов}{product of homomorphisms}
$h$, $g$.
}

\DefProof{product of homomorphisms is homomorphism, A vector space}
{
Равенство
\eqRef{f o u=h o g o u}{\SideNS}
следует из коммутативности диаграммы
\eqRef{diagram product of homomorphisms, A vector space}{\SideNS}.
Равенство
\DrawEq{(h o g)o(u+v)=}{\SideWS vector space}
является следствием равенств
\eqRef{\SideWS homomorphism, f av=}1,
\eqRef{f o u=h o g o u}{\SideNS}.
Равенство
\ShowEq{(h o g)o(av)= \SideNS}
является следствием равенств
\eqRef{\SideWS homomorphism, f av=}1,
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.
Теорема является следствием теоремы
\refTheorem{define homomorphism A module}{\SideNS(1)}
и равенств
\eqRef{(h o g)o(u+v)=}{\SideWS vector space},
\EqRef{(h o g)o(av)= \SideNS}.
}

\DefLabeledTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS}
{
Пусть $V$, $W$ - \SideRu вые $A$\Hyph векторные пространства
и отображения
\DrawEq[gVW,]{f: A->B}-
\DrawEq[hVW{}]{f: A->B}-
- гомоморфизмы
\SideRu вого $A$\Hyph векторного пространства.
Пусть отображение
\DrawEq[fVW{}]{f: A->B}-
определено равенством
\DrawEq{sum of homomorphisms f o v=}{\SideWS vector space}
Отображение $f$ является гомоморфизмом
\SideRu вого $A$\Hyph векторного пространства
и называется
\AddIndex{суммой
\ShowEq{f=g+h}
гомоморфизмов}{sum of maps}
$g$ and $h$.
}

\DefProof{sum of homomorphisms is homomorphism, A vector space}
{
Согласно теореме
\refTheorem{definition of vector space}{\SideNS}
(равенство
\eqRef{commutative law}{\SideWS vector space}),
равенство
\newline
\DrawEq{(g+h)o(u+v)=}{\SideWS vector space}
\begin{sloppypar}
\noindent
является следствием равенств
\eqRef{homomorphism, f v+w=}{\SideNS},
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.
Согласно теореме
\refTheorem{definition of vector space}{\SideNS}
(равенство
\eqRef{distributive law, \SideWS module, 1}1),
равенство
\ShowEq{(g+h)o(av)= \SideNS}
\end{sloppypar}
\noindent
является следствием равенств
\eqRef{\SideWS homomorphism, f av=}1,
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.

Теорема является следствием теоремы
\refTheorem{define homomorphism A module}{\SideNS(1)}
и равенств
\eqRef{(g+h)o(u+v)=}{\SideWS vector space},
\EqRef{(g+h)o(av)= \SideNS}.
}

\DefLabeledTheorem{sum of homomorphisms, A vector space}{\SideNS-\Cols}
{
Пусть $V$, $W$ -
\SideRu вые $A$\Hyph векторные пространства \ColsNA.
\ShowEq{Let be Basis of vector space}VAV
\ShowEq{Let be Basis of vector space}WAW
Гомоморфизм
\ShowEq{vf: A->B}fVW{}%
является суммой гомоморфизмов
\ShowEq{vf: A->B}gVW,%
\ShowEq{vf: A->B}hVW{}%
тогда и только тогда, когда
матрица $f$ гомоморфизма $\Vector f$
относительно базисов
\ShowEq{Bases eVW}VW{}{}
равна сумме матрицы $g$ гомоморфизма $\Vector g$
относительно базисов
\ShowEq{Bases eVW}VW{}{}
и матрицы $h$ гомоморфизма $\Vector h$
относительно базисов
\ShowEq{Bases eVW}VW{}.
}

\DefProof{sum of homomorphisms, A vector space}
{
Согласно теореме
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}
\DrawEq[afUV]{f o (ae)=a o f e, vector space \Product-\Cols}{f sum \Product-\Cols}
\DrawEq[agUV]{f o (ae)=a o f e, vector space \Product-\Cols}{g sum \Product-\Cols}
\DrawEq[ahUV]{f o (ae)=a o f e, vector space \Product-\Cols}{h sum \Product-\Cols}
Согласно теореме
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS},
равенство
\ShowEq{fov=gov+hov \SideNS-\Cols}
является следствием равенств
\eqRef{a.\Product.(b1+b2)=}1,
\eqRef{(b1+b2).\Product.a=}1,
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{g sum \Product-\Cols},
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{h sum \Product-\Cols}.
Равенство
\ShowEq{f=g+h}
является следствием равенств
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{f sum \Product-\Cols},
\EqRef{fov=gov+hov \SideNS-\Cols}
и теоремы
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}.

Пусть
\ShowEq{f=g+h}
Согласно теореме
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)},
существуют гомоморфизмы
\ShowEq{vf: A->B}fUV,%
\ShowEq{vf: A->B}gUV,%
\ShowEq{vf: A->B}hUV{}%
такие, что
\ShowEq{fov=(g+h)ov \SideNS-\Cols}
Из равенства
\EqRef{fov=(g+h)ov \SideNS-\Cols}
и теоремы
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS}
следует, что
гомоморфизм $\Vector f$
является суммой гомоморфизмов $\Vector g$, $\Vector h$.
}

\AddEq{definition: vector space of maps B->A n}
{
\begin{ShadedDefinition}
\labelDefinition{\SideWS vector space of maps B->A n}
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Для любого множества $B$
и любого целого $n>0$
мы определим \SideRu\To $\Base$\Hyph векторное пространство
\ShowEq{\SideWS vector space of maps B->A n}
используя определение по индукции
\ShowEq{\SideWS vector space of maps B->A k}
\end{ShadedDefinition}
}

\DefLabeledDefinition{vector space of algebra A n}{\SideNS}
{
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Для любого целого $n>0$
мы определим \SideRu\To $\Base$\Hyph векторное пространство
\ShowEq{\SideWS vector space of algebra A n}
используя определение по индукции
\ShowEq{\SideWS vector space of algebra A k}
}

\DefTheorem{coordinates of vector of vector space}
{
Координаты вектора $v\in V$ относительно базиса $\Basis e$
левого $\Base$\Hyph векторного пространства $V$
определены однозначно.
}

\DefLabeledTheorem{coordinates of vector}{\SideNS-\Cols}
{
Координаты вектора $v\in V$ относительно базиса $\Basis e$
\SideRu\Which \FreeRuB $\Base$\Hyph \VectorSetRuB $V$
определены однозначно.
Из равенства
\DrawEq{e*v=e*w,\SideNS}{\Cols}
следует, что
\ShowEq{=> v=w}
}

\DefProof{coordinates of vector}
{
Согласно теореме
\refTheorem{basis over division algebra}{\SideNS},
система векторов
\ShowEq{expansion relative basis, vector space, 0}
линейно зависима и в уравнении
\DrawEq{expansion relative basis, vector space, 1}{\SideNS-\Cols}
по крайней мере $b$ отлично от $0$. Тогда равенство
\DrawEq{expansion relative basis, vector space, 2}{\SideNS-\Cols}
следует из
\eqRef{expansion relative basis, vector space, 1}{\SideNS-\Cols}.
Равенство
\DrawEq{expansion relative basis, vector space}{\SideNS-\Cols}
является следствием из равенства
\eqRef{expansion relative basis, vector space, 2}{\SideNS-\Cols}.

Допустим мы имеем другое разложение
\DrawEq{expansion relative basis, vector space, 3}{\SideNS-\Cols}
Вычтя
\eqRef{expansion relative basis, vector space}{\SideNS-\Cols}
из
\eqRef{expansion relative basis, vector space, 3}{\SideNS-\Cols},
мы получим
\DrawEq{expansion relative basis, vector space, 4}{\SideNS-\Cols}
Так как векторы \ARow ei линейно независимы,
то равенство
\DrawEq{expansion relative basis, vector space, 5}{\SideNS-\Cols}
является следствием равенства
\eqRef{expansion relative basis, vector space, 4}{\SideNS-\Cols}.
Утверждение теоремы является следствием равенства
\eqRef{expansion relative basis, vector space, 5}{\SideNS-\Cols}.
}

\DefProof{coordinates of vector 2022}
{
Согласно теореме
\refTheorem{basis over division algebra}{\SideNS},
система векторов
\ShowEq{expansion relative basis, vector space, (0)}
линейно зависима и в уравнении
\ShowEq{expansion relative basis, vector space, 1 \SideNS}
по крайней мере $b$ отлично от $0$. Тогда равенство
\ShowEq{expansion relative basis, vector space, 2 \SideNS}
следует из
\EqRef{expansion relative basis, vector space, 1 \SideNS}.
Равенство
\ShowEq{expansion relative basis, vector space \SideNS}
является следствием из равенства
\EqRef{expansion relative basis, vector space, 2 \SideNS}.

Допустим мы имеем другое разложение
\ShowEq{expansion relative basis, vector space, 3 \SideNS}
Вычтя
\EqRef{expansion relative basis, vector space \SideNS}
из
\EqRef{expansion relative basis, vector space, 3 \SideNS},
мы получим
\ShowEq{expansion relative basis, vector space, 4 \SideNS}
Так как векторы \ARow ei линейно независимы,
то равенство
\DrawEq{expansion relative basis, vector space, 5()}{\SideNS}
является следствием равенства
\EqRef{expansion relative basis, vector space, 4 \SideNS}.
Утверждение теоремы является следствием равенства
\eqRef{expansion relative basis, vector space, 5()}{\SideNS}.
}

\DefProof{coordinates of vector *}
{
Теорема является следствием теоремы
\refTheorem{coordinates of vector}{\SideNS-*}.
}

\DefExample{system of linear equations, right vector space of columns}
{
Пусть $V$ - правое $A$\Hyph векторное пространство столбцов и
строка
\ShowEq{rcd linear span, 0}
задаёт множество векторов.
Вектор $\Vector b$
линейно зависит от векторов $\aD{\Vector a}i$,
если линейное уравнение
\DrawEq{rcd linear span, 2}f
где
\DrawEq[xn]{a=(a1.n col)}{}
столбец неизвестных коэффициентов разложения,
имеет решение.
Предположим, что
\DrawEq[{}jJ]{basis e of module cols}-
- базис.
Тогда векторы
\ShowEq{rcd linear span, 6}
имеют разложение
\ShowEq{rcd linear span, 7}
Если мы подставим \EqRef{rcd linear span, b}
и \EqRef{rcd linear span, ai}
в
\eqRef{rcd linear span, 2}f,
мы получим
\DrawEq{rcd linear span, 8}f
Применяя теорему \RefTheorem{coordinates of vector of vector space}
к
\eqRef{rcd linear span, 8}f,
мы получим
\AddIndex{систему линейных уравнений}
{system of linear equations}
\DrawEq{system of rcd linear equations}f

Если мы положим
\ShowEq{a1n= b= column}
то мы можем записать систему линейных уравнений
\eqRef{system of rcd linear equations}f
в следующей форме
\ShowEq{star rows system of linear equations 1}
Равенство
\ShowEq{star rows system of linear equations}
является следствием равенств
\ePrints{339295394}%
\ifx\Semafor\ValueOn%
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
и
\else%
\EqRef{rc-product of matrices},
\fi%
\EqRef{star rows system of linear equations 1}.
Записывая сумму
\EqRef{star rows system of linear equations}
в виде строки, мы получим
\DrawEq{star rows system of linear equations 2}2
Мы видим в системе линейных уравнений
\eqRef{star rows system of linear equations 2}2,
что $A$\Hyph столбец $b$ является правой линейной комбинацией $A$\Hyph столбцов
\ShowEq{aD1n}
}

\DefLabeledDefinition{rank of matrix}{\Product}
{
Если подматрица $\aUD aST$ - \ProductType невырожденная матрица,
то мы будем говорить, что
\ProductType ранг матрицы $a$ не меньше, чем $\gik$.
{\bf\ProductType ранг матрицы} $a$,
\ShowEq{\Product-rank of matrix}
- это максимальное значение $\gik$.
Мы будем называть соответствующую подматрицу
{\bf \ProductType главной подматрицей}.
}

\DefLabeledTheorem{vector space of maps B->A}{\SideNS}
{
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Для любого множества $B$
представление
\ShowEq{representation \SideWS vector space of maps B->A}
является \SideRu вым векторным пространством
\ShowEq{\SideWS vector space of maps B->A}
над $D$\Hyph алгеброй $A$.
}

\DefProof{vector space of maps B->A}
{
Согласно теореме
\RefTheorem{set of maps B->A is Abelian group},
множество отображений $A^B$ является абелевой группой.
Из равенства
\ShowEq{\SideWS a(h+g)=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}
следует, что отображение $f(a)$ является эндоморфизмом абелевой группы $A^B$.
Из равенств
\ShowEq{\SideWS (a1+a2)h=}
\ShowEq{\SideWS a1a2h=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{representation of algebra}
следует, что отображение $f$ является
представлением $D$\Hyph алгебры $A$ в абелевой группы $A^B$.
Теорема является следствием определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
}

\DefText{linear span, vector space}
{
\subsection{\SideRuC вое
\texorpdfstring{$A$}{A}-векторное пространство \ColsNA}
\ShowText{linear span in vector space}
}

\DefLabeledDefinition{coordinates of vector}{\SideWS \VectorSetNS}
{
Пусть $\Basis e$ - квазибазис \SideRu\Which $\Base$\Hyph \VectorSetRuB $V$,
и вектор
\ShowEq{vv in V}vV
имеет разложение
\DrawEq{vv=ve \SideWS module}{Definition}
относительно квазибазиса $\Basis e$.
$\Base_{\BaseExt}$\Hyph числа $\ACol vi$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно квазибазиса $\Basis e$.
Матрица $\Base_{\BaseExt}$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в квазибазисе $\Basis e$.
}

\DefLabeledTheorem{matrix and system of linear equations}{\SideNS-\Cols}
{
Рассмотрим матрицу
\DrawEq{matrix a = set ai \Cols}{\SideNS}
Тогда система линейных уравнений
\eqRef{a*x=b \SideNS}{\Cols}
может быть записана в следующей форме
\ShowEq{a*x=b \SideNS-\Cols}
\DrawEq{a*x=b 1 \SideNS-\Cols}1
}

\DefProof{matrix and system of linear equations}
{
Равенство
\EqRef{a*x=b \SideNS-\Cols}
является следствием равенств
\eqRef{linear span, b \SideNS}{b \Cols},
\eqRef{a=(a1.n set)}{xm \SideNS-\Cols},
\eqRef{a*x=b \SideNS}{\Cols}
\eqRef{matrix a = set ai \Cols}{\SideNS}
и определения
\RefDefinition{\RowNWS over \ColNWS product}.
}

\DefLabeledTheoremNote{nonsingular system of linear equations}{\SideNS-\Cols}
{
Решение невырожденной системы линейных уравнений
\newline
\FrameEqRef{a*x=b 1 \SideNS-\Cols}1
\newline
определено однозначно и может быть записано в любой
из следующих форм\,\footnotemark
\DrawEq{x=a-*b, matrix \SideNS}{\Cols}
\DrawEq{x=a-*b, quasideterminant \SideNS}{\Cols}
}
{
Мы можем найти решение системы
\eqRef{a*x=b 1 \SideNS-\Cols}1
в теореме
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=19}{1.6.1}.
Я повторяю это утверждение, так как я слегка изменил обозначения.
}

\DefProof{nonsingular system of linear equations}
{
Умножая обе части равенства
\eqRef{a*x=b 1 \SideNS-\Cols}1
слева на $a^{\InverseVal}$, мы получим
\eqRef{x=a-*b, matrix \SideNS}{\Cols}.
Пользуясь определением
\newline
\FrameEqRef{quasideterminant and inverse}{\Product}
\newline
мы получим
\eqRef{x=a-*b, quasideterminant \SideNS}{\Cols}.
Решение системы единственно
в силу теоремы
\RefTheorem{two rc-products equal}.
}

\DefLabeledDefinition{nonsingular system of linear equations}{\SideNS-\Cols}
{
Предположим, что $a$
- \ProductType невырожденная матрица. Мы будем называть соответствующую
систему линейных уравнений
\newline
\FrameEqRef{a*x=b 1 \SideNS-\Cols}1
\newline
\AddIndex{невырожденной системой линейных уравнений}
{nonsingular system of linear equations}.
}

\DefLabeledTheorem{linear span and system of equations}{\SideNS-\Cols}
{
Пусть
\DrawEq[{}jJ]{basis e of module}-
- базис.
Пусть векторы
\ShowEq{linear span, 6}
имеют разложение
\DrawEq[b]{linear span, b \SideNS}{b \Cols}
\DrawEq[{\ARow ai}{}]{linear span, b \SideNS}{a \Cols}
Вектор $\Vector b$
линейно зависит от векторов $\ARow{\Vector a}i$
\ShowEq{linear span, 1}
если существует \ColWS $A$\Hyph чисел
\DrawEq[xm]{a=(a1.n set)}{xm \SideNS-\Cols}
которые удовлетворяют
\AddIndex{системе линейных уравнений}
{system of linear equations}
\DrawEq{a*x=b \SideNS}{\Cols}
}

\DefProof{linear span and system of equations}
{
Равенство
\DrawEq{e*b=e*a*x \SideNS}{\Cols}
является следствием равенств
\eqRef{linear span, 2 \SideNS}{\SideNS-\Cols},
\eqRef{linear span, b \SideNS}{b \Cols},
\eqRef{linear span, b \SideNS}{a \Cols}.
Равенство
\DrawEq{b=a*x \SideNS}{\Cols}
является следствием равенства
\eqRef{e*b=e*a*x \SideNS}{\Cols}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
Равенство
\eqRef{a*x=b \SideNS}{\Cols}
является следствием равенства
\eqRef{b=a*x \SideNS}{\Cols}.
}

\DefLabeledTheorem{linear span is vector space}{\SideNS-\Cols}
{
$\spanb$ - подпространство \SideRu вого $A$\Hyph векторного пространства $V$ \ColsNA.
}

\DefProof{linear span is vector space}
{
Предположим, что
\ShowEq{linear span, vector space, 1}
Согласно теореме
\refTheorem{vector in linear span}{\SideNS-\Cols}
\DrawEq[bb]{linear span, 2 \SideNS}{b \SideNS-\Cols}
\DrawEq[cc]{linear span, 2 \SideNS}{c \SideNS-\Cols}
Тогда
\ShowEq{linear span, 3 \SideNS}
Это доказывает утверждение.
}

\DefLabeledDefinition{module type}{\SideNS-\Cols}
{
Мы представили множество векторов
\ShowEq{\RowN() 1n}vm{}
в виде
\RowA матрицы
\DrawEq[vm]{a=(a1.n \RowN)}{}
и множество $\Base_{\BaseExt}$\Hyph чисел
\ShowEq{\ColNS() 1n}cm{}
в виде
\ColA матрицы
\DrawEq[cm]{a=(a1.n \ColNS)}{cm \SideNS-\Cols}
Соответствующее представление \SideRu\Which $\Base$\Hyph \VectorSetRuB $V$ мы будем называть
\AddIndex{\SideRu\What $\Base$\Hyph \VectorSetRuE \ColsNA}{\SideWS A-\ColNWS space},
а $V$\Hyph число мы будем называть
\AddIndex{вектор\Hyph \ColWS}{\ColNWS vector}.
}

\DefLabeledTheorem{linear combination in module type}{\SideNS-\Cols}
{
Мы можем записать линейную комбинацию
\ShowEq{linear combination, \SideNS-\Cols}cvm
векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде \ProductType произведения матриц
\DrawEq[cvm]{w.e, \SideNS-\Cols}{cv}
}

\DefProof{linear combination in module type}
{
Теорема является следствием определений
\refDefinition{linear combination of vectors}{\SideNS},
\refDefinition{module type}{\SideNS-\Cols}.
}

\DefLabeledTheorem{vector in linear span}{\SideNS-\Cols}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsA и
\RowRuWS
\ShowEq{linear span, 0}
задаёт множество векторов.
Вектор $\Vector b$
линейно зависит от векторов $\ARow{\Vector a}i$
\ShowEq{linear span, 1}
если существует \ColWS $A$\Hyph чисел
\DrawEq[xm]{a=(a1.n set)}{}
так\FinA, что верно равенство
\DrawEq[bx]{linear span, 2 \SideNS}{\SideNS-\Cols}
}

\DefProof{vector in linear span}
{
Равенство
\eqRef{linear span, 2 \SideNS}{\SideNS-\Cols}
является следствием определения
\refDefinition{linear span, vector space}{\SideNS-\Cols}
и теоремы
\refTheorem{linear combination in module type}{\SideNS-\Cols}.
}

\DefLabeledDefinition{linear span, vector space}{\SideNS-\Cols}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsA и
\ShowEq{linear span, set}
- множество векторов.
\AddIndex{Линейная оболочка}{linear span, vector space}
в \SideRu вом $A$\Hyph векторном пространстве \ColsA - это множество
\ShowEq{linear span, vector space}
векторов, линейно зависимых от векторов
\ARow {\Vector a}i.
}

\DefLabeledTheorem{vector space of algebra A}{\SideNS}
{
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Представление, порождённое \SideRu вым сдвигом,
\ShowEq{representation \SideWS vector space of algebra A}
является \SideRu вым векторным пространством
\ShowEq{\SideWS vector space of algebra A}
над $D$\Hyph алгеброй $A$.
}

\DefProof{vector space of algebra A}
{
Согласно определениям
\refDefinition{module over algebra}{\SideWS \VectorSetNS},
\RefDefinition{algebra over ring},
$D$\Hyph алгебра $A$ является абелевой группой.
Из равенства
\ShowEq{\SideWS a(b+c)=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}
следует, что отображение
\ShowEq{\SideWS a->ab}
является эндоморфизмом абелевой группы $A$.
Из равенств
\ShowEq{\SideWS (a1+a2)b=}
\ShowEq{\SideWS a1a2b=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{representation of algebra}
следует, что отображение $f$ является
представлением $D$\Hyph алгебры $A$ в абелевой группе $A$.
Теорема является следствием определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
}

\AddEq{def row text}
{%
\def\ColWS{строка }%
\def\ColC{Cтрока }%
\def\ColA{строки }%
\def\ColB{ой строкой }%
\def\ColBNS{ой строкой}%
\def\ColumnC{ая строка }%
\def\ColumnCNS{ая строка}%
\def\FinA{ая}%
\def\FinB{ей }%
\def\FinC{й }%
\def\endC{ая }%
\def\ColsRu{строки }%
\def\ColsA{строк }%
\def\ColsNA{строк}%
\def\EndA{ых }%
\def\RowRuWS{столбец }%
\def\RowsNSA{столбцов}%
\def\RowA{столбца }%
\def\RowsRWSA{столбцов }%
}

\AddEq{def col text}
{%
\def\ColWS{столбец }%
\def\ColC{Cтолбец }%
\def\ColA{столбца }%
\def\ColB{ым столбцом }%
\def\ColBNS{ым столбцом}%
\def\ColumnC{ый столбец }%
\def\ColumnCNS{ый столбец}%
\def\FinA{ой}%
\def\FinB{им }%
\def\FinC{го }%
\def\endC{ий }%
\def\ColsRu{столбцы }%
\def\ColsA{столбцов }%
\def\ColsNA{столбцов}%
\def\EndA{ых }%
\def\RowsNSA{строк}%
\def\RowA{строки }%
\def\RowsRWSA{строк }%
\def\RowRuWS{строка }%
}

\DefLabeledDefinition{spectrum of matrix}{\Product}
{
Множество
\ShowEq{spectrum of matrix}
всех левых и правых
\ProductType собственных значений называется
\ProductType спектром матрицы a.
}

\DefLabeledTheorem{vector space over algebra}{\SideNS}
{
Следующая диаграмма представлений описывает \SideRu вое $A$\Hyph векторное пространство $V$
\DrawEq[{}{}{}{}]{diagram of representations, \SideWS module}1
В диаграмме представлений
\EqRef{diagram of representations, \SideWS module}
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
коммутативного кольца $D$ и $D$\Hyph алгебры $A$
в абелевой группе $V$
\ShowEq{\SideWS module, a d v}
}

\DefProof{vector space over algebra}
{
Диаграмма представлений
\EqRef{diagram of representations, \SideWS module}
является следствием определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теоремы
\RefTheorem{Free Algebra over Ring}.
Равенство
\EqRef{\SideWS module, a d v}
является следствием утверждения, что
\SideRu вое преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph векторного пространства $V$.
}

\DefLabeledTheorem{definition of vector space}{\SideNS}
{
Пусть $V$ является \SideRu вым $A$\Hyph векторным пространством.
$V$\Hyph числа удовлетворяют соотношениям
\begin{itemize}
\item
\AddIndex{закон коммутативности}{commutative law}
\DrawEq{commutative law}{\SideWS vector space}
\item
если $D$\Hyph алгебра $A$ ассоциативна,
то верен
\AddIndex{закон ассоциативности}{associative law}
\DrawEq{associative law, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{закон унитарности}{unitarity law}
\ShowEq{unitarity law, \SideWS A-module}
\end{itemize}
для любых
\ShowEq{p,q in A, v,w in V}
}

\DefProof{definition of vector space}
{
Равенство
\eqRef{commutative law}{\SideWS vector space}
является следствием определений
\refDefinition{module over algebra}{vector space},
\refDefinition{module over algebra}{\SideWS \VectorSetNS}.
Равенство
\eqRef{distributive law, \SideWS module, 1}1
следует из утверждения,
что \SideRu востороннее преобразование $p$ является эндоморфизмом абелевой группы $V$.
Равенство
\eqRef{distributive law, \SideWS module, 2}1
следует из утверждения, что представление
$g_{3,4}$
является гомоморфизмом аддитивной группы
$D$\Hyph алгебры $A$.
Равенство
\EqRef{unitarity law, \SideWS A-module}
следует из утверждения, что представление
$g_{3,4}$
является \SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$.
Равенство
\eqRef{associative law, \SideWS module}1
следует из утверждения, что представление
$g_{3,4}$
является \SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$,
если $D$\Hyph алгебра $A$ ассоциативна.
}

\DefLabeledTheorem{coordinate matrix of vector}{\SideNS-\Cols}
{
Если мы запишем векторы базиса $\Basis e$
в виде \RowA матрицы
\DrawEq[en]{a=(a1.n \RowN)}{type \SideNS-\Cols}
и координаты вектора
\ShowEq{w=w*e \SideNS-\Cols}w{}
относительно базиса $\Basis e$ в виде
\ColA матрицы
\DrawEq[wn]{a=(a1.n \ColNS)}{type \SideNS-\Cols}
то мы можем представить вектор
$\Vector w$
в виде \ProductType произведения матриц
\DrawEq[w]{vector w=w*e \SideNS-\Cols}w
}

\DefProof{coordinate matrix of vector}
{
Теорема является следствием теоремы
\refTheorem{linear combination in module type}{\SideNS-\Cols}.
}

\DefLabeledExample{Vector Space Type}{\SideNS-\Cols}
{
\ePrints{2022.01.05}
\ifx\Semafor\ValueOff
Мы представили множество векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде
\RowA матрицы
\DrawEq[vm]{a=(a1.n \RowN)}{}
и множество $A$\Hyph чисел
\ShowEq{\ColNWS set 1n}cm{}
в виде
\ColA матрицы
\DrawEq[cm]{a=(a1.n \ColNS)}{cm \SideNS-\Cols}
Поэтому мы можем записать линейную комбинацию векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде \ProductType произведения матриц
\DrawEq[{\ParmA}{\ParmB}m]{w.e, \SideNS-\Cols}{\ParmA\ParmB}
В частности,
если 
\else
Если 
\fi
мы запишем векторы базиса $\Basis e$ в виде
\RowA матрицы
\DrawEq[en]{a=(a1.n \RowN)}{\SideNS-\Cols}
и координаты вектора
\ShowEq{w=w*e \SideNS-\Cols}w{}
относительно базиса $\Basis e$ в виде
\ColA матрицы
\DrawEq[wn]{a=(a1.n \ColNS)}{\SideNS-\Cols}
то мы можем представить вектор
$\Vector w$
в виде \ProductType произведения матриц
\DrawEq[w]{vector w=w*e \SideNS-\Cols}w
Соответствующее представление векторного пространства $V$ мы будем называть
\AddIndex{\SideRu вым $A$\Hyph векторным пространством \ColsNA}{\SideWS A-\ColNWS space},
а $V$\Hyph число мы будем называть
\AddIndex{вектор\Hyph \ColWS}{\ColNWS vector}.
}

\DefRemark{Left and Right Eigenvalues not equal 0}
{
Согласно данному выше определению,
множества левых и правых \ProductType собственных значений совпадают.
Однако мы рассмотрели самый простой случай.
Кон рассматривает определения

\ShowEq{def right}
\ShowEq{\DefCol}
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
\ShowEq{def left}
\ShowEq{\DefRow}
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1

\noindent
где $a_2$ - \ProductType невырожденная матрица,
как начальную точку для исследования.
}

\AddEq{remark: Left and Right Eigenvalues not equal}
{
Мы предполагаем, что кратность всех \SideRu вых \ProductType собственных значений
\nTimes матрица $a_2$ равна $1$.
Допустим \nTimes матрица $a_2$ не имеет $\gin$
\SideRu вых \ProductType собственных значений,
но имеет
\ShowEq{gik<gin}
\SideRu вых \ProductType собственных значений.
В этом случае, матрица $u_2$ в равенстве

\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1

\noindent
является
\ShowEq{gin x gik \SideNS}
матрицей, и матрица $a_1$
является \nTimes[k] матрицей.
Однако из равенства
\eqRef{A \ProductS U=U \ProductS D \SideNS}1
не следует, что
\ShowEq{rank rc u2 =k}

Если
\ShowEq{rank rc u2 =k}
то существует
\ShowEq{gin x gik \OtherSideNS}
матрица
\ShowEq{a in left}w{u_2}{\OtherSideNS}{}
такая, что
\ShowEq{w rc u2=Ek \SideNS}
Равенство
\ShowEq{w rc a2 rc u2=a1 \SideNS}
является следствием равенств
\eqRef{A \ProductS U=U \ProductS D \SideNS}1,
\EqRef{w rc u2=Ek \SideNS}.

Если
\ShowEq{rank rc u2 <k}
то между 
\SideRu выми собственными векторами
существует линейная зависимость.
В этом случае
множества левых и правых \ProductType собственных значений не совпадают.
}

\DefText[4]{define homomorphism of vector space(1)}
{
Согласно определениям
\ShowRef{define homomorphism A module}
отображение
\DrawEq[gA]{homomorphism D algebra #1#2}{\SideWS vector}
явлется гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
Следовательно, равенства
\ShowEq{ref homomorphism of A vector space(#1)}{#1}{#2}{#3}
являются следствием теоремы
\refTheorem{linear map of D module}{#1#2}.
}

\DefText[4]{define homomorphism of vector space()}
{
}

\AddEq{remark: colinear vectors}
{
Векторы $v$ и
\ShowEq{av \SideNS}
называются
\AddIndex{колинеарными}{colinear vectors}
с\OtherSideRu ва.
Из утверждения, что векторы $v$ и $w$
колинеарны с\OtherSideRu ва
не следует, что
векторы $v$ и $w$ линейно зависимы с\SideRu ва.
}

\DefText[7]{be extended basis}
{
Пусть базис
\DrawEq[{#1}{#2}{#3}{#4}{#5}{#6}]{extended basis}{#7}
является расширением базиса \eV[1][.]
}

\DefLabeledTheorem{Two bases of module}{\SideNS-\Cols}
{
\ShowEq{Let be basis of algebra}{}{}kKD{}A{}-
\ShowEq{Let be basis of module}1{}iI{\SideRu\Which}A{}V{}
Тогда множество $V$\Hyph чисел
\DrawEq[2{}{}{}ik]{extended basis}{\SideNS-\Cols}
является базисом $D$\Hyph \VectorSetRuB $V$.
Базис \eV[2] называется расширением базиса \eV[1][.]
}

\DefProofRef{Two bases of module}{\SideNS-\Cols}
{
Теорема является следствием теоремы
\refTheorem{basis over division algebra}{\SideNS}
и лемм
\refLemma{Two bases of module 1}{\SideNS-\Cols},
\refLemma{Two bases of module 2}{\SideNS-\Cols}.
}

\DefLabeledLemma{Two bases of module 1}{\SideNS-\Cols}
{
Множество $V$\Hyph чисел \EBase 2{ik}
порождает $D$\Hyph \VectorSetRuA $V$.
}

\DefLemmaProof{Two bases of module 1}
{
Пусть
\DrawEq{Two bases of module 1 a}{\SideNS-\Cols}
произвольное $V$\Hyph число.
For any $A$\Hyph number \ACol ai,
согласно определению
\RefDefinition{algebra over ring}
и соглашению
\RefConvention{basis of algebra as basis of module},
существуют $D$\Hyph числа \ACol a{ik} такие, что
\DrawEq{Two bases of module 1 ai}{\SideNS-\Cols}
Равенство
\DrawEq{Two bases of module 1 a=ai}{\SideNS-\Cols}
является следствием равенств
\eqRef{extended basis}{\SideNS-\Cols},
\eqRef{Two bases of module 1 a}{\SideNS-\Cols},
\eqRef{Two bases of module 1 ai}{\SideNS-\Cols}.
Лемма
является следствием равенства
\eqRef{Two bases of module 1 a=ai}{\SideNS-\Cols}.
}

\DefLabeledLemma{Two bases of module 2}{\SideNS-\Cols}
{
Множество $V$\Hyph чисел \EBase 2{ik}
линейно независимо над кольцом $D$.
}

\DefLemmaProof{Two bases of module 2}
{
Пусть
\DrawEq{extended basis 1}{\SideNS-\Cols}
Равенство
\DrawEq{extended basis 2}{\SideNS-\Cols}
является следствием равенств
\eqRef{extended basis}{\SideNS-\Cols},
\eqRef{extended basis 1}{\SideNS-\Cols}.
Согласно теореме
\refTheorem{basis over division algebra}{\SideNS},
равенство
\DrawEq{extended basis 3}{\SideNS-\Cols}
является следствием равенства
\eqRef{extended basis 2}{\SideNS-\Cols}.
Равенство
\DrawEq{extended basis 4}{\SideNS-\Cols}
является следствием равенства
\eqRef{extended basis 3}{\SideNS-\Cols}.
Следовательно,
множество $V$\Hyph чисел \EBase 2{ik}
линейно независимо над кольцом $D$.
}

\DefLabeledTheorem{product vector over scalar}{\SideNS}
{
\ShowEq{ab in A,v in V}
\DrawEq{(av)b=a(vb)}{\SideNS}
}

\DefProof{product vector over scalar}
{
Согласно теореме
\refTheorem{similarity transformation}{\SideNS-\Cols}
и определению
\refDefinition{product vector over scalar}{\SideNS},
равенство
\ShowEq{(av)b= \SideNS}
является следствием равенства
\eqRef{\SideWS homomorphism, f av=}1.

Равенство
\eqRef{(av)b=a(vb)}{\SideNS}
является следствием равенства
\EqRef{(av)b= \SideNS}.
}

\DefLabeledDefinition{product vector over scalar}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
Билинейное отображение
\DrawEq{\OtherSideWS A*V->V}2
порождённое \OtherSideRu восторонним представлением
\ShowEq{twin to \SideWS product}
называется
\AddIndex{\OtherSideRu восторонним произведением}{\OtherSideNS-side product}
вектора на скаляр.
}

\DefLabeledLemma{rcd dcr basis}{\SideNS}
{
Мы можем отождествить многообразие базисов
\ShowEq{basis manifold of V, \SideNS-cols}{\aD En}{\GL nA}{}
и множество \ProductType невырожденных матриц \GL nA.
}

\AddEq{proof: rcd dcr basis 1}
{
\begin{sloppypar}
{\sc Доказательство.}
Согласно замечанию
\refRemark{identify basis and matrix of coordinates}{\SideNS-\Cols},
мы можем отождествить базис $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$
и матрицу $e$ координат базиса $\Basis e$
относительно базиса $\Basis{\aD En}$
\ShowEq{be=e cr En \SideNS}
\hfill\(\odot\)
\end{sloppypar}
}

\DefLabeledDefinition{dimension of vector space}{\SideNS}
{
Мы будем называть
\AddIndex{размерностью \SideRu вого $A$\Hyph векторного пространства}{dimension of vector space}
число векторов в базисе.
}

\DefLabeledTheorem{coordinate matrix of basis}{\Product-\Cols}
{
\ShowEq{Let V be vector space of}.
Координатная матрица базиса $\Basis{g}$ относительно базиса $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$ является \ProductType невырожденной матрицей.
}

\DefProof{coordinate matrix of basis}
{
Согласно теореме
\refTheorem{rank of matrix}{\Product-\Cols},
\CR ранг координатной матрицы базиса $\Basis{g}$ относительно базиса $\Basis e$
равен размерности левого $A$\Hyph пространства столбцов,
откуда следует утверждение теоремы.
}

\DefLabeledTheorem{automorphism of vector space}{\Product-\Cols}
{
\ShowEq{Let V be vector space of}.
Пусть $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
Тогда любой автоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства
$V$ имеет вид
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{automorphism}
где $f$ - \ProductType невырожденная матрица.
}

\DefProof{automorphism of vector space}
{
Равенство
\eqRef{v1=v2*a \SideNS-\Cols}{automorphism}
следует из теоремы
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}.
Так как $\Vector f$ - изоморфизм,
то для каждого вектора $\Vector v'$ существует единственный вектор $\Vector v$ такой, что
\ShowEq{v'=fov}
Следовательно, система линейных уравнений
\eqRef{v1=v2*a \SideNS-\Cols}{automorphism}
имеет единственное решение. Согласно следствию
\RefCorollary{nonsingular rows system of linear equations}
матрица $f$ \ProductType невырожденна.
}

\DefLabeledTheorem{Automorphisms of vector space form a group}{\Product-\Cols}
{
Матрицы автоморфизмов \SideRu вого $A$\Hyph пространства \ColsA порождают группу \Group nA.
}

\DefProof{Automorphisms of vector space form a group}
{
Если даны два автоморфизма $\Vector f$ и $\Vector g$, то мы можем записать
\ShowEq{Automorphisms of vector space, \Product-\Cols}
Следовательно, результирующий автоморфизм имеет матрицу $f\ProductVal g$.
}

\DefLabeledTheorem{av=bv=>a=b}{\SideNS-\Cols}
{
Если \SideRu вое $A$\Hyph векторное пространство $V$
имеет конечную размерность,
то из утверждения
\DrawEq{av=bv, v \SideNS}{\Cols}
следует, что $a=b$.
}

\DefProof{av=bv=>a=b}
{
Пусть множество векторов
\DrawEq[{}jJ]{basis e of module cols}-
является базисом левого $A$\Hyph векторного пространство $V$.
Согласно теоремам
\refTheorem{definition of vector space}{\SideNS},
\refTheorem{coordinates of vector}{\SideNS-\Cols},
равенство
\ShowEq{avi=bvi \SideNS-\Cols}
является следствием равенства
\eqRef{av=bv, v \SideNS}{\Cols}.
Теорема следует из равенства
\EqRef{avi=bvi \SideNS-\Cols},
если мы положим $v=\aD e1$.
}

\DefText[7]{matrix of numbers}
{
Пусть
\ShowEq{matrix fIJ}{#3}{#4}{#5}{#6}{#7}
матрица $#1_{#2}$\Hyph чисел.
}

\DefText[9]{matrix of numbers and C}
{
Пусть
\ShowEq{matrix fIJ}{#3}{#4}{#5}{#6}{#7}
матрица $#1_{#2}$\Hyph чисел,
которая удовлетворяют равенству
\ShowRef{algebra, homomorphism and product}{#8}{#9}{#3}
}

\DefText{map be homomorphism of ring (1)}
{%
Пусть отображение
\DrawEq[h{D_1}{D_2}{}]{f: A->B}{}
является гомоморфизмом кольца $D_1$ в кольцо $D_2$.
}

\DefText{map be homomorphism of ring ()}
{%
}

\DefLabeledTheorem[6]{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrices of numbers(#2#3)}{#4}{#5}{#1}{#2}
Отображение\refFootnote{homomorphism of A module}{\SideNS-\Cols(#1#2#3)}
\newline
\FrameEqRef[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{Vector \SideNS-\Cols}
\newline
определённое равенством
\ShowText{define homomorphism A module by matrix(#1#2#3)}
является гомоморфизмом
\SideRu вого $A$\Hyph векторного пространства \ColsNA.
Гомоморфизм
\eqRef{homomorphism A module #1#2#3}{Vector \SideNS-\Cols},
который имеет%
\ShowText{define homomorphism by given matrix(#2)}%
определён однозначно.
}

\DefText{define homomorphism by given matrix(1)}
{
данное множество матриц $(g,f)$,
}

\DefText{define homomorphism by given matrix()}
{
данную матрицу $f$,
}

\DefText[4]{matrix generates homomorphism (1)}
{
Согласно теореме
\refTheorem{matrix generates D algebra homomorphism}{\Cols(#1#2)},
отображение
\DrawEq[{\Vector g}A]{homomorphism D algebra #1#2}{(\SideNS-\Cols)algebra}
является гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$
и гомоморфизм
\eqRef{homomorphism D algebra #1#2}{(\SideNS-\Cols)algebra}
определён однозначно.

}

\DefText[4]{matrix generates homomorphism ()}
{
}

\DefProof[7]{matrix generates A module homomorphism}
{
\ShowText{matrix generates homomorphism (#2)}{#1}{#2}{#4}{#5}
Равенство
\DrawEq{fo(v+w) (#2)\SideNS-\Cols}{(#1#2)}
\begin{sloppypar}
\noindent
является следствием равенств
\ShowRef{matrix generates A module homomorphism(#2)}{#2}{#3}{#7}
Из равенства
\eqRef{fo(v+w) (#2)\SideNS-\Cols}{(#1#2)}
следует, что отображение $\Vector f$ является гомоморфизмом
абелевой группы.
Равенство
\end{sloppypar}
\DrawEq{fo(va) (#2)\SideNS-\Cols}{(#1#2)}
является следствием равенства
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}1.
Из равенства
\eqRef{fo(va) (#2)\SideNS-\Cols}{(#1#2)},
и определений
\RefDefinition{Morphism of Diagram of Representations},
\refDefinition{homomorphism A module}{\SideNS(#1#2#3)}
следует, что отображение
\newline
\FrameEqRef[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{Vector \SideNS-\Cols}
\newline
\begin{sloppypar}
\noindent
является гомоморфизмом
$A_{#2}$\Hyph \VectorSetRuB \ColsA $V_{#3}$
в $A_{#5}$\Hyph \VectorSetRuA \ColsA $V_{#6}$.
\end{sloppypar}

Пусть $f$ -
матрица гомоморфизмов $\Vector f$, $\Vector g$
относительно базисов
\ShowEq{Bases eVW}VW{}.%
Равенство
\ShowEq{fov=gov \SideNS-\Cols}
является следствием теоремы
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}.
Следовательно, $\Vector f=\Vector g$.
}

\DefLabeledTheorem[6]{homomorphism A module}{\SideNS-\Cols(#1#2#3)}
{
Гомоморфизм\refFootnote{homomorphism of A module}{\SideNS-\Cols(#1#2#3)}
\DrawEq[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{Vector \SideNS-\Cols}
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRu\To $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$
имеет представление
\ShowText{g:A1->A2, D module(#1#2#3)}
\ShowText{f o (ae)=a o f e (#2#3)}{#1}{#2}{#3}
относительно выбранных базисов.
Здесь
\begin{itemize}
\ShowText{homomorphism of vector space, algebra(#2)}{#1}{#2}{#3}{#4}{#5}{#6}
\ShowText{homomorphism of vector space, algebra 1}{#1}{#2}{#3}{#4}{#5}{#6}
\end{itemize}
\ShowText{matrix of homomorphism relative bases #2#3}{#1}{#2}{#3}
}

\DefText[3]{matrix of homomorphism relative bases 11}
{
Множество матриц $(g,f)$ определено однозначно и называется
{\bf координатами гомоморфизма}
\eqRef{homomorphism A module #1#2#3}{Vector \SideNS}
относительно базисов \eV[V_1][,] \eV[V_2][.]
}

\DefText[3]{matrix of homomorphism relative bases 1}
{
Матрица $f$ определена однозначно и называется
{\bf матрицей гомоморфизма}
$\Vector f$ относительно базисов \eV[1][,] \eV[2][.]
}

\DefText[6]{Proof, homomorphism of vector space(1)}
{
Согласно определениям
\ShowRef{Proof, homomorphism of vector space}{#1}{#2}{#3}%
отображение
\DrawEq[{\Vector g}A]{homomorphism D algebra #1#2}{\SideNS-\Cols}
явлется гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#4}$\Hyph алгебру $A_{#5}$.
Следовательно, равенства
\ShowRef{Proof, homomorphism of vector space 1}{#1}{#2}{#3}%
следуют из равенств
\ShowRef{Proof, homomorphism of vector space 2}{#1}{#2}{#3}%
Из теоремы
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
следует что матрица $g$ определена однозначно.

}

\DefText[6]{Proof, homomorphism of vector space()}
{%
}

\DefProof[6]{homomorphism A module}
{
\ShowText{Proof, homomorphism of vector space(#2)}{#1}{#2}{#3}{#4}{#5}{#6}%
Вектор
\ShowEq{vv in V}v{V_1}
имеет разложение
\DrawEq[v{V_1}]{\SideWS homomorphism \Product, 1}{v#1#2#3}
относительно базиса \eV[V_1][.]
Вектор
\ShowEq{vv in V}w{V_2}
имеет разложение
\DrawEq[w{V_2}]{\SideWS homomorphism \Product, 1}{w#1#2#3}
относительно базиса \eV[V_2][.]
Так кaк $\Vector f$ - гомоморфизм,
то равенство
\DrawEq{vv=v*eV \SideWS \Product(#2)}{(#1)}
является следствием равенств
\eqRef{homomorphism, f v+w=}{f(#1#2)\SideWS A module},
\eqRef{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module}.
$V_2$\Hyph число
\ShowEq{Vector f(e) \Cols}
имеет разложение
\DrawEq{f o ei=fij ej \SideWS \Product}{#1#2#3}
относительно базиса \eV[V_2][.]
Равенство
\DrawEq{vb=a cr f cr e \SideWS \Product(#2)}{(#1)}
является следствием равенств
\eqRef{vv=v*eV \SideWS \Product(#2)}{(#1)},
\eqRef{f o ei=fij ej \SideWS \Product}{#1#2#3}.
Равенство
\eqRef{v1=v2*a \SideNS-\Cols}{\SideNS(#1#2#3)}
следует из сравнения
\eqRef{\SideWS homomorphism \Product, 1}{w#1#2#3}
и \eqRef{vb=a cr f cr e \SideWS \Product(#2)}{(#1)} и
теоремы 
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
Из равенства
\eqRef{f o ei=fij ej \SideWS \Product}{#1#2#3}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}
следует что матрица $f$ определена однозначно.
}

\DefText{notation for homomorphism of module}
{
Мы будем пользоваться записью
\DrawEq{f circ a =}{}
для образа гомоморфизма $f$.
}

\DefText{be division algebra}
{
Пусть $D$\Hyph алгебра $A$ является алгеброй с делением.
}

\DefTheorem{division algebra has unit}
{
\ShowText{be division algebra}
$D$\Hyph алгебра $A$ имеет единицу.
}

\DefTheorem{division D algebra, ring D is the field}
{
\ShowText{be division algebra}
Кольцо $D$ является полем
и подмножеством центра $D$\Hyph алгебры $A$.
}

\AddEq[3]{remark: homomorphism of vector space 2}
{
На основании теорем
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)},
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)}
мы идентифицируем гомоморфизм
$\Vector f$
\SideRu вого $A$\Hyph векторного пространства $V$ \ColsA и
матрицу его представления
\newline
\FrameEqRef[afVW]{f o (ae)=a o f e, vector space \Product-\Cols}1
}

\DefLabeledDefinition{similarity transformation}{\SideNS}
{
Эндоморфизм
\ShowEq{\SideWS map a En}a{}
\SideRu вого $A$\Hyph векторного пространства $V$
называется
\AddIndex{преобразованием подобия}{similarity transformation}
относительно базиса $\Basis e$.
}

\AddEq{passive transformation for two bases}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть базисы
\ShowEq{basis e1 e2}
связаны пассивным преобразованием $g$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
}

\DefLabeledTheorem{covariance of eigenvalue}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$.

\begin{Statement}
\labelStatement{covariance of eigenvalue \SideNS-\Cols}
Собственное значение $b$
эндоморфизма $\Vector f$
относительно базиса $\Basis e_1$
не зависит от выбора базиса $\Basis e_2$.
\hfill\(\odot\)
\end{Statement}

\begin{Statement}
\labelStatement{covariance of eigenvector \SideNS-\Cols}
Собственный вектор $\Vector v$
эндоморфизма $\Vector f$,
соответствующий собственному значение $b$,
не зависит от выбора базиса $\Basis e_2$.
\hfill\(\odot\)
\end{Statement}
}

\DefProof{covariance of eigenvalue}
{
Пусть
\ShowEq{Ai, i=}f
- матрица эндоморфизма $f$ относительно базиса $\Basis e_i$.
Пусть $b$ - собственное значение
эндоморфизма $\Vector f$
относительно базиса $\Basis e_1$
и
$\Vector v$ собственный вектор
эндоморфизма $\Vector f$,
соответствующее собственному значение $b$.
Пусть
\ShowEq{Ai, i=}v
- матрица вектора $\Vector v$ относительно базиса $\Basis e_i$.

Предположим сперва, что
\ShowEq{basis e1=e2}
Тогда базисы
\ShowEq{basis e1 e2}
связаны пассивным преобразованием $\aD En$
\DrawEq[12{\aD En^{}{}}{}]{e2i=aij e1j \Product-\Cols}{}
Согласно теореме
\refTheorem{similarity transformation, change of basis}{\SideNS-\Cols},
преобразование подобия
\ShowEq{\SideWS map a En}b1
имеет матрицу
\ShowEq{ga*g- \SideNS-En}
относительно базиса $\Basis e_2$.
Следовательно, согласно теореме
\refTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols},
мы доказали следующие утверждения.

\begin{ShadedLemma}
\labelLemma{matrix f-bEn singular \SideNS-\Cols}
Матрица
\ShowEq{f-bEn \SideNS}1{}
\ProductType вырождена
\hfill\(\odot\)
\end{ShadedLemma}

\begin{ShadedLemma}
\labelLemma{vector v1 f-bEn \SideNS-\Cols}
Вектор \ColWS $v_1$ удовлетворяет ситеме линейных уравнений
\ShowEq{(f-bEn)v \Product-\Cols}
\hfill\(\odot\)
\end{ShadedLemma}

Предположим, что
\ShowEq{basis e1 ne e2}
Согласно теореме
\refTheorem{exists representation, commuting with active}{\SideNS-\Cols},
существует единственное пассивное преобразование
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
и $g$ - \ProductType невырожденая матрица.
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[fg{\SideNS}{\Cols}]{f2=a f1 a-}{covariance \SideNS-\Cols}
\begin{sloppypar}
\noindent
Согласно теореме
\refTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols},
если $b$ - собственное значение эндоморфизма $\Vector f$,
то мы должны доказать лемму
\RefLemma{matrix f-ae singular \SideNS-\Cols}.
\end{sloppypar}

\begin{ShadedLemma}
\labelLemma{matrix f-ae singular \SideNS-\Cols}
Матрица
\[\ShowEq{(f-ae)v matrix}f2bg\]
\ProductType вырождена
\hfill\(\odot\)
\end{ShadedLemma}

\begin{sloppypar}
Так как равенство
\ShowEq{f-ae->f-be}
следует из равенства
\eqRef{f2=a f1 a-}{covariance \SideNS-\Cols},
то лемма
\RefLemma{matrix f-ae singular \SideNS-\Cols}
следует из леммы
\RefLemma{matrix f-bEn singular \SideNS-\Cols}.
Следовательно, мы доказали утверждение
\RefStatement{covariance of eigenvalue \SideNS-\Cols}.
\end{sloppypar}

Согласно теореме
\refTheorem{eigenvector coordinates}{\SideNS-\Cols},
если $\Vector v$ - собственный вектор эндоморфизма $\Vector f$,
то мы должны доказать лемму
\RefLemma{vector v2 f-bEn \SideNS-\Cols}.

\begin{ShadedLemma}
\labelLemma{vector v2 f-bEn \SideNS-\Cols}
Вектор \ColWS $v_2$ удовлетворяет ситеме линейных уравнений
\ShowEq{(f-bEn)v2 \Product-\Cols}
\end{ShadedLemma}

\begin{sloppypar}
{\sc Доказательство.}
Согласно теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
\DrawEq[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{covariance \SideNS-\Cols}
Так как равенство
\ShowEq{f-ae->f-be \SideNS-\Cols}
следует из равенств
\eqRef{f2=a f1 a-}{covariance \SideNS-\Cols},
\eqRef{v2=v1g-}{covariance \SideNS-\Cols},
то лемма
\RefLemma{vector v2 f-bEn \SideNS-\Cols}
следует из леммы
\RefLemma{matrix f-bEn singular \SideNS-\Cols}.
\hfill\(\odot\)
\end{sloppypar}

Следовательно, мы доказали утверждение
\RefStatement{covariance of eigenvector \SideNS-\Cols}.
}

\DefLabeledTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols}
{
\ShowEq{passive transformation for two bases}
Пусть $f$ - матрица эндоморфизма $\Vector f$
относительно базиса $\Basis e_2$.
$A$\Hyph число $b$ является собственным значением
эндоморфизма $\Vector f$ тогда и только тогда, когда матрица
\DrawEq[f{}bg]{(f-ae)v matrix}{\SideNS-\Cols}
\ProductType вырождена.
}

\DefProof{eigenvalue of endomorphism, matrix is singular}
{
Теорема является следствием теорем
\RefTheorem{star rows system of linear equations},
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\DefLabeledTheorem{eigenvector coordinates}{\SideNS-\Cols}
{
\ShowEq{passive transformation for two bases}
Пусть $f$ - матрица эндоморфизма $\Vector f$
и $v$ - матрица вектора $\Vector v$
относительно базиса $\Basis e_2$.
Вектор $\Vector v$ является
собственным вектором
эндоморфизма $\Vector f$
относительно базиса $\Basis e_1$
тогда и только тогда, когда
существует $A$\Hyph число $b$ такое, что
система линейных уравнений
\DrawEq[fgbv]{(f-ae)v \Product-\Cols}{fgbv}
имеет нетривиальное решение.
}

\DefProof{eigenvector coordinates}
{
Согласно теоремам
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)},
\refTheorem{similarity transformation, change of basis}{\SideNS-\Cols},
равенство
\ShowEq{e*f*v=e*ae*v \SideNS-\Cols}
является следствием равенства
\eqRef{fov=b e o v}{\SideNS}.
Равенство
\eqRef{(f-ae)v \Product-\Cols}{fgbv}
является следствием равенства
\EqRef{e*f*v=e*ae*v \SideNS-\Cols}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
Так как равенство $\Vector v=0$ для нас не интересно,
система линейных уравнений
\eqRef{(f-ae)v \Product-\Cols}{fgbv}
должна иметь нетривиальное решение.
}

\AddEq{remark: eigenvector coordinates}
{
Определение
\refDefinition{Eigenvalue of Endomorphism}{\SideNS}
не зависит от структуры координат
\SideRu вого $A$\Hyph векторного пространства $V$.
Когда мы выбираем базис $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$,
мы видим дополнительную структуру,
которая отражена в теоремах
\refTheorem{eigenvector coordinates}{\SideNS-cols},
\refTheorem{eigenvector coordinates}{\SideNS-rows}.
}

\AddEq{remark: eigenvector of matrix}
{
Одна и таже матрица может соответствовать различным эндоморфизмам
в зависимости рассматриваем ли мы левое или правое
$A$\Hyph векторного пространство.
Поэтому мы должны рассмотреть все определения
собственных векторов, которые могут соответсвовать данной матрице.
Из теорем
\refTheorem{eigenvector coordinates}{left-cols},
\refTheorem{eigenvector coordinates}{right-cols},
\refTheorem{eigenvector coordinates}{left-rows},
\refTheorem{eigenvector coordinates}{right-rows}
следует, что для данной матрицы существует
четыре вида собственных векторов и
четыре вида собственных чисел.
Пара собственный вектор и собственное значение определённого вида
используется в решении задачи,
где возникает соответствующий вид $A$\Hyph векторного пространства.
Это утверждение отражено в названии
собственного вектора и собственного значения.

Собственный вектор эндоморфизма зависит от
выбора двух базисов. Однако когда мы
рассматриваем собственный вектор матрицы,
для нас важен не выбор базисов,
а матрица пассивного преобразования между этими базисами.
}

\DefLabeledDefinition{eigenvalues of pair of matrices}{\Product}
{
$A$\Hyph число $b$ называется
{\bf \ProductType собственным значением}
пары матриц $(f,g)$,
где $g$ - \ProductType невырожденная матрица,
если матрица
\DrawEq[f{}bg]{(f-ae)v matrix}{}
\ProductType вырожденная матрица.
}

\DefLabeledDefinition{eigenvector of pair of matrices}{\Product-\ColN}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением пары матриц
\ShowEq{pair of matrices \Product-\ColN},
где $g$ - \ProductType невырожденная матрица.
\ColC $v$ называется
{\bf собственн\ColB}
пары матриц $(f,g)$, соответствующ\FinB \ProductType собственному значению $b$,
если верно равенство
\DrawEq{\Product-eigen\Cols(f,g)}{}
}

\AddEq{proof: eigencolumn of matrix}
{
Определение
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN}
является следствием определения
\refDefinition{eigenvalues of pair of matrices}{\Product}
и теоремы
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\AddEq{proof: eigenrow of matrix}
{
Поскольку
\ShowEq{bg.\Product.g-}
то определение
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN}
является следствием определения
\refDefinition{eigenvalues of pair of matrices}{\Product}
и теоремы
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\AddEq{theorem: representation Ao2->V}
{
\begin{ShadedTheorem}
\labelTheorem{representation Ao2->V \SideNS}
Пусть $f$, $g(\Basis e)$
парные представления $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$
и $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть произведение в $D$\Hyph модуле
\AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{}
Тогда представление
\ShowEq{representation Ao2->V}
$D$\Hyph алгебры \AoxA A в $D$\Hyph модуле $V$
определеное равенством
\ShowEq{representation Ao2->V =}
является левым \AoxA A\Hyph модулем.
\end{ShadedTheorem}
}

\AddEq{theorem: twin representation in vector space}
{
\begin{ShadedTheorem}
\labelTheorem{twin representation in \SideWS vector space}
\ShowEq{Let V be vector space}{}
\ShowEq{f:A->*B}fAV
Эффективное \OtherSideRu востороннее представление
\ShowEq{f:A->*B}{g(\Basis e)}AV
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V$
зависит от базиса $\Basis e$ \SideRu вого $A$\Hyph векторного пространства $V$.
Следующая диаграмма
\newline
\DrawEq{twin representations of algebra}{\SideNS}
коммутативна для любых $a$, $b\in A$.
\end{ShadedTheorem}
}

\DefProof{twin representation in vector space}
{
Коммутативность диаграммы
\eqRef{twin representations of algebra}{\SideNS}
является следствием равенства
\eqRef{(av)b=a(vb)}{\SideNS}.
}

\DefLabeledDefinition{twin representation in vector space}{\SideNS}
{
Мы будем называть представления $f$ и $g(\Basis e)$,
рассмотренные в теореме
\RefTheorem{twin representation in \SideWS vector space},
{\bf парными представлениями}
$D$\Hyph алгебры $A$.
Равенство
\eqRef{(av)b=a(vb)}{\SideNS}
представляет
{\bf закон ассоциативности}
для парных представлений.
Это позволяет нам писать подобное выражение не пользуясь скобками.
}

\DefLabeledTheorem{set of similarity transformations}{\SideNS}
{
Пусть $V$ - \SideRu\-вое $A$\Hyph векторное пространство столбцов
и $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
Множество преобразований подобия
\ShowEq{\SideWS map a En}a{}
\SideRu вого $A$\Hyph векторного пространства $V$
является \OtherSideRu восторонним эффективным представлением
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V$.
}

\DefProof{set of similarity transformations}
{
Рассмотрим множество матриц
\ShowEq{\SideWS a En}
преобразований подобия
\ShowEq{\SideWS map a En}a{}
относительно базиса $\Basis e$.
Пусть $V^*$ - множество координат $V$\Hyph чисел
относительно базиса $\Basis e$.
Согласно теоремам
\RefTheorem{Geometric objects form A vector space, \SideNS-cols},
\RefTheorem{Geometric objects form A vector space, \SideNS-rows},
множество $V^*$ является \SideRu вым $A$\Hyph векторным пространством.
Согласно теореме
\refTheorem{similarity transformation}{\SideNS-\Cols}
отображение
\ShowEq{\SideWS map a En}a{}
является эндоморфизмом
\SideRu вого $A$\Hyph векторного пространства столбцов.

\ColRowLemma{map a in A->aE in hom is homomorphism}

\ColRowProof{map a in A->aE in hom is homomorphism}

\ColRowProof{set of similarity transformations 1}
}

\AddEq{proof: set of similarity transformations 1}
{
Согласно определению
\refDefinition{side representation of group}{\SideNS}
и лемме
\refLemma{map a in A->aE in hom is homomorphism}{\SideNS-\Cols},
отображение
\eqRef{a in A->aE hom \SideNS}{\Cols}
является \OtherSideRu восторонним представлением
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V^*$.
Согласно теореме
\RefTheorem{division algebra},
из равенства
\ShowEq{aEn=bEn \SideNS}
следует, что $a=b$.
Согласно определению
\RefDefinition{effective representation of algebra},
представление
\eqRef{a in A->aE hom \SideNS}{\Cols}
эффективно.

Согласно теоремам
\refTheorem{passive transformation and sum of endomorphisms}{\SideNS-\Cols},
\RefTheorem{passive transformation and product of endomorphisms, vector space, \SideNS-\Cols},
представление
\eqRef{a in A->aE hom \SideNS}{\Cols}
ковариантно относительно выбора базиса
\SideRu вого $A$\Hyph векторного пространства $V$.
Согласно теореме
\refTheorem{similarity transformation}{\SideNS-\Cols}
множество отображений
\ShowEq{\SideWS map a En}a{}
является \OtherSideRu восторонним представлением
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V$.
}

\DefLabeledLemma{map a in A->aE in hom is homomorphism}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
Отображение
\DrawEq{a in A->aE hom \SideNS}{\Cols}
является гомоморфизмом $D$\Hyph алгебры $A$.
}

\AddEq{proof: map a in A->aE in hom is homomorphism}
{
{\sc Доказательство.}
Согласно теореме
\refTheorem{homomorphism from A1 to A2, D algebra}1,
лемма является следствием равенств
\ShowEq{(a+b)aE \SideNS}
\ShowEq{(daE)v \SideNS}
\ShowEq{(ab)E \SideNS-\Cols}
\hfill\(\odot\)
}

\DefText{passive transformation and endomorphism}
{
Мы рассмотрим преобразование координат эндоморфизма
\SideRu вого $A$\Hyph векторного пространства \ColsA
в теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols}.
}

\DefLabeledTheorem{passive transformation and endomorphism}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
$\Basis e_1$, $\Basis e_2$ - базисы в \SideRu вом $A$\Hyph векторном пространстве $V$.
Пусть базисы $\Basis e_1$, $\Basis e_2$ связаны пассивным преобразованием $g$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}%g
Пусть $f$ - эндоморфизм \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть
\ShowEq{Ai, i=}f
- матрица эндоморфизма $f$ относительно базиса $\Basis e_i$.
Тогда
\DrawEq[fg{\SideNS}{\Cols}]{f2=a f1 a-}{g \SideNS-\Cols}
}

\AddEq[1]{remark: passive transformation and endomorphism}
{
Пусть
\ShowEq{Ai, i=}{#1}
- матрица вектора $#1$ относительно базиса $\Basis e_i$.
Тогда
\DrawEq[{#1}1{#1}2g{}]{v1=v2*a \SideNS-\Cols}{#1}
следует из теоремы
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\AddEq{proof: passive transformation and endomorphism}
{
{\sc Доказательство теоремы
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols}.}
Пусть эндоморфизм $f$ отображает вектор $v$ в вектор $w$
\DrawEq{w=f o v}{\SideNS-\Cols}
\ShowEq{passive transformation and endomorphism}

Согласно теореме
\refTheorem{homomorphism A module}{\SideNS-cols(1)},
равенства
\DrawEq[w1v1f1]{v1=v2*a \SideNS-\Cols}{v1}
\DrawEq[w2v2f2]{v1=v2*a \SideNS-\Cols}{v2}
являются следствием равенства
\eqRef{w=f o v}{\SideNS-\Cols}.
Равенство
\DrawEq[g]{w2=...v2 a f1 \SideNS-\Cols}g
является следствием равенств
\eqRef{v1=v2*a \SideNS-\Cols}v,
\eqRef{v1=v2*a \SideNS-\Cols}{v1},
\eqRef{v1=v2*a \SideNS-\Cols}w.
Так как $g$ - невырожденная матрица,
то равенство
\DrawEq[g]{w2=...v2 a f1 a- \SideNS-\Cols}g
является следствием равенства
\eqRef{w2=...v2 a f1 \SideNS-\Cols}g.
Равенство
\DrawEq[g]{v2 f2=v2 a f1 a- \SideNS-\Cols}g
является следствием равенств
\eqRef{v1=v2*a \SideNS-\Cols}{v2},
\eqRef{w2=...v2 a f1 a- \SideNS-\Cols}g.
Равенство
\eqRef{f2=a f1 a-}{g \SideNS-\Cols}
является следствием равенства
\eqRef{v2 f2=v2 a f1 a- \SideNS-\Cols}g.
\qed
}

\DefText[2]{coordinates of vector with respect to basis (1,2) cols}
{
Пусть
\DrawEq[{#1_i}n]{a=(a1.n col)}{#2,\SideNS-\Cols}
матрица координат вектора $\Vector{#1}$
относительно базиса
\ShowEq{Basis e i=1#2}
}

\DefText[2]{coordinates of vector with respect to basis (1,2) rows}
{
Пусть
\ShowEq{phantom a**b}
\DrawEq[{#1_i^{}{}}n]{a=(a1.n row)}{}
\ShowEq{phantom a**b}
матрица координат вектора $\Vector{#1}$
относительно базиса
\ShowEq{Basis e i=1#2}
}

\AddEq[2]{convention: passive transformation maps the basis 1->2}
{%
Пусть пассивное преобразование $g\in #1$ отображает базис \eV[1]
в базис \eV[2]
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{12 #2}
}

\DefLabeledTheorem{passive transformation of vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
\ShowConvention{passive transformation maps the basis 1->2}{G(V_*)}1
\ShowText{coordinates of vector with respect to basis (1,2) \Cols}v2
Преобразования координат
\DrawEq[v1v2g{}]{v1=v2*a \SideNS-\Cols}{v21g}
\DrawEq[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{12 \SideNS-\Cols}
не зависят от вектора $\Vector v$ или базиса $\Basis e$, а
определенно исключительно координатами вектора $\Vector v$
относительно базиса $\Basis e$.
}

\DefProof{passive transformation of vector space}
{
Согласно теореме
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
\ShowEq{v=vi ei 12, \SideNS-\Cols}
Равенство
\ShowEq{v1 cr e1=v2 cr g cr e1, \SideNS-\Cols}
является следствием равенств
\eqRef{e2i=aij e1j \Product-\Cols}{12 1},
\EqRef{v=vi ei 12, \SideNS-\Cols}.
Согласно теореме
\refTheorem{coordinates of vector}{\SideNS-\Cols},
преобразование координат
\eqRef{v1=v2*a \SideNS-\Cols}{v21g}
является следствием равенства
\EqRef{v1 cr e1=v2 cr g cr e1, \SideNS-\Cols}.
Так как $g$ - \ProductType невырожденная матрица, то
преобразование координат
\eqRef{v2=v1g-}{12 \SideNS-\Cols}
является следстием равенства
\eqRef{v1=v2*a \SideNS-\Cols}{v21g}.
}

\DefLabeledTheorem{passive transformation and sum of endomorphisms}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
Пусть эндоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства $V$ является суммой эндоморфизмов
$\Vector f_1$, $\Vector f_2$.
Матрица $f$ эндоморфизма $\Vector f$ равна сумме матриц $f_1$, $f_2$ эндоморфизмов
$\Vector f_1$, $\Vector f_2$
и это равенство не зависит от выбора базиса.
}

\AddEq{two endomorphisms and two bases}
{
Пусть $\Basis e$, $\Basis e'$ - базисы \SideRu вого $A$\Hyph векторного пространства $V$
и связаны пассивным преобразованием $g$
\ShowEq{\SideWS e'=e*a}{}
Пусть $f$
- матрица эндоморфизма $\Vector f$ относительно базиса $\Basis e$.
Пусть $f'$
- матрица эндоморфизма $\Vector f$ относительно базиса $\Basis e'$.
Пусть
\ShowEq{Ai, i=}f
- матрица эндоморфизма $\Vector f_i$ относительно базиса $\Basis e$.
Пусть
\ShowEq{Ai, i=}{f'}
- матрица эндоморфизма $\Vector f_i$ относительно базиса $\Basis e'$.
}

\DefProof{passive transformation and sum of endomorphisms}
{
\ShowEq{two endomorphisms and two bases}
Согласно теореме
\refTheorem{sum of homomorphisms, A vector space}{\SideNS-\Cols},
\DrawEq[{}{}]{f=f1+f2 endo}{\SideNS-\Cols}
\DrawEq[{'}{}]{f=f1+f2 endo}{\SideNS-\Cols'}
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[{}{}]{f'=g f g- \SideNS-\Cols}f
\DrawEq[1]{f'=g f g- \SideNS-\Cols}1
\DrawEq[2]{f'=g f g- \SideNS-\Cols}2
Равенство
\ShowEq{f1+f2=g.g- \SideNS-\Cols}
является следствием равенств
\ShowEq{f1+f2=g.g-}
Из равенств
\eqRef{f=f1+f2 endo}{\SideNS-\Cols'},
\EqRef{f1+f2=g.g- \SideNS-\Cols}
следует, что равенство
\eqRef{f=f1+f2 endo}{\SideNS-\Cols}
ковариантно относительно выбора базиса
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{theorem: passive transformation and product of endomorphisms}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation and product of endomorphisms, vector space, \SideNS-\Cols}
\ShowEq{Let V be vector space of}.
Пусть эндоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства $V$
является произведением эндоморфизмов
$\Vector f_1$, $\Vector f_2$.
Матрица $f$ эндоморфизма $\Vector f$ равна
\ProductType произведению матриц
\ShowEq{f1 f2 \SideNS}
эндоморфизмов
\ShowEq{vf1 vf2 \SideNS}
и это равенство не зависит от выбора базиса.
\end{ShadedTheorem}
}

\DefLabeledDefinition{coordinates of geometric object, vector space}{\SideNS-\Cols}
{
Мы будем называть
орбиту
\ShowEq{def coordinates of geometric object, \SideNS-\Cols}
представления $F_1$
многообразием {\bf координат геометрического объекта}
в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsNA.
Для любого базиса
\newline
\FrameEqRef[{V1}{V2}g{}]{e2i=aij e1j \Product-\Cols}{GOeV}
\newline
соответствующая точка
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
орбиты  определяет
{\bf координаты геометрического объекта}
в координатном \SideRu вом $A$\Hyph векторном пространстве
относительно базиса \eV[V2].
}

\DefLabeledDefinition{Left and Right Eigenvalues}{\SideNS-\Cols}
{
Пусть $a_2$ - \nTimes матрица,
которая \ProductType подобна диагональной матрице $a_1$
\ShowEq{D diagonal matrix}{a_1}n
Следовательно, существует \ProductType невырожденая матрица $u_2$ такая, что
\DrawEq{U-*A*U=D \Product-\SideNS}1
\DrawEq[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
\ColC
\ShowEq{ARow u2i \Cols}u2i
матрицы $u_2$ удовлетворяет равенству
\DrawEq[2u]{A*Ui=Ui di \Product-\SideNS}u
$A$\Hyph число $b(\gi i)$ называется \SideRu вым \ProductType {\bf собственным значением}.
Вектор\Hyph\ColWS
\ShowEq{ARow u2i \Cols}u2i
называется
\AddIndex{собственн\ColBNS}{eigen\ColN},
соответствующ\FinB \SideRu вому \ProductType собственному значению $b(\gi i)$.
}

\DefLabeledTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
{
Собственный вектор
\ShowEq{ARow u2i \Cols}u2i
матрицы $a_2$,
соответствующий \SideRu вому \ProductType собственному значению $b(\gi i)$,
не зависит от выбора базиса $\Basis e_2$
\ShowEq{e1i=u2i*e2 \SideNS-\Cols}
}

\AddEq{remark: Eigenvector does not depend on basis}
{
Равенство
\EqRef{e1i=u2i*e2 \SideNS-\Cols}
является следствием равенства
\eqRef{e2i=aij e1j \Product-\Cols}{21u2}.
Однако смысл этих равенств различный.
Равенство
\eqRef{e2i=aij e1j \Product-\Cols}{21u2}
является представлением пассивного преобразования.
Мы видим
в равенстве
\EqRef{e1i=u2i*e2 \SideNS-\Cols}
разложение собственного вектора
для данного \SideRu вого \ProductType собственного значения относительно выбранного базиса.
Задача доказательства теоремы
\refTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
- раскрыть смысл равенства
\EqRef{e1i=u2i*e2 \SideNS-\Cols}.
}

\DefProof{Eigenvector does not depend on basis}
{
Согласно теореме
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)},
мы можем рассматривать матрицу $a_2$ как матрицу автоморфизма $a$
\SideRu вого $A$\Hyph векторного пространства относительно базиса $\Basis e_2$.
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
матрица $u_2$ является матрицей пассивного преобразования
\DrawEq[21u2]{e2i=aij e1j \Product-\Cols}{21u2}
и матрица $a_1$ является матрицей автоморфизма $a$
\SideRu вого $A$\Hyph векторного пространства относительно базиса $\Basis e_1$.

Матрица координат базиса $\Basis e_1$ относительно базиса $\Basis e_1$
- это единичная матрица $\aD En$.
Следовательно, вектор
\ShowEq{ARow u2i \Cols}e1i
является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductType собственному значению $b(\gi i)$
\DrawEq[1e]{A*Ui=Ui di \Product-\SideNS}e
Равенство
\ShowEq{U-*A*U*E=E*D \Product-\SideNS}
является следствием равенств
\eqRef{U-*A*U=D \Product-\SideNS}1,
\eqRef{A*Ui=Ui di \Product-\SideNS}e.
Равенство
\ShowEq{A*U*E=U*E*D \Product-\SideNS}
является следствием равенства
\EqRef{U-*A*U*E=E*D \Product-\SideNS}.
Равенство
\ShowEq{U*Ei=Ui \Product-\SideNS}
является следствием равенств
\eqRef{A*Ui=Ui di \Product-\SideNS}u,
\EqRef{A*U*E=U*E*D \Product-\SideNS}.
Теорема является следствием равенств
\eqRef{e2i=aij e1j \Product-\Cols}{21u2},
\EqRef{U*Ei=Ui \Product-\SideNS}.
}

\DefLabeledTheorem{right eigenvalue is eigenvalue}{\SideNS-\Cols}
{
Любое \SideRu вое \ProductType собственное значение $b(\gi i)$
является \ProductType собственным значением.
Собственн\ColumnC $\ARow ui$,
соответствующ\endC \SideRu вому \ProductType собственному значению $b(\gi i)$,
является собственн\ColBNS,
соответствующ\FinB \ProductType собственному значению $b(\gi i)$.
}

\DefProof{right eigenvalue is eigenvalue}
{
Все элементы строки матрицы
\DrawEq{a1-di En}{\Product-\SideNS}
равны нулю.
Следовательно, матрица
\eqRef{a1-di En}{\Product-\SideNS}
\ProductType вырождена
и \SideRu вое \ProductType собственное значение $b(\gii)$
является \ProductType собственным значением.
Поскольку
\DrawEq{e1ij=01 \Cols}{\SideNS}
то собственный вектор
\ShowEq{ARow u2i \Cols}e1i,
соответствующий \SideRu вому \ProductType собственному значению $b(\gii)$,
является собственным вектором, соответствующим \ProductType собственному значению $b(\gii)$.
Равенство
\ShowEq{a1*e1=di e1 \Product-\SideNS}
является следствием определения
\refDefinition{eigenvector of matrix}{\Product-\Cols}.

Из равенства
\eqRef{U-*A*U=D \Product-\SideNS}1
следует, что мы можем записать матрицу
\eqRef{a1-di En}{\Product-\SideNS}
в виде
\ShowEq{U-*A*U-di En \Product-\SideNS}
Так как матрица
\eqRef{a1-di En}{\Product-\SideNS}
\ProductType вырождена,
то матрица
\ShowEq{A-U-*di*U \Product-\SideNS}
также \ProductType вырождена.
Следовательно,
\SideRu вое \ProductType собственное значение $b(\gii)$ матрицы $a_2$
является \ProductType собственным значением
пары матриц $(a_2,u_2)$.

Равенства
\ShowEq{U-*A*U*e1=di e1 \Product-\SideNS}
\ShowEq{A*U*e1=... \Product-\SideNS}
являются следствием равенств
\eqRef{U-*A*U=D \Product-\SideNS}1,
\EqRef{a1*e1=di e1 \Product-\SideNS}.
Из равенств
\EqRef{e1i=u2i*e2 \SideNS-\Cols},
\EqRef{A*U*e1=... \Product-\SideNS}
и из теоремы
\refTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
следует, что
собственн\ColumnC
\ShowEq{ARow u2i \Cols}u2i
матрицы $a_2$,
соответствующий \SideRu вому \ProductType собственному значению $b(\gi i)$,
является
собственн\ColB
\ShowEq{ARow u2i \Cols}u2i
пары матриц $(a_2,u_2)$, соответствующ\FinB \ProductType собственному значению $b(\gii)$.
}

\DefLabeledRemark{right eigenvalue is eigenvalue}{\SideNS-\Cols}
{
Равенство
\ShowEq{di*ui=ui*di \Product-\SideNS}
является следствием теоремы
\refTheorem{right eigenvalue is eigenvalue}{\SideNS-\Cols}.
Равенство
\EqRef{di*ui=ui*di \Product-\SideNS}
кажется необычным.
Однако, если мы его слегка изменим
\ShowEq{di*ui=ui*di 1 \Product-\SideNS}
то равенство
\EqRef{di*ui=ui*di 1 \Product-\SideNS}
следует из равенства
\EqRef{e1i=u2i*e2 \SideNS-\Cols}.
}

\DefLabeledTheorem[1]{Eigenvalue a ox a, c in AAA[b]}{\SideNS-\Cols}
{
Пусть вектор\Hyph\ColWS $v$ является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$
матрицы $a$.
Пусть $A$\Hyph число $b$ удовлетворяет условию
\DrawEq[b{}{s#1}]{b in AAA[a]}{bs#1-\Cols}
Тогда
для любого многочлена
\DrawEq{p(c) p in D}{\SideNS-\Cols}
вектор\Hyph\ColWS
\ShowEq{eigenvector cv \SideNS-\Cols}
\ShowEq{c=p(b)}
также является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$.
}

\DefProof[2]{Eigenvalue a ox a, c in AAA[b]}
{
Согласно теореме
\RefTheorem{c in Za=> p(c) in Za},
равенство
\ShowEq{as ox as o cv = ..., \SideNS-\Cols}
является следствием условия
\eqRef{b in AAA[a]}{bs#1-\Cols}.
Согласно определению
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols},
из равенства
\EqRef{as ox as o cv = ..., \SideNS-\Cols}
следует, что
вектор\Hyph\ColWS $#2$ является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$
матрицы $a$.
}

\DefLabeledDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
{
$A$\Hyph число $b$ называется
\SideRu вым \ProductTypeO {\bf собственным значением}
матрицы $a$,
если существует вектор\Hyph\ColWS $v$ такой, что
\DrawEq[v]{Eigenvalue of Linear Map \SideNS-\Cols}d
Вектор\Hyph\ColWS $v$ называется
{\bf собственн\ColBNS}, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$.
}

\DefLabeledTheorem[1]{Eigenvalue of Linear Map a ox a, 1}{\SideNS-\Cols}
{
Пусть элементы матрицы $a$ удовлетворяют равенству
\DrawEq{as ox as=a1 ox a2, #1}{\SideNS-\Cols}
Тогда \SideRu вое \ProductTypeO собственное значение $b$
является \SideRu вым \ProductType собственным значением матрицы $a_{#1}$.
}

\DefProofRef[1]{Eigenvalue of Linear Map a ox a, 1}{\SideNS-\Cols}
{
Равенство
\DrawEq{as ox as o v = v a12, #1, \Cols}{1-\SideNS}
является следствием равенства
\FrameEqRef{as ox as=a1 ox a2, #1}{\SideNS-\Cols}.
\newline
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols}
является следствием равенства
\eqRef{as ox as o v = v a12, #1, \Cols}{1-\SideNS}.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}
является следствием определения
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
\SideRu вого \ProductTypeO собственного значения
матрицы $a$.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
является следствием равенств
\EqRef{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols},
\EqRef{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}.
Теорема является следствием равенства
\EqRef{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
и определения
\refDefinition{Left and Right Eigenvalues}{\SideNS-\Cols}
\SideRu вого \ProductType собственного значения
матрицы $a_{#1}$.
}

\DefLabeledTheorem[1]{Eigenvalue of Linear Map a ox a, 2}{\SideNS-\Cols}
{
Пусть элементы матрицы $a$ удовлетворяют равенству
\DrawEq{as ox as=a1 ox a2, #1}{\SideNS-\Cols}
Тогда \SideRu вое \ProductTypeO собственное значение $b$
является \ProductTypeA собственным значением матрицы $a_{#1}$.
}

\DefProofRef[1]{Eigenvalue of Linear Map a ox a, 2}{\SideNS-\Cols}
{
Равенство
\DrawEq{as ox as o v = v a12, #1, \Cols}{2-\SideNS}
является следствием равенства
\FrameEqRef{as ox as=a1 ox a2, #1}{\SideNS-\Cols}.
\newline
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols}
является следствием равенства
\eqRef{as ox as o v = v a12, #1, \Cols}{2-\SideNS}.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}
является следствием определения
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
\SideRu вого \ProductTypeO собственного значения
матрицы $a$.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
является следствием равенств
\EqRef{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols},
\EqRef{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}.
Теорема является следствием равенства
\EqRef{as ox as o v = v a12, matrix, #1 \SideNS-\Cols},
определения
\refDefinition{eigenvalue of matrix}{\ProductA}
\ProductType собственного значения
матрицы $a_{#1}$
и определения
\refDefinition{eigenvector of matrix}{\ProductA-\Cols}
соответствующего собственного вектора $v$.
}

\DefLabeledTheoremNote[1]{n eigenvectors}{#1}
{
Пусть $\Base$ - \AlgebraRu
и $V$ - $\Base$\Hyph векторное пространство.
Если эндоморфизм имеет $\gik$ различных
собственных значений\,\footnotemark
\ShowEq{di 1n}bk,
то собственные вектора
\ShowEq{di 1n}vk,
относящиеся к различным собственным значениям,
линейно независимы.
}
{
Смотри также теорему на странице
\citeBib{Kurosh: High Algebra}\Hyph 210.
}

\AddEq{remark: n eigenvectors}
{
Однако теорема
\refTheorem{n eigenvectors}{algebra}
не верна.
Мы рассмотрим отдельно доказательства
для левого и правого $A$\Hyph векторного пространств.
}

\DefProof{n eigenvectors}
{
Мы будем доказывать теорему индукцией по $\gik$.

Поскольку собственный вектор отличен от нуля, теорема верна для $\gik=\gi 1$.

\begin{Statement}
\labelStatement{theorem is true for k=m-1 \SideNS}
Пусть теорема верна для $\gik=\gim-\gi 1$.
\hfill\(\odot\)
\end{Statement}

\begin{sloppypar}
Согласно теоремам
\ShowEq{ref 1 for n eigenvectors}
мы можем положить, что
\ShowEq{e2=e1}
Пусть
\ShowEq{di 1n+1}bm{}
- различные собственные значения и
\ShowEq{di 1n+1}vm{}
- соответствующие собственные векторы
\ShowEq{fovi=di vi \SideNS}
\ShowEq{di ne dj}
Пусть утверждение
\RefStatement{ai vi=0 \SideNS}
верно.
\end{sloppypar}

\begin{Statement}
\labelStatement{ai vi=0 \SideNS}
Существует линейная зависимость
\ShowEq{ai vi=0 \SideNS}
где
\ShowEq{a1 ne 0}
\hfill\(\odot\)
\end{Statement}

Равенство
\ShowEq{ai f vi=0 \SideNS}
является следствием равенства
\EqRef{ai vi=0 \SideNS}
и теоремы
\ShowEq{ref 2 for n eigenvectors}
Равенство
\ShowEq{ai di vi=0 \SideNS}
является следствием равенств
\EqRef{fovi=di vi \SideNS},
\EqRef{ai f vi=0 \SideNS}.
Так как произведение не коммутативно,
мы не можем упростить выражение
\EqRef{ai di vi=0 \SideNS}
до линейной зависимости.
}

\AddEq{remark: Eigenvalue and conjugate class}
{
Из теорем
\refTheorem{Eigenvalue and conjugate class}{\SideNS-\Cols},
\refTheorem{Coefficient comutes with matrix}{\SideNS-\Cols}
следует, что множество собственных \ColsNA,
соответствующих данному \SideRu вому \ProductType собственному значению,
не является $A$\Hyph векторным пространством.
}

\DefLabeledTheorem{Eigenvalue and conjugate class}{\SideNS-\Cols}
{
Пусть $A$\Hyph число $b$ - \SideRu вое \ProductType собственное значение матрицы
$a_2$.\refFootnote{Eigenvalue and conjugate class}{\Product}
Тогда любое $A$\Hyph число, $A$\Hyph сопряжённое с $A$\Hyph числом $b$,
является \SideRu вым \ProductType собственным значением матрицы $a_2$.
}

\DefLabeledFootnote{Eigenvalue and conjugate class}{\Product}
{
Смотри аналогичное утверждение и доказательство на странице
\citeBib{Cohn: Skew Fields}\Hyph 375.
}

\DefProof{Eigenvalue and conjugate class}
{
Пусть $v$ -
собственн\ColumnCNS, соответствующ\FinB \SideRu вому \ProductType собственному значению $b$.
Пусть $c\ne 0$ - $A$\Hyph число.
Утверждение теоремы является следствием равенства
\ShowEq{conjugate eigenvalue \SideNS-\Cols}
}

\DefLabeledTheorem[2]{Coefficient comutes with matrix}{\SideNS-\Cols}
{
Пусть $v$ - собственн\ColumnCNS, соответствующ\endC \SideRu вому \ProductType собственному значению $b$.
Вектор $#1#2$
является собственн\ColB, соответствующ\FinB \SideRu вому \ProductType собственному значению $b$
тогда и только тогда, когда
$A$\Hyph число $c$ коммутирует со всеми элементами матрицы $a_2$.
}

\DefProof[2]{Coefficient comutes with matrix}
{
Вектор $#1#2$
является собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductType собственному значению $b$
тогда и только тогда, когда
верно следующее равенство
\ShowEq{Coefficient comutes with matrix \SideNS-\Cols}
Равенство
\EqRef{Coefficient comutes with matrix \SideNS-\Cols}
верно тогда и только тогда, когда
$A$\Hyph число $c$ коммутирует со всеми элементами матрицы $a_2$.
}

\DefLabeledDefinition{geometric object, vector space}{\SideNS-\Cols}
{
Допустим даны координаты $w_1$ вектора $\Vector w$
относительно базиса  \eV[W1][.]
Мы будем называть
множество векторов
\DrawEq[w2{w_2}{W2}]{geometric object representative, \SideNS-\Cols}{w=we}
{\bf геометрическим объектом},
определённым в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsNA.
Для любого базиса  \eV[W2][,]
соответствующая точка
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
многообразия координат определяет вектор
\DrawEq[w2{w_2}{W2}]{geometric object representative, \SideNS-\Cols}{w=we 1}
который называется
{\bf представителем геометрического объекта}
в \SideRu вом $A$\Hyph векторном пространстве $V$ в базисе \eV[V2][.]
}

\AddEq{remark: geometric object, vector space}
{
Так как геометрический объект - это орбита представления,
то согласно теореме
\RefTheorem{proper definition of orbit}
определение геометрического объекта корректно.

Мы будем также говорить, что $\Vector w$ - это
\AddIndex{геометрический объект типа $F$}{type of geometric object}.

Определения
\refDefinition{coordinates of geometric object, vector space}{\SideNS-cols},
\refDefinition{coordinates of geometric object, vector space}{\SideNS-rows}
строят геометрический объект в координатном пространстве.
Определения
\refDefinition{geometric object, vector space}{\SideNS-cols},
\refDefinition{geometric object, vector space}{\SideNS-rows}
предполагают,
что мы выбрали базис в векторном пространстве $W$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.
}

\DefText{Geometric Object of Vector Space}
{
\begin{sloppypar}
Предположим, что $V$, $W$ - \SideRu вые $A$\Hyph векторные пространства \ColsA.
Пусть $G(V_*)$ -  группа симметрий
\SideRu вого $A$\Hyph векторного пространства $V$.
Гомоморфизм
\DrawEq[F{G(V_*)}{GL(W_*)}{}]{f: A->B}{FG \SideNS-\Cols}
отображает пассивное преобразование $g\in G(V_*)$
\DrawEq[{V1}{V2}g{}]{e2i=aij e1j \Product-\Cols}{GOeV}
\SideRu вого $A$\Hyph векторного пространства $V$
в пассивное преобразование
\ShowEq{Fg in GL}
\DrawEq[{W1}{W2}{F(g)}{}]{e2i=aij e1j \Product-\Cols}{GOeW}
\SideRu вого $A$\Hyph векторного пространства $W$.
\end{sloppypar}

Тогда координатное преобразование в
\SideRu вом $A$\Hyph векторном пространстве $W$ принимает вид
\DrawEq{coordinate transformation, vector space W, \SideNS-\Cols}1
Следовательно, отображение
\DrawEq{F1(g)=F(g)**-\Product}{\SideNS}
является \OtherSideRu восторонним представлением
\ShowEq{f:A->*B}{F_1}{G(V_*)}{W_*}
группы $G(V_*)$ на множестве $W_*$.
}

\DefProof{passive transformation and product of endomorphisms}
{
\ShowEq{two endomorphisms and two bases}
Согласно теореме
\RefTheorem{product of homomorphisms, \SideWS A vector space, \ColN},
\DrawEq[{}{}]{f=f1*f2 endo \SideNS-\Cols}{\Product}
\DrawEq[{'}{}]{f=f1*f2 endo \SideNS-\Cols}{\Product'}
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[{}{}]{f'=g f g- \SideNS-\Cols}{f*}
\DrawEq[1]{f'=g f g- \SideNS-\Cols}{1*}
\DrawEq[2]{f'=g f g- \SideNS-\Cols}{2*}
Равенство
\ShowEq{f1*f2=g.g- \SideNS-\Cols}
является следствием равенств
\ShowEq{f1*f2=g.g-}
Из равенств
\eqRef{f=f1*f2 endo \SideNS-\Cols}{\Product'},
\EqRef{f1*f2=g.g- \SideNS-\Cols}
следует, что равенство
\eqRef{f=f1*f2 endo \SideNS-\Cols}{\Product}
ковариантно относительно выбора базиса
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{theorem: finite dimension->representation is free}
{
\begin{ShadedTheorem}
\labelTheorem{finite dimension->representation is free, \SideNS}
Если \SideRu вое $A$\Hyph векторное пространство $V$
имеет конечную размерность,
то соответствующее представление свободно.
\end{ShadedTheorem}
}

\DefProof{finite dimension->representation is free}
{
Теорема является следствием определения
\RefDefinition{free representation of algebra}
и теорем
\refTheorem{av=bv=>a=b}{\SideNS-cols},
\refTheorem{av=bv=>a=b}{\SideNS-rows}.
}

\AddEq[1]{Let V be vector space}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство#1
}

\AddEq[1]{Let V be vector space of}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsNA#1
}

\AddEq{Let V be vector space of and}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsA и
}

\AddEq{Let V be vector space of and basis}
{
\ShowEq{Let V be vector space of and}
$\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{Let V be vector space and basis}
{
\ShowEq{Let V be vector space}{}
и $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{remark: automorphism of vector space, group}
{
\ShowEq{Let V be vector space of}.
Мы доказали в теореме
\refTheorem{automorphism of vector space}{\Product-\Cols},
что если задан базис
\SideRu вого $A$\Hyph векторного пространства $V$,
то любой автоморфизм $\Vector f$
\SideRu вого $A$\Hyph векторного пространства $V$ можно отождествить
с \ProductType невырожденной матрицей $f$.
Соответствующее преобразование координат вектора
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{}
называется
\AddIndex{линейным преобразованием}{linear transformation}.
}

\DefLabeledDefinition{Symmetry Group}{\SideNS-\Cols}
{
Нормальная подгруппа $G(V)$ группы $GL(V)$, которая порождает
автоморфизмы, сохраняющие свойства заданной структуры
называется
{\bf группой симметрии}.

Не нарушая общности, мы будем отождествлять элемент $g$ группы $G(V)$
с соответствующим автоморфизмом
и записывать его действие на вектор $v\in V$ в виде
\ShowEq{v*g, \SideNS-\Cols}
}

\DefText{definition: linear G* representation}
{
Мы будем называть \OtherSideRu востороннее представление
группы $G$ в \SideRu вом $A$\Hyph векторном пространстве
\AddIndex{линейным $G$\Hyph представлением}{linear G* representation}.
}

\DefText{linear G* representation}
{
Если в \SideRu вом $A$\Hyph векторном пространстве $V$ определена дополнительная структура,
не всякий автоморфизм сохраняет свойства заданной структуры.
Например, если мы определим норму в
\SideRu вом $A$\Hyph векторном пространстве $V$,
то для нас интересны автоморфизмы, которые сохраняют норму вектора.
}

\DefLabeledDefinition{active G-representation}{\SideNS}
{
Мы будем называть \OtherSideRu востороннее представление
группы $G(V)$ на множестве базисов \SideRu вого $A$\Hyph векторного пространства $V$
\AddIndex{активным \SideRu восторонним $G$\Hyph представлением}
{active representation, vector space}.
}

\DefText{active G-representation}
{
Если базис \eV задан, то
мы можем отождествить автоморфизм
\SideRu вого $A$\Hyph векторного пространства $V$
и его координаты относительно базиса \eV[][.]
Множество $G(V_*)$ координат автоморфизмов
относительно базиса \eV является группой,
изоморфной группе $G(V)$.

Не всякие два базиса могут быть связаны
преобразованием группы симметрии
потому, что не всякое невырожденное линейное преобразование принадлежит
представлению группы $G(V)$.
Таким образом, множество базисов
можно представить как объединение орбит группы $G(V)$.
В частности, если базис $\eV\in G(V)$,
то орбита базиса \eV совпадает с группой $G(V)$.
}

\DefLabeledTheorem{representation on basis manifold, vector space}{\SideNS}
{
Активное \OtherSideRu востороннее $G(V)$\Hyph представление на многообразии базисов
однотранзитивно.
}

\DefProof{representation on basis manifold, vector space}
{
Теорема является следствием теоремы
\refTheorem{active representation is single transitive}{\SideNS-cols},
и определений
\refDefinition{basis manifold of vector space}{\SideNS-cols},
а также теорема является следствием теоремы
\refTheorem{active representation is single transitive}{\SideNS-rows}
и определений
\refDefinition{basis manifold of vector space}{\SideNS-rows}.
}

\DefLabeledDefinition{basis manifold of vector space}{\SideNS-\Cols}
{
Мы будем называть орбиту
\ShowEq{basis manifold of vector space, \SideNS-\Cols}
выбранного базиса $\Basis e$
{\bf многообразием базисов}
\SideRu вого $A$\Hyph векторного пространства $V$ \ColsA.
}

\DefLabeledTheorem{active transformations, vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Автоморфизмы \SideRu вого $A$\Hyph векторного пространства \ColsA порождают
\OtherSideRu востороннее линейное
эффективное \Group nA\Hyph представление.
}

\DefProof{active transformations, vector space}
{
Пусть $a$, $b$ - матрицы автоморфизмов $\Vector a$ и $\Vector b$
относительно базиса $\Basis e$.
Согласно теореме
\refTheorem{homomorphism A module}{\SideNS-\Cols(1)}
преобразование координат имеет вид
\DrawEq[{v'}{}v{}a{}]{v1=v2*a \SideNS-\Cols}{v'}
\DrawEq[{v''}{}{v'}{}b{}]{v1=v2*a \SideNS-\Cols}{v''}
Равенство
\ShowEq{a*b, \SideNS-\Cols}
\DrawEq[{v''}{}v{}{\TheProduct}{}]{v1=v2*a \SideNS-\Cols}{}
\begin{sloppypar}
\noindent
является следствием равенств
\eqRef{v1=v2*a \SideNS-\Cols}{v'},
\eqRef{v1=v2*a \SideNS-\Cols}{v''}.
Согласно теореме
\RefTheorem{product of homomorphisms, \SideWS A vector space, \ColN},
произведение автоморфизмов $\Vector a$ и $\Vector b$
имеет матрицу \TheProduct.
Следовательно, автоморфизмы \SideRu вого $A$\Hyph векторного пространства \ColsA порождают
\OtherSideRu востороннее линейное
\Group nA\Hyph представление.
\end{sloppypar}

Нам осталось показать,
что ядро неэффективности состоит только
из единичного элемента. Тождественное преобразование
удовлетворяет равенству
\ShowEq{active transformations, vector space, 2, \SideNS-\Cols}
Выбирая значения координат в форме
\ShowEq{ai=delta ik, \Cols},
где $\gik$ задано, мы получим
\ShowEq{identity transformation, vector space, \SideNS-\Cols}
Из \EqRef{identity transformation, vector space, \SideNS-\Cols} следует
\ShowEq{identity transformation, vector space, 1, \Cols}
Поскольку $\gik$ произвольно, мы приходим к заключению $a=\delta$.
}

\DefLabeledTheorem{active transformations, basis, vector space}{\SideNS-\Cols}
{
Автоморфизм $a$, действуя на каждый вектор базиса
в \SideRu вом $A$\Hyph векторном пространстве \ColsA,
отображает базис в другой базис.
}

\DefProof{active transformations, basis, vector space}
{
Пусть $\Basis e$ - базис в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsA.
Согласно теореме
\refTheorem{automorphism of vector space}{\Product-\Cols},
вектор
\ShowEq{vector of basis \Cols}e
отображается в вектор
\ShowEq{vector of basis \Cols}{e'}
\DrawEq{automorphism, vector space, 1, \SideNS-\Cols}1
\begin{sloppypar}
\noindent
Если векторы
\ShowEq{vector of basis \Cols}{e'}
линейно зависимы,
то в линейной комбинации
\ShowEq{automorphism, vector space, 2, \SideNS-\Cols}
\end{sloppypar}
\noindent
$\lambda\ne 0$.
Из равенств \eqRef{automorphism, vector space, 1, \SideNS-\Cols}1
и \EqRef{automorphism, vector space, 2, \SideNS-\Cols} следует, что
\ShowEq{automorphism, vector space, 3, \SideNS-\Cols}
и $\lambda\ne 0$. Это
противоречит утверждению, что векторы
\ShowEq{vector of basis \Cols}e
линейно независимы.
Следовательно, векторы
\ShowEq{vector of basis \Cols}{e'}
линейно независимы
и порождают базис.
}

\DefText{extend linear representation to set of bases 1}
{
Таким образом, мы можем распространить
\OtherSideRu востороннее линейное $GL(V_*)$\Hyph представление
в \SideRu вом $A$\Hyph векторном пространстве $V_*$
на множество базисов
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\DefText{extend linear representation to set of bases 2}
{
Мы будем называть преобразование этого \OtherSideRu востороннего представления
на множестве базисов
\SideRu вого $A$\Hyph векторного пространства $V$
\AddIndex{активным преобразованием}{active transformation, vector space}
потому, что гоморфизм \SideRu вого $A$\Hyph векторного пространства породил это преобразование
(\BlueText{Смотри также определение в разделе
\citeBib{Korn}\Hyph 14.1\Hyph 3,
а также определение на странице
\citeBib{Rashevsky}\Hyph 214}).

\ePrints{2022.01.05,2022.11.26}%
\ifx\Semafor\ValueOn%
\FrameCiteBib{Korn}

\FrameCiteBib{Rashevsky}
\fi
}

\DefText{extend linear representation to set of bases 3}
{
\begin{sloppypar}
Соответственно определению мы будем записывать действие
активного преобразования $a\in GL(V_*)$ на базис $\Basis e$ в форме
\ShowEq{active transformation, vector space, \SideNS-\Cols}.
Рассмотрим равенство
\DrawEq{active transformation ae x=a ex, \SideNS-\Cols}1
Выражение
\ShowEq{active transformation, vector space, \SideNS-\Cols}{}
в левой части равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
является образом базиса \eV при активном преобразовании $a$.
Выражение
\ShowEq{active transformation ae x=a ex 1, \SideNS-\Cols}
в правой части равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
является разложением вектора $\Vector v$ относительно базиса \eV[][.]
Следовательно,
выражение в правой части равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
является образом вектора $\Vector v$ относительно эндоморфизма $a$
и выражение в левой части равенства
\newline
\FrameEqRef{active transformation ae x=a ex, \SideNS-\Cols}1
\newline
является разложением образа вектора $\Vector v$
относительно образа базиса \eV[][.]
Следовательно, из равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
следует, что эндоморфизм $a$ \SideRu вого $A$\Hyph векторного пространства и
соответствующее активное преобразование $a$ действуют синхронно
и координаты $a\circ \Vector v$ образа вектора $\Vector v$ относительно
образа
\ShowEq{active transformation, vector space, \SideNS-\Cols}{}
базиса \eV
совпадают с координатами вектора $\Vector v$ относительно базиса $\Basis e$.
\end{sloppypar}
}

\DefLabeledTheorem{active representation is single transitive}{\SideNS-\Cols}
{
Активное \OtherSideRu востороннее \Group nA\Hyph представление на множестве базисов
однотранзитивно.
Множество базисов, отождествлённое с траекторией
\ShowEq{basis manifold of V, \SideNS-\Cols}e{\Group nA}{}
активного \OtherSideRu востороннего \Group nA\Hyph представления
называется
{\bf многообразием базисов}
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\DefLabeledTheorem{exists representation, commuting with active}{\SideNS-\Cols}
{
На многообразии базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
\SideRu вого $A$\Hyph векторного пространства \ColsA
существует однотранзитивное
\SideRu востороннее $G(V)$\Hyph представление, перестановочное с активным.
}

\AddEq{proof: exists representation, commuting with active}
{
\begin{sloppypar}
\begin{proof}
Из теоремы
\refTheorem{representation on basis manifold, vector space}{\SideNS}
следует, что многообразие базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
является однородным пространством группы $G$.
Теорема является следствием теоремы
\RefTheorem{two representations of group}.
\end{proof}
\end{sloppypar}
}

\AddEq{remark: passive transformation, vector space}
{
\ePrints{2022.11.26,MObject}%
\ifx\Semafor\ValueOn%
Преобразование
\else
Как мы видим из замечания
\RefRemark{one representation of group}
преобразование
\fi
\SideRu востороннего $G(V)$\Hyph представления отличается от активного преобразования
и не может быть сведено к
преобразованию пространства $V$.
}

\DefLabeledDefinition{passive transformation, vector space}{\SideNS-\Cols}
{
Преобразование
\SideRu востороннего $G(V)$\Hyph представления называется
{\bf пассивным преобразованием}
многообразия базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
\SideRu вого $A$\Hyph векторного пространства \ColsA,
а \SideRu востороннее $G(V)$\Hyph представление называется
{\bf пассивным \SideRu восторонним $G(V)$\Hyph представлением}.
Согласно определению
мы будем записывать пассивное преобразование базиса $\Basis e$,
порождённое элементом $a\in G(V)$, в форме
\ShowEq{passive transformation symbol, \SideNS-\Cols}
}

\AddEq[1]{table: Passive and Active Representations}
{
\ShowEq{def #1}\SideRu вое $A$\Hyph векторное&\ShowEq{def #1}\ShowEq{\DefRow}\Group nA&
\ShowEq{def #1}\OtherSideRu востороннее&\ShowEq{def #1}\SideRu востороннее\\
пространство строк&&&\\
\hline
\ShowEq{def #1}\SideRu вое $A$\Hyph векторное&\ShowEq{def #1}\ShowEq{\DefCol}\Group nA&
\ShowEq{def #1}\OtherSideRu востороннее&\ShowEq{def #1}\SideRu востороннее\\
пространство столбцов&&&\\
\hline
}

\DefLabeledTheorem{principle of covariance}{\SideNS}%-\Cols}
{
{\bf(Принцип ковариантности).}
Представитель геометрического объекта не зависит от выбора
базиса \eV[V2][.]
}

\DefProof{principle of covariance}
{
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Basis e_V$,
базис $\Basis e_W$
и координаты геометрического объекта $w^\alpha$.
Соответствующий представитель геометрического объекта
имеет вид
\DrawEq[w{}wW]{geometric object representative, \SideNS-\Cols}{}
Предположим базис $\Basis e'_V$ связан
с базисом $\Basis e_V$
пассивным преобразованием
\DrawEq[V]{passive transformation e->e', \SideNS-\Cols}{}
Согласно построению это порождает пассивное преобразование
\newline
\FrameEqRef[{W1}{W2}{F(g)}{}]{e2i=aij e1j \Product-\Cols}{GOeW}
\newline
и координатное преобразование
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
Соответствующий представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3, \SideNS-\Cols}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
}

\AddEq{definition: sum of geometric objects}
{
\begin{ShadedDefinition}
\labelDefinition{sum of geometric objects, \SideNS-\Cols}
\ShowEq{Let V be vector space of and}
\ShowEq{sum of geometric objects, 1}
геометрические объекты одного и того же типа,
определённые в \SideRu вом $A$\Hyph векторном пространстве $V$.
Геометрический объект
\ShowEq{sum of geometric objects, 2}
называется \AddIndex{суммой
\ShowEq{sum of geometric objects, 3}
геометрических объектов}{sum of geometric objects}
$\Vector w_1$ и $\Vector w_2$.
\end{ShadedDefinition}
}

\AddEq{definition: product of geometric object and constant}
{
\begin{ShadedDefinition}
\labelDefinition{product of geometric object and constant, \SideNS-\Cols}
\ShowEq{Let V be vector space of and}
\DrawEq[w1{w_1}W]{geometric object representative, \SideNS-\Cols}{}
геометрический объект,
определённый в \SideRu вом $A$\Hyph векторном пространстве $V$.
Геометрический объект
\ShowEq{product of geometric object and constant, 2, \SideNS}
называется \AddIndex{произведением
\ShowEq{product of geometric object and constant, 3, \SideNS}
геометрического объекта $\Vector w_1$ и константы $k\in A$}
{product of geometric object and constant}.
\end{ShadedDefinition}
}

\AddEq{theorem: Geometric objects form A vector space}
{
\begin{ShadedTheorem}
\labelTheorem{Geometric objects form A vector space, \SideNS-\Cols}
Геометрические объекты типа $F$,
определённые в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsNA,
образуют \SideRu вое $A$\Hyph векторное пространство \ColsNA.
\end{ShadedTheorem}
}

\DefProof{Geometric objects form A vector space}
{
Утверждение теорем
\RefTheorem{Geometric objects form A vector space, \SideNS-cols},
\RefTheorem{Geometric objects form A vector space, \SideNS-rows}
следует из непосредственной проверки
свойств векторного пространства.
}

\DefLabeledTheorem{coordinate matrix of basis and passive transformation}{\SideNS-\Cols}
{
Координатная матрица базиса $\Basis e'$ относительно базиса $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$ \ColsA
совпадает с матрицей пассивного преобразования, отображающего
базис $\Basis e$ в базис $\Basis e'$.
}

\DefProof{coordinate matrix of basis and passive transformation}
{
Согласно теореме
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
координатная матрица базиса $\Basis e'$ относительно базиса $\Basis e$
состоит из \ColsNA, являющихся координатными матрицами векторов
$\aD{\Vector e'}i$ относительно базиса $\Basis e$. Следовательно,
\ShowEq{coordinate matrix of basis and passive transformation, \SideNS-\Cols}{e'}
В тоже время пассивное преобразование $a$, связывающее два базиса, имеет вид
\ShowEq{coordinate matrix of basis and passive transformation, \SideNS-\Cols}{a}
В силу теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols},
\ShowEq{coordinate matrix of basis and passive transformation, \Cols}
для любого $\gii$. Это доказывает теорему.
}

\DefLabeledSloppyRemark{identify basis and matrix of coordinates}{\SideNS-\Cols}
{
Согласно теоремам
\RefTheorem{single transitive representation of group},
\refTheorem{coordinate matrix of basis and passive transformation}{\SideNS-\Cols},
мы можем отождествить базис $\Basis e'$ 
многообразия базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
\SideRu вого $A$\Hyph векторного пространства столбцов
и матрицу $g$ координат базиса $\Basis e'$
относительно базиса $\Basis e$
\DrawEq[{}{}]{passive transformation e->e', \SideNS-\Cols}1
Если $\Basis e'=\Basis e$, то равенство
\eqRef{passive transformation e->e', \SideNS-\Cols}1
принимает вид
\ShowEq{passive transformation e->e, \SideNS-\Cols}
Опираясь на равенство
\EqRef{passive transformation e->e, \SideNS-\Cols}
мы будем пользоваться записью
\ShowEq{basis manifold of V, \SideNS-\Cols}{\aD En}G{}
для многообразия базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG.
}

\DefText{Passive Transformation}
{
Активное преобразование изменяет базисы и векторы согласовано
и координаты вектора относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к преобразованию
координат вектора относительно базиса.
}

\DefText{transformation of coordinates of vector}
{
Мы рассмотрим преобразование координат вектора в теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\AddEq{remark: active representation is single transitive}
{
Чтобы доказать теоремы
\refTheorem{active representation is single transitive}{\SideNS-cols},
\refTheorem{active representation is single transitive}{\SideNS-rows},
достаточно показать, что для любых двух базисов
определено по крайней мере одно преобразование \OtherSideRu востороннего представления
и это преобразование единственно.
}

\AddEq{left active representation is single transitive}
{
координатной матрицы исходного базиса и матрицы автоморфизма
\ShowEq{left e'=e*a}{}
}

\AddEq{right active representation is single transitive}
{
матрицы автоморфизма и координатной матрицы исходного базиса
\ShowEq{right e'=e*a}{}
}

\DefProofSloppy{active representation is single transitive}
{
Гомоморфизм $a$, действуя на базис $\Basis e$ имеет вид
\DrawEq{automorphism, vector space, 1, \SideNS-\Cols}{}
где
\ShowEq{vector of basis \Cols}{e'}
- координатная матрица вектора
\ShowEq{vector of basis \Cols}{\Vector e'}
относительно базиса $\Basis h$ и
\ShowEq{vector of basis \Cols}e
- координатная матрица вектора
\ShowEq{vector of basis \Cols}{\Vector e}
относительно базиса $\Basis h$.
Следовательно, координатная матрица образа базиса равна
\ProductType произведению
\ShowEq{\SideWS active representation is single transitive}
В силу теоремы
\refTheorem{coordinate matrix of basis}{\Product-\Cols},
матрицы $g$ и $e$ невырождены. Следовательно, матрица
\ShowEq{homomorphism on A basis, \SideNS-\Cols}
является матрицей автоморфизма, отображающего базис $\Basis e$
в базис $\Basis e'$.

Допустим элементы $g_1$, $g_2$ группы $G$ и базис $\Basis e$ таковы, что
\ShowEq{two transformations on basis manifold, \SideNS-\Cols}
В силу теорем
\refTheorem{coordinate matrix of basis}{\Product-\Cols}
и
\RefTheorem{two cr-products equal}
справедливо равенство $g_1=g_2$.
Отсюда следует утверждение теоремы.
}

\DefLabeledTheorem{representation of homomorphism relative different bases}{\SideNS-\Cols}
{
Пусть
\ShowEq{Bases e12}V{}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$ столбцов.
Пусть
\ShowEq{Bases e12}W{}
- базисы \SideRu вого $A$\Hyph векторного пространства $W$ столбцов.
Пусть $a_1$ - матрица гомоморфизма
\DrawEq{A:V->W}{different bases \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW1{}
и $a_2$ - матрица гомоморфизма
\eqRef{A:V->W}{different bases \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW2.
Если базис $\Basis e_{V1}$ имеет координатную матрицу $b$ относительно
базиса $\Basis e_{V2}$
\DrawEq[Vb]{coordinate matrix, f, g, \SideNS-\Cols}{}
и $\Basis e_{W1}$ имеет координатную матрицу $c$ относительно
базиса $\Basis e_{W2}$
\DrawEq[Wc]{coordinate matrix, f, g, \SideNS-\Cols}C
то матрицы $a_1$ и $a_2$ связаны соотношением
\DrawEq[c]{representation of homomorphism relative different bases, \SideNS-\Cols}{}
}

\DefProof{representation of homomorphism relative different bases}
{
Вектор $\Vector v\in V$ имеет разложение
\ShowEq{expansion of vector v, \SideNS-\Cols}
относительно базисов
\ShowEq{Bases e12}V.
Так как $a$ - гомоморфизм, то мы можем записать его в форме
\ShowEq{representation of homomorphism relative different bases, 1, \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW1{}
и
\ShowEq{representation of homomorphism relative different bases, 2, \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW2.
В силу теоремы
\refTheorem{coordinate matrix of basis}{\Product-\Cols}
матрица $c$ имеет \ProductType обратную и из равенства
\eqRef{coordinate matrix, f, g, \SideNS-\Cols}C следует
\ShowEq{coordinate matrix, W2, W1, \SideNS-\Cols}
Равенство
\ShowEq{representation of homomorphism relative different bases, 3, \SideNS-\Cols}
\begin{sloppypar}
\noindent
является следствием равенств
\EqRef{representation of homomorphism relative different bases, 2, \SideNS-\Cols},
\EqRef{coordinate matrix, W2, W1, \SideNS-\Cols}.
В силу теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}
сравнение равенств
\EqRef{representation of homomorphism relative different bases, 1, \SideNS-\Cols}
и \EqRef{representation of homomorphism relative different bases, 3, \SideNS-\Cols} даёт
\ShowEq{representation of homomorphism relative different bases, 4, \SideNS-\Cols}
Так как вектор $a$ - произвольный вектор,
утверждение теоремы
является следствием теоремы
\refTheorem{active transformations, vector space}{\SideNS-\Cols}
и равенства
\EqRef{representation of homomorphism relative different bases, 4, \SideNS-\Cols}.
\end{sloppypar}
}

\DefLabeledTheorem{coordinate transformations form representation, vector space}{\SideNS-\Cols}
{
Преобразования координат
\newline
\FrameEqRef[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{12 \SideNS-\Cols}
\newline
порождают эффективное линейное
\OtherSideRu востороннее контравариантное $G$\Hyph представление, называемое
{\bf координатным представлением в \SideRu вом $A$\Hyph векторном пространстве}
\ColsNA.
}

\DefProof{coordinate transformations form representation, vector space}
{
\ShowText{passive representation of left vector space}
Согласно определению
\RefDefinition{Left side contravariant representation},
преобразования координат
порождают линейное правостороннее контравариантное $G$\Hyph представление.
Если координатное преобразование не изменяет векторы $\delta_k$,
то ему соответствует единица группы $G$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
}

\AddEq{theorem: representation of automorphism relative different bases}
{
\begin{ShadedTheorem}
\labelTheorem{representation of automorphism relative different bases, \SideNS-\Cols}
Пусть $\Vector a$ - автоморфизм
левого $A$\Hyph векторного пространства $V$ столбцов.
Пусть $a_1$ - матрица этого автоморфизма, заданная
относительно базиса $\Basis e_1$, и
$a_2$ - матрица того же автоморфизма, заданная
относительно базиса $\Basis e_2$.
Если базис $\Basis e_1$ имеет координатную матрицу $b$ относительно
базиса $\Basis e_2$
\DrawEq[{}b]{coordinate matrix, f, g, \SideNS-\Cols}{}
то матрицы $a_1$ и $a_2$ связаны соотношением
\DrawEq[b]{representation of homomorphism relative different bases, \SideNS-\Cols}{}
\end{ShadedTheorem}
}

\DefProof{representation of automorphism relative different bases}
{
Утверждение является следствием теоремы
\refTheorem{representation of homomorphism relative different bases}{\SideNS-\Cols},
так как в данном случае $c=b$.
}

\DefLabeledTheorem[4]{basis of vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
\ShowEq{Let be basis of vector space}{#2}iIA{#1}V{#2}{\Cols}-
\ShowEq{Let be basis of vector space}{#4}jJA{#3}V{#4}{\Cols}-
Если $|\gi I|$ и $|\gi J|$ - конечные числа, то
\ShowEq{|I|=|J|}
}

\DefProof{basis of vector space}
{
Предположим, что
\ShowEq{|I|=m}Im{}
и
\ShowEq{|I|=m}Jn.
Предположим, что
\DrawEq{m<n gi}{1 \SideNS-\Cols}
Так как $\Basis e_1$ - базис, любой вектор
\ShowEq{basis e2 of V \Cols}
имеет разложение
\ShowEq{basis e2 relative e1 \SideNS-\Cols}
Так как $\Basis e_2$ - базис,
\DrawEq{basis e2 of V lambda}{\SideNS-\Cols}
следует из
\ShowEq{basis e2 relative e1, lambda, \SideNS-\Cols}
Так как $\Basis e_1$ - базис, мы получим
\ShowEq{basis e2 relative e1, lambda=0, \SideNS-\Cols}
Согласно
\eqRef{m<n gi}{1 \SideNS-\Cols},
\ShowEq{Rank a<m \Product}
и система линейных уравнений
\EqRef{basis e2 relative e1, lambda=0, \SideNS-\Cols}
имеет больше переменных, чем уравнений. Согласно теореме
\RefTheorem{star rows system of linear equations, solution},
$\lambda\ne 0$, что противоречит
утверждению \eqRef{basis e2 of V lambda}{\SideNS-\Cols}. 
Следовательно, утверждение
\DrawEq{m<n gi}-
неверно.
Таким же образом мы можем доказать, что утверждение
\ShowEq{n<m gi}
неверно.
Это завершает доказательство теоремы.
}

\AddEq{definition: linearly independent, AoxA module}
{
\begin{ShadedDefinition}
\labelDefinition{linearly independent, AoxA module \Cols}
Пусть $V$ левый \AoxA A\Hyph модуль \ColsNA.
Множество векторов
\ShowEq{Vector A \Cols}
левого \AoxA A\Hyph модуля $V$
{\bf линейно независимо},
если из равенства
\ShowEq{AoxA linearly independent \Cols}
следует
\ShowEq{AoxA linearly independent 1 \Cols}.
В противном случае, множество векторов $\aD ai$
{\bf линейно зависимо}.
\end{ShadedDefinition}
}

\AddEq{definition: basis, AoxA module}
{
\begin{ShadedDefinition}
\labelDefinition{basis, AoxA module \Cols}
Мы называем множество векторов
\ShowEq{basis, AoxA module \Cols}
\AddIndex{базисом}{basis}
\AoxA A\Hyph модуля $V$,
если множество векторов
\ShowEq{basis vector \Cols}
линейно независимо и, добавив к этой системе любой другой вектор,
мы получим новое множество, которое является линейно зависимым.
\end{ShadedDefinition}
}

\DefLabeledDefinition{Eigenvalue of Endomorphism}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
Вектор $v\in V$ называется
{\bf собственным вектором}
эндоморфизма
\ShowEq{f:A->B}{\Vector f}VV
относительно базиса $\Basis e$,
если существует $b\in A$ такое, что
\DrawEq[bv]{fov=b e o v}{\SideNS}
$A$\Hyph число $b$ называется
{\bf собственным значением}
эндоморфизма $f$
относительно базиса $\Basis e$.
}

\DefLabeledTheorem{no endomorphism fov=bv}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
Если
\ShowEq{b not in ZA},
то не существует эндоморфизма $\Vector f$ такого, что
\ShowEq{fov=bv \SideNS}
%где $f$ - матрица эндоморфизма $\Vector f$.
}

\DefProofSloppy{no endomorphism fov=bv}
{
Допустим, что существует эндоморфизм $\Vector f$
такой, что равенство
\EqRef{fov=bv \SideNS}
верно.
Равенство
\ShowEq{b(av)=a(bv) \SideNS}
является следствием равенств
\eqRef{associative law, \SideWS module}1,
\eqRef{\SideWS homomorphism, f av=}1,
\EqRef{fov=bv \SideNS}.
Согласно теореме
\refTheorem{av=bv=>a=b}{\SideNS-\Cols},
равенство
\DrawEq{ab=ba}{\SideNS}
для любого $a\in A$
является следствием равенства
\EqRef{b(av)=a(bv) \SideNS}.
Равенство
\eqRef{ab=ba}{\SideNS}
для любого $a\in A$
противоречит утверждению
\ShowEq{b not in ZA}.
Следовательно, рассматриваемый эндоморфизм $\Vector f$
не существует.
}

\AddEq{remark: Eigenvalue of Endomorphism}
{
\begin{sloppypar}
Согласно теореме
\refTheorem{no endomorphism fov=bv}{\SideNS},
в отличие от \OtherSideRu востороннего произведения
вектора на скаляр
\SideRu востороннее произведение
вектора на скаляр
не является эндоморфизмом
\SideRu вого $A$\Hyph векторного пространства.
Из сравнения определения
\refDefinition{similarity transformation}{\SideNS}
и теоремы
\refTheorem{no endomorphism fov=bv}{\SideNS}
следует, что преобразование подобия
играет в некоммутативной алгебре
такую же роль,
что преобразование подобия
играет в коммутативной алгебре.
\end{sloppypar}
}

\DefLabeledTheorem{similarity transformation, change of basis}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть базисы
\ShowEq{basis e1 e2}
связаны пассивным преобразованием $g$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
Преобразование подобия
\ShowEq{\SideWS map a En}a1
имеет матрицу
\DrawEq[ag]{ga*g- \SideNS-\Cols}a
относительно базиса $\Basis e_2$.
}

\DefProof{similarity transformation, change of basis}
{
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
преобразование подобия
\ShowEq{\SideWS map a En}a1
имеет матрицу
\ShowEq{ga*g- 1 \SideNS-\Cols}
относительно базиса $\Basis e_2$.
Теорема является следствием выражения
\EqRef{ga*g- 1 \SideNS-\Cols}.
}

\DefLabeledTheorem{similarity transformation}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Пусть
\ShowEq{dim V=n}
и $\aD En$ - \nTimes единичная матрица.
Для любого $A$\Hyph числа $a$, существует эндоморфизм
\ShowEq{\SideWS map a En}a{}
\SideRu вого $A$\Hyph векторного пространства $V$,
который имеет матрицу
\ShowEq{\SideWS a En}
относительно базиса $\Basis e$.
}

\DefProof{similarity transformation}
{
Пусть $\Basis e$ - базис
\SideRu вого $A$\Hyph векторного пространства столбцов.
Согласно теореме
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)}
и определению
\refDefinition{iso end aut morphism vector space}{\SideNS},
отображение
\ShowEq{v in V -> av in V \SideNS-\Cols}
является эндоморфизмом
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\DefLabeledDefinitionNote{iso end aut morphism vector space}{\SideNS}
{
Гомоморфизм
\ShowEq{f:A->B}fVW
назывется\,\footnotemark
\AddIndex{изоморфизмом}{isomorphism}
между \SideRu выми $A$\Hyph векторными пространствами $V$ и $W$,
если соответствие $f^{-1}$ является гомоморфизмом.
Гомоморфизм
\ShowEq{f:A->B}fVV
источником и целью которого является одно и тоже
\SideRu вое $A$\Hyph векторное пространство,
называется
\AddIndex{эндоморфизмом}{endomorphism}.
Эндоморфизм
\ShowEq{f:A->B}fVV
\SideRu вого $A$\Hyph векторного пространства $V$
назывется
\AddIndex{автоморфизмом}{automorphism},
если соответствие $f^{-1}$ является эндоморфизмом.
}
{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}

\DefText{Basis Manifold}
{
\section{Размерность \SideRu вого \texorpdfstring{$A$}{A}\Hyph векторного пространства}

\ShowText{Dimension of Vector Space}

\section{Многообразие базисов \SideRu вого \texorpdfstring{$A$}{A}-векторного пространства}
%\labelSection{Basis Manifold for Vector Space}

\ShowEq{Basis Manifold for Vector Space}

\section{Пассивное преобразование в \SideRu вом \texorpdfstring{$A$}{A}-векторном пространстве}

\ShowEq{Passive Transformation}
}

\DefLabeledTheorem[3]{rank of matrix}{\Product-\Cols}
{
Предположим, что $a$ - матрица,
\ShowEq{\Product-rank a=k<m}{#1}
и $\SA T$ - \ProductType главная подматрица.
Тогда \ColWS \ARow a{#2} является
\SideRu вой линейной комбинацией \ColsA \ARow a{#3}
\ShowEq{rank of matrix, \Product-\Cols}
\ShowEq{rank of matrix, 1, \Product-\Cols}
\ShowEq{rank of matrix, 2, \Product-\Cols}
}

\DefProof[5]{rank of matrix}
{
Если матрица $a$ имеет $\gik$ \RowsNSA, то, полагая, что \ColWS \ARow a{#2}
- \SideRu вая линейная комбинация
\EqRef{rank of matrix, 1, \Product-\Cols}
\ColsA \ARow a{#3} с коэффициентами $\Coef$,
мы получим систему \SideRu вых линейных уравнений
\EqRef{rank of matrix, 2, \Product-\Cols}.
Мы положим, что $\ACol x{#4}=\Coef$ - это неизвестные переменные
в системе \SideRu вых линейных уравнений
\EqRef{rank of matrix, 2, \Product-\Cols}.
Согласно теореме
\refTheorem{nonsingular system of linear equations}{\SideNS-\Cols},
система \SideRu вых линейных уравнений
\EqRef{rank of matrix, 2, \Product-\Cols}
имеет единственное решение
и это решение нетривиально потому, что все \ProductType квазидетерминанты
отличны от $0$.

Остаётся доказать утверждение в случае, когда число \RowsRWSA матрицы $a$
больше чем $\gik$.
Пусть нам даны \ColWS \ARow a{#2} и \RowRuWS $\ACol a{#5}$.
Согласно предположению, подматрица
$\SATpr$ - \ProductType вырожденная матрица
и её \ProductType квазидетерминант
\DrawEq{singular matrix and quasideterminant}{\SideNS-\Cols}
Согласно равенству
\eqRef{j i quasideterminant =}{\Product}
равенство
\eqRef{singular matrix and quasideterminant}{\SideNS-\Cols}
имеет вид
\ShowEq{rank of matrix, 4, \Product}
Матрица
\ShowEq{rank of matrix, 5, \Product-\Cols}
не зависит от $\gi{#5}$. Следовательно, для любых
\ShowEq{\rIn}
\ShowEq{rank of matrix, 6, \Product-\Cols}
Чтобы доказать равенство
\EqRef{rank of matrix, 2, \Product-\Cols},
\ \ не\-обходимо доказать равенство
\ShowEq{rank of matrix, 9, \Product-\Cols}
Из равенства
\ShowEq{rank of matrix, 7, \Product-\Cols}
следует, что
\ShowEq{rank of matrix, 8, \Product-\Cols}
Равенство
\EqRef{rank of matrix, 9, \Product-\Cols}
является следствием равенств
\EqRef{rank of matrix, 5, \Product-\Cols},
\EqRef{rank of matrix, 8, \Product-\Cols}.
Равенство
\EqRef{rank of matrix, 2, \Product-\Cols}
является следствием равенств
\EqRef{rank of matrix, 6, \Product-\Cols},
\EqRef{rank of matrix, 9, \Product-\Cols}.
}

\DefLabeledTheorem{set of eigenvectors is vector space}{\Product-\Cols}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением
матрицы $a$.
Множество собственн\EndA \ColsA
матрицы $a$, соответствующих \ProductType собственному значению $b$,
является \SideRu вым $A$\Hyph векторным пространством \ColsNA.
}

\DefProof{set of eigenvectors is vector space}
{
Согласно определениям
\refDefinition{eigenvalue of matrix}{\Product},
\refDefinition{eigenvector of matrix}{\Product-\Cols},
координаты собственно\FinC \ColA
являются решением системы линейных уравнений
\ShowEq{\Product-eigen\Cols=0}
с \ProductType вырожденной матрицей \ShowEq{f-bEn \SideNS}{}.
Согласно теореме
\RefTheorem{Solutions homogenous system of linear equations},
множество решений системы линейных уравнений
\EqRef{\Product-eigen\Cols=0}
является \SideRu вым $A$\Hyph векторным пространством \ColsNA.
}

\DefLabeledTheorem{set of eigenvectors fg is vector space}{\Product-\Cols}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением пары матриц
\ShowEq{pair of matrices \Product-\ColN},
где $g$ - \ProductType невырожденная матрица.
Множество собственн\EndA \ColsA
пары матриц $(f,g)$, соответствующих \ProductType собственному значению $b$,
является \SideRu вым $A$\Hyph векторным пространством \ColsNA.
}

\DefProof{set of eigenvectors fg is vector space}
{
Согласно определениям
\refDefinition{eigenvalues of pair of matrices}{\Product},
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN},
координаты собственно\FinC \ColA
являются решением системы линейных уравнений
\ShowEq{\Product-eigen\Cols=0 fg}
с \ProductType вырожденной матрицей
\[f-\ShowEq{ga*g- \SideNS-\Cols}bg\]
Согласно теореме
\RefTheorem{Solutions homogenous system of linear equations},
множество решений системы линейных уравнений
\EqRef{\Product-eigen\Cols=0 fg}
является \SideRu вым пространст\-вом \ColsNA.
}

\DefRemark{simplify definitions of eigenvalue}
{
Пусть
\ShowEq{gij in ZA}
Тогда
\ShowEq{gb rc g-=b}
\ShowEq{gb cr g-=b}
Из равенств
\EqRef{gb rc g-=b},
\EqRef{gb cr g-=b}
следует, что,
если выполнено
условие
\EqRef{gij in ZA},
то мы можем упростить определения
собственного значения и собственного вектора матрицы
и получить определения,
которые будут соответствовать определениям
в коммутативной алгебре.
}

\DefLabeledTheorem{columns of matrix are linearly dependent}{\Product-\Cols}
{
Предположим, что матрица $a$ имеет $\gi{\Lbls}$ \ColsNA.
Если
\ShowEq{\Product-rank a=k<m}{\Lbls}
то \ColsRu матрицы линейно зависимы с\SideRu ва
\DrawEq[{\lambda}a]{columns of matrix are linearly dependent}{}
}

\DefProof[1]{columns of matrix are linearly dependent}
{
Предположим, что \ColWS \ARow a{#1} является \SideRu вой линейной комбинацией \ColsA
\EqRef{rank of matrix, 1, \Product-\Cols}. Мы положим
\ShowEq{\Cols-of-matrix linearly dependent, 1}
и остальные
\ShowEq{\Cols-of-matrix linearly dependent, 2}
}

